Benchmarking Geospatial Foundation Models under Calibrated Label Errors

Earth-observation labels from maps, older products or hurried annotation arrive misaligned, coarse, loosely outlined or incomplete. Geospatial foundation models (GFMs) are nevertheless benchmarked with labels taken as correct. A practitioner therefore cannot tell which encoder to choose when the labels are imperfect. We present a benchmark protocol for fine-tuning under such labels. Four spatially structured error types are calibrated to equal label mIoU and applied identically to every model and seed. Every contrast is paired and read against an equivalence margin of $\pm 3$ points and a minimum detectable effect. We apply it to nine encoders, six decoder heads and ten datasets. In an exploratory reading at a matched learning rate the satellite-pretrained and web-pretrained DINOv3 encoders are equivalent within the margin on 8 of 9 datasets. Multispectral GFMs and an ImageNet ResNet-50 are equivalent within the margin on about half of them. Labels with random offsets cost the least at equal label quality. Under other decoder heads the verdicts mostly hold on FLAIR-2 and are decoder dependent on HLS Burn Scars. On four of five real label pairs the real label costs more than its matched simulated type. No choice of pretraining data makes an encoder consistently more robust, so the encoder is better chosen by its accuracy under imperfect labels.

==> generated/config_macros.tex <==
%
%
\newcommand{\GbTwoSATburn}{69.4}  %
\newcommand{\BoundaryDPxBurn}{14}  %
\newcommand{\BoundaryDMBurn}{420}  %
\newcommand{\BoundaryDMNarrowBurn}{90}  %
\newcommand{\NCalTilesBurn}{684}  %
\newcommand{\NRealisations}{8}
\newcommand{\CalTol}{0.01}
\newcommand{\CalTargetLOne}{0.85}
\newcommand{\CalTargetLTwo}{0.70}
\newcommand{\KnobBurnShiftLOne}{20}  %
\newcommand{\KnobMBurnShiftLOne}{600}  %
\newcommand{\KnobMUnitBurnShiftLOne}{m}
\newcommand{\CalMiouBurnShiftLOne}{0.848}
\newcommand{\FlipBurnShiftLOne}{3.4}  %
\newcommand{\KnobBurnShiftLTwo}{60}  %
\newcommand{\KnobMBurnShiftLTwo}{1.8}  %
\newcommand{\KnobMUnitBurnShiftLTwo}{km}
\newcommand{\CalMiouBurnShiftLTwo}{0.700}
\newcommand{\FlipBurnShiftLTwo}{7.8}  %
\newcommand{\CalIouBurnedBurnShiftLTwo}{48.5}  %
\newcommand{\CalIouClassMinBurnShiftLTwo}{48.5}  %
\newcommand{\CalIouClassMaxBurnShiftLTwo}{91.6}  %
\newcommand{\RealMiouBurnShiftLTwoROne}{70.0}  %
\newcommand{\RealMiouBurnShiftLTwoRTwo}{69.8}  %
\newcommand{\RealMiouBurnShiftLTwoRThree}{69.8}  %
\newcommand{\RealMiouBurnShiftLTwoRFour}{70.0}  %
\newcommand{\RealMiouBurnShiftLTwoRFive}{69.7}  %
\newcommand{\RealRangeBurnShiftLTwo}{0.3}  %
\newcommand{\RealHarshestBurnShiftLTwo}{5}  %
\newcommand{\RealOffTolBurnShiftLTwo}{none}  %
\newcommand{\RealOffTolExtBurnShiftLTwo}{none}  %
\newcommand{\KnobBurnCoarseLOne}{57}  %
\newcommand{\KnobMBurnCoarseLOne}{1.7}  %
\newcommand{\KnobMUnitBurnCoarseLOne}{km}
\newcommand{\CalMiouBurnCoarseLOne}{0.850}
\newcommand{\FlipBurnCoarseLOne}{3.3}  %
\newcommand{\KnobBurnCoarseLTwo}{192}  %
\newcommand{\KnobMBurnCoarseLTwo}{5.8}  %
\newcommand{\KnobMUnitBurnCoarseLTwo}{km}
\newcommand{\CalMiouBurnCoarseLTwo}{0.703}
\newcommand{\FlipBurnCoarseLTwo}{6.7}  %
\newcommand{\CalIouBurnedBurnCoarseLTwo}{47.8}  %
\newcommand{\CalIouClassMinBurnCoarseLTwo}{47.8}  %
\newcommand{\CalIouClassMaxBurnCoarseLTwo}{92.8}  %
\newcommand{\RealMiouBurnCoarseLTwoROne}{70.3}  %
\newcommand{\RealMiouBurnCoarseLTwoRTwo}{70.3}  %
\newcommand{\RealMiouBurnCoarseLTwoRThree}{69.9}  %
\newcommand{\RealMiouBurnCoarseLTwoRFour}{70.0}  %
\newcommand{\RealMiouBurnCoarseLTwoRFive}{70.4}  %
\newcommand{\RealRangeBurnCoarseLTwo}{0.4}  %
\newcommand{\RealHarshestBurnCoarseLTwo}{3}  %
\newcommand{\RealOffTolBurnCoarseLTwo}{none}  %
\newcommand{\RealOffTolExtBurnCoarseLTwo}{none}  %
\newcommand{\KnobBurnBoundaryLOne}{11}  %
\newcommand{\KnobMBurnBoundaryLOne}{330}  %
\newcommand{\KnobMUnitBurnBoundaryLOne}{m}
\newcommand{\CalMiouBurnBoundaryLOne}{0.850}
\newcommand{\FlipBurnBoundaryLOne}{3.4}  %
\newcommand{\KnobBurnBoundaryLTwo}{32}  %
\newcommand{\KnobMBurnBoundaryLTwo}{960}  %
\newcommand{\KnobMUnitBurnBoundaryLTwo}{m}
\newcommand{\CalMiouBurnBoundaryLTwo}{0.700}
\newcommand{\FlipBurnBoundaryLTwo}{8.2}  %
\newcommand{\CalIouBurnedBurnBoundaryLTwo}{48.9}  %
\newcommand{\CalIouClassMinBurnBoundaryLTwo}{48.9}  %
\newcommand{\CalIouClassMaxBurnBoundaryLTwo}{91.1}  %
\newcommand{\RealMiouBurnBoundaryLTwoROne}{70.0}  %
\newcommand{\RealMiouBurnBoundaryLTwoRTwo}{69.7}  %
\newcommand{\RealMiouBurnBoundaryLTwoRThree}{70.4}  %
\newcommand{\RealMiouBurnBoundaryLTwoRFour}{69.7}  %
\newcommand{\RealMiouBurnBoundaryLTwoRFive}{70.4}  %
\newcommand{\RealRangeBurnBoundaryLTwo}{0.8}  %
\newcommand{\RealHarshestBurnBoundaryLTwo}{2}  %
\newcommand{\RealOffTolBurnBoundaryLTwo}{none}  %
\newcommand{\RealOffTolExtBurnBoundaryLTwo}{none}  %
\newcommand{\KnobBurnOmissionLOne}{0.28}  %
\newcommand{\CalMiouBurnOmissionLOne}{0.849}
\newcommand{\FlipBurnOmissionLOne}{3.0}  %
\newcommand{\KnobBurnOmissionLTwo}{0.53}  %
\newcommand{\CalMiouBurnOmissionLTwo}{0.703}
\newcommand{\FlipBurnOmissionLTwo}{5.9}  %
\newcommand{\CalIouBurnedBurnOmissionLTwo}{46.9}  %
\newcommand{\CalIouClassMinBurnOmissionLTwo}{46.9}  %
\newcommand{\CalIouClassMaxBurnOmissionLTwo}{93.7}  %
\newcommand{\RealMiouBurnOmissionLTwoROne}{70.3}  %
\newcommand{\RealMiouBurnOmissionLTwoRTwo}{74.7}  %
\newcommand{\RealMiouBurnOmissionLTwoRThree}{68.1}  %
\newcommand{\RealMiouBurnOmissionLTwoRFour}{70.0}  %
\newcommand{\RealMiouBurnOmissionLTwoRFive}{70.1}  %
\newcommand{\RealRangeBurnOmissionLTwo}{6.6}  %
\newcommand{\RealHarshestBurnOmissionLTwo}{3}  %
\newcommand{\RealOffTolBurnOmissionLTwo}{2 and 3}  %
\newcommand{\RealOffTolExtBurnOmissionLTwo}{7 and 8}  %
\newcommand{\BoundaryDPxFlair}{14}  %
\newcommand{\BoundaryDMFlair}{2.8}  %
\newcommand{\BoundaryDMNarrowFlair}{0.6}  %
\newcommand{\NCalTilesFlair}{1250}  %
\newcommand{\KnobFlairShiftLOne}{10}  %
\newcommand{\KnobMFlairShiftLOne}{2.0}  %
\newcommand{\KnobMUnitFlairShiftLOne}{m}
\newcommand{\CalMiouFlairShiftLOne}{0.848}
\newcommand{\FlipFlairShiftLOne}{9.5}  %
\newcommand{\KnobFlairShiftLTwo}{29}  %
\newcommand{\KnobMFlairShiftLTwo}{5.8}  %
\newcommand{\KnobMUnitFlairShiftLTwo}{m}
\newcommand{\CalMiouFlairShiftLTwo}{0.700}
\newcommand{\FlipFlairShiftLTwo}{21.1}  %
\newcommand{\CalIouClassMinFlairShiftLTwo}{53.4}  %
\newcommand{\CalIouClassMaxFlairShiftLTwo}{91.3}  %
\newcommand{\RealMiouFlairShiftLTwoROne}{70.0}  %
\newcommand{\RealMiouFlairShiftLTwoRTwo}{69.7}  %
\newcommand{\RealMiouFlairShiftLTwoRThree}{69.8}  %
\newcommand{\RealMiouFlairShiftLTwoRFour}{69.7}  %
\newcommand{\RealMiouFlairShiftLTwoRFive}{69.7}  %
\newcommand{\RealRangeFlairShiftLTwo}{0.3}  %
\newcommand{\RealHarshestFlairShiftLTwo}{4}  %
\newcommand{\RealOffTolFlairShiftLTwo}{none}  %
\newcommand{\RealOffTolExtFlairShiftLTwo}{none}  %
\newcommand{\KnobFlairCoarseLOne}{29}  %
\newcommand{\KnobMFlairCoarseLOne}{5.8}  %
\newcommand{\KnobMUnitFlairCoarseLOne}{m}
\newcommand{\CalMiouFlairCoarseLOne}{0.849}
\newcommand{\FlipFlairCoarseLOne}{9.6}  %
\newcommand{\KnobFlairCoarseLTwo}{105}  %
\newcommand{\KnobMFlairCoarseLTwo}{21}  %
\newcommand{\KnobMUnitFlairCoarseLTwo}{m}
\newcommand{\CalMiouFlairCoarseLTwo}{0.700}
\newcommand{\FlipFlairCoarseLTwo}{21.2}  %
\newcommand{\CalIouClassMinFlairCoarseLTwo}{53.9}  %
\newcommand{\CalIouClassMaxFlairCoarseLTwo}{89.7}  %
\newcommand{\RealMiouFlairCoarseLTwoROne}{70.0}  %
\newcommand{\RealMiouFlairCoarseLTwoRTwo}{70.0}  %
\newcommand{\RealMiouFlairCoarseLTwoRThree}{70.1}  %
\newcommand{\RealMiouFlairCoarseLTwoRFour}{70.1}  %
\newcommand{\RealMiouFlairCoarseLTwoRFive}{70.1}  %
\newcommand{\RealRangeFlairCoarseLTwo}{0.1}  %
\newcommand{\RealHarshestFlairCoarseLTwo}{1}  %
\newcommand{\RealOffTolFlairCoarseLTwo}{none}  %
\newcommand{\RealOffTolExtFlairCoarseLTwo}{none}  %
\newcommand{\KnobFlairBoundaryLOne}{16}  %
\newcommand{\KnobMFlairBoundaryLOne}{3.2}  %
\newcommand{\KnobMUnitFlairBoundaryLOne}{m}
\newcommand{\CalMiouFlairBoundaryLOne}{0.846}
\newcommand{\FlipFlairBoundaryLOne}{8.4}  %
\newcommand{\KnobFlairBoundaryLTwo}{52}  %
\newcommand{\KnobMFlairBoundaryLTwo}{10}  %
\newcommand{\KnobMUnitFlairBoundaryLTwo}{m}
\newcommand{\CalMiouFlairBoundaryLTwo}{0.702}
\newcommand{\FlipFlairBoundaryLTwo}{18.2}  %
\newcommand{\CalIouClassMinFlairBoundaryLTwo}{43.4}  %
\newcommand{\CalIouClassMaxFlairBoundaryLTwo}{87.4}  %
\newcommand{\RealMiouFlairBoundaryLTwoROne}{70.2}  %
\newcommand{\RealMiouFlairBoundaryLTwoRTwo}{69.9}  %
\newcommand{\RealMiouFlairBoundaryLTwoRThree}{70.6}  %
\newcommand{\RealMiouFlairBoundaryLTwoRFour}{70.3}  %
\newcommand{\RealMiouFlairBoundaryLTwoRFive}{70.4}  %
\newcommand{\RealRangeFlairBoundaryLTwo}{0.7}  %
\newcommand{\RealHarshestFlairBoundaryLTwo}{2}  %
\newcommand{\RealOffTolFlairBoundaryLTwo}{none}  %
\newcommand{\RealOffTolExtFlairBoundaryLTwo}{6 and 8}  %
\newcommand{\KnobFlairOmissionLOne}{0.07}  %
\newcommand{\CalMiouFlairOmissionLOne}{0.849}
\newcommand{\FlipFlairOmissionLOne}{7.4}  %
\newcommand{\KnobFlairOmissionLTwo}{0.18}  %
\newcommand{\CalMiouFlairOmissionLTwo}{0.698}
\newcommand{\FlipFlairOmissionLTwo}{17.4}  %
\newcommand{\CalIouClassMinFlairOmissionLTwo}{35.1}  %
\newcommand{\CalIouClassMaxFlairOmissionLTwo}{85.6}  %
\newcommand{\RealMiouFlairOmissionLTwoROne}{69.8}  %
\newcommand{\RealMiouFlairOmissionLTwoRTwo}{72.9}  %
\newcommand{\RealMiouFlairOmissionLTwoRThree}{73.4}  %
\newcommand{\RealMiouFlairOmissionLTwoRFour}{71.4}  %
\newcommand{\RealMiouFlairOmissionLTwoRFive}{70.2}  %
\newcommand{\RealRangeFlairOmissionLTwo}{3.5}  %
\newcommand{\RealHarshestFlairOmissionLTwo}{1}  %
\newcommand{\RealOffTolFlairOmissionLTwo}{2, 3 and 4}  %
\newcommand{\RealOffTolExtFlairOmissionLTwo}{6 and 7}  %
\newcommand{\CalMiouMinLOne}{0.846}  %
\newcommand{\CalMiouMaxLOne}{0.850}
\newcommand{\CalMiouMinLTwo}{0.698}  %
\newcommand{\CalMiouMaxLTwo}{0.703}
\newcommand{\RealMiouMinLOne}{0.806}  %
\newcommand{\RealMiouMaxLOne}{0.897}
\newcommand{\RealMiouMinLTwo}{0.679}  %
\newcommand{\RealMiouMaxLTwo}{0.747}
\newcommand{\NFlairSource}{4{,}049}
\newcommand{\NFlairTrain}{1{,}000}
\newcommand{\NFlairVal}{250}
\newcommand{\NBurnTrain}{524}  %
\newcommand{\SubsetTilesBurn}{131}  %
\newcommand{\SubsetTilesFlair}{250}  %
\newcommand{\NBurnVal}{160}  %
\newcommand{\WorstBurn}{coarse}
\newcommand{\WorstTwoBurn}{omission}
\newcommand{\RankingBurn}{coarse, omission, boundary, shift}
\newcommand{\WorstTieSdBurn}{2.05}  %
\newcommand{\WorstFlair}{omission}
\newcommand{\WorstTwoFlair}{coarse}
\newcommand{\RankingFlair}{omission, coarse, boundary, shift}
\newcommand{\WorstTieSdFlair}{0.66}  %
\newcommand{\LvdLrMult}{\ensuremath{\times1/3}}
\newcommand{\AsixLrMult}{\ensuremath{\times1}}
\newcommand{\VitrLrMultBurn}{\ensuremath{\times1}}  %
\newcommand{\VitrLrMultFlair}{\ensuremath{\times3}}  %
\newcommand{\RunsAOne}{450}
\newcommand{\RunsATwo}{4}
\newcommand{\RunsAThree}{60}
\newcommand{\RunsAFour}{50}
\newcommand{\RunsAFive}{10}
\newcommand{\RunsASix}{32}
\newcommand{\RunsASeven}{10}
\newcommand{\RunsNOne}{4}
\newcommand{\RunsNTwo}{16}
\newcommand{\RunsNThree}{8}
\newcommand{\RunsNFour}{10}
\newcommand{\RunsNFive}{60}
\newcommand{\RunsNSix}{44}
\newcommand{\RunsSOne}{50}
\newcommand{\RunsSTwo}{20}
\newcommand{\RunsSThree}{100}
\newcommand{\RunsSFour}{100}
\newcommand{\RunsSFive}{104}
\newcommand{\RunsSSix}{100}
\newcommand{\RunsCore}{698}  %
\newcommand{\RunsStretch}{534}  %
\newcommand{\RunsTotal}{1{,}232}
\newcommand{\RunsNSeven}{550}  %
\newcommand{\NSevenJobsPro}{370}
\newcommand{\NSevenLaneHoursPro}{28.5}
\newcommand{\NSevenJobsRtx}{0}
\newcommand{\NSevenLaneHoursRtx}{0.0}
\newcommand{\NSevenJobsGb}{0}
\newcommand{\NSevenLaneHoursGb}{0.0}
\newcommand{\NSevenJobsRtxFiveZeroSixZeroTi}{0}
\newcommand{\NSevenLaneHoursRtxFiveZeroSixZeroTi}{0.0}
\newcommand{\NSevenJobsRtxThreeZeroEightZeroTi}{90}
\newcommand{\NSevenLaneHoursRtxThreeZeroEightZeroTi}{21.0}
\newcommand{\NSevenJobsRtxThreeZeroEightZero}{90}
\newcommand{\NSevenLaneHoursRtxThreeZeroEightZero}{12.0}
\newcommand{\NSevenLaneHoursTotal}{61.5}
\newcommand{\NSevenMakespanH}{29}  %
\newcommand{\NSevenLanes}{RTX PRO 6000 (370), RTX 3080 (90), RTX 3080 Ti (90)}  %
\newcommand{\RunsNEight}{194}  %
\newcommand{\NEightJobsPro}{94}
\newcommand{\NEightLaneHoursPro}{7.5}
\newcommand{\NEightJobsRtx}{0}
\newcommand{\NEightLaneHoursRtx}{0.0}
\newcommand{\NEightJobsGb}{0}
\newcommand{\NEightLaneHoursGb}{0.0}
\newcommand{\NEightJobsRtxFiveZeroSixZeroTi}{0}
\newcommand{\NEightLaneHoursRtxFiveZeroSixZeroTi}{0.0}
\newcommand{\NEightJobsRtxThreeZeroEightZeroTi}{50}
\newcommand{\NEightLaneHoursRtxThreeZeroEightZeroTi}{11.7}
\newcommand{\NEightJobsRtxThreeZeroEightZero}{50}
\newcommand{\NEightLaneHoursRtxThreeZeroEightZero}{6.7}
\newcommand{\NEightLaneHoursTotal}{25.8}
\newcommand{\NEightMakespanH}{12}  %
\newcommand{\NEightLanes}{RTX PRO 6000 (94), RTX 3080 (50), RTX 3080 Ti (50)}  %
\newcommand{\RunsNNine}{550}  %
\newcommand{\NNineJobsPro}{370}
\newcommand{\NNineLaneHoursPro}{28.5}
\newcommand{\NNineJobsRtx}{0}
\newcommand{\NNineLaneHoursRtx}{0.0}
\newcommand{\NNineJobsGb}{0}
\newcommand{\NNineLaneHoursGb}{0.0}
\newcommand{\NNineJobsRtxFiveZeroSixZeroTi}{0}
\newcommand{\NNineLaneHoursRtxFiveZeroSixZeroTi}{0.0}
\newcommand{\NNineJobsRtxThreeZeroEightZeroTi}{90}
\newcommand{\NNineLaneHoursRtxThreeZeroEightZeroTi}{21.0}
\newcommand{\NNineJobsRtxThreeZeroEightZero}{90}
\newcommand{\NNineLaneHoursRtxThreeZeroEightZero}{12.0}
\newcommand{\NNineLaneHoursTotal}{61.5}
\newcommand{\NNineMakespanH}{29}  %
\newcommand{\NNineLanes}{RTX PRO 6000 (370), RTX 3080 (90), RTX 3080 Ti (90)}  %
\newcommand{\RunsNTen}{550}  %
\newcommand{\NTenJobsPro}{370}
\newcommand{\NTenLaneHoursPro}{28.5}
\newcommand{\NTenJobsRtx}{0}
\newcommand{\NTenLaneHoursRtx}{0.0}
\newcommand{\NTenJobsGb}{0}
\newcommand{\NTenLaneHoursGb}{0.0}
\newcommand{\NTenJobsRtxFiveZeroSixZeroTi}{0}
\newcommand{\NTenLaneHoursRtxFiveZeroSixZeroTi}{0.0}
\newcommand{\NTenJobsRtxThreeZeroEightZeroTi}{90}
\newcommand{\NTenLaneHoursRtxThreeZeroEightZeroTi}{21.0}
\newcommand{\NTenJobsRtxThreeZeroEightZero}{90}
\newcommand{\NTenLaneHoursRtxThreeZeroEightZero}{12.0}
\newcommand{\NTenLaneHoursTotal}{61.5}
\newcommand{\NTenMakespanH}{29}  %
\newcommand{\NTenLanes}{RTX PRO 6000 (370), RTX 3080 (90), RTX 3080 Ti (90)}  %
\newcommand{\RunsNEightAliased}{6}  %
\newcommand{\ParamsDecUNetSAT}{15.6}  %
\newcommand{\ParamsDecSegfSAT}{0.98}  %
\newcommand{\ParamsDecMtwoFSAT}{4.69}  %
\newcommand{\ParamsDecSamSAT}{4.40}  %
\newcommand{\ParamsDecMtwoFBurnSAT}{4.68}  %
\newcommand{\ParamsDecSamBurnSAT}{2.86}  %
\newcommand{\ParamsDecUNetLVD}{15.6}  %
\newcommand{\ParamsDecSegfLVD}{0.98}  %
\newcommand{\ParamsDecMtwoFLVD}{4.69}  %
\newcommand{\ParamsDecSamLVD}{4.40}  %
\newcommand{\ParamsDecMtwoFBurnLVD}{4.68}  %
\newcommand{\ParamsDecSamBurnLVD}{2.86}  %
\newcommand{\ParamsDecUNetDOFA}{15.6}  %
\newcommand{\ParamsDecSegfDOFA}{0.98}  %
\newcommand{\ParamsDecMtwoFDOFA}{4.69}  %
\newcommand{\ParamsDecSamDOFA}{4.40}  %
\newcommand{\ParamsDecMtwoFBurnDOFA}{4.68}  %
\newcommand{\ParamsDecSamBurnDOFA}{2.86}  %
\newcommand{\ParamsDecUNetTM}{15.6}  %
\newcommand{\ParamsDecSegfTM}{0.98}  %
\newcommand{\ParamsDecMtwoFTM}{4.69}  %
\newcommand{\ParamsDecSamTM}{4.40}  %
\newcommand{\ParamsDecMtwoFBurnTM}{4.68}  %
\newcommand{\ParamsDecSamBurnTM}{2.86}  %
\newcommand{\ParamsDecUNetRN}{20.3}  %
\newcommand{\ParamsDecSegfRN}{1.25}  %
\newcommand{\ParamsDecMtwoFRN}{4.95}  %
\newcommand{\ParamsDecSamRN}{4.40}  %
\newcommand{\ParamsDecMtwoFBurnRN}{4.94}  %
\newcommand{\ParamsDecSamBurnRN}{2.86}  %
\newcommand{\GceQ}{0.7}  %
\newcommand{\BootBeta}{0.95}  %
\newcommand{\RealLabelMiouChes}{0.571}  %
\newcommand{\RealFlipRateChes}{21.2}  %
\newcommand{\RealLabelMiouCsTwelve}{0.331}  %
\newcommand{\RealFlipRateCsTwelve}{26.5}  %
\newcommand{\RealLabelMiouDfc}{0.675}  %
\newcommand{\RealFlipRateDfc}{12.5}  %
\newcommand{\RealLabelMiouEnva}{0.483}  %
\newcommand{\RealFlipRateEnva}{42.2}  %
\newcommand{\RealLabelMiouKuro}{0.893}  %
\newcommand{\RealFlipRateKuro}{1.1}  %
\newcommand{\LrTargetMiou}{0.623}  %
\newcommand{\LrTargetNPairs}{6}  %
\newcommand{\HwMixedCellsSAT}{100}  %
\newcommand{\HwMixedCellsLVD}{113}  %
\newcommand{\HwMixedCellsDOFA}{125}  %
\newcommand{\HwMixedCellsTM}{76}  %
\newcommand{\HwMixedCellsRN}{126}  %
\newcommand{\HwMixedCellsPrithvi}{81}  %
\newcommand{\HwMixedCellsCore}{540}  %
\newcommand{\HwMixedCellsAOne}{16}  %
\newcommand{\HwMixedCellsNSix}{9}  %
\newcommand{\HwMixedModelsAOne}{4}  %
\newcommand{\HwMixedCondsAOne}{\etype{boundary} L1 and \etype{shift} L1}  %
\newcommand{\HwMixedCondsNSixBurn}{boundary L2, clean, omission L2 and shift L2}  %
\newcommand{\HwMixedCellsNSixBurn}{4}
\newcommand{\HwMixedCondsNSixFlair}{boundary L2, clean, coarse L2, omission L2 and shift L2}  %
\newcommand{\HwMixedCellsNSixFlair}{5}
\newcommand{\GpuRatioPro}{1.44}  %
\newcommand{\GpuRatioCellsPro}{72}
\newcommand{\GpuRatioGb}{3.02}  %
\newcommand{\GpuRatioCellsGb}{51}
\newcommand{\GpuHoursPro}{375}  %
\newcommand{\GpuHoursGb}{195}  %
\newcommand{\GpuHoursRtx}{46}  %
\newcommand{\GpuHoursRtxEquiv}{372}  %
\newcommand{\NBurnTest}{120}  %
\newcommand{\NFlairTest}{3{,}022}  %
\newcommand{\NFlairClasses}{13}  %
\newcommand{\NBurnClasses}{2}  %
\newcommand{\NBurnBands}{6}  %
\newcommand{\NSeeds}{5}  %
\newcommand{\MaxEpochs}{50}  %
\newcommand{\PatienceChecks}{5}  %
\newcommand{\ValEvery}{2}  %
\newcommand{\CropPx}{224}  %
\newcommand{\TilePx}{512}  %
\newcommand{\MemCrops}{64}  %
\newcommand{\TostMargin}{3}  %
\newcommand{\SubsetPct}{25}  %
\newcommand{\CostRatio}{4 to 1}  %
\newcommand{\AlphaFam}{0.05}  %
\newcommand{\NFiveMde}{4}  %
\newcommand{\CollapseIoU}{0.15}  %
\newcommand{\NFiveSeeds}{6 to 8}  %
\newcommand{\NFiveSeedsAt}{3}  %
\newcommand{\Ndf}{4}  %
\newcommand{\CalSeed}{1}  %
\newcommand{\WeightDecay}{0.01}  %
\newcommand{\TileGrid}{3}  %
\newcommand{\CiLevel}{95}  %
\newcommand{\ResBurnM}{30}  %
\newcommand{\ResFlairM}{0.2}  %
\newcommand{\MdeFactor}{2.1}  %
\newcommand{\MdePower}{80}  %
\newcommand{\MdeAlpha}{0.025}  %
\newcommand{\BoundaryDPxNarrow}{3}  %
\newcommand{\NSOneTrain}{252}  %
\newcommand{\NSOneVal}{89}  %
\newcommand{\NSOneTest}{90}  %
\newcommand{\NSOneBands}{13}  %
\newcommand{\ResSOneM}{10}  %
\newcommand{\NSOneEvents}{11}  %
\newcommand{\NSOneHandChips}{446}  %


==> generated/macros.tex <==
%
\providecommand{\gcvdry}[1]{\textcolor{red}{#1}}
%
%
\newcommand{\nDinovThreeConvnextLburnBoundaryLOne}{5}
\newcommand{\miouDinovThreeConvnextLburnBoundaryLOne}{78.9}
\newcommand{\miouCIDinovThreeConvnextLburnBoundaryLOne}{1.9}
\newcommand{\dropDinovThreeConvnextLburnBoundaryLOne}{2.7}
\newcommand{\dropCIDinovThreeConvnextLburnBoundaryLOne}{2.2}
\newcommand{\retDinovThreeConvnextLburnBoundaryLOne}{0.967}
\newcommand{\retCIDinovThreeConvnextLburnBoundaryLOne}{0.027}
\newcommand{\nDinovThreeConvnextLburnBoundaryLTwo}{5}
\newcommand{\miouDinovThreeConvnextLburnBoundaryLTwo}{70.0}
\newcommand{\miouCIDinovThreeConvnextLburnBoundaryLTwo}{3.0}
\newcommand{\dropDinovThreeConvnextLburnBoundaryLTwo}{11.6}
\newcommand{\dropCIDinovThreeConvnextLburnBoundaryLTwo}{4.4}
\newcommand{\retDinovThreeConvnextLburnBoundaryLTwo}{0.859}
\newcommand{\retCIDinovThreeConvnextLburnBoundaryLTwo}{0.052}
\newcommand{\nDinovThreeConvnextLburnClean}{5}
\newcommand{\miouDinovThreeConvnextLburnClean}{81.6}
\newcommand{\miouCIDinovThreeConvnextLburnClean}{2.1}
\newcommand{\nDinovThreeConvnextLburnCleanVarTrainSubsetCleanTwoFive}{5}
\newcommand{\miouDinovThreeConvnextLburnCleanVarTrainSubsetCleanTwoFive}{74.6}
\newcommand{\miouCIDinovThreeConvnextLburnCleanVarTrainSubsetCleanTwoFive}{4.9}
\newcommand{\nDinovThreeConvnextLburnCoarseLOne}{5}
\newcommand{\miouDinovThreeConvnextLburnCoarseLOne}{77.9}
\newcommand{\miouCIDinovThreeConvnextLburnCoarseLOne}{1.1}
\newcommand{\dropDinovThreeConvnextLburnCoarseLOne}{3.8}
\newcommand{\dropCIDinovThreeConvnextLburnCoarseLOne}{2.2}
\newcommand{\retDinovThreeConvnextLburnCoarseLOne}{0.954}
\newcommand{\retCIDinovThreeConvnextLburnCoarseLOne}{0.026}
\newcommand{\nDinovThreeConvnextLburnCoarseLTwo}{5}
\newcommand{\miouDinovThreeConvnextLburnCoarseLTwo}{64.3}
\newcommand{\miouCIDinovThreeConvnextLburnCoarseLTwo}{3.1}
\newcommand{\dropDinovThreeConvnextLburnCoarseLTwo}{17.3}
\newcommand{\dropCIDinovThreeConvnextLburnCoarseLTwo}{3.7}
\newcommand{\retDinovThreeConvnextLburnCoarseLTwo}{0.788}
\newcommand{\retCIDinovThreeConvnextLburnCoarseLTwo}{0.042}
\newcommand{\nDinovThreeConvnextLburnOmissionLOne}{5}
\newcommand{\miouDinovThreeConvnextLburnOmissionLOne}{76.2}
\newcommand{\miouCIDinovThreeConvnextLburnOmissionLOne}{2.8}
\newcommand{\dropDinovThreeConvnextLburnOmissionLOne}{5.5}
\newcommand{\dropCIDinovThreeConvnextLburnOmissionLOne}{4.2}
\newcommand{\retDinovThreeConvnextLburnOmissionLOne}{0.934}
\newcommand{\retCIDinovThreeConvnextLburnOmissionLOne}{0.050}
\newcommand{\nDinovThreeConvnextLburnOmissionLTwo}{5}
\newcommand{\miouDinovThreeConvnextLburnOmissionLTwo}{60.3}
\newcommand{\miouCIDinovThreeConvnextLburnOmissionLTwo}{10.2}
\newcommand{\dropDinovThreeConvnextLburnOmissionLTwo}{21.3}
\newcommand{\dropCIDinovThreeConvnextLburnOmissionLTwo}{11.5}
\newcommand{\retDinovThreeConvnextLburnOmissionLTwo}{0.740}
\newcommand{\retCIDinovThreeConvnextLburnOmissionLTwo}{0.135}
\newcommand{\nDinovThreeConvnextLburnShiftLOne}{5}
\newcommand{\miouDinovThreeConvnextLburnShiftLOne}{79.3}
\newcommand{\miouCIDinovThreeConvnextLburnShiftLOne}{4.8}
\newcommand{\dropDinovThreeConvnextLburnShiftLOne}{2.3}
\newcommand{\dropCIDinovThreeConvnextLburnShiftLOne}{5.1}
\newcommand{\retDinovThreeConvnextLburnShiftLOne}{0.972}
\newcommand{\retCIDinovThreeConvnextLburnShiftLOne}{0.063}
\newcommand{\nDinovThreeConvnextLburnShiftLTwo}{5}
\newcommand{\miouDinovThreeConvnextLburnShiftLTwo}{67.9}
\newcommand{\miouCIDinovThreeConvnextLburnShiftLTwo}{9.2}
\newcommand{\dropDinovThreeConvnextLburnShiftLTwo}{13.8}
\newcommand{\dropCIDinovThreeConvnextLburnShiftLTwo}{9.3}
\newcommand{\retDinovThreeConvnextLburnShiftLTwo}{0.831}
\newcommand{\retCIDinovThreeConvnextLburnShiftLTwo}{0.114}
\newcommand{\nDinovThreeConvnextLflairBoundaryLOne}{5}
\newcommand{\miouDinovThreeConvnextLflairBoundaryLOne}{45.8}
\newcommand{\miouCIDinovThreeConvnextLflairBoundaryLOne}{1.4}
\newcommand{\dropDinovThreeConvnextLflairBoundaryLOne}{1.8}
\newcommand{\dropCIDinovThreeConvnextLflairBoundaryLOne}{1.6}
\newcommand{\retDinovThreeConvnextLflairBoundaryLOne}{0.963}
\newcommand{\retCIDinovThreeConvnextLflairBoundaryLOne}{0.033}
\newcommand{\nDinovThreeConvnextLflairBoundaryLTwo}{5}
\newcommand{\miouDinovThreeConvnextLflairBoundaryLTwo}{43.9}
\newcommand{\miouCIDinovThreeConvnextLflairBoundaryLTwo}{0.9}
\newcommand{\dropDinovThreeConvnextLflairBoundaryLTwo}{3.6}
\newcommand{\dropCIDinovThreeConvnextLflairBoundaryLTwo}{2.2}
\newcommand{\retDinovThreeConvnextLflairBoundaryLTwo}{0.924}
\newcommand{\retCIDinovThreeConvnextLflairBoundaryLTwo}{0.044}
\newcommand{\nDinovThreeConvnextLflairClean}{5}
\newcommand{\miouDinovThreeConvnextLflairClean}{47.6}
\newcommand{\miouCIDinovThreeConvnextLflairClean}{1.4}
\newcommand{\nDinovThreeConvnextLflairCleanVarTrainSubsetCleanTwoFive}{5}
\newcommand{\miouDinovThreeConvnextLflairCleanVarTrainSubsetCleanTwoFive}{43.5}
\newcommand{\miouCIDinovThreeConvnextLflairCleanVarTrainSubsetCleanTwoFive}{1.8}
\newcommand{\nDinovThreeConvnextLflairCoarseLOne}{5}
\newcommand{\miouDinovThreeConvnextLflairCoarseLOne}{46.7}
\newcommand{\miouCIDinovThreeConvnextLflairCoarseLOne}{1.0}
\newcommand{\dropDinovThreeConvnextLflairCoarseLOne}{0.8}
\newcommand{\dropCIDinovThreeConvnextLflairCoarseLOne}{1.5}
\newcommand{\retDinovThreeConvnextLflairCoarseLOne}{0.983}
\newcommand{\retCIDinovThreeConvnextLflairCoarseLOne}{0.031}
\newcommand{\nDinovThreeConvnextLflairCoarseLTwo}{5}
\newcommand{\miouDinovThreeConvnextLflairCoarseLTwo}{41.9}
\newcommand{\miouCIDinovThreeConvnextLflairCoarseLTwo}{1.1}
\newcommand{\dropDinovThreeConvnextLflairCoarseLTwo}{5.7}
\newcommand{\dropCIDinovThreeConvnextLflairCoarseLTwo}{1.0}
\newcommand{\retDinovThreeConvnextLflairCoarseLTwo}{0.881}
\newcommand{\retCIDinovThreeConvnextLflairCoarseLTwo}{0.019}
\newcommand{\nDinovThreeConvnextLflairOmissionLOne}{5}
\newcommand{\miouDinovThreeConvnextLflairOmissionLOne}{45.9}
\newcommand{\miouCIDinovThreeConvnextLflairOmissionLOne}{2.6}
\newcommand{\dropDinovThreeConvnextLflairOmissionLOne}{1.7}
\newcommand{\dropCIDinovThreeConvnextLflairOmissionLOne}{2.0}
\newcommand{\retDinovThreeConvnextLflairOmissionLOne}{0.965}
\newcommand{\retCIDinovThreeConvnextLflairOmissionLOne}{0.042}
\newcommand{\nDinovThreeConvnextLflairOmissionLTwo}{5}
\newcommand{\miouDinovThreeConvnextLflairOmissionLTwo}{43.5}
\newcommand{\miouCIDinovThreeConvnextLflairOmissionLTwo}{1.9}
\newcommand{\dropDinovThreeConvnextLflairOmissionLTwo}{4.0}
\newcommand{\dropCIDinovThreeConvnextLflairOmissionLTwo}{2.4}
\newcommand{\retDinovThreeConvnextLflairOmissionLTwo}{0.916}
\newcommand{\retCIDinovThreeConvnextLflairOmissionLTwo}{0.050}
\newcommand{\nDinovThreeConvnextLflairShiftLOne}{5}
\newcommand{\miouDinovThreeConvnextLflairShiftLOne}{47.1}
\newcommand{\miouCIDinovThreeConvnextLflairShiftLOne}{1.6}
\newcommand{\dropDinovThreeConvnextLflairShiftLOne}{0.5}
\newcommand{\dropCIDinovThreeConvnextLflairShiftLOne}{2.0}
\newcommand{\retDinovThreeConvnextLflairShiftLOne}{0.990}
\newcommand{\retCIDinovThreeConvnextLflairShiftLOne}{0.043}
\newcommand{\nDinovThreeConvnextLflairShiftLTwo}{5}
\newcommand{\miouDinovThreeConvnextLflairShiftLTwo}{44.9}
\newcommand{\miouCIDinovThreeConvnextLflairShiftLTwo}{1.3}
\newcommand{\dropDinovThreeConvnextLflairShiftLTwo}{2.6}
\newcommand{\dropCIDinovThreeConvnextLflairShiftLTwo}{2.2}
\newcommand{\retDinovThreeConvnextLflairShiftLTwo}{0.945}
\newcommand{\retCIDinovThreeConvnextLflairShiftLTwo}{0.045}
\newcommand{\nLVDburnBoundaryLOne}{5}
\newcommand{\miouLVDburnBoundaryLOne}{78.3}
\newcommand{\miouCILVDburnBoundaryLOne}{0.8}
\newcommand{\dropLVDburnBoundaryLOne}{3.7}
\newcommand{\dropCILVDburnBoundaryLOne}{1.2}
\newcommand{\retLVDburnBoundaryLOne}{0.955}
\newcommand{\retCILVDburnBoundaryLOne}{0.015}
\newcommand{\nLVDburnBoundaryLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouLVDburnBoundaryLOneVarDecoderMaskTwoformerFull}{77.8}
\newcommand{\miouCILVDburnBoundaryLOneVarDecoderMaskTwoformerFull}{1.5}
\newcommand{\dropLVDburnBoundaryLOneVarDecoderMaskTwoformerFull}{1.2}
\newcommand{\dropCILVDburnBoundaryLOneVarDecoderMaskTwoformerFull}{3.7}
\newcommand{\retLVDburnBoundaryLOneVarDecoderMaskTwoformerFull}{0.986}
\newcommand{\retCILVDburnBoundaryLOneVarDecoderMaskTwoformerFull}{0.047}
\newcommand{\nLVDburnBoundaryLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDburnBoundaryLOneVarDecoderMaskTwoformerLite}{79.5}
\newcommand{\miouCILVDburnBoundaryLOneVarDecoderMaskTwoformerLite}{2.1}
\newcommand{\dropLVDburnBoundaryLOneVarDecoderMaskTwoformerLite}{3.9}
\newcommand{\dropCILVDburnBoundaryLOneVarDecoderMaskTwoformerLite}{1.3}
\newcommand{\retLVDburnBoundaryLOneVarDecoderMaskTwoformerLite}{0.953}
\newcommand{\retCILVDburnBoundaryLOneVarDecoderMaskTwoformerLite}{0.017}
\newcommand{\nLVDburnBoundaryLOneVarDecoderSamLite}{5}
\newcommand{\miouLVDburnBoundaryLOneVarDecoderSamLite}{78.7}
\newcommand{\miouCILVDburnBoundaryLOneVarDecoderSamLite}{2.6}
\newcommand{\dropLVDburnBoundaryLOneVarDecoderSamLite}{3.9}
\newcommand{\dropCILVDburnBoundaryLOneVarDecoderSamLite}{3.6}
\newcommand{\retLVDburnBoundaryLOneVarDecoderSamLite}{0.953}
\newcommand{\retCILVDburnBoundaryLOneVarDecoderSamLite}{0.043}
\newcommand{\nLVDburnBoundaryLOneVarDecoderSamPretrained}{5}
\newcommand{\miouLVDburnBoundaryLOneVarDecoderSamPretrained}{72.5}
\newcommand{\miouCILVDburnBoundaryLOneVarDecoderSamPretrained}{19.2}
\newcommand{\dropLVDburnBoundaryLOneVarDecoderSamPretrained}{1.5}
\newcommand{\dropCILVDburnBoundaryLOneVarDecoderSamPretrained}{3.1}
\newcommand{\retLVDburnBoundaryLOneVarDecoderSamPretrained}{0.982}
\newcommand{\retCILVDburnBoundaryLOneVarDecoderSamPretrained}{0.037}
\newcommand{\nLVDburnBoundaryLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDburnBoundaryLOneVarDecoderSegformerMlp}{79.2}
\newcommand{\miouCILVDburnBoundaryLOneVarDecoderSegformerMlp}{1.6}
\newcommand{\dropLVDburnBoundaryLOneVarDecoderSegformerMlp}{4.2}
\newcommand{\dropCILVDburnBoundaryLOneVarDecoderSegformerMlp}{2.6}
\newcommand{\retLVDburnBoundaryLOneVarDecoderSegformerMlp}{0.950}
\newcommand{\retCILVDburnBoundaryLOneVarDecoderSegformerMlp}{0.031}
\newcommand{\nLVDburnBoundaryLTwo}{8}
\newcommand{\miouLVDburnBoundaryLTwo}{69.6}
\newcommand{\miouCILVDburnBoundaryLTwo}{1.4}
\newcommand{\dropLVDburnBoundaryLTwo}{12.2}
\newcommand{\dropCILVDburnBoundaryLTwo}{2.4}
\newcommand{\retLVDburnBoundaryLTwo}{0.852}
\newcommand{\retCILVDburnBoundaryLTwo}{0.028}
\newcommand{\nLVDburnBoundaryLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouLVDburnBoundaryLTwoVarDecoderMaskTwoformerFull}{53.0}
\newcommand{\miouCILVDburnBoundaryLTwoVarDecoderMaskTwoformerFull}{14.0}
\newcommand{\dropLVDburnBoundaryLTwoVarDecoderMaskTwoformerFull}{26.0}
\newcommand{\dropCILVDburnBoundaryLTwoVarDecoderMaskTwoformerFull}{15.6}
\newcommand{\retLVDburnBoundaryLTwoVarDecoderMaskTwoformerFull}{0.673}
\newcommand{\retCILVDburnBoundaryLTwoVarDecoderMaskTwoformerFull}{0.194}
\newcommand{\nLVDburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}{5}
\newcommand{\miouLVDburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}{44.8}
\newcommand{\miouCILVDburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}{0.0}
\newcommand{\dropLVDburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}{24.0}
\newcommand{\dropCILVDburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}{2.8}
\newcommand{\retLVDburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}{0.652}
\newcommand{\retCILVDburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}{0.027}
\newcommand{\nLVDburnBoundaryLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDburnBoundaryLTwoVarDecoderMaskTwoformerLite}{67.6}
\newcommand{\miouCILVDburnBoundaryLTwoVarDecoderMaskTwoformerLite}{2.3}
\newcommand{\dropLVDburnBoundaryLTwoVarDecoderMaskTwoformerLite}{15.8}
\newcommand{\dropCILVDburnBoundaryLTwoVarDecoderMaskTwoformerLite}{1.9}
\newcommand{\retLVDburnBoundaryLTwoVarDecoderMaskTwoformerLite}{0.811}
\newcommand{\retCILVDburnBoundaryLTwoVarDecoderMaskTwoformerLite}{0.023}
\newcommand{\nLVDburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}{5}
\newcommand{\miouLVDburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}{44.8}
\newcommand{\miouCILVDburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}{0.0}
\newcommand{\dropLVDburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}{0.0}
\newcommand{\dropCILVDburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}{0.0}
\newcommand{\retLVDburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}{1.000}
\newcommand{\retCILVDburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}{0.000}
\newcommand{\nLVDburnBoundaryLTwoVarDecoderSamLite}{5}
\newcommand{\miouLVDburnBoundaryLTwoVarDecoderSamLite}{68.6}
\newcommand{\miouCILVDburnBoundaryLTwoVarDecoderSamLite}{2.3}
\newcommand{\dropLVDburnBoundaryLTwoVarDecoderSamLite}{14.0}
\newcommand{\dropCILVDburnBoundaryLTwoVarDecoderSamLite}{1.9}
\newcommand{\retLVDburnBoundaryLTwoVarDecoderSamLite}{0.831}
\newcommand{\retCILVDburnBoundaryLTwoVarDecoderSamLite}{0.022}
\newcommand{\nLVDburnBoundaryLTwoVarDecoderSamLiteLrMultOne}{5}
\newcommand{\miouLVDburnBoundaryLTwoVarDecoderSamLiteLrMultOne}{60.7}
\newcommand{\miouCILVDburnBoundaryLTwoVarDecoderSamLiteLrMultOne}{2.7}
\newcommand{\dropLVDburnBoundaryLTwoVarDecoderSamLiteLrMultOne}{13.9}
\newcommand{\dropCILVDburnBoundaryLTwoVarDecoderSamLiteLrMultOne}{6.1}
\newcommand{\retLVDburnBoundaryLTwoVarDecoderSamLiteLrMultOne}{0.817}
\newcommand{\retCILVDburnBoundaryLTwoVarDecoderSamLiteLrMultOne}{0.073}
\newcommand{\nLVDburnBoundaryLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouLVDburnBoundaryLTwoVarDecoderSamPretrained}{49.7}
\newcommand{\miouCILVDburnBoundaryLTwoVarDecoderSamPretrained}{13.7}
\newcommand{\dropLVDburnBoundaryLTwoVarDecoderSamPretrained}{24.2}
\newcommand{\dropCILVDburnBoundaryLTwoVarDecoderSamPretrained}{20.3}
\newcommand{\retLVDburnBoundaryLTwoVarDecoderSamPretrained}{0.700}
\newcommand{\retCILVDburnBoundaryLTwoVarDecoderSamPretrained}{0.253}
\newcommand{\nLVDburnBoundaryLTwoVarDecoderSamPretrainedLrMultOne}{5}
\newcommand{\miouLVDburnBoundaryLTwoVarDecoderSamPretrainedLrMultOne}{50.5}
\newcommand{\miouCILVDburnBoundaryLTwoVarDecoderSamPretrainedLrMultOne}{9.9}
\newcommand{\dropLVDburnBoundaryLTwoVarDecoderSamPretrainedLrMultOne}{24.2}
\newcommand{\dropCILVDburnBoundaryLTwoVarDecoderSamPretrainedLrMultOne}{11.5}
\newcommand{\retLVDburnBoundaryLTwoVarDecoderSamPretrainedLrMultOne}{0.678}
\newcommand{\retCILVDburnBoundaryLTwoVarDecoderSamPretrainedLrMultOne}{0.149}
\newcommand{\nLVDburnBoundaryLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDburnBoundaryLTwoVarDecoderSegformerMlp}{68.3}
\newcommand{\miouCILVDburnBoundaryLTwoVarDecoderSegformerMlp}{2.5}
\newcommand{\dropLVDburnBoundaryLTwoVarDecoderSegformerMlp}{15.1}
\newcommand{\dropCILVDburnBoundaryLTwoVarDecoderSegformerMlp}{3.4}
\newcommand{\retLVDburnBoundaryLTwoVarDecoderSegformerMlp}{0.819}
\newcommand{\retCILVDburnBoundaryLTwoVarDecoderSegformerMlp}{0.039}
\newcommand{\nLVDburnBoundaryLTwoVarDecoderSegformerMlpLrMultOne}{5}
\newcommand{\miouLVDburnBoundaryLTwoVarDecoderSegformerMlpLrMultOne}{64.1}
\newcommand{\miouCILVDburnBoundaryLTwoVarDecoderSegformerMlpLrMultOne}{3.3}
\newcommand{\dropLVDburnBoundaryLTwoVarDecoderSegformerMlpLrMultOne}{15.2}
\newcommand{\dropCILVDburnBoundaryLTwoVarDecoderSegformerMlpLrMultOne}{4.0}
\newcommand{\retLVDburnBoundaryLTwoVarDecoderSegformerMlpLrMultOne}{0.808}
\newcommand{\retCILVDburnBoundaryLTwoVarDecoderSegformerMlpLrMultOne}{0.048}
\newcommand{\nLVDburnBoundaryLTwoVarLossBootstrap}{5}
\newcommand{\miouLVDburnBoundaryLTwoVarLossBootstrap}{70.2}
\newcommand{\miouCILVDburnBoundaryLTwoVarLossBootstrap}{4.9}
\newcommand{\dropLVDburnBoundaryLTwoVarLossBootstrap}{11.8}
\newcommand{\dropCILVDburnBoundaryLTwoVarLossBootstrap}{5.9}
\newcommand{\retLVDburnBoundaryLTwoVarLossBootstrap}{0.856}
\newcommand{\retCILVDburnBoundaryLTwoVarLossBootstrap}{0.068}
\newcommand{\nLVDburnBoundaryLTwoVarLossGce}{5}
\newcommand{\miouLVDburnBoundaryLTwoVarLossGce}{69.9}
\newcommand{\miouCILVDburnBoundaryLTwoVarLossGce}{2.2}
\newcommand{\dropLVDburnBoundaryLTwoVarLossGce}{11.3}
\newcommand{\dropCILVDburnBoundaryLTwoVarLossGce}{2.1}
\newcommand{\retLVDburnBoundaryLTwoVarLossGce}{0.860}
\newcommand{\retCILVDburnBoundaryLTwoVarLossGce}{0.026}
\newcommand{\nLVDburnBoundaryLTwoVarLrMultOne}{5}
\newcommand{\miouLVDburnBoundaryLTwoVarLrMultOne}{63.5}
\newcommand{\miouCILVDburnBoundaryLTwoVarLrMultOne}{2.8}
\newcommand{\dropLVDburnBoundaryLTwoVarLrMultOne}{14.8}
\newcommand{\dropCILVDburnBoundaryLTwoVarLrMultOne}{4.1}
\newcommand{\retLVDburnBoundaryLTwoVarLrMultOne}{0.811}
\newcommand{\retCILVDburnBoundaryLTwoVarLrMultOne}{0.046}
\newcommand{\nLVDburnBoundaryLR}{5}
\newcommand{\miouLVDburnBoundaryLR}{63.3}
\newcommand{\miouCILVDburnBoundaryLR}{4.8}
\newcommand{\dropLVDburnBoundaryLR}{18.7}
\newcommand{\dropCILVDburnBoundaryLR}{4.2}
\newcommand{\retLVDburnBoundaryLR}{0.772}
\newcommand{\retCILVDburnBoundaryLR}{0.053}
\newcommand{\nLVDburnBoundaryLRVarLrMultOne}{5}
\newcommand{\miouLVDburnBoundaryLRVarLrMultOne}{56.0}
\newcommand{\miouCILVDburnBoundaryLRVarLrMultOne}{4.4}
\newcommand{\dropLVDburnBoundaryLRVarLrMultOne}{22.3}
\newcommand{\dropCILVDburnBoundaryLRVarLrMultOne}{5.5}
\newcommand{\retLVDburnBoundaryLRVarLrMultOne}{0.716}
\newcommand{\retCILVDburnBoundaryLRVarLrMultOne}{0.064}
\newcommand{\nLVDburnClean}{8}
\newcommand{\miouLVDburnClean}{81.8}
\newcommand{\miouCILVDburnClean}{1.3}
\newcommand{\nLVDburnCleanVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouLVDburnCleanVarDecoderMaskTwoformerFull}{79.0}
\newcommand{\miouCILVDburnCleanVarDecoderMaskTwoformerFull}{3.9}
\newcommand{\nLVDburnCleanVarDecoderMaskTwoformerFullLrMultOne}{5}
\newcommand{\miouLVDburnCleanVarDecoderMaskTwoformerFullLrMultOne}{68.7}
\newcommand{\miouCILVDburnCleanVarDecoderMaskTwoformerFullLrMultOne}{2.8}
\newcommand{\nLVDburnCleanVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDburnCleanVarDecoderMaskTwoformerLite}{83.4}
\newcommand{\miouCILVDburnCleanVarDecoderMaskTwoformerLite}{0.8}
\newcommand{\nLVDburnCleanVarDecoderMaskTwoformerLiteLrMultOne}{5}
\newcommand{\miouLVDburnCleanVarDecoderMaskTwoformerLiteLrMultOne}{44.8}
\newcommand{\miouCILVDburnCleanVarDecoderMaskTwoformerLiteLrMultOne}{0.0}
\newcommand{\nLVDburnCleanVarDecoderSamLite}{5}
\newcommand{\miouLVDburnCleanVarDecoderSamLite}{82.5}
\newcommand{\miouCILVDburnCleanVarDecoderSamLite}{2.0}
\newcommand{\nLVDburnCleanVarDecoderSamLiteLrMultOne}{5}
\newcommand{\miouLVDburnCleanVarDecoderSamLiteLrMultOne}{74.6}
\newcommand{\miouCILVDburnCleanVarDecoderSamLiteLrMultOne}{6.0}
\newcommand{\nLVDburnCleanVarDecoderSamPretrained}{5}
\newcommand{\miouLVDburnCleanVarDecoderSamPretrained}{73.9}
\newcommand{\miouCILVDburnCleanVarDecoderSamPretrained}{20.4}
\newcommand{\nLVDburnCleanVarDecoderSamPretrainedLrMultOne}{5}
\newcommand{\miouLVDburnCleanVarDecoderSamPretrainedLrMultOne}{74.7}
\newcommand{\miouCILVDburnCleanVarDecoderSamPretrainedLrMultOne}{2.8}
\newcommand{\nLVDburnCleanVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDburnCleanVarDecoderSegformerMlp}{83.4}
\newcommand{\miouCILVDburnCleanVarDecoderSegformerMlp}{1.3}
\newcommand{\nLVDburnCleanVarDecoderSegformerMlpLrMultOne}{5}
\newcommand{\miouLVDburnCleanVarDecoderSegformerMlpLrMultOne}{79.4}
\newcommand{\miouCILVDburnCleanVarDecoderSegformerMlpLrMultOne}{1.8}
\newcommand{\nLVDburnCleanVarLossBootstrap}{5}
\newcommand{\miouLVDburnCleanVarLossBootstrap}{82.0}
\newcommand{\miouCILVDburnCleanVarLossBootstrap}{2.2}
\newcommand{\nLVDburnCleanVarLossGce}{5}
\newcommand{\miouLVDburnCleanVarLossGce}{81.3}
\newcommand{\miouCILVDburnCleanVarLossGce}{0.1}
\newcommand{\nLVDburnCleanVarLrMultOne}{5}
\newcommand{\miouLVDburnCleanVarLrMultOne}{78.3}
\newcommand{\miouCILVDburnCleanVarLrMultOne}{3.0}
\newcommand{\nLVDburnCleanVarLrMultThree}{1}
\newcommand{\miouLVDburnCleanVarLrMultThree}{53.1}
\newcommand{\miouCILVDburnCleanVarLrMultThree}{--}
\newcommand{\nLVDburnCleanVarTrainSubsetCleanTwoFive}{5}
\newcommand{\miouLVDburnCleanVarTrainSubsetCleanTwoFive}{77.5}
\newcommand{\miouCILVDburnCleanVarTrainSubsetCleanTwoFive}{1.9}
\newcommand{\nLVDburnCoarseLOne}{5}
\newcommand{\miouLVDburnCoarseLOne}{79.4}
\newcommand{\miouCILVDburnCoarseLOne}{1.0}
\newcommand{\dropLVDburnCoarseLOne}{2.7}
\newcommand{\dropCILVDburnCoarseLOne}{1.5}
\newcommand{\retLVDburnCoarseLOne}{0.968}
\newcommand{\retCILVDburnCoarseLOne}{0.018}
\newcommand{\nLVDburnCoarseLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouLVDburnCoarseLOneVarDecoderMaskTwoformerFull}{76.8}
\newcommand{\miouCILVDburnCoarseLOneVarDecoderMaskTwoformerFull}{3.2}
\newcommand{\dropLVDburnCoarseLOneVarDecoderMaskTwoformerFull}{2.2}
\newcommand{\dropCILVDburnCoarseLOneVarDecoderMaskTwoformerFull}{4.0}
\newcommand{\retLVDburnCoarseLOneVarDecoderMaskTwoformerFull}{0.973}
\newcommand{\retCILVDburnCoarseLOneVarDecoderMaskTwoformerFull}{0.052}
\newcommand{\nLVDburnCoarseLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDburnCoarseLOneVarDecoderMaskTwoformerLite}{78.1}
\newcommand{\miouCILVDburnCoarseLOneVarDecoderMaskTwoformerLite}{1.4}
\newcommand{\dropLVDburnCoarseLOneVarDecoderMaskTwoformerLite}{5.2}
\newcommand{\dropCILVDburnCoarseLOneVarDecoderMaskTwoformerLite}{1.8}
\newcommand{\retLVDburnCoarseLOneVarDecoderMaskTwoformerLite}{0.937}
\newcommand{\retCILVDburnCoarseLOneVarDecoderMaskTwoformerLite}{0.021}
\newcommand{\nLVDburnCoarseLOneVarDecoderSamLite}{5}
\newcommand{\miouLVDburnCoarseLOneVarDecoderSamLite}{77.9}
\newcommand{\miouCILVDburnCoarseLOneVarDecoderSamLite}{1.2}
\newcommand{\dropLVDburnCoarseLOneVarDecoderSamLite}{4.6}
\newcommand{\dropCILVDburnCoarseLOneVarDecoderSamLite}{1.2}
\newcommand{\retLVDburnCoarseLOneVarDecoderSamLite}{0.944}
\newcommand{\retCILVDburnCoarseLOneVarDecoderSamLite}{0.013}
\newcommand{\nLVDburnCoarseLOneVarDecoderSamPretrained}{5}
\newcommand{\miouLVDburnCoarseLOneVarDecoderSamPretrained}{64.2}
\newcommand{\miouCILVDburnCoarseLOneVarDecoderSamPretrained}{22.1}
\newcommand{\dropLVDburnCoarseLOneVarDecoderSamPretrained}{9.7}
\newcommand{\dropCILVDburnCoarseLOneVarDecoderSamPretrained}{18.3}
\newcommand{\retLVDburnCoarseLOneVarDecoderSamPretrained}{0.880}
\newcommand{\retCILVDburnCoarseLOneVarDecoderSamPretrained}{0.227}
\newcommand{\nLVDburnCoarseLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDburnCoarseLOneVarDecoderSegformerMlp}{79.7}
\newcommand{\miouCILVDburnCoarseLOneVarDecoderSegformerMlp}{1.0}
\newcommand{\dropLVDburnCoarseLOneVarDecoderSegformerMlp}{3.6}
\newcommand{\dropCILVDburnCoarseLOneVarDecoderSegformerMlp}{1.5}
\newcommand{\retLVDburnCoarseLOneVarDecoderSegformerMlp}{0.956}
\newcommand{\retCILVDburnCoarseLOneVarDecoderSegformerMlp}{0.018}
\newcommand{\nLVDburnCoarseLTwo}{8}
\newcommand{\miouLVDburnCoarseLTwo}{66.4}
\newcommand{\miouCILVDburnCoarseLTwo}{1.8}
\newcommand{\dropLVDburnCoarseLTwo}{15.5}
\newcommand{\dropCILVDburnCoarseLTwo}{1.8}
\newcommand{\retLVDburnCoarseLTwo}{0.811}
\newcommand{\retCILVDburnCoarseLTwo}{0.021}
\newcommand{\nLVDburnCoarseLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouLVDburnCoarseLTwoVarDecoderMaskTwoformerFull}{44.8}
\newcommand{\miouCILVDburnCoarseLTwoVarDecoderMaskTwoformerFull}{0.0}
\newcommand{\dropLVDburnCoarseLTwoVarDecoderMaskTwoformerFull}{34.3}
\newcommand{\dropCILVDburnCoarseLTwoVarDecoderMaskTwoformerFull}{3.9}
\newcommand{\retLVDburnCoarseLTwoVarDecoderMaskTwoformerFull}{0.567}
\newcommand{\retCILVDburnCoarseLTwoVarDecoderMaskTwoformerFull}{0.028}
\newcommand{\nLVDburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}{5}
\newcommand{\miouLVDburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}{44.8}
\newcommand{\miouCILVDburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}{0.0}
\newcommand{\dropLVDburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}{24.0}
\newcommand{\dropCILVDburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}{2.8}
\newcommand{\retLVDburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}{0.652}
\newcommand{\retCILVDburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}{0.027}
\newcommand{\nLVDburnCoarseLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDburnCoarseLTwoVarDecoderMaskTwoformerLite}{64.1}
\newcommand{\miouCILVDburnCoarseLTwoVarDecoderMaskTwoformerLite}{2.4}
\newcommand{\dropLVDburnCoarseLTwoVarDecoderMaskTwoformerLite}{19.3}
\newcommand{\dropCILVDburnCoarseLTwoVarDecoderMaskTwoformerLite}{1.9}
\newcommand{\retLVDburnCoarseLTwoVarDecoderMaskTwoformerLite}{0.769}
\newcommand{\retCILVDburnCoarseLTwoVarDecoderMaskTwoformerLite}{0.024}
\newcommand{\nLVDburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}{5}
\newcommand{\miouLVDburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}{44.8}
\newcommand{\miouCILVDburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}{0.0}
\newcommand{\dropLVDburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}{0.0}
\newcommand{\dropCILVDburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}{0.0}
\newcommand{\retLVDburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}{1.000}
\newcommand{\retCILVDburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}{0.000}
\newcommand{\nLVDburnCoarseLTwoVarDecoderSamLite}{5}
\newcommand{\miouLVDburnCoarseLTwoVarDecoderSamLite}{54.8}
\newcommand{\miouCILVDburnCoarseLTwoVarDecoderSamLite}{11.5}
\newcommand{\dropLVDburnCoarseLTwoVarDecoderSamLite}{27.8}
\newcommand{\dropCILVDburnCoarseLTwoVarDecoderSamLite}{11.5}
\newcommand{\retLVDburnCoarseLTwoVarDecoderSamLite}{0.664}
\newcommand{\retCILVDburnCoarseLTwoVarDecoderSamLite}{0.140}
\newcommand{\nLVDburnCoarseLTwoVarDecoderSamLiteLrMultOne}{5}
\newcommand{\miouLVDburnCoarseLTwoVarDecoderSamLiteLrMultOne}{44.8}
\newcommand{\miouCILVDburnCoarseLTwoVarDecoderSamLiteLrMultOne}{0.0}
\newcommand{\dropLVDburnCoarseLTwoVarDecoderSamLiteLrMultOne}{29.8}
\newcommand{\dropCILVDburnCoarseLTwoVarDecoderSamLiteLrMultOne}{6.0}
\newcommand{\retLVDburnCoarseLTwoVarDecoderSamLiteLrMultOne}{0.603}
\newcommand{\retCILVDburnCoarseLTwoVarDecoderSamLiteLrMultOne}{0.052}
\newcommand{\nLVDburnCoarseLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouLVDburnCoarseLTwoVarDecoderSamPretrained}{49.1}
\newcommand{\miouCILVDburnCoarseLTwoVarDecoderSamPretrained}{12.0}
\newcommand{\dropLVDburnCoarseLTwoVarDecoderSamPretrained}{24.8}
\newcommand{\dropCILVDburnCoarseLTwoVarDecoderSamPretrained}{19.8}
\newcommand{\retLVDburnCoarseLTwoVarDecoderSamPretrained}{0.693}
\newcommand{\retCILVDburnCoarseLTwoVarDecoderSamPretrained}{0.247}
\newcommand{\nLVDburnCoarseLTwoVarDecoderSamPretrainedLrMultOne}{5}
\newcommand{\miouLVDburnCoarseLTwoVarDecoderSamPretrainedLrMultOne}{46.6}
\newcommand{\miouCILVDburnCoarseLTwoVarDecoderSamPretrainedLrMultOne}{5.1}
\newcommand{\dropLVDburnCoarseLTwoVarDecoderSamPretrainedLrMultOne}{28.1}
\newcommand{\dropCILVDburnCoarseLTwoVarDecoderSamPretrainedLrMultOne}{4.7}
\newcommand{\retLVDburnCoarseLTwoVarDecoderSamPretrainedLrMultOne}{0.624}
\newcommand{\retCILVDburnCoarseLTwoVarDecoderSamPretrainedLrMultOne}{0.062}
\newcommand{\nLVDburnCoarseLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDburnCoarseLTwoVarDecoderSegformerMlp}{65.5}
\newcommand{\miouCILVDburnCoarseLTwoVarDecoderSegformerMlp}{2.6}
\newcommand{\dropLVDburnCoarseLTwoVarDecoderSegformerMlp}{17.9}
\newcommand{\dropCILVDburnCoarseLTwoVarDecoderSegformerMlp}{1.7}
\newcommand{\retLVDburnCoarseLTwoVarDecoderSegformerMlp}{0.785}
\newcommand{\retCILVDburnCoarseLTwoVarDecoderSegformerMlp}{0.022}
\newcommand{\nLVDburnCoarseLTwoVarDecoderSegformerMlpLrMultOne}{5}
\newcommand{\miouLVDburnCoarseLTwoVarDecoderSegformerMlpLrMultOne}{60.8}
\newcommand{\miouCILVDburnCoarseLTwoVarDecoderSegformerMlpLrMultOne}{3.9}
\newcommand{\dropLVDburnCoarseLTwoVarDecoderSegformerMlpLrMultOne}{18.6}
\newcommand{\dropCILVDburnCoarseLTwoVarDecoderSegformerMlpLrMultOne}{3.0}
\newcommand{\retLVDburnCoarseLTwoVarDecoderSegformerMlpLrMultOne}{0.765}
\newcommand{\retCILVDburnCoarseLTwoVarDecoderSegformerMlpLrMultOne}{0.040}
\newcommand{\nLVDburnCoarseLTwoVarLossBootstrap}{5}
\newcommand{\miouLVDburnCoarseLTwoVarLossBootstrap}{67.0}
\newcommand{\miouCILVDburnCoarseLTwoVarLossBootstrap}{2.0}
\newcommand{\dropLVDburnCoarseLTwoVarLossBootstrap}{15.1}
\newcommand{\dropCILVDburnCoarseLTwoVarLossBootstrap}{1.4}
\newcommand{\retLVDburnCoarseLTwoVarLossBootstrap}{0.816}
\newcommand{\retCILVDburnCoarseLTwoVarLossBootstrap}{0.015}
\newcommand{\nLVDburnCoarseLTwoVarLossGce}{5}
\newcommand{\miouLVDburnCoarseLTwoVarLossGce}{65.3}
\newcommand{\miouCILVDburnCoarseLTwoVarLossGce}{1.8}
\newcommand{\dropLVDburnCoarseLTwoVarLossGce}{16.0}
\newcommand{\dropCILVDburnCoarseLTwoVarLossGce}{1.9}
\newcommand{\retLVDburnCoarseLTwoVarLossGce}{0.803}
\newcommand{\retCILVDburnCoarseLTwoVarLossGce}{0.023}
\newcommand{\nLVDburnCoarseLTwoVarLrMultZeroOneOneOneOne}{2}
\newcommand{\miouLVDburnCoarseLTwoVarLrMultZeroOneOneOneOne}{68.7}
\newcommand{\miouCILVDburnCoarseLTwoVarLrMultZeroOneOneOneOne}{19.8}
\newcommand{\dropLVDburnCoarseLTwoVarLrMultZeroOneOneOneOne}{13.6}
\newcommand{\dropCILVDburnCoarseLTwoVarLrMultZeroOneOneOneOne}{15.9}
\newcommand{\retLVDburnCoarseLTwoVarLrMultZeroOneOneOneOne}{0.835}
\newcommand{\retCILVDburnCoarseLTwoVarLrMultZeroOneOneOneOne}{0.201}
\newcommand{\nLVDburnCoarseLTwoVarLrMultOne}{5}
\newcommand{\miouLVDburnCoarseLTwoVarLrMultOne}{52.0}
\newcommand{\miouCILVDburnCoarseLTwoVarLrMultOne}{8.5}
\newcommand{\dropLVDburnCoarseLTwoVarLrMultOne}{26.3}
\newcommand{\dropCILVDburnCoarseLTwoVarLrMultOne}{7.9}
\newcommand{\retLVDburnCoarseLTwoVarLrMultOne}{0.664}
\newcommand{\retCILVDburnCoarseLTwoVarLrMultOne}{0.103}
\newcommand{\nLVDburnCoarseLR}{5}
\newcommand{\miouLVDburnCoarseLR}{62.3}
\newcommand{\miouCILVDburnCoarseLR}{2.9}
\newcommand{\dropLVDburnCoarseLR}{19.7}
\newcommand{\dropCILVDburnCoarseLR}{2.6}
\newcommand{\retLVDburnCoarseLR}{0.759}
\newcommand{\retCILVDburnCoarseLR}{0.032}
\newcommand{\nLVDburnCoarseLRVarLrMultOne}{5}
\newcommand{\miouLVDburnCoarseLRVarLrMultOne}{51.3}
\newcommand{\miouCILVDburnCoarseLRVarLrMultOne}{6.2}
\newcommand{\dropLVDburnCoarseLRVarLrMultOne}{27.1}
\newcommand{\dropCILVDburnCoarseLRVarLrMultOne}{7.3}
\newcommand{\retLVDburnCoarseLRVarLrMultOne}{0.655}
\newcommand{\retCILVDburnCoarseLRVarLrMultOne}{0.086}
\newcommand{\nLVDburnOmissionLOne}{5}
\newcommand{\miouLVDburnOmissionLOne}{74.4}
\newcommand{\miouCILVDburnOmissionLOne}{3.5}
\newcommand{\dropLVDburnOmissionLOne}{7.6}
\newcommand{\dropCILVDburnOmissionLOne}{3.5}
\newcommand{\retLVDburnOmissionLOne}{0.907}
\newcommand{\retCILVDburnOmissionLOne}{0.042}
\newcommand{\nLVDburnOmissionLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouLVDburnOmissionLOneVarDecoderMaskTwoformerFull}{74.1}
\newcommand{\miouCILVDburnOmissionLOneVarDecoderMaskTwoformerFull}{5.8}
\newcommand{\dropLVDburnOmissionLOneVarDecoderMaskTwoformerFull}{4.9}
\newcommand{\dropCILVDburnOmissionLOneVarDecoderMaskTwoformerFull}{8.2}
\newcommand{\retLVDburnOmissionLOneVarDecoderMaskTwoformerFull}{0.940}
\newcommand{\retCILVDburnOmissionLOneVarDecoderMaskTwoformerFull}{0.100}
\newcommand{\nLVDburnOmissionLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDburnOmissionLOneVarDecoderMaskTwoformerLite}{72.2}
\newcommand{\miouCILVDburnOmissionLOneVarDecoderMaskTwoformerLite}{3.4}
\newcommand{\dropLVDburnOmissionLOneVarDecoderMaskTwoformerLite}{11.1}
\newcommand{\dropCILVDburnOmissionLOneVarDecoderMaskTwoformerLite}{3.7}
\newcommand{\retLVDburnOmissionLOneVarDecoderMaskTwoformerLite}{0.867}
\newcommand{\retCILVDburnOmissionLOneVarDecoderMaskTwoformerLite}{0.044}
\newcommand{\nLVDburnOmissionLOneVarDecoderSamLite}{5}
\newcommand{\miouLVDburnOmissionLOneVarDecoderSamLite}{74.1}
\newcommand{\miouCILVDburnOmissionLOneVarDecoderSamLite}{4.0}
\newcommand{\dropLVDburnOmissionLOneVarDecoderSamLite}{8.4}
\newcommand{\dropCILVDburnOmissionLOneVarDecoderSamLite}{3.5}
\newcommand{\retLVDburnOmissionLOneVarDecoderSamLite}{0.898}
\newcommand{\retCILVDburnOmissionLOneVarDecoderSamLite}{0.043}
\newcommand{\nLVDburnOmissionLOneVarDecoderSamPretrained}{5}
\newcommand{\miouLVDburnOmissionLOneVarDecoderSamPretrained}{67.7}
\newcommand{\miouCILVDburnOmissionLOneVarDecoderSamPretrained}{16.2}
\newcommand{\dropLVDburnOmissionLOneVarDecoderSamPretrained}{6.3}
\newcommand{\dropCILVDburnOmissionLOneVarDecoderSamPretrained}{7.2}
\newcommand{\retLVDburnOmissionLOneVarDecoderSamPretrained}{0.924}
\newcommand{\retCILVDburnOmissionLOneVarDecoderSamPretrained}{0.086}
\newcommand{\nLVDburnOmissionLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDburnOmissionLOneVarDecoderSegformerMlp}{72.4}
\newcommand{\miouCILVDburnOmissionLOneVarDecoderSegformerMlp}{6.3}
\newcommand{\dropLVDburnOmissionLOneVarDecoderSegformerMlp}{11.0}
\newcommand{\dropCILVDburnOmissionLOneVarDecoderSegformerMlp}{5.2}
\newcommand{\retLVDburnOmissionLOneVarDecoderSegformerMlp}{0.868}
\newcommand{\retCILVDburnOmissionLOneVarDecoderSegformerMlp}{0.065}
\newcommand{\nLVDburnOmissionLTwo}{8}
\newcommand{\miouLVDburnOmissionLTwo}{64.9}
\newcommand{\miouCILVDburnOmissionLTwo}{2.0}
\newcommand{\dropLVDburnOmissionLTwo}{16.9}
\newcommand{\dropCILVDburnOmissionLTwo}{2.5}
\newcommand{\retLVDburnOmissionLTwo}{0.794}
\newcommand{\retCILVDburnOmissionLTwo}{0.029}
\newcommand{\nLVDburnOmissionLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouLVDburnOmissionLTwoVarDecoderMaskTwoformerFull}{64.9}
\newcommand{\miouCILVDburnOmissionLTwoVarDecoderMaskTwoformerFull}{4.5}
\newcommand{\dropLVDburnOmissionLTwoVarDecoderMaskTwoformerFull}{14.2}
\newcommand{\dropCILVDburnOmissionLTwoVarDecoderMaskTwoformerFull}{5.6}
\newcommand{\retLVDburnOmissionLTwoVarDecoderMaskTwoformerFull}{0.821}
\newcommand{\retCILVDburnOmissionLTwoVarDecoderMaskTwoformerFull}{0.064}
\newcommand{\nLVDburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}{5}
\newcommand{\miouLVDburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}{57.9}
\newcommand{\miouCILVDburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}{4.5}
\newcommand{\dropLVDburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}{10.8}
\newcommand{\dropCILVDburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}{4.2}
\newcommand{\retLVDburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}{0.843}
\newcommand{\retCILVDburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}{0.059}
\newcommand{\nLVDburnOmissionLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDburnOmissionLTwoVarDecoderMaskTwoformerLite}{51.0}
\newcommand{\miouCILVDburnOmissionLTwoVarDecoderMaskTwoformerLite}{11.2}
\newcommand{\dropLVDburnOmissionLTwoVarDecoderMaskTwoformerLite}{32.4}
\newcommand{\dropCILVDburnOmissionLTwoVarDecoderMaskTwoformerLite}{11.6}
\newcommand{\retLVDburnOmissionLTwoVarDecoderMaskTwoformerLite}{0.612}
\newcommand{\retCILVDburnOmissionLTwoVarDecoderMaskTwoformerLite}{0.138}
\newcommand{\nLVDburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}{5}
\newcommand{\miouLVDburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}{44.8}
\newcommand{\miouCILVDburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}{0.0}
\newcommand{\dropLVDburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}{0.0}
\newcommand{\dropCILVDburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}{0.0}
\newcommand{\retLVDburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}{1.000}
\newcommand{\retCILVDburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}{0.000}
\newcommand{\nLVDburnOmissionLTwoVarDecoderSamLite}{5}
\newcommand{\miouLVDburnOmissionLTwoVarDecoderSamLite}{61.4}
\newcommand{\miouCILVDburnOmissionLTwoVarDecoderSamLite}{7.8}
\newcommand{\dropLVDburnOmissionLTwoVarDecoderSamLite}{21.1}
\newcommand{\dropCILVDburnOmissionLTwoVarDecoderSamLite}{6.9}
\newcommand{\retLVDburnOmissionLTwoVarDecoderSamLite}{0.743}
\newcommand{\retCILVDburnOmissionLTwoVarDecoderSamLite}{0.086}
\newcommand{\nLVDburnOmissionLTwoVarDecoderSamLiteLrMultOne}{5}
\newcommand{\miouLVDburnOmissionLTwoVarDecoderSamLiteLrMultOne}{45.0}
\newcommand{\miouCILVDburnOmissionLTwoVarDecoderSamLiteLrMultOne}{0.5}
\newcommand{\dropLVDburnOmissionLTwoVarDecoderSamLiteLrMultOne}{29.6}
\newcommand{\dropCILVDburnOmissionLTwoVarDecoderSamLiteLrMultOne}{5.9}
\newcommand{\retLVDburnOmissionLTwoVarDecoderSamLiteLrMultOne}{0.605}
\newcommand{\retCILVDburnOmissionLTwoVarDecoderSamLiteLrMultOne}{0.050}
\newcommand{\nLVDburnOmissionLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouLVDburnOmissionLTwoVarDecoderSamPretrained}{60.1}
\newcommand{\miouCILVDburnOmissionLTwoVarDecoderSamPretrained}{12.1}
\newcommand{\dropLVDburnOmissionLTwoVarDecoderSamPretrained}{13.8}
\newcommand{\dropCILVDburnOmissionLTwoVarDecoderSamPretrained}{10.5}
\newcommand{\retLVDburnOmissionLTwoVarDecoderSamPretrained}{0.829}
\newcommand{\retCILVDburnOmissionLTwoVarDecoderSamPretrained}{0.131}
\newcommand{\nLVDburnOmissionLTwoVarDecoderSamPretrainedLrMultOne}{5}
\newcommand{\miouLVDburnOmissionLTwoVarDecoderSamPretrainedLrMultOne}{44.8}
\newcommand{\miouCILVDburnOmissionLTwoVarDecoderSamPretrainedLrMultOne}{0.0}
\newcommand{\dropLVDburnOmissionLTwoVarDecoderSamPretrainedLrMultOne}{29.9}
\newcommand{\dropCILVDburnOmissionLTwoVarDecoderSamPretrainedLrMultOne}{2.8}
\newcommand{\retLVDburnOmissionLTwoVarDecoderSamPretrainedLrMultOne}{0.600}
\newcommand{\retCILVDburnOmissionLTwoVarDecoderSamPretrainedLrMultOne}{0.023}
\newcommand{\nLVDburnOmissionLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDburnOmissionLTwoVarDecoderSegformerMlp}{64.8}
\newcommand{\miouCILVDburnOmissionLTwoVarDecoderSegformerMlp}{5.6}
\newcommand{\dropLVDburnOmissionLTwoVarDecoderSegformerMlp}{18.6}
\newcommand{\dropCILVDburnOmissionLTwoVarDecoderSegformerMlp}{4.8}
\newcommand{\retLVDburnOmissionLTwoVarDecoderSegformerMlp}{0.777}
\newcommand{\retCILVDburnOmissionLTwoVarDecoderSegformerMlp}{0.059}
\newcommand{\nLVDburnOmissionLTwoVarDecoderSegformerMlpLrMultOne}{5}
\newcommand{\miouLVDburnOmissionLTwoVarDecoderSegformerMlpLrMultOne}{59.7}
\newcommand{\miouCILVDburnOmissionLTwoVarDecoderSegformerMlpLrMultOne}{3.3}
\newcommand{\dropLVDburnOmissionLTwoVarDecoderSegformerMlpLrMultOne}{19.6}
\newcommand{\dropCILVDburnOmissionLTwoVarDecoderSegformerMlpLrMultOne}{3.2}
\newcommand{\retLVDburnOmissionLTwoVarDecoderSegformerMlpLrMultOne}{0.753}
\newcommand{\retCILVDburnOmissionLTwoVarDecoderSegformerMlpLrMultOne}{0.040}
\newcommand{\nLVDburnOmissionLTwoVarLossBootstrap}{5}
\newcommand{\miouLVDburnOmissionLTwoVarLossBootstrap}{64.8}
\newcommand{\miouCILVDburnOmissionLTwoVarLossBootstrap}{8.6}
\newcommand{\dropLVDburnOmissionLTwoVarLossBootstrap}{17.3}
\newcommand{\dropCILVDburnOmissionLTwoVarLossBootstrap}{9.1}
\newcommand{\retLVDburnOmissionLTwoVarLossBootstrap}{0.790}
\newcommand{\retCILVDburnOmissionLTwoVarLossBootstrap}{0.111}
\newcommand{\nLVDburnOmissionLTwoVarLossGce}{5}
\newcommand{\miouLVDburnOmissionLTwoVarLossGce}{61.5}
\newcommand{\miouCILVDburnOmissionLTwoVarLossGce}{6.7}
\newcommand{\dropLVDburnOmissionLTwoVarLossGce}{19.8}
\newcommand{\dropCILVDburnOmissionLTwoVarLossGce}{6.8}
\newcommand{\retLVDburnOmissionLTwoVarLossGce}{0.757}
\newcommand{\retCILVDburnOmissionLTwoVarLossGce}{0.084}
\newcommand{\nLVDburnOmissionLTwoVarLrMultOne}{5}
\newcommand{\miouLVDburnOmissionLTwoVarLrMultOne}{56.1}
\newcommand{\miouCILVDburnOmissionLTwoVarLrMultOne}{9.2}
\newcommand{\dropLVDburnOmissionLTwoVarLrMultOne}{22.2}
\newcommand{\dropCILVDburnOmissionLTwoVarLrMultOne}{8.1}
\newcommand{\retLVDburnOmissionLTwoVarLrMultOne}{0.716}
\newcommand{\retCILVDburnOmissionLTwoVarLrMultOne}{0.106}
\newcommand{\nLVDburnOmissionLR}{5}
\newcommand{\miouLVDburnOmissionLR}{51.4}
\newcommand{\miouCILVDburnOmissionLR}{7.6}
\newcommand{\dropLVDburnOmissionLR}{30.6}
\newcommand{\dropCILVDburnOmissionLR}{8.0}
\newcommand{\retLVDburnOmissionLR}{0.627}
\newcommand{\retCILVDburnOmissionLR}{0.096}
\newcommand{\nLVDburnOmissionLRVarLrMultOne}{5}
\newcommand{\miouLVDburnOmissionLRVarLrMultOne}{47.5}
\newcommand{\miouCILVDburnOmissionLRVarLrMultOne}{7.4}
\newcommand{\dropLVDburnOmissionLRVarLrMultOne}{30.8}
\newcommand{\dropCILVDburnOmissionLRVarLrMultOne}{6.3}
\newcommand{\retLVDburnOmissionLRVarLrMultOne}{0.606}
\newcommand{\retCILVDburnOmissionLRVarLrMultOne}{0.082}
\newcommand{\nLVDburnShiftLOne}{5}
\newcommand{\miouLVDburnShiftLOne}{81.0}
\newcommand{\miouCILVDburnShiftLOne}{2.1}
\newcommand{\dropLVDburnShiftLOne}{1.1}
\newcommand{\dropCILVDburnShiftLOne}{2.9}
\newcommand{\retLVDburnShiftLOne}{0.987}
\newcommand{\retCILVDburnShiftLOne}{0.036}
\newcommand{\nLVDburnShiftLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouLVDburnShiftLOneVarDecoderMaskTwoformerFull}{78.0}
\newcommand{\miouCILVDburnShiftLOneVarDecoderMaskTwoformerFull}{1.7}
\newcommand{\dropLVDburnShiftLOneVarDecoderMaskTwoformerFull}{1.1}
\newcommand{\dropCILVDburnShiftLOneVarDecoderMaskTwoformerFull}{5.0}
\newcommand{\retLVDburnShiftLOneVarDecoderMaskTwoformerFull}{0.988}
\newcommand{\retCILVDburnShiftLOneVarDecoderMaskTwoformerFull}{0.064}
\newcommand{\nLVDburnShiftLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDburnShiftLOneVarDecoderMaskTwoformerLite}{80.2}
\newcommand{\miouCILVDburnShiftLOneVarDecoderMaskTwoformerLite}{1.5}
\newcommand{\dropLVDburnShiftLOneVarDecoderMaskTwoformerLite}{3.2}
\newcommand{\dropCILVDburnShiftLOneVarDecoderMaskTwoformerLite}{1.3}
\newcommand{\retLVDburnShiftLOneVarDecoderMaskTwoformerLite}{0.962}
\newcommand{\retCILVDburnShiftLOneVarDecoderMaskTwoformerLite}{0.016}
\newcommand{\nLVDburnShiftLOneVarDecoderSamLite}{5}
\newcommand{\miouLVDburnShiftLOneVarDecoderSamLite}{78.6}
\newcommand{\miouCILVDburnShiftLOneVarDecoderSamLite}{1.9}
\newcommand{\dropLVDburnShiftLOneVarDecoderSamLite}{3.9}
\newcommand{\dropCILVDburnShiftLOneVarDecoderSamLite}{2.9}
\newcommand{\retLVDburnShiftLOneVarDecoderSamLite}{0.953}
\newcommand{\retCILVDburnShiftLOneVarDecoderSamLite}{0.034}
\newcommand{\nLVDburnShiftLOneVarDecoderSamPretrained}{5}
\newcommand{\miouLVDburnShiftLOneVarDecoderSamPretrained}{65.6}
\newcommand{\miouCILVDburnShiftLOneVarDecoderSamPretrained}{23.6}
\newcommand{\dropLVDburnShiftLOneVarDecoderSamPretrained}{8.4}
\newcommand{\dropCILVDburnShiftLOneVarDecoderSamPretrained}{21.7}
\newcommand{\retLVDburnShiftLOneVarDecoderSamPretrained}{0.901}
\newcommand{\retCILVDburnShiftLOneVarDecoderSamPretrained}{0.258}
\newcommand{\nLVDburnShiftLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDburnShiftLOneVarDecoderSegformerMlp}{81.8}
\newcommand{\miouCILVDburnShiftLOneVarDecoderSegformerMlp}{1.5}
\newcommand{\dropLVDburnShiftLOneVarDecoderSegformerMlp}{1.6}
\newcommand{\dropCILVDburnShiftLOneVarDecoderSegformerMlp}{1.4}
\newcommand{\retLVDburnShiftLOneVarDecoderSegformerMlp}{0.981}
\newcommand{\retCILVDburnShiftLOneVarDecoderSegformerMlp}{0.017}
\newcommand{\nLVDburnShiftLTwo}{8}
\newcommand{\miouLVDburnShiftLTwo}{71.0}
\newcommand{\miouCILVDburnShiftLTwo}{1.3}
\newcommand{\dropLVDburnShiftLTwo}{10.8}
\newcommand{\dropCILVDburnShiftLTwo}{1.9}
\newcommand{\retLVDburnShiftLTwo}{0.869}
\newcommand{\retCILVDburnShiftLTwo}{0.021}
\newcommand{\nLVDburnShiftLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouLVDburnShiftLTwoVarDecoderMaskTwoformerFull}{66.2}
\newcommand{\miouCILVDburnShiftLTwoVarDecoderMaskTwoformerFull}{3.0}
\newcommand{\dropLVDburnShiftLTwoVarDecoderMaskTwoformerFull}{12.8}
\newcommand{\dropCILVDburnShiftLTwoVarDecoderMaskTwoformerFull}{3.1}
\newcommand{\retLVDburnShiftLTwoVarDecoderMaskTwoformerFull}{0.838}
\newcommand{\retCILVDburnShiftLTwoVarDecoderMaskTwoformerFull}{0.035}
\newcommand{\nLVDburnShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}{5}
\newcommand{\miouLVDburnShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}{47.0}
\newcommand{\miouCILVDburnShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}{6.2}
\newcommand{\dropLVDburnShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}{21.7}
\newcommand{\dropCILVDburnShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}{8.2}
\newcommand{\retLVDburnShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}{0.686}
\newcommand{\retCILVDburnShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}{0.112}
\newcommand{\nLVDburnShiftLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDburnShiftLTwoVarDecoderMaskTwoformerLite}{67.1}
\newcommand{\miouCILVDburnShiftLTwoVarDecoderMaskTwoformerLite}{4.5}
\newcommand{\dropLVDburnShiftLTwoVarDecoderMaskTwoformerLite}{16.3}
\newcommand{\dropCILVDburnShiftLTwoVarDecoderMaskTwoformerLite}{3.8}
\newcommand{\retLVDburnShiftLTwoVarDecoderMaskTwoformerLite}{0.805}
\newcommand{\retCILVDburnShiftLTwoVarDecoderMaskTwoformerLite}{0.048}
\newcommand{\nLVDburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}{5}
\newcommand{\miouLVDburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}{44.8}
\newcommand{\miouCILVDburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}{0.0}
\newcommand{\dropLVDburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}{0.0}
\newcommand{\dropCILVDburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}{0.0}
\newcommand{\retLVDburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}{1.000}
\newcommand{\retCILVDburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}{0.000}
\newcommand{\nLVDburnShiftLTwoVarDecoderSamLite}{5}
\newcommand{\miouLVDburnShiftLTwoVarDecoderSamLite}{68.7}
\newcommand{\miouCILVDburnShiftLTwoVarDecoderSamLite}{2.9}
\newcommand{\dropLVDburnShiftLTwoVarDecoderSamLite}{13.8}
\newcommand{\dropCILVDburnShiftLTwoVarDecoderSamLite}{4.5}
\newcommand{\retLVDburnShiftLTwoVarDecoderSamLite}{0.833}
\newcommand{\retCILVDburnShiftLTwoVarDecoderSamLite}{0.051}
\newcommand{\nLVDburnShiftLTwoVarDecoderSamLiteLrMultOne}{5}
\newcommand{\miouLVDburnShiftLTwoVarDecoderSamLiteLrMultOne}{54.4}
\newcommand{\miouCILVDburnShiftLTwoVarDecoderSamLiteLrMultOne}{11.8}
\newcommand{\dropLVDburnShiftLTwoVarDecoderSamLiteLrMultOne}{20.1}
\newcommand{\dropCILVDburnShiftLTwoVarDecoderSamLiteLrMultOne}{9.4}
\newcommand{\retLVDburnShiftLTwoVarDecoderSamLiteLrMultOne}{0.729}
\newcommand{\retCILVDburnShiftLTwoVarDecoderSamLiteLrMultOne}{0.130}
\newcommand{\nLVDburnShiftLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouLVDburnShiftLTwoVarDecoderSamPretrained}{55.4}
\newcommand{\miouCILVDburnShiftLTwoVarDecoderSamPretrained}{18.1}
\newcommand{\dropLVDburnShiftLTwoVarDecoderSamPretrained}{18.5}
\newcommand{\dropCILVDburnShiftLTwoVarDecoderSamPretrained}{21.2}
\newcommand{\retLVDburnShiftLTwoVarDecoderSamPretrained}{0.773}
\newcommand{\retCILVDburnShiftLTwoVarDecoderSamPretrained}{0.261}
\newcommand{\nLVDburnShiftLTwoVarDecoderSamPretrainedLrMultOne}{5}
\newcommand{\miouLVDburnShiftLTwoVarDecoderSamPretrainedLrMultOne}{44.8}
\newcommand{\miouCILVDburnShiftLTwoVarDecoderSamPretrainedLrMultOne}{0.0}
\newcommand{\dropLVDburnShiftLTwoVarDecoderSamPretrainedLrMultOne}{29.9}
\newcommand{\dropCILVDburnShiftLTwoVarDecoderSamPretrainedLrMultOne}{2.8}
\newcommand{\retLVDburnShiftLTwoVarDecoderSamPretrainedLrMultOne}{0.600}
\newcommand{\retCILVDburnShiftLTwoVarDecoderSamPretrainedLrMultOne}{0.023}
\newcommand{\nLVDburnShiftLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDburnShiftLTwoVarDecoderSegformerMlp}{72.0}
\newcommand{\miouCILVDburnShiftLTwoVarDecoderSegformerMlp}{1.6}
\newcommand{\dropLVDburnShiftLTwoVarDecoderSegformerMlp}{11.3}
\newcommand{\dropCILVDburnShiftLTwoVarDecoderSegformerMlp}{1.7}
\newcommand{\retLVDburnShiftLTwoVarDecoderSegformerMlp}{0.864}
\newcommand{\retCILVDburnShiftLTwoVarDecoderSegformerMlp}{0.019}
\newcommand{\nLVDburnShiftLTwoVarDecoderSegformerMlpLrMultOne}{5}
\newcommand{\miouLVDburnShiftLTwoVarDecoderSegformerMlpLrMultOne}{64.9}
\newcommand{\miouCILVDburnShiftLTwoVarDecoderSegformerMlpLrMultOne}{2.0}
\newcommand{\dropLVDburnShiftLTwoVarDecoderSegformerMlpLrMultOne}{14.5}
\newcommand{\dropCILVDburnShiftLTwoVarDecoderSegformerMlpLrMultOne}{2.1}
\newcommand{\retLVDburnShiftLTwoVarDecoderSegformerMlpLrMultOne}{0.818}
\newcommand{\retCILVDburnShiftLTwoVarDecoderSegformerMlpLrMultOne}{0.025}
\newcommand{\nLVDburnShiftLTwoVarLossBootstrap}{5}
\newcommand{\miouLVDburnShiftLTwoVarLossBootstrap}{69.7}
\newcommand{\miouCILVDburnShiftLTwoVarLossBootstrap}{2.0}
\newcommand{\dropLVDburnShiftLTwoVarLossBootstrap}{12.3}
\newcommand{\dropCILVDburnShiftLTwoVarLossBootstrap}{3.3}
\newcommand{\retLVDburnShiftLTwoVarLossBootstrap}{0.850}
\newcommand{\retCILVDburnShiftLTwoVarLossBootstrap}{0.038}
\newcommand{\nLVDburnShiftLTwoVarLossGce}{5}
\newcommand{\miouLVDburnShiftLTwoVarLossGce}{71.9}
\newcommand{\miouCILVDburnShiftLTwoVarLossGce}{1.4}
\newcommand{\dropLVDburnShiftLTwoVarLossGce}{9.4}
\newcommand{\dropCILVDburnShiftLTwoVarLossGce}{1.3}
\newcommand{\retLVDburnShiftLTwoVarLossGce}{0.885}
\newcommand{\retCILVDburnShiftLTwoVarLossGce}{0.016}
\newcommand{\nLVDburnShiftLTwoVarLrMultOne}{5}
\newcommand{\miouLVDburnShiftLTwoVarLrMultOne}{63.5}
\newcommand{\miouCILVDburnShiftLTwoVarLrMultOne}{6.0}
\newcommand{\dropLVDburnShiftLTwoVarLrMultOne}{14.8}
\newcommand{\dropCILVDburnShiftLTwoVarLrMultOne}{4.5}
\newcommand{\retLVDburnShiftLTwoVarLrMultOne}{0.811}
\newcommand{\retCILVDburnShiftLTwoVarLrMultOne}{0.059}
\newcommand{\nLVDburnShiftLR}{5}
\newcommand{\miouLVDburnShiftLR}{65.9}
\newcommand{\miouCILVDburnShiftLR}{0.7}
\newcommand{\dropLVDburnShiftLR}{16.1}
\newcommand{\dropCILVDburnShiftLR}{1.5}
\newcommand{\retLVDburnShiftLR}{0.803}
\newcommand{\retCILVDburnShiftLR}{0.016}
\newcommand{\nLVDburnShiftLRVarLrMultOne}{5}
\newcommand{\miouLVDburnShiftLRVarLrMultOne}{54.7}
\newcommand{\miouCILVDburnShiftLRVarLrMultOne}{9.8}
\newcommand{\dropLVDburnShiftLRVarLrMultOne}{23.6}
\newcommand{\dropCILVDburnShiftLRVarLrMultOne}{9.9}
\newcommand{\retLVDburnShiftLRVarLrMultOne}{0.699}
\newcommand{\retCILVDburnShiftLRVarLrMultOne}{0.125}
\newcommand{\nLVDChesBoundaryLOne}{5}
\newcommand{\miouLVDChesBoundaryLOne}{75.8}
\newcommand{\miouCILVDChesBoundaryLOne}{1.3}
\newcommand{\dropLVDChesBoundaryLOne}{3.5}
\newcommand{\dropCILVDChesBoundaryLOne}{2.4}
\newcommand{\retLVDChesBoundaryLOne}{0.956}
\newcommand{\retCILVDChesBoundaryLOne}{0.030}
\newcommand{\nLVDChesBoundaryLTwo}{5}
\newcommand{\miouLVDChesBoundaryLTwo}{68.0}
\newcommand{\miouCILVDChesBoundaryLTwo}{1.4}
\newcommand{\dropLVDChesBoundaryLTwo}{11.3}
\newcommand{\dropCILVDChesBoundaryLTwo}{2.0}
\newcommand{\retLVDChesBoundaryLTwo}{0.858}
\newcommand{\retCILVDChesBoundaryLTwo}{0.024}
\newcommand{\nLVDChesBoundaryLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDChesBoundaryLTwoVarDecoderMaskTwoformerLite}{61.6}
\newcommand{\miouCILVDChesBoundaryLTwoVarDecoderMaskTwoformerLite}{5.1}
\newcommand{\dropLVDChesBoundaryLTwoVarDecoderMaskTwoformerLite}{18.6}
\newcommand{\dropCILVDChesBoundaryLTwoVarDecoderMaskTwoformerLite}{4.9}
\newcommand{\retLVDChesBoundaryLTwoVarDecoderMaskTwoformerLite}{0.768}
\newcommand{\retCILVDChesBoundaryLTwoVarDecoderMaskTwoformerLite}{0.061}
\newcommand{\nLVDChesBoundaryLTwoVarDecoderSamLite}{5}
\newcommand{\miouLVDChesBoundaryLTwoVarDecoderSamLite}{68.4}
\newcommand{\miouCILVDChesBoundaryLTwoVarDecoderSamLite}{1.1}
\newcommand{\dropLVDChesBoundaryLTwoVarDecoderSamLite}{11.2}
\newcommand{\dropCILVDChesBoundaryLTwoVarDecoderSamLite}{0.9}
\newcommand{\retLVDChesBoundaryLTwoVarDecoderSamLite}{0.859}
\newcommand{\retCILVDChesBoundaryLTwoVarDecoderSamLite}{0.011}
\newcommand{\nLVDChesBoundaryLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDChesBoundaryLTwoVarDecoderSegformerMlp}{69.5}
\newcommand{\miouCILVDChesBoundaryLTwoVarDecoderSegformerMlp}{1.1}
\newcommand{\dropLVDChesBoundaryLTwoVarDecoderSegformerMlp}{11.2}
\newcommand{\dropCILVDChesBoundaryLTwoVarDecoderSegformerMlp}{0.8}
\newcommand{\retLVDChesBoundaryLTwoVarDecoderSegformerMlp}{0.861}
\newcommand{\retCILVDChesBoundaryLTwoVarDecoderSegformerMlp}{0.010}
\newcommand{\nLVDChesBoundaryLTwoVarLrMultOne}{5}
\newcommand{\miouLVDChesBoundaryLTwoVarLrMultOne}{68.7}
\newcommand{\miouCILVDChesBoundaryLTwoVarLrMultOne}{1.1}
\newcommand{\dropLVDChesBoundaryLTwoVarLrMultOne}{12.0}
\newcommand{\dropCILVDChesBoundaryLTwoVarLrMultOne}{3.1}
\newcommand{\retLVDChesBoundaryLTwoVarLrMultOne}{0.852}
\newcommand{\retCILVDChesBoundaryLTwoVarLrMultOne}{0.036}
\newcommand{\nLVDChesClean}{5}
\newcommand{\miouLVDChesClean}{79.3}
\newcommand{\miouCILVDChesClean}{1.4}
\newcommand{\nLVDChesCleanVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDChesCleanVarDecoderMaskTwoformerLite}{80.2}
\newcommand{\miouCILVDChesCleanVarDecoderMaskTwoformerLite}{0.4}
\newcommand{\nLVDChesCleanVarDecoderSamLite}{5}
\newcommand{\miouLVDChesCleanVarDecoderSamLite}{79.6}
\newcommand{\miouCILVDChesCleanVarDecoderSamLite}{0.8}
\newcommand{\nLVDChesCleanVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDChesCleanVarDecoderSegformerMlp}{80.7}
\newcommand{\miouCILVDChesCleanVarDecoderSegformerMlp}{0.9}
\newcommand{\nLVDChesCleanVarLrMultOne}{5}
\newcommand{\miouLVDChesCleanVarLrMultOne}{80.6}
\newcommand{\miouCILVDChesCleanVarLrMultOne}{2.3}
\newcommand{\nLVDChesCoarseLOne}{5}
\newcommand{\miouLVDChesCoarseLOne}{77.7}
\newcommand{\miouCILVDChesCoarseLOne}{0.9}
\newcommand{\dropLVDChesCoarseLOne}{1.6}
\newcommand{\dropCILVDChesCoarseLOne}{1.9}
\newcommand{\retLVDChesCoarseLOne}{0.980}
\newcommand{\retCILVDChesCoarseLOne}{0.024}
\newcommand{\nLVDChesCoarseLTwo}{5}
\newcommand{\miouLVDChesCoarseLTwo}{68.5}
\newcommand{\miouCILVDChesCoarseLTwo}{0.6}
\newcommand{\dropLVDChesCoarseLTwo}{10.8}
\newcommand{\dropCILVDChesCoarseLTwo}{1.3}
\newcommand{\retLVDChesCoarseLTwo}{0.864}
\newcommand{\retCILVDChesCoarseLTwo}{0.014}
\newcommand{\nLVDChesCoarseLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDChesCoarseLTwoVarDecoderMaskTwoformerLite}{68.7}
\newcommand{\miouCILVDChesCoarseLTwoVarDecoderMaskTwoformerLite}{0.4}
\newcommand{\dropLVDChesCoarseLTwoVarDecoderMaskTwoformerLite}{11.5}
\newcommand{\dropCILVDChesCoarseLTwoVarDecoderMaskTwoformerLite}{0.4}
\newcommand{\retLVDChesCoarseLTwoVarDecoderMaskTwoformerLite}{0.857}
\newcommand{\retCILVDChesCoarseLTwoVarDecoderMaskTwoformerLite}{0.005}
\newcommand{\nLVDChesCoarseLTwoVarDecoderSamLite}{5}
\newcommand{\miouLVDChesCoarseLTwoVarDecoderSamLite}{68.6}
\newcommand{\miouCILVDChesCoarseLTwoVarDecoderSamLite}{1.0}
\newcommand{\dropLVDChesCoarseLTwoVarDecoderSamLite}{11.0}
\newcommand{\dropCILVDChesCoarseLTwoVarDecoderSamLite}{0.8}
\newcommand{\retLVDChesCoarseLTwoVarDecoderSamLite}{0.861}
\newcommand{\retCILVDChesCoarseLTwoVarDecoderSamLite}{0.010}
\newcommand{\nLVDChesCoarseLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDChesCoarseLTwoVarDecoderSegformerMlp}{68.9}
\newcommand{\miouCILVDChesCoarseLTwoVarDecoderSegformerMlp}{0.9}
\newcommand{\dropLVDChesCoarseLTwoVarDecoderSegformerMlp}{11.9}
\newcommand{\dropCILVDChesCoarseLTwoVarDecoderSegformerMlp}{1.2}
\newcommand{\retLVDChesCoarseLTwoVarDecoderSegformerMlp}{0.853}
\newcommand{\retCILVDChesCoarseLTwoVarDecoderSegformerMlp}{0.014}
\newcommand{\nLVDChesCoarseLTwoVarLrMultOne}{5}
\newcommand{\miouLVDChesCoarseLTwoVarLrMultOne}{69.3}
\newcommand{\miouCILVDChesCoarseLTwoVarLrMultOne}{0.8}
\newcommand{\dropLVDChesCoarseLTwoVarLrMultOne}{11.4}
\newcommand{\dropCILVDChesCoarseLTwoVarLrMultOne}{2.3}
\newcommand{\retLVDChesCoarseLTwoVarLrMultOne}{0.860}
\newcommand{\retCILVDChesCoarseLTwoVarLrMultOne}{0.026}
\newcommand{\nLVDChesNlcdREAL}{5}
\newcommand{\miouLVDChesNlcdREAL}{59.1}
\newcommand{\miouCILVDChesNlcdREAL}{2.3}
\newcommand{\dropLVDChesNlcdREAL}{20.3}
\newcommand{\dropCILVDChesNlcdREAL}{3.2}
\newcommand{\retLVDChesNlcdREAL}{0.745}
\newcommand{\retCILVDChesNlcdREAL}{0.037}
\newcommand{\nLVDChesOmissionLOne}{5}
\newcommand{\miouLVDChesOmissionLOne}{75.4}
\newcommand{\miouCILVDChesOmissionLOne}{3.8}
\newcommand{\dropLVDChesOmissionLOne}{3.9}
\newcommand{\dropCILVDChesOmissionLOne}{2.7}
\newcommand{\retLVDChesOmissionLOne}{0.951}
\newcommand{\retCILVDChesOmissionLOne}{0.035}
\newcommand{\nLVDChesOmissionLTwo}{5}
\newcommand{\miouLVDChesOmissionLTwo}{66.3}
\newcommand{\miouCILVDChesOmissionLTwo}{2.1}
\newcommand{\dropLVDChesOmissionLTwo}{13.1}
\newcommand{\dropCILVDChesOmissionLTwo}{1.6}
\newcommand{\retLVDChesOmissionLTwo}{0.835}
\newcommand{\retCILVDChesOmissionLTwo}{0.021}
\newcommand{\nLVDChesOmissionLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDChesOmissionLTwoVarDecoderMaskTwoformerLite}{64.3}
\newcommand{\miouCILVDChesOmissionLTwoVarDecoderMaskTwoformerLite}{9.0}
\newcommand{\dropLVDChesOmissionLTwoVarDecoderMaskTwoformerLite}{15.9}
\newcommand{\dropCILVDChesOmissionLTwoVarDecoderMaskTwoformerLite}{8.8}
\newcommand{\retLVDChesOmissionLTwoVarDecoderMaskTwoformerLite}{0.802}
\newcommand{\retCILVDChesOmissionLTwoVarDecoderMaskTwoformerLite}{0.111}
\newcommand{\nLVDChesOmissionLTwoVarDecoderSamLite}{5}
\newcommand{\miouLVDChesOmissionLTwoVarDecoderSamLite}{68.4}
\newcommand{\miouCILVDChesOmissionLTwoVarDecoderSamLite}{2.1}
\newcommand{\dropLVDChesOmissionLTwoVarDecoderSamLite}{11.3}
\newcommand{\dropCILVDChesOmissionLTwoVarDecoderSamLite}{1.4}
\newcommand{\retLVDChesOmissionLTwoVarDecoderSamLite}{0.858}
\newcommand{\retCILVDChesOmissionLTwoVarDecoderSamLite}{0.019}
\newcommand{\nLVDChesOmissionLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDChesOmissionLTwoVarDecoderSegformerMlp}{67.8}
\newcommand{\miouCILVDChesOmissionLTwoVarDecoderSegformerMlp}{3.6}
\newcommand{\dropLVDChesOmissionLTwoVarDecoderSegformerMlp}{12.9}
\newcommand{\dropCILVDChesOmissionLTwoVarDecoderSegformerMlp}{2.9}
\newcommand{\retLVDChesOmissionLTwoVarDecoderSegformerMlp}{0.840}
\newcommand{\retCILVDChesOmissionLTwoVarDecoderSegformerMlp}{0.037}
\newcommand{\nLVDChesOmissionLTwoVarLrMultOne}{5}
\newcommand{\miouLVDChesOmissionLTwoVarLrMultOne}{66.7}
\newcommand{\miouCILVDChesOmissionLTwoVarLrMultOne}{2.9}
\newcommand{\dropLVDChesOmissionLTwoVarLrMultOne}{13.9}
\newcommand{\dropCILVDChesOmissionLTwoVarLrMultOne}{4.0}
\newcommand{\retLVDChesOmissionLTwoVarLrMultOne}{0.828}
\newcommand{\retCILVDChesOmissionLTwoVarLrMultOne}{0.048}
\newcommand{\nLVDChesShiftLOne}{5}
\newcommand{\miouLVDChesShiftLOne}{78.6}
\newcommand{\miouCILVDChesShiftLOne}{1.0}
\newcommand{\dropLVDChesShiftLOne}{0.7}
\newcommand{\dropCILVDChesShiftLOne}{1.2}
\newcommand{\retLVDChesShiftLOne}{0.992}
\newcommand{\retCILVDChesShiftLOne}{0.015}
\newcommand{\nLVDChesShiftLTwo}{5}
\newcommand{\miouLVDChesShiftLTwo}{73.5}
\newcommand{\miouCILVDChesShiftLTwo}{1.0}
\newcommand{\dropLVDChesShiftLTwo}{5.8}
\newcommand{\dropCILVDChesShiftLTwo}{1.3}
\newcommand{\retLVDChesShiftLTwo}{0.927}
\newcommand{\retCILVDChesShiftLTwo}{0.016}
\newcommand{\nLVDChesShiftLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDChesShiftLTwoVarDecoderMaskTwoformerLite}{72.8}
\newcommand{\miouCILVDChesShiftLTwoVarDecoderMaskTwoformerLite}{0.6}
\newcommand{\dropLVDChesShiftLTwoVarDecoderMaskTwoformerLite}{7.5}
\newcommand{\dropCILVDChesShiftLTwoVarDecoderMaskTwoformerLite}{0.7}
\newcommand{\retLVDChesShiftLTwoVarDecoderMaskTwoformerLite}{0.907}
\newcommand{\retCILVDChesShiftLTwoVarDecoderMaskTwoformerLite}{0.009}
\newcommand{\nLVDChesShiftLTwoVarDecoderSamLite}{5}
\newcommand{\miouLVDChesShiftLTwoVarDecoderSamLite}{72.5}
\newcommand{\miouCILVDChesShiftLTwoVarDecoderSamLite}{1.6}
\newcommand{\dropLVDChesShiftLTwoVarDecoderSamLite}{7.1}
\newcommand{\dropCILVDChesShiftLTwoVarDecoderSamLite}{1.7}
\newcommand{\retLVDChesShiftLTwoVarDecoderSamLite}{0.910}
\newcommand{\retCILVDChesShiftLTwoVarDecoderSamLite}{0.021}
\newcommand{\nLVDChesShiftLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDChesShiftLTwoVarDecoderSegformerMlp}{74.2}
\newcommand{\miouCILVDChesShiftLTwoVarDecoderSegformerMlp}{1.4}
\newcommand{\dropLVDChesShiftLTwoVarDecoderSegformerMlp}{6.5}
\newcommand{\dropCILVDChesShiftLTwoVarDecoderSegformerMlp}{1.4}
\newcommand{\retLVDChesShiftLTwoVarDecoderSegformerMlp}{0.919}
\newcommand{\retCILVDChesShiftLTwoVarDecoderSegformerMlp}{0.018}
\newcommand{\nLVDChesShiftLTwoVarLrMultOne}{5}
\newcommand{\miouLVDChesShiftLTwoVarLrMultOne}{75.0}
\newcommand{\miouCILVDChesShiftLTwoVarLrMultOne}{0.7}
\newcommand{\dropLVDChesShiftLTwoVarLrMultOne}{5.7}
\newcommand{\dropCILVDChesShiftLTwoVarLrMultOne}{2.3}
\newcommand{\retLVDChesShiftLTwoVarLrMultOne}{0.930}
\newcommand{\retCILVDChesShiftLTwoVarLrMultOne}{0.027}
\newcommand{\nLVDCsTwelveBoundaryLOne}{5}
\newcommand{\miouLVDCsTwelveBoundaryLOne}{67.3}
\newcommand{\miouCILVDCsTwelveBoundaryLOne}{0.7}
\newcommand{\dropLVDCsTwelveBoundaryLOne}{2.2}
\newcommand{\dropCILVDCsTwelveBoundaryLOne}{1.2}
\newcommand{\retLVDCsTwelveBoundaryLOne}{0.968}
\newcommand{\retCILVDCsTwelveBoundaryLOne}{0.018}
\newcommand{\nLVDCsTwelveBoundaryLTwo}{5}
\newcommand{\miouLVDCsTwelveBoundaryLTwo}{63.6}
\newcommand{\miouCILVDCsTwelveBoundaryLTwo}{0.6}
\newcommand{\dropLVDCsTwelveBoundaryLTwo}{6.0}
\newcommand{\dropCILVDCsTwelveBoundaryLTwo}{0.8}
\newcommand{\retLVDCsTwelveBoundaryLTwo}{0.914}
\newcommand{\retCILVDCsTwelveBoundaryLTwo}{0.011}
\newcommand{\nLVDCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}{62.5}
\newcommand{\miouCILVDCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}{1.3}
\newcommand{\dropLVDCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}{7.0}
\newcommand{\dropCILVDCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}{1.4}
\newcommand{\retLVDCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}{0.899}
\newcommand{\retCILVDCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}{0.020}
\newcommand{\nLVDCsTwelveBoundaryLTwoVarDecoderSamLite}{5}
\newcommand{\miouLVDCsTwelveBoundaryLTwoVarDecoderSamLite}{64.0}
\newcommand{\miouCILVDCsTwelveBoundaryLTwoVarDecoderSamLite}{1.1}
\newcommand{\dropLVDCsTwelveBoundaryLTwoVarDecoderSamLite}{5.5}
\newcommand{\dropCILVDCsTwelveBoundaryLTwoVarDecoderSamLite}{1.4}
\newcommand{\retLVDCsTwelveBoundaryLTwoVarDecoderSamLite}{0.921}
\newcommand{\retCILVDCsTwelveBoundaryLTwoVarDecoderSamLite}{0.020}
\newcommand{\nLVDCsTwelveBoundaryLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDCsTwelveBoundaryLTwoVarDecoderSegformerMlp}{63.9}
\newcommand{\miouCILVDCsTwelveBoundaryLTwoVarDecoderSegformerMlp}{0.5}
\newcommand{\dropLVDCsTwelveBoundaryLTwoVarDecoderSegformerMlp}{5.9}
\newcommand{\dropCILVDCsTwelveBoundaryLTwoVarDecoderSegformerMlp}{0.5}
\newcommand{\retLVDCsTwelveBoundaryLTwoVarDecoderSegformerMlp}{0.915}
\newcommand{\retCILVDCsTwelveBoundaryLTwoVarDecoderSegformerMlp}{0.007}
\newcommand{\nLVDCsTwelveBoundaryLTwoVarLrMultOne}{5}
\newcommand{\miouLVDCsTwelveBoundaryLTwoVarLrMultOne}{63.1}
\newcommand{\miouCILVDCsTwelveBoundaryLTwoVarLrMultOne}{1.4}
\newcommand{\dropLVDCsTwelveBoundaryLTwoVarLrMultOne}{4.8}
\newcommand{\dropCILVDCsTwelveBoundaryLTwoVarLrMultOne}{1.4}
\newcommand{\retLVDCsTwelveBoundaryLTwoVarLrMultOne}{0.929}
\newcommand{\retCILVDCsTwelveBoundaryLTwoVarLrMultOne}{0.019}
\newcommand{\nLVDCsTwelveClean}{5}
\newcommand{\miouLVDCsTwelveClean}{69.6}
\newcommand{\miouCILVDCsTwelveClean}{0.9}
\newcommand{\nLVDCsTwelveCleanVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDCsTwelveCleanVarDecoderMaskTwoformerLite}{69.6}
\newcommand{\miouCILVDCsTwelveCleanVarDecoderMaskTwoformerLite}{0.3}
\newcommand{\nLVDCsTwelveCleanVarDecoderSamLite}{5}
\newcommand{\miouLVDCsTwelveCleanVarDecoderSamLite}{69.5}
\newcommand{\miouCILVDCsTwelveCleanVarDecoderSamLite}{0.6}
\newcommand{\nLVDCsTwelveCleanVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDCsTwelveCleanVarDecoderSegformerMlp}{69.8}
\newcommand{\miouCILVDCsTwelveCleanVarDecoderSegformerMlp}{0.9}
\newcommand{\nLVDCsTwelveCleanVarLrMultOne}{5}
\newcommand{\miouLVDCsTwelveCleanVarLrMultOne}{67.9}
\newcommand{\miouCILVDCsTwelveCleanVarLrMultOne}{1.8}
\newcommand{\nLVDCsTwelveCoarseLOne}{5}
\newcommand{\miouLVDCsTwelveCoarseLOne}{67.7}
\newcommand{\miouCILVDCsTwelveCoarseLOne}{1.0}
\newcommand{\dropLVDCsTwelveCoarseLOne}{1.9}
\newcommand{\dropCILVDCsTwelveCoarseLOne}{1.3}
\newcommand{\retLVDCsTwelveCoarseLOne}{0.972}
\newcommand{\retCILVDCsTwelveCoarseLOne}{0.019}
\newcommand{\nLVDCsTwelveCoarseLTwo}{5}
\newcommand{\miouLVDCsTwelveCoarseLTwo}{61.8}
\newcommand{\miouCILVDCsTwelveCoarseLTwo}{0.6}
\newcommand{\dropLVDCsTwelveCoarseLTwo}{7.8}
\newcommand{\dropCILVDCsTwelveCoarseLTwo}{0.8}
\newcommand{\retLVDCsTwelveCoarseLTwo}{0.887}
\newcommand{\retCILVDCsTwelveCoarseLTwo}{0.010}
\newcommand{\nLVDCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}{60.7}
\newcommand{\miouCILVDCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}{2.9}
\newcommand{\dropLVDCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}{8.9}
\newcommand{\dropCILVDCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}{3.0}
\newcommand{\retLVDCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}{0.873}
\newcommand{\retCILVDCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}{0.043}
\newcommand{\nLVDCsTwelveCoarseLTwoVarDecoderSamLite}{5}
\newcommand{\miouLVDCsTwelveCoarseLTwoVarDecoderSamLite}{61.0}
\newcommand{\miouCILVDCsTwelveCoarseLTwoVarDecoderSamLite}{0.7}
\newcommand{\dropLVDCsTwelveCoarseLTwoVarDecoderSamLite}{8.5}
\newcommand{\dropCILVDCsTwelveCoarseLTwoVarDecoderSamLite}{1.0}
\newcommand{\retLVDCsTwelveCoarseLTwoVarDecoderSamLite}{0.878}
\newcommand{\retCILVDCsTwelveCoarseLTwoVarDecoderSamLite}{0.014}
\newcommand{\nLVDCsTwelveCoarseLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDCsTwelveCoarseLTwoVarDecoderSegformerMlp}{62.2}
\newcommand{\miouCILVDCsTwelveCoarseLTwoVarDecoderSegformerMlp}{1.3}
\newcommand{\dropLVDCsTwelveCoarseLTwoVarDecoderSegformerMlp}{7.6}
\newcommand{\dropCILVDCsTwelveCoarseLTwoVarDecoderSegformerMlp}{1.8}
\newcommand{\retLVDCsTwelveCoarseLTwoVarDecoderSegformerMlp}{0.892}
\newcommand{\retCILVDCsTwelveCoarseLTwoVarDecoderSegformerMlp}{0.024}
\newcommand{\nLVDCsTwelveCoarseLTwoVarLrMultOne}{5}
\newcommand{\miouLVDCsTwelveCoarseLTwoVarLrMultOne}{60.6}
\newcommand{\miouCILVDCsTwelveCoarseLTwoVarLrMultOne}{0.4}
\newcommand{\dropLVDCsTwelveCoarseLTwoVarLrMultOne}{7.3}
\newcommand{\dropCILVDCsTwelveCoarseLTwoVarLrMultOne}{1.9}
\newcommand{\retLVDCsTwelveCoarseLTwoVarLrMultOne}{0.892}
\newcommand{\retCILVDCsTwelveCoarseLTwoVarLrMultOne}{0.024}
\newcommand{\nLVDCsTwelveOmissionLOne}{5}
\newcommand{\miouLVDCsTwelveOmissionLOne}{66.9}
\newcommand{\miouCILVDCsTwelveOmissionLOne}{0.5}
\newcommand{\dropLVDCsTwelveOmissionLOne}{2.7}
\newcommand{\dropCILVDCsTwelveOmissionLOne}{1.3}
\newcommand{\retLVDCsTwelveOmissionLOne}{0.961}
\newcommand{\retCILVDCsTwelveOmissionLOne}{0.018}
\newcommand{\nLVDCsTwelveOmissionLTwo}{5}
\newcommand{\miouLVDCsTwelveOmissionLTwo}{62.7}
\newcommand{\miouCILVDCsTwelveOmissionLTwo}{0.4}
\newcommand{\dropLVDCsTwelveOmissionLTwo}{6.9}
\newcommand{\dropCILVDCsTwelveOmissionLTwo}{1.0}
\newcommand{\retLVDCsTwelveOmissionLTwo}{0.901}
\newcommand{\retCILVDCsTwelveOmissionLTwo}{0.013}
\newcommand{\nLVDCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}{61.5}
\newcommand{\miouCILVDCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}{1.7}
\newcommand{\dropLVDCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}{8.1}
\newcommand{\dropCILVDCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}{1.9}
\newcommand{\retLVDCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}{0.884}
\newcommand{\retCILVDCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}{0.026}
\newcommand{\nLVDCsTwelveOmissionLTwoVarDecoderSamLite}{5}
\newcommand{\miouLVDCsTwelveOmissionLTwoVarDecoderSamLite}{62.7}
\newcommand{\miouCILVDCsTwelveOmissionLTwoVarDecoderSamLite}{0.8}
\newcommand{\dropLVDCsTwelveOmissionLTwoVarDecoderSamLite}{6.8}
\newcommand{\dropCILVDCsTwelveOmissionLTwoVarDecoderSamLite}{1.2}
\newcommand{\retLVDCsTwelveOmissionLTwoVarDecoderSamLite}{0.902}
\newcommand{\retCILVDCsTwelveOmissionLTwoVarDecoderSamLite}{0.016}
\newcommand{\nLVDCsTwelveOmissionLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDCsTwelveOmissionLTwoVarDecoderSegformerMlp}{63.5}
\newcommand{\miouCILVDCsTwelveOmissionLTwoVarDecoderSegformerMlp}{0.8}
\newcommand{\dropLVDCsTwelveOmissionLTwoVarDecoderSegformerMlp}{6.3}
\newcommand{\dropCILVDCsTwelveOmissionLTwoVarDecoderSegformerMlp}{0.9}
\newcommand{\retLVDCsTwelveOmissionLTwoVarDecoderSegformerMlp}{0.910}
\newcommand{\retCILVDCsTwelveOmissionLTwoVarDecoderSegformerMlp}{0.012}
\newcommand{\nLVDCsTwelveOmissionLTwoVarLrMultOne}{5}
\newcommand{\miouLVDCsTwelveOmissionLTwoVarLrMultOne}{61.6}
\newcommand{\miouCILVDCsTwelveOmissionLTwoVarLrMultOne}{2.6}
\newcommand{\dropLVDCsTwelveOmissionLTwoVarLrMultOne}{6.3}
\newcommand{\dropCILVDCsTwelveOmissionLTwoVarLrMultOne}{2.9}
\newcommand{\retLVDCsTwelveOmissionLTwoVarLrMultOne}{0.908}
\newcommand{\retCILVDCsTwelveOmissionLTwoVarLrMultOne}{0.042}
\newcommand{\nLVDCsTwelveSTwocloudlessREAL}{5}
\newcommand{\miouLVDCsTwelveSTwocloudlessREAL}{35.1}
\newcommand{\miouCILVDCsTwelveSTwocloudlessREAL}{0.3}
\newcommand{\dropLVDCsTwelveSTwocloudlessREAL}{34.5}
\newcommand{\dropCILVDCsTwelveSTwocloudlessREAL}{1.0}
\newcommand{\retLVDCsTwelveSTwocloudlessREAL}{0.504}
\newcommand{\retCILVDCsTwelveSTwocloudlessREAL}{0.008}
\newcommand{\nLVDCsTwelveShiftLOne}{5}
\newcommand{\miouLVDCsTwelveShiftLOne}{68.5}
\newcommand{\miouCILVDCsTwelveShiftLOne}{1.1}
\newcommand{\dropLVDCsTwelveShiftLOne}{1.1}
\newcommand{\dropCILVDCsTwelveShiftLOne}{1.4}
\newcommand{\retLVDCsTwelveShiftLOne}{0.985}
\newcommand{\retCILVDCsTwelveShiftLOne}{0.020}
\newcommand{\nLVDCsTwelveShiftLTwo}{5}
\newcommand{\miouLVDCsTwelveShiftLTwo}{64.7}
\newcommand{\miouCILVDCsTwelveShiftLTwo}{1.0}
\newcommand{\dropLVDCsTwelveShiftLTwo}{4.8}
\newcommand{\dropCILVDCsTwelveShiftLTwo}{1.8}
\newcommand{\retLVDCsTwelveShiftLTwo}{0.931}
\newcommand{\retCILVDCsTwelveShiftLTwo}{0.025}
\newcommand{\nLVDCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}{64.6}
\newcommand{\miouCILVDCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}{0.5}
\newcommand{\dropLVDCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}{4.9}
\newcommand{\dropCILVDCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}{0.7}
\newcommand{\retLVDCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}{0.929}
\newcommand{\retCILVDCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}{0.010}
\newcommand{\nLVDCsTwelveShiftLTwoVarDecoderSamLite}{5}
\newcommand{\miouLVDCsTwelveShiftLTwoVarDecoderSamLite}{64.1}
\newcommand{\miouCILVDCsTwelveShiftLTwoVarDecoderSamLite}{0.5}
\newcommand{\dropLVDCsTwelveShiftLTwoVarDecoderSamLite}{5.4}
\newcommand{\dropCILVDCsTwelveShiftLTwoVarDecoderSamLite}{0.7}
\newcommand{\retLVDCsTwelveShiftLTwoVarDecoderSamLite}{0.922}
\newcommand{\retCILVDCsTwelveShiftLTwoVarDecoderSamLite}{0.010}
\newcommand{\nLVDCsTwelveShiftLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDCsTwelveShiftLTwoVarDecoderSegformerMlp}{65.0}
\newcommand{\miouCILVDCsTwelveShiftLTwoVarDecoderSegformerMlp}{1.1}
\newcommand{\dropLVDCsTwelveShiftLTwoVarDecoderSegformerMlp}{4.8}
\newcommand{\dropCILVDCsTwelveShiftLTwoVarDecoderSegformerMlp}{1.3}
\newcommand{\retLVDCsTwelveShiftLTwoVarDecoderSegformerMlp}{0.931}
\newcommand{\retCILVDCsTwelveShiftLTwoVarDecoderSegformerMlp}{0.018}
\newcommand{\nLVDCsTwelveShiftLTwoVarLrMultOne}{5}
\newcommand{\miouLVDCsTwelveShiftLTwoVarLrMultOne}{62.9}
\newcommand{\miouCILVDCsTwelveShiftLTwoVarLrMultOne}{1.4}
\newcommand{\dropLVDCsTwelveShiftLTwoVarLrMultOne}{5.0}
\newcommand{\dropCILVDCsTwelveShiftLTwoVarLrMultOne}{1.3}
\newcommand{\retLVDCsTwelveShiftLTwoVarLrMultOne}{0.927}
\newcommand{\retCILVDCsTwelveShiftLTwoVarLrMultOne}{0.018}
\newcommand{\nLVDDfcBoundaryLOne}{5}
\newcommand{\miouLVDDfcBoundaryLOne}{42.4}
\newcommand{\miouCILVDDfcBoundaryLOne}{0.9}
\newcommand{\dropLVDDfcBoundaryLOne}{0.8}
\newcommand{\dropCILVDDfcBoundaryLOne}{1.0}
\newcommand{\retLVDDfcBoundaryLOne}{0.982}
\newcommand{\retCILVDDfcBoundaryLOne}{0.023}
\newcommand{\nLVDDfcBoundaryLTwo}{5}
\newcommand{\miouLVDDfcBoundaryLTwo}{38.0}
\newcommand{\miouCILVDDfcBoundaryLTwo}{6.3}
\newcommand{\dropLVDDfcBoundaryLTwo}{5.2}
\newcommand{\dropCILVDDfcBoundaryLTwo}{6.6}
\newcommand{\retLVDDfcBoundaryLTwo}{0.880}
\newcommand{\retCILVDDfcBoundaryLTwo}{0.151}
\newcommand{\nLVDDfcBoundaryLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDDfcBoundaryLTwoVarDecoderMaskTwoformerLite}{37.2}
\newcommand{\miouCILVDDfcBoundaryLTwoVarDecoderMaskTwoformerLite}{2.4}
\newcommand{\dropLVDDfcBoundaryLTwoVarDecoderMaskTwoformerLite}{5.8}
\newcommand{\dropCILVDDfcBoundaryLTwoVarDecoderMaskTwoformerLite}{2.8}
\newcommand{\retLVDDfcBoundaryLTwoVarDecoderMaskTwoformerLite}{0.866}
\newcommand{\retCILVDDfcBoundaryLTwoVarDecoderMaskTwoformerLite}{0.063}
\newcommand{\nLVDDfcBoundaryLTwoVarDecoderSamLite}{5}
\newcommand{\miouLVDDfcBoundaryLTwoVarDecoderSamLite}{35.6}
\newcommand{\miouCILVDDfcBoundaryLTwoVarDecoderSamLite}{2.9}
\newcommand{\dropLVDDfcBoundaryLTwoVarDecoderSamLite}{6.0}
\newcommand{\dropCILVDDfcBoundaryLTwoVarDecoderSamLite}{2.7}
\newcommand{\retLVDDfcBoundaryLTwoVarDecoderSamLite}{0.856}
\newcommand{\retCILVDDfcBoundaryLTwoVarDecoderSamLite}{0.067}
\newcommand{\nLVDDfcBoundaryLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDDfcBoundaryLTwoVarDecoderSegformerMlp}{41.2}
\newcommand{\miouCILVDDfcBoundaryLTwoVarDecoderSegformerMlp}{0.5}
\newcommand{\dropLVDDfcBoundaryLTwoVarDecoderSegformerMlp}{2.8}
\newcommand{\dropCILVDDfcBoundaryLTwoVarDecoderSegformerMlp}{0.7}
\newcommand{\retLVDDfcBoundaryLTwoVarDecoderSegformerMlp}{0.936}
\newcommand{\retCILVDDfcBoundaryLTwoVarDecoderSegformerMlp}{0.015}
\newcommand{\nLVDDfcBoundaryLTwoVarLrMultOne}{5}
\newcommand{\miouLVDDfcBoundaryLTwoVarLrMultOne}{35.9}
\newcommand{\miouCILVDDfcBoundaryLTwoVarLrMultOne}{2.2}
\newcommand{\dropLVDDfcBoundaryLTwoVarLrMultOne}{4.2}
\newcommand{\dropCILVDDfcBoundaryLTwoVarLrMultOne}{6.1}
\newcommand{\retLVDDfcBoundaryLTwoVarLrMultOne}{0.904}
\newcommand{\retCILVDDfcBoundaryLTwoVarLrMultOne}{0.156}
\newcommand{\nLVDDfcClean}{5}
\newcommand{\miouLVDDfcClean}{43.2}
\newcommand{\miouCILVDDfcClean}{0.7}
\newcommand{\nLVDDfcCleanVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDDfcCleanVarDecoderMaskTwoformerLite}{43.0}
\newcommand{\miouCILVDDfcCleanVarDecoderMaskTwoformerLite}{0.9}
\newcommand{\nLVDDfcCleanVarDecoderSamLite}{5}
\newcommand{\miouLVDDfcCleanVarDecoderSamLite}{41.6}
\newcommand{\miouCILVDDfcCleanVarDecoderSamLite}{0.7}
\newcommand{\nLVDDfcCleanVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDDfcCleanVarDecoderSegformerMlp}{44.0}
\newcommand{\miouCILVDDfcCleanVarDecoderSegformerMlp}{0.8}
\newcommand{\nLVDDfcCleanVarLrMultOne}{5}
\newcommand{\miouLVDDfcCleanVarLrMultOne}{40.1}
\newcommand{\miouCILVDDfcCleanVarLrMultOne}{4.9}
\newcommand{\nLVDDfcCleanVarTrainSubsetRealcov}{5}
\newcommand{\miouLVDDfcCleanVarTrainSubsetRealcov}{43.2}
\newcommand{\miouCILVDDfcCleanVarTrainSubsetRealcov}{0.6}
\newcommand{\nLVDDfcCoarseLOne}{5}
\newcommand{\miouLVDDfcCoarseLOne}{42.9}
\newcommand{\miouCILVDDfcCoarseLOne}{0.6}
\newcommand{\dropLVDDfcCoarseLOne}{0.3}
\newcommand{\dropCILVDDfcCoarseLOne}{0.7}
\newcommand{\retLVDDfcCoarseLOne}{0.993}
\newcommand{\retCILVDDfcCoarseLOne}{0.016}
\newcommand{\nLVDDfcCoarseLTwo}{5}
\newcommand{\miouLVDDfcCoarseLTwo}{41.6}
\newcommand{\miouCILVDDfcCoarseLTwo}{1.0}
\newcommand{\dropLVDDfcCoarseLTwo}{1.5}
\newcommand{\dropCILVDDfcCoarseLTwo}{0.9}
\newcommand{\retLVDDfcCoarseLTwo}{0.964}
\newcommand{\retCILVDDfcCoarseLTwo}{0.022}
\newcommand{\nLVDDfcCoarseLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDDfcCoarseLTwoVarDecoderMaskTwoformerLite}{41.9}
\newcommand{\miouCILVDDfcCoarseLTwoVarDecoderMaskTwoformerLite}{1.2}
\newcommand{\dropLVDDfcCoarseLTwoVarDecoderMaskTwoformerLite}{1.1}
\newcommand{\dropCILVDDfcCoarseLTwoVarDecoderMaskTwoformerLite}{1.9}
\newcommand{\retLVDDfcCoarseLTwoVarDecoderMaskTwoformerLite}{0.974}
\newcommand{\retCILVDDfcCoarseLTwoVarDecoderMaskTwoformerLite}{0.043}
\newcommand{\nLVDDfcCoarseLTwoVarDecoderSamLite}{5}
\newcommand{\miouLVDDfcCoarseLTwoVarDecoderSamLite}{41.5}
\newcommand{\miouCILVDDfcCoarseLTwoVarDecoderSamLite}{0.8}
\newcommand{\dropLVDDfcCoarseLTwoVarDecoderSamLite}{0.0}
\newcommand{\dropCILVDDfcCoarseLTwoVarDecoderSamLite}{1.2}
\newcommand{\retLVDDfcCoarseLTwoVarDecoderSamLite}{0.999}
\newcommand{\retCILVDDfcCoarseLTwoVarDecoderSamLite}{0.030}
\newcommand{\nLVDDfcCoarseLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDDfcCoarseLTwoVarDecoderSegformerMlp}{42.2}
\newcommand{\miouCILVDDfcCoarseLTwoVarDecoderSegformerMlp}{0.6}
\newcommand{\dropLVDDfcCoarseLTwoVarDecoderSegformerMlp}{1.7}
\newcommand{\dropCILVDDfcCoarseLTwoVarDecoderSegformerMlp}{0.6}
\newcommand{\retLVDDfcCoarseLTwoVarDecoderSegformerMlp}{0.960}
\newcommand{\retCILVDDfcCoarseLTwoVarDecoderSegformerMlp}{0.014}
\newcommand{\nLVDDfcCoarseLTwoVarLrMultOne}{5}
\newcommand{\miouLVDDfcCoarseLTwoVarLrMultOne}{39.6}
\newcommand{\miouCILVDDfcCoarseLTwoVarLrMultOne}{1.3}
\newcommand{\dropLVDDfcCoarseLTwoVarLrMultOne}{0.6}
\newcommand{\dropCILVDDfcCoarseLTwoVarLrMultOne}{4.9}
\newcommand{\retLVDDfcCoarseLTwoVarLrMultOne}{0.995}
\newcommand{\retCILVDDfcCoarseLTwoVarLrMultOne}{0.140}
\newcommand{\nLVDDfcModisREALVarTrainSubsetRealcov}{5}
\newcommand{\miouLVDDfcModisREALVarTrainSubsetRealcov}{37.1}
\newcommand{\miouCILVDDfcModisREALVarTrainSubsetRealcov}{1.9}
\newcommand{\dropLVDDfcModisREALVarTrainSubsetRealcov}{6.1}
\newcommand{\dropCILVDDfcModisREALVarTrainSubsetRealcov}{1.9}
\newcommand{\retLVDDfcModisREALVarTrainSubsetRealcov}{0.859}
\newcommand{\retCILVDDfcModisREALVarTrainSubsetRealcov}{0.045}
\newcommand{\nLVDDfcOmissionLOne}{5}
\newcommand{\miouLVDDfcOmissionLOne}{41.8}
\newcommand{\miouCILVDDfcOmissionLOne}{0.9}
\newcommand{\dropLVDDfcOmissionLOne}{1.4}
\newcommand{\dropCILVDDfcOmissionLOne}{1.4}
\newcommand{\retLVDDfcOmissionLOne}{0.967}
\newcommand{\retCILVDDfcOmissionLOne}{0.031}
\newcommand{\nLVDDfcOmissionLTwo}{5}
\newcommand{\miouLVDDfcOmissionLTwo}{40.0}
\newcommand{\miouCILVDDfcOmissionLTwo}{0.8}
\newcommand{\dropLVDDfcOmissionLTwo}{3.2}
\newcommand{\dropCILVDDfcOmissionLTwo}{1.2}
\newcommand{\retLVDDfcOmissionLTwo}{0.927}
\newcommand{\retCILVDDfcOmissionLTwo}{0.028}
\newcommand{\nLVDDfcOmissionLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDDfcOmissionLTwoVarDecoderMaskTwoformerLite}{38.4}
\newcommand{\miouCILVDDfcOmissionLTwoVarDecoderMaskTwoformerLite}{1.8}
\newcommand{\dropLVDDfcOmissionLTwoVarDecoderMaskTwoformerLite}{4.6}
\newcommand{\dropCILVDDfcOmissionLTwoVarDecoderMaskTwoformerLite}{2.4}
\newcommand{\retLVDDfcOmissionLTwoVarDecoderMaskTwoformerLite}{0.893}
\newcommand{\retCILVDDfcOmissionLTwoVarDecoderMaskTwoformerLite}{0.054}
\newcommand{\nLVDDfcOmissionLTwoVarDecoderSamLite}{5}
\newcommand{\miouLVDDfcOmissionLTwoVarDecoderSamLite}{38.6}
\newcommand{\miouCILVDDfcOmissionLTwoVarDecoderSamLite}{2.6}
\newcommand{\dropLVDDfcOmissionLTwoVarDecoderSamLite}{3.0}
\newcommand{\dropCILVDDfcOmissionLTwoVarDecoderSamLite}{3.1}
\newcommand{\retLVDDfcOmissionLTwoVarDecoderSamLite}{0.928}
\newcommand{\retCILVDDfcOmissionLTwoVarDecoderSamLite}{0.074}
\newcommand{\nLVDDfcOmissionLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDDfcOmissionLTwoVarDecoderSegformerMlp}{41.3}
\newcommand{\miouCILVDDfcOmissionLTwoVarDecoderSegformerMlp}{1.0}
\newcommand{\dropLVDDfcOmissionLTwoVarDecoderSegformerMlp}{2.7}
\newcommand{\dropCILVDDfcOmissionLTwoVarDecoderSegformerMlp}{1.5}
\newcommand{\retLVDDfcOmissionLTwoVarDecoderSegformerMlp}{0.939}
\newcommand{\retCILVDDfcOmissionLTwoVarDecoderSegformerMlp}{0.033}
\newcommand{\nLVDDfcOmissionLTwoVarLrMultOne}{5}
\newcommand{\miouLVDDfcOmissionLTwoVarLrMultOne}{35.2}
\newcommand{\miouCILVDDfcOmissionLTwoVarLrMultOne}{2.0}
\newcommand{\dropLVDDfcOmissionLTwoVarLrMultOne}{4.9}
\newcommand{\dropCILVDDfcOmissionLTwoVarLrMultOne}{3.3}
\newcommand{\retLVDDfcOmissionLTwoVarLrMultOne}{0.883}
\newcommand{\retCILVDDfcOmissionLTwoVarLrMultOne}{0.078}
\newcommand{\nLVDDfcShiftLOne}{5}
\newcommand{\miouLVDDfcShiftLOne}{43.3}
\newcommand{\miouCILVDDfcShiftLOne}{1.0}
\newcommand{\dropLVDDfcShiftLOne}{\ensuremath{-}0.1}
\newcommand{\dropCILVDDfcShiftLOne}{0.4}
\newcommand{\retLVDDfcShiftLOne}{1.003}
\newcommand{\retCILVDDfcShiftLOne}{0.009}
\newcommand{\nLVDDfcShiftLTwo}{5}
\newcommand{\miouLVDDfcShiftLTwo}{43.0}
\newcommand{\miouCILVDDfcShiftLTwo}{0.9}
\newcommand{\dropLVDDfcShiftLTwo}{0.2}
\newcommand{\dropCILVDDfcShiftLTwo}{1.0}
\newcommand{\retLVDDfcShiftLTwo}{0.995}
\newcommand{\retCILVDDfcShiftLTwo}{0.022}
\newcommand{\nLVDDfcShiftLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDDfcShiftLTwoVarDecoderMaskTwoformerLite}{42.3}
\newcommand{\miouCILVDDfcShiftLTwoVarDecoderMaskTwoformerLite}{2.7}
\newcommand{\dropLVDDfcShiftLTwoVarDecoderMaskTwoformerLite}{0.7}
\newcommand{\dropCILVDDfcShiftLTwoVarDecoderMaskTwoformerLite}{2.3}
\newcommand{\retLVDDfcShiftLTwoVarDecoderMaskTwoformerLite}{0.983}
\newcommand{\retCILVDDfcShiftLTwoVarDecoderMaskTwoformerLite}{0.053}
\newcommand{\nLVDDfcShiftLTwoVarDecoderSamLite}{5}
\newcommand{\miouLVDDfcShiftLTwoVarDecoderSamLite}{41.4}
\newcommand{\miouCILVDDfcShiftLTwoVarDecoderSamLite}{1.3}
\newcommand{\dropLVDDfcShiftLTwoVarDecoderSamLite}{0.1}
\newcommand{\dropCILVDDfcShiftLTwoVarDecoderSamLite}{1.3}
\newcommand{\retLVDDfcShiftLTwoVarDecoderSamLite}{0.997}
\newcommand{\retCILVDDfcShiftLTwoVarDecoderSamLite}{0.030}
\newcommand{\nLVDDfcShiftLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDDfcShiftLTwoVarDecoderSegformerMlp}{44.2}
\newcommand{\miouCILVDDfcShiftLTwoVarDecoderSegformerMlp}{0.8}
\newcommand{\dropLVDDfcShiftLTwoVarDecoderSegformerMlp}{\ensuremath{-}0.2}
\newcommand{\dropCILVDDfcShiftLTwoVarDecoderSegformerMlp}{1.0}
\newcommand{\retLVDDfcShiftLTwoVarDecoderSegformerMlp}{1.005}
\newcommand{\retCILVDDfcShiftLTwoVarDecoderSegformerMlp}{0.023}
\newcommand{\nLVDDfcShiftLTwoVarLrMultOne}{5}
\newcommand{\miouLVDDfcShiftLTwoVarLrMultOne}{41.7}
\newcommand{\miouCILVDDfcShiftLTwoVarLrMultOne}{2.3}
\newcommand{\dropLVDDfcShiftLTwoVarLrMultOne}{\ensuremath{-}1.5}
\newcommand{\dropCILVDDfcShiftLTwoVarLrMultOne}{2.8}
\newcommand{\retLVDDfcShiftLTwoVarLrMultOne}{1.043}
\newcommand{\retCILVDDfcShiftLTwoVarLrMultOne}{0.085}
\newcommand{\nLVDEnvaBoundaryLOne}{5}
\newcommand{\miouLVDEnvaBoundaryLOne}{59.8}
\newcommand{\miouCILVDEnvaBoundaryLOne}{3.9}
\newcommand{\dropLVDEnvaBoundaryLOne}{3.2}
\newcommand{\dropCILVDEnvaBoundaryLOne}{4.0}
\newcommand{\retLVDEnvaBoundaryLOne}{0.949}
\newcommand{\retCILVDEnvaBoundaryLOne}{0.065}
\newcommand{\nLVDEnvaBoundaryLTwo}{5}
\newcommand{\miouLVDEnvaBoundaryLTwo}{52.1}
\newcommand{\miouCILVDEnvaBoundaryLTwo}{6.7}
\newcommand{\dropLVDEnvaBoundaryLTwo}{10.9}
\newcommand{\dropCILVDEnvaBoundaryLTwo}{6.8}
\newcommand{\retLVDEnvaBoundaryLTwo}{0.828}
\newcommand{\retCILVDEnvaBoundaryLTwo}{0.107}
\newcommand{\nLVDEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}{52.5}
\newcommand{\miouCILVDEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}{4.2}
\newcommand{\dropLVDEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}{8.2}
\newcommand{\dropCILVDEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}{3.1}
\newcommand{\retLVDEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}{0.865}
\newcommand{\retCILVDEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}{0.052}
\newcommand{\nLVDEnvaBoundaryLTwoVarDecoderSamLite}{5}
\newcommand{\miouLVDEnvaBoundaryLTwoVarDecoderSamLite}{51.4}
\newcommand{\miouCILVDEnvaBoundaryLTwoVarDecoderSamLite}{4.6}
\newcommand{\dropLVDEnvaBoundaryLTwoVarDecoderSamLite}{4.1}
\newcommand{\dropCILVDEnvaBoundaryLTwoVarDecoderSamLite}{4.6}
\newcommand{\retLVDEnvaBoundaryLTwoVarDecoderSamLite}{0.926}
\newcommand{\retCILVDEnvaBoundaryLTwoVarDecoderSamLite}{0.081}
\newcommand{\nLVDEnvaBoundaryLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDEnvaBoundaryLTwoVarDecoderSegformerMlp}{54.3}
\newcommand{\miouCILVDEnvaBoundaryLTwoVarDecoderSegformerMlp}{6.2}
\newcommand{\dropLVDEnvaBoundaryLTwoVarDecoderSegformerMlp}{9.7}
\newcommand{\dropCILVDEnvaBoundaryLTwoVarDecoderSegformerMlp}{6.6}
\newcommand{\retLVDEnvaBoundaryLTwoVarDecoderSegformerMlp}{0.849}
\newcommand{\retCILVDEnvaBoundaryLTwoVarDecoderSegformerMlp}{0.102}
\newcommand{\nLVDEnvaBoundaryLTwoVarLrMultOne}{5}
\newcommand{\miouLVDEnvaBoundaryLTwoVarLrMultOne}{54.5}
\newcommand{\miouCILVDEnvaBoundaryLTwoVarLrMultOne}{5.2}
\newcommand{\dropLVDEnvaBoundaryLTwoVarLrMultOne}{7.3}
\newcommand{\dropCILVDEnvaBoundaryLTwoVarLrMultOne}{3.7}
\newcommand{\retLVDEnvaBoundaryLTwoVarLrMultOne}{0.882}
\newcommand{\retCILVDEnvaBoundaryLTwoVarLrMultOne}{0.057}
\newcommand{\nLVDEnvaClean}{5}
\newcommand{\miouLVDEnvaClean}{63.0}
\newcommand{\miouCILVDEnvaClean}{1.1}
\newcommand{\nLVDEnvaCleanVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDEnvaCleanVarDecoderMaskTwoformerLite}{60.6}
\newcommand{\miouCILVDEnvaCleanVarDecoderMaskTwoformerLite}{2.5}
\newcommand{\nLVDEnvaCleanVarDecoderSamLite}{5}
\newcommand{\miouLVDEnvaCleanVarDecoderSamLite}{55.5}
\newcommand{\miouCILVDEnvaCleanVarDecoderSamLite}{3.2}
\newcommand{\nLVDEnvaCleanVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDEnvaCleanVarDecoderSegformerMlp}{63.9}
\newcommand{\miouCILVDEnvaCleanVarDecoderSegformerMlp}{1.0}
\newcommand{\nLVDEnvaCleanVarLrMultOne}{5}
\newcommand{\miouLVDEnvaCleanVarLrMultOne}{61.8}
\newcommand{\miouCILVDEnvaCleanVarLrMultOne}{4.6}
\newcommand{\nLVDEnvaCoarseLOne}{5}
\newcommand{\miouLVDEnvaCoarseLOne}{62.7}
\newcommand{\miouCILVDEnvaCoarseLOne}{1.6}
\newcommand{\dropLVDEnvaCoarseLOne}{0.3}
\newcommand{\dropCILVDEnvaCoarseLOne}{1.4}
\newcommand{\retLVDEnvaCoarseLOne}{0.996}
\newcommand{\retCILVDEnvaCoarseLOne}{0.022}
\newcommand{\nLVDEnvaCoarseLTwo}{5}
\newcommand{\miouLVDEnvaCoarseLTwo}{59.5}
\newcommand{\miouCILVDEnvaCoarseLTwo}{3.5}
\newcommand{\dropLVDEnvaCoarseLTwo}{3.5}
\newcommand{\dropCILVDEnvaCoarseLTwo}{3.3}
\newcommand{\retLVDEnvaCoarseLTwo}{0.944}
\newcommand{\retCILVDEnvaCoarseLTwo}{0.053}
\newcommand{\nLVDEnvaCoarseLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDEnvaCoarseLTwoVarDecoderMaskTwoformerLite}{59.6}
\newcommand{\miouCILVDEnvaCoarseLTwoVarDecoderMaskTwoformerLite}{1.6}
\newcommand{\dropLVDEnvaCoarseLTwoVarDecoderMaskTwoformerLite}{1.1}
\newcommand{\dropCILVDEnvaCoarseLTwoVarDecoderMaskTwoformerLite}{2.1}
\newcommand{\retLVDEnvaCoarseLTwoVarDecoderMaskTwoformerLite}{0.983}
\newcommand{\retCILVDEnvaCoarseLTwoVarDecoderMaskTwoformerLite}{0.036}
\newcommand{\nLVDEnvaCoarseLTwoVarDecoderSamLite}{5}
\newcommand{\miouLVDEnvaCoarseLTwoVarDecoderSamLite}{55.0}
\newcommand{\miouCILVDEnvaCoarseLTwoVarDecoderSamLite}{2.1}
\newcommand{\dropLVDEnvaCoarseLTwoVarDecoderSamLite}{0.5}
\newcommand{\dropCILVDEnvaCoarseLTwoVarDecoderSamLite}{2.1}
\newcommand{\retLVDEnvaCoarseLTwoVarDecoderSamLite}{0.991}
\newcommand{\retCILVDEnvaCoarseLTwoVarDecoderSamLite}{0.035}
\newcommand{\nLVDEnvaCoarseLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDEnvaCoarseLTwoVarDecoderSegformerMlp}{63.1}
\newcommand{\miouCILVDEnvaCoarseLTwoVarDecoderSegformerMlp}{0.6}
\newcommand{\dropLVDEnvaCoarseLTwoVarDecoderSegformerMlp}{0.8}
\newcommand{\dropCILVDEnvaCoarseLTwoVarDecoderSegformerMlp}{1.4}
\newcommand{\retLVDEnvaCoarseLTwoVarDecoderSegformerMlp}{0.987}
\newcommand{\retCILVDEnvaCoarseLTwoVarDecoderSegformerMlp}{0.021}
\newcommand{\nLVDEnvaCoarseLTwoVarLrMultOne}{5}
\newcommand{\miouLVDEnvaCoarseLTwoVarLrMultOne}{60.1}
\newcommand{\miouCILVDEnvaCoarseLTwoVarLrMultOne}{3.7}
\newcommand{\dropLVDEnvaCoarseLTwoVarLrMultOne}{1.7}
\newcommand{\dropCILVDEnvaCoarseLTwoVarLrMultOne}{6.9}
\newcommand{\retLVDEnvaCoarseLTwoVarLrMultOne}{0.977}
\newcommand{\retCILVDEnvaCoarseLTwoVarLrMultOne}{0.118}
\newcommand{\nLVDEnvaNlcdREAL}{5}
\newcommand{\miouLVDEnvaNlcdREAL}{33.0}
\newcommand{\miouCILVDEnvaNlcdREAL}{6.1}
\newcommand{\dropLVDEnvaNlcdREAL}{30.0}
\newcommand{\dropCILVDEnvaNlcdREAL}{6.5}
\newcommand{\retLVDEnvaNlcdREAL}{0.524}
\newcommand{\retCILVDEnvaNlcdREAL}{0.101}
\newcommand{\nLVDEnvaOmissionLOne}{5}
\newcommand{\miouLVDEnvaOmissionLOne}{57.3}
\newcommand{\miouCILVDEnvaOmissionLOne}{9.2}
\newcommand{\dropLVDEnvaOmissionLOne}{5.7}
\newcommand{\dropCILVDEnvaOmissionLOne}{9.7}
\newcommand{\retLVDEnvaOmissionLOne}{0.911}
\newcommand{\retCILVDEnvaOmissionLOne}{0.153}
\newcommand{\nLVDEnvaOmissionLTwo}{5}
\newcommand{\miouLVDEnvaOmissionLTwo}{48.8}
\newcommand{\miouCILVDEnvaOmissionLTwo}{4.7}
\newcommand{\dropLVDEnvaOmissionLTwo}{14.2}
\newcommand{\dropCILVDEnvaOmissionLTwo}{4.8}
\newcommand{\retLVDEnvaOmissionLTwo}{0.775}
\newcommand{\retCILVDEnvaOmissionLTwo}{0.076}
\newcommand{\nLVDEnvaOmissionLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDEnvaOmissionLTwoVarDecoderMaskTwoformerLite}{52.4}
\newcommand{\miouCILVDEnvaOmissionLTwoVarDecoderMaskTwoformerLite}{4.1}
\newcommand{\dropLVDEnvaOmissionLTwoVarDecoderMaskTwoformerLite}{8.2}
\newcommand{\dropCILVDEnvaOmissionLTwoVarDecoderMaskTwoformerLite}{5.4}
\newcommand{\retLVDEnvaOmissionLTwoVarDecoderMaskTwoformerLite}{0.866}
\newcommand{\retCILVDEnvaOmissionLTwoVarDecoderMaskTwoformerLite}{0.086}
\newcommand{\nLVDEnvaOmissionLTwoVarDecoderSamLite}{5}
\newcommand{\miouLVDEnvaOmissionLTwoVarDecoderSamLite}{51.1}
\newcommand{\miouCILVDEnvaOmissionLTwoVarDecoderSamLite}{2.8}
\newcommand{\dropLVDEnvaOmissionLTwoVarDecoderSamLite}{4.4}
\newcommand{\dropCILVDEnvaOmissionLTwoVarDecoderSamLite}{3.5}
\newcommand{\retLVDEnvaOmissionLTwoVarDecoderSamLite}{0.922}
\newcommand{\retCILVDEnvaOmissionLTwoVarDecoderSamLite}{0.058}
\newcommand{\nLVDEnvaOmissionLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDEnvaOmissionLTwoVarDecoderSegformerMlp}{56.0}
\newcommand{\miouCILVDEnvaOmissionLTwoVarDecoderSegformerMlp}{6.2}
\newcommand{\dropLVDEnvaOmissionLTwoVarDecoderSegformerMlp}{8.0}
\newcommand{\dropCILVDEnvaOmissionLTwoVarDecoderSegformerMlp}{5.9}
\newcommand{\retLVDEnvaOmissionLTwoVarDecoderSegformerMlp}{0.875}
\newcommand{\retCILVDEnvaOmissionLTwoVarDecoderSegformerMlp}{0.094}
\newcommand{\nLVDEnvaOmissionLTwoVarLrMultOne}{5}
\newcommand{\miouLVDEnvaOmissionLTwoVarLrMultOne}{55.4}
\newcommand{\miouCILVDEnvaOmissionLTwoVarLrMultOne}{8.9}
\newcommand{\dropLVDEnvaOmissionLTwoVarLrMultOne}{6.4}
\newcommand{\dropCILVDEnvaOmissionLTwoVarLrMultOne}{10.4}
\newcommand{\retLVDEnvaOmissionLTwoVarLrMultOne}{0.900}
\newcommand{\retCILVDEnvaOmissionLTwoVarLrMultOne}{0.165}
\newcommand{\nLVDEnvaShiftLOne}{5}
\newcommand{\miouLVDEnvaShiftLOne}{62.9}
\newcommand{\miouCILVDEnvaShiftLOne}{0.7}
\newcommand{\dropLVDEnvaShiftLOne}{0.1}
\newcommand{\dropCILVDEnvaShiftLOne}{0.8}
\newcommand{\retLVDEnvaShiftLOne}{0.998}
\newcommand{\retCILVDEnvaShiftLOne}{0.013}
\newcommand{\nLVDEnvaShiftLTwo}{5}
\newcommand{\miouLVDEnvaShiftLTwo}{60.6}
\newcommand{\miouCILVDEnvaShiftLTwo}{1.1}
\newcommand{\dropLVDEnvaShiftLTwo}{2.4}
\newcommand{\dropCILVDEnvaShiftLTwo}{1.5}
\newcommand{\retLVDEnvaShiftLTwo}{0.962}
\newcommand{\retCILVDEnvaShiftLTwo}{0.024}
\newcommand{\nLVDEnvaShiftLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDEnvaShiftLTwoVarDecoderMaskTwoformerLite}{61.2}
\newcommand{\miouCILVDEnvaShiftLTwoVarDecoderMaskTwoformerLite}{1.5}
\newcommand{\dropLVDEnvaShiftLTwoVarDecoderMaskTwoformerLite}{\ensuremath{-}0.6}
\newcommand{\dropCILVDEnvaShiftLTwoVarDecoderMaskTwoformerLite}{2.2}
\newcommand{\retLVDEnvaShiftLTwoVarDecoderMaskTwoformerLite}{1.010}
\newcommand{\retCILVDEnvaShiftLTwoVarDecoderMaskTwoformerLite}{0.038}
\newcommand{\nLVDEnvaShiftLTwoVarDecoderSamLite}{5}
\newcommand{\miouLVDEnvaShiftLTwoVarDecoderSamLite}{54.4}
\newcommand{\miouCILVDEnvaShiftLTwoVarDecoderSamLite}{3.4}
\newcommand{\dropLVDEnvaShiftLTwoVarDecoderSamLite}{1.1}
\newcommand{\dropCILVDEnvaShiftLTwoVarDecoderSamLite}{1.9}
\newcommand{\retLVDEnvaShiftLTwoVarDecoderSamLite}{0.981}
\newcommand{\retCILVDEnvaShiftLTwoVarDecoderSamLite}{0.035}
\newcommand{\nLVDEnvaShiftLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDEnvaShiftLTwoVarDecoderSegformerMlp}{63.4}
\newcommand{\miouCILVDEnvaShiftLTwoVarDecoderSegformerMlp}{0.6}
\newcommand{\dropLVDEnvaShiftLTwoVarDecoderSegformerMlp}{0.5}
\newcommand{\dropCILVDEnvaShiftLTwoVarDecoderSegformerMlp}{0.8}
\newcommand{\retLVDEnvaShiftLTwoVarDecoderSegformerMlp}{0.993}
\newcommand{\retCILVDEnvaShiftLTwoVarDecoderSegformerMlp}{0.013}
\newcommand{\nLVDEnvaShiftLTwoVarLrMultOne}{5}
\newcommand{\miouLVDEnvaShiftLTwoVarLrMultOne}{61.4}
\newcommand{\miouCILVDEnvaShiftLTwoVarLrMultOne}{3.7}
\newcommand{\dropLVDEnvaShiftLTwoVarLrMultOne}{0.4}
\newcommand{\dropCILVDEnvaShiftLTwoVarLrMultOne}{6.8}
\newcommand{\retLVDEnvaShiftLTwoVarLrMultOne}{0.997}
\newcommand{\retCILVDEnvaShiftLTwoVarLrMultOne}{0.118}
\newcommand{\nLVDflairBoundaryLOne}{5}
\newcommand{\miouLVDflairBoundaryLOne}{49.9}
\newcommand{\miouCILVDflairBoundaryLOne}{1.9}
\newcommand{\dropLVDflairBoundaryLOne}{1.0}
\newcommand{\dropCILVDflairBoundaryLOne}{2.3}
\newcommand{\retLVDflairBoundaryLOne}{0.982}
\newcommand{\retCILVDflairBoundaryLOne}{0.045}
\newcommand{\nLVDflairBoundaryLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouLVDflairBoundaryLOneVarDecoderMaskTwoformerFull}{48.2}
\newcommand{\miouCILVDflairBoundaryLOneVarDecoderMaskTwoformerFull}{1.0}
\newcommand{\dropLVDflairBoundaryLOneVarDecoderMaskTwoformerFull}{1.0}
\newcommand{\dropCILVDflairBoundaryLOneVarDecoderMaskTwoformerFull}{0.6}
\newcommand{\retLVDflairBoundaryLOneVarDecoderMaskTwoformerFull}{0.980}
\newcommand{\retCILVDflairBoundaryLOneVarDecoderMaskTwoformerFull}{0.012}
\newcommand{\nLVDflairBoundaryLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDflairBoundaryLOneVarDecoderMaskTwoformerLite}{48.6}
\newcommand{\miouCILVDflairBoundaryLOneVarDecoderMaskTwoformerLite}{1.1}
\newcommand{\dropLVDflairBoundaryLOneVarDecoderMaskTwoformerLite}{1.9}
\newcommand{\dropCILVDflairBoundaryLOneVarDecoderMaskTwoformerLite}{0.9}
\newcommand{\retLVDflairBoundaryLOneVarDecoderMaskTwoformerLite}{0.963}
\newcommand{\retCILVDflairBoundaryLOneVarDecoderMaskTwoformerLite}{0.018}
\newcommand{\nLVDflairBoundaryLOneVarDecoderSamLite}{5}
\newcommand{\miouLVDflairBoundaryLOneVarDecoderSamLite}{44.4}
\newcommand{\miouCILVDflairBoundaryLOneVarDecoderSamLite}{0.6}
\newcommand{\dropLVDflairBoundaryLOneVarDecoderSamLite}{1.8}
\newcommand{\dropCILVDflairBoundaryLOneVarDecoderSamLite}{1.7}
\newcommand{\retLVDflairBoundaryLOneVarDecoderSamLite}{0.962}
\newcommand{\retCILVDflairBoundaryLOneVarDecoderSamLite}{0.036}
\newcommand{\nLVDflairBoundaryLOneVarDecoderSamPretrained}{5}
\newcommand{\miouLVDflairBoundaryLOneVarDecoderSamPretrained}{43.7}
\newcommand{\miouCILVDflairBoundaryLOneVarDecoderSamPretrained}{1.3}
\newcommand{\dropLVDflairBoundaryLOneVarDecoderSamPretrained}{1.4}
\newcommand{\dropCILVDflairBoundaryLOneVarDecoderSamPretrained}{0.7}
\newcommand{\retLVDflairBoundaryLOneVarDecoderSamPretrained}{0.968}
\newcommand{\retCILVDflairBoundaryLOneVarDecoderSamPretrained}{0.014}
\newcommand{\nLVDflairBoundaryLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDflairBoundaryLOneVarDecoderSegformerMlp}{49.8}
\newcommand{\miouCILVDflairBoundaryLOneVarDecoderSegformerMlp}{0.5}
\newcommand{\dropLVDflairBoundaryLOneVarDecoderSegformerMlp}{1.5}
\newcommand{\dropCILVDflairBoundaryLOneVarDecoderSegformerMlp}{1.0}
\newcommand{\retLVDflairBoundaryLOneVarDecoderSegformerMlp}{0.971}
\newcommand{\retCILVDflairBoundaryLOneVarDecoderSegformerMlp}{0.019}
\newcommand{\nLVDflairBoundaryLTwo}{8}
\newcommand{\miouLVDflairBoundaryLTwo}{46.8}
\newcommand{\miouCILVDflairBoundaryLTwo}{0.5}
\newcommand{\dropLVDflairBoundaryLTwo}{3.9}
\newcommand{\dropCILVDflairBoundaryLTwo}{0.7}
\newcommand{\retLVDflairBoundaryLTwo}{0.923}
\newcommand{\retCILVDflairBoundaryLTwo}{0.012}
\newcommand{\nLVDflairBoundaryLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouLVDflairBoundaryLTwoVarDecoderMaskTwoformerFull}{44.8}
\newcommand{\miouCILVDflairBoundaryLTwoVarDecoderMaskTwoformerFull}{2.0}
\newcommand{\dropLVDflairBoundaryLTwoVarDecoderMaskTwoformerFull}{4.3}
\newcommand{\dropCILVDflairBoundaryLTwoVarDecoderMaskTwoformerFull}{1.7}
\newcommand{\retLVDflairBoundaryLTwoVarDecoderMaskTwoformerFull}{0.912}
\newcommand{\retCILVDflairBoundaryLTwoVarDecoderMaskTwoformerFull}{0.036}
\newcommand{\nLVDflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}{5}
\newcommand{\miouLVDflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}{48.0}
\newcommand{\miouCILVDflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}{1.5}
\newcommand{\dropLVDflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}{2.7}
\newcommand{\dropCILVDflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}{1.5}
\newcommand{\retLVDflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}{0.947}
\newcommand{\retCILVDflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}{0.030}
\newcommand{\nLVDflairBoundaryLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDflairBoundaryLTwoVarDecoderMaskTwoformerLite}{43.8}
\newcommand{\miouCILVDflairBoundaryLTwoVarDecoderMaskTwoformerLite}{1.7}
\newcommand{\dropLVDflairBoundaryLTwoVarDecoderMaskTwoformerLite}{6.6}
\newcommand{\dropCILVDflairBoundaryLTwoVarDecoderMaskTwoformerLite}{1.1}
\newcommand{\retLVDflairBoundaryLTwoVarDecoderMaskTwoformerLite}{0.869}
\newcommand{\retCILVDflairBoundaryLTwoVarDecoderMaskTwoformerLite}{0.023}
\newcommand{\nLVDflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}{5}
\newcommand{\miouLVDflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}{46.0}
\newcommand{\miouCILVDflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}{1.9}
\newcommand{\dropLVDflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}{5.8}
\newcommand{\dropCILVDflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}{1.6}
\newcommand{\retLVDflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}{0.889}
\newcommand{\retCILVDflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}{0.032}
\newcommand{\nLVDflairBoundaryLTwoVarDecoderSamLite}{5}
\newcommand{\miouLVDflairBoundaryLTwoVarDecoderSamLite}{41.2}
\newcommand{\miouCILVDflairBoundaryLTwoVarDecoderSamLite}{1.5}
\newcommand{\dropLVDflairBoundaryLTwoVarDecoderSamLite}{5.0}
\newcommand{\dropCILVDflairBoundaryLTwoVarDecoderSamLite}{1.9}
\newcommand{\retLVDflairBoundaryLTwoVarDecoderSamLite}{0.892}
\newcommand{\retCILVDflairBoundaryLTwoVarDecoderSamLite}{0.039}
\newcommand{\nLVDflairBoundaryLTwoVarDecoderSamLiteLrMultOne}{5}
\newcommand{\miouLVDflairBoundaryLTwoVarDecoderSamLiteLrMultOne}{44.3}
\newcommand{\miouCILVDflairBoundaryLTwoVarDecoderSamLiteLrMultOne}{1.3}
\newcommand{\dropLVDflairBoundaryLTwoVarDecoderSamLiteLrMultOne}{4.5}
\newcommand{\dropCILVDflairBoundaryLTwoVarDecoderSamLiteLrMultOne}{1.1}
\newcommand{\retLVDflairBoundaryLTwoVarDecoderSamLiteLrMultOne}{0.908}
\newcommand{\retCILVDflairBoundaryLTwoVarDecoderSamLiteLrMultOne}{0.022}
\newcommand{\nLVDflairBoundaryLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouLVDflairBoundaryLTwoVarDecoderSamPretrained}{39.8}
\newcommand{\miouCILVDflairBoundaryLTwoVarDecoderSamPretrained}{2.7}
\newcommand{\dropLVDflairBoundaryLTwoVarDecoderSamPretrained}{5.3}
\newcommand{\dropCILVDflairBoundaryLTwoVarDecoderSamPretrained}{1.7}
\newcommand{\retLVDflairBoundaryLTwoVarDecoderSamPretrained}{0.883}
\newcommand{\retCILVDflairBoundaryLTwoVarDecoderSamPretrained}{0.038}
\newcommand{\nLVDflairBoundaryLTwoVarDecoderSamPretrainedLrMultOne}{5}
\newcommand{\miouLVDflairBoundaryLTwoVarDecoderSamPretrainedLrMultOne}{42.8}
\newcommand{\miouCILVDflairBoundaryLTwoVarDecoderSamPretrainedLrMultOne}{0.7}
\newcommand{\dropLVDflairBoundaryLTwoVarDecoderSamPretrainedLrMultOne}{4.6}
\newcommand{\dropCILVDflairBoundaryLTwoVarDecoderSamPretrainedLrMultOne}{1.3}
\newcommand{\retLVDflairBoundaryLTwoVarDecoderSamPretrainedLrMultOne}{0.904}
\newcommand{\retCILVDflairBoundaryLTwoVarDecoderSamPretrainedLrMultOne}{0.025}
\newcommand{\nLVDflairBoundaryLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDflairBoundaryLTwoVarDecoderSegformerMlp}{47.6}
\newcommand{\miouCILVDflairBoundaryLTwoVarDecoderSegformerMlp}{1.0}
\newcommand{\dropLVDflairBoundaryLTwoVarDecoderSegformerMlp}{3.7}
\newcommand{\dropCILVDflairBoundaryLTwoVarDecoderSegformerMlp}{1.1}
\newcommand{\retLVDflairBoundaryLTwoVarDecoderSegformerMlp}{0.929}
\newcommand{\retCILVDflairBoundaryLTwoVarDecoderSegformerMlp}{0.021}
\newcommand{\nLVDflairBoundaryLTwoVarDecoderSegformerMlpLrMultOne}{5}
\newcommand{\miouLVDflairBoundaryLTwoVarDecoderSegformerMlpLrMultOne}{47.8}
\newcommand{\miouCILVDflairBoundaryLTwoVarDecoderSegformerMlpLrMultOne}{1.3}
\newcommand{\dropLVDflairBoundaryLTwoVarDecoderSegformerMlpLrMultOne}{4.2}
\newcommand{\dropCILVDflairBoundaryLTwoVarDecoderSegformerMlpLrMultOne}{1.2}
\newcommand{\retLVDflairBoundaryLTwoVarDecoderSegformerMlpLrMultOne}{0.920}
\newcommand{\retCILVDflairBoundaryLTwoVarDecoderSegformerMlpLrMultOne}{0.023}
\newcommand{\nLVDflairBoundaryLTwoVarLossBootstrap}{5}
\newcommand{\miouLVDflairBoundaryLTwoVarLossBootstrap}{46.9}
\newcommand{\miouCILVDflairBoundaryLTwoVarLossBootstrap}{0.7}
\newcommand{\dropLVDflairBoundaryLTwoVarLossBootstrap}{4.4}
\newcommand{\dropCILVDflairBoundaryLTwoVarLossBootstrap}{1.4}
\newcommand{\retLVDflairBoundaryLTwoVarLossBootstrap}{0.914}
\newcommand{\retCILVDflairBoundaryLTwoVarLossBootstrap}{0.027}
\newcommand{\nLVDflairBoundaryLTwoVarLossGce}{5}
\newcommand{\miouLVDflairBoundaryLTwoVarLossGce}{45.8}
\newcommand{\miouCILVDflairBoundaryLTwoVarLossGce}{0.8}
\newcommand{\dropLVDflairBoundaryLTwoVarLossGce}{4.5}
\newcommand{\dropCILVDflairBoundaryLTwoVarLossGce}{1.3}
\newcommand{\retLVDflairBoundaryLTwoVarLossGce}{0.910}
\newcommand{\retCILVDflairBoundaryLTwoVarLossGce}{0.025}
\newcommand{\nLVDflairBoundaryLTwoVarLrMultOne}{5}
\newcommand{\miouLVDflairBoundaryLTwoVarLrMultOne}{47.2}
\newcommand{\miouCILVDflairBoundaryLTwoVarLrMultOne}{1.7}
\newcommand{\dropLVDflairBoundaryLTwoVarLrMultOne}{3.9}
\newcommand{\dropCILVDflairBoundaryLTwoVarLrMultOne}{2.2}
\newcommand{\retLVDflairBoundaryLTwoVarLrMultOne}{0.924}
\newcommand{\retCILVDflairBoundaryLTwoVarLrMultOne}{0.041}
\newcommand{\nLVDflairBoundaryLR}{5}
\newcommand{\miouLVDflairBoundaryLR}{46.5}
\newcommand{\miouCILVDflairBoundaryLR}{0.5}
\newcommand{\dropLVDflairBoundaryLR}{4.3}
\newcommand{\dropCILVDflairBoundaryLR}{1.4}
\newcommand{\retLVDflairBoundaryLR}{0.916}
\newcommand{\retCILVDflairBoundaryLR}{0.025}
\newcommand{\nLVDflairBoundaryLRVarLrMultOne}{5}
\newcommand{\miouLVDflairBoundaryLRVarLrMultOne}{45.4}
\newcommand{\miouCILVDflairBoundaryLRVarLrMultOne}{1.6}
\newcommand{\dropLVDflairBoundaryLRVarLrMultOne}{5.7}
\newcommand{\dropCILVDflairBoundaryLRVarLrMultOne}{2.2}
\newcommand{\retLVDflairBoundaryLRVarLrMultOne}{0.888}
\newcommand{\retCILVDflairBoundaryLRVarLrMultOne}{0.042}
\newcommand{\nLVDflairClean}{8}
\newcommand{\miouLVDflairClean}{50.7}
\newcommand{\miouCILVDflairClean}{0.7}
\newcommand{\nLVDflairCleanVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouLVDflairCleanVarDecoderMaskTwoformerFull}{49.2}
\newcommand{\miouCILVDflairCleanVarDecoderMaskTwoformerFull}{0.7}
\newcommand{\nLVDflairCleanVarDecoderMaskTwoformerFullLrMultOne}{5}
\newcommand{\miouLVDflairCleanVarDecoderMaskTwoformerFullLrMultOne}{50.7}
\newcommand{\miouCILVDflairCleanVarDecoderMaskTwoformerFullLrMultOne}{0.5}
\newcommand{\nLVDflairCleanVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDflairCleanVarDecoderMaskTwoformerLite}{50.4}
\newcommand{\miouCILVDflairCleanVarDecoderMaskTwoformerLite}{0.6}
\newcommand{\nLVDflairCleanVarDecoderMaskTwoformerLiteLrMultOne}{5}
\newcommand{\miouLVDflairCleanVarDecoderMaskTwoformerLiteLrMultOne}{51.8}
\newcommand{\miouCILVDflairCleanVarDecoderMaskTwoformerLiteLrMultOne}{0.8}
\newcommand{\nLVDflairCleanVarDecoderSamLite}{5}
\newcommand{\miouLVDflairCleanVarDecoderSamLite}{46.2}
\newcommand{\miouCILVDflairCleanVarDecoderSamLite}{1.4}
\newcommand{\nLVDflairCleanVarDecoderSamLiteLrMultOne}{5}
\newcommand{\miouLVDflairCleanVarDecoderSamLiteLrMultOne}{48.8}
\newcommand{\miouCILVDflairCleanVarDecoderSamLiteLrMultOne}{0.8}
\newcommand{\nLVDflairCleanVarDecoderSamPretrained}{5}
\newcommand{\miouLVDflairCleanVarDecoderSamPretrained}{45.1}
\newcommand{\miouCILVDflairCleanVarDecoderSamPretrained}{1.5}
\newcommand{\nLVDflairCleanVarDecoderSamPretrainedLrMultOne}{5}
\newcommand{\miouLVDflairCleanVarDecoderSamPretrainedLrMultOne}{47.3}
\newcommand{\miouCILVDflairCleanVarDecoderSamPretrainedLrMultOne}{1.7}
\newcommand{\nLVDflairCleanVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDflairCleanVarDecoderSegformerMlp}{51.3}
\newcommand{\miouCILVDflairCleanVarDecoderSegformerMlp}{1.1}
\newcommand{\nLVDflairCleanVarDecoderSegformerMlpLrMultOne}{5}
\newcommand{\miouLVDflairCleanVarDecoderSegformerMlpLrMultOne}{52.0}
\newcommand{\miouCILVDflairCleanVarDecoderSegformerMlpLrMultOne}{0.7}
\newcommand{\nLVDflairCleanVarLossBootstrap}{5}
\newcommand{\miouLVDflairCleanVarLossBootstrap}{51.3}
\newcommand{\miouCILVDflairCleanVarLossBootstrap}{0.8}
\newcommand{\nLVDflairCleanVarLossGce}{5}
\newcommand{\miouLVDflairCleanVarLossGce}{50.4}
\newcommand{\miouCILVDflairCleanVarLossGce}{0.8}
\newcommand{\nLVDflairCleanVarLrMultOne}{5}
\newcommand{\miouLVDflairCleanVarLrMultOne}{51.2}
\newcommand{\miouCILVDflairCleanVarLrMultOne}{0.8}
\newcommand{\nLVDflairCleanVarLrMultThree}{1}
\newcommand{\miouLVDflairCleanVarLrMultThree}{49.9}
\newcommand{\miouCILVDflairCleanVarLrMultThree}{--}
\newcommand{\nLVDflairCleanVarTrainSubsetCleanTwoFive}{5}
\newcommand{\miouLVDflairCleanVarTrainSubsetCleanTwoFive}{46.5}
\newcommand{\miouCILVDflairCleanVarTrainSubsetCleanTwoFive}{1.2}
\newcommand{\nLVDflairCoarseLOne}{5}
\newcommand{\miouLVDflairCoarseLOne}{50.1}
\newcommand{\miouCILVDflairCoarseLOne}{0.9}
\newcommand{\dropLVDflairCoarseLOne}{0.7}
\newcommand{\dropCILVDflairCoarseLOne}{1.9}
\newcommand{\retLVDflairCoarseLOne}{0.987}
\newcommand{\retCILVDflairCoarseLOne}{0.036}
\newcommand{\nLVDflairCoarseLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouLVDflairCoarseLOneVarDecoderMaskTwoformerFull}{48.3}
\newcommand{\miouCILVDflairCoarseLOneVarDecoderMaskTwoformerFull}{1.0}
\newcommand{\dropLVDflairCoarseLOneVarDecoderMaskTwoformerFull}{0.8}
\newcommand{\dropCILVDflairCoarseLOneVarDecoderMaskTwoformerFull}{0.6}
\newcommand{\retLVDflairCoarseLOneVarDecoderMaskTwoformerFull}{0.983}
\newcommand{\retCILVDflairCoarseLOneVarDecoderMaskTwoformerFull}{0.012}
\newcommand{\nLVDflairCoarseLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDflairCoarseLOneVarDecoderMaskTwoformerLite}{49.4}
\newcommand{\miouCILVDflairCoarseLOneVarDecoderMaskTwoformerLite}{0.7}
\newcommand{\dropLVDflairCoarseLOneVarDecoderMaskTwoformerLite}{1.1}
\newcommand{\dropCILVDflairCoarseLOneVarDecoderMaskTwoformerLite}{0.8}
\newcommand{\retLVDflairCoarseLOneVarDecoderMaskTwoformerLite}{0.979}
\newcommand{\retCILVDflairCoarseLOneVarDecoderMaskTwoformerLite}{0.015}
\newcommand{\nLVDflairCoarseLOneVarDecoderSamLite}{5}
\newcommand{\miouLVDflairCoarseLOneVarDecoderSamLite}{45.3}
\newcommand{\miouCILVDflairCoarseLOneVarDecoderSamLite}{1.6}
\newcommand{\dropLVDflairCoarseLOneVarDecoderSamLite}{0.9}
\newcommand{\dropCILVDflairCoarseLOneVarDecoderSamLite}{0.5}
\newcommand{\retLVDflairCoarseLOneVarDecoderSamLite}{0.980}
\newcommand{\retCILVDflairCoarseLOneVarDecoderSamLite}{0.010}
\newcommand{\nLVDflairCoarseLOneVarDecoderSamPretrained}{5}
\newcommand{\miouLVDflairCoarseLOneVarDecoderSamPretrained}{44.2}
\newcommand{\miouCILVDflairCoarseLOneVarDecoderSamPretrained}{1.2}
\newcommand{\dropLVDflairCoarseLOneVarDecoderSamPretrained}{0.9}
\newcommand{\dropCILVDflairCoarseLOneVarDecoderSamPretrained}{0.4}
\newcommand{\retLVDflairCoarseLOneVarDecoderSamPretrained}{0.979}
\newcommand{\retCILVDflairCoarseLOneVarDecoderSamPretrained}{0.009}
\newcommand{\nLVDflairCoarseLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDflairCoarseLOneVarDecoderSegformerMlp}{50.3}
\newcommand{\miouCILVDflairCoarseLOneVarDecoderSegformerMlp}{0.8}
\newcommand{\dropLVDflairCoarseLOneVarDecoderSegformerMlp}{0.9}
\newcommand{\dropCILVDflairCoarseLOneVarDecoderSegformerMlp}{1.2}
\newcommand{\retLVDflairCoarseLOneVarDecoderSegformerMlp}{0.982}
\newcommand{\retCILVDflairCoarseLOneVarDecoderSegformerMlp}{0.024}
\newcommand{\nLVDflairCoarseLTwo}{8}
\newcommand{\miouLVDflairCoarseLTwo}{45.9}
\newcommand{\miouCILVDflairCoarseLTwo}{0.6}
\newcommand{\dropLVDflairCoarseLTwo}{4.8}
\newcommand{\dropCILVDflairCoarseLTwo}{1.0}
\newcommand{\retLVDflairCoarseLTwo}{0.906}
\newcommand{\retCILVDflairCoarseLTwo}{0.018}
\newcommand{\nLVDflairCoarseLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouLVDflairCoarseLTwoVarDecoderMaskTwoformerFull}{42.2}
\newcommand{\miouCILVDflairCoarseLTwoVarDecoderMaskTwoformerFull}{1.1}
\newcommand{\dropLVDflairCoarseLTwoVarDecoderMaskTwoformerFull}{7.0}
\newcommand{\dropCILVDflairCoarseLTwoVarDecoderMaskTwoformerFull}{1.0}
\newcommand{\retLVDflairCoarseLTwoVarDecoderMaskTwoformerFull}{0.858}
\newcommand{\retCILVDflairCoarseLTwoVarDecoderMaskTwoformerFull}{0.020}
\newcommand{\nLVDflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}{5}
\newcommand{\miouLVDflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}{43.5}
\newcommand{\miouCILVDflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}{1.5}
\newcommand{\dropLVDflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}{7.2}
\newcommand{\dropCILVDflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}{1.5}
\newcommand{\retLVDflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}{0.858}
\newcommand{\retCILVDflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}{0.029}
\newcommand{\nLVDflairCoarseLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDflairCoarseLTwoVarDecoderMaskTwoformerLite}{44.5}
\newcommand{\miouCILVDflairCoarseLTwoVarDecoderMaskTwoformerLite}{0.8}
\newcommand{\dropLVDflairCoarseLTwoVarDecoderMaskTwoformerLite}{6.0}
\newcommand{\dropCILVDflairCoarseLTwoVarDecoderMaskTwoformerLite}{1.0}
\newcommand{\retLVDflairCoarseLTwoVarDecoderMaskTwoformerLite}{0.881}
\newcommand{\retCILVDflairCoarseLTwoVarDecoderMaskTwoformerLite}{0.018}
\newcommand{\nLVDflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}{5}
\newcommand{\miouLVDflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}{45.2}
\newcommand{\miouCILVDflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}{1.2}
\newcommand{\dropLVDflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}{6.6}
\newcommand{\dropCILVDflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}{1.4}
\newcommand{\retLVDflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}{0.873}
\newcommand{\retCILVDflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}{0.026}
\newcommand{\nLVDflairCoarseLTwoVarDecoderSamLite}{5}
\newcommand{\miouLVDflairCoarseLTwoVarDecoderSamLite}{41.2}
\newcommand{\miouCILVDflairCoarseLTwoVarDecoderSamLite}{0.8}
\newcommand{\dropLVDflairCoarseLTwoVarDecoderSamLite}{4.9}
\newcommand{\dropCILVDflairCoarseLTwoVarDecoderSamLite}{1.2}
\newcommand{\retLVDflairCoarseLTwoVarDecoderSamLite}{0.893}
\newcommand{\retCILVDflairCoarseLTwoVarDecoderSamLite}{0.023}
\newcommand{\nLVDflairCoarseLTwoVarDecoderSamLiteLrMultOne}{5}
\newcommand{\miouLVDflairCoarseLTwoVarDecoderSamLiteLrMultOne}{42.9}
\newcommand{\miouCILVDflairCoarseLTwoVarDecoderSamLiteLrMultOne}{1.3}
\newcommand{\dropLVDflairCoarseLTwoVarDecoderSamLiteLrMultOne}{5.8}
\newcommand{\dropCILVDflairCoarseLTwoVarDecoderSamLiteLrMultOne}{1.4}
\newcommand{\retLVDflairCoarseLTwoVarDecoderSamLiteLrMultOne}{0.880}
\newcommand{\retCILVDflairCoarseLTwoVarDecoderSamLiteLrMultOne}{0.028}
\newcommand{\nLVDflairCoarseLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouLVDflairCoarseLTwoVarDecoderSamPretrained}{38.5}
\newcommand{\miouCILVDflairCoarseLTwoVarDecoderSamPretrained}{2.1}
\newcommand{\dropLVDflairCoarseLTwoVarDecoderSamPretrained}{6.7}
\newcommand{\dropCILVDflairCoarseLTwoVarDecoderSamPretrained}{1.4}
\newcommand{\retLVDflairCoarseLTwoVarDecoderSamPretrained}{0.852}
\newcommand{\retCILVDflairCoarseLTwoVarDecoderSamPretrained}{0.033}
\newcommand{\nLVDflairCoarseLTwoVarDecoderSamPretrainedLrMultOne}{5}
\newcommand{\miouLVDflairCoarseLTwoVarDecoderSamPretrainedLrMultOne}{42.5}
\newcommand{\miouCILVDflairCoarseLTwoVarDecoderSamPretrainedLrMultOne}{1.1}
\newcommand{\dropLVDflairCoarseLTwoVarDecoderSamPretrainedLrMultOne}{4.8}
\newcommand{\dropCILVDflairCoarseLTwoVarDecoderSamPretrainedLrMultOne}{2.1}
\newcommand{\retLVDflairCoarseLTwoVarDecoderSamPretrainedLrMultOne}{0.899}
\newcommand{\retCILVDflairCoarseLTwoVarDecoderSamPretrainedLrMultOne}{0.041}
\newcommand{\nLVDflairCoarseLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDflairCoarseLTwoVarDecoderSegformerMlp}{46.1}
\newcommand{\miouCILVDflairCoarseLTwoVarDecoderSegformerMlp}{0.5}
\newcommand{\dropLVDflairCoarseLTwoVarDecoderSegformerMlp}{5.2}
\newcommand{\dropCILVDflairCoarseLTwoVarDecoderSegformerMlp}{0.8}
\newcommand{\retLVDflairCoarseLTwoVarDecoderSegformerMlp}{0.900}
\newcommand{\retCILVDflairCoarseLTwoVarDecoderSegformerMlp}{0.013}
\newcommand{\nLVDflairCoarseLTwoVarDecoderSegformerMlpLrMultOne}{5}
\newcommand{\miouLVDflairCoarseLTwoVarDecoderSegformerMlpLrMultOne}{46.1}
\newcommand{\miouCILVDflairCoarseLTwoVarDecoderSegformerMlpLrMultOne}{1.5}
\newcommand{\dropLVDflairCoarseLTwoVarDecoderSegformerMlpLrMultOne}{5.8}
\newcommand{\dropCILVDflairCoarseLTwoVarDecoderSegformerMlpLrMultOne}{2.0}
\newcommand{\retLVDflairCoarseLTwoVarDecoderSegformerMlpLrMultOne}{0.888}
\newcommand{\retCILVDflairCoarseLTwoVarDecoderSegformerMlpLrMultOne}{0.037}
\newcommand{\nLVDflairCoarseLTwoVarLossBootstrap}{5}
\newcommand{\miouLVDflairCoarseLTwoVarLossBootstrap}{45.8}
\newcommand{\miouCILVDflairCoarseLTwoVarLossBootstrap}{0.8}
\newcommand{\dropLVDflairCoarseLTwoVarLossBootstrap}{5.5}
\newcommand{\dropCILVDflairCoarseLTwoVarLossBootstrap}{1.6}
\newcommand{\retLVDflairCoarseLTwoVarLossBootstrap}{0.893}
\newcommand{\retCILVDflairCoarseLTwoVarLossBootstrap}{0.029}
\newcommand{\nLVDflairCoarseLTwoVarLossGce}{5}
\newcommand{\miouLVDflairCoarseLTwoVarLossGce}{45.1}
\newcommand{\miouCILVDflairCoarseLTwoVarLossGce}{0.9}
\newcommand{\dropLVDflairCoarseLTwoVarLossGce}{5.3}
\newcommand{\dropCILVDflairCoarseLTwoVarLossGce}{0.2}
\newcommand{\retLVDflairCoarseLTwoVarLossGce}{0.895}
\newcommand{\retCILVDflairCoarseLTwoVarLossGce}{0.005}
\newcommand{\nLVDflairCoarseLTwoVarLrMultOne}{5}
\newcommand{\miouLVDflairCoarseLTwoVarLrMultOne}{45.4}
\newcommand{\miouCILVDflairCoarseLTwoVarLrMultOne}{0.5}
\newcommand{\dropLVDflairCoarseLTwoVarLrMultOne}{5.8}
\newcommand{\dropCILVDflairCoarseLTwoVarLrMultOne}{0.9}
\newcommand{\retLVDflairCoarseLTwoVarLrMultOne}{0.887}
\newcommand{\retCILVDflairCoarseLTwoVarLrMultOne}{0.016}
\newcommand{\nLVDflairCoarseLR}{5}
\newcommand{\miouLVDflairCoarseLR}{40.9}
\newcommand{\miouCILVDflairCoarseLR}{1.0}
\newcommand{\dropLVDflairCoarseLR}{10.0}
\newcommand{\dropCILVDflairCoarseLR}{1.9}
\newcommand{\retLVDflairCoarseLR}{0.804}
\newcommand{\retCILVDflairCoarseLR}{0.033}
\newcommand{\nLVDflairCoarseLRVarLrMultOne}{5}
\newcommand{\miouLVDflairCoarseLRVarLrMultOne}{40.6}
\newcommand{\miouCILVDflairCoarseLRVarLrMultOne}{1.2}
\newcommand{\dropLVDflairCoarseLRVarLrMultOne}{10.5}
\newcommand{\dropCILVDflairCoarseLRVarLrMultOne}{1.6}
\newcommand{\retLVDflairCoarseLRVarLrMultOne}{0.795}
\newcommand{\retCILVDflairCoarseLRVarLrMultOne}{0.029}
\newcommand{\nLVDflairOmissionLOne}{5}
\newcommand{\miouLVDflairOmissionLOne}{49.7}
\newcommand{\miouCILVDflairOmissionLOne}{1.1}
\newcommand{\dropLVDflairOmissionLOne}{1.2}
\newcommand{\dropCILVDflairOmissionLOne}{1.8}
\newcommand{\retLVDflairOmissionLOne}{0.978}
\newcommand{\retCILVDflairOmissionLOne}{0.034}
\newcommand{\nLVDflairOmissionLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouLVDflairOmissionLOneVarDecoderMaskTwoformerFull}{48.0}
\newcommand{\miouCILVDflairOmissionLOneVarDecoderMaskTwoformerFull}{1.4}
\newcommand{\dropLVDflairOmissionLOneVarDecoderMaskTwoformerFull}{1.2}
\newcommand{\dropCILVDflairOmissionLOneVarDecoderMaskTwoformerFull}{0.9}
\newcommand{\retLVDflairOmissionLOneVarDecoderMaskTwoformerFull}{0.975}
\newcommand{\retCILVDflairOmissionLOneVarDecoderMaskTwoformerFull}{0.019}
\newcommand{\nLVDflairOmissionLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDflairOmissionLOneVarDecoderMaskTwoformerLite}{48.7}
\newcommand{\miouCILVDflairOmissionLOneVarDecoderMaskTwoformerLite}{0.9}
\newcommand{\dropLVDflairOmissionLOneVarDecoderMaskTwoformerLite}{1.8}
\newcommand{\dropCILVDflairOmissionLOneVarDecoderMaskTwoformerLite}{1.0}
\newcommand{\retLVDflairOmissionLOneVarDecoderMaskTwoformerLite}{0.965}
\newcommand{\retCILVDflairOmissionLOneVarDecoderMaskTwoformerLite}{0.019}
\newcommand{\nLVDflairOmissionLOneVarDecoderSamLite}{5}
\newcommand{\miouLVDflairOmissionLOneVarDecoderSamLite}{44.3}
\newcommand{\miouCILVDflairOmissionLOneVarDecoderSamLite}{1.8}
\newcommand{\dropLVDflairOmissionLOneVarDecoderSamLite}{1.9}
\newcommand{\dropCILVDflairOmissionLOneVarDecoderSamLite}{0.7}
\newcommand{\retLVDflairOmissionLOneVarDecoderSamLite}{0.959}
\newcommand{\retCILVDflairOmissionLOneVarDecoderSamLite}{0.016}
\newcommand{\nLVDflairOmissionLOneVarDecoderSamPretrained}{5}
\newcommand{\miouLVDflairOmissionLOneVarDecoderSamPretrained}{43.4}
\newcommand{\miouCILVDflairOmissionLOneVarDecoderSamPretrained}{1.2}
\newcommand{\dropLVDflairOmissionLOneVarDecoderSamPretrained}{1.7}
\newcommand{\dropCILVDflairOmissionLOneVarDecoderSamPretrained}{0.7}
\newcommand{\retLVDflairOmissionLOneVarDecoderSamPretrained}{0.963}
\newcommand{\retCILVDflairOmissionLOneVarDecoderSamPretrained}{0.014}
\newcommand{\nLVDflairOmissionLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDflairOmissionLOneVarDecoderSegformerMlp}{50.0}
\newcommand{\miouCILVDflairOmissionLOneVarDecoderSegformerMlp}{0.8}
\newcommand{\dropLVDflairOmissionLOneVarDecoderSegformerMlp}{1.3}
\newcommand{\dropCILVDflairOmissionLOneVarDecoderSegformerMlp}{0.8}
\newcommand{\retLVDflairOmissionLOneVarDecoderSegformerMlp}{0.974}
\newcommand{\retCILVDflairOmissionLOneVarDecoderSegformerMlp}{0.015}
\newcommand{\nLVDflairOmissionLTwo}{8}
\newcommand{\miouLVDflairOmissionLTwo}{47.3}
\newcommand{\miouCILVDflairOmissionLTwo}{0.8}
\newcommand{\dropLVDflairOmissionLTwo}{3.4}
\newcommand{\dropCILVDflairOmissionLTwo}{1.4}
\newcommand{\retLVDflairOmissionLTwo}{0.932}
\newcommand{\retCILVDflairOmissionLTwo}{0.026}
\newcommand{\nLVDflairOmissionLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouLVDflairOmissionLTwoVarDecoderMaskTwoformerFull}{45.9}
\newcommand{\miouCILVDflairOmissionLTwoVarDecoderMaskTwoformerFull}{1.4}
\newcommand{\dropLVDflairOmissionLTwoVarDecoderMaskTwoformerFull}{3.3}
\newcommand{\dropCILVDflairOmissionLTwoVarDecoderMaskTwoformerFull}{1.0}
\newcommand{\retLVDflairOmissionLTwoVarDecoderMaskTwoformerFull}{0.932}
\newcommand{\retCILVDflairOmissionLTwoVarDecoderMaskTwoformerFull}{0.021}
\newcommand{\nLVDflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}{5}
\newcommand{\miouLVDflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}{48.6}
\newcommand{\miouCILVDflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}{1.2}
\newcommand{\dropLVDflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}{2.1}
\newcommand{\dropCILVDflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}{1.1}
\newcommand{\retLVDflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}{0.958}
\newcommand{\retCILVDflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}{0.021}
\newcommand{\nLVDflairOmissionLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDflairOmissionLTwoVarDecoderMaskTwoformerLite}{43.9}
\newcommand{\miouCILVDflairOmissionLTwoVarDecoderMaskTwoformerLite}{1.5}
\newcommand{\dropLVDflairOmissionLTwoVarDecoderMaskTwoformerLite}{6.6}
\newcommand{\dropCILVDflairOmissionLTwoVarDecoderMaskTwoformerLite}{1.6}
\newcommand{\retLVDflairOmissionLTwoVarDecoderMaskTwoformerLite}{0.870}
\newcommand{\retCILVDflairOmissionLTwoVarDecoderMaskTwoformerLite}{0.031}
\newcommand{\nLVDflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}{5}
\newcommand{\miouLVDflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}{46.2}
\newcommand{\miouCILVDflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}{0.9}
\newcommand{\dropLVDflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}{5.6}
\newcommand{\dropCILVDflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}{1.2}
\newcommand{\retLVDflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}{0.893}
\newcommand{\retCILVDflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}{0.022}
\newcommand{\nLVDflairOmissionLTwoVarDecoderSamLite}{5}
\newcommand{\miouLVDflairOmissionLTwoVarDecoderSamLite}{41.5}
\newcommand{\miouCILVDflairOmissionLTwoVarDecoderSamLite}{2.1}
\newcommand{\dropLVDflairOmissionLTwoVarDecoderSamLite}{4.6}
\newcommand{\dropCILVDflairOmissionLTwoVarDecoderSamLite}{1.4}
\newcommand{\retLVDflairOmissionLTwoVarDecoderSamLite}{0.900}
\newcommand{\retCILVDflairOmissionLTwoVarDecoderSamLite}{0.031}
\newcommand{\nLVDflairOmissionLTwoVarDecoderSamLiteLrMultOne}{5}
\newcommand{\miouLVDflairOmissionLTwoVarDecoderSamLiteLrMultOne}{44.5}
\newcommand{\miouCILVDflairOmissionLTwoVarDecoderSamLiteLrMultOne}{1.5}
\newcommand{\dropLVDflairOmissionLTwoVarDecoderSamLiteLrMultOne}{4.3}
\newcommand{\dropCILVDflairOmissionLTwoVarDecoderSamLiteLrMultOne}{2.1}
\newcommand{\retLVDflairOmissionLTwoVarDecoderSamLiteLrMultOne}{0.913}
\newcommand{\retCILVDflairOmissionLTwoVarDecoderSamLiteLrMultOne}{0.041}
\newcommand{\nLVDflairOmissionLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouLVDflairOmissionLTwoVarDecoderSamPretrained}{40.2}
\newcommand{\miouCILVDflairOmissionLTwoVarDecoderSamPretrained}{2.7}
\newcommand{\dropLVDflairOmissionLTwoVarDecoderSamPretrained}{4.9}
\newcommand{\dropCILVDflairOmissionLTwoVarDecoderSamPretrained}{1.6}
\newcommand{\retLVDflairOmissionLTwoVarDecoderSamPretrained}{0.891}
\newcommand{\retCILVDflairOmissionLTwoVarDecoderSamPretrained}{0.037}
\newcommand{\nLVDflairOmissionLTwoVarDecoderSamPretrainedLrMultOne}{5}
\newcommand{\miouLVDflairOmissionLTwoVarDecoderSamPretrainedLrMultOne}{42.4}
\newcommand{\miouCILVDflairOmissionLTwoVarDecoderSamPretrainedLrMultOne}{2.6}
\newcommand{\dropLVDflairOmissionLTwoVarDecoderSamPretrainedLrMultOne}{4.9}
\newcommand{\dropCILVDflairOmissionLTwoVarDecoderSamPretrainedLrMultOne}{2.0}
\newcommand{\retLVDflairOmissionLTwoVarDecoderSamPretrainedLrMultOne}{0.897}
\newcommand{\retCILVDflairOmissionLTwoVarDecoderSamPretrainedLrMultOne}{0.044}
\newcommand{\nLVDflairOmissionLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDflairOmissionLTwoVarDecoderSegformerMlp}{47.8}
\newcommand{\miouCILVDflairOmissionLTwoVarDecoderSegformerMlp}{0.6}
\newcommand{\dropLVDflairOmissionLTwoVarDecoderSegformerMlp}{3.5}
\newcommand{\dropCILVDflairOmissionLTwoVarDecoderSegformerMlp}{0.9}
\newcommand{\retLVDflairOmissionLTwoVarDecoderSegformerMlp}{0.932}
\newcommand{\retCILVDflairOmissionLTwoVarDecoderSegformerMlp}{0.017}
\newcommand{\nLVDflairOmissionLTwoVarDecoderSegformerMlpLrMultOne}{5}
\newcommand{\miouLVDflairOmissionLTwoVarDecoderSegformerMlpLrMultOne}{48.4}
\newcommand{\miouCILVDflairOmissionLTwoVarDecoderSegformerMlpLrMultOne}{1.2}
\newcommand{\dropLVDflairOmissionLTwoVarDecoderSegformerMlpLrMultOne}{3.6}
\newcommand{\dropCILVDflairOmissionLTwoVarDecoderSegformerMlpLrMultOne}{1.7}
\newcommand{\retLVDflairOmissionLTwoVarDecoderSegformerMlpLrMultOne}{0.932}
\newcommand{\retCILVDflairOmissionLTwoVarDecoderSegformerMlpLrMultOne}{0.033}
\newcommand{\nLVDflairOmissionLTwoVarLossBootstrap}{5}
\newcommand{\miouLVDflairOmissionLTwoVarLossBootstrap}{47.3}
\newcommand{\miouCILVDflairOmissionLTwoVarLossBootstrap}{1.2}
\newcommand{\dropLVDflairOmissionLTwoVarLossBootstrap}{4.0}
\newcommand{\dropCILVDflairOmissionLTwoVarLossBootstrap}{1.5}
\newcommand{\retLVDflairOmissionLTwoVarLossBootstrap}{0.922}
\newcommand{\retCILVDflairOmissionLTwoVarLossBootstrap}{0.028}
\newcommand{\nLVDflairOmissionLTwoVarLossGce}{5}
\newcommand{\miouLVDflairOmissionLTwoVarLossGce}{46.4}
\newcommand{\miouCILVDflairOmissionLTwoVarLossGce}{2.6}
\newcommand{\dropLVDflairOmissionLTwoVarLossGce}{4.0}
\newcommand{\dropCILVDflairOmissionLTwoVarLossGce}{3.2}
\newcommand{\retLVDflairOmissionLTwoVarLossGce}{0.921}
\newcommand{\retCILVDflairOmissionLTwoVarLossGce}{0.062}
\newcommand{\nLVDflairOmissionLTwoVarLrMultZeroOneOneOneOne}{2}
\newcommand{\miouLVDflairOmissionLTwoVarLrMultZeroOneOneOneOne}{45.8}
\newcommand{\miouCILVDflairOmissionLTwoVarLrMultZeroOneOneOneOne}{0.8}
\newcommand{\dropLVDflairOmissionLTwoVarLrMultZeroOneOneOneOne}{5.9}
\newcommand{\dropCILVDflairOmissionLTwoVarLrMultZeroOneOneOneOne}{1.3}
\newcommand{\retLVDflairOmissionLTwoVarLrMultZeroOneOneOneOne}{0.885}
\newcommand{\retCILVDflairOmissionLTwoVarLrMultZeroOneOneOneOne}{0.020}
\newcommand{\nLVDflairOmissionLTwoVarLrMultOne}{5}
\newcommand{\miouLVDflairOmissionLTwoVarLrMultOne}{47.7}
\newcommand{\miouCILVDflairOmissionLTwoVarLrMultOne}{1.4}
\newcommand{\dropLVDflairOmissionLTwoVarLrMultOne}{3.5}
\newcommand{\dropCILVDflairOmissionLTwoVarLrMultOne}{1.7}
\newcommand{\retLVDflairOmissionLTwoVarLrMultOne}{0.932}
\newcommand{\retCILVDflairOmissionLTwoVarLrMultOne}{0.032}
\newcommand{\nLVDflairOmissionLR}{5}
\newcommand{\miouLVDflairOmissionLR}{44.8}
\newcommand{\miouCILVDflairOmissionLR}{1.2}
\newcommand{\dropLVDflairOmissionLR}{6.1}
\newcommand{\dropCILVDflairOmissionLR}{2.0}
\newcommand{\retLVDflairOmissionLR}{0.881}
\newcommand{\retCILVDflairOmissionLR}{0.038}
\newcommand{\nLVDflairOmissionLRVarLrMultOne}{5}
\newcommand{\miouLVDflairOmissionLRVarLrMultOne}{44.6}
\newcommand{\miouCILVDflairOmissionLRVarLrMultOne}{1.2}
\newcommand{\dropLVDflairOmissionLRVarLrMultOne}{6.6}
\newcommand{\dropCILVDflairOmissionLRVarLrMultOne}{1.6}
\newcommand{\retLVDflairOmissionLRVarLrMultOne}{0.871}
\newcommand{\retCILVDflairOmissionLRVarLrMultOne}{0.029}
\newcommand{\nLVDflairShiftLOne}{5}
\newcommand{\miouLVDflairShiftLOne}{50.5}
\newcommand{\miouCILVDflairShiftLOne}{1.0}
\newcommand{\dropLVDflairShiftLOne}{0.3}
\newcommand{\dropCILVDflairShiftLOne}{1.7}
\newcommand{\retLVDflairShiftLOne}{0.995}
\newcommand{\retCILVDflairShiftLOne}{0.033}
\newcommand{\nLVDflairShiftLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouLVDflairShiftLOneVarDecoderMaskTwoformerFull}{48.5}
\newcommand{\miouCILVDflairShiftLOneVarDecoderMaskTwoformerFull}{1.4}
\newcommand{\dropLVDflairShiftLOneVarDecoderMaskTwoformerFull}{0.6}
\newcommand{\dropCILVDflairShiftLOneVarDecoderMaskTwoformerFull}{0.8}
\newcommand{\retLVDflairShiftLOneVarDecoderMaskTwoformerFull}{0.987}
\newcommand{\retCILVDflairShiftLOneVarDecoderMaskTwoformerFull}{0.017}
\newcommand{\nLVDflairShiftLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDflairShiftLOneVarDecoderMaskTwoformerLite}{49.7}
\newcommand{\miouCILVDflairShiftLOneVarDecoderMaskTwoformerLite}{0.7}
\newcommand{\dropLVDflairShiftLOneVarDecoderMaskTwoformerLite}{0.8}
\newcommand{\dropCILVDflairShiftLOneVarDecoderMaskTwoformerLite}{0.6}
\newcommand{\retLVDflairShiftLOneVarDecoderMaskTwoformerLite}{0.985}
\newcommand{\retCILVDflairShiftLOneVarDecoderMaskTwoformerLite}{0.013}
\newcommand{\nLVDflairShiftLOneVarDecoderSamLite}{5}
\newcommand{\miouLVDflairShiftLOneVarDecoderSamLite}{45.5}
\newcommand{\miouCILVDflairShiftLOneVarDecoderSamLite}{1.4}
\newcommand{\dropLVDflairShiftLOneVarDecoderSamLite}{0.6}
\newcommand{\dropCILVDflairShiftLOneVarDecoderSamLite}{1.0}
\newcommand{\retLVDflairShiftLOneVarDecoderSamLite}{0.986}
\newcommand{\retCILVDflairShiftLOneVarDecoderSamLite}{0.021}
\newcommand{\nLVDflairShiftLOneVarDecoderSamPretrained}{5}
\newcommand{\miouLVDflairShiftLOneVarDecoderSamPretrained}{44.3}
\newcommand{\miouCILVDflairShiftLOneVarDecoderSamPretrained}{1.4}
\newcommand{\dropLVDflairShiftLOneVarDecoderSamPretrained}{0.8}
\newcommand{\dropCILVDflairShiftLOneVarDecoderSamPretrained}{1.3}
\newcommand{\retLVDflairShiftLOneVarDecoderSamPretrained}{0.982}
\newcommand{\retCILVDflairShiftLOneVarDecoderSamPretrained}{0.028}
\newcommand{\nLVDflairShiftLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDflairShiftLOneVarDecoderSegformerMlp}{50.4}
\newcommand{\miouCILVDflairShiftLOneVarDecoderSegformerMlp}{0.9}
\newcommand{\dropLVDflairShiftLOneVarDecoderSegformerMlp}{0.9}
\newcommand{\dropCILVDflairShiftLOneVarDecoderSegformerMlp}{1.3}
\newcommand{\retLVDflairShiftLOneVarDecoderSegformerMlp}{0.983}
\newcommand{\retCILVDflairShiftLOneVarDecoderSegformerMlp}{0.026}
\newcommand{\nLVDflairShiftLTwo}{8}
\newcommand{\miouLVDflairShiftLTwo}{48.9}
\newcommand{\miouCILVDflairShiftLTwo}{0.6}
\newcommand{\dropLVDflairShiftLTwo}{1.8}
\newcommand{\dropCILVDflairShiftLTwo}{0.6}
\newcommand{\retLVDflairShiftLTwo}{0.964}
\newcommand{\retCILVDflairShiftLTwo}{0.012}
\newcommand{\nLVDflairShiftLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouLVDflairShiftLTwoVarDecoderMaskTwoformerFull}{46.1}
\newcommand{\miouCILVDflairShiftLTwoVarDecoderMaskTwoformerFull}{0.5}
\newcommand{\dropLVDflairShiftLTwoVarDecoderMaskTwoformerFull}{3.0}
\newcommand{\dropCILVDflairShiftLTwoVarDecoderMaskTwoformerFull}{0.7}
\newcommand{\retLVDflairShiftLTwoVarDecoderMaskTwoformerFull}{0.938}
\newcommand{\retCILVDflairShiftLTwoVarDecoderMaskTwoformerFull}{0.013}
\newcommand{\nLVDflairShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}{5}
\newcommand{\miouLVDflairShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}{46.8}
\newcommand{\miouCILVDflairShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}{1.0}
\newcommand{\dropLVDflairShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}{3.9}
\newcommand{\dropCILVDflairShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}{1.3}
\newcommand{\retLVDflairShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}{0.923}
\newcommand{\retCILVDflairShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}{0.025}
\newcommand{\nLVDflairShiftLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDflairShiftLTwoVarDecoderMaskTwoformerLite}{47.1}
\newcommand{\miouCILVDflairShiftLTwoVarDecoderMaskTwoformerLite}{0.9}
\newcommand{\dropLVDflairShiftLTwoVarDecoderMaskTwoformerLite}{3.4}
\newcommand{\dropCILVDflairShiftLTwoVarDecoderMaskTwoformerLite}{1.2}
\newcommand{\retLVDflairShiftLTwoVarDecoderMaskTwoformerLite}{0.933}
\newcommand{\retCILVDflairShiftLTwoVarDecoderMaskTwoformerLite}{0.023}
\newcommand{\nLVDflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}{5}
\newcommand{\miouLVDflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}{47.6}
\newcommand{\miouCILVDflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}{0.9}
\newcommand{\dropLVDflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}{4.1}
\newcommand{\dropCILVDflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}{0.7}
\newcommand{\retLVDflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}{0.920}
\newcommand{\retCILVDflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}{0.014}
\newcommand{\nLVDflairShiftLTwoVarDecoderSamLite}{5}
\newcommand{\miouLVDflairShiftLTwoVarDecoderSamLite}{43.1}
\newcommand{\miouCILVDflairShiftLTwoVarDecoderSamLite}{0.6}
\newcommand{\dropLVDflairShiftLTwoVarDecoderSamLite}{3.0}
\newcommand{\dropCILVDflairShiftLTwoVarDecoderSamLite}{0.8}
\newcommand{\retLVDflairShiftLTwoVarDecoderSamLite}{0.935}
\newcommand{\retCILVDflairShiftLTwoVarDecoderSamLite}{0.016}
\newcommand{\nLVDflairShiftLTwoVarDecoderSamLiteLrMultOne}{5}
\newcommand{\miouLVDflairShiftLTwoVarDecoderSamLiteLrMultOne}{44.6}
\newcommand{\miouCILVDflairShiftLTwoVarDecoderSamLiteLrMultOne}{0.4}
\newcommand{\dropLVDflairShiftLTwoVarDecoderSamLiteLrMultOne}{4.2}
\newcommand{\dropCILVDflairShiftLTwoVarDecoderSamLiteLrMultOne}{0.8}
\newcommand{\retLVDflairShiftLTwoVarDecoderSamLiteLrMultOne}{0.915}
\newcommand{\retCILVDflairShiftLTwoVarDecoderSamLiteLrMultOne}{0.015}
\newcommand{\nLVDflairShiftLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouLVDflairShiftLTwoVarDecoderSamPretrained}{41.1}
\newcommand{\miouCILVDflairShiftLTwoVarDecoderSamPretrained}{2.1}
\newcommand{\dropLVDflairShiftLTwoVarDecoderSamPretrained}{4.0}
\newcommand{\dropCILVDflairShiftLTwoVarDecoderSamPretrained}{2.1}
\newcommand{\retLVDflairShiftLTwoVarDecoderSamPretrained}{0.912}
\newcommand{\retCILVDflairShiftLTwoVarDecoderSamPretrained}{0.045}
\newcommand{\nLVDflairShiftLTwoVarDecoderSamPretrainedLrMultOne}{5}
\newcommand{\miouLVDflairShiftLTwoVarDecoderSamPretrainedLrMultOne}{43.3}
\newcommand{\miouCILVDflairShiftLTwoVarDecoderSamPretrainedLrMultOne}{0.5}
\newcommand{\dropLVDflairShiftLTwoVarDecoderSamPretrainedLrMultOne}{4.0}
\newcommand{\dropCILVDflairShiftLTwoVarDecoderSamPretrainedLrMultOne}{2.0}
\newcommand{\retLVDflairShiftLTwoVarDecoderSamPretrainedLrMultOne}{0.917}
\newcommand{\retCILVDflairShiftLTwoVarDecoderSamPretrainedLrMultOne}{0.039}
\newcommand{\nLVDflairShiftLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDflairShiftLTwoVarDecoderSegformerMlp}{48.9}
\newcommand{\miouCILVDflairShiftLTwoVarDecoderSegformerMlp}{0.8}
\newcommand{\dropLVDflairShiftLTwoVarDecoderSegformerMlp}{2.4}
\newcommand{\dropCILVDflairShiftLTwoVarDecoderSegformerMlp}{1.5}
\newcommand{\retLVDflairShiftLTwoVarDecoderSegformerMlp}{0.953}
\newcommand{\retCILVDflairShiftLTwoVarDecoderSegformerMlp}{0.028}
\newcommand{\nLVDflairShiftLTwoVarDecoderSegformerMlpLrMultOne}{5}
\newcommand{\miouLVDflairShiftLTwoVarDecoderSegformerMlpLrMultOne}{49.1}
\newcommand{\miouCILVDflairShiftLTwoVarDecoderSegformerMlpLrMultOne}{0.4}
\newcommand{\dropLVDflairShiftLTwoVarDecoderSegformerMlpLrMultOne}{2.9}
\newcommand{\dropCILVDflairShiftLTwoVarDecoderSegformerMlpLrMultOne}{0.6}
\newcommand{\retLVDflairShiftLTwoVarDecoderSegformerMlpLrMultOne}{0.945}
\newcommand{\retCILVDflairShiftLTwoVarDecoderSegformerMlpLrMultOne}{0.011}
\newcommand{\nLVDflairShiftLTwoVarLossBootstrap}{5}
\newcommand{\miouLVDflairShiftLTwoVarLossBootstrap}{48.6}
\newcommand{\miouCILVDflairShiftLTwoVarLossBootstrap}{0.7}
\newcommand{\dropLVDflairShiftLTwoVarLossBootstrap}{2.7}
\newcommand{\dropCILVDflairShiftLTwoVarLossBootstrap}{1.2}
\newcommand{\retLVDflairShiftLTwoVarLossBootstrap}{0.948}
\newcommand{\retCILVDflairShiftLTwoVarLossBootstrap}{0.022}
\newcommand{\nLVDflairShiftLTwoVarLossGce}{5}
\newcommand{\miouLVDflairShiftLTwoVarLossGce}{47.2}
\newcommand{\miouCILVDflairShiftLTwoVarLossGce}{1.7}
\newcommand{\dropLVDflairShiftLTwoVarLossGce}{3.2}
\newcommand{\dropCILVDflairShiftLTwoVarLossGce}{1.9}
\newcommand{\retLVDflairShiftLTwoVarLossGce}{0.936}
\newcommand{\retCILVDflairShiftLTwoVarLossGce}{0.037}
\newcommand{\nLVDflairShiftLTwoVarLrMultOne}{5}
\newcommand{\miouLVDflairShiftLTwoVarLrMultOne}{48.4}
\newcommand{\miouCILVDflairShiftLTwoVarLrMultOne}{0.2}
\newcommand{\dropLVDflairShiftLTwoVarLrMultOne}{2.7}
\newcommand{\dropCILVDflairShiftLTwoVarLrMultOne}{0.6}
\newcommand{\retLVDflairShiftLTwoVarLrMultOne}{0.947}
\newcommand{\retCILVDflairShiftLTwoVarLrMultOne}{0.010}
\newcommand{\nLVDflairShiftLR}{5}
\newcommand{\miouLVDflairShiftLR}{45.7}
\newcommand{\miouCILVDflairShiftLR}{0.5}
\newcommand{\dropLVDflairShiftLR}{5.1}
\newcommand{\dropCILVDflairShiftLR}{1.4}
\newcommand{\retLVDflairShiftLR}{0.900}
\newcommand{\retCILVDflairShiftLR}{0.026}
\newcommand{\nLVDflairShiftLRVarLrMultOne}{5}
\newcommand{\miouLVDflairShiftLRVarLrMultOne}{44.6}
\newcommand{\miouCILVDflairShiftLRVarLrMultOne}{1.1}
\newcommand{\dropLVDflairShiftLRVarLrMultOne}{6.6}
\newcommand{\dropCILVDflairShiftLRVarLrMultOne}{1.4}
\newcommand{\retLVDflairShiftLRVarLrMultOne}{0.871}
\newcommand{\retCILVDflairShiftLRVarLrMultOne}{0.025}
\newcommand{\nLVDKuroBoundaryLOne}{5}
\newcommand{\miouLVDKuroBoundaryLOne}{57.5}
\newcommand{\miouCILVDKuroBoundaryLOne}{0.8}
\newcommand{\dropLVDKuroBoundaryLOne}{2.3}
\newcommand{\dropCILVDKuroBoundaryLOne}{2.5}
\newcommand{\retLVDKuroBoundaryLOne}{0.962}
\newcommand{\retCILVDKuroBoundaryLOne}{0.041}
\newcommand{\nLVDKuroBoundaryLTwo}{5}
\newcommand{\miouLVDKuroBoundaryLTwo}{51.7}
\newcommand{\miouCILVDKuroBoundaryLTwo}{1.6}
\newcommand{\dropLVDKuroBoundaryLTwo}{8.1}
\newcommand{\dropCILVDKuroBoundaryLTwo}{1.0}
\newcommand{\retLVDKuroBoundaryLTwo}{0.865}
\newcommand{\retCILVDKuroBoundaryLTwo}{0.013}
\newcommand{\nLVDKuroBoundaryLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDKuroBoundaryLTwoVarDecoderMaskTwoformerLite}{49.0}
\newcommand{\miouCILVDKuroBoundaryLTwoVarDecoderMaskTwoformerLite}{2.3}
\newcommand{\dropLVDKuroBoundaryLTwoVarDecoderMaskTwoformerLite}{3.6}
\newcommand{\dropCILVDKuroBoundaryLTwoVarDecoderMaskTwoformerLite}{3.6}
\newcommand{\retLVDKuroBoundaryLTwoVarDecoderMaskTwoformerLite}{0.932}
\newcommand{\retCILVDKuroBoundaryLTwoVarDecoderMaskTwoformerLite}{0.065}
\newcommand{\nLVDKuroBoundaryLTwoVarDecoderSamLite}{5}
\newcommand{\miouLVDKuroBoundaryLTwoVarDecoderSamLite}{51.7}
\newcommand{\miouCILVDKuroBoundaryLTwoVarDecoderSamLite}{4.7}
\newcommand{\dropLVDKuroBoundaryLTwoVarDecoderSamLite}{9.2}
\newcommand{\dropCILVDKuroBoundaryLTwoVarDecoderSamLite}{4.7}
\newcommand{\retLVDKuroBoundaryLTwoVarDecoderSamLite}{0.849}
\newcommand{\retCILVDKuroBoundaryLTwoVarDecoderSamLite}{0.077}
\newcommand{\nLVDKuroBoundaryLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDKuroBoundaryLTwoVarDecoderSegformerMlp}{51.9}
\newcommand{\miouCILVDKuroBoundaryLTwoVarDecoderSegformerMlp}{2.9}
\newcommand{\dropLVDKuroBoundaryLTwoVarDecoderSegformerMlp}{5.5}
\newcommand{\dropCILVDKuroBoundaryLTwoVarDecoderSegformerMlp}{2.4}
\newcommand{\retLVDKuroBoundaryLTwoVarDecoderSegformerMlp}{0.905}
\newcommand{\retCILVDKuroBoundaryLTwoVarDecoderSegformerMlp}{0.042}
\newcommand{\nLVDKuroBoundaryLTwoVarLrMultOne}{5}
\newcommand{\miouLVDKuroBoundaryLTwoVarLrMultOne}{47.5}
\newcommand{\miouCILVDKuroBoundaryLTwoVarLrMultOne}{2.3}
\newcommand{\dropLVDKuroBoundaryLTwoVarLrMultOne}{6.8}
\newcommand{\dropCILVDKuroBoundaryLTwoVarLrMultOne}{3.8}
\newcommand{\retLVDKuroBoundaryLTwoVarLrMultOne}{0.877}
\newcommand{\retCILVDKuroBoundaryLTwoVarLrMultOne}{0.065}
\newcommand{\nLVDKuroCemsREALVarTrainSubsetRealcov}{5}
\newcommand{\miouLVDKuroCemsREALVarTrainSubsetRealcov}{51.0}
\newcommand{\miouCILVDKuroCemsREALVarTrainSubsetRealcov}{1.9}
\newcommand{\dropLVDKuroCemsREALVarTrainSubsetRealcov}{2.4}
\newcommand{\dropCILVDKuroCemsREALVarTrainSubsetRealcov}{2.8}
\newcommand{\retLVDKuroCemsREALVarTrainSubsetRealcov}{0.955}
\newcommand{\retCILVDKuroCemsREALVarTrainSubsetRealcov}{0.050}
\newcommand{\nLVDKuroClean}{5}
\newcommand{\miouLVDKuroClean}{59.8}
\newcommand{\miouCILVDKuroClean}{2.4}
\newcommand{\nLVDKuroCleanVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDKuroCleanVarDecoderMaskTwoformerLite}{52.7}
\newcommand{\miouCILVDKuroCleanVarDecoderMaskTwoformerLite}{2.7}
\newcommand{\nLVDKuroCleanVarDecoderSamLite}{5}
\newcommand{\miouLVDKuroCleanVarDecoderSamLite}{61.0}
\newcommand{\miouCILVDKuroCleanVarDecoderSamLite}{0.8}
\newcommand{\nLVDKuroCleanVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDKuroCleanVarDecoderSegformerMlp}{57.3}
\newcommand{\miouCILVDKuroCleanVarDecoderSegformerMlp}{1.4}
\newcommand{\nLVDKuroCleanVarLrMultOne}{5}
\newcommand{\miouLVDKuroCleanVarLrMultOne}{54.3}
\newcommand{\miouCILVDKuroCleanVarLrMultOne}{3.8}
\newcommand{\nLVDKuroCleanVarTrainSubsetRealcov}{5}
\newcommand{\miouLVDKuroCleanVarTrainSubsetRealcov}{53.4}
\newcommand{\miouCILVDKuroCleanVarTrainSubsetRealcov}{1.9}
\newcommand{\nLVDKuroCoarseLOne}{5}
\newcommand{\miouLVDKuroCoarseLOne}{57.4}
\newcommand{\miouCILVDKuroCoarseLOne}{5.2}
\newcommand{\dropLVDKuroCoarseLOne}{2.4}
\newcommand{\dropCILVDKuroCoarseLOne}{5.9}
\newcommand{\retLVDKuroCoarseLOne}{0.960}
\newcommand{\retCILVDKuroCoarseLOne}{0.098}
\newcommand{\nLVDKuroCoarseLTwo}{5}
\newcommand{\miouLVDKuroCoarseLTwo}{50.7}
\newcommand{\miouCILVDKuroCoarseLTwo}{2.2}
\newcommand{\dropLVDKuroCoarseLTwo}{9.1}
\newcommand{\dropCILVDKuroCoarseLTwo}{3.9}
\newcommand{\retLVDKuroCoarseLTwo}{0.849}
\newcommand{\retCILVDKuroCoarseLTwo}{0.060}
\newcommand{\nLVDKuroCoarseLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDKuroCoarseLTwoVarDecoderMaskTwoformerLite}{46.2}
\newcommand{\miouCILVDKuroCoarseLTwoVarDecoderMaskTwoformerLite}{2.4}
\newcommand{\dropLVDKuroCoarseLTwoVarDecoderMaskTwoformerLite}{6.4}
\newcommand{\dropCILVDKuroCoarseLTwoVarDecoderMaskTwoformerLite}{2.4}
\newcommand{\retLVDKuroCoarseLTwoVarDecoderMaskTwoformerLite}{0.879}
\newcommand{\retCILVDKuroCoarseLTwoVarDecoderMaskTwoformerLite}{0.043}
\newcommand{\nLVDKuroCoarseLTwoVarDecoderSamLite}{5}
\newcommand{\miouLVDKuroCoarseLTwoVarDecoderSamLite}{50.3}
\newcommand{\miouCILVDKuroCoarseLTwoVarDecoderSamLite}{1.0}
\newcommand{\dropLVDKuroCoarseLTwoVarDecoderSamLite}{10.6}
\newcommand{\dropCILVDKuroCoarseLTwoVarDecoderSamLite}{1.4}
\newcommand{\retLVDKuroCoarseLTwoVarDecoderSamLite}{0.826}
\newcommand{\retCILVDKuroCoarseLTwoVarDecoderSamLite}{0.021}
\newcommand{\nLVDKuroCoarseLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDKuroCoarseLTwoVarDecoderSegformerMlp}{51.0}
\newcommand{\miouCILVDKuroCoarseLTwoVarDecoderSegformerMlp}{2.1}
\newcommand{\dropLVDKuroCoarseLTwoVarDecoderSegformerMlp}{6.4}
\newcommand{\dropCILVDKuroCoarseLTwoVarDecoderSegformerMlp}{2.0}
\newcommand{\retLVDKuroCoarseLTwoVarDecoderSegformerMlp}{0.889}
\newcommand{\retCILVDKuroCoarseLTwoVarDecoderSegformerMlp}{0.034}
\newcommand{\nLVDKuroCoarseLTwoVarLrMultOne}{5}
\newcommand{\miouLVDKuroCoarseLTwoVarLrMultOne}{45.0}
\newcommand{\miouCILVDKuroCoarseLTwoVarLrMultOne}{3.6}
\newcommand{\dropLVDKuroCoarseLTwoVarLrMultOne}{9.2}
\newcommand{\dropCILVDKuroCoarseLTwoVarLrMultOne}{4.4}
\newcommand{\retLVDKuroCoarseLTwoVarLrMultOne}{0.831}
\newcommand{\retCILVDKuroCoarseLTwoVarLrMultOne}{0.073}
\newcommand{\nLVDKuroOmissionLOne}{5}
\newcommand{\miouLVDKuroOmissionLOne}{57.7}
\newcommand{\miouCILVDKuroOmissionLOne}{2.3}
\newcommand{\dropLVDKuroOmissionLOne}{2.0}
\newcommand{\dropCILVDKuroOmissionLOne}{3.0}
\newcommand{\retLVDKuroOmissionLOne}{0.966}
\newcommand{\retCILVDKuroOmissionLOne}{0.051}
\newcommand{\nLVDKuroOmissionLTwo}{5}
\newcommand{\miouLVDKuroOmissionLTwo}{50.8}
\newcommand{\miouCILVDKuroOmissionLTwo}{4.0}
\newcommand{\dropLVDKuroOmissionLTwo}{9.0}
\newcommand{\dropCILVDKuroOmissionLTwo}{2.7}
\newcommand{\retLVDKuroOmissionLTwo}{0.849}
\newcommand{\retCILVDKuroOmissionLTwo}{0.046}
\newcommand{\nLVDKuroOmissionLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDKuroOmissionLTwoVarDecoderMaskTwoformerLite}{41.4}
\newcommand{\miouCILVDKuroOmissionLTwoVarDecoderMaskTwoformerLite}{1.4}
\newcommand{\dropLVDKuroOmissionLTwoVarDecoderMaskTwoformerLite}{11.3}
\newcommand{\dropCILVDKuroOmissionLTwoVarDecoderMaskTwoformerLite}{2.9}
\newcommand{\retLVDKuroOmissionLTwoVarDecoderMaskTwoformerLite}{0.787}
\newcommand{\retCILVDKuroOmissionLTwoVarDecoderMaskTwoformerLite}{0.045}
\newcommand{\nLVDKuroOmissionLTwoVarDecoderSamLite}{5}
\newcommand{\miouLVDKuroOmissionLTwoVarDecoderSamLite}{49.6}
\newcommand{\miouCILVDKuroOmissionLTwoVarDecoderSamLite}{2.0}
\newcommand{\dropLVDKuroOmissionLTwoVarDecoderSamLite}{11.3}
\newcommand{\dropCILVDKuroOmissionLTwoVarDecoderSamLite}{2.3}
\newcommand{\retLVDKuroOmissionLTwoVarDecoderSamLite}{0.814}
\newcommand{\retCILVDKuroOmissionLTwoVarDecoderSamLite}{0.037}
\newcommand{\nLVDKuroOmissionLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDKuroOmissionLTwoVarDecoderSegformerMlp}{47.7}
\newcommand{\miouCILVDKuroOmissionLTwoVarDecoderSegformerMlp}{3.6}
\newcommand{\dropLVDKuroOmissionLTwoVarDecoderSegformerMlp}{9.6}
\newcommand{\dropCILVDKuroOmissionLTwoVarDecoderSegformerMlp}{3.5}
\newcommand{\retLVDKuroOmissionLTwoVarDecoderSegformerMlp}{0.833}
\newcommand{\retCILVDKuroOmissionLTwoVarDecoderSegformerMlp}{0.061}
\newcommand{\nLVDKuroOmissionLTwoVarLrMultOne}{5}
\newcommand{\miouLVDKuroOmissionLTwoVarLrMultOne}{43.8}
\newcommand{\miouCILVDKuroOmissionLTwoVarLrMultOne}{2.9}
\newcommand{\dropLVDKuroOmissionLTwoVarLrMultOne}{10.5}
\newcommand{\dropCILVDKuroOmissionLTwoVarLrMultOne}{3.7}
\newcommand{\retLVDKuroOmissionLTwoVarLrMultOne}{0.808}
\newcommand{\retCILVDKuroOmissionLTwoVarLrMultOne}{0.058}
\newcommand{\nLVDKuroShiftLOne}{5}
\newcommand{\miouLVDKuroShiftLOne}{58.5}
\newcommand{\miouCILVDKuroShiftLOne}{1.5}
\newcommand{\dropLVDKuroShiftLOne}{1.3}
\newcommand{\dropCILVDKuroShiftLOne}{2.7}
\newcommand{\retLVDKuroShiftLOne}{0.979}
\newcommand{\retCILVDKuroShiftLOne}{0.044}
\newcommand{\nLVDKuroShiftLTwo}{5}
\newcommand{\miouLVDKuroShiftLTwo}{56.2}
\newcommand{\miouCILVDKuroShiftLTwo}{1.6}
\newcommand{\dropLVDKuroShiftLTwo}{3.6}
\newcommand{\dropCILVDKuroShiftLTwo}{3.1}
\newcommand{\retLVDKuroShiftLTwo}{0.941}
\newcommand{\retCILVDKuroShiftLTwo}{0.052}
\newcommand{\nLVDKuroShiftLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDKuroShiftLTwoVarDecoderMaskTwoformerLite}{51.6}
\newcommand{\miouCILVDKuroShiftLTwoVarDecoderMaskTwoformerLite}{1.2}
\newcommand{\dropLVDKuroShiftLTwoVarDecoderMaskTwoformerLite}{1.1}
\newcommand{\dropCILVDKuroShiftLTwoVarDecoderMaskTwoformerLite}{3.4}
\newcommand{\retLVDKuroShiftLTwoVarDecoderMaskTwoformerLite}{0.981}
\newcommand{\retCILVDKuroShiftLTwoVarDecoderMaskTwoformerLite}{0.064}
\newcommand{\nLVDKuroShiftLTwoVarDecoderSamLite}{5}
\newcommand{\miouLVDKuroShiftLTwoVarDecoderSamLite}{53.9}
\newcommand{\miouCILVDKuroShiftLTwoVarDecoderSamLite}{0.8}
\newcommand{\dropLVDKuroShiftLTwoVarDecoderSamLite}{7.1}
\newcommand{\dropCILVDKuroShiftLTwoVarDecoderSamLite}{1.4}
\newcommand{\retLVDKuroShiftLTwoVarDecoderSamLite}{0.884}
\newcommand{\retCILVDKuroShiftLTwoVarDecoderSamLite}{0.022}
\newcommand{\nLVDKuroShiftLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDKuroShiftLTwoVarDecoderSegformerMlp}{54.5}
\newcommand{\miouCILVDKuroShiftLTwoVarDecoderSegformerMlp}{3.3}
\newcommand{\dropLVDKuroShiftLTwoVarDecoderSegformerMlp}{2.8}
\newcommand{\dropCILVDKuroShiftLTwoVarDecoderSegformerMlp}{3.9}
\newcommand{\retLVDKuroShiftLTwoVarDecoderSegformerMlp}{0.951}
\newcommand{\retCILVDKuroShiftLTwoVarDecoderSegformerMlp}{0.067}
\newcommand{\nLVDKuroShiftLTwoVarLrMultOne}{5}
\newcommand{\miouLVDKuroShiftLTwoVarLrMultOne}{49.1}
\newcommand{\miouCILVDKuroShiftLTwoVarLrMultOne}{4.0}
\newcommand{\dropLVDKuroShiftLTwoVarLrMultOne}{5.1}
\newcommand{\dropCILVDKuroShiftLTwoVarLrMultOne}{6.4}
\newcommand{\retLVDKuroShiftLTwoVarLrMultOne}{0.909}
\newcommand{\retCILVDKuroShiftLTwoVarLrMultOne}{0.112}
\newcommand{\nLVDOemBoundaryLOne}{5}
\newcommand{\miouLVDOemBoundaryLOne}{59.9}
\newcommand{\miouCILVDOemBoundaryLOne}{1.2}
\newcommand{\dropLVDOemBoundaryLOne}{3.4}
\newcommand{\dropCILVDOemBoundaryLOne}{1.6}
\newcommand{\retLVDOemBoundaryLOne}{0.946}
\newcommand{\retCILVDOemBoundaryLOne}{0.025}
\newcommand{\nLVDOemBoundaryLTwo}{5}
\newcommand{\miouLVDOemBoundaryLTwo}{54.2}
\newcommand{\miouCILVDOemBoundaryLTwo}{1.5}
\newcommand{\dropLVDOemBoundaryLTwo}{9.2}
\newcommand{\dropCILVDOemBoundaryLTwo}{1.0}
\newcommand{\retLVDOemBoundaryLTwo}{0.855}
\newcommand{\retCILVDOemBoundaryLTwo}{0.016}
\newcommand{\nLVDOemBoundaryLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDOemBoundaryLTwoVarDecoderMaskTwoformerLite}{51.4}
\newcommand{\miouCILVDOemBoundaryLTwoVarDecoderMaskTwoformerLite}{0.9}
\newcommand{\dropLVDOemBoundaryLTwoVarDecoderMaskTwoformerLite}{10.3}
\newcommand{\dropCILVDOemBoundaryLTwoVarDecoderMaskTwoformerLite}{0.8}
\newcommand{\retLVDOemBoundaryLTwoVarDecoderMaskTwoformerLite}{0.832}
\newcommand{\retCILVDOemBoundaryLTwoVarDecoderMaskTwoformerLite}{0.012}
\newcommand{\nLVDOemBoundaryLTwoVarDecoderSamLite}{5}
\newcommand{\miouLVDOemBoundaryLTwoVarDecoderSamLite}{52.2}
\newcommand{\miouCILVDOemBoundaryLTwoVarDecoderSamLite}{1.4}
\newcommand{\dropLVDOemBoundaryLTwoVarDecoderSamLite}{8.3}
\newcommand{\dropCILVDOemBoundaryLTwoVarDecoderSamLite}{1.4}
\newcommand{\retLVDOemBoundaryLTwoVarDecoderSamLite}{0.863}
\newcommand{\retCILVDOemBoundaryLTwoVarDecoderSamLite}{0.022}
\newcommand{\nLVDOemBoundaryLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDOemBoundaryLTwoVarDecoderSegformerMlp}{55.1}
\newcommand{\miouCILVDOemBoundaryLTwoVarDecoderSegformerMlp}{0.6}
\newcommand{\dropLVDOemBoundaryLTwoVarDecoderSegformerMlp}{8.1}
\newcommand{\dropCILVDOemBoundaryLTwoVarDecoderSegformerMlp}{0.7}
\newcommand{\retLVDOemBoundaryLTwoVarDecoderSegformerMlp}{0.872}
\newcommand{\retCILVDOemBoundaryLTwoVarDecoderSegformerMlp}{0.010}
\newcommand{\nLVDOemBoundaryLTwoVarLrMultOne}{5}
\newcommand{\miouLVDOemBoundaryLTwoVarLrMultOne}{54.6}
\newcommand{\miouCILVDOemBoundaryLTwoVarLrMultOne}{0.8}
\newcommand{\dropLVDOemBoundaryLTwoVarLrMultOne}{10.1}
\newcommand{\dropCILVDOemBoundaryLTwoVarLrMultOne}{0.9}
\newcommand{\retLVDOemBoundaryLTwoVarLrMultOne}{0.844}
\newcommand{\retCILVDOemBoundaryLTwoVarLrMultOne}{0.013}
\newcommand{\nLVDOemClean}{5}
\newcommand{\miouLVDOemClean}{63.4}
\newcommand{\miouCILVDOemClean}{0.5}
\newcommand{\nLVDOemCleanVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDOemCleanVarDecoderMaskTwoformerLite}{61.7}
\newcommand{\miouCILVDOemCleanVarDecoderMaskTwoformerLite}{1.0}
\newcommand{\nLVDOemCleanVarDecoderSamLite}{5}
\newcommand{\miouLVDOemCleanVarDecoderSamLite}{60.4}
\newcommand{\miouCILVDOemCleanVarDecoderSamLite}{1.0}
\newcommand{\nLVDOemCleanVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDOemCleanVarDecoderSegformerMlp}{63.2}
\newcommand{\miouCILVDOemCleanVarDecoderSegformerMlp}{0.4}
\newcommand{\nLVDOemCleanVarLrMultOne}{5}
\newcommand{\miouLVDOemCleanVarLrMultOne}{64.7}
\newcommand{\miouCILVDOemCleanVarLrMultOne}{0.5}
\newcommand{\nLVDOemCoarseLOne}{5}
\newcommand{\miouLVDOemCoarseLOne}{62.5}
\newcommand{\miouCILVDOemCoarseLOne}{1.0}
\newcommand{\dropLVDOemCoarseLOne}{0.9}
\newcommand{\dropCILVDOemCoarseLOne}{0.7}
\newcommand{\retLVDOemCoarseLOne}{0.986}
\newcommand{\retCILVDOemCoarseLOne}{0.011}
\newcommand{\nLVDOemCoarseLTwo}{5}
\newcommand{\miouLVDOemCoarseLTwo}{57.8}
\newcommand{\miouCILVDOemCoarseLTwo}{1.3}
\newcommand{\dropLVDOemCoarseLTwo}{5.6}
\newcommand{\dropCILVDOemCoarseLTwo}{1.5}
\newcommand{\retLVDOemCoarseLTwo}{0.912}
\newcommand{\retCILVDOemCoarseLTwo}{0.023}
\newcommand{\nLVDOemCoarseLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDOemCoarseLTwoVarDecoderMaskTwoformerLite}{57.2}
\newcommand{\miouCILVDOemCoarseLTwoVarDecoderMaskTwoformerLite}{0.8}
\newcommand{\dropLVDOemCoarseLTwoVarDecoderMaskTwoformerLite}{4.6}
\newcommand{\dropCILVDOemCoarseLTwoVarDecoderMaskTwoformerLite}{0.8}
\newcommand{\retLVDOemCoarseLTwoVarDecoderMaskTwoformerLite}{0.926}
\newcommand{\retCILVDOemCoarseLTwoVarDecoderMaskTwoformerLite}{0.013}
\newcommand{\nLVDOemCoarseLTwoVarDecoderSamLite}{5}
\newcommand{\miouLVDOemCoarseLTwoVarDecoderSamLite}{56.5}
\newcommand{\miouCILVDOemCoarseLTwoVarDecoderSamLite}{1.0}
\newcommand{\dropLVDOemCoarseLTwoVarDecoderSamLite}{3.9}
\newcommand{\dropCILVDOemCoarseLTwoVarDecoderSamLite}{0.6}
\newcommand{\retLVDOemCoarseLTwoVarDecoderSamLite}{0.935}
\newcommand{\retCILVDOemCoarseLTwoVarDecoderSamLite}{0.010}
\newcommand{\nLVDOemCoarseLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDOemCoarseLTwoVarDecoderSegformerMlp}{56.7}
\newcommand{\miouCILVDOemCoarseLTwoVarDecoderSegformerMlp}{0.7}
\newcommand{\dropLVDOemCoarseLTwoVarDecoderSegformerMlp}{6.5}
\newcommand{\dropCILVDOemCoarseLTwoVarDecoderSegformerMlp}{0.8}
\newcommand{\retLVDOemCoarseLTwoVarDecoderSegformerMlp}{0.897}
\newcommand{\retCILVDOemCoarseLTwoVarDecoderSegformerMlp}{0.012}
\newcommand{\nLVDOemCoarseLTwoVarLrMultOne}{5}
\newcommand{\miouLVDOemCoarseLTwoVarLrMultOne}{58.8}
\newcommand{\miouCILVDOemCoarseLTwoVarLrMultOne}{0.9}
\newcommand{\dropLVDOemCoarseLTwoVarLrMultOne}{5.9}
\newcommand{\dropCILVDOemCoarseLTwoVarLrMultOne}{1.0}
\newcommand{\retLVDOemCoarseLTwoVarLrMultOne}{0.908}
\newcommand{\retCILVDOemCoarseLTwoVarLrMultOne}{0.016}
\newcommand{\nLVDOemOmissionLOne}{5}
\newcommand{\miouLVDOemOmissionLOne}{60.5}
\newcommand{\miouCILVDOemOmissionLOne}{1.0}
\newcommand{\dropLVDOemOmissionLOne}{2.9}
\newcommand{\dropCILVDOemOmissionLOne}{1.1}
\newcommand{\retLVDOemOmissionLOne}{0.954}
\newcommand{\retCILVDOemOmissionLOne}{0.017}
\newcommand{\nLVDOemOmissionLTwo}{5}
\newcommand{\miouLVDOemOmissionLTwo}{54.2}
\newcommand{\miouCILVDOemOmissionLTwo}{1.1}
\newcommand{\dropLVDOemOmissionLTwo}{9.2}
\newcommand{\dropCILVDOemOmissionLTwo}{1.3}
\newcommand{\retLVDOemOmissionLTwo}{0.855}
\newcommand{\retCILVDOemOmissionLTwo}{0.020}
\newcommand{\nLVDOemOmissionLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDOemOmissionLTwoVarDecoderMaskTwoformerLite}{53.0}
\newcommand{\miouCILVDOemOmissionLTwoVarDecoderMaskTwoformerLite}{1.9}
\newcommand{\dropLVDOemOmissionLTwoVarDecoderMaskTwoformerLite}{8.7}
\newcommand{\dropCILVDOemOmissionLTwoVarDecoderMaskTwoformerLite}{1.0}
\newcommand{\retLVDOemOmissionLTwoVarDecoderMaskTwoformerLite}{0.858}
\newcommand{\retCILVDOemOmissionLTwoVarDecoderMaskTwoformerLite}{0.018}
\newcommand{\nLVDOemOmissionLTwoVarDecoderSamLite}{5}
\newcommand{\miouLVDOemOmissionLTwoVarDecoderSamLite}{52.5}
\newcommand{\miouCILVDOemOmissionLTwoVarDecoderSamLite}{0.5}
\newcommand{\dropLVDOemOmissionLTwoVarDecoderSamLite}{7.9}
\newcommand{\dropCILVDOemOmissionLTwoVarDecoderSamLite}{1.4}
\newcommand{\retLVDOemOmissionLTwoVarDecoderSamLite}{0.869}
\newcommand{\retCILVDOemOmissionLTwoVarDecoderSamLite}{0.021}
\newcommand{\nLVDOemOmissionLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDOemOmissionLTwoVarDecoderSegformerMlp}{54.8}
\newcommand{\miouCILVDOemOmissionLTwoVarDecoderSegformerMlp}{1.9}
\newcommand{\dropLVDOemOmissionLTwoVarDecoderSegformerMlp}{8.4}
\newcommand{\dropCILVDOemOmissionLTwoVarDecoderSegformerMlp}{2.1}
\newcommand{\retLVDOemOmissionLTwoVarDecoderSegformerMlp}{0.867}
\newcommand{\retCILVDOemOmissionLTwoVarDecoderSegformerMlp}{0.033}
\newcommand{\nLVDOemOmissionLTwoVarLrMultOne}{5}
\newcommand{\miouLVDOemOmissionLTwoVarLrMultOne}{54.2}
\newcommand{\miouCILVDOemOmissionLTwoVarLrMultOne}{1.9}
\newcommand{\dropLVDOemOmissionLTwoVarLrMultOne}{10.5}
\newcommand{\dropCILVDOemOmissionLTwoVarLrMultOne}{2.2}
\newcommand{\retLVDOemOmissionLTwoVarLrMultOne}{0.837}
\newcommand{\retCILVDOemOmissionLTwoVarLrMultOne}{0.033}
\newcommand{\nLVDOemShiftLOne}{5}
\newcommand{\miouLVDOemShiftLOne}{62.6}
\newcommand{\miouCILVDOemShiftLOne}{0.9}
\newcommand{\dropLVDOemShiftLOne}{0.7}
\newcommand{\dropCILVDOemShiftLOne}{1.1}
\newcommand{\retLVDOemShiftLOne}{0.989}
\newcommand{\retCILVDOemShiftLOne}{0.017}
\newcommand{\nLVDOemShiftLTwo}{5}
\newcommand{\miouLVDOemShiftLTwo}{60.3}
\newcommand{\miouCILVDOemShiftLTwo}{1.4}
\newcommand{\dropLVDOemShiftLTwo}{3.0}
\newcommand{\dropCILVDOemShiftLTwo}{1.0}
\newcommand{\retLVDOemShiftLTwo}{0.952}
\newcommand{\retCILVDOemShiftLTwo}{0.017}
\newcommand{\nLVDOemShiftLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDOemShiftLTwoVarDecoderMaskTwoformerLite}{58.2}
\newcommand{\miouCILVDOemShiftLTwoVarDecoderMaskTwoformerLite}{1.7}
\newcommand{\dropLVDOemShiftLTwoVarDecoderMaskTwoformerLite}{3.5}
\newcommand{\dropCILVDOemShiftLTwoVarDecoderMaskTwoformerLite}{1.4}
\newcommand{\retLVDOemShiftLTwoVarDecoderMaskTwoformerLite}{0.943}
\newcommand{\retCILVDOemShiftLTwoVarDecoderMaskTwoformerLite}{0.023}
\newcommand{\nLVDOemShiftLTwoVarDecoderSamLite}{5}
\newcommand{\miouLVDOemShiftLTwoVarDecoderSamLite}{57.9}
\newcommand{\miouCILVDOemShiftLTwoVarDecoderSamLite}{0.8}
\newcommand{\dropLVDOemShiftLTwoVarDecoderSamLite}{2.6}
\newcommand{\dropCILVDOemShiftLTwoVarDecoderSamLite}{0.7}
\newcommand{\retLVDOemShiftLTwoVarDecoderSamLite}{0.958}
\newcommand{\retCILVDOemShiftLTwoVarDecoderSamLite}{0.012}
\newcommand{\nLVDOemShiftLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDOemShiftLTwoVarDecoderSegformerMlp}{59.6}
\newcommand{\miouCILVDOemShiftLTwoVarDecoderSegformerMlp}{1.5}
\newcommand{\dropLVDOemShiftLTwoVarDecoderSegformerMlp}{3.6}
\newcommand{\dropCILVDOemShiftLTwoVarDecoderSegformerMlp}{1.5}
\newcommand{\retLVDOemShiftLTwoVarDecoderSegformerMlp}{0.943}
\newcommand{\retCILVDOemShiftLTwoVarDecoderSegformerMlp}{0.023}
\newcommand{\nLVDOemShiftLTwoVarLrMultOne}{5}
\newcommand{\miouLVDOemShiftLTwoVarLrMultOne}{60.2}
\newcommand{\miouCILVDOemShiftLTwoVarLrMultOne}{1.9}
\newcommand{\dropLVDOemShiftLTwoVarLrMultOne}{4.5}
\newcommand{\dropCILVDOemShiftLTwoVarLrMultOne}{2.1}
\newcommand{\retLVDOemShiftLTwoVarLrMultOne}{0.930}
\newcommand{\retCILVDOemShiftLTwoVarLrMultOne}{0.032}
\newcommand{\nLVDsenClean}{5}
\newcommand{\miouLVDsenClean}{65.7}
\newcommand{\miouCILVDsenClean}{7.1}
\newcommand{\nLVDsenOtsuLTwo}{5}
\newcommand{\miouLVDsenOtsuLTwo}{60.4}
\newcommand{\miouCILVDsenOtsuLTwo}{7.2}
\newcommand{\dropLVDsenOtsuLTwo}{5.3}
\newcommand{\dropCILVDsenOtsuLTwo}{12.4}
\newcommand{\retLVDsenOtsuLTwo}{0.928}
\newcommand{\retCILVDsenOtsuLTwo}{0.177}
\newcommand{\nLVDSnTwoBoundaryLOne}{5}
\newcommand{\miouLVDSnTwoBoundaryLOne}{83.2}
\newcommand{\miouCILVDSnTwoBoundaryLOne}{0.3}
\newcommand{\dropLVDSnTwoBoundaryLOne}{2.8}
\newcommand{\dropCILVDSnTwoBoundaryLOne}{0.3}
\newcommand{\retLVDSnTwoBoundaryLOne}{0.967}
\newcommand{\retCILVDSnTwoBoundaryLOne}{0.004}
\newcommand{\nLVDSnTwoBoundaryLTwo}{5}
\newcommand{\miouLVDSnTwoBoundaryLTwo}{75.8}
\newcommand{\miouCILVDSnTwoBoundaryLTwo}{0.7}
\newcommand{\dropLVDSnTwoBoundaryLTwo}{10.2}
\newcommand{\dropCILVDSnTwoBoundaryLTwo}{0.6}
\newcommand{\retLVDSnTwoBoundaryLTwo}{0.882}
\newcommand{\retCILVDSnTwoBoundaryLTwo}{0.007}
\newcommand{\nLVDSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}{70.5}
\newcommand{\miouCILVDSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}{12.7}
\newcommand{\dropLVDSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}{15.2}
\newcommand{\dropCILVDSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}{12.7}
\newcommand{\retLVDSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}{0.823}
\newcommand{\retCILVDSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}{0.148}
\newcommand{\nLVDSnTwoBoundaryLTwoVarDecoderSamLite}{5}
\newcommand{\miouLVDSnTwoBoundaryLTwoVarDecoderSamLite}{77.0}
\newcommand{\miouCILVDSnTwoBoundaryLTwoVarDecoderSamLite}{1.2}
\newcommand{\dropLVDSnTwoBoundaryLTwoVarDecoderSamLite}{8.8}
\newcommand{\dropCILVDSnTwoBoundaryLTwoVarDecoderSamLite}{1.1}
\newcommand{\retLVDSnTwoBoundaryLTwoVarDecoderSamLite}{0.898}
\newcommand{\retCILVDSnTwoBoundaryLTwoVarDecoderSamLite}{0.013}
\newcommand{\nLVDSnTwoBoundaryLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDSnTwoBoundaryLTwoVarDecoderSegformerMlp}{76.8}
\newcommand{\miouCILVDSnTwoBoundaryLTwoVarDecoderSegformerMlp}{0.7}
\newcommand{\dropLVDSnTwoBoundaryLTwoVarDecoderSegformerMlp}{8.6}
\newcommand{\dropCILVDSnTwoBoundaryLTwoVarDecoderSegformerMlp}{0.9}
\newcommand{\retLVDSnTwoBoundaryLTwoVarDecoderSegformerMlp}{0.900}
\newcommand{\retCILVDSnTwoBoundaryLTwoVarDecoderSegformerMlp}{0.011}
\newcommand{\nLVDSnTwoBoundaryLTwoVarLrMultOne}{5}
\newcommand{\miouLVDSnTwoBoundaryLTwoVarLrMultOne}{75.7}
\newcommand{\miouCILVDSnTwoBoundaryLTwoVarLrMultOne}{1.0}
\newcommand{\dropLVDSnTwoBoundaryLTwoVarLrMultOne}{11.3}
\newcommand{\dropCILVDSnTwoBoundaryLTwoVarLrMultOne}{1.1}
\newcommand{\retLVDSnTwoBoundaryLTwoVarLrMultOne}{0.870}
\newcommand{\retCILVDSnTwoBoundaryLTwoVarLrMultOne}{0.012}
\newcommand{\nLVDSnTwoClean}{5}
\newcommand{\miouLVDSnTwoClean}{86.0}
\newcommand{\miouCILVDSnTwoClean}{0.4}
\newcommand{\nLVDSnTwoCleanVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDSnTwoCleanVarDecoderMaskTwoformerLite}{85.7}
\newcommand{\miouCILVDSnTwoCleanVarDecoderMaskTwoformerLite}{0.7}
\newcommand{\nLVDSnTwoCleanVarDecoderSamLite}{5}
\newcommand{\miouLVDSnTwoCleanVarDecoderSamLite}{85.8}
\newcommand{\miouCILVDSnTwoCleanVarDecoderSamLite}{0.1}
\newcommand{\nLVDSnTwoCleanVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDSnTwoCleanVarDecoderSegformerMlp}{85.4}
\newcommand{\miouCILVDSnTwoCleanVarDecoderSegformerMlp}{0.4}
\newcommand{\nLVDSnTwoCleanVarLrMultOne}{5}
\newcommand{\miouLVDSnTwoCleanVarLrMultOne}{86.9}
\newcommand{\miouCILVDSnTwoCleanVarLrMultOne}{0.4}
\newcommand{\nLVDSnTwoCoarseLOne}{5}
\newcommand{\miouLVDSnTwoCoarseLOne}{84.1}
\newcommand{\miouCILVDSnTwoCoarseLOne}{0.2}
\newcommand{\dropLVDSnTwoCoarseLOne}{1.9}
\newcommand{\dropCILVDSnTwoCoarseLOne}{0.2}
\newcommand{\retLVDSnTwoCoarseLOne}{0.978}
\newcommand{\retCILVDSnTwoCoarseLOne}{0.003}
\newcommand{\nLVDSnTwoCoarseLTwo}{5}
\newcommand{\miouLVDSnTwoCoarseLTwo}{74.6}
\newcommand{\miouCILVDSnTwoCoarseLTwo}{0.6}
\newcommand{\dropLVDSnTwoCoarseLTwo}{11.4}
\newcommand{\dropCILVDSnTwoCoarseLTwo}{0.7}
\newcommand{\retLVDSnTwoCoarseLTwo}{0.867}
\newcommand{\retCILVDSnTwoCoarseLTwo}{0.008}
\newcommand{\nLVDSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}{71.3}
\newcommand{\miouCILVDSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}{1.6}
\newcommand{\dropLVDSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}{14.4}
\newcommand{\dropCILVDSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}{1.7}
\newcommand{\retLVDSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}{0.832}
\newcommand{\retCILVDSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}{0.019}
\newcommand{\nLVDSnTwoCoarseLTwoVarDecoderSamLite}{5}
\newcommand{\miouLVDSnTwoCoarseLTwoVarDecoderSamLite}{71.7}
\newcommand{\miouCILVDSnTwoCoarseLTwoVarDecoderSamLite}{2.0}
\newcommand{\dropLVDSnTwoCoarseLTwoVarDecoderSamLite}{14.1}
\newcommand{\dropCILVDSnTwoCoarseLTwoVarDecoderSamLite}{2.0}
\newcommand{\retLVDSnTwoCoarseLTwoVarDecoderSamLite}{0.836}
\newcommand{\retCILVDSnTwoCoarseLTwoVarDecoderSamLite}{0.023}
\newcommand{\nLVDSnTwoCoarseLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDSnTwoCoarseLTwoVarDecoderSegformerMlp}{74.3}
\newcommand{\miouCILVDSnTwoCoarseLTwoVarDecoderSegformerMlp}{1.4}
\newcommand{\dropLVDSnTwoCoarseLTwoVarDecoderSegformerMlp}{11.1}
\newcommand{\dropCILVDSnTwoCoarseLTwoVarDecoderSegformerMlp}{1.0}
\newcommand{\retLVDSnTwoCoarseLTwoVarDecoderSegformerMlp}{0.870}
\newcommand{\retCILVDSnTwoCoarseLTwoVarDecoderSegformerMlp}{0.012}
\newcommand{\nLVDSnTwoCoarseLTwoVarLrMultOne}{5}
\newcommand{\miouLVDSnTwoCoarseLTwoVarLrMultOne}{74.0}
\newcommand{\miouCILVDSnTwoCoarseLTwoVarLrMultOne}{1.2}
\newcommand{\dropLVDSnTwoCoarseLTwoVarLrMultOne}{12.9}
\newcommand{\dropCILVDSnTwoCoarseLTwoVarLrMultOne}{1.2}
\newcommand{\retLVDSnTwoCoarseLTwoVarLrMultOne}{0.852}
\newcommand{\retCILVDSnTwoCoarseLTwoVarLrMultOne}{0.014}
\newcommand{\nLVDSnTwoOmissionLOne}{5}
\newcommand{\miouLVDSnTwoOmissionLOne}{81.6}
\newcommand{\miouCILVDSnTwoOmissionLOne}{0.8}
\newcommand{\dropLVDSnTwoOmissionLOne}{4.5}
\newcommand{\dropCILVDSnTwoOmissionLOne}{0.7}
\newcommand{\retLVDSnTwoOmissionLOne}{0.948}
\newcommand{\retCILVDSnTwoOmissionLOne}{0.008}
\newcommand{\nLVDSnTwoOmissionLTwo}{5}
\newcommand{\miouLVDSnTwoOmissionLTwo}{73.3}
\newcommand{\miouCILVDSnTwoOmissionLTwo}{4.5}
\newcommand{\dropLVDSnTwoOmissionLTwo}{12.7}
\newcommand{\dropCILVDSnTwoOmissionLTwo}{4.9}
\newcommand{\retLVDSnTwoOmissionLTwo}{0.852}
\newcommand{\retCILVDSnTwoOmissionLTwo}{0.056}
\newcommand{\nLVDSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}{57.2}
\newcommand{\miouCILVDSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}{11.4}
\newcommand{\dropLVDSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}{28.5}
\newcommand{\dropCILVDSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}{11.2}
\newcommand{\retLVDSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}{0.667}
\newcommand{\retCILVDSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}{0.131}
\newcommand{\nLVDSnTwoOmissionLTwoVarDecoderSamLite}{5}
\newcommand{\miouLVDSnTwoOmissionLTwoVarDecoderSamLite}{65.5}
\newcommand{\miouCILVDSnTwoOmissionLTwoVarDecoderSamLite}{4.4}
\newcommand{\dropLVDSnTwoOmissionLTwoVarDecoderSamLite}{20.3}
\newcommand{\dropCILVDSnTwoOmissionLTwoVarDecoderSamLite}{4.4}
\newcommand{\retLVDSnTwoOmissionLTwoVarDecoderSamLite}{0.764}
\newcommand{\retCILVDSnTwoOmissionLTwoVarDecoderSamLite}{0.051}
\newcommand{\nLVDSnTwoOmissionLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDSnTwoOmissionLTwoVarDecoderSegformerMlp}{73.7}
\newcommand{\miouCILVDSnTwoOmissionLTwoVarDecoderSegformerMlp}{3.6}
\newcommand{\dropLVDSnTwoOmissionLTwoVarDecoderSegformerMlp}{11.7}
\newcommand{\dropCILVDSnTwoOmissionLTwoVarDecoderSegformerMlp}{3.5}
\newcommand{\retLVDSnTwoOmissionLTwoVarDecoderSegformerMlp}{0.863}
\newcommand{\retCILVDSnTwoOmissionLTwoVarDecoderSegformerMlp}{0.041}
\newcommand{\nLVDSnTwoOmissionLTwoVarLrMultOne}{5}
\newcommand{\miouLVDSnTwoOmissionLTwoVarLrMultOne}{70.5}
\newcommand{\miouCILVDSnTwoOmissionLTwoVarLrMultOne}{4.3}
\newcommand{\dropLVDSnTwoOmissionLTwoVarLrMultOne}{16.4}
\newcommand{\dropCILVDSnTwoOmissionLTwoVarLrMultOne}{4.5}
\newcommand{\retLVDSnTwoOmissionLTwoVarLrMultOne}{0.811}
\newcommand{\retCILVDSnTwoOmissionLTwoVarLrMultOne}{0.051}
\newcommand{\nLVDSnTwoShiftLOne}{5}
\newcommand{\miouLVDSnTwoShiftLOne}{84.4}
\newcommand{\miouCILVDSnTwoShiftLOne}{0.7}
\newcommand{\dropLVDSnTwoShiftLOne}{1.6}
\newcommand{\dropCILVDSnTwoShiftLOne}{0.3}
\newcommand{\retLVDSnTwoShiftLOne}{0.981}
\newcommand{\retCILVDSnTwoShiftLOne}{0.004}
\newcommand{\nLVDSnTwoShiftLTwo}{5}
\newcommand{\miouLVDSnTwoShiftLTwo}{78.9}
\newcommand{\miouCILVDSnTwoShiftLTwo}{0.8}
\newcommand{\dropLVDSnTwoShiftLTwo}{7.1}
\newcommand{\dropCILVDSnTwoShiftLTwo}{0.8}
\newcommand{\retLVDSnTwoShiftLTwo}{0.917}
\newcommand{\retCILVDSnTwoShiftLTwo}{0.009}
\newcommand{\nLVDSnTwoShiftLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouLVDSnTwoShiftLTwoVarDecoderMaskTwoformerLite}{77.6}
\newcommand{\miouCILVDSnTwoShiftLTwoVarDecoderMaskTwoformerLite}{0.6}
\newcommand{\dropLVDSnTwoShiftLTwoVarDecoderMaskTwoformerLite}{8.0}
\newcommand{\dropCILVDSnTwoShiftLTwoVarDecoderMaskTwoformerLite}{0.3}
\newcommand{\retLVDSnTwoShiftLTwoVarDecoderMaskTwoformerLite}{0.906}
\newcommand{\retCILVDSnTwoShiftLTwoVarDecoderMaskTwoformerLite}{0.003}
\newcommand{\nLVDSnTwoShiftLTwoVarDecoderSamLite}{5}
\newcommand{\miouLVDSnTwoShiftLTwoVarDecoderSamLite}{76.2}
\newcommand{\miouCILVDSnTwoShiftLTwoVarDecoderSamLite}{0.7}
\newcommand{\dropLVDSnTwoShiftLTwoVarDecoderSamLite}{9.6}
\newcommand{\dropCILVDSnTwoShiftLTwoVarDecoderSamLite}{0.7}
\newcommand{\retLVDSnTwoShiftLTwoVarDecoderSamLite}{0.888}
\newcommand{\retCILVDSnTwoShiftLTwoVarDecoderSamLite}{0.008}
\newcommand{\nLVDSnTwoShiftLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouLVDSnTwoShiftLTwoVarDecoderSegformerMlp}{77.8}
\newcommand{\miouCILVDSnTwoShiftLTwoVarDecoderSegformerMlp}{0.8}
\newcommand{\dropLVDSnTwoShiftLTwoVarDecoderSegformerMlp}{7.6}
\newcommand{\dropCILVDSnTwoShiftLTwoVarDecoderSegformerMlp}{0.7}
\newcommand{\retLVDSnTwoShiftLTwoVarDecoderSegformerMlp}{0.911}
\newcommand{\retCILVDSnTwoShiftLTwoVarDecoderSegformerMlp}{0.008}
\newcommand{\nLVDSnTwoShiftLTwoVarLrMultOne}{5}
\newcommand{\miouLVDSnTwoShiftLTwoVarLrMultOne}{79.0}
\newcommand{\miouCILVDSnTwoShiftLTwoVarLrMultOne}{0.2}
\newcommand{\dropLVDSnTwoShiftLTwoVarLrMultOne}{8.0}
\newcommand{\dropCILVDSnTwoShiftLTwoVarLrMultOne}{0.6}
\newcommand{\retLVDSnTwoShiftLTwoVarLrMultOne}{0.909}
\newcommand{\retCILVDSnTwoShiftLTwoVarLrMultOne}{0.007}
\newcommand{\nSATburnBoundaryLOne}{5}
\newcommand{\miouSATburnBoundaryLOne}{72.6}
\newcommand{\miouCISATburnBoundaryLOne}{2.9}
\newcommand{\dropSATburnBoundaryLOne}{3.3}
\newcommand{\dropCISATburnBoundaryLOne}{4.4}
\newcommand{\retSATburnBoundaryLOne}{0.958}
\newcommand{\retCISATburnBoundaryLOne}{0.057}
\newcommand{\nSATburnBoundaryLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouSATburnBoundaryLOneVarDecoderMaskTwoformerFull}{62.6}
\newcommand{\miouCISATburnBoundaryLOneVarDecoderMaskTwoformerFull}{4.7}
\newcommand{\dropSATburnBoundaryLOneVarDecoderMaskTwoformerFull}{8.0}
\newcommand{\dropCISATburnBoundaryLOneVarDecoderMaskTwoformerFull}{7.8}
\newcommand{\retSATburnBoundaryLOneVarDecoderMaskTwoformerFull}{0.890}
\newcommand{\retCISATburnBoundaryLOneVarDecoderMaskTwoformerFull}{0.102}
\newcommand{\nSATburnBoundaryLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATburnBoundaryLOneVarDecoderMaskTwoformerLite}{58.8}
\newcommand{\miouCISATburnBoundaryLOneVarDecoderMaskTwoformerLite}{15.5}
\newcommand{\dropSATburnBoundaryLOneVarDecoderMaskTwoformerLite}{1.2}
\newcommand{\dropCISATburnBoundaryLOneVarDecoderMaskTwoformerLite}{28.0}
\newcommand{\retSATburnBoundaryLOneVarDecoderMaskTwoformerLite}{1.050}
\newcommand{\retCISATburnBoundaryLOneVarDecoderMaskTwoformerLite}{0.486}
\newcommand{\nSATburnBoundaryLOneVarDecoderSamLite}{5}
\newcommand{\miouSATburnBoundaryLOneVarDecoderSamLite}{66.2}
\newcommand{\miouCISATburnBoundaryLOneVarDecoderSamLite}{7.3}
\newcommand{\dropSATburnBoundaryLOneVarDecoderSamLite}{7.6}
\newcommand{\dropCISATburnBoundaryLOneVarDecoderSamLite}{8.4}
\newcommand{\retSATburnBoundaryLOneVarDecoderSamLite}{0.899}
\newcommand{\retCISATburnBoundaryLOneVarDecoderSamLite}{0.111}
\newcommand{\nSATburnBoundaryLOneVarDecoderSamPretrained}{5}
\newcommand{\miouSATburnBoundaryLOneVarDecoderSamPretrained}{64.4}
\newcommand{\miouCISATburnBoundaryLOneVarDecoderSamPretrained}{14.4}
\newcommand{\dropSATburnBoundaryLOneVarDecoderSamPretrained}{\ensuremath{-}0.3}
\newcommand{\dropCISATburnBoundaryLOneVarDecoderSamPretrained}{7.1}
\newcommand{\retSATburnBoundaryLOneVarDecoderSamPretrained}{1.008}
\newcommand{\retCISATburnBoundaryLOneVarDecoderSamPretrained}{0.104}
\newcommand{\nSATburnBoundaryLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouSATburnBoundaryLOneVarDecoderSegformerMlp}{70.1}
\newcommand{\miouCISATburnBoundaryLOneVarDecoderSegformerMlp}{8.2}
\newcommand{\dropSATburnBoundaryLOneVarDecoderSegformerMlp}{9.9}
\newcommand{\dropCISATburnBoundaryLOneVarDecoderSegformerMlp}{10.2}
\newcommand{\retSATburnBoundaryLOneVarDecoderSegformerMlp}{0.878}
\newcommand{\retCISATburnBoundaryLOneVarDecoderSegformerMlp}{0.124}
\newcommand{\nSATburnBoundaryLTwo}{8}
\newcommand{\miouSATburnBoundaryLTwo}{61.9}
\newcommand{\miouCISATburnBoundaryLTwo}{3.2}
\newcommand{\dropSATburnBoundaryLTwo}{15.1}
\newcommand{\dropCISATburnBoundaryLTwo}{3.2}
\newcommand{\retSATburnBoundaryLTwo}{0.804}
\newcommand{\retCISATburnBoundaryLTwo}{0.040}
\newcommand{\nSATburnBoundaryLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouSATburnBoundaryLTwoVarDecoderMaskTwoformerFull}{57.4}
\newcommand{\miouCISATburnBoundaryLTwoVarDecoderMaskTwoformerFull}{4.9}
\newcommand{\dropSATburnBoundaryLTwoVarDecoderMaskTwoformerFull}{13.2}
\newcommand{\dropCISATburnBoundaryLTwoVarDecoderMaskTwoformerFull}{5.8}
\newcommand{\retSATburnBoundaryLTwoVarDecoderMaskTwoformerFull}{0.815}
\newcommand{\retCISATburnBoundaryLTwoVarDecoderMaskTwoformerFull}{0.075}
\newcommand{\nSATburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{62.9}
\newcommand{\miouCISATburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{3.7}
\newcommand{\dropSATburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{14.2}
\newcommand{\dropCISATburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{4.5}
\newcommand{\retSATburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{0.816}
\newcommand{\retCISATburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{0.054}
\newcommand{\nSATburnBoundaryLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATburnBoundaryLTwoVarDecoderMaskTwoformerLite}{51.9}
\newcommand{\miouCISATburnBoundaryLTwoVarDecoderMaskTwoformerLite}{11.0}
\newcommand{\dropSATburnBoundaryLTwoVarDecoderMaskTwoformerLite}{8.1}
\newcommand{\dropCISATburnBoundaryLTwoVarDecoderMaskTwoformerLite}{23.1}
\newcommand{\retSATburnBoundaryLTwoVarDecoderMaskTwoformerLite}{0.918}
\newcommand{\retCISATburnBoundaryLTwoVarDecoderMaskTwoformerLite}{0.377}
\newcommand{\nSATburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{65.4}
\newcommand{\miouCISATburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{2.2}
\newcommand{\dropSATburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{15.9}
\newcommand{\dropCISATburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{2.9}
\newcommand{\retSATburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{0.805}
\newcommand{\retCISATburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{0.033}
\newcommand{\nSATburnBoundaryLTwoVarDecoderSamLite}{5}
\newcommand{\miouSATburnBoundaryLTwoVarDecoderSamLite}{63.2}
\newcommand{\miouCISATburnBoundaryLTwoVarDecoderSamLite}{2.5}
\newcommand{\dropSATburnBoundaryLTwoVarDecoderSamLite}{10.6}
\newcommand{\dropCISATburnBoundaryLTwoVarDecoderSamLite}{3.5}
\newcommand{\retSATburnBoundaryLTwoVarDecoderSamLite}{0.857}
\newcommand{\retCISATburnBoundaryLTwoVarDecoderSamLite}{0.044}
\newcommand{\nSATburnBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATburnBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{67.6}
\newcommand{\miouCISATburnBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{1.4}
\newcommand{\dropSATburnBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{6.7}
\newcommand{\dropCISATburnBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{3.4}
\newcommand{\retSATburnBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{0.911}
\newcommand{\retCISATburnBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{0.041}
\newcommand{\nSATburnBoundaryLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouSATburnBoundaryLTwoVarDecoderSamPretrained}{55.5}
\newcommand{\miouCISATburnBoundaryLTwoVarDecoderSamPretrained}{12.2}
\newcommand{\dropSATburnBoundaryLTwoVarDecoderSamPretrained}{8.7}
\newcommand{\dropCISATburnBoundaryLTwoVarDecoderSamPretrained}{20.2}
\newcommand{\retSATburnBoundaryLTwoVarDecoderSamPretrained}{0.901}
\newcommand{\retCISATburnBoundaryLTwoVarDecoderSamPretrained}{0.380}
\newcommand{\nSATburnBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATburnBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{62.2}
\newcommand{\miouCISATburnBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{12.1}
\newcommand{\dropSATburnBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{15.7}
\newcommand{\dropCISATburnBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{12.7}
\newcommand{\retSATburnBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{0.800}
\newcommand{\retCISATburnBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{0.162}
\newcommand{\nSATburnBoundaryLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouSATburnBoundaryLTwoVarDecoderSegformerMlp}{63.7}
\newcommand{\miouCISATburnBoundaryLTwoVarDecoderSegformerMlp}{2.4}
\newcommand{\dropSATburnBoundaryLTwoVarDecoderSegformerMlp}{16.3}
\newcommand{\dropCISATburnBoundaryLTwoVarDecoderSegformerMlp}{2.8}
\newcommand{\retSATburnBoundaryLTwoVarDecoderSegformerMlp}{0.797}
\newcommand{\retCISATburnBoundaryLTwoVarDecoderSegformerMlp}{0.032}
\newcommand{\nSATburnBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATburnBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{69.9}
\newcommand{\miouCISATburnBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{2.6}
\newcommand{\dropSATburnBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{13.6}
\newcommand{\dropCISATburnBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{4.1}
\newcommand{\retSATburnBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{0.837}
\newcommand{\retCISATburnBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{0.045}
\newcommand{\nSATburnBoundaryLTwoVarLossBootstrap}{5}
\newcommand{\miouSATburnBoundaryLTwoVarLossBootstrap}{61.8}
\newcommand{\miouCISATburnBoundaryLTwoVarLossBootstrap}{2.4}
\newcommand{\dropSATburnBoundaryLTwoVarLossBootstrap}{10.4}
\newcommand{\dropCISATburnBoundaryLTwoVarLossBootstrap}{4.6}
\newcommand{\retSATburnBoundaryLTwoVarLossBootstrap}{0.857}
\newcommand{\retCISATburnBoundaryLTwoVarLossBootstrap}{0.058}
\newcommand{\nSATburnBoundaryLTwoVarLossGce}{5}
\newcommand{\miouSATburnBoundaryLTwoVarLossGce}{62.8}
\newcommand{\miouCISATburnBoundaryLTwoVarLossGce}{2.3}
\newcommand{\dropSATburnBoundaryLTwoVarLossGce}{7.8}
\newcommand{\dropCISATburnBoundaryLTwoVarLossGce}{5.5}
\newcommand{\retSATburnBoundaryLTwoVarLossGce}{0.893}
\newcommand{\retCISATburnBoundaryLTwoVarLossGce}{0.072}
\newcommand{\nSATburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{70.5}
\newcommand{\miouCISATburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{2.5}
\newcommand{\dropSATburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{10.9}
\newcommand{\dropCISATburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{5.1}
\newcommand{\retSATburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{0.867}
\newcommand{\retCISATburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{0.059}
\newcommand{\nSATburnBoundaryLR}{5}
\newcommand{\miouSATburnBoundaryLR}{57.2}
\newcommand{\miouCISATburnBoundaryLR}{4.2}
\newcommand{\dropSATburnBoundaryLR}{18.6}
\newcommand{\dropCISATburnBoundaryLR}{4.7}
\newcommand{\retSATburnBoundaryLR}{0.755}
\newcommand{\retCISATburnBoundaryLR}{0.059}
\newcommand{\nSATburnBoundaryLRVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATburnBoundaryLRVarLrMultZeroThreeThreeThreeThree}{62.2}
\newcommand{\miouCISATburnBoundaryLRVarLrMultZeroThreeThreeThreeThree}{4.9}
\newcommand{\dropSATburnBoundaryLRVarLrMultZeroThreeThreeThreeThree}{19.2}
\newcommand{\dropCISATburnBoundaryLRVarLrMultZeroThreeThreeThreeThree}{4.5}
\newcommand{\retSATburnBoundaryLRVarLrMultZeroThreeThreeThreeThree}{0.764}
\newcommand{\retCISATburnBoundaryLRVarLrMultZeroThreeThreeThreeThree}{0.055}
\newcommand{\nSATburnClean}{8}
\newcommand{\miouSATburnClean}{77.0}
\newcommand{\miouCISATburnClean}{2.6}
\newcommand{\nSATburnCleanVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouSATburnCleanVarDecoderMaskTwoformerFull}{70.5}
\newcommand{\miouCISATburnCleanVarDecoderMaskTwoformerFull}{5.0}
\newcommand{\nSATburnCleanVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATburnCleanVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{77.2}
\newcommand{\miouCISATburnCleanVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{3.1}
\newcommand{\nSATburnCleanVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATburnCleanVarDecoderMaskTwoformerLite}{60.0}
\newcommand{\miouCISATburnCleanVarDecoderMaskTwoformerLite}{19.6}
\newcommand{\nSATburnCleanVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATburnCleanVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{81.3}
\newcommand{\miouCISATburnCleanVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{2.1}
\newcommand{\nSATburnCleanVarDecoderSamLite}{5}
\newcommand{\miouSATburnCleanVarDecoderSamLite}{73.7}
\newcommand{\miouCISATburnCleanVarDecoderSamLite}{2.2}
\newcommand{\nSATburnCleanVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATburnCleanVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{74.4}
\newcommand{\miouCISATburnCleanVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{3.9}
\newcommand{\nSATburnCleanVarDecoderSamPretrained}{5}
\newcommand{\miouSATburnCleanVarDecoderSamPretrained}{64.1}
\newcommand{\miouCISATburnCleanVarDecoderSamPretrained}{14.7}
\newcommand{\nSATburnCleanVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATburnCleanVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{77.9}
\newcommand{\miouCISATburnCleanVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{3.3}
\newcommand{\nSATburnCleanVarDecoderSegformerMlp}{5}
\newcommand{\miouSATburnCleanVarDecoderSegformerMlp}{80.0}
\newcommand{\miouCISATburnCleanVarDecoderSegformerMlp}{2.4}
\newcommand{\nSATburnCleanVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATburnCleanVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{83.6}
\newcommand{\miouCISATburnCleanVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{1.6}
\newcommand{\nSATburnCleanVarFrozenEncoderTrue}{5}
\newcommand{\miouSATburnCleanVarFrozenEncoderTrue}{74.0}
\newcommand{\miouCISATburnCleanVarFrozenEncoderTrue}{1.9}
\newcommand{\nSATburnCleanVarLossBootstrap}{5}
\newcommand{\miouSATburnCleanVarLossBootstrap}{72.2}
\newcommand{\miouCISATburnCleanVarLossBootstrap}{3.1}
\newcommand{\nSATburnCleanVarLossGce}{5}
\newcommand{\miouSATburnCleanVarLossGce}{70.6}
\newcommand{\miouCISATburnCleanVarLossGce}{6.6}
\newcommand{\nSATburnCleanVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATburnCleanVarLrMultZeroThreeThreeThreeThree}{81.3}
\newcommand{\miouCISATburnCleanVarLrMultZeroThreeThreeThreeThree}{2.6}
\newcommand{\nSATburnCleanVarLrMultThree}{1}
\newcommand{\miouSATburnCleanVarLrMultThree}{57.2}
\newcommand{\miouCISATburnCleanVarLrMultThree}{--}
\newcommand{\nSATburnCleanVarTrainSubsetCleanTwoFive}{5}
\newcommand{\miouSATburnCleanVarTrainSubsetCleanTwoFive}{68.3}
\newcommand{\miouCISATburnCleanVarTrainSubsetCleanTwoFive}{8.2}
\newcommand{\nSATburnCoarseLOne}{5}
\newcommand{\miouSATburnCoarseLOne}{72.9}
\newcommand{\miouCISATburnCoarseLOne}{3.8}
\newcommand{\dropSATburnCoarseLOne}{3.0}
\newcommand{\dropCISATburnCoarseLOne}{4.4}
\newcommand{\retSATburnCoarseLOne}{0.961}
\newcommand{\retCISATburnCoarseLOne}{0.057}
\newcommand{\nSATburnCoarseLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouSATburnCoarseLOneVarDecoderMaskTwoformerFull}{64.4}
\newcommand{\miouCISATburnCoarseLOneVarDecoderMaskTwoformerFull}{6.2}
\newcommand{\dropSATburnCoarseLOneVarDecoderMaskTwoformerFull}{6.1}
\newcommand{\dropCISATburnCoarseLOneVarDecoderMaskTwoformerFull}{8.6}
\newcommand{\retSATburnCoarseLOneVarDecoderMaskTwoformerFull}{0.916}
\newcommand{\retCISATburnCoarseLOneVarDecoderMaskTwoformerFull}{0.116}
\newcommand{\nSATburnCoarseLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATburnCoarseLOneVarDecoderMaskTwoformerLite}{58.1}
\newcommand{\miouCISATburnCoarseLOneVarDecoderMaskTwoformerLite}{14.3}
\newcommand{\dropSATburnCoarseLOneVarDecoderMaskTwoformerLite}{1.9}
\newcommand{\dropCISATburnCoarseLOneVarDecoderMaskTwoformerLite}{16.7}
\newcommand{\retSATburnCoarseLOneVarDecoderMaskTwoformerLite}{1.004}
\newcommand{\retCISATburnCoarseLOneVarDecoderMaskTwoformerLite}{0.329}
\newcommand{\nSATburnCoarseLOneVarDecoderSamLite}{5}
\newcommand{\miouSATburnCoarseLOneVarDecoderSamLite}{67.8}
\newcommand{\miouCISATburnCoarseLOneVarDecoderSamLite}{2.7}
\newcommand{\dropSATburnCoarseLOneVarDecoderSamLite}{5.9}
\newcommand{\dropCISATburnCoarseLOneVarDecoderSamLite}{3.6}
\newcommand{\retSATburnCoarseLOneVarDecoderSamLite}{0.921}
\newcommand{\retCISATburnCoarseLOneVarDecoderSamLite}{0.047}
\newcommand{\nSATburnCoarseLOneVarDecoderSamPretrained}{5}
\newcommand{\miouSATburnCoarseLOneVarDecoderSamPretrained}{64.5}
\newcommand{\miouCISATburnCoarseLOneVarDecoderSamPretrained}{13.7}
\newcommand{\dropSATburnCoarseLOneVarDecoderSamPretrained}{\ensuremath{-}0.4}
\newcommand{\dropCISATburnCoarseLOneVarDecoderSamPretrained}{19.3}
\newcommand{\retSATburnCoarseLOneVarDecoderSamPretrained}{1.041}
\newcommand{\retCISATburnCoarseLOneVarDecoderSamPretrained}{0.383}
\newcommand{\nSATburnCoarseLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouSATburnCoarseLOneVarDecoderSegformerMlp}{75.3}
\newcommand{\miouCISATburnCoarseLOneVarDecoderSegformerMlp}{2.6}
\newcommand{\dropSATburnCoarseLOneVarDecoderSegformerMlp}{4.7}
\newcommand{\dropCISATburnCoarseLOneVarDecoderSegformerMlp}{3.0}
\newcommand{\retSATburnCoarseLOneVarDecoderSegformerMlp}{0.942}
\newcommand{\retCISATburnCoarseLOneVarDecoderSegformerMlp}{0.038}
\newcommand{\nSATburnCoarseLTwo}{8}
\newcommand{\miouSATburnCoarseLTwo}{55.3}
\newcommand{\miouCISATburnCoarseLTwo}{3.2}
\newcommand{\dropSATburnCoarseLTwo}{21.7}
\newcommand{\dropCISATburnCoarseLTwo}{4.0}
\newcommand{\retSATburnCoarseLTwo}{0.720}
\newcommand{\retCISATburnCoarseLTwo}{0.047}
\newcommand{\nSATburnCoarseLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouSATburnCoarseLTwoVarDecoderMaskTwoformerFull}{44.8}
\newcommand{\miouCISATburnCoarseLTwoVarDecoderMaskTwoformerFull}{0.0}
\newcommand{\dropSATburnCoarseLTwoVarDecoderMaskTwoformerFull}{25.8}
\newcommand{\dropCISATburnCoarseLTwoVarDecoderMaskTwoformerFull}{5.0}
\newcommand{\retSATburnCoarseLTwoVarDecoderMaskTwoformerFull}{0.637}
\newcommand{\retCISATburnCoarseLTwoVarDecoderMaskTwoformerFull}{0.044}
\newcommand{\nSATburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{51.9}
\newcommand{\miouCISATburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{12.1}
\newcommand{\dropSATburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{25.3}
\newcommand{\dropCISATburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{11.8}
\newcommand{\retSATburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{0.672}
\newcommand{\retCISATburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{0.151}
\newcommand{\nSATburnCoarseLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATburnCoarseLTwoVarDecoderMaskTwoformerLite}{53.2}
\newcommand{\miouCISATburnCoarseLTwoVarDecoderMaskTwoformerLite}{9.6}
\newcommand{\dropSATburnCoarseLTwoVarDecoderMaskTwoformerLite}{6.8}
\newcommand{\dropCISATburnCoarseLTwoVarDecoderMaskTwoformerLite}{22.1}
\newcommand{\retSATburnCoarseLTwoVarDecoderMaskTwoformerLite}{0.938}
\newcommand{\retCISATburnCoarseLTwoVarDecoderMaskTwoformerLite}{0.349}
\newcommand{\nSATburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{64.2}
\newcommand{\miouCISATburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{1.8}
\newcommand{\dropSATburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{17.2}
\newcommand{\dropCISATburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{3.2}
\newcommand{\retSATburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{0.789}
\newcommand{\retCISATburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{0.035}
\newcommand{\nSATburnCoarseLTwoVarDecoderSamLite}{5}
\newcommand{\miouSATburnCoarseLTwoVarDecoderSamLite}{44.8}
\newcommand{\miouCISATburnCoarseLTwoVarDecoderSamLite}{0.0}
\newcommand{\dropSATburnCoarseLTwoVarDecoderSamLite}{29.0}
\newcommand{\dropCISATburnCoarseLTwoVarDecoderSamLite}{2.2}
\newcommand{\retSATburnCoarseLTwoVarDecoderSamLite}{0.608}
\newcommand{\retCISATburnCoarseLTwoVarDecoderSamLite}{0.019}
\newcommand{\nSATburnCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATburnCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{58.1}
\newcommand{\miouCISATburnCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{9.5}
\newcommand{\dropSATburnCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{16.2}
\newcommand{\dropCISATburnCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{10.7}
\newcommand{\retSATburnCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{0.783}
\newcommand{\retCISATburnCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{0.138}
\newcommand{\nSATburnCoarseLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouSATburnCoarseLTwoVarDecoderSamPretrained}{47.9}
\newcommand{\miouCISATburnCoarseLTwoVarDecoderSamPretrained}{8.7}
\newcommand{\dropSATburnCoarseLTwoVarDecoderSamPretrained}{16.2}
\newcommand{\dropCISATburnCoarseLTwoVarDecoderSamPretrained}{16.2}
\newcommand{\retSATburnCoarseLTwoVarDecoderSamPretrained}{0.769}
\newcommand{\retCISATburnCoarseLTwoVarDecoderSamPretrained}{0.220}
\newcommand{\nSATburnCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATburnCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{59.3}
\newcommand{\miouCISATburnCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{10.2}
\newcommand{\dropSATburnCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{18.6}
\newcommand{\dropCISATburnCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{7.8}
\newcommand{\retSATburnCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{0.760}
\newcommand{\retCISATburnCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{0.111}
\newcommand{\nSATburnCoarseLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouSATburnCoarseLTwoVarDecoderSegformerMlp}{54.9}
\newcommand{\miouCISATburnCoarseLTwoVarDecoderSegformerMlp}{6.3}
\newcommand{\dropSATburnCoarseLTwoVarDecoderSegformerMlp}{25.0}
\newcommand{\dropCISATburnCoarseLTwoVarDecoderSegformerMlp}{5.4}
\newcommand{\retSATburnCoarseLTwoVarDecoderSegformerMlp}{0.686}
\newcommand{\retCISATburnCoarseLTwoVarDecoderSegformerMlp}{0.070}
\newcommand{\nSATburnCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATburnCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{65.4}
\newcommand{\miouCISATburnCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{1.8}
\newcommand{\dropSATburnCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{18.1}
\newcommand{\dropCISATburnCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{2.6}
\newcommand{\retSATburnCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{0.783}
\newcommand{\retCISATburnCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{0.028}
\newcommand{\nSATburnCoarseLTwoVarEarlyStoppingFalse}{2}
\newcommand{\miouSATburnCoarseLTwoVarEarlyStoppingFalse}{60.5}
\newcommand{\miouCISATburnCoarseLTwoVarEarlyStoppingFalse}{31.6}
\newcommand{\dropSATburnCoarseLTwoVarEarlyStoppingFalse}{16.5}
\newcommand{\dropCISATburnCoarseLTwoVarEarlyStoppingFalse}{33.8}
\newcommand{\retSATburnCoarseLTwoVarEarlyStoppingFalse}{0.786}
\newcommand{\retCISATburnCoarseLTwoVarEarlyStoppingFalse}{0.433}
\newcommand{\nSATburnCoarseLTwoVarEarlyStoppingFalseFrozenEncoderTrue}{2}
\newcommand{\miouSATburnCoarseLTwoVarEarlyStoppingFalseFrozenEncoderTrue}{60.5}
\newcommand{\miouCISATburnCoarseLTwoVarEarlyStoppingFalseFrozenEncoderTrue}{12.5}
\newcommand{\dropSATburnCoarseLTwoVarEarlyStoppingFalseFrozenEncoderTrue}{14.1}
\newcommand{\dropCISATburnCoarseLTwoVarEarlyStoppingFalseFrozenEncoderTrue}{8.5}
\newcommand{\retSATburnCoarseLTwoVarEarlyStoppingFalseFrozenEncoderTrue}{0.811}
\newcommand{\retCISATburnCoarseLTwoVarEarlyStoppingFalseFrozenEncoderTrue}{0.124}
\newcommand{\nSATburnCoarseLTwoVarFrozenEncoderTrue}{5}
\newcommand{\miouSATburnCoarseLTwoVarFrozenEncoderTrue}{60.6}
\newcommand{\miouCISATburnCoarseLTwoVarFrozenEncoderTrue}{1.4}
\newcommand{\dropSATburnCoarseLTwoVarFrozenEncoderTrue}{13.5}
\newcommand{\dropCISATburnCoarseLTwoVarFrozenEncoderTrue}{0.6}
\newcommand{\retSATburnCoarseLTwoVarFrozenEncoderTrue}{0.818}
\newcommand{\retCISATburnCoarseLTwoVarFrozenEncoderTrue}{0.005}
\newcommand{\nSATburnCoarseLTwoVarLossBootstrap}{5}
\newcommand{\miouSATburnCoarseLTwoVarLossBootstrap}{58.3}
\newcommand{\miouCISATburnCoarseLTwoVarLossBootstrap}{5.0}
\newcommand{\dropSATburnCoarseLTwoVarLossBootstrap}{13.9}
\newcommand{\dropCISATburnCoarseLTwoVarLossBootstrap}{7.3}
\newcommand{\retSATburnCoarseLTwoVarLossBootstrap}{0.809}
\newcommand{\retCISATburnCoarseLTwoVarLossBootstrap}{0.093}
\newcommand{\nSATburnCoarseLTwoVarLossGce}{5}
\newcommand{\miouSATburnCoarseLTwoVarLossGce}{56.8}
\newcommand{\miouCISATburnCoarseLTwoVarLossGce}{5.0}
\newcommand{\dropSATburnCoarseLTwoVarLossGce}{13.7}
\newcommand{\dropCISATburnCoarseLTwoVarLossGce}{5.6}
\newcommand{\retSATburnCoarseLTwoVarLossGce}{0.807}
\newcommand{\retCISATburnCoarseLTwoVarLossGce}{0.069}
\newcommand{\nSATburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{66.2}
\newcommand{\miouCISATburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{2.4}
\newcommand{\dropSATburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{15.2}
\newcommand{\dropCISATburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{2.7}
\newcommand{\retSATburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.814}
\newcommand{\retCISATburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.030}
\newcommand{\nSATburnCoarseLTwoVarLrMultThree}{2}
\newcommand{\miouSATburnCoarseLTwoVarLrMultThree}{50.0}
\newcommand{\miouCISATburnCoarseLTwoVarLrMultThree}{66.4}
\newcommand{\dropSATburnCoarseLTwoVarLrMultThree}{27.0}
\newcommand{\dropCISATburnCoarseLTwoVarLrMultThree}{64.1}
\newcommand{\retSATburnCoarseLTwoVarLrMultThree}{0.649}
\newcommand{\retCISATburnCoarseLTwoVarLrMultThree}{0.843}
\newcommand{\nSATburnCoarseLTwoVarValLabelsClean}{5}
\newcommand{\miouSATburnCoarseLTwoVarValLabelsClean}{56.4}
\newcommand{\miouCISATburnCoarseLTwoVarValLabelsClean}{9.7}
\newcommand{\dropSATburnCoarseLTwoVarValLabelsClean}{19.5}
\newcommand{\dropCISATburnCoarseLTwoVarValLabelsClean}{10.7}
\newcommand{\retSATburnCoarseLTwoVarValLabelsClean}{0.744}
\newcommand{\retCISATburnCoarseLTwoVarValLabelsClean}{0.137}
\newcommand{\nSATburnCoarseLR}{5}
\newcommand{\miouSATburnCoarseLR}{52.2}
\newcommand{\miouCISATburnCoarseLR}{8.0}
\newcommand{\dropSATburnCoarseLR}{23.7}
\newcommand{\dropCISATburnCoarseLR}{8.9}
\newcommand{\retSATburnCoarseLR}{0.688}
\newcommand{\retCISATburnCoarseLR}{0.113}
\newcommand{\nSATburnCoarseLRVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATburnCoarseLRVarLrMultZeroThreeThreeThreeThree}{63.9}
\newcommand{\miouCISATburnCoarseLRVarLrMultZeroThreeThreeThreeThree}{1.1}
\newcommand{\dropSATburnCoarseLRVarLrMultZeroThreeThreeThreeThree}{17.5}
\newcommand{\dropCISATburnCoarseLRVarLrMultZeroThreeThreeThreeThree}{3.2}
\newcommand{\retSATburnCoarseLRVarLrMultZeroThreeThreeThreeThree}{0.786}
\newcommand{\retCISATburnCoarseLRVarLrMultZeroThreeThreeThreeThree}{0.034}
\newcommand{\nSATburnOmissionLOne}{5}
\newcommand{\miouSATburnOmissionLOne}{66.9}
\newcommand{\miouCISATburnOmissionLOne}{4.0}
\newcommand{\dropSATburnOmissionLOne}{9.0}
\newcommand{\dropCISATburnOmissionLOne}{3.4}
\newcommand{\retSATburnOmissionLOne}{0.882}
\newcommand{\retCISATburnOmissionLOne}{0.045}
\newcommand{\nSATburnOmissionLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouSATburnOmissionLOneVarDecoderMaskTwoformerFull}{67.2}
\newcommand{\miouCISATburnOmissionLOneVarDecoderMaskTwoformerFull}{5.8}
\newcommand{\dropSATburnOmissionLOneVarDecoderMaskTwoformerFull}{3.3}
\newcommand{\dropCISATburnOmissionLOneVarDecoderMaskTwoformerFull}{10.0}
\newcommand{\retSATburnOmissionLOneVarDecoderMaskTwoformerFull}{0.958}
\newcommand{\retCISATburnOmissionLOneVarDecoderMaskTwoformerFull}{0.134}
\newcommand{\nSATburnOmissionLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATburnOmissionLOneVarDecoderMaskTwoformerLite}{44.8}
\newcommand{\miouCISATburnOmissionLOneVarDecoderMaskTwoformerLite}{0.0}
\newcommand{\dropSATburnOmissionLOneVarDecoderMaskTwoformerLite}{15.2}
\newcommand{\dropCISATburnOmissionLOneVarDecoderMaskTwoformerLite}{19.6}
\newcommand{\retSATburnOmissionLOneVarDecoderMaskTwoformerLite}{0.789}
\newcommand{\retCISATburnOmissionLOneVarDecoderMaskTwoformerLite}{0.256}
\newcommand{\nSATburnOmissionLOneVarDecoderSamLite}{5}
\newcommand{\miouSATburnOmissionLOneVarDecoderSamLite}{64.1}
\newcommand{\miouCISATburnOmissionLOneVarDecoderSamLite}{2.1}
\newcommand{\dropSATburnOmissionLOneVarDecoderSamLite}{9.6}
\newcommand{\dropCISATburnOmissionLOneVarDecoderSamLite}{2.8}
\newcommand{\retSATburnOmissionLOneVarDecoderSamLite}{0.870}
\newcommand{\retCISATburnOmissionLOneVarDecoderSamLite}{0.035}
\newcommand{\nSATburnOmissionLOneVarDecoderSamPretrained}{5}
\newcommand{\miouSATburnOmissionLOneVarDecoderSamPretrained}{58.9}
\newcommand{\miouCISATburnOmissionLOneVarDecoderSamPretrained}{12.2}
\newcommand{\dropSATburnOmissionLOneVarDecoderSamPretrained}{5.2}
\newcommand{\dropCISATburnOmissionLOneVarDecoderSamPretrained}{13.1}
\newcommand{\retSATburnOmissionLOneVarDecoderSamPretrained}{0.936}
\newcommand{\retCISATburnOmissionLOneVarDecoderSamPretrained}{0.228}
\newcommand{\nSATburnOmissionLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouSATburnOmissionLOneVarDecoderSegformerMlp}{66.0}
\newcommand{\miouCISATburnOmissionLOneVarDecoderSegformerMlp}{5.6}
\newcommand{\dropSATburnOmissionLOneVarDecoderSegformerMlp}{14.0}
\newcommand{\dropCISATburnOmissionLOneVarDecoderSegformerMlp}{6.9}
\newcommand{\retSATburnOmissionLOneVarDecoderSegformerMlp}{0.826}
\newcommand{\retCISATburnOmissionLOneVarDecoderSegformerMlp}{0.083}
\newcommand{\nSATburnOmissionLTwo}{8}
\newcommand{\miouSATburnOmissionLTwo}{55.8}
\newcommand{\miouCISATburnOmissionLTwo}{4.4}
\newcommand{\dropSATburnOmissionLTwo}{21.2}
\newcommand{\dropCISATburnOmissionLTwo}{6.2}
\newcommand{\retSATburnOmissionLTwo}{0.728}
\newcommand{\retCISATburnOmissionLTwo}{0.073}
\newcommand{\nSATburnOmissionLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouSATburnOmissionLTwoVarDecoderMaskTwoformerFull}{57.2}
\newcommand{\miouCISATburnOmissionLTwoVarDecoderMaskTwoformerFull}{2.3}
\newcommand{\dropSATburnOmissionLTwoVarDecoderMaskTwoformerFull}{13.3}
\newcommand{\dropCISATburnOmissionLTwoVarDecoderMaskTwoformerFull}{3.8}
\newcommand{\retSATburnOmissionLTwoVarDecoderMaskTwoformerFull}{0.812}
\newcommand{\retCISATburnOmissionLTwoVarDecoderMaskTwoformerFull}{0.042}
\newcommand{\nSATburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{63.6}
\newcommand{\miouCISATburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{3.7}
\newcommand{\dropSATburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{13.5}
\newcommand{\dropCISATburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{5.1}
\newcommand{\retSATburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{0.826}
\newcommand{\retCISATburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{0.062}
\newcommand{\nSATburnOmissionLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATburnOmissionLTwoVarDecoderMaskTwoformerLite}{44.8}
\newcommand{\miouCISATburnOmissionLTwoVarDecoderMaskTwoformerLite}{0.0}
\newcommand{\dropSATburnOmissionLTwoVarDecoderMaskTwoformerLite}{15.2}
\newcommand{\dropCISATburnOmissionLTwoVarDecoderMaskTwoformerLite}{19.6}
\newcommand{\retSATburnOmissionLTwoVarDecoderMaskTwoformerLite}{0.789}
\newcommand{\retCISATburnOmissionLTwoVarDecoderMaskTwoformerLite}{0.256}
\newcommand{\nSATburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{50.5}
\newcommand{\miouCISATburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{11.2}
\newcommand{\dropSATburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{30.8}
\newcommand{\dropCISATburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{10.5}
\newcommand{\retSATburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{0.620}
\newcommand{\retCISATburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{0.132}
\newcommand{\nSATburnOmissionLTwoVarDecoderSamLite}{5}
\newcommand{\miouSATburnOmissionLTwoVarDecoderSamLite}{48.0}
\newcommand{\miouCISATburnOmissionLTwoVarDecoderSamLite}{7.3}
\newcommand{\dropSATburnOmissionLTwoVarDecoderSamLite}{25.7}
\newcommand{\dropCISATburnOmissionLTwoVarDecoderSamLite}{9.4}
\newcommand{\retSATburnOmissionLTwoVarDecoderSamLite}{0.653}
\newcommand{\retCISATburnOmissionLTwoVarDecoderSamLite}{0.121}
\newcommand{\nSATburnOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATburnOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{56.5}
\newcommand{\miouCISATburnOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{10.0}
\newcommand{\dropSATburnOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{17.9}
\newcommand{\dropCISATburnOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{10.6}
\newcommand{\retSATburnOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{0.760}
\newcommand{\retCISATburnOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{0.138}
\newcommand{\nSATburnOmissionLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouSATburnOmissionLTwoVarDecoderSamPretrained}{54.3}
\newcommand{\miouCISATburnOmissionLTwoVarDecoderSamPretrained}{9.0}
\newcommand{\dropSATburnOmissionLTwoVarDecoderSamPretrained}{9.9}
\newcommand{\dropCISATburnOmissionLTwoVarDecoderSamPretrained}{19.3}
\newcommand{\retSATburnOmissionLTwoVarDecoderSamPretrained}{0.882}
\newcommand{\retCISATburnOmissionLTwoVarDecoderSamPretrained}{0.346}
\newcommand{\nSATburnOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATburnOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{55.9}
\newcommand{\miouCISATburnOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{3.9}
\newcommand{\dropSATburnOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{22.0}
\newcommand{\dropCISATburnOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{7.0}
\newcommand{\retSATburnOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{0.720}
\newcommand{\retCISATburnOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{0.079}
\newcommand{\nSATburnOmissionLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouSATburnOmissionLTwoVarDecoderSegformerMlp}{58.9}
\newcommand{\miouCISATburnOmissionLTwoVarDecoderSegformerMlp}{3.1}
\newcommand{\dropSATburnOmissionLTwoVarDecoderSegformerMlp}{21.1}
\newcommand{\dropCISATburnOmissionLTwoVarDecoderSegformerMlp}{3.3}
\newcommand{\retSATburnOmissionLTwoVarDecoderSegformerMlp}{0.737}
\newcommand{\retCISATburnOmissionLTwoVarDecoderSegformerMlp}{0.038}
\newcommand{\nSATburnOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATburnOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{61.6}
\newcommand{\miouCISATburnOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{8.8}
\newcommand{\dropSATburnOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{21.9}
\newcommand{\dropCISATburnOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{9.2}
\newcommand{\retSATburnOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{0.738}
\newcommand{\retCISATburnOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{0.109}
\newcommand{\nSATburnOmissionLTwoVarLossBootstrap}{5}
\newcommand{\miouSATburnOmissionLTwoVarLossBootstrap}{53.2}
\newcommand{\miouCISATburnOmissionLTwoVarLossBootstrap}{5.9}
\newcommand{\dropSATburnOmissionLTwoVarLossBootstrap}{19.0}
\newcommand{\dropCISATburnOmissionLTwoVarLossBootstrap}{7.2}
\newcommand{\retSATburnOmissionLTwoVarLossBootstrap}{0.738}
\newcommand{\retCISATburnOmissionLTwoVarLossBootstrap}{0.093}
\newcommand{\nSATburnOmissionLTwoVarLossGce}{5}
\newcommand{\miouSATburnOmissionLTwoVarLossGce}{53.9}
\newcommand{\miouCISATburnOmissionLTwoVarLossGce}{3.2}
\newcommand{\dropSATburnOmissionLTwoVarLossGce}{16.6}
\newcommand{\dropCISATburnOmissionLTwoVarLossGce}{5.8}
\newcommand{\retSATburnOmissionLTwoVarLossGce}{0.767}
\newcommand{\retCISATburnOmissionLTwoVarLossGce}{0.064}
\newcommand{\nSATburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{63.6}
\newcommand{\miouCISATburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{7.2}
\newcommand{\dropSATburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{17.8}
\newcommand{\dropCISATburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{7.8}
\newcommand{\retSATburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{0.782}
\newcommand{\retCISATburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{0.092}
\newcommand{\nSATburnOmissionLR}{5}
\newcommand{\miouSATburnOmissionLR}{49.5}
\newcommand{\miouCISATburnOmissionLR}{7.7}
\newcommand{\dropSATburnOmissionLR}{26.3}
\newcommand{\dropCISATburnOmissionLR}{6.5}
\newcommand{\retSATburnOmissionLR}{0.652}
\newcommand{\retCISATburnOmissionLR}{0.090}
\newcommand{\nSATburnOmissionLRVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATburnOmissionLRVarLrMultZeroThreeThreeThreeThree}{52.4}
\newcommand{\miouCISATburnOmissionLRVarLrMultZeroThreeThreeThreeThree}{7.4}
\newcommand{\dropSATburnOmissionLRVarLrMultZeroThreeThreeThreeThree}{28.9}
\newcommand{\dropCISATburnOmissionLRVarLrMultZeroThreeThreeThreeThree}{7.1}
\newcommand{\retSATburnOmissionLRVarLrMultZeroThreeThreeThreeThree}{0.645}
\newcommand{\retCISATburnOmissionLRVarLrMultZeroThreeThreeThreeThree}{0.087}
\newcommand{\nSATburnShiftLOne}{5}
\newcommand{\miouSATburnShiftLOne}{75.7}
\newcommand{\miouCISATburnShiftLOne}{3.4}
\newcommand{\dropSATburnShiftLOne}{0.1}
\newcommand{\dropCISATburnShiftLOne}{4.8}
\newcommand{\retSATburnShiftLOne}{0.999}
\newcommand{\retCISATburnShiftLOne}{0.063}
\newcommand{\nSATburnShiftLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouSATburnShiftLOneVarDecoderMaskTwoformerFull}{67.3}
\newcommand{\miouCISATburnShiftLOneVarDecoderMaskTwoformerFull}{2.5}
\newcommand{\dropSATburnShiftLOneVarDecoderMaskTwoformerFull}{3.2}
\newcommand{\dropCISATburnShiftLOneVarDecoderMaskTwoformerFull}{4.0}
\newcommand{\retSATburnShiftLOneVarDecoderMaskTwoformerFull}{0.956}
\newcommand{\retCISATburnShiftLOneVarDecoderMaskTwoformerFull}{0.051}
\newcommand{\nSATburnShiftLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATburnShiftLOneVarDecoderMaskTwoformerLite}{63.7}
\newcommand{\miouCISATburnShiftLOneVarDecoderMaskTwoformerLite}{14.6}
\newcommand{\dropSATburnShiftLOneVarDecoderMaskTwoformerLite}{\ensuremath{-}3.7}
\newcommand{\dropCISATburnShiftLOneVarDecoderMaskTwoformerLite}{14.6}
\newcommand{\retSATburnShiftLOneVarDecoderMaskTwoformerLite}{1.094}
\newcommand{\retCISATburnShiftLOneVarDecoderMaskTwoformerLite}{0.303}
\newcommand{\nSATburnShiftLOneVarDecoderSamLite}{5}
\newcommand{\miouSATburnShiftLOneVarDecoderSamLite}{70.7}
\newcommand{\miouCISATburnShiftLOneVarDecoderSamLite}{2.6}
\newcommand{\dropSATburnShiftLOneVarDecoderSamLite}{3.1}
\newcommand{\dropCISATburnShiftLOneVarDecoderSamLite}{4.3}
\newcommand{\retSATburnShiftLOneVarDecoderSamLite}{0.959}
\newcommand{\retCISATburnShiftLOneVarDecoderSamLite}{0.057}
\newcommand{\nSATburnShiftLOneVarDecoderSamPretrained}{5}
\newcommand{\miouSATburnShiftLOneVarDecoderSamPretrained}{64.3}
\newcommand{\miouCISATburnShiftLOneVarDecoderSamPretrained}{13.7}
\newcommand{\dropSATburnShiftLOneVarDecoderSamPretrained}{\ensuremath{-}0.1}
\newcommand{\dropCISATburnShiftLOneVarDecoderSamPretrained}{8.3}
\newcommand{\retSATburnShiftLOneVarDecoderSamPretrained}{1.007}
\newcommand{\retCISATburnShiftLOneVarDecoderSamPretrained}{0.122}
\newcommand{\nSATburnShiftLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouSATburnShiftLOneVarDecoderSegformerMlp}{68.8}
\newcommand{\miouCISATburnShiftLOneVarDecoderSegformerMlp}{16.9}
\newcommand{\dropSATburnShiftLOneVarDecoderSegformerMlp}{11.2}
\newcommand{\dropCISATburnShiftLOneVarDecoderSegformerMlp}{18.7}
\newcommand{\retSATburnShiftLOneVarDecoderSegformerMlp}{0.863}
\newcommand{\retCISATburnShiftLOneVarDecoderSegformerMlp}{0.229}
\newcommand{\nSATburnShiftLTwo}{8}
\newcommand{\miouSATburnShiftLTwo}{62.3}
\newcommand{\miouCISATburnShiftLTwo}{2.2}
\newcommand{\dropSATburnShiftLTwo}{14.7}
\newcommand{\dropCISATburnShiftLTwo}{2.9}
\newcommand{\retSATburnShiftLTwo}{0.810}
\newcommand{\retCISATburnShiftLTwo}{0.034}
\newcommand{\nSATburnShiftLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouSATburnShiftLTwoVarDecoderMaskTwoformerFull}{58.0}
\newcommand{\miouCISATburnShiftLTwoVarDecoderMaskTwoformerFull}{3.3}
\newcommand{\dropSATburnShiftLTwoVarDecoderMaskTwoformerFull}{12.5}
\newcommand{\dropCISATburnShiftLTwoVarDecoderMaskTwoformerFull}{6.1}
\newcommand{\retSATburnShiftLTwoVarDecoderMaskTwoformerFull}{0.825}
\newcommand{\retCISATburnShiftLTwoVarDecoderMaskTwoformerFull}{0.075}
\newcommand{\nSATburnShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATburnShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{64.3}
\newcommand{\miouCISATburnShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{3.1}
\newcommand{\dropSATburnShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{12.9}
\newcommand{\dropCISATburnShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{4.2}
\newcommand{\retSATburnShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{0.834}
\newcommand{\retCISATburnShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{0.051}
\newcommand{\nSATburnShiftLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATburnShiftLTwoVarDecoderMaskTwoformerLite}{59.4}
\newcommand{\miouCISATburnShiftLTwoVarDecoderMaskTwoformerLite}{5.7}
\newcommand{\dropSATburnShiftLTwoVarDecoderMaskTwoformerLite}{0.6}
\newcommand{\dropCISATburnShiftLTwoVarDecoderMaskTwoformerLite}{23.5}
\newcommand{\retSATburnShiftLTwoVarDecoderMaskTwoformerLite}{1.056}
\newcommand{\retCISATburnShiftLTwoVarDecoderMaskTwoformerLite}{0.397}
\newcommand{\nSATburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{70.7}
\newcommand{\miouCISATburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{1.9}
\newcommand{\dropSATburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{10.6}
\newcommand{\dropCISATburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{2.7}
\newcommand{\retSATburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{0.870}
\newcommand{\retCISATburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{0.031}
\newcommand{\nSATburnShiftLTwoVarDecoderSamLite}{5}
\newcommand{\miouSATburnShiftLTwoVarDecoderSamLite}{57.7}
\newcommand{\miouCISATburnShiftLTwoVarDecoderSamLite}{10.0}
\newcommand{\dropSATburnShiftLTwoVarDecoderSamLite}{16.0}
\newcommand{\dropCISATburnShiftLTwoVarDecoderSamLite}{7.9}
\newcommand{\retSATburnShiftLTwoVarDecoderSamLite}{0.781}
\newcommand{\retCISATburnShiftLTwoVarDecoderSamLite}{0.116}
\newcommand{\nSATburnShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATburnShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{64.5}
\newcommand{\miouCISATburnShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{2.5}
\newcommand{\dropSATburnShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{9.9}
\newcommand{\dropCISATburnShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{5.1}
\newcommand{\retSATburnShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{0.869}
\newcommand{\retCISATburnShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{0.064}
\newcommand{\nSATburnShiftLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouSATburnShiftLTwoVarDecoderSamPretrained}{52.8}
\newcommand{\miouCISATburnShiftLTwoVarDecoderSamPretrained}{10.5}
\newcommand{\dropSATburnShiftLTwoVarDecoderSamPretrained}{11.4}
\newcommand{\dropCISATburnShiftLTwoVarDecoderSamPretrained}{10.9}
\newcommand{\retSATburnShiftLTwoVarDecoderSamPretrained}{0.835}
\newcommand{\retCISATburnShiftLTwoVarDecoderSamPretrained}{0.160}
\newcommand{\nSATburnShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATburnShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{54.1}
\newcommand{\miouCISATburnShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{15.9}
\newcommand{\dropSATburnShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{23.7}
\newcommand{\dropCISATburnShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{13.1}
\newcommand{\retSATburnShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{0.692}
\newcommand{\retCISATburnShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{0.177}
\newcommand{\nSATburnShiftLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouSATburnShiftLTwoVarDecoderSegformerMlp}{64.9}
\newcommand{\miouCISATburnShiftLTwoVarDecoderSegformerMlp}{5.0}
\newcommand{\dropSATburnShiftLTwoVarDecoderSegformerMlp}{15.1}
\newcommand{\dropCISATburnShiftLTwoVarDecoderSegformerMlp}{4.8}
\newcommand{\retSATburnShiftLTwoVarDecoderSegformerMlp}{0.812}
\newcommand{\retCISATburnShiftLTwoVarDecoderSegformerMlp}{0.060}
\newcommand{\nSATburnShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATburnShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{68.6}
\newcommand{\miouCISATburnShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{3.7}
\newcommand{\dropSATburnShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{15.0}
\newcommand{\dropCISATburnShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{3.7}
\newcommand{\retSATburnShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{0.820}
\newcommand{\retCISATburnShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{0.043}
\newcommand{\nSATburnShiftLTwoVarLossBootstrap}{5}
\newcommand{\miouSATburnShiftLTwoVarLossBootstrap}{62.4}
\newcommand{\miouCISATburnShiftLTwoVarLossBootstrap}{3.4}
\newcommand{\dropSATburnShiftLTwoVarLossBootstrap}{9.7}
\newcommand{\dropCISATburnShiftLTwoVarLossBootstrap}{3.8}
\newcommand{\retSATburnShiftLTwoVarLossBootstrap}{0.866}
\newcommand{\retCISATburnShiftLTwoVarLossBootstrap}{0.049}
\newcommand{\nSATburnShiftLTwoVarLossGce}{5}
\newcommand{\miouSATburnShiftLTwoVarLossGce}{64.2}
\newcommand{\miouCISATburnShiftLTwoVarLossGce}{2.1}
\newcommand{\dropSATburnShiftLTwoVarLossGce}{6.4}
\newcommand{\dropCISATburnShiftLTwoVarLossGce}{7.8}
\newcommand{\retSATburnShiftLTwoVarLossGce}{0.914}
\newcommand{\retCISATburnShiftLTwoVarLossGce}{0.103}
\newcommand{\nSATburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{69.4}
\newcommand{\miouCISATburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{2.5}
\newcommand{\dropSATburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{11.9}
\newcommand{\dropCISATburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{2.6}
\newcommand{\retSATburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.854}
\newcommand{\retCISATburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.029}
\newcommand{\nSATburnShiftLR}{5}
\newcommand{\miouSATburnShiftLR}{55.7}
\newcommand{\miouCISATburnShiftLR}{7.5}
\newcommand{\dropSATburnShiftLR}{20.1}
\newcommand{\dropCISATburnShiftLR}{8.7}
\newcommand{\retSATburnShiftLR}{0.736}
\newcommand{\retCISATburnShiftLR}{0.110}
\newcommand{\nSATburnShiftLRVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATburnShiftLRVarLrMultZeroThreeThreeThreeThree}{65.1}
\newcommand{\miouCISATburnShiftLRVarLrMultZeroThreeThreeThreeThree}{1.6}
\newcommand{\dropSATburnShiftLRVarLrMultZeroThreeThreeThreeThree}{16.2}
\newcommand{\dropCISATburnShiftLRVarLrMultZeroThreeThreeThreeThree}{2.2}
\newcommand{\retSATburnShiftLRVarLrMultZeroThreeThreeThreeThree}{0.801}
\newcommand{\retCISATburnShiftLRVarLrMultZeroThreeThreeThreeThree}{0.022}
\newcommand{\nSATChesBoundaryLOne}{5}
\newcommand{\miouSATChesBoundaryLOne}{79.1}
\newcommand{\miouCISATChesBoundaryLOne}{0.8}
\newcommand{\dropSATChesBoundaryLOne}{2.2}
\newcommand{\dropCISATChesBoundaryLOne}{1.0}
\newcommand{\retSATChesBoundaryLOne}{0.974}
\newcommand{\retCISATChesBoundaryLOne}{0.012}
\newcommand{\nSATChesBoundaryLTwo}{5}
\newcommand{\miouSATChesBoundaryLTwo}{69.3}
\newcommand{\miouCISATChesBoundaryLTwo}{0.6}
\newcommand{\dropSATChesBoundaryLTwo}{12.0}
\newcommand{\dropCISATChesBoundaryLTwo}{0.9}
\newcommand{\retSATChesBoundaryLTwo}{0.852}
\newcommand{\retCISATChesBoundaryLTwo}{0.010}
\newcommand{\nSATChesBoundaryLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATChesBoundaryLTwoVarDecoderMaskTwoformerLite}{68.5}
\newcommand{\miouCISATChesBoundaryLTwoVarDecoderMaskTwoformerLite}{1.8}
\newcommand{\dropSATChesBoundaryLTwoVarDecoderMaskTwoformerLite}{12.9}
\newcommand{\dropCISATChesBoundaryLTwoVarDecoderMaskTwoformerLite}{2.3}
\newcommand{\retSATChesBoundaryLTwoVarDecoderMaskTwoformerLite}{0.842}
\newcommand{\retCISATChesBoundaryLTwoVarDecoderMaskTwoformerLite}{0.026}
\newcommand{\nSATChesBoundaryLTwoVarDecoderSamLite}{5}
\newcommand{\miouSATChesBoundaryLTwoVarDecoderSamLite}{69.0}
\newcommand{\miouCISATChesBoundaryLTwoVarDecoderSamLite}{1.3}
\newcommand{\dropSATChesBoundaryLTwoVarDecoderSamLite}{11.8}
\newcommand{\dropCISATChesBoundaryLTwoVarDecoderSamLite}{1.2}
\newcommand{\retSATChesBoundaryLTwoVarDecoderSamLite}{0.854}
\newcommand{\retCISATChesBoundaryLTwoVarDecoderSamLite}{0.015}
\newcommand{\nSATChesBoundaryLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouSATChesBoundaryLTwoVarDecoderSegformerMlp}{71.4}
\newcommand{\miouCISATChesBoundaryLTwoVarDecoderSegformerMlp}{1.1}
\newcommand{\dropSATChesBoundaryLTwoVarDecoderSegformerMlp}{9.7}
\newcommand{\dropCISATChesBoundaryLTwoVarDecoderSegformerMlp}{1.2}
\newcommand{\retSATChesBoundaryLTwoVarDecoderSegformerMlp}{0.880}
\newcommand{\retCISATChesBoundaryLTwoVarDecoderSegformerMlp}{0.014}
\newcommand{\nSATChesBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATChesBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{69.3}
\newcommand{\miouCISATChesBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{0.6}
\newcommand{\dropSATChesBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{10.8}
\newcommand{\dropCISATChesBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{0.6}
\newcommand{\retSATChesBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{0.865}
\newcommand{\retCISATChesBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{0.007}
\newcommand{\nSATChesClean}{5}
\newcommand{\miouSATChesClean}{81.3}
\newcommand{\miouCISATChesClean}{0.9}
\newcommand{\nSATChesCleanVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATChesCleanVarDecoderMaskTwoformerLite}{81.4}
\newcommand{\miouCISATChesCleanVarDecoderMaskTwoformerLite}{1.5}
\newcommand{\nSATChesCleanVarDecoderSamLite}{5}
\newcommand{\miouSATChesCleanVarDecoderSamLite}{80.8}
\newcommand{\miouCISATChesCleanVarDecoderSamLite}{0.8}
\newcommand{\nSATChesCleanVarDecoderSegformerMlp}{5}
\newcommand{\miouSATChesCleanVarDecoderSegformerMlp}{81.1}
\newcommand{\miouCISATChesCleanVarDecoderSegformerMlp}{1.3}
\newcommand{\nSATChesCleanVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATChesCleanVarLrMultZeroThreeThreeThreeThree}{80.1}
\newcommand{\miouCISATChesCleanVarLrMultZeroThreeThreeThreeThree}{0.5}
\newcommand{\nSATChesCoarseLOne}{5}
\newcommand{\miouSATChesCoarseLOne}{80.7}
\newcommand{\miouCISATChesCoarseLOne}{0.6}
\newcommand{\dropSATChesCoarseLOne}{0.6}
\newcommand{\dropCISATChesCoarseLOne}{1.1}
\newcommand{\retSATChesCoarseLOne}{0.992}
\newcommand{\retCISATChesCoarseLOne}{0.013}
\newcommand{\nSATChesCoarseLTwo}{5}
\newcommand{\miouSATChesCoarseLTwo}{69.5}
\newcommand{\miouCISATChesCoarseLTwo}{1.0}
\newcommand{\dropSATChesCoarseLTwo}{11.8}
\newcommand{\dropCISATChesCoarseLTwo}{0.8}
\newcommand{\retSATChesCoarseLTwo}{0.854}
\newcommand{\retCISATChesCoarseLTwo}{0.010}
\newcommand{\nSATChesCoarseLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATChesCoarseLTwoVarDecoderMaskTwoformerLite}{69.4}
\newcommand{\miouCISATChesCoarseLTwoVarDecoderMaskTwoformerLite}{0.8}
\newcommand{\dropSATChesCoarseLTwoVarDecoderMaskTwoformerLite}{12.0}
\newcommand{\dropCISATChesCoarseLTwoVarDecoderMaskTwoformerLite}{1.2}
\newcommand{\retSATChesCoarseLTwoVarDecoderMaskTwoformerLite}{0.852}
\newcommand{\retCISATChesCoarseLTwoVarDecoderMaskTwoformerLite}{0.013}
\newcommand{\nSATChesCoarseLTwoVarDecoderSamLite}{5}
\newcommand{\miouSATChesCoarseLTwoVarDecoderSamLite}{68.1}
\newcommand{\miouCISATChesCoarseLTwoVarDecoderSamLite}{0.6}
\newcommand{\dropSATChesCoarseLTwoVarDecoderSamLite}{12.7}
\newcommand{\dropCISATChesCoarseLTwoVarDecoderSamLite}{1.3}
\newcommand{\retSATChesCoarseLTwoVarDecoderSamLite}{0.843}
\newcommand{\retCISATChesCoarseLTwoVarDecoderSamLite}{0.015}
\newcommand{\nSATChesCoarseLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouSATChesCoarseLTwoVarDecoderSegformerMlp}{69.4}
\newcommand{\miouCISATChesCoarseLTwoVarDecoderSegformerMlp}{0.4}
\newcommand{\dropSATChesCoarseLTwoVarDecoderSegformerMlp}{11.7}
\newcommand{\dropCISATChesCoarseLTwoVarDecoderSegformerMlp}{1.6}
\newcommand{\retSATChesCoarseLTwoVarDecoderSegformerMlp}{0.855}
\newcommand{\retCISATChesCoarseLTwoVarDecoderSegformerMlp}{0.018}
\newcommand{\nSATChesCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATChesCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{69.2}
\newcommand{\miouCISATChesCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{1.0}
\newcommand{\dropSATChesCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{10.9}
\newcommand{\dropCISATChesCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{1.0}
\newcommand{\retSATChesCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.864}
\newcommand{\retCISATChesCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.012}
\newcommand{\nSATChesNlcdREAL}{5}
\newcommand{\miouSATChesNlcdREAL}{59.9}
\newcommand{\miouCISATChesNlcdREAL}{0.5}
\newcommand{\dropSATChesNlcdREAL}{21.4}
\newcommand{\dropCISATChesNlcdREAL}{1.1}
\newcommand{\retSATChesNlcdREAL}{0.737}
\newcommand{\retCISATChesNlcdREAL}{0.011}
\newcommand{\nSATChesOmissionLOne}{5}
\newcommand{\miouSATChesOmissionLOne}{78.4}
\newcommand{\miouCISATChesOmissionLOne}{1.8}
\newcommand{\dropSATChesOmissionLOne}{2.9}
\newcommand{\dropCISATChesOmissionLOne}{2.5}
\newcommand{\retSATChesOmissionLOne}{0.964}
\newcommand{\retCISATChesOmissionLOne}{0.030}
\newcommand{\nSATChesOmissionLTwo}{5}
\newcommand{\miouSATChesOmissionLTwo}{70.9}
\newcommand{\miouCISATChesOmissionLTwo}{4.4}
\newcommand{\dropSATChesOmissionLTwo}{10.4}
\newcommand{\dropCISATChesOmissionLTwo}{5.0}
\newcommand{\retSATChesOmissionLTwo}{0.872}
\newcommand{\retCISATChesOmissionLTwo}{0.060}
\newcommand{\nSATChesOmissionLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATChesOmissionLTwoVarDecoderMaskTwoformerLite}{68.9}
\newcommand{\miouCISATChesOmissionLTwoVarDecoderMaskTwoformerLite}{9.9}
\newcommand{\dropSATChesOmissionLTwoVarDecoderMaskTwoformerLite}{12.6}
\newcommand{\dropCISATChesOmissionLTwoVarDecoderMaskTwoformerLite}{10.1}
\newcommand{\retSATChesOmissionLTwoVarDecoderMaskTwoformerLite}{0.846}
\newcommand{\retCISATChesOmissionLTwoVarDecoderMaskTwoformerLite}{0.122}
\newcommand{\nSATChesOmissionLTwoVarDecoderSamLite}{5}
\newcommand{\miouSATChesOmissionLTwoVarDecoderSamLite}{71.3}
\newcommand{\miouCISATChesOmissionLTwoVarDecoderSamLite}{2.5}
\newcommand{\dropSATChesOmissionLTwoVarDecoderSamLite}{9.5}
\newcommand{\dropCISATChesOmissionLTwoVarDecoderSamLite}{2.5}
\newcommand{\retSATChesOmissionLTwoVarDecoderSamLite}{0.883}
\newcommand{\retCISATChesOmissionLTwoVarDecoderSamLite}{0.031}
\newcommand{\nSATChesOmissionLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouSATChesOmissionLTwoVarDecoderSegformerMlp}{70.8}
\newcommand{\miouCISATChesOmissionLTwoVarDecoderSegformerMlp}{4.4}
\newcommand{\dropSATChesOmissionLTwoVarDecoderSegformerMlp}{10.4}
\newcommand{\dropCISATChesOmissionLTwoVarDecoderSegformerMlp}{4.9}
\newcommand{\retSATChesOmissionLTwoVarDecoderSegformerMlp}{0.873}
\newcommand{\retCISATChesOmissionLTwoVarDecoderSegformerMlp}{0.060}
\newcommand{\nSATChesOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATChesOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{69.7}
\newcommand{\miouCISATChesOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{2.3}
\newcommand{\dropSATChesOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{10.4}
\newcommand{\dropCISATChesOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{2.4}
\newcommand{\retSATChesOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{0.870}
\newcommand{\retCISATChesOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{0.029}
\newcommand{\nSATChesShiftLOne}{5}
\newcommand{\miouSATChesShiftLOne}{80.7}
\newcommand{\miouCISATChesShiftLOne}{1.2}
\newcommand{\dropSATChesShiftLOne}{0.5}
\newcommand{\dropCISATChesShiftLOne}{1.7}
\newcommand{\retSATChesShiftLOne}{0.993}
\newcommand{\retCISATChesShiftLOne}{0.021}
\newcommand{\nSATChesShiftLTwo}{5}
\newcommand{\miouSATChesShiftLTwo}{74.9}
\newcommand{\miouCISATChesShiftLTwo}{1.1}
\newcommand{\dropSATChesShiftLTwo}{6.4}
\newcommand{\dropCISATChesShiftLTwo}{1.4}
\newcommand{\retSATChesShiftLTwo}{0.921}
\newcommand{\retCISATChesShiftLTwo}{0.017}
\newcommand{\nSATChesShiftLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATChesShiftLTwoVarDecoderMaskTwoformerLite}{73.2}
\newcommand{\miouCISATChesShiftLTwoVarDecoderMaskTwoformerLite}{1.1}
\newcommand{\dropSATChesShiftLTwoVarDecoderMaskTwoformerLite}{8.3}
\newcommand{\dropCISATChesShiftLTwoVarDecoderMaskTwoformerLite}{1.0}
\newcommand{\retSATChesShiftLTwoVarDecoderMaskTwoformerLite}{0.899}
\newcommand{\retCISATChesShiftLTwoVarDecoderMaskTwoformerLite}{0.011}
\newcommand{\nSATChesShiftLTwoVarDecoderSamLite}{5}
\newcommand{\miouSATChesShiftLTwoVarDecoderSamLite}{73.1}
\newcommand{\miouCISATChesShiftLTwoVarDecoderSamLite}{0.9}
\newcommand{\dropSATChesShiftLTwoVarDecoderSamLite}{7.7}
\newcommand{\dropCISATChesShiftLTwoVarDecoderSamLite}{1.3}
\newcommand{\retSATChesShiftLTwoVarDecoderSamLite}{0.905}
\newcommand{\retCISATChesShiftLTwoVarDecoderSamLite}{0.015}
\newcommand{\nSATChesShiftLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouSATChesShiftLTwoVarDecoderSegformerMlp}{74.2}
\newcommand{\miouCISATChesShiftLTwoVarDecoderSegformerMlp}{0.9}
\newcommand{\dropSATChesShiftLTwoVarDecoderSegformerMlp}{7.0}
\newcommand{\dropCISATChesShiftLTwoVarDecoderSegformerMlp}{0.6}
\newcommand{\retSATChesShiftLTwoVarDecoderSegformerMlp}{0.914}
\newcommand{\retCISATChesShiftLTwoVarDecoderSegformerMlp}{0.006}
\newcommand{\nSATChesShiftLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATChesShiftLTwoVarLrMultZeroThreeThreeThreeThree}{74.1}
\newcommand{\miouCISATChesShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.8}
\newcommand{\dropSATChesShiftLTwoVarLrMultZeroThreeThreeThreeThree}{6.0}
\newcommand{\dropCISATChesShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.8}
\newcommand{\retSATChesShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.925}
\newcommand{\retCISATChesShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.010}
\newcommand{\nSATCsTwelveBoundaryLOne}{5}
\newcommand{\miouSATCsTwelveBoundaryLOne}{65.2}
\newcommand{\miouCISATCsTwelveBoundaryLOne}{1.4}
\newcommand{\dropSATCsTwelveBoundaryLOne}{1.4}
\newcommand{\dropCISATCsTwelveBoundaryLOne}{2.2}
\newcommand{\retSATCsTwelveBoundaryLOne}{0.979}
\newcommand{\retCISATCsTwelveBoundaryLOne}{0.033}
\newcommand{\nSATCsTwelveBoundaryLTwo}{5}
\newcommand{\miouSATCsTwelveBoundaryLTwo}{61.3}
\newcommand{\miouCISATCsTwelveBoundaryLTwo}{0.9}
\newcommand{\dropSATCsTwelveBoundaryLTwo}{5.2}
\newcommand{\dropCISATCsTwelveBoundaryLTwo}{1.0}
\newcommand{\retSATCsTwelveBoundaryLTwo}{0.922}
\newcommand{\retCISATCsTwelveBoundaryLTwo}{0.014}
\newcommand{\nSATCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}{60.7}
\newcommand{\miouCISATCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}{1.0}
\newcommand{\dropSATCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}{5.4}
\newcommand{\dropCISATCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}{2.2}
\newcommand{\retSATCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}{0.919}
\newcommand{\retCISATCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}{0.032}
\newcommand{\nSATCsTwelveBoundaryLTwoVarDecoderSamLite}{5}
\newcommand{\miouSATCsTwelveBoundaryLTwoVarDecoderSamLite}{61.2}
\newcommand{\miouCISATCsTwelveBoundaryLTwoVarDecoderSamLite}{0.8}
\newcommand{\dropSATCsTwelveBoundaryLTwoVarDecoderSamLite}{6.3}
\newcommand{\dropCISATCsTwelveBoundaryLTwoVarDecoderSamLite}{2.1}
\newcommand{\retSATCsTwelveBoundaryLTwoVarDecoderSamLite}{0.906}
\newcommand{\retCISATCsTwelveBoundaryLTwoVarDecoderSamLite}{0.029}
\newcommand{\nSATCsTwelveBoundaryLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouSATCsTwelveBoundaryLTwoVarDecoderSegformerMlp}{61.9}
\newcommand{\miouCISATCsTwelveBoundaryLTwoVarDecoderSegformerMlp}{0.4}
\newcommand{\dropSATCsTwelveBoundaryLTwoVarDecoderSegformerMlp}{5.5}
\newcommand{\dropCISATCsTwelveBoundaryLTwoVarDecoderSegformerMlp}{1.7}
\newcommand{\retSATCsTwelveBoundaryLTwoVarDecoderSegformerMlp}{0.919}
\newcommand{\retCISATCsTwelveBoundaryLTwoVarDecoderSegformerMlp}{0.023}
\newcommand{\nSATCsTwelveBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATCsTwelveBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{62.4}
\newcommand{\miouCISATCsTwelveBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{1.1}
\newcommand{\dropSATCsTwelveBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{6.3}
\newcommand{\dropCISATCsTwelveBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{1.4}
\newcommand{\retSATCsTwelveBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{0.909}
\newcommand{\retCISATCsTwelveBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{0.020}
\newcommand{\nSATCsTwelveClean}{5}
\newcommand{\miouSATCsTwelveClean}{66.6}
\newcommand{\miouCISATCsTwelveClean}{1.4}
\newcommand{\nSATCsTwelveCleanVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATCsTwelveCleanVarDecoderMaskTwoformerLite}{66.1}
\newcommand{\miouCISATCsTwelveCleanVarDecoderMaskTwoformerLite}{1.5}
\newcommand{\nSATCsTwelveCleanVarDecoderSamLite}{5}
\newcommand{\miouSATCsTwelveCleanVarDecoderSamLite}{67.5}
\newcommand{\miouCISATCsTwelveCleanVarDecoderSamLite}{1.7}
\newcommand{\nSATCsTwelveCleanVarDecoderSegformerMlp}{5}
\newcommand{\miouSATCsTwelveCleanVarDecoderSegformerMlp}{67.4}
\newcommand{\miouCISATCsTwelveCleanVarDecoderSegformerMlp}{1.8}
\newcommand{\nSATCsTwelveCleanVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATCsTwelveCleanVarLrMultZeroThreeThreeThreeThree}{68.7}
\newcommand{\miouCISATCsTwelveCleanVarLrMultZeroThreeThreeThreeThree}{0.4}
\newcommand{\nSATCsTwelveCoarseLOne}{5}
\newcommand{\miouSATCsTwelveCoarseLOne}{65.8}
\newcommand{\miouCISATCsTwelveCoarseLOne}{1.4}
\newcommand{\dropSATCsTwelveCoarseLOne}{0.7}
\newcommand{\dropCISATCsTwelveCoarseLOne}{2.3}
\newcommand{\retSATCsTwelveCoarseLOne}{0.990}
\newcommand{\retCISATCsTwelveCoarseLOne}{0.034}
\newcommand{\nSATCsTwelveCoarseLTwo}{5}
\newcommand{\miouSATCsTwelveCoarseLTwo}{59.9}
\newcommand{\miouCISATCsTwelveCoarseLTwo}{1.1}
\newcommand{\dropSATCsTwelveCoarseLTwo}{6.7}
\newcommand{\dropCISATCsTwelveCoarseLTwo}{1.7}
\newcommand{\retSATCsTwelveCoarseLTwo}{0.900}
\newcommand{\retCISATCsTwelveCoarseLTwo}{0.025}
\newcommand{\nSATCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}{59.7}
\newcommand{\miouCISATCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}{1.0}
\newcommand{\dropSATCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}{6.4}
\newcommand{\dropCISATCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}{1.9}
\newcommand{\retSATCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}{0.903}
\newcommand{\retCISATCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}{0.027}
\newcommand{\nSATCsTwelveCoarseLTwoVarDecoderSamLite}{5}
\newcommand{\miouSATCsTwelveCoarseLTwoVarDecoderSamLite}{59.3}
\newcommand{\miouCISATCsTwelveCoarseLTwoVarDecoderSamLite}{1.2}
\newcommand{\dropSATCsTwelveCoarseLTwoVarDecoderSamLite}{8.3}
\newcommand{\dropCISATCsTwelveCoarseLTwoVarDecoderSamLite}{2.2}
\newcommand{\retSATCsTwelveCoarseLTwoVarDecoderSamLite}{0.878}
\newcommand{\retCISATCsTwelveCoarseLTwoVarDecoderSamLite}{0.030}
\newcommand{\nSATCsTwelveCoarseLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouSATCsTwelveCoarseLTwoVarDecoderSegformerMlp}{59.8}
\newcommand{\miouCISATCsTwelveCoarseLTwoVarDecoderSegformerMlp}{1.0}
\newcommand{\dropSATCsTwelveCoarseLTwoVarDecoderSegformerMlp}{7.5}
\newcommand{\dropCISATCsTwelveCoarseLTwoVarDecoderSegformerMlp}{2.8}
\newcommand{\retSATCsTwelveCoarseLTwoVarDecoderSegformerMlp}{0.888}
\newcommand{\retCISATCsTwelveCoarseLTwoVarDecoderSegformerMlp}{0.039}
\newcommand{\nSATCsTwelveCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATCsTwelveCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{61.0}
\newcommand{\miouCISATCsTwelveCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.8}
\newcommand{\dropSATCsTwelveCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{7.7}
\newcommand{\dropCISATCsTwelveCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{1.0}
\newcommand{\retSATCsTwelveCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.888}
\newcommand{\retCISATCsTwelveCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.014}
\newcommand{\nSATCsTwelveOmissionLOne}{5}
\newcommand{\miouSATCsTwelveOmissionLOne}{63.6}
\newcommand{\miouCISATCsTwelveOmissionLOne}{1.5}
\newcommand{\dropSATCsTwelveOmissionLOne}{3.0}
\newcommand{\dropCISATCsTwelveOmissionLOne}{1.6}
\newcommand{\retSATCsTwelveOmissionLOne}{0.956}
\newcommand{\retCISATCsTwelveOmissionLOne}{0.024}
\newcommand{\nSATCsTwelveOmissionLTwo}{5}
\newcommand{\miouSATCsTwelveOmissionLTwo}{59.9}
\newcommand{\miouCISATCsTwelveOmissionLTwo}{1.5}
\newcommand{\dropSATCsTwelveOmissionLTwo}{6.6}
\newcommand{\dropCISATCsTwelveOmissionLTwo}{2.7}
\newcommand{\retSATCsTwelveOmissionLTwo}{0.901}
\newcommand{\retCISATCsTwelveOmissionLTwo}{0.038}
\newcommand{\nSATCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}{59.0}
\newcommand{\miouCISATCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}{1.6}
\newcommand{\dropSATCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}{7.2}
\newcommand{\dropCISATCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}{1.5}
\newcommand{\retSATCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}{0.891}
\newcommand{\retCISATCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}{0.022}
\newcommand{\nSATCsTwelveOmissionLTwoVarDecoderSamLite}{5}
\newcommand{\miouSATCsTwelveOmissionLTwoVarDecoderSamLite}{60.5}
\newcommand{\miouCISATCsTwelveOmissionLTwoVarDecoderSamLite}{1.2}
\newcommand{\dropSATCsTwelveOmissionLTwoVarDecoderSamLite}{7.1}
\newcommand{\dropCISATCsTwelveOmissionLTwoVarDecoderSamLite}{1.4}
\newcommand{\retSATCsTwelveOmissionLTwoVarDecoderSamLite}{0.896}
\newcommand{\retCISATCsTwelveOmissionLTwoVarDecoderSamLite}{0.020}
\newcommand{\nSATCsTwelveOmissionLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouSATCsTwelveOmissionLTwoVarDecoderSegformerMlp}{61.0}
\newcommand{\miouCISATCsTwelveOmissionLTwoVarDecoderSegformerMlp}{1.7}
\newcommand{\dropSATCsTwelveOmissionLTwoVarDecoderSegformerMlp}{6.4}
\newcommand{\dropCISATCsTwelveOmissionLTwoVarDecoderSegformerMlp}{2.9}
\newcommand{\retSATCsTwelveOmissionLTwoVarDecoderSegformerMlp}{0.905}
\newcommand{\retCISATCsTwelveOmissionLTwoVarDecoderSegformerMlp}{0.041}
\newcommand{\nSATCsTwelveOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATCsTwelveOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{60.4}
\newcommand{\miouCISATCsTwelveOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{1.6}
\newcommand{\dropSATCsTwelveOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{8.2}
\newcommand{\dropCISATCsTwelveOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{1.6}
\newcommand{\retSATCsTwelveOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{0.880}
\newcommand{\retCISATCsTwelveOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{0.023}
\newcommand{\nSATCsTwelveSTwocloudlessREAL}{5}
\newcommand{\miouSATCsTwelveSTwocloudlessREAL}{34.4}
\newcommand{\miouCISATCsTwelveSTwocloudlessREAL}{0.5}
\newcommand{\dropSATCsTwelveSTwocloudlessREAL}{32.2}
\newcommand{\dropCISATCsTwelveSTwocloudlessREAL}{1.6}
\newcommand{\retSATCsTwelveSTwocloudlessREAL}{0.516}
\newcommand{\retCISATCsTwelveSTwocloudlessREAL}{0.015}
\newcommand{\nSATCsTwelveShiftLOne}{5}
\newcommand{\miouSATCsTwelveShiftLOne}{66.4}
\newcommand{\miouCISATCsTwelveShiftLOne}{1.0}
\newcommand{\dropSATCsTwelveShiftLOne}{0.1}
\newcommand{\dropCISATCsTwelveShiftLOne}{0.6}
\newcommand{\retSATCsTwelveShiftLOne}{0.998}
\newcommand{\retCISATCsTwelveShiftLOne}{0.009}
\newcommand{\nSATCsTwelveShiftLTwo}{5}
\newcommand{\miouSATCsTwelveShiftLTwo}{61.6}
\newcommand{\miouCISATCsTwelveShiftLTwo}{0.6}
\newcommand{\dropSATCsTwelveShiftLTwo}{4.9}
\newcommand{\dropCISATCsTwelveShiftLTwo}{1.8}
\newcommand{\retSATCsTwelveShiftLTwo}{0.926}
\newcommand{\retCISATCsTwelveShiftLTwo}{0.025}
\newcommand{\nSATCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}{62.4}
\newcommand{\miouCISATCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}{1.5}
\newcommand{\dropSATCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}{3.7}
\newcommand{\dropCISATCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}{1.8}
\newcommand{\retSATCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}{0.943}
\newcommand{\retCISATCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}{0.027}
\newcommand{\nSATCsTwelveShiftLTwoVarDecoderSamLite}{5}
\newcommand{\miouSATCsTwelveShiftLTwoVarDecoderSamLite}{61.6}
\newcommand{\miouCISATCsTwelveShiftLTwoVarDecoderSamLite}{1.0}
\newcommand{\dropSATCsTwelveShiftLTwoVarDecoderSamLite}{5.9}
\newcommand{\dropCISATCsTwelveShiftLTwoVarDecoderSamLite}{1.9}
\newcommand{\retSATCsTwelveShiftLTwoVarDecoderSamLite}{0.912}
\newcommand{\retCISATCsTwelveShiftLTwoVarDecoderSamLite}{0.026}
\newcommand{\nSATCsTwelveShiftLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouSATCsTwelveShiftLTwoVarDecoderSegformerMlp}{63.1}
\newcommand{\miouCISATCsTwelveShiftLTwoVarDecoderSegformerMlp}{1.9}
\newcommand{\dropSATCsTwelveShiftLTwoVarDecoderSegformerMlp}{4.3}
\newcommand{\dropCISATCsTwelveShiftLTwoVarDecoderSegformerMlp}{3.4}
\newcommand{\retSATCsTwelveShiftLTwoVarDecoderSegformerMlp}{0.937}
\newcommand{\retCISATCsTwelveShiftLTwoVarDecoderSegformerMlp}{0.049}
\newcommand{\nSATCsTwelveShiftLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATCsTwelveShiftLTwoVarLrMultZeroThreeThreeThreeThree}{64.0}
\newcommand{\miouCISATCsTwelveShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.6}
\newcommand{\dropSATCsTwelveShiftLTwoVarLrMultZeroThreeThreeThreeThree}{4.6}
\newcommand{\dropCISATCsTwelveShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.3}
\newcommand{\retSATCsTwelveShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.932}
\newcommand{\retCISATCsTwelveShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.005}
\newcommand{\nSATDfcBoundaryLOne}{5}
\newcommand{\miouSATDfcBoundaryLOne}{38.6}
\newcommand{\miouCISATDfcBoundaryLOne}{2.2}
\newcommand{\dropSATDfcBoundaryLOne}{1.9}
\newcommand{\dropCISATDfcBoundaryLOne}{2.7}
\newcommand{\retSATDfcBoundaryLOne}{0.953}
\newcommand{\retCISATDfcBoundaryLOne}{0.065}
\newcommand{\nSATDfcBoundaryLTwo}{5}
\newcommand{\miouSATDfcBoundaryLTwo}{34.2}
\newcommand{\miouCISATDfcBoundaryLTwo}{2.5}
\newcommand{\dropSATDfcBoundaryLTwo}{6.3}
\newcommand{\dropCISATDfcBoundaryLTwo}{2.4}
\newcommand{\retSATDfcBoundaryLTwo}{0.844}
\newcommand{\retCISATDfcBoundaryLTwo}{0.058}
\newcommand{\nSATDfcBoundaryLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATDfcBoundaryLTwoVarDecoderMaskTwoformerLite}{36.1}
\newcommand{\miouCISATDfcBoundaryLTwoVarDecoderMaskTwoformerLite}{1.4}
\newcommand{\dropSATDfcBoundaryLTwoVarDecoderMaskTwoformerLite}{4.5}
\newcommand{\dropCISATDfcBoundaryLTwoVarDecoderMaskTwoformerLite}{1.3}
\newcommand{\retSATDfcBoundaryLTwoVarDecoderMaskTwoformerLite}{0.889}
\newcommand{\retCISATDfcBoundaryLTwoVarDecoderMaskTwoformerLite}{0.031}
\newcommand{\nSATDfcBoundaryLTwoVarDecoderSamLite}{5}
\newcommand{\miouSATDfcBoundaryLTwoVarDecoderSamLite}{35.1}
\newcommand{\miouCISATDfcBoundaryLTwoVarDecoderSamLite}{2.4}
\newcommand{\dropSATDfcBoundaryLTwoVarDecoderSamLite}{4.0}
\newcommand{\dropCISATDfcBoundaryLTwoVarDecoderSamLite}{3.2}
\newcommand{\retSATDfcBoundaryLTwoVarDecoderSamLite}{0.899}
\newcommand{\retCISATDfcBoundaryLTwoVarDecoderSamLite}{0.080}
\newcommand{\nSATDfcBoundaryLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouSATDfcBoundaryLTwoVarDecoderSegformerMlp}{35.7}
\newcommand{\miouCISATDfcBoundaryLTwoVarDecoderSegformerMlp}{3.5}
\newcommand{\dropSATDfcBoundaryLTwoVarDecoderSegformerMlp}{6.3}
\newcommand{\dropCISATDfcBoundaryLTwoVarDecoderSegformerMlp}{4.6}
\newcommand{\retSATDfcBoundaryLTwoVarDecoderSegformerMlp}{0.852}
\newcommand{\retCISATDfcBoundaryLTwoVarDecoderSegformerMlp}{0.105}
\newcommand{\nSATDfcBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATDfcBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{35.4}
\newcommand{\miouCISATDfcBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{4.1}
\newcommand{\dropSATDfcBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{5.6}
\newcommand{\dropCISATDfcBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{4.9}
\newcommand{\retSATDfcBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{0.865}
\newcommand{\retCISATDfcBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{0.116}
\newcommand{\nSATDfcClean}{5}
\newcommand{\miouSATDfcClean}{40.5}
\newcommand{\miouCISATDfcClean}{1.2}
\newcommand{\nSATDfcCleanVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATDfcCleanVarDecoderMaskTwoformerLite}{40.6}
\newcommand{\miouCISATDfcCleanVarDecoderMaskTwoformerLite}{1.2}
\newcommand{\nSATDfcCleanVarDecoderSamLite}{5}
\newcommand{\miouSATDfcCleanVarDecoderSamLite}{39.1}
\newcommand{\miouCISATDfcCleanVarDecoderSamLite}{2.3}
\newcommand{\nSATDfcCleanVarDecoderSegformerMlp}{5}
\newcommand{\miouSATDfcCleanVarDecoderSegformerMlp}{42.0}
\newcommand{\miouCISATDfcCleanVarDecoderSegformerMlp}{1.5}
\newcommand{\nSATDfcCleanVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATDfcCleanVarLrMultZeroThreeThreeThreeThree}{41.0}
\newcommand{\miouCISATDfcCleanVarLrMultZeroThreeThreeThreeThree}{1.1}
\newcommand{\nSATDfcCleanVarTrainSubsetRealcov}{5}
\newcommand{\miouSATDfcCleanVarTrainSubsetRealcov}{39.9}
\newcommand{\miouCISATDfcCleanVarTrainSubsetRealcov}{1.3}
\newcommand{\nSATDfcCoarseLOne}{5}
\newcommand{\miouSATDfcCoarseLOne}{37.7}
\newcommand{\miouCISATDfcCoarseLOne}{6.4}
\newcommand{\dropSATDfcCoarseLOne}{2.8}
\newcommand{\dropCISATDfcCoarseLOne}{6.4}
\newcommand{\retSATDfcCoarseLOne}{0.930}
\newcommand{\retCISATDfcCoarseLOne}{0.159}
\newcommand{\nSATDfcCoarseLTwo}{5}
\newcommand{\miouSATDfcCoarseLTwo}{38.8}
\newcommand{\miouCISATDfcCoarseLTwo}{1.3}
\newcommand{\dropSATDfcCoarseLTwo}{1.7}
\newcommand{\dropCISATDfcCoarseLTwo}{1.8}
\newcommand{\retSATDfcCoarseLTwo}{0.958}
\newcommand{\retCISATDfcCoarseLTwo}{0.045}
\newcommand{\nSATDfcCoarseLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATDfcCoarseLTwoVarDecoderMaskTwoformerLite}{38.2}
\newcommand{\miouCISATDfcCoarseLTwoVarDecoderMaskTwoformerLite}{1.7}
\newcommand{\dropSATDfcCoarseLTwoVarDecoderMaskTwoformerLite}{2.4}
\newcommand{\dropCISATDfcCoarseLTwoVarDecoderMaskTwoformerLite}{2.8}
\newcommand{\retSATDfcCoarseLTwoVarDecoderMaskTwoformerLite}{0.941}
\newcommand{\retCISATDfcCoarseLTwoVarDecoderMaskTwoformerLite}{0.065}
\newcommand{\nSATDfcCoarseLTwoVarDecoderSamLite}{5}
\newcommand{\miouSATDfcCoarseLTwoVarDecoderSamLite}{38.5}
\newcommand{\miouCISATDfcCoarseLTwoVarDecoderSamLite}{1.6}
\newcommand{\dropSATDfcCoarseLTwoVarDecoderSamLite}{0.6}
\newcommand{\dropCISATDfcCoarseLTwoVarDecoderSamLite}{3.3}
\newcommand{\retSATDfcCoarseLTwoVarDecoderSamLite}{0.988}
\newcommand{\retCISATDfcCoarseLTwoVarDecoderSamLite}{0.088}
\newcommand{\nSATDfcCoarseLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouSATDfcCoarseLTwoVarDecoderSegformerMlp}{39.5}
\newcommand{\miouCISATDfcCoarseLTwoVarDecoderSegformerMlp}{1.7}
\newcommand{\dropSATDfcCoarseLTwoVarDecoderSegformerMlp}{2.5}
\newcommand{\dropCISATDfcCoarseLTwoVarDecoderSegformerMlp}{0.9}
\newcommand{\retSATDfcCoarseLTwoVarDecoderSegformerMlp}{0.941}
\newcommand{\retCISATDfcCoarseLTwoVarDecoderSegformerMlp}{0.021}
\newcommand{\nSATDfcCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATDfcCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{39.7}
\newcommand{\miouCISATDfcCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{1.3}
\newcommand{\dropSATDfcCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{1.4}
\newcommand{\dropCISATDfcCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.5}
\newcommand{\retSATDfcCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.967}
\newcommand{\retCISATDfcCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.012}
\newcommand{\nSATDfcModisREALVarTrainSubsetRealcov}{5}
\newcommand{\miouSATDfcModisREALVarTrainSubsetRealcov}{32.5}
\newcommand{\miouCISATDfcModisREALVarTrainSubsetRealcov}{3.0}
\newcommand{\dropSATDfcModisREALVarTrainSubsetRealcov}{7.4}
\newcommand{\dropCISATDfcModisREALVarTrainSubsetRealcov}{3.5}
\newcommand{\retSATDfcModisREALVarTrainSubsetRealcov}{0.815}
\newcommand{\retCISATDfcModisREALVarTrainSubsetRealcov}{0.083}
\newcommand{\nSATDfcOmissionLOne}{5}
\newcommand{\miouSATDfcOmissionLOne}{37.5}
\newcommand{\miouCISATDfcOmissionLOne}{2.7}
\newcommand{\dropSATDfcOmissionLOne}{3.0}
\newcommand{\dropCISATDfcOmissionLOne}{2.2}
\newcommand{\retSATDfcOmissionLOne}{0.926}
\newcommand{\retCISATDfcOmissionLOne}{0.054}
\newcommand{\nSATDfcOmissionLTwo}{5}
\newcommand{\miouSATDfcOmissionLTwo}{36.6}
\newcommand{\miouCISATDfcOmissionLTwo}{1.7}
\newcommand{\dropSATDfcOmissionLTwo}{4.0}
\newcommand{\dropCISATDfcOmissionLTwo}{2.1}
\newcommand{\retSATDfcOmissionLTwo}{0.903}
\newcommand{\retCISATDfcOmissionLTwo}{0.050}
\newcommand{\nSATDfcOmissionLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATDfcOmissionLTwoVarDecoderMaskTwoformerLite}{35.7}
\newcommand{\miouCISATDfcOmissionLTwoVarDecoderMaskTwoformerLite}{2.2}
\newcommand{\dropSATDfcOmissionLTwoVarDecoderMaskTwoformerLite}{4.9}
\newcommand{\dropCISATDfcOmissionLTwoVarDecoderMaskTwoformerLite}{1.9}
\newcommand{\retSATDfcOmissionLTwoVarDecoderMaskTwoformerLite}{0.880}
\newcommand{\retCISATDfcOmissionLTwoVarDecoderMaskTwoformerLite}{0.047}
\newcommand{\nSATDfcOmissionLTwoVarDecoderSamLite}{5}
\newcommand{\miouSATDfcOmissionLTwoVarDecoderSamLite}{34.9}
\newcommand{\miouCISATDfcOmissionLTwoVarDecoderSamLite}{2.8}
\newcommand{\dropSATDfcOmissionLTwoVarDecoderSamLite}{4.2}
\newcommand{\dropCISATDfcOmissionLTwoVarDecoderSamLite}{1.2}
\newcommand{\retSATDfcOmissionLTwoVarDecoderSamLite}{0.892}
\newcommand{\retCISATDfcOmissionLTwoVarDecoderSamLite}{0.033}
\newcommand{\nSATDfcOmissionLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouSATDfcOmissionLTwoVarDecoderSegformerMlp}{36.9}
\newcommand{\miouCISATDfcOmissionLTwoVarDecoderSegformerMlp}{1.6}
\newcommand{\dropSATDfcOmissionLTwoVarDecoderSegformerMlp}{5.1}
\newcommand{\dropCISATDfcOmissionLTwoVarDecoderSegformerMlp}{1.8}
\newcommand{\retSATDfcOmissionLTwoVarDecoderSegformerMlp}{0.879}
\newcommand{\retCISATDfcOmissionLTwoVarDecoderSegformerMlp}{0.041}
\newcommand{\nSATDfcOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATDfcOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{36.1}
\newcommand{\miouCISATDfcOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{1.3}
\newcommand{\dropSATDfcOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{4.9}
\newcommand{\dropCISATDfcOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{1.4}
\newcommand{\retSATDfcOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{0.880}
\newcommand{\retCISATDfcOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{0.033}
\newcommand{\nSATDfcShiftLOne}{5}
\newcommand{\miouSATDfcShiftLOne}{39.3}
\newcommand{\miouCISATDfcShiftLOne}{3.2}
\newcommand{\dropSATDfcShiftLOne}{1.3}
\newcommand{\dropCISATDfcShiftLOne}{2.9}
\newcommand{\retSATDfcShiftLOne}{0.969}
\newcommand{\retCISATDfcShiftLOne}{0.071}
\newcommand{\nSATDfcShiftLTwo}{5}
\newcommand{\miouSATDfcShiftLTwo}{40.8}
\newcommand{\miouCISATDfcShiftLTwo}{0.8}
\newcommand{\dropSATDfcShiftLTwo}{\ensuremath{-}0.2}
\newcommand{\dropCISATDfcShiftLTwo}{0.9}
\newcommand{\retSATDfcShiftLTwo}{1.006}
\newcommand{\retCISATDfcShiftLTwo}{0.022}
\newcommand{\nSATDfcShiftLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATDfcShiftLTwoVarDecoderMaskTwoformerLite}{40.5}
\newcommand{\miouCISATDfcShiftLTwoVarDecoderMaskTwoformerLite}{0.8}
\newcommand{\dropSATDfcShiftLTwoVarDecoderMaskTwoformerLite}{0.1}
\newcommand{\dropCISATDfcShiftLTwoVarDecoderMaskTwoformerLite}{1.5}
\newcommand{\retSATDfcShiftLTwoVarDecoderMaskTwoformerLite}{0.997}
\newcommand{\retCISATDfcShiftLTwoVarDecoderMaskTwoformerLite}{0.037}
\newcommand{\nSATDfcShiftLTwoVarDecoderSamLite}{5}
\newcommand{\miouSATDfcShiftLTwoVarDecoderSamLite}{39.1}
\newcommand{\miouCISATDfcShiftLTwoVarDecoderSamLite}{1.2}
\newcommand{\dropSATDfcShiftLTwoVarDecoderSamLite}{0.0}
\newcommand{\dropCISATDfcShiftLTwoVarDecoderSamLite}{2.2}
\newcommand{\retSATDfcShiftLTwoVarDecoderSamLite}{1.003}
\newcommand{\retCISATDfcShiftLTwoVarDecoderSamLite}{0.060}
\newcommand{\nSATDfcShiftLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouSATDfcShiftLTwoVarDecoderSegformerMlp}{41.7}
\newcommand{\miouCISATDfcShiftLTwoVarDecoderSegformerMlp}{1.0}
\newcommand{\dropSATDfcShiftLTwoVarDecoderSegformerMlp}{0.2}
\newcommand{\dropCISATDfcShiftLTwoVarDecoderSegformerMlp}{1.6}
\newcommand{\retSATDfcShiftLTwoVarDecoderSegformerMlp}{0.995}
\newcommand{\retCISATDfcShiftLTwoVarDecoderSegformerMlp}{0.039}
\newcommand{\nSATDfcShiftLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATDfcShiftLTwoVarLrMultZeroThreeThreeThreeThree}{40.8}
\newcommand{\miouCISATDfcShiftLTwoVarLrMultZeroThreeThreeThreeThree}{1.1}
\newcommand{\dropSATDfcShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.3}
\newcommand{\dropCISATDfcShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.7}
\newcommand{\retSATDfcShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.994}
\newcommand{\retCISATDfcShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.017}
\newcommand{\nSATEnvaBoundaryLOne}{5}
\newcommand{\miouSATEnvaBoundaryLOne}{60.3}
\newcommand{\miouCISATEnvaBoundaryLOne}{0.8}
\newcommand{\dropSATEnvaBoundaryLOne}{1.5}
\newcommand{\dropCISATEnvaBoundaryLOne}{1.2}
\newcommand{\retSATEnvaBoundaryLOne}{0.975}
\newcommand{\retCISATEnvaBoundaryLOne}{0.020}
\newcommand{\nSATEnvaBoundaryLTwo}{5}
\newcommand{\miouSATEnvaBoundaryLTwo}{55.3}
\newcommand{\miouCISATEnvaBoundaryLTwo}{2.4}
\newcommand{\dropSATEnvaBoundaryLTwo}{6.5}
\newcommand{\dropCISATEnvaBoundaryLTwo}{2.5}
\newcommand{\retSATEnvaBoundaryLTwo}{0.894}
\newcommand{\retCISATEnvaBoundaryLTwo}{0.040}
\newcommand{\nSATEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}{36.4}
\newcommand{\miouCISATEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}{8.8}
\newcommand{\dropSATEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}{8.4}
\newcommand{\dropCISATEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}{6.5}
\newcommand{\retSATEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}{0.814}
\newcommand{\retCISATEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}{0.140}
\newcommand{\nSATEnvaBoundaryLTwoVarDecoderSamLite}{5}
\newcommand{\miouSATEnvaBoundaryLTwoVarDecoderSamLite}{44.1}
\newcommand{\miouCISATEnvaBoundaryLTwoVarDecoderSamLite}{7.2}
\newcommand{\dropSATEnvaBoundaryLTwoVarDecoderSamLite}{0.4}
\newcommand{\dropCISATEnvaBoundaryLTwoVarDecoderSamLite}{2.8}
\newcommand{\retSATEnvaBoundaryLTwoVarDecoderSamLite}{0.991}
\newcommand{\retCISATEnvaBoundaryLTwoVarDecoderSamLite}{0.056}
\newcommand{\nSATEnvaBoundaryLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouSATEnvaBoundaryLTwoVarDecoderSegformerMlp}{51.9}
\newcommand{\miouCISATEnvaBoundaryLTwoVarDecoderSegformerMlp}{10.2}
\newcommand{\dropSATEnvaBoundaryLTwoVarDecoderSegformerMlp}{5.0}
\newcommand{\dropCISATEnvaBoundaryLTwoVarDecoderSegformerMlp}{8.1}
\newcommand{\retSATEnvaBoundaryLTwoVarDecoderSegformerMlp}{0.909}
\newcommand{\retCISATEnvaBoundaryLTwoVarDecoderSegformerMlp}{0.149}
\newcommand{\nSATEnvaBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATEnvaBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{52.1}
\newcommand{\miouCISATEnvaBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{7.0}
\newcommand{\dropSATEnvaBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{6.9}
\newcommand{\dropCISATEnvaBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{6.3}
\newcommand{\retSATEnvaBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{0.883}
\newcommand{\retCISATEnvaBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{0.108}
\newcommand{\nSATEnvaClean}{5}
\newcommand{\miouSATEnvaClean}{61.8}
\newcommand{\miouCISATEnvaClean}{0.5}
\newcommand{\nSATEnvaCleanVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATEnvaCleanVarDecoderMaskTwoformerLite}{44.9}
\newcommand{\miouCISATEnvaCleanVarDecoderMaskTwoformerLite}{9.9}
\newcommand{\nSATEnvaCleanVarDecoderSamLite}{5}
\newcommand{\miouSATEnvaCleanVarDecoderSamLite}{44.5}
\newcommand{\miouCISATEnvaCleanVarDecoderSamLite}{7.4}
\newcommand{\nSATEnvaCleanVarDecoderSegformerMlp}{5}
\newcommand{\miouSATEnvaCleanVarDecoderSegformerMlp}{56.9}
\newcommand{\miouCISATEnvaCleanVarDecoderSegformerMlp}{3.7}
\newcommand{\nSATEnvaCleanVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATEnvaCleanVarLrMultZeroThreeThreeThreeThree}{59.0}
\newcommand{\miouCISATEnvaCleanVarLrMultZeroThreeThreeThreeThree}{2.4}
\newcommand{\nSATEnvaCoarseLOne}{5}
\newcommand{\miouSATEnvaCoarseLOne}{61.5}
\newcommand{\miouCISATEnvaCoarseLOne}{0.4}
\newcommand{\dropSATEnvaCoarseLOne}{0.3}
\newcommand{\dropCISATEnvaCoarseLOne}{0.8}
\newcommand{\retSATEnvaCoarseLOne}{0.995}
\newcommand{\retCISATEnvaCoarseLOne}{0.013}
\newcommand{\nSATEnvaCoarseLTwo}{5}
\newcommand{\miouSATEnvaCoarseLTwo}{57.9}
\newcommand{\miouCISATEnvaCoarseLTwo}{1.2}
\newcommand{\dropSATEnvaCoarseLTwo}{3.9}
\newcommand{\dropCISATEnvaCoarseLTwo}{1.3}
\newcommand{\retSATEnvaCoarseLTwo}{0.937}
\newcommand{\retCISATEnvaCoarseLTwo}{0.021}
\newcommand{\nSATEnvaCoarseLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATEnvaCoarseLTwoVarDecoderMaskTwoformerLite}{44.6}
\newcommand{\miouCISATEnvaCoarseLTwoVarDecoderMaskTwoformerLite}{8.2}
\newcommand{\dropSATEnvaCoarseLTwoVarDecoderMaskTwoformerLite}{0.3}
\newcommand{\dropCISATEnvaCoarseLTwoVarDecoderMaskTwoformerLite}{5.9}
\newcommand{\retSATEnvaCoarseLTwoVarDecoderMaskTwoformerLite}{1.002}
\newcommand{\retCISATEnvaCoarseLTwoVarDecoderMaskTwoformerLite}{0.124}
\newcommand{\nSATEnvaCoarseLTwoVarDecoderSamLite}{5}
\newcommand{\miouSATEnvaCoarseLTwoVarDecoderSamLite}{39.4}
\newcommand{\miouCISATEnvaCoarseLTwoVarDecoderSamLite}{6.1}
\newcommand{\dropSATEnvaCoarseLTwoVarDecoderSamLite}{5.1}
\newcommand{\dropCISATEnvaCoarseLTwoVarDecoderSamLite}{4.1}
\newcommand{\retSATEnvaCoarseLTwoVarDecoderSamLite}{0.887}
\newcommand{\retCISATEnvaCoarseLTwoVarDecoderSamLite}{0.081}
\newcommand{\nSATEnvaCoarseLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouSATEnvaCoarseLTwoVarDecoderSegformerMlp}{56.2}
\newcommand{\miouCISATEnvaCoarseLTwoVarDecoderSegformerMlp}{9.0}
\newcommand{\dropSATEnvaCoarseLTwoVarDecoderSegformerMlp}{0.7}
\newcommand{\dropCISATEnvaCoarseLTwoVarDecoderSegformerMlp}{6.3}
\newcommand{\retSATEnvaCoarseLTwoVarDecoderSegformerMlp}{0.985}
\newcommand{\retCISATEnvaCoarseLTwoVarDecoderSegformerMlp}{0.119}
\newcommand{\nSATEnvaCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATEnvaCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{54.9}
\newcommand{\miouCISATEnvaCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{4.7}
\newcommand{\dropSATEnvaCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{4.1}
\newcommand{\dropCISATEnvaCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{3.9}
\newcommand{\retSATEnvaCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.930}
\newcommand{\retCISATEnvaCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.067}
\newcommand{\nSATEnvaNlcdREAL}{5}
\newcommand{\miouSATEnvaNlcdREAL}{40.0}
\newcommand{\miouCISATEnvaNlcdREAL}{2.5}
\newcommand{\dropSATEnvaNlcdREAL}{21.8}
\newcommand{\dropCISATEnvaNlcdREAL}{2.7}
\newcommand{\retSATEnvaNlcdREAL}{0.648}
\newcommand{\retCISATEnvaNlcdREAL}{0.043}
\newcommand{\nSATEnvaOmissionLOne}{5}
\newcommand{\miouSATEnvaOmissionLOne}{57.7}
\newcommand{\miouCISATEnvaOmissionLOne}{3.0}
\newcommand{\dropSATEnvaOmissionLOne}{4.2}
\newcommand{\dropCISATEnvaOmissionLOne}{2.6}
\newcommand{\retSATEnvaOmissionLOne}{0.933}
\newcommand{\retCISATEnvaOmissionLOne}{0.042}
\newcommand{\nSATEnvaOmissionLTwo}{5}
\newcommand{\miouSATEnvaOmissionLTwo}{50.1}
\newcommand{\miouCISATEnvaOmissionLTwo}{8.4}
\newcommand{\dropSATEnvaOmissionLTwo}{11.8}
\newcommand{\dropCISATEnvaOmissionLTwo}{8.6}
\newcommand{\retSATEnvaOmissionLTwo}{0.810}
\newcommand{\retCISATEnvaOmissionLTwo}{0.138}
\newcommand{\nSATEnvaOmissionLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATEnvaOmissionLTwoVarDecoderMaskTwoformerLite}{33.3}
\newcommand{\miouCISATEnvaOmissionLTwoVarDecoderMaskTwoformerLite}{4.7}
\newcommand{\dropSATEnvaOmissionLTwoVarDecoderMaskTwoformerLite}{11.5}
\newcommand{\dropCISATEnvaOmissionLTwoVarDecoderMaskTwoformerLite}{8.4}
\newcommand{\retSATEnvaOmissionLTwoVarDecoderMaskTwoformerLite}{0.755}
\newcommand{\retCISATEnvaOmissionLTwoVarDecoderMaskTwoformerLite}{0.135}
\newcommand{\nSATEnvaOmissionLTwoVarDecoderSamLite}{5}
\newcommand{\miouSATEnvaOmissionLTwoVarDecoderSamLite}{42.5}
\newcommand{\miouCISATEnvaOmissionLTwoVarDecoderSamLite}{4.8}
\newcommand{\dropSATEnvaOmissionLTwoVarDecoderSamLite}{2.0}
\newcommand{\dropCISATEnvaOmissionLTwoVarDecoderSamLite}{3.8}
\newcommand{\retSATEnvaOmissionLTwoVarDecoderSamLite}{0.961}
\newcommand{\retCISATEnvaOmissionLTwoVarDecoderSamLite}{0.080}
\newcommand{\nSATEnvaOmissionLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouSATEnvaOmissionLTwoVarDecoderSegformerMlp}{49.3}
\newcommand{\miouCISATEnvaOmissionLTwoVarDecoderSegformerMlp}{5.0}
\newcommand{\dropSATEnvaOmissionLTwoVarDecoderSegformerMlp}{7.6}
\newcommand{\dropCISATEnvaOmissionLTwoVarDecoderSegformerMlp}{7.1}
\newcommand{\retSATEnvaOmissionLTwoVarDecoderSegformerMlp}{0.869}
\newcommand{\retCISATEnvaOmissionLTwoVarDecoderSegformerMlp}{0.116}
\newcommand{\nSATEnvaOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATEnvaOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{46.1}
\newcommand{\miouCISATEnvaOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{6.6}
\newcommand{\dropSATEnvaOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{12.9}
\newcommand{\dropCISATEnvaOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{5.0}
\newcommand{\retSATEnvaOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{0.781}
\newcommand{\retCISATEnvaOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{0.092}
\newcommand{\nSATEnvaShiftLOne}{5}
\newcommand{\miouSATEnvaShiftLOne}{61.1}
\newcommand{\miouCISATEnvaShiftLOne}{1.1}
\newcommand{\dropSATEnvaShiftLOne}{0.8}
\newcommand{\dropCISATEnvaShiftLOne}{1.5}
\newcommand{\retSATEnvaShiftLOne}{0.988}
\newcommand{\retCISATEnvaShiftLOne}{0.024}
\newcommand{\nSATEnvaShiftLTwo}{5}
\newcommand{\miouSATEnvaShiftLTwo}{58.9}
\newcommand{\miouCISATEnvaShiftLTwo}{1.6}
\newcommand{\dropSATEnvaShiftLTwo}{3.0}
\newcommand{\dropCISATEnvaShiftLTwo}{1.5}
\newcommand{\retSATEnvaShiftLTwo}{0.952}
\newcommand{\retCISATEnvaShiftLTwo}{0.025}
\newcommand{\nSATEnvaShiftLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATEnvaShiftLTwoVarDecoderMaskTwoformerLite}{44.6}
\newcommand{\miouCISATEnvaShiftLTwoVarDecoderMaskTwoformerLite}{10.3}
\newcommand{\dropSATEnvaShiftLTwoVarDecoderMaskTwoformerLite}{0.3}
\newcommand{\dropCISATEnvaShiftLTwoVarDecoderMaskTwoformerLite}{2.2}
\newcommand{\retSATEnvaShiftLTwoVarDecoderMaskTwoformerLite}{0.994}
\newcommand{\retCISATEnvaShiftLTwoVarDecoderMaskTwoformerLite}{0.052}
\newcommand{\nSATEnvaShiftLTwoVarDecoderSamLite}{5}
\newcommand{\miouSATEnvaShiftLTwoVarDecoderSamLite}{43.5}
\newcommand{\miouCISATEnvaShiftLTwoVarDecoderSamLite}{7.1}
\newcommand{\dropSATEnvaShiftLTwoVarDecoderSamLite}{1.0}
\newcommand{\dropCISATEnvaShiftLTwoVarDecoderSamLite}{2.2}
\newcommand{\retSATEnvaShiftLTwoVarDecoderSamLite}{0.978}
\newcommand{\retCISATEnvaShiftLTwoVarDecoderSamLite}{0.043}
\newcommand{\nSATEnvaShiftLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouSATEnvaShiftLTwoVarDecoderSegformerMlp}{57.2}
\newcommand{\miouCISATEnvaShiftLTwoVarDecoderSegformerMlp}{8.6}
\newcommand{\dropSATEnvaShiftLTwoVarDecoderSegformerMlp}{\ensuremath{-}0.3}
\newcommand{\dropCISATEnvaShiftLTwoVarDecoderSegformerMlp}{6.2}
\newcommand{\retSATEnvaShiftLTwoVarDecoderSegformerMlp}{1.003}
\newcommand{\retCISATEnvaShiftLTwoVarDecoderSegformerMlp}{0.114}
\newcommand{\nSATEnvaShiftLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATEnvaShiftLTwoVarLrMultZeroThreeThreeThreeThree}{57.8}
\newcommand{\miouCISATEnvaShiftLTwoVarLrMultZeroThreeThreeThreeThree}{2.3}
\newcommand{\dropSATEnvaShiftLTwoVarLrMultZeroThreeThreeThreeThree}{1.2}
\newcommand{\dropCISATEnvaShiftLTwoVarLrMultZeroThreeThreeThreeThree}{1.6}
\newcommand{\retSATEnvaShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.980}
\newcommand{\retCISATEnvaShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.027}
\newcommand{\nSATflairBoundaryLOne}{5}
\newcommand{\miouSATflairBoundaryLOne}{49.4}
\newcommand{\miouCISATflairBoundaryLOne}{0.7}
\newcommand{\dropSATflairBoundaryLOne}{2.8}
\newcommand{\dropCISATflairBoundaryLOne}{0.8}
\newcommand{\retSATflairBoundaryLOne}{0.946}
\newcommand{\retCISATflairBoundaryLOne}{0.015}
\newcommand{\nSATflairBoundaryLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouSATflairBoundaryLOneVarDecoderMaskTwoformerFull}{44.5}
\newcommand{\miouCISATflairBoundaryLOneVarDecoderMaskTwoformerFull}{1.2}
\newcommand{\dropSATflairBoundaryLOneVarDecoderMaskTwoformerFull}{1.9}
\newcommand{\dropCISATflairBoundaryLOneVarDecoderMaskTwoformerFull}{1.6}
\newcommand{\retSATflairBoundaryLOneVarDecoderMaskTwoformerFull}{0.959}
\newcommand{\retCISATflairBoundaryLOneVarDecoderMaskTwoformerFull}{0.033}
\newcommand{\nSATflairBoundaryLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATflairBoundaryLOneVarDecoderMaskTwoformerLite}{48.0}
\newcommand{\miouCISATflairBoundaryLOneVarDecoderMaskTwoformerLite}{1.1}
\newcommand{\dropSATflairBoundaryLOneVarDecoderMaskTwoformerLite}{2.1}
\newcommand{\dropCISATflairBoundaryLOneVarDecoderMaskTwoformerLite}{0.7}
\newcommand{\retSATflairBoundaryLOneVarDecoderMaskTwoformerLite}{0.958}
\newcommand{\retCISATflairBoundaryLOneVarDecoderMaskTwoformerLite}{0.014}
\newcommand{\nSATflairBoundaryLOneVarDecoderSamLite}{5}
\newcommand{\miouSATflairBoundaryLOneVarDecoderSamLite}{44.3}
\newcommand{\miouCISATflairBoundaryLOneVarDecoderSamLite}{1.3}
\newcommand{\dropSATflairBoundaryLOneVarDecoderSamLite}{2.0}
\newcommand{\dropCISATflairBoundaryLOneVarDecoderSamLite}{1.2}
\newcommand{\retSATflairBoundaryLOneVarDecoderSamLite}{0.958}
\newcommand{\retCISATflairBoundaryLOneVarDecoderSamLite}{0.025}
\newcommand{\nSATflairBoundaryLOneVarDecoderSamPretrained}{5}
\newcommand{\miouSATflairBoundaryLOneVarDecoderSamPretrained}{42.9}
\newcommand{\miouCISATflairBoundaryLOneVarDecoderSamPretrained}{1.8}
\newcommand{\dropSATflairBoundaryLOneVarDecoderSamPretrained}{1.9}
\newcommand{\dropCISATflairBoundaryLOneVarDecoderSamPretrained}{2.3}
\newcommand{\retSATflairBoundaryLOneVarDecoderSamPretrained}{0.959}
\newcommand{\retCISATflairBoundaryLOneVarDecoderSamPretrained}{0.051}
\newcommand{\nSATflairBoundaryLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouSATflairBoundaryLOneVarDecoderSegformerMlp}{49.3}
\newcommand{\miouCISATflairBoundaryLOneVarDecoderSegformerMlp}{1.5}
\newcommand{\dropSATflairBoundaryLOneVarDecoderSegformerMlp}{1.2}
\newcommand{\dropCISATflairBoundaryLOneVarDecoderSegformerMlp}{1.0}
\newcommand{\retSATflairBoundaryLOneVarDecoderSegformerMlp}{0.976}
\newcommand{\retCISATflairBoundaryLOneVarDecoderSegformerMlp}{0.020}
\newcommand{\nSATflairBoundaryLTwo}{8}
\newcommand{\miouSATflairBoundaryLTwo}{45.6}
\newcommand{\miouCISATflairBoundaryLTwo}{1.0}
\newcommand{\dropSATflairBoundaryLTwo}{6.9}
\newcommand{\dropCISATflairBoundaryLTwo}{0.8}
\newcommand{\retSATflairBoundaryLTwo}{0.869}
\newcommand{\retCISATflairBoundaryLTwo}{0.016}
\newcommand{\nSATflairBoundaryLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouSATflairBoundaryLTwoVarDecoderMaskTwoformerFull}{41.9}
\newcommand{\miouCISATflairBoundaryLTwoVarDecoderMaskTwoformerFull}{1.8}
\newcommand{\dropSATflairBoundaryLTwoVarDecoderMaskTwoformerFull}{4.5}
\newcommand{\dropCISATflairBoundaryLTwoVarDecoderMaskTwoformerFull}{1.8}
\newcommand{\retSATflairBoundaryLTwoVarDecoderMaskTwoformerFull}{0.903}
\newcommand{\retCISATflairBoundaryLTwoVarDecoderMaskTwoformerFull}{0.038}
\newcommand{\nSATflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{40.0}
\newcommand{\miouCISATflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{2.1}
\newcommand{\dropSATflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{4.0}
\newcommand{\dropCISATflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{1.5}
\newcommand{\retSATflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{0.909}
\newcommand{\retCISATflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{0.033}
\newcommand{\nSATflairBoundaryLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATflairBoundaryLTwoVarDecoderMaskTwoformerLite}{43.1}
\newcommand{\miouCISATflairBoundaryLTwoVarDecoderMaskTwoformerLite}{0.4}
\newcommand{\dropSATflairBoundaryLTwoVarDecoderMaskTwoformerLite}{7.1}
\newcommand{\dropCISATflairBoundaryLTwoVarDecoderMaskTwoformerLite}{1.3}
\newcommand{\retSATflairBoundaryLTwoVarDecoderMaskTwoformerLite}{0.859}
\newcommand{\retCISATflairBoundaryLTwoVarDecoderMaskTwoformerLite}{0.022}
\newcommand{\nSATflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{39.2}
\newcommand{\miouCISATflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{1.4}
\newcommand{\dropSATflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{7.1}
\newcommand{\dropCISATflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{0.6}
\newcommand{\retSATflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{0.847}
\newcommand{\retCISATflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{0.014}
\newcommand{\nSATflairBoundaryLTwoVarDecoderSamLite}{5}
\newcommand{\miouSATflairBoundaryLTwoVarDecoderSamLite}{40.4}
\newcommand{\miouCISATflairBoundaryLTwoVarDecoderSamLite}{1.3}
\newcommand{\dropSATflairBoundaryLTwoVarDecoderSamLite}{6.0}
\newcommand{\dropCISATflairBoundaryLTwoVarDecoderSamLite}{1.4}
\newcommand{\retSATflairBoundaryLTwoVarDecoderSamLite}{0.872}
\newcommand{\retCISATflairBoundaryLTwoVarDecoderSamLite}{0.026}
\newcommand{\nSATflairBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATflairBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{36.9}
\newcommand{\miouCISATflairBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{2.4}
\newcommand{\dropSATflairBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{5.0}
\newcommand{\dropCISATflairBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{2.9}
\newcommand{\retSATflairBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{0.881}
\newcommand{\retCISATflairBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{0.068}
\newcommand{\nSATflairBoundaryLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouSATflairBoundaryLTwoVarDecoderSamPretrained}{38.7}
\newcommand{\miouCISATflairBoundaryLTwoVarDecoderSamPretrained}{1.4}
\newcommand{\dropSATflairBoundaryLTwoVarDecoderSamPretrained}{6.0}
\newcommand{\dropCISATflairBoundaryLTwoVarDecoderSamPretrained}{1.4}
\newcommand{\retSATflairBoundaryLTwoVarDecoderSamPretrained}{0.865}
\newcommand{\retCISATflairBoundaryLTwoVarDecoderSamPretrained}{0.029}
\newcommand{\nSATflairBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATflairBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{34.5}
\newcommand{\miouCISATflairBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{2.7}
\newcommand{\dropSATflairBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{5.5}
\newcommand{\dropCISATflairBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{0.8}
\newcommand{\retSATflairBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{0.863}
\newcommand{\retCISATflairBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{0.025}
\newcommand{\nSATflairBoundaryLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouSATflairBoundaryLTwoVarDecoderSegformerMlp}{44.8}
\newcommand{\miouCISATflairBoundaryLTwoVarDecoderSegformerMlp}{1.5}
\newcommand{\dropSATflairBoundaryLTwoVarDecoderSegformerMlp}{5.7}
\newcommand{\dropCISATflairBoundaryLTwoVarDecoderSegformerMlp}{0.8}
\newcommand{\retSATflairBoundaryLTwoVarDecoderSegformerMlp}{0.886}
\newcommand{\retCISATflairBoundaryLTwoVarDecoderSegformerMlp}{0.014}
\newcommand{\nSATflairBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATflairBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{43.2}
\newcommand{\miouCISATflairBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{1.9}
\newcommand{\dropSATflairBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{4.9}
\newcommand{\dropCISATflairBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{1.9}
\newcommand{\retSATflairBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{0.899}
\newcommand{\retCISATflairBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{0.038}
\newcommand{\nSATflairBoundaryLTwoVarLossBootstrap}{5}
\newcommand{\miouSATflairBoundaryLTwoVarLossBootstrap}{45.6}
\newcommand{\miouCISATflairBoundaryLTwoVarLossBootstrap}{1.0}
\newcommand{\dropSATflairBoundaryLTwoVarLossBootstrap}{6.1}
\newcommand{\dropCISATflairBoundaryLTwoVarLossBootstrap}{0.6}
\newcommand{\retSATflairBoundaryLTwoVarLossBootstrap}{0.881}
\newcommand{\retCISATflairBoundaryLTwoVarLossBootstrap}{0.012}
\newcommand{\nSATflairBoundaryLTwoVarLossGce}{5}
\newcommand{\miouSATflairBoundaryLTwoVarLossGce}{42.8}
\newcommand{\miouCISATflairBoundaryLTwoVarLossGce}{1.5}
\newcommand{\dropSATflairBoundaryLTwoVarLossGce}{7.0}
\newcommand{\dropCISATflairBoundaryLTwoVarLossGce}{2.9}
\newcommand{\retSATflairBoundaryLTwoVarLossGce}{0.860}
\newcommand{\retCISATflairBoundaryLTwoVarLossGce}{0.052}
\newcommand{\nSATflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{44.6}
\newcommand{\miouCISATflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{0.8}
\newcommand{\dropSATflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{5.9}
\newcommand{\dropCISATflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{0.4}
\newcommand{\retSATflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{0.883}
\newcommand{\retCISATflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{0.008}
\newcommand{\nSATflairBoundaryLR}{5}
\newcommand{\miouSATflairBoundaryLR}{43.3}
\newcommand{\miouCISATflairBoundaryLR}{0.8}
\newcommand{\dropSATflairBoundaryLR}{8.9}
\newcommand{\dropCISATflairBoundaryLR}{0.8}
\newcommand{\retSATflairBoundaryLR}{0.829}
\newcommand{\retCISATflairBoundaryLR}{0.016}
\newcommand{\nSATflairBoundaryLRVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATflairBoundaryLRVarLrMultZeroThreeThreeThreeThree}{43.7}
\newcommand{\miouCISATflairBoundaryLRVarLrMultZeroThreeThreeThreeThree}{0.5}
\newcommand{\dropSATflairBoundaryLRVarLrMultZeroThreeThreeThreeThree}{6.8}
\newcommand{\dropCISATflairBoundaryLRVarLrMultZeroThreeThreeThreeThree}{1.3}
\newcommand{\retSATflairBoundaryLRVarLrMultZeroThreeThreeThreeThree}{0.865}
\newcommand{\retCISATflairBoundaryLRVarLrMultZeroThreeThreeThreeThree}{0.023}
\newcommand{\nSATflairClean}{8}
\newcommand{\miouSATflairClean}{52.4}
\newcommand{\miouCISATflairClean}{0.3}
\newcommand{\nSATflairCleanVarClassWeightedTrue}{5}
\newcommand{\miouSATflairCleanVarClassWeightedTrue}{50.3}
\newcommand{\miouCISATflairCleanVarClassWeightedTrue}{1.6}
\newcommand{\nSATflairCleanVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouSATflairCleanVarDecoderMaskTwoformerFull}{46.5}
\newcommand{\miouCISATflairCleanVarDecoderMaskTwoformerFull}{1.0}
\newcommand{\nSATflairCleanVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATflairCleanVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{44.0}
\newcommand{\miouCISATflairCleanVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{1.8}
\newcommand{\nSATflairCleanVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATflairCleanVarDecoderMaskTwoformerLite}{50.2}
\newcommand{\miouCISATflairCleanVarDecoderMaskTwoformerLite}{1.6}
\newcommand{\nSATflairCleanVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATflairCleanVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{46.2}
\newcommand{\miouCISATflairCleanVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{1.2}
\newcommand{\nSATflairCleanVarDecoderSamLite}{5}
\newcommand{\miouSATflairCleanVarDecoderSamLite}{46.3}
\newcommand{\miouCISATflairCleanVarDecoderSamLite}{1.9}
\newcommand{\nSATflairCleanVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATflairCleanVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{41.9}
\newcommand{\miouCISATflairCleanVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{0.8}
\newcommand{\nSATflairCleanVarDecoderSamPretrained}{5}
\newcommand{\miouSATflairCleanVarDecoderSamPretrained}{44.8}
\newcommand{\miouCISATflairCleanVarDecoderSamPretrained}{1.6}
\newcommand{\nSATflairCleanVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATflairCleanVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{39.9}
\newcommand{\miouCISATflairCleanVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{2.2}
\newcommand{\nSATflairCleanVarDecoderSegformerMlp}{5}
\newcommand{\miouSATflairCleanVarDecoderSegformerMlp}{50.5}
\newcommand{\miouCISATflairCleanVarDecoderSegformerMlp}{2.0}
\newcommand{\nSATflairCleanVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATflairCleanVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{48.0}
\newcommand{\miouCISATflairCleanVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{1.5}
\newcommand{\nSATflairCleanVarFrozenEncoderTrue}{5}
\newcommand{\miouSATflairCleanVarFrozenEncoderTrue}{45.9}
\newcommand{\miouCISATflairCleanVarFrozenEncoderTrue}{1.1}
\newcommand{\nSATflairCleanVarLossBootstrap}{5}
\newcommand{\miouSATflairCleanVarLossBootstrap}{51.7}
\newcommand{\miouCISATflairCleanVarLossBootstrap}{0.6}
\newcommand{\nSATflairCleanVarLossGce}{5}
\newcommand{\miouSATflairCleanVarLossGce}{49.9}
\newcommand{\miouCISATflairCleanVarLossGce}{2.2}
\newcommand{\nSATflairCleanVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATflairCleanVarLrMultZeroThreeThreeThreeThree}{50.5}
\newcommand{\miouCISATflairCleanVarLrMultZeroThreeThreeThreeThree}{0.9}
\newcommand{\nSATflairCleanVarLrMultThree}{1}
\newcommand{\miouSATflairCleanVarLrMultThree}{53.0}
\newcommand{\miouCISATflairCleanVarLrMultThree}{--}
\newcommand{\nSATflairCleanVarTrainSubsetCleanTwoFive}{5}
\newcommand{\miouSATflairCleanVarTrainSubsetCleanTwoFive}{44.6}
\newcommand{\miouCISATflairCleanVarTrainSubsetCleanTwoFive}{1.3}
\newcommand{\nSATflairCoarseLOne}{5}
\newcommand{\miouSATflairCoarseLOne}{50.8}
\newcommand{\miouCISATflairCoarseLOne}{1.2}
\newcommand{\dropSATflairCoarseLOne}{1.5}
\newcommand{\dropCISATflairCoarseLOne}{1.0}
\newcommand{\retSATflairCoarseLOne}{0.972}
\newcommand{\retCISATflairCoarseLOne}{0.018}
\newcommand{\nSATflairCoarseLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouSATflairCoarseLOneVarDecoderMaskTwoformerFull}{45.9}
\newcommand{\miouCISATflairCoarseLOneVarDecoderMaskTwoformerFull}{1.1}
\newcommand{\dropSATflairCoarseLOneVarDecoderMaskTwoformerFull}{0.6}
\newcommand{\dropCISATflairCoarseLOneVarDecoderMaskTwoformerFull}{0.4}
\newcommand{\retSATflairCoarseLOneVarDecoderMaskTwoformerFull}{0.988}
\newcommand{\retCISATflairCoarseLOneVarDecoderMaskTwoformerFull}{0.010}
\newcommand{\nSATflairCoarseLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATflairCoarseLOneVarDecoderMaskTwoformerLite}{49.1}
\newcommand{\miouCISATflairCoarseLOneVarDecoderMaskTwoformerLite}{1.0}
\newcommand{\dropSATflairCoarseLOneVarDecoderMaskTwoformerLite}{1.0}
\newcommand{\dropCISATflairCoarseLOneVarDecoderMaskTwoformerLite}{0.9}
\newcommand{\retSATflairCoarseLOneVarDecoderMaskTwoformerLite}{0.980}
\newcommand{\retCISATflairCoarseLOneVarDecoderMaskTwoformerLite}{0.017}
\newcommand{\nSATflairCoarseLOneVarDecoderSamLite}{5}
\newcommand{\miouSATflairCoarseLOneVarDecoderSamLite}{45.2}
\newcommand{\miouCISATflairCoarseLOneVarDecoderSamLite}{1.1}
\newcommand{\dropSATflairCoarseLOneVarDecoderSamLite}{1.1}
\newcommand{\dropCISATflairCoarseLOneVarDecoderSamLite}{1.8}
\newcommand{\retSATflairCoarseLOneVarDecoderSamLite}{0.977}
\newcommand{\retCISATflairCoarseLOneVarDecoderSamLite}{0.039}
\newcommand{\nSATflairCoarseLOneVarDecoderSamPretrained}{5}
\newcommand{\miouSATflairCoarseLOneVarDecoderSamPretrained}{43.6}
\newcommand{\miouCISATflairCoarseLOneVarDecoderSamPretrained}{2.5}
\newcommand{\dropSATflairCoarseLOneVarDecoderSamPretrained}{1.2}
\newcommand{\dropCISATflairCoarseLOneVarDecoderSamPretrained}{2.3}
\newcommand{\retSATflairCoarseLOneVarDecoderSamPretrained}{0.974}
\newcommand{\retCISATflairCoarseLOneVarDecoderSamPretrained}{0.051}
\newcommand{\nSATflairCoarseLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouSATflairCoarseLOneVarDecoderSegformerMlp}{49.7}
\newcommand{\miouCISATflairCoarseLOneVarDecoderSegformerMlp}{1.6}
\newcommand{\dropSATflairCoarseLOneVarDecoderSegformerMlp}{0.8}
\newcommand{\dropCISATflairCoarseLOneVarDecoderSegformerMlp}{1.2}
\newcommand{\retSATflairCoarseLOneVarDecoderSegformerMlp}{0.984}
\newcommand{\retCISATflairCoarseLOneVarDecoderSegformerMlp}{0.023}
\newcommand{\nSATflairCoarseLTwo}{8}
\newcommand{\miouSATflairCoarseLTwo}{46.1}
\newcommand{\miouCISATflairCoarseLTwo}{0.8}
\newcommand{\dropSATflairCoarseLTwo}{6.3}
\newcommand{\dropCISATflairCoarseLTwo}{0.7}
\newcommand{\retSATflairCoarseLTwo}{0.879}
\newcommand{\retCISATflairCoarseLTwo}{0.013}
\newcommand{\nSATflairCoarseLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouSATflairCoarseLTwoVarDecoderMaskTwoformerFull}{39.1}
\newcommand{\miouCISATflairCoarseLTwoVarDecoderMaskTwoformerFull}{1.7}
\newcommand{\dropSATflairCoarseLTwoVarDecoderMaskTwoformerFull}{7.4}
\newcommand{\dropCISATflairCoarseLTwoVarDecoderMaskTwoformerFull}{1.8}
\newcommand{\retSATflairCoarseLTwoVarDecoderMaskTwoformerFull}{0.841}
\newcommand{\retCISATflairCoarseLTwoVarDecoderMaskTwoformerFull}{0.037}
\newcommand{\nSATflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{36.0}
\newcommand{\miouCISATflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{2.8}
\newcommand{\dropSATflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{8.0}
\newcommand{\dropCISATflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{1.8}
\newcommand{\retSATflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{0.817}
\newcommand{\retCISATflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{0.043}
\newcommand{\nSATflairCoarseLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATflairCoarseLTwoVarDecoderMaskTwoformerLite}{43.5}
\newcommand{\miouCISATflairCoarseLTwoVarDecoderMaskTwoformerLite}{1.2}
\newcommand{\dropSATflairCoarseLTwoVarDecoderMaskTwoformerLite}{6.7}
\newcommand{\dropCISATflairCoarseLTwoVarDecoderMaskTwoformerLite}{0.7}
\newcommand{\retSATflairCoarseLTwoVarDecoderMaskTwoformerLite}{0.867}
\newcommand{\retCISATflairCoarseLTwoVarDecoderMaskTwoformerLite}{0.013}
\newcommand{\nSATflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{41.1}
\newcommand{\miouCISATflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{1.1}
\newcommand{\dropSATflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{5.1}
\newcommand{\dropCISATflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{0.3}
\newcommand{\retSATflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{0.889}
\newcommand{\retCISATflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{0.006}
\newcommand{\nSATflairCoarseLTwoVarDecoderSamLite}{5}
\newcommand{\miouSATflairCoarseLTwoVarDecoderSamLite}{40.0}
\newcommand{\miouCISATflairCoarseLTwoVarDecoderSamLite}{1.8}
\newcommand{\dropSATflairCoarseLTwoVarDecoderSamLite}{6.3}
\newcommand{\dropCISATflairCoarseLTwoVarDecoderSamLite}{1.4}
\newcommand{\retSATflairCoarseLTwoVarDecoderSamLite}{0.865}
\newcommand{\retCISATflairCoarseLTwoVarDecoderSamLite}{0.028}
\newcommand{\nSATflairCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATflairCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{36.9}
\newcommand{\miouCISATflairCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{1.7}
\newcommand{\dropSATflairCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{5.0}
\newcommand{\dropCISATflairCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{1.2}
\newcommand{\retSATflairCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{0.881}
\newcommand{\retCISATflairCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{0.030}
\newcommand{\nSATflairCoarseLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouSATflairCoarseLTwoVarDecoderSamPretrained}{39.9}
\newcommand{\miouCISATflairCoarseLTwoVarDecoderSamPretrained}{1.7}
\newcommand{\dropSATflairCoarseLTwoVarDecoderSamPretrained}{4.8}
\newcommand{\dropCISATflairCoarseLTwoVarDecoderSamPretrained}{2.7}
\newcommand{\retSATflairCoarseLTwoVarDecoderSamPretrained}{0.893}
\newcommand{\retCISATflairCoarseLTwoVarDecoderSamPretrained}{0.058}
\newcommand{\nSATflairCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATflairCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{35.3}
\newcommand{\miouCISATflairCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{3.6}
\newcommand{\dropSATflairCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{4.6}
\newcommand{\dropCISATflairCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{1.6}
\newcommand{\retSATflairCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{0.883}
\newcommand{\retCISATflairCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{0.047}
\newcommand{\nSATflairCoarseLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouSATflairCoarseLTwoVarDecoderSegformerMlp}{44.9}
\newcommand{\miouCISATflairCoarseLTwoVarDecoderSegformerMlp}{1.1}
\newcommand{\dropSATflairCoarseLTwoVarDecoderSegformerMlp}{5.6}
\newcommand{\dropCISATflairCoarseLTwoVarDecoderSegformerMlp}{1.1}
\newcommand{\retSATflairCoarseLTwoVarDecoderSegformerMlp}{0.889}
\newcommand{\retCISATflairCoarseLTwoVarDecoderSegformerMlp}{0.019}
\newcommand{\nSATflairCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATflairCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{43.5}
\newcommand{\miouCISATflairCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{1.2}
\newcommand{\dropSATflairCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{4.5}
\newcommand{\dropCISATflairCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{1.3}
\newcommand{\retSATflairCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{0.906}
\newcommand{\retCISATflairCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{0.024}
\newcommand{\nSATflairCoarseLTwoVarLossBootstrap}{5}
\newcommand{\miouSATflairCoarseLTwoVarLossBootstrap}{45.7}
\newcommand{\miouCISATflairCoarseLTwoVarLossBootstrap}{0.3}
\newcommand{\dropSATflairCoarseLTwoVarLossBootstrap}{6.0}
\newcommand{\dropCISATflairCoarseLTwoVarLossBootstrap}{0.7}
\newcommand{\retSATflairCoarseLTwoVarLossBootstrap}{0.884}
\newcommand{\retCISATflairCoarseLTwoVarLossBootstrap}{0.013}
\newcommand{\nSATflairCoarseLTwoVarLossGce}{5}
\newcommand{\miouSATflairCoarseLTwoVarLossGce}{44.1}
\newcommand{\miouCISATflairCoarseLTwoVarLossGce}{1.6}
\newcommand{\dropSATflairCoarseLTwoVarLossGce}{5.8}
\newcommand{\dropCISATflairCoarseLTwoVarLossGce}{2.1}
\newcommand{\retSATflairCoarseLTwoVarLossGce}{0.885}
\newcommand{\retCISATflairCoarseLTwoVarLossGce}{0.039}
\newcommand{\nSATflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{45.1}
\newcommand{\miouCISATflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.6}
\newcommand{\dropSATflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{5.4}
\newcommand{\dropCISATflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.9}
\newcommand{\retSATflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.894}
\newcommand{\retCISATflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.016}
\newcommand{\nSATflairCoarseLR}{5}
\newcommand{\miouSATflairCoarseLR}{39.9}
\newcommand{\miouCISATflairCoarseLR}{1.2}
\newcommand{\dropSATflairCoarseLR}{12.3}
\newcommand{\dropCISATflairCoarseLR}{1.0}
\newcommand{\retSATflairCoarseLR}{0.764}
\newcommand{\retCISATflairCoarseLR}{0.020}
\newcommand{\nSATflairCoarseLRVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATflairCoarseLRVarLrMultZeroThreeThreeThreeThree}{39.3}
\newcommand{\miouCISATflairCoarseLRVarLrMultZeroThreeThreeThreeThree}{1.0}
\newcommand{\dropSATflairCoarseLRVarLrMultZeroThreeThreeThreeThree}{11.3}
\newcommand{\dropCISATflairCoarseLRVarLrMultZeroThreeThreeThreeThree}{1.7}
\newcommand{\retSATflairCoarseLRVarLrMultZeroThreeThreeThreeThree}{0.777}
\newcommand{\retCISATflairCoarseLRVarLrMultZeroThreeThreeThreeThree}{0.031}
\newcommand{\nSATflairOmissionLOne}{5}
\newcommand{\miouSATflairOmissionLOne}{49.4}
\newcommand{\miouCISATflairOmissionLOne}{0.6}
\newcommand{\dropSATflairOmissionLOne}{2.8}
\newcommand{\dropCISATflairOmissionLOne}{0.4}
\newcommand{\retSATflairOmissionLOne}{0.947}
\newcommand{\retCISATflairOmissionLOne}{0.007}
\newcommand{\nSATflairOmissionLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouSATflairOmissionLOneVarDecoderMaskTwoformerFull}{45.0}
\newcommand{\miouCISATflairOmissionLOneVarDecoderMaskTwoformerFull}{2.1}
\newcommand{\dropSATflairOmissionLOneVarDecoderMaskTwoformerFull}{1.4}
\newcommand{\dropCISATflairOmissionLOneVarDecoderMaskTwoformerFull}{1.2}
\newcommand{\retSATflairOmissionLOneVarDecoderMaskTwoformerFull}{0.969}
\newcommand{\retCISATflairOmissionLOneVarDecoderMaskTwoformerFull}{0.026}
\newcommand{\nSATflairOmissionLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATflairOmissionLOneVarDecoderMaskTwoformerLite}{47.2}
\newcommand{\miouCISATflairOmissionLOneVarDecoderMaskTwoformerLite}{1.2}
\newcommand{\dropSATflairOmissionLOneVarDecoderMaskTwoformerLite}{3.0}
\newcommand{\dropCISATflairOmissionLOneVarDecoderMaskTwoformerLite}{1.7}
\newcommand{\retSATflairOmissionLOneVarDecoderMaskTwoformerLite}{0.941}
\newcommand{\retCISATflairOmissionLOneVarDecoderMaskTwoformerLite}{0.033}
\newcommand{\nSATflairOmissionLOneVarDecoderSamLite}{5}
\newcommand{\miouSATflairOmissionLOneVarDecoderSamLite}{44.2}
\newcommand{\miouCISATflairOmissionLOneVarDecoderSamLite}{1.6}
\newcommand{\dropSATflairOmissionLOneVarDecoderSamLite}{2.1}
\newcommand{\dropCISATflairOmissionLOneVarDecoderSamLite}{1.3}
\newcommand{\retSATflairOmissionLOneVarDecoderSamLite}{0.954}
\newcommand{\retCISATflairOmissionLOneVarDecoderSamLite}{0.027}
\newcommand{\nSATflairOmissionLOneVarDecoderSamPretrained}{5}
\newcommand{\miouSATflairOmissionLOneVarDecoderSamPretrained}{42.5}
\newcommand{\miouCISATflairOmissionLOneVarDecoderSamPretrained}{3.3}
\newcommand{\dropSATflairOmissionLOneVarDecoderSamPretrained}{2.2}
\newcommand{\dropCISATflairOmissionLOneVarDecoderSamPretrained}{2.2}
\newcommand{\retSATflairOmissionLOneVarDecoderSamPretrained}{0.950}
\newcommand{\retCISATflairOmissionLOneVarDecoderSamPretrained}{0.051}
\newcommand{\nSATflairOmissionLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouSATflairOmissionLOneVarDecoderSegformerMlp}{48.5}
\newcommand{\miouCISATflairOmissionLOneVarDecoderSegformerMlp}{1.3}
\newcommand{\dropSATflairOmissionLOneVarDecoderSegformerMlp}{2.1}
\newcommand{\dropCISATflairOmissionLOneVarDecoderSegformerMlp}{0.7}
\newcommand{\retSATflairOmissionLOneVarDecoderSegformerMlp}{0.959}
\newcommand{\retCISATflairOmissionLOneVarDecoderSegformerMlp}{0.012}
\newcommand{\nSATflairOmissionLTwo}{8}
\newcommand{\miouSATflairOmissionLTwo}{44.4}
\newcommand{\miouCISATflairOmissionLTwo}{1.4}
\newcommand{\dropSATflairOmissionLTwo}{8.0}
\newcommand{\dropCISATflairOmissionLTwo}{1.2}
\newcommand{\retSATflairOmissionLTwo}{0.847}
\newcommand{\retCISATflairOmissionLTwo}{0.022}
\newcommand{\nSATflairOmissionLTwoVarClassWeightedTrue}{5}
\newcommand{\miouSATflairOmissionLTwoVarClassWeightedTrue}{43.1}
\newcommand{\miouCISATflairOmissionLTwoVarClassWeightedTrue}{2.5}
\newcommand{\dropSATflairOmissionLTwoVarClassWeightedTrue}{7.3}
\newcommand{\dropCISATflairOmissionLTwoVarClassWeightedTrue}{1.9}
\newcommand{\retSATflairOmissionLTwoVarClassWeightedTrue}{0.855}
\newcommand{\retCISATflairOmissionLTwoVarClassWeightedTrue}{0.038}
\newcommand{\nSATflairOmissionLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouSATflairOmissionLTwoVarDecoderMaskTwoformerFull}{42.9}
\newcommand{\miouCISATflairOmissionLTwoVarDecoderMaskTwoformerFull}{2.5}
\newcommand{\dropSATflairOmissionLTwoVarDecoderMaskTwoformerFull}{3.6}
\newcommand{\dropCISATflairOmissionLTwoVarDecoderMaskTwoformerFull}{1.8}
\newcommand{\retSATflairOmissionLTwoVarDecoderMaskTwoformerFull}{0.922}
\newcommand{\retCISATflairOmissionLTwoVarDecoderMaskTwoformerFull}{0.039}
\newcommand{\nSATflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{39.7}
\newcommand{\miouCISATflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{1.9}
\newcommand{\dropSATflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{4.4}
\newcommand{\dropCISATflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{1.4}
\newcommand{\retSATflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{0.901}
\newcommand{\retCISATflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{0.030}
\newcommand{\nSATflairOmissionLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATflairOmissionLTwoVarDecoderMaskTwoformerLite}{42.8}
\newcommand{\miouCISATflairOmissionLTwoVarDecoderMaskTwoformerLite}{1.9}
\newcommand{\dropSATflairOmissionLTwoVarDecoderMaskTwoformerLite}{7.3}
\newcommand{\dropCISATflairOmissionLTwoVarDecoderMaskTwoformerLite}{2.3}
\newcommand{\retSATflairOmissionLTwoVarDecoderMaskTwoformerLite}{0.855}
\newcommand{\retCISATflairOmissionLTwoVarDecoderMaskTwoformerLite}{0.043}
\newcommand{\nSATflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{40.0}
\newcommand{\miouCISATflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{1.7}
\newcommand{\dropSATflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{6.2}
\newcommand{\dropCISATflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{1.9}
\newcommand{\retSATflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{0.865}
\newcommand{\retCISATflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{0.039}
\newcommand{\nSATflairOmissionLTwoVarDecoderSamLite}{5}
\newcommand{\miouSATflairOmissionLTwoVarDecoderSamLite}{40.9}
\newcommand{\miouCISATflairOmissionLTwoVarDecoderSamLite}{1.6}
\newcommand{\dropSATflairOmissionLTwoVarDecoderSamLite}{5.5}
\newcommand{\dropCISATflairOmissionLTwoVarDecoderSamLite}{3.2}
\newcommand{\retSATflairOmissionLTwoVarDecoderSamLite}{0.884}
\newcommand{\retCISATflairOmissionLTwoVarDecoderSamLite}{0.066}
\newcommand{\nSATflairOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATflairOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{36.2}
\newcommand{\miouCISATflairOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{1.8}
\newcommand{\dropSATflairOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{5.7}
\newcommand{\dropCISATflairOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{1.6}
\newcommand{\retSATflairOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{0.863}
\newcommand{\retCISATflairOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{0.038}
\newcommand{\nSATflairOmissionLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouSATflairOmissionLTwoVarDecoderSamPretrained}{39.1}
\newcommand{\miouCISATflairOmissionLTwoVarDecoderSamPretrained}{2.3}
\newcommand{\dropSATflairOmissionLTwoVarDecoderSamPretrained}{5.7}
\newcommand{\dropCISATflairOmissionLTwoVarDecoderSamPretrained}{1.6}
\newcommand{\retSATflairOmissionLTwoVarDecoderSamPretrained}{0.874}
\newcommand{\retCISATflairOmissionLTwoVarDecoderSamPretrained}{0.036}
\newcommand{\nSATflairOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATflairOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{34.1}
\newcommand{\miouCISATflairOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{3.7}
\newcommand{\dropSATflairOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{5.8}
\newcommand{\dropCISATflairOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{2.4}
\newcommand{\retSATflairOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{0.854}
\newcommand{\retCISATflairOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{0.064}
\newcommand{\nSATflairOmissionLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouSATflairOmissionLTwoVarDecoderSegformerMlp}{44.9}
\newcommand{\miouCISATflairOmissionLTwoVarDecoderSegformerMlp}{2.8}
\newcommand{\dropSATflairOmissionLTwoVarDecoderSegformerMlp}{5.6}
\newcommand{\dropCISATflairOmissionLTwoVarDecoderSegformerMlp}{2.5}
\newcommand{\retSATflairOmissionLTwoVarDecoderSegformerMlp}{0.888}
\newcommand{\retCISATflairOmissionLTwoVarDecoderSegformerMlp}{0.049}
\newcommand{\nSATflairOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATflairOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{43.0}
\newcommand{\miouCISATflairOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{1.7}
\newcommand{\dropSATflairOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{5.0}
\newcommand{\dropCISATflairOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{0.9}
\newcommand{\retSATflairOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{0.896}
\newcommand{\retCISATflairOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{0.019}
\newcommand{\nSATflairOmissionLTwoVarEarlyStoppingFalse}{2}
\newcommand{\miouSATflairOmissionLTwoVarEarlyStoppingFalse}{44.4}
\newcommand{\miouCISATflairOmissionLTwoVarEarlyStoppingFalse}{8.6}
\newcommand{\dropSATflairOmissionLTwoVarEarlyStoppingFalse}{7.9}
\newcommand{\dropCISATflairOmissionLTwoVarEarlyStoppingFalse}{9.0}
\newcommand{\retSATflairOmissionLTwoVarEarlyStoppingFalse}{0.848}
\newcommand{\retCISATflairOmissionLTwoVarEarlyStoppingFalse}{0.171}
\newcommand{\nSATflairOmissionLTwoVarEarlyStoppingFalseFrozenEncoderTrue}{2}
\newcommand{\miouSATflairOmissionLTwoVarEarlyStoppingFalseFrozenEncoderTrue}{41.1}
\newcommand{\miouCISATflairOmissionLTwoVarEarlyStoppingFalseFrozenEncoderTrue}{5.9}
\newcommand{\dropSATflairOmissionLTwoVarEarlyStoppingFalseFrozenEncoderTrue}{5.0}
\newcommand{\dropCISATflairOmissionLTwoVarEarlyStoppingFalseFrozenEncoderTrue}{11.2}
\newcommand{\retSATflairOmissionLTwoVarEarlyStoppingFalseFrozenEncoderTrue}{0.892}
\newcommand{\retCISATflairOmissionLTwoVarEarlyStoppingFalseFrozenEncoderTrue}{0.231}
\newcommand{\nSATflairOmissionLTwoVarFrozenEncoderTrue}{5}
\newcommand{\miouSATflairOmissionLTwoVarFrozenEncoderTrue}{40.9}
\newcommand{\miouCISATflairOmissionLTwoVarFrozenEncoderTrue}{1.6}
\newcommand{\dropSATflairOmissionLTwoVarFrozenEncoderTrue}{5.0}
\newcommand{\dropCISATflairOmissionLTwoVarFrozenEncoderTrue}{2.7}
\newcommand{\retSATflairOmissionLTwoVarFrozenEncoderTrue}{0.892}
\newcommand{\retCISATflairOmissionLTwoVarFrozenEncoderTrue}{0.056}
\newcommand{\nSATflairOmissionLTwoVarLossBootstrap}{5}
\newcommand{\miouSATflairOmissionLTwoVarLossBootstrap}{44.2}
\newcommand{\miouCISATflairOmissionLTwoVarLossBootstrap}{1.4}
\newcommand{\dropSATflairOmissionLTwoVarLossBootstrap}{7.5}
\newcommand{\dropCISATflairOmissionLTwoVarLossBootstrap}{1.9}
\newcommand{\retSATflairOmissionLTwoVarLossBootstrap}{0.855}
\newcommand{\retCISATflairOmissionLTwoVarLossBootstrap}{0.035}
\newcommand{\nSATflairOmissionLTwoVarLossGce}{5}
\newcommand{\miouSATflairOmissionLTwoVarLossGce}{44.1}
\newcommand{\miouCISATflairOmissionLTwoVarLossGce}{2.4}
\newcommand{\dropSATflairOmissionLTwoVarLossGce}{5.7}
\newcommand{\dropCISATflairOmissionLTwoVarLossGce}{3.0}
\newcommand{\retSATflairOmissionLTwoVarLossGce}{0.886}
\newcommand{\retCISATflairOmissionLTwoVarLossGce}{0.057}
\newcommand{\nSATflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{44.4}
\newcommand{\miouCISATflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{1.2}
\newcommand{\dropSATflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{6.1}
\newcommand{\dropCISATflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{1.8}
\newcommand{\retSATflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{0.878}
\newcommand{\retCISATflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{0.034}
\newcommand{\nSATflairOmissionLTwoVarLrMultThree}{2}
\newcommand{\miouSATflairOmissionLTwoVarLrMultThree}{45.1}
\newcommand{\miouCISATflairOmissionLTwoVarLrMultThree}{0.4}
\newcommand{\dropSATflairOmissionLTwoVarLrMultThree}{7.2}
\newcommand{\dropCISATflairOmissionLTwoVarLrMultThree}{0.1}
\newcommand{\retSATflairOmissionLTwoVarLrMultThree}{0.862}
\newcommand{\retCISATflairOmissionLTwoVarLrMultThree}{0.002}
\newcommand{\nSATflairOmissionLTwoVarValLabelsClean}{5}
\newcommand{\miouSATflairOmissionLTwoVarValLabelsClean}{45.1}
\newcommand{\miouCISATflairOmissionLTwoVarValLabelsClean}{0.7}
\newcommand{\dropSATflairOmissionLTwoVarValLabelsClean}{7.1}
\newcommand{\dropCISATflairOmissionLTwoVarValLabelsClean}{0.8}
\newcommand{\retSATflairOmissionLTwoVarValLabelsClean}{0.865}
\newcommand{\retCISATflairOmissionLTwoVarValLabelsClean}{0.014}
\newcommand{\nSATflairOmissionLR}{5}
\newcommand{\miouSATflairOmissionLR}{40.8}
\newcommand{\miouCISATflairOmissionLR}{1.6}
\newcommand{\dropSATflairOmissionLR}{11.4}
\newcommand{\dropCISATflairOmissionLR}{1.6}
\newcommand{\retSATflairOmissionLR}{0.782}
\newcommand{\retCISATflairOmissionLR}{0.031}
\newcommand{\nSATflairOmissionLRVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATflairOmissionLRVarLrMultZeroThreeThreeThreeThree}{40.7}
\newcommand{\miouCISATflairOmissionLRVarLrMultZeroThreeThreeThreeThree}{1.6}
\newcommand{\dropSATflairOmissionLRVarLrMultZeroThreeThreeThreeThree}{9.9}
\newcommand{\dropCISATflairOmissionLRVarLrMultZeroThreeThreeThreeThree}{1.4}
\newcommand{\retSATflairOmissionLRVarLrMultZeroThreeThreeThreeThree}{0.805}
\newcommand{\retCISATflairOmissionLRVarLrMultZeroThreeThreeThreeThree}{0.028}
\newcommand{\nSATflairShiftLOne}{5}
\newcommand{\miouSATflairShiftLOne}{50.9}
\newcommand{\miouCISATflairShiftLOne}{1.3}
\newcommand{\dropSATflairShiftLOne}{1.3}
\newcommand{\dropCISATflairShiftLOne}{1.3}
\newcommand{\retSATflairShiftLOne}{0.975}
\newcommand{\retCISATflairShiftLOne}{0.024}
\newcommand{\nSATflairShiftLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouSATflairShiftLOneVarDecoderMaskTwoformerFull}{45.7}
\newcommand{\miouCISATflairShiftLOneVarDecoderMaskTwoformerFull}{1.9}
\newcommand{\dropSATflairShiftLOneVarDecoderMaskTwoformerFull}{0.7}
\newcommand{\dropCISATflairShiftLOneVarDecoderMaskTwoformerFull}{1.4}
\newcommand{\retSATflairShiftLOneVarDecoderMaskTwoformerFull}{0.984}
\newcommand{\retCISATflairShiftLOneVarDecoderMaskTwoformerFull}{0.031}
\newcommand{\nSATflairShiftLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATflairShiftLOneVarDecoderMaskTwoformerLite}{47.8}
\newcommand{\miouCISATflairShiftLOneVarDecoderMaskTwoformerLite}{1.3}
\newcommand{\dropSATflairShiftLOneVarDecoderMaskTwoformerLite}{2.3}
\newcommand{\dropCISATflairShiftLOneVarDecoderMaskTwoformerLite}{2.1}
\newcommand{\retSATflairShiftLOneVarDecoderMaskTwoformerLite}{0.954}
\newcommand{\retCISATflairShiftLOneVarDecoderMaskTwoformerLite}{0.040}
\newcommand{\nSATflairShiftLOneVarDecoderSamLite}{5}
\newcommand{\miouSATflairShiftLOneVarDecoderSamLite}{44.9}
\newcommand{\miouCISATflairShiftLOneVarDecoderSamLite}{1.1}
\newcommand{\dropSATflairShiftLOneVarDecoderSamLite}{1.5}
\newcommand{\dropCISATflairShiftLOneVarDecoderSamLite}{2.4}
\newcommand{\retSATflairShiftLOneVarDecoderSamLite}{0.969}
\newcommand{\retCISATflairShiftLOneVarDecoderSamLite}{0.052}
\newcommand{\nSATflairShiftLOneVarDecoderSamPretrained}{5}
\newcommand{\miouSATflairShiftLOneVarDecoderSamPretrained}{44.4}
\newcommand{\miouCISATflairShiftLOneVarDecoderSamPretrained}{0.7}
\newcommand{\dropSATflairShiftLOneVarDecoderSamPretrained}{0.3}
\newcommand{\dropCISATflairShiftLOneVarDecoderSamPretrained}{1.3}
\newcommand{\retSATflairShiftLOneVarDecoderSamPretrained}{0.994}
\newcommand{\retCISATflairShiftLOneVarDecoderSamPretrained}{0.030}
\newcommand{\nSATflairShiftLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouSATflairShiftLOneVarDecoderSegformerMlp}{50.1}
\newcommand{\miouCISATflairShiftLOneVarDecoderSegformerMlp}{1.3}
\newcommand{\dropSATflairShiftLOneVarDecoderSegformerMlp}{0.4}
\newcommand{\dropCISATflairShiftLOneVarDecoderSegformerMlp}{1.3}
\newcommand{\retSATflairShiftLOneVarDecoderSegformerMlp}{0.992}
\newcommand{\retCISATflairShiftLOneVarDecoderSegformerMlp}{0.025}
\newcommand{\nSATflairShiftLTwo}{8}
\newcommand{\miouSATflairShiftLTwo}{48.3}
\newcommand{\miouCISATflairShiftLTwo}{0.8}
\newcommand{\dropSATflairShiftLTwo}{4.1}
\newcommand{\dropCISATflairShiftLTwo}{0.5}
\newcommand{\retSATflairShiftLTwo}{0.922}
\newcommand{\retCISATflairShiftLTwo}{0.009}
\newcommand{\nSATflairShiftLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouSATflairShiftLTwoVarDecoderMaskTwoformerFull}{42.5}
\newcommand{\miouCISATflairShiftLTwoVarDecoderMaskTwoformerFull}{1.1}
\newcommand{\dropSATflairShiftLTwoVarDecoderMaskTwoformerFull}{3.9}
\newcommand{\dropCISATflairShiftLTwoVarDecoderMaskTwoformerFull}{1.3}
\newcommand{\retSATflairShiftLTwoVarDecoderMaskTwoformerFull}{0.916}
\newcommand{\retCISATflairShiftLTwoVarDecoderMaskTwoformerFull}{0.028}
\newcommand{\nSATflairShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATflairShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{40.0}
\newcommand{\miouCISATflairShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{1.4}
\newcommand{\dropSATflairShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{4.0}
\newcommand{\dropCISATflairShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{1.2}
\newcommand{\retSATflairShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{0.909}
\newcommand{\retCISATflairShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{0.025}
\newcommand{\nSATflairShiftLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATflairShiftLTwoVarDecoderMaskTwoformerLite}{45.8}
\newcommand{\miouCISATflairShiftLTwoVarDecoderMaskTwoformerLite}{0.5}
\newcommand{\dropSATflairShiftLTwoVarDecoderMaskTwoformerLite}{4.3}
\newcommand{\dropCISATflairShiftLTwoVarDecoderMaskTwoformerLite}{1.8}
\newcommand{\retSATflairShiftLTwoVarDecoderMaskTwoformerLite}{0.914}
\newcommand{\retCISATflairShiftLTwoVarDecoderMaskTwoformerLite}{0.033}
\newcommand{\nSATflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{43.1}
\newcommand{\miouCISATflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{1.1}
\newcommand{\dropSATflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{3.1}
\newcommand{\dropCISATflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{0.4}
\newcommand{\retSATflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{0.933}
\newcommand{\retCISATflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{0.007}
\newcommand{\nSATflairShiftLTwoVarDecoderSamLite}{5}
\newcommand{\miouSATflairShiftLTwoVarDecoderSamLite}{41.8}
\newcommand{\miouCISATflairShiftLTwoVarDecoderSamLite}{1.9}
\newcommand{\dropSATflairShiftLTwoVarDecoderSamLite}{4.5}
\newcommand{\dropCISATflairShiftLTwoVarDecoderSamLite}{2.2}
\newcommand{\retSATflairShiftLTwoVarDecoderSamLite}{0.904}
\newcommand{\retCISATflairShiftLTwoVarDecoderSamLite}{0.045}
\newcommand{\nSATflairShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATflairShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{38.5}
\newcommand{\miouCISATflairShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{0.6}
\newcommand{\dropSATflairShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{3.4}
\newcommand{\dropCISATflairShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{0.5}
\newcommand{\retSATflairShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{0.918}
\newcommand{\retCISATflairShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{0.011}
\newcommand{\nSATflairShiftLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouSATflairShiftLTwoVarDecoderSamPretrained}{40.3}
\newcommand{\miouCISATflairShiftLTwoVarDecoderSamPretrained}{2.7}
\newcommand{\dropSATflairShiftLTwoVarDecoderSamPretrained}{4.4}
\newcommand{\dropCISATflairShiftLTwoVarDecoderSamPretrained}{2.2}
\newcommand{\retSATflairShiftLTwoVarDecoderSamPretrained}{0.901}
\newcommand{\retCISATflairShiftLTwoVarDecoderSamPretrained}{0.050}
\newcommand{\nSATflairShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATflairShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{37.1}
\newcommand{\miouCISATflairShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{1.4}
\newcommand{\dropSATflairShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{2.9}
\newcommand{\dropCISATflairShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{1.5}
\newcommand{\retSATflairShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{0.929}
\newcommand{\retCISATflairShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{0.037}
\newcommand{\nSATflairShiftLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouSATflairShiftLTwoVarDecoderSegformerMlp}{47.1}
\newcommand{\miouCISATflairShiftLTwoVarDecoderSegformerMlp}{2.0}
\newcommand{\dropSATflairShiftLTwoVarDecoderSegformerMlp}{3.4}
\newcommand{\dropCISATflairShiftLTwoVarDecoderSegformerMlp}{1.6}
\newcommand{\retSATflairShiftLTwoVarDecoderSegformerMlp}{0.933}
\newcommand{\retCISATflairShiftLTwoVarDecoderSegformerMlp}{0.032}
\newcommand{\nSATflairShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATflairShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{45.8}
\newcommand{\miouCISATflairShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{0.7}
\newcommand{\dropSATflairShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{2.2}
\newcommand{\dropCISATflairShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{1.0}
\newcommand{\retSATflairShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{0.954}
\newcommand{\retCISATflairShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{0.019}
\newcommand{\nSATflairShiftLTwoVarLossBootstrap}{5}
\newcommand{\miouSATflairShiftLTwoVarLossBootstrap}{47.8}
\newcommand{\miouCISATflairShiftLTwoVarLossBootstrap}{1.1}
\newcommand{\dropSATflairShiftLTwoVarLossBootstrap}{4.0}
\newcommand{\dropCISATflairShiftLTwoVarLossBootstrap}{0.5}
\newcommand{\retSATflairShiftLTwoVarLossBootstrap}{0.924}
\newcommand{\retCISATflairShiftLTwoVarLossBootstrap}{0.010}
\newcommand{\nSATflairShiftLTwoVarLossGce}{5}
\newcommand{\miouSATflairShiftLTwoVarLossGce}{46.3}
\newcommand{\miouCISATflairShiftLTwoVarLossGce}{2.4}
\newcommand{\dropSATflairShiftLTwoVarLossGce}{3.5}
\newcommand{\dropCISATflairShiftLTwoVarLossGce}{2.8}
\newcommand{\retSATflairShiftLTwoVarLossGce}{0.930}
\newcommand{\retCISATflairShiftLTwoVarLossGce}{0.055}
\newcommand{\nSATflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{47.5}
\newcommand{\miouCISATflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.9}
\newcommand{\dropSATflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{3.0}
\newcommand{\dropCISATflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.8}
\newcommand{\retSATflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.941}
\newcommand{\retCISATflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.016}
\newcommand{\nSATflairShiftLR}{5}
\newcommand{\miouSATflairShiftLR}{44.7}
\newcommand{\miouCISATflairShiftLR}{0.8}
\newcommand{\dropSATflairShiftLR}{7.5}
\newcommand{\dropCISATflairShiftLR}{0.8}
\newcommand{\retSATflairShiftLR}{0.856}
\newcommand{\retCISATflairShiftLR}{0.015}
\newcommand{\nSATflairShiftLRVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATflairShiftLRVarLrMultZeroThreeThreeThreeThree}{44.3}
\newcommand{\miouCISATflairShiftLRVarLrMultZeroThreeThreeThreeThree}{0.7}
\newcommand{\dropSATflairShiftLRVarLrMultZeroThreeThreeThreeThree}{6.3}
\newcommand{\dropCISATflairShiftLRVarLrMultZeroThreeThreeThreeThree}{0.6}
\newcommand{\retSATflairShiftLRVarLrMultZeroThreeThreeThreeThree}{0.876}
\newcommand{\retCISATflairShiftLRVarLrMultZeroThreeThreeThreeThree}{0.011}
\newcommand{\nSATKuroBoundaryLOne}{5}
\newcommand{\miouSATKuroBoundaryLOne}{52.4}
\newcommand{\miouCISATKuroBoundaryLOne}{5.1}
\newcommand{\dropSATKuroBoundaryLOne}{0.6}
\newcommand{\dropCISATKuroBoundaryLOne}{4.5}
\newcommand{\retSATKuroBoundaryLOne}{0.990}
\newcommand{\retCISATKuroBoundaryLOne}{0.086}
\newcommand{\nSATKuroBoundaryLTwo}{5}
\newcommand{\miouSATKuroBoundaryLTwo}{46.0}
\newcommand{\miouCISATKuroBoundaryLTwo}{2.8}
\newcommand{\dropSATKuroBoundaryLTwo}{6.9}
\newcommand{\dropCISATKuroBoundaryLTwo}{6.0}
\newcommand{\retSATKuroBoundaryLTwo}{0.874}
\newcommand{\retCISATKuroBoundaryLTwo}{0.100}
\newcommand{\nSATKuroBoundaryLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATKuroBoundaryLTwoVarDecoderMaskTwoformerLite}{45.9}
\newcommand{\miouCISATKuroBoundaryLTwoVarDecoderMaskTwoformerLite}{2.4}
\newcommand{\dropSATKuroBoundaryLTwoVarDecoderMaskTwoformerLite}{8.7}
\newcommand{\dropCISATKuroBoundaryLTwoVarDecoderMaskTwoformerLite}{2.9}
\newcommand{\retSATKuroBoundaryLTwoVarDecoderMaskTwoformerLite}{0.841}
\newcommand{\retCISATKuroBoundaryLTwoVarDecoderMaskTwoformerLite}{0.047}
\newcommand{\nSATKuroBoundaryLTwoVarDecoderSamLite}{5}
\newcommand{\miouSATKuroBoundaryLTwoVarDecoderSamLite}{50.9}
\newcommand{\miouCISATKuroBoundaryLTwoVarDecoderSamLite}{2.9}
\newcommand{\dropSATKuroBoundaryLTwoVarDecoderSamLite}{7.5}
\newcommand{\dropCISATKuroBoundaryLTwoVarDecoderSamLite}{2.5}
\newcommand{\retSATKuroBoundaryLTwoVarDecoderSamLite}{0.872}
\newcommand{\retCISATKuroBoundaryLTwoVarDecoderSamLite}{0.044}
\newcommand{\nSATKuroBoundaryLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouSATKuroBoundaryLTwoVarDecoderSegformerMlp}{50.5}
\newcommand{\miouCISATKuroBoundaryLTwoVarDecoderSegformerMlp}{1.8}
\newcommand{\dropSATKuroBoundaryLTwoVarDecoderSegformerMlp}{6.3}
\newcommand{\dropCISATKuroBoundaryLTwoVarDecoderSegformerMlp}{3.0}
\newcommand{\retSATKuroBoundaryLTwoVarDecoderSegformerMlp}{0.890}
\newcommand{\retCISATKuroBoundaryLTwoVarDecoderSegformerMlp}{0.047}
\newcommand{\nSATKuroBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATKuroBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{51.6}
\newcommand{\miouCISATKuroBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{2.0}
\newcommand{\dropSATKuroBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{6.4}
\newcommand{\dropCISATKuroBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{2.1}
\newcommand{\retSATKuroBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{0.890}
\newcommand{\retCISATKuroBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{0.035}
\newcommand{\nSATKuroCemsREALVarTrainSubsetRealcov}{5}
\newcommand{\miouSATKuroCemsREALVarTrainSubsetRealcov}{48.8}
\newcommand{\miouCISATKuroCemsREALVarTrainSubsetRealcov}{6.1}
\newcommand{\dropSATKuroCemsREALVarTrainSubsetRealcov}{0.3}
\newcommand{\dropCISATKuroCemsREALVarTrainSubsetRealcov}{8.3}
\newcommand{\retSATKuroCemsREALVarTrainSubsetRealcov}{1.001}
\newcommand{\retCISATKuroCemsREALVarTrainSubsetRealcov}{0.174}
\newcommand{\nSATKuroClean}{5}
\newcommand{\miouSATKuroClean}{53.0}
\newcommand{\miouCISATKuroClean}{5.3}
\newcommand{\nSATKuroCleanVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATKuroCleanVarDecoderMaskTwoformerLite}{54.6}
\newcommand{\miouCISATKuroCleanVarDecoderMaskTwoformerLite}{3.0}
\newcommand{\nSATKuroCleanVarDecoderSamLite}{5}
\newcommand{\miouSATKuroCleanVarDecoderSamLite}{58.4}
\newcommand{\miouCISATKuroCleanVarDecoderSamLite}{0.9}
\newcommand{\nSATKuroCleanVarDecoderSegformerMlp}{5}
\newcommand{\miouSATKuroCleanVarDecoderSegformerMlp}{56.9}
\newcommand{\miouCISATKuroCleanVarDecoderSegformerMlp}{3.6}
\newcommand{\nSATKuroCleanVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATKuroCleanVarLrMultZeroThreeThreeThreeThree}{58.0}
\newcommand{\miouCISATKuroCleanVarLrMultZeroThreeThreeThreeThree}{1.6}
\newcommand{\nSATKuroCleanVarTrainSubsetRealcov}{5}
\newcommand{\miouSATKuroCleanVarTrainSubsetRealcov}{49.0}
\newcommand{\miouCISATKuroCleanVarTrainSubsetRealcov}{4.4}
\newcommand{\nSATKuroCoarseLOne}{5}
\newcommand{\miouSATKuroCoarseLOne}{56.1}
\newcommand{\miouCISATKuroCoarseLOne}{2.3}
\newcommand{\dropSATKuroCoarseLOne}{\ensuremath{-}3.1}
\newcommand{\dropCISATKuroCoarseLOne}{5.1}
\newcommand{\retSATKuroCoarseLOne}{1.063}
\newcommand{\retCISATKuroCoarseLOne}{0.098}
\newcommand{\nSATKuroCoarseLTwo}{5}
\newcommand{\miouSATKuroCoarseLTwo}{45.4}
\newcommand{\miouCISATKuroCoarseLTwo}{1.1}
\newcommand{\dropSATKuroCoarseLTwo}{7.6}
\newcommand{\dropCISATKuroCoarseLTwo}{5.9}
\newcommand{\retSATKuroCoarseLTwo}{0.861}
\newcommand{\retCISATKuroCoarseLTwo}{0.094}
\newcommand{\nSATKuroCoarseLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATKuroCoarseLTwoVarDecoderMaskTwoformerLite}{44.3}
\newcommand{\miouCISATKuroCoarseLTwoVarDecoderMaskTwoformerLite}{4.6}
\newcommand{\dropSATKuroCoarseLTwoVarDecoderMaskTwoformerLite}{10.3}
\newcommand{\dropCISATKuroCoarseLTwoVarDecoderMaskTwoformerLite}{5.2}
\newcommand{\retSATKuroCoarseLTwoVarDecoderMaskTwoformerLite}{0.812}
\newcommand{\retCISATKuroCoarseLTwoVarDecoderMaskTwoformerLite}{0.089}
\newcommand{\nSATKuroCoarseLTwoVarDecoderSamLite}{5}
\newcommand{\miouSATKuroCoarseLTwoVarDecoderSamLite}{46.6}
\newcommand{\miouCISATKuroCoarseLTwoVarDecoderSamLite}{2.3}
\newcommand{\dropSATKuroCoarseLTwoVarDecoderSamLite}{11.8}
\newcommand{\dropCISATKuroCoarseLTwoVarDecoderSamLite}{3.0}
\newcommand{\retSATKuroCoarseLTwoVarDecoderSamLite}{0.798}
\newcommand{\retCISATKuroCoarseLTwoVarDecoderSamLite}{0.049}
\newcommand{\nSATKuroCoarseLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouSATKuroCoarseLTwoVarDecoderSegformerMlp}{49.4}
\newcommand{\miouCISATKuroCoarseLTwoVarDecoderSegformerMlp}{0.9}
\newcommand{\dropSATKuroCoarseLTwoVarDecoderSegformerMlp}{7.4}
\newcommand{\dropCISATKuroCoarseLTwoVarDecoderSegformerMlp}{4.0}
\newcommand{\retSATKuroCoarseLTwoVarDecoderSegformerMlp}{0.871}
\newcommand{\retCISATKuroCoarseLTwoVarDecoderSegformerMlp}{0.061}
\newcommand{\nSATKuroCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATKuroCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{49.8}
\newcommand{\miouCISATKuroCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.9}
\newcommand{\dropSATKuroCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{8.2}
\newcommand{\dropCISATKuroCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{2.0}
\newcommand{\retSATKuroCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.859}
\newcommand{\retCISATKuroCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.031}
\newcommand{\nSATKuroOmissionLOne}{5}
\newcommand{\miouSATKuroOmissionLOne}{48.1}
\newcommand{\miouCISATKuroOmissionLOne}{3.5}
\newcommand{\dropSATKuroOmissionLOne}{4.9}
\newcommand{\dropCISATKuroOmissionLOne}{4.7}
\newcommand{\retSATKuroOmissionLOne}{0.910}
\newcommand{\retCISATKuroOmissionLOne}{0.082}
\newcommand{\nSATKuroOmissionLTwo}{5}
\newcommand{\miouSATKuroOmissionLTwo}{43.9}
\newcommand{\miouCISATKuroOmissionLTwo}{3.4}
\newcommand{\dropSATKuroOmissionLTwo}{9.1}
\newcommand{\dropCISATKuroOmissionLTwo}{3.7}
\newcommand{\retSATKuroOmissionLTwo}{0.830}
\newcommand{\retCISATKuroOmissionLTwo}{0.057}
\newcommand{\nSATKuroOmissionLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATKuroOmissionLTwoVarDecoderMaskTwoformerLite}{45.2}
\newcommand{\miouCISATKuroOmissionLTwoVarDecoderMaskTwoformerLite}{3.9}
\newcommand{\dropSATKuroOmissionLTwoVarDecoderMaskTwoformerLite}{9.4}
\newcommand{\dropCISATKuroOmissionLTwoVarDecoderMaskTwoformerLite}{5.9}
\newcommand{\retSATKuroOmissionLTwoVarDecoderMaskTwoformerLite}{0.830}
\newcommand{\retCISATKuroOmissionLTwoVarDecoderMaskTwoformerLite}{0.103}
\newcommand{\nSATKuroOmissionLTwoVarDecoderSamLite}{5}
\newcommand{\miouSATKuroOmissionLTwoVarDecoderSamLite}{50.2}
\newcommand{\miouCISATKuroOmissionLTwoVarDecoderSamLite}{3.0}
\newcommand{\dropSATKuroOmissionLTwoVarDecoderSamLite}{8.1}
\newcommand{\dropCISATKuroOmissionLTwoVarDecoderSamLite}{2.4}
\newcommand{\retSATKuroOmissionLTwoVarDecoderSamLite}{0.860}
\newcommand{\retCISATKuroOmissionLTwoVarDecoderSamLite}{0.043}
\newcommand{\nSATKuroOmissionLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouSATKuroOmissionLTwoVarDecoderSegformerMlp}{44.2}
\newcommand{\miouCISATKuroOmissionLTwoVarDecoderSegformerMlp}{4.2}
\newcommand{\dropSATKuroOmissionLTwoVarDecoderSegformerMlp}{12.6}
\newcommand{\dropCISATKuroOmissionLTwoVarDecoderSegformerMlp}{7.3}
\newcommand{\retSATKuroOmissionLTwoVarDecoderSegformerMlp}{0.781}
\newcommand{\retCISATKuroOmissionLTwoVarDecoderSegformerMlp}{0.116}
\newcommand{\nSATKuroOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATKuroOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{50.9}
\newcommand{\miouCISATKuroOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{1.5}
\newcommand{\dropSATKuroOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{7.1}
\newcommand{\dropCISATKuroOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{2.3}
\newcommand{\retSATKuroOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{0.878}
\newcommand{\retCISATKuroOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{0.038}
\newcommand{\nSATKuroShiftLOne}{5}
\newcommand{\miouSATKuroShiftLOne}{50.8}
\newcommand{\miouCISATKuroShiftLOne}{6.4}
\newcommand{\dropSATKuroShiftLOne}{2.1}
\newcommand{\dropCISATKuroShiftLOne}{3.0}
\newcommand{\retSATKuroShiftLOne}{0.959}
\newcommand{\retCISATKuroShiftLOne}{0.061}
\newcommand{\nSATKuroShiftLTwo}{5}
\newcommand{\miouSATKuroShiftLTwo}{50.6}
\newcommand{\miouCISATKuroShiftLTwo}{2.1}
\newcommand{\dropSATKuroShiftLTwo}{2.3}
\newcommand{\dropCISATKuroShiftLTwo}{6.2}
\newcommand{\retSATKuroShiftLTwo}{0.961}
\newcommand{\retCISATKuroShiftLTwo}{0.111}
\newcommand{\nSATKuroShiftLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATKuroShiftLTwoVarDecoderMaskTwoformerLite}{48.1}
\newcommand{\miouCISATKuroShiftLTwoVarDecoderMaskTwoformerLite}{5.7}
\newcommand{\dropSATKuroShiftLTwoVarDecoderMaskTwoformerLite}{6.4}
\newcommand{\dropCISATKuroShiftLTwoVarDecoderMaskTwoformerLite}{6.5}
\newcommand{\retSATKuroShiftLTwoVarDecoderMaskTwoformerLite}{0.884}
\newcommand{\retCISATKuroShiftLTwoVarDecoderMaskTwoformerLite}{0.121}
\newcommand{\nSATKuroShiftLTwoVarDecoderSamLite}{5}
\newcommand{\miouSATKuroShiftLTwoVarDecoderSamLite}{50.6}
\newcommand{\miouCISATKuroShiftLTwoVarDecoderSamLite}{2.5}
\newcommand{\dropSATKuroShiftLTwoVarDecoderSamLite}{7.8}
\newcommand{\dropCISATKuroShiftLTwoVarDecoderSamLite}{2.4}
\newcommand{\retSATKuroShiftLTwoVarDecoderSamLite}{0.867}
\newcommand{\retCISATKuroShiftLTwoVarDecoderSamLite}{0.041}
\newcommand{\nSATKuroShiftLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouSATKuroShiftLTwoVarDecoderSegformerMlp}{50.1}
\newcommand{\miouCISATKuroShiftLTwoVarDecoderSegformerMlp}{3.2}
\newcommand{\dropSATKuroShiftLTwoVarDecoderSegformerMlp}{6.8}
\newcommand{\dropCISATKuroShiftLTwoVarDecoderSegformerMlp}{5.3}
\newcommand{\retSATKuroShiftLTwoVarDecoderSegformerMlp}{0.883}
\newcommand{\retCISATKuroShiftLTwoVarDecoderSegformerMlp}{0.089}
\newcommand{\nSATKuroShiftLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATKuroShiftLTwoVarLrMultZeroThreeThreeThreeThree}{55.2}
\newcommand{\miouCISATKuroShiftLTwoVarLrMultZeroThreeThreeThreeThree}{1.5}
\newcommand{\dropSATKuroShiftLTwoVarLrMultZeroThreeThreeThreeThree}{2.8}
\newcommand{\dropCISATKuroShiftLTwoVarLrMultZeroThreeThreeThreeThree}{1.7}
\newcommand{\retSATKuroShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.952}
\newcommand{\retCISATKuroShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.029}
\newcommand{\nSATOemBoundaryLOne}{5}
\newcommand{\miouSATOemBoundaryLOne}{60.0}
\newcommand{\miouCISATOemBoundaryLOne}{0.7}
\newcommand{\dropSATOemBoundaryLOne}{3.4}
\newcommand{\dropCISATOemBoundaryLOne}{0.9}
\newcommand{\retSATOemBoundaryLOne}{0.946}
\newcommand{\retCISATOemBoundaryLOne}{0.013}
\newcommand{\nSATOemBoundaryLTwo}{5}
\newcommand{\miouSATOemBoundaryLTwo}{52.7}
\newcommand{\miouCISATOemBoundaryLTwo}{0.9}
\newcommand{\dropSATOemBoundaryLTwo}{10.8}
\newcommand{\dropCISATOemBoundaryLTwo}{1.3}
\newcommand{\retSATOemBoundaryLTwo}{0.831}
\newcommand{\retCISATOemBoundaryLTwo}{0.018}
\newcommand{\nSATOemBoundaryLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATOemBoundaryLTwoVarDecoderMaskTwoformerLite}{52.9}
\newcommand{\miouCISATOemBoundaryLTwoVarDecoderMaskTwoformerLite}{1.3}
\newcommand{\dropSATOemBoundaryLTwoVarDecoderMaskTwoformerLite}{9.5}
\newcommand{\dropCISATOemBoundaryLTwoVarDecoderMaskTwoformerLite}{1.8}
\newcommand{\retSATOemBoundaryLTwoVarDecoderMaskTwoformerLite}{0.848}
\newcommand{\retCISATOemBoundaryLTwoVarDecoderMaskTwoformerLite}{0.027}
\newcommand{\nSATOemBoundaryLTwoVarDecoderSamLite}{5}
\newcommand{\miouSATOemBoundaryLTwoVarDecoderSamLite}{53.8}
\newcommand{\miouCISATOemBoundaryLTwoVarDecoderSamLite}{0.4}
\newcommand{\dropSATOemBoundaryLTwoVarDecoderSamLite}{7.5}
\newcommand{\dropCISATOemBoundaryLTwoVarDecoderSamLite}{0.7}
\newcommand{\retSATOemBoundaryLTwoVarDecoderSamLite}{0.878}
\newcommand{\retCISATOemBoundaryLTwoVarDecoderSamLite}{0.009}
\newcommand{\nSATOemBoundaryLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouSATOemBoundaryLTwoVarDecoderSegformerMlp}{54.1}
\newcommand{\miouCISATOemBoundaryLTwoVarDecoderSegformerMlp}{0.6}
\newcommand{\dropSATOemBoundaryLTwoVarDecoderSegformerMlp}{9.7}
\newcommand{\dropCISATOemBoundaryLTwoVarDecoderSegformerMlp}{0.9}
\newcommand{\retSATOemBoundaryLTwoVarDecoderSegformerMlp}{0.848}
\newcommand{\retCISATOemBoundaryLTwoVarDecoderSegformerMlp}{0.013}
\newcommand{\nSATOemBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATOemBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{52.2}
\newcommand{\miouCISATOemBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{1.0}
\newcommand{\dropSATOemBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{9.2}
\newcommand{\dropCISATOemBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{0.5}
\newcommand{\retSATOemBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{0.850}
\newcommand{\retCISATOemBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{0.010}
\newcommand{\nSATOemClean}{5}
\newcommand{\miouSATOemClean}{63.5}
\newcommand{\miouCISATOemClean}{0.8}
\newcommand{\nSATOemCleanVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATOemCleanVarDecoderMaskTwoformerLite}{62.5}
\newcommand{\miouCISATOemCleanVarDecoderMaskTwoformerLite}{0.9}
\newcommand{\nSATOemCleanVarDecoderSamLite}{5}
\newcommand{\miouSATOemCleanVarDecoderSamLite}{61.2}
\newcommand{\miouCISATOemCleanVarDecoderSamLite}{0.9}
\newcommand{\nSATOemCleanVarDecoderSegformerMlp}{5}
\newcommand{\miouSATOemCleanVarDecoderSegformerMlp}{63.8}
\newcommand{\miouCISATOemCleanVarDecoderSegformerMlp}{0.6}
\newcommand{\nSATOemCleanVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATOemCleanVarLrMultZeroThreeThreeThreeThree}{61.5}
\newcommand{\miouCISATOemCleanVarLrMultZeroThreeThreeThreeThree}{0.6}
\newcommand{\nSATOemCoarseLOne}{5}
\newcommand{\miouSATOemCoarseLOne}{62.3}
\newcommand{\miouCISATOemCoarseLOne}{0.8}
\newcommand{\dropSATOemCoarseLOne}{1.2}
\newcommand{\dropCISATOemCoarseLOne}{0.5}
\newcommand{\retSATOemCoarseLOne}{0.981}
\newcommand{\retCISATOemCoarseLOne}{0.008}
\newcommand{\nSATOemCoarseLTwo}{5}
\newcommand{\miouSATOemCoarseLTwo}{57.6}
\newcommand{\miouCISATOemCoarseLTwo}{0.7}
\newcommand{\dropSATOemCoarseLTwo}{5.9}
\newcommand{\dropCISATOemCoarseLTwo}{1.1}
\newcommand{\retSATOemCoarseLTwo}{0.908}
\newcommand{\retCISATOemCoarseLTwo}{0.016}
\newcommand{\nSATOemCoarseLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATOemCoarseLTwoVarDecoderMaskTwoformerLite}{56.8}
\newcommand{\miouCISATOemCoarseLTwoVarDecoderMaskTwoformerLite}{0.5}
\newcommand{\dropSATOemCoarseLTwoVarDecoderMaskTwoformerLite}{5.6}
\newcommand{\dropCISATOemCoarseLTwoVarDecoderMaskTwoformerLite}{0.6}
\newcommand{\retSATOemCoarseLTwoVarDecoderMaskTwoformerLite}{0.910}
\newcommand{\retCISATOemCoarseLTwoVarDecoderMaskTwoformerLite}{0.009}
\newcommand{\nSATOemCoarseLTwoVarDecoderSamLite}{5}
\newcommand{\miouSATOemCoarseLTwoVarDecoderSamLite}{55.9}
\newcommand{\miouCISATOemCoarseLTwoVarDecoderSamLite}{1.0}
\newcommand{\dropSATOemCoarseLTwoVarDecoderSamLite}{5.3}
\newcommand{\dropCISATOemCoarseLTwoVarDecoderSamLite}{0.9}
\newcommand{\retSATOemCoarseLTwoVarDecoderSamLite}{0.913}
\newcommand{\retCISATOemCoarseLTwoVarDecoderSamLite}{0.014}
\newcommand{\nSATOemCoarseLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouSATOemCoarseLTwoVarDecoderSegformerMlp}{57.3}
\newcommand{\miouCISATOemCoarseLTwoVarDecoderSegformerMlp}{1.4}
\newcommand{\dropSATOemCoarseLTwoVarDecoderSegformerMlp}{6.5}
\newcommand{\dropCISATOemCoarseLTwoVarDecoderSegformerMlp}{1.9}
\newcommand{\retSATOemCoarseLTwoVarDecoderSegformerMlp}{0.898}
\newcommand{\retCISATOemCoarseLTwoVarDecoderSegformerMlp}{0.029}
\newcommand{\nSATOemCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATOemCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{56.8}
\newcommand{\miouCISATOemCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.8}
\newcommand{\dropSATOemCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{4.7}
\newcommand{\dropCISATOemCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{1.0}
\newcommand{\retSATOemCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.924}
\newcommand{\retCISATOemCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.016}
\newcommand{\nSATOemOmissionLOne}{5}
\newcommand{\miouSATOemOmissionLOne}{59.6}
\newcommand{\miouCISATOemOmissionLOne}{1.6}
\newcommand{\dropSATOemOmissionLOne}{3.9}
\newcommand{\dropCISATOemOmissionLOne}{1.6}
\newcommand{\retSATOemOmissionLOne}{0.938}
\newcommand{\retCISATOemOmissionLOne}{0.026}
\newcommand{\nSATOemOmissionLTwo}{5}
\newcommand{\miouSATOemOmissionLTwo}{52.8}
\newcommand{\miouCISATOemOmissionLTwo}{1.1}
\newcommand{\dropSATOemOmissionLTwo}{10.7}
\newcommand{\dropCISATOemOmissionLTwo}{1.2}
\newcommand{\retSATOemOmissionLTwo}{0.831}
\newcommand{\retCISATOemOmissionLTwo}{0.019}
\newcommand{\nSATOemOmissionLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATOemOmissionLTwoVarDecoderMaskTwoformerLite}{51.7}
\newcommand{\miouCISATOemOmissionLTwoVarDecoderMaskTwoformerLite}{2.2}
\newcommand{\dropSATOemOmissionLTwoVarDecoderMaskTwoformerLite}{10.8}
\newcommand{\dropCISATOemOmissionLTwoVarDecoderMaskTwoformerLite}{2.6}
\newcommand{\retSATOemOmissionLTwoVarDecoderMaskTwoformerLite}{0.827}
\newcommand{\retCISATOemOmissionLTwoVarDecoderMaskTwoformerLite}{0.040}
\newcommand{\nSATOemOmissionLTwoVarDecoderSamLite}{5}
\newcommand{\miouSATOemOmissionLTwoVarDecoderSamLite}{52.7}
\newcommand{\miouCISATOemOmissionLTwoVarDecoderSamLite}{1.0}
\newcommand{\dropSATOemOmissionLTwoVarDecoderSamLite}{8.5}
\newcommand{\dropCISATOemOmissionLTwoVarDecoderSamLite}{0.8}
\newcommand{\retSATOemOmissionLTwoVarDecoderSamLite}{0.861}
\newcommand{\retCISATOemOmissionLTwoVarDecoderSamLite}{0.013}
\newcommand{\nSATOemOmissionLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouSATOemOmissionLTwoVarDecoderSegformerMlp}{54.3}
\newcommand{\miouCISATOemOmissionLTwoVarDecoderSegformerMlp}{1.5}
\newcommand{\dropSATOemOmissionLTwoVarDecoderSegformerMlp}{9.5}
\newcommand{\dropCISATOemOmissionLTwoVarDecoderSegformerMlp}{2.0}
\newcommand{\retSATOemOmissionLTwoVarDecoderSegformerMlp}{0.852}
\newcommand{\retCISATOemOmissionLTwoVarDecoderSegformerMlp}{0.030}
\newcommand{\nSATOemOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATOemOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{51.5}
\newcommand{\miouCISATOemOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{0.7}
\newcommand{\dropSATOemOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{10.0}
\newcommand{\dropCISATOemOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{0.4}
\newcommand{\retSATOemOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{0.837}
\newcommand{\retCISATOemOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{0.007}
\newcommand{\nSATOemShiftLOne}{5}
\newcommand{\miouSATOemShiftLOne}{63.3}
\newcommand{\miouCISATOemShiftLOne}{0.4}
\newcommand{\dropSATOemShiftLOne}{0.2}
\newcommand{\dropCISATOemShiftLOne}{0.7}
\newcommand{\retSATOemShiftLOne}{0.997}
\newcommand{\retCISATOemShiftLOne}{0.011}
\newcommand{\nSATOemShiftLTwo}{5}
\newcommand{\miouSATOemShiftLTwo}{60.4}
\newcommand{\miouCISATOemShiftLTwo}{1.1}
\newcommand{\dropSATOemShiftLTwo}{3.1}
\newcommand{\dropCISATOemShiftLTwo}{0.7}
\newcommand{\retSATOemShiftLTwo}{0.951}
\newcommand{\retCISATOemShiftLTwo}{0.012}
\newcommand{\nSATOemShiftLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATOemShiftLTwoVarDecoderMaskTwoformerLite}{58.8}
\newcommand{\miouCISATOemShiftLTwoVarDecoderMaskTwoformerLite}{1.6}
\newcommand{\dropSATOemShiftLTwoVarDecoderMaskTwoformerLite}{3.6}
\newcommand{\dropCISATOemShiftLTwoVarDecoderMaskTwoformerLite}{2.1}
\newcommand{\retSATOemShiftLTwoVarDecoderMaskTwoformerLite}{0.942}
\newcommand{\retCISATOemShiftLTwoVarDecoderMaskTwoformerLite}{0.033}
\newcommand{\nSATOemShiftLTwoVarDecoderSamLite}{5}
\newcommand{\miouSATOemShiftLTwoVarDecoderSamLite}{58.1}
\newcommand{\miouCISATOemShiftLTwoVarDecoderSamLite}{1.4}
\newcommand{\dropSATOemShiftLTwoVarDecoderSamLite}{3.1}
\newcommand{\dropCISATOemShiftLTwoVarDecoderSamLite}{1.4}
\newcommand{\retSATOemShiftLTwoVarDecoderSamLite}{0.949}
\newcommand{\retCISATOemShiftLTwoVarDecoderSamLite}{0.022}
\newcommand{\nSATOemShiftLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouSATOemShiftLTwoVarDecoderSegformerMlp}{59.8}
\newcommand{\miouCISATOemShiftLTwoVarDecoderSegformerMlp}{1.9}
\newcommand{\dropSATOemShiftLTwoVarDecoderSegformerMlp}{4.0}
\newcommand{\dropCISATOemShiftLTwoVarDecoderSegformerMlp}{2.3}
\newcommand{\retSATOemShiftLTwoVarDecoderSegformerMlp}{0.938}
\newcommand{\retCISATOemShiftLTwoVarDecoderSegformerMlp}{0.035}
\newcommand{\nSATOemShiftLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATOemShiftLTwoVarLrMultZeroThreeThreeThreeThree}{59.0}
\newcommand{\miouCISATOemShiftLTwoVarLrMultZeroThreeThreeThreeThree}{1.1}
\newcommand{\dropSATOemShiftLTwoVarLrMultZeroThreeThreeThreeThree}{2.5}
\newcommand{\dropCISATOemShiftLTwoVarLrMultZeroThreeThreeThreeThree}{1.0}
\newcommand{\retSATOemShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.959}
\newcommand{\retCISATOemShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.016}
\newcommand{\nSATsenClean}{5}
\newcommand{\miouSATsenClean}{69.1}
\newcommand{\miouCISATsenClean}{3.0}
\newcommand{\nSATsenOtsuLTwo}{5}
\newcommand{\miouSATsenOtsuLTwo}{61.9}
\newcommand{\miouCISATsenOtsuLTwo}{3.9}
\newcommand{\dropSATsenOtsuLTwo}{7.2}
\newcommand{\dropCISATsenOtsuLTwo}{6.5}
\newcommand{\retSATsenOtsuLTwo}{0.897}
\newcommand{\retCISATsenOtsuLTwo}{0.093}
\newcommand{\nSATSnTwoBoundaryLOne}{5}
\newcommand{\miouSATSnTwoBoundaryLOne}{82.8}
\newcommand{\miouCISATSnTwoBoundaryLOne}{0.6}
\newcommand{\dropSATSnTwoBoundaryLOne}{3.0}
\newcommand{\dropCISATSnTwoBoundaryLOne}{0.6}
\newcommand{\retSATSnTwoBoundaryLOne}{0.965}
\newcommand{\retCISATSnTwoBoundaryLOne}{0.007}
\newcommand{\nSATSnTwoBoundaryLTwo}{5}
\newcommand{\miouSATSnTwoBoundaryLTwo}{75.2}
\newcommand{\miouCISATSnTwoBoundaryLTwo}{2.3}
\newcommand{\dropSATSnTwoBoundaryLTwo}{10.6}
\newcommand{\dropCISATSnTwoBoundaryLTwo}{2.2}
\newcommand{\retSATSnTwoBoundaryLTwo}{0.877}
\newcommand{\retCISATSnTwoBoundaryLTwo}{0.026}
\newcommand{\nSATSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}{69.2}
\newcommand{\miouCISATSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}{15.2}
\newcommand{\dropSATSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}{16.3}
\newcommand{\dropCISATSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}{14.8}
\newcommand{\retSATSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}{0.809}
\newcommand{\retCISATSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}{0.175}
\newcommand{\nSATSnTwoBoundaryLTwoVarDecoderSamLite}{5}
\newcommand{\miouSATSnTwoBoundaryLTwoVarDecoderSamLite}{75.2}
\newcommand{\miouCISATSnTwoBoundaryLTwoVarDecoderSamLite}{0.7}
\newcommand{\dropSATSnTwoBoundaryLTwoVarDecoderSamLite}{9.7}
\newcommand{\dropCISATSnTwoBoundaryLTwoVarDecoderSamLite}{0.8}
\newcommand{\retSATSnTwoBoundaryLTwoVarDecoderSamLite}{0.886}
\newcommand{\retCISATSnTwoBoundaryLTwoVarDecoderSamLite}{0.010}
\newcommand{\nSATSnTwoBoundaryLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouSATSnTwoBoundaryLTwoVarDecoderSegformerMlp}{74.7}
\newcommand{\miouCISATSnTwoBoundaryLTwoVarDecoderSegformerMlp}{2.0}
\newcommand{\dropSATSnTwoBoundaryLTwoVarDecoderSegformerMlp}{10.2}
\newcommand{\dropCISATSnTwoBoundaryLTwoVarDecoderSegformerMlp}{2.2}
\newcommand{\retSATSnTwoBoundaryLTwoVarDecoderSegformerMlp}{0.880}
\newcommand{\retCISATSnTwoBoundaryLTwoVarDecoderSegformerMlp}{0.026}
\newcommand{\nSATSnTwoBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATSnTwoBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{74.9}
\newcommand{\miouCISATSnTwoBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{1.1}
\newcommand{\dropSATSnTwoBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{9.5}
\newcommand{\dropCISATSnTwoBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{0.9}
\newcommand{\retSATSnTwoBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{0.888}
\newcommand{\retCISATSnTwoBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{0.011}
\newcommand{\nSATSnTwoClean}{5}
\newcommand{\miouSATSnTwoClean}{85.8}
\newcommand{\miouCISATSnTwoClean}{0.2}
\newcommand{\nSATSnTwoCleanVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATSnTwoCleanVarDecoderMaskTwoformerLite}{85.4}
\newcommand{\miouCISATSnTwoCleanVarDecoderMaskTwoformerLite}{0.5}
\newcommand{\nSATSnTwoCleanVarDecoderSamLite}{5}
\newcommand{\miouSATSnTwoCleanVarDecoderSamLite}{84.9}
\newcommand{\miouCISATSnTwoCleanVarDecoderSamLite}{0.3}
\newcommand{\nSATSnTwoCleanVarDecoderSegformerMlp}{5}
\newcommand{\miouSATSnTwoCleanVarDecoderSegformerMlp}{84.9}
\newcommand{\miouCISATSnTwoCleanVarDecoderSegformerMlp}{0.2}
\newcommand{\nSATSnTwoCleanVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATSnTwoCleanVarLrMultZeroThreeThreeThreeThree}{84.3}
\newcommand{\miouCISATSnTwoCleanVarLrMultZeroThreeThreeThreeThree}{0.4}
\newcommand{\nSATSnTwoCoarseLOne}{5}
\newcommand{\miouSATSnTwoCoarseLOne}{83.1}
\newcommand{\miouCISATSnTwoCoarseLOne}{0.6}
\newcommand{\dropSATSnTwoCoarseLOne}{2.7}
\newcommand{\dropCISATSnTwoCoarseLOne}{0.7}
\newcommand{\retSATSnTwoCoarseLOne}{0.969}
\newcommand{\retCISATSnTwoCoarseLOne}{0.008}
\newcommand{\nSATSnTwoCoarseLTwo}{5}
\newcommand{\miouSATSnTwoCoarseLTwo}{73.1}
\newcommand{\miouCISATSnTwoCoarseLTwo}{1.8}
\newcommand{\dropSATSnTwoCoarseLTwo}{12.7}
\newcommand{\dropCISATSnTwoCoarseLTwo}{1.7}
\newcommand{\retSATSnTwoCoarseLTwo}{0.852}
\newcommand{\retCISATSnTwoCoarseLTwo}{0.020}
\newcommand{\nSATSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}{71.4}
\newcommand{\miouCISATSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}{1.0}
\newcommand{\dropSATSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}{14.1}
\newcommand{\dropCISATSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}{1.0}
\newcommand{\retSATSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}{0.836}
\newcommand{\retCISATSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}{0.011}
\newcommand{\nSATSnTwoCoarseLTwoVarDecoderSamLite}{5}
\newcommand{\miouSATSnTwoCoarseLTwoVarDecoderSamLite}{70.5}
\newcommand{\miouCISATSnTwoCoarseLTwoVarDecoderSamLite}{1.0}
\newcommand{\dropSATSnTwoCoarseLTwoVarDecoderSamLite}{14.5}
\newcommand{\dropCISATSnTwoCoarseLTwoVarDecoderSamLite}{1.1}
\newcommand{\retSATSnTwoCoarseLTwoVarDecoderSamLite}{0.830}
\newcommand{\retCISATSnTwoCoarseLTwoVarDecoderSamLite}{0.012}
\newcommand{\nSATSnTwoCoarseLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouSATSnTwoCoarseLTwoVarDecoderSegformerMlp}{71.1}
\newcommand{\miouCISATSnTwoCoarseLTwoVarDecoderSegformerMlp}{3.0}
\newcommand{\dropSATSnTwoCoarseLTwoVarDecoderSegformerMlp}{13.9}
\newcommand{\dropCISATSnTwoCoarseLTwoVarDecoderSegformerMlp}{2.9}
\newcommand{\retSATSnTwoCoarseLTwoVarDecoderSegformerMlp}{0.837}
\newcommand{\retCISATSnTwoCoarseLTwoVarDecoderSegformerMlp}{0.034}
\newcommand{\nSATSnTwoCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATSnTwoCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{73.0}
\newcommand{\miouCISATSnTwoCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{1.4}
\newcommand{\dropSATSnTwoCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{11.3}
\newcommand{\dropCISATSnTwoCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{1.6}
\newcommand{\retSATSnTwoCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.866}
\newcommand{\retCISATSnTwoCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.018}
\newcommand{\nSATSnTwoOmissionLOne}{5}
\newcommand{\miouSATSnTwoOmissionLOne}{81.2}
\newcommand{\miouCISATSnTwoOmissionLOne}{0.9}
\newcommand{\dropSATSnTwoOmissionLOne}{4.7}
\newcommand{\dropCISATSnTwoOmissionLOne}{1.0}
\newcommand{\retSATSnTwoOmissionLOne}{0.946}
\newcommand{\retCISATSnTwoOmissionLOne}{0.012}
\newcommand{\nSATSnTwoOmissionLTwo}{5}
\newcommand{\miouSATSnTwoOmissionLTwo}{71.1}
\newcommand{\miouCISATSnTwoOmissionLTwo}{5.7}
\newcommand{\dropSATSnTwoOmissionLTwo}{14.7}
\newcommand{\dropCISATSnTwoOmissionLTwo}{5.6}
\newcommand{\retSATSnTwoOmissionLTwo}{0.828}
\newcommand{\retCISATSnTwoOmissionLTwo}{0.065}
\newcommand{\nSATSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}{59.9}
\newcommand{\miouCISATSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}{12.3}
\newcommand{\dropSATSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}{25.6}
\newcommand{\dropCISATSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}{11.9}
\newcommand{\retSATSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}{0.700}
\newcommand{\retCISATSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}{0.142}
\newcommand{\nSATSnTwoOmissionLTwoVarDecoderSamLite}{5}
\newcommand{\miouSATSnTwoOmissionLTwoVarDecoderSamLite}{62.7}
\newcommand{\miouCISATSnTwoOmissionLTwoVarDecoderSamLite}{5.4}
\newcommand{\dropSATSnTwoOmissionLTwoVarDecoderSamLite}{22.3}
\newcommand{\dropCISATSnTwoOmissionLTwoVarDecoderSamLite}{5.3}
\newcommand{\retSATSnTwoOmissionLTwoVarDecoderSamLite}{0.738}
\newcommand{\retCISATSnTwoOmissionLTwoVarDecoderSamLite}{0.062}
\newcommand{\nSATSnTwoOmissionLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouSATSnTwoOmissionLTwoVarDecoderSegformerMlp}{66.2}
\newcommand{\miouCISATSnTwoOmissionLTwoVarDecoderSegformerMlp}{4.9}
\newcommand{\dropSATSnTwoOmissionLTwoVarDecoderSegformerMlp}{18.8}
\newcommand{\dropCISATSnTwoOmissionLTwoVarDecoderSegformerMlp}{4.7}
\newcommand{\retSATSnTwoOmissionLTwoVarDecoderSegformerMlp}{0.779}
\newcommand{\retCISATSnTwoOmissionLTwoVarDecoderSegformerMlp}{0.056}
\newcommand{\nSATSnTwoOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATSnTwoOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{69.9}
\newcommand{\miouCISATSnTwoOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{3.7}
\newcommand{\dropSATSnTwoOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{14.5}
\newcommand{\dropCISATSnTwoOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{3.9}
\newcommand{\retSATSnTwoOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{0.828}
\newcommand{\retCISATSnTwoOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{0.046}
\newcommand{\nSATSnTwoShiftLOne}{5}
\newcommand{\miouSATSnTwoShiftLOne}{84.4}
\newcommand{\miouCISATSnTwoShiftLOne}{0.4}
\newcommand{\dropSATSnTwoShiftLOne}{1.4}
\newcommand{\dropCISATSnTwoShiftLOne}{0.3}
\newcommand{\retSATSnTwoShiftLOne}{0.984}
\newcommand{\retCISATSnTwoShiftLOne}{0.003}
\newcommand{\nSATSnTwoShiftLTwo}{5}
\newcommand{\miouSATSnTwoShiftLTwo}{78.1}
\newcommand{\miouCISATSnTwoShiftLTwo}{0.5}
\newcommand{\dropSATSnTwoShiftLTwo}{7.7}
\newcommand{\dropCISATSnTwoShiftLTwo}{0.7}
\newcommand{\retSATSnTwoShiftLTwo}{0.910}
\newcommand{\retCISATSnTwoShiftLTwo}{0.008}
\newcommand{\nSATSnTwoShiftLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouSATSnTwoShiftLTwoVarDecoderMaskTwoformerLite}{76.1}
\newcommand{\miouCISATSnTwoShiftLTwoVarDecoderMaskTwoformerLite}{1.4}
\newcommand{\dropSATSnTwoShiftLTwoVarDecoderMaskTwoformerLite}{9.3}
\newcommand{\dropCISATSnTwoShiftLTwoVarDecoderMaskTwoformerLite}{1.7}
\newcommand{\retSATSnTwoShiftLTwoVarDecoderMaskTwoformerLite}{0.891}
\newcommand{\retCISATSnTwoShiftLTwoVarDecoderMaskTwoformerLite}{0.019}
\newcommand{\nSATSnTwoShiftLTwoVarDecoderSamLite}{5}
\newcommand{\miouSATSnTwoShiftLTwoVarDecoderSamLite}{75.0}
\newcommand{\miouCISATSnTwoShiftLTwoVarDecoderSamLite}{0.9}
\newcommand{\dropSATSnTwoShiftLTwoVarDecoderSamLite}{9.9}
\newcommand{\dropCISATSnTwoShiftLTwoVarDecoderSamLite}{0.7}
\newcommand{\retSATSnTwoShiftLTwoVarDecoderSamLite}{0.884}
\newcommand{\retCISATSnTwoShiftLTwoVarDecoderSamLite}{0.008}
\newcommand{\nSATSnTwoShiftLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouSATSnTwoShiftLTwoVarDecoderSegformerMlp}{76.4}
\newcommand{\miouCISATSnTwoShiftLTwoVarDecoderSegformerMlp}{1.1}
\newcommand{\dropSATSnTwoShiftLTwoVarDecoderSegformerMlp}{8.5}
\newcommand{\dropCISATSnTwoShiftLTwoVarDecoderSegformerMlp}{0.9}
\newcommand{\retSATSnTwoShiftLTwoVarDecoderSegformerMlp}{0.899}
\newcommand{\retCISATSnTwoShiftLTwoVarDecoderSegformerMlp}{0.011}
\newcommand{\nSATSnTwoShiftLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouSATSnTwoShiftLTwoVarLrMultZeroThreeThreeThreeThree}{77.8}
\newcommand{\miouCISATSnTwoShiftLTwoVarLrMultZeroThreeThreeThreeThree}{1.0}
\newcommand{\dropSATSnTwoShiftLTwoVarLrMultZeroThreeThreeThreeThree}{6.6}
\newcommand{\dropCISATSnTwoShiftLTwoVarLrMultZeroThreeThreeThreeThree}{1.0}
\newcommand{\retSATSnTwoShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.922}
\newcommand{\retCISATSnTwoShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.012}
\newcommand{\nDOFAburnBoundaryLOne}{5}
\newcommand{\miouDOFAburnBoundaryLOne}{82.4}
\newcommand{\miouCIDOFAburnBoundaryLOne}{1.0}
\newcommand{\dropDOFAburnBoundaryLOne}{3.1}
\newcommand{\dropCIDOFAburnBoundaryLOne}{1.6}
\newcommand{\retDOFAburnBoundaryLOne}{0.964}
\newcommand{\retCIDOFAburnBoundaryLOne}{0.018}
\newcommand{\nDOFAburnBoundaryLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouDOFAburnBoundaryLOneVarDecoderMaskTwoformerFull}{84.2}
\newcommand{\miouCIDOFAburnBoundaryLOneVarDecoderMaskTwoformerFull}{1.9}
\newcommand{\dropDOFAburnBoundaryLOneVarDecoderMaskTwoformerFull}{2.5}
\newcommand{\dropCIDOFAburnBoundaryLOneVarDecoderMaskTwoformerFull}{2.0}
\newcommand{\retDOFAburnBoundaryLOneVarDecoderMaskTwoformerFull}{0.971}
\newcommand{\retCIDOFAburnBoundaryLOneVarDecoderMaskTwoformerFull}{0.024}
\newcommand{\nDOFAburnBoundaryLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouDOFAburnBoundaryLOneVarDecoderMaskTwoformerLite}{81.9}
\newcommand{\miouCIDOFAburnBoundaryLOneVarDecoderMaskTwoformerLite}{1.0}
\newcommand{\dropDOFAburnBoundaryLOneVarDecoderMaskTwoformerLite}{4.6}
\newcommand{\dropCIDOFAburnBoundaryLOneVarDecoderMaskTwoformerLite}{1.4}
\newcommand{\retDOFAburnBoundaryLOneVarDecoderMaskTwoformerLite}{0.947}
\newcommand{\retCIDOFAburnBoundaryLOneVarDecoderMaskTwoformerLite}{0.015}
\newcommand{\nDOFAburnBoundaryLOneVarDecoderSamLite}{5}
\newcommand{\miouDOFAburnBoundaryLOneVarDecoderSamLite}{82.8}
\newcommand{\miouCIDOFAburnBoundaryLOneVarDecoderSamLite}{1.3}
\newcommand{\dropDOFAburnBoundaryLOneVarDecoderSamLite}{4.4}
\newcommand{\dropCIDOFAburnBoundaryLOneVarDecoderSamLite}{2.9}
\newcommand{\retDOFAburnBoundaryLOneVarDecoderSamLite}{0.950}
\newcommand{\retCIDOFAburnBoundaryLOneVarDecoderSamLite}{0.033}
\newcommand{\nDOFAburnBoundaryLOneVarDecoderSamPretrained}{5}
\newcommand{\miouDOFAburnBoundaryLOneVarDecoderSamPretrained}{81.8}
\newcommand{\miouCIDOFAburnBoundaryLOneVarDecoderSamPretrained}{0.7}
\newcommand{\dropDOFAburnBoundaryLOneVarDecoderSamPretrained}{3.6}
\newcommand{\dropCIDOFAburnBoundaryLOneVarDecoderSamPretrained}{1.0}
\newcommand{\retDOFAburnBoundaryLOneVarDecoderSamPretrained}{0.958}
\newcommand{\retCIDOFAburnBoundaryLOneVarDecoderSamPretrained}{0.011}
\newcommand{\nDOFAburnBoundaryLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouDOFAburnBoundaryLOneVarDecoderSegformerMlp}{83.0}
\newcommand{\miouCIDOFAburnBoundaryLOneVarDecoderSegformerMlp}{1.0}
\newcommand{\dropDOFAburnBoundaryLOneVarDecoderSegformerMlp}{3.8}
\newcommand{\dropCIDOFAburnBoundaryLOneVarDecoderSegformerMlp}{0.9}
\newcommand{\retDOFAburnBoundaryLOneVarDecoderSegformerMlp}{0.956}
\newcommand{\retCIDOFAburnBoundaryLOneVarDecoderSegformerMlp}{0.010}
\newcommand{\nDOFAburnBoundaryLTwo}{8}
\newcommand{\miouDOFAburnBoundaryLTwo}{70.8}
\newcommand{\miouCIDOFAburnBoundaryLTwo}{1.6}
\newcommand{\dropDOFAburnBoundaryLTwo}{14.7}
\newcommand{\dropCIDOFAburnBoundaryLTwo}{1.9}
\newcommand{\retDOFAburnBoundaryLTwo}{0.828}
\newcommand{\retCIDOFAburnBoundaryLTwo}{0.022}
\newcommand{\nDOFAburnBoundaryLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouDOFAburnBoundaryLTwoVarDecoderMaskTwoformerFull}{71.5}
\newcommand{\miouCIDOFAburnBoundaryLTwoVarDecoderMaskTwoformerFull}{1.9}
\newcommand{\dropDOFAburnBoundaryLTwoVarDecoderMaskTwoformerFull}{15.3}
\newcommand{\dropCIDOFAburnBoundaryLTwoVarDecoderMaskTwoformerFull}{2.3}
\newcommand{\retDOFAburnBoundaryLTwoVarDecoderMaskTwoformerFull}{0.824}
\newcommand{\retCIDOFAburnBoundaryLTwoVarDecoderMaskTwoformerFull}{0.025}
\newcommand{\nDOFAburnBoundaryLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouDOFAburnBoundaryLTwoVarDecoderMaskTwoformerLite}{69.8}
\newcommand{\miouCIDOFAburnBoundaryLTwoVarDecoderMaskTwoformerLite}{2.9}
\newcommand{\dropDOFAburnBoundaryLTwoVarDecoderMaskTwoformerLite}{16.7}
\newcommand{\dropCIDOFAburnBoundaryLTwoVarDecoderMaskTwoformerLite}{2.8}
\newcommand{\retDOFAburnBoundaryLTwoVarDecoderMaskTwoformerLite}{0.807}
\newcommand{\retCIDOFAburnBoundaryLTwoVarDecoderMaskTwoformerLite}{0.032}
\newcommand{\nDOFAburnBoundaryLTwoVarDecoderSamLite}{5}
\newcommand{\miouDOFAburnBoundaryLTwoVarDecoderSamLite}{74.3}
\newcommand{\miouCIDOFAburnBoundaryLTwoVarDecoderSamLite}{2.4}
\newcommand{\dropDOFAburnBoundaryLTwoVarDecoderSamLite}{12.8}
\newcommand{\dropCIDOFAburnBoundaryLTwoVarDecoderSamLite}{2.5}
\newcommand{\retDOFAburnBoundaryLTwoVarDecoderSamLite}{0.853}
\newcommand{\retCIDOFAburnBoundaryLTwoVarDecoderSamLite}{0.027}
\newcommand{\nDOFAburnBoundaryLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouDOFAburnBoundaryLTwoVarDecoderSamPretrained}{73.7}
\newcommand{\miouCIDOFAburnBoundaryLTwoVarDecoderSamPretrained}{2.2}
\newcommand{\dropDOFAburnBoundaryLTwoVarDecoderSamPretrained}{11.7}
\newcommand{\dropCIDOFAburnBoundaryLTwoVarDecoderSamPretrained}{2.5}
\newcommand{\retDOFAburnBoundaryLTwoVarDecoderSamPretrained}{0.863}
\newcommand{\retCIDOFAburnBoundaryLTwoVarDecoderSamPretrained}{0.029}
\newcommand{\nDOFAburnBoundaryLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouDOFAburnBoundaryLTwoVarDecoderSegformerMlp}{71.7}
\newcommand{\miouCIDOFAburnBoundaryLTwoVarDecoderSegformerMlp}{2.2}
\newcommand{\dropDOFAburnBoundaryLTwoVarDecoderSegformerMlp}{15.1}
\newcommand{\dropCIDOFAburnBoundaryLTwoVarDecoderSegformerMlp}{2.7}
\newcommand{\retDOFAburnBoundaryLTwoVarDecoderSegformerMlp}{0.826}
\newcommand{\retCIDOFAburnBoundaryLTwoVarDecoderSegformerMlp}{0.030}
\newcommand{\nDOFAburnBoundaryLTwoVarLossBootstrap}{5}
\newcommand{\miouDOFAburnBoundaryLTwoVarLossBootstrap}{72.4}
\newcommand{\miouCIDOFAburnBoundaryLTwoVarLossBootstrap}{2.3}
\newcommand{\dropDOFAburnBoundaryLTwoVarLossBootstrap}{14.0}
\newcommand{\dropCIDOFAburnBoundaryLTwoVarLossBootstrap}{2.1}
\newcommand{\retDOFAburnBoundaryLTwoVarLossBootstrap}{0.838}
\newcommand{\retCIDOFAburnBoundaryLTwoVarLossBootstrap}{0.024}
\newcommand{\nDOFAburnBoundaryLTwoVarLossGce}{5}
\newcommand{\miouDOFAburnBoundaryLTwoVarLossGce}{72.0}
\newcommand{\miouCIDOFAburnBoundaryLTwoVarLossGce}{1.6}
\newcommand{\dropDOFAburnBoundaryLTwoVarLossGce}{14.8}
\newcommand{\dropCIDOFAburnBoundaryLTwoVarLossGce}{2.1}
\newcommand{\retDOFAburnBoundaryLTwoVarLossGce}{0.829}
\newcommand{\retCIDOFAburnBoundaryLTwoVarLossGce}{0.023}
\newcommand{\nDOFAburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouDOFAburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{70.1}
\newcommand{\miouCIDOFAburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{1.6}
\newcommand{\dropDOFAburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{13.6}
\newcommand{\dropCIDOFAburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{1.3}
\newcommand{\retDOFAburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{0.838}
\newcommand{\retCIDOFAburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{0.014}
\newcommand{\nDOFAburnBoundaryLR}{5}
\newcommand{\miouDOFAburnBoundaryLR}{65.0}
\newcommand{\miouCIDOFAburnBoundaryLR}{4.4}
\newcommand{\dropDOFAburnBoundaryLR}{20.5}
\newcommand{\dropCIDOFAburnBoundaryLR}{4.7}
\newcommand{\retDOFAburnBoundaryLR}{0.760}
\newcommand{\retCIDOFAburnBoundaryLR}{0.054}
\newcommand{\nDOFAburnClean}{8}
\newcommand{\miouDOFAburnClean}{85.5}
\newcommand{\miouCIDOFAburnClean}{0.7}
\newcommand{\nDOFAburnCleanVarBandsRgb}{5}
\newcommand{\miouDOFAburnCleanVarBandsRgb}{81.6}
\newcommand{\miouCIDOFAburnCleanVarBandsRgb}{1.0}
\newcommand{\nDOFAburnCleanVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouDOFAburnCleanVarDecoderMaskTwoformerFull}{86.8}
\newcommand{\miouCIDOFAburnCleanVarDecoderMaskTwoformerFull}{1.2}
\newcommand{\nDOFAburnCleanVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouDOFAburnCleanVarDecoderMaskTwoformerLite}{86.4}
\newcommand{\miouCIDOFAburnCleanVarDecoderMaskTwoformerLite}{1.2}
\newcommand{\nDOFAburnCleanVarDecoderSamLite}{5}
\newcommand{\miouDOFAburnCleanVarDecoderSamLite}{87.1}
\newcommand{\miouCIDOFAburnCleanVarDecoderSamLite}{2.0}
\newcommand{\nDOFAburnCleanVarDecoderSamPretrained}{5}
\newcommand{\miouDOFAburnCleanVarDecoderSamPretrained}{85.4}
\newcommand{\miouCIDOFAburnCleanVarDecoderSamPretrained}{0.9}
\newcommand{\nDOFAburnCleanVarDecoderSegformerMlp}{5}
\newcommand{\miouDOFAburnCleanVarDecoderSegformerMlp}{86.8}
\newcommand{\miouCIDOFAburnCleanVarDecoderSegformerMlp}{1.2}
\newcommand{\nDOFAburnCleanVarFrozenEncoderTrue}{5}
\newcommand{\miouDOFAburnCleanVarFrozenEncoderTrue}{79.0}
\newcommand{\miouCIDOFAburnCleanVarFrozenEncoderTrue}{1.7}
\newcommand{\nDOFAburnCleanVarLossBootstrap}{5}
\newcommand{\miouDOFAburnCleanVarLossBootstrap}{86.4}
\newcommand{\miouCIDOFAburnCleanVarLossBootstrap}{0.7}
\newcommand{\nDOFAburnCleanVarLossGce}{5}
\newcommand{\miouDOFAburnCleanVarLossGce}{86.8}
\newcommand{\miouCIDOFAburnCleanVarLossGce}{1.6}
\newcommand{\nDOFAburnCleanVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouDOFAburnCleanVarLrMultZeroThreeThreeThreeThree}{83.7}
\newcommand{\miouCIDOFAburnCleanVarLrMultZeroThreeThreeThreeThree}{1.5}
\newcommand{\nDOFAburnCleanVarTrainSubsetCleanTwoFive}{5}
\newcommand{\miouDOFAburnCleanVarTrainSubsetCleanTwoFive}{79.9}
\newcommand{\miouCIDOFAburnCleanVarTrainSubsetCleanTwoFive}{4.4}
\newcommand{\nDOFAburnCoarseLOne}{5}
\newcommand{\miouDOFAburnCoarseLOne}{82.2}
\newcommand{\miouCIDOFAburnCoarseLOne}{1.3}
\newcommand{\dropDOFAburnCoarseLOne}{3.4}
\newcommand{\dropCIDOFAburnCoarseLOne}{2.1}
\newcommand{\retDOFAburnCoarseLOne}{0.961}
\newcommand{\retCIDOFAburnCoarseLOne}{0.025}
\newcommand{\nDOFAburnCoarseLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouDOFAburnCoarseLOneVarDecoderMaskTwoformerFull}{82.9}
\newcommand{\miouCIDOFAburnCoarseLOneVarDecoderMaskTwoformerFull}{1.4}
\newcommand{\dropDOFAburnCoarseLOneVarDecoderMaskTwoformerFull}{3.9}
\newcommand{\dropCIDOFAburnCoarseLOneVarDecoderMaskTwoformerFull}{1.7}
\newcommand{\retDOFAburnCoarseLOneVarDecoderMaskTwoformerFull}{0.956}
\newcommand{\retCIDOFAburnCoarseLOneVarDecoderMaskTwoformerFull}{0.020}
\newcommand{\nDOFAburnCoarseLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouDOFAburnCoarseLOneVarDecoderMaskTwoformerLite}{82.0}
\newcommand{\miouCIDOFAburnCoarseLOneVarDecoderMaskTwoformerLite}{1.0}
\newcommand{\dropDOFAburnCoarseLOneVarDecoderMaskTwoformerLite}{4.5}
\newcommand{\dropCIDOFAburnCoarseLOneVarDecoderMaskTwoformerLite}{1.9}
\newcommand{\retDOFAburnCoarseLOneVarDecoderMaskTwoformerLite}{0.948}
\newcommand{\retCIDOFAburnCoarseLOneVarDecoderMaskTwoformerLite}{0.021}
\newcommand{\nDOFAburnCoarseLOneVarDecoderSamLite}{5}
\newcommand{\miouDOFAburnCoarseLOneVarDecoderSamLite}{82.3}
\newcommand{\miouCIDOFAburnCoarseLOneVarDecoderSamLite}{1.1}
\newcommand{\dropDOFAburnCoarseLOneVarDecoderSamLite}{4.8}
\newcommand{\dropCIDOFAburnCoarseLOneVarDecoderSamLite}{3.0}
\newcommand{\retDOFAburnCoarseLOneVarDecoderSamLite}{0.945}
\newcommand{\retCIDOFAburnCoarseLOneVarDecoderSamLite}{0.033}
\newcommand{\nDOFAburnCoarseLOneVarDecoderSamPretrained}{5}
\newcommand{\miouDOFAburnCoarseLOneVarDecoderSamPretrained}{81.5}
\newcommand{\miouCIDOFAburnCoarseLOneVarDecoderSamPretrained}{1.5}
\newcommand{\dropDOFAburnCoarseLOneVarDecoderSamPretrained}{3.9}
\newcommand{\dropCIDOFAburnCoarseLOneVarDecoderSamPretrained}{1.1}
\newcommand{\retDOFAburnCoarseLOneVarDecoderSamPretrained}{0.954}
\newcommand{\retCIDOFAburnCoarseLOneVarDecoderSamPretrained}{0.013}
\newcommand{\nDOFAburnCoarseLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouDOFAburnCoarseLOneVarDecoderSegformerMlp}{81.9}
\newcommand{\miouCIDOFAburnCoarseLOneVarDecoderSegformerMlp}{1.4}
\newcommand{\dropDOFAburnCoarseLOneVarDecoderSegformerMlp}{4.9}
\newcommand{\dropCIDOFAburnCoarseLOneVarDecoderSegformerMlp}{2.2}
\newcommand{\retDOFAburnCoarseLOneVarDecoderSegformerMlp}{0.944}
\newcommand{\retCIDOFAburnCoarseLOneVarDecoderSegformerMlp}{0.024}
\newcommand{\nDOFAburnCoarseLTwo}{8}
\newcommand{\miouDOFAburnCoarseLTwo}{66.1}
\newcommand{\miouCIDOFAburnCoarseLTwo}{2.9}
\newcommand{\dropDOFAburnCoarseLTwo}{19.4}
\newcommand{\dropCIDOFAburnCoarseLTwo}{3.0}
\newcommand{\retDOFAburnCoarseLTwo}{0.773}
\newcommand{\retCIDOFAburnCoarseLTwo}{0.034}
\newcommand{\nDOFAburnCoarseLTwoVarBandsRgb}{5}
\newcommand{\miouDOFAburnCoarseLTwoVarBandsRgb}{67.2}
\newcommand{\miouCIDOFAburnCoarseLTwoVarBandsRgb}{2.3}
\newcommand{\dropDOFAburnCoarseLTwoVarBandsRgb}{14.5}
\newcommand{\dropCIDOFAburnCoarseLTwoVarBandsRgb}{2.3}
\newcommand{\retDOFAburnCoarseLTwoVarBandsRgb}{0.823}
\newcommand{\retCIDOFAburnCoarseLTwoVarBandsRgb}{0.028}
\newcommand{\nDOFAburnCoarseLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouDOFAburnCoarseLTwoVarDecoderMaskTwoformerFull}{60.6}
\newcommand{\miouCIDOFAburnCoarseLTwoVarDecoderMaskTwoformerFull}{6.4}
\newcommand{\dropDOFAburnCoarseLTwoVarDecoderMaskTwoformerFull}{26.2}
\newcommand{\dropCIDOFAburnCoarseLTwoVarDecoderMaskTwoformerFull}{7.2}
\newcommand{\retDOFAburnCoarseLTwoVarDecoderMaskTwoformerFull}{0.699}
\newcommand{\retCIDOFAburnCoarseLTwoVarDecoderMaskTwoformerFull}{0.081}
\newcommand{\nDOFAburnCoarseLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouDOFAburnCoarseLTwoVarDecoderMaskTwoformerLite}{65.9}
\newcommand{\miouCIDOFAburnCoarseLTwoVarDecoderMaskTwoformerLite}{4.2}
\newcommand{\dropDOFAburnCoarseLTwoVarDecoderMaskTwoformerLite}{20.5}
\newcommand{\dropCIDOFAburnCoarseLTwoVarDecoderMaskTwoformerLite}{4.1}
\newcommand{\retDOFAburnCoarseLTwoVarDecoderMaskTwoformerLite}{0.763}
\newcommand{\retCIDOFAburnCoarseLTwoVarDecoderMaskTwoformerLite}{0.047}
\newcommand{\nDOFAburnCoarseLTwoVarDecoderSamLite}{5}
\newcommand{\miouDOFAburnCoarseLTwoVarDecoderSamLite}{67.1}
\newcommand{\miouCIDOFAburnCoarseLTwoVarDecoderSamLite}{3.3}
\newcommand{\dropDOFAburnCoarseLTwoVarDecoderSamLite}{20.0}
\newcommand{\dropCIDOFAburnCoarseLTwoVarDecoderSamLite}{4.4}
\newcommand{\retDOFAburnCoarseLTwoVarDecoderSamLite}{0.771}
\newcommand{\retCIDOFAburnCoarseLTwoVarDecoderSamLite}{0.047}
\newcommand{\nDOFAburnCoarseLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouDOFAburnCoarseLTwoVarDecoderSamPretrained}{64.8}
\newcommand{\miouCIDOFAburnCoarseLTwoVarDecoderSamPretrained}{4.1}
\newcommand{\dropDOFAburnCoarseLTwoVarDecoderSamPretrained}{20.6}
\newcommand{\dropCIDOFAburnCoarseLTwoVarDecoderSamPretrained}{4.5}
\newcommand{\retDOFAburnCoarseLTwoVarDecoderSamPretrained}{0.759}
\newcommand{\retCIDOFAburnCoarseLTwoVarDecoderSamPretrained}{0.051}
\newcommand{\nDOFAburnCoarseLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouDOFAburnCoarseLTwoVarDecoderSegformerMlp}{64.1}
\newcommand{\miouCIDOFAburnCoarseLTwoVarDecoderSegformerMlp}{2.7}
\newcommand{\dropDOFAburnCoarseLTwoVarDecoderSegformerMlp}{22.7}
\newcommand{\dropCIDOFAburnCoarseLTwoVarDecoderSegformerMlp}{3.1}
\newcommand{\retDOFAburnCoarseLTwoVarDecoderSegformerMlp}{0.738}
\newcommand{\retCIDOFAburnCoarseLTwoVarDecoderSegformerMlp}{0.034}
\newcommand{\nDOFAburnCoarseLTwoVarFrozenEncoderTrue}{5}
\newcommand{\miouDOFAburnCoarseLTwoVarFrozenEncoderTrue}{60.7}
\newcommand{\miouCIDOFAburnCoarseLTwoVarFrozenEncoderTrue}{3.5}
\newcommand{\dropDOFAburnCoarseLTwoVarFrozenEncoderTrue}{18.3}
\newcommand{\dropCIDOFAburnCoarseLTwoVarFrozenEncoderTrue}{4.0}
\newcommand{\retDOFAburnCoarseLTwoVarFrozenEncoderTrue}{0.769}
\newcommand{\retCIDOFAburnCoarseLTwoVarFrozenEncoderTrue}{0.048}
\newcommand{\nDOFAburnCoarseLTwoVarLossBootstrap}{5}
\newcommand{\miouDOFAburnCoarseLTwoVarLossBootstrap}{64.7}
\newcommand{\miouCIDOFAburnCoarseLTwoVarLossBootstrap}{4.6}
\newcommand{\dropDOFAburnCoarseLTwoVarLossBootstrap}{21.7}
\newcommand{\dropCIDOFAburnCoarseLTwoVarLossBootstrap}{4.3}
\newcommand{\retDOFAburnCoarseLTwoVarLossBootstrap}{0.749}
\newcommand{\retCIDOFAburnCoarseLTwoVarLossBootstrap}{0.051}
\newcommand{\nDOFAburnCoarseLTwoVarLossGce}{5}
\newcommand{\miouDOFAburnCoarseLTwoVarLossGce}{66.9}
\newcommand{\miouCIDOFAburnCoarseLTwoVarLossGce}{5.4}
\newcommand{\dropDOFAburnCoarseLTwoVarLossGce}{19.8}
\newcommand{\dropCIDOFAburnCoarseLTwoVarLossGce}{5.8}
\newcommand{\retDOFAburnCoarseLTwoVarLossGce}{0.772}
\newcommand{\retCIDOFAburnCoarseLTwoVarLossGce}{0.065}
\newcommand{\nDOFAburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouDOFAburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{63.4}
\newcommand{\miouCIDOFAburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{4.0}
\newcommand{\dropDOFAburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{20.2}
\newcommand{\dropCIDOFAburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{3.8}
\newcommand{\retDOFAburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.758}
\newcommand{\retCIDOFAburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.046}
\newcommand{\nDOFAburnCoarseLR}{5}
\newcommand{\miouDOFAburnCoarseLR}{61.3}
\newcommand{\miouCIDOFAburnCoarseLR}{2.9}
\newcommand{\dropDOFAburnCoarseLR}{24.2}
\newcommand{\dropCIDOFAburnCoarseLR}{2.8}
\newcommand{\retDOFAburnCoarseLR}{0.717}
\newcommand{\retCIDOFAburnCoarseLR}{0.033}
\newcommand{\nDOFAburnOmissionLOne}{5}
\newcommand{\miouDOFAburnOmissionLOne}{76.9}
\newcommand{\miouCIDOFAburnOmissionLOne}{2.9}
\newcommand{\dropDOFAburnOmissionLOne}{8.6}
\newcommand{\dropCIDOFAburnOmissionLOne}{3.7}
\newcommand{\retDOFAburnOmissionLOne}{0.900}
\newcommand{\retCIDOFAburnOmissionLOne}{0.043}
\newcommand{\nDOFAburnOmissionLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouDOFAburnOmissionLOneVarDecoderMaskTwoformerFull}{84.1}
\newcommand{\miouCIDOFAburnOmissionLOneVarDecoderMaskTwoformerFull}{2.1}
\newcommand{\dropDOFAburnOmissionLOneVarDecoderMaskTwoformerFull}{2.7}
\newcommand{\dropCIDOFAburnOmissionLOneVarDecoderMaskTwoformerFull}{2.6}
\newcommand{\retDOFAburnOmissionLOneVarDecoderMaskTwoformerFull}{0.969}
\newcommand{\retCIDOFAburnOmissionLOneVarDecoderMaskTwoformerFull}{0.030}
\newcommand{\nDOFAburnOmissionLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouDOFAburnOmissionLOneVarDecoderMaskTwoformerLite}{79.6}
\newcommand{\miouCIDOFAburnOmissionLOneVarDecoderMaskTwoformerLite}{2.4}
\newcommand{\dropDOFAburnOmissionLOneVarDecoderMaskTwoformerLite}{6.9}
\newcommand{\dropCIDOFAburnOmissionLOneVarDecoderMaskTwoformerLite}{1.4}
\newcommand{\retDOFAburnOmissionLOneVarDecoderMaskTwoformerLite}{0.920}
\newcommand{\retCIDOFAburnOmissionLOneVarDecoderMaskTwoformerLite}{0.017}
\newcommand{\nDOFAburnOmissionLOneVarDecoderSamLite}{5}
\newcommand{\miouDOFAburnOmissionLOneVarDecoderSamLite}{81.8}
\newcommand{\miouCIDOFAburnOmissionLOneVarDecoderSamLite}{3.5}
\newcommand{\dropDOFAburnOmissionLOneVarDecoderSamLite}{5.3}
\newcommand{\dropCIDOFAburnOmissionLOneVarDecoderSamLite}{3.8}
\newcommand{\retDOFAburnOmissionLOneVarDecoderSamLite}{0.939}
\newcommand{\retCIDOFAburnOmissionLOneVarDecoderSamLite}{0.043}
\newcommand{\nDOFAburnOmissionLOneVarDecoderSamPretrained}{5}
\newcommand{\miouDOFAburnOmissionLOneVarDecoderSamPretrained}{73.4}
\newcommand{\miouCIDOFAburnOmissionLOneVarDecoderSamPretrained}{20.2}
\newcommand{\dropDOFAburnOmissionLOneVarDecoderSamPretrained}{12.0}
\newcommand{\dropCIDOFAburnOmissionLOneVarDecoderSamPretrained}{20.0}
\newcommand{\retDOFAburnOmissionLOneVarDecoderSamPretrained}{0.860}
\newcommand{\retCIDOFAburnOmissionLOneVarDecoderSamPretrained}{0.235}
\newcommand{\nDOFAburnOmissionLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouDOFAburnOmissionLOneVarDecoderSegformerMlp}{75.1}
\newcommand{\miouCIDOFAburnOmissionLOneVarDecoderSegformerMlp}{3.7}
\newcommand{\dropDOFAburnOmissionLOneVarDecoderSegformerMlp}{11.7}
\newcommand{\dropCIDOFAburnOmissionLOneVarDecoderSegformerMlp}{2.8}
\newcommand{\retDOFAburnOmissionLOneVarDecoderSegformerMlp}{0.865}
\newcommand{\retCIDOFAburnOmissionLOneVarDecoderSegformerMlp}{0.034}
\newcommand{\nDOFAburnOmissionLTwo}{8}
\newcommand{\miouDOFAburnOmissionLTwo}{61.1}
\newcommand{\miouCIDOFAburnOmissionLTwo}{4.5}
\newcommand{\dropDOFAburnOmissionLTwo}{24.4}
\newcommand{\dropCIDOFAburnOmissionLTwo}{4.4}
\newcommand{\retDOFAburnOmissionLTwo}{0.714}
\newcommand{\retCIDOFAburnOmissionLTwo}{0.052}
\newcommand{\nDOFAburnOmissionLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouDOFAburnOmissionLTwoVarDecoderMaskTwoformerFull}{66.6}
\newcommand{\miouCIDOFAburnOmissionLTwoVarDecoderMaskTwoformerFull}{8.8}
\newcommand{\dropDOFAburnOmissionLTwoVarDecoderMaskTwoformerFull}{20.2}
\newcommand{\dropCIDOFAburnOmissionLTwoVarDecoderMaskTwoformerFull}{9.8}
\newcommand{\retDOFAburnOmissionLTwoVarDecoderMaskTwoformerFull}{0.768}
\newcommand{\retCIDOFAburnOmissionLTwoVarDecoderMaskTwoformerFull}{0.111}
\newcommand{\nDOFAburnOmissionLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouDOFAburnOmissionLTwoVarDecoderMaskTwoformerLite}{59.2}
\newcommand{\miouCIDOFAburnOmissionLTwoVarDecoderMaskTwoformerLite}{3.1}
\newcommand{\dropDOFAburnOmissionLTwoVarDecoderMaskTwoformerLite}{27.3}
\newcommand{\dropCIDOFAburnOmissionLTwoVarDecoderMaskTwoformerLite}{3.9}
\newcommand{\retDOFAburnOmissionLTwoVarDecoderMaskTwoformerLite}{0.685}
\newcommand{\retCIDOFAburnOmissionLTwoVarDecoderMaskTwoformerLite}{0.042}
\newcommand{\nDOFAburnOmissionLTwoVarDecoderSamLite}{5}
\newcommand{\miouDOFAburnOmissionLTwoVarDecoderSamLite}{66.2}
\newcommand{\miouCIDOFAburnOmissionLTwoVarDecoderSamLite}{2.8}
\newcommand{\dropDOFAburnOmissionLTwoVarDecoderSamLite}{20.9}
\newcommand{\dropCIDOFAburnOmissionLTwoVarDecoderSamLite}{1.6}
\newcommand{\retDOFAburnOmissionLTwoVarDecoderSamLite}{0.760}
\newcommand{\retCIDOFAburnOmissionLTwoVarDecoderSamLite}{0.020}
\newcommand{\nDOFAburnOmissionLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouDOFAburnOmissionLTwoVarDecoderSamPretrained}{55.9}
\newcommand{\miouCIDOFAburnOmissionLTwoVarDecoderSamPretrained}{9.2}
\newcommand{\dropDOFAburnOmissionLTwoVarDecoderSamPretrained}{29.5}
\newcommand{\dropCIDOFAburnOmissionLTwoVarDecoderSamPretrained}{8.6}
\newcommand{\retDOFAburnOmissionLTwoVarDecoderSamPretrained}{0.654}
\newcommand{\retCIDOFAburnOmissionLTwoVarDecoderSamPretrained}{0.103}
\newcommand{\nDOFAburnOmissionLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouDOFAburnOmissionLTwoVarDecoderSegformerMlp}{55.7}
\newcommand{\miouCIDOFAburnOmissionLTwoVarDecoderSegformerMlp}{6.6}
\newcommand{\dropDOFAburnOmissionLTwoVarDecoderSegformerMlp}{31.1}
\newcommand{\dropCIDOFAburnOmissionLTwoVarDecoderSegformerMlp}{5.9}
\newcommand{\retDOFAburnOmissionLTwoVarDecoderSegformerMlp}{0.642}
\newcommand{\retCIDOFAburnOmissionLTwoVarDecoderSegformerMlp}{0.070}
\newcommand{\nDOFAburnOmissionLTwoVarLossBootstrap}{5}
\newcommand{\miouDOFAburnOmissionLTwoVarLossBootstrap}{64.4}
\newcommand{\miouCIDOFAburnOmissionLTwoVarLossBootstrap}{6.2}
\newcommand{\dropDOFAburnOmissionLTwoVarLossBootstrap}{22.0}
\newcommand{\dropCIDOFAburnOmissionLTwoVarLossBootstrap}{5.9}
\newcommand{\retDOFAburnOmissionLTwoVarLossBootstrap}{0.745}
\newcommand{\retCIDOFAburnOmissionLTwoVarLossBootstrap}{0.069}
\newcommand{\nDOFAburnOmissionLTwoVarLossGce}{5}
\newcommand{\miouDOFAburnOmissionLTwoVarLossGce}{64.7}
\newcommand{\miouCIDOFAburnOmissionLTwoVarLossGce}{4.7}
\newcommand{\dropDOFAburnOmissionLTwoVarLossGce}{22.1}
\newcommand{\dropCIDOFAburnOmissionLTwoVarLossGce}{5.9}
\newcommand{\retDOFAburnOmissionLTwoVarLossGce}{0.745}
\newcommand{\retCIDOFAburnOmissionLTwoVarLossGce}{0.064}
\newcommand{\nDOFAburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouDOFAburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{59.7}
\newcommand{\miouCIDOFAburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{8.3}
\newcommand{\dropDOFAburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{24.0}
\newcommand{\dropCIDOFAburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{7.4}
\newcommand{\retDOFAburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{0.712}
\newcommand{\retCIDOFAburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{0.090}
\newcommand{\nDOFAburnOmissionLR}{5}
\newcommand{\miouDOFAburnOmissionLR}{54.4}
\newcommand{\miouCIDOFAburnOmissionLR}{3.7}
\newcommand{\dropDOFAburnOmissionLR}{31.1}
\newcommand{\dropCIDOFAburnOmissionLR}{3.2}
\newcommand{\retDOFAburnOmissionLR}{0.636}
\newcommand{\retCIDOFAburnOmissionLR}{0.039}
\newcommand{\nDOFAburnShiftLOne}{5}
\newcommand{\miouDOFAburnShiftLOne}{84.2}
\newcommand{\miouCIDOFAburnShiftLOne}{1.4}
\newcommand{\dropDOFAburnShiftLOne}{1.4}
\newcommand{\dropCIDOFAburnShiftLOne}{0.6}
\newcommand{\retDOFAburnShiftLOne}{0.984}
\newcommand{\retCIDOFAburnShiftLOne}{0.008}
\newcommand{\nDOFAburnShiftLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouDOFAburnShiftLOneVarDecoderMaskTwoformerFull}{84.3}
\newcommand{\miouCIDOFAburnShiftLOneVarDecoderMaskTwoformerFull}{1.3}
\newcommand{\dropDOFAburnShiftLOneVarDecoderMaskTwoformerFull}{2.5}
\newcommand{\dropCIDOFAburnShiftLOneVarDecoderMaskTwoformerFull}{2.1}
\newcommand{\retDOFAburnShiftLOneVarDecoderMaskTwoformerFull}{0.971}
\newcommand{\retCIDOFAburnShiftLOneVarDecoderMaskTwoformerFull}{0.024}
\newcommand{\nDOFAburnShiftLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouDOFAburnShiftLOneVarDecoderMaskTwoformerLite}{83.1}
\newcommand{\miouCIDOFAburnShiftLOneVarDecoderMaskTwoformerLite}{0.5}
\newcommand{\dropDOFAburnShiftLOneVarDecoderMaskTwoformerLite}{3.3}
\newcommand{\dropCIDOFAburnShiftLOneVarDecoderMaskTwoformerLite}{1.2}
\newcommand{\retDOFAburnShiftLOneVarDecoderMaskTwoformerLite}{0.962}
\newcommand{\retCIDOFAburnShiftLOneVarDecoderMaskTwoformerLite}{0.013}
\newcommand{\nDOFAburnShiftLOneVarDecoderSamLite}{5}
\newcommand{\miouDOFAburnShiftLOneVarDecoderSamLite}{84.0}
\newcommand{\miouCIDOFAburnShiftLOneVarDecoderSamLite}{0.6}
\newcommand{\dropDOFAburnShiftLOneVarDecoderSamLite}{3.1}
\newcommand{\dropCIDOFAburnShiftLOneVarDecoderSamLite}{2.4}
\newcommand{\retDOFAburnShiftLOneVarDecoderSamLite}{0.965}
\newcommand{\retCIDOFAburnShiftLOneVarDecoderSamLite}{0.027}
\newcommand{\nDOFAburnShiftLOneVarDecoderSamPretrained}{5}
\newcommand{\miouDOFAburnShiftLOneVarDecoderSamPretrained}{83.5}
\newcommand{\miouCIDOFAburnShiftLOneVarDecoderSamPretrained}{1.6}
\newcommand{\dropDOFAburnShiftLOneVarDecoderSamPretrained}{1.9}
\newcommand{\dropCIDOFAburnShiftLOneVarDecoderSamPretrained}{2.0}
\newcommand{\retDOFAburnShiftLOneVarDecoderSamPretrained}{0.977}
\newcommand{\retCIDOFAburnShiftLOneVarDecoderSamPretrained}{0.023}
\newcommand{\nDOFAburnShiftLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouDOFAburnShiftLOneVarDecoderSegformerMlp}{84.0}
\newcommand{\miouCIDOFAburnShiftLOneVarDecoderSegformerMlp}{1.5}
\newcommand{\dropDOFAburnShiftLOneVarDecoderSegformerMlp}{2.9}
\newcommand{\dropCIDOFAburnShiftLOneVarDecoderSegformerMlp}{2.4}
\newcommand{\retDOFAburnShiftLOneVarDecoderSegformerMlp}{0.967}
\newcommand{\retCIDOFAburnShiftLOneVarDecoderSegformerMlp}{0.027}
\newcommand{\nDOFAburnShiftLTwo}{8}
\newcommand{\miouDOFAburnShiftLTwo}{74.6}
\newcommand{\miouCIDOFAburnShiftLTwo}{1.2}
\newcommand{\dropDOFAburnShiftLTwo}{10.9}
\newcommand{\dropCIDOFAburnShiftLTwo}{1.2}
\newcommand{\retDOFAburnShiftLTwo}{0.873}
\newcommand{\retCIDOFAburnShiftLTwo}{0.014}
\newcommand{\nDOFAburnShiftLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouDOFAburnShiftLTwoVarDecoderMaskTwoformerFull}{73.3}
\newcommand{\miouCIDOFAburnShiftLTwoVarDecoderMaskTwoformerFull}{2.3}
\newcommand{\dropDOFAburnShiftLTwoVarDecoderMaskTwoformerFull}{13.5}
\newcommand{\dropCIDOFAburnShiftLTwoVarDecoderMaskTwoformerFull}{2.9}
\newcommand{\retDOFAburnShiftLTwoVarDecoderMaskTwoformerFull}{0.845}
\newcommand{\retCIDOFAburnShiftLTwoVarDecoderMaskTwoformerFull}{0.032}
\newcommand{\nDOFAburnShiftLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouDOFAburnShiftLTwoVarDecoderMaskTwoformerLite}{73.3}
\newcommand{\miouCIDOFAburnShiftLTwoVarDecoderMaskTwoformerLite}{1.5}
\newcommand{\dropDOFAburnShiftLTwoVarDecoderMaskTwoformerLite}{13.1}
\newcommand{\dropCIDOFAburnShiftLTwoVarDecoderMaskTwoformerLite}{2.1}
\newcommand{\retDOFAburnShiftLTwoVarDecoderMaskTwoformerLite}{0.849}
\newcommand{\retCIDOFAburnShiftLTwoVarDecoderMaskTwoformerLite}{0.023}
\newcommand{\nDOFAburnShiftLTwoVarDecoderSamLite}{5}
\newcommand{\miouDOFAburnShiftLTwoVarDecoderSamLite}{72.9}
\newcommand{\miouCIDOFAburnShiftLTwoVarDecoderSamLite}{1.5}
\newcommand{\dropDOFAburnShiftLTwoVarDecoderSamLite}{14.2}
\newcommand{\dropCIDOFAburnShiftLTwoVarDecoderSamLite}{1.8}
\newcommand{\retDOFAburnShiftLTwoVarDecoderSamLite}{0.837}
\newcommand{\retCIDOFAburnShiftLTwoVarDecoderSamLite}{0.018}
\newcommand{\nDOFAburnShiftLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouDOFAburnShiftLTwoVarDecoderSamPretrained}{74.1}
\newcommand{\miouCIDOFAburnShiftLTwoVarDecoderSamPretrained}{1.9}
\newcommand{\dropDOFAburnShiftLTwoVarDecoderSamPretrained}{11.4}
\newcommand{\dropCIDOFAburnShiftLTwoVarDecoderSamPretrained}{1.8}
\newcommand{\retDOFAburnShiftLTwoVarDecoderSamPretrained}{0.867}
\newcommand{\retCIDOFAburnShiftLTwoVarDecoderSamPretrained}{0.022}
\newcommand{\nDOFAburnShiftLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouDOFAburnShiftLTwoVarDecoderSegformerMlp}{72.5}
\newcommand{\miouCIDOFAburnShiftLTwoVarDecoderSegformerMlp}{1.5}
\newcommand{\dropDOFAburnShiftLTwoVarDecoderSegformerMlp}{14.4}
\newcommand{\dropCIDOFAburnShiftLTwoVarDecoderSegformerMlp}{1.2}
\newcommand{\retDOFAburnShiftLTwoVarDecoderSegformerMlp}{0.835}
\newcommand{\retCIDOFAburnShiftLTwoVarDecoderSegformerMlp}{0.014}
\newcommand{\nDOFAburnShiftLTwoVarLossBootstrap}{5}
\newcommand{\miouDOFAburnShiftLTwoVarLossBootstrap}{73.1}
\newcommand{\miouCIDOFAburnShiftLTwoVarLossBootstrap}{1.8}
\newcommand{\dropDOFAburnShiftLTwoVarLossBootstrap}{13.3}
\newcommand{\dropCIDOFAburnShiftLTwoVarLossBootstrap}{1.6}
\newcommand{\retDOFAburnShiftLTwoVarLossBootstrap}{0.846}
\newcommand{\retCIDOFAburnShiftLTwoVarLossBootstrap}{0.019}
\newcommand{\nDOFAburnShiftLTwoVarLossGce}{5}
\newcommand{\miouDOFAburnShiftLTwoVarLossGce}{75.0}
\newcommand{\miouCIDOFAburnShiftLTwoVarLossGce}{2.0}
\newcommand{\dropDOFAburnShiftLTwoVarLossGce}{11.8}
\newcommand{\dropCIDOFAburnShiftLTwoVarLossGce}{2.9}
\newcommand{\retDOFAburnShiftLTwoVarLossGce}{0.864}
\newcommand{\retCIDOFAburnShiftLTwoVarLossGce}{0.032}
\newcommand{\nDOFAburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouDOFAburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{73.2}
\newcommand{\miouCIDOFAburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{1.3}
\newcommand{\dropDOFAburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{10.5}
\newcommand{\dropCIDOFAburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{1.6}
\newcommand{\retDOFAburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.875}
\newcommand{\retCIDOFAburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.018}
\newcommand{\nDOFAburnShiftLR}{5}
\newcommand{\miouDOFAburnShiftLR}{65.2}
\newcommand{\miouCIDOFAburnShiftLR}{5.6}
\newcommand{\dropDOFAburnShiftLR}{20.4}
\newcommand{\dropCIDOFAburnShiftLR}{5.7}
\newcommand{\retDOFAburnShiftLR}{0.762}
\newcommand{\retCIDOFAburnShiftLR}{0.066}
\newcommand{\nDOFAChesBoundaryLOne}{5}
\newcommand{\miouDOFAChesBoundaryLOne}{79.8}
\newcommand{\miouCIDOFAChesBoundaryLOne}{0.8}
\newcommand{\dropDOFAChesBoundaryLOne}{3.2}
\newcommand{\dropCIDOFAChesBoundaryLOne}{0.6}
\newcommand{\retDOFAChesBoundaryLOne}{0.962}
\newcommand{\retCIDOFAChesBoundaryLOne}{0.007}
\newcommand{\nDOFAChesBoundaryLTwo}{5}
\newcommand{\miouDOFAChesBoundaryLTwo}{70.1}
\newcommand{\miouCIDOFAChesBoundaryLTwo}{2.8}
\newcommand{\dropDOFAChesBoundaryLTwo}{12.9}
\newcommand{\dropCIDOFAChesBoundaryLTwo}{2.7}
\newcommand{\retDOFAChesBoundaryLTwo}{0.845}
\newcommand{\retCIDOFAChesBoundaryLTwo}{0.032}
\newcommand{\nDOFAChesClean}{5}
\newcommand{\miouDOFAChesClean}{83.0}
\newcommand{\miouCIDOFAChesClean}{0.2}
\newcommand{\nDOFAChesCoarseLOne}{5}
\newcommand{\miouDOFAChesCoarseLOne}{80.9}
\newcommand{\miouCIDOFAChesCoarseLOne}{0.9}
\newcommand{\dropDOFAChesCoarseLOne}{2.1}
\newcommand{\dropCIDOFAChesCoarseLOne}{0.8}
\newcommand{\retDOFAChesCoarseLOne}{0.975}
\newcommand{\retCIDOFAChesCoarseLOne}{0.010}
\newcommand{\nDOFAChesCoarseLTwo}{5}
\newcommand{\miouDOFAChesCoarseLTwo}{70.0}
\newcommand{\miouCIDOFAChesCoarseLTwo}{0.7}
\newcommand{\dropDOFAChesCoarseLTwo}{13.0}
\newcommand{\dropCIDOFAChesCoarseLTwo}{0.8}
\newcommand{\retDOFAChesCoarseLTwo}{0.843}
\newcommand{\retCIDOFAChesCoarseLTwo}{0.009}
\newcommand{\nDOFAChesNlcdREAL}{5}
\newcommand{\miouDOFAChesNlcdREAL}{60.7}
\newcommand{\miouCIDOFAChesNlcdREAL}{1.5}
\newcommand{\dropDOFAChesNlcdREAL}{22.3}
\newcommand{\dropCIDOFAChesNlcdREAL}{1.3}
\newcommand{\retDOFAChesNlcdREAL}{0.732}
\newcommand{\retCIDOFAChesNlcdREAL}{0.016}
\newcommand{\nDOFAChesOmissionLOne}{5}
\newcommand{\miouDOFAChesOmissionLOne}{79.1}
\newcommand{\miouCIDOFAChesOmissionLOne}{1.2}
\newcommand{\dropDOFAChesOmissionLOne}{4.0}
\newcommand{\dropCIDOFAChesOmissionLOne}{1.3}
\newcommand{\retDOFAChesOmissionLOne}{0.952}
\newcommand{\retCIDOFAChesOmissionLOne}{0.015}
\newcommand{\nDOFAChesOmissionLTwo}{5}
\newcommand{\miouDOFAChesOmissionLTwo}{69.0}
\newcommand{\miouCIDOFAChesOmissionLTwo}{4.8}
\newcommand{\dropDOFAChesOmissionLTwo}{14.0}
\newcommand{\dropCIDOFAChesOmissionLTwo}{4.8}
\newcommand{\retDOFAChesOmissionLTwo}{0.832}
\newcommand{\retCIDOFAChesOmissionLTwo}{0.058}
\newcommand{\nDOFAChesShiftLOne}{5}
\newcommand{\miouDOFAChesShiftLOne}{81.8}
\newcommand{\miouCIDOFAChesShiftLOne}{0.5}
\newcommand{\dropDOFAChesShiftLOne}{1.2}
\newcommand{\dropCIDOFAChesShiftLOne}{0.4}
\newcommand{\retDOFAChesShiftLOne}{0.985}
\newcommand{\retCIDOFAChesShiftLOne}{0.005}
\newcommand{\nDOFAChesShiftLTwo}{5}
\newcommand{\miouDOFAChesShiftLTwo}{75.0}
\newcommand{\miouCIDOFAChesShiftLTwo}{1.1}
\newcommand{\dropDOFAChesShiftLTwo}{8.0}
\newcommand{\dropCIDOFAChesShiftLTwo}{1.2}
\newcommand{\retDOFAChesShiftLTwo}{0.903}
\newcommand{\retCIDOFAChesShiftLTwo}{0.015}
\newcommand{\nDOFACsTwelveBoundaryLOne}{5}
\newcommand{\miouDOFACsTwelveBoundaryLOne}{63.0}
\newcommand{\miouCIDOFACsTwelveBoundaryLOne}{1.1}
\newcommand{\dropDOFACsTwelveBoundaryLOne}{2.8}
\newcommand{\dropCIDOFACsTwelveBoundaryLOne}{1.4}
\newcommand{\retDOFACsTwelveBoundaryLOne}{0.957}
\newcommand{\retCIDOFACsTwelveBoundaryLOne}{0.021}
\newcommand{\nDOFACsTwelveBoundaryLTwo}{5}
\newcommand{\miouDOFACsTwelveBoundaryLTwo}{58.4}
\newcommand{\miouCIDOFACsTwelveBoundaryLTwo}{1.2}
\newcommand{\dropDOFACsTwelveBoundaryLTwo}{7.5}
\newcommand{\dropCIDOFACsTwelveBoundaryLTwo}{1.7}
\newcommand{\retDOFACsTwelveBoundaryLTwo}{0.886}
\newcommand{\retCIDOFACsTwelveBoundaryLTwo}{0.025}
\newcommand{\nDOFACsTwelveClean}{5}
\newcommand{\miouDOFACsTwelveClean}{65.9}
\newcommand{\miouCIDOFACsTwelveClean}{0.7}
\newcommand{\nDOFACsTwelveCoarseLOne}{5}
\newcommand{\miouDOFACsTwelveCoarseLOne}{64.2}
\newcommand{\miouCIDOFACsTwelveCoarseLOne}{1.4}
\newcommand{\dropDOFACsTwelveCoarseLOne}{1.7}
\newcommand{\dropCIDOFACsTwelveCoarseLOne}{2.0}
\newcommand{\retDOFACsTwelveCoarseLOne}{0.974}
\newcommand{\retCIDOFACsTwelveCoarseLOne}{0.029}
\newcommand{\nDOFACsTwelveCoarseLTwo}{5}
\newcommand{\miouDOFACsTwelveCoarseLTwo}{57.6}
\newcommand{\miouCIDOFACsTwelveCoarseLTwo}{1.1}
\newcommand{\dropDOFACsTwelveCoarseLTwo}{8.3}
\newcommand{\dropCIDOFACsTwelveCoarseLTwo}{0.7}
\newcommand{\retDOFACsTwelveCoarseLTwo}{0.874}
\newcommand{\retCIDOFACsTwelveCoarseLTwo}{0.012}
\newcommand{\nDOFACsTwelveOmissionLOne}{5}
\newcommand{\miouDOFACsTwelveOmissionLOne}{62.2}
\newcommand{\miouCIDOFACsTwelveOmissionLOne}{1.2}
\newcommand{\dropDOFACsTwelveOmissionLOne}{3.6}
\newcommand{\dropCIDOFACsTwelveOmissionLOne}{0.8}
\newcommand{\retDOFACsTwelveOmissionLOne}{0.945}
\newcommand{\retCIDOFACsTwelveOmissionLOne}{0.012}
\newcommand{\nDOFACsTwelveOmissionLTwo}{5}
\newcommand{\miouDOFACsTwelveOmissionLTwo}{57.8}
\newcommand{\miouCIDOFACsTwelveOmissionLTwo}{1.7}
\newcommand{\dropDOFACsTwelveOmissionLTwo}{8.1}
\newcommand{\dropCIDOFACsTwelveOmissionLTwo}{1.3}
\newcommand{\retDOFACsTwelveOmissionLTwo}{0.877}
\newcommand{\retCIDOFACsTwelveOmissionLTwo}{0.021}
\newcommand{\nDOFACsTwelveSTwocloudlessREAL}{5}
\newcommand{\miouDOFACsTwelveSTwocloudlessREAL}{34.5}
\newcommand{\miouCIDOFACsTwelveSTwocloudlessREAL}{0.5}
\newcommand{\dropDOFACsTwelveSTwocloudlessREAL}{31.4}
\newcommand{\dropCIDOFACsTwelveSTwocloudlessREAL}{1.2}
\newcommand{\retDOFACsTwelveSTwocloudlessREAL}{0.523}
\newcommand{\retCIDOFACsTwelveSTwocloudlessREAL}{0.013}
\newcommand{\nDOFACsTwelveShiftLOne}{5}
\newcommand{\miouDOFACsTwelveShiftLOne}{65.5}
\newcommand{\miouCIDOFACsTwelveShiftLOne}{0.7}
\newcommand{\dropDOFACsTwelveShiftLOne}{0.3}
\newcommand{\dropCIDOFACsTwelveShiftLOne}{0.6}
\newcommand{\retDOFACsTwelveShiftLOne}{0.995}
\newcommand{\retCIDOFACsTwelveShiftLOne}{0.009}
\newcommand{\nDOFACsTwelveShiftLTwo}{5}
\newcommand{\miouDOFACsTwelveShiftLTwo}{61.1}
\newcommand{\miouCIDOFACsTwelveShiftLTwo}{0.3}
\newcommand{\dropDOFACsTwelveShiftLTwo}{4.8}
\newcommand{\dropCIDOFACsTwelveShiftLTwo}{0.5}
\newcommand{\retDOFACsTwelveShiftLTwo}{0.927}
\newcommand{\retCIDOFACsTwelveShiftLTwo}{0.007}
\newcommand{\nDOFADfcBoundaryLOne}{5}
\newcommand{\miouDOFADfcBoundaryLOne}{35.3}
\newcommand{\miouCIDOFADfcBoundaryLOne}{1.0}
\newcommand{\dropDOFADfcBoundaryLOne}{1.2}
\newcommand{\dropCIDOFADfcBoundaryLOne}{2.0}
\newcommand{\retDOFADfcBoundaryLOne}{0.969}
\newcommand{\retCIDOFADfcBoundaryLOne}{0.056}
\newcommand{\nDOFADfcBoundaryLTwo}{5}
\newcommand{\miouDOFADfcBoundaryLTwo}{33.7}
\newcommand{\miouCIDOFADfcBoundaryLTwo}{2.0}
\newcommand{\dropDOFADfcBoundaryLTwo}{2.9}
\newcommand{\dropCIDOFADfcBoundaryLTwo}{2.7}
\newcommand{\retDOFADfcBoundaryLTwo}{0.923}
\newcommand{\retCIDOFADfcBoundaryLTwo}{0.076}
\newcommand{\nDOFADfcClean}{5}
\newcommand{\miouDOFADfcClean}{36.5}
\newcommand{\miouCIDOFADfcClean}{1.7}
\newcommand{\nDOFADfcCleanVarTrainSubsetRealcov}{5}
\newcommand{\miouDOFADfcCleanVarTrainSubsetRealcov}{36.7}
\newcommand{\miouCIDOFADfcCleanVarTrainSubsetRealcov}{1.0}
\newcommand{\nDOFADfcCoarseLOne}{5}
\newcommand{\miouDOFADfcCoarseLOne}{37.0}
\newcommand{\miouCIDOFADfcCoarseLOne}{0.4}
\newcommand{\dropDOFADfcCoarseLOne}{\ensuremath{-}0.5}
\newcommand{\dropCIDOFADfcCoarseLOne}{1.9}
\newcommand{\retDOFADfcCoarseLOne}{1.015}
\newcommand{\retCIDOFADfcCoarseLOne}{0.053}
\newcommand{\nDOFADfcCoarseLTwo}{5}
\newcommand{\miouDOFADfcCoarseLTwo}{36.3}
\newcommand{\miouCIDOFADfcCoarseLTwo}{1.0}
\newcommand{\dropDOFADfcCoarseLTwo}{0.3}
\newcommand{\dropCIDOFADfcCoarseLTwo}{1.4}
\newcommand{\retDOFADfcCoarseLTwo}{0.994}
\newcommand{\retCIDOFADfcCoarseLTwo}{0.040}
\newcommand{\nDOFADfcModisREALVarTrainSubsetRealcov}{5}
\newcommand{\miouDOFADfcModisREALVarTrainSubsetRealcov}{33.5}
\newcommand{\miouCIDOFADfcModisREALVarTrainSubsetRealcov}{1.5}
\newcommand{\dropDOFADfcModisREALVarTrainSubsetRealcov}{3.1}
\newcommand{\dropCIDOFADfcModisREALVarTrainSubsetRealcov}{1.8}
\newcommand{\retDOFADfcModisREALVarTrainSubsetRealcov}{0.915}
\newcommand{\retCIDOFADfcModisREALVarTrainSubsetRealcov}{0.049}
\newcommand{\nDOFADfcOmissionLOne}{5}
\newcommand{\miouDOFADfcOmissionLOne}{35.6}
\newcommand{\miouCIDOFADfcOmissionLOne}{1.3}
\newcommand{\dropDOFADfcOmissionLOne}{0.9}
\newcommand{\dropCIDOFADfcOmissionLOne}{1.8}
\newcommand{\retDOFADfcOmissionLOne}{0.976}
\newcommand{\retCIDOFADfcOmissionLOne}{0.049}
\newcommand{\nDOFADfcOmissionLTwo}{5}
\newcommand{\miouDOFADfcOmissionLTwo}{33.3}
\newcommand{\miouCIDOFADfcOmissionLTwo}{1.9}
\newcommand{\dropDOFADfcOmissionLTwo}{3.2}
\newcommand{\dropCIDOFADfcOmissionLTwo}{2.8}
\newcommand{\retDOFADfcOmissionLTwo}{0.914}
\newcommand{\retCIDOFADfcOmissionLTwo}{0.077}
\newcommand{\nDOFADfcShiftLOne}{5}
\newcommand{\miouDOFADfcShiftLOne}{37.0}
\newcommand{\miouCIDOFADfcShiftLOne}{0.3}
\newcommand{\dropDOFADfcShiftLOne}{\ensuremath{-}0.5}
\newcommand{\dropCIDOFADfcShiftLOne}{1.5}
\newcommand{\retDOFADfcShiftLOne}{1.014}
\newcommand{\retCIDOFADfcShiftLOne}{0.042}
\newcommand{\nDOFADfcShiftLTwo}{5}
\newcommand{\miouDOFADfcShiftLTwo}{37.2}
\newcommand{\miouCIDOFADfcShiftLTwo}{1.0}
\newcommand{\dropDOFADfcShiftLTwo}{\ensuremath{-}0.7}
\newcommand{\dropCIDOFADfcShiftLTwo}{1.8}
\newcommand{\retDOFADfcShiftLTwo}{1.020}
\newcommand{\retCIDOFADfcShiftLTwo}{0.054}
\newcommand{\nDOFAEnvaBoundaryLOne}{5}
\newcommand{\miouDOFAEnvaBoundaryLOne}{48.8}
\newcommand{\miouCIDOFAEnvaBoundaryLOne}{6.4}
\newcommand{\dropDOFAEnvaBoundaryLOne}{\ensuremath{-}0.7}
\newcommand{\dropCIDOFAEnvaBoundaryLOne}{4.5}
\newcommand{\retDOFAEnvaBoundaryLOne}{1.012}
\newcommand{\retCIDOFAEnvaBoundaryLOne}{0.093}
\newcommand{\nDOFAEnvaBoundaryLTwo}{5}
\newcommand{\miouDOFAEnvaBoundaryLTwo}{43.4}
\newcommand{\miouCIDOFAEnvaBoundaryLTwo}{4.1}
\newcommand{\dropDOFAEnvaBoundaryLTwo}{4.7}
\newcommand{\dropCIDOFAEnvaBoundaryLTwo}{3.5}
\newcommand{\retDOFAEnvaBoundaryLTwo}{0.902}
\newcommand{\retCIDOFAEnvaBoundaryLTwo}{0.071}
\newcommand{\nDOFAEnvaClean}{5}
\newcommand{\miouDOFAEnvaClean}{48.1}
\newcommand{\miouCIDOFAEnvaClean}{2.2}
\newcommand{\nDOFAEnvaCoarseLOne}{5}
\newcommand{\miouDOFAEnvaCoarseLOne}{49.1}
\newcommand{\miouCIDOFAEnvaCoarseLOne}{3.8}
\newcommand{\dropDOFAEnvaCoarseLOne}{\ensuremath{-}1.0}
\newcommand{\dropCIDOFAEnvaCoarseLOne}{3.3}
\newcommand{\retDOFAEnvaCoarseLOne}{1.022}
\newcommand{\retCIDOFAEnvaCoarseLOne}{0.071}
\newcommand{\nDOFAEnvaCoarseLTwo}{5}
\newcommand{\miouDOFAEnvaCoarseLTwo}{44.6}
\newcommand{\miouCIDOFAEnvaCoarseLTwo}{3.8}
\newcommand{\dropDOFAEnvaCoarseLTwo}{3.5}
\newcommand{\dropCIDOFAEnvaCoarseLTwo}{2.4}
\newcommand{\retDOFAEnvaCoarseLTwo}{0.928}
\newcommand{\retCIDOFAEnvaCoarseLTwo}{0.052}
\newcommand{\nDOFAEnvaNlcdREAL}{5}
\newcommand{\miouDOFAEnvaNlcdREAL}{27.4}
\newcommand{\miouCIDOFAEnvaNlcdREAL}{2.8}
\newcommand{\dropDOFAEnvaNlcdREAL}{20.7}
\newcommand{\dropCIDOFAEnvaNlcdREAL}{4.2}
\newcommand{\retDOFAEnvaNlcdREAL}{0.570}
\newcommand{\retCIDOFAEnvaNlcdREAL}{0.073}
\newcommand{\nDOFAEnvaOmissionLOne}{5}
\newcommand{\miouDOFAEnvaOmissionLOne}{42.4}
\newcommand{\miouCIDOFAEnvaOmissionLOne}{4.5}
\newcommand{\dropDOFAEnvaOmissionLOne}{5.7}
\newcommand{\dropCIDOFAEnvaOmissionLOne}{5.7}
\newcommand{\retDOFAEnvaOmissionLOne}{0.884}
\newcommand{\retCIDOFAEnvaOmissionLOne}{0.115}
\newcommand{\nDOFAEnvaOmissionLTwo}{5}
\newcommand{\miouDOFAEnvaOmissionLTwo}{35.1}
\newcommand{\miouCIDOFAEnvaOmissionLTwo}{12.9}
\newcommand{\dropDOFAEnvaOmissionLTwo}{13.0}
\newcommand{\dropCIDOFAEnvaOmissionLTwo}{14.4}
\newcommand{\retDOFAEnvaOmissionLTwo}{0.735}
\newcommand{\retCIDOFAEnvaOmissionLTwo}{0.301}
\newcommand{\nDOFAEnvaShiftLOne}{5}
\newcommand{\miouDOFAEnvaShiftLOne}{48.0}
\newcommand{\miouCIDOFAEnvaShiftLOne}{3.9}
\newcommand{\dropDOFAEnvaShiftLOne}{0.1}
\newcommand{\dropCIDOFAEnvaShiftLOne}{2.4}
\newcommand{\retDOFAEnvaShiftLOne}{0.997}
\newcommand{\retCIDOFAEnvaShiftLOne}{0.049}
\newcommand{\nDOFAEnvaShiftLTwo}{5}
\newcommand{\miouDOFAEnvaShiftLTwo}{47.5}
\newcommand{\miouCIDOFAEnvaShiftLTwo}{4.1}
\newcommand{\dropDOFAEnvaShiftLTwo}{0.6}
\newcommand{\dropCIDOFAEnvaShiftLTwo}{3.2}
\newcommand{\retDOFAEnvaShiftLTwo}{0.988}
\newcommand{\retCIDOFAEnvaShiftLTwo}{0.065}
\newcommand{\nDOFAflairBoundaryLOne}{5}
\newcommand{\miouDOFAflairBoundaryLOne}{45.7}
\newcommand{\miouCIDOFAflairBoundaryLOne}{0.8}
\newcommand{\dropDOFAflairBoundaryLOne}{1.8}
\newcommand{\dropCIDOFAflairBoundaryLOne}{1.5}
\newcommand{\retDOFAflairBoundaryLOne}{0.963}
\newcommand{\retCIDOFAflairBoundaryLOne}{0.031}
\newcommand{\nDOFAflairBoundaryLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouDOFAflairBoundaryLOneVarDecoderMaskTwoformerFull}{47.0}
\newcommand{\miouCIDOFAflairBoundaryLOneVarDecoderMaskTwoformerFull}{0.9}
\newcommand{\dropDOFAflairBoundaryLOneVarDecoderMaskTwoformerFull}{1.0}
\newcommand{\dropCIDOFAflairBoundaryLOneVarDecoderMaskTwoformerFull}{0.6}
\newcommand{\retDOFAflairBoundaryLOneVarDecoderMaskTwoformerFull}{0.979}
\newcommand{\retCIDOFAflairBoundaryLOneVarDecoderMaskTwoformerFull}{0.013}
\newcommand{\nDOFAflairBoundaryLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouDOFAflairBoundaryLOneVarDecoderMaskTwoformerLite}{46.2}
\newcommand{\miouCIDOFAflairBoundaryLOneVarDecoderMaskTwoformerLite}{1.5}
\newcommand{\dropDOFAflairBoundaryLOneVarDecoderMaskTwoformerLite}{2.0}
\newcommand{\dropCIDOFAflairBoundaryLOneVarDecoderMaskTwoformerLite}{1.6}
\newcommand{\retDOFAflairBoundaryLOneVarDecoderMaskTwoformerLite}{0.958}
\newcommand{\retCIDOFAflairBoundaryLOneVarDecoderMaskTwoformerLite}{0.033}
\newcommand{\nDOFAflairBoundaryLOneVarDecoderSamLite}{5}
\newcommand{\miouDOFAflairBoundaryLOneVarDecoderSamLite}{46.0}
\newcommand{\miouCIDOFAflairBoundaryLOneVarDecoderSamLite}{0.7}
\newcommand{\dropDOFAflairBoundaryLOneVarDecoderSamLite}{1.5}
\newcommand{\dropCIDOFAflairBoundaryLOneVarDecoderSamLite}{0.6}
\newcommand{\retDOFAflairBoundaryLOneVarDecoderSamLite}{0.968}
\newcommand{\retCIDOFAflairBoundaryLOneVarDecoderSamLite}{0.013}
\newcommand{\nDOFAflairBoundaryLOneVarDecoderSamPretrained}{5}
\newcommand{\miouDOFAflairBoundaryLOneVarDecoderSamPretrained}{43.7}
\newcommand{\miouCIDOFAflairBoundaryLOneVarDecoderSamPretrained}{1.1}
\newcommand{\dropDOFAflairBoundaryLOneVarDecoderSamPretrained}{1.4}
\newcommand{\dropCIDOFAflairBoundaryLOneVarDecoderSamPretrained}{1.0}
\newcommand{\retDOFAflairBoundaryLOneVarDecoderSamPretrained}{0.969}
\newcommand{\retCIDOFAflairBoundaryLOneVarDecoderSamPretrained}{0.021}
\newcommand{\nDOFAflairBoundaryLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouDOFAflairBoundaryLOneVarDecoderSegformerMlp}{46.4}
\newcommand{\miouCIDOFAflairBoundaryLOneVarDecoderSegformerMlp}{0.7}
\newcommand{\dropDOFAflairBoundaryLOneVarDecoderSegformerMlp}{1.3}
\newcommand{\dropCIDOFAflairBoundaryLOneVarDecoderSegformerMlp}{1.1}
\newcommand{\retDOFAflairBoundaryLOneVarDecoderSegformerMlp}{0.974}
\newcommand{\retCIDOFAflairBoundaryLOneVarDecoderSegformerMlp}{0.022}
\newcommand{\nDOFAflairBoundaryLTwo}{5}
\newcommand{\miouDOFAflairBoundaryLTwo}{42.7}
\newcommand{\miouCIDOFAflairBoundaryLTwo}{1.7}
\newcommand{\dropDOFAflairBoundaryLTwo}{4.8}
\newcommand{\dropCIDOFAflairBoundaryLTwo}{1.5}
\newcommand{\retDOFAflairBoundaryLTwo}{0.898}
\newcommand{\retCIDOFAflairBoundaryLTwo}{0.031}
\newcommand{\nDOFAflairBoundaryLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouDOFAflairBoundaryLTwoVarDecoderMaskTwoformerFull}{44.7}
\newcommand{\miouCIDOFAflairBoundaryLTwoVarDecoderMaskTwoformerFull}{0.7}
\newcommand{\dropDOFAflairBoundaryLTwoVarDecoderMaskTwoformerFull}{3.3}
\newcommand{\dropCIDOFAflairBoundaryLTwoVarDecoderMaskTwoformerFull}{1.0}
\newcommand{\retDOFAflairBoundaryLTwoVarDecoderMaskTwoformerFull}{0.931}
\newcommand{\retCIDOFAflairBoundaryLTwoVarDecoderMaskTwoformerFull}{0.021}
\newcommand{\nDOFAflairBoundaryLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouDOFAflairBoundaryLTwoVarDecoderMaskTwoformerLite}{42.2}
\newcommand{\miouCIDOFAflairBoundaryLTwoVarDecoderMaskTwoformerLite}{1.1}
\newcommand{\dropDOFAflairBoundaryLTwoVarDecoderMaskTwoformerLite}{6.0}
\newcommand{\dropCIDOFAflairBoundaryLTwoVarDecoderMaskTwoformerLite}{2.0}
\newcommand{\retDOFAflairBoundaryLTwoVarDecoderMaskTwoformerLite}{0.876}
\newcommand{\retCIDOFAflairBoundaryLTwoVarDecoderMaskTwoformerLite}{0.038}
\newcommand{\nDOFAflairBoundaryLTwoVarDecoderSamLite}{5}
\newcommand{\miouDOFAflairBoundaryLTwoVarDecoderSamLite}{42.0}
\newcommand{\miouCIDOFAflairBoundaryLTwoVarDecoderSamLite}{0.7}
\newcommand{\dropDOFAflairBoundaryLTwoVarDecoderSamLite}{5.5}
\newcommand{\dropCIDOFAflairBoundaryLTwoVarDecoderSamLite}{1.0}
\newcommand{\retDOFAflairBoundaryLTwoVarDecoderSamLite}{0.885}
\newcommand{\retCIDOFAflairBoundaryLTwoVarDecoderSamLite}{0.021}
\newcommand{\nDOFAflairBoundaryLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouDOFAflairBoundaryLTwoVarDecoderSamPretrained}{39.2}
\newcommand{\miouCIDOFAflairBoundaryLTwoVarDecoderSamPretrained}{1.2}
\newcommand{\dropDOFAflairBoundaryLTwoVarDecoderSamPretrained}{5.9}
\newcommand{\dropCIDOFAflairBoundaryLTwoVarDecoderSamPretrained}{1.3}
\newcommand{\retDOFAflairBoundaryLTwoVarDecoderSamPretrained}{0.869}
\newcommand{\retCIDOFAflairBoundaryLTwoVarDecoderSamPretrained}{0.029}
\newcommand{\nDOFAflairBoundaryLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouDOFAflairBoundaryLTwoVarDecoderSegformerMlp}{42.4}
\newcommand{\miouCIDOFAflairBoundaryLTwoVarDecoderSegformerMlp}{1.7}
\newcommand{\dropDOFAflairBoundaryLTwoVarDecoderSegformerMlp}{5.2}
\newcommand{\dropCIDOFAflairBoundaryLTwoVarDecoderSegformerMlp}{2.4}
\newcommand{\retDOFAflairBoundaryLTwoVarDecoderSegformerMlp}{0.890}
\newcommand{\retCIDOFAflairBoundaryLTwoVarDecoderSegformerMlp}{0.047}
\newcommand{\nDOFAflairBoundaryLTwoVarLossBootstrap}{5}
\newcommand{\miouDOFAflairBoundaryLTwoVarLossBootstrap}{42.1}
\newcommand{\miouCIDOFAflairBoundaryLTwoVarLossBootstrap}{0.8}
\newcommand{\dropDOFAflairBoundaryLTwoVarLossBootstrap}{5.1}
\newcommand{\dropCIDOFAflairBoundaryLTwoVarLossBootstrap}{1.5}
\newcommand{\retDOFAflairBoundaryLTwoVarLossBootstrap}{0.893}
\newcommand{\retCIDOFAflairBoundaryLTwoVarLossBootstrap}{0.029}
\newcommand{\nDOFAflairBoundaryLTwoVarLossGce}{5}
\newcommand{\miouDOFAflairBoundaryLTwoVarLossGce}{38.2}
\newcommand{\miouCIDOFAflairBoundaryLTwoVarLossGce}{2.3}
\newcommand{\dropDOFAflairBoundaryLTwoVarLossGce}{5.6}
\newcommand{\dropCIDOFAflairBoundaryLTwoVarLossGce}{3.4}
\newcommand{\retDOFAflairBoundaryLTwoVarLossGce}{0.873}
\newcommand{\retCIDOFAflairBoundaryLTwoVarLossGce}{0.070}
\newcommand{\nDOFAflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouDOFAflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{42.0}
\newcommand{\miouCIDOFAflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{1.4}
\newcommand{\dropDOFAflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{4.7}
\newcommand{\dropCIDOFAflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{1.7}
\newcommand{\retDOFAflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{0.899}
\newcommand{\retCIDOFAflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{0.036}
\newcommand{\nDOFAflairBoundaryLR}{5}
\newcommand{\miouDOFAflairBoundaryLR}{41.2}
\newcommand{\miouCIDOFAflairBoundaryLR}{1.1}
\newcommand{\dropDOFAflairBoundaryLR}{6.3}
\newcommand{\dropCIDOFAflairBoundaryLR}{0.8}
\newcommand{\retDOFAflairBoundaryLR}{0.868}
\newcommand{\retCIDOFAflairBoundaryLR}{0.017}
\newcommand{\nDOFAflairClean}{5}
\newcommand{\miouDOFAflairClean}{47.5}
\newcommand{\miouCIDOFAflairClean}{1.0}
\newcommand{\nDOFAflairCleanVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouDOFAflairCleanVarDecoderMaskTwoformerFull}{48.0}
\newcommand{\miouCIDOFAflairCleanVarDecoderMaskTwoformerFull}{0.5}
\newcommand{\nDOFAflairCleanVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouDOFAflairCleanVarDecoderMaskTwoformerLite}{48.2}
\newcommand{\miouCIDOFAflairCleanVarDecoderMaskTwoformerLite}{1.3}
\newcommand{\nDOFAflairCleanVarDecoderSamLite}{5}
\newcommand{\miouDOFAflairCleanVarDecoderSamLite}{47.5}
\newcommand{\miouCIDOFAflairCleanVarDecoderSamLite}{0.5}
\newcommand{\nDOFAflairCleanVarDecoderSamPretrained}{5}
\newcommand{\miouDOFAflairCleanVarDecoderSamPretrained}{45.1}
\newcommand{\miouCIDOFAflairCleanVarDecoderSamPretrained}{1.2}
\newcommand{\nDOFAflairCleanVarDecoderSegformerMlp}{5}
\newcommand{\miouDOFAflairCleanVarDecoderSegformerMlp}{47.6}
\newcommand{\miouCIDOFAflairCleanVarDecoderSegformerMlp}{1.0}
\newcommand{\nDOFAflairCleanVarFrozenEncoderTrue}{5}
\newcommand{\miouDOFAflairCleanVarFrozenEncoderTrue}{44.4}
\newcommand{\miouCIDOFAflairCleanVarFrozenEncoderTrue}{0.7}
\newcommand{\nDOFAflairCleanVarLossBootstrap}{5}
\newcommand{\miouDOFAflairCleanVarLossBootstrap}{47.2}
\newcommand{\miouCIDOFAflairCleanVarLossBootstrap}{0.9}
\newcommand{\nDOFAflairCleanVarLossGce}{5}
\newcommand{\miouDOFAflairCleanVarLossGce}{43.8}
\newcommand{\miouCIDOFAflairCleanVarLossGce}{2.3}
\newcommand{\nDOFAflairCleanVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouDOFAflairCleanVarLrMultZeroThreeThreeThreeThree}{46.7}
\newcommand{\miouCIDOFAflairCleanVarLrMultZeroThreeThreeThreeThree}{0.7}
\newcommand{\nDOFAflairCleanVarTrainSubsetCleanTwoFive}{5}
\newcommand{\miouDOFAflairCleanVarTrainSubsetCleanTwoFive}{43.1}
\newcommand{\miouCIDOFAflairCleanVarTrainSubsetCleanTwoFive}{1.6}
\newcommand{\nDOFAflairCoarseLOne}{5}
\newcommand{\miouDOFAflairCoarseLOne}{47.0}
\newcommand{\miouCIDOFAflairCoarseLOne}{1.3}
\newcommand{\dropDOFAflairCoarseLOne}{0.6}
\newcommand{\dropCIDOFAflairCoarseLOne}{1.7}
\newcommand{\retDOFAflairCoarseLOne}{0.988}
\newcommand{\retCIDOFAflairCoarseLOne}{0.036}
\newcommand{\nDOFAflairCoarseLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouDOFAflairCoarseLOneVarDecoderMaskTwoformerFull}{47.3}
\newcommand{\miouCIDOFAflairCoarseLOneVarDecoderMaskTwoformerFull}{0.6}
\newcommand{\dropDOFAflairCoarseLOneVarDecoderMaskTwoformerFull}{0.8}
\newcommand{\dropCIDOFAflairCoarseLOneVarDecoderMaskTwoformerFull}{0.6}
\newcommand{\retDOFAflairCoarseLOneVarDecoderMaskTwoformerFull}{0.984}
\newcommand{\retCIDOFAflairCoarseLOneVarDecoderMaskTwoformerFull}{0.012}
\newcommand{\nDOFAflairCoarseLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouDOFAflairCoarseLOneVarDecoderMaskTwoformerLite}{47.1}
\newcommand{\miouCIDOFAflairCoarseLOneVarDecoderMaskTwoformerLite}{1.5}
\newcommand{\dropDOFAflairCoarseLOneVarDecoderMaskTwoformerLite}{1.1}
\newcommand{\dropCIDOFAflairCoarseLOneVarDecoderMaskTwoformerLite}{1.3}
\newcommand{\retDOFAflairCoarseLOneVarDecoderMaskTwoformerLite}{0.977}
\newcommand{\retCIDOFAflairCoarseLOneVarDecoderMaskTwoformerLite}{0.027}
\newcommand{\nDOFAflairCoarseLOneVarDecoderSamLite}{5}
\newcommand{\miouDOFAflairCoarseLOneVarDecoderSamLite}{45.6}
\newcommand{\miouCIDOFAflairCoarseLOneVarDecoderSamLite}{1.0}
\newcommand{\dropDOFAflairCoarseLOneVarDecoderSamLite}{1.8}
\newcommand{\dropCIDOFAflairCoarseLOneVarDecoderSamLite}{0.6}
\newcommand{\retDOFAflairCoarseLOneVarDecoderSamLite}{0.961}
\newcommand{\retCIDOFAflairCoarseLOneVarDecoderSamLite}{0.013}
\newcommand{\nDOFAflairCoarseLOneVarDecoderSamPretrained}{5}
\newcommand{\miouDOFAflairCoarseLOneVarDecoderSamPretrained}{43.8}
\newcommand{\miouCIDOFAflairCoarseLOneVarDecoderSamPretrained}{1.4}
\newcommand{\dropDOFAflairCoarseLOneVarDecoderSamPretrained}{1.2}
\newcommand{\dropCIDOFAflairCoarseLOneVarDecoderSamPretrained}{1.3}
\newcommand{\retDOFAflairCoarseLOneVarDecoderSamPretrained}{0.973}
\newcommand{\retCIDOFAflairCoarseLOneVarDecoderSamPretrained}{0.029}
\newcommand{\nDOFAflairCoarseLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouDOFAflairCoarseLOneVarDecoderSegformerMlp}{47.2}
\newcommand{\miouCIDOFAflairCoarseLOneVarDecoderSegformerMlp}{0.6}
\newcommand{\dropDOFAflairCoarseLOneVarDecoderSegformerMlp}{0.4}
\newcommand{\dropCIDOFAflairCoarseLOneVarDecoderSegformerMlp}{1.4}
\newcommand{\retDOFAflairCoarseLOneVarDecoderSegformerMlp}{0.991}
\newcommand{\retCIDOFAflairCoarseLOneVarDecoderSegformerMlp}{0.028}
\newcommand{\nDOFAflairCoarseLTwo}{5}
\newcommand{\miouDOFAflairCoarseLTwo}{42.2}
\newcommand{\miouCIDOFAflairCoarseLTwo}{1.5}
\newcommand{\dropDOFAflairCoarseLTwo}{5.3}
\newcommand{\dropCIDOFAflairCoarseLTwo}{1.3}
\newcommand{\retDOFAflairCoarseLTwo}{0.889}
\newcommand{\retCIDOFAflairCoarseLTwo}{0.027}
\newcommand{\nDOFAflairCoarseLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouDOFAflairCoarseLTwoVarDecoderMaskTwoformerFull}{41.2}
\newcommand{\miouCIDOFAflairCoarseLTwoVarDecoderMaskTwoformerFull}{0.5}
\newcommand{\dropDOFAflairCoarseLTwoVarDecoderMaskTwoformerFull}{6.8}
\newcommand{\dropCIDOFAflairCoarseLTwoVarDecoderMaskTwoformerFull}{0.8}
\newcommand{\retDOFAflairCoarseLTwoVarDecoderMaskTwoformerFull}{0.858}
\newcommand{\retCIDOFAflairCoarseLTwoVarDecoderMaskTwoformerFull}{0.016}
\newcommand{\nDOFAflairCoarseLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouDOFAflairCoarseLTwoVarDecoderMaskTwoformerLite}{41.5}
\newcommand{\miouCIDOFAflairCoarseLTwoVarDecoderMaskTwoformerLite}{1.2}
\newcommand{\dropDOFAflairCoarseLTwoVarDecoderMaskTwoformerLite}{6.7}
\newcommand{\dropCIDOFAflairCoarseLTwoVarDecoderMaskTwoformerLite}{1.7}
\newcommand{\retDOFAflairCoarseLTwoVarDecoderMaskTwoformerLite}{0.860}
\newcommand{\retCIDOFAflairCoarseLTwoVarDecoderMaskTwoformerLite}{0.032}
\newcommand{\nDOFAflairCoarseLTwoVarDecoderSamLite}{5}
\newcommand{\miouDOFAflairCoarseLTwoVarDecoderSamLite}{41.7}
\newcommand{\miouCIDOFAflairCoarseLTwoVarDecoderSamLite}{1.1}
\newcommand{\dropDOFAflairCoarseLTwoVarDecoderSamLite}{5.7}
\newcommand{\dropCIDOFAflairCoarseLTwoVarDecoderSamLite}{1.5}
\newcommand{\retDOFAflairCoarseLTwoVarDecoderSamLite}{0.879}
\newcommand{\retCIDOFAflairCoarseLTwoVarDecoderSamLite}{0.030}
\newcommand{\nDOFAflairCoarseLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouDOFAflairCoarseLTwoVarDecoderSamPretrained}{38.7}
\newcommand{\miouCIDOFAflairCoarseLTwoVarDecoderSamPretrained}{1.0}
\newcommand{\dropDOFAflairCoarseLTwoVarDecoderSamPretrained}{6.4}
\newcommand{\dropCIDOFAflairCoarseLTwoVarDecoderSamPretrained}{1.3}
\newcommand{\retDOFAflairCoarseLTwoVarDecoderSamPretrained}{0.858}
\newcommand{\retCIDOFAflairCoarseLTwoVarDecoderSamPretrained}{0.026}
\newcommand{\nDOFAflairCoarseLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouDOFAflairCoarseLTwoVarDecoderSegformerMlp}{41.3}
\newcommand{\miouCIDOFAflairCoarseLTwoVarDecoderSegformerMlp}{1.3}
\newcommand{\dropDOFAflairCoarseLTwoVarDecoderSegformerMlp}{6.3}
\newcommand{\dropCIDOFAflairCoarseLTwoVarDecoderSegformerMlp}{1.2}
\newcommand{\retDOFAflairCoarseLTwoVarDecoderSegformerMlp}{0.868}
\newcommand{\retCIDOFAflairCoarseLTwoVarDecoderSegformerMlp}{0.025}
\newcommand{\nDOFAflairCoarseLTwoVarLossBootstrap}{5}
\newcommand{\miouDOFAflairCoarseLTwoVarLossBootstrap}{41.7}
\newcommand{\miouCIDOFAflairCoarseLTwoVarLossBootstrap}{1.5}
\newcommand{\dropDOFAflairCoarseLTwoVarLossBootstrap}{5.5}
\newcommand{\dropCIDOFAflairCoarseLTwoVarLossBootstrap}{1.9}
\newcommand{\retDOFAflairCoarseLTwoVarLossBootstrap}{0.884}
\newcommand{\retCIDOFAflairCoarseLTwoVarLossBootstrap}{0.040}
\newcommand{\nDOFAflairCoarseLTwoVarLossGce}{5}
\newcommand{\miouDOFAflairCoarseLTwoVarLossGce}{36.7}
\newcommand{\miouCIDOFAflairCoarseLTwoVarLossGce}{3.4}
\newcommand{\dropDOFAflairCoarseLTwoVarLossGce}{7.1}
\newcommand{\dropCIDOFAflairCoarseLTwoVarLossGce}{4.7}
\newcommand{\retDOFAflairCoarseLTwoVarLossGce}{0.839}
\newcommand{\retCIDOFAflairCoarseLTwoVarLossGce}{0.098}
\newcommand{\nDOFAflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouDOFAflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{42.2}
\newcommand{\miouCIDOFAflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{1.3}
\newcommand{\dropDOFAflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{4.6}
\newcommand{\dropCIDOFAflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.8}
\newcommand{\retDOFAflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.902}
\newcommand{\retCIDOFAflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.017}
\newcommand{\nDOFAflairCoarseLR}{5}
\newcommand{\miouDOFAflairCoarseLR}{37.0}
\newcommand{\miouCIDOFAflairCoarseLR}{1.1}
\newcommand{\dropDOFAflairCoarseLR}{10.5}
\newcommand{\dropCIDOFAflairCoarseLR}{0.9}
\newcommand{\retDOFAflairCoarseLR}{0.778}
\newcommand{\retCIDOFAflairCoarseLR}{0.019}
\newcommand{\nDOFAflairOmissionLOne}{5}
\newcommand{\miouDOFAflairOmissionLOne}{46.1}
\newcommand{\miouCIDOFAflairOmissionLOne}{1.1}
\newcommand{\dropDOFAflairOmissionLOne}{1.4}
\newcommand{\dropCIDOFAflairOmissionLOne}{1.4}
\newcommand{\retDOFAflairOmissionLOne}{0.970}
\newcommand{\retCIDOFAflairOmissionLOne}{0.028}
\newcommand{\nDOFAflairOmissionLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouDOFAflairOmissionLOneVarDecoderMaskTwoformerFull}{47.7}
\newcommand{\miouCIDOFAflairOmissionLOneVarDecoderMaskTwoformerFull}{1.4}
\newcommand{\dropDOFAflairOmissionLOneVarDecoderMaskTwoformerFull}{0.3}
\newcommand{\dropCIDOFAflairOmissionLOneVarDecoderMaskTwoformerFull}{1.6}
\newcommand{\retDOFAflairOmissionLOneVarDecoderMaskTwoformerFull}{0.993}
\newcommand{\retCIDOFAflairOmissionLOneVarDecoderMaskTwoformerFull}{0.033}
\newcommand{\nDOFAflairOmissionLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouDOFAflairOmissionLOneVarDecoderMaskTwoformerLite}{46.1}
\newcommand{\miouCIDOFAflairOmissionLOneVarDecoderMaskTwoformerLite}{1.5}
\newcommand{\dropDOFAflairOmissionLOneVarDecoderMaskTwoformerLite}{2.1}
\newcommand{\dropCIDOFAflairOmissionLOneVarDecoderMaskTwoformerLite}{1.4}
\newcommand{\retDOFAflairOmissionLOneVarDecoderMaskTwoformerLite}{0.957}
\newcommand{\retCIDOFAflairOmissionLOneVarDecoderMaskTwoformerLite}{0.029}
\newcommand{\nDOFAflairOmissionLOneVarDecoderSamLite}{5}
\newcommand{\miouDOFAflairOmissionLOneVarDecoderSamLite}{45.4}
\newcommand{\miouCIDOFAflairOmissionLOneVarDecoderSamLite}{1.0}
\newcommand{\dropDOFAflairOmissionLOneVarDecoderSamLite}{2.0}
\newcommand{\dropCIDOFAflairOmissionLOneVarDecoderSamLite}{1.0}
\newcommand{\retDOFAflairOmissionLOneVarDecoderSamLite}{0.957}
\newcommand{\retCIDOFAflairOmissionLOneVarDecoderSamLite}{0.021}
\newcommand{\nDOFAflairOmissionLOneVarDecoderSamPretrained}{5}
\newcommand{\miouDOFAflairOmissionLOneVarDecoderSamPretrained}{42.9}
\newcommand{\miouCIDOFAflairOmissionLOneVarDecoderSamPretrained}{1.2}
\newcommand{\dropDOFAflairOmissionLOneVarDecoderSamPretrained}{2.2}
\newcommand{\dropCIDOFAflairOmissionLOneVarDecoderSamPretrained}{1.5}
\newcommand{\retDOFAflairOmissionLOneVarDecoderSamPretrained}{0.951}
\newcommand{\retCIDOFAflairOmissionLOneVarDecoderSamPretrained}{0.033}
\newcommand{\nDOFAflairOmissionLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouDOFAflairOmissionLOneVarDecoderSegformerMlp}{46.2}
\newcommand{\miouCIDOFAflairOmissionLOneVarDecoderSegformerMlp}{1.2}
\newcommand{\dropDOFAflairOmissionLOneVarDecoderSegformerMlp}{1.4}
\newcommand{\dropCIDOFAflairOmissionLOneVarDecoderSegformerMlp}{1.9}
\newcommand{\retDOFAflairOmissionLOneVarDecoderSegformerMlp}{0.970}
\newcommand{\retCIDOFAflairOmissionLOneVarDecoderSegformerMlp}{0.040}
\newcommand{\nDOFAflairOmissionLTwo}{5}
\newcommand{\miouDOFAflairOmissionLTwo}{43.3}
\newcommand{\miouCIDOFAflairOmissionLTwo}{1.4}
\newcommand{\dropDOFAflairOmissionLTwo}{4.2}
\newcommand{\dropCIDOFAflairOmissionLTwo}{1.3}
\newcommand{\retDOFAflairOmissionLTwo}{0.912}
\newcommand{\retCIDOFAflairOmissionLTwo}{0.027}
\newcommand{\nDOFAflairOmissionLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouDOFAflairOmissionLTwoVarDecoderMaskTwoformerFull}{44.8}
\newcommand{\miouCIDOFAflairOmissionLTwoVarDecoderMaskTwoformerFull}{2.3}
\newcommand{\dropDOFAflairOmissionLTwoVarDecoderMaskTwoformerFull}{3.3}
\newcommand{\dropCIDOFAflairOmissionLTwoVarDecoderMaskTwoformerFull}{2.1}
\newcommand{\retDOFAflairOmissionLTwoVarDecoderMaskTwoformerFull}{0.932}
\newcommand{\retCIDOFAflairOmissionLTwoVarDecoderMaskTwoformerFull}{0.044}
\newcommand{\nDOFAflairOmissionLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouDOFAflairOmissionLTwoVarDecoderMaskTwoformerLite}{42.5}
\newcommand{\miouCIDOFAflairOmissionLTwoVarDecoderMaskTwoformerLite}{2.6}
\newcommand{\dropDOFAflairOmissionLTwoVarDecoderMaskTwoformerLite}{5.7}
\newcommand{\dropCIDOFAflairOmissionLTwoVarDecoderMaskTwoformerLite}{3.0}
\newcommand{\retDOFAflairOmissionLTwoVarDecoderMaskTwoformerLite}{0.883}
\newcommand{\retCIDOFAflairOmissionLTwoVarDecoderMaskTwoformerLite}{0.061}
\newcommand{\nDOFAflairOmissionLTwoVarDecoderSamLite}{5}
\newcommand{\miouDOFAflairOmissionLTwoVarDecoderSamLite}{42.7}
\newcommand{\miouCIDOFAflairOmissionLTwoVarDecoderSamLite}{1.8}
\newcommand{\dropDOFAflairOmissionLTwoVarDecoderSamLite}{4.8}
\newcommand{\dropCIDOFAflairOmissionLTwoVarDecoderSamLite}{1.9}
\newcommand{\retDOFAflairOmissionLTwoVarDecoderSamLite}{0.899}
\newcommand{\retCIDOFAflairOmissionLTwoVarDecoderSamLite}{0.040}
\newcommand{\nDOFAflairOmissionLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouDOFAflairOmissionLTwoVarDecoderSamPretrained}{39.8}
\newcommand{\miouCIDOFAflairOmissionLTwoVarDecoderSamPretrained}{1.6}
\newcommand{\dropDOFAflairOmissionLTwoVarDecoderSamPretrained}{5.3}
\newcommand{\dropCIDOFAflairOmissionLTwoVarDecoderSamPretrained}{2.1}
\newcommand{\retDOFAflairOmissionLTwoVarDecoderSamPretrained}{0.883}
\newcommand{\retCIDOFAflairOmissionLTwoVarDecoderSamPretrained}{0.045}
\newcommand{\nDOFAflairOmissionLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouDOFAflairOmissionLTwoVarDecoderSegformerMlp}{44.2}
\newcommand{\miouCIDOFAflairOmissionLTwoVarDecoderSegformerMlp}{1.2}
\newcommand{\dropDOFAflairOmissionLTwoVarDecoderSegformerMlp}{3.5}
\newcommand{\dropCIDOFAflairOmissionLTwoVarDecoderSegformerMlp}{1.5}
\newcommand{\retDOFAflairOmissionLTwoVarDecoderSegformerMlp}{0.927}
\newcommand{\retCIDOFAflairOmissionLTwoVarDecoderSegformerMlp}{0.032}
\newcommand{\nDOFAflairOmissionLTwoVarFrozenEncoderTrue}{5}
\newcommand{\miouDOFAflairOmissionLTwoVarFrozenEncoderTrue}{41.7}
\newcommand{\miouCIDOFAflairOmissionLTwoVarFrozenEncoderTrue}{1.0}
\newcommand{\dropDOFAflairOmissionLTwoVarFrozenEncoderTrue}{2.7}
\newcommand{\dropCIDOFAflairOmissionLTwoVarFrozenEncoderTrue}{1.0}
\newcommand{\retDOFAflairOmissionLTwoVarFrozenEncoderTrue}{0.939}
\newcommand{\retCIDOFAflairOmissionLTwoVarFrozenEncoderTrue}{0.021}
\newcommand{\nDOFAflairOmissionLTwoVarLossBootstrap}{5}
\newcommand{\miouDOFAflairOmissionLTwoVarLossBootstrap}{42.9}
\newcommand{\miouCIDOFAflairOmissionLTwoVarLossBootstrap}{1.0}
\newcommand{\dropDOFAflairOmissionLTwoVarLossBootstrap}{4.3}
\newcommand{\dropCIDOFAflairOmissionLTwoVarLossBootstrap}{0.7}
\newcommand{\retDOFAflairOmissionLTwoVarLossBootstrap}{0.908}
\newcommand{\retCIDOFAflairOmissionLTwoVarLossBootstrap}{0.015}
\newcommand{\nDOFAflairOmissionLTwoVarLossGce}{5}
\newcommand{\miouDOFAflairOmissionLTwoVarLossGce}{36.7}
\newcommand{\miouCIDOFAflairOmissionLTwoVarLossGce}{5.4}
\newcommand{\dropDOFAflairOmissionLTwoVarLossGce}{7.1}
\newcommand{\dropCIDOFAflairOmissionLTwoVarLossGce}{5.2}
\newcommand{\retDOFAflairOmissionLTwoVarLossGce}{0.839}
\newcommand{\retCIDOFAflairOmissionLTwoVarLossGce}{0.118}
\newcommand{\nDOFAflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouDOFAflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{43.2}
\newcommand{\miouCIDOFAflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{2.4}
\newcommand{\dropDOFAflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{3.6}
\newcommand{\dropCIDOFAflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{3.0}
\newcommand{\retDOFAflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{0.924}
\newcommand{\retCIDOFAflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{0.062}
\newcommand{\nDOFAflairOmissionLR}{5}
\newcommand{\miouDOFAflairOmissionLR}{39.8}
\newcommand{\miouCIDOFAflairOmissionLR}{1.6}
\newcommand{\dropDOFAflairOmissionLR}{7.7}
\newcommand{\dropCIDOFAflairOmissionLR}{2.3}
\newcommand{\retDOFAflairOmissionLR}{0.838}
\newcommand{\retCIDOFAflairOmissionLR}{0.046}
\newcommand{\nDOFAflairShiftLOne}{5}
\newcommand{\miouDOFAflairShiftLOne}{47.2}
\newcommand{\miouCIDOFAflairShiftLOne}{1.2}
\newcommand{\dropDOFAflairShiftLOne}{0.3}
\newcommand{\dropCIDOFAflairShiftLOne}{1.6}
\newcommand{\retDOFAflairShiftLOne}{0.994}
\newcommand{\retCIDOFAflairShiftLOne}{0.034}
\newcommand{\nDOFAflairShiftLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouDOFAflairShiftLOneVarDecoderMaskTwoformerFull}{48.0}
\newcommand{\miouCIDOFAflairShiftLOneVarDecoderMaskTwoformerFull}{0.7}
\newcommand{\dropDOFAflairShiftLOneVarDecoderMaskTwoformerFull}{0.0}
\newcommand{\dropCIDOFAflairShiftLOneVarDecoderMaskTwoformerFull}{0.9}
\newcommand{\retDOFAflairShiftLOneVarDecoderMaskTwoformerFull}{1.000}
\newcommand{\retCIDOFAflairShiftLOneVarDecoderMaskTwoformerFull}{0.020}
\newcommand{\nDOFAflairShiftLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouDOFAflairShiftLOneVarDecoderMaskTwoformerLite}{47.1}
\newcommand{\miouCIDOFAflairShiftLOneVarDecoderMaskTwoformerLite}{0.6}
\newcommand{\dropDOFAflairShiftLOneVarDecoderMaskTwoformerLite}{1.1}
\newcommand{\dropCIDOFAflairShiftLOneVarDecoderMaskTwoformerLite}{1.0}
\newcommand{\retDOFAflairShiftLOneVarDecoderMaskTwoformerLite}{0.978}
\newcommand{\retCIDOFAflairShiftLOneVarDecoderMaskTwoformerLite}{0.019}
\newcommand{\nDOFAflairShiftLOneVarDecoderSamLite}{5}
\newcommand{\miouDOFAflairShiftLOneVarDecoderSamLite}{46.9}
\newcommand{\miouCIDOFAflairShiftLOneVarDecoderSamLite}{1.0}
\newcommand{\dropDOFAflairShiftLOneVarDecoderSamLite}{0.5}
\newcommand{\dropCIDOFAflairShiftLOneVarDecoderSamLite}{0.8}
\newcommand{\retDOFAflairShiftLOneVarDecoderSamLite}{0.989}
\newcommand{\retCIDOFAflairShiftLOneVarDecoderSamLite}{0.017}
\newcommand{\nDOFAflairShiftLOneVarDecoderSamPretrained}{5}
\newcommand{\miouDOFAflairShiftLOneVarDecoderSamPretrained}{44.4}
\newcommand{\miouCIDOFAflairShiftLOneVarDecoderSamPretrained}{1.3}
\newcommand{\dropDOFAflairShiftLOneVarDecoderSamPretrained}{0.6}
\newcommand{\dropCIDOFAflairShiftLOneVarDecoderSamPretrained}{2.2}
\newcommand{\retDOFAflairShiftLOneVarDecoderSamPretrained}{0.986}
\newcommand{\retCIDOFAflairShiftLOneVarDecoderSamPretrained}{0.049}
\newcommand{\nDOFAflairShiftLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouDOFAflairShiftLOneVarDecoderSegformerMlp}{47.8}
\newcommand{\miouCIDOFAflairShiftLOneVarDecoderSegformerMlp}{1.0}
\newcommand{\dropDOFAflairShiftLOneVarDecoderSegformerMlp}{\ensuremath{-}0.2}
\newcommand{\dropCIDOFAflairShiftLOneVarDecoderSegformerMlp}{1.7}
\newcommand{\retDOFAflairShiftLOneVarDecoderSegformerMlp}{1.004}
\newcommand{\retCIDOFAflairShiftLOneVarDecoderSegformerMlp}{0.035}
\newcommand{\nDOFAflairShiftLTwo}{5}
\newcommand{\miouDOFAflairShiftLTwo}{44.6}
\newcommand{\miouCIDOFAflairShiftLTwo}{0.8}
\newcommand{\dropDOFAflairShiftLTwo}{2.9}
\newcommand{\dropCIDOFAflairShiftLTwo}{1.0}
\newcommand{\retDOFAflairShiftLTwo}{0.939}
\newcommand{\retCIDOFAflairShiftLTwo}{0.020}
\newcommand{\nDOFAflairShiftLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouDOFAflairShiftLTwoVarDecoderMaskTwoformerFull}{43.7}
\newcommand{\miouCIDOFAflairShiftLTwoVarDecoderMaskTwoformerFull}{1.2}
\newcommand{\dropDOFAflairShiftLTwoVarDecoderMaskTwoformerFull}{4.3}
\newcommand{\dropCIDOFAflairShiftLTwoVarDecoderMaskTwoformerFull}{1.2}
\newcommand{\retDOFAflairShiftLTwoVarDecoderMaskTwoformerFull}{0.910}
\newcommand{\retCIDOFAflairShiftLTwoVarDecoderMaskTwoformerFull}{0.025}
\newcommand{\nDOFAflairShiftLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouDOFAflairShiftLTwoVarDecoderMaskTwoformerLite}{43.7}
\newcommand{\miouCIDOFAflairShiftLTwoVarDecoderMaskTwoformerLite}{1.6}
\newcommand{\dropDOFAflairShiftLTwoVarDecoderMaskTwoformerLite}{4.5}
\newcommand{\dropCIDOFAflairShiftLTwoVarDecoderMaskTwoformerLite}{2.3}
\newcommand{\retDOFAflairShiftLTwoVarDecoderMaskTwoformerLite}{0.907}
\newcommand{\retCIDOFAflairShiftLTwoVarDecoderMaskTwoformerLite}{0.046}
\newcommand{\nDOFAflairShiftLTwoVarDecoderSamLite}{5}
\newcommand{\miouDOFAflairShiftLTwoVarDecoderSamLite}{43.0}
\newcommand{\miouCIDOFAflairShiftLTwoVarDecoderSamLite}{1.1}
\newcommand{\dropDOFAflairShiftLTwoVarDecoderSamLite}{4.4}
\newcommand{\dropCIDOFAflairShiftLTwoVarDecoderSamLite}{0.9}
\newcommand{\retDOFAflairShiftLTwoVarDecoderSamLite}{0.907}
\newcommand{\retCIDOFAflairShiftLTwoVarDecoderSamLite}{0.019}
\newcommand{\nDOFAflairShiftLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouDOFAflairShiftLTwoVarDecoderSamPretrained}{41.1}
\newcommand{\miouCIDOFAflairShiftLTwoVarDecoderSamPretrained}{0.8}
\newcommand{\dropDOFAflairShiftLTwoVarDecoderSamPretrained}{3.9}
\newcommand{\dropCIDOFAflairShiftLTwoVarDecoderSamPretrained}{1.8}
\newcommand{\retDOFAflairShiftLTwoVarDecoderSamPretrained}{0.913}
\newcommand{\retCIDOFAflairShiftLTwoVarDecoderSamPretrained}{0.037}
\newcommand{\nDOFAflairShiftLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouDOFAflairShiftLTwoVarDecoderSegformerMlp}{44.3}
\newcommand{\miouCIDOFAflairShiftLTwoVarDecoderSegformerMlp}{0.8}
\newcommand{\dropDOFAflairShiftLTwoVarDecoderSegformerMlp}{3.3}
\newcommand{\dropCIDOFAflairShiftLTwoVarDecoderSegformerMlp}{1.5}
\newcommand{\retDOFAflairShiftLTwoVarDecoderSegformerMlp}{0.931}
\newcommand{\retCIDOFAflairShiftLTwoVarDecoderSegformerMlp}{0.030}
\newcommand{\nDOFAflairShiftLTwoVarLossBootstrap}{5}
\newcommand{\miouDOFAflairShiftLTwoVarLossBootstrap}{43.9}
\newcommand{\miouCIDOFAflairShiftLTwoVarLossBootstrap}{1.0}
\newcommand{\dropDOFAflairShiftLTwoVarLossBootstrap}{3.3}
\newcommand{\dropCIDOFAflairShiftLTwoVarLossBootstrap}{1.4}
\newcommand{\retDOFAflairShiftLTwoVarLossBootstrap}{0.931}
\newcommand{\retCIDOFAflairShiftLTwoVarLossBootstrap}{0.028}
\newcommand{\nDOFAflairShiftLTwoVarLossGce}{5}
\newcommand{\miouDOFAflairShiftLTwoVarLossGce}{40.5}
\newcommand{\miouCIDOFAflairShiftLTwoVarLossGce}{2.6}
\newcommand{\dropDOFAflairShiftLTwoVarLossGce}{3.4}
\newcommand{\dropCIDOFAflairShiftLTwoVarLossGce}{2.2}
\newcommand{\retDOFAflairShiftLTwoVarLossGce}{0.924}
\newcommand{\retCIDOFAflairShiftLTwoVarLossGce}{0.050}
\newcommand{\nDOFAflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouDOFAflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{44.1}
\newcommand{\miouCIDOFAflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.9}
\newcommand{\dropDOFAflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{2.6}
\newcommand{\dropCIDOFAflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.9}
\newcommand{\retDOFAflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.944}
\newcommand{\retCIDOFAflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.019}
\newcommand{\nDOFAflairShiftLR}{5}
\newcommand{\miouDOFAflairShiftLR}{40.4}
\newcommand{\miouCIDOFAflairShiftLR}{1.3}
\newcommand{\dropDOFAflairShiftLR}{7.1}
\newcommand{\dropCIDOFAflairShiftLR}{1.5}
\newcommand{\retDOFAflairShiftLR}{0.850}
\newcommand{\retCIDOFAflairShiftLR}{0.031}
\newcommand{\nDOFAKuroBoundaryLOne}{5}
\newcommand{\miouDOFAKuroBoundaryLOne}{53.6}
\newcommand{\miouCIDOFAKuroBoundaryLOne}{4.0}
\newcommand{\dropDOFAKuroBoundaryLOne}{\ensuremath{-}0.1}
\newcommand{\dropCIDOFAKuroBoundaryLOne}{3.0}
\newcommand{\retDOFAKuroBoundaryLOne}{1.001}
\newcommand{\retCIDOFAKuroBoundaryLOne}{0.057}
\newcommand{\nDOFAKuroBoundaryLTwo}{5}
\newcommand{\miouDOFAKuroBoundaryLTwo}{50.1}
\newcommand{\miouCIDOFAKuroBoundaryLTwo}{3.5}
\newcommand{\dropDOFAKuroBoundaryLTwo}{3.5}
\newcommand{\dropCIDOFAKuroBoundaryLTwo}{3.6}
\newcommand{\retDOFAKuroBoundaryLTwo}{0.936}
\newcommand{\retCIDOFAKuroBoundaryLTwo}{0.064}
\newcommand{\nDOFAKuroCemsREALVarTrainSubsetRealcov}{5}
\newcommand{\miouDOFAKuroCemsREALVarTrainSubsetRealcov}{49.5}
\newcommand{\miouCIDOFAKuroCemsREALVarTrainSubsetRealcov}{2.0}
\newcommand{\dropDOFAKuroCemsREALVarTrainSubsetRealcov}{0.5}
\newcommand{\dropCIDOFAKuroCemsREALVarTrainSubsetRealcov}{3.5}
\newcommand{\retDOFAKuroCemsREALVarTrainSubsetRealcov}{0.991}
\newcommand{\retCIDOFAKuroCemsREALVarTrainSubsetRealcov}{0.068}
\newcommand{\nDOFAKuroClean}{5}
\newcommand{\miouDOFAKuroClean}{53.5}
\newcommand{\miouCIDOFAKuroClean}{2.2}
\newcommand{\nDOFAKuroCleanVarTrainSubsetRealcov}{5}
\newcommand{\miouDOFAKuroCleanVarTrainSubsetRealcov}{50.0}
\newcommand{\miouCIDOFAKuroCleanVarTrainSubsetRealcov}{1.6}
\newcommand{\nDOFAKuroCoarseLOne}{5}
\newcommand{\miouDOFAKuroCoarseLOne}{53.7}
\newcommand{\miouCIDOFAKuroCoarseLOne}{2.8}
\newcommand{\dropDOFAKuroCoarseLOne}{\ensuremath{-}0.2}
\newcommand{\dropCIDOFAKuroCoarseLOne}{1.2}
\newcommand{\retDOFAKuroCoarseLOne}{1.003}
\newcommand{\retCIDOFAKuroCoarseLOne}{0.023}
\newcommand{\nDOFAKuroCoarseLTwo}{5}
\newcommand{\miouDOFAKuroCoarseLTwo}{48.4}
\newcommand{\miouCIDOFAKuroCoarseLTwo}{3.0}
\newcommand{\dropDOFAKuroCoarseLTwo}{5.1}
\newcommand{\dropCIDOFAKuroCoarseLTwo}{4.8}
\newcommand{\retDOFAKuroCoarseLTwo}{0.906}
\newcommand{\retCIDOFAKuroCoarseLTwo}{0.084}
\newcommand{\nDOFAKuroOmissionLOne}{5}
\newcommand{\miouDOFAKuroOmissionLOne}{49.4}
\newcommand{\miouCIDOFAKuroOmissionLOne}{7.2}
\newcommand{\dropDOFAKuroOmissionLOne}{4.1}
\newcommand{\dropCIDOFAKuroOmissionLOne}{5.7}
\newcommand{\retDOFAKuroOmissionLOne}{0.922}
\newcommand{\retCIDOFAKuroOmissionLOne}{0.109}
\newcommand{\nDOFAKuroOmissionLTwo}{5}
\newcommand{\miouDOFAKuroOmissionLTwo}{44.3}
\newcommand{\miouCIDOFAKuroOmissionLTwo}{8.0}
\newcommand{\dropDOFAKuroOmissionLTwo}{9.2}
\newcommand{\dropCIDOFAKuroOmissionLTwo}{6.2}
\newcommand{\retDOFAKuroOmissionLTwo}{0.826}
\newcommand{\retCIDOFAKuroOmissionLTwo}{0.125}
\newcommand{\nDOFAKuroShiftLOne}{5}
\newcommand{\miouDOFAKuroShiftLOne}{50.8}
\newcommand{\miouCIDOFAKuroShiftLOne}{4.1}
\newcommand{\dropDOFAKuroShiftLOne}{2.7}
\newcommand{\dropCIDOFAKuroShiftLOne}{5.0}
\newcommand{\retDOFAKuroShiftLOne}{0.951}
\newcommand{\retCIDOFAKuroShiftLOne}{0.089}
\newcommand{\nDOFAKuroShiftLTwo}{5}
\newcommand{\miouDOFAKuroShiftLTwo}{50.7}
\newcommand{\miouCIDOFAKuroShiftLTwo}{3.1}
\newcommand{\dropDOFAKuroShiftLTwo}{2.8}
\newcommand{\dropCIDOFAKuroShiftLTwo}{1.5}
\newcommand{\retDOFAKuroShiftLTwo}{0.947}
\newcommand{\retCIDOFAKuroShiftLTwo}{0.030}
\newcommand{\nDOFAOemBoundaryLOne}{5}
\newcommand{\miouDOFAOemBoundaryLOne}{58.3}
\newcommand{\miouCIDOFAOemBoundaryLOne}{1.1}
\newcommand{\dropDOFAOemBoundaryLOne}{2.7}
\newcommand{\dropCIDOFAOemBoundaryLOne}{1.2}
\newcommand{\retDOFAOemBoundaryLOne}{0.956}
\newcommand{\retCIDOFAOemBoundaryLOne}{0.019}
\newcommand{\nDOFAOemBoundaryLTwo}{5}
\newcommand{\miouDOFAOemBoundaryLTwo}{51.3}
\newcommand{\miouCIDOFAOemBoundaryLTwo}{0.7}
\newcommand{\dropDOFAOemBoundaryLTwo}{9.7}
\newcommand{\dropCIDOFAOemBoundaryLTwo}{0.6}
\newcommand{\retDOFAOemBoundaryLTwo}{0.841}
\newcommand{\retCIDOFAOemBoundaryLTwo}{0.008}
\newcommand{\nDOFAOemClean}{5}
\newcommand{\miouDOFAOemClean}{61.0}
\newcommand{\miouCIDOFAOemClean}{1.0}
\newcommand{\nDOFAOemCoarseLOne}{5}
\newcommand{\miouDOFAOemCoarseLOne}{59.0}
\newcommand{\miouCIDOFAOemCoarseLOne}{1.2}
\newcommand{\dropDOFAOemCoarseLOne}{2.0}
\newcommand{\dropCIDOFAOemCoarseLOne}{1.8}
\newcommand{\retDOFAOemCoarseLOne}{0.967}
\newcommand{\retCIDOFAOemCoarseLOne}{0.028}
\newcommand{\nDOFAOemCoarseLTwo}{5}
\newcommand{\miouDOFAOemCoarseLTwo}{56.2}
\newcommand{\miouCIDOFAOemCoarseLTwo}{0.6}
\newcommand{\dropDOFAOemCoarseLTwo}{4.8}
\newcommand{\dropCIDOFAOemCoarseLTwo}{0.6}
\newcommand{\retDOFAOemCoarseLTwo}{0.921}
\newcommand{\retCIDOFAOemCoarseLTwo}{0.009}
\newcommand{\nDOFAOemOmissionLOne}{5}
\newcommand{\miouDOFAOemOmissionLOne}{57.8}
\newcommand{\miouCIDOFAOemOmissionLOne}{1.6}
\newcommand{\dropDOFAOemOmissionLOne}{3.1}
\newcommand{\dropCIDOFAOemOmissionLOne}{1.7}
\newcommand{\retDOFAOemOmissionLOne}{0.949}
\newcommand{\retCIDOFAOemOmissionLOne}{0.028}
\newcommand{\nDOFAOemOmissionLTwo}{5}
\newcommand{\miouDOFAOemOmissionLTwo}{51.9}
\newcommand{\miouCIDOFAOemOmissionLTwo}{0.7}
\newcommand{\dropDOFAOemOmissionLTwo}{9.1}
\newcommand{\dropCIDOFAOemOmissionLTwo}{1.5}
\newcommand{\retDOFAOemOmissionLTwo}{0.851}
\newcommand{\retCIDOFAOemOmissionLTwo}{0.023}
\newcommand{\nDOFAOemShiftLOne}{5}
\newcommand{\miouDOFAOemShiftLOne}{60.1}
\newcommand{\miouCIDOFAOemShiftLOne}{1.0}
\newcommand{\dropDOFAOemShiftLOne}{0.9}
\newcommand{\dropCIDOFAOemShiftLOne}{1.8}
\newcommand{\retDOFAOemShiftLOne}{0.985}
\newcommand{\retCIDOFAOemShiftLOne}{0.030}
\newcommand{\nDOFAOemShiftLTwo}{5}
\newcommand{\miouDOFAOemShiftLTwo}{57.4}
\newcommand{\miouCIDOFAOemShiftLTwo}{1.1}
\newcommand{\dropDOFAOemShiftLTwo}{3.6}
\newcommand{\dropCIDOFAOemShiftLTwo}{1.5}
\newcommand{\retDOFAOemShiftLTwo}{0.941}
\newcommand{\retCIDOFAOemShiftLTwo}{0.024}
\newcommand{\nDOFAsenClean}{5}
\newcommand{\miouDOFAsenClean}{83.7}
\newcommand{\miouCIDOFAsenClean}{1.3}
\newcommand{\nDOFAsenOtsuLTwo}{5}
\newcommand{\miouDOFAsenOtsuLTwo}{74.9}
\newcommand{\miouCIDOFAsenOtsuLTwo}{1.2}
\newcommand{\dropDOFAsenOtsuLTwo}{8.8}
\newcommand{\dropCIDOFAsenOtsuLTwo}{1.9}
\newcommand{\retDOFAsenOtsuLTwo}{0.894}
\newcommand{\retCIDOFAsenOtsuLTwo}{0.022}
\newcommand{\nDOFASnTwoBoundaryLOne}{5}
\newcommand{\miouDOFASnTwoBoundaryLOne}{81.7}
\newcommand{\miouCIDOFASnTwoBoundaryLOne}{0.2}
\newcommand{\dropDOFASnTwoBoundaryLOne}{2.5}
\newcommand{\dropCIDOFASnTwoBoundaryLOne}{0.7}
\newcommand{\retDOFASnTwoBoundaryLOne}{0.970}
\newcommand{\retCIDOFASnTwoBoundaryLOne}{0.009}
\newcommand{\nDOFASnTwoBoundaryLTwo}{5}
\newcommand{\miouDOFASnTwoBoundaryLTwo}{72.5}
\newcommand{\miouCIDOFASnTwoBoundaryLTwo}{1.3}
\newcommand{\dropDOFASnTwoBoundaryLTwo}{11.7}
\newcommand{\dropCIDOFASnTwoBoundaryLTwo}{1.6}
\newcommand{\retDOFASnTwoBoundaryLTwo}{0.861}
\newcommand{\retCIDOFASnTwoBoundaryLTwo}{0.018}
\newcommand{\nDOFASnTwoClean}{5}
\newcommand{\miouDOFASnTwoClean}{84.2}
\newcommand{\miouCIDOFASnTwoClean}{0.6}
\newcommand{\nDOFASnTwoCoarseLOne}{5}
\newcommand{\miouDOFASnTwoCoarseLOne}{82.0}
\newcommand{\miouCIDOFASnTwoCoarseLOne}{0.5}
\newcommand{\dropDOFASnTwoCoarseLOne}{2.2}
\newcommand{\dropCIDOFASnTwoCoarseLOne}{0.5}
\newcommand{\retDOFASnTwoCoarseLOne}{0.974}
\newcommand{\retCIDOFASnTwoCoarseLOne}{0.006}
\newcommand{\nDOFASnTwoCoarseLTwo}{5}
\newcommand{\miouDOFASnTwoCoarseLTwo}{72.2}
\newcommand{\miouCIDOFASnTwoCoarseLTwo}{0.6}
\newcommand{\dropDOFASnTwoCoarseLTwo}{12.0}
\newcommand{\dropCIDOFASnTwoCoarseLTwo}{1.2}
\newcommand{\retDOFASnTwoCoarseLTwo}{0.858}
\newcommand{\retCIDOFASnTwoCoarseLTwo}{0.013}
\newcommand{\nDOFASnTwoOmissionLOne}{5}
\newcommand{\miouDOFASnTwoOmissionLOne}{78.3}
\newcommand{\miouCIDOFASnTwoOmissionLOne}{2.7}
\newcommand{\dropDOFASnTwoOmissionLOne}{5.9}
\newcommand{\dropCIDOFASnTwoOmissionLOne}{2.1}
\newcommand{\retDOFASnTwoOmissionLOne}{0.930}
\newcommand{\retCIDOFASnTwoOmissionLOne}{0.026}
\newcommand{\nDOFASnTwoOmissionLTwo}{5}
\newcommand{\miouDOFASnTwoOmissionLTwo}{68.8}
\newcommand{\miouCIDOFASnTwoOmissionLTwo}{1.6}
\newcommand{\dropDOFASnTwoOmissionLTwo}{15.4}
\newcommand{\dropCIDOFASnTwoOmissionLTwo}{1.8}
\newcommand{\retDOFASnTwoOmissionLTwo}{0.817}
\newcommand{\retCIDOFASnTwoOmissionLTwo}{0.021}
\newcommand{\nDOFASnTwoShiftLOne}{5}
\newcommand{\miouDOFASnTwoShiftLOne}{82.5}
\newcommand{\miouCIDOFASnTwoShiftLOne}{1.0}
\newcommand{\dropDOFASnTwoShiftLOne}{1.7}
\newcommand{\dropCIDOFASnTwoShiftLOne}{1.3}
\newcommand{\retDOFASnTwoShiftLOne}{0.980}
\newcommand{\retCIDOFASnTwoShiftLOne}{0.015}
\newcommand{\nDOFASnTwoShiftLTwo}{5}
\newcommand{\miouDOFASnTwoShiftLTwo}{75.9}
\newcommand{\miouCIDOFASnTwoShiftLTwo}{0.6}
\newcommand{\dropDOFASnTwoShiftLTwo}{8.3}
\newcommand{\dropCIDOFASnTwoShiftLTwo}{0.3}
\newcommand{\retDOFASnTwoShiftLTwo}{0.902}
\newcommand{\retCIDOFASnTwoShiftLTwo}{0.004}
\newcommand{\nPRIburnBoundaryLOne}{5}
\newcommand{\miouPRIburnBoundaryLOne}{85.4}
\newcommand{\miouCIPRIburnBoundaryLOne}{2.8}
\newcommand{\dropPRIburnBoundaryLOne}{3.3}
\newcommand{\dropCIPRIburnBoundaryLOne}{3.5}
\newcommand{\retPRIburnBoundaryLOne}{0.963}
\newcommand{\retCIPRIburnBoundaryLOne}{0.039}
\newcommand{\nPRIburnBoundaryLTwo}{5}
\newcommand{\miouPRIburnBoundaryLTwo}{73.8}
\newcommand{\miouCIPRIburnBoundaryLTwo}{3.7}
\newcommand{\dropPRIburnBoundaryLTwo}{14.9}
\newcommand{\dropCIPRIburnBoundaryLTwo}{4.3}
\newcommand{\retPRIburnBoundaryLTwo}{0.833}
\newcommand{\retCIPRIburnBoundaryLTwo}{0.048}
\newcommand{\nPRIburnClean}{5}
\newcommand{\miouPRIburnClean}{88.6}
\newcommand{\miouCIPRIburnClean}{0.9}
\newcommand{\nPRIburnCleanVarTrainSubsetCleanTwoFive}{5}
\newcommand{\miouPRIburnCleanVarTrainSubsetCleanTwoFive}{86.0}
\newcommand{\miouCIPRIburnCleanVarTrainSubsetCleanTwoFive}{2.1}
\newcommand{\nPRIburnCoarseLOne}{5}
\newcommand{\miouPRIburnCoarseLOne}{85.2}
\newcommand{\miouCIPRIburnCoarseLOne}{0.7}
\newcommand{\dropPRIburnCoarseLOne}{3.4}
\newcommand{\dropCIPRIburnCoarseLOne}{0.6}
\newcommand{\retPRIburnCoarseLOne}{0.961}
\newcommand{\retCIPRIburnCoarseLOne}{0.007}
\newcommand{\nPRIburnCoarseLTwo}{5}
\newcommand{\miouPRIburnCoarseLTwo}{71.6}
\newcommand{\miouCIPRIburnCoarseLTwo}{3.0}
\newcommand{\dropPRIburnCoarseLTwo}{17.1}
\newcommand{\dropCIPRIburnCoarseLTwo}{2.5}
\newcommand{\retPRIburnCoarseLTwo}{0.807}
\newcommand{\retCIPRIburnCoarseLTwo}{0.029}
\newcommand{\nPRIburnOmissionLOne}{5}
\newcommand{\miouPRIburnOmissionLOne}{84.8}
\newcommand{\miouCIPRIburnOmissionLOne}{1.2}
\newcommand{\dropPRIburnOmissionLOne}{3.9}
\newcommand{\dropCIPRIburnOmissionLOne}{1.4}
\newcommand{\retPRIburnOmissionLOne}{0.956}
\newcommand{\retCIPRIburnOmissionLOne}{0.015}
\newcommand{\nPRIburnOmissionLTwo}{5}
\newcommand{\miouPRIburnOmissionLTwo}{79.9}
\newcommand{\miouCIPRIburnOmissionLTwo}{2.9}
\newcommand{\dropPRIburnOmissionLTwo}{8.7}
\newcommand{\dropCIPRIburnOmissionLTwo}{3.5}
\newcommand{\retPRIburnOmissionLTwo}{0.902}
\newcommand{\retCIPRIburnOmissionLTwo}{0.039}
\newcommand{\nPRIburnShiftLOne}{5}
\newcommand{\miouPRIburnShiftLOne}{86.7}
\newcommand{\miouCIPRIburnShiftLOne}{0.8}
\newcommand{\dropPRIburnShiftLOne}{2.0}
\newcommand{\dropCIPRIburnShiftLOne}{0.8}
\newcommand{\retPRIburnShiftLOne}{0.978}
\newcommand{\retCIPRIburnShiftLOne}{0.008}
\newcommand{\nPRIburnShiftLTwo}{5}
\newcommand{\miouPRIburnShiftLTwo}{77.4}
\newcommand{\miouCIPRIburnShiftLTwo}{1.0}
\newcommand{\dropPRIburnShiftLTwo}{11.2}
\newcommand{\dropCIPRIburnShiftLTwo}{1.1}
\newcommand{\retPRIburnShiftLTwo}{0.873}
\newcommand{\retCIPRIburnShiftLTwo}{0.012}
\newcommand{\nPRIflairBoundaryLOne}{5}
\newcommand{\miouPRIflairBoundaryLOne}{36.9}
\newcommand{\miouCIPRIflairBoundaryLOne}{1.6}
\newcommand{\dropPRIflairBoundaryLOne}{2.5}
\newcommand{\dropCIPRIflairBoundaryLOne}{1.8}
\newcommand{\retPRIflairBoundaryLOne}{0.936}
\newcommand{\retCIPRIflairBoundaryLOne}{0.044}
\newcommand{\nPRIflairBoundaryLTwo}{5}
\newcommand{\miouPRIflairBoundaryLTwo}{33.5}
\newcommand{\miouCIPRIflairBoundaryLTwo}{2.6}
\newcommand{\dropPRIflairBoundaryLTwo}{6.0}
\newcommand{\dropCIPRIflairBoundaryLTwo}{2.9}
\newcommand{\retPRIflairBoundaryLTwo}{0.850}
\newcommand{\retCIPRIflairBoundaryLTwo}{0.071}
\newcommand{\nPRIflairClean}{5}
\newcommand{\miouPRIflairClean}{39.4}
\newcommand{\miouCIPRIflairClean}{1.7}
\newcommand{\nPRIflairCleanVarTrainSubsetCleanTwoFive}{5}
\newcommand{\miouPRIflairCleanVarTrainSubsetCleanTwoFive}{32.7}
\newcommand{\miouCIPRIflairCleanVarTrainSubsetCleanTwoFive}{1.2}
\newcommand{\nPRIflairCoarseLOne}{5}
\newcommand{\miouPRIflairCoarseLOne}{38.2}
\newcommand{\miouCIPRIflairCoarseLOne}{1.4}
\newcommand{\dropPRIflairCoarseLOne}{1.3}
\newcommand{\dropCIPRIflairCoarseLOne}{2.9}
\newcommand{\retPRIflairCoarseLOne}{0.969}
\newcommand{\retCIPRIflairCoarseLOne}{0.072}
\newcommand{\nPRIflairCoarseLTwo}{5}
\newcommand{\miouPRIflairCoarseLTwo}{33.4}
\newcommand{\miouCIPRIflairCoarseLTwo}{0.6}
\newcommand{\dropPRIflairCoarseLTwo}{6.0}
\newcommand{\dropCIPRIflairCoarseLTwo}{1.5}
\newcommand{\retPRIflairCoarseLTwo}{0.848}
\newcommand{\retCIPRIflairCoarseLTwo}{0.032}
\newcommand{\nPRIflairOmissionLOne}{5}
\newcommand{\miouPRIflairOmissionLOne}{36.6}
\newcommand{\miouCIPRIflairOmissionLOne}{2.8}
\newcommand{\dropPRIflairOmissionLOne}{2.8}
\newcommand{\dropCIPRIflairOmissionLOne}{3.1}
\newcommand{\retPRIflairOmissionLOne}{0.929}
\newcommand{\retCIPRIflairOmissionLOne}{0.075}
\newcommand{\nPRIflairOmissionLTwo}{5}
\newcommand{\miouPRIflairOmissionLTwo}{34.7}
\newcommand{\miouCIPRIflairOmissionLTwo}{1.8}
\newcommand{\dropPRIflairOmissionLTwo}{4.7}
\newcommand{\dropCIPRIflairOmissionLTwo}{2.9}
\newcommand{\retPRIflairOmissionLTwo}{0.882}
\newcommand{\retCIPRIflairOmissionLTwo}{0.069}
\newcommand{\nPRIflairShiftLOne}{5}
\newcommand{\miouPRIflairShiftLOne}{38.3}
\newcommand{\miouCIPRIflairShiftLOne}{1.3}
\newcommand{\dropPRIflairShiftLOne}{1.1}
\newcommand{\dropCIPRIflairShiftLOne}{1.8}
\newcommand{\retPRIflairShiftLOne}{0.972}
\newcommand{\retCIPRIflairShiftLOne}{0.046}
\newcommand{\nPRIflairShiftLTwo}{5}
\newcommand{\miouPRIflairShiftLTwo}{35.1}
\newcommand{\miouCIPRIflairShiftLTwo}{2.0}
\newcommand{\dropPRIflairShiftLTwo}{4.3}
\newcommand{\dropCIPRIflairShiftLTwo}{2.3}
\newcommand{\retPRIflairShiftLTwo}{0.892}
\newcommand{\retCIPRIflairShiftLTwo}{0.056}
\newcommand{\nRNburnBoundaryLOne}{5}
\newcommand{\miouRNburnBoundaryLOne}{85.6}
\newcommand{\miouCIRNburnBoundaryLOne}{0.8}
\newcommand{\dropRNburnBoundaryLOne}{2.5}
\newcommand{\dropCIRNburnBoundaryLOne}{1.6}
\newcommand{\retRNburnBoundaryLOne}{0.971}
\newcommand{\retCIRNburnBoundaryLOne}{0.018}
\newcommand{\nRNburnBoundaryLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouRNburnBoundaryLOneVarDecoderMaskTwoformerFull}{85.6}
\newcommand{\miouCIRNburnBoundaryLOneVarDecoderMaskTwoformerFull}{0.5}
\newcommand{\dropRNburnBoundaryLOneVarDecoderMaskTwoformerFull}{2.3}
\newcommand{\dropCIRNburnBoundaryLOneVarDecoderMaskTwoformerFull}{0.8}
\newcommand{\retRNburnBoundaryLOneVarDecoderMaskTwoformerFull}{0.973}
\newcommand{\retCIRNburnBoundaryLOneVarDecoderMaskTwoformerFull}{0.009}
\newcommand{\nRNburnBoundaryLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouRNburnBoundaryLOneVarDecoderMaskTwoformerLite}{62.5}
\newcommand{\miouCIRNburnBoundaryLOneVarDecoderMaskTwoformerLite}{12.6}
\newcommand{\dropRNburnBoundaryLOneVarDecoderMaskTwoformerLite}{1.2}
\newcommand{\dropCIRNburnBoundaryLOneVarDecoderMaskTwoformerLite}{2.6}
\newcommand{\retRNburnBoundaryLOneVarDecoderMaskTwoformerLite}{0.983}
\newcommand{\retCIRNburnBoundaryLOneVarDecoderMaskTwoformerLite}{0.039}
\newcommand{\nRNburnBoundaryLOneVarDecoderSamLite}{5}
\newcommand{\miouRNburnBoundaryLOneVarDecoderSamLite}{86.2}
\newcommand{\miouCIRNburnBoundaryLOneVarDecoderSamLite}{1.0}
\newcommand{\dropRNburnBoundaryLOneVarDecoderSamLite}{1.4}
\newcommand{\dropCIRNburnBoundaryLOneVarDecoderSamLite}{0.8}
\newcommand{\retRNburnBoundaryLOneVarDecoderSamLite}{0.984}
\newcommand{\retCIRNburnBoundaryLOneVarDecoderSamLite}{0.009}
\newcommand{\nRNburnBoundaryLOneVarDecoderSamPretrained}{5}
\newcommand{\miouRNburnBoundaryLOneVarDecoderSamPretrained}{77.4}
\newcommand{\miouCIRNburnBoundaryLOneVarDecoderSamPretrained}{22.7}
\newcommand{\dropRNburnBoundaryLOneVarDecoderSamPretrained}{1.9}
\newcommand{\dropCIRNburnBoundaryLOneVarDecoderSamPretrained}{1.5}
\newcommand{\retRNburnBoundaryLOneVarDecoderSamPretrained}{0.978}
\newcommand{\retCIRNburnBoundaryLOneVarDecoderSamPretrained}{0.017}
\newcommand{\nRNburnBoundaryLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouRNburnBoundaryLOneVarDecoderSegformerMlp}{83.2}
\newcommand{\miouCIRNburnBoundaryLOneVarDecoderSegformerMlp}{1.1}
\newcommand{\dropRNburnBoundaryLOneVarDecoderSegformerMlp}{5.0}
\newcommand{\dropCIRNburnBoundaryLOneVarDecoderSegformerMlp}{1.2}
\newcommand{\retRNburnBoundaryLOneVarDecoderSegformerMlp}{0.943}
\newcommand{\retCIRNburnBoundaryLOneVarDecoderSegformerMlp}{0.014}
\newcommand{\nRNburnBoundaryLTwo}{8}
\newcommand{\miouRNburnBoundaryLTwo}{75.2}
\newcommand{\miouCIRNburnBoundaryLTwo}{2.5}
\newcommand{\dropRNburnBoundaryLTwo}{13.1}
\newcommand{\dropCIRNburnBoundaryLTwo}{2.7}
\newcommand{\retRNburnBoundaryLTwo}{0.852}
\newcommand{\retCIRNburnBoundaryLTwo}{0.030}
\newcommand{\nRNburnBoundaryLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouRNburnBoundaryLTwoVarDecoderMaskTwoformerFull}{74.2}
\newcommand{\miouCIRNburnBoundaryLTwoVarDecoderMaskTwoformerFull}{1.5}
\newcommand{\dropRNburnBoundaryLTwoVarDecoderMaskTwoformerFull}{13.7}
\newcommand{\dropCIRNburnBoundaryLTwoVarDecoderMaskTwoformerFull}{1.3}
\newcommand{\retRNburnBoundaryLTwoVarDecoderMaskTwoformerFull}{0.844}
\newcommand{\retCIRNburnBoundaryLTwoVarDecoderMaskTwoformerFull}{0.015}
\newcommand{\nRNburnBoundaryLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouRNburnBoundaryLTwoVarDecoderMaskTwoformerLite}{55.8}
\newcommand{\miouCIRNburnBoundaryLTwoVarDecoderMaskTwoformerLite}{12.7}
\newcommand{\dropRNburnBoundaryLTwoVarDecoderMaskTwoformerLite}{7.9}
\newcommand{\dropCIRNburnBoundaryLTwoVarDecoderMaskTwoformerLite}{11.5}
\newcommand{\retRNburnBoundaryLTwoVarDecoderMaskTwoformerLite}{0.885}
\newcommand{\retCIRNburnBoundaryLTwoVarDecoderMaskTwoformerLite}{0.169}
\newcommand{\nRNburnBoundaryLTwoVarDecoderSamLite}{5}
\newcommand{\miouRNburnBoundaryLTwoVarDecoderSamLite}{78.0}
\newcommand{\miouCIRNburnBoundaryLTwoVarDecoderSamLite}{1.3}
\newcommand{\dropRNburnBoundaryLTwoVarDecoderSamLite}{9.7}
\newcommand{\dropCIRNburnBoundaryLTwoVarDecoderSamLite}{1.0}
\newcommand{\retRNburnBoundaryLTwoVarDecoderSamLite}{0.890}
\newcommand{\retCIRNburnBoundaryLTwoVarDecoderSamLite}{0.012}
\newcommand{\nRNburnBoundaryLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouRNburnBoundaryLTwoVarDecoderSamPretrained}{51.2}
\newcommand{\miouCIRNburnBoundaryLTwoVarDecoderSamPretrained}{17.7}
\newcommand{\dropRNburnBoundaryLTwoVarDecoderSamPretrained}{28.2}
\newcommand{\dropCIRNburnBoundaryLTwoVarDecoderSamPretrained}{26.3}
\newcommand{\retRNburnBoundaryLTwoVarDecoderSamPretrained}{0.680}
\newcommand{\retCIRNburnBoundaryLTwoVarDecoderSamPretrained}{0.298}
\newcommand{\nRNburnBoundaryLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouRNburnBoundaryLTwoVarDecoderSegformerMlp}{74.7}
\newcommand{\miouCIRNburnBoundaryLTwoVarDecoderSegformerMlp}{1.7}
\newcommand{\dropRNburnBoundaryLTwoVarDecoderSegformerMlp}{13.5}
\newcommand{\dropCIRNburnBoundaryLTwoVarDecoderSegformerMlp}{2.2}
\newcommand{\retRNburnBoundaryLTwoVarDecoderSegformerMlp}{0.847}
\newcommand{\retCIRNburnBoundaryLTwoVarDecoderSegformerMlp}{0.023}
\newcommand{\nRNburnBoundaryLTwoVarLossBootstrap}{5}
\newcommand{\miouRNburnBoundaryLTwoVarLossBootstrap}{75.2}
\newcommand{\miouCIRNburnBoundaryLTwoVarLossBootstrap}{4.1}
\newcommand{\dropRNburnBoundaryLTwoVarLossBootstrap}{13.1}
\newcommand{\dropCIRNburnBoundaryLTwoVarLossBootstrap}{4.1}
\newcommand{\retRNburnBoundaryLTwoVarLossBootstrap}{0.852}
\newcommand{\retCIRNburnBoundaryLTwoVarLossBootstrap}{0.046}
\newcommand{\nRNburnBoundaryLTwoVarLossGce}{5}
\newcommand{\miouRNburnBoundaryLTwoVarLossGce}{77.4}
\newcommand{\miouCIRNburnBoundaryLTwoVarLossGce}{2.0}
\newcommand{\dropRNburnBoundaryLTwoVarLossGce}{11.3}
\newcommand{\dropCIRNburnBoundaryLTwoVarLossGce}{1.7}
\newcommand{\retRNburnBoundaryLTwoVarLossGce}{0.873}
\newcommand{\retCIRNburnBoundaryLTwoVarLossGce}{0.019}
\newcommand{\nRNburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouRNburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{76.0}
\newcommand{\miouCIRNburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{2.7}
\newcommand{\dropRNburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{12.4}
\newcommand{\dropCIRNburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{3.2}
\newcommand{\retRNburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{0.860}
\newcommand{\retCIRNburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{0.035}
\newcommand{\nRNburnBoundaryLR}{5}
\newcommand{\miouRNburnBoundaryLR}{69.5}
\newcommand{\miouCIRNburnBoundaryLR}{4.0}
\newcommand{\dropRNburnBoundaryLR}{18.6}
\newcommand{\dropCIRNburnBoundaryLR}{4.5}
\newcommand{\retRNburnBoundaryLR}{0.789}
\newcommand{\retCIRNburnBoundaryLR}{0.050}
\newcommand{\nRNburnClean}{8}
\newcommand{\miouRNburnClean}{88.3}
\newcommand{\miouCIRNburnClean}{0.8}
\newcommand{\nRNburnCleanVarBandsRgb}{5}
\newcommand{\miouRNburnCleanVarBandsRgb}{78.9}
\newcommand{\miouCIRNburnCleanVarBandsRgb}{1.7}
\newcommand{\nRNburnCleanVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouRNburnCleanVarDecoderMaskTwoformerFull}{88.0}
\newcommand{\miouCIRNburnCleanVarDecoderMaskTwoformerFull}{0.5}
\newcommand{\nRNburnCleanVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouRNburnCleanVarDecoderMaskTwoformerLite}{63.7}
\newcommand{\miouCIRNburnCleanVarDecoderMaskTwoformerLite}{13.2}
\newcommand{\nRNburnCleanVarDecoderSamLite}{5}
\newcommand{\miouRNburnCleanVarDecoderSamLite}{87.6}
\newcommand{\miouCIRNburnCleanVarDecoderSamLite}{0.6}
\newcommand{\nRNburnCleanVarDecoderSamPretrained}{5}
\newcommand{\miouRNburnCleanVarDecoderSamPretrained}{79.4}
\newcommand{\miouCIRNburnCleanVarDecoderSamPretrained}{24.0}
\newcommand{\nRNburnCleanVarDecoderSegformerMlp}{5}
\newcommand{\miouRNburnCleanVarDecoderSegformerMlp}{88.2}
\newcommand{\miouCIRNburnCleanVarDecoderSegformerMlp}{1.4}
\newcommand{\nRNburnCleanVarInitRandom}{5}
\newcommand{\miouRNburnCleanVarInitRandom}{82.9}
\newcommand{\miouCIRNburnCleanVarInitRandom}{2.9}
\newcommand{\nRNburnCleanVarInitRandomLrMultThree}{1}
\newcommand{\miouRNburnCleanVarInitRandomLrMultThree}{79.4}
\newcommand{\miouCIRNburnCleanVarInitRandomLrMultThree}{--}
\newcommand{\nRNburnCleanVarLossBootstrap}{5}
\newcommand{\miouRNburnCleanVarLossBootstrap}{88.3}
\newcommand{\miouCIRNburnCleanVarLossBootstrap}{0.5}
\newcommand{\nRNburnCleanVarLossGce}{5}
\newcommand{\miouRNburnCleanVarLossGce}{88.7}
\newcommand{\miouCIRNburnCleanVarLossGce}{0.8}
\newcommand{\nRNburnCleanVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouRNburnCleanVarLrMultZeroThreeThreeThreeThree}{88.4}
\newcommand{\miouCIRNburnCleanVarLrMultZeroThreeThreeThreeThree}{1.1}
\newcommand{\nRNburnCleanVarTrainSubsetCleanTwoFive}{5}
\newcommand{\miouRNburnCleanVarTrainSubsetCleanTwoFive}{86.4}
\newcommand{\miouCIRNburnCleanVarTrainSubsetCleanTwoFive}{1.9}
\newcommand{\nRNburnCoarseLOne}{5}
\newcommand{\miouRNburnCoarseLOne}{84.2}
\newcommand{\miouCIRNburnCoarseLOne}{1.5}
\newcommand{\dropRNburnCoarseLOne}{4.0}
\newcommand{\dropCIRNburnCoarseLOne}{1.8}
\newcommand{\retRNburnCoarseLOne}{0.955}
\newcommand{\retCIRNburnCoarseLOne}{0.020}
\newcommand{\nRNburnCoarseLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouRNburnCoarseLOneVarDecoderMaskTwoformerFull}{84.8}
\newcommand{\miouCIRNburnCoarseLOneVarDecoderMaskTwoformerFull}{1.3}
\newcommand{\dropRNburnCoarseLOneVarDecoderMaskTwoformerFull}{3.2}
\newcommand{\dropCIRNburnCoarseLOneVarDecoderMaskTwoformerFull}{1.0}
\newcommand{\retRNburnCoarseLOneVarDecoderMaskTwoformerFull}{0.964}
\newcommand{\retCIRNburnCoarseLOneVarDecoderMaskTwoformerFull}{0.011}
\newcommand{\nRNburnCoarseLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouRNburnCoarseLOneVarDecoderMaskTwoformerLite}{62.6}
\newcommand{\miouCIRNburnCoarseLOneVarDecoderMaskTwoformerLite}{12.5}
\newcommand{\dropRNburnCoarseLOneVarDecoderMaskTwoformerLite}{1.1}
\newcommand{\dropCIRNburnCoarseLOneVarDecoderMaskTwoformerLite}{1.5}
\newcommand{\retRNburnCoarseLOneVarDecoderMaskTwoformerLite}{0.984}
\newcommand{\retCIRNburnCoarseLOneVarDecoderMaskTwoformerLite}{0.022}
\newcommand{\nRNburnCoarseLOneVarDecoderSamLite}{5}
\newcommand{\miouRNburnCoarseLOneVarDecoderSamLite}{84.9}
\newcommand{\miouCIRNburnCoarseLOneVarDecoderSamLite}{1.5}
\newcommand{\dropRNburnCoarseLOneVarDecoderSamLite}{2.7}
\newcommand{\dropCIRNburnCoarseLOneVarDecoderSamLite}{1.2}
\newcommand{\retRNburnCoarseLOneVarDecoderSamLite}{0.969}
\newcommand{\retCIRNburnCoarseLOneVarDecoderSamLite}{0.014}
\newcommand{\nRNburnCoarseLOneVarDecoderSamPretrained}{5}
\newcommand{\miouRNburnCoarseLOneVarDecoderSamPretrained}{76.5}
\newcommand{\miouCIRNburnCoarseLOneVarDecoderSamPretrained}{22.0}
\newcommand{\dropRNburnCoarseLOneVarDecoderSamPretrained}{2.9}
\newcommand{\dropCIRNburnCoarseLOneVarDecoderSamPretrained}{2.6}
\newcommand{\retRNburnCoarseLOneVarDecoderSamPretrained}{0.967}
\newcommand{\retCIRNburnCoarseLOneVarDecoderSamPretrained}{0.029}
\newcommand{\nRNburnCoarseLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouRNburnCoarseLOneVarDecoderSegformerMlp}{84.6}
\newcommand{\miouCIRNburnCoarseLOneVarDecoderSegformerMlp}{1.8}
\newcommand{\dropRNburnCoarseLOneVarDecoderSegformerMlp}{3.7}
\newcommand{\dropCIRNburnCoarseLOneVarDecoderSegformerMlp}{2.3}
\newcommand{\retRNburnCoarseLOneVarDecoderSegformerMlp}{0.959}
\newcommand{\retCIRNburnCoarseLOneVarDecoderSegformerMlp}{0.026}
\newcommand{\nRNburnCoarseLTwo}{8}
\newcommand{\miouRNburnCoarseLTwo}{70.5}
\newcommand{\miouCIRNburnCoarseLTwo}{2.3}
\newcommand{\dropRNburnCoarseLTwo}{17.8}
\newcommand{\dropCIRNburnCoarseLTwo}{2.7}
\newcommand{\retRNburnCoarseLTwo}{0.798}
\newcommand{\retCIRNburnCoarseLTwo}{0.030}
\newcommand{\nRNburnCoarseLTwoVarBandsRgb}{5}
\newcommand{\miouRNburnCoarseLTwoVarBandsRgb}{64.7}
\newcommand{\miouCIRNburnCoarseLTwoVarBandsRgb}{2.0}
\newcommand{\dropRNburnCoarseLTwoVarBandsRgb}{14.2}
\newcommand{\dropCIRNburnCoarseLTwoVarBandsRgb}{3.3}
\newcommand{\retRNburnCoarseLTwoVarBandsRgb}{0.820}
\newcommand{\retCIRNburnCoarseLTwoVarBandsRgb}{0.039}
\newcommand{\nRNburnCoarseLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouRNburnCoarseLTwoVarDecoderMaskTwoformerFull}{70.1}
\newcommand{\miouCIRNburnCoarseLTwoVarDecoderMaskTwoformerFull}{4.1}
\newcommand{\dropRNburnCoarseLTwoVarDecoderMaskTwoformerFull}{17.9}
\newcommand{\dropCIRNburnCoarseLTwoVarDecoderMaskTwoformerFull}{4.2}
\newcommand{\retRNburnCoarseLTwoVarDecoderMaskTwoformerFull}{0.797}
\newcommand{\retCIRNburnCoarseLTwoVarDecoderMaskTwoformerFull}{0.047}
\newcommand{\nRNburnCoarseLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouRNburnCoarseLTwoVarDecoderMaskTwoformerLite}{63.6}
\newcommand{\miouCIRNburnCoarseLTwoVarDecoderMaskTwoformerLite}{2.3}
\newcommand{\dropRNburnCoarseLTwoVarDecoderMaskTwoformerLite}{0.1}
\newcommand{\dropCIRNburnCoarseLTwoVarDecoderMaskTwoformerLite}{11.8}
\newcommand{\retRNburnCoarseLTwoVarDecoderMaskTwoformerLite}{1.025}
\newcommand{\retCIRNburnCoarseLTwoVarDecoderMaskTwoformerLite}{0.241}
\newcommand{\nRNburnCoarseLTwoVarDecoderSamLite}{5}
\newcommand{\miouRNburnCoarseLTwoVarDecoderSamLite}{71.2}
\newcommand{\miouCIRNburnCoarseLTwoVarDecoderSamLite}{2.7}
\newcommand{\dropRNburnCoarseLTwoVarDecoderSamLite}{16.5}
\newcommand{\dropCIRNburnCoarseLTwoVarDecoderSamLite}{2.9}
\newcommand{\retRNburnCoarseLTwoVarDecoderSamLite}{0.812}
\newcommand{\retCIRNburnCoarseLTwoVarDecoderSamLite}{0.032}
\newcommand{\nRNburnCoarseLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouRNburnCoarseLTwoVarDecoderSamPretrained}{55.5}
\newcommand{\miouCIRNburnCoarseLTwoVarDecoderSamPretrained}{18.3}
\newcommand{\dropRNburnCoarseLTwoVarDecoderSamPretrained}{23.8}
\newcommand{\dropCIRNburnCoarseLTwoVarDecoderSamPretrained}{23.4}
\newcommand{\retRNburnCoarseLTwoVarDecoderSamPretrained}{0.729}
\newcommand{\retCIRNburnCoarseLTwoVarDecoderSamPretrained}{0.266}
\newcommand{\nRNburnCoarseLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouRNburnCoarseLTwoVarDecoderSegformerMlp}{70.9}
\newcommand{\miouCIRNburnCoarseLTwoVarDecoderSegformerMlp}{2.2}
\newcommand{\dropRNburnCoarseLTwoVarDecoderSegformerMlp}{17.3}
\newcommand{\dropCIRNburnCoarseLTwoVarDecoderSegformerMlp}{1.8}
\newcommand{\retRNburnCoarseLTwoVarDecoderSegformerMlp}{0.804}
\newcommand{\retCIRNburnCoarseLTwoVarDecoderSegformerMlp}{0.021}
\newcommand{\nRNburnCoarseLTwoVarInitRandom}{5}
\newcommand{\miouRNburnCoarseLTwoVarInitRandom}{70.2}
\newcommand{\miouCIRNburnCoarseLTwoVarInitRandom}{1.7}
\newcommand{\dropRNburnCoarseLTwoVarInitRandom}{12.7}
\newcommand{\dropCIRNburnCoarseLTwoVarInitRandom}{2.3}
\newcommand{\retRNburnCoarseLTwoVarInitRandom}{0.847}
\newcommand{\retCIRNburnCoarseLTwoVarInitRandom}{0.024}
\newcommand{\nRNburnCoarseLTwoVarLossBootstrap}{5}
\newcommand{\miouRNburnCoarseLTwoVarLossBootstrap}{70.6}
\newcommand{\miouCIRNburnCoarseLTwoVarLossBootstrap}{3.5}
\newcommand{\dropRNburnCoarseLTwoVarLossBootstrap}{17.7}
\newcommand{\dropCIRNburnCoarseLTwoVarLossBootstrap}{3.8}
\newcommand{\retRNburnCoarseLTwoVarLossBootstrap}{0.800}
\newcommand{\retCIRNburnCoarseLTwoVarLossBootstrap}{0.042}
\newcommand{\nRNburnCoarseLTwoVarLossGce}{5}
\newcommand{\miouRNburnCoarseLTwoVarLossGce}{72.1}
\newcommand{\miouCIRNburnCoarseLTwoVarLossGce}{1.8}
\newcommand{\dropRNburnCoarseLTwoVarLossGce}{16.6}
\newcommand{\dropCIRNburnCoarseLTwoVarLossGce}{1.2}
\newcommand{\retRNburnCoarseLTwoVarLossGce}{0.813}
\newcommand{\retCIRNburnCoarseLTwoVarLossGce}{0.014}
\newcommand{\nRNburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouRNburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{70.2}
\newcommand{\miouCIRNburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{2.2}
\newcommand{\dropRNburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{18.2}
\newcommand{\dropCIRNburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{3.1}
\newcommand{\retRNburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.794}
\newcommand{\retCIRNburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.033}
\newcommand{\nRNburnCoarseLR}{5}
\newcommand{\miouRNburnCoarseLR}{66.8}
\newcommand{\miouCIRNburnCoarseLR}{2.6}
\newcommand{\dropRNburnCoarseLR}{21.3}
\newcommand{\dropCIRNburnCoarseLR}{2.0}
\newcommand{\retRNburnCoarseLR}{0.758}
\newcommand{\retCIRNburnCoarseLR}{0.024}
\newcommand{\nRNburnOmissionLOne}{5}
\newcommand{\miouRNburnOmissionLOne}{84.2}
\newcommand{\miouCIRNburnOmissionLOne}{1.2}
\newcommand{\dropRNburnOmissionLOne}{3.9}
\newcommand{\dropCIRNburnOmissionLOne}{1.3}
\newcommand{\retRNburnOmissionLOne}{0.956}
\newcommand{\retCIRNburnOmissionLOne}{0.014}
\newcommand{\nRNburnOmissionLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouRNburnOmissionLOneVarDecoderMaskTwoformerFull}{87.0}
\newcommand{\miouCIRNburnOmissionLOneVarDecoderMaskTwoformerFull}{1.2}
\newcommand{\dropRNburnOmissionLOneVarDecoderMaskTwoformerFull}{1.0}
\newcommand{\dropCIRNburnOmissionLOneVarDecoderMaskTwoformerFull}{1.1}
\newcommand{\retRNburnOmissionLOneVarDecoderMaskTwoformerFull}{0.989}
\newcommand{\retCIRNburnOmissionLOneVarDecoderMaskTwoformerFull}{0.013}
\newcommand{\nRNburnOmissionLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouRNburnOmissionLOneVarDecoderMaskTwoformerLite}{64.0}
\newcommand{\miouCIRNburnOmissionLOneVarDecoderMaskTwoformerLite}{16.9}
\newcommand{\dropRNburnOmissionLOneVarDecoderMaskTwoformerLite}{\ensuremath{-}0.3}
\newcommand{\dropCIRNburnOmissionLOneVarDecoderMaskTwoformerLite}{20.0}
\newcommand{\retRNburnOmissionLOneVarDecoderMaskTwoformerLite}{1.028}
\newcommand{\retCIRNburnOmissionLOneVarDecoderMaskTwoformerLite}{0.329}
\newcommand{\nRNburnOmissionLOneVarDecoderSamLite}{5}
\newcommand{\miouRNburnOmissionLOneVarDecoderSamLite}{85.8}
\newcommand{\miouCIRNburnOmissionLOneVarDecoderSamLite}{2.9}
\newcommand{\dropRNburnOmissionLOneVarDecoderSamLite}{1.8}
\newcommand{\dropCIRNburnOmissionLOneVarDecoderSamLite}{3.1}
\newcommand{\retRNburnOmissionLOneVarDecoderSamLite}{0.979}
\newcommand{\retCIRNburnOmissionLOneVarDecoderSamLite}{0.036}
\newcommand{\nRNburnOmissionLOneVarDecoderSamPretrained}{5}
\newcommand{\miouRNburnOmissionLOneVarDecoderSamPretrained}{60.0}
\newcommand{\miouCIRNburnOmissionLOneVarDecoderSamPretrained}{25.9}
\newcommand{\dropRNburnOmissionLOneVarDecoderSamPretrained}{19.4}
\newcommand{\dropCIRNburnOmissionLOneVarDecoderSamPretrained}{27.5}
\newcommand{\retRNburnOmissionLOneVarDecoderSamPretrained}{0.780}
\newcommand{\retCIRNburnOmissionLOneVarDecoderSamPretrained}{0.311}
\newcommand{\nRNburnOmissionLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouRNburnOmissionLOneVarDecoderSegformerMlp}{84.4}
\newcommand{\miouCIRNburnOmissionLOneVarDecoderSegformerMlp}{2.1}
\newcommand{\dropRNburnOmissionLOneVarDecoderSegformerMlp}{3.8}
\newcommand{\dropCIRNburnOmissionLOneVarDecoderSegformerMlp}{3.3}
\newcommand{\retRNburnOmissionLOneVarDecoderSegformerMlp}{0.957}
\newcommand{\retCIRNburnOmissionLOneVarDecoderSegformerMlp}{0.037}
\newcommand{\nRNburnOmissionLTwo}{8}
\newcommand{\miouRNburnOmissionLTwo}{71.0}
\newcommand{\miouCIRNburnOmissionLTwo}{8.4}
\newcommand{\dropRNburnOmissionLTwo}{17.3}
\newcommand{\dropCIRNburnOmissionLTwo}{8.7}
\newcommand{\retRNburnOmissionLTwo}{0.805}
\newcommand{\retCIRNburnOmissionLTwo}{0.097}
\newcommand{\nRNburnOmissionLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouRNburnOmissionLTwoVarDecoderMaskTwoformerFull}{82.7}
\newcommand{\miouCIRNburnOmissionLTwoVarDecoderMaskTwoformerFull}{2.8}
\newcommand{\dropRNburnOmissionLTwoVarDecoderMaskTwoformerFull}{5.2}
\newcommand{\dropCIRNburnOmissionLTwoVarDecoderMaskTwoformerFull}{2.9}
\newcommand{\retRNburnOmissionLTwoVarDecoderMaskTwoformerFull}{0.940}
\newcommand{\retCIRNburnOmissionLTwoVarDecoderMaskTwoformerFull}{0.033}
\newcommand{\nRNburnOmissionLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouRNburnOmissionLTwoVarDecoderMaskTwoformerLite}{49.4}
\newcommand{\miouCIRNburnOmissionLTwoVarDecoderMaskTwoformerLite}{10.3}
\newcommand{\dropRNburnOmissionLTwoVarDecoderMaskTwoformerLite}{14.3}
\newcommand{\dropCIRNburnOmissionLTwoVarDecoderMaskTwoformerLite}{23.4}
\newcommand{\retRNburnOmissionLTwoVarDecoderMaskTwoformerLite}{0.822}
\newcommand{\retCIRNburnOmissionLTwoVarDecoderMaskTwoformerLite}{0.424}
\newcommand{\nRNburnOmissionLTwoVarDecoderSamLite}{5}
\newcommand{\miouRNburnOmissionLTwoVarDecoderSamLite}{74.5}
\newcommand{\miouCIRNburnOmissionLTwoVarDecoderSamLite}{4.7}
\newcommand{\dropRNburnOmissionLTwoVarDecoderSamLite}{13.1}
\newcommand{\dropCIRNburnOmissionLTwoVarDecoderSamLite}{5.2}
\newcommand{\retRNburnOmissionLTwoVarDecoderSamLite}{0.850}
\newcommand{\retCIRNburnOmissionLTwoVarDecoderSamLite}{0.059}
\newcommand{\nRNburnOmissionLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouRNburnOmissionLTwoVarDecoderSamPretrained}{44.8}
\newcommand{\miouCIRNburnOmissionLTwoVarDecoderSamPretrained}{0.0}
\newcommand{\dropRNburnOmissionLTwoVarDecoderSamPretrained}{34.6}
\newcommand{\dropCIRNburnOmissionLTwoVarDecoderSamPretrained}{24.0}
\newcommand{\retRNburnOmissionLTwoVarDecoderSamPretrained}{0.607}
\newcommand{\retCIRNburnOmissionLTwoVarDecoderSamPretrained}{0.273}
\newcommand{\nRNburnOmissionLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouRNburnOmissionLTwoVarDecoderSegformerMlp}{74.3}
\newcommand{\miouCIRNburnOmissionLTwoVarDecoderSegformerMlp}{5.4}
\newcommand{\dropRNburnOmissionLTwoVarDecoderSegformerMlp}{13.9}
\newcommand{\dropCIRNburnOmissionLTwoVarDecoderSegformerMlp}{4.8}
\newcommand{\retRNburnOmissionLTwoVarDecoderSegformerMlp}{0.842}
\newcommand{\retCIRNburnOmissionLTwoVarDecoderSegformerMlp}{0.054}
\newcommand{\nRNburnOmissionLTwoVarInitRandom}{5}
\newcommand{\miouRNburnOmissionLTwoVarInitRandom}{64.5}
\newcommand{\miouCIRNburnOmissionLTwoVarInitRandom}{16.2}
\newcommand{\dropRNburnOmissionLTwoVarInitRandom}{18.4}
\newcommand{\dropCIRNburnOmissionLTwoVarInitRandom}{13.6}
\newcommand{\retRNburnOmissionLTwoVarInitRandom}{0.775}
\newcommand{\retCIRNburnOmissionLTwoVarInitRandom}{0.173}
\newcommand{\nRNburnOmissionLTwoVarLossBootstrap}{5}
\newcommand{\miouRNburnOmissionLTwoVarLossBootstrap}{72.3}
\newcommand{\miouCIRNburnOmissionLTwoVarLossBootstrap}{15.0}
\newcommand{\dropRNburnOmissionLTwoVarLossBootstrap}{16.0}
\newcommand{\dropCIRNburnOmissionLTwoVarLossBootstrap}{15.1}
\newcommand{\retRNburnOmissionLTwoVarLossBootstrap}{0.819}
\newcommand{\retCIRNburnOmissionLTwoVarLossBootstrap}{0.171}
\newcommand{\nRNburnOmissionLTwoVarLossGce}{5}
\newcommand{\miouRNburnOmissionLTwoVarLossGce}{63.6}
\newcommand{\miouCIRNburnOmissionLTwoVarLossGce}{15.9}
\newcommand{\dropRNburnOmissionLTwoVarLossGce}{25.1}
\newcommand{\dropCIRNburnOmissionLTwoVarLossGce}{15.6}
\newcommand{\retRNburnOmissionLTwoVarLossGce}{0.717}
\newcommand{\retCIRNburnOmissionLTwoVarLossGce}{0.177}
\newcommand{\nRNburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouRNburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{74.9}
\newcommand{\miouCIRNburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{7.4}
\newcommand{\dropRNburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{13.5}
\newcommand{\dropCIRNburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{8.1}
\newcommand{\retRNburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{0.848}
\newcommand{\retCIRNburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{0.090}
\newcommand{\nRNburnOmissionLR}{5}
\newcommand{\miouRNburnOmissionLR}{56.8}
\newcommand{\miouCIRNburnOmissionLR}{8.5}
\newcommand{\dropRNburnOmissionLR}{31.3}
\newcommand{\dropCIRNburnOmissionLR}{8.2}
\newcommand{\retRNburnOmissionLR}{0.645}
\newcommand{\retCIRNburnOmissionLR}{0.094}
\newcommand{\nRNburnShiftLOne}{5}
\newcommand{\miouRNburnShiftLOne}{85.8}
\newcommand{\miouCIRNburnShiftLOne}{0.6}
\newcommand{\dropRNburnShiftLOne}{2.3}
\newcommand{\dropCIRNburnShiftLOne}{0.7}
\newcommand{\retRNburnShiftLOne}{0.974}
\newcommand{\retCIRNburnShiftLOne}{0.007}
\newcommand{\nRNburnShiftLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouRNburnShiftLOneVarDecoderMaskTwoformerFull}{85.3}
\newcommand{\miouCIRNburnShiftLOneVarDecoderMaskTwoformerFull}{1.1}
\newcommand{\dropRNburnShiftLOneVarDecoderMaskTwoformerFull}{2.7}
\newcommand{\dropCIRNburnShiftLOneVarDecoderMaskTwoformerFull}{1.1}
\newcommand{\retRNburnShiftLOneVarDecoderMaskTwoformerFull}{0.969}
\newcommand{\retCIRNburnShiftLOneVarDecoderMaskTwoformerFull}{0.012}
\newcommand{\nRNburnShiftLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouRNburnShiftLOneVarDecoderMaskTwoformerLite}{61.4}
\newcommand{\miouCIRNburnShiftLOneVarDecoderMaskTwoformerLite}{11.6}
\newcommand{\dropRNburnShiftLOneVarDecoderMaskTwoformerLite}{2.2}
\newcommand{\dropCIRNburnShiftLOneVarDecoderMaskTwoformerLite}{2.5}
\newcommand{\retRNburnShiftLOneVarDecoderMaskTwoformerLite}{0.968}
\newcommand{\retCIRNburnShiftLOneVarDecoderMaskTwoformerLite}{0.036}
\newcommand{\nRNburnShiftLOneVarDecoderSamLite}{5}
\newcommand{\miouRNburnShiftLOneVarDecoderSamLite}{86.6}
\newcommand{\miouCIRNburnShiftLOneVarDecoderSamLite}{0.5}
\newcommand{\dropRNburnShiftLOneVarDecoderSamLite}{1.0}
\newcommand{\dropCIRNburnShiftLOneVarDecoderSamLite}{1.1}
\newcommand{\retRNburnShiftLOneVarDecoderSamLite}{0.989}
\newcommand{\retCIRNburnShiftLOneVarDecoderSamLite}{0.013}
\newcommand{\nRNburnShiftLOneVarDecoderSamPretrained}{5}
\newcommand{\miouRNburnShiftLOneVarDecoderSamPretrained}{69.7}
\newcommand{\miouCIRNburnShiftLOneVarDecoderSamPretrained}{28.2}
\newcommand{\dropRNburnShiftLOneVarDecoderSamPretrained}{9.7}
\newcommand{\dropCIRNburnShiftLOneVarDecoderSamPretrained}{23.2}
\newcommand{\retRNburnShiftLOneVarDecoderSamPretrained}{0.890}
\newcommand{\retCIRNburnShiftLOneVarDecoderSamPretrained}{0.264}
\newcommand{\nRNburnShiftLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouRNburnShiftLOneVarDecoderSegformerMlp}{85.8}
\newcommand{\miouCIRNburnShiftLOneVarDecoderSegformerMlp}{1.2}
\newcommand{\dropRNburnShiftLOneVarDecoderSegformerMlp}{2.4}
\newcommand{\dropCIRNburnShiftLOneVarDecoderSegformerMlp}{2.0}
\newcommand{\retRNburnShiftLOneVarDecoderSegformerMlp}{0.973}
\newcommand{\retCIRNburnShiftLOneVarDecoderSegformerMlp}{0.023}
\newcommand{\nRNburnShiftLTwo}{8}
\newcommand{\miouRNburnShiftLTwo}{76.1}
\newcommand{\miouCIRNburnShiftLTwo}{1.2}
\newcommand{\dropRNburnShiftLTwo}{12.1}
\newcommand{\dropCIRNburnShiftLTwo}{1.5}
\newcommand{\retRNburnShiftLTwo}{0.863}
\newcommand{\retCIRNburnShiftLTwo}{0.016}
\newcommand{\nRNburnShiftLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouRNburnShiftLTwoVarDecoderMaskTwoformerFull}{76.4}
\newcommand{\miouCIRNburnShiftLTwoVarDecoderMaskTwoformerFull}{1.9}
\newcommand{\dropRNburnShiftLTwoVarDecoderMaskTwoformerFull}{11.5}
\newcommand{\dropCIRNburnShiftLTwoVarDecoderMaskTwoformerFull}{2.0}
\newcommand{\retRNburnShiftLTwoVarDecoderMaskTwoformerFull}{0.869}
\newcommand{\retCIRNburnShiftLTwoVarDecoderMaskTwoformerFull}{0.022}
\newcommand{\nRNburnShiftLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouRNburnShiftLTwoVarDecoderMaskTwoformerLite}{59.6}
\newcommand{\miouCIRNburnShiftLTwoVarDecoderMaskTwoformerLite}{12.2}
\newcommand{\dropRNburnShiftLTwoVarDecoderMaskTwoformerLite}{4.1}
\newcommand{\dropCIRNburnShiftLTwoVarDecoderMaskTwoformerLite}{8.2}
\newcommand{\retRNburnShiftLTwoVarDecoderMaskTwoformerLite}{0.941}
\newcommand{\retCIRNburnShiftLTwoVarDecoderMaskTwoformerLite}{0.118}
\newcommand{\nRNburnShiftLTwoVarDecoderSamLite}{5}
\newcommand{\miouRNburnShiftLTwoVarDecoderSamLite}{77.4}
\newcommand{\miouCIRNburnShiftLTwoVarDecoderSamLite}{1.4}
\newcommand{\dropRNburnShiftLTwoVarDecoderSamLite}{10.3}
\newcommand{\dropCIRNburnShiftLTwoVarDecoderSamLite}{1.6}
\newcommand{\retRNburnShiftLTwoVarDecoderSamLite}{0.883}
\newcommand{\retCIRNburnShiftLTwoVarDecoderSamLite}{0.018}
\newcommand{\nRNburnShiftLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouRNburnShiftLTwoVarDecoderSamPretrained}{51.0}
\newcommand{\miouCIRNburnShiftLTwoVarDecoderSamPretrained}{17.3}
\newcommand{\dropRNburnShiftLTwoVarDecoderSamPretrained}{28.3}
\newcommand{\dropCIRNburnShiftLTwoVarDecoderSamPretrained}{26.2}
\newcommand{\retRNburnShiftLTwoVarDecoderSamPretrained}{0.679}
\newcommand{\retCIRNburnShiftLTwoVarDecoderSamPretrained}{0.296}
\newcommand{\nRNburnShiftLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouRNburnShiftLTwoVarDecoderSegformerMlp}{76.7}
\newcommand{\miouCIRNburnShiftLTwoVarDecoderSegformerMlp}{1.1}
\newcommand{\dropRNburnShiftLTwoVarDecoderSegformerMlp}{11.6}
\newcommand{\dropCIRNburnShiftLTwoVarDecoderSegformerMlp}{2.4}
\newcommand{\retRNburnShiftLTwoVarDecoderSegformerMlp}{0.869}
\newcommand{\retCIRNburnShiftLTwoVarDecoderSegformerMlp}{0.025}
\newcommand{\nRNburnShiftLTwoVarLossBootstrap}{5}
\newcommand{\miouRNburnShiftLTwoVarLossBootstrap}{77.0}
\newcommand{\miouCIRNburnShiftLTwoVarLossBootstrap}{1.7}
\newcommand{\dropRNburnShiftLTwoVarLossBootstrap}{11.3}
\newcommand{\dropCIRNburnShiftLTwoVarLossBootstrap}{1.4}
\newcommand{\retRNburnShiftLTwoVarLossBootstrap}{0.872}
\newcommand{\retCIRNburnShiftLTwoVarLossBootstrap}{0.016}
\newcommand{\nRNburnShiftLTwoVarLossGce}{5}
\newcommand{\miouRNburnShiftLTwoVarLossGce}{77.8}
\newcommand{\miouCIRNburnShiftLTwoVarLossGce}{2.9}
\newcommand{\dropRNburnShiftLTwoVarLossGce}{10.9}
\newcommand{\dropCIRNburnShiftLTwoVarLossGce}{3.4}
\newcommand{\retRNburnShiftLTwoVarLossGce}{0.878}
\newcommand{\retCIRNburnShiftLTwoVarLossGce}{0.037}
\newcommand{\nRNburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouRNburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{75.9}
\newcommand{\miouCIRNburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{1.3}
\newcommand{\dropRNburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{12.5}
\newcommand{\dropCIRNburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{2.0}
\newcommand{\retRNburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.859}
\newcommand{\retCIRNburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.021}
\newcommand{\nRNburnShiftLR}{5}
\newcommand{\miouRNburnShiftLR}{69.6}
\newcommand{\miouCIRNburnShiftLR}{4.3}
\newcommand{\dropRNburnShiftLR}{18.5}
\newcommand{\dropCIRNburnShiftLR}{4.5}
\newcommand{\retRNburnShiftLR}{0.790}
\newcommand{\retCIRNburnShiftLR}{0.050}
\newcommand{\nRNChesBoundaryLOne}{5}
\newcommand{\miouRNChesBoundaryLOne}{80.6}
\newcommand{\miouCIRNChesBoundaryLOne}{0.3}
\newcommand{\dropRNChesBoundaryLOne}{1.9}
\newcommand{\dropCIRNChesBoundaryLOne}{0.8}
\newcommand{\retRNChesBoundaryLOne}{0.977}
\newcommand{\retCIRNChesBoundaryLOne}{0.010}
\newcommand{\nRNChesBoundaryLTwo}{5}
\newcommand{\miouRNChesBoundaryLTwo}{73.6}
\newcommand{\miouCIRNChesBoundaryLTwo}{2.2}
\newcommand{\dropRNChesBoundaryLTwo}{8.8}
\newcommand{\dropCIRNChesBoundaryLTwo}{2.2}
\newcommand{\retRNChesBoundaryLTwo}{0.893}
\newcommand{\retCIRNChesBoundaryLTwo}{0.027}
\newcommand{\nRNChesClean}{5}
\newcommand{\miouRNChesClean}{82.5}
\newcommand{\miouCIRNChesClean}{0.7}
\newcommand{\nRNChesCoarseLOne}{5}
\newcommand{\miouRNChesCoarseLOne}{80.8}
\newcommand{\miouCIRNChesCoarseLOne}{0.3}
\newcommand{\dropRNChesCoarseLOne}{1.7}
\newcommand{\dropCIRNChesCoarseLOne}{0.9}
\newcommand{\retRNChesCoarseLOne}{0.979}
\newcommand{\retCIRNChesCoarseLOne}{0.010}
\newcommand{\nRNChesCoarseLTwo}{5}
\newcommand{\miouRNChesCoarseLTwo}{69.8}
\newcommand{\miouCIRNChesCoarseLTwo}{0.4}
\newcommand{\dropRNChesCoarseLTwo}{12.6}
\newcommand{\dropCIRNChesCoarseLTwo}{1.2}
\newcommand{\retRNChesCoarseLTwo}{0.847}
\newcommand{\retCIRNChesCoarseLTwo}{0.013}
\newcommand{\nRNChesNlcdREAL}{5}
\newcommand{\miouRNChesNlcdREAL}{59.6}
\newcommand{\miouCIRNChesNlcdREAL}{4.2}
\newcommand{\dropRNChesNlcdREAL}{22.9}
\newcommand{\dropCIRNChesNlcdREAL}{4.9}
\newcommand{\retRNChesNlcdREAL}{0.723}
\newcommand{\retCIRNChesNlcdREAL}{0.058}
\newcommand{\nRNChesOmissionLOne}{5}
\newcommand{\miouRNChesOmissionLOne}{80.2}
\newcommand{\miouCIRNChesOmissionLOne}{1.5}
\newcommand{\dropRNChesOmissionLOne}{2.2}
\newcommand{\dropCIRNChesOmissionLOne}{1.3}
\newcommand{\retRNChesOmissionLOne}{0.973}
\newcommand{\retCIRNChesOmissionLOne}{0.015}
\newcommand{\nRNChesOmissionLTwo}{5}
\newcommand{\miouRNChesOmissionLTwo}{77.9}
\newcommand{\miouCIRNChesOmissionLTwo}{1.4}
\newcommand{\dropRNChesOmissionLTwo}{4.6}
\newcommand{\dropCIRNChesOmissionLTwo}{1.2}
\newcommand{\retRNChesOmissionLTwo}{0.944}
\newcommand{\retCIRNChesOmissionLTwo}{0.014}
\newcommand{\nRNChesShiftLOne}{5}
\newcommand{\miouRNChesShiftLOne}{80.6}
\newcommand{\miouCIRNChesShiftLOne}{1.2}
\newcommand{\dropRNChesShiftLOne}{1.8}
\newcommand{\dropCIRNChesShiftLOne}{0.7}
\newcommand{\retRNChesShiftLOne}{0.978}
\newcommand{\retCIRNChesShiftLOne}{0.009}
\newcommand{\nRNChesShiftLTwo}{5}
\newcommand{\miouRNChesShiftLTwo}{73.8}
\newcommand{\miouCIRNChesShiftLTwo}{0.9}
\newcommand{\dropRNChesShiftLTwo}{8.6}
\newcommand{\dropCIRNChesShiftLTwo}{0.9}
\newcommand{\retRNChesShiftLTwo}{0.895}
\newcommand{\retCIRNChesShiftLTwo}{0.011}
\newcommand{\nRNCsTwelveBoundaryLOne}{5}
\newcommand{\miouRNCsTwelveBoundaryLOne}{61.8}
\newcommand{\miouCIRNCsTwelveBoundaryLOne}{1.3}
\newcommand{\dropRNCsTwelveBoundaryLOne}{2.3}
\newcommand{\dropCIRNCsTwelveBoundaryLOne}{1.0}
\newcommand{\retRNCsTwelveBoundaryLOne}{0.965}
\newcommand{\retCIRNCsTwelveBoundaryLOne}{0.015}
\newcommand{\nRNCsTwelveBoundaryLTwo}{5}
\newcommand{\miouRNCsTwelveBoundaryLTwo}{56.4}
\newcommand{\miouCIRNCsTwelveBoundaryLTwo}{4.2}
\newcommand{\dropRNCsTwelveBoundaryLTwo}{7.6}
\newcommand{\dropCIRNCsTwelveBoundaryLTwo}{3.5}
\newcommand{\retRNCsTwelveBoundaryLTwo}{0.880}
\newcommand{\retCIRNCsTwelveBoundaryLTwo}{0.056}
\newcommand{\nRNCsTwelveClean}{5}
\newcommand{\miouRNCsTwelveClean}{64.0}
\newcommand{\miouCIRNCsTwelveClean}{0.9}
\newcommand{\nRNCsTwelveCoarseLOne}{5}
\newcommand{\miouRNCsTwelveCoarseLOne}{61.8}
\newcommand{\miouCIRNCsTwelveCoarseLOne}{0.5}
\newcommand{\dropRNCsTwelveCoarseLOne}{2.2}
\newcommand{\dropCIRNCsTwelveCoarseLOne}{0.7}
\newcommand{\retRNCsTwelveCoarseLOne}{0.966}
\newcommand{\retCIRNCsTwelveCoarseLOne}{0.011}
\newcommand{\nRNCsTwelveCoarseLTwo}{5}
\newcommand{\miouRNCsTwelveCoarseLTwo}{56.2}
\newcommand{\miouCIRNCsTwelveCoarseLTwo}{1.5}
\newcommand{\dropRNCsTwelveCoarseLTwo}{7.8}
\newcommand{\dropCIRNCsTwelveCoarseLTwo}{1.7}
\newcommand{\retRNCsTwelveCoarseLTwo}{0.878}
\newcommand{\retCIRNCsTwelveCoarseLTwo}{0.025}
\newcommand{\nRNCsTwelveOmissionLOne}{5}
\newcommand{\miouRNCsTwelveOmissionLOne}{60.3}
\newcommand{\miouCIRNCsTwelveOmissionLOne}{1.0}
\newcommand{\dropRNCsTwelveOmissionLOne}{3.8}
\newcommand{\dropCIRNCsTwelveOmissionLOne}{1.0}
\newcommand{\retRNCsTwelveOmissionLOne}{0.941}
\newcommand{\retCIRNCsTwelveOmissionLOne}{0.015}
\newcommand{\nRNCsTwelveOmissionLTwo}{5}
\newcommand{\miouRNCsTwelveOmissionLTwo}{57.7}
\newcommand{\miouCIRNCsTwelveOmissionLTwo}{0.9}
\newcommand{\dropRNCsTwelveOmissionLTwo}{6.3}
\newcommand{\dropCIRNCsTwelveOmissionLTwo}{1.5}
\newcommand{\retRNCsTwelveOmissionLTwo}{0.902}
\newcommand{\retCIRNCsTwelveOmissionLTwo}{0.023}
\newcommand{\nRNCsTwelveSTwocloudlessREAL}{5}
\newcommand{\miouRNCsTwelveSTwocloudlessREAL}{34.9}
\newcommand{\miouCIRNCsTwelveSTwocloudlessREAL}{0.2}
\newcommand{\dropRNCsTwelveSTwocloudlessREAL}{29.1}
\newcommand{\dropCIRNCsTwelveSTwocloudlessREAL}{0.9}
\newcommand{\retRNCsTwelveSTwocloudlessREAL}{0.546}
\newcommand{\retCIRNCsTwelveSTwocloudlessREAL}{0.008}
\newcommand{\nRNCsTwelveShiftLOne}{5}
\newcommand{\miouRNCsTwelveShiftLOne}{62.7}
\newcommand{\miouCIRNCsTwelveShiftLOne}{0.7}
\newcommand{\dropRNCsTwelveShiftLOne}{1.3}
\newcommand{\dropCIRNCsTwelveShiftLOne}{0.9}
\newcommand{\retRNCsTwelveShiftLOne}{0.979}
\newcommand{\retCIRNCsTwelveShiftLOne}{0.014}
\newcommand{\nRNCsTwelveShiftLTwo}{5}
\newcommand{\miouRNCsTwelveShiftLTwo}{58.7}
\newcommand{\miouCIRNCsTwelveShiftLTwo}{2.0}
\newcommand{\dropRNCsTwelveShiftLTwo}{5.3}
\newcommand{\dropCIRNCsTwelveShiftLTwo}{2.0}
\newcommand{\retRNCsTwelveShiftLTwo}{0.917}
\newcommand{\retCIRNCsTwelveShiftLTwo}{0.030}
\newcommand{\nRNDfcBoundaryLOne}{5}
\newcommand{\miouRNDfcBoundaryLOne}{39.3}
\newcommand{\miouCIRNDfcBoundaryLOne}{1.2}
\newcommand{\dropRNDfcBoundaryLOne}{\ensuremath{-}0.5}
\newcommand{\dropCIRNDfcBoundaryLOne}{2.3}
\newcommand{\retRNDfcBoundaryLOne}{1.014}
\newcommand{\retCIRNDfcBoundaryLOne}{0.061}
\newcommand{\nRNDfcBoundaryLTwo}{5}
\newcommand{\miouRNDfcBoundaryLTwo}{36.2}
\newcommand{\miouCIRNDfcBoundaryLTwo}{3.1}
\newcommand{\dropRNDfcBoundaryLTwo}{2.5}
\newcommand{\dropCIRNDfcBoundaryLTwo}{3.0}
\newcommand{\retRNDfcBoundaryLTwo}{0.935}
\newcommand{\retCIRNDfcBoundaryLTwo}{0.077}
\newcommand{\nRNDfcClean}{5}
\newcommand{\miouRNDfcClean}{38.8}
\newcommand{\miouCIRNDfcClean}{1.3}
\newcommand{\nRNDfcCleanVarTrainSubsetRealcov}{5}
\newcommand{\miouRNDfcCleanVarTrainSubsetRealcov}{39.7}
\newcommand{\miouCIRNDfcCleanVarTrainSubsetRealcov}{0.5}
\newcommand{\nRNDfcCoarseLOne}{5}
\newcommand{\miouRNDfcCoarseLOne}{39.6}
\newcommand{\miouCIRNDfcCoarseLOne}{1.3}
\newcommand{\dropRNDfcCoarseLOne}{\ensuremath{-}0.8}
\newcommand{\dropCIRNDfcCoarseLOne}{1.4}
\newcommand{\retRNDfcCoarseLOne}{1.021}
\newcommand{\retCIRNDfcCoarseLOne}{0.036}
\newcommand{\nRNDfcCoarseLTwo}{5}
\newcommand{\miouRNDfcCoarseLTwo}{37.9}
\newcommand{\miouCIRNDfcCoarseLTwo}{1.5}
\newcommand{\dropRNDfcCoarseLTwo}{0.8}
\newcommand{\dropCIRNDfcCoarseLTwo}{2.5}
\newcommand{\retRNDfcCoarseLTwo}{0.979}
\newcommand{\retCIRNDfcCoarseLTwo}{0.062}
\newcommand{\nRNDfcModisREALVarTrainSubsetRealcov}{5}
\newcommand{\miouRNDfcModisREALVarTrainSubsetRealcov}{35.2}
\newcommand{\miouCIRNDfcModisREALVarTrainSubsetRealcov}{2.0}
\newcommand{\dropRNDfcModisREALVarTrainSubsetRealcov}{4.5}
\newcommand{\dropCIRNDfcModisREALVarTrainSubsetRealcov}{1.6}
\newcommand{\retRNDfcModisREALVarTrainSubsetRealcov}{0.887}
\newcommand{\retCIRNDfcModisREALVarTrainSubsetRealcov}{0.041}
\newcommand{\nRNDfcOmissionLOne}{5}
\newcommand{\miouRNDfcOmissionLOne}{38.0}
\newcommand{\miouCIRNDfcOmissionLOne}{2.9}
\newcommand{\dropRNDfcOmissionLOne}{0.8}
\newcommand{\dropCIRNDfcOmissionLOne}{2.7}
\newcommand{\retRNDfcOmissionLOne}{0.981}
\newcommand{\retCIRNDfcOmissionLOne}{0.069}
\newcommand{\nRNDfcOmissionLTwo}{5}
\newcommand{\miouRNDfcOmissionLTwo}{37.2}
\newcommand{\miouCIRNDfcOmissionLTwo}{2.2}
\newcommand{\dropRNDfcOmissionLTwo}{1.5}
\newcommand{\dropCIRNDfcOmissionLTwo}{2.7}
\newcommand{\retRNDfcOmissionLTwo}{0.961}
\newcommand{\retCIRNDfcOmissionLTwo}{0.070}
\newcommand{\nRNDfcShiftLOne}{5}
\newcommand{\miouRNDfcShiftLOne}{39.8}
\newcommand{\miouCIRNDfcShiftLOne}{0.5}
\newcommand{\dropRNDfcShiftLOne}{\ensuremath{-}1.1}
\newcommand{\dropCIRNDfcShiftLOne}{1.5}
\newcommand{\retRNDfcShiftLOne}{1.028}
\newcommand{\retCIRNDfcShiftLOne}{0.040}
\newcommand{\nRNDfcShiftLTwo}{5}
\newcommand{\miouRNDfcShiftLTwo}{38.9}
\newcommand{\miouCIRNDfcShiftLTwo}{1.7}
\newcommand{\dropRNDfcShiftLTwo}{\ensuremath{-}0.2}
\newcommand{\dropCIRNDfcShiftLTwo}{1.6}
\newcommand{\retRNDfcShiftLTwo}{1.004}
\newcommand{\retCIRNDfcShiftLTwo}{0.042}
\newcommand{\nRNEnvaBoundaryLOne}{5}
\newcommand{\miouRNEnvaBoundaryLOne}{46.1}
\newcommand{\miouCIRNEnvaBoundaryLOne}{8.1}
\newcommand{\dropRNEnvaBoundaryLOne}{3.0}
\newcommand{\dropCIRNEnvaBoundaryLOne}{8.6}
\newcommand{\retRNEnvaBoundaryLOne}{0.942}
\newcommand{\retCIRNEnvaBoundaryLOne}{0.178}
\newcommand{\nRNEnvaBoundaryLTwo}{5}
\newcommand{\miouRNEnvaBoundaryLTwo}{31.1}
\newcommand{\miouCIRNEnvaBoundaryLTwo}{7.1}
\newcommand{\dropRNEnvaBoundaryLTwo}{18.0}
\newcommand{\dropCIRNEnvaBoundaryLTwo}{2.8}
\newcommand{\retRNEnvaBoundaryLTwo}{0.629}
\newcommand{\retCIRNEnvaBoundaryLTwo}{0.083}
\newcommand{\nRNEnvaClean}{5}
\newcommand{\miouRNEnvaClean}{49.1}
\newcommand{\miouCIRNEnvaClean}{4.9}
\newcommand{\nRNEnvaCoarseLOne}{5}
\newcommand{\miouRNEnvaCoarseLOne}{52.3}
\newcommand{\miouCIRNEnvaCoarseLOne}{4.6}
\newcommand{\dropRNEnvaCoarseLOne}{\ensuremath{-}3.2}
\newcommand{\dropCIRNEnvaCoarseLOne}{4.1}
\newcommand{\retRNEnvaCoarseLOne}{1.068}
\newcommand{\retCIRNEnvaCoarseLOne}{0.091}
\newcommand{\nRNEnvaCoarseLTwo}{5}
\newcommand{\miouRNEnvaCoarseLTwo}{46.8}
\newcommand{\miouCIRNEnvaCoarseLTwo}{8.6}
\newcommand{\dropRNEnvaCoarseLTwo}{2.3}
\newcommand{\dropCIRNEnvaCoarseLTwo}{8.4}
\newcommand{\retRNEnvaCoarseLTwo}{0.955}
\newcommand{\retCIRNEnvaCoarseLTwo}{0.176}
\newcommand{\nRNEnvaNlcdREAL}{5}
\newcommand{\miouRNEnvaNlcdREAL}{24.7}
\newcommand{\miouCIRNEnvaNlcdREAL}{3.0}
\newcommand{\dropRNEnvaNlcdREAL}{24.4}
\newcommand{\dropCIRNEnvaNlcdREAL}{7.0}
\newcommand{\retRNEnvaNlcdREAL}{0.507}
\newcommand{\retCIRNEnvaNlcdREAL}{0.100}
\newcommand{\nRNEnvaOmissionLOne}{5}
\newcommand{\miouRNEnvaOmissionLOne}{34.1}
\newcommand{\miouCIRNEnvaOmissionLOne}{6.6}
\newcommand{\dropRNEnvaOmissionLOne}{15.0}
\newcommand{\dropCIRNEnvaOmissionLOne}{10.7}
\newcommand{\retRNEnvaOmissionLOne}{0.703}
\newcommand{\retCIRNEnvaOmissionLOne}{0.181}
\newcommand{\nRNEnvaOmissionLTwo}{5}
\newcommand{\miouRNEnvaOmissionLTwo}{28.8}
\newcommand{\miouCIRNEnvaOmissionLTwo}{7.0}
\newcommand{\dropRNEnvaOmissionLTwo}{20.3}
\newcommand{\dropCIRNEnvaOmissionLTwo}{7.2}
\newcommand{\retRNEnvaOmissionLTwo}{0.588}
\newcommand{\retCIRNEnvaOmissionLTwo}{0.137}
\newcommand{\nRNEnvaShiftLOne}{5}
\newcommand{\miouRNEnvaShiftLOne}{52.5}
\newcommand{\miouCIRNEnvaShiftLOne}{2.6}
\newcommand{\dropRNEnvaShiftLOne}{\ensuremath{-}3.4}
\newcommand{\dropCIRNEnvaShiftLOne}{5.0}
\newcommand{\retRNEnvaShiftLOne}{1.074}
\newcommand{\retCIRNEnvaShiftLOne}{0.111}
\newcommand{\nRNEnvaShiftLTwo}{5}
\newcommand{\miouRNEnvaShiftLTwo}{41.4}
\newcommand{\miouCIRNEnvaShiftLTwo}{7.0}
\newcommand{\dropRNEnvaShiftLTwo}{7.7}
\newcommand{\dropCIRNEnvaShiftLTwo}{8.6}
\newcommand{\retRNEnvaShiftLTwo}{0.847}
\newcommand{\retCIRNEnvaShiftLTwo}{0.170}
\newcommand{\nRNflairBoundaryLOne}{5}
\newcommand{\miouRNflairBoundaryLOne}{42.6}
\newcommand{\miouCIRNflairBoundaryLOne}{1.7}
\newcommand{\dropRNflairBoundaryLOne}{1.9}
\newcommand{\dropCIRNflairBoundaryLOne}{1.5}
\newcommand{\retRNflairBoundaryLOne}{0.958}
\newcommand{\retCIRNflairBoundaryLOne}{0.034}
\newcommand{\nRNflairBoundaryLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouRNflairBoundaryLOneVarDecoderMaskTwoformerFull}{43.6}
\newcommand{\miouCIRNflairBoundaryLOneVarDecoderMaskTwoformerFull}{0.6}
\newcommand{\dropRNflairBoundaryLOneVarDecoderMaskTwoformerFull}{2.2}
\newcommand{\dropCIRNflairBoundaryLOneVarDecoderMaskTwoformerFull}{1.8}
\newcommand{\retRNflairBoundaryLOneVarDecoderMaskTwoformerFull}{0.953}
\newcommand{\retCIRNflairBoundaryLOneVarDecoderMaskTwoformerFull}{0.037}
\newcommand{\nRNflairBoundaryLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouRNflairBoundaryLOneVarDecoderMaskTwoformerLite}{41.8}
\newcommand{\miouCIRNflairBoundaryLOneVarDecoderMaskTwoformerLite}{3.4}
\newcommand{\dropRNflairBoundaryLOneVarDecoderMaskTwoformerLite}{2.3}
\newcommand{\dropCIRNflairBoundaryLOneVarDecoderMaskTwoformerLite}{2.7}
\newcommand{\retRNflairBoundaryLOneVarDecoderMaskTwoformerLite}{0.948}
\newcommand{\retCIRNflairBoundaryLOneVarDecoderMaskTwoformerLite}{0.062}
\newcommand{\nRNflairBoundaryLOneVarDecoderSamLite}{5}
\newcommand{\miouRNflairBoundaryLOneVarDecoderSamLite}{42.0}
\newcommand{\miouCIRNflairBoundaryLOneVarDecoderSamLite}{1.8}
\newcommand{\dropRNflairBoundaryLOneVarDecoderSamLite}{1.8}
\newcommand{\dropCIRNflairBoundaryLOneVarDecoderSamLite}{2.8}
\newcommand{\retRNflairBoundaryLOneVarDecoderSamLite}{0.961}
\newcommand{\retCIRNflairBoundaryLOneVarDecoderSamLite}{0.063}
\newcommand{\nRNflairBoundaryLOneVarDecoderSamPretrained}{5}
\newcommand{\miouRNflairBoundaryLOneVarDecoderSamPretrained}{39.2}
\newcommand{\miouCIRNflairBoundaryLOneVarDecoderSamPretrained}{4.5}
\newcommand{\dropRNflairBoundaryLOneVarDecoderSamPretrained}{1.3}
\newcommand{\dropCIRNflairBoundaryLOneVarDecoderSamPretrained}{4.7}
\newcommand{\retRNflairBoundaryLOneVarDecoderSamPretrained}{0.969}
\newcommand{\retCIRNflairBoundaryLOneVarDecoderSamPretrained}{0.114}
\newcommand{\nRNflairBoundaryLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouRNflairBoundaryLOneVarDecoderSegformerMlp}{42.9}
\newcommand{\miouCIRNflairBoundaryLOneVarDecoderSegformerMlp}{1.8}
\newcommand{\dropRNflairBoundaryLOneVarDecoderSegformerMlp}{1.7}
\newcommand{\dropCIRNflairBoundaryLOneVarDecoderSegformerMlp}{2.2}
\newcommand{\retRNflairBoundaryLOneVarDecoderSegformerMlp}{0.962}
\newcommand{\retCIRNflairBoundaryLOneVarDecoderSegformerMlp}{0.048}
\newcommand{\nRNflairBoundaryLTwo}{5}
\newcommand{\miouRNflairBoundaryLTwo}{40.8}
\newcommand{\miouCIRNflairBoundaryLTwo}{2.4}
\newcommand{\dropRNflairBoundaryLTwo}{3.7}
\newcommand{\dropCIRNflairBoundaryLTwo}{3.5}
\newcommand{\retRNflairBoundaryLTwo}{0.919}
\newcommand{\retCIRNflairBoundaryLTwo}{0.075}
\newcommand{\nRNflairBoundaryLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouRNflairBoundaryLTwoVarDecoderMaskTwoformerFull}{41.3}
\newcommand{\miouCIRNflairBoundaryLTwoVarDecoderMaskTwoformerFull}{1.4}
\newcommand{\dropRNflairBoundaryLTwoVarDecoderMaskTwoformerFull}{4.5}
\newcommand{\dropCIRNflairBoundaryLTwoVarDecoderMaskTwoformerFull}{1.9}
\newcommand{\retRNflairBoundaryLTwoVarDecoderMaskTwoformerFull}{0.903}
\newcommand{\retCIRNflairBoundaryLTwoVarDecoderMaskTwoformerFull}{0.040}
\newcommand{\nRNflairBoundaryLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouRNflairBoundaryLTwoVarDecoderMaskTwoformerLite}{39.1}
\newcommand{\miouCIRNflairBoundaryLTwoVarDecoderMaskTwoformerLite}{2.2}
\newcommand{\dropRNflairBoundaryLTwoVarDecoderMaskTwoformerLite}{4.9}
\newcommand{\dropCIRNflairBoundaryLTwoVarDecoderMaskTwoformerLite}{2.5}
\newcommand{\retRNflairBoundaryLTwoVarDecoderMaskTwoformerLite}{0.889}
\newcommand{\retCIRNflairBoundaryLTwoVarDecoderMaskTwoformerLite}{0.056}
\newcommand{\nRNflairBoundaryLTwoVarDecoderSamLite}{5}
\newcommand{\miouRNflairBoundaryLTwoVarDecoderSamLite}{41.1}
\newcommand{\miouCIRNflairBoundaryLTwoVarDecoderSamLite}{0.8}
\newcommand{\dropRNflairBoundaryLTwoVarDecoderSamLite}{2.7}
\newcommand{\dropCIRNflairBoundaryLTwoVarDecoderSamLite}{1.7}
\newcommand{\retRNflairBoundaryLTwoVarDecoderSamLite}{0.939}
\newcommand{\retCIRNflairBoundaryLTwoVarDecoderSamLite}{0.038}
\newcommand{\nRNflairBoundaryLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouRNflairBoundaryLTwoVarDecoderSamPretrained}{36.0}
\newcommand{\miouCIRNflairBoundaryLTwoVarDecoderSamPretrained}{2.8}
\newcommand{\dropRNflairBoundaryLTwoVarDecoderSamPretrained}{4.5}
\newcommand{\dropCIRNflairBoundaryLTwoVarDecoderSamPretrained}{2.1}
\newcommand{\retRNflairBoundaryLTwoVarDecoderSamPretrained}{0.890}
\newcommand{\retCIRNflairBoundaryLTwoVarDecoderSamPretrained}{0.051}
\newcommand{\nRNflairBoundaryLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouRNflairBoundaryLTwoVarDecoderSegformerMlp}{41.3}
\newcommand{\miouCIRNflairBoundaryLTwoVarDecoderSegformerMlp}{0.7}
\newcommand{\dropRNflairBoundaryLTwoVarDecoderSegformerMlp}{3.4}
\newcommand{\dropCIRNflairBoundaryLTwoVarDecoderSegformerMlp}{0.5}
\newcommand{\retRNflairBoundaryLTwoVarDecoderSegformerMlp}{0.925}
\newcommand{\retCIRNflairBoundaryLTwoVarDecoderSegformerMlp}{0.010}
\newcommand{\nRNflairBoundaryLTwoVarLossBootstrap}{5}
\newcommand{\miouRNflairBoundaryLTwoVarLossBootstrap}{40.6}
\newcommand{\miouCIRNflairBoundaryLTwoVarLossBootstrap}{1.4}
\newcommand{\dropRNflairBoundaryLTwoVarLossBootstrap}{3.7}
\newcommand{\dropCIRNflairBoundaryLTwoVarLossBootstrap}{1.9}
\newcommand{\retRNflairBoundaryLTwoVarLossBootstrap}{0.917}
\newcommand{\retCIRNflairBoundaryLTwoVarLossBootstrap}{0.042}
\newcommand{\nRNflairBoundaryLTwoVarLossGce}{5}
\newcommand{\miouRNflairBoundaryLTwoVarLossGce}{38.3}
\newcommand{\miouCIRNflairBoundaryLTwoVarLossGce}{1.0}
\newcommand{\dropRNflairBoundaryLTwoVarLossGce}{1.7}
\newcommand{\dropCIRNflairBoundaryLTwoVarLossGce}{0.9}
\newcommand{\retRNflairBoundaryLTwoVarLossGce}{0.958}
\newcommand{\retCIRNflairBoundaryLTwoVarLossGce}{0.023}
\newcommand{\nRNflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouRNflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{40.3}
\newcommand{\miouCIRNflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{2.3}
\newcommand{\dropRNflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{3.9}
\newcommand{\dropCIRNflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{3.2}
\newcommand{\retRNflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{0.912}
\newcommand{\retCIRNflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{0.069}
\newcommand{\nRNflairBoundaryLR}{5}
\newcommand{\miouRNflairBoundaryLR}{40.6}
\newcommand{\miouCIRNflairBoundaryLR}{1.7}
\newcommand{\dropRNflairBoundaryLR}{3.9}
\newcommand{\dropCIRNflairBoundaryLR}{2.1}
\newcommand{\retRNflairBoundaryLR}{0.914}
\newcommand{\retCIRNflairBoundaryLR}{0.045}
\newcommand{\nRNflairClean}{5}
\newcommand{\miouRNflairClean}{44.5}
\newcommand{\miouCIRNflairClean}{1.7}
\newcommand{\nRNflairCleanVarClassWeightedTrue}{5}
\newcommand{\miouRNflairCleanVarClassWeightedTrue}{41.2}
\newcommand{\miouCIRNflairCleanVarClassWeightedTrue}{3.0}
\newcommand{\nRNflairCleanVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouRNflairCleanVarDecoderMaskTwoformerFull}{45.8}
\newcommand{\miouCIRNflairCleanVarDecoderMaskTwoformerFull}{1.3}
\newcommand{\nRNflairCleanVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouRNflairCleanVarDecoderMaskTwoformerLite}{44.0}
\newcommand{\miouCIRNflairCleanVarDecoderMaskTwoformerLite}{1.2}
\newcommand{\nRNflairCleanVarDecoderSamLite}{5}
\newcommand{\miouRNflairCleanVarDecoderSamLite}{43.8}
\newcommand{\miouCIRNflairCleanVarDecoderSamLite}{1.5}
\newcommand{\nRNflairCleanVarDecoderSamPretrained}{5}
\newcommand{\miouRNflairCleanVarDecoderSamPretrained}{40.5}
\newcommand{\miouCIRNflairCleanVarDecoderSamPretrained}{1.6}
\newcommand{\nRNflairCleanVarDecoderSegformerMlp}{5}
\newcommand{\miouRNflairCleanVarDecoderSegformerMlp}{44.6}
\newcommand{\miouCIRNflairCleanVarDecoderSegformerMlp}{1.0}
\newcommand{\nRNflairCleanVarInitRandom}{5}
\newcommand{\miouRNflairCleanVarInitRandom}{35.5}
\newcommand{\miouCIRNflairCleanVarInitRandom}{2.9}
\newcommand{\nRNflairCleanVarInitRandomLrMultThree}{1}
\newcommand{\miouRNflairCleanVarInitRandomLrMultThree}{33.7}
\newcommand{\miouCIRNflairCleanVarInitRandomLrMultThree}{--}
\newcommand{\nRNflairCleanVarLossBootstrap}{5}
\newcommand{\miouRNflairCleanVarLossBootstrap}{44.3}
\newcommand{\miouCIRNflairCleanVarLossBootstrap}{0.7}
\newcommand{\nRNflairCleanVarLossGce}{5}
\newcommand{\miouRNflairCleanVarLossGce}{40.0}
\newcommand{\miouCIRNflairCleanVarLossGce}{0.4}
\newcommand{\nRNflairCleanVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouRNflairCleanVarLrMultZeroThreeThreeThreeThree}{44.2}
\newcommand{\miouCIRNflairCleanVarLrMultZeroThreeThreeThreeThree}{2.1}
\newcommand{\nRNflairCleanVarTrainSubsetCleanTwoFive}{5}
\newcommand{\miouRNflairCleanVarTrainSubsetCleanTwoFive}{38.9}
\newcommand{\miouCIRNflairCleanVarTrainSubsetCleanTwoFive}{2.2}
\newcommand{\nRNflairCoarseLOne}{5}
\newcommand{\miouRNflairCoarseLOne}{43.6}
\newcommand{\miouCIRNflairCoarseLOne}{1.7}
\newcommand{\dropRNflairCoarseLOne}{0.9}
\newcommand{\dropCIRNflairCoarseLOne}{2.4}
\newcommand{\retRNflairCoarseLOne}{0.981}
\newcommand{\retCIRNflairCoarseLOne}{0.052}
\newcommand{\nRNflairCoarseLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouRNflairCoarseLOneVarDecoderMaskTwoformerFull}{45.2}
\newcommand{\miouCIRNflairCoarseLOneVarDecoderMaskTwoformerFull}{1.1}
\newcommand{\dropRNflairCoarseLOneVarDecoderMaskTwoformerFull}{0.5}
\newcommand{\dropCIRNflairCoarseLOneVarDecoderMaskTwoformerFull}{2.2}
\newcommand{\retRNflairCoarseLOneVarDecoderMaskTwoformerFull}{0.989}
\newcommand{\retCIRNflairCoarseLOneVarDecoderMaskTwoformerFull}{0.048}
\newcommand{\nRNflairCoarseLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouRNflairCoarseLOneVarDecoderMaskTwoformerLite}{42.6}
\newcommand{\miouCIRNflairCoarseLOneVarDecoderMaskTwoformerLite}{1.0}
\newcommand{\dropRNflairCoarseLOneVarDecoderMaskTwoformerLite}{1.5}
\newcommand{\dropCIRNflairCoarseLOneVarDecoderMaskTwoformerLite}{1.2}
\newcommand{\retRNflairCoarseLOneVarDecoderMaskTwoformerLite}{0.967}
\newcommand{\retCIRNflairCoarseLOneVarDecoderMaskTwoformerLite}{0.027}
\newcommand{\nRNflairCoarseLOneVarDecoderSamLite}{5}
\newcommand{\miouRNflairCoarseLOneVarDecoderSamLite}{42.9}
\newcommand{\miouCIRNflairCoarseLOneVarDecoderSamLite}{1.4}
\newcommand{\dropRNflairCoarseLOneVarDecoderSamLite}{0.8}
\newcommand{\dropCIRNflairCoarseLOneVarDecoderSamLite}{2.4}
\newcommand{\retRNflairCoarseLOneVarDecoderSamLite}{0.982}
\newcommand{\retCIRNflairCoarseLOneVarDecoderSamLite}{0.053}
\newcommand{\nRNflairCoarseLOneVarDecoderSamPretrained}{5}
\newcommand{\miouRNflairCoarseLOneVarDecoderSamPretrained}{39.3}
\newcommand{\miouCIRNflairCoarseLOneVarDecoderSamPretrained}{3.3}
\newcommand{\dropRNflairCoarseLOneVarDecoderSamPretrained}{1.2}
\newcommand{\dropCIRNflairCoarseLOneVarDecoderSamPretrained}{1.9}
\newcommand{\retRNflairCoarseLOneVarDecoderSamPretrained}{0.969}
\newcommand{\retCIRNflairCoarseLOneVarDecoderSamPretrained}{0.049}
\newcommand{\nRNflairCoarseLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouRNflairCoarseLOneVarDecoderSegformerMlp}{43.3}
\newcommand{\miouCIRNflairCoarseLOneVarDecoderSegformerMlp}{0.7}
\newcommand{\dropRNflairCoarseLOneVarDecoderSegformerMlp}{1.3}
\newcommand{\dropCIRNflairCoarseLOneVarDecoderSegformerMlp}{0.7}
\newcommand{\retRNflairCoarseLOneVarDecoderSegformerMlp}{0.970}
\newcommand{\retCIRNflairCoarseLOneVarDecoderSegformerMlp}{0.016}
\newcommand{\nRNflairCoarseLTwo}{5}
\newcommand{\miouRNflairCoarseLTwo}{38.8}
\newcommand{\miouCIRNflairCoarseLTwo}{0.9}
\newcommand{\dropRNflairCoarseLTwo}{5.7}
\newcommand{\dropCIRNflairCoarseLTwo}{2.4}
\newcommand{\retRNflairCoarseLTwo}{0.873}
\newcommand{\retCIRNflairCoarseLTwo}{0.049}
\newcommand{\nRNflairCoarseLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouRNflairCoarseLTwoVarDecoderMaskTwoformerFull}{37.6}
\newcommand{\miouCIRNflairCoarseLTwoVarDecoderMaskTwoformerFull}{1.0}
\newcommand{\dropRNflairCoarseLTwoVarDecoderMaskTwoformerFull}{8.2}
\newcommand{\dropCIRNflairCoarseLTwoVarDecoderMaskTwoformerFull}{2.0}
\newcommand{\retRNflairCoarseLTwoVarDecoderMaskTwoformerFull}{0.822}
\newcommand{\retCIRNflairCoarseLTwoVarDecoderMaskTwoformerFull}{0.039}
\newcommand{\nRNflairCoarseLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouRNflairCoarseLTwoVarDecoderMaskTwoformerLite}{38.2}
\newcommand{\miouCIRNflairCoarseLTwoVarDecoderMaskTwoformerLite}{1.9}
\newcommand{\dropRNflairCoarseLTwoVarDecoderMaskTwoformerLite}{5.8}
\newcommand{\dropCIRNflairCoarseLTwoVarDecoderMaskTwoformerLite}{3.1}
\newcommand{\retRNflairCoarseLTwoVarDecoderMaskTwoformerLite}{0.869}
\newcommand{\retCIRNflairCoarseLTwoVarDecoderMaskTwoformerLite}{0.067}
\newcommand{\nRNflairCoarseLTwoVarDecoderSamLite}{5}
\newcommand{\miouRNflairCoarseLTwoVarDecoderSamLite}{39.3}
\newcommand{\miouCIRNflairCoarseLTwoVarDecoderSamLite}{1.2}
\newcommand{\dropRNflairCoarseLTwoVarDecoderSamLite}{4.5}
\newcommand{\dropCIRNflairCoarseLTwoVarDecoderSamLite}{2.4}
\newcommand{\retRNflairCoarseLTwoVarDecoderSamLite}{0.898}
\newcommand{\retCIRNflairCoarseLTwoVarDecoderSamLite}{0.052}
\newcommand{\nRNflairCoarseLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouRNflairCoarseLTwoVarDecoderSamPretrained}{34.7}
\newcommand{\miouCIRNflairCoarseLTwoVarDecoderSamPretrained}{3.6}
\newcommand{\dropRNflairCoarseLTwoVarDecoderSamPretrained}{5.8}
\newcommand{\dropCIRNflairCoarseLTwoVarDecoderSamPretrained}{3.1}
\newcommand{\retRNflairCoarseLTwoVarDecoderSamPretrained}{0.858}
\newcommand{\retCIRNflairCoarseLTwoVarDecoderSamPretrained}{0.076}
\newcommand{\nRNflairCoarseLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouRNflairCoarseLTwoVarDecoderSegformerMlp}{39.6}
\newcommand{\miouCIRNflairCoarseLTwoVarDecoderSegformerMlp}{0.3}
\newcommand{\dropRNflairCoarseLTwoVarDecoderSegformerMlp}{5.0}
\newcommand{\dropCIRNflairCoarseLTwoVarDecoderSegformerMlp}{1.0}
\newcommand{\retRNflairCoarseLTwoVarDecoderSegformerMlp}{0.888}
\newcommand{\retCIRNflairCoarseLTwoVarDecoderSegformerMlp}{0.019}
\newcommand{\nRNflairCoarseLTwoVarInitRandom}{5}
\newcommand{\miouRNflairCoarseLTwoVarInitRandom}{31.8}
\newcommand{\miouCIRNflairCoarseLTwoVarInitRandom}{1.8}
\newcommand{\dropRNflairCoarseLTwoVarInitRandom}{3.7}
\newcommand{\dropCIRNflairCoarseLTwoVarInitRandom}{3.2}
\newcommand{\retRNflairCoarseLTwoVarInitRandom}{0.899}
\newcommand{\retCIRNflairCoarseLTwoVarInitRandom}{0.090}
\newcommand{\nRNflairCoarseLTwoVarLossBootstrap}{5}
\newcommand{\miouRNflairCoarseLTwoVarLossBootstrap}{38.8}
\newcommand{\miouCIRNflairCoarseLTwoVarLossBootstrap}{1.2}
\newcommand{\dropRNflairCoarseLTwoVarLossBootstrap}{5.4}
\newcommand{\dropCIRNflairCoarseLTwoVarLossBootstrap}{1.5}
\newcommand{\retRNflairCoarseLTwoVarLossBootstrap}{0.877}
\newcommand{\retCIRNflairCoarseLTwoVarLossBootstrap}{0.034}
\newcommand{\nRNflairCoarseLTwoVarLossGce}{5}
\newcommand{\miouRNflairCoarseLTwoVarLossGce}{33.7}
\newcommand{\miouCIRNflairCoarseLTwoVarLossGce}{2.0}
\newcommand{\dropRNflairCoarseLTwoVarLossGce}{6.2}
\newcommand{\dropCIRNflairCoarseLTwoVarLossGce}{2.1}
\newcommand{\retRNflairCoarseLTwoVarLossGce}{0.844}
\newcommand{\retCIRNflairCoarseLTwoVarLossGce}{0.053}
\newcommand{\nRNflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouRNflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{38.5}
\newcommand{\miouCIRNflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{1.6}
\newcommand{\dropRNflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{5.7}
\newcommand{\dropCIRNflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.6}
\newcommand{\retRNflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.870}
\newcommand{\retCIRNflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.009}
\newcommand{\nRNflairCoarseLR}{5}
\newcommand{\miouRNflairCoarseLR}{33.6}
\newcommand{\miouCIRNflairCoarseLR}{1.5}
\newcommand{\dropRNflairCoarseLR}{10.8}
\newcommand{\dropCIRNflairCoarseLR}{2.4}
\newcommand{\retRNflairCoarseLR}{0.757}
\newcommand{\retCIRNflairCoarseLR}{0.047}
\newcommand{\nRNflairOmissionLOne}{5}
\newcommand{\miouRNflairOmissionLOne}{44.3}
\newcommand{\miouCIRNflairOmissionLOne}{0.5}
\newcommand{\dropRNflairOmissionLOne}{0.2}
\newcommand{\dropCIRNflairOmissionLOne}{1.9}
\newcommand{\retRNflairOmissionLOne}{0.997}
\newcommand{\retCIRNflairOmissionLOne}{0.043}
\newcommand{\nRNflairOmissionLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouRNflairOmissionLOneVarDecoderMaskTwoformerFull}{44.8}
\newcommand{\miouCIRNflairOmissionLOneVarDecoderMaskTwoformerFull}{1.8}
\newcommand{\dropRNflairOmissionLOneVarDecoderMaskTwoformerFull}{0.9}
\newcommand{\dropCIRNflairOmissionLOneVarDecoderMaskTwoformerFull}{1.7}
\newcommand{\retRNflairOmissionLOneVarDecoderMaskTwoformerFull}{0.980}
\newcommand{\retCIRNflairOmissionLOneVarDecoderMaskTwoformerFull}{0.037}
\newcommand{\nRNflairOmissionLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouRNflairOmissionLOneVarDecoderMaskTwoformerLite}{42.5}
\newcommand{\miouCIRNflairOmissionLOneVarDecoderMaskTwoformerLite}{0.9}
\newcommand{\dropRNflairOmissionLOneVarDecoderMaskTwoformerLite}{1.6}
\newcommand{\dropCIRNflairOmissionLOneVarDecoderMaskTwoformerLite}{1.5}
\newcommand{\retRNflairOmissionLOneVarDecoderMaskTwoformerLite}{0.965}
\newcommand{\retCIRNflairOmissionLOneVarDecoderMaskTwoformerLite}{0.033}
\newcommand{\nRNflairOmissionLOneVarDecoderSamLite}{5}
\newcommand{\miouRNflairOmissionLOneVarDecoderSamLite}{43.2}
\newcommand{\miouCIRNflairOmissionLOneVarDecoderSamLite}{1.1}
\newcommand{\dropRNflairOmissionLOneVarDecoderSamLite}{0.5}
\newcommand{\dropCIRNflairOmissionLOneVarDecoderSamLite}{2.3}
\newcommand{\retRNflairOmissionLOneVarDecoderSamLite}{0.989}
\newcommand{\retCIRNflairOmissionLOneVarDecoderSamLite}{0.052}
\newcommand{\nRNflairOmissionLOneVarDecoderSamPretrained}{5}
\newcommand{\miouRNflairOmissionLOneVarDecoderSamPretrained}{38.9}
\newcommand{\miouCIRNflairOmissionLOneVarDecoderSamPretrained}{2.8}
\newcommand{\dropRNflairOmissionLOneVarDecoderSamPretrained}{1.6}
\newcommand{\dropCIRNflairOmissionLOneVarDecoderSamPretrained}{2.4}
\newcommand{\retRNflairOmissionLOneVarDecoderSamPretrained}{0.961}
\newcommand{\retCIRNflairOmissionLOneVarDecoderSamPretrained}{0.059}
\newcommand{\nRNflairOmissionLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouRNflairOmissionLOneVarDecoderSegformerMlp}{43.7}
\newcommand{\miouCIRNflairOmissionLOneVarDecoderSegformerMlp}{0.8}
\newcommand{\dropRNflairOmissionLOneVarDecoderSegformerMlp}{0.9}
\newcommand{\dropCIRNflairOmissionLOneVarDecoderSegformerMlp}{1.2}
\newcommand{\retRNflairOmissionLOneVarDecoderSegformerMlp}{0.979}
\newcommand{\retCIRNflairOmissionLOneVarDecoderSegformerMlp}{0.027}
\newcommand{\nRNflairOmissionLTwo}{5}
\newcommand{\miouRNflairOmissionLTwo}{40.9}
\newcommand{\miouCIRNflairOmissionLTwo}{1.1}
\newcommand{\dropRNflairOmissionLTwo}{3.6}
\newcommand{\dropCIRNflairOmissionLTwo}{1.4}
\newcommand{\retRNflairOmissionLTwo}{0.920}
\newcommand{\retCIRNflairOmissionLTwo}{0.029}
\newcommand{\nRNflairOmissionLTwoVarClassWeightedTrue}{5}
\newcommand{\miouRNflairOmissionLTwoVarClassWeightedTrue}{38.7}
\newcommand{\miouCIRNflairOmissionLTwoVarClassWeightedTrue}{1.5}
\newcommand{\dropRNflairOmissionLTwoVarClassWeightedTrue}{2.5}
\newcommand{\dropCIRNflairOmissionLTwoVarClassWeightedTrue}{3.6}
\newcommand{\retRNflairOmissionLTwoVarClassWeightedTrue}{0.942}
\newcommand{\retCIRNflairOmissionLTwoVarClassWeightedTrue}{0.089}
\newcommand{\nRNflairOmissionLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouRNflairOmissionLTwoVarDecoderMaskTwoformerFull}{41.3}
\newcommand{\miouCIRNflairOmissionLTwoVarDecoderMaskTwoformerFull}{4.0}
\newcommand{\dropRNflairOmissionLTwoVarDecoderMaskTwoformerFull}{4.5}
\newcommand{\dropCIRNflairOmissionLTwoVarDecoderMaskTwoformerFull}{3.7}
\newcommand{\retRNflairOmissionLTwoVarDecoderMaskTwoformerFull}{0.902}
\newcommand{\retCIRNflairOmissionLTwoVarDecoderMaskTwoformerFull}{0.081}
\newcommand{\nRNflairOmissionLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouRNflairOmissionLTwoVarDecoderMaskTwoformerLite}{40.0}
\newcommand{\miouCIRNflairOmissionLTwoVarDecoderMaskTwoformerLite}{1.2}
\newcommand{\dropRNflairOmissionLTwoVarDecoderMaskTwoformerLite}{4.0}
\newcommand{\dropCIRNflairOmissionLTwoVarDecoderMaskTwoformerLite}{1.5}
\newcommand{\retRNflairOmissionLTwoVarDecoderMaskTwoformerLite}{0.909}
\newcommand{\retCIRNflairOmissionLTwoVarDecoderMaskTwoformerLite}{0.034}
\newcommand{\nRNflairOmissionLTwoVarDecoderSamLite}{5}
\newcommand{\miouRNflairOmissionLTwoVarDecoderSamLite}{39.5}
\newcommand{\miouCIRNflairOmissionLTwoVarDecoderSamLite}{1.8}
\newcommand{\dropRNflairOmissionLTwoVarDecoderSamLite}{4.2}
\newcommand{\dropCIRNflairOmissionLTwoVarDecoderSamLite}{2.8}
\newcommand{\retRNflairOmissionLTwoVarDecoderSamLite}{0.904}
\newcommand{\retCIRNflairOmissionLTwoVarDecoderSamLite}{0.061}
\newcommand{\nRNflairOmissionLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouRNflairOmissionLTwoVarDecoderSamPretrained}{37.2}
\newcommand{\miouCIRNflairOmissionLTwoVarDecoderSamPretrained}{1.2}
\newcommand{\dropRNflairOmissionLTwoVarDecoderSamPretrained}{3.3}
\newcommand{\dropCIRNflairOmissionLTwoVarDecoderSamPretrained}{2.2}
\newcommand{\retRNflairOmissionLTwoVarDecoderSamPretrained}{0.920}
\newcommand{\retCIRNflairOmissionLTwoVarDecoderSamPretrained}{0.053}
\newcommand{\nRNflairOmissionLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouRNflairOmissionLTwoVarDecoderSegformerMlp}{40.6}
\newcommand{\miouCIRNflairOmissionLTwoVarDecoderSegformerMlp}{2.0}
\newcommand{\dropRNflairOmissionLTwoVarDecoderSegformerMlp}{4.1}
\newcommand{\dropCIRNflairOmissionLTwoVarDecoderSegformerMlp}{2.9}
\newcommand{\retRNflairOmissionLTwoVarDecoderSegformerMlp}{0.910}
\newcommand{\retCIRNflairOmissionLTwoVarDecoderSegformerMlp}{0.063}
\newcommand{\nRNflairOmissionLTwoVarInitRandom}{5}
\newcommand{\miouRNflairOmissionLTwoVarInitRandom}{34.5}
\newcommand{\miouCIRNflairOmissionLTwoVarInitRandom}{1.3}
\newcommand{\dropRNflairOmissionLTwoVarInitRandom}{0.9}
\newcommand{\dropCIRNflairOmissionLTwoVarInitRandom}{3.7}
\newcommand{\retRNflairOmissionLTwoVarInitRandom}{0.978}
\newcommand{\retCIRNflairOmissionLTwoVarInitRandom}{0.110}
\newcommand{\nRNflairOmissionLTwoVarLossBootstrap}{5}
\newcommand{\miouRNflairOmissionLTwoVarLossBootstrap}{41.0}
\newcommand{\miouCIRNflairOmissionLTwoVarLossBootstrap}{2.6}
\newcommand{\dropRNflairOmissionLTwoVarLossBootstrap}{3.3}
\newcommand{\dropCIRNflairOmissionLTwoVarLossBootstrap}{2.8}
\newcommand{\retRNflairOmissionLTwoVarLossBootstrap}{0.926}
\newcommand{\retCIRNflairOmissionLTwoVarLossBootstrap}{0.062}
\newcommand{\nRNflairOmissionLTwoVarLossGce}{5}
\newcommand{\miouRNflairOmissionLTwoVarLossGce}{38.0}
\newcommand{\miouCIRNflairOmissionLTwoVarLossGce}{1.5}
\newcommand{\dropRNflairOmissionLTwoVarLossGce}{2.0}
\newcommand{\dropCIRNflairOmissionLTwoVarLossGce}{1.6}
\newcommand{\retRNflairOmissionLTwoVarLossGce}{0.949}
\newcommand{\retCIRNflairOmissionLTwoVarLossGce}{0.039}
\newcommand{\nRNflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouRNflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{41.7}
\newcommand{\miouCIRNflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{1.5}
\newcommand{\dropRNflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{2.5}
\newcommand{\dropCIRNflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{0.8}
\newcommand{\retRNflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{0.943}
\newcommand{\retCIRNflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{0.017}
\newcommand{\nRNflairOmissionLR}{5}
\newcommand{\miouRNflairOmissionLR}{37.4}
\newcommand{\miouCIRNflairOmissionLR}{4.0}
\newcommand{\dropRNflairOmissionLR}{7.1}
\newcommand{\dropCIRNflairOmissionLR}{4.5}
\newcommand{\retRNflairOmissionLR}{0.842}
\newcommand{\retCIRNflairOmissionLR}{0.096}
\newcommand{\nRNflairShiftLOne}{5}
\newcommand{\miouRNflairShiftLOne}{43.7}
\newcommand{\miouCIRNflairShiftLOne}{1.0}
\newcommand{\dropRNflairShiftLOne}{0.8}
\newcommand{\dropCIRNflairShiftLOne}{1.2}
\newcommand{\retRNflairShiftLOne}{0.982}
\newcommand{\retCIRNflairShiftLOne}{0.026}
\newcommand{\nRNflairShiftLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouRNflairShiftLOneVarDecoderMaskTwoformerFull}{45.2}
\newcommand{\miouCIRNflairShiftLOneVarDecoderMaskTwoformerFull}{0.5}
\newcommand{\dropRNflairShiftLOneVarDecoderMaskTwoformerFull}{0.6}
\newcommand{\dropCIRNflairShiftLOneVarDecoderMaskTwoformerFull}{0.8}
\newcommand{\retRNflairShiftLOneVarDecoderMaskTwoformerFull}{0.987}
\newcommand{\retCIRNflairShiftLOneVarDecoderMaskTwoformerFull}{0.016}
\newcommand{\nRNflairShiftLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouRNflairShiftLOneVarDecoderMaskTwoformerLite}{42.2}
\newcommand{\miouCIRNflairShiftLOneVarDecoderMaskTwoformerLite}{1.4}
\newcommand{\dropRNflairShiftLOneVarDecoderMaskTwoformerLite}{1.8}
\newcommand{\dropCIRNflairShiftLOneVarDecoderMaskTwoformerLite}{1.0}
\newcommand{\retRNflairShiftLOneVarDecoderMaskTwoformerLite}{0.958}
\newcommand{\retCIRNflairShiftLOneVarDecoderMaskTwoformerLite}{0.022}
\newcommand{\nRNflairShiftLOneVarDecoderSamLite}{5}
\newcommand{\miouRNflairShiftLOneVarDecoderSamLite}{42.9}
\newcommand{\miouCIRNflairShiftLOneVarDecoderSamLite}{0.9}
\newcommand{\dropRNflairShiftLOneVarDecoderSamLite}{0.9}
\newcommand{\dropCIRNflairShiftLOneVarDecoderSamLite}{2.1}
\newcommand{\retRNflairShiftLOneVarDecoderSamLite}{0.981}
\newcommand{\retCIRNflairShiftLOneVarDecoderSamLite}{0.046}
\newcommand{\nRNflairShiftLOneVarDecoderSamPretrained}{5}
\newcommand{\miouRNflairShiftLOneVarDecoderSamPretrained}{38.0}
\newcommand{\miouCIRNflairShiftLOneVarDecoderSamPretrained}{3.2}
\newcommand{\dropRNflairShiftLOneVarDecoderSamPretrained}{2.5}
\newcommand{\dropCIRNflairShiftLOneVarDecoderSamPretrained}{2.5}
\newcommand{\retRNflairShiftLOneVarDecoderSamPretrained}{0.937}
\newcommand{\retCIRNflairShiftLOneVarDecoderSamPretrained}{0.062}
\newcommand{\nRNflairShiftLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouRNflairShiftLOneVarDecoderSegformerMlp}{43.3}
\newcommand{\miouCIRNflairShiftLOneVarDecoderSegformerMlp}{2.4}
\newcommand{\dropRNflairShiftLOneVarDecoderSegformerMlp}{1.3}
\newcommand{\dropCIRNflairShiftLOneVarDecoderSegformerMlp}{2.7}
\newcommand{\retRNflairShiftLOneVarDecoderSegformerMlp}{0.971}
\newcommand{\retCIRNflairShiftLOneVarDecoderSegformerMlp}{0.059}
\newcommand{\nRNflairShiftLTwo}{5}
\newcommand{\miouRNflairShiftLTwo}{40.6}
\newcommand{\miouCIRNflairShiftLTwo}{1.2}
\newcommand{\dropRNflairShiftLTwo}{3.8}
\newcommand{\dropCIRNflairShiftLTwo}{0.9}
\newcommand{\retRNflairShiftLTwo}{0.914}
\newcommand{\retCIRNflairShiftLTwo}{0.018}
\newcommand{\nRNflairShiftLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouRNflairShiftLTwoVarDecoderMaskTwoformerFull}{40.3}
\newcommand{\miouCIRNflairShiftLTwoVarDecoderMaskTwoformerFull}{0.9}
\newcommand{\dropRNflairShiftLTwoVarDecoderMaskTwoformerFull}{5.5}
\newcommand{\dropCIRNflairShiftLTwoVarDecoderMaskTwoformerFull}{1.8}
\newcommand{\retRNflairShiftLTwoVarDecoderMaskTwoformerFull}{0.881}
\newcommand{\retCIRNflairShiftLTwoVarDecoderMaskTwoformerFull}{0.037}
\newcommand{\nRNflairShiftLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouRNflairShiftLTwoVarDecoderMaskTwoformerLite}{40.2}
\newcommand{\miouCIRNflairShiftLTwoVarDecoderMaskTwoformerLite}{0.7}
\newcommand{\dropRNflairShiftLTwoVarDecoderMaskTwoformerLite}{3.9}
\newcommand{\dropCIRNflairShiftLTwoVarDecoderMaskTwoformerLite}{1.8}
\newcommand{\retRNflairShiftLTwoVarDecoderMaskTwoformerLite}{0.912}
\newcommand{\retCIRNflairShiftLTwoVarDecoderMaskTwoformerLite}{0.040}
\newcommand{\nRNflairShiftLTwoVarDecoderSamLite}{5}
\newcommand{\miouRNflairShiftLTwoVarDecoderSamLite}{40.5}
\newcommand{\miouCIRNflairShiftLTwoVarDecoderSamLite}{1.8}
\newcommand{\dropRNflairShiftLTwoVarDecoderSamLite}{3.3}
\newcommand{\dropCIRNflairShiftLTwoVarDecoderSamLite}{2.2}
\newcommand{\retRNflairShiftLTwoVarDecoderSamLite}{0.926}
\newcommand{\retCIRNflairShiftLTwoVarDecoderSamLite}{0.049}
\newcommand{\nRNflairShiftLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouRNflairShiftLTwoVarDecoderSamPretrained}{37.0}
\newcommand{\miouCIRNflairShiftLTwoVarDecoderSamPretrained}{4.0}
\newcommand{\dropRNflairShiftLTwoVarDecoderSamPretrained}{3.5}
\newcommand{\dropCIRNflairShiftLTwoVarDecoderSamPretrained}{4.2}
\newcommand{\retRNflairShiftLTwoVarDecoderSamPretrained}{0.915}
\newcommand{\retCIRNflairShiftLTwoVarDecoderSamPretrained}{0.101}
\newcommand{\nRNflairShiftLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouRNflairShiftLTwoVarDecoderSegformerMlp}{40.9}
\newcommand{\miouCIRNflairShiftLTwoVarDecoderSegformerMlp}{0.6}
\newcommand{\dropRNflairShiftLTwoVarDecoderSegformerMlp}{3.7}
\newcommand{\dropCIRNflairShiftLTwoVarDecoderSegformerMlp}{0.9}
\newcommand{\retRNflairShiftLTwoVarDecoderSegformerMlp}{0.918}
\newcommand{\retCIRNflairShiftLTwoVarDecoderSegformerMlp}{0.019}
\newcommand{\nRNflairShiftLTwoVarLossBootstrap}{5}
\newcommand{\miouRNflairShiftLTwoVarLossBootstrap}{40.9}
\newcommand{\miouCIRNflairShiftLTwoVarLossBootstrap}{1.8}
\newcommand{\dropRNflairShiftLTwoVarLossBootstrap}{3.4}
\newcommand{\dropCIRNflairShiftLTwoVarLossBootstrap}{1.7}
\newcommand{\retRNflairShiftLTwoVarLossBootstrap}{0.924}
\newcommand{\retCIRNflairShiftLTwoVarLossBootstrap}{0.039}
\newcommand{\nRNflairShiftLTwoVarLossGce}{5}
\newcommand{\miouRNflairShiftLTwoVarLossGce}{35.5}
\newcommand{\miouCIRNflairShiftLTwoVarLossGce}{1.9}
\newcommand{\dropRNflairShiftLTwoVarLossGce}{4.5}
\newcommand{\dropCIRNflairShiftLTwoVarLossGce}{1.7}
\newcommand{\retRNflairShiftLTwoVarLossGce}{0.887}
\newcommand{\retCIRNflairShiftLTwoVarLossGce}{0.043}
\newcommand{\nRNflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouRNflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{41.1}
\newcommand{\miouCIRNflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{1.3}
\newcommand{\dropRNflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{3.1}
\newcommand{\dropCIRNflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{1.7}
\newcommand{\retRNflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.931}
\newcommand{\retCIRNflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.037}
\newcommand{\nRNflairShiftLR}{5}
\newcommand{\miouRNflairShiftLR}{37.2}
\newcommand{\miouCIRNflairShiftLR}{1.6}
\newcommand{\dropRNflairShiftLR}{7.3}
\newcommand{\dropCIRNflairShiftLR}{1.6}
\newcommand{\retRNflairShiftLR}{0.837}
\newcommand{\retCIRNflairShiftLR}{0.034}
\newcommand{\nRNKuroBoundaryLOne}{5}
\newcommand{\miouRNKuroBoundaryLOne}{32.4}
\newcommand{\miouCIRNKuroBoundaryLOne}{3.9}
\newcommand{\dropRNKuroBoundaryLOne}{0.1}
\newcommand{\dropCIRNKuroBoundaryLOne}{0.2}
\newcommand{\retRNKuroBoundaryLOne}{0.998}
\newcommand{\retCIRNKuroBoundaryLOne}{0.005}
\newcommand{\nRNKuroBoundaryLTwo}{5}
\newcommand{\miouRNKuroBoundaryLTwo}{31.6}
\newcommand{\miouCIRNKuroBoundaryLTwo}{1.5}
\newcommand{\dropRNKuroBoundaryLTwo}{1.0}
\newcommand{\dropCIRNKuroBoundaryLTwo}{4.7}
\newcommand{\retRNKuroBoundaryLTwo}{0.978}
\newcommand{\retCIRNKuroBoundaryLTwo}{0.127}
\newcommand{\nRNKuroCemsREALVarTrainSubsetRealcov}{5}
\newcommand{\miouRNKuroCemsREALVarTrainSubsetRealcov}{31.6}
\newcommand{\miouCIRNKuroCemsREALVarTrainSubsetRealcov}{1.7}
\newcommand{\dropRNKuroCemsREALVarTrainSubsetRealcov}{\ensuremath{-}0.1}
\newcommand{\dropCIRNKuroCemsREALVarTrainSubsetRealcov}{0.3}
\newcommand{\retRNKuroCemsREALVarTrainSubsetRealcov}{1.004}
\newcommand{\retCIRNKuroCemsREALVarTrainSubsetRealcov}{0.010}
\newcommand{\nRNKuroClean}{5}
\newcommand{\miouRNKuroClean}{32.5}
\newcommand{\miouCIRNKuroClean}{4.1}
\newcommand{\nRNKuroCleanVarTrainSubsetRealcov}{5}
\newcommand{\miouRNKuroCleanVarTrainSubsetRealcov}{31.5}
\newcommand{\miouCIRNKuroCleanVarTrainSubsetRealcov}{1.3}
\newcommand{\nRNKuroCoarseLOne}{5}
\newcommand{\miouRNKuroCoarseLOne}{32.2}
\newcommand{\miouCIRNKuroCoarseLOne}{3.3}
\newcommand{\dropRNKuroCoarseLOne}{0.3}
\newcommand{\dropCIRNKuroCoarseLOne}{5.9}
\newcommand{\retRNKuroCoarseLOne}{1.000}
\newcommand{\retCIRNKuroCoarseLOne}{0.170}
\newcommand{\nRNKuroCoarseLTwo}{5}
\newcommand{\miouRNKuroCoarseLTwo}{34.3}
\newcommand{\miouCIRNKuroCoarseLTwo}{5.6}
\newcommand{\dropRNKuroCoarseLTwo}{\ensuremath{-}1.8}
\newcommand{\dropCIRNKuroCoarseLTwo}{8.2}
\newcommand{\retRNKuroCoarseLTwo}{1.067}
\newcommand{\retCIRNKuroCoarseLTwo}{0.243}
\newcommand{\nRNKuroOmissionLOne}{5}
\newcommand{\miouRNKuroOmissionLOne}{31.0}
\newcommand{\miouCIRNKuroOmissionLOne}{0.1}
\newcommand{\dropRNKuroOmissionLOne}{1.5}
\newcommand{\dropCIRNKuroOmissionLOne}{4.1}
\newcommand{\retRNKuroOmissionLOne}{0.962}
\newcommand{\retCIRNKuroOmissionLOne}{0.108}
\newcommand{\nRNKuroOmissionLTwo}{5}
\newcommand{\miouRNKuroOmissionLTwo}{31.0}
\newcommand{\miouCIRNKuroOmissionLTwo}{0.0}
\newcommand{\dropRNKuroOmissionLTwo}{1.5}
\newcommand{\dropCIRNKuroOmissionLTwo}{4.1}
\newcommand{\retRNKuroOmissionLTwo}{0.961}
\newcommand{\retCIRNKuroOmissionLTwo}{0.107}
\newcommand{\nRNKuroShiftLOne}{5}
\newcommand{\miouRNKuroShiftLOne}{31.0}
\newcommand{\miouCIRNKuroShiftLOne}{0.0}
\newcommand{\dropRNKuroShiftLOne}{1.5}
\newcommand{\dropCIRNKuroShiftLOne}{4.1}
\newcommand{\retRNKuroShiftLOne}{0.961}
\newcommand{\retCIRNKuroShiftLOne}{0.107}
\newcommand{\nRNKuroShiftLTwo}{5}
\newcommand{\miouRNKuroShiftLTwo}{31.0}
\newcommand{\miouCIRNKuroShiftLTwo}{0.0}
\newcommand{\dropRNKuroShiftLTwo}{1.5}
\newcommand{\dropCIRNKuroShiftLTwo}{4.1}
\newcommand{\retRNKuroShiftLTwo}{0.961}
\newcommand{\retCIRNKuroShiftLTwo}{0.107}
\newcommand{\nRNOemBoundaryLOne}{5}
\newcommand{\miouRNOemBoundaryLOne}{53.3}
\newcommand{\miouCIRNOemBoundaryLOne}{0.7}
\newcommand{\dropRNOemBoundaryLOne}{2.4}
\newcommand{\dropCIRNOemBoundaryLOne}{1.2}
\newcommand{\retRNOemBoundaryLOne}{0.958}
\newcommand{\retCIRNOemBoundaryLOne}{0.022}
\newcommand{\nRNOemBoundaryLTwo}{5}
\newcommand{\miouRNOemBoundaryLTwo}{48.8}
\newcommand{\miouCIRNOemBoundaryLTwo}{1.3}
\newcommand{\dropRNOemBoundaryLTwo}{6.9}
\newcommand{\dropCIRNOemBoundaryLTwo}{1.5}
\newcommand{\retRNOemBoundaryLTwo}{0.877}
\newcommand{\retCIRNOemBoundaryLTwo}{0.026}
\newcommand{\nRNOemClean}{5}
\newcommand{\miouRNOemClean}{55.6}
\newcommand{\miouCIRNOemClean}{0.7}
\newcommand{\nRNOemCoarseLOne}{5}
\newcommand{\miouRNOemCoarseLOne}{53.7}
\newcommand{\miouCIRNOemCoarseLOne}{1.5}
\newcommand{\dropRNOemCoarseLOne}{2.0}
\newcommand{\dropCIRNOemCoarseLOne}{1.1}
\newcommand{\retRNOemCoarseLOne}{0.965}
\newcommand{\retCIRNOemCoarseLOne}{0.021}
\newcommand{\nRNOemCoarseLTwo}{5}
\newcommand{\miouRNOemCoarseLTwo}{49.7}
\newcommand{\miouCIRNOemCoarseLTwo}{1.0}
\newcommand{\dropRNOemCoarseLTwo}{6.0}
\newcommand{\dropCIRNOemCoarseLTwo}{1.6}
\newcommand{\retRNOemCoarseLTwo}{0.893}
\newcommand{\retCIRNOemCoarseLTwo}{0.027}
\newcommand{\nRNOemOmissionLOne}{5}
\newcommand{\miouRNOemOmissionLOne}{53.5}
\newcommand{\miouCIRNOemOmissionLOne}{1.1}
\newcommand{\dropRNOemOmissionLOne}{2.1}
\newcommand{\dropCIRNOemOmissionLOne}{1.5}
\newcommand{\retRNOemOmissionLOne}{0.962}
\newcommand{\retCIRNOemOmissionLOne}{0.027}
\newcommand{\nRNOemOmissionLTwo}{5}
\newcommand{\miouRNOemOmissionLTwo}{50.9}
\newcommand{\miouCIRNOemOmissionLTwo}{0.3}
\newcommand{\dropRNOemOmissionLTwo}{4.8}
\newcommand{\dropCIRNOemOmissionLTwo}{0.7}
\newcommand{\retRNOemOmissionLTwo}{0.914}
\newcommand{\retCIRNOemOmissionLTwo}{0.011}
\newcommand{\nRNOemShiftLOne}{5}
\newcommand{\miouRNOemShiftLOne}{53.6}
\newcommand{\miouCIRNOemShiftLOne}{2.8}
\newcommand{\dropRNOemShiftLOne}{2.0}
\newcommand{\dropCIRNOemShiftLOne}{3.0}
\newcommand{\retRNOemShiftLOne}{0.965}
\newcommand{\retCIRNOemShiftLOne}{0.054}
\newcommand{\nRNOemShiftLTwo}{5}
\newcommand{\miouRNOemShiftLTwo}{51.7}
\newcommand{\miouCIRNOemShiftLTwo}{0.8}
\newcommand{\dropRNOemShiftLTwo}{3.9}
\newcommand{\dropCIRNOemShiftLTwo}{1.3}
\newcommand{\retRNOemShiftLTwo}{0.930}
\newcommand{\retCIRNOemShiftLTwo}{0.023}
\newcommand{\nRNsenClean}{5}
\newcommand{\miouRNsenClean}{89.4}
\newcommand{\miouCIRNsenClean}{0.4}
\newcommand{\nRNsenOtsuLTwo}{5}
\newcommand{\miouRNsenOtsuLTwo}{73.7}
\newcommand{\miouCIRNsenOtsuLTwo}{1.5}
\newcommand{\dropRNsenOtsuLTwo}{15.7}
\newcommand{\dropCIRNsenOtsuLTwo}{1.3}
\newcommand{\retRNsenOtsuLTwo}{0.824}
\newcommand{\retCIRNsenOtsuLTwo}{0.015}
\newcommand{\nRNSnTwoBoundaryLOne}{5}
\newcommand{\miouRNSnTwoBoundaryLOne}{78.4}
\newcommand{\miouCIRNSnTwoBoundaryLOne}{2.9}
\newcommand{\dropRNSnTwoBoundaryLOne}{3.4}
\newcommand{\dropCIRNSnTwoBoundaryLOne}{3.9}
\newcommand{\retRNSnTwoBoundaryLOne}{0.959}
\newcommand{\retCIRNSnTwoBoundaryLOne}{0.046}
\newcommand{\nRNSnTwoBoundaryLTwo}{5}
\newcommand{\miouRNSnTwoBoundaryLTwo}{72.5}
\newcommand{\miouCIRNSnTwoBoundaryLTwo}{0.8}
\newcommand{\dropRNSnTwoBoundaryLTwo}{9.2}
\newcommand{\dropCIRNSnTwoBoundaryLTwo}{2.0}
\newcommand{\retRNSnTwoBoundaryLTwo}{0.887}
\newcommand{\retCIRNSnTwoBoundaryLTwo}{0.022}
\newcommand{\nRNSnTwoClean}{5}
\newcommand{\miouRNSnTwoClean}{81.7}
\newcommand{\miouCIRNSnTwoClean}{1.9}
\newcommand{\nRNSnTwoCoarseLOne}{5}
\newcommand{\miouRNSnTwoCoarseLOne}{79.2}
\newcommand{\miouCIRNSnTwoCoarseLOne}{1.3}
\newcommand{\dropRNSnTwoCoarseLOne}{2.6}
\newcommand{\dropCIRNSnTwoCoarseLOne}{2.3}
\newcommand{\retRNSnTwoCoarseLOne}{0.969}
\newcommand{\retCIRNSnTwoCoarseLOne}{0.027}
\newcommand{\nRNSnTwoCoarseLTwo}{5}
\newcommand{\miouRNSnTwoCoarseLTwo}{68.1}
\newcommand{\miouCIRNSnTwoCoarseLTwo}{0.7}
\newcommand{\dropRNSnTwoCoarseLTwo}{13.7}
\newcommand{\dropCIRNSnTwoCoarseLTwo}{2.5}
\newcommand{\retRNSnTwoCoarseLTwo}{0.833}
\newcommand{\retCIRNSnTwoCoarseLTwo}{0.027}
\newcommand{\nRNSnTwoOmissionLOne}{5}
\newcommand{\miouRNSnTwoOmissionLOne}{78.6}
\newcommand{\miouCIRNSnTwoOmissionLOne}{1.2}
\newcommand{\dropRNSnTwoOmissionLOne}{3.1}
\newcommand{\dropCIRNSnTwoOmissionLOne}{2.0}
\newcommand{\retRNSnTwoOmissionLOne}{0.962}
\newcommand{\retCIRNSnTwoOmissionLOne}{0.024}
\newcommand{\nRNSnTwoOmissionLTwo}{5}
\newcommand{\miouRNSnTwoOmissionLTwo}{58.4}
\newcommand{\miouCIRNSnTwoOmissionLTwo}{7.7}
\newcommand{\dropRNSnTwoOmissionLTwo}{23.3}
\newcommand{\dropCIRNSnTwoOmissionLTwo}{7.7}
\newcommand{\retRNSnTwoOmissionLTwo}{0.715}
\newcommand{\retCIRNSnTwoOmissionLTwo}{0.092}
\newcommand{\nRNSnTwoShiftLOne}{5}
\newcommand{\miouRNSnTwoShiftLOne}{80.3}
\newcommand{\miouCIRNSnTwoShiftLOne}{1.8}
\newcommand{\dropRNSnTwoShiftLOne}{1.4}
\newcommand{\dropCIRNSnTwoShiftLOne}{2.2}
\newcommand{\retRNSnTwoShiftLOne}{0.983}
\newcommand{\retCIRNSnTwoShiftLOne}{0.026}
\newcommand{\nRNSnTwoShiftLTwo}{5}
\newcommand{\miouRNSnTwoShiftLTwo}{72.6}
\newcommand{\miouCIRNSnTwoShiftLTwo}{0.4}
\newcommand{\dropRNSnTwoShiftLTwo}{9.1}
\newcommand{\dropCIRNSnTwoShiftLTwo}{2.1}
\newcommand{\retRNSnTwoShiftLTwo}{0.889}
\newcommand{\retCIRNSnTwoShiftLTwo}{0.023}
\newcommand{\nResnetFiveZeroSslFoureoburnBoundaryLOne}{5}
\newcommand{\miouResnetFiveZeroSslFoureoburnBoundaryLOne}{85.7}
\newcommand{\miouCIResnetFiveZeroSslFoureoburnBoundaryLOne}{1.1}
\newcommand{\dropResnetFiveZeroSslFoureoburnBoundaryLOne}{2.5}
\newcommand{\dropCIResnetFiveZeroSslFoureoburnBoundaryLOne}{1.5}
\newcommand{\retResnetFiveZeroSslFoureoburnBoundaryLOne}{0.971}
\newcommand{\retCIResnetFiveZeroSslFoureoburnBoundaryLOne}{0.017}
\newcommand{\nResnetFiveZeroSslFoureoburnBoundaryLTwo}{5}
\newcommand{\miouResnetFiveZeroSslFoureoburnBoundaryLTwo}{77.0}
\newcommand{\miouCIResnetFiveZeroSslFoureoburnBoundaryLTwo}{1.8}
\newcommand{\dropResnetFiveZeroSslFoureoburnBoundaryLTwo}{11.2}
\newcommand{\dropCIResnetFiveZeroSslFoureoburnBoundaryLTwo}{1.9}
\newcommand{\retResnetFiveZeroSslFoureoburnBoundaryLTwo}{0.873}
\newcommand{\retCIResnetFiveZeroSslFoureoburnBoundaryLTwo}{0.021}
\newcommand{\nResnetFiveZeroSslFoureoburnClean}{5}
\newcommand{\miouResnetFiveZeroSslFoureoburnClean}{88.2}
\newcommand{\miouCIResnetFiveZeroSslFoureoburnClean}{0.8}
\newcommand{\nResnetFiveZeroSslFoureoburnCleanVarTrainSubsetCleanTwoFive}{5}
\newcommand{\miouResnetFiveZeroSslFoureoburnCleanVarTrainSubsetCleanTwoFive}{87.3}
\newcommand{\miouCIResnetFiveZeroSslFoureoburnCleanVarTrainSubsetCleanTwoFive}{1.2}
\newcommand{\nResnetFiveZeroSslFoureoburnCoarseLOne}{5}
\newcommand{\miouResnetFiveZeroSslFoureoburnCoarseLOne}{83.8}
\newcommand{\miouCIResnetFiveZeroSslFoureoburnCoarseLOne}{1.9}
\newcommand{\dropResnetFiveZeroSslFoureoburnCoarseLOne}{4.4}
\newcommand{\dropCIResnetFiveZeroSslFoureoburnCoarseLOne}{2.0}
\newcommand{\retResnetFiveZeroSslFoureoburnCoarseLOne}{0.950}
\newcommand{\retCIResnetFiveZeroSslFoureoburnCoarseLOne}{0.022}
\newcommand{\nResnetFiveZeroSslFoureoburnCoarseLTwo}{5}
\newcommand{\miouResnetFiveZeroSslFoureoburnCoarseLTwo}{70.8}
\newcommand{\miouCIResnetFiveZeroSslFoureoburnCoarseLTwo}{3.8}
\newcommand{\dropResnetFiveZeroSslFoureoburnCoarseLTwo}{17.4}
\newcommand{\dropCIResnetFiveZeroSslFoureoburnCoarseLTwo}{3.9}
\newcommand{\retResnetFiveZeroSslFoureoburnCoarseLTwo}{0.803}
\newcommand{\retCIResnetFiveZeroSslFoureoburnCoarseLTwo}{0.044}
\newcommand{\nResnetFiveZeroSslFoureoburnOmissionLOne}{5}
\newcommand{\miouResnetFiveZeroSslFoureoburnOmissionLOne}{85.7}
\newcommand{\miouCIResnetFiveZeroSslFoureoburnOmissionLOne}{2.1}
\newcommand{\dropResnetFiveZeroSslFoureoburnOmissionLOne}{2.5}
\newcommand{\dropCIResnetFiveZeroSslFoureoburnOmissionLOne}{1.7}
\newcommand{\retResnetFiveZeroSslFoureoburnOmissionLOne}{0.971}
\newcommand{\retCIResnetFiveZeroSslFoureoburnOmissionLOne}{0.019}
\newcommand{\nResnetFiveZeroSslFoureoburnOmissionLTwo}{5}
\newcommand{\miouResnetFiveZeroSslFoureoburnOmissionLTwo}{60.5}
\newcommand{\miouCIResnetFiveZeroSslFoureoburnOmissionLTwo}{14.1}
\newcommand{\dropResnetFiveZeroSslFoureoburnOmissionLTwo}{27.6}
\newcommand{\dropCIResnetFiveZeroSslFoureoburnOmissionLTwo}{13.5}
\newcommand{\retResnetFiveZeroSslFoureoburnOmissionLTwo}{0.686}
\newcommand{\retCIResnetFiveZeroSslFoureoburnOmissionLTwo}{0.154}
\newcommand{\nResnetFiveZeroSslFoureoburnShiftLOne}{5}
\newcommand{\miouResnetFiveZeroSslFoureoburnShiftLOne}{86.0}
\newcommand{\miouCIResnetFiveZeroSslFoureoburnShiftLOne}{0.5}
\newcommand{\dropResnetFiveZeroSslFoureoburnShiftLOne}{2.2}
\newcommand{\dropCIResnetFiveZeroSslFoureoburnShiftLOne}{0.6}
\newcommand{\retResnetFiveZeroSslFoureoburnShiftLOne}{0.975}
\newcommand{\retCIResnetFiveZeroSslFoureoburnShiftLOne}{0.007}
\newcommand{\nResnetFiveZeroSslFoureoburnShiftLTwo}{5}
\newcommand{\miouResnetFiveZeroSslFoureoburnShiftLTwo}{76.7}
\newcommand{\miouCIResnetFiveZeroSslFoureoburnShiftLTwo}{1.1}
\newcommand{\dropResnetFiveZeroSslFoureoburnShiftLTwo}{11.4}
\newcommand{\dropCIResnetFiveZeroSslFoureoburnShiftLTwo}{1.2}
\newcommand{\retResnetFiveZeroSslFoureoburnShiftLTwo}{0.870}
\newcommand{\retCIResnetFiveZeroSslFoureoburnShiftLTwo}{0.014}
\newcommand{\nResnetFiveZeroSslFoureoflairBoundaryLOne}{5}
\newcommand{\miouResnetFiveZeroSslFoureoflairBoundaryLOne}{40.4}
\newcommand{\miouCIResnetFiveZeroSslFoureoflairBoundaryLOne}{0.8}
\newcommand{\dropResnetFiveZeroSslFoureoflairBoundaryLOne}{2.1}
\newcommand{\dropCIResnetFiveZeroSslFoureoflairBoundaryLOne}{1.2}
\newcommand{\retResnetFiveZeroSslFoureoflairBoundaryLOne}{0.950}
\newcommand{\retCIResnetFiveZeroSslFoureoflairBoundaryLOne}{0.026}
\newcommand{\nResnetFiveZeroSslFoureoflairBoundaryLTwo}{5}
\newcommand{\miouResnetFiveZeroSslFoureoflairBoundaryLTwo}{39.0}
\newcommand{\miouCIResnetFiveZeroSslFoureoflairBoundaryLTwo}{0.6}
\newcommand{\dropResnetFiveZeroSslFoureoflairBoundaryLTwo}{3.6}
\newcommand{\dropCIResnetFiveZeroSslFoureoflairBoundaryLTwo}{1.3}
\newcommand{\retResnetFiveZeroSslFoureoflairBoundaryLTwo}{0.917}
\newcommand{\retCIResnetFiveZeroSslFoureoflairBoundaryLTwo}{0.028}
\newcommand{\nResnetFiveZeroSslFoureoflairClean}{5}
\newcommand{\miouResnetFiveZeroSslFoureoflairClean}{42.5}
\newcommand{\miouCIResnetFiveZeroSslFoureoflairClean}{1.2}
\newcommand{\nResnetFiveZeroSslFoureoflairCleanVarTrainSubsetCleanTwoFive}{5}
\newcommand{\miouResnetFiveZeroSslFoureoflairCleanVarTrainSubsetCleanTwoFive}{36.8}
\newcommand{\miouCIResnetFiveZeroSslFoureoflairCleanVarTrainSubsetCleanTwoFive}{2.0}
\newcommand{\nResnetFiveZeroSslFoureoflairCoarseLOne}{5}
\newcommand{\miouResnetFiveZeroSslFoureoflairCoarseLOne}{40.9}
\newcommand{\miouCIResnetFiveZeroSslFoureoflairCoarseLOne}{1.3}
\newcommand{\dropResnetFiveZeroSslFoureoflairCoarseLOne}{1.6}
\newcommand{\dropCIResnetFiveZeroSslFoureoflairCoarseLOne}{1.8}
\newcommand{\retResnetFiveZeroSslFoureoflairCoarseLOne}{0.962}
\newcommand{\retCIResnetFiveZeroSslFoureoflairCoarseLOne}{0.041}
\newcommand{\nResnetFiveZeroSslFoureoflairCoarseLTwo}{5}
\newcommand{\miouResnetFiveZeroSslFoureoflairCoarseLTwo}{36.8}
\newcommand{\miouCIResnetFiveZeroSslFoureoflairCoarseLTwo}{1.3}
\newcommand{\dropResnetFiveZeroSslFoureoflairCoarseLTwo}{5.8}
\newcommand{\dropCIResnetFiveZeroSslFoureoflairCoarseLTwo}{2.2}
\newcommand{\retResnetFiveZeroSslFoureoflairCoarseLTwo}{0.865}
\newcommand{\retCIResnetFiveZeroSslFoureoflairCoarseLTwo}{0.049}
\newcommand{\nResnetFiveZeroSslFoureoflairOmissionLOne}{5}
\newcommand{\miouResnetFiveZeroSslFoureoflairOmissionLOne}{40.8}
\newcommand{\miouCIResnetFiveZeroSslFoureoflairOmissionLOne}{0.9}
\newcommand{\dropResnetFiveZeroSslFoureoflairOmissionLOne}{1.7}
\newcommand{\dropCIResnetFiveZeroSslFoureoflairOmissionLOne}{1.2}
\newcommand{\retResnetFiveZeroSslFoureoflairOmissionLOne}{0.960}
\newcommand{\retCIResnetFiveZeroSslFoureoflairOmissionLOne}{0.028}
\newcommand{\nResnetFiveZeroSslFoureoflairOmissionLTwo}{5}
\newcommand{\miouResnetFiveZeroSslFoureoflairOmissionLTwo}{38.8}
\newcommand{\miouCIResnetFiveZeroSslFoureoflairOmissionLTwo}{1.0}
\newcommand{\dropResnetFiveZeroSslFoureoflairOmissionLTwo}{3.7}
\newcommand{\dropCIResnetFiveZeroSslFoureoflairOmissionLTwo}{2.0}
\newcommand{\retResnetFiveZeroSslFoureoflairOmissionLTwo}{0.912}
\newcommand{\retCIResnetFiveZeroSslFoureoflairOmissionLTwo}{0.045}
\newcommand{\nResnetFiveZeroSslFoureoflairShiftLOne}{5}
\newcommand{\miouResnetFiveZeroSslFoureoflairShiftLOne}{41.7}
\newcommand{\miouCIResnetFiveZeroSslFoureoflairShiftLOne}{0.5}
\newcommand{\dropResnetFiveZeroSslFoureoflairShiftLOne}{0.8}
\newcommand{\dropCIResnetFiveZeroSslFoureoflairShiftLOne}{1.1}
\newcommand{\retResnetFiveZeroSslFoureoflairShiftLOne}{0.981}
\newcommand{\retCIResnetFiveZeroSslFoureoflairShiftLOne}{0.026}
\newcommand{\nResnetFiveZeroSslFoureoflairShiftLTwo}{5}
\newcommand{\miouResnetFiveZeroSslFoureoflairShiftLTwo}{39.0}
\newcommand{\miouCIResnetFiveZeroSslFoureoflairShiftLTwo}{0.7}
\newcommand{\dropResnetFiveZeroSslFoureoflairShiftLTwo}{3.5}
\newcommand{\dropCIResnetFiveZeroSslFoureoflairShiftLTwo}{1.2}
\newcommand{\retResnetFiveZeroSslFoureoflairShiftLTwo}{0.917}
\newcommand{\retCIResnetFiveZeroSslFoureoflairShiftLTwo}{0.026}
\newcommand{\nTMburnBoundaryLOne}{5}
\newcommand{\miouTMburnBoundaryLOne}{83.9}
\newcommand{\miouCITMburnBoundaryLOne}{1.2}
\newcommand{\dropTMburnBoundaryLOne}{2.2}
\newcommand{\dropCITMburnBoundaryLOne}{1.6}
\newcommand{\retTMburnBoundaryLOne}{0.974}
\newcommand{\retCITMburnBoundaryLOne}{0.018}
\newcommand{\nTMburnBoundaryLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouTMburnBoundaryLOneVarDecoderMaskTwoformerFull}{85.2}
\newcommand{\miouCITMburnBoundaryLOneVarDecoderMaskTwoformerFull}{0.5}
\newcommand{\dropTMburnBoundaryLOneVarDecoderMaskTwoformerFull}{2.2}
\newcommand{\dropCITMburnBoundaryLOneVarDecoderMaskTwoformerFull}{2.2}
\newcommand{\retTMburnBoundaryLOneVarDecoderMaskTwoformerFull}{0.975}
\newcommand{\retCITMburnBoundaryLOneVarDecoderMaskTwoformerFull}{0.024}
\newcommand{\nTMburnBoundaryLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouTMburnBoundaryLOneVarDecoderMaskTwoformerLite}{84.6}
\newcommand{\miouCITMburnBoundaryLOneVarDecoderMaskTwoformerLite}{0.8}
\newcommand{\dropTMburnBoundaryLOneVarDecoderMaskTwoformerLite}{3.6}
\newcommand{\dropCITMburnBoundaryLOneVarDecoderMaskTwoformerLite}{1.5}
\newcommand{\retTMburnBoundaryLOneVarDecoderMaskTwoformerLite}{0.960}
\newcommand{\retCITMburnBoundaryLOneVarDecoderMaskTwoformerLite}{0.017}
\newcommand{\nTMburnBoundaryLOneVarDecoderSamLite}{5}
\newcommand{\miouTMburnBoundaryLOneVarDecoderSamLite}{84.6}
\newcommand{\miouCITMburnBoundaryLOneVarDecoderSamLite}{1.3}
\newcommand{\dropTMburnBoundaryLOneVarDecoderSamLite}{4.1}
\newcommand{\dropCITMburnBoundaryLOneVarDecoderSamLite}{2.1}
\newcommand{\retTMburnBoundaryLOneVarDecoderSamLite}{0.954}
\newcommand{\retCITMburnBoundaryLOneVarDecoderSamLite}{0.023}
\newcommand{\nTMburnBoundaryLOneVarDecoderSamPretrained}{5}
\newcommand{\miouTMburnBoundaryLOneVarDecoderSamPretrained}{83.6}
\newcommand{\miouCITMburnBoundaryLOneVarDecoderSamPretrained}{0.7}
\newcommand{\dropTMburnBoundaryLOneVarDecoderSamPretrained}{4.2}
\newcommand{\dropCITMburnBoundaryLOneVarDecoderSamPretrained}{2.1}
\newcommand{\retTMburnBoundaryLOneVarDecoderSamPretrained}{0.952}
\newcommand{\retCITMburnBoundaryLOneVarDecoderSamPretrained}{0.023}
\newcommand{\nTMburnBoundaryLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouTMburnBoundaryLOneVarDecoderSegformerMlp}{84.6}
\newcommand{\miouCITMburnBoundaryLOneVarDecoderSegformerMlp}{1.4}
\newcommand{\dropTMburnBoundaryLOneVarDecoderSegformerMlp}{2.8}
\newcommand{\dropCITMburnBoundaryLOneVarDecoderSegformerMlp}{2.5}
\newcommand{\retTMburnBoundaryLOneVarDecoderSegformerMlp}{0.968}
\newcommand{\retCITMburnBoundaryLOneVarDecoderSegformerMlp}{0.028}
\newcommand{\nTMburnBoundaryLTwo}{8}
\newcommand{\miouTMburnBoundaryLTwo}{74.5}
\newcommand{\miouCITMburnBoundaryLTwo}{1.5}
\newcommand{\dropTMburnBoundaryLTwo}{11.9}
\newcommand{\dropCITMburnBoundaryLTwo}{2.1}
\newcommand{\retTMburnBoundaryLTwo}{0.863}
\newcommand{\retCITMburnBoundaryLTwo}{0.023}
\newcommand{\nTMburnBoundaryLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouTMburnBoundaryLTwoVarDecoderMaskTwoformerFull}{73.5}
\newcommand{\miouCITMburnBoundaryLTwoVarDecoderMaskTwoformerFull}{2.4}
\newcommand{\dropTMburnBoundaryLTwoVarDecoderMaskTwoformerFull}{13.9}
\newcommand{\dropCITMburnBoundaryLTwoVarDecoderMaskTwoformerFull}{3.8}
\newcommand{\retTMburnBoundaryLTwoVarDecoderMaskTwoformerFull}{0.842}
\newcommand{\retCITMburnBoundaryLTwoVarDecoderMaskTwoformerFull}{0.040}
\newcommand{\nTMburnBoundaryLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouTMburnBoundaryLTwoVarDecoderMaskTwoformerLite}{76.4}
\newcommand{\miouCITMburnBoundaryLTwoVarDecoderMaskTwoformerLite}{4.5}
\newcommand{\dropTMburnBoundaryLTwoVarDecoderMaskTwoformerLite}{11.8}
\newcommand{\dropCITMburnBoundaryLTwoVarDecoderMaskTwoformerLite}{5.1}
\newcommand{\retTMburnBoundaryLTwoVarDecoderMaskTwoformerLite}{0.866}
\newcommand{\retCITMburnBoundaryLTwoVarDecoderMaskTwoformerLite}{0.057}
\newcommand{\nTMburnBoundaryLTwoVarDecoderSamLite}{5}
\newcommand{\miouTMburnBoundaryLTwoVarDecoderSamLite}{77.5}
\newcommand{\miouCITMburnBoundaryLTwoVarDecoderSamLite}{1.5}
\newcommand{\dropTMburnBoundaryLTwoVarDecoderSamLite}{11.1}
\newcommand{\dropCITMburnBoundaryLTwoVarDecoderSamLite}{2.1}
\newcommand{\retTMburnBoundaryLTwoVarDecoderSamLite}{0.875}
\newcommand{\retCITMburnBoundaryLTwoVarDecoderSamLite}{0.023}
\newcommand{\nTMburnBoundaryLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouTMburnBoundaryLTwoVarDecoderSamPretrained}{77.5}
\newcommand{\miouCITMburnBoundaryLTwoVarDecoderSamPretrained}{3.4}
\newcommand{\dropTMburnBoundaryLTwoVarDecoderSamPretrained}{10.3}
\newcommand{\dropCITMburnBoundaryLTwoVarDecoderSamPretrained}{4.5}
\newcommand{\retTMburnBoundaryLTwoVarDecoderSamPretrained}{0.883}
\newcommand{\retCITMburnBoundaryLTwoVarDecoderSamPretrained}{0.050}
\newcommand{\nTMburnBoundaryLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouTMburnBoundaryLTwoVarDecoderSegformerMlp}{74.7}
\newcommand{\miouCITMburnBoundaryLTwoVarDecoderSegformerMlp}{3.0}
\newcommand{\dropTMburnBoundaryLTwoVarDecoderSegformerMlp}{12.7}
\newcommand{\dropCITMburnBoundaryLTwoVarDecoderSegformerMlp}{3.7}
\newcommand{\retTMburnBoundaryLTwoVarDecoderSegformerMlp}{0.854}
\newcommand{\retCITMburnBoundaryLTwoVarDecoderSegformerMlp}{0.041}
\newcommand{\nTMburnBoundaryLTwoVarLossBootstrap}{5}
\newcommand{\miouTMburnBoundaryLTwoVarLossBootstrap}{74.2}
\newcommand{\miouCITMburnBoundaryLTwoVarLossBootstrap}{2.1}
\newcommand{\dropTMburnBoundaryLTwoVarLossBootstrap}{12.1}
\newcommand{\dropCITMburnBoundaryLTwoVarLossBootstrap}{3.5}
\newcommand{\retTMburnBoundaryLTwoVarLossBootstrap}{0.860}
\newcommand{\retCITMburnBoundaryLTwoVarLossBootstrap}{0.038}
\newcommand{\nTMburnBoundaryLTwoVarLossGce}{5}
\newcommand{\miouTMburnBoundaryLTwoVarLossGce}{73.5}
\newcommand{\miouCITMburnBoundaryLTwoVarLossGce}{1.6}
\newcommand{\dropTMburnBoundaryLTwoVarLossGce}{13.7}
\newcommand{\dropCITMburnBoundaryLTwoVarLossGce}{1.3}
\newcommand{\retTMburnBoundaryLTwoVarLossGce}{0.843}
\newcommand{\retCITMburnBoundaryLTwoVarLossGce}{0.015}
\newcommand{\nTMburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouTMburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{74.8}
\newcommand{\miouCITMburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{3.2}
\newcommand{\dropTMburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{10.4}
\newcommand{\dropCITMburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{3.0}
\newcommand{\retTMburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{0.878}
\newcommand{\retCITMburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{0.034}
\newcommand{\nTMburnBoundaryLR}{5}
\newcommand{\miouTMburnBoundaryLR}{66.7}
\newcommand{\miouCITMburnBoundaryLR}{3.2}
\newcommand{\dropTMburnBoundaryLR}{19.5}
\newcommand{\dropCITMburnBoundaryLR}{4.2}
\newcommand{\retTMburnBoundaryLR}{0.774}
\newcommand{\retCITMburnBoundaryLR}{0.046}
\newcommand{\nTMburnClean}{8}
\newcommand{\miouTMburnClean}{86.3}
\newcommand{\miouCITMburnClean}{1.0}
\newcommand{\nTMburnCleanVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouTMburnCleanVarDecoderMaskTwoformerFull}{87.4}
\newcommand{\miouCITMburnCleanVarDecoderMaskTwoformerFull}{1.9}
\newcommand{\nTMburnCleanVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouTMburnCleanVarDecoderMaskTwoformerLite}{88.2}
\newcommand{\miouCITMburnCleanVarDecoderMaskTwoformerLite}{1.1}
\newcommand{\nTMburnCleanVarDecoderSamLite}{5}
\newcommand{\miouTMburnCleanVarDecoderSamLite}{88.7}
\newcommand{\miouCITMburnCleanVarDecoderSamLite}{1.0}
\newcommand{\nTMburnCleanVarDecoderSamPretrained}{5}
\newcommand{\miouTMburnCleanVarDecoderSamPretrained}{87.8}
\newcommand{\miouCITMburnCleanVarDecoderSamPretrained}{1.6}
\newcommand{\nTMburnCleanVarDecoderSegformerMlp}{5}
\newcommand{\miouTMburnCleanVarDecoderSegformerMlp}{87.4}
\newcommand{\miouCITMburnCleanVarDecoderSegformerMlp}{1.3}
\newcommand{\nTMburnCleanVarFrozenEncoderTrue}{5}
\newcommand{\miouTMburnCleanVarFrozenEncoderTrue}{81.6}
\newcommand{\miouCITMburnCleanVarFrozenEncoderTrue}{1.5}
\newcommand{\nTMburnCleanVarLossBootstrap}{5}
\newcommand{\miouTMburnCleanVarLossBootstrap}{86.3}
\newcommand{\miouCITMburnCleanVarLossBootstrap}{1.9}
\newcommand{\nTMburnCleanVarLossGce}{5}
\newcommand{\miouTMburnCleanVarLossGce}{87.2}
\newcommand{\miouCITMburnCleanVarLossGce}{0.7}
\newcommand{\nTMburnCleanVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouTMburnCleanVarLrMultZeroThreeThreeThreeThree}{85.1}
\newcommand{\miouCITMburnCleanVarLrMultZeroThreeThreeThreeThree}{3.2}
\newcommand{\nTMburnCleanVarTrainSubsetCleanTwoFive}{5}
\newcommand{\miouTMburnCleanVarTrainSubsetCleanTwoFive}{82.0}
\newcommand{\miouCITMburnCleanVarTrainSubsetCleanTwoFive}{2.2}
\newcommand{\nTMburnCoarseLOne}{5}
\newcommand{\miouTMburnCoarseLOne}{82.0}
\newcommand{\miouCITMburnCoarseLOne}{1.9}
\newcommand{\dropTMburnCoarseLOne}{4.2}
\newcommand{\dropCITMburnCoarseLOne}{2.7}
\newcommand{\retTMburnCoarseLOne}{0.952}
\newcommand{\retCITMburnCoarseLOne}{0.031}
\newcommand{\nTMburnCoarseLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouTMburnCoarseLOneVarDecoderMaskTwoformerFull}{84.8}
\newcommand{\miouCITMburnCoarseLOneVarDecoderMaskTwoformerFull}{0.9}
\newcommand{\dropTMburnCoarseLOneVarDecoderMaskTwoformerFull}{2.5}
\newcommand{\dropCITMburnCoarseLOneVarDecoderMaskTwoformerFull}{2.6}
\newcommand{\retTMburnCoarseLOneVarDecoderMaskTwoformerFull}{0.971}
\newcommand{\retCITMburnCoarseLOneVarDecoderMaskTwoformerFull}{0.029}
\newcommand{\nTMburnCoarseLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouTMburnCoarseLOneVarDecoderMaskTwoformerLite}{84.6}
\newcommand{\miouCITMburnCoarseLOneVarDecoderMaskTwoformerLite}{1.7}
\newcommand{\dropTMburnCoarseLOneVarDecoderMaskTwoformerLite}{3.6}
\newcommand{\dropCITMburnCoarseLOneVarDecoderMaskTwoformerLite}{1.9}
\newcommand{\retTMburnCoarseLOneVarDecoderMaskTwoformerLite}{0.959}
\newcommand{\retCITMburnCoarseLOneVarDecoderMaskTwoformerLite}{0.021}
\newcommand{\nTMburnCoarseLOneVarDecoderSamLite}{5}
\newcommand{\miouTMburnCoarseLOneVarDecoderSamLite}{84.2}
\newcommand{\miouCITMburnCoarseLOneVarDecoderSamLite}{0.7}
\newcommand{\dropTMburnCoarseLOneVarDecoderSamLite}{4.5}
\newcommand{\dropCITMburnCoarseLOneVarDecoderSamLite}{0.9}
\newcommand{\retTMburnCoarseLOneVarDecoderSamLite}{0.950}
\newcommand{\retCITMburnCoarseLOneVarDecoderSamLite}{0.010}
\newcommand{\nTMburnCoarseLOneVarDecoderSamPretrained}{5}
\newcommand{\miouTMburnCoarseLOneVarDecoderSamPretrained}{83.5}
\newcommand{\miouCITMburnCoarseLOneVarDecoderSamPretrained}{1.5}
\newcommand{\dropTMburnCoarseLOneVarDecoderSamPretrained}{4.3}
\newcommand{\dropCITMburnCoarseLOneVarDecoderSamPretrained}{2.1}
\newcommand{\retTMburnCoarseLOneVarDecoderSamPretrained}{0.951}
\newcommand{\retCITMburnCoarseLOneVarDecoderSamPretrained}{0.023}
\newcommand{\nTMburnCoarseLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouTMburnCoarseLOneVarDecoderSegformerMlp}{83.7}
\newcommand{\miouCITMburnCoarseLOneVarDecoderSegformerMlp}{1.1}
\newcommand{\dropTMburnCoarseLOneVarDecoderSegformerMlp}{3.7}
\newcommand{\dropCITMburnCoarseLOneVarDecoderSegformerMlp}{1.3}
\newcommand{\retTMburnCoarseLOneVarDecoderSegformerMlp}{0.958}
\newcommand{\retCITMburnCoarseLOneVarDecoderSegformerMlp}{0.014}
\newcommand{\nTMburnCoarseLTwo}{8}
\newcommand{\miouTMburnCoarseLTwo}{68.5}
\newcommand{\miouCITMburnCoarseLTwo}{2.6}
\newcommand{\dropTMburnCoarseLTwo}{17.9}
\newcommand{\dropCITMburnCoarseLTwo}{2.9}
\newcommand{\retTMburnCoarseLTwo}{0.793}
\newcommand{\retCITMburnCoarseLTwo}{0.033}
\newcommand{\nTMburnCoarseLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouTMburnCoarseLTwoVarDecoderMaskTwoformerFull}{69.8}
\newcommand{\miouCITMburnCoarseLTwoVarDecoderMaskTwoformerFull}{3.0}
\newcommand{\dropTMburnCoarseLTwoVarDecoderMaskTwoformerFull}{17.6}
\newcommand{\dropCITMburnCoarseLTwoVarDecoderMaskTwoformerFull}{2.6}
\newcommand{\retTMburnCoarseLTwoVarDecoderMaskTwoformerFull}{0.799}
\newcommand{\retCITMburnCoarseLTwoVarDecoderMaskTwoformerFull}{0.029}
\newcommand{\nTMburnCoarseLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouTMburnCoarseLTwoVarDecoderMaskTwoformerLite}{67.0}
\newcommand{\miouCITMburnCoarseLTwoVarDecoderMaskTwoformerLite}{8.2}
\newcommand{\dropTMburnCoarseLTwoVarDecoderMaskTwoformerLite}{21.2}
\newcommand{\dropCITMburnCoarseLTwoVarDecoderMaskTwoformerLite}{7.5}
\newcommand{\retTMburnCoarseLTwoVarDecoderMaskTwoformerLite}{0.760}
\newcommand{\retCITMburnCoarseLTwoVarDecoderMaskTwoformerLite}{0.087}
\newcommand{\nTMburnCoarseLTwoVarDecoderSamLite}{5}
\newcommand{\miouTMburnCoarseLTwoVarDecoderSamLite}{69.2}
\newcommand{\miouCITMburnCoarseLTwoVarDecoderSamLite}{1.9}
\newcommand{\dropTMburnCoarseLTwoVarDecoderSamLite}{19.4}
\newcommand{\dropCITMburnCoarseLTwoVarDecoderSamLite}{2.5}
\newcommand{\retTMburnCoarseLTwoVarDecoderSamLite}{0.781}
\newcommand{\retCITMburnCoarseLTwoVarDecoderSamLite}{0.026}
\newcommand{\nTMburnCoarseLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouTMburnCoarseLTwoVarDecoderSamPretrained}{69.0}
\newcommand{\miouCITMburnCoarseLTwoVarDecoderSamPretrained}{4.1}
\newcommand{\dropTMburnCoarseLTwoVarDecoderSamPretrained}{18.8}
\newcommand{\dropCITMburnCoarseLTwoVarDecoderSamPretrained}{5.2}
\newcommand{\retTMburnCoarseLTwoVarDecoderSamPretrained}{0.786}
\newcommand{\retCITMburnCoarseLTwoVarDecoderSamPretrained}{0.055}
\newcommand{\nTMburnCoarseLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouTMburnCoarseLTwoVarDecoderSegformerMlp}{68.2}
\newcommand{\miouCITMburnCoarseLTwoVarDecoderSegformerMlp}{2.6}
\newcommand{\dropTMburnCoarseLTwoVarDecoderSegformerMlp}{19.2}
\newcommand{\dropCITMburnCoarseLTwoVarDecoderSegformerMlp}{3.3}
\newcommand{\retTMburnCoarseLTwoVarDecoderSegformerMlp}{0.780}
\newcommand{\retCITMburnCoarseLTwoVarDecoderSegformerMlp}{0.035}
\newcommand{\nTMburnCoarseLTwoVarFrozenEncoderTrue}{5}
\newcommand{\miouTMburnCoarseLTwoVarFrozenEncoderTrue}{68.2}
\newcommand{\miouCITMburnCoarseLTwoVarFrozenEncoderTrue}{2.4}
\newcommand{\dropTMburnCoarseLTwoVarFrozenEncoderTrue}{13.4}
\newcommand{\dropCITMburnCoarseLTwoVarFrozenEncoderTrue}{2.0}
\newcommand{\retTMburnCoarseLTwoVarFrozenEncoderTrue}{0.836}
\newcommand{\retCITMburnCoarseLTwoVarFrozenEncoderTrue}{0.024}
\newcommand{\nTMburnCoarseLTwoVarLossBootstrap}{5}
\newcommand{\miouTMburnCoarseLTwoVarLossBootstrap}{68.2}
\newcommand{\miouCITMburnCoarseLTwoVarLossBootstrap}{3.7}
\newcommand{\dropTMburnCoarseLTwoVarLossBootstrap}{18.1}
\newcommand{\dropCITMburnCoarseLTwoVarLossBootstrap}{3.2}
\newcommand{\retTMburnCoarseLTwoVarLossBootstrap}{0.790}
\newcommand{\retCITMburnCoarseLTwoVarLossBootstrap}{0.037}
\newcommand{\nTMburnCoarseLTwoVarLossGce}{5}
\newcommand{\miouTMburnCoarseLTwoVarLossGce}{66.3}
\newcommand{\miouCITMburnCoarseLTwoVarLossGce}{3.8}
\newcommand{\dropTMburnCoarseLTwoVarLossGce}{20.9}
\newcommand{\dropCITMburnCoarseLTwoVarLossGce}{3.7}
\newcommand{\retTMburnCoarseLTwoVarLossGce}{0.761}
\newcommand{\retCITMburnCoarseLTwoVarLossGce}{0.043}
\newcommand{\nTMburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouTMburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{69.8}
\newcommand{\miouCITMburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{2.9}
\newcommand{\dropTMburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{15.3}
\newcommand{\dropCITMburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{3.5}
\newcommand{\retTMburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.820}
\newcommand{\retCITMburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.036}
\newcommand{\nTMburnCoarseLR}{5}
\newcommand{\miouTMburnCoarseLR}{63.8}
\newcommand{\miouCITMburnCoarseLR}{4.1}
\newcommand{\dropTMburnCoarseLR}{22.4}
\newcommand{\dropCITMburnCoarseLR}{5.0}
\newcommand{\retTMburnCoarseLR}{0.740}
\newcommand{\retCITMburnCoarseLR}{0.056}
\newcommand{\nTMburnOmissionLOne}{5}
\newcommand{\miouTMburnOmissionLOne}{81.3}
\newcommand{\miouCITMburnOmissionLOne}{1.6}
\newcommand{\dropTMburnOmissionLOne}{4.9}
\newcommand{\dropCITMburnOmissionLOne}{2.2}
\newcommand{\retTMburnOmissionLOne}{0.944}
\newcommand{\retCITMburnOmissionLOne}{0.025}
\newcommand{\nTMburnOmissionLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouTMburnOmissionLOneVarDecoderMaskTwoformerFull}{83.0}
\newcommand{\miouCITMburnOmissionLOneVarDecoderMaskTwoformerFull}{3.2}
\newcommand{\dropTMburnOmissionLOneVarDecoderMaskTwoformerFull}{4.3}
\newcommand{\dropCITMburnOmissionLOneVarDecoderMaskTwoformerFull}{3.2}
\newcommand{\retTMburnOmissionLOneVarDecoderMaskTwoformerFull}{0.950}
\newcommand{\retCITMburnOmissionLOneVarDecoderMaskTwoformerFull}{0.036}
\newcommand{\nTMburnOmissionLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouTMburnOmissionLOneVarDecoderMaskTwoformerLite}{78.4}
\newcommand{\miouCITMburnOmissionLOneVarDecoderMaskTwoformerLite}{10.3}
\newcommand{\dropTMburnOmissionLOneVarDecoderMaskTwoformerLite}{9.8}
\newcommand{\dropCITMburnOmissionLOneVarDecoderMaskTwoformerLite}{10.5}
\newcommand{\retTMburnOmissionLOneVarDecoderMaskTwoformerLite}{0.889}
\newcommand{\retCITMburnOmissionLOneVarDecoderMaskTwoformerLite}{0.118}
\newcommand{\nTMburnOmissionLOneVarDecoderSamLite}{5}
\newcommand{\miouTMburnOmissionLOneVarDecoderSamLite}{81.7}
\newcommand{\miouCITMburnOmissionLOneVarDecoderSamLite}{4.5}
\newcommand{\dropTMburnOmissionLOneVarDecoderSamLite}{7.0}
\newcommand{\dropCITMburnOmissionLOneVarDecoderSamLite}{4.0}
\newcommand{\retTMburnOmissionLOneVarDecoderSamLite}{0.921}
\newcommand{\retCITMburnOmissionLOneVarDecoderSamLite}{0.046}
\newcommand{\nTMburnOmissionLOneVarDecoderSamPretrained}{5}
\newcommand{\miouTMburnOmissionLOneVarDecoderSamPretrained}{83.4}
\newcommand{\miouCITMburnOmissionLOneVarDecoderSamPretrained}{1.9}
\newcommand{\dropTMburnOmissionLOneVarDecoderSamPretrained}{4.4}
\newcommand{\dropCITMburnOmissionLOneVarDecoderSamPretrained}{2.4}
\newcommand{\retTMburnOmissionLOneVarDecoderSamPretrained}{0.950}
\newcommand{\retCITMburnOmissionLOneVarDecoderSamPretrained}{0.027}
\newcommand{\nTMburnOmissionLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouTMburnOmissionLOneVarDecoderSegformerMlp}{79.6}
\newcommand{\miouCITMburnOmissionLOneVarDecoderSegformerMlp}{2.0}
\newcommand{\dropTMburnOmissionLOneVarDecoderSegformerMlp}{7.8}
\newcommand{\dropCITMburnOmissionLOneVarDecoderSegformerMlp}{2.5}
\newcommand{\retTMburnOmissionLOneVarDecoderSegformerMlp}{0.911}
\newcommand{\retCITMburnOmissionLOneVarDecoderSegformerMlp}{0.028}
\newcommand{\nTMburnOmissionLTwo}{8}
\newcommand{\miouTMburnOmissionLTwo}{75.0}
\newcommand{\miouCITMburnOmissionLTwo}{3.7}
\newcommand{\dropTMburnOmissionLTwo}{11.4}
\newcommand{\dropCITMburnOmissionLTwo}{3.3}
\newcommand{\retTMburnOmissionLTwo}{0.868}
\newcommand{\retCITMburnOmissionLTwo}{0.039}
\newcommand{\nTMburnOmissionLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouTMburnOmissionLTwoVarDecoderMaskTwoformerFull}{74.6}
\newcommand{\miouCITMburnOmissionLTwoVarDecoderMaskTwoformerFull}{3.0}
\newcommand{\dropTMburnOmissionLTwoVarDecoderMaskTwoformerFull}{12.8}
\newcommand{\dropCITMburnOmissionLTwoVarDecoderMaskTwoformerFull}{4.8}
\newcommand{\retTMburnOmissionLTwoVarDecoderMaskTwoformerFull}{0.854}
\newcommand{\retCITMburnOmissionLTwoVarDecoderMaskTwoformerFull}{0.052}
\newcommand{\nTMburnOmissionLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouTMburnOmissionLTwoVarDecoderMaskTwoformerLite}{65.2}
\newcommand{\miouCITMburnOmissionLTwoVarDecoderMaskTwoformerLite}{16.7}
\newcommand{\dropTMburnOmissionLTwoVarDecoderMaskTwoformerLite}{23.0}
\newcommand{\dropCITMburnOmissionLTwoVarDecoderMaskTwoformerLite}{15.8}
\newcommand{\retTMburnOmissionLTwoVarDecoderMaskTwoformerLite}{0.738}
\newcommand{\retCITMburnOmissionLTwoVarDecoderMaskTwoformerLite}{0.183}
\newcommand{\nTMburnOmissionLTwoVarDecoderSamLite}{5}
\newcommand{\miouTMburnOmissionLTwoVarDecoderSamLite}{67.0}
\newcommand{\miouCITMburnOmissionLTwoVarDecoderSamLite}{13.1}
\newcommand{\dropTMburnOmissionLTwoVarDecoderSamLite}{21.7}
\newcommand{\dropCITMburnOmissionLTwoVarDecoderSamLite}{12.7}
\newcommand{\retTMburnOmissionLTwoVarDecoderSamLite}{0.755}
\newcommand{\retCITMburnOmissionLTwoVarDecoderSamLite}{0.144}
\newcommand{\nTMburnOmissionLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouTMburnOmissionLTwoVarDecoderSamPretrained}{71.0}
\newcommand{\miouCITMburnOmissionLTwoVarDecoderSamPretrained}{8.0}
\newcommand{\dropTMburnOmissionLTwoVarDecoderSamPretrained}{16.8}
\newcommand{\dropCITMburnOmissionLTwoVarDecoderSamPretrained}{8.1}
\newcommand{\retTMburnOmissionLTwoVarDecoderSamPretrained}{0.809}
\newcommand{\retCITMburnOmissionLTwoVarDecoderSamPretrained}{0.092}
\newcommand{\nTMburnOmissionLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouTMburnOmissionLTwoVarDecoderSegformerMlp}{68.6}
\newcommand{\miouCITMburnOmissionLTwoVarDecoderSegformerMlp}{7.0}
\newcommand{\dropTMburnOmissionLTwoVarDecoderSegformerMlp}{18.8}
\newcommand{\dropCITMburnOmissionLTwoVarDecoderSegformerMlp}{6.9}
\newcommand{\retTMburnOmissionLTwoVarDecoderSegformerMlp}{0.785}
\newcommand{\retCITMburnOmissionLTwoVarDecoderSegformerMlp}{0.079}
\newcommand{\nTMburnOmissionLTwoVarLossBootstrap}{5}
\newcommand{\miouTMburnOmissionLTwoVarLossBootstrap}{75.2}
\newcommand{\miouCITMburnOmissionLTwoVarLossBootstrap}{3.9}
\newcommand{\dropTMburnOmissionLTwoVarLossBootstrap}{11.1}
\newcommand{\dropCITMburnOmissionLTwoVarLossBootstrap}{2.2}
\newcommand{\retTMburnOmissionLTwoVarLossBootstrap}{0.871}
\newcommand{\retCITMburnOmissionLTwoVarLossBootstrap}{0.028}
\newcommand{\nTMburnOmissionLTwoVarLossGce}{5}
\newcommand{\miouTMburnOmissionLTwoVarLossGce}{76.7}
\newcommand{\miouCITMburnOmissionLTwoVarLossGce}{3.2}
\newcommand{\dropTMburnOmissionLTwoVarLossGce}{10.5}
\newcommand{\dropCITMburnOmissionLTwoVarLossGce}{2.9}
\newcommand{\retTMburnOmissionLTwoVarLossGce}{0.880}
\newcommand{\retCITMburnOmissionLTwoVarLossGce}{0.033}
\newcommand{\nTMburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouTMburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{75.1}
\newcommand{\miouCITMburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{5.9}
\newcommand{\dropTMburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{10.0}
\newcommand{\dropCITMburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{8.4}
\newcommand{\retTMburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{0.884}
\newcommand{\retCITMburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{0.093}
\newcommand{\nTMburnOmissionLR}{5}
\newcommand{\miouTMburnOmissionLR}{59.1}
\newcommand{\miouCITMburnOmissionLR}{12.0}
\newcommand{\dropTMburnOmissionLR}{27.1}
\newcommand{\dropCITMburnOmissionLR}{10.5}
\newcommand{\retTMburnOmissionLR}{0.685}
\newcommand{\retCITMburnOmissionLR}{0.127}
\newcommand{\nTMburnShiftLOne}{5}
\newcommand{\miouTMburnShiftLOne}{82.8}
\newcommand{\miouCITMburnShiftLOne}{2.3}
\newcommand{\dropTMburnShiftLOne}{3.4}
\newcommand{\dropCITMburnShiftLOne}{3.0}
\newcommand{\retTMburnShiftLOne}{0.961}
\newcommand{\retCITMburnShiftLOne}{0.034}
\newcommand{\nTMburnShiftLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouTMburnShiftLOneVarDecoderMaskTwoformerFull}{85.2}
\newcommand{\miouCITMburnShiftLOneVarDecoderMaskTwoformerFull}{0.5}
\newcommand{\dropTMburnShiftLOneVarDecoderMaskTwoformerFull}{2.2}
\newcommand{\dropCITMburnShiftLOneVarDecoderMaskTwoformerFull}{2.1}
\newcommand{\retTMburnShiftLOneVarDecoderMaskTwoformerFull}{0.975}
\newcommand{\retCITMburnShiftLOneVarDecoderMaskTwoformerFull}{0.023}
\newcommand{\nTMburnShiftLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouTMburnShiftLOneVarDecoderMaskTwoformerLite}{84.5}
\newcommand{\miouCITMburnShiftLOneVarDecoderMaskTwoformerLite}{1.3}
\newcommand{\dropTMburnShiftLOneVarDecoderMaskTwoformerLite}{3.7}
\newcommand{\dropCITMburnShiftLOneVarDecoderMaskTwoformerLite}{1.3}
\newcommand{\retTMburnShiftLOneVarDecoderMaskTwoformerLite}{0.958}
\newcommand{\retCITMburnShiftLOneVarDecoderMaskTwoformerLite}{0.014}
\newcommand{\nTMburnShiftLOneVarDecoderSamLite}{5}
\newcommand{\miouTMburnShiftLOneVarDecoderSamLite}{84.3}
\newcommand{\miouCITMburnShiftLOneVarDecoderSamLite}{1.1}
\newcommand{\dropTMburnShiftLOneVarDecoderSamLite}{4.4}
\newcommand{\dropCITMburnShiftLOneVarDecoderSamLite}{0.5}
\newcommand{\retTMburnShiftLOneVarDecoderSamLite}{0.951}
\newcommand{\retCITMburnShiftLOneVarDecoderSamLite}{0.006}
\newcommand{\nTMburnShiftLOneVarDecoderSamPretrained}{5}
\newcommand{\miouTMburnShiftLOneVarDecoderSamPretrained}{84.7}
\newcommand{\miouCITMburnShiftLOneVarDecoderSamPretrained}{1.9}
\newcommand{\dropTMburnShiftLOneVarDecoderSamPretrained}{3.1}
\newcommand{\dropCITMburnShiftLOneVarDecoderSamPretrained}{3.3}
\newcommand{\retTMburnShiftLOneVarDecoderSamPretrained}{0.965}
\newcommand{\retCITMburnShiftLOneVarDecoderSamPretrained}{0.037}
\newcommand{\nTMburnShiftLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouTMburnShiftLOneVarDecoderSegformerMlp}{85.1}
\newcommand{\miouCITMburnShiftLOneVarDecoderSegformerMlp}{1.4}
\newcommand{\dropTMburnShiftLOneVarDecoderSegformerMlp}{2.3}
\newcommand{\dropCITMburnShiftLOneVarDecoderSegformerMlp}{1.9}
\newcommand{\retTMburnShiftLOneVarDecoderSegformerMlp}{0.973}
\newcommand{\retCITMburnShiftLOneVarDecoderSegformerMlp}{0.022}
\newcommand{\nTMburnShiftLTwo}{8}
\newcommand{\miouTMburnShiftLTwo}{76.5}
\newcommand{\miouCITMburnShiftLTwo}{1.0}
\newcommand{\dropTMburnShiftLTwo}{9.8}
\newcommand{\dropCITMburnShiftLTwo}{1.5}
\newcommand{\retTMburnShiftLTwo}{0.887}
\newcommand{\retCITMburnShiftLTwo}{0.016}
\newcommand{\nTMburnShiftLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouTMburnShiftLTwoVarDecoderMaskTwoformerFull}{76.6}
\newcommand{\miouCITMburnShiftLTwoVarDecoderMaskTwoformerFull}{0.8}
\newcommand{\dropTMburnShiftLTwoVarDecoderMaskTwoformerFull}{10.8}
\newcommand{\dropCITMburnShiftLTwoVarDecoderMaskTwoformerFull}{1.7}
\newcommand{\retTMburnShiftLTwoVarDecoderMaskTwoformerFull}{0.877}
\newcommand{\retCITMburnShiftLTwoVarDecoderMaskTwoformerFull}{0.017}
\newcommand{\nTMburnShiftLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouTMburnShiftLTwoVarDecoderMaskTwoformerLite}{76.8}
\newcommand{\miouCITMburnShiftLTwoVarDecoderMaskTwoformerLite}{2.0}
\newcommand{\dropTMburnShiftLTwoVarDecoderMaskTwoformerLite}{11.4}
\newcommand{\dropCITMburnShiftLTwoVarDecoderMaskTwoformerLite}{2.7}
\newcommand{\retTMburnShiftLTwoVarDecoderMaskTwoformerLite}{0.871}
\newcommand{\retCITMburnShiftLTwoVarDecoderMaskTwoformerLite}{0.029}
\newcommand{\nTMburnShiftLTwoVarDecoderSamLite}{5}
\newcommand{\miouTMburnShiftLTwoVarDecoderSamLite}{75.5}
\newcommand{\miouCITMburnShiftLTwoVarDecoderSamLite}{2.2}
\newcommand{\dropTMburnShiftLTwoVarDecoderSamLite}{13.1}
\newcommand{\dropCITMburnShiftLTwoVarDecoderSamLite}{2.1}
\newcommand{\retTMburnShiftLTwoVarDecoderSamLite}{0.852}
\newcommand{\retCITMburnShiftLTwoVarDecoderSamLite}{0.023}
\newcommand{\nTMburnShiftLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouTMburnShiftLTwoVarDecoderSamPretrained}{76.7}
\newcommand{\miouCITMburnShiftLTwoVarDecoderSamPretrained}{2.7}
\newcommand{\dropTMburnShiftLTwoVarDecoderSamPretrained}{11.1}
\newcommand{\dropCITMburnShiftLTwoVarDecoderSamPretrained}{3.3}
\newcommand{\retTMburnShiftLTwoVarDecoderSamPretrained}{0.874}
\newcommand{\retCITMburnShiftLTwoVarDecoderSamPretrained}{0.037}
\newcommand{\nTMburnShiftLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouTMburnShiftLTwoVarDecoderSegformerMlp}{75.5}
\newcommand{\miouCITMburnShiftLTwoVarDecoderSegformerMlp}{2.3}
\newcommand{\dropTMburnShiftLTwoVarDecoderSegformerMlp}{11.9}
\newcommand{\dropCITMburnShiftLTwoVarDecoderSegformerMlp}{3.2}
\newcommand{\retTMburnShiftLTwoVarDecoderSegformerMlp}{0.864}
\newcommand{\retCITMburnShiftLTwoVarDecoderSegformerMlp}{0.035}
\newcommand{\nTMburnShiftLTwoVarLossBootstrap}{5}
\newcommand{\miouTMburnShiftLTwoVarLossBootstrap}{76.1}
\newcommand{\miouCITMburnShiftLTwoVarLossBootstrap}{3.2}
\newcommand{\dropTMburnShiftLTwoVarLossBootstrap}{10.2}
\newcommand{\dropCITMburnShiftLTwoVarLossBootstrap}{4.9}
\newcommand{\retTMburnShiftLTwoVarLossBootstrap}{0.882}
\newcommand{\retCITMburnShiftLTwoVarLossBootstrap}{0.055}
\newcommand{\nTMburnShiftLTwoVarLossGce}{5}
\newcommand{\miouTMburnShiftLTwoVarLossGce}{76.4}
\newcommand{\miouCITMburnShiftLTwoVarLossGce}{1.8}
\newcommand{\dropTMburnShiftLTwoVarLossGce}{10.8}
\newcommand{\dropCITMburnShiftLTwoVarLossGce}{1.1}
\newcommand{\retTMburnShiftLTwoVarLossGce}{0.876}
\newcommand{\retCITMburnShiftLTwoVarLossGce}{0.014}
\newcommand{\nTMburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouTMburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{77.2}
\newcommand{\miouCITMburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{1.5}
\newcommand{\dropTMburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{7.9}
\newcommand{\dropCITMburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{3.2}
\newcommand{\retTMburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.908}
\newcommand{\retCITMburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.034}
\newcommand{\nTMburnShiftLR}{5}
\newcommand{\miouTMburnShiftLR}{68.6}
\newcommand{\miouCITMburnShiftLR}{3.7}
\newcommand{\dropTMburnShiftLR}{17.6}
\newcommand{\dropCITMburnShiftLR}{3.3}
\newcommand{\retTMburnShiftLR}{0.796}
\newcommand{\retCITMburnShiftLR}{0.038}
\newcommand{\nTMChesBoundaryLOne}{5}
\newcommand{\miouTMChesBoundaryLOne}{78.0}
\newcommand{\miouCITMChesBoundaryLOne}{0.6}
\newcommand{\dropTMChesBoundaryLOne}{4.1}
\newcommand{\dropCITMChesBoundaryLOne}{0.8}
\newcommand{\retTMChesBoundaryLOne}{0.950}
\newcommand{\retCITMChesBoundaryLOne}{0.009}
\newcommand{\nTMChesBoundaryLTwo}{5}
\newcommand{\miouTMChesBoundaryLTwo}{71.6}
\newcommand{\miouCITMChesBoundaryLTwo}{1.3}
\newcommand{\dropTMChesBoundaryLTwo}{10.5}
\newcommand{\dropCITMChesBoundaryLTwo}{1.5}
\newcommand{\retTMChesBoundaryLTwo}{0.872}
\newcommand{\retCITMChesBoundaryLTwo}{0.017}
\newcommand{\nTMChesClean}{5}
\newcommand{\miouTMChesClean}{82.0}
\newcommand{\miouCITMChesClean}{0.6}
\newcommand{\nTMChesCoarseLOne}{5}
\newcommand{\miouTMChesCoarseLOne}{80.3}
\newcommand{\miouCITMChesCoarseLOne}{0.6}
\newcommand{\dropTMChesCoarseLOne}{1.7}
\newcommand{\dropCITMChesCoarseLOne}{0.8}
\newcommand{\retTMChesCoarseLOne}{0.979}
\newcommand{\retCITMChesCoarseLOne}{0.009}
\newcommand{\nTMChesCoarseLTwo}{5}
\newcommand{\miouTMChesCoarseLTwo}{69.8}
\newcommand{\miouCITMChesCoarseLTwo}{0.9}
\newcommand{\dropTMChesCoarseLTwo}{12.3}
\newcommand{\dropCITMChesCoarseLTwo}{0.8}
\newcommand{\retTMChesCoarseLTwo}{0.850}
\newcommand{\retCITMChesCoarseLTwo}{0.010}
\newcommand{\nTMChesNlcdREAL}{5}
\newcommand{\miouTMChesNlcdREAL}{62.1}
\newcommand{\miouCITMChesNlcdREAL}{1.0}
\newcommand{\dropTMChesNlcdREAL}{20.0}
\newcommand{\dropCITMChesNlcdREAL}{0.7}
\newcommand{\retTMChesNlcdREAL}{0.756}
\newcommand{\retCITMChesNlcdREAL}{0.009}
\newcommand{\nTMChesOmissionLOne}{5}
\newcommand{\miouTMChesOmissionLOne}{78.4}
\newcommand{\miouCITMChesOmissionLOne}{2.1}
\newcommand{\dropTMChesOmissionLOne}{3.7}
\newcommand{\dropCITMChesOmissionLOne}{2.1}
\newcommand{\retTMChesOmissionLOne}{0.955}
\newcommand{\retCITMChesOmissionLOne}{0.026}
\newcommand{\nTMChesOmissionLTwo}{5}
\newcommand{\miouTMChesOmissionLTwo}{72.5}
\newcommand{\miouCITMChesOmissionLTwo}{3.0}
\newcommand{\dropTMChesOmissionLTwo}{9.5}
\newcommand{\dropCITMChesOmissionLTwo}{2.7}
\newcommand{\retTMChesOmissionLTwo}{0.884}
\newcommand{\retCITMChesOmissionLTwo}{0.034}
\newcommand{\nTMChesShiftLOne}{5}
\newcommand{\miouTMChesShiftLOne}{81.1}
\newcommand{\miouCITMChesShiftLOne}{0.6}
\newcommand{\dropTMChesShiftLOne}{1.0}
\newcommand{\dropCITMChesShiftLOne}{0.8}
\newcommand{\retTMChesShiftLOne}{0.988}
\newcommand{\retCITMChesShiftLOne}{0.009}
\newcommand{\nTMChesShiftLTwo}{5}
\newcommand{\miouTMChesShiftLTwo}{74.6}
\newcommand{\miouCITMChesShiftLTwo}{0.7}
\newcommand{\dropTMChesShiftLTwo}{7.4}
\newcommand{\dropCITMChesShiftLTwo}{1.2}
\newcommand{\retTMChesShiftLTwo}{0.910}
\newcommand{\retCITMChesShiftLTwo}{0.014}
\newcommand{\nTMCsTwelveBoundaryLOne}{5}
\newcommand{\miouTMCsTwelveBoundaryLOne}{67.8}
\newcommand{\miouCITMCsTwelveBoundaryLOne}{0.4}
\newcommand{\dropTMCsTwelveBoundaryLOne}{1.7}
\newcommand{\dropCITMCsTwelveBoundaryLOne}{1.0}
\newcommand{\retTMCsTwelveBoundaryLOne}{0.976}
\newcommand{\retCITMCsTwelveBoundaryLOne}{0.014}
\newcommand{\nTMCsTwelveBoundaryLTwo}{5}
\newcommand{\miouTMCsTwelveBoundaryLTwo}{62.0}
\newcommand{\miouCITMCsTwelveBoundaryLTwo}{0.9}
\newcommand{\dropTMCsTwelveBoundaryLTwo}{7.5}
\newcommand{\dropCITMCsTwelveBoundaryLTwo}{0.8}
\newcommand{\retTMCsTwelveBoundaryLTwo}{0.892}
\newcommand{\retCITMCsTwelveBoundaryLTwo}{0.011}
\newcommand{\nTMCsTwelveClean}{5}
\newcommand{\miouTMCsTwelveClean}{69.5}
\newcommand{\miouCITMCsTwelveClean}{0.6}
\newcommand{\nTMCsTwelveCoarseLOne}{5}
\newcommand{\miouTMCsTwelveCoarseLOne}{67.6}
\newcommand{\miouCITMCsTwelveCoarseLOne}{1.1}
\newcommand{\dropTMCsTwelveCoarseLOne}{1.9}
\newcommand{\dropCITMCsTwelveCoarseLOne}{1.4}
\newcommand{\retTMCsTwelveCoarseLOne}{0.973}
\newcommand{\retCITMCsTwelveCoarseLOne}{0.020}
\newcommand{\nTMCsTwelveCoarseLTwo}{5}
\newcommand{\miouTMCsTwelveCoarseLTwo}{61.1}
\newcommand{\miouCITMCsTwelveCoarseLTwo}{0.3}
\newcommand{\dropTMCsTwelveCoarseLTwo}{8.5}
\newcommand{\dropCITMCsTwelveCoarseLTwo}{0.4}
\newcommand{\retTMCsTwelveCoarseLTwo}{0.878}
\newcommand{\retCITMCsTwelveCoarseLTwo}{0.005}
\newcommand{\nTMCsTwelveOmissionLOne}{5}
\newcommand{\miouTMCsTwelveOmissionLOne}{66.0}
\newcommand{\miouCITMCsTwelveOmissionLOne}{1.7}
\newcommand{\dropTMCsTwelveOmissionLOne}{3.5}
\newcommand{\dropCITMCsTwelveOmissionLOne}{2.2}
\newcommand{\retTMCsTwelveOmissionLOne}{0.950}
\newcommand{\retCITMCsTwelveOmissionLOne}{0.031}
\newcommand{\nTMCsTwelveOmissionLTwo}{5}
\newcommand{\miouTMCsTwelveOmissionLTwo}{62.2}
\newcommand{\miouCITMCsTwelveOmissionLTwo}{1.2}
\newcommand{\dropTMCsTwelveOmissionLTwo}{7.3}
\newcommand{\dropCITMCsTwelveOmissionLTwo}{1.0}
\newcommand{\retTMCsTwelveOmissionLTwo}{0.895}
\newcommand{\retCITMCsTwelveOmissionLTwo}{0.014}
\newcommand{\nTMCsTwelveSTwocloudlessREAL}{5}
\newcommand{\miouTMCsTwelveSTwocloudlessREAL}{34.8}
\newcommand{\miouCITMCsTwelveSTwocloudlessREAL}{0.2}
\newcommand{\dropTMCsTwelveSTwocloudlessREAL}{34.7}
\newcommand{\dropCITMCsTwelveSTwocloudlessREAL}{0.6}
\newcommand{\retTMCsTwelveSTwocloudlessREAL}{0.501}
\newcommand{\retCITMCsTwelveSTwocloudlessREAL}{0.005}
\newcommand{\nTMCsTwelveShiftLOne}{5}
\newcommand{\miouTMCsTwelveShiftLOne}{68.5}
\newcommand{\miouCITMCsTwelveShiftLOne}{0.7}
\newcommand{\dropTMCsTwelveShiftLOne}{1.0}
\newcommand{\dropCITMCsTwelveShiftLOne}{1.2}
\newcommand{\retTMCsTwelveShiftLOne}{0.985}
\newcommand{\retCITMCsTwelveShiftLOne}{0.017}
\newcommand{\nTMCsTwelveShiftLTwo}{5}
\newcommand{\miouTMCsTwelveShiftLTwo}{64.0}
\newcommand{\miouCITMCsTwelveShiftLTwo}{0.7}
\newcommand{\dropTMCsTwelveShiftLTwo}{5.6}
\newcommand{\dropCITMCsTwelveShiftLTwo}{1.1}
\newcommand{\retTMCsTwelveShiftLTwo}{0.920}
\newcommand{\retCITMCsTwelveShiftLTwo}{0.015}
\newcommand{\nTMDfcBoundaryLOne}{5}
\newcommand{\miouTMDfcBoundaryLOne}{37.7}
\newcommand{\miouCITMDfcBoundaryLOne}{1.8}
\newcommand{\dropTMDfcBoundaryLOne}{1.1}
\newcommand{\dropCITMDfcBoundaryLOne}{2.5}
\newcommand{\retTMDfcBoundaryLOne}{0.971}
\newcommand{\retCITMDfcBoundaryLOne}{0.065}
\newcommand{\nTMDfcBoundaryLTwo}{5}
\newcommand{\miouTMDfcBoundaryLTwo}{34.7}
\newcommand{\miouCITMDfcBoundaryLTwo}{3.7}
\newcommand{\dropTMDfcBoundaryLTwo}{4.2}
\newcommand{\dropCITMDfcBoundaryLTwo}{4.4}
\newcommand{\retTMDfcBoundaryLTwo}{0.893}
\newcommand{\retCITMDfcBoundaryLTwo}{0.111}
\newcommand{\nTMDfcClean}{5}
\newcommand{\miouTMDfcClean}{38.9}
\newcommand{\miouCITMDfcClean}{0.8}
\newcommand{\nTMDfcCleanVarTrainSubsetRealcov}{5}
\newcommand{\miouTMDfcCleanVarTrainSubsetRealcov}{38.3}
\newcommand{\miouCITMDfcCleanVarTrainSubsetRealcov}{0.4}
\newcommand{\nTMDfcCoarseLOne}{5}
\newcommand{\miouTMDfcCoarseLOne}{38.2}
\newcommand{\miouCITMDfcCoarseLOne}{1.6}
\newcommand{\dropTMDfcCoarseLOne}{0.7}
\newcommand{\dropCITMDfcCoarseLOne}{2.0}
\newcommand{\retTMDfcCoarseLOne}{0.982}
\newcommand{\retCITMDfcCoarseLOne}{0.052}
\newcommand{\nTMDfcCoarseLTwo}{5}
\newcommand{\miouTMDfcCoarseLTwo}{36.4}
\newcommand{\miouCITMDfcCoarseLTwo}{1.7}
\newcommand{\dropTMDfcCoarseLTwo}{2.5}
\newcommand{\dropCITMDfcCoarseLTwo}{2.3}
\newcommand{\retTMDfcCoarseLTwo}{0.936}
\newcommand{\retCITMDfcCoarseLTwo}{0.059}
\newcommand{\nTMDfcModisREALVarTrainSubsetRealcov}{5}
\newcommand{\miouTMDfcModisREALVarTrainSubsetRealcov}{35.5}
\newcommand{\miouCITMDfcModisREALVarTrainSubsetRealcov}{1.1}
\newcommand{\dropTMDfcModisREALVarTrainSubsetRealcov}{2.7}
\newcommand{\dropCITMDfcModisREALVarTrainSubsetRealcov}{1.2}
\newcommand{\retTMDfcModisREALVarTrainSubsetRealcov}{0.929}
\newcommand{\retCITMDfcModisREALVarTrainSubsetRealcov}{0.030}
\newcommand{\nTMDfcOmissionLOne}{5}
\newcommand{\miouTMDfcOmissionLOne}{36.4}
\newcommand{\miouCITMDfcOmissionLOne}{3.0}
\newcommand{\dropTMDfcOmissionLOne}{2.5}
\newcommand{\dropCITMDfcOmissionLOne}{2.7}
\newcommand{\retTMDfcOmissionLOne}{0.935}
\newcommand{\retCITMDfcOmissionLOne}{0.069}
\newcommand{\nTMDfcOmissionLTwo}{5}
\newcommand{\miouTMDfcOmissionLTwo}{33.0}
\newcommand{\miouCITMDfcOmissionLTwo}{1.5}
\newcommand{\dropTMDfcOmissionLTwo}{5.8}
\newcommand{\dropCITMDfcOmissionLTwo}{1.4}
\newcommand{\retTMDfcOmissionLTwo}{0.850}
\newcommand{\retCITMDfcOmissionLTwo}{0.036}
\newcommand{\nTMDfcShiftLOne}{5}
\newcommand{\miouTMDfcShiftLOne}{38.1}
\newcommand{\miouCITMDfcShiftLOne}{0.4}
\newcommand{\dropTMDfcShiftLOne}{0.8}
\newcommand{\dropCITMDfcShiftLOne}{0.8}
\newcommand{\retTMDfcShiftLOne}{0.980}
\newcommand{\retCITMDfcShiftLOne}{0.021}
\newcommand{\nTMDfcShiftLTwo}{5}
\newcommand{\miouTMDfcShiftLTwo}{37.6}
\newcommand{\miouCITMDfcShiftLTwo}{1.0}
\newcommand{\dropTMDfcShiftLTwo}{1.2}
\newcommand{\dropCITMDfcShiftLTwo}{1.4}
\newcommand{\retTMDfcShiftLTwo}{0.969}
\newcommand{\retCITMDfcShiftLTwo}{0.035}
\newcommand{\nTMEnvaBoundaryLOne}{5}
\newcommand{\miouTMEnvaBoundaryLOne}{44.0}
\newcommand{\miouCITMEnvaBoundaryLOne}{11.9}
\newcommand{\dropTMEnvaBoundaryLOne}{5.0}
\newcommand{\dropCITMEnvaBoundaryLOne}{10.0}
\newcommand{\retTMEnvaBoundaryLOne}{0.894}
\newcommand{\retCITMEnvaBoundaryLOne}{0.216}
\newcommand{\nTMEnvaBoundaryLTwo}{5}
\newcommand{\miouTMEnvaBoundaryLTwo}{41.5}
\newcommand{\miouCITMEnvaBoundaryLTwo}{7.3}
\newcommand{\dropTMEnvaBoundaryLTwo}{7.5}
\newcommand{\dropCITMEnvaBoundaryLTwo}{6.9}
\newcommand{\retTMEnvaBoundaryLTwo}{0.847}
\newcommand{\retCITMEnvaBoundaryLTwo}{0.140}
\newcommand{\nTMEnvaClean}{5}
\newcommand{\miouTMEnvaClean}{49.0}
\newcommand{\miouCITMEnvaClean}{2.7}
\newcommand{\nTMEnvaCoarseLOne}{5}
\newcommand{\miouTMEnvaCoarseLOne}{49.9}
\newcommand{\miouCITMEnvaCoarseLOne}{3.1}
\newcommand{\dropTMEnvaCoarseLOne}{\ensuremath{-}0.9}
\newcommand{\dropCITMEnvaCoarseLOne}{3.8}
\newcommand{\retTMEnvaCoarseLOne}{1.019}
\newcommand{\retCITMEnvaCoarseLOne}{0.081}
\newcommand{\nTMEnvaCoarseLTwo}{5}
\newcommand{\miouTMEnvaCoarseLTwo}{45.9}
\newcommand{\miouCITMEnvaCoarseLTwo}{3.7}
\newcommand{\dropTMEnvaCoarseLTwo}{3.0}
\newcommand{\dropCITMEnvaCoarseLTwo}{5.9}
\newcommand{\retTMEnvaCoarseLTwo}{0.941}
\newcommand{\retCITMEnvaCoarseLTwo}{0.119}
\newcommand{\nTMEnvaNlcdREAL}{5}
\newcommand{\miouTMEnvaNlcdREAL}{22.9}
\newcommand{\miouCITMEnvaNlcdREAL}{1.2}
\newcommand{\dropTMEnvaNlcdREAL}{26.1}
\newcommand{\dropCITMEnvaNlcdREAL}{3.2}
\newcommand{\retTMEnvaNlcdREAL}{0.468}
\newcommand{\retCITMEnvaNlcdREAL}{0.039}
\newcommand{\nTMEnvaOmissionLOne}{5}
\newcommand{\miouTMEnvaOmissionLOne}{44.5}
\newcommand{\miouCITMEnvaOmissionLOne}{10.9}
\newcommand{\dropTMEnvaOmissionLOne}{4.5}
\newcommand{\dropCITMEnvaOmissionLOne}{11.1}
\newcommand{\retTMEnvaOmissionLOne}{0.910}
\newcommand{\retCITMEnvaOmissionLOne}{0.229}
\newcommand{\nTMEnvaOmissionLTwo}{5}
\newcommand{\miouTMEnvaOmissionLTwo}{34.4}
\newcommand{\miouCITMEnvaOmissionLTwo}{9.7}
\newcommand{\dropTMEnvaOmissionLTwo}{14.6}
\newcommand{\dropCITMEnvaOmissionLTwo}{7.4}
\newcommand{\retTMEnvaOmissionLTwo}{0.699}
\newcommand{\retCITMEnvaOmissionLTwo}{0.163}
\newcommand{\nTMEnvaShiftLOne}{5}
\newcommand{\miouTMEnvaShiftLOne}{49.6}
\newcommand{\miouCITMEnvaShiftLOne}{3.5}
\newcommand{\dropTMEnvaShiftLOne}{\ensuremath{-}0.6}
\newcommand{\dropCITMEnvaShiftLOne}{1.6}
\newcommand{\retTMEnvaShiftLOne}{1.012}
\newcommand{\retCITMEnvaShiftLOne}{0.033}
\newcommand{\nTMEnvaShiftLTwo}{5}
\newcommand{\miouTMEnvaShiftLTwo}{46.7}
\newcommand{\miouCITMEnvaShiftLTwo}{5.1}
\newcommand{\dropTMEnvaShiftLTwo}{2.3}
\newcommand{\dropCITMEnvaShiftLTwo}{3.5}
\newcommand{\retTMEnvaShiftLTwo}{0.952}
\newcommand{\retCITMEnvaShiftLTwo}{0.074}
\newcommand{\nTMflairBoundaryLOne}{5}
\newcommand{\miouTMflairBoundaryLOne}{39.0}
\newcommand{\miouCITMflairBoundaryLOne}{0.6}
\newcommand{\dropTMflairBoundaryLOne}{1.5}
\newcommand{\dropCITMflairBoundaryLOne}{1.2}
\newcommand{\retTMflairBoundaryLOne}{0.964}
\newcommand{\retCITMflairBoundaryLOne}{0.030}
\newcommand{\nTMflairBoundaryLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouTMflairBoundaryLOneVarDecoderMaskTwoformerFull}{41.6}
\newcommand{\miouCITMflairBoundaryLOneVarDecoderMaskTwoformerFull}{1.0}
\newcommand{\dropTMflairBoundaryLOneVarDecoderMaskTwoformerFull}{1.2}
\newcommand{\dropCITMflairBoundaryLOneVarDecoderMaskTwoformerFull}{1.0}
\newcommand{\retTMflairBoundaryLOneVarDecoderMaskTwoformerFull}{0.971}
\newcommand{\retCITMflairBoundaryLOneVarDecoderMaskTwoformerFull}{0.024}
\newcommand{\nTMflairBoundaryLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouTMflairBoundaryLOneVarDecoderMaskTwoformerLite}{38.9}
\newcommand{\miouCITMflairBoundaryLOneVarDecoderMaskTwoformerLite}{1.9}
\newcommand{\dropTMflairBoundaryLOneVarDecoderMaskTwoformerLite}{2.5}
\newcommand{\dropCITMflairBoundaryLOneVarDecoderMaskTwoformerLite}{1.6}
\newcommand{\retTMflairBoundaryLOneVarDecoderMaskTwoformerLite}{0.939}
\newcommand{\retCITMflairBoundaryLOneVarDecoderMaskTwoformerLite}{0.038}
\newcommand{\nTMflairBoundaryLOneVarDecoderSamLite}{5}
\newcommand{\miouTMflairBoundaryLOneVarDecoderSamLite}{38.3}
\newcommand{\miouCITMflairBoundaryLOneVarDecoderSamLite}{0.7}
\newcommand{\dropTMflairBoundaryLOneVarDecoderSamLite}{1.9}
\newcommand{\dropCITMflairBoundaryLOneVarDecoderSamLite}{0.2}
\newcommand{\retTMflairBoundaryLOneVarDecoderSamLite}{0.952}
\newcommand{\retCITMflairBoundaryLOneVarDecoderSamLite}{0.006}
\newcommand{\nTMflairBoundaryLOneVarDecoderSamPretrained}{5}
\newcommand{\miouTMflairBoundaryLOneVarDecoderSamPretrained}{37.6}
\newcommand{\miouCITMflairBoundaryLOneVarDecoderSamPretrained}{0.8}
\newcommand{\dropTMflairBoundaryLOneVarDecoderSamPretrained}{1.7}
\newcommand{\dropCITMflairBoundaryLOneVarDecoderSamPretrained}{2.1}
\newcommand{\retTMflairBoundaryLOneVarDecoderSamPretrained}{0.958}
\newcommand{\retCITMflairBoundaryLOneVarDecoderSamPretrained}{0.054}
\newcommand{\nTMflairBoundaryLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouTMflairBoundaryLOneVarDecoderSegformerMlp}{39.6}
\newcommand{\miouCITMflairBoundaryLOneVarDecoderSegformerMlp}{0.5}
\newcommand{\dropTMflairBoundaryLOneVarDecoderSegformerMlp}{2.3}
\newcommand{\dropCITMflairBoundaryLOneVarDecoderSegformerMlp}{0.5}
\newcommand{\retTMflairBoundaryLOneVarDecoderSegformerMlp}{0.945}
\newcommand{\retCITMflairBoundaryLOneVarDecoderSegformerMlp}{0.011}
\newcommand{\nTMflairBoundaryLTwo}{5}
\newcommand{\miouTMflairBoundaryLTwo}{34.4}
\newcommand{\miouCITMflairBoundaryLTwo}{1.2}
\newcommand{\dropTMflairBoundaryLTwo}{6.1}
\newcommand{\dropCITMflairBoundaryLTwo}{1.9}
\newcommand{\retTMflairBoundaryLTwo}{0.851}
\newcommand{\retCITMflairBoundaryLTwo}{0.044}
\newcommand{\nTMflairBoundaryLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouTMflairBoundaryLTwoVarDecoderMaskTwoformerFull}{38.3}
\newcommand{\miouCITMflairBoundaryLTwoVarDecoderMaskTwoformerFull}{1.7}
\newcommand{\dropTMflairBoundaryLTwoVarDecoderMaskTwoformerFull}{4.5}
\newcommand{\dropCITMflairBoundaryLTwoVarDecoderMaskTwoformerFull}{1.7}
\newcommand{\retTMflairBoundaryLTwoVarDecoderMaskTwoformerFull}{0.895}
\newcommand{\retCITMflairBoundaryLTwoVarDecoderMaskTwoformerFull}{0.038}
\newcommand{\nTMflairBoundaryLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouTMflairBoundaryLTwoVarDecoderMaskTwoformerLite}{35.7}
\newcommand{\miouCITMflairBoundaryLTwoVarDecoderMaskTwoformerLite}{1.9}
\newcommand{\dropTMflairBoundaryLTwoVarDecoderMaskTwoformerLite}{5.7}
\newcommand{\dropCITMflairBoundaryLTwoVarDecoderMaskTwoformerLite}{1.6}
\newcommand{\retTMflairBoundaryLTwoVarDecoderMaskTwoformerLite}{0.863}
\newcommand{\retCITMflairBoundaryLTwoVarDecoderMaskTwoformerLite}{0.038}
\newcommand{\nTMflairBoundaryLTwoVarDecoderSamLite}{5}
\newcommand{\miouTMflairBoundaryLTwoVarDecoderSamLite}{33.9}
\newcommand{\miouCITMflairBoundaryLTwoVarDecoderSamLite}{1.3}
\newcommand{\dropTMflairBoundaryLTwoVarDecoderSamLite}{6.3}
\newcommand{\dropCITMflairBoundaryLTwoVarDecoderSamLite}{1.4}
\newcommand{\retTMflairBoundaryLTwoVarDecoderSamLite}{0.843}
\newcommand{\retCITMflairBoundaryLTwoVarDecoderSamLite}{0.034}
\newcommand{\nTMflairBoundaryLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouTMflairBoundaryLTwoVarDecoderSamPretrained}{31.8}
\newcommand{\miouCITMflairBoundaryLTwoVarDecoderSamPretrained}{1.3}
\newcommand{\dropTMflairBoundaryLTwoVarDecoderSamPretrained}{7.5}
\newcommand{\dropCITMflairBoundaryLTwoVarDecoderSamPretrained}{2.2}
\newcommand{\retTMflairBoundaryLTwoVarDecoderSamPretrained}{0.810}
\newcommand{\retCITMflairBoundaryLTwoVarDecoderSamPretrained}{0.052}
\newcommand{\nTMflairBoundaryLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouTMflairBoundaryLTwoVarDecoderSegformerMlp}{34.3}
\newcommand{\miouCITMflairBoundaryLTwoVarDecoderSegformerMlp}{1.7}
\newcommand{\dropTMflairBoundaryLTwoVarDecoderSegformerMlp}{7.6}
\newcommand{\dropCITMflairBoundaryLTwoVarDecoderSegformerMlp}{1.7}
\newcommand{\retTMflairBoundaryLTwoVarDecoderSegformerMlp}{0.818}
\newcommand{\retCITMflairBoundaryLTwoVarDecoderSegformerMlp}{0.040}
\newcommand{\nTMflairBoundaryLTwoVarLossBootstrap}{5}
\newcommand{\miouTMflairBoundaryLTwoVarLossBootstrap}{33.7}
\newcommand{\miouCITMflairBoundaryLTwoVarLossBootstrap}{0.9}
\newcommand{\dropTMflairBoundaryLTwoVarLossBootstrap}{7.1}
\newcommand{\dropCITMflairBoundaryLTwoVarLossBootstrap}{1.1}
\newcommand{\retTMflairBoundaryLTwoVarLossBootstrap}{0.826}
\newcommand{\retCITMflairBoundaryLTwoVarLossBootstrap}{0.021}
\newcommand{\nTMflairBoundaryLTwoVarLossGce}{5}
\newcommand{\miouTMflairBoundaryLTwoVarLossGce}{30.2}
\newcommand{\miouCITMflairBoundaryLTwoVarLossGce}{4.3}
\newcommand{\dropTMflairBoundaryLTwoVarLossGce}{6.9}
\newcommand{\dropCITMflairBoundaryLTwoVarLossGce}{3.7}
\newcommand{\retTMflairBoundaryLTwoVarLossGce}{0.813}
\newcommand{\retCITMflairBoundaryLTwoVarLossGce}{0.103}
\newcommand{\nTMflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouTMflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{32.9}
\newcommand{\miouCITMflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{1.0}
\newcommand{\dropTMflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{5.3}
\newcommand{\dropCITMflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{1.6}
\newcommand{\retTMflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{0.863}
\newcommand{\retCITMflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{0.037}
\newcommand{\nTMflairBoundaryLR}{5}
\newcommand{\miouTMflairBoundaryLR}{32.4}
\newcommand{\miouCITMflairBoundaryLR}{0.8}
\newcommand{\dropTMflairBoundaryLR}{8.0}
\newcommand{\dropCITMflairBoundaryLR}{1.1}
\newcommand{\retTMflairBoundaryLR}{0.802}
\newcommand{\retCITMflairBoundaryLR}{0.023}
\newcommand{\nTMflairClean}{5}
\newcommand{\miouTMflairClean}{40.5}
\newcommand{\miouCITMflairClean}{1.2}
\newcommand{\nTMflairCleanVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouTMflairCleanVarDecoderMaskTwoformerFull}{42.8}
\newcommand{\miouCITMflairCleanVarDecoderMaskTwoformerFull}{1.0}
\newcommand{\nTMflairCleanVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouTMflairCleanVarDecoderMaskTwoformerLite}{41.4}
\newcommand{\miouCITMflairCleanVarDecoderMaskTwoformerLite}{1.3}
\newcommand{\nTMflairCleanVarDecoderSamLite}{5}
\newcommand{\miouTMflairCleanVarDecoderSamLite}{40.2}
\newcommand{\miouCITMflairCleanVarDecoderSamLite}{0.6}
\newcommand{\nTMflairCleanVarDecoderSamPretrained}{5}
\newcommand{\miouTMflairCleanVarDecoderSamPretrained}{39.3}
\newcommand{\miouCITMflairCleanVarDecoderSamPretrained}{1.5}
\newcommand{\nTMflairCleanVarDecoderSegformerMlp}{5}
\newcommand{\miouTMflairCleanVarDecoderSegformerMlp}{41.9}
\newcommand{\miouCITMflairCleanVarDecoderSegformerMlp}{0.5}
\newcommand{\nTMflairCleanVarFrozenEncoderTrue}{5}
\newcommand{\miouTMflairCleanVarFrozenEncoderTrue}{35.9}
\newcommand{\miouCITMflairCleanVarFrozenEncoderTrue}{2.1}
\newcommand{\nTMflairCleanVarLossBootstrap}{5}
\newcommand{\miouTMflairCleanVarLossBootstrap}{40.8}
\newcommand{\miouCITMflairCleanVarLossBootstrap}{1.8}
\newcommand{\nTMflairCleanVarLossGce}{5}
\newcommand{\miouTMflairCleanVarLossGce}{37.1}
\newcommand{\miouCITMflairCleanVarLossGce}{1.1}
\newcommand{\nTMflairCleanVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouTMflairCleanVarLrMultZeroThreeThreeThreeThree}{38.2}
\newcommand{\miouCITMflairCleanVarLrMultZeroThreeThreeThreeThree}{1.6}
\newcommand{\nTMflairCleanVarTrainSubsetCleanTwoFive}{5}
\newcommand{\miouTMflairCleanVarTrainSubsetCleanTwoFive}{31.3}
\newcommand{\miouCITMflairCleanVarTrainSubsetCleanTwoFive}{2.8}
\newcommand{\nTMflairCoarseLOne}{5}
\newcommand{\miouTMflairCoarseLOne}{39.6}
\newcommand{\miouCITMflairCoarseLOne}{0.6}
\newcommand{\dropTMflairCoarseLOne}{0.8}
\newcommand{\dropCITMflairCoarseLOne}{1.5}
\newcommand{\retTMflairCoarseLOne}{0.980}
\newcommand{\retCITMflairCoarseLOne}{0.037}
\newcommand{\nTMflairCoarseLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouTMflairCoarseLOneVarDecoderMaskTwoformerFull}{42.5}
\newcommand{\miouCITMflairCoarseLOneVarDecoderMaskTwoformerFull}{0.9}
\newcommand{\dropTMflairCoarseLOneVarDecoderMaskTwoformerFull}{0.3}
\newcommand{\dropCITMflairCoarseLOneVarDecoderMaskTwoformerFull}{1.3}
\newcommand{\retTMflairCoarseLOneVarDecoderMaskTwoformerFull}{0.993}
\newcommand{\retCITMflairCoarseLOneVarDecoderMaskTwoformerFull}{0.030}
\newcommand{\nTMflairCoarseLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouTMflairCoarseLOneVarDecoderMaskTwoformerLite}{40.6}
\newcommand{\miouCITMflairCoarseLOneVarDecoderMaskTwoformerLite}{1.1}
\newcommand{\dropTMflairCoarseLOneVarDecoderMaskTwoformerLite}{0.8}
\newcommand{\dropCITMflairCoarseLOneVarDecoderMaskTwoformerLite}{0.6}
\newcommand{\retTMflairCoarseLOneVarDecoderMaskTwoformerLite}{0.981}
\newcommand{\retCITMflairCoarseLOneVarDecoderMaskTwoformerLite}{0.015}
\newcommand{\nTMflairCoarseLOneVarDecoderSamLite}{5}
\newcommand{\miouTMflairCoarseLOneVarDecoderSamLite}{39.9}
\newcommand{\miouCITMflairCoarseLOneVarDecoderSamLite}{1.1}
\newcommand{\dropTMflairCoarseLOneVarDecoderSamLite}{0.3}
\newcommand{\dropCITMflairCoarseLOneVarDecoderSamLite}{0.8}
\newcommand{\retTMflairCoarseLOneVarDecoderSamLite}{0.994}
\newcommand{\retCITMflairCoarseLOneVarDecoderSamLite}{0.021}
\newcommand{\nTMflairCoarseLOneVarDecoderSamPretrained}{5}
\newcommand{\miouTMflairCoarseLOneVarDecoderSamPretrained}{38.3}
\newcommand{\miouCITMflairCoarseLOneVarDecoderSamPretrained}{1.8}
\newcommand{\dropTMflairCoarseLOneVarDecoderSamPretrained}{1.0}
\newcommand{\dropCITMflairCoarseLOneVarDecoderSamPretrained}{2.7}
\newcommand{\retTMflairCoarseLOneVarDecoderSamPretrained}{0.975}
\newcommand{\retCITMflairCoarseLOneVarDecoderSamPretrained}{0.069}
\newcommand{\nTMflairCoarseLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouTMflairCoarseLOneVarDecoderSegformerMlp}{40.1}
\newcommand{\miouCITMflairCoarseLOneVarDecoderSegformerMlp}{0.7}
\newcommand{\dropTMflairCoarseLOneVarDecoderSegformerMlp}{1.8}
\newcommand{\dropCITMflairCoarseLOneVarDecoderSegformerMlp}{1.0}
\newcommand{\retTMflairCoarseLOneVarDecoderSegformerMlp}{0.956}
\newcommand{\retCITMflairCoarseLOneVarDecoderSegformerMlp}{0.024}
\newcommand{\nTMflairCoarseLTwo}{5}
\newcommand{\miouTMflairCoarseLTwo}{34.8}
\newcommand{\miouCITMflairCoarseLTwo}{1.6}
\newcommand{\dropTMflairCoarseLTwo}{5.6}
\newcommand{\dropCITMflairCoarseLTwo}{2.0}
\newcommand{\retTMflairCoarseLTwo}{0.861}
\newcommand{\retCITMflairCoarseLTwo}{0.047}
\newcommand{\nTMflairCoarseLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouTMflairCoarseLTwoVarDecoderMaskTwoformerFull}{34.9}
\newcommand{\miouCITMflairCoarseLTwoVarDecoderMaskTwoformerFull}{0.8}
\newcommand{\dropTMflairCoarseLTwoVarDecoderMaskTwoformerFull}{7.9}
\newcommand{\dropCITMflairCoarseLTwoVarDecoderMaskTwoformerFull}{1.5}
\newcommand{\retTMflairCoarseLTwoVarDecoderMaskTwoformerFull}{0.815}
\newcommand{\retCITMflairCoarseLTwoVarDecoderMaskTwoformerFull}{0.031}
\newcommand{\nTMflairCoarseLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouTMflairCoarseLTwoVarDecoderMaskTwoformerLite}{35.6}
\newcommand{\miouCITMflairCoarseLTwoVarDecoderMaskTwoformerLite}{1.8}
\newcommand{\dropTMflairCoarseLTwoVarDecoderMaskTwoformerLite}{5.8}
\newcommand{\dropCITMflairCoarseLTwoVarDecoderMaskTwoformerLite}{1.9}
\newcommand{\retTMflairCoarseLTwoVarDecoderMaskTwoformerLite}{0.860}
\newcommand{\retCITMflairCoarseLTwoVarDecoderMaskTwoformerLite}{0.044}
\newcommand{\nTMflairCoarseLTwoVarDecoderSamLite}{5}
\newcommand{\miouTMflairCoarseLTwoVarDecoderSamLite}{35.2}
\newcommand{\miouCITMflairCoarseLTwoVarDecoderSamLite}{0.7}
\newcommand{\dropTMflairCoarseLTwoVarDecoderSamLite}{5.0}
\newcommand{\dropCITMflairCoarseLTwoVarDecoderSamLite}{1.0}
\newcommand{\retTMflairCoarseLTwoVarDecoderSamLite}{0.875}
\newcommand{\retCITMflairCoarseLTwoVarDecoderSamLite}{0.024}
\newcommand{\nTMflairCoarseLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouTMflairCoarseLTwoVarDecoderSamPretrained}{32.0}
\newcommand{\miouCITMflairCoarseLTwoVarDecoderSamPretrained}{1.7}
\newcommand{\dropTMflairCoarseLTwoVarDecoderSamPretrained}{7.2}
\newcommand{\dropCITMflairCoarseLTwoVarDecoderSamPretrained}{3.2}
\newcommand{\retTMflairCoarseLTwoVarDecoderSamPretrained}{0.817}
\newcommand{\retCITMflairCoarseLTwoVarDecoderSamPretrained}{0.077}
\newcommand{\nTMflairCoarseLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouTMflairCoarseLTwoVarDecoderSegformerMlp}{36.6}
\newcommand{\miouCITMflairCoarseLTwoVarDecoderSegformerMlp}{1.1}
\newcommand{\dropTMflairCoarseLTwoVarDecoderSegformerMlp}{5.3}
\newcommand{\dropCITMflairCoarseLTwoVarDecoderSegformerMlp}{1.5}
\newcommand{\retTMflairCoarseLTwoVarDecoderSegformerMlp}{0.873}
\newcommand{\retCITMflairCoarseLTwoVarDecoderSegformerMlp}{0.034}
\newcommand{\nTMflairCoarseLTwoVarLossBootstrap}{5}
\newcommand{\miouTMflairCoarseLTwoVarLossBootstrap}{34.8}
\newcommand{\miouCITMflairCoarseLTwoVarLossBootstrap}{1.0}
\newcommand{\dropTMflairCoarseLTwoVarLossBootstrap}{6.0}
\newcommand{\dropCITMflairCoarseLTwoVarLossBootstrap}{1.3}
\newcommand{\retTMflairCoarseLTwoVarLossBootstrap}{0.854}
\newcommand{\retCITMflairCoarseLTwoVarLossBootstrap}{0.027}
\newcommand{\nTMflairCoarseLTwoVarLossGce}{5}
\newcommand{\miouTMflairCoarseLTwoVarLossGce}{32.4}
\newcommand{\miouCITMflairCoarseLTwoVarLossGce}{1.5}
\newcommand{\dropTMflairCoarseLTwoVarLossGce}{4.7}
\newcommand{\dropCITMflairCoarseLTwoVarLossGce}{1.0}
\newcommand{\retTMflairCoarseLTwoVarLossGce}{0.872}
\newcommand{\retCITMflairCoarseLTwoVarLossGce}{0.029}
\newcommand{\nTMflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouTMflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{33.7}
\newcommand{\miouCITMflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{1.6}
\newcommand{\dropTMflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{4.4}
\newcommand{\dropCITMflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.8}
\newcommand{\retTMflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.884}
\newcommand{\retCITMflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{0.020}
\newcommand{\nTMflairCoarseLR}{5}
\newcommand{\miouTMflairCoarseLR}{30.9}
\newcommand{\miouCITMflairCoarseLR}{1.5}
\newcommand{\dropTMflairCoarseLR}{9.6}
\newcommand{\dropCITMflairCoarseLR}{2.5}
\newcommand{\retTMflairCoarseLR}{0.764}
\newcommand{\retCITMflairCoarseLR}{0.056}
\newcommand{\nTMflairOmissionLOne}{5}
\newcommand{\miouTMflairOmissionLOne}{37.1}
\newcommand{\miouCITMflairOmissionLOne}{2.2}
\newcommand{\dropTMflairOmissionLOne}{3.3}
\newcommand{\dropCITMflairOmissionLOne}{1.9}
\newcommand{\retTMflairOmissionLOne}{0.918}
\newcommand{\retCITMflairOmissionLOne}{0.047}
\newcommand{\nTMflairOmissionLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouTMflairOmissionLOneVarDecoderMaskTwoformerFull}{41.5}
\newcommand{\miouCITMflairOmissionLOneVarDecoderMaskTwoformerFull}{1.5}
\newcommand{\dropTMflairOmissionLOneVarDecoderMaskTwoformerFull}{1.3}
\newcommand{\dropCITMflairOmissionLOneVarDecoderMaskTwoformerFull}{1.4}
\newcommand{\retTMflairOmissionLOneVarDecoderMaskTwoformerFull}{0.970}
\newcommand{\retCITMflairOmissionLOneVarDecoderMaskTwoformerFull}{0.034}
\newcommand{\nTMflairOmissionLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouTMflairOmissionLOneVarDecoderMaskTwoformerLite}{38.7}
\newcommand{\miouCITMflairOmissionLOneVarDecoderMaskTwoformerLite}{1.8}
\newcommand{\dropTMflairOmissionLOneVarDecoderMaskTwoformerLite}{2.7}
\newcommand{\dropCITMflairOmissionLOneVarDecoderMaskTwoformerLite}{2.5}
\newcommand{\retTMflairOmissionLOneVarDecoderMaskTwoformerLite}{0.935}
\newcommand{\retCITMflairOmissionLOneVarDecoderMaskTwoformerLite}{0.058}
\newcommand{\nTMflairOmissionLOneVarDecoderSamLite}{5}
\newcommand{\miouTMflairOmissionLOneVarDecoderSamLite}{38.8}
\newcommand{\miouCITMflairOmissionLOneVarDecoderSamLite}{1.2}
\newcommand{\dropTMflairOmissionLOneVarDecoderSamLite}{1.4}
\newcommand{\dropCITMflairOmissionLOneVarDecoderSamLite}{0.9}
\newcommand{\retTMflairOmissionLOneVarDecoderSamLite}{0.966}
\newcommand{\retCITMflairOmissionLOneVarDecoderSamLite}{0.021}
\newcommand{\nTMflairOmissionLOneVarDecoderSamPretrained}{5}
\newcommand{\miouTMflairOmissionLOneVarDecoderSamPretrained}{37.1}
\newcommand{\miouCITMflairOmissionLOneVarDecoderSamPretrained}{1.0}
\newcommand{\dropTMflairOmissionLOneVarDecoderSamPretrained}{2.2}
\newcommand{\dropCITMflairOmissionLOneVarDecoderSamPretrained}{1.3}
\newcommand{\retTMflairOmissionLOneVarDecoderSamPretrained}{0.946}
\newcommand{\retCITMflairOmissionLOneVarDecoderSamPretrained}{0.033}
\newcommand{\nTMflairOmissionLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouTMflairOmissionLOneVarDecoderSegformerMlp}{39.6}
\newcommand{\miouCITMflairOmissionLOneVarDecoderSegformerMlp}{1.0}
\newcommand{\dropTMflairOmissionLOneVarDecoderSegformerMlp}{2.4}
\newcommand{\dropCITMflairOmissionLOneVarDecoderSegformerMlp}{1.0}
\newcommand{\retTMflairOmissionLOneVarDecoderSegformerMlp}{0.944}
\newcommand{\retCITMflairOmissionLOneVarDecoderSegformerMlp}{0.024}
\newcommand{\nTMflairOmissionLTwo}{5}
\newcommand{\miouTMflairOmissionLTwo}{35.0}
\newcommand{\miouCITMflairOmissionLTwo}{1.0}
\newcommand{\dropTMflairOmissionLTwo}{5.5}
\newcommand{\dropCITMflairOmissionLTwo}{1.6}
\newcommand{\retTMflairOmissionLTwo}{0.866}
\newcommand{\retCITMflairOmissionLTwo}{0.037}
\newcommand{\nTMflairOmissionLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouTMflairOmissionLTwoVarDecoderMaskTwoformerFull}{38.3}
\newcommand{\miouCITMflairOmissionLTwoVarDecoderMaskTwoformerFull}{1.0}
\newcommand{\dropTMflairOmissionLTwoVarDecoderMaskTwoformerFull}{4.5}
\newcommand{\dropCITMflairOmissionLTwoVarDecoderMaskTwoformerFull}{1.4}
\newcommand{\retTMflairOmissionLTwoVarDecoderMaskTwoformerFull}{0.894}
\newcommand{\retCITMflairOmissionLTwoVarDecoderMaskTwoformerFull}{0.032}
\newcommand{\nTMflairOmissionLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouTMflairOmissionLTwoVarDecoderMaskTwoformerLite}{35.0}
\newcommand{\miouCITMflairOmissionLTwoVarDecoderMaskTwoformerLite}{2.0}
\newcommand{\dropTMflairOmissionLTwoVarDecoderMaskTwoformerLite}{6.4}
\newcommand{\dropCITMflairOmissionLTwoVarDecoderMaskTwoformerLite}{1.8}
\newcommand{\retTMflairOmissionLTwoVarDecoderMaskTwoformerLite}{0.845}
\newcommand{\retCITMflairOmissionLTwoVarDecoderMaskTwoformerLite}{0.042}
\newcommand{\nTMflairOmissionLTwoVarDecoderSamLite}{5}
\newcommand{\miouTMflairOmissionLTwoVarDecoderSamLite}{34.5}
\newcommand{\miouCITMflairOmissionLTwoVarDecoderSamLite}{2.5}
\newcommand{\dropTMflairOmissionLTwoVarDecoderSamLite}{5.6}
\newcommand{\dropCITMflairOmissionLTwoVarDecoderSamLite}{2.3}
\newcommand{\retTMflairOmissionLTwoVarDecoderSamLite}{0.859}
\newcommand{\retCITMflairOmissionLTwoVarDecoderSamLite}{0.056}
\newcommand{\nTMflairOmissionLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouTMflairOmissionLTwoVarDecoderSamPretrained}{33.8}
\newcommand{\miouCITMflairOmissionLTwoVarDecoderSamPretrained}{2.4}
\newcommand{\dropTMflairOmissionLTwoVarDecoderSamPretrained}{5.4}
\newcommand{\dropCITMflairOmissionLTwoVarDecoderSamPretrained}{2.1}
\newcommand{\retTMflairOmissionLTwoVarDecoderSamPretrained}{0.862}
\newcommand{\retCITMflairOmissionLTwoVarDecoderSamPretrained}{0.054}
\newcommand{\nTMflairOmissionLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouTMflairOmissionLTwoVarDecoderSegformerMlp}{36.1}
\newcommand{\miouCITMflairOmissionLTwoVarDecoderSegformerMlp}{2.3}
\newcommand{\dropTMflairOmissionLTwoVarDecoderSegformerMlp}{5.8}
\newcommand{\dropCITMflairOmissionLTwoVarDecoderSegformerMlp}{2.3}
\newcommand{\retTMflairOmissionLTwoVarDecoderSegformerMlp}{0.861}
\newcommand{\retCITMflairOmissionLTwoVarDecoderSegformerMlp}{0.054}
\newcommand{\nTMflairOmissionLTwoVarFrozenEncoderTrue}{5}
\newcommand{\miouTMflairOmissionLTwoVarFrozenEncoderTrue}{34.2}
\newcommand{\miouCITMflairOmissionLTwoVarFrozenEncoderTrue}{1.4}
\newcommand{\dropTMflairOmissionLTwoVarFrozenEncoderTrue}{1.7}
\newcommand{\dropCITMflairOmissionLTwoVarFrozenEncoderTrue}{2.7}
\newcommand{\retTMflairOmissionLTwoVarFrozenEncoderTrue}{0.955}
\newcommand{\retCITMflairOmissionLTwoVarFrozenEncoderTrue}{0.075}
\newcommand{\nTMflairOmissionLTwoVarLossBootstrap}{5}
\newcommand{\miouTMflairOmissionLTwoVarLossBootstrap}{35.3}
\newcommand{\miouCITMflairOmissionLTwoVarLossBootstrap}{1.2}
\newcommand{\dropTMflairOmissionLTwoVarLossBootstrap}{5.5}
\newcommand{\dropCITMflairOmissionLTwoVarLossBootstrap}{1.7}
\newcommand{\retTMflairOmissionLTwoVarLossBootstrap}{0.865}
\newcommand{\retCITMflairOmissionLTwoVarLossBootstrap}{0.036}
\newcommand{\nTMflairOmissionLTwoVarLossGce}{5}
\newcommand{\miouTMflairOmissionLTwoVarLossGce}{31.5}
\newcommand{\miouCITMflairOmissionLTwoVarLossGce}{2.4}
\newcommand{\dropTMflairOmissionLTwoVarLossGce}{5.6}
\newcommand{\dropCITMflairOmissionLTwoVarLossGce}{2.5}
\newcommand{\retTMflairOmissionLTwoVarLossGce}{0.850}
\newcommand{\retCITMflairOmissionLTwoVarLossGce}{0.065}
\newcommand{\nTMflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouTMflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{34.1}
\newcommand{\miouCITMflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{1.0}
\newcommand{\dropTMflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{4.1}
\newcommand{\dropCITMflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{1.3}
\newcommand{\retTMflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{0.893}
\newcommand{\retCITMflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{0.032}
\newcommand{\nTMflairOmissionLR}{5}
\newcommand{\miouTMflairOmissionLR}{33.8}
\newcommand{\miouCITMflairOmissionLR}{1.3}
\newcommand{\dropTMflairOmissionLR}{6.6}
\newcommand{\dropCITMflairOmissionLR}{2.1}
\newcommand{\retTMflairOmissionLR}{0.837}
\newcommand{\retCITMflairOmissionLR}{0.048}
\newcommand{\nTMflairShiftLOne}{5}
\newcommand{\miouTMflairShiftLOne}{39.5}
\newcommand{\miouCITMflairShiftLOne}{1.6}
\newcommand{\dropTMflairShiftLOne}{1.0}
\newcommand{\dropCITMflairShiftLOne}{0.7}
\newcommand{\retTMflairShiftLOne}{0.976}
\newcommand{\retCITMflairShiftLOne}{0.018}
\newcommand{\nTMflairShiftLOneVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouTMflairShiftLOneVarDecoderMaskTwoformerFull}{42.7}
\newcommand{\miouCITMflairShiftLOneVarDecoderMaskTwoformerFull}{1.0}
\newcommand{\dropTMflairShiftLOneVarDecoderMaskTwoformerFull}{0.1}
\newcommand{\dropCITMflairShiftLOneVarDecoderMaskTwoformerFull}{1.6}
\newcommand{\retTMflairShiftLOneVarDecoderMaskTwoformerFull}{0.998}
\newcommand{\retCITMflairShiftLOneVarDecoderMaskTwoformerFull}{0.038}
\newcommand{\nTMflairShiftLOneVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouTMflairShiftLOneVarDecoderMaskTwoformerLite}{40.6}
\newcommand{\miouCITMflairShiftLOneVarDecoderMaskTwoformerLite}{2.0}
\newcommand{\dropTMflairShiftLOneVarDecoderMaskTwoformerLite}{0.8}
\newcommand{\dropCITMflairShiftLOneVarDecoderMaskTwoformerLite}{2.7}
\newcommand{\retTMflairShiftLOneVarDecoderMaskTwoformerLite}{0.982}
\newcommand{\retCITMflairShiftLOneVarDecoderMaskTwoformerLite}{0.064}
\newcommand{\nTMflairShiftLOneVarDecoderSamLite}{5}
\newcommand{\miouTMflairShiftLOneVarDecoderSamLite}{39.5}
\newcommand{\miouCITMflairShiftLOneVarDecoderSamLite}{0.5}
\newcommand{\dropTMflairShiftLOneVarDecoderSamLite}{0.7}
\newcommand{\dropCITMflairShiftLOneVarDecoderSamLite}{0.9}
\newcommand{\retTMflairShiftLOneVarDecoderSamLite}{0.982}
\newcommand{\retCITMflairShiftLOneVarDecoderSamLite}{0.022}
\newcommand{\nTMflairShiftLOneVarDecoderSamPretrained}{5}
\newcommand{\miouTMflairShiftLOneVarDecoderSamPretrained}{39.0}
\newcommand{\miouCITMflairShiftLOneVarDecoderSamPretrained}{0.8}
\newcommand{\dropTMflairShiftLOneVarDecoderSamPretrained}{0.3}
\newcommand{\dropCITMflairShiftLOneVarDecoderSamPretrained}{1.0}
\newcommand{\retTMflairShiftLOneVarDecoderSamPretrained}{0.993}
\newcommand{\retCITMflairShiftLOneVarDecoderSamPretrained}{0.026}
\newcommand{\nTMflairShiftLOneVarDecoderSegformerMlp}{5}
\newcommand{\miouTMflairShiftLOneVarDecoderSegformerMlp}{41.2}
\newcommand{\miouCITMflairShiftLOneVarDecoderSegformerMlp}{0.6}
\newcommand{\dropTMflairShiftLOneVarDecoderSegformerMlp}{0.7}
\newcommand{\dropCITMflairShiftLOneVarDecoderSegformerMlp}{0.5}
\newcommand{\retTMflairShiftLOneVarDecoderSegformerMlp}{0.984}
\newcommand{\retCITMflairShiftLOneVarDecoderSegformerMlp}{0.013}
\newcommand{\nTMflairShiftLTwo}{5}
\newcommand{\miouTMflairShiftLTwo}{36.7}
\newcommand{\miouCITMflairShiftLTwo}{1.4}
\newcommand{\dropTMflairShiftLTwo}{3.7}
\newcommand{\dropCITMflairShiftLTwo}{2.2}
\newcommand{\retTMflairShiftLTwo}{0.908}
\newcommand{\retCITMflairShiftLTwo}{0.052}
\newcommand{\nTMflairShiftLTwoVarDecoderMaskTwoformerFull}{5}
\newcommand{\miouTMflairShiftLTwoVarDecoderMaskTwoformerFull}{37.7}
\newcommand{\miouCITMflairShiftLTwoVarDecoderMaskTwoformerFull}{1.3}
\newcommand{\dropTMflairShiftLTwoVarDecoderMaskTwoformerFull}{5.1}
\newcommand{\dropCITMflairShiftLTwoVarDecoderMaskTwoformerFull}{1.2}
\newcommand{\retTMflairShiftLTwoVarDecoderMaskTwoformerFull}{0.880}
\newcommand{\retCITMflairShiftLTwoVarDecoderMaskTwoformerFull}{0.028}
\newcommand{\nTMflairShiftLTwoVarDecoderMaskTwoformerLite}{5}
\newcommand{\miouTMflairShiftLTwoVarDecoderMaskTwoformerLite}{36.8}
\newcommand{\miouCITMflairShiftLTwoVarDecoderMaskTwoformerLite}{1.4}
\newcommand{\dropTMflairShiftLTwoVarDecoderMaskTwoformerLite}{4.6}
\newcommand{\dropCITMflairShiftLTwoVarDecoderMaskTwoformerLite}{2.3}
\newcommand{\retTMflairShiftLTwoVarDecoderMaskTwoformerLite}{0.889}
\newcommand{\retCITMflairShiftLTwoVarDecoderMaskTwoformerLite}{0.051}
\newcommand{\nTMflairShiftLTwoVarDecoderSamLite}{5}
\newcommand{\miouTMflairShiftLTwoVarDecoderSamLite}{36.7}
\newcommand{\miouCITMflairShiftLTwoVarDecoderSamLite}{1.7}
\newcommand{\dropTMflairShiftLTwoVarDecoderSamLite}{3.4}
\newcommand{\dropCITMflairShiftLTwoVarDecoderSamLite}{1.6}
\newcommand{\retTMflairShiftLTwoVarDecoderSamLite}{0.914}
\newcommand{\retCITMflairShiftLTwoVarDecoderSamLite}{0.039}
\newcommand{\nTMflairShiftLTwoVarDecoderSamPretrained}{5}
\newcommand{\miouTMflairShiftLTwoVarDecoderSamPretrained}{33.9}
\newcommand{\miouCITMflairShiftLTwoVarDecoderSamPretrained}{3.4}
\newcommand{\dropTMflairShiftLTwoVarDecoderSamPretrained}{5.4}
\newcommand{\dropCITMflairShiftLTwoVarDecoderSamPretrained}{3.3}
\newcommand{\retTMflairShiftLTwoVarDecoderSamPretrained}{0.863}
\newcommand{\retCITMflairShiftLTwoVarDecoderSamPretrained}{0.081}
\newcommand{\nTMflairShiftLTwoVarDecoderSegformerMlp}{5}
\newcommand{\miouTMflairShiftLTwoVarDecoderSegformerMlp}{37.0}
\newcommand{\miouCITMflairShiftLTwoVarDecoderSegformerMlp}{0.7}
\newcommand{\dropTMflairShiftLTwoVarDecoderSegformerMlp}{4.9}
\newcommand{\dropCITMflairShiftLTwoVarDecoderSegformerMlp}{1.0}
\newcommand{\retTMflairShiftLTwoVarDecoderSegformerMlp}{0.883}
\newcommand{\retCITMflairShiftLTwoVarDecoderSegformerMlp}{0.022}
\newcommand{\nTMflairShiftLTwoVarLossBootstrap}{5}
\newcommand{\miouTMflairShiftLTwoVarLossBootstrap}{36.9}
\newcommand{\miouCITMflairShiftLTwoVarLossBootstrap}{0.6}
\newcommand{\dropTMflairShiftLTwoVarLossBootstrap}{3.9}
\newcommand{\dropCITMflairShiftLTwoVarLossBootstrap}{1.7}
\newcommand{\retTMflairShiftLTwoVarLossBootstrap}{0.904}
\newcommand{\retCITMflairShiftLTwoVarLossBootstrap}{0.039}
\newcommand{\nTMflairShiftLTwoVarLossGce}{5}
\newcommand{\miouTMflairShiftLTwoVarLossGce}{33.9}
\newcommand{\miouCITMflairShiftLTwoVarLossGce}{2.6}
\newcommand{\dropTMflairShiftLTwoVarLossGce}{3.2}
\newcommand{\dropCITMflairShiftLTwoVarLossGce}{2.6}
\newcommand{\retTMflairShiftLTwoVarLossGce}{0.914}
\newcommand{\retCITMflairShiftLTwoVarLossGce}{0.071}
\newcommand{\nTMflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{5}
\newcommand{\miouTMflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{35.1}
\newcommand{\miouCITMflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.9}
\newcommand{\dropTMflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{3.0}
\newcommand{\dropCITMflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{1.1}
\newcommand{\retTMflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.921}
\newcommand{\retCITMflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{0.026}
\newcommand{\nTMflairShiftLR}{5}
\newcommand{\miouTMflairShiftLR}{33.9}
\newcommand{\miouCITMflairShiftLR}{0.6}
\newcommand{\dropTMflairShiftLR}{6.6}
\newcommand{\dropCITMflairShiftLR}{1.6}
\newcommand{\retTMflairShiftLR}{0.838}
\newcommand{\retCITMflairShiftLR}{0.035}
\newcommand{\nTMKuroBoundaryLOne}{5}
\newcommand{\miouTMKuroBoundaryLOne}{54.4}
\newcommand{\miouCITMKuroBoundaryLOne}{2.8}
\newcommand{\dropTMKuroBoundaryLOne}{3.6}
\newcommand{\dropCITMKuroBoundaryLOne}{3.4}
\newcommand{\retTMKuroBoundaryLOne}{0.938}
\newcommand{\retCITMKuroBoundaryLOne}{0.058}
\newcommand{\nTMKuroBoundaryLTwo}{5}
\newcommand{\miouTMKuroBoundaryLTwo}{50.4}
\newcommand{\miouCITMKuroBoundaryLTwo}{3.2}
\newcommand{\dropTMKuroBoundaryLTwo}{7.6}
\newcommand{\dropCITMKuroBoundaryLTwo}{4.1}
\newcommand{\retTMKuroBoundaryLTwo}{0.870}
\newcommand{\retCITMKuroBoundaryLTwo}{0.068}
\newcommand{\nTMKuroCemsREALVarTrainSubsetRealcov}{5}
\newcommand{\miouTMKuroCemsREALVarTrainSubsetRealcov}{53.4}
\newcommand{\miouCITMKuroCemsREALVarTrainSubsetRealcov}{1.4}
\newcommand{\dropTMKuroCemsREALVarTrainSubsetRealcov}{0.7}
\newcommand{\dropCITMKuroCemsREALVarTrainSubsetRealcov}{1.7}
\newcommand{\retTMKuroCemsREALVarTrainSubsetRealcov}{0.987}
\newcommand{\retCITMKuroCemsREALVarTrainSubsetRealcov}{0.032}
\newcommand{\nTMKuroClean}{5}
\newcommand{\miouTMKuroClean}{58.0}
\newcommand{\miouCITMKuroClean}{1.4}
\newcommand{\nTMKuroCleanVarTrainSubsetRealcov}{5}
\newcommand{\miouTMKuroCleanVarTrainSubsetRealcov}{54.1}
\newcommand{\miouCITMKuroCleanVarTrainSubsetRealcov}{1.0}
\newcommand{\nTMKuroCoarseLOne}{5}
\newcommand{\miouTMKuroCoarseLOne}{57.1}
\newcommand{\miouCITMKuroCoarseLOne}{2.8}
\newcommand{\dropTMKuroCoarseLOne}{0.9}
\newcommand{\dropCITMKuroCoarseLOne}{3.2}
\newcommand{\retTMKuroCoarseLOne}{0.985}
\newcommand{\retCITMKuroCoarseLOne}{0.055}
\newcommand{\nTMKuroCoarseLTwo}{5}
\newcommand{\miouTMKuroCoarseLTwo}{49.2}
\newcommand{\miouCITMKuroCoarseLTwo}{3.0}
\newcommand{\dropTMKuroCoarseLTwo}{8.8}
\newcommand{\dropCITMKuroCoarseLTwo}{3.3}
\newcommand{\retTMKuroCoarseLTwo}{0.848}
\newcommand{\retCITMKuroCoarseLTwo}{0.055}
\newcommand{\nTMKuroOmissionLOne}{5}
\newcommand{\miouTMKuroOmissionLOne}{54.2}
\newcommand{\miouCITMKuroOmissionLOne}{2.2}
\newcommand{\dropTMKuroOmissionLOne}{3.8}
\newcommand{\dropCITMKuroOmissionLOne}{2.0}
\newcommand{\retTMKuroOmissionLOne}{0.934}
\newcommand{\retCITMKuroOmissionLOne}{0.034}
\newcommand{\nTMKuroOmissionLTwo}{5}
\newcommand{\miouTMKuroOmissionLTwo}{47.1}
\newcommand{\miouCITMKuroOmissionLTwo}{2.9}
\newcommand{\dropTMKuroOmissionLTwo}{10.9}
\newcommand{\dropCITMKuroOmissionLTwo}{4.0}
\newcommand{\retTMKuroOmissionLTwo}{0.813}
\newcommand{\retCITMKuroOmissionLTwo}{0.064}
\newcommand{\nTMKuroShiftLOne}{5}
\newcommand{\miouTMKuroShiftLOne}{56.1}
\newcommand{\miouCITMKuroShiftLOne}{2.4}
\newcommand{\dropTMKuroShiftLOne}{1.9}
\newcommand{\dropCITMKuroShiftLOne}{1.9}
\newcommand{\retTMKuroShiftLOne}{0.967}
\newcommand{\retCITMKuroShiftLOne}{0.033}
\newcommand{\nTMKuroShiftLTwo}{5}
\newcommand{\miouTMKuroShiftLTwo}{54.5}
\newcommand{\miouCITMKuroShiftLTwo}{1.3}
\newcommand{\dropTMKuroShiftLTwo}{3.5}
\newcommand{\dropCITMKuroShiftLTwo}{2.6}
\newcommand{\retTMKuroShiftLTwo}{0.939}
\newcommand{\retCITMKuroShiftLTwo}{0.043}
\newcommand{\nTMOemBoundaryLOne}{5}
\newcommand{\miouTMOemBoundaryLOne}{53.7}
\newcommand{\miouCITMOemBoundaryLOne}{0.7}
\newcommand{\dropTMOemBoundaryLOne}{1.5}
\newcommand{\dropCITMOemBoundaryLOne}{1.0}
\newcommand{\retTMOemBoundaryLOne}{0.972}
\newcommand{\retCITMOemBoundaryLOne}{0.018}
\newcommand{\nTMOemBoundaryLTwo}{5}
\newcommand{\miouTMOemBoundaryLTwo}{46.4}
\newcommand{\miouCITMOemBoundaryLTwo}{1.8}
\newcommand{\dropTMOemBoundaryLTwo}{8.9}
\newcommand{\dropCITMOemBoundaryLTwo}{1.9}
\newcommand{\retTMOemBoundaryLTwo}{0.839}
\newcommand{\retCITMOemBoundaryLTwo}{0.034}
\newcommand{\nTMOemClean}{5}
\newcommand{\miouTMOemClean}{55.2}
\newcommand{\miouCITMOemClean}{1.0}
\newcommand{\nTMOemCoarseLOne}{5}
\newcommand{\miouTMOemCoarseLOne}{55.4}
\newcommand{\miouCITMOemCoarseLOne}{1.3}
\newcommand{\dropTMOemCoarseLOne}{\ensuremath{-}0.2}
\newcommand{\dropCITMOemCoarseLOne}{0.6}
\newcommand{\retTMOemCoarseLOne}{1.004}
\newcommand{\retCITMOemCoarseLOne}{0.011}
\newcommand{\nTMOemCoarseLTwo}{5}
\newcommand{\miouTMOemCoarseLTwo}{50.6}
\newcommand{\miouCITMOemCoarseLTwo}{0.5}
\newcommand{\dropTMOemCoarseLTwo}{4.7}
\newcommand{\dropCITMOemCoarseLTwo}{1.1}
\newcommand{\retTMOemCoarseLTwo}{0.916}
\newcommand{\retCITMOemCoarseLTwo}{0.019}
\newcommand{\nTMOemOmissionLOne}{5}
\newcommand{\miouTMOemOmissionLOne}{52.3}
\newcommand{\miouCITMOemOmissionLOne}{0.9}
\newcommand{\dropTMOemOmissionLOne}{2.9}
\newcommand{\dropCITMOemOmissionLOne}{0.6}
\newcommand{\retTMOemOmissionLOne}{0.947}
\newcommand{\retCITMOemOmissionLOne}{0.010}
\newcommand{\nTMOemOmissionLTwo}{5}
\newcommand{\miouTMOemOmissionLTwo}{47.3}
\newcommand{\miouCITMOemOmissionLTwo}{0.8}
\newcommand{\dropTMOemOmissionLTwo}{7.9}
\newcommand{\dropCITMOemOmissionLTwo}{1.7}
\newcommand{\retTMOemOmissionLTwo}{0.857}
\newcommand{\retCITMOemOmissionLTwo}{0.028}
\newcommand{\nTMOemShiftLOne}{5}
\newcommand{\miouTMOemShiftLOne}{54.3}
\newcommand{\miouCITMOemShiftLOne}{1.3}
\newcommand{\dropTMOemShiftLOne}{0.9}
\newcommand{\dropCITMOemShiftLOne}{0.9}
\newcommand{\retTMOemShiftLOne}{0.984}
\newcommand{\retCITMOemShiftLOne}{0.017}
\newcommand{\nTMOemShiftLTwo}{5}
\newcommand{\miouTMOemShiftLTwo}{52.9}
\newcommand{\miouCITMOemShiftLTwo}{0.5}
\newcommand{\dropTMOemShiftLTwo}{2.4}
\newcommand{\dropCITMOemShiftLTwo}{0.8}
\newcommand{\retTMOemShiftLTwo}{0.957}
\newcommand{\retCITMOemShiftLTwo}{0.014}
\newcommand{\nTMsenClean}{5}
\newcommand{\miouTMsenClean}{87.5}
\newcommand{\miouCITMsenClean}{1.4}
\newcommand{\nTMsenOtsuLTwo}{5}
\newcommand{\miouTMsenOtsuLTwo}{71.4}
\newcommand{\miouCITMsenOtsuLTwo}{1.7}
\newcommand{\dropTMsenOtsuLTwo}{16.1}
\newcommand{\dropCITMsenOtsuLTwo}{2.4}
\newcommand{\retTMsenOtsuLTwo}{0.816}
\newcommand{\retCITMsenOtsuLTwo}{0.025}
\newcommand{\nTMSnTwoBoundaryLOne}{5}
\newcommand{\miouTMSnTwoBoundaryLOne}{80.2}
\newcommand{\miouCITMSnTwoBoundaryLOne}{0.7}
\newcommand{\dropTMSnTwoBoundaryLOne}{3.3}
\newcommand{\dropCITMSnTwoBoundaryLOne}{0.9}
\newcommand{\retTMSnTwoBoundaryLOne}{0.961}
\newcommand{\retCITMSnTwoBoundaryLOne}{0.010}
\newcommand{\nTMSnTwoBoundaryLTwo}{5}
\newcommand{\miouTMSnTwoBoundaryLTwo}{72.8}
\newcommand{\miouCITMSnTwoBoundaryLTwo}{0.9}
\newcommand{\dropTMSnTwoBoundaryLTwo}{10.7}
\newcommand{\dropCITMSnTwoBoundaryLTwo}{0.8}
\newcommand{\retTMSnTwoBoundaryLTwo}{0.872}
\newcommand{\retCITMSnTwoBoundaryLTwo}{0.010}
\newcommand{\nTMSnTwoClean}{5}
\newcommand{\miouTMSnTwoClean}{83.4}
\newcommand{\miouCITMSnTwoClean}{0.4}
\newcommand{\nTMSnTwoCoarseLOne}{5}
\newcommand{\miouTMSnTwoCoarseLOne}{81.3}
\newcommand{\miouCITMSnTwoCoarseLOne}{0.6}
\newcommand{\dropTMSnTwoCoarseLOne}{2.2}
\newcommand{\dropCITMSnTwoCoarseLOne}{0.7}
\newcommand{\retTMSnTwoCoarseLOne}{0.974}
\newcommand{\retCITMSnTwoCoarseLOne}{0.009}
\newcommand{\nTMSnTwoCoarseLTwo}{5}
\newcommand{\miouTMSnTwoCoarseLTwo}{71.2}
\newcommand{\miouCITMSnTwoCoarseLTwo}{1.2}
\newcommand{\dropTMSnTwoCoarseLTwo}{12.3}
\newcommand{\dropCITMSnTwoCoarseLTwo}{1.1}
\newcommand{\retTMSnTwoCoarseLTwo}{0.853}
\newcommand{\retCITMSnTwoCoarseLTwo}{0.013}
\newcommand{\nTMSnTwoOmissionLOne}{5}
\newcommand{\miouTMSnTwoOmissionLOne}{77.6}
\newcommand{\miouCITMSnTwoOmissionLOne}{1.6}
\newcommand{\dropTMSnTwoOmissionLOne}{5.9}
\newcommand{\dropCITMSnTwoOmissionLOne}{1.8}
\newcommand{\retTMSnTwoOmissionLOne}{0.930}
\newcommand{\retCITMSnTwoOmissionLOne}{0.021}
\newcommand{\nTMSnTwoOmissionLTwo}{5}
\newcommand{\miouTMSnTwoOmissionLTwo}{67.8}
\newcommand{\miouCITMSnTwoOmissionLTwo}{1.6}
\newcommand{\dropTMSnTwoOmissionLTwo}{15.6}
\newcommand{\dropCITMSnTwoOmissionLTwo}{1.8}
\newcommand{\retTMSnTwoOmissionLTwo}{0.813}
\newcommand{\retCITMSnTwoOmissionLTwo}{0.021}
\newcommand{\nTMSnTwoShiftLOne}{5}
\newcommand{\miouTMSnTwoShiftLOne}{81.6}
\newcommand{\miouCITMSnTwoShiftLOne}{0.7}
\newcommand{\dropTMSnTwoShiftLOne}{1.8}
\newcommand{\dropCITMSnTwoShiftLOne}{0.9}
\newcommand{\retTMSnTwoShiftLOne}{0.978}
\newcommand{\retCITMSnTwoShiftLOne}{0.010}
\newcommand{\nTMSnTwoShiftLTwo}{5}
\newcommand{\miouTMSnTwoShiftLTwo}{75.4}
\newcommand{\miouCITMSnTwoShiftLTwo}{0.8}
\newcommand{\dropTMSnTwoShiftLTwo}{8.0}
\newcommand{\dropCITMSnTwoShiftLTwo}{0.8}
\newcommand{\retTMSnTwoShiftLTwo}{0.904}
\newcommand{\retCITMSnTwoShiftLTwo}{0.010}
\newcommand{\nVitlRandomburnBoundaryLOneVarInitRandom}{5}
\newcommand{\miouVitlRandomburnBoundaryLOneVarInitRandom}{69.1}
\newcommand{\miouCIVitlRandomburnBoundaryLOneVarInitRandom}{1.0}
\newcommand{\dropVitlRandomburnBoundaryLOneVarInitRandom}{\ensuremath{-}0.2}
\newcommand{\dropCIVitlRandomburnBoundaryLOneVarInitRandom}{2.3}
\newcommand{\retVitlRandomburnBoundaryLOneVarInitRandom}{1.003}
\newcommand{\retCIVitlRandomburnBoundaryLOneVarInitRandom}{0.035}
\newcommand{\nVitlRandomburnBoundaryLTwoVarInitRandom}{5}
\newcommand{\miouVitlRandomburnBoundaryLTwoVarInitRandom}{64.8}
\newcommand{\miouCIVitlRandomburnBoundaryLTwoVarInitRandom}{1.7}
\newcommand{\dropVitlRandomburnBoundaryLTwoVarInitRandom}{4.2}
\newcommand{\dropCIVitlRandomburnBoundaryLTwoVarInitRandom}{3.2}
\newcommand{\retVitlRandomburnBoundaryLTwoVarInitRandom}{0.940}
\newcommand{\retCIVitlRandomburnBoundaryLTwoVarInitRandom}{0.045}
\newcommand{\nVitlRandomburnCleanVarInitRandom}{5}
\newcommand{\miouVitlRandomburnCleanVarInitRandom}{69.0}
\newcommand{\miouCIVitlRandomburnCleanVarInitRandom}{2.0}
\newcommand{\nVitlRandomburnCleanVarInitRandomLrMultOneZero}{1}
\newcommand{\miouVitlRandomburnCleanVarInitRandomLrMultOneZero}{61.4}
\newcommand{\miouCIVitlRandomburnCleanVarInitRandomLrMultOneZero}{--}
\newcommand{\nVitlRandomburnCleanVarInitRandomLrMultThree}{1}
\newcommand{\miouVitlRandomburnCleanVarInitRandomLrMultThree}{67.6}
\newcommand{\miouCIVitlRandomburnCleanVarInitRandomLrMultThree}{--}
\newcommand{\nVitlRandomburnCleanVarInitRandomTrainSubsetCleanTwoFive}{5}
\newcommand{\miouVitlRandomburnCleanVarInitRandomTrainSubsetCleanTwoFive}{61.7}
\newcommand{\miouCIVitlRandomburnCleanVarInitRandomTrainSubsetCleanTwoFive}{2.5}
\newcommand{\nVitlRandomburnCoarseLOneVarInitRandom}{5}
\newcommand{\miouVitlRandomburnCoarseLOneVarInitRandom}{68.2}
\newcommand{\miouCIVitlRandomburnCoarseLOneVarInitRandom}{1.1}
\newcommand{\dropVitlRandomburnCoarseLOneVarInitRandom}{0.8}
\newcommand{\dropCIVitlRandomburnCoarseLOneVarInitRandom}{2.6}
\newcommand{\retVitlRandomburnCoarseLOneVarInitRandom}{0.989}
\newcommand{\retCIVitlRandomburnCoarseLOneVarInitRandom}{0.038}
\newcommand{\nVitlRandomburnCoarseLTwoVarInitRandom}{5}
\newcommand{\miouVitlRandomburnCoarseLTwoVarInitRandom}{59.1}
\newcommand{\miouCIVitlRandomburnCoarseLTwoVarInitRandom}{2.2}
\newcommand{\dropVitlRandomburnCoarseLTwoVarInitRandom}{9.9}
\newcommand{\dropCIVitlRandomburnCoarseLTwoVarInitRandom}{2.9}
\newcommand{\retVitlRandomburnCoarseLTwoVarInitRandom}{0.858}
\newcommand{\retCIVitlRandomburnCoarseLTwoVarInitRandom}{0.039}
\newcommand{\nVitlRandomburnOmissionLOneVarInitRandom}{5}
\newcommand{\miouVitlRandomburnOmissionLOneVarInitRandom}{65.3}
\newcommand{\miouCIVitlRandomburnOmissionLOneVarInitRandom}{4.6}
\newcommand{\dropVitlRandomburnOmissionLOneVarInitRandom}{3.6}
\newcommand{\dropCIVitlRandomburnOmissionLOneVarInitRandom}{5.6}
\newcommand{\retVitlRandomburnOmissionLOneVarInitRandom}{0.948}
\newcommand{\retCIVitlRandomburnOmissionLOneVarInitRandom}{0.081}
\newcommand{\nVitlRandomburnOmissionLTwoVarInitRandom}{5}
\newcommand{\miouVitlRandomburnOmissionLTwoVarInitRandom}{54.7}
\newcommand{\miouCIVitlRandomburnOmissionLTwoVarInitRandom}{8.2}
\newcommand{\dropVitlRandomburnOmissionLTwoVarInitRandom}{14.3}
\newcommand{\dropCIVitlRandomburnOmissionLTwoVarInitRandom}{10.1}
\newcommand{\retVitlRandomburnOmissionLTwoVarInitRandom}{0.795}
\newcommand{\retCIVitlRandomburnOmissionLTwoVarInitRandom}{0.141}
\newcommand{\nVitlRandomburnShiftLOneVarInitRandom}{5}
\newcommand{\miouVitlRandomburnShiftLOneVarInitRandom}{69.0}
\newcommand{\miouCIVitlRandomburnShiftLOneVarInitRandom}{1.4}
\newcommand{\dropVitlRandomburnShiftLOneVarInitRandom}{0.0}
\newcommand{\dropCIVitlRandomburnShiftLOneVarInitRandom}{2.5}
\newcommand{\retVitlRandomburnShiftLOneVarInitRandom}{1.000}
\newcommand{\retCIVitlRandomburnShiftLOneVarInitRandom}{0.037}
\newcommand{\nVitlRandomburnShiftLTwoVarInitRandom}{5}
\newcommand{\miouVitlRandomburnShiftLTwoVarInitRandom}{63.4}
\newcommand{\miouCIVitlRandomburnShiftLTwoVarInitRandom}{2.4}
\newcommand{\dropVitlRandomburnShiftLTwoVarInitRandom}{5.6}
\newcommand{\dropCIVitlRandomburnShiftLTwoVarInitRandom}{4.2}
\newcommand{\retVitlRandomburnShiftLTwoVarInitRandom}{0.920}
\newcommand{\retCIVitlRandomburnShiftLTwoVarInitRandom}{0.059}
\newcommand{\nVitlRandomflairBoundaryLOneVarInitRandom}{5}
\newcommand{\miouVitlRandomflairBoundaryLOneVarInitRandom}{27.1}
\newcommand{\miouCIVitlRandomflairBoundaryLOneVarInitRandom}{1.5}
\newcommand{\dropVitlRandomflairBoundaryLOneVarInitRandom}{0.4}
\newcommand{\dropCIVitlRandomflairBoundaryLOneVarInitRandom}{2.1}
\newcommand{\retVitlRandomflairBoundaryLOneVarInitRandom}{0.988}
\newcommand{\retCIVitlRandomflairBoundaryLOneVarInitRandom}{0.076}
\newcommand{\nVitlRandomflairBoundaryLTwoVarInitRandom}{5}
\newcommand{\miouVitlRandomflairBoundaryLTwoVarInitRandom}{25.4}
\newcommand{\miouCIVitlRandomflairBoundaryLTwoVarInitRandom}{1.3}
\newcommand{\dropVitlRandomflairBoundaryLTwoVarInitRandom}{2.1}
\newcommand{\dropCIVitlRandomflairBoundaryLTwoVarInitRandom}{1.1}
\newcommand{\retVitlRandomflairBoundaryLTwoVarInitRandom}{0.925}
\newcommand{\retCIVitlRandomflairBoundaryLTwoVarInitRandom}{0.040}
\newcommand{\nVitlRandomflairCleanVarInitRandom}{5}
\newcommand{\miouVitlRandomflairCleanVarInitRandom}{27.5}
\newcommand{\miouCIVitlRandomflairCleanVarInitRandom}{1.5}
\newcommand{\nVitlRandomflairCleanVarInitRandomLrMultOne}{1}
\newcommand{\miouVitlRandomflairCleanVarInitRandomLrMultOne}{24.3}
\newcommand{\miouCIVitlRandomflairCleanVarInitRandomLrMultOne}{--}
\newcommand{\nVitlRandomflairCleanVarInitRandomLrMultOneZero}{1}
\newcommand{\miouVitlRandomflairCleanVarInitRandomLrMultOneZero}{25.3}
\newcommand{\miouCIVitlRandomflairCleanVarInitRandomLrMultOneZero}{--}
\newcommand{\nVitlRandomflairCleanVarInitRandomTrainSubsetCleanTwoFive}{5}
\newcommand{\miouVitlRandomflairCleanVarInitRandomTrainSubsetCleanTwoFive}{21.1}
\newcommand{\miouCIVitlRandomflairCleanVarInitRandomTrainSubsetCleanTwoFive}{0.8}
\newcommand{\nVitlRandomflairCoarseLOneVarInitRandom}{5}
\newcommand{\miouVitlRandomflairCoarseLOneVarInitRandom}{27.1}
\newcommand{\miouCIVitlRandomflairCoarseLOneVarInitRandom}{0.9}
\newcommand{\dropVitlRandomflairCoarseLOneVarInitRandom}{0.4}
\newcommand{\dropCIVitlRandomflairCoarseLOneVarInitRandom}{1.6}
\newcommand{\retVitlRandomflairCoarseLOneVarInitRandom}{0.986}
\newcommand{\retCIVitlRandomflairCoarseLOneVarInitRandom}{0.061}
\newcommand{\nVitlRandomflairCoarseLTwoVarInitRandom}{5}
\newcommand{\miouVitlRandomflairCoarseLTwoVarInitRandom}{24.0}
\newcommand{\miouCIVitlRandomflairCoarseLTwoVarInitRandom}{1.8}
\newcommand{\dropVitlRandomflairCoarseLTwoVarInitRandom}{3.5}
\newcommand{\dropCIVitlRandomflairCoarseLTwoVarInitRandom}{2.8}
\newcommand{\retVitlRandomflairCoarseLTwoVarInitRandom}{0.875}
\newcommand{\retCIVitlRandomflairCoarseLTwoVarInitRandom}{0.097}
\newcommand{\nVitlRandomflairOmissionLOneVarInitRandom}{5}
\newcommand{\miouVitlRandomflairOmissionLOneVarInitRandom}{27.1}
\newcommand{\miouCIVitlRandomflairOmissionLOneVarInitRandom}{1.5}
\newcommand{\dropVitlRandomflairOmissionLOneVarInitRandom}{0.4}
\newcommand{\dropCIVitlRandomflairOmissionLOneVarInitRandom}{2.8}
\newcommand{\retVitlRandomflairOmissionLOneVarInitRandom}{0.989}
\newcommand{\retCIVitlRandomflairOmissionLOneVarInitRandom}{0.101}
\newcommand{\nVitlRandomflairOmissionLTwoVarInitRandom}{5}
\newcommand{\miouVitlRandomflairOmissionLTwoVarInitRandom}{25.7}
\newcommand{\miouCIVitlRandomflairOmissionLTwoVarInitRandom}{1.8}
\newcommand{\dropVitlRandomflairOmissionLTwoVarInitRandom}{1.8}
\newcommand{\dropCIVitlRandomflairOmissionLTwoVarInitRandom}{2.2}
\newcommand{\retVitlRandomflairOmissionLTwoVarInitRandom}{0.935}
\newcommand{\retCIVitlRandomflairOmissionLTwoVarInitRandom}{0.082}
\newcommand{\nVitlRandomflairShiftLOneVarInitRandom}{5}
\newcommand{\miouVitlRandomflairShiftLOneVarInitRandom}{27.2}
\newcommand{\miouCIVitlRandomflairShiftLOneVarInitRandom}{1.5}
\newcommand{\dropVitlRandomflairShiftLOneVarInitRandom}{0.3}
\newcommand{\dropCIVitlRandomflairShiftLOneVarInitRandom}{2.1}
\newcommand{\retVitlRandomflairShiftLOneVarInitRandom}{0.991}
\newcommand{\retCIVitlRandomflairShiftLOneVarInitRandom}{0.078}
\newcommand{\nVitlRandomflairShiftLTwoVarInitRandom}{5}
\newcommand{\miouVitlRandomflairShiftLTwoVarInitRandom}{25.0}
\newcommand{\miouCIVitlRandomflairShiftLTwoVarInitRandom}{1.5}
\newcommand{\dropVitlRandomflairShiftLTwoVarInitRandom}{2.5}
\newcommand{\dropCIVitlRandomflairShiftLTwoVarInitRandom}{1.3}
\newcommand{\retVitlRandomflairShiftLTwoVarInitRandom}{0.910}
\newcommand{\retCIVitlRandomflairShiftLTwoVarInitRandom}{0.047}
\newcommand{\hlMeanDropLTwoSATburn}{18.1}
\newcommand{\hlMeanDropLTwoSATflair}{6.3}
\newcommand{\hlMeanDropLTwoLVDburn}{13.8}
\newcommand{\hlMeanDropLTwoLVDflair}{3.5}
\newcommand{\hlMeanDropLTwoDOFAburn}{17.3}
\newcommand{\hlMeanDropLTwoDOFAflair}{4.3}
\newcommand{\hlMeanDropLTwoTMburn}{12.7}
\newcommand{\hlMeanDropLTwoTMflair}{5.2}
\newcommand{\hlMeanDropLTwoRNburn}{15.1}
\newcommand{\hlMeanDropLTwoRNflair}{4.2}
\newcommand{\hlMeanDropLTwoPRIburn}{13.0}
\newcommand{\hlMeanDropLTwoPRIflair}{5.2}
\newcommand{\miouRNSSLburnClean}{88.2}
\newcommand{\hlMeanDropLTwoRNSSLburn}{16.9}
\newcommand{\miouRNSSLflairClean}{42.5}
\newcommand{\hlMeanDropLTwoRNSSLflair}{4.2}
\newcommand{\miouVITRburnClean}{69.0}
\newcommand{\hlMeanDropLTwoVITRburn}{8.5}
\newcommand{\miouVITRflairClean}{27.5}
\newcommand{\hlMeanDropLTwoVITRflair}{2.5}
\newcommand{\miouCNXLburnClean}{81.6}
\newcommand{\hlMeanDropLTwoCNXLburn}{16.0}
\newcommand{\miouCNXLflairClean}{47.6}
\newcommand{\hlMeanDropLTwoCNXLflair}{4.0}
\newcommand{\statFOneburnN}{8}
\newcommand{\statFOneburnEst}{4.3}
\newcommand{\statFOneburnCILo}{1.3}
\newcommand{\statFOneburnCIHi}{7.3}
\newcommand{\statFOneburnP}{0.011}
\newcommand{\statFOneburnPHolm}{0.011}
\newcommand{\statFOneburnMde}{4.8}
\newcommand{\statFOneburnWelchP}{0.015}
\newcommand{\statFOneburnTostN}{8}
\newcommand{\statFOneburnTostEst}{4.3}
\newcommand{\statFOneburnTostCILo}{1.9}
\newcommand{\statFOneburnTostCIHi}{6.7}
\newcommand{\statFOneburnTostP}{0.835}
\newcommand{\statFOneburnTostEquivalent}{no}
\newcommand{\statFOneflairN}{8}
\newcommand{\statFOneflairEst}{2.8}
\newcommand{\statFOneflairCILo}{1.8}
\newcommand{\statFOneflairCIHi}{3.8}
\newcommand{\statFOneflairP}{\ensuremath{<}0.001}
\newcommand{\statFOneflairPHolm}{\ensuremath{<}0.001}
\newcommand{\statFOneflairMde}{1.6}
\newcommand{\statFOneflairWelchP}{\ensuremath{<}0.001}
\newcommand{\statFOneflairTostN}{8}
\newcommand{\statFOneflairTostEst}{2.8}
\newcommand{\statFOneflairTostCILo}{2.0}
\newcommand{\statFOneflairTostCIHi}{3.6}
\newcommand{\statFOneflairTostP}{0.342}
\newcommand{\statFOneflairTostEquivalent}{no}
\newcommand{\statFTwoburnN}{8}
\newcommand{\statFTwoburnEst}{0.0}
\newcommand{\statFTwoburnCILo}{\ensuremath{-}2.8}
\newcommand{\statFTwoburnCIHi}{2.7}
\newcommand{\statFTwoburnP}{0.971}
\newcommand{\statFTwoburnPHolm}{1.000}
\newcommand{\statFTwoburnMde}{4.4}
\newcommand{\statFTwoburnWelchP}{0.976}
\newcommand{\statFTwoburnTostN}{8}
\newcommand{\statFTwoburnTostEst}{0.0}
\newcommand{\statFTwoburnTostCILo}{\ensuremath{-}2.2}
\newcommand{\statFTwoburnTostCIHi}{2.1}
\newcommand{\statFTwoburnTostP}{0.019}
\newcommand{\statFTwoburnTostEquivalent}{yes}
\newcommand{\statFTwoflairN}{5}
\newcommand{\statFTwoflairEst}{0.6}
\newcommand{\statFTwoflairCILo}{\ensuremath{-}2.0}
\newcommand{\statFTwoflairCIHi}{3.1}
\newcommand{\statFTwoflairP}{0.569}
\newcommand{\statFTwoflairPHolm}{1.000}
\newcommand{\statFTwoflairMde}{4.2}
\newcommand{\statFTwoflairWelchP}{0.464}
\newcommand{\statFTwoflairTostN}{5}
\newcommand{\statFTwoflairTostEst}{0.6}
\newcommand{\statFTwoflairTostCILo}{\ensuremath{-}1.4}
\newcommand{\statFTwoflairTostCIHi}{2.5}
\newcommand{\statFTwoflairTostP}{0.029}
\newcommand{\statFTwoflairTostEquivalent}{yes}
\newcommand{\statFThreeburnN}{5}
\newcommand{\statFThreeburnEst}{\ensuremath{-}5.4}
\newcommand{\statFThreeburnCILo}{\ensuremath{-}8.3}
\newcommand{\statFThreeburnCIHi}{\ensuremath{-}2.4}
\newcommand{\statFThreeburnP}{0.007}
\newcommand{\statFThreeburnPHolm}{0.007}
\newcommand{\statFThreeburnMde}{4.9}
\newcommand{\statFThreeburnWelchP}{0.001}
\newcommand{\statFThreeburnTostN}{5}
\newcommand{\statFThreeburnTostEst}{\ensuremath{-}5.4}
\newcommand{\statFThreeburnTostCILo}{\ensuremath{-}7.6}
\newcommand{\statFThreeburnTostCIHi}{\ensuremath{-}3.1}
\newcommand{\statFThreeburnTostP}{0.956}
\newcommand{\statFThreeburnTostEquivalent}{no}
\newcommand{\statFThreeflairN}{5}
\newcommand{\statFThreeflairEst}{\ensuremath{-}2.8}
\newcommand{\statFThreeflairCILo}{\ensuremath{-}3.8}
\newcommand{\statFThreeflairCIHi}{\ensuremath{-}1.9}
\newcommand{\statFThreeflairP}{0.001}
\newcommand{\statFThreeflairPHolm}{0.002}
\newcommand{\statFThreeflairMde}{1.5}
\newcommand{\statFThreeflairWelchP}{\ensuremath{<}0.001}
\newcommand{\statFThreeflairTostN}{5}
\newcommand{\statFThreeflairTostEst}{\ensuremath{-}2.8}
\newcommand{\statFThreeflairTostCILo}{\ensuremath{-}3.5}
\newcommand{\statFThreeflairTostCIHi}{\ensuremath{-}2.1}
\newcommand{\statFThreeflairTostP}{0.308}
\newcommand{\statFThreeflairTostEquivalent}{no}
\newcommand{\statFFourburnN}{5}
\newcommand{\statFFourburnEst}{14.4}
\newcommand{\statFFourburnCILo}{12.0}
\newcommand{\statFFourburnCIHi}{16.8}
\newcommand{\statFFourburnP}{\ensuremath{<}0.001}
\newcommand{\statFFourburnPHolm}{\ensuremath{<}0.001}
\newcommand{\statFFourburnMde}{4.0}
\newcommand{\statFFourburnWelchP}{\ensuremath{<}0.001}
\newcommand{\statFFourburnTostN}{5}
\newcommand{\statFFourburnTostEst}{14.4}
\newcommand{\statFFourburnTostCILo}{12.5}
\newcommand{\statFFourburnTostCIHi}{16.2}
\newcommand{\statFFourburnTostP}{1.000}
\newcommand{\statFFourburnTostEquivalent}{no}
\newcommand{\statFFourflairN}{5}
\newcommand{\statFFourflairEst}{\ensuremath{-}1.2}
\newcommand{\statFFourflairCILo}{\ensuremath{-}2.3}
\newcommand{\statFFourflairCIHi}{\ensuremath{-}0.1}
\newcommand{\statFFourflairP}{0.036}
\newcommand{\statFFourflairPHolm}{0.036}
\newcommand{\statFFourflairMde}{1.8}
\newcommand{\statFFourflairWelchP}{0.021}
\newcommand{\statFFourflairTostN}{5}
\newcommand{\statFFourflairTostEst}{\ensuremath{-}1.2}
\newcommand{\statFFourflairTostCILo}{\ensuremath{-}2.1}
\newcommand{\statFFourflairTostCIHi}{\ensuremath{-}0.4}
\newcommand{\statFFourflairTostP}{0.006}
\newcommand{\statFFourflairTostEquivalent}{yes}
\newcommand{\hlNRunsDuplicate}{0}
\newcommand{\hlNRunsTotal}{10,127}
\newcommand{\hlNRunsAnalysed}{10,017}
\newcommand{\hlNRunsCoreAnalysed}{758}
\newcommand{\hlNRunsExtAnalysed}{474}
\newcommand{\hlNRunsPostReviewAnalysed}{3,769}
\newcommand{\hlNRunsExtDatasetsAnalysed}{3,150}
\newcommand{\hlNRunsReviewAnalysed}{1,866}
\newcommand{\hlNRunsExcluded}{110}
\newcommand{\hlNRunsExcludedBlocks}{N17 and Q0}
\newcommand{\hlNRunsNSix}{44}
\newcommand{\hlHwBlockClassesSOne}{GB10 (30) and RTX PRO 6000 (20)}
\newcommand{\hlHwBlockNClassesSOne}{2}
\newcommand{\hlHwBlockMainClassSOne}{GB10}
\newcommand{\hlHwBlockClassesSTwo}{GB10 (10) and RTX PRO 6000 (10)}
\newcommand{\hlHwBlockNClassesSTwo}{2}
\newcommand{\hlHwBlockMainClassSTwo}{RTX PRO 6000}
\newcommand{\hlHwBlockClassesSThree}{GB10 (25), RTX 4090 (30) and RTX PRO 6000 (45)}
\newcommand{\hlHwBlockNClassesSThree}{3}
\newcommand{\hlHwBlockMainClassSThree}{RTX PRO 6000}
\newcommand{\hlHwBlockClassesSFour}{RTX 4090 (90) and RTX PRO 6000 (10)}
\newcommand{\hlHwBlockNClassesSFour}{2}
\newcommand{\hlHwBlockMainClassSFour}{RTX 4090}
\newcommand{\hlHwBlockClassesSFive}{RTX PRO 6000 (104)}
\newcommand{\hlHwBlockNClassesSFive}{1}
\newcommand{\hlHwBlockMainClassSFive}{RTX PRO 6000}
\newcommand{\hlHwBlockClassesSSix}{RTX PRO 6000 (100)}
\newcommand{\hlHwBlockNClassesSSix}{1}
\newcommand{\hlHwBlockMainClassSSix}{RTX PRO 6000}
\newcommand{\hlNCells}{1622}
\newcommand{\hlNCellsComplete}{1604}
\newcommand{\hlRetSATburn}{76.5}
\newcommand{\hlRetLVDburn}{83.1}
\newcommand{\hlRetDiffburn}{\ensuremath{-}6.6}
\newcommand{\hlRetDiffCILoburn}{\ensuremath{-}9.8}
\newcommand{\hlRetDiffCIHiburn}{\ensuremath{-}3.4}
\newcommand{\hlRetDiffNburn}{8}
\newcommand{\hlRetSATflair}{87.9}
\newcommand{\hlRetLVDflair}{93.1}
\newcommand{\hlRetDiffflair}{\ensuremath{-}5.2}
\newcommand{\hlRetDiffCILoflair}{\ensuremath{-}7.1}
\newcommand{\hlRetDiffCIHiflair}{\ensuremath{-}3.3}
\newcommand{\hlRetDiffNflair}{8}
\newcommand{\hlWorstTypeburn}{coarse}
\newcommand{\hlWorstTypeDropburn}{18.4}
\newcommand{\hlWorstTypeChes}{coarse}
\newcommand{\hlWorstTypeDropChes}{12.1}
\newcommand{\hlWorstTypeCsTwelve}{coarse}
\newcommand{\hlWorstTypeDropCsTwelve}{7.8}
\newcommand{\hlWorstTypeDfc}{boundary}
\newcommand{\hlWorstTypeDropDfc}{4.2}
\newcommand{\hlWorstTypeEnva}{omission}
\newcommand{\hlWorstTypeDropEnva}{14.8}
\newcommand{\hlWorstTypeflair}{coarse}
\newcommand{\hlWorstTypeDropflair}{5.6}
\newcommand{\hlWorstTypeKuro}{omission}
\newcommand{\hlWorstTypeDropKuro}{7.9}
\newcommand{\hlWorstTypeOem}{boundary}
\newcommand{\hlWorstTypeDropOem}{9.1}
\newcommand{\hlWorstTypeSnTwo}{omission}
\newcommand{\hlWorstTypeDropSnTwo}{16.4}
\newcommand{\hlCElevenWorstburn}{coarse}
\newcommand{\hlCElevenWorstflair}{omission}
\newcommand{\hlRetMeanSATburn}{76.5}
\newcommand{\hlRetMeanSATflair}{87.9}
\newcommand{\hlRetMeanLVDburn}{83.1}
\newcommand{\hlRetMeanLVDflair}{93.1}
\newcommand{\hlRetMeanDOFAburn}{79.7}
\newcommand{\hlRetMeanDOFAflair}{90.9}
\newcommand{\hlRetMeanTMburn}{85.3}
\newcommand{\hlRetMeanTMflair}{87.1}
\newcommand{\hlRetMeanRNburn}{82.9}
\newcommand{\hlRetMeanRNflair}{90.6}
\newcommand{\hlRNRGBburn}{78.9}
\newcommand{\hlRNRGBburnN}{5}
\newcommand{\hlTypeRankburnOne}{coarse}
\newcommand{\hlTypeRankDropburnOne}{18.4}
\newcommand{\hlTypeRankDiffburnOne}{0.2}
\newcommand{\hlTypeRankDiffCILoburnOne}{\ensuremath{-}2.0}
\newcommand{\hlTypeRankDiffCIHiburnOne}{2.4}
\newcommand{\hlTypeRankburnTwo}{omission}
\newcommand{\hlTypeRankDropburnTwo}{18.2}
\newcommand{\hlTypeRankDiffburnTwo}{4.8}
\newcommand{\hlTypeRankDiffCILoburnTwo}{2.6}
\newcommand{\hlTypeRankDiffCIHiburnTwo}{7.1}
\newcommand{\hlTypeRankburnThree}{boundary}
\newcommand{\hlTypeRankDropburnThree}{13.4}
\newcommand{\hlTypeRankDiffburnThree}{1.7}
\newcommand{\hlTypeRankDiffCILoburnThree}{0.6}
\newcommand{\hlTypeRankDiffCIHiburnThree}{2.8}
\newcommand{\hlTypeRankburnFour}{shift}
\newcommand{\hlTypeRankDropburnFour}{11.7}
\newcommand{\hlHTwoDiffburn}{4.8}
\newcommand{\hlHTwoDiffCILoburn}{2.6}
\newcommand{\hlHTwoDiffCIHiburn}{7.1}
\newcommand{\hlHTwoDiffNburn}{40}
\newcommand{\hlTypeRankChesOne}{coarse}
\newcommand{\hlTypeRankDropChesOne}{12.1}
\newcommand{\hlTypeRankDiffChesOne}{1.0}
\newcommand{\hlTypeRankDiffCILoChesOne}{0.1}
\newcommand{\hlTypeRankDiffCIHiChesOne}{1.9}
\newcommand{\hlTypeRankChesTwo}{boundary}
\newcommand{\hlTypeRankDropChesTwo}{11.1}
\newcommand{\hlTypeRankDiffChesTwo}{0.8}
\newcommand{\hlTypeRankDiffCILoChesTwo}{\ensuremath{-}0.8}
\newcommand{\hlTypeRankDiffCIHiChesTwo}{2.4}
\newcommand{\hlTypeRankChesThree}{omission}
\newcommand{\hlTypeRankDropChesThree}{10.3}
\newcommand{\hlTypeRankDiffChesThree}{3.1}
\newcommand{\hlTypeRankDiffCILoChesThree}{1.1}
\newcommand{\hlTypeRankDiffCIHiChesThree}{5.0}
\newcommand{\hlTypeRankChesFour}{shift}
\newcommand{\hlTypeRankDropChesFour}{7.3}
\newcommand{\hlHTwoDiffChes}{\ensuremath{-}0.8}
\newcommand{\hlHTwoDiffCILoChes}{\ensuremath{-}2.4}
\newcommand{\hlHTwoDiffCIHiChes}{0.8}
\newcommand{\hlHTwoDiffNChes}{25}
\newcommand{\hlTypeRankCsTwelveOne}{coarse}
\newcommand{\hlTypeRankDropCsTwelveOne}{7.8}
\newcommand{\hlTypeRankDiffCsTwelveOne}{0.8}
\newcommand{\hlTypeRankDiffCILoCsTwelveOne}{0.3}
\newcommand{\hlTypeRankDiffCIHiCsTwelveOne}{1.2}
\newcommand{\hlTypeRankCsTwelveTwo}{omission}
\newcommand{\hlTypeRankDropCsTwelveTwo}{7.0}
\newcommand{\hlTypeRankDiffCsTwelveTwo}{0.3}
\newcommand{\hlTypeRankDiffCILoCsTwelveTwo}{\ensuremath{-}0.6}
\newcommand{\hlTypeRankDiffCIHiCsTwelveTwo}{1.1}
\newcommand{\hlTypeRankCsTwelveThree}{boundary}
\newcommand{\hlTypeRankDropCsTwelveThree}{6.8}
\newcommand{\hlTypeRankDiffCsTwelveThree}{1.7}
\newcommand{\hlTypeRankDiffCILoCsTwelveThree}{0.9}
\newcommand{\hlTypeRankDiffCIHiCsTwelveThree}{2.5}
\newcommand{\hlTypeRankCsTwelveFour}{shift}
\newcommand{\hlTypeRankDropCsTwelveFour}{5.1}
\newcommand{\hlHTwoDiffCsTwelve}{0.3}
\newcommand{\hlHTwoDiffCILoCsTwelve}{\ensuremath{-}0.6}
\newcommand{\hlHTwoDiffCIHiCsTwelve}{1.1}
\newcommand{\hlHTwoDiffNCsTwelve}{25}
\newcommand{\hlTypeRankDfcOne}{boundary}
\newcommand{\hlTypeRankDropDfcOne}{4.2}
\newcommand{\hlTypeRankDiffDfcOne}{0.7}
\newcommand{\hlTypeRankDiffCILoDfcOne}{\ensuremath{-}0.6}
\newcommand{\hlTypeRankDiffCIHiDfcOne}{2.0}
\newcommand{\hlTypeRankDfcTwo}{omission}
\newcommand{\hlTypeRankDropDfcTwo}{3.5}
\newcommand{\hlTypeRankDiffDfcTwo}{2.2}
\newcommand{\hlTypeRankDiffCILoDfcTwo}{1.4}
\newcommand{\hlTypeRankDiffCIHiDfcTwo}{3.0}
\newcommand{\hlTypeRankDfcThree}{coarse}
\newcommand{\hlTypeRankDropDfcThree}{1.4}
\newcommand{\hlTypeRankDiffDfcThree}{1.3}
\newcommand{\hlTypeRankDiffCILoDfcThree}{0.7}
\newcommand{\hlTypeRankDiffCIHiDfcThree}{1.9}
\newcommand{\hlTypeRankDfcFour}{shift}
\newcommand{\hlTypeRankDropDfcFour}{0.1}
\newcommand{\hlHTwoDiffDfc}{\ensuremath{-}0.7}
\newcommand{\hlHTwoDiffCILoDfc}{\ensuremath{-}2.0}
\newcommand{\hlHTwoDiffCIHiDfc}{0.6}
\newcommand{\hlHTwoDiffNDfc}{25}
\newcommand{\hlTypeRankEnvaOne}{omission}
\newcommand{\hlTypeRankDropEnvaOne}{14.8}
\newcommand{\hlTypeRankDiffEnvaOne}{5.2}
\newcommand{\hlTypeRankDiffCILoEnvaOne}{2.1}
\newcommand{\hlTypeRankDiffCIHiEnvaOne}{8.4}
\newcommand{\hlTypeRankEnvaTwo}{boundary}
\newcommand{\hlTypeRankDropEnvaTwo}{9.5}
\newcommand{\hlTypeRankDiffEnvaTwo}{6.3}
\newcommand{\hlTypeRankDiffCILoEnvaTwo}{3.2}
\newcommand{\hlTypeRankDiffCIHiEnvaTwo}{9.4}
\newcommand{\hlTypeRankEnvaThree}{coarse}
\newcommand{\hlTypeRankDropEnvaThree}{3.2}
\newcommand{\hlTypeRankDiffEnvaThree}{0.0}
\newcommand{\hlTypeRankDiffCILoEnvaThree}{\ensuremath{-}2.5}
\newcommand{\hlTypeRankDiffCIHiEnvaThree}{2.6}
\newcommand{\hlTypeRankEnvaFour}{shift}
\newcommand{\hlTypeRankDropEnvaFour}{3.2}
\newcommand{\hlHTwoDiffEnva}{5.2}
\newcommand{\hlHTwoDiffCILoEnva}{2.1}
\newcommand{\hlHTwoDiffCIHiEnva}{8.4}
\newcommand{\hlHTwoDiffNEnva}{25}
\newcommand{\hlTypeRankflairOne}{coarse}
\newcommand{\hlTypeRankDropflairOne}{5.6}
\newcommand{\hlTypeRankDiffflairOne}{0.4}
\newcommand{\hlTypeRankDiffCILoflairOne}{\ensuremath{-}0.1}
\newcommand{\hlTypeRankDiffCIHiflairOne}{1.0}
\newcommand{\hlTypeRankflairTwo}{boundary}
\newcommand{\hlTypeRankDropflairTwo}{5.1}
\newcommand{\hlTypeRankDiffflairTwo}{0.0}
\newcommand{\hlTypeRankDiffCILoflairTwo}{\ensuremath{-}0.6}
\newcommand{\hlTypeRankDiffCIHiflairTwo}{0.7}
\newcommand{\hlTypeRankflairThree}{omission}
\newcommand{\hlTypeRankDropflairThree}{4.9}
\newcommand{\hlTypeRankDiffflairThree}{1.9}
\newcommand{\hlTypeRankDiffCILoflairThree}{1.2}
\newcommand{\hlTypeRankDiffCIHiflairThree}{2.5}
\newcommand{\hlTypeRankflairFour}{shift}
\newcommand{\hlTypeRankDropflairFour}{3.3}
\newcommand{\hlHTwoDiffflair}{0.0}
\newcommand{\hlHTwoDiffCILoflair}{\ensuremath{-}0.7}
\newcommand{\hlHTwoDiffCIHiflair}{0.6}
\newcommand{\hlHTwoDiffNflair}{31}
\newcommand{\hlTypeRankKuroOne}{omission}
\newcommand{\hlTypeRankDropKuroOne}{7.9}
\newcommand{\hlTypeRankDiffKuroOne}{2.2}
\newcommand{\hlTypeRankDiffCILoKuroOne}{0.3}
\newcommand{\hlTypeRankDiffCIHiKuroOne}{4.1}
\newcommand{\hlTypeRankKuroTwo}{coarse}
\newcommand{\hlTypeRankDropKuroTwo}{5.8}
\newcommand{\hlTypeRankDiffKuroTwo}{0.4}
\newcommand{\hlTypeRankDiffCILoKuroTwo}{\ensuremath{-}0.9}
\newcommand{\hlTypeRankDiffCIHiKuroTwo}{1.6}
\newcommand{\hlTypeRankKuroThree}{boundary}
\newcommand{\hlTypeRankDropKuroThree}{5.4}
\newcommand{\hlTypeRankDiffKuroThree}{2.6}
\newcommand{\hlTypeRankDiffCILoKuroThree}{1.3}
\newcommand{\hlTypeRankDiffCIHiKuroThree}{4.0}
\newcommand{\hlTypeRankKuroFour}{shift}
\newcommand{\hlTypeRankDropKuroFour}{2.8}
\newcommand{\hlHTwoDiffKuro}{2.5}
\newcommand{\hlHTwoDiffCILoKuro}{1.0}
\newcommand{\hlHTwoDiffCIHiKuro}{4.1}
\newcommand{\hlHTwoDiffNKuro}{25}
\newcommand{\hlTypeRankOemOne}{boundary}
\newcommand{\hlTypeRankDropOemOne}{9.1}
\newcommand{\hlTypeRankDiffOemOne}{0.7}
\newcommand{\hlTypeRankDiffCILoOemOne}{0.1}
\newcommand{\hlTypeRankDiffCIHiOemOne}{1.3}
\newcommand{\hlTypeRankOemTwo}{omission}
\newcommand{\hlTypeRankDropOemTwo}{8.3}
\newcommand{\hlTypeRankDiffOemTwo}{3.0}
\newcommand{\hlTypeRankDiffCILoOemTwo}{2.0}
\newcommand{\hlTypeRankDiffCIHiOemTwo}{4.0}
\newcommand{\hlTypeRankOemThree}{coarse}
\newcommand{\hlTypeRankDropOemThree}{5.4}
\newcommand{\hlTypeRankDiffOemThree}{2.2}
\newcommand{\hlTypeRankDiffCILoOemThree}{1.7}
\newcommand{\hlTypeRankDiffCIHiOemThree}{2.6}
\newcommand{\hlTypeRankOemFour}{shift}
\newcommand{\hlTypeRankDropOemFour}{3.2}
\newcommand{\hlHTwoDiffOem}{\ensuremath{-}0.7}
\newcommand{\hlHTwoDiffCILoOem}{\ensuremath{-}1.3}
\newcommand{\hlHTwoDiffCIHiOem}{\ensuremath{-}0.1}
\newcommand{\hlHTwoDiffNOem}{25}
\newcommand{\hlTypeRankSnTwoOne}{omission}
\newcommand{\hlTypeRankDropSnTwoOne}{16.4}
\newcommand{\hlTypeRankDiffSnTwoOne}{4.0}
\newcommand{\hlTypeRankDiffCILoSnTwoOne}{2.0}
\newcommand{\hlTypeRankDiffCIHiSnTwoOne}{5.9}
\newcommand{\hlTypeRankSnTwoTwo}{coarse}
\newcommand{\hlTypeRankDropSnTwoTwo}{12.4}
\newcommand{\hlTypeRankDiffSnTwoTwo}{1.9}
\newcommand{\hlTypeRankDiffCILoSnTwoTwo}{1.1}
\newcommand{\hlTypeRankDiffCIHiSnTwoTwo}{2.7}
\newcommand{\hlTypeRankSnTwoThree}{boundary}
\newcommand{\hlTypeRankDropSnTwoThree}{10.5}
\newcommand{\hlTypeRankDiffSnTwoThree}{2.4}
\newcommand{\hlTypeRankDiffCILoSnTwoThree}{1.7}
\newcommand{\hlTypeRankDiffCIHiSnTwoThree}{3.1}
\newcommand{\hlTypeRankSnTwoFour}{shift}
\newcommand{\hlTypeRankDropSnTwoFour}{8.1}
\newcommand{\hlHTwoDiffSnTwo}{5.9}
\newcommand{\hlHTwoDiffCILoSnTwo}{3.6}
\newcommand{\hlHTwoDiffCIHiSnTwo}{8.2}
\newcommand{\hlHTwoDiffNSnTwo}{25}
\newcommand{\hlMemRateSATburn}{72.6}
\newcommand{\hlMemRateCISATburn}{10.5}
\newcommand{\hlMemPerClassSATburnBackground}{18.4}
\newcommand{\hlMemPerClassSATburnBackgroundCI}{15.8}
\newcommand{\hlMemPerClassSATburnBurnScar}{79.2}
\newcommand{\hlMemPerClassSATburnBurnScarCI}{13.9}
\newcommand{\hlMemRateLVDburn}{81.0}
\newcommand{\hlMemRateCILVDburn}{5.2}
\newcommand{\hlMemPerClassLVDburnBackground}{20.4}
\newcommand{\hlMemPerClassLVDburnBackgroundCI}{10.3}
\newcommand{\hlMemPerClassLVDburnBurnScar}{88.0}
\newcommand{\hlMemPerClassLVDburnBurnScarCI}{5.7}
\newcommand{\hlMemRateDOFAburn}{80.7}
\newcommand{\hlMemRateCIDOFAburn}{7.2}
\newcommand{\hlMemPerClassDOFAburnBackground}{17.1}
\newcommand{\hlMemPerClassDOFAburnBackgroundCI}{11.1}
\newcommand{\hlMemPerClassDOFAburnBurnScar}{87.9}
\newcommand{\hlMemPerClassDOFAburnBurnScarCI}{6.7}
\newcommand{\hlMemRateTMburn}{75.8}
\newcommand{\hlMemRateCITMburn}{5.0}
\newcommand{\hlMemPerClassTMburnBackground}{15.3}
\newcommand{\hlMemPerClassTMburnBackgroundCI}{14.9}
\newcommand{\hlMemPerClassTMburnBurnScar}{82.6}
\newcommand{\hlMemPerClassTMburnBurnScarCI}{5.2}
\newcommand{\hlMemRateRNburn}{80.4}
\newcommand{\hlMemRateCIRNburn}{5.2}
\newcommand{\hlMemPerClassRNburnBackground}{22.1}
\newcommand{\hlMemPerClassRNburnBackgroundCI}{15.6}
\newcommand{\hlMemPerClassRNburnBurnScar}{87.1}
\newcommand{\hlMemPerClassRNburnBurnScarCI}{4.2}
\newcommand{\hlMemRateSATNSixburn}{82.3}
\newcommand{\hlMemRateCISATNSixburn}{5.0}
\newcommand{\hlMemPerClassSATNSixburnBackground}{21.1}
\newcommand{\hlMemPerClassSATNSixburnBackgroundCI}{13.7}
\newcommand{\hlMemPerClassSATNSixburnBurnScar}{89.9}
\newcommand{\hlMemPerClassSATNSixburnBurnScarCI}{2.3}
\newcommand{\hlMemRateSATflair}{43.1}
\newcommand{\hlMemRateCISATflair}{13.1}
\newcommand{\hlMemRateLVDflair}{25.2}
\newcommand{\hlMemRateCILVDflair}{7.6}
\newcommand{\hlMemRateDOFAflair}{37.6}
\newcommand{\hlMemRateCIDOFAflair}{7.3}
\newcommand{\hlMemRateTMflair}{37.0}
\newcommand{\hlMemRateCITMflair}{9.4}
\newcommand{\hlMemRateRNflair}{18.6}
\newcommand{\hlMemRateCIRNflair}{5.6}
\newcommand{\hlMemRateSATNSixflair}{39.1}
\newcommand{\hlMemRateCISATNSixflair}{14.6}
\newcommand{\hlNCollapsedburn}{9}
\newcommand{\hlRealSlopeburnOmission}{\ensuremath{-}1.36}
\newcommand{\hlRealSlopeflairOmission}{\ensuremath{-}0.44}
\newcommand{\hlBreakEvenburn}{\ensuremath{>}4.0}
\newcommand{\hlBreakEvenFStarburn}{0.006}
\newcommand{\hlBreakEvenExtrapolatedburn}{yes}
\newcommand{\hlBreakEvenflair}{3.0}
\newcommand{\hlBreakEvenFStarflair}{0.335}
\newcommand{\hlBreakEvenExtrapolatedflair}{no}
\newcommand{\hlFlipRankburn}{\etype{omission}, \etype{coarse}, \etype{boundary} and \etype{shift}}
\newcommand{\hlFlipRankCommonPctburn}{5.88}
\newcommand{\hlFlipRankChangedburn}{yes}
\newcommand{\hlFlipRankflair}{\etype{omission}, \etype{boundary}, \etype{coarse} and \etype{shift}}
\newcommand{\hlFlipRankCommonPctflair}{16.71}
\newcommand{\hlFlipRankChangedflair}{yes}
\newcommand{\hlAblContrastAThreeburnEst}{\ensuremath{-}5.4}
\newcommand{\hlAblContrastAThreeburnCILo}{\ensuremath{-}8.3}
\newcommand{\hlAblContrastAThreeburnCIHi}{\ensuremath{-}2.4}
\newcommand{\hlAblContrastAThreeburnN}{5}
\newcommand{\hlAblContrastAFourburnEst}{14.4}
\newcommand{\hlAblContrastAFourburnCILo}{12.0}
\newcommand{\hlAblContrastAFourburnCIHi}{16.8}
\newcommand{\hlAblContrastAFourburnN}{5}
\newcommand{\hlAblContrastAFiveburnEst}{\ensuremath{-}2.3}
\newcommand{\hlAblContrastAFiveburnCILo}{\ensuremath{-}15.8}
\newcommand{\hlAblContrastAFiveburnCIHi}{11.3}
\newcommand{\hlAblContrastAFiveburnN}{5}
\newcommand{\hlAblContrastASixburnEst}{\ensuremath{-}5.7}
\newcommand{\hlAblContrastASixburnCILo}{\ensuremath{-}12.0}
\newcommand{\hlAblContrastASixburnCIHi}{0.5}
\newcommand{\hlAblContrastASixburnN}{5}
\newcommand{\hlAblContrastNSixburnEst}{\ensuremath{-}3.9}
\newcommand{\hlAblContrastNSixburnCILo}{\ensuremath{-}8.3}
\newcommand{\hlAblContrastNSixburnCIHi}{0.6}
\newcommand{\hlAblContrastNSixburnN}{5}
\newcommand{\hlAblContrastAThreeflairEst}{\ensuremath{-}2.8}
\newcommand{\hlAblContrastAThreeflairCILo}{\ensuremath{-}3.8}
\newcommand{\hlAblContrastAThreeflairCIHi}{\ensuremath{-}1.9}
\newcommand{\hlAblContrastAThreeflairN}{5}
\newcommand{\hlAblContrastAFourflairEst}{\ensuremath{-}1.2}
\newcommand{\hlAblContrastAFourflairCILo}{\ensuremath{-}2.3}
\newcommand{\hlAblContrastAFourflairCIHi}{\ensuremath{-}0.1}
\newcommand{\hlAblContrastAFourflairN}{5}
\newcommand{\hlAblContrastAFiveflairEst}{\ensuremath{-}1.1}
\newcommand{\hlAblContrastAFiveflairCILo}{\ensuremath{-}2.3}
\newcommand{\hlAblContrastAFiveflairCIHi}{0.1}
\newcommand{\hlAblContrastAFiveflairN}{5}
\newcommand{\hlAblContrastASixflairEst}{\ensuremath{-}2.7}
\newcommand{\hlAblContrastASixflairCILo}{\ensuremath{-}6.8}
\newcommand{\hlAblContrastASixflairCIHi}{1.5}
\newcommand{\hlAblContrastASixflairN}{5}
\newcommand{\hlAblContrastNSixflairEst}{\ensuremath{-}1.4}
\newcommand{\hlAblContrastNSixflairCILo}{\ensuremath{-}2.6}
\newcommand{\hlAblContrastNSixflairCIHi}{\ensuremath{-}0.2}
\newcommand{\hlAblContrastNSixflairN}{5}
\newcommand{\hlWinnersCurseAThreeburnEst}{\ensuremath{-}6.1}
\newcommand{\hlWinnersCurseAThreeburnCILo}{\ensuremath{-}9.3}
\newcommand{\hlWinnersCurseAThreeburnCIHi}{\ensuremath{-}2.8}
\newcommand{\hlWinnersCurseAThreeburnN}{4}
\newcommand{\hlWinnersCurseAFourburnEst}{15.1}
\newcommand{\hlWinnersCurseAFourburnCILo}{13.0}
\newcommand{\hlWinnersCurseAFourburnCIHi}{17.2}
\newcommand{\hlWinnersCurseAFourburnN}{4}
\newcommand{\hlWinnersCurseAFiveburnEst}{\ensuremath{-}4.2}
\newcommand{\hlWinnersCurseAFiveburnCILo}{\ensuremath{-}22.6}
\newcommand{\hlWinnersCurseAFiveburnCIHi}{14.2}
\newcommand{\hlWinnersCurseAFiveburnN}{4}
\newcommand{\hlWinnersCurseASixburnEst}{\ensuremath{-}6.4}
\newcommand{\hlWinnersCurseASixburnCILo}{\ensuremath{-}15.2}
\newcommand{\hlWinnersCurseASixburnCIHi}{2.4}
\newcommand{\hlWinnersCurseASixburnN}{4}
\newcommand{\hlWinnersCurseNSixburnEst}{\ensuremath{-}4.7}
\newcommand{\hlWinnersCurseNSixburnCILo}{\ensuremath{-}10.3}
\newcommand{\hlWinnersCurseNSixburnCIHi}{1.0}
\newcommand{\hlWinnersCurseNSixburnN}{4}
\newcommand{\hlWinnersCurseAThreeflairEst}{\ensuremath{-}2.8}
\newcommand{\hlWinnersCurseAThreeflairCILo}{\ensuremath{-}4.2}
\newcommand{\hlWinnersCurseAThreeflairCIHi}{\ensuremath{-}1.5}
\newcommand{\hlWinnersCurseAThreeflairN}{4}
\newcommand{\hlWinnersCurseAFourflairEst}{\ensuremath{-}1.0}
\newcommand{\hlWinnersCurseAFourflairCILo}{\ensuremath{-}2.5}
\newcommand{\hlWinnersCurseAFourflairCIHi}{0.4}
\newcommand{\hlWinnersCurseAFourflairN}{4}
\newcommand{\hlWinnersCurseAFiveflairEst}{\ensuremath{-}1.2}
\newcommand{\hlWinnersCurseAFiveflairCILo}{\ensuremath{-}3.0}
\newcommand{\hlWinnersCurseAFiveflairCIHi}{0.6}
\newcommand{\hlWinnersCurseAFiveflairN}{4}
\newcommand{\hlWinnersCurseASixflairEst}{\ensuremath{-}2.7}
\newcommand{\hlWinnersCurseASixflairCILo}{\ensuremath{-}8.9}
\newcommand{\hlWinnersCurseASixflairCIHi}{3.5}
\newcommand{\hlWinnersCurseASixflairN}{4}
\newcommand{\hlWinnersCurseNSixflairEst}{\ensuremath{-}1.6}
\newcommand{\hlWinnersCurseNSixflairCILo}{\ensuremath{-}3.1}
\newcommand{\hlWinnersCurseNSixflairCIHi}{\ensuremath{-}0.1}
\newcommand{\hlWinnersCurseNSixflairN}{4}
\newcommand{\hlHwNSixCellsburn}{\etype{boundary} \Ltwo, clean, \etype{omission} \Ltwo and \etype{shift} \Ltwo}
\newcommand{\hlHwNSixCellsNburn}{4}
\newcommand{\hlHwNSixDropDiffMaxburn}{3.1}
\newcommand{\hlHwMixedNburn}{37}
\newcommand{\hlHwMixedAOneNburn}{33}
\newcommand{\hlHwMixedAOneLOneNburn}{8}
\newcommand{\hlHwDropDiffMeanburn}{1.9}
\newcommand{\hlHwDropDiffMaxburn}{6.8}
\newcommand{\hlHwCleanDiffMaxburn}{3.1}
\newcommand{\hlHwDropDiffSignedMeanburn}{0.2}
\newcommand{\hlHwNSixCellsflair}{\etype{boundary} \Ltwo, clean, \etype{coarse} \Ltwo, \etype{omission} \Ltwo and \etype{shift} \Ltwo}
\newcommand{\hlHwNSixCellsNflair}{5}
\newcommand{\hlHwNSixDropDiffMaxflair}{1.3}
\newcommand{\hlHwMixedNflair}{23}
\newcommand{\hlHwMixedAOneNflair}{18}
\newcommand{\hlHwMixedAOneLOneNflair}{8}
\newcommand{\hlHwDropDiffMeanflair}{0.8}
\newcommand{\hlHwDropDiffMaxflair}{2.3}
\newcommand{\hlHwCleanDiffMaxflair}{0.9}
\newcommand{\hlHwDropDiffSignedMeanflair}{\ensuremath{-}0.3}
\newcommand{\hlSeedExtraCellsN}{35}
\newcommand{\hlSeedExtraBlocks}{N13, N5}
\newcommand{\hlSeedExtraSeeds}{6 to 8}
\newcommand{\hlSeedExtraCellsburn}{LVD boundary \Ltwo, LVD clean, LVD coarse \Ltwo, LVD omission \Ltwo, LVD shift \Ltwo, SAT boundary \Ltwo, SAT clean, SAT coarse \Ltwo, SAT omission \Ltwo, SAT shift \Ltwo, DOFA boundary \Ltwo, DOFA clean, DOFA coarse \Ltwo, DOFA omission \Ltwo, DOFA shift \Ltwo, RN boundary \Ltwo, RN clean, RN coarse \Ltwo, RN omission \Ltwo, RN shift \Ltwo, TM boundary \Ltwo, TM clean, TM coarse \Ltwo, TM omission \Ltwo, TM shift \Ltwo}
\newcommand{\hlSeedExtraCellsflair}{LVD boundary \Ltwo, LVD clean, LVD coarse \Ltwo, LVD omission \Ltwo, LVD shift \Ltwo, SAT boundary \Ltwo, SAT clean, SAT coarse \Ltwo, SAT omission \Ltwo, SAT shift \Ltwo}
\newcommand{\hlSThreeDropDOFAburnEst}{\ensuremath{-}4.9}
\newcommand{\hlSThreeDropDOFAburnCILo}{\ensuremath{-}7.2}
\newcommand{\hlSThreeDropDOFAburnCIHi}{\ensuremath{-}2.6}
\newcommand{\hlSThreeDropDOFAburnN}{5}
\newcommand{\hlSThreeDropDOFAburnA}{13.0}
\newcommand{\hlSThreeDropDOFAburnB}{17.9}
\newcommand{\hlSThreeRetDOFAburnEst}{6.3}
\newcommand{\hlSThreeRetDOFAburnCILo}{3.8}
\newcommand{\hlSThreeRetDOFAburnCIHi}{8.7}
\newcommand{\hlSThreeRetDOFAburnN}{5}
\newcommand{\hlSThreeRetDOFAburnA}{85.4}
\newcommand{\hlSThreeRetDOFAburnB}{79.1}
\newcommand{\hlSFourDropRNburnEst}{1.0}
\newcommand{\hlSFourDropRNburnCILo}{\ensuremath{-}3.4}
\newcommand{\hlSFourDropRNburnCIHi}{5.5}
\newcommand{\hlSFourDropRNburnN}{5}
\newcommand{\hlSFourDropRNburnA}{16.9}
\newcommand{\hlSFourDropRNburnB}{15.9}
\newcommand{\hlSFourRetRNburnEst}{\ensuremath{-}1.2}
\newcommand{\hlSFourRetRNburnCILo}{\ensuremath{-}6.2}
\newcommand{\hlSFourRetRNburnCIHi}{3.8}
\newcommand{\hlSFourRetRNburnN}{5}
\newcommand{\hlSFourRetRNburnA}{80.8}
\newcommand{\hlSFourRetRNburnB}{82.0}
\newcommand{\hlSFiveDropSATburnEst}{\ensuremath{-}9.3}
\newcommand{\hlSFiveDropSATburnCILo}{\ensuremath{-}14.9}
\newcommand{\hlSFiveDropSATburnCIHi}{\ensuremath{-}3.7}
\newcommand{\hlSFiveDropSATburnN}{5}
\newcommand{\hlSFiveDropSATburnA}{8.5}
\newcommand{\hlSFiveDropSATburnB}{17.8}
\newcommand{\hlSFiveRetSATburnEst}{11.2}
\newcommand{\hlSFiveRetSATburnCILo}{3.6}
\newcommand{\hlSFiveRetSATburnCIHi}{18.8}
\newcommand{\hlSFiveRetSATburnN}{5}
\newcommand{\hlSFiveRetSATburnA}{87.8}
\newcommand{\hlSFiveRetSATburnB}{76.6}
\newcommand{\hlSFiveDropLVDburnEst}{\ensuremath{-}5.6}
\newcommand{\hlSFiveDropLVDburnCILo}{\ensuremath{-}11.4}
\newcommand{\hlSFiveDropLVDburnCIHi}{0.2}
\newcommand{\hlSFiveDropLVDburnN}{5}
\newcommand{\hlSFiveDropLVDburnA}{8.5}
\newcommand{\hlSFiveDropLVDburnB}{14.1}
\newcommand{\hlSFiveRetLVDburnEst}{5.0}
\newcommand{\hlSFiveRetLVDburnCILo}{\ensuremath{-}2.7}
\newcommand{\hlSFiveRetLVDburnCIHi}{12.6}
\newcommand{\hlSFiveRetLVDburnN}{5}
\newcommand{\hlSFiveRetLVDburnA}{87.8}
\newcommand{\hlSFiveRetLVDburnB}{82.8}
\newcommand{\hlSSixDropSATburnEst}{\ensuremath{-}1.8}
\newcommand{\hlSSixDropSATburnCILo}{\ensuremath{-}5.2}
\newcommand{\hlSSixDropSATburnCIHi}{1.6}
\newcommand{\hlSSixDropSATburnN}{5}
\newcommand{\hlSSixDropSATburnA}{16.0}
\newcommand{\hlSSixDropSATburnB}{17.8}
\newcommand{\hlSSixRetSATburnEst}{3.9}
\newcommand{\hlSSixRetSATburnCILo}{0.1}
\newcommand{\hlSSixRetSATburnCIHi}{7.7}
\newcommand{\hlSSixRetSATburnN}{5}
\newcommand{\hlSSixRetSATburnA}{80.4}
\newcommand{\hlSSixRetSATburnB}{76.6}
\newcommand{\hlSSixDropLVDburnEst}{1.9}
\newcommand{\hlSSixDropLVDburnCILo}{\ensuremath{-}3.5}
\newcommand{\hlSSixDropLVDburnCIHi}{7.3}
\newcommand{\hlSSixDropLVDburnN}{5}
\newcommand{\hlSSixDropLVDburnA}{16.0}
\newcommand{\hlSSixDropLVDburnB}{14.1}
\newcommand{\hlSSixRetLVDburnEst}{\ensuremath{-}2.4}
\newcommand{\hlSSixRetLVDburnCILo}{\ensuremath{-}8.5}
\newcommand{\hlSSixRetLVDburnCIHi}{3.8}
\newcommand{\hlSSixRetLVDburnN}{5}
\newcommand{\hlSSixRetLVDburnA}{80.4}
\newcommand{\hlSSixRetLVDburnB}{82.8}
\newcommand{\hlSThreeBudgetburnEst}{14.4}
\newcommand{\hlSThreeBudgetburnCILo}{9.9}
\newcommand{\hlSThreeBudgetburnCIHi}{18.8}
\newcommand{\hlSThreeBudgetburnN}{5}
\newcommand{\hlSThreeBudgetburnA}{86.0}
\newcommand{\hlSThreeBudgetburnB}{71.6}
\newcommand{\hlSFourBudgetburnEst}{16.5}
\newcommand{\hlSFourBudgetburnCILo}{12.1}
\newcommand{\hlSFourBudgetburnCIHi}{20.9}
\newcommand{\hlSFourBudgetburnN}{5}
\newcommand{\hlSFourBudgetburnA}{87.3}
\newcommand{\hlSFourBudgetburnB}{70.8}
\newcommand{\hlSFiveBudgetburnEst}{2.5}
\newcommand{\hlSFiveBudgetburnCILo}{\ensuremath{-}1.1}
\newcommand{\hlSFiveBudgetburnCIHi}{6.2}
\newcommand{\hlSFiveBudgetburnN}{5}
\newcommand{\hlSFiveBudgetburnA}{61.7}
\newcommand{\hlSFiveBudgetburnB}{59.1}
\newcommand{\hlSSixBudgetburnEst}{10.3}
\newcommand{\hlSSixBudgetburnCILo}{5.4}
\newcommand{\hlSSixBudgetburnCIHi}{15.2}
\newcommand{\hlSSixBudgetburnN}{5}
\newcommand{\hlSSixBudgetburnA}{74.6}
\newcommand{\hlSSixBudgetburnB}{64.3}
\newcommand{\hlSThreeDropDOFAflairEst}{0.9}
\newcommand{\hlSThreeDropDOFAflairCILo}{\ensuremath{-}0.7}
\newcommand{\hlSThreeDropDOFAflairCIHi}{2.6}
\newcommand{\hlSThreeDropDOFAflairN}{5}
\newcommand{\hlSThreeDropDOFAflairA}{5.2}
\newcommand{\hlSThreeDropDOFAflairB}{4.3}
\newcommand{\hlSThreeRetDOFAflairEst}{\ensuremath{-}4.1}
\newcommand{\hlSThreeRetDOFAflairCILo}{\ensuremath{-}7.9}
\newcommand{\hlSThreeRetDOFAflairCIHi}{\ensuremath{-}0.4}
\newcommand{\hlSThreeRetDOFAflairN}{5}
\newcommand{\hlSThreeRetDOFAflairA}{86.8}
\newcommand{\hlSThreeRetDOFAflairB}{90.9}
\newcommand{\hlSFourDropRNflairEst}{0.0}
\newcommand{\hlSFourDropRNflairCILo}{\ensuremath{-}2.8}
\newcommand{\hlSFourDropRNflairCIHi}{2.7}
\newcommand{\hlSFourDropRNflairN}{5}
\newcommand{\hlSFourDropRNflairA}{4.2}
\newcommand{\hlSFourDropRNflairB}{4.2}
\newcommand{\hlSFourRetRNflairEst}{\ensuremath{-}0.4}
\newcommand{\hlSFourRetRNflairCILo}{\ensuremath{-}6.3}
\newcommand{\hlSFourRetRNflairCIHi}{5.6}
\newcommand{\hlSFourRetRNflairN}{5}
\newcommand{\hlSFourRetRNflairA}{90.3}
\newcommand{\hlSFourRetRNflairB}{90.6}
\newcommand{\hlSFiveDropSATflairEst}{\ensuremath{-}4.0}
\newcommand{\hlSFiveDropSATflairCILo}{\ensuremath{-}5.9}
\newcommand{\hlSFiveDropSATflairCIHi}{\ensuremath{-}2.1}
\newcommand{\hlSFiveDropSATflairN}{5}
\newcommand{\hlSFiveDropSATflairA}{2.5}
\newcommand{\hlSFiveDropSATflairB}{6.5}
\newcommand{\hlSFiveRetSATflairEst}{3.6}
\newcommand{\hlSFiveRetSATflairCILo}{\ensuremath{-}2.3}
\newcommand{\hlSFiveRetSATflairCIHi}{9.5}
\newcommand{\hlSFiveRetSATflairN}{5}
\newcommand{\hlSFiveRetSATflairA}{91.1}
\newcommand{\hlSFiveRetSATflairB}{87.5}
\newcommand{\hlSFiveDropLVDflairEst}{\ensuremath{-}1.1}
\newcommand{\hlSFiveDropLVDflairCILo}{\ensuremath{-}2.8}
\newcommand{\hlSFiveDropLVDflairCIHi}{0.6}
\newcommand{\hlSFiveDropLVDflairN}{5}
\newcommand{\hlSFiveDropLVDflairA}{2.5}
\newcommand{\hlSFiveDropLVDflairB}{3.6}
\newcommand{\hlSFiveRetLVDflairEst}{\ensuremath{-}1.8}
\newcommand{\hlSFiveRetLVDflairCILo}{\ensuremath{-}6.9}
\newcommand{\hlSFiveRetLVDflairCIHi}{3.2}
\newcommand{\hlSFiveRetLVDflairN}{5}
\newcommand{\hlSFiveRetLVDflairA}{91.1}
\newcommand{\hlSFiveRetLVDflairB}{93.0}
\newcommand{\hlSSixDropSATflairEst}{\ensuremath{-}2.5}
\newcommand{\hlSSixDropSATflairCILo}{\ensuremath{-}3.9}
\newcommand{\hlSSixDropSATflairCIHi}{\ensuremath{-}1.1}
\newcommand{\hlSSixDropSATflairN}{5}
\newcommand{\hlSSixDropSATflairA}{4.0}
\newcommand{\hlSSixDropSATflairB}{6.5}
\newcommand{\hlSSixRetSATflairEst}{4.1}
\newcommand{\hlSSixRetSATflairCILo}{1.3}
\newcommand{\hlSSixRetSATflairCIHi}{6.9}
\newcommand{\hlSSixRetSATflairN}{5}
\newcommand{\hlSSixRetSATflairA}{91.6}
\newcommand{\hlSSixRetSATflairB}{87.5}
\newcommand{\hlSSixDropLVDflairEst}{0.4}
\newcommand{\hlSSixDropLVDflairCILo}{\ensuremath{-}1.1}
\newcommand{\hlSSixDropLVDflairCIHi}{1.9}
\newcommand{\hlSSixDropLVDflairN}{5}
\newcommand{\hlSSixDropLVDflairA}{4.0}
\newcommand{\hlSSixDropLVDflairB}{3.6}
\newcommand{\hlSSixRetLVDflairEst}{\ensuremath{-}1.3}
\newcommand{\hlSSixRetLVDflairCILo}{\ensuremath{-}4.2}
\newcommand{\hlSSixRetLVDflairCIHi}{1.5}
\newcommand{\hlSSixRetLVDflairN}{5}
\newcommand{\hlSSixRetLVDflairA}{91.6}
\newcommand{\hlSSixRetLVDflairB}{93.0}
\newcommand{\hlSThreeBudgetflairEst}{\ensuremath{-}2.0}
\newcommand{\hlSThreeBudgetflairCILo}{\ensuremath{-}5.0}
\newcommand{\hlSThreeBudgetflairCIHi}{1.0}
\newcommand{\hlSThreeBudgetflairN}{5}
\newcommand{\hlSThreeBudgetflairA}{32.7}
\newcommand{\hlSThreeBudgetflairB}{34.7}
\newcommand{\hlSFourBudgetflairEst}{\ensuremath{-}2.0}
\newcommand{\hlSFourBudgetflairCILo}{\ensuremath{-}4.0}
\newcommand{\hlSFourBudgetflairCIHi}{0.0}
\newcommand{\hlSFourBudgetflairN}{5}
\newcommand{\hlSFourBudgetflairA}{36.8}
\newcommand{\hlSFourBudgetflairB}{38.8}
\newcommand{\hlSFiveBudgetflairEst}{\ensuremath{-}4.6}
\newcommand{\hlSFiveBudgetflairCILo}{\ensuremath{-}6.1}
\newcommand{\hlSFiveBudgetflairCIHi}{\ensuremath{-}3.1}
\newcommand{\hlSFiveBudgetflairN}{5}
\newcommand{\hlSFiveBudgetflairA}{21.1}
\newcommand{\hlSFiveBudgetflairB}{25.7}
\newcommand{\hlSSixBudgetflairEst}{\ensuremath{-}0.1}
\newcommand{\hlSSixBudgetflairCILo}{\ensuremath{-}2.1}
\newcommand{\hlSSixBudgetflairCIHi}{2.0}
\newcommand{\hlSSixBudgetflairN}{5}
\newcommand{\hlSSixBudgetflairA}{43.5}
\newcommand{\hlSSixBudgetflairB}{43.5}
\newcommand{\hlSTwoDeltaSATflairEst}{\ensuremath{-}0.9}
\newcommand{\hlSTwoDeltaSATflairCILo}{\ensuremath{-}4.3}
\newcommand{\hlSTwoDeltaSATflairCIHi}{2.5}
\newcommand{\hlSTwoDeltaSATflairN}{5}
\newcommand{\hlSTwoDeltaSATflairA}{7.3}
\newcommand{\hlSTwoDeltaSATflairB}{8.2}
\newcommand{\hlSTwoDeltaRNflairEst}{\ensuremath{-}1.1}
\newcommand{\hlSTwoDeltaRNflairCILo}{\ensuremath{-}5.0}
\newcommand{\hlSTwoDeltaRNflairCIHi}{2.9}
\newcommand{\hlSTwoDeltaRNflairN}{5}
\newcommand{\hlSTwoDeltaRNflairA}{2.5}
\newcommand{\hlSTwoDeltaRNflairB}{3.6}
\newcommand{\hlSOneDropSATsenEst}{7.2}
\newcommand{\hlSOneDropSATsenCILo}{0.7}
\newcommand{\hlSOneDropSATsenCIHi}{13.8}
\newcommand{\hlSOneDropSATsenN}{5}
\newcommand{\hlSOneDropSATsenA}{7.2}
\newcommand{\hlSOneDropSATsenB}{0.0}
\newcommand{\hlSOneDropLVDsenEst}{5.3}
\newcommand{\hlSOneDropLVDsenCILo}{\ensuremath{-}7.1}
\newcommand{\hlSOneDropLVDsenCIHi}{17.7}
\newcommand{\hlSOneDropLVDsenN}{5}
\newcommand{\hlSOneDropLVDsenA}{5.3}
\newcommand{\hlSOneDropLVDsenB}{0.0}
\newcommand{\hlSOneDropDOFAsenEst}{8.8}
\newcommand{\hlSOneDropDOFAsenCILo}{6.9}
\newcommand{\hlSOneDropDOFAsenCIHi}{10.8}
\newcommand{\hlSOneDropDOFAsenN}{5}
\newcommand{\hlSOneDropDOFAsenA}{8.8}
\newcommand{\hlSOneDropDOFAsenB}{0.0}
\newcommand{\hlSOneDropTMsenEst}{16.1}
\newcommand{\hlSOneDropTMsenCILo}{13.7}
\newcommand{\hlSOneDropTMsenCIHi}{18.4}
\newcommand{\hlSOneDropTMsenN}{5}
\newcommand{\hlSOneDropTMsenA}{16.1}
\newcommand{\hlSOneDropTMsenB}{0.0}
\newcommand{\hlSOneDropRNsenEst}{15.7}
\newcommand{\hlSOneDropRNsenCILo}{14.4}
\newcommand{\hlSOneDropRNsenCIHi}{17.1}
\newcommand{\hlSOneDropRNsenN}{5}
\newcommand{\hlSOneDropRNsenA}{15.7}
\newcommand{\hlSOneDropRNsenB}{0.0}
\newcommand{\hlSOneDropMeansenEst}{10.6}
\newcommand{\hlSOneDropMeansenCILo}{7.9}
\newcommand{\hlSOneDropMeansenCIHi}{13.4}
\newcommand{\hlSOneDropMeansenN}{25}
\newcommand{\hlSOneDropMeansenA}{10.6}
\newcommand{\hlSOneDropMeansenB}{0.0}
\newcommand{\hlFamilySeedsAllFive}{no}
\newcommand{\hlBdropGapOmissionNarrowburn}{\ensuremath{-}2.3}
\newcommand{\hlBdropGapOmissionNarrowburnCILo}{\ensuremath{-}3.4}
\newcommand{\hlBdropGapOmissionNarrowburnCIHi}{\ensuremath{-}1.1}
\newcommand{\hlBdropGapOmissionNarrowburnN}{40}
\newcommand{\hlBdropGapBoundaryNarrowburn}{\ensuremath{-}4.3}
\newcommand{\hlBdropGapBoundaryNarrowburnCILo}{\ensuremath{-}5.4}
\newcommand{\hlBdropGapBoundaryNarrowburnCIHi}{\ensuremath{-}3.3}
\newcommand{\hlBdropGapBoundaryNarrowburnN}{40}
\newcommand{\hlBdropGapOmissionNarrowflair}{\ensuremath{-}0.6}
\newcommand{\hlBdropGapOmissionNarrowflairCILo}{\ensuremath{-}1.1}
\newcommand{\hlBdropGapOmissionNarrowflairCIHi}{\ensuremath{-}0.1}
\newcommand{\hlBdropGapOmissionNarrowflairN}{31}
\newcommand{\hlBdropGapBoundaryNarrowflair}{\ensuremath{-}0.5}
\newcommand{\hlBdropGapBoundaryNarrowflairCILo}{\ensuremath{-}0.9}
\newcommand{\hlBdropGapBoundaryNarrowflairCIHi}{\ensuremath{-}0.1}
\newcommand{\hlBdropGapBoundaryNarrowflairN}{31}
\newcommand{\hlBdropGapOmissionWideburn}{1.2}
\newcommand{\hlBdropGapOmissionWideburnCILo}{\ensuremath{-}0.4}
\newcommand{\hlBdropGapOmissionWideburnCIHi}{2.8}
\newcommand{\hlBdropGapOmissionWideburnN}{40}
\newcommand{\hlBdropGapBoundaryWideburn}{\ensuremath{-}3.3}
\newcommand{\hlBdropGapBoundaryWideburnCILo}{\ensuremath{-}4.5}
\newcommand{\hlBdropGapBoundaryWideburnCIHi}{\ensuremath{-}2.2}
\newcommand{\hlBdropGapBoundaryWideburnN}{40}
\newcommand{\hlBdropGapOmissionWideflair}{1.1}
\newcommand{\hlBdropGapOmissionWideflairCILo}{0.4}
\newcommand{\hlBdropGapOmissionWideflairCIHi}{1.7}
\newcommand{\hlBdropGapOmissionWideflairN}{31}
\newcommand{\hlBdropGapBoundaryWideflair}{0.2}
\newcommand{\hlBdropGapBoundaryWideflairCILo}{\ensuremath{-}0.4}
\newcommand{\hlBdropGapBoundaryWideflairCIHi}{0.7}
\newcommand{\hlBdropGapBoundaryWideflairN}{31}
\newcommand{\hlBdropRankNarrowburn}{\etype{boundary}, \etype{omission}, \etype{shift} and \etype{coarse}}
\newcommand{\hlBdropShiftLastNarrowburn}{no}
\newcommand{\hlBdropNarrowburnBoundary}{13.2}
\newcommand{\hlBdropNarrowburnOmission}{11.2}
\newcommand{\hlBdropNarrowburnShift}{8.9}
\newcommand{\hlBdropNarrowburnCoarse}{8.7}
\newcommand{\hlBdropGapShiftNarrowburn}{2.3}
\newcommand{\hlBdropGapShiftCILoNarrowburn}{1.1}
\newcommand{\hlBdropGapShiftCIHiNarrowburn}{3.4}
\newcommand{\hlBdropGapShiftTypeNarrowburn}{omission}
\newcommand{\hlBdropRankNarrowflair}{\etype{coarse}, \etype{omission}, \etype{boundary} and \etype{shift}}
\newcommand{\hlBdropShiftLastNarrowflair}{yes}
\newcommand{\hlBdropNarrowflairCoarse}{3.6}
\newcommand{\hlBdropNarrowflairOmission}{3.2}
\newcommand{\hlBdropNarrowflairBoundary}{3.2}
\newcommand{\hlBdropNarrowflairShift}{2.8}
\newcommand{\hlBdropGapShiftNarrowflair}{0.5}
\newcommand{\hlBdropGapShiftCILoNarrowflair}{0.1}
\newcommand{\hlBdropGapShiftCIHiNarrowflair}{0.9}
\newcommand{\hlBdropGapShiftTypeNarrowflair}{boundary}
\newcommand{\hlBdropRankWideburn}{\etype{boundary}, \etype{coarse}, \etype{shift} and \etype{omission}}
\newcommand{\hlBdropShiftLastWideburn}{no}
\newcommand{\hlBdropWideburnBoundary}{24.4}
\newcommand{\hlBdropWideburnCoarse}{23.4}
\newcommand{\hlBdropWideburnShift}{21.1}
\newcommand{\hlBdropWideburnOmission}{19.9}
\newcommand{\hlBdropGapShiftWideburn}{2.3}
\newcommand{\hlBdropGapShiftCILoWideburn}{1.2}
\newcommand{\hlBdropGapShiftCIHiWideburn}{3.5}
\newcommand{\hlBdropGapShiftTypeWideburn}{coarse}
\newcommand{\hlBdropRankWideflair}{\etype{coarse}, \etype{shift}, \etype{boundary} and \etype{omission}}
\newcommand{\hlBdropShiftLastWideflair}{no}
\newcommand{\hlBdropWideflairCoarse}{10.0}
\newcommand{\hlBdropWideflairShift}{6.9}
\newcommand{\hlBdropWideflairBoundary}{6.6}
\newcommand{\hlBdropWideflairOmission}{5.6}
\newcommand{\hlBdropGapShiftWideflair}{3.1}
\newcommand{\hlBdropGapShiftCILoWideflair}{2.8}
\newcommand{\hlBdropGapShiftCIHiWideflair}{3.5}
\newcommand{\hlBdropGapShiftTypeWideflair}{coarse}
\newcommand{\hlPcDropBuildingShift}{11.2}
\newcommand{\hlPcDropCILoBuildingShift}{10.1}
\newcommand{\hlPcDropCIHiBuildingShift}{12.3}
\newcommand{\hlPcDropBuildingCoarse}{21.2}
\newcommand{\hlPcDropCILoBuildingCoarse}{19.6}
\newcommand{\hlPcDropCIHiBuildingCoarse}{22.9}
\newcommand{\hlPcDropBuildingBoundary}{12.0}
\newcommand{\hlPcDropCILoBuildingBoundary}{9.9}
\newcommand{\hlPcDropCIHiBuildingBoundary}{14.0}
\newcommand{\hlPcDropBuildingOmission}{8.4}
\newcommand{\hlPcDropCILoBuildingOmission}{6.4}
\newcommand{\hlPcDropCIHiBuildingOmission}{10.4}
\newcommand{\hlPcDropPerviousShift}{3.9}
\newcommand{\hlPcDropCILoPerviousShift}{3.0}
\newcommand{\hlPcDropCIHiPerviousShift}{4.8}
\newcommand{\hlPcDropPerviousCoarse}{5.3}
\newcommand{\hlPcDropCILoPerviousCoarse}{4.3}
\newcommand{\hlPcDropCIHiPerviousCoarse}{6.3}
\newcommand{\hlPcDropPerviousBoundary}{5.2}
\newcommand{\hlPcDropCILoPerviousBoundary}{4.1}
\newcommand{\hlPcDropCIHiPerviousBoundary}{6.2}
\newcommand{\hlPcDropPerviousOmission}{5.6}
\newcommand{\hlPcDropCILoPerviousOmission}{4.4}
\newcommand{\hlPcDropCIHiPerviousOmission}{6.8}
\newcommand{\hlPcDropImperviousShift}{9.5}
\newcommand{\hlPcDropCILoImperviousShift}{8.7}
\newcommand{\hlPcDropCIHiImperviousShift}{10.2}
\newcommand{\hlPcDropImperviousCoarse}{15.7}
\newcommand{\hlPcDropCILoImperviousCoarse}{14.9}
\newcommand{\hlPcDropCIHiImperviousCoarse}{16.5}
\newcommand{\hlPcDropImperviousBoundary}{9.2}
\newcommand{\hlPcDropCILoImperviousBoundary}{7.9}
\newcommand{\hlPcDropCIHiImperviousBoundary}{10.5}
\newcommand{\hlPcDropImperviousOmission}{6.6}
\newcommand{\hlPcDropCILoImperviousOmission}{5.8}
\newcommand{\hlPcDropCIHiImperviousOmission}{7.5}
\newcommand{\hlPcDropBareSoilShift}{1.6}
\newcommand{\hlPcDropCILoBareSoilShift}{\ensuremath{-}0.1}
\newcommand{\hlPcDropCIHiBareSoilShift}{3.2}
\newcommand{\hlPcDropBareSoilCoarse}{3.3}
\newcommand{\hlPcDropCILoBareSoilCoarse}{1.1}
\newcommand{\hlPcDropCIHiBareSoilCoarse}{5.5}
\newcommand{\hlPcDropBareSoilBoundary}{5.8}
\newcommand{\hlPcDropCILoBareSoilBoundary}{3.7}
\newcommand{\hlPcDropCIHiBareSoilBoundary}{8.0}
\newcommand{\hlPcDropBareSoilOmission}{6.4}
\newcommand{\hlPcDropCILoBareSoilOmission}{3.8}
\newcommand{\hlPcDropCIHiBareSoilOmission}{8.9}
\newcommand{\hlPcDropWaterShift}{3.1}
\newcommand{\hlPcDropCILoWaterShift}{2.0}
\newcommand{\hlPcDropCIHiWaterShift}{4.2}
\newcommand{\hlPcDropWaterCoarse}{4.6}
\newcommand{\hlPcDropCILoWaterCoarse}{3.6}
\newcommand{\hlPcDropCIHiWaterCoarse}{5.7}
\newcommand{\hlPcDropWaterBoundary}{6.1}
\newcommand{\hlPcDropCILoWaterBoundary}{4.8}
\newcommand{\hlPcDropCIHiWaterBoundary}{7.4}
\newcommand{\hlPcDropWaterOmission}{6.7}
\newcommand{\hlPcDropCILoWaterOmission}{5.1}
\newcommand{\hlPcDropCIHiWaterOmission}{8.4}
\newcommand{\hlPcDropConiferousShift}{\ensuremath{-}1.0}
\newcommand{\hlPcDropCILoConiferousShift}{\ensuremath{-}2.8}
\newcommand{\hlPcDropCIHiConiferousShift}{0.8}
\newcommand{\hlPcDropConiferousCoarse}{0.4}
\newcommand{\hlPcDropCILoConiferousCoarse}{\ensuremath{-}1.9}
\newcommand{\hlPcDropCIHiConiferousCoarse}{2.7}
\newcommand{\hlPcDropConiferousBoundary}{6.3}
\newcommand{\hlPcDropCILoConiferousBoundary}{3.1}
\newcommand{\hlPcDropCIHiConiferousBoundary}{9.4}
\newcommand{\hlPcDropConiferousOmission}{4.9}
\newcommand{\hlPcDropCILoConiferousOmission}{2.1}
\newcommand{\hlPcDropCIHiConiferousOmission}{7.7}
\newcommand{\hlPcDropDeciduousShift}{3.3}
\newcommand{\hlPcDropCILoDeciduousShift}{2.6}
\newcommand{\hlPcDropCIHiDeciduousShift}{3.9}
\newcommand{\hlPcDropDeciduousCoarse}{5.6}
\newcommand{\hlPcDropCILoDeciduousCoarse}{5.0}
\newcommand{\hlPcDropCIHiDeciduousCoarse}{6.3}
\newcommand{\hlPcDropDeciduousBoundary}{5.7}
\newcommand{\hlPcDropCILoDeciduousBoundary}{4.8}
\newcommand{\hlPcDropCIHiDeciduousBoundary}{6.6}
\newcommand{\hlPcDropDeciduousOmission}{6.5}
\newcommand{\hlPcDropCILoDeciduousOmission}{5.0}
\newcommand{\hlPcDropCIHiDeciduousOmission}{8.0}
\newcommand{\hlPcDropBrushwoodShift}{1.9}
\newcommand{\hlPcDropCILoBrushwoodShift}{1.3}
\newcommand{\hlPcDropCIHiBrushwoodShift}{2.4}
\newcommand{\hlPcDropBrushwoodCoarse}{2.9}
\newcommand{\hlPcDropCILoBrushwoodCoarse}{2.3}
\newcommand{\hlPcDropCIHiBrushwoodCoarse}{3.4}
\newcommand{\hlPcDropBrushwoodBoundary}{4.8}
\newcommand{\hlPcDropCILoBrushwoodBoundary}{4.0}
\newcommand{\hlPcDropCIHiBrushwoodBoundary}{5.5}
\newcommand{\hlPcDropBrushwoodOmission}{4.2}
\newcommand{\hlPcDropCILoBrushwoodOmission}{3.4}
\newcommand{\hlPcDropCIHiBrushwoodOmission}{5.1}
\newcommand{\hlPcDropVineyardShift}{2.0}
\newcommand{\hlPcDropCILoVineyardShift}{0.9}
\newcommand{\hlPcDropCIHiVineyardShift}{3.1}
\newcommand{\hlPcDropVineyardCoarse}{4.7}
\newcommand{\hlPcDropCILoVineyardCoarse}{3.8}
\newcommand{\hlPcDropCIHiVineyardCoarse}{5.6}
\newcommand{\hlPcDropVineyardBoundary}{3.9}
\newcommand{\hlPcDropCILoVineyardBoundary}{2.6}
\newcommand{\hlPcDropCIHiVineyardBoundary}{5.3}
\newcommand{\hlPcDropVineyardOmission}{5.5}
\newcommand{\hlPcDropCILoVineyardOmission}{3.9}
\newcommand{\hlPcDropCIHiVineyardOmission}{7.2}
\newcommand{\hlPcDropHerbaceousShift}{4.0}
\newcommand{\hlPcDropCILoHerbaceousShift}{2.9}
\newcommand{\hlPcDropCIHiHerbaceousShift}{5.1}
\newcommand{\hlPcDropHerbaceousCoarse}{6.7}
\newcommand{\hlPcDropCILoHerbaceousCoarse}{5.7}
\newcommand{\hlPcDropCIHiHerbaceousCoarse}{7.8}
\newcommand{\hlPcDropHerbaceousBoundary}{6.4}
\newcommand{\hlPcDropCILoHerbaceousBoundary}{5.3}
\newcommand{\hlPcDropCIHiHerbaceousBoundary}{7.5}
\newcommand{\hlPcDropHerbaceousOmission}{5.7}
\newcommand{\hlPcDropCILoHerbaceousOmission}{4.3}
\newcommand{\hlPcDropCIHiHerbaceousOmission}{7.2}
\newcommand{\hlPcDropAgriculturalShift}{0.5}
\newcommand{\hlPcDropCILoAgriculturalShift}{\ensuremath{-}0.2}
\newcommand{\hlPcDropCIHiAgriculturalShift}{1.2}
\newcommand{\hlPcDropAgriculturalCoarse}{1.0}
\newcommand{\hlPcDropCILoAgriculturalCoarse}{0.1}
\newcommand{\hlPcDropCIHiAgriculturalCoarse}{1.8}
\newcommand{\hlPcDropAgriculturalBoundary}{1.1}
\newcommand{\hlPcDropCILoAgriculturalBoundary}{0.1}
\newcommand{\hlPcDropCIHiAgriculturalBoundary}{2.0}
\newcommand{\hlPcDropAgriculturalOmission}{3.7}
\newcommand{\hlPcDropCILoAgriculturalOmission}{2.2}
\newcommand{\hlPcDropCIHiAgriculturalOmission}{5.3}
\newcommand{\hlPcDropPlowedShift}{2.1}
\newcommand{\hlPcDropCILoPlowedShift}{\ensuremath{-}0.2}
\newcommand{\hlPcDropCIHiPlowedShift}{4.3}
\newcommand{\hlPcDropPlowedCoarse}{0.8}
\newcommand{\hlPcDropCILoPlowedCoarse}{\ensuremath{-}1.0}
\newcommand{\hlPcDropCIHiPlowedCoarse}{2.6}
\newcommand{\hlPcDropPlowedBoundary}{0.4}
\newcommand{\hlPcDropCILoPlowedBoundary}{\ensuremath{-}0.9}
\newcommand{\hlPcDropCIHiPlowedBoundary}{1.6}
\newcommand{\hlPcDropPlowedOmission}{1.8}
\newcommand{\hlPcDropCILoPlowedOmission}{\ensuremath{-}0.4}
\newcommand{\hlPcDropCIHiPlowedOmission}{3.9}
\newcommand{\hlPcDropOtherShift}{0.0}
\newcommand{\hlPcDropCILoOtherShift}{\ensuremath{-}0.2}
\newcommand{\hlPcDropCIHiOtherShift}{0.1}
\newcommand{\hlPcDropOtherCoarse}{\ensuremath{-}0.1}
\newcommand{\hlPcDropCILoOtherCoarse}{\ensuremath{-}0.2}
\newcommand{\hlPcDropCIHiOtherCoarse}{0.1}
\newcommand{\hlPcDropOtherBoundary}{0.0}
\newcommand{\hlPcDropCILoOtherBoundary}{\ensuremath{-}0.3}
\newcommand{\hlPcDropCIHiOtherBoundary}{0.2}
\newcommand{\hlPcDropOtherOmission}{0.0}
\newcommand{\hlPcDropCILoOtherOmission}{\ensuremath{-}0.1}
\newcommand{\hlPcDropCIHiOtherOmission}{0.1}
\newcommand{\hlOmRawSATburn}{21.2}
\newcommand{\hlOmAdjSATburn}{21.1}
\newcommand{\hlOmRawLVDburn}{16.9}
\newcommand{\hlOmAdjLVDburn}{16.8}
\newcommand{\hlOmRawDOFAburn}{24.4}
\newcommand{\hlOmAdjDOFAburn}{24.4}
\newcommand{\hlOmRawTMburn}{11.4}
\newcommand{\hlOmAdjTMburn}{11.4}
\newcommand{\hlOmRawRNburn}{17.3}
\newcommand{\hlOmAdjRNburn}{17.3}
\newcommand{\hlOmRawMeanburn}{18.2}
\newcommand{\hlOmAdjMeanburn}{18.2}
\newcommand{\hlHTwoAdjburn}{4.8}
\newcommand{\hlHTwoAdjCILoburn}{2.7}
\newcommand{\hlHTwoAdjCIHiburn}{6.9}
\newcommand{\hlOmRawRankburn}{2}
\newcommand{\hlOmAdjRankburn}{2}
\newcommand{\hlOmRawSATflair}{8.0}
\newcommand{\hlOmAdjSATflair}{8.8}
\newcommand{\hlOmRawLVDflair}{3.4}
\newcommand{\hlOmAdjLVDflair}{4.2}
\newcommand{\hlOmRawDOFAflair}{4.2}
\newcommand{\hlOmAdjDOFAflair}{4.9}
\newcommand{\hlOmRawTMflair}{5.5}
\newcommand{\hlOmAdjTMflair}{6.1}
\newcommand{\hlOmRawRNflair}{3.6}
\newcommand{\hlOmAdjRNflair}{4.3}
\newcommand{\hlOmRawMeanflair}{5.1}
\newcommand{\hlOmAdjMeanflair}{5.8}
\newcommand{\hlHTwoAdjflair}{0.7}
\newcommand{\hlHTwoAdjCILoflair}{0.1}
\newcommand{\hlHTwoAdjCIHiflair}{1.3}
\newcommand{\hlOmRawRankflair}{3}
\newcommand{\hlOmAdjRankflair}{1}
\newcommand{\hlFThreeRawflairEst}{\ensuremath{-}2.8}
\newcommand{\hlFThreeRawflairCILo}{\ensuremath{-}3.8}
\newcommand{\hlFThreeRawflairCIHi}{\ensuremath{-}1.9}
\newcommand{\hlFThreeRawflairP}{0.001}
\newcommand{\hlFThreeRawflairPHolm}{0.002}
\newcommand{\hlFThreeRawflairN}{5}
\newcommand{\hlFThreeAdjflairEst}{\ensuremath{-}2.8}
\newcommand{\hlFThreeAdjflairCILo}{\ensuremath{-}3.8}
\newcommand{\hlFThreeAdjflairCIHi}{\ensuremath{-}1.9}
\newcommand{\hlFThreeAdjflairP}{0.001}
\newcommand{\hlFThreeAdjflairPHolm}{0.002}
\newcommand{\hlFThreeAdjflairN}{5}
\newcommand{\hlFThreeAdjflairIncludesZero}{no}
\newcommand{\hlFThreeAdjflairVerdict}{established}
\newcommand{\hlFThreeAdjflairSlopeArm}{\ensuremath{-}0.42}
\newcommand{\hlFFourRawflairEst}{\ensuremath{-}1.2}
\newcommand{\hlFFourRawflairCILo}{\ensuremath{-}2.3}
\newcommand{\hlFFourRawflairCIHi}{\ensuremath{-}0.1}
\newcommand{\hlFFourRawflairP}{0.036}
\newcommand{\hlFFourRawflairPHolm}{0.036}
\newcommand{\hlFFourRawflairN}{5}
\newcommand{\hlFFourAdjflairEst}{\ensuremath{-}0.6}
\newcommand{\hlFFourAdjflairCILo}{\ensuremath{-}2.0}
\newcommand{\hlFFourAdjflairCIHi}{0.9}
\newcommand{\hlFFourAdjflairP}{0.353}
\newcommand{\hlFFourAdjflairPHolm}{0.353}
\newcommand{\hlFFourAdjflairN}{5}
\newcommand{\hlFFourAdjflairIncludesZero}{yes}
\newcommand{\hlFFourAdjflairVerdict}{undetermined}
\newcommand{\hlCollFOneAllEst}{4.3}
\newcommand{\hlCollFOneAllCILo}{1.3}
\newcommand{\hlCollFOneAllCIHi}{7.3}
\newcommand{\hlCollFOneAllN}{8}
\newcommand{\hlCollFTwoAllEst}{0.0}
\newcommand{\hlCollFTwoAllCILo}{\ensuremath{-}2.8}
\newcommand{\hlCollFTwoAllCIHi}{2.7}
\newcommand{\hlCollFTwoAllN}{8}
\newcommand{\hlCollFThreeAllEst}{\ensuremath{-}5.4}
\newcommand{\hlCollFThreeAllCILo}{\ensuremath{-}8.3}
\newcommand{\hlCollFThreeAllCIHi}{\ensuremath{-}2.4}
\newcommand{\hlCollFThreeAllN}{5}
\newcommand{\hlCollFFourAllEst}{14.4}
\newcommand{\hlCollFFourAllCILo}{12.0}
\newcommand{\hlCollFFourAllCIHi}{16.8}
\newcommand{\hlCollFFourAllN}{5}
\newcommand{\hlCollHTwoAllEst}{4.8}
\newcommand{\hlCollHTwoAllCILo}{2.6}
\newcommand{\hlCollHTwoAllCIHi}{7.1}
\newcommand{\hlCollHTwoAllN}{40}
\newcommand{\hlCollTypeMeanCoarseAll}{18.4}
\newcommand{\hlCollTypeMeanOmissionAll}{18.2}
\newcommand{\hlCollTypeMeanBoundaryAll}{13.4}
\newcommand{\hlCollTypeMeanShiftAll}{11.7}
\newcommand{\hlCollFOneWithoutEst}{3.1}
\newcommand{\hlCollFOneWithoutCILo}{1.0}
\newcommand{\hlCollFOneWithoutCIHi}{5.2}
\newcommand{\hlCollFOneWithoutN}{8}
\newcommand{\hlCollFTwoWithoutEst}{0.7}
\newcommand{\hlCollFTwoWithoutCILo}{\ensuremath{-}0.7}
\newcommand{\hlCollFTwoWithoutCIHi}{2.0}
\newcommand{\hlCollFTwoWithoutN}{8}
\newcommand{\hlCollFThreeWithoutEst}{\ensuremath{-}4.5}
\newcommand{\hlCollFThreeWithoutCILo}{\ensuremath{-}7.0}
\newcommand{\hlCollFThreeWithoutCIHi}{\ensuremath{-}2.0}
\newcommand{\hlCollFThreeWithoutN}{4}
\newcommand{\hlCollFFourWithoutEst}{14.7}
\newcommand{\hlCollFFourWithoutCILo}{11.3}
\newcommand{\hlCollFFourWithoutCIHi}{18.1}
\newcommand{\hlCollFFourWithoutN}{4}
\newcommand{\hlCollHTwoWithoutEst}{3.6}
\newcommand{\hlCollHTwoWithoutCILo}{1.6}
\newcommand{\hlCollHTwoWithoutCIHi}{5.6}
\newcommand{\hlCollHTwoWithoutN}{36}
\newcommand{\hlCollTypeMeanCoarseWithout}{18.2}
\newcommand{\hlCollTypeMeanOmissionWithout}{16.8}
\newcommand{\hlCollTypeMeanBoundaryWithout}{13.4}
\newcommand{\hlCollTypeMeanShiftWithout}{11.7}
\newcommand{\hlCollapsedMainGridN}{5}
\newcommand{\hlCollapsedIoUMax}{14.8}
\newcommand{\hlCollapsedEpochMin}{2}
\newcommand{\hlCollapsedEpochMax}{16}
\newcommand{\hlBreakEvenModelMinburn}{\ensuremath{>}4.0}
\newcommand{\hlBreakEvenModelMaxburn}{\ensuremath{>}4.0}
\newcommand{\hlBreakEvenModelAboveburn}{5}
\newcommand{\hlBreakEvenModelNburn}{5}
\newcommand{\hlBreakEvenSATburn}{\ensuremath{>}4.0}
\newcommand{\hlBreakEvenLVDburn}{\ensuremath{>}4.0}
\newcommand{\hlBreakEvenDOFAburn}{\ensuremath{>}4.0}
\newcommand{\hlBreakEvenTMburn}{\ensuremath{>}4.0}
\newcommand{\hlBreakEvenRNburn}{\ensuremath{>}4.0}
\newcommand{\hlBreakEvenSeedMinburn}{\ensuremath{>}4.0}
\newcommand{\hlBreakEvenSeedMaxburn}{\ensuremath{>}4.0}
\newcommand{\hlBreakEvenSeedAboveburn}{5}
\newcommand{\hlBreakEvenSeedNburn}{5}
\newcommand{\hlBreakEvenModelMinflair}{2.3}
\newcommand{\hlBreakEvenModelMaxflair}{\ensuremath{>}4.0}
\newcommand{\hlBreakEvenModelAboveflair}{1}
\newcommand{\hlBreakEvenModelNflair}{5}
\newcommand{\hlBreakEvenSATflair}{\ensuremath{>}4.0}
\newcommand{\hlBreakEvenLVDflair}{3.1}
\newcommand{\hlBreakEvenDOFAflair}{3.7}
\newcommand{\hlBreakEvenTMflair}{2.3}
\newcommand{\hlBreakEvenRNflair}{2.4}
\newcommand{\hlBreakEvenSeedMinflair}{2.5}
\newcommand{\hlBreakEvenSeedMaxflair}{3.9}
\newcommand{\hlBreakEvenSeedAboveflair}{0}
\newcommand{\hlBreakEvenSeedNflair}{5}
\newcommand{\hlTypeRankLOneburnOne}{omission}
\newcommand{\hlTypeRankLOneburnTwo}{coarse}
\newcommand{\hlTypeRankLOneburnThree}{boundary}
\newcommand{\hlTypeRankLOneburnFour}{shift}
\newcommand{\hlTypeRankLOneChesOne}{omission}
\newcommand{\hlTypeRankLOneChesTwo}{boundary}
\newcommand{\hlTypeRankLOneChesThree}{coarse}
\newcommand{\hlTypeRankLOneChesFour}{shift}
\newcommand{\hlTypeRankLOneCsTwelveOne}{omission}
\newcommand{\hlTypeRankLOneCsTwelveTwo}{boundary}
\newcommand{\hlTypeRankLOneCsTwelveThree}{coarse}
\newcommand{\hlTypeRankLOneCsTwelveFour}{shift}
\newcommand{\hlTypeRankLOneDfcOne}{omission}
\newcommand{\hlTypeRankLOneDfcTwo}{boundary}
\newcommand{\hlTypeRankLOneDfcThree}{coarse}
\newcommand{\hlTypeRankLOneDfcFour}{shift}
\newcommand{\hlTypeRankLOneEnvaOne}{omission}
\newcommand{\hlTypeRankLOneEnvaTwo}{boundary}
\newcommand{\hlTypeRankLOneEnvaThree}{shift}
\newcommand{\hlTypeRankLOneEnvaFour}{coarse}
\newcommand{\hlTypeRankLOneflairOne}{boundary}
\newcommand{\hlTypeRankLOneflairTwo}{omission}
\newcommand{\hlTypeRankLOneflairThree}{coarse}
\newcommand{\hlTypeRankLOneflairFour}{shift}
\newcommand{\hlTypeRankLOneKuroOne}{omission}
\newcommand{\hlTypeRankLOneKuroTwo}{shift}
\newcommand{\hlTypeRankLOneKuroThree}{boundary}
\newcommand{\hlTypeRankLOneKuroFour}{coarse}
\newcommand{\hlTypeRankLOneOemOne}{omission}
\newcommand{\hlTypeRankLOneOemTwo}{boundary}
\newcommand{\hlTypeRankLOneOemThree}{coarse}
\newcommand{\hlTypeRankLOneOemFour}{shift}
\newcommand{\hlTypeRankLOneSnTwoOne}{omission}
\newcommand{\hlTypeRankLOneSnTwoTwo}{boundary}
\newcommand{\hlTypeRankLOneSnTwoThree}{coarse}
\newcommand{\hlTypeRankLOneSnTwoFour}{shift}
\newcommand{\hlMixedConvergedburn}{yes}
\newcommand{\hlMixedUsableburn}{yes}
\newcommand{\hlMixedCoefburnCoarse}{5.7}
\newcommand{\hlMixedSEburnCoarse}{2.6}
\newcommand{\hlMixedCoefburnOmission}{9.7}
\newcommand{\hlMixedSEburnOmission}{2.6}
\newcommand{\hlMixedCoefburnShift}{2.2}
\newcommand{\hlMixedSEburnShift}{2.6}
\newcommand{\hlMixedConvergedflair}{yes}
\newcommand{\hlMixedUsableflair}{yes}
\newcommand{\hlMixedCoefflairCoarse}{2.0}
\newcommand{\hlMixedSEflairCoarse}{0.7}
\newcommand{\hlMixedCoefflairOmission}{0.4}
\newcommand{\hlMixedSEflairOmission}{0.7}
\newcommand{\hlMixedCoefflairShift}{\ensuremath{-}1.0}
\newcommand{\hlMixedSEflairShift}{0.7}
\newcommand{\hlGpuHours}{2,382}
\newcommand{\hlGpuHoursCore}{101}
\newcommand{\hlNRunsGpu}{10127}
\newcommand{\hlNRunsGpuCore}{758}
\newcommand{\hlNRunsGpuExt}{9369}
\newcommand{\hlRetDsDiffSAT}{11.4}
\newcommand{\hlRetDsDiffCILoSAT}{8.0}
\newcommand{\hlRetDsDiffCIHiSAT}{14.8}
\newcommand{\hlRetDsDiffLVD}{10.0}
\newcommand{\hlRetDsDiffCILoLVD}{7.3}
\newcommand{\hlRetDsDiffCIHiLVD}{12.7}
\newcommand{\hlRetDsDiffDOFA}{11.8}
\newcommand{\hlRetDsDiffCILoDOFA}{9.9}
\newcommand{\hlRetDsDiffCIHiDOFA}{13.8}
\newcommand{\hlRetDsDiffTM}{2.1}
\newcommand{\hlRetDsDiffCILoTM}{\ensuremath{-}0.8}
\newcommand{\hlRetDsDiffCIHiTM}{5.1}
\newcommand{\hlRetDsDiffRN}{8.6}
\newcommand{\hlRetDsDiffCILoRN}{3.8}
\newcommand{\hlRetDsDiffCIHiRN}{13.5}
\newcommand{\hlHOneSeedburnEst}{1.7}
\newcommand{\hlHOneSeedburnCILo}{0.5}
\newcommand{\hlHOneSeedburnCIHi}{2.9}
\newcommand{\hlHOneSeedburnN}{8}
\newcommand{\hlHOneSeedburnIncludesZero}{no}
\newcommand{\hlHTwoSeedburnEst}{4.8}
\newcommand{\hlHTwoSeedburnCILo}{1.2}
\newcommand{\hlHTwoSeedburnCIHi}{8.5}
\newcommand{\hlHTwoSeedburnN}{8}
\newcommand{\hlHTwoSeedburnIncludesZero}{no}
\newcommand{\hlHTwoAdjSeedburnEst}{4.8}
\newcommand{\hlHTwoAdjSeedburnCILo}{2.1}
\newcommand{\hlHTwoAdjSeedburnCIHi}{7.5}
\newcommand{\hlHTwoAdjSeedburnN}{8}
\newcommand{\hlHTwoAdjSeedburnIncludesZero}{no}
\newcommand{\hlHOneSeedflairEst}{1.7}
\newcommand{\hlHOneSeedflairCILo}{1.0}
\newcommand{\hlHOneSeedflairCIHi}{2.4}
\newcommand{\hlHOneSeedflairN}{5}
\newcommand{\hlHOneSeedflairIncludesZero}{no}
\newcommand{\hlHTwoSeedflairEst}{\ensuremath{-}0.2}
\newcommand{\hlHTwoSeedflairCILo}{\ensuremath{-}1.8}
\newcommand{\hlHTwoSeedflairCIHi}{1.4}
\newcommand{\hlHTwoSeedflairN}{5}
\newcommand{\hlHTwoSeedflairIncludesZero}{yes}
\newcommand{\hlHTwoAdjSeedflairEst}{0.5}
\newcommand{\hlHTwoAdjSeedflairCILo}{\ensuremath{-}1.0}
\newcommand{\hlHTwoAdjSeedflairCIHi}{2.0}
\newcommand{\hlHTwoAdjSeedflairN}{5}
\newcommand{\hlHTwoAdjSeedflairIncludesZero}{yes}
\newcommand{\hlHwSThreeCellsNburn}{10}
\newcommand{\hlHwSThreeNClassesburn}{3}
\newcommand{\hlHwSThreeRangeMaxLTwoburn}{6.8}
\newcommand{\hlHwSThreeRangeMaxTypeLTwoburn}{boundary}
\newcommand{\hlHwSThreeRangeMeanLTwoburn}{3.4}
\newcommand{\hlHwSThreeRangeMinLTwoburn}{1.2}
\newcommand{\hlHwSThreeCellsNflair}{10}
\newcommand{\hlHwSThreeNClassesflair}{3}
\newcommand{\hlHwSThreeRangeMaxLTwoflair}{4.0}
\newcommand{\hlHwSThreeRangeMaxTypeLTwoflair}{boundary}
\newcommand{\hlHwSThreeRangeMeanLTwoflair}{3.5}
\newcommand{\hlHwSThreeRangeMinLTwoflair}{2.7}
\newcommand{\hlCollapsedExtN}{4}
\newcommand{\hlCollapsedExtSThreeN}{0}
\newcommand{\hlCollapsedExtModelsN}{3}
\newcommand{\hlCollapsedExtTypes}{\etype{omission} \Ltwo}
\newcommand{\hlCollapsedExtList}{\cnxl seed 3, \rnssl seed 3, \vitr seed 3 and \vitr seed 4}
\newcommand{\hlOtsuLabelMiouTrain}{68.3}
\newcommand{\hlOtsuLabelMiouFracTrain}{0.683}
\newcommand{\hlOtsuFlipRateTrain}{7.9}
\newcommand{\hlOtsuNTilesTrain}{252}
\newcommand{\hlOtsuIoUWaterTrain}{45.1}
\newcommand{\hlOtsuIoUNotWaterTrain}{91.5}
\newcommand{\hlOtsuLabelMiouVal}{71.1}
\newcommand{\hlOtsuLabelMiouFracVal}{0.711}
\newcommand{\hlOtsuFlipRateVal}{7.7}
\newcommand{\hlOtsuNTilesVal}{89}
\newcommand{\hlOtsuIoUWaterVal}{50.6}
\newcommand{\hlOtsuIoUNotWaterVal}{91.6}
\newcommand{\hlOtsuLabelMiouAll}{69.1}
\newcommand{\hlOtsuLabelMiouFracAll}{0.691}
\newcommand{\hlOtsuFlipRateAll}{7.9}
\newcommand{\hlOtsuNTilesAll}{341}
\newcommand{\hlOtsuIoUWaterAll}{46.6}
\newcommand{\hlOtsuIoUNotWaterAll}{91.6}
\newcommand{\hlVeFOneFiveburnEst}{3.7}
\newcommand{\hlVeFOneFiveburnN}{5}
\newcommand{\hlVeFOneFiveburnP}{0.040}
\newcommand{\hlVeFOneFiveburnCILo}{0.3}
\newcommand{\hlVeFOneFiveburnCIHi}{7.1}
\newcommand{\hlVeFOneSignFlipburnEst}{4.3}
\newcommand{\hlVeFOneSignFlipburnN}{8}
\newcommand{\hlVeFOneSignFlipburnP}{0.016}
\newcommand{\hlVeFOneSignFlipburnFloorFive}{0.0625}
\newcommand{\hlVeNSixTostburnEst}{\ensuremath{-}0.2}
\newcommand{\hlVeNSixTostburnN}{5}
\newcommand{\hlVeNSixTostburnP}{0.044}
\newcommand{\hlVeNSixTostburnCILo}{\ensuremath{-}2.9}
\newcommand{\hlVeNSixTostburnCIHi}{2.5}
\newcommand{\hlVeNSixTostburnEquivalent}{yes}
\newcommand{\hlVeNSixMdeburnEst}{5.8}
\newcommand{\hlVeNSixMdeburnN}{5}
\newcommand{\hlVeNSixMdeburnP}{--}
\newcommand{\hlVeNFiveMdeThreeburnEst}{3.9}
\newcommand{\hlVeNFiveMdeThreeburnN}{3}
\newcommand{\hlVeNFiveMdeThreeburnP}{--}
\newcommand{\hlVeNFiveMdeFiveburnEst}{5.7}
\newcommand{\hlVeNFiveMdeFiveburnN}{5}
\newcommand{\hlVeNFiveMdeFiveburnP}{--}
\newcommand{\hlVeFFourLOneburnEst}{\ensuremath{-}1.3}
\newcommand{\hlVeFFourLOneburnN}{5}
\newcommand{\hlVeFFourLOneburnP}{0.030}
\newcommand{\hlVeFFourLOneburnCILo}{\ensuremath{-}2.4}
\newcommand{\hlVeFFourLOneburnCIHi}{\ensuremath{-}0.2}
\newcommand{\hlVeSThreeTMburnEst}{0.0}
\newcommand{\hlVeSThreeTMburnN}{5}
\newcommand{\hlVeSThreeTMburnP}{0.970}
\newcommand{\hlVeSThreeTMburnCILo}{\ensuremath{-}3.3}
\newcommand{\hlVeSThreeTMburnCIHi}{3.4}
\newcommand{\hlVeDOFARNburnEst}{2.3}
\newcommand{\hlVeDOFARNburnN}{8}
\newcommand{\hlVeDOFARNburnP}{0.105}
\newcommand{\hlVeDOFARNburnCILo}{\ensuremath{-}0.6}
\newcommand{\hlVeDOFARNburnCIHi}{5.1}
\newcommand{\hlVeTMRNburnEst}{\ensuremath{-}2.4}
\newcommand{\hlVeTMRNburnN}{8}
\newcommand{\hlVeTMRNburnP}{0.114}
\newcommand{\hlVeTMRNburnCILo}{\ensuremath{-}5.4}
\newcommand{\hlVeTMRNburnCIHi}{0.7}
\newcommand{\hlVeFrozenSATburnEst}{6.5}
\newcommand{\hlVeFrozenSATburnN}{5}
\newcommand{\hlVeFrozenSATburnP}{0.043}
\newcommand{\hlVeFrozenSATburnCILo}{0.3}
\newcommand{\hlVeFrozenSATburnCIHi}{12.6}
\newcommand{\hlVeFrozenDOFAburnEst}{\ensuremath{-}4.2}
\newcommand{\hlVeFrozenDOFAburnN}{5}
\newcommand{\hlVeFrozenDOFAburnP}{0.006}
\newcommand{\hlVeFrozenDOFAburnCILo}{\ensuremath{-}6.4}
\newcommand{\hlVeFrozenDOFAburnCIHi}{\ensuremath{-}2.1}
\newcommand{\hlVeFrozenTMburnEst}{1.0}
\newcommand{\hlVeFrozenTMburnN}{5}
\newcommand{\hlVeFrozenTMburnP}{0.618}
\newcommand{\hlVeFrozenTMburnCILo}{\ensuremath{-}4.1}
\newcommand{\hlVeFrozenTMburnCIHi}{6.0}
\newcommand{\hlVeMemSATLVDburnEst}{\ensuremath{-}8.4}
\newcommand{\hlVeMemSATLVDburnN}{8}
\newcommand{\hlVeMemSATLVDburnP}{0.226}
\newcommand{\hlVeMemSATLVDburnCILo}{\ensuremath{-}23.5}
\newcommand{\hlVeMemSATLVDburnCIHi}{6.6}
\newcommand{\hlVeNoisyLVDSATburnEst}{9.1}
\newcommand{\hlVeNoisyLVDSATburnN}{8}
\newcommand{\hlVeNoisyLVDSATburnP}{\ensuremath{<}0.001}
\newcommand{\hlVeNoisyLVDSATburnCILo}{7.5}
\newcommand{\hlVeNoisyLVDSATburnCIHi}{10.8}
\newcommand{\hlVeNoisyLVDSATNSixburnEst}{0.5}
\newcommand{\hlVeNoisyLVDSATNSixburnN}{5}
\newcommand{\hlVeNoisyLVDSATNSixburnP}{0.501}
\newcommand{\hlVeNoisyLVDSATNSixburnCILo}{\ensuremath{-}1.4}
\newcommand{\hlVeNoisyLVDSATNSixburnCIHi}{2.4}
\newcommand{\hlVeFrozenSATNSixburnEst}{\ensuremath{-}5.6}
\newcommand{\hlVeFrozenSATNSixburnN}{5}
\newcommand{\hlVeFrozenSATNSixburnP}{0.005}
\newcommand{\hlVeFrozenSATNSixburnCILo}{\ensuremath{-}8.5}
\newcommand{\hlVeFrozenSATNSixburnCIHi}{\ensuremath{-}2.8}
\newcommand{\hlVeFOneFiveflairEst}{2.9}
\newcommand{\hlVeFOneFiveflairN}{5}
\newcommand{\hlVeFOneFiveflairP}{0.007}
\newcommand{\hlVeFOneFiveflairCILo}{1.3}
\newcommand{\hlVeFOneFiveflairCIHi}{4.5}
\newcommand{\hlVeFOneSignFlipflairEst}{2.8}
\newcommand{\hlVeFOneSignFlipflairN}{8}
\newcommand{\hlVeFOneSignFlipflairP}{0.008}
\newcommand{\hlVeFOneSignFlipflairFloorFive}{0.0625}
\newcommand{\hlVeNSixTostflairEst}{1.5}
\newcommand{\hlVeNSixTostflairN}{5}
\newcommand{\hlVeNSixTostflairP}{0.006}
\newcommand{\hlVeNSixTostflairCILo}{0.8}
\newcommand{\hlVeNSixTostflairCIHi}{2.2}
\newcommand{\hlVeNSixTostflairEquivalent}{yes}
\newcommand{\hlVeNSixMdeflairEst}{1.6}
\newcommand{\hlVeNSixMdeflairN}{5}
\newcommand{\hlVeNSixMdeflairP}{--}
\newcommand{\hlVeNFiveMdeThreeflairEst}{2.1}
\newcommand{\hlVeNFiveMdeThreeflairN}{3}
\newcommand{\hlVeNFiveMdeThreeflairP}{--}
\newcommand{\hlVeNFiveMdeFiveflairEst}{2.6}
\newcommand{\hlVeNFiveMdeFiveflairN}{5}
\newcommand{\hlVeNFiveMdeFiveflairP}{--}
\newcommand{\hlVeFFourLOneflairEst}{\ensuremath{-}4.5}
\newcommand{\hlVeFFourLOneflairN}{5}
\newcommand{\hlVeFFourLOneflairP}{\ensuremath{<}0.001}
\newcommand{\hlVeFFourLOneflairCILo}{\ensuremath{-}5.1}
\newcommand{\hlVeFFourLOneflairCIHi}{\ensuremath{-}3.8}
\newcommand{\hlVeSThreeTMflairEst}{0.0}
\newcommand{\hlVeSThreeTMflairN}{5}
\newcommand{\hlVeSThreeTMflairP}{0.966}
\newcommand{\hlVeSThreeTMflairCILo}{\ensuremath{-}1.4}
\newcommand{\hlVeSThreeTMflairCIHi}{1.4}
\newcommand{\hlVeDOFARNflairEst}{0.1}
\newcommand{\hlVeDOFARNflairN}{5}
\newcommand{\hlVeDOFARNflairP}{0.875}
\newcommand{\hlVeDOFARNflairCILo}{\ensuremath{-}1.8}
\newcommand{\hlVeDOFARNflairCIHi}{2.0}
\newcommand{\hlVeTMRNflairEst}{1.0}
\newcommand{\hlVeTMRNflairN}{5}
\newcommand{\hlVeTMRNflairP}{0.442}
\newcommand{\hlVeTMRNflairCILo}{\ensuremath{-}2.3}
\newcommand{\hlVeTMRNflairCIHi}{4.4}
\newcommand{\hlVeFrozenSATflairEst}{\ensuremath{-}3.2}
\newcommand{\hlVeFrozenSATflairN}{5}
\newcommand{\hlVeFrozenSATflairP}{0.006}
\newcommand{\hlVeFrozenSATflairCILo}{\ensuremath{-}4.8}
\newcommand{\hlVeFrozenSATflairCIHi}{\ensuremath{-}1.5}
\newcommand{\hlVeFrozenDOFAflairEst}{\ensuremath{-}1.6}
\newcommand{\hlVeFrozenDOFAflairN}{5}
\newcommand{\hlVeFrozenDOFAflairP}{0.041}
\newcommand{\hlVeFrozenDOFAflairCILo}{\ensuremath{-}3.1}
\newcommand{\hlVeFrozenDOFAflairCIHi}{\ensuremath{-}0.1}
\newcommand{\hlVeFrozenTMflairEst}{\ensuremath{-}0.8}
\newcommand{\hlVeFrozenTMflairN}{5}
\newcommand{\hlVeFrozenTMflairP}{0.257}
\newcommand{\hlVeFrozenTMflairCILo}{\ensuremath{-}2.6}
\newcommand{\hlVeFrozenTMflairCIHi}{0.9}
\newcommand{\hlVeMemSATLVDflairEst}{17.9}
\newcommand{\hlVeMemSATLVDflairN}{8}
\newcommand{\hlVeMemSATLVDflairP}{0.055}
\newcommand{\hlVeMemSATLVDflairCILo}{\ensuremath{-}0.5}
\newcommand{\hlVeMemSATLVDflairCIHi}{36.4}
\newcommand{\hlVeNoisyLVDSATflairEst}{1.1}
\newcommand{\hlVeNoisyLVDSATflairN}{8}
\newcommand{\hlVeNoisyLVDSATflairP}{0.009}
\newcommand{\hlVeNoisyLVDSATflairCILo}{0.4}
\newcommand{\hlVeNoisyLVDSATflairCIHi}{1.9}
\newcommand{\hlVeNoisyLVDSATNSixflairEst}{1.8}
\newcommand{\hlVeNoisyLVDSATNSixflairN}{5}
\newcommand{\hlVeNoisyLVDSATNSixflairP}{0.001}
\newcommand{\hlVeNoisyLVDSATNSixflairCILo}{1.2}
\newcommand{\hlVeNoisyLVDSATNSixflairCIHi}{2.4}
\newcommand{\hlVeFrozenSATNSixflairEst}{\ensuremath{-}3.5}
\newcommand{\hlVeFrozenSATNSixflairN}{5}
\newcommand{\hlVeFrozenSATNSixflairP}{0.010}
\newcommand{\hlVeFrozenSATNSixflairCILo}{\ensuremath{-}5.6}
\newcommand{\hlVeFrozenSATNSixflairCIHi}{\ensuremath{-}1.4}
\newcommand{\hlVeFTwoCollTostburnEst}{0.7}
\newcommand{\hlVeFTwoCollTostburnN}{8}
\newcommand{\hlVeFTwoCollTostburnP}{0.002}
\newcommand{\hlVeFTwoCollTostburnCILo}{\ensuremath{-}0.4}
\newcommand{\hlVeFTwoCollTostburnCIHi}{1.8}
\newcommand{\hlVeFTwoCollTostburnEquivalent}{yes}
\newcommand{\hlDecMeanDropUNetburn}{15.7}
\newcommand{\hlDecCleanUNetburn}{83.5}
\newcommand{\hlDecInvburnEst}{1.4}
\newcommand{\hlDecInvburnCILo}{0.0}
\newcommand{\hlDecInvburnCIHi}{2.8}
\newcommand{\hlDecInvburnTostCILo}{0.3}
\newcommand{\hlDecInvburnTostCIHi}{2.6}
\newcommand{\hlDecInvburnMde}{2.2}
\newcommand{\hlDecInvburnPHolm}{0.097}
\newcommand{\hlDecInvburnN}{25}
\newcommand{\hlDecInvSATburnEst}{1.6}
\newcommand{\hlDecInvSATburnCILo}{\ensuremath{-}1.8}
\newcommand{\hlDecInvSATburnCIHi}{5.0}
\newcommand{\hlDecInvLVDburnEst}{1.6}
\newcommand{\hlDecInvLVDburnCILo}{0.5}
\newcommand{\hlDecInvLVDburnCIHi}{2.8}
\newcommand{\hlDecInvDOFAburnEst}{3.0}
\newcommand{\hlDecInvDOFAburnCILo}{1.5}
\newcommand{\hlDecInvDOFAburnCIHi}{4.5}
\newcommand{\hlDecInvTMburnEst}{2.7}
\newcommand{\hlDecInvTMburnCILo}{\ensuremath{-}2.1}
\newcommand{\hlDecInvTMburnCIHi}{7.6}
\newcommand{\hlDecInvRNburnEst}{\ensuremath{-}1.8}
\newcommand{\hlDecInvRNburnCILo}{\ensuremath{-}8.2}
\newcommand{\hlDecInvRNburnCIHi}{4.6}
\newcommand{\hlDecNSixburnEst}{1.4}
\newcommand{\hlDecNSixburnCILo}{\ensuremath{-}2.1}
\newcommand{\hlDecNSixburnCIHi}{5.0}
\newcommand{\hlDecNSixburnTostCILo}{\ensuremath{-}1.3}
\newcommand{\hlDecNSixburnTostCIHi}{4.2}
\newcommand{\hlDecNSixburnMde}{5.8}
\newcommand{\hlDecNSixburnPHolm}{0.319}
\newcommand{\hlDecNSixburnN}{5}
\newcommand{\hlDecFTwoburnEst}{4.2}
\newcommand{\hlDecFTwoburnCILo}{1.2}
\newcommand{\hlDecFTwoburnCIHi}{7.1}
\newcommand{\hlDecFTwoburnTostCILo}{1.9}
\newcommand{\hlDecFTwoburnTostCIHi}{6.5}
\newcommand{\hlDecFTwoburnMde}{4.9}
\newcommand{\hlDecFTwoburnPHolm}{0.017}
\newcommand{\hlDecFTwoburnN}{5}
\newcommand{\hlDecFOneburnEst}{3.7}
\newcommand{\hlDecFOneburnCILo}{1.5}
\newcommand{\hlDecFOneburnCIHi}{5.8}
\newcommand{\hlDecFOneburnTostCILo}{2.0}
\newcommand{\hlDecFOneburnTostCIHi}{5.3}
\newcommand{\hlDecFOneburnMde}{3.5}
\newcommand{\hlDecFOneburnPHolm}{0.009}
\newcommand{\hlDecFOneburnN}{5}
\newcommand{\hlDecFOneOneburnEst}{2.4}
\newcommand{\hlDecFOneOneburnCILo}{1.1}
\newcommand{\hlDecFOneOneburnCIHi}{3.7}
\newcommand{\hlDecFOneOneburnTostCILo}{1.4}
\newcommand{\hlDecFOneOneburnTostCIHi}{3.4}
\newcommand{\hlDecFOneOneburnMde}{2.1}
\newcommand{\hlDecFOneOneburnPHolm}{0.007}
\newcommand{\hlDecFOneOneburnN}{5}
\newcommand{\hlDecTypeRankburnOne}{omission}
\newcommand{\hlDecTypeRankburnTwo}{coarse}
\newcommand{\hlDecTypeRankburnThree}{boundary}
\newcommand{\hlDecTypeRankburnFour}{shift}
\newcommand{\hlDecVerdictburn}{Equivalent within $\pm$\TostMargin, SegFormer head loses more}
\newcommand{\hlDecVerdictNSixburn}{Undetermined, MDE 5.8}
\newcommand{\hlDecVerdictFTwoburn}{\rn loses less}
\newcommand{\hlDecInvSegfburnEst}{1.4}
\newcommand{\hlDecInvSegfburnCILo}{0.0}
\newcommand{\hlDecInvSegfburnCIHi}{2.8}
\newcommand{\hlDecInvSegfburnTostCILo}{0.3}
\newcommand{\hlDecInvSegfburnTostCIHi}{2.6}
\newcommand{\hlDecInvSegfburnMde}{2.2}
\newcommand{\hlDecInvSegfburnPHolm}{0.097}
\newcommand{\hlDecInvSegfburnN}{25}
\newcommand{\hlDecInvSegfSATburnEst}{1.6}
\newcommand{\hlDecInvSegfSATburnCILo}{\ensuremath{-}1.8}
\newcommand{\hlDecInvSegfSATburnCIHi}{5.0}
\newcommand{\hlDecInvSegfLVDburnEst}{1.6}
\newcommand{\hlDecInvSegfLVDburnCILo}{0.5}
\newcommand{\hlDecInvSegfLVDburnCIHi}{2.8}
\newcommand{\hlDecInvSegfDOFAburnEst}{3.0}
\newcommand{\hlDecInvSegfDOFAburnCILo}{1.5}
\newcommand{\hlDecInvSegfDOFAburnCIHi}{4.5}
\newcommand{\hlDecInvSegfTMburnEst}{2.7}
\newcommand{\hlDecInvSegfTMburnCILo}{\ensuremath{-}2.1}
\newcommand{\hlDecInvSegfTMburnCIHi}{7.6}
\newcommand{\hlDecInvSegfRNburnEst}{\ensuremath{-}1.8}
\newcommand{\hlDecInvSegfRNburnCILo}{\ensuremath{-}8.2}
\newcommand{\hlDecInvSegfRNburnCIHi}{4.6}
\newcommand{\hlDecNSixSegfburnEst}{1.4}
\newcommand{\hlDecNSixSegfburnCILo}{\ensuremath{-}2.1}
\newcommand{\hlDecNSixSegfburnCIHi}{5.0}
\newcommand{\hlDecNSixSegfburnTostCILo}{\ensuremath{-}1.3}
\newcommand{\hlDecNSixSegfburnTostCIHi}{4.2}
\newcommand{\hlDecNSixSegfburnMde}{5.8}
\newcommand{\hlDecNSixSegfburnPHolm}{0.319}
\newcommand{\hlDecNSixSegfburnN}{5}
\newcommand{\hlDecFTwoSegfburnEst}{4.2}
\newcommand{\hlDecFTwoSegfburnCILo}{1.2}
\newcommand{\hlDecFTwoSegfburnCIHi}{7.1}
\newcommand{\hlDecFTwoSegfburnTostCILo}{1.9}
\newcommand{\hlDecFTwoSegfburnTostCIHi}{6.5}
\newcommand{\hlDecFTwoSegfburnMde}{4.9}
\newcommand{\hlDecFTwoSegfburnPHolm}{0.017}
\newcommand{\hlDecFTwoSegfburnN}{5}
\newcommand{\hlDecFOneSegfburnEst}{3.7}
\newcommand{\hlDecFOneSegfburnCILo}{1.5}
\newcommand{\hlDecFOneSegfburnCIHi}{5.8}
\newcommand{\hlDecFOneSegfburnTostCILo}{2.0}
\newcommand{\hlDecFOneSegfburnTostCIHi}{5.3}
\newcommand{\hlDecFOneSegfburnMde}{3.5}
\newcommand{\hlDecFOneSegfburnPHolm}{0.009}
\newcommand{\hlDecFOneSegfburnN}{5}
\newcommand{\hlDecFOneOneSegfburnEst}{2.4}
\newcommand{\hlDecFOneOneSegfburnCILo}{1.1}
\newcommand{\hlDecFOneOneSegfburnCIHi}{3.7}
\newcommand{\hlDecFOneOneSegfburnTostCILo}{1.4}
\newcommand{\hlDecFOneOneSegfburnTostCIHi}{3.4}
\newcommand{\hlDecFOneOneSegfburnMde}{2.1}
\newcommand{\hlDecFOneOneSegfburnPHolm}{0.007}
\newcommand{\hlDecFOneOneSegfburnN}{5}
\newcommand{\hlDecTypeRankSegfburnOne}{omission}
\newcommand{\hlDecTypeRankSegfburnTwo}{coarse}
\newcommand{\hlDecTypeRankSegfburnThree}{boundary}
\newcommand{\hlDecTypeRankSegfburnFour}{shift}
\newcommand{\hlDecVerdictSegfburn}{Equivalent within $\pm$\TostMargin, SegFormer head loses more}
\newcommand{\hlDecVerdictNSixSegfburn}{Undetermined, MDE 5.8}
\newcommand{\hlDecVerdictFTwoSegfburn}{\rn loses less}
\newcommand{\hlDecMeanDropSegfburn}{17.1}
\newcommand{\hlDecCleanSegfburn}{85.2}
\newcommand{\hlDecInvMtwoFburnEst}{\ensuremath{-}1.4}
\newcommand{\hlDecInvMtwoFburnCILo}{\ensuremath{-}5.7}
\newcommand{\hlDecInvMtwoFburnCIHi}{2.9}
\newcommand{\hlDecInvMtwoFburnTostCILo}{\ensuremath{-}5.0}
\newcommand{\hlDecInvMtwoFburnTostCIHi}{2.1}
\newcommand{\hlDecInvMtwoFburnMde}{6.8}
\newcommand{\hlDecInvMtwoFburnPHolm}{0.502}
\newcommand{\hlDecInvMtwoFburnN}{25}
\newcommand{\hlDecInvMtwoFSATburnEst}{\ensuremath{-}10.1}
\newcommand{\hlDecInvMtwoFSATburnCILo}{\ensuremath{-}29.6}
\newcommand{\hlDecInvMtwoFSATburnCIHi}{9.4}
\newcommand{\hlDecInvMtwoFLVDburnEst}{6.8}
\newcommand{\hlDecInvMtwoFLVDburnCILo}{5.2}
\newcommand{\hlDecInvMtwoFLVDburnCIHi}{8.5}
\newcommand{\hlDecInvMtwoFDOFAburnEst}{1.5}
\newcommand{\hlDecInvMtwoFDOFAburnCILo}{0.6}
\newcommand{\hlDecInvMtwoFDOFAburnCIHi}{2.5}
\newcommand{\hlDecInvMtwoFTMburnEst}{3.9}
\newcommand{\hlDecInvMtwoFTMburnCILo}{\ensuremath{-}2.2}
\newcommand{\hlDecInvMtwoFTMburnCIHi}{10.0}
\newcommand{\hlDecInvMtwoFRNburnEst}{\ensuremath{-}9.3}
\newcommand{\hlDecInvMtwoFRNburnCILo}{\ensuremath{-}19.9}
\newcommand{\hlDecInvMtwoFRNburnCIHi}{1.3}
\newcommand{\hlDecNSixMtwoFburnEst}{\ensuremath{-}2.3}
\newcommand{\hlDecNSixMtwoFburnCILo}{\ensuremath{-}4.6}
\newcommand{\hlDecNSixMtwoFburnCIHi}{0.0}
\newcommand{\hlDecNSixMtwoFburnTostCILo}{\ensuremath{-}4.1}
\newcommand{\hlDecNSixMtwoFburnTostCIHi}{\ensuremath{-}0.5}
\newcommand{\hlDecNSixMtwoFburnMde}{3.8}
\newcommand{\hlDecNSixMtwoFburnPHolm}{0.052}
\newcommand{\hlDecNSixMtwoFburnN}{5}
\newcommand{\hlDecFTwoMtwoFburnEst}{11.5}
\newcommand{\hlDecFTwoMtwoFburnCILo}{0.9}
\newcommand{\hlDecFTwoMtwoFburnCIHi}{22.1}
\newcommand{\hlDecFTwoMtwoFburnTostCILo}{3.4}
\newcommand{\hlDecFTwoMtwoFburnTostCIHi}{19.7}
\newcommand{\hlDecFTwoMtwoFburnMde}{17.5}
\newcommand{\hlDecFTwoMtwoFburnPHolm}{0.039}
\newcommand{\hlDecFTwoMtwoFburnN}{5}
\newcommand{\hlDecFOneMtwoFburnEst}{\ensuremath{-}13.3}
\newcommand{\hlDecFOneMtwoFburnCILo}{\ensuremath{-}34.8}
\newcommand{\hlDecFOneMtwoFburnCIHi}{8.3}
\newcommand{\hlDecFOneMtwoFburnTostCILo}{\ensuremath{-}29.8}
\newcommand{\hlDecFOneMtwoFburnTostCIHi}{3.3}
\newcommand{\hlDecFOneMtwoFburnMde}{35.6}
\newcommand{\hlDecFOneMtwoFburnPHolm}{0.162}
\newcommand{\hlDecFOneMtwoFburnN}{5}
\newcommand{\hlDecFOneOneMtwoFburnEst}{7.7}
\newcommand{\hlDecFOneOneMtwoFburnCILo}{\ensuremath{-}13.1}
\newcommand{\hlDecFOneOneMtwoFburnCIHi}{28.4}
\newcommand{\hlDecFOneOneMtwoFburnTostCILo}{\ensuremath{-}8.3}
\newcommand{\hlDecFOneOneMtwoFburnTostCIHi}{23.6}
\newcommand{\hlDecFOneOneMtwoFburnMde}{34.3}
\newcommand{\hlDecFOneOneMtwoFburnPHolm}{0.363}
\newcommand{\hlDecFOneOneMtwoFburnN}{5}
\newcommand{\hlDecTypeRankMtwoFburnOne}{omission}
\newcommand{\hlDecTypeRankMtwoFburnTwo}{coarse}
\newcommand{\hlDecTypeRankMtwoFburnThree}{boundary}
\newcommand{\hlDecTypeRankMtwoFburnFour}{shift}
\newcommand{\hlDecVerdictMtwoFburn}{Undetermined, MDE 6.8}
\newcommand{\hlDecVerdictNSixMtwoFburn}{Undetermined, MDE 3.8}
\newcommand{\hlDecVerdictFTwoMtwoFburn}{\rn loses less}
\newcommand{\hlDecMeanDropMtwoFburn}{14.3}
\newcommand{\hlDecCleanMtwoFburn}{76.3}
\newcommand{\hlDecInvSamburnEst}{1.3}
\newcommand{\hlDecInvSamburnCILo}{\ensuremath{-}0.3}
\newcommand{\hlDecInvSamburnCIHi}{3.0}
\newcommand{\hlDecInvSamburnTostCILo}{\ensuremath{-}0.1}
\newcommand{\hlDecInvSamburnTostCIHi}{2.7}
\newcommand{\hlDecInvSamburnMde}{2.6}
\newcommand{\hlDecInvSamburnPHolm}{0.226}
\newcommand{\hlDecInvSamburnN}{25}
\newcommand{\hlDecInvSamSATburnEst}{2.5}
\newcommand{\hlDecInvSamSATburnCILo}{1.0}
\newcommand{\hlDecInvSamSATburnCIHi}{4.0}
\newcommand{\hlDecInvSamLVDburnEst}{5.1}
\newcommand{\hlDecInvSamLVDburnCILo}{1.8}
\newcommand{\hlDecInvSamLVDburnCIHi}{8.3}
\newcommand{\hlDecInvSamDOFAburnEst}{\ensuremath{-}0.9}
\newcommand{\hlDecInvSamDOFAburnCILo}{\ensuremath{-}3.5}
\newcommand{\hlDecInvSamDOFAburnCIHi}{1.8}
\newcommand{\hlDecInvSamTMburnEst}{3.4}
\newcommand{\hlDecInvSamTMburnCILo}{\ensuremath{-}1.1}
\newcommand{\hlDecInvSamTMburnCIHi}{8.0}
\newcommand{\hlDecInvSamRNburnEst}{\ensuremath{-}3.5}
\newcommand{\hlDecInvSamRNburnCILo}{\ensuremath{-}7.6}
\newcommand{\hlDecInvSamRNburnCIHi}{0.6}
\newcommand{\hlDecNSixSamburnEst}{\ensuremath{-}6.5}
\newcommand{\hlDecNSixSamburnCILo}{\ensuremath{-}14.4}
\newcommand{\hlDecNSixSamburnCIHi}{1.4}
\newcommand{\hlDecNSixSamburnTostCILo}{\ensuremath{-}12.5}
\newcommand{\hlDecNSixSamburnTostCIHi}{\ensuremath{-}0.4}
\newcommand{\hlDecNSixSamburnMde}{13.0}
\newcommand{\hlDecNSixSamburnPHolm}{0.084}
\newcommand{\hlDecNSixSamburnN}{5}
\newcommand{\hlDecFTwoSamburnEst}{4.3}
\newcommand{\hlDecFTwoSamburnCILo}{2.3}
\newcommand{\hlDecFTwoSamburnCIHi}{6.3}
\newcommand{\hlDecFTwoSamburnTostCILo}{2.8}
\newcommand{\hlDecFTwoSamburnTostCIHi}{5.8}
\newcommand{\hlDecFTwoSamburnMde}{3.2}
\newcommand{\hlDecFTwoSamburnPHolm}{0.004}
\newcommand{\hlDecFTwoSamburnN}{5}
\newcommand{\hlDecFOneSamburnEst}{1.1}
\newcommand{\hlDecFOneSamburnCILo}{\ensuremath{-}5.0}
\newcommand{\hlDecFOneSamburnCIHi}{7.3}
\newcommand{\hlDecFOneSamburnTostCILo}{\ensuremath{-}3.6}
\newcommand{\hlDecFOneSamburnTostCIHi}{5.8}
\newcommand{\hlDecFOneSamburnMde}{10.1}
\newcommand{\hlDecFOneSamburnPHolm}{0.637}
\newcommand{\hlDecFOneSamburnN}{5}
\newcommand{\hlDecFOneOneSamburnEst}{\ensuremath{-}3.0}
\newcommand{\hlDecFOneOneSamburnCILo}{\ensuremath{-}8.6}
\newcommand{\hlDecFOneOneSamburnCIHi}{2.5}
\newcommand{\hlDecFOneOneSamburnTostCILo}{\ensuremath{-}7.3}
\newcommand{\hlDecFOneOneSamburnTostCIHi}{1.2}
\newcommand{\hlDecFOneOneSamburnMde}{9.1}
\newcommand{\hlDecFOneOneSamburnPHolm}{0.201}
\newcommand{\hlDecFOneOneSamburnN}{5}
\newcommand{\hlDecTypeRankSamburnOne}{coarse}
\newcommand{\hlDecTypeRankSamburnTwo}{omission}
\newcommand{\hlDecTypeRankSamburnThree}{shift}
\newcommand{\hlDecTypeRankSamburnFour}{boundary}
\newcommand{\hlDecVerdictSamburn}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlDecVerdictNSixSamburn}{Undetermined, MDE 13.0}
\newcommand{\hlDecVerdictFTwoSamburn}{\rn loses less}
\newcommand{\hlDecMeanDropSamburn}{17.0}
\newcommand{\hlDecCleanSamburn}{83.9}
\newcommand{\hlDecInvMtwoFFburnEst}{0.8}
\newcommand{\hlDecInvMtwoFFburnCILo}{\ensuremath{-}1.2}
\newcommand{\hlDecInvMtwoFFburnCIHi}{2.8}
\newcommand{\hlDecInvMtwoFFburnTostCILo}{\ensuremath{-}0.8}
\newcommand{\hlDecInvMtwoFFburnTostCIHi}{2.5}
\newcommand{\hlDecInvMtwoFFburnMde}{3.1}
\newcommand{\hlDecInvMtwoFFburnPHolm}{0.809}
\newcommand{\hlDecInvMtwoFFburnN}{25}
\newcommand{\hlDecInvMtwoFFSATburnEst}{\ensuremath{-}1.6}
\newcommand{\hlDecInvMtwoFFSATburnCILo}{\ensuremath{-}4.4}
\newcommand{\hlDecInvMtwoFFSATburnCIHi}{1.2}
\newcommand{\hlDecInvMtwoFFLVDburnEst}{7.7}
\newcommand{\hlDecInvMtwoFFLVDburnCILo}{3.2}
\newcommand{\hlDecInvMtwoFFLVDburnCIHi}{12.3}
\newcommand{\hlDecInvMtwoFFDOFAburnEst}{0.9}
\newcommand{\hlDecInvMtwoFFDOFAburnCILo}{\ensuremath{-}3.2}
\newcommand{\hlDecInvMtwoFFDOFAburnCIHi}{5.0}
\newcommand{\hlDecInvMtwoFFTMburnEst}{0.8}
\newcommand{\hlDecInvMtwoFFTMburnCILo}{\ensuremath{-}1.9}
\newcommand{\hlDecInvMtwoFFTMburnCIHi}{3.5}
\newcommand{\hlDecInvMtwoFFRNburnEst}{\ensuremath{-}3.8}
\newcommand{\hlDecInvMtwoFFRNburnCILo}{\ensuremath{-}8.0}
\newcommand{\hlDecInvMtwoFFRNburnCIHi}{0.4}
\newcommand{\hlDecNSixMtwoFFburnEst}{\ensuremath{-}5.4}
\newcommand{\hlDecNSixMtwoFFburnCILo}{\ensuremath{-}14.3}
\newcommand{\hlDecNSixMtwoFFburnCIHi}{3.6}
\newcommand{\hlDecNSixMtwoFFburnTostCILo}{\ensuremath{-}12.2}
\newcommand{\hlDecNSixMtwoFFburnTostCIHi}{1.5}
\newcommand{\hlDecNSixMtwoFFburnMde}{14.8}
\newcommand{\hlDecNSixMtwoFFburnPHolm}{0.173}
\newcommand{\hlDecNSixMtwoFFburnN}{5}
\newcommand{\hlDecFTwoMtwoFFburnEst}{4.2}
\newcommand{\hlDecFTwoMtwoFFburnCILo}{1.4}
\newcommand{\hlDecFTwoMtwoFFburnCIHi}{6.9}
\newcommand{\hlDecFTwoMtwoFFburnTostCILo}{2.1}
\newcommand{\hlDecFTwoMtwoFFburnTostCIHi}{6.3}
\newcommand{\hlDecFTwoMtwoFFburnMde}{4.5}
\newcommand{\hlDecFTwoMtwoFFburnPHolm}{0.013}
\newcommand{\hlDecFTwoMtwoFFburnN}{5}
\newcommand{\hlDecFOneMtwoFFburnEst}{\ensuremath{-}5.6}
\newcommand{\hlDecFOneMtwoFFburnCILo}{\ensuremath{-}11.2}
\newcommand{\hlDecFOneMtwoFFburnCIHi}{\ensuremath{-}0.1}
\newcommand{\hlDecFOneMtwoFFburnTostCILo}{\ensuremath{-}9.9}
\newcommand{\hlDecFOneMtwoFFburnTostCIHi}{\ensuremath{-}1.4}
\newcommand{\hlDecFOneMtwoFFburnMde}{9.2}
\newcommand{\hlDecFOneMtwoFFburnPHolm}{0.048}
\newcommand{\hlDecFOneMtwoFFburnN}{5}
\newcommand{\hlDecFOneOneMtwoFFburnEst}{\ensuremath{-}3.9}
\newcommand{\hlDecFOneOneMtwoFFburnCILo}{\ensuremath{-}7.1}
\newcommand{\hlDecFOneOneMtwoFFburnCIHi}{\ensuremath{-}0.8}
\newcommand{\hlDecFOneOneMtwoFFburnTostCILo}{\ensuremath{-}6.3}
\newcommand{\hlDecFOneOneMtwoFFburnTostCIHi}{\ensuremath{-}1.5}
\newcommand{\hlDecFOneOneMtwoFFburnMde}{5.2}
\newcommand{\hlDecFOneOneMtwoFFburnPHolm}{0.025}
\newcommand{\hlDecFOneOneMtwoFFburnN}{5}
\newcommand{\hlDecTypeRankMtwoFFburnOne}{coarse}
\newcommand{\hlDecTypeRankMtwoFFburnTwo}{boundary}
\newcommand{\hlDecTypeRankMtwoFFburnThree}{omission}
\newcommand{\hlDecTypeRankMtwoFFburnFour}{shift}
\newcommand{\hlDecVerdictMtwoFFburn}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlDecVerdictNSixMtwoFFburn}{Undetermined, MDE 14.8}
\newcommand{\hlDecVerdictFTwoMtwoFFburn}{\rn loses less}
\newcommand{\hlDecMeanDropMtwoFFburn}{16.5}
\newcommand{\hlDecCleanMtwoFFburn}{82.3}
\newcommand{\hlDecInvSamPreburnEst}{2.9}
\newcommand{\hlDecInvSamPreburnCILo}{\ensuremath{-}2.2}
\newcommand{\hlDecInvSamPreburnCIHi}{8.0}
\newcommand{\hlDecInvSamPreburnTostCILo}{\ensuremath{-}1.3}
\newcommand{\hlDecInvSamPreburnTostCIHi}{7.2}
\newcommand{\hlDecInvSamPreburnMde}{8.0}
\newcommand{\hlDecInvSamPreburnPHolm}{0.260}
\newcommand{\hlDecInvSamPreburnN}{25}
\newcommand{\hlDecInvSamPreSATburnEst}{\ensuremath{-}6.3}
\newcommand{\hlDecInvSamPreSATburnCILo}{\ensuremath{-}19.6}
\newcommand{\hlDecInvSamPreSATburnCIHi}{7.0}
\newcommand{\hlDecInvSamPreLVDburnEst}{6.3}
\newcommand{\hlDecInvSamPreLVDburnCILo}{\ensuremath{-}9.0}
\newcommand{\hlDecInvSamPreLVDburnCIHi}{21.5}
\newcommand{\hlDecInvSamPreDOFAburnEst}{0.4}
\newcommand{\hlDecInvSamPreDOFAburnCILo}{\ensuremath{-}1.9}
\newcommand{\hlDecInvSamPreDOFAburnCIHi}{2.8}
\newcommand{\hlDecInvSamPreTMburnEst}{1.3}
\newcommand{\hlDecInvSamPreTMburnCILo}{\ensuremath{-}1.9}
\newcommand{\hlDecInvSamPreTMburnCIHi}{4.5}
\newcommand{\hlDecInvSamPreRNburnEst}{12.9}
\newcommand{\hlDecInvSamPreRNburnCILo}{\ensuremath{-}11.6}
\newcommand{\hlDecInvSamPreRNburnCIHi}{37.3}
\newcommand{\hlDecNSixSamPreburnEst}{\ensuremath{-}0.4}
\newcommand{\hlDecNSixSamPreburnCILo}{\ensuremath{-}19.4}
\newcommand{\hlDecNSixSamPreburnCIHi}{18.7}
\newcommand{\hlDecNSixSamPreburnTostCILo}{\ensuremath{-}15.0}
\newcommand{\hlDecNSixSamPreburnTostCIHi}{14.3}
\newcommand{\hlDecNSixSamPreburnMde}{31.5}
\newcommand{\hlDecNSixSamPreburnPHolm}{0.960}
\newcommand{\hlDecNSixSamPreburnN}{5}
\newcommand{\hlDecFTwoSamPreburnEst}{\ensuremath{-}12.5}
\newcommand{\hlDecFTwoSamPreburnCILo}{\ensuremath{-}35.4}
\newcommand{\hlDecFTwoSamPreburnCIHi}{10.5}
\newcommand{\hlDecFTwoSamPreburnTostCILo}{\ensuremath{-}30.1}
\newcommand{\hlDecFTwoSamPreburnTostCIHi}{5.1}
\newcommand{\hlDecFTwoSamPreburnMde}{37.9}
\newcommand{\hlDecFTwoSamPreburnPHolm}{0.206}
\newcommand{\hlDecFTwoSamPreburnN}{5}
\newcommand{\hlDecFOneSamPreburnEst}{\ensuremath{-}8.8}
\newcommand{\hlDecFOneSamPreburnCILo}{\ensuremath{-}36.1}
\newcommand{\hlDecFOneSamPreburnCIHi}{18.5}
\newcommand{\hlDecFOneSamPreburnTostCILo}{\ensuremath{-}29.8}
\newcommand{\hlDecFOneSamPreburnTostCIHi}{12.1}
\newcommand{\hlDecFOneSamPreburnMde}{45.0}
\newcommand{\hlDecFOneSamPreburnPHolm}{0.420}
\newcommand{\hlDecFOneSamPreburnN}{5}
\newcommand{\hlDecFOneOneSamPreburnEst}{\ensuremath{-}16.5}
\newcommand{\hlDecFOneOneSamPreburnCILo}{\ensuremath{-}32.3}
\newcommand{\hlDecFOneOneSamPreburnCIHi}{\ensuremath{-}0.7}
\newcommand{\hlDecFOneOneSamPreburnTostCILo}{\ensuremath{-}28.6}
\newcommand{\hlDecFOneOneSamPreburnTostCIHi}{\ensuremath{-}4.4}
\newcommand{\hlDecFOneOneSamPreburnMde}{26.1}
\newcommand{\hlDecFOneOneSamPreburnPHolm}{0.044}
\newcommand{\hlDecFOneOneSamPreburnN}{5}
\newcommand{\hlDecTypeRankSamPreburnOne}{omission}
\newcommand{\hlDecTypeRankSamPreburnTwo}{coarse}
\newcommand{\hlDecTypeRankSamPreburnThree}{boundary}
\newcommand{\hlDecTypeRankSamPreburnFour}{shift}
\newcommand{\hlDecVerdictSamPreburn}{Undetermined, MDE 8.0}
\newcommand{\hlDecVerdictNSixSamPreburn}{Undetermined, MDE 31.5}
\newcommand{\hlDecVerdictFTwoSamPreburn}{Undetermined, MDE 37.9}
\newcommand{\hlDecMeanDropSamPreburn}{18.6}
\newcommand{\hlDecCleanSamPreburn}{78.1}
\newcommand{\hlMraDropSATOneburn}{17.8}
\newcommand{\hlMraRetSATOneburn}{76.6}
\newcommand{\hlMraCleanSATOneburn}{75.8}
\newcommand{\hlMraDropSATThirdburn}{13.9}
\newcommand{\hlMraRetSATThirdburn}{82.9}
\newcommand{\hlMraCleanSATThirdburn}{81.3}
\newcommand{\hlMraRateDiffSATburnEst}{\ensuremath{-}3.9}
\newcommand{\hlMraRateDiffSATburnCILo}{\ensuremath{-}8.3}
\newcommand{\hlMraRateDiffSATburnCIHi}{0.6}
\newcommand{\hlMraBestRateSATburn}{$\times$1/3}
\newcommand{\hlMraDropLVDOneburn}{19.5}
\newcommand{\hlMraRetLVDOneburn}{75.1}
\newcommand{\hlMraCleanLVDOneburn}{78.3}
\newcommand{\hlMraDropLVDThirdburn}{14.1}
\newcommand{\hlMraRetLVDThirdburn}{82.8}
\newcommand{\hlMraCleanLVDThirdburn}{82.0}
\newcommand{\hlMraRateDiffLVDburnEst}{\ensuremath{-}5.4}
\newcommand{\hlMraRateDiffLVDburnCILo}{\ensuremath{-}8.2}
\newcommand{\hlMraRateDiffLVDburnCIHi}{\ensuremath{-}2.7}
\newcommand{\hlMraBestRateLVDburn}{$\times$1/3}
\newcommand{\hlMraDropDOFAOneburn}{17.9}
\newcommand{\hlMraRetDOFAOneburn}{79.1}
\newcommand{\hlMraCleanDOFAOneburn}{85.5}
\newcommand{\hlMraDropDOFAThirdburn}{17.1}
\newcommand{\hlMraRetDOFAThirdburn}{79.6}
\newcommand{\hlMraCleanDOFAThirdburn}{83.7}
\newcommand{\hlMraRateDiffDOFAburnEst}{\ensuremath{-}0.8}
\newcommand{\hlMraRateDiffDOFAburnCILo}{\ensuremath{-}2.5}
\newcommand{\hlMraRateDiffDOFAburnCIHi}{0.9}
\newcommand{\hlMraBestRateDOFAburn}{$\times$1/3}
\newcommand{\hlMraDropTMOneburn}{12.9}
\newcommand{\hlMraRetTMOneburn}{85.0}
\newcommand{\hlMraCleanTMOneburn}{86.2}
\newcommand{\hlMraDropTMThirdburn}{10.9}
\newcommand{\hlMraRetTMThirdburn}{87.3}
\newcommand{\hlMraCleanTMThirdburn}{85.1}
\newcommand{\hlMraRateDiffTMburnEst}{\ensuremath{-}2.0}
\newcommand{\hlMraRateDiffTMburnCILo}{\ensuremath{-}5.5}
\newcommand{\hlMraRateDiffTMburnCIHi}{1.5}
\newcommand{\hlMraBestRateTMburn}{$\times$1/3}
\newcommand{\hlMraDropRNOneburn}{15.9}
\newcommand{\hlMraRetRNOneburn}{82.0}
\newcommand{\hlMraCleanRNOneburn}{88.1}
\newcommand{\hlMraDropRNThirdburn}{14.1}
\newcommand{\hlMraRetRNThirdburn}{84.0}
\newcommand{\hlMraCleanRNThirdburn}{88.4}
\newcommand{\hlMraRateDiffRNburnEst}{\ensuremath{-}1.7}
\newcommand{\hlMraRateDiffRNburnCILo}{\ensuremath{-}6.9}
\newcommand{\hlMraRateDiffRNburnCIHi}{3.4}
\newcommand{\hlMraBestRateRNburn}{$\times$1/3}
\newcommand{\hlMraFTwoThirdburnEst}{\ensuremath{-}0.2}
\newcommand{\hlMraFTwoThirdburnCILo}{\ensuremath{-}3.4}
\newcommand{\hlMraFTwoThirdburnCIHi}{3.1}
\newcommand{\hlMraFTwoThirdburnTostCILo}{\ensuremath{-}2.7}
\newcommand{\hlMraFTwoThirdburnTostCIHi}{2.4}
\newcommand{\hlMraFTwoThirdburnMde}{5.4}
\newcommand{\hlMraFTwoThirdburnPHolm}{1.000}
\newcommand{\hlMraFTwoThirdburnN}{5}
\newcommand{\hlMraFOneOneburnEst}{\ensuremath{-}1.7}
\newcommand{\hlMraFOneOneburnCILo}{\ensuremath{-}5.2}
\newcommand{\hlMraFOneOneburnCIHi}{1.7}
\newcommand{\hlMraFOneOneburnTostCILo}{\ensuremath{-}4.4}
\newcommand{\hlMraFOneOneburnTostCIHi}{0.9}
\newcommand{\hlMraFOneOneburnMde}{5.7}
\newcommand{\hlMraFOneOneburnPHolm}{0.240}
\newcommand{\hlMraFOneOneburnN}{5}
\newcommand{\hlMraVerdictburn}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlMraVerdictFOneburn}{Undetermined, MDE 5.7}
\newcommand{\hlDecFullVsLiteburnEst}{2.2}
\newcommand{\hlDecFullVsLiteburnCILo}{\ensuremath{-}1.2}
\newcommand{\hlDecFullVsLiteburnCIHi}{5.7}
\newcommand{\hlDecFullVsLiteburnTostCILo}{\ensuremath{-}0.6}
\newcommand{\hlDecFullVsLiteburnTostCIHi}{5.1}
\newcommand{\hlDecFullVsLiteburnMde}{5.5}
\newcommand{\hlDecFullVsLiteburnPHolm}{0.197}
\newcommand{\hlDecFullVsLiteburnN}{25}
\newcommand{\hlDecVerdictFullVsLiteburn}{Undetermined, MDE 5.5}
\newcommand{\hlDecPretrainedVsScratchburnEst}{1.6}
\newcommand{\hlDecPretrainedVsScratchburnCILo}{\ensuremath{-}3.9}
\newcommand{\hlDecPretrainedVsScratchburnCIHi}{7.1}
\newcommand{\hlDecPretrainedVsScratchburnTostCILo}{\ensuremath{-}2.9}
\newcommand{\hlDecPretrainedVsScratchburnTostCIHi}{6.1}
\newcommand{\hlDecPretrainedVsScratchburnMde}{8.6}
\newcommand{\hlDecPretrainedVsScratchburnPHolm}{0.550}
\newcommand{\hlDecPretrainedVsScratchburnN}{25}
\newcommand{\hlDecVerdictPretrainedVsScratchburn}{Undetermined, MDE 8.6}
\newcommand{\hlDecMeanDropUNetflair}{4.8}
\newcommand{\hlDecCleanUNetflair}{47.1}
\newcommand{\hlDecInvflairEst}{\ensuremath{-}0.1}
\newcommand{\hlDecInvflairCILo}{\ensuremath{-}0.7}
\newcommand{\hlDecInvflairCIHi}{0.5}
\newcommand{\hlDecInvflairTostCILo}{\ensuremath{-}0.6}
\newcommand{\hlDecInvflairTostCIHi}{0.4}
\newcommand{\hlDecInvflairMde}{0.9}
\newcommand{\hlDecInvflairPHolm}{0.721}
\newcommand{\hlDecInvflairN}{25}
\newcommand{\hlDecInvSATflairEst}{\ensuremath{-}1.4}
\newcommand{\hlDecInvSATflairCILo}{\ensuremath{-}2.6}
\newcommand{\hlDecInvSATflairCIHi}{\ensuremath{-}0.2}
\newcommand{\hlDecInvLVDflairEst}{0.1}
\newcommand{\hlDecInvLVDflairCILo}{\ensuremath{-}1.3}
\newcommand{\hlDecInvLVDflairCIHi}{1.5}
\newcommand{\hlDecInvDOFAflairEst}{0.3}
\newcommand{\hlDecInvDOFAflairCILo}{\ensuremath{-}1.3}
\newcommand{\hlDecInvDOFAflairCIHi}{1.8}
\newcommand{\hlDecInvTMflairEst}{0.7}
\newcommand{\hlDecInvTMflairCILo}{\ensuremath{-}0.8}
\newcommand{\hlDecInvTMflairCIHi}{2.1}
\newcommand{\hlDecInvRNflairEst}{\ensuremath{-}0.2}
\newcommand{\hlDecInvRNflairCILo}{\ensuremath{-}2.6}
\newcommand{\hlDecInvRNflairCIHi}{2.3}
\newcommand{\hlDecNSixflairEst}{0.5}
\newcommand{\hlDecNSixflairCILo}{\ensuremath{-}1.4}
\newcommand{\hlDecNSixflairCIHi}{2.3}
\newcommand{\hlDecNSixflairTostCILo}{\ensuremath{-}1.0}
\newcommand{\hlDecNSixflairTostCIHi}{1.9}
\newcommand{\hlDecNSixflairMde}{3.1}
\newcommand{\hlDecNSixflairPHolm}{0.521}
\newcommand{\hlDecNSixflairN}{5}
\newcommand{\hlDecFTwoflairEst}{1.2}
\newcommand{\hlDecFTwoflairCILo}{\ensuremath{-}0.2}
\newcommand{\hlDecFTwoflairCIHi}{2.7}
\newcommand{\hlDecFTwoflairTostCILo}{0.1}
\newcommand{\hlDecFTwoflairTostCIHi}{2.3}
\newcommand{\hlDecFTwoflairMde}{2.4}
\newcommand{\hlDecFTwoflairPHolm}{0.082}
\newcommand{\hlDecFTwoflairN}{5}
\newcommand{\hlDecFOneflairEst}{1.4}
\newcommand{\hlDecFOneflairCILo}{0.5}
\newcommand{\hlDecFOneflairCIHi}{2.3}
\newcommand{\hlDecFOneflairTostCILo}{0.7}
\newcommand{\hlDecFOneflairTostCIHi}{2.1}
\newcommand{\hlDecFOneflairMde}{1.5}
\newcommand{\hlDecFOneflairPHolm}{0.012}
\newcommand{\hlDecFOneflairN}{5}
\newcommand{\hlDecFOneOneflairEst}{1.0}
\newcommand{\hlDecFOneOneflairCILo}{0.6}
\newcommand{\hlDecFOneOneflairCIHi}{1.4}
\newcommand{\hlDecFOneOneflairTostCILo}{0.7}
\newcommand{\hlDecFOneOneflairTostCIHi}{1.3}
\newcommand{\hlDecFOneOneflairMde}{0.6}
\newcommand{\hlDecFOneOneflairPHolm}{0.002}
\newcommand{\hlDecFOneOneflairN}{5}
\newcommand{\hlDecTypeRankflairOne}{coarse}
\newcommand{\hlDecTypeRankflairTwo}{boundary}
\newcommand{\hlDecTypeRankflairThree}{omission}
\newcommand{\hlDecTypeRankflairFour}{shift}
\newcommand{\hlDecVerdictflair}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlDecVerdictNSixflair}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlDecVerdictFTwoflair}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlDecInvSegfflairEst}{\ensuremath{-}0.1}
\newcommand{\hlDecInvSegfflairCILo}{\ensuremath{-}0.7}
\newcommand{\hlDecInvSegfflairCIHi}{0.5}
\newcommand{\hlDecInvSegfflairTostCILo}{\ensuremath{-}0.6}
\newcommand{\hlDecInvSegfflairTostCIHi}{0.4}
\newcommand{\hlDecInvSegfflairMde}{0.9}
\newcommand{\hlDecInvSegfflairPHolm}{0.721}
\newcommand{\hlDecInvSegfflairN}{25}
\newcommand{\hlDecInvSegfSATflairEst}{\ensuremath{-}1.4}
\newcommand{\hlDecInvSegfSATflairCILo}{\ensuremath{-}2.6}
\newcommand{\hlDecInvSegfSATflairCIHi}{\ensuremath{-}0.2}
\newcommand{\hlDecInvSegfLVDflairEst}{0.1}
\newcommand{\hlDecInvSegfLVDflairCILo}{\ensuremath{-}1.3}
\newcommand{\hlDecInvSegfLVDflairCIHi}{1.5}
\newcommand{\hlDecInvSegfDOFAflairEst}{0.3}
\newcommand{\hlDecInvSegfDOFAflairCILo}{\ensuremath{-}1.3}
\newcommand{\hlDecInvSegfDOFAflairCIHi}{1.8}
\newcommand{\hlDecInvSegfTMflairEst}{0.7}
\newcommand{\hlDecInvSegfTMflairCILo}{\ensuremath{-}0.8}
\newcommand{\hlDecInvSegfTMflairCIHi}{2.1}
\newcommand{\hlDecInvSegfRNflairEst}{\ensuremath{-}0.2}
\newcommand{\hlDecInvSegfRNflairCILo}{\ensuremath{-}2.6}
\newcommand{\hlDecInvSegfRNflairCIHi}{2.3}
\newcommand{\hlDecNSixSegfflairEst}{0.5}
\newcommand{\hlDecNSixSegfflairCILo}{\ensuremath{-}1.4}
\newcommand{\hlDecNSixSegfflairCIHi}{2.3}
\newcommand{\hlDecNSixSegfflairTostCILo}{\ensuremath{-}1.0}
\newcommand{\hlDecNSixSegfflairTostCIHi}{1.9}
\newcommand{\hlDecNSixSegfflairMde}{3.1}
\newcommand{\hlDecNSixSegfflairPHolm}{0.521}
\newcommand{\hlDecNSixSegfflairN}{5}
\newcommand{\hlDecFTwoSegfflairEst}{1.2}
\newcommand{\hlDecFTwoSegfflairCILo}{\ensuremath{-}0.2}
\newcommand{\hlDecFTwoSegfflairCIHi}{2.7}
\newcommand{\hlDecFTwoSegfflairTostCILo}{0.1}
\newcommand{\hlDecFTwoSegfflairTostCIHi}{2.3}
\newcommand{\hlDecFTwoSegfflairMde}{2.4}
\newcommand{\hlDecFTwoSegfflairPHolm}{0.082}
\newcommand{\hlDecFTwoSegfflairN}{5}
\newcommand{\hlDecFOneSegfflairEst}{1.4}
\newcommand{\hlDecFOneSegfflairCILo}{0.5}
\newcommand{\hlDecFOneSegfflairCIHi}{2.3}
\newcommand{\hlDecFOneSegfflairTostCILo}{0.7}
\newcommand{\hlDecFOneSegfflairTostCIHi}{2.1}
\newcommand{\hlDecFOneSegfflairMde}{1.5}
\newcommand{\hlDecFOneSegfflairPHolm}{0.012}
\newcommand{\hlDecFOneSegfflairN}{5}
\newcommand{\hlDecFOneOneSegfflairEst}{1.0}
\newcommand{\hlDecFOneOneSegfflairCILo}{0.6}
\newcommand{\hlDecFOneOneSegfflairCIHi}{1.4}
\newcommand{\hlDecFOneOneSegfflairTostCILo}{0.7}
\newcommand{\hlDecFOneOneSegfflairTostCIHi}{1.3}
\newcommand{\hlDecFOneOneSegfflairMde}{0.6}
\newcommand{\hlDecFOneOneSegfflairPHolm}{0.002}
\newcommand{\hlDecFOneOneSegfflairN}{5}
\newcommand{\hlDecTypeRankSegfflairOne}{coarse}
\newcommand{\hlDecTypeRankSegfflairTwo}{boundary}
\newcommand{\hlDecTypeRankSegfflairThree}{omission}
\newcommand{\hlDecTypeRankSegfflairFour}{shift}
\newcommand{\hlDecVerdictSegfflair}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlDecVerdictNSixSegfflair}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlDecVerdictFTwoSegfflair}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlDecMeanDropSegfflair}{4.7}
\newcommand{\hlDecCleanSegfflair}{47.2}
\newcommand{\hlDecInvMtwoFflairEst}{0.8}
\newcommand{\hlDecInvMtwoFflairCILo}{0.2}
\newcommand{\hlDecInvMtwoFflairCIHi}{1.5}
\newcommand{\hlDecInvMtwoFflairTostCILo}{0.3}
\newcommand{\hlDecInvMtwoFflairTostCIHi}{1.4}
\newcommand{\hlDecInvMtwoFflairMde}{1.0}
\newcommand{\hlDecInvMtwoFflairPHolm}{0.020}
\newcommand{\hlDecInvMtwoFflairN}{25}
\newcommand{\hlDecInvMtwoFSATflairEst}{\ensuremath{-}0.2}
\newcommand{\hlDecInvMtwoFSATflairCILo}{\ensuremath{-}1.5}
\newcommand{\hlDecInvMtwoFSATflairCIHi}{1.2}
\newcommand{\hlDecInvMtwoFLVDflairEst}{2.0}
\newcommand{\hlDecInvMtwoFLVDflairCILo}{0.5}
\newcommand{\hlDecInvMtwoFLVDflairCIHi}{3.6}
\newcommand{\hlDecInvMtwoFDOFAflairEst}{1.4}
\newcommand{\hlDecInvMtwoFDOFAflairCILo}{\ensuremath{-}0.5}
\newcommand{\hlDecInvMtwoFDOFAflairCIHi}{3.3}
\newcommand{\hlDecInvMtwoFTMflairEst}{0.4}
\newcommand{\hlDecInvMtwoFTMflairCILo}{\ensuremath{-}0.9}
\newcommand{\hlDecInvMtwoFTMflairCIHi}{1.7}
\newcommand{\hlDecInvMtwoFRNflairEst}{0.5}
\newcommand{\hlDecInvMtwoFRNflairCILo}{\ensuremath{-}1.9}
\newcommand{\hlDecInvMtwoFRNflairCIHi}{2.8}
\newcommand{\hlDecNSixMtwoFflairEst}{\ensuremath{-}0.2}
\newcommand{\hlDecNSixMtwoFflairCILo}{\ensuremath{-}1.1}
\newcommand{\hlDecNSixMtwoFflairCIHi}{0.6}
\newcommand{\hlDecNSixMtwoFflairTostCILo}{\ensuremath{-}0.9}
\newcommand{\hlDecNSixMtwoFflairTostCIHi}{0.4}
\newcommand{\hlDecNSixMtwoFflairMde}{1.4}
\newcommand{\hlDecNSixMtwoFflairPHolm}{0.463}
\newcommand{\hlDecNSixMtwoFflairN}{5}
\newcommand{\hlDecFTwoMtwoFflairEst}{1.0}
\newcommand{\hlDecFTwoMtwoFflairCILo}{\ensuremath{-}2.3}
\newcommand{\hlDecFTwoMtwoFflairCIHi}{4.4}
\newcommand{\hlDecFTwoMtwoFflairTostCILo}{\ensuremath{-}1.6}
\newcommand{\hlDecFTwoMtwoFflairTostCIHi}{3.6}
\newcommand{\hlDecFTwoMtwoFflairMde}{5.6}
\newcommand{\hlDecFTwoMtwoFflairPHolm}{0.442}
\newcommand{\hlDecFTwoMtwoFflairN}{5}
\newcommand{\hlDecFOneMtwoFflairEst}{0.7}
\newcommand{\hlDecFOneMtwoFflairCILo}{\ensuremath{-}0.5}
\newcommand{\hlDecFOneMtwoFflairCIHi}{2.0}
\newcommand{\hlDecFOneMtwoFflairTostCILo}{\ensuremath{-}0.2}
\newcommand{\hlDecFOneMtwoFflairTostCIHi}{1.7}
\newcommand{\hlDecFOneMtwoFflairMde}{2.0}
\newcommand{\hlDecFOneMtwoFflairPHolm}{0.180}
\newcommand{\hlDecFOneMtwoFflairN}{5}
\newcommand{\hlDecFOneOneMtwoFflairEst}{0.8}
\newcommand{\hlDecFOneOneMtwoFflairCILo}{\ensuremath{-}0.5}
\newcommand{\hlDecFOneOneMtwoFflairCIHi}{2.2}
\newcommand{\hlDecFOneOneMtwoFflairTostCILo}{\ensuremath{-}0.2}
\newcommand{\hlDecFOneOneMtwoFflairTostCIHi}{1.9}
\newcommand{\hlDecFOneOneMtwoFflairMde}{2.3}
\newcommand{\hlDecFOneOneMtwoFflairPHolm}{0.161}
\newcommand{\hlDecFOneOneMtwoFflairN}{5}
\newcommand{\hlDecTypeRankMtwoFflairOne}{coarse}
\newcommand{\hlDecTypeRankMtwoFflairTwo}{boundary}
\newcommand{\hlDecTypeRankMtwoFflairThree}{omission}
\newcommand{\hlDecTypeRankMtwoFflairFour}{shift}
\newcommand{\hlDecVerdictMtwoFflair}{Equivalent within $\pm$\TostMargin, Mask2Former head loses more}
\newcommand{\hlDecVerdictNSixMtwoFflair}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlDecVerdictFTwoMtwoFflair}{Undetermined, MDE 5.6}
\newcommand{\hlDecMeanDropMtwoFflair}{5.6}
\newcommand{\hlDecCleanMtwoFflair}{46.9}
\newcommand{\hlDecInvSamflairEst}{0.0}
\newcommand{\hlDecInvSamflairCILo}{\ensuremath{-}0.6}
\newcommand{\hlDecInvSamflairCIHi}{0.6}
\newcommand{\hlDecInvSamflairTostCILo}{\ensuremath{-}0.5}
\newcommand{\hlDecInvSamflairTostCIHi}{0.5}
\newcommand{\hlDecInvSamflairMde}{1.0}
\newcommand{\hlDecInvSamflairPHolm}{0.996}
\newcommand{\hlDecInvSamflairN}{25}
\newcommand{\hlDecInvSamSATflairEst}{\ensuremath{-}1.0}
\newcommand{\hlDecInvSamSATflairCILo}{\ensuremath{-}2.4}
\newcommand{\hlDecInvSamSATflairCIHi}{0.5}
\newcommand{\hlDecInvSamLVDflairEst}{0.8}
\newcommand{\hlDecInvSamLVDflairCILo}{\ensuremath{-}1.2}
\newcommand{\hlDecInvSamLVDflairCIHi}{2.8}
\newcommand{\hlDecInvSamDOFAflairEst}{0.8}
\newcommand{\hlDecInvSamDOFAflairCILo}{\ensuremath{-}0.1}
\newcommand{\hlDecInvSamDOFAflairCIHi}{1.7}
\newcommand{\hlDecInvSamTMflairEst}{\ensuremath{-}0.1}
\newcommand{\hlDecInvSamTMflairCILo}{\ensuremath{-}2.5}
\newcommand{\hlDecInvSamTMflairCIHi}{2.3}
\newcommand{\hlDecInvSamRNflairEst}{\ensuremath{-}0.5}
\newcommand{\hlDecInvSamRNflairCILo}{\ensuremath{-}2.5}
\newcommand{\hlDecInvSamRNflairCIHi}{1.4}
\newcommand{\hlDecNSixSamflairEst}{0.4}
\newcommand{\hlDecNSixSamflairCILo}{\ensuremath{-}1.1}
\newcommand{\hlDecNSixSamflairCIHi}{1.9}
\newcommand{\hlDecNSixSamflairTostCILo}{\ensuremath{-}0.8}
\newcommand{\hlDecNSixSamflairTostCIHi}{1.6}
\newcommand{\hlDecNSixSamflairMde}{2.5}
\newcommand{\hlDecNSixSamflairPHolm}{0.521}
\newcommand{\hlDecNSixSamflairN}{5}
\newcommand{\hlDecFTwoSamflairEst}{1.4}
\newcommand{\hlDecFTwoSamflairCILo}{\ensuremath{-}0.5}
\newcommand{\hlDecFTwoSamflairCIHi}{3.3}
\newcommand{\hlDecFTwoSamflairTostCILo}{0.0}
\newcommand{\hlDecFTwoSamflairTostCIHi}{2.9}
\newcommand{\hlDecFTwoSamflairMde}{3.1}
\newcommand{\hlDecFTwoSamflairPHolm}{0.103}
\newcommand{\hlDecFTwoSamflairN}{5}
\newcommand{\hlDecFOneSamflairEst}{1.1}
\newcommand{\hlDecFOneSamflairCILo}{\ensuremath{-}1.1}
\newcommand{\hlDecFOneSamflairCIHi}{3.4}
\newcommand{\hlDecFOneSamflairTostCILo}{\ensuremath{-}0.6}
\newcommand{\hlDecFOneSamflairTostCIHi}{2.9}
\newcommand{\hlDecFOneSamflairMde}{3.8}
\newcommand{\hlDecFOneSamflairPHolm}{0.236}
\newcommand{\hlDecFOneSamflairN}{5}
\newcommand{\hlDecFOneOneSamflairEst}{0.9}
\newcommand{\hlDecFOneOneSamflairCILo}{\ensuremath{-}0.5}
\newcommand{\hlDecFOneOneSamflairCIHi}{2.3}
\newcommand{\hlDecFOneOneSamflairTostCILo}{\ensuremath{-}0.2}
\newcommand{\hlDecFOneOneSamflairTostCIHi}{1.9}
\newcommand{\hlDecFOneOneSamflairMde}{2.3}
\newcommand{\hlDecFOneOneSamflairPHolm}{0.161}
\newcommand{\hlDecFOneOneSamflairN}{5}
\newcommand{\hlDecTypeRankSamflairOne}{coarse}
\newcommand{\hlDecTypeRankSamflairTwo}{boundary}
\newcommand{\hlDecTypeRankSamflairThree}{omission}
\newcommand{\hlDecTypeRankSamflairFour}{shift}
\newcommand{\hlDecVerdictSamflair}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlDecVerdictNSixSamflair}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlDecVerdictFTwoSamflair}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlDecMeanDropSamflair}{4.8}
\newcommand{\hlDecCleanSamflair}{44.8}
\newcommand{\hlDecInvMtwoFFflairEst}{0.2}
\newcommand{\hlDecInvMtwoFFflairCILo}{\ensuremath{-}0.5}
\newcommand{\hlDecInvMtwoFFflairCIHi}{0.9}
\newcommand{\hlDecInvMtwoFFflairTostCILo}{\ensuremath{-}0.3}
\newcommand{\hlDecInvMtwoFFflairTostCIHi}{0.8}
\newcommand{\hlDecInvMtwoFFflairMde}{1.1}
\newcommand{\hlDecInvMtwoFFflairPHolm}{0.809}
\newcommand{\hlDecInvMtwoFFflairN}{25}
\newcommand{\hlDecInvMtwoFFSATflairEst}{\ensuremath{-}1.6}
\newcommand{\hlDecInvMtwoFFSATflairCILo}{\ensuremath{-}3.3}
\newcommand{\hlDecInvMtwoFFSATflairCIHi}{0.0}
\newcommand{\hlDecInvMtwoFFLVDflairEst}{0.8}
\newcommand{\hlDecInvMtwoFFLVDflairCILo}{\ensuremath{-}0.7}
\newcommand{\hlDecInvMtwoFFLVDflairCIHi}{2.4}
\newcommand{\hlDecInvMtwoFFDOFAflairEst}{0.1}
\newcommand{\hlDecInvMtwoFFDOFAflairCILo}{\ensuremath{-}0.5}
\newcommand{\hlDecInvMtwoFFDOFAflairCIHi}{0.8}
\newcommand{\hlDecInvMtwoFFTMflairEst}{0.3}
\newcommand{\hlDecInvMtwoFFTMflairCILo}{\ensuremath{-}1.9}
\newcommand{\hlDecInvMtwoFFTMflairCIHi}{2.5}
\newcommand{\hlDecInvMtwoFFRNflairEst}{1.5}
\newcommand{\hlDecInvMtwoFFRNflairCILo}{\ensuremath{-}0.4}
\newcommand{\hlDecInvMtwoFFRNflairCIHi}{3.4}
\newcommand{\hlDecNSixMtwoFFflairEst}{0.7}
\newcommand{\hlDecNSixMtwoFFflairCILo}{\ensuremath{-}0.7}
\newcommand{\hlDecNSixMtwoFFflairCIHi}{2.0}
\newcommand{\hlDecNSixMtwoFFflairTostCILo}{\ensuremath{-}0.3}
\newcommand{\hlDecNSixMtwoFFflairTostCIHi}{1.7}
\newcommand{\hlDecNSixMtwoFFflairMde}{2.2}
\newcommand{\hlDecNSixMtwoFFflairPHolm}{0.227}
\newcommand{\hlDecNSixMtwoFFflairN}{5}
\newcommand{\hlDecFTwoMtwoFFflairEst}{\ensuremath{-}0.7}
\newcommand{\hlDecFTwoMtwoFFflairCILo}{\ensuremath{-}2.0}
\newcommand{\hlDecFTwoMtwoFFflairCIHi}{0.7}
\newcommand{\hlDecFTwoMtwoFFflairTostCILo}{\ensuremath{-}1.7}
\newcommand{\hlDecFTwoMtwoFFflairTostCIHi}{0.3}
\newcommand{\hlDecFTwoMtwoFFflairMde}{2.2}
\newcommand{\hlDecFTwoMtwoFFflairPHolm}{0.234}
\newcommand{\hlDecFTwoMtwoFFflairN}{5}
\newcommand{\hlDecFOneMtwoFFflairEst}{0.5}
\newcommand{\hlDecFOneMtwoFFflairCILo}{\ensuremath{-}0.8}
\newcommand{\hlDecFOneMtwoFFflairCIHi}{1.7}
\newcommand{\hlDecFOneMtwoFFflairTostCILo}{\ensuremath{-}0.5}
\newcommand{\hlDecFOneMtwoFFflairTostCIHi}{1.4}
\newcommand{\hlDecFOneMtwoFFflairMde}{2.0}
\newcommand{\hlDecFOneMtwoFFflairPHolm}{0.364}
\newcommand{\hlDecFOneMtwoFFflairN}{5}
\newcommand{\hlDecFOneOneMtwoFFflairEst}{0.9}
\newcommand{\hlDecFOneOneMtwoFFflairCILo}{\ensuremath{-}0.4}
\newcommand{\hlDecFOneOneMtwoFFflairCIHi}{2.2}
\newcommand{\hlDecFOneOneMtwoFFflairTostCILo}{\ensuremath{-}0.1}
\newcommand{\hlDecFOneOneMtwoFFflairTostCIHi}{1.9}
\newcommand{\hlDecFOneOneMtwoFFflairMde}{2.2}
\newcommand{\hlDecFOneOneMtwoFFflairPHolm}{0.133}
\newcommand{\hlDecFOneOneMtwoFFflairN}{5}
\newcommand{\hlDecTypeRankMtwoFFflairOne}{coarse}
\newcommand{\hlDecTypeRankMtwoFFflairTwo}{shift}
\newcommand{\hlDecTypeRankMtwoFFflairThree}{boundary}
\newcommand{\hlDecTypeRankMtwoFFflairFour}{omission}
\newcommand{\hlDecVerdictMtwoFFflair}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlDecVerdictNSixMtwoFFflair}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlDecVerdictFTwoMtwoFFflair}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlDecMeanDropMtwoFFflair}{5.0}
\newcommand{\hlDecCleanMtwoFFflair}{46.5}
\newcommand{\hlDecInvSamPreflairEst}{0.5}
\newcommand{\hlDecInvSamPreflairCILo}{\ensuremath{-}0.2}
\newcommand{\hlDecInvSamPreflairCIHi}{1.2}
\newcommand{\hlDecInvSamPreflairTostCILo}{0.0}
\newcommand{\hlDecInvSamPreflairTostCIHi}{1.1}
\newcommand{\hlDecInvSamPreflairMde}{1.1}
\newcommand{\hlDecInvSamPreflairPHolm}{0.260}
\newcommand{\hlDecInvSamPreflairN}{25}
\newcommand{\hlDecInvSamPreSATflairEst}{\ensuremath{-}1.3}
\newcommand{\hlDecInvSamPreSATflairCILo}{\ensuremath{-}2.4}
\newcommand{\hlDecInvSamPreSATflairCIHi}{\ensuremath{-}0.1}
\newcommand{\hlDecInvSamPreLVDflairEst}{1.6}
\newcommand{\hlDecInvSamPreLVDflairCILo}{0.5}
\newcommand{\hlDecInvSamPreLVDflairCIHi}{2.8}
\newcommand{\hlDecInvSamPreDOFAflairEst}{1.1}
\newcommand{\hlDecInvSamPreDOFAflairCILo}{\ensuremath{-}0.4}
\newcommand{\hlDecInvSamPreDOFAflairCIHi}{2.6}
\newcommand{\hlDecInvSamPreTMflairEst}{1.2}
\newcommand{\hlDecInvSamPreTMflairCILo}{\ensuremath{-}1.6}
\newcommand{\hlDecInvSamPreTMflairCIHi}{3.9}
\newcommand{\hlDecInvSamPreRNflairEst}{0.0}
\newcommand{\hlDecInvSamPreRNflairCILo}{\ensuremath{-}1.9}
\newcommand{\hlDecInvSamPreRNflairCIHi}{2.0}
\newcommand{\hlDecNSixSamPreflairEst}{\ensuremath{-}0.5}
\newcommand{\hlDecNSixSamPreflairCILo}{\ensuremath{-}1.6}
\newcommand{\hlDecNSixSamPreflairCIHi}{0.5}
\newcommand{\hlDecNSixSamPreflairTostCILo}{\ensuremath{-}1.3}
\newcommand{\hlDecNSixSamPreflairTostCIHi}{0.3}
\newcommand{\hlDecNSixSamPreflairMde}{1.7}
\newcommand{\hlDecNSixSamPreflairPHolm}{0.245}
\newcommand{\hlDecNSixSamPreflairN}{5}
\newcommand{\hlDecFTwoSamPreflairEst}{1.7}
\newcommand{\hlDecFTwoSamPreflairCILo}{0.7}
\newcommand{\hlDecFTwoSamPreflairCIHi}{2.6}
\newcommand{\hlDecFTwoSamPreflairTostCILo}{1.0}
\newcommand{\hlDecFTwoSamPreflairTostCIHi}{2.4}
\newcommand{\hlDecFTwoSamPreflairMde}{1.5}
\newcommand{\hlDecFTwoSamPreflairPHolm}{0.007}
\newcommand{\hlDecFTwoSamPreflairN}{5}
\newcommand{\hlDecFOneSamPreflairEst}{0.0}
\newcommand{\hlDecFOneSamPreflairCILo}{\ensuremath{-}1.8}
\newcommand{\hlDecFOneSamPreflairCIHi}{1.9}
\newcommand{\hlDecFOneSamPreflairTostCILo}{\ensuremath{-}1.4}
\newcommand{\hlDecFOneSamPreflairTostCIHi}{1.5}
\newcommand{\hlDecFOneSamPreflairMde}{3.1}
\newcommand{\hlDecFOneSamPreflairPHolm}{0.955}
\newcommand{\hlDecFOneSamPreflairN}{5}
\newcommand{\hlDecFOneOneSamPreflairEst}{0.7}
\newcommand{\hlDecFOneOneSamPreflairCILo}{\ensuremath{-}0.8}
\newcommand{\hlDecFOneOneSamPreflairCIHi}{2.2}
\newcommand{\hlDecFOneOneSamPreflairTostCILo}{\ensuremath{-}0.5}
\newcommand{\hlDecFOneOneSamPreflairTostCIHi}{1.8}
\newcommand{\hlDecFOneOneSamPreflairMde}{2.5}
\newcommand{\hlDecFOneOneSamPreflairPHolm}{0.279}
\newcommand{\hlDecFOneOneSamPreflairN}{5}
\newcommand{\hlDecTypeRankSamPreflairOne}{coarse}
\newcommand{\hlDecTypeRankSamPreflairTwo}{boundary}
\newcommand{\hlDecTypeRankSamPreflairThree}{omission}
\newcommand{\hlDecTypeRankSamPreflairFour}{shift}
\newcommand{\hlDecVerdictSamPreflair}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlDecVerdictNSixSamPreflair}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlDecVerdictFTwoSamPreflair}{Equivalent within $\pm$\TostMargin, \rn loses less}
\newcommand{\hlDecMeanDropSamPreflair}{5.3}
\newcommand{\hlDecCleanSamPreflair}{42.9}
\newcommand{\hlMraDropSATOneflair}{6.5}
\newcommand{\hlMraRetSATOneflair}{87.5}
\newcommand{\hlMraCleanSATOneflair}{52.2}
\newcommand{\hlMraDropSATThirdflair}{5.1}
\newcommand{\hlMraRetSATThirdflair}{89.9}
\newcommand{\hlMraCleanSATThirdflair}{50.5}
\newcommand{\hlMraRateDiffSATflairEst}{\ensuremath{-}1.4}
\newcommand{\hlMraRateDiffSATflairCILo}{\ensuremath{-}2.6}
\newcommand{\hlMraRateDiffSATflairCIHi}{\ensuremath{-}0.2}
\newcommand{\hlMraBestRateSATflair}{$\times$1/3}
\newcommand{\hlMraDropLVDOneflair}{4.0}
\newcommand{\hlMraRetLVDOneflair}{92.2}
\newcommand{\hlMraCleanLVDOneflair}{51.2}
\newcommand{\hlMraDropLVDThirdflair}{3.6}
\newcommand{\hlMraRetLVDThirdflair}{93.0}
\newcommand{\hlMraCleanLVDThirdflair}{50.8}
\newcommand{\hlMraRateDiffLVDflairEst}{\ensuremath{-}0.4}
\newcommand{\hlMraRateDiffLVDflairCILo}{\ensuremath{-}1.9}
\newcommand{\hlMraRateDiffLVDflairCIHi}{1.2}
\newcommand{\hlMraBestRateLVDflair}{$\times$1/3}
\newcommand{\hlMraDropDOFAOneflair}{4.3}
\newcommand{\hlMraRetDOFAOneflair}{90.9}
\newcommand{\hlMraCleanDOFAOneflair}{47.5}
\newcommand{\hlMraDropDOFAThirdflair}{3.9}
\newcommand{\hlMraRetDOFAThirdflair}{91.7}
\newcommand{\hlMraCleanDOFAThirdflair}{46.7}
\newcommand{\hlMraRateDiffDOFAflairEst}{\ensuremath{-}0.4}
\newcommand{\hlMraRateDiffDOFAflairCILo}{\ensuremath{-}1.3}
\newcommand{\hlMraRateDiffDOFAflairCIHi}{0.4}
\newcommand{\hlMraBestRateDOFAflair}{$\times$1/3}
\newcommand{\hlMraDropTMOneflair}{5.2}
\newcommand{\hlMraRetTMOneflair}{87.1}
\newcommand{\hlMraCleanTMOneflair}{40.5}
\newcommand{\hlMraDropTMThirdflair}{4.2}
\newcommand{\hlMraRetTMThirdflair}{89.0}
\newcommand{\hlMraCleanTMThirdflair}{38.2}
\newcommand{\hlMraRateDiffTMflairEst}{\ensuremath{-}1.0}
\newcommand{\hlMraRateDiffTMflairCILo}{\ensuremath{-}3.3}
\newcommand{\hlMraRateDiffTMflairCIHi}{1.3}
\newcommand{\hlMraBestRateTMflair}{$\times$1/3}
\newcommand{\hlMraDropRNOneflair}{4.2}
\newcommand{\hlMraRetRNOneflair}{90.6}
\newcommand{\hlMraCleanRNOneflair}{44.5}
\newcommand{\hlMraDropRNThirdflair}{3.8}
\newcommand{\hlMraRetRNThirdflair}{91.4}
\newcommand{\hlMraCleanRNThirdflair}{44.2}
\newcommand{\hlMraRateDiffRNflairEst}{\ensuremath{-}0.4}
\newcommand{\hlMraRateDiffRNflairCILo}{\ensuremath{-}2.0}
\newcommand{\hlMraRateDiffRNflairCIHi}{1.3}
\newcommand{\hlMraBestRateRNflair}{$\times$1/3}
\newcommand{\hlMraFTwoThirdflairEst}{0.2}
\newcommand{\hlMraFTwoThirdflairCILo}{\ensuremath{-}1.3}
\newcommand{\hlMraFTwoThirdflairCIHi}{1.8}
\newcommand{\hlMraFTwoThirdflairTostCILo}{\ensuremath{-}1.0}
\newcommand{\hlMraFTwoThirdflairTostCIHi}{1.4}
\newcommand{\hlMraFTwoThirdflairMde}{2.5}
\newcommand{\hlMraFTwoThirdflairPHolm}{1.000}
\newcommand{\hlMraFTwoThirdflairN}{5}
\newcommand{\hlMraFOneOneflairEst}{2.5}
\newcommand{\hlMraFOneOneflairCILo}{1.1}
\newcommand{\hlMraFOneOneflairCIHi}{4.0}
\newcommand{\hlMraFOneOneflairTostCILo}{1.4}
\newcommand{\hlMraFOneOneflairTostCIHi}{3.6}
\newcommand{\hlMraFOneOneflairMde}{2.4}
\newcommand{\hlMraFOneOneflairPHolm}{0.016}
\newcommand{\hlMraFOneOneflairN}{5}
\newcommand{\hlMraVerdictflair}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlMraVerdictFOneflair}{\lvd loses less}
\newcommand{\hlDecFullVsLiteflairEst}{\ensuremath{-}0.6}
\newcommand{\hlDecFullVsLiteflairCILo}{\ensuremath{-}1.3}
\newcommand{\hlDecFullVsLiteflairCIHi}{0.1}
\newcommand{\hlDecFullVsLiteflairTostCILo}{\ensuremath{-}1.2}
\newcommand{\hlDecFullVsLiteflairTostCIHi}{\ensuremath{-}0.1}
\newcommand{\hlDecFullVsLiteflairMde}{1.1}
\newcommand{\hlDecFullVsLiteflairPHolm}{0.148}
\newcommand{\hlDecFullVsLiteflairN}{25}
\newcommand{\hlDecVerdictFullVsLiteflair}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlDecPretrainedVsScratchflairEst}{0.5}
\newcommand{\hlDecPretrainedVsScratchflairCILo}{0.0}
\newcommand{\hlDecPretrainedVsScratchflairCIHi}{1.1}
\newcommand{\hlDecPretrainedVsScratchflairTostCILo}{0.1}
\newcommand{\hlDecPretrainedVsScratchflairTostCIHi}{1.0}
\newcommand{\hlDecPretrainedVsScratchflairMde}{0.8}
\newcommand{\hlDecPretrainedVsScratchflairPHolm}{0.103}
\newcommand{\hlDecPretrainedVsScratchflairN}{25}
\newcommand{\hlDecVerdictPretrainedVsScratchflair}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlLrRefDropSATburnLOne}{3.8}
\newcommand{\hlLrRefDropSATburnLTwo}{17.8}
\newcommand{\hlLrRefDropLVDburnLOne}{3.8}
\newcommand{\hlLrRefDropLVDburnLTwo}{14.1}
\newcommand{\hlLrRefDropDOFAburnLOne}{4.1}
\newcommand{\hlLrRefDropDOFAburnLTwo}{17.9}
\newcommand{\hlLrRefDropTMburnLOne}{3.7}
\newcommand{\hlLrRefDropTMburnLTwo}{12.9}
\newcommand{\hlLrRefDropRNburnLOne}{3.2}
\newcommand{\hlLrRefDropRNburnLTwo}{15.9}
\newcommand{\hlLrRefDropburnLOne}{3.7}
\newcommand{\hlLrRefDropburnLTwo}{15.7}
\newcommand{\hlLrRefDropSATflairLOne}{2.1}
\newcommand{\hlLrRefDropSATflairLTwo}{6.5}
\newcommand{\hlLrRefDropLVDflairLOne}{0.8}
\newcommand{\hlLrRefDropLVDflairLTwo}{3.6}
\newcommand{\hlLrRefDropDOFAflairLOne}{1.0}
\newcommand{\hlLrRefDropDOFAflairLTwo}{4.3}
\newcommand{\hlLrRefDropTMflairLOne}{1.6}
\newcommand{\hlLrRefDropTMflairLTwo}{5.2}
\newcommand{\hlLrRefDropRNflairLOne}{0.9}
\newcommand{\hlLrRefDropRNflairLTwo}{4.2}
\newcommand{\hlLrRefDropflairLOne}{1.3}
\newcommand{\hlLrRefDropflairLTwo}{4.8}
\newcommand{\hlLrDropSATburnShift}{20.1}
\newcommand{\hlLrDropSATburnShiftCILo}{11.4}
\newcommand{\hlLrDropSATburnShiftCIHi}{28.8}
\newcommand{\hlLrDropSATburnCoarse}{23.7}
\newcommand{\hlLrDropSATburnCoarseCILo}{14.8}
\newcommand{\hlLrDropSATburnCoarseCIHi}{32.6}
\newcommand{\hlLrDropSATburnBoundary}{18.6}
\newcommand{\hlLrDropSATburnBoundaryCILo}{14.0}
\newcommand{\hlLrDropSATburnBoundaryCIHi}{23.3}
\newcommand{\hlLrDropSATburnOmission}{26.3}
\newcommand{\hlLrDropSATburnOmissionCILo}{19.9}
\newcommand{\hlLrDropSATburnOmissionCIHi}{32.8}
\newcommand{\hlLrMeanDropSATburn}{22.2}
\newcommand{\hlLrDropLVDburnShift}{16.1}
\newcommand{\hlLrDropLVDburnShiftCILo}{14.6}
\newcommand{\hlLrDropLVDburnShiftCIHi}{17.7}
\newcommand{\hlLrDropLVDburnCoarse}{19.7}
\newcommand{\hlLrDropLVDburnCoarseCILo}{17.1}
\newcommand{\hlLrDropLVDburnCoarseCIHi}{22.3}
\newcommand{\hlLrDropLVDburnBoundary}{18.7}
\newcommand{\hlLrDropLVDburnBoundaryCILo}{14.5}
\newcommand{\hlLrDropLVDburnBoundaryCIHi}{22.9}
\newcommand{\hlLrDropLVDburnOmission}{30.6}
\newcommand{\hlLrDropLVDburnOmissionCILo}{22.6}
\newcommand{\hlLrDropLVDburnOmissionCIHi}{38.7}
\newcommand{\hlLrMeanDropLVDburn}{21.3}
\newcommand{\hlLrDropDOFAburnShift}{20.4}
\newcommand{\hlLrDropDOFAburnShiftCILo}{14.6}
\newcommand{\hlLrDropDOFAburnShiftCIHi}{26.1}
\newcommand{\hlLrDropDOFAburnCoarse}{24.2}
\newcommand{\hlLrDropDOFAburnCoarseCILo}{21.4}
\newcommand{\hlLrDropDOFAburnCoarseCIHi}{27.0}
\newcommand{\hlLrDropDOFAburnBoundary}{20.5}
\newcommand{\hlLrDropDOFAburnBoundaryCILo}{15.8}
\newcommand{\hlLrDropDOFAburnBoundaryCIHi}{25.2}
\newcommand{\hlLrDropDOFAburnOmission}{31.1}
\newcommand{\hlLrDropDOFAburnOmissionCILo}{27.9}
\newcommand{\hlLrDropDOFAburnOmissionCIHi}{34.3}
\newcommand{\hlLrMeanDropDOFAburn}{24.0}
\newcommand{\hlLrDropTMburnShift}{17.6}
\newcommand{\hlLrDropTMburnShiftCILo}{14.2}
\newcommand{\hlLrDropTMburnShiftCIHi}{20.9}
\newcommand{\hlLrDropTMburnCoarse}{22.4}
\newcommand{\hlLrDropTMburnCoarseCILo}{17.4}
\newcommand{\hlLrDropTMburnCoarseCIHi}{27.4}
\newcommand{\hlLrDropTMburnBoundary}{19.5}
\newcommand{\hlLrDropTMburnBoundaryCILo}{15.3}
\newcommand{\hlLrDropTMburnBoundaryCIHi}{23.6}
\newcommand{\hlLrDropTMburnOmission}{27.1}
\newcommand{\hlLrDropTMburnOmissionCILo}{16.6}
\newcommand{\hlLrDropTMburnOmissionCIHi}{37.6}
\newcommand{\hlLrMeanDropTMburn}{21.6}
\newcommand{\hlLrDropRNburnShift}{18.5}
\newcommand{\hlLrDropRNburnShiftCILo}{14.0}
\newcommand{\hlLrDropRNburnShiftCIHi}{22.9}
\newcommand{\hlLrDropRNburnCoarse}{21.3}
\newcommand{\hlLrDropRNburnCoarseCILo}{19.3}
\newcommand{\hlLrDropRNburnCoarseCIHi}{23.3}
\newcommand{\hlLrDropRNburnBoundary}{18.6}
\newcommand{\hlLrDropRNburnBoundaryCILo}{14.1}
\newcommand{\hlLrDropRNburnBoundaryCIHi}{23.2}
\newcommand{\hlLrDropRNburnOmission}{31.3}
\newcommand{\hlLrDropRNburnOmissionCILo}{23.1}
\newcommand{\hlLrDropRNburnOmissionCIHi}{39.5}
\newcommand{\hlLrMeanDropRNburn}{22.4}
\newcommand{\hlLrMeanDropburn}{22.3}
\newcommand{\hlLrTypeRankburnOne}{omission}
\newcommand{\hlLrTypeRankburnTwo}{coarse}
\newcommand{\hlLrTypeRankburnThree}{boundary}
\newcommand{\hlLrTypeRankburnFour}{shift}
\newcommand{\hlLrRankSameburn}{no}
\newcommand{\hlLrRankVerdictburn}{Ranking differs from \Ltwo}
\newcommand{\hlLrNSixburnEst}{\ensuremath{-}0.9}
\newcommand{\hlLrNSixburnCILo}{\ensuremath{-}5.0}
\newcommand{\hlLrNSixburnCIHi}{3.2}
\newcommand{\hlLrNSixburnTostCILo}{\ensuremath{-}4.0}
\newcommand{\hlLrNSixburnTostCIHi}{2.3}
\newcommand{\hlLrNSixburnMde}{6.8}
\newcommand{\hlLrNSixburnPHolm}{0.591}
\newcommand{\hlLrNSixburnN}{5}
\newcommand{\hlLrFTwoburnEst}{0.4}
\newcommand{\hlLrFTwoburnCILo}{\ensuremath{-}2.2}
\newcommand{\hlLrFTwoburnCIHi}{3.0}
\newcommand{\hlLrFTwoburnTostCILo}{\ensuremath{-}1.6}
\newcommand{\hlLrFTwoburnTostCIHi}{2.4}
\newcommand{\hlLrFTwoburnMde}{4.3}
\newcommand{\hlLrFTwoburnPHolm}{1.000}
\newcommand{\hlLrFTwoburnN}{5}
\newcommand{\hlLrFOneburnEst}{0.9}
\newcommand{\hlLrFOneburnCILo}{\ensuremath{-}3.8}
\newcommand{\hlLrFOneburnCIHi}{5.5}
\newcommand{\hlLrFOneburnTostCILo}{\ensuremath{-}2.7}
\newcommand{\hlLrFOneburnTostCIHi}{4.4}
\newcommand{\hlLrFOneburnMde}{7.7}
\newcommand{\hlLrFOneburnPHolm}{0.632}
\newcommand{\hlLrFOneburnN}{5}
\newcommand{\hlLrFOneOneburnEst}{\ensuremath{-}3.8}
\newcommand{\hlLrFOneOneburnCILo}{\ensuremath{-}8.6}
\newcommand{\hlLrFOneOneburnCIHi}{1.1}
\newcommand{\hlLrFOneOneburnTostCILo}{\ensuremath{-}7.5}
\newcommand{\hlLrFOneOneburnTostCIHi}{0.0}
\newcommand{\hlLrFOneOneburnMde}{8.0}
\newcommand{\hlLrFOneOneburnPHolm}{0.098}
\newcommand{\hlLrFOneOneburnN}{5}
\newcommand{\hlLrMinusLTwoburnEst}{6.6}
\newcommand{\hlLrMinusLTwoburnCILo}{5.3}
\newcommand{\hlLrMinusLTwoburnCIHi}{7.9}
\newcommand{\hlLrMinusLTwoburnTostCILo}{5.5}
\newcommand{\hlLrMinusLTwoburnTostCIHi}{7.7}
\newcommand{\hlLrMinusLTwoburnMde}{2.0}
\newcommand{\hlLrMinusLTwoburnPHolm}{\ensuremath{<}0.001}
\newcommand{\hlLrMinusLTwoburnN}{25}
\newcommand{\hlLrMinusLOneburnEst}{18.6}
\newcommand{\hlLrMinusLOneburnCILo}{17.6}
\newcommand{\hlLrMinusLOneburnCIHi}{19.6}
\newcommand{\hlLrMinusLOneburnTostCILo}{17.8}
\newcommand{\hlLrMinusLOneburnTostCIHi}{19.4}
\newcommand{\hlLrMinusLOneburnMde}{1.6}
\newcommand{\hlLrMinusLOneburnPHolm}{\ensuremath{<}0.001}
\newcommand{\hlLrMinusLOneburnN}{25}
\newcommand{\hlLrVerdictburn}{\Lpair{} loses more than \Ltwo}
\newcommand{\hlLrVerdictNSixburn}{Undetermined, MDE 6.8}
\newcommand{\hlLrVerdictFTwoburn}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlLrDropSATflairShift}{7.5}
\newcommand{\hlLrDropSATflairShiftCILo}{6.7}
\newcommand{\hlLrDropSATflairShiftCIHi}{8.3}
\newcommand{\hlLrDropSATflairCoarse}{12.3}
\newcommand{\hlLrDropSATflairCoarseCILo}{11.3}
\newcommand{\hlLrDropSATflairCoarseCIHi}{13.3}
\newcommand{\hlLrDropSATflairBoundary}{8.9}
\newcommand{\hlLrDropSATflairBoundaryCILo}{8.1}
\newcommand{\hlLrDropSATflairBoundaryCIHi}{9.8}
\newcommand{\hlLrDropSATflairOmission}{11.4}
\newcommand{\hlLrDropSATflairOmissionCILo}{9.8}
\newcommand{\hlLrDropSATflairOmissionCIHi}{13.0}
\newcommand{\hlLrMeanDropSATflair}{10.1}
\newcommand{\hlLrDropLVDflairShift}{5.1}
\newcommand{\hlLrDropLVDflairShiftCILo}{3.6}
\newcommand{\hlLrDropLVDflairShiftCIHi}{6.5}
\newcommand{\hlLrDropLVDflairCoarse}{10.0}
\newcommand{\hlLrDropLVDflairCoarseCILo}{8.1}
\newcommand{\hlLrDropLVDflairCoarseCIHi}{11.8}
\newcommand{\hlLrDropLVDflairBoundary}{4.3}
\newcommand{\hlLrDropLVDflairBoundaryCILo}{2.9}
\newcommand{\hlLrDropLVDflairBoundaryCIHi}{5.7}
\newcommand{\hlLrDropLVDflairOmission}{6.1}
\newcommand{\hlLrDropLVDflairOmissionCILo}{4.0}
\newcommand{\hlLrDropLVDflairOmissionCIHi}{8.1}
\newcommand{\hlLrMeanDropLVDflair}{6.4}
\newcommand{\hlLrDropDOFAflairShift}{7.1}
\newcommand{\hlLrDropDOFAflairShiftCILo}{5.6}
\newcommand{\hlLrDropDOFAflairShiftCIHi}{8.6}
\newcommand{\hlLrDropDOFAflairCoarse}{10.5}
\newcommand{\hlLrDropDOFAflairCoarseCILo}{9.6}
\newcommand{\hlLrDropDOFAflairCoarseCIHi}{11.5}
\newcommand{\hlLrDropDOFAflairBoundary}{6.3}
\newcommand{\hlLrDropDOFAflairBoundaryCILo}{5.4}
\newcommand{\hlLrDropDOFAflairBoundaryCIHi}{7.1}
\newcommand{\hlLrDropDOFAflairOmission}{7.7}
\newcommand{\hlLrDropDOFAflairOmissionCILo}{5.4}
\newcommand{\hlLrDropDOFAflairOmissionCIHi}{10.0}
\newcommand{\hlLrMeanDropDOFAflair}{7.9}
\newcommand{\hlLrDropTMflairShift}{6.6}
\newcommand{\hlLrDropTMflairShiftCILo}{5.0}
\newcommand{\hlLrDropTMflairShiftCIHi}{8.2}
\newcommand{\hlLrDropTMflairCoarse}{9.6}
\newcommand{\hlLrDropTMflairCoarseCILo}{7.1}
\newcommand{\hlLrDropTMflairCoarseCIHi}{12.1}
\newcommand{\hlLrDropTMflairBoundary}{8.0}
\newcommand{\hlLrDropTMflairBoundaryCILo}{6.9}
\newcommand{\hlLrDropTMflairBoundaryCIHi}{9.1}
\newcommand{\hlLrDropTMflairOmission}{6.6}
\newcommand{\hlLrDropTMflairOmissionCILo}{4.5}
\newcommand{\hlLrDropTMflairOmissionCIHi}{8.7}
\newcommand{\hlLrMeanDropTMflair}{7.7}
\newcommand{\hlLrDropRNflairShift}{7.3}
\newcommand{\hlLrDropRNflairShiftCILo}{5.6}
\newcommand{\hlLrDropRNflairShiftCIHi}{8.9}
\newcommand{\hlLrDropRNflairCoarse}{10.8}
\newcommand{\hlLrDropRNflairCoarseCILo}{8.4}
\newcommand{\hlLrDropRNflairCoarseCIHi}{13.3}
\newcommand{\hlLrDropRNflairBoundary}{3.9}
\newcommand{\hlLrDropRNflairBoundaryCILo}{1.8}
\newcommand{\hlLrDropRNflairBoundaryCIHi}{6.0}
\newcommand{\hlLrDropRNflairOmission}{7.1}
\newcommand{\hlLrDropRNflairOmissionCILo}{2.6}
\newcommand{\hlLrDropRNflairOmissionCIHi}{11.5}
\newcommand{\hlLrMeanDropRNflair}{7.3}
\newcommand{\hlLrMeanDropflair}{7.9}
\newcommand{\hlLrTypeRankflairOne}{coarse}
\newcommand{\hlLrTypeRankflairTwo}{omission}
\newcommand{\hlLrTypeRankflairThree}{shift}
\newcommand{\hlLrTypeRankflairFour}{boundary}
\newcommand{\hlLrRankSameflair}{no}
\newcommand{\hlLrRankVerdictflair}{Ranking differs from \Ltwo}
\newcommand{\hlLrNSixflairEst}{2.2}
\newcommand{\hlLrNSixflairCILo}{1.2}
\newcommand{\hlLrNSixflairCIHi}{3.2}
\newcommand{\hlLrNSixflairTostCILo}{1.4}
\newcommand{\hlLrNSixflairTostCIHi}{3.0}
\newcommand{\hlLrNSixflairMde}{1.6}
\newcommand{\hlLrNSixflairPHolm}{0.007}
\newcommand{\hlLrNSixflairN}{5}
\newcommand{\hlLrFTwoflairEst}{0.5}
\newcommand{\hlLrFTwoflairCILo}{\ensuremath{-}2.2}
\newcommand{\hlLrFTwoflairCIHi}{3.3}
\newcommand{\hlLrFTwoflairTostCILo}{\ensuremath{-}1.6}
\newcommand{\hlLrFTwoflairTostCIHi}{2.7}
\newcommand{\hlLrFTwoflairMde}{4.5}
\newcommand{\hlLrFTwoflairPHolm}{1.000}
\newcommand{\hlLrFTwoflairN}{5}
\newcommand{\hlLrFOneflairEst}{3.7}
\newcommand{\hlLrFOneflairCILo}{2.3}
\newcommand{\hlLrFOneflairCIHi}{5.1}
\newcommand{\hlLrFOneflairTostCILo}{2.6}
\newcommand{\hlLrFOneflairTostCIHi}{4.8}
\newcommand{\hlLrFOneflairMde}{2.3}
\newcommand{\hlLrFOneflairPHolm}{0.004}
\newcommand{\hlLrFOneflairN}{5}
\newcommand{\hlLrFOneOneflairEst}{2.7}
\newcommand{\hlLrFOneOneflairCILo}{1.2}
\newcommand{\hlLrFOneOneflairCIHi}{4.2}
\newcommand{\hlLrFOneOneflairTostCILo}{1.5}
\newcommand{\hlLrFOneOneflairTostCIHi}{3.9}
\newcommand{\hlLrFOneOneflairMde}{2.5}
\newcommand{\hlLrFOneOneflairPHolm}{0.015}
\newcommand{\hlLrFOneOneflairN}{5}
\newcommand{\hlLrMinusLTwoflairEst}{3.1}
\newcommand{\hlLrMinusLTwoflairCILo}{2.8}
\newcommand{\hlLrMinusLTwoflairCIHi}{3.4}
\newcommand{\hlLrMinusLTwoflairTostCILo}{2.8}
\newcommand{\hlLrMinusLTwoflairTostCIHi}{3.4}
\newcommand{\hlLrMinusLTwoflairMde}{0.5}
\newcommand{\hlLrMinusLTwoflairPHolm}{\ensuremath{<}0.001}
\newcommand{\hlLrMinusLTwoflairN}{25}
\newcommand{\hlLrMinusLOneflairEst}{6.6}
\newcommand{\hlLrMinusLOneflairCILo}{6.1}
\newcommand{\hlLrMinusLOneflairCIHi}{7.0}
\newcommand{\hlLrMinusLOneflairTostCILo}{6.2}
\newcommand{\hlLrMinusLOneflairTostCIHi}{6.9}
\newcommand{\hlLrMinusLOneflairMde}{0.7}
\newcommand{\hlLrMinusLOneflairPHolm}{\ensuremath{<}0.001}
\newcommand{\hlLrMinusLOneflairN}{25}
\newcommand{\hlLrVerdictflair}{\Lpair{} loses more than \Ltwo}
\newcommand{\hlLrVerdictNSixflair}{Equivalent within $\pm$\TostMargin, \lvd loses less}
\newcommand{\hlLrVerdictFTwoflair}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlSeedExtNSATburn}{8}
\newcommand{\hlSeedExtNLVDburn}{8}
\newcommand{\hlSeedExtNDOFAburn}{8}
\newcommand{\hlSeedExtNTMburn}{8}
\newcommand{\hlSeedExtNRNburn}{8}
\newcommand{\hlSeedExtFOneFiveburnEst}{3.7}
\newcommand{\hlSeedExtFOneFiveburnCILo}{0.3}
\newcommand{\hlSeedExtFOneFiveburnCIHi}{7.1}
\newcommand{\hlSeedExtFOneFiveburnTostCILo}{1.1}
\newcommand{\hlSeedExtFOneFiveburnTostCIHi}{6.3}
\newcommand{\hlSeedExtFOneFiveburnMde}{5.7}
\newcommand{\hlSeedExtFOneFiveburnPHolm}{0.040}
\newcommand{\hlSeedExtFOneFiveburnN}{5}
\newcommand{\hlSeedExtFOneAllburnEst}{4.3}
\newcommand{\hlSeedExtFOneAllburnCILo}{1.3}
\newcommand{\hlSeedExtFOneAllburnCIHi}{7.3}
\newcommand{\hlSeedExtFOneAllburnTostCILo}{1.9}
\newcommand{\hlSeedExtFOneAllburnTostCIHi}{6.7}
\newcommand{\hlSeedExtFOneAllburnMde}{4.8}
\newcommand{\hlSeedExtFOneAllburnPHolm}{0.011}
\newcommand{\hlSeedExtFOneAllburnN}{8}
\newcommand{\hlFOneExtburnEst}{4.3}
\newcommand{\hlFOneExtburnCILo}{1.3}
\newcommand{\hlFOneExtburnCIHi}{7.3}
\newcommand{\hlFOneExtburnTostCILo}{1.9}
\newcommand{\hlFOneExtburnTostCIHi}{6.7}
\newcommand{\hlFOneExtburnMde}{4.8}
\newcommand{\hlFOneExtburnPHolm}{0.011}
\newcommand{\hlFOneExtburnN}{8}
\newcommand{\hlFOneExtVerdictburn}{\lvd loses less}
\newcommand{\hlFOneExtFiveburnEst}{3.7}
\newcommand{\hlFOneExtFiveburnCILo}{0.3}
\newcommand{\hlFOneExtFiveburnCIHi}{7.1}
\newcommand{\hlFOneExtFiveburnTostCILo}{1.1}
\newcommand{\hlFOneExtFiveburnTostCIHi}{6.3}
\newcommand{\hlFOneExtFiveburnMde}{5.7}
\newcommand{\hlFOneExtFiveburnPHolm}{0.040}
\newcommand{\hlFOneExtFiveburnN}{5}
\newcommand{\hlFOneExtFiveVerdictburn}{\lvd loses less}
\newcommand{\hlSeedExtFTwoFiveburnEst}{\ensuremath{-}0.5}
\newcommand{\hlSeedExtFTwoFiveburnCILo}{\ensuremath{-}5.4}
\newcommand{\hlSeedExtFTwoFiveburnCIHi}{4.4}
\newcommand{\hlSeedExtFTwoFiveburnTostCILo}{\ensuremath{-}4.3}
\newcommand{\hlSeedExtFTwoFiveburnTostCIHi}{3.3}
\newcommand{\hlSeedExtFTwoFiveburnMde}{8.1}
\newcommand{\hlSeedExtFTwoFiveburnPHolm}{1.000}
\newcommand{\hlSeedExtFTwoFiveburnN}{5}
\newcommand{\hlSeedExtFTwoAllburnEst}{0.0}
\newcommand{\hlSeedExtFTwoAllburnCILo}{\ensuremath{-}2.8}
\newcommand{\hlSeedExtFTwoAllburnCIHi}{2.7}
\newcommand{\hlSeedExtFTwoAllburnTostCILo}{\ensuremath{-}2.2}
\newcommand{\hlSeedExtFTwoAllburnTostCIHi}{2.1}
\newcommand{\hlSeedExtFTwoAllburnMde}{4.4}
\newcommand{\hlSeedExtFTwoAllburnPHolm}{1.000}
\newcommand{\hlSeedExtFTwoAllburnN}{8}
\newcommand{\hlFTwoExtburnEst}{0.0}
\newcommand{\hlFTwoExtburnCILo}{\ensuremath{-}2.8}
\newcommand{\hlFTwoExtburnCIHi}{2.7}
\newcommand{\hlFTwoExtburnTostCILo}{\ensuremath{-}2.2}
\newcommand{\hlFTwoExtburnTostCIHi}{2.1}
\newcommand{\hlFTwoExtburnMde}{4.4}
\newcommand{\hlFTwoExtburnPHolm}{1.000}
\newcommand{\hlFTwoExtburnN}{8}
\newcommand{\hlFTwoExtVerdictburn}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlFTwoExtFiveburnEst}{\ensuremath{-}0.5}
\newcommand{\hlFTwoExtFiveburnCILo}{\ensuremath{-}5.4}
\newcommand{\hlFTwoExtFiveburnCIHi}{4.4}
\newcommand{\hlFTwoExtFiveburnTostCILo}{\ensuremath{-}4.3}
\newcommand{\hlFTwoExtFiveburnTostCIHi}{3.3}
\newcommand{\hlFTwoExtFiveburnMde}{8.1}
\newcommand{\hlFTwoExtFiveburnPHolm}{1.000}
\newcommand{\hlFTwoExtFiveburnN}{5}
\newcommand{\hlFTwoExtFiveVerdictburn}{Undetermined, MDE 8.1}
\newcommand{\hlSeedExtNSATflair}{8}
\newcommand{\hlSeedExtNLVDflair}{8}
\newcommand{\hlSeedExtNDOFAflair}{5}
\newcommand{\hlSeedExtNTMflair}{5}
\newcommand{\hlSeedExtNRNflair}{5}
\newcommand{\hlSeedExtFOneFiveflairEst}{2.9}
\newcommand{\hlSeedExtFOneFiveflairCILo}{1.3}
\newcommand{\hlSeedExtFOneFiveflairCIHi}{4.5}
\newcommand{\hlSeedExtFOneFiveflairTostCILo}{1.7}
\newcommand{\hlSeedExtFOneFiveflairTostCIHi}{4.1}
\newcommand{\hlSeedExtFOneFiveflairMde}{2.6}
\newcommand{\hlSeedExtFOneFiveflairPHolm}{0.014}
\newcommand{\hlSeedExtFOneFiveflairN}{5}
\newcommand{\hlSeedExtFOneAllflairEst}{2.8}
\newcommand{\hlSeedExtFOneAllflairCILo}{1.8}
\newcommand{\hlSeedExtFOneAllflairCIHi}{3.8}
\newcommand{\hlSeedExtFOneAllflairTostCILo}{2.0}
\newcommand{\hlSeedExtFOneAllflairTostCIHi}{3.6}
\newcommand{\hlSeedExtFOneAllflairMde}{1.6}
\newcommand{\hlSeedExtFOneAllflairPHolm}{\ensuremath{<}0.001}
\newcommand{\hlSeedExtFOneAllflairN}{8}
\newcommand{\hlFOneExtflairEst}{2.8}
\newcommand{\hlFOneExtflairCILo}{1.8}
\newcommand{\hlFOneExtflairCIHi}{3.8}
\newcommand{\hlFOneExtflairTostCILo}{2.0}
\newcommand{\hlFOneExtflairTostCIHi}{3.6}
\newcommand{\hlFOneExtflairMde}{1.6}
\newcommand{\hlFOneExtflairPHolm}{\ensuremath{<}0.001}
\newcommand{\hlFOneExtflairN}{8}
\newcommand{\hlFOneExtVerdictflair}{\lvd loses less}
\newcommand{\hlFOneExtFiveflairEst}{2.9}
\newcommand{\hlFOneExtFiveflairCILo}{1.3}
\newcommand{\hlFOneExtFiveflairCIHi}{4.5}
\newcommand{\hlFOneExtFiveflairTostCILo}{1.7}
\newcommand{\hlFOneExtFiveflairTostCIHi}{4.1}
\newcommand{\hlFOneExtFiveflairMde}{2.6}
\newcommand{\hlFOneExtFiveflairPHolm}{0.014}
\newcommand{\hlFOneExtFiveflairN}{5}
\newcommand{\hlFOneExtFiveVerdictflair}{\lvd loses less}
\newcommand{\hlSeedExtFTwoFiveflairEst}{0.6}
\newcommand{\hlSeedExtFTwoFiveflairCILo}{\ensuremath{-}2.0}
\newcommand{\hlSeedExtFTwoFiveflairCIHi}{3.1}
\newcommand{\hlSeedExtFTwoFiveflairTostCILo}{\ensuremath{-}1.4}
\newcommand{\hlSeedExtFTwoFiveflairTostCIHi}{2.5}
\newcommand{\hlSeedExtFTwoFiveflairMde}{4.2}
\newcommand{\hlSeedExtFTwoFiveflairPHolm}{1.000}
\newcommand{\hlSeedExtFTwoFiveflairN}{5}
\newcommand{\hlSeedExtFTwoAllflairEst}{0.6}
\newcommand{\hlSeedExtFTwoAllflairCILo}{\ensuremath{-}2.0}
\newcommand{\hlSeedExtFTwoAllflairCIHi}{3.1}
\newcommand{\hlSeedExtFTwoAllflairTostCILo}{\ensuremath{-}1.4}
\newcommand{\hlSeedExtFTwoAllflairTostCIHi}{2.5}
\newcommand{\hlSeedExtFTwoAllflairMde}{4.2}
\newcommand{\hlSeedExtFTwoAllflairPHolm}{1.000}
\newcommand{\hlSeedExtFTwoAllflairN}{5}
\newcommand{\hlFTwoExtflairEst}{0.6}
\newcommand{\hlFTwoExtflairCILo}{\ensuremath{-}2.0}
\newcommand{\hlFTwoExtflairCIHi}{3.1}
\newcommand{\hlFTwoExtflairTostCILo}{\ensuremath{-}1.4}
\newcommand{\hlFTwoExtflairTostCIHi}{2.5}
\newcommand{\hlFTwoExtflairMde}{4.2}
\newcommand{\hlFTwoExtflairPHolm}{1.000}
\newcommand{\hlFTwoExtflairN}{5}
\newcommand{\hlFTwoExtVerdictflair}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlFTwoExtFiveflairEst}{0.6}
\newcommand{\hlFTwoExtFiveflairCILo}{\ensuremath{-}2.0}
\newcommand{\hlFTwoExtFiveflairCIHi}{3.1}
\newcommand{\hlFTwoExtFiveflairTostCILo}{\ensuremath{-}1.4}
\newcommand{\hlFTwoExtFiveflairTostCIHi}{2.5}
\newcommand{\hlFTwoExtFiveflairMde}{4.2}
\newcommand{\hlFTwoExtFiveflairPHolm}{1.000}
\newcommand{\hlFTwoExtFiveflairN}{5}
\newcommand{\hlFTwoExtFiveVerdictflair}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlLossDropCESATburn}{17.8}
\newcommand{\hlLossCleanCESATburn}{75.8}
\newcommand{\hlLossDropCELVDburn}{14.1}
\newcommand{\hlLossCleanCELVDburn}{82.0}
\newcommand{\hlLossDropCEDOFAburn}{17.9}
\newcommand{\hlLossCleanCEDOFAburn}{85.5}
\newcommand{\hlLossDropCETMburn}{12.9}
\newcommand{\hlLossCleanCETMburn}{86.2}
\newcommand{\hlLossDropCERNburn}{15.9}
\newcommand{\hlLossCleanCERNburn}{88.1}
\newcommand{\hlLossDropCEburn}{15.7}
\newcommand{\hlLossCleanCEburn}{83.5}
\newcommand{\hlMitGceburnEst}{\ensuremath{-}1.2}
\newcommand{\hlMitGceburnCILo}{\ensuremath{-}2.9}
\newcommand{\hlMitGceburnCIHi}{0.4}
\newcommand{\hlMitGceburnTostCILo}{\ensuremath{-}2.6}
\newcommand{\hlMitGceburnTostCIHi}{0.2}
\newcommand{\hlMitGceburnMde}{2.7}
\newcommand{\hlMitGceburnPHolm}{0.285}
\newcommand{\hlMitGceburnN}{25}
\newcommand{\hlLossInvGceburnEst}{\ensuremath{-}1.2}
\newcommand{\hlLossInvGceburnCILo}{\ensuremath{-}2.9}
\newcommand{\hlLossInvGceburnCIHi}{0.4}
\newcommand{\hlLossInvGceburnTostCILo}{\ensuremath{-}2.6}
\newcommand{\hlLossInvGceburnTostCIHi}{0.2}
\newcommand{\hlLossInvGceburnMde}{2.7}
\newcommand{\hlLossInvGceburnPHolm}{0.285}
\newcommand{\hlLossInvGceburnN}{25}
\newcommand{\hlMitGceSATburnEst}{\ensuremath{-}6.6}
\newcommand{\hlMitGceSATburnCILo}{\ensuremath{-}13.0}
\newcommand{\hlMitGceSATburnCIHi}{\ensuremath{-}0.3}
\newcommand{\hlLossInvGceSATburnEst}{\ensuremath{-}6.6}
\newcommand{\hlLossInvGceSATburnCILo}{\ensuremath{-}13.0}
\newcommand{\hlLossInvGceSATburnCIHi}{\ensuremath{-}0.3}
\newcommand{\hlLossInvGceSATburnTostCILo}{\ensuremath{-}11.6}
\newcommand{\hlLossInvGceSATburnTostCIHi}{\ensuremath{-}1.7}
\newcommand{\hlLossInvGceSATburnMde}{10.6}
\newcommand{\hlLossInvGceSATburnPHolm}{0.089}
\newcommand{\hlLossInvGceSATburnN}{5}
\newcommand{\hlMitGceDropSATburn}{11.1}
\newcommand{\hlMitGceCleanSATburn}{70.6}
\newcommand{\hlLossDropGceSATburn}{11.1}
\newcommand{\hlLossCleanGceSATburn}{70.6}
\newcommand{\hlMitGceLVDburnEst}{0.0}
\newcommand{\hlMitGceLVDburnCILo}{\ensuremath{-}1.7}
\newcommand{\hlMitGceLVDburnCIHi}{1.7}
\newcommand{\hlLossInvGceLVDburnEst}{0.0}
\newcommand{\hlLossInvGceLVDburnCILo}{\ensuremath{-}1.7}
\newcommand{\hlLossInvGceLVDburnCIHi}{1.7}
\newcommand{\hlLossInvGceLVDburnTostCILo}{\ensuremath{-}1.3}
\newcommand{\hlLossInvGceLVDburnTostCIHi}{1.3}
\newcommand{\hlLossInvGceLVDburnMde}{2.8}
\newcommand{\hlLossInvGceLVDburnPHolm}{0.967}
\newcommand{\hlLossInvGceLVDburnN}{5}
\newcommand{\hlMitGceDropLVDburn}{14.1}
\newcommand{\hlMitGceCleanLVDburn}{81.3}
\newcommand{\hlLossDropGceLVDburn}{14.1}
\newcommand{\hlLossCleanGceLVDburn}{81.3}
\newcommand{\hlMitGceDOFAburnEst}{\ensuremath{-}0.7}
\newcommand{\hlMitGceDOFAburnCILo}{\ensuremath{-}4.2}
\newcommand{\hlMitGceDOFAburnCIHi}{2.8}
\newcommand{\hlLossInvGceDOFAburnEst}{\ensuremath{-}0.7}
\newcommand{\hlLossInvGceDOFAburnCILo}{\ensuremath{-}4.2}
\newcommand{\hlLossInvGceDOFAburnCIHi}{2.8}
\newcommand{\hlLossInvGceDOFAburnTostCILo}{\ensuremath{-}3.4}
\newcommand{\hlLossInvGceDOFAburnTostCIHi}{2.0}
\newcommand{\hlLossInvGceDOFAburnMde}{5.8}
\newcommand{\hlLossInvGceDOFAburnPHolm}{0.603}
\newcommand{\hlLossInvGceDOFAburnN}{5}
\newcommand{\hlMitGceDropDOFAburn}{17.1}
\newcommand{\hlMitGceCleanDOFAburn}{86.8}
\newcommand{\hlLossDropGceDOFAburn}{17.1}
\newcommand{\hlLossCleanGceDOFAburn}{86.8}
\newcommand{\hlMitGceTMburnEst}{1.0}
\newcommand{\hlMitGceTMburnCILo}{\ensuremath{-}1.5}
\newcommand{\hlMitGceTMburnCIHi}{3.6}
\newcommand{\hlLossInvGceTMburnEst}{1.0}
\newcommand{\hlLossInvGceTMburnCILo}{\ensuremath{-}1.5}
\newcommand{\hlLossInvGceTMburnCIHi}{3.6}
\newcommand{\hlLossInvGceTMburnTostCILo}{\ensuremath{-}0.9}
\newcommand{\hlLossInvGceTMburnTostCIHi}{3.0}
\newcommand{\hlLossInvGceTMburnMde}{4.2}
\newcommand{\hlLossInvGceTMburnPHolm}{0.640}
\newcommand{\hlLossInvGceTMburnN}{5}
\newcommand{\hlMitGceDropTMburn}{14.0}
\newcommand{\hlMitGceCleanTMburn}{87.2}
\newcommand{\hlLossDropGceTMburn}{14.0}
\newcommand{\hlLossCleanGceTMburn}{87.2}
\newcommand{\hlMitGceRNburnEst}{0.1}
\newcommand{\hlMitGceRNburnCILo}{\ensuremath{-}4.4}
\newcommand{\hlMitGceRNburnCIHi}{4.5}
\newcommand{\hlLossInvGceRNburnEst}{0.1}
\newcommand{\hlLossInvGceRNburnCILo}{\ensuremath{-}4.4}
\newcommand{\hlLossInvGceRNburnCIHi}{4.5}
\newcommand{\hlLossInvGceRNburnTostCILo}{\ensuremath{-}3.4}
\newcommand{\hlLossInvGceRNburnTostCIHi}{3.5}
\newcommand{\hlLossInvGceRNburnMde}{7.3}
\newcommand{\hlLossInvGceRNburnPHolm}{0.992}
\newcommand{\hlLossInvGceRNburnN}{5}
\newcommand{\hlMitGceDropRNburn}{16.0}
\newcommand{\hlMitGceCleanRNburn}{88.7}
\newcommand{\hlLossDropGceRNburn}{16.0}
\newcommand{\hlLossCleanGceRNburn}{88.7}
\newcommand{\hlLossDropGceburn}{14.5}
\newcommand{\hlLossCleanGceburn}{82.9}
\newcommand{\hlMitGceShiftburnEst}{\ensuremath{-}1.5}
\newcommand{\hlMitGceShiftburnCILo}{\ensuremath{-}3.7}
\newcommand{\hlMitGceShiftburnCIHi}{0.6}
\newcommand{\hlMitGceCoarseburnEst}{\ensuremath{-}1.7}
\newcommand{\hlMitGceCoarseburnCILo}{\ensuremath{-}4.1}
\newcommand{\hlMitGceCoarseburnCIHi}{0.7}
\newcommand{\hlMitGceBoundaryburnEst}{\ensuremath{-}1.6}
\newcommand{\hlMitGceBoundaryburnCILo}{\ensuremath{-}3.5}
\newcommand{\hlMitGceBoundaryburnCIHi}{0.3}
\newcommand{\hlMitGceOmissionburnEst}{\ensuremath{-}0.1}
\newcommand{\hlMitGceOmissionburnCILo}{\ensuremath{-}2.8}
\newcommand{\hlMitGceOmissionburnCIHi}{2.6}
\newcommand{\hlMitGceCleanCostburnEst}{\ensuremath{-}0.6}
\newcommand{\hlMitGceCleanCostburnCILo}{\ensuremath{-}1.9}
\newcommand{\hlMitGceCleanCostburnCIHi}{0.7}
\newcommand{\hlLossCleanInvGceburnEst}{\ensuremath{-}0.6}
\newcommand{\hlLossCleanInvGceburnCILo}{\ensuremath{-}1.9}
\newcommand{\hlLossCleanInvGceburnCIHi}{0.7}
\newcommand{\hlLossCleanInvGceburnTostCILo}{\ensuremath{-}1.7}
\newcommand{\hlLossCleanInvGceburnTostCIHi}{0.5}
\newcommand{\hlLossCleanInvGceburnMde}{2.1}
\newcommand{\hlLossCleanInvGceburnPHolm}{0.340}
\newcommand{\hlLossCleanInvGceburnN}{25}
\newcommand{\hlMitVerdictGceburn}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlLossVerdictGceburn}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlMitBootburnEst}{\ensuremath{-}1.2}
\newcommand{\hlMitBootburnCILo}{\ensuremath{-}2.5}
\newcommand{\hlMitBootburnCIHi}{0.1}
\newcommand{\hlMitBootburnTostCILo}{\ensuremath{-}2.3}
\newcommand{\hlMitBootburnTostCIHi}{\ensuremath{-}0.1}
\newcommand{\hlMitBootburnMde}{2.1}
\newcommand{\hlMitBootburnPHolm}{0.153}
\newcommand{\hlMitBootburnN}{25}
\newcommand{\hlLossInvBootburnEst}{\ensuremath{-}1.2}
\newcommand{\hlLossInvBootburnCILo}{\ensuremath{-}2.5}
\newcommand{\hlLossInvBootburnCIHi}{0.1}
\newcommand{\hlLossInvBootburnTostCILo}{\ensuremath{-}2.3}
\newcommand{\hlLossInvBootburnTostCIHi}{\ensuremath{-}0.1}
\newcommand{\hlLossInvBootburnMde}{2.1}
\newcommand{\hlLossInvBootburnPHolm}{0.153}
\newcommand{\hlLossInvBootburnN}{25}
\newcommand{\hlMitBootSATburnEst}{\ensuremath{-}4.5}
\newcommand{\hlMitBootSATburnCILo}{\ensuremath{-}9.0}
\newcommand{\hlMitBootSATburnCIHi}{\ensuremath{-}0.1}
\newcommand{\hlLossInvBootSATburnEst}{\ensuremath{-}4.5}
\newcommand{\hlLossInvBootSATburnCILo}{\ensuremath{-}9.0}
\newcommand{\hlLossInvBootSATburnCIHi}{\ensuremath{-}0.1}
\newcommand{\hlLossInvBootSATburnTostCILo}{\ensuremath{-}8.0}
\newcommand{\hlLossInvBootSATburnTostCIHi}{\ensuremath{-}1.1}
\newcommand{\hlLossInvBootSATburnMde}{7.4}
\newcommand{\hlLossInvBootSATburnPHolm}{0.096}
\newcommand{\hlLossInvBootSATburnN}{5}
\newcommand{\hlMitBootDropSATburn}{13.3}
\newcommand{\hlMitBootCleanSATburn}{72.2}
\newcommand{\hlLossDropBootSATburn}{13.3}
\newcommand{\hlLossCleanBootSATburn}{72.2}
\newcommand{\hlMitBootLVDburnEst}{0.0}
\newcommand{\hlMitBootLVDburnCILo}{\ensuremath{-}3.5}
\newcommand{\hlMitBootLVDburnCIHi}{3.6}
\newcommand{\hlLossInvBootLVDburnEst}{0.0}
\newcommand{\hlLossInvBootLVDburnCILo}{\ensuremath{-}3.5}
\newcommand{\hlLossInvBootLVDburnCIHi}{3.6}
\newcommand{\hlLossInvBootLVDburnTostCILo}{\ensuremath{-}2.7}
\newcommand{\hlLossInvBootLVDburnTostCIHi}{2.8}
\newcommand{\hlLossInvBootLVDburnMde}{5.9}
\newcommand{\hlLossInvBootLVDburnPHolm}{0.978}
\newcommand{\hlLossInvBootLVDburnN}{5}
\newcommand{\hlMitBootDropLVDburn}{14.1}
\newcommand{\hlMitBootCleanLVDburn}{82.0}
\newcommand{\hlLossDropBootLVDburn}{14.1}
\newcommand{\hlLossCleanBootLVDburn}{82.0}
\newcommand{\hlMitBootDOFAburnEst}{\ensuremath{-}0.1}
\newcommand{\hlMitBootDOFAburnCILo}{\ensuremath{-}1.7}
\newcommand{\hlMitBootDOFAburnCIHi}{1.5}
\newcommand{\hlLossInvBootDOFAburnEst}{\ensuremath{-}0.1}
\newcommand{\hlLossInvBootDOFAburnCILo}{\ensuremath{-}1.7}
\newcommand{\hlLossInvBootDOFAburnCIHi}{1.5}
\newcommand{\hlLossInvBootDOFAburnTostCILo}{\ensuremath{-}1.3}
\newcommand{\hlLossInvBootDOFAburnTostCIHi}{1.2}
\newcommand{\hlLossInvBootDOFAburnMde}{2.7}
\newcommand{\hlLossInvBootDOFAburnPHolm}{1.000}
\newcommand{\hlLossInvBootDOFAburnN}{5}
\newcommand{\hlMitBootDropDOFAburn}{17.8}
\newcommand{\hlMitBootCleanDOFAburn}{86.4}
\newcommand{\hlLossDropBootDOFAburn}{17.8}
\newcommand{\hlLossCleanBootDOFAburn}{86.4}
\newcommand{\hlMitBootTMburnEst}{\ensuremath{-}0.1}
\newcommand{\hlMitBootTMburnCILo}{\ensuremath{-}1.5}
\newcommand{\hlMitBootTMburnCIHi}{1.4}
\newcommand{\hlLossInvBootTMburnEst}{\ensuremath{-}0.1}
\newcommand{\hlLossInvBootTMburnCILo}{\ensuremath{-}1.5}
\newcommand{\hlLossInvBootTMburnCIHi}{1.4}
\newcommand{\hlLossInvBootTMburnTostCILo}{\ensuremath{-}1.2}
\newcommand{\hlLossInvBootTMburnTostCIHi}{1.1}
\newcommand{\hlLossInvBootTMburnMde}{2.4}
\newcommand{\hlLossInvBootTMburnPHolm}{0.977}
\newcommand{\hlLossInvBootTMburnN}{5}
\newcommand{\hlMitBootDropTMburn}{12.9}
\newcommand{\hlMitBootCleanTMburn}{86.3}
\newcommand{\hlLossDropBootTMburn}{12.9}
\newcommand{\hlLossCleanBootTMburn}{86.3}
\newcommand{\hlMitBootRNburnEst}{\ensuremath{-}1.4}
\newcommand{\hlMitBootRNburnCILo}{\ensuremath{-}6.9}
\newcommand{\hlMitBootRNburnCIHi}{4.2}
\newcommand{\hlLossInvBootRNburnEst}{\ensuremath{-}1.4}
\newcommand{\hlLossInvBootRNburnCILo}{\ensuremath{-}6.9}
\newcommand{\hlLossInvBootRNburnCIHi}{4.2}
\newcommand{\hlLossInvBootRNburnTostCILo}{\ensuremath{-}5.7}
\newcommand{\hlLossInvBootRNburnTostCIHi}{2.9}
\newcommand{\hlLossInvBootRNburnMde}{9.2}
\newcommand{\hlLossInvBootRNburnPHolm}{1.000}
\newcommand{\hlLossInvBootRNburnN}{5}
\newcommand{\hlMitBootDropRNburn}{14.5}
\newcommand{\hlMitBootCleanRNburn}{88.3}
\newcommand{\hlLossDropBootRNburn}{14.5}
\newcommand{\hlLossCleanBootRNburn}{88.3}
\newcommand{\hlLossDropBootburn}{14.5}
\newcommand{\hlLossCleanBootburn}{83.0}
\newcommand{\hlMitBootShiftburnEst}{0.0}
\newcommand{\hlMitBootShiftburnCILo}{\ensuremath{-}1.3}
\newcommand{\hlMitBootShiftburnCIHi}{1.3}
\newcommand{\hlMitBootCoarseburnEst}{\ensuremath{-}1.8}
\newcommand{\hlMitBootCoarseburnCILo}{\ensuremath{-}4.2}
\newcommand{\hlMitBootCoarseburnCIHi}{0.5}
\newcommand{\hlMitBootBoundaryburnEst}{\ensuremath{-}1.1}
\newcommand{\hlMitBootBoundaryburnCILo}{\ensuremath{-}2.8}
\newcommand{\hlMitBootBoundaryburnCIHi}{0.6}
\newcommand{\hlMitBootOmissionburnEst}{\ensuremath{-}1.9}
\newcommand{\hlMitBootOmissionburnCILo}{\ensuremath{-}5.0}
\newcommand{\hlMitBootOmissionburnCIHi}{1.2}
\newcommand{\hlMitBootCleanCostburnEst}{\ensuremath{-}0.5}
\newcommand{\hlMitBootCleanCostburnCILo}{\ensuremath{-}1.4}
\newcommand{\hlMitBootCleanCostburnCIHi}{0.4}
\newcommand{\hlLossCleanInvBootburnEst}{\ensuremath{-}0.5}
\newcommand{\hlLossCleanInvBootburnCILo}{\ensuremath{-}1.4}
\newcommand{\hlLossCleanInvBootburnCIHi}{0.4}
\newcommand{\hlLossCleanInvBootburnTostCILo}{\ensuremath{-}1.2}
\newcommand{\hlLossCleanInvBootburnTostCIHi}{0.3}
\newcommand{\hlLossCleanInvBootburnMde}{1.4}
\newcommand{\hlLossCleanInvBootburnPHolm}{0.279}
\newcommand{\hlLossCleanInvBootburnN}{25}
\newcommand{\hlMitVerdictBootburn}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlLossVerdictBootburn}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlLossDropCESATflair}{6.5}
\newcommand{\hlLossCleanCESATflair}{52.2}
\newcommand{\hlLossDropCELVDflair}{3.6}
\newcommand{\hlLossCleanCELVDflair}{50.8}
\newcommand{\hlLossDropCEDOFAflair}{4.3}
\newcommand{\hlLossCleanCEDOFAflair}{47.5}
\newcommand{\hlLossDropCETMflair}{5.2}
\newcommand{\hlLossCleanCETMflair}{40.5}
\newcommand{\hlLossDropCERNflair}{4.2}
\newcommand{\hlLossCleanCERNflair}{44.5}
\newcommand{\hlLossDropCEflair}{4.8}
\newcommand{\hlLossCleanCEflair}{47.1}
\newcommand{\hlMitGceflairEst}{0.1}
\newcommand{\hlMitGceflairCILo}{\ensuremath{-}0.8}
\newcommand{\hlMitGceflairCIHi}{0.9}
\newcommand{\hlMitGceflairTostCILo}{\ensuremath{-}0.6}
\newcommand{\hlMitGceflairTostCIHi}{0.8}
\newcommand{\hlMitGceflairMde}{1.3}
\newcommand{\hlMitGceflairPHolm}{0.819}
\newcommand{\hlMitGceflairN}{25}
\newcommand{\hlLossInvGceflairEst}{0.1}
\newcommand{\hlLossInvGceflairCILo}{\ensuremath{-}0.8}
\newcommand{\hlLossInvGceflairCIHi}{0.9}
\newcommand{\hlLossInvGceflairTostCILo}{\ensuremath{-}0.6}
\newcommand{\hlLossInvGceflairTostCIHi}{0.8}
\newcommand{\hlLossInvGceflairMde}{1.3}
\newcommand{\hlLossInvGceflairPHolm}{0.819}
\newcommand{\hlLossInvGceflairN}{25}
\newcommand{\hlMitGceSATflairEst}{\ensuremath{-}1.0}
\newcommand{\hlMitGceSATflairCILo}{\ensuremath{-}4.0}
\newcommand{\hlMitGceSATflairCIHi}{2.0}
\newcommand{\hlLossInvGceSATflairEst}{\ensuremath{-}1.0}
\newcommand{\hlLossInvGceSATflairCILo}{\ensuremath{-}4.0}
\newcommand{\hlLossInvGceSATflairCIHi}{2.0}
\newcommand{\hlLossInvGceSATflairTostCILo}{\ensuremath{-}3.3}
\newcommand{\hlLossInvGceSATflairTostCIHi}{1.3}
\newcommand{\hlLossInvGceSATflairMde}{4.9}
\newcommand{\hlLossInvGceSATflairPHolm}{0.404}
\newcommand{\hlLossInvGceSATflairN}{5}
\newcommand{\hlMitGceDropSATflair}{5.5}
\newcommand{\hlMitGceCleanSATflair}{49.9}
\newcommand{\hlLossDropGceSATflair}{5.5}
\newcommand{\hlLossCleanGceSATflair}{49.9}
\newcommand{\hlMitGceLVDflairEst}{0.7}
\newcommand{\hlMitGceLVDflairCILo}{0.1}
\newcommand{\hlMitGceLVDflairCIHi}{1.3}
\newcommand{\hlLossInvGceLVDflairEst}{0.7}
\newcommand{\hlLossInvGceLVDflairCILo}{0.1}
\newcommand{\hlLossInvGceLVDflairCIHi}{1.3}
\newcommand{\hlLossInvGceLVDflairTostCILo}{0.2}
\newcommand{\hlLossInvGceLVDflairTostCIHi}{1.1}
\newcommand{\hlLossInvGceLVDflairMde}{1.0}
\newcommand{\hlLossInvGceLVDflairPHolm}{0.065}
\newcommand{\hlLossInvGceLVDflairN}{5}
\newcommand{\hlMitGceDropLVDflair}{4.3}
\newcommand{\hlMitGceCleanLVDflair}{50.4}
\newcommand{\hlLossDropGceLVDflair}{4.3}
\newcommand{\hlLossCleanGceLVDflair}{50.4}
\newcommand{\hlMitGceDOFAflairEst}{1.5}
\newcommand{\hlMitGceDOFAflairCILo}{\ensuremath{-}1.8}
\newcommand{\hlMitGceDOFAflairCIHi}{4.8}
\newcommand{\hlLossInvGceDOFAflairEst}{1.5}
\newcommand{\hlLossInvGceDOFAflairCILo}{\ensuremath{-}1.8}
\newcommand{\hlLossInvGceDOFAflairCIHi}{4.8}
\newcommand{\hlLossInvGceDOFAflairTostCILo}{\ensuremath{-}1.1}
\newcommand{\hlLossInvGceDOFAflairTostCIHi}{4.0}
\newcommand{\hlLossInvGceDOFAflairMde}{5.5}
\newcommand{\hlLossInvGceDOFAflairPHolm}{0.565}
\newcommand{\hlLossInvGceDOFAflairN}{5}
\newcommand{\hlMitGceDropDOFAflair}{5.8}
\newcommand{\hlMitGceCleanDOFAflair}{43.8}
\newcommand{\hlLossDropGceDOFAflair}{5.8}
\newcommand{\hlLossCleanGceDOFAflair}{43.8}
\newcommand{\hlMitGceTMflairEst}{\ensuremath{-}0.1}
\newcommand{\hlMitGceTMflairCILo}{\ensuremath{-}2.7}
\newcommand{\hlMitGceTMflairCIHi}{2.4}
\newcommand{\hlLossInvGceTMflairEst}{\ensuremath{-}0.1}
\newcommand{\hlLossInvGceTMflairCILo}{\ensuremath{-}2.7}
\newcommand{\hlLossInvGceTMflairCIHi}{2.4}
\newcommand{\hlLossInvGceTMflairTostCILo}{\ensuremath{-}2.1}
\newcommand{\hlLossInvGceTMflairTostCIHi}{1.8}
\newcommand{\hlLossInvGceTMflairMde}{4.2}
\newcommand{\hlLossInvGceTMflairPHolm}{0.902}
\newcommand{\hlLossInvGceTMflairN}{5}
\newcommand{\hlMitGceDropTMflair}{5.1}
\newcommand{\hlMitGceCleanTMflair}{37.1}
\newcommand{\hlLossDropGceTMflair}{5.1}
\newcommand{\hlLossCleanGceTMflair}{37.1}
\newcommand{\hlMitGceRNflairEst}{\ensuremath{-}0.6}
\newcommand{\hlMitGceRNflairCILo}{\ensuremath{-}2.7}
\newcommand{\hlMitGceRNflairCIHi}{1.6}
\newcommand{\hlLossInvGceRNflairEst}{\ensuremath{-}0.6}
\newcommand{\hlLossInvGceRNflairCILo}{\ensuremath{-}2.7}
\newcommand{\hlLossInvGceRNflairCIHi}{1.6}
\newcommand{\hlLossInvGceRNflairTostCILo}{\ensuremath{-}2.2}
\newcommand{\hlLossInvGceRNflairTostCIHi}{1.1}
\newcommand{\hlLossInvGceRNflairMde}{3.5}
\newcommand{\hlLossInvGceRNflairPHolm}{0.992}
\newcommand{\hlLossInvGceRNflairN}{5}
\newcommand{\hlMitGceDropRNflair}{3.6}
\newcommand{\hlMitGceCleanRNflair}{40.0}
\newcommand{\hlLossDropGceRNflair}{3.6}
\newcommand{\hlLossCleanGceRNflair}{40.0}
\newcommand{\hlLossDropGceflair}{4.9}
\newcommand{\hlLossCleanGceflair}{44.2}
\newcommand{\hlMitGceShiftflairEst}{0.2}
\newcommand{\hlMitGceShiftflairCILo}{\ensuremath{-}0.7}
\newcommand{\hlMitGceShiftflairCIHi}{1.1}
\newcommand{\hlMitGceCoarseflairEst}{0.3}
\newcommand{\hlMitGceCoarseflairCILo}{\ensuremath{-}0.8}
\newcommand{\hlMitGceCoarseflairCIHi}{1.3}
\newcommand{\hlMitGceBoundaryflairEst}{0.0}
\newcommand{\hlMitGceBoundaryflairCILo}{\ensuremath{-}1.2}
\newcommand{\hlMitGceBoundaryflairCIHi}{1.1}
\newcommand{\hlMitGceOmissionflairEst}{\ensuremath{-}0.1}
\newcommand{\hlMitGceOmissionflairCILo}{\ensuremath{-}1.3}
\newcommand{\hlMitGceOmissionflairCIHi}{1.1}
\newcommand{\hlMitGceCleanCostflairEst}{\ensuremath{-}2.9}
\newcommand{\hlMitGceCleanCostflairCILo}{\ensuremath{-}3.6}
\newcommand{\hlMitGceCleanCostflairCIHi}{\ensuremath{-}2.1}
\newcommand{\hlLossCleanInvGceflairEst}{\ensuremath{-}2.9}
\newcommand{\hlLossCleanInvGceflairCILo}{\ensuremath{-}3.6}
\newcommand{\hlLossCleanInvGceflairCIHi}{\ensuremath{-}2.1}
\newcommand{\hlLossCleanInvGceflairTostCILo}{\ensuremath{-}3.5}
\newcommand{\hlLossCleanInvGceflairTostCIHi}{\ensuremath{-}2.2}
\newcommand{\hlLossCleanInvGceflairMde}{1.2}
\newcommand{\hlLossCleanInvGceflairPHolm}{\ensuremath{<}0.001}
\newcommand{\hlLossCleanInvGceflairN}{25}
\newcommand{\hlMitVerdictGceflair}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlLossVerdictGceflair}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlMitBootflairEst}{0.1}
\newcommand{\hlMitBootflairCILo}{\ensuremath{-}0.5}
\newcommand{\hlMitBootflairCIHi}{0.6}
\newcommand{\hlMitBootflairTostCILo}{\ensuremath{-}0.4}
\newcommand{\hlMitBootflairTostCIHi}{0.5}
\newcommand{\hlMitBootflairMde}{0.8}
\newcommand{\hlMitBootflairPHolm}{0.774}
\newcommand{\hlMitBootflairN}{25}
\newcommand{\hlLossInvBootflairEst}{0.1}
\newcommand{\hlLossInvBootflairCILo}{\ensuremath{-}0.5}
\newcommand{\hlLossInvBootflairCIHi}{0.6}
\newcommand{\hlLossInvBootflairTostCILo}{\ensuremath{-}0.4}
\newcommand{\hlLossInvBootflairTostCIHi}{0.5}
\newcommand{\hlLossInvBootflairMde}{0.8}
\newcommand{\hlLossInvBootflairPHolm}{0.774}
\newcommand{\hlLossInvBootflairN}{25}
\newcommand{\hlMitBootSATflairEst}{\ensuremath{-}0.6}
\newcommand{\hlMitBootSATflairCILo}{\ensuremath{-}1.5}
\newcommand{\hlMitBootSATflairCIHi}{0.3}
\newcommand{\hlLossInvBootSATflairEst}{\ensuremath{-}0.6}
\newcommand{\hlLossInvBootSATflairCILo}{\ensuremath{-}1.5}
\newcommand{\hlLossInvBootSATflairCIHi}{0.3}
\newcommand{\hlLossInvBootSATflairTostCILo}{\ensuremath{-}1.3}
\newcommand{\hlLossInvBootSATflairTostCIHi}{0.1}
\newcommand{\hlLossInvBootSATflairMde}{1.5}
\newcommand{\hlLossInvBootSATflairPHolm}{0.142}
\newcommand{\hlLossInvBootSATflairN}{5}
\newcommand{\hlMitBootDropSATflair}{5.9}
\newcommand{\hlMitBootCleanSATflair}{51.7}
\newcommand{\hlLossDropBootSATflair}{5.9}
\newcommand{\hlLossCleanBootSATflair}{51.7}
\newcommand{\hlMitBootLVDflairEst}{0.6}
\newcommand{\hlMitBootLVDflairCILo}{\ensuremath{-}1.0}
\newcommand{\hlMitBootLVDflairCIHi}{2.1}
\newcommand{\hlLossInvBootLVDflairEst}{0.6}
\newcommand{\hlLossInvBootLVDflairCILo}{\ensuremath{-}1.0}
\newcommand{\hlLossInvBootLVDflairCIHi}{2.1}
\newcommand{\hlLossInvBootLVDflairTostCILo}{\ensuremath{-}0.6}
\newcommand{\hlLossInvBootLVDflairTostCIHi}{1.8}
\newcommand{\hlLossInvBootLVDflairMde}{2.6}
\newcommand{\hlLossInvBootLVDflairPHolm}{0.749}
\newcommand{\hlLossInvBootLVDflairN}{5}
\newcommand{\hlMitBootDropLVDflair}{4.2}
\newcommand{\hlMitBootCleanLVDflair}{51.3}
\newcommand{\hlLossDropBootLVDflair}{4.2}
\newcommand{\hlLossCleanBootLVDflair}{51.3}
\newcommand{\hlMitBootDOFAflairEst}{0.2}
\newcommand{\hlMitBootDOFAflairCILo}{\ensuremath{-}1.0}
\newcommand{\hlMitBootDOFAflairCIHi}{1.4}
\newcommand{\hlLossInvBootDOFAflairEst}{0.2}
\newcommand{\hlLossInvBootDOFAflairCILo}{\ensuremath{-}1.0}
\newcommand{\hlLossInvBootDOFAflairCIHi}{1.4}
\newcommand{\hlLossInvBootDOFAflairTostCILo}{\ensuremath{-}0.7}
\newcommand{\hlLossInvBootDOFAflairTostCIHi}{1.2}
\newcommand{\hlLossInvBootDOFAflairMde}{2.0}
\newcommand{\hlLossInvBootDOFAflairPHolm}{1.000}
\newcommand{\hlLossInvBootDOFAflairN}{5}
\newcommand{\hlMitBootDropDOFAflair}{4.6}
\newcommand{\hlMitBootCleanDOFAflair}{47.2}
\newcommand{\hlLossDropBootDOFAflair}{4.6}
\newcommand{\hlLossCleanBootDOFAflair}{47.2}
\newcommand{\hlMitBootTMflairEst}{0.4}
\newcommand{\hlMitBootTMflairCILo}{\ensuremath{-}1.1}
\newcommand{\hlMitBootTMflairCIHi}{2.0}
\newcommand{\hlLossInvBootTMflairEst}{0.4}
\newcommand{\hlLossInvBootTMflairCILo}{\ensuremath{-}1.1}
\newcommand{\hlLossInvBootTMflairCIHi}{2.0}
\newcommand{\hlLossInvBootTMflairTostCILo}{\ensuremath{-}0.8}
\newcommand{\hlLossInvBootTMflairTostCIHi}{1.6}
\newcommand{\hlLossInvBootTMflairMde}{2.6}
\newcommand{\hlLossInvBootTMflairPHolm}{0.977}
\newcommand{\hlLossInvBootTMflairN}{5}
\newcommand{\hlMitBootDropTMflair}{5.6}
\newcommand{\hlMitBootCleanTMflair}{40.8}
\newcommand{\hlLossDropBootTMflair}{5.6}
\newcommand{\hlLossCleanBootTMflair}{40.8}
\newcommand{\hlMitBootRNflairEst}{\ensuremath{-}0.3}
\newcommand{\hlMitBootRNflairCILo}{\ensuremath{-}2.8}
\newcommand{\hlMitBootRNflairCIHi}{2.3}
\newcommand{\hlLossInvBootRNflairEst}{\ensuremath{-}0.3}
\newcommand{\hlLossInvBootRNflairCILo}{\ensuremath{-}2.8}
\newcommand{\hlLossInvBootRNflairCIHi}{2.3}
\newcommand{\hlLossInvBootRNflairTostCILo}{\ensuremath{-}2.2}
\newcommand{\hlLossInvBootRNflairTostCIHi}{1.7}
\newcommand{\hlLossInvBootRNflairMde}{4.3}
\newcommand{\hlLossInvBootRNflairPHolm}{1.000}
\newcommand{\hlLossInvBootRNflairN}{5}
\newcommand{\hlMitBootDropRNflair}{3.9}
\newcommand{\hlMitBootCleanRNflair}{44.3}
\newcommand{\hlLossDropBootRNflair}{3.9}
\newcommand{\hlLossCleanBootRNflair}{44.3}
\newcommand{\hlLossDropBootflair}{4.8}
\newcommand{\hlLossCleanBootflair}{47.1}
\newcommand{\hlMitBootShiftflairEst}{0.1}
\newcommand{\hlMitBootShiftflairCILo}{\ensuremath{-}0.5}
\newcommand{\hlMitBootShiftflairCIHi}{0.7}
\newcommand{\hlMitBootCoarseflairEst}{0.1}
\newcommand{\hlMitBootCoarseflairCILo}{\ensuremath{-}0.5}
\newcommand{\hlMitBootCoarseflairCIHi}{0.8}
\newcommand{\hlMitBootBoundaryflairEst}{0.1}
\newcommand{\hlMitBootBoundaryflairCILo}{\ensuremath{-}0.6}
\newcommand{\hlMitBootBoundaryflairCIHi}{0.9}
\newcommand{\hlMitBootOmissionflairEst}{\ensuremath{-}0.1}
\newcommand{\hlMitBootOmissionflairCILo}{\ensuremath{-}0.7}
\newcommand{\hlMitBootOmissionflairCIHi}{0.6}
\newcommand{\hlMitBootCleanCostflairEst}{0.0}
\newcommand{\hlMitBootCleanCostflairCILo}{\ensuremath{-}0.5}
\newcommand{\hlMitBootCleanCostflairCIHi}{0.5}
\newcommand{\hlLossCleanInvBootflairEst}{0.0}
\newcommand{\hlLossCleanInvBootflairCILo}{\ensuremath{-}0.5}
\newcommand{\hlLossCleanInvBootflairCIHi}{0.5}
\newcommand{\hlLossCleanInvBootflairTostCILo}{\ensuremath{-}0.4}
\newcommand{\hlLossCleanInvBootflairTostCIHi}{0.4}
\newcommand{\hlLossCleanInvBootflairMde}{0.8}
\newcommand{\hlLossCleanInvBootflairPHolm}{0.889}
\newcommand{\hlLossCleanInvBootflairN}{25}
\newcommand{\hlMitVerdictBootflair}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlLossVerdictBootflair}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlExtMeanDropSATChes}{10.2}
\newcommand{\hlExtMeanDropLVDChes}{10.2}
\newcommand{\hlExtMeanDropDOFAChes}{12.0}
\newcommand{\hlExtMeanDropTMChes}{9.9}
\newcommand{\hlExtMeanDropRNChes}{8.7}
\newcommand{\hlExtMeanDropChes}{10.2}
\newcommand{\hlExtCleanChes}{81.6}
\newcommand{\hlExtTypeRankChesOne}{coarse}
\newcommand{\hlExtTypeRankChesTwo}{boundary}
\newcommand{\hlExtTypeRankChesThree}{omission}
\newcommand{\hlExtTypeRankChesFour}{shift}
\newcommand{\hlExtFOneChesEst}{\ensuremath{-}0.1}
\newcommand{\hlExtFOneChesCILo}{\ensuremath{-}2.1}
\newcommand{\hlExtFOneChesCIHi}{2.0}
\newcommand{\hlExtFOneChesTostCILo}{\ensuremath{-}1.6}
\newcommand{\hlExtFOneChesTostCIHi}{1.5}
\newcommand{\hlExtFOneChesMde}{3.4}
\newcommand{\hlExtFOneChesPHolm}{1.000}
\newcommand{\hlExtFOneChesN}{5}
\newcommand{\hlExtVerdictFOneChes}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlExtFTwoChesEst}{2.3}
\newcommand{\hlExtFTwoChesCILo}{1.2}
\newcommand{\hlExtFTwoChesCIHi}{3.4}
\newcommand{\hlExtFTwoChesTostCILo}{1.4}
\newcommand{\hlExtFTwoChesTostCIHi}{3.1}
\newcommand{\hlExtFTwoChesMde}{1.8}
\newcommand{\hlExtFTwoChesPHolm}{0.028}
\newcommand{\hlExtFTwoChesN}{5}
\newcommand{\hlExtVerdictFTwoChes}{\rn loses less}
\newcommand{\hlExtNSixChesEst}{\ensuremath{-}0.7}
\newcommand{\hlExtNSixChesCILo}{\ensuremath{-}1.9}
\newcommand{\hlExtNSixChesCIHi}{0.5}
\newcommand{\hlExtNSixChesTostCILo}{\ensuremath{-}1.6}
\newcommand{\hlExtNSixChesTostCIHi}{0.2}
\newcommand{\hlExtNSixChesMde}{2.0}
\newcommand{\hlExtNSixChesPHolm}{1.000}
\newcommand{\hlExtNSixChesN}{5}
\newcommand{\hlExtVerdictNSixChes}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlExtHFiveChesEst}{0.8}
\newcommand{\hlExtHFiveChesCILo}{\ensuremath{-}0.1}
\newcommand{\hlExtHFiveChesCIHi}{1.6}
\newcommand{\hlExtHFiveChesTostCILo}{0.1}
\newcommand{\hlExtHFiveChesTostCIHi}{1.4}
\newcommand{\hlExtHFiveChesMde}{1.3}
\newcommand{\hlExtHFiveChesPHolm}{0.365}
\newcommand{\hlExtHFiveChesN}{10}
\newcommand{\hlExtVerdictHFiveChes}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlExtFOneOneChesEst}{\ensuremath{-}0.6}
\newcommand{\hlExtFOneOneChesCILo}{\ensuremath{-}1.7}
\newcommand{\hlExtFOneOneChesCIHi}{0.6}
\newcommand{\hlExtFOneOneChesTostCILo}{\ensuremath{-}1.5}
\newcommand{\hlExtFOneOneChesTostCIHi}{0.3}
\newcommand{\hlExtFOneOneChesMde}{1.9}
\newcommand{\hlExtFOneOneChesPHolm}{1.000}
\newcommand{\hlExtFOneOneChesN}{5}
\newcommand{\hlExtHFiveSegfChesEst}{0.0}
\newcommand{\hlExtHFiveSegfChesCILo}{\ensuremath{-}0.9}
\newcommand{\hlExtHFiveSegfChesCIHi}{0.8}
\newcommand{\hlExtHFiveSegfChesTostCILo}{\ensuremath{-}0.7}
\newcommand{\hlExtHFiveSegfChesTostCIHi}{0.6}
\newcommand{\hlExtHFiveSegfChesMde}{1.3}
\newcommand{\hlExtHFiveSegfChesPHolm}{0.928}
\newcommand{\hlExtHFiveSegfChesN}{10}
\newcommand{\hlExtHFiveMtwoFChesEst}{2.2}
\newcommand{\hlExtHFiveMtwoFChesCILo}{0.6}
\newcommand{\hlExtHFiveMtwoFChesCIHi}{3.8}
\newcommand{\hlExtHFiveMtwoFChesTostCILo}{0.9}
\newcommand{\hlExtHFiveMtwoFChesTostCIHi}{3.5}
\newcommand{\hlExtHFiveMtwoFChesMde}{2.6}
\newcommand{\hlExtHFiveMtwoFChesPHolm}{0.013}
\newcommand{\hlExtHFiveMtwoFChesN}{10}
\newcommand{\hlExtHFiveSamChesEst}{0.1}
\newcommand{\hlExtHFiveSamChesCILo}{\ensuremath{-}0.9}
\newcommand{\hlExtHFiveSamChesCIHi}{1.2}
\newcommand{\hlExtHFiveSamChesTostCILo}{\ensuremath{-}0.7}
\newcommand{\hlExtHFiveSamChesTostCIHi}{1.0}
\newcommand{\hlExtHFiveSamChesMde}{1.7}
\newcommand{\hlExtHFiveSamChesPHolm}{0.819}
\newcommand{\hlExtHFiveSamChesN}{10}
\newcommand{\hlRealDropSATChes}{21.4}
\newcommand{\hlRealDropSATChesCILo}{20.3}
\newcommand{\hlRealDropSATChesCIHi}{22.5}
\newcommand{\hlRealDropLVDChes}{20.3}
\newcommand{\hlRealDropLVDChesCILo}{17.1}
\newcommand{\hlRealDropLVDChesCIHi}{23.4}
\newcommand{\hlRealDropDOFAChes}{22.3}
\newcommand{\hlRealDropDOFAChesCILo}{20.9}
\newcommand{\hlRealDropDOFAChesCIHi}{23.6}
\newcommand{\hlRealDropTMChes}{20.0}
\newcommand{\hlRealDropTMChesCILo}{19.3}
\newcommand{\hlRealDropTMChesCIHi}{20.6}
\newcommand{\hlRealDropRNChes}{22.9}
\newcommand{\hlRealDropRNChesCILo}{17.9}
\newcommand{\hlRealDropRNChesCIHi}{27.8}
\newcommand{\hlRealDropChes}{21.4}
\newcommand{\hlRealDropChesCILo}{20.4}
\newcommand{\hlRealDropChesCIHi}{22.3}
\newcommand{\hlRealDropChesN}{25}
\newcommand{\hlRealMatchedDropChes}{12.1}
\newcommand{\hlRealVsSynthChes}{9.2}
\newcommand{\hlRealVsSynthChesEst}{9.2}
\newcommand{\hlRealVsSynthChesCILo}{8.5}
\newcommand{\hlRealVsSynthChesCIHi}{10.0}
\newcommand{\hlRealVsSynthChesTostCILo}{8.6}
\newcommand{\hlRealVsSynthChesTostCIHi}{9.9}
\newcommand{\hlRealVsSynthChesMde}{1.2}
\newcommand{\hlRealVsSynthChesPHolm}{\ensuremath{<}0.001}
\newcommand{\hlRealVsSynthChesN}{25}
\newcommand{\hlRealVerdictChes}{Real costs more}
\newcommand{\hlRealMatchedTypeChes}{coarse}
\newcommand{\hlRealMatchedLevelChes}{\Ltwo}
\newcommand{\hlRealBaselineChes}{clean run on the full training subset}
\newcommand{\hlExtMeanDropSATCsTwelve}{5.9}
\newcommand{\hlExtMeanDropLVDCsTwelve}{6.4}
\newcommand{\hlExtMeanDropDOFACsTwelve}{7.2}
\newcommand{\hlExtMeanDropTMCsTwelve}{7.2}
\newcommand{\hlExtMeanDropRNCsTwelve}{6.8}
\newcommand{\hlExtMeanDropCsTwelve}{6.7}
\newcommand{\hlExtCleanCsTwelve}{67.1}
\newcommand{\hlExtTypeRankCsTwelveOne}{coarse}
\newcommand{\hlExtTypeRankCsTwelveTwo}{omission}
\newcommand{\hlExtTypeRankCsTwelveThree}{boundary}
\newcommand{\hlExtTypeRankCsTwelveFour}{shift}
\newcommand{\hlExtFOneCsTwelveEst}{\ensuremath{-}0.5}
\newcommand{\hlExtFOneCsTwelveCILo}{\ensuremath{-}2.6}
\newcommand{\hlExtFOneCsTwelveCIHi}{1.5}
\newcommand{\hlExtFOneCsTwelveTostCILo}{\ensuremath{-}2.1}
\newcommand{\hlExtFOneCsTwelveTostCIHi}{1.1}
\newcommand{\hlExtFOneCsTwelveMde}{3.4}
\newcommand{\hlExtFOneCsTwelvePHolm}{1.000}
\newcommand{\hlExtFOneCsTwelveN}{5}
\newcommand{\hlExtVerdictFOneCsTwelve}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlExtFTwoCsTwelveEst}{0.4}
\newcommand{\hlExtFTwoCsTwelveCILo}{\ensuremath{-}0.9}
\newcommand{\hlExtFTwoCsTwelveCIHi}{1.8}
\newcommand{\hlExtFTwoCsTwelveTostCILo}{\ensuremath{-}0.6}
\newcommand{\hlExtFTwoCsTwelveTostCIHi}{1.5}
\newcommand{\hlExtFTwoCsTwelveMde}{2.2}
\newcommand{\hlExtFTwoCsTwelvePHolm}{0.425}
\newcommand{\hlExtFTwoCsTwelveN}{5}
\newcommand{\hlExtVerdictFTwoCsTwelve}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlExtNSixCsTwelveEst}{0.3}
\newcommand{\hlExtNSixCsTwelveCILo}{\ensuremath{-}0.9}
\newcommand{\hlExtNSixCsTwelveCIHi}{1.6}
\newcommand{\hlExtNSixCsTwelveTostCILo}{\ensuremath{-}0.6}
\newcommand{\hlExtNSixCsTwelveTostCIHi}{1.3}
\newcommand{\hlExtNSixCsTwelveMde}{2.0}
\newcommand{\hlExtNSixCsTwelvePHolm}{1.000}
\newcommand{\hlExtNSixCsTwelveN}{5}
\newcommand{\hlExtVerdictNSixCsTwelve}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlExtHFiveCsTwelveEst}{0.3}
\newcommand{\hlExtHFiveCsTwelveCILo}{\ensuremath{-}0.4}
\newcommand{\hlExtHFiveCsTwelveCIHi}{0.9}
\newcommand{\hlExtHFiveCsTwelveTostCILo}{\ensuremath{-}0.2}
\newcommand{\hlExtHFiveCsTwelveTostCIHi}{0.8}
\newcommand{\hlExtHFiveCsTwelveMde}{1.0}
\newcommand{\hlExtHFiveCsTwelvePHolm}{1.000}
\newcommand{\hlExtHFiveCsTwelveN}{10}
\newcommand{\hlExtVerdictHFiveCsTwelve}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlExtFOneOneCsTwelveEst}{0.0}
\newcommand{\hlExtFOneOneCsTwelveCILo}{\ensuremath{-}1.1}
\newcommand{\hlExtFOneOneCsTwelveCIHi}{1.1}
\newcommand{\hlExtFOneOneCsTwelveTostCILo}{\ensuremath{-}0.8}
\newcommand{\hlExtFOneOneCsTwelveTostCIHi}{0.9}
\newcommand{\hlExtFOneOneCsTwelveMde}{1.8}
\newcommand{\hlExtFOneOneCsTwelvePHolm}{1.000}
\newcommand{\hlExtFOneOneCsTwelveN}{5}
\newcommand{\hlExtHFiveSegfCsTwelveEst}{\ensuremath{-}0.1}
\newcommand{\hlExtHFiveSegfCsTwelveCILo}{\ensuremath{-}1.0}
\newcommand{\hlExtHFiveSegfCsTwelveCIHi}{0.8}
\newcommand{\hlExtHFiveSegfCsTwelveTostCILo}{\ensuremath{-}0.8}
\newcommand{\hlExtHFiveSegfCsTwelveTostCIHi}{0.7}
\newcommand{\hlExtHFiveSegfCsTwelveMde}{1.5}
\newcommand{\hlExtHFiveSegfCsTwelvePHolm}{0.832}
\newcommand{\hlExtHFiveSegfCsTwelveN}{10}
\newcommand{\hlExtHFiveMtwoFCsTwelveEst}{0.3}
\newcommand{\hlExtHFiveMtwoFCsTwelveCILo}{\ensuremath{-}0.6}
\newcommand{\hlExtHFiveMtwoFCsTwelveCIHi}{1.2}
\newcommand{\hlExtHFiveMtwoFCsTwelveTostCILo}{\ensuremath{-}0.4}
\newcommand{\hlExtHFiveMtwoFCsTwelveTostCIHi}{1.1}
\newcommand{\hlExtHFiveMtwoFCsTwelveMde}{1.4}
\newcommand{\hlExtHFiveMtwoFCsTwelvePHolm}{0.423}
\newcommand{\hlExtHFiveMtwoFCsTwelveN}{10}
\newcommand{\hlExtHFiveSamCsTwelveEst}{0.6}
\newcommand{\hlExtHFiveSamCsTwelveCILo}{\ensuremath{-}0.5}
\newcommand{\hlExtHFiveSamCsTwelveCIHi}{1.7}
\newcommand{\hlExtHFiveSamCsTwelveTostCILo}{\ensuremath{-}0.3}
\newcommand{\hlExtHFiveSamCsTwelveTostCIHi}{1.5}
\newcommand{\hlExtHFiveSamCsTwelveMde}{1.8}
\newcommand{\hlExtHFiveSamCsTwelvePHolm}{0.272}
\newcommand{\hlExtHFiveSamCsTwelveN}{10}
\newcommand{\hlRealDropSATCsTwelve}{32.2}
\newcommand{\hlRealDropSATCsTwelveCILo}{30.6}
\newcommand{\hlRealDropSATCsTwelveCIHi}{33.9}
\newcommand{\hlRealDropLVDCsTwelve}{34.5}
\newcommand{\hlRealDropLVDCsTwelveCILo}{33.5}
\newcommand{\hlRealDropLVDCsTwelveCIHi}{35.5}
\newcommand{\hlRealDropDOFACsTwelve}{31.4}
\newcommand{\hlRealDropDOFACsTwelveCILo}{30.2}
\newcommand{\hlRealDropDOFACsTwelveCIHi}{32.6}
\newcommand{\hlRealDropTMCsTwelve}{34.7}
\newcommand{\hlRealDropTMCsTwelveCILo}{34.1}
\newcommand{\hlRealDropTMCsTwelveCIHi}{35.3}
\newcommand{\hlRealDropRNCsTwelve}{29.1}
\newcommand{\hlRealDropRNCsTwelveCILo}{28.2}
\newcommand{\hlRealDropRNCsTwelveCIHi}{30.0}
\newcommand{\hlRealDropCsTwelve}{32.4}
\newcommand{\hlRealDropCsTwelveCILo}{31.4}
\newcommand{\hlRealDropCsTwelveCIHi}{33.3}
\newcommand{\hlRealDropCsTwelveN}{25}
\newcommand{\hlRealMatchedDropCsTwelve}{7.8}
\newcommand{\hlRealVsSynthCsTwelve}{24.6}
\newcommand{\hlRealVsSynthCsTwelveEst}{24.6}
\newcommand{\hlRealVsSynthCsTwelveCILo}{23.6}
\newcommand{\hlRealVsSynthCsTwelveCIHi}{25.5}
\newcommand{\hlRealVsSynthCsTwelveTostCILo}{23.8}
\newcommand{\hlRealVsSynthCsTwelveTostCIHi}{25.3}
\newcommand{\hlRealVsSynthCsTwelveMde}{1.5}
\newcommand{\hlRealVsSynthCsTwelvePHolm}{\ensuremath{<}0.001}
\newcommand{\hlRealVsSynthCsTwelveN}{25}
\newcommand{\hlRealVerdictCsTwelve}{Real costs more}
\newcommand{\hlRealMatchedTypeCsTwelve}{coarse}
\newcommand{\hlRealMatchedLevelCsTwelve}{\Ltwo}
\newcommand{\hlRealBaselineCsTwelve}{clean run on the full training subset}
\newcommand{\hlExtMeanDropSATDfc}{2.9}
\newcommand{\hlExtMeanDropLVDDfc}{2.5}
\newcommand{\hlExtMeanDropDOFADfc}{1.4}
\newcommand{\hlExtMeanDropTMDfc}{3.4}
\newcommand{\hlExtMeanDropRNDfc}{1.2}
\newcommand{\hlExtMeanDropDfc}{2.3}
\newcommand{\hlExtCleanDfc}{39.6}
\newcommand{\hlExtTypeRankDfcOne}{boundary}
\newcommand{\hlExtTypeRankDfcTwo}{omission}
\newcommand{\hlExtTypeRankDfcThree}{coarse}
\newcommand{\hlExtTypeRankDfcFour}{shift}
\newcommand{\hlExtFOneDfcEst}{0.4}
\newcommand{\hlExtFOneDfcCILo}{\ensuremath{-}0.7}
\newcommand{\hlExtFOneDfcCIHi}{1.6}
\newcommand{\hlExtFOneDfcTostCILo}{\ensuremath{-}0.5}
\newcommand{\hlExtFOneDfcTostCIHi}{1.3}
\newcommand{\hlExtFOneDfcMde}{1.9}
\newcommand{\hlExtFOneDfcPHolm}{1.000}
\newcommand{\hlExtFOneDfcN}{5}
\newcommand{\hlExtVerdictFOneDfc}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlExtFTwoDfcEst}{1.2}
\newcommand{\hlExtFTwoDfcCILo}{\ensuremath{-}0.5}
\newcommand{\hlExtFTwoDfcCIHi}{3.0}
\newcommand{\hlExtFTwoDfcTostCILo}{\ensuremath{-}0.1}
\newcommand{\hlExtFTwoDfcTostCIHi}{2.6}
\newcommand{\hlExtFTwoDfcMde}{2.8}
\newcommand{\hlExtFTwoDfcPHolm}{0.283}
\newcommand{\hlExtFTwoDfcN}{5}
\newcommand{\hlExtVerdictFTwoDfc}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlExtNSixDfcEst}{0.5}
\newcommand{\hlExtNSixDfcCILo}{\ensuremath{-}1.7}
\newcommand{\hlExtNSixDfcCIHi}{2.7}
\newcommand{\hlExtNSixDfcTostCILo}{\ensuremath{-}1.2}
\newcommand{\hlExtNSixDfcTostCIHi}{2.2}
\newcommand{\hlExtNSixDfcMde}{3.6}
\newcommand{\hlExtNSixDfcPHolm}{1.000}
\newcommand{\hlExtNSixDfcN}{5}
\newcommand{\hlExtVerdictNSixDfc}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlExtHFiveDfcEst}{\ensuremath{-}0.1}
\newcommand{\hlExtHFiveDfcCILo}{\ensuremath{-}0.9}
\newcommand{\hlExtHFiveDfcCIHi}{0.7}
\newcommand{\hlExtHFiveDfcTostCILo}{\ensuremath{-}0.8}
\newcommand{\hlExtHFiveDfcTostCIHi}{0.6}
\newcommand{\hlExtHFiveDfcMde}{1.3}
\newcommand{\hlExtHFiveDfcPHolm}{1.000}
\newcommand{\hlExtHFiveDfcN}{10}
\newcommand{\hlExtVerdictHFiveDfc}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlExtFOneOneDfcEst}{0.9}
\newcommand{\hlExtFOneOneDfcCILo}{\ensuremath{-}2.7}
\newcommand{\hlExtFOneOneDfcCIHi}{4.5}
\newcommand{\hlExtFOneOneDfcTostCILo}{\ensuremath{-}1.8}
\newcommand{\hlExtFOneOneDfcTostCIHi}{3.7}
\newcommand{\hlExtFOneOneDfcMde}{5.9}
\newcommand{\hlExtFOneOneDfcPHolm}{1.000}
\newcommand{\hlExtFOneOneDfcN}{5}
\newcommand{\hlExtHFiveSegfDfcEst}{\ensuremath{-}0.1}
\newcommand{\hlExtHFiveSegfDfcCILo}{\ensuremath{-}1.3}
\newcommand{\hlExtHFiveSegfDfcCIHi}{1.1}
\newcommand{\hlExtHFiveSegfDfcTostCILo}{\ensuremath{-}1.1}
\newcommand{\hlExtHFiveSegfDfcTostCIHi}{0.9}
\newcommand{\hlExtHFiveSegfDfcMde}{1.9}
\newcommand{\hlExtHFiveSegfDfcPHolm}{0.855}
\newcommand{\hlExtHFiveSegfDfcN}{10}
\newcommand{\hlExtHFiveMtwoFDfcEst}{0.3}
\newcommand{\hlExtHFiveMtwoFDfcCILo}{\ensuremath{-}0.8}
\newcommand{\hlExtHFiveMtwoFDfcCIHi}{1.4}
\newcommand{\hlExtHFiveMtwoFDfcTostCILo}{\ensuremath{-}0.6}
\newcommand{\hlExtHFiveMtwoFDfcTostCIHi}{1.2}
\newcommand{\hlExtHFiveMtwoFDfcMde}{1.7}
\newcommand{\hlExtHFiveMtwoFDfcPHolm}{0.557}
\newcommand{\hlExtHFiveMtwoFDfcN}{10}
\newcommand{\hlExtHFiveSamDfcEst}{\ensuremath{-}0.5}
\newcommand{\hlExtHFiveSamDfcCILo}{\ensuremath{-}1.7}
\newcommand{\hlExtHFiveSamDfcCIHi}{0.7}
\newcommand{\hlExtHFiveSamDfcTostCILo}{\ensuremath{-}1.4}
\newcommand{\hlExtHFiveSamDfcTostCIHi}{0.4}
\newcommand{\hlExtHFiveSamDfcMde}{1.9}
\newcommand{\hlExtHFiveSamDfcPHolm}{0.361}
\newcommand{\hlExtHFiveSamDfcN}{10}
\newcommand{\hlRealDropSATDfc}{7.4}
\newcommand{\hlRealDropSATDfcCILo}{4.0}
\newcommand{\hlRealDropSATDfcCIHi}{10.9}
\newcommand{\hlRealDropLVDDfc}{6.1}
\newcommand{\hlRealDropLVDDfcCILo}{4.2}
\newcommand{\hlRealDropLVDDfcCIHi}{8.1}
\newcommand{\hlRealDropDOFADfc}{3.1}
\newcommand{\hlRealDropDOFADfcCILo}{1.3}
\newcommand{\hlRealDropDOFADfcCIHi}{5.0}
\newcommand{\hlRealDropTMDfc}{2.7}
\newcommand{\hlRealDropTMDfcCILo}{1.6}
\newcommand{\hlRealDropTMDfcCIHi}{3.9}
\newcommand{\hlRealDropRNDfc}{4.5}
\newcommand{\hlRealDropRNDfcCILo}{2.9}
\newcommand{\hlRealDropRNDfcCIHi}{6.1}
\newcommand{\hlRealDropDfc}{4.8}
\newcommand{\hlRealDropDfcCILo}{3.8}
\newcommand{\hlRealDropDfcCIHi}{5.8}
\newcommand{\hlRealDropDfcN}{25}
\newcommand{\hlRealMatchedDropDfc}{1.4}
\newcommand{\hlRealVsSynthDfc}{3.4}
\newcommand{\hlRealVsSynthDfcEst}{3.4}
\newcommand{\hlRealVsSynthDfcCILo}{2.2}
\newcommand{\hlRealVsSynthDfcCIHi}{4.6}
\newcommand{\hlRealVsSynthDfcTostCILo}{2.4}
\newcommand{\hlRealVsSynthDfcTostCIHi}{4.4}
\newcommand{\hlRealVsSynthDfcMde}{1.9}
\newcommand{\hlRealVsSynthDfcPHolm}{\ensuremath{<}0.001}
\newcommand{\hlRealVsSynthDfcN}{25}
\newcommand{\hlRealVerdictDfc}{Real costs more}
\newcommand{\hlRealMatchedTypeDfc}{coarse}
\newcommand{\hlRealMatchedLevelDfc}{\Ltwo}
\newcommand{\hlRealBaselineDfc}{clean run on the tiles the real labels cover}
\newcommand{\hlExtMeanDropSATEnva}{6.3}
\newcommand{\hlExtMeanDropLVDEnva}{7.7}
\newcommand{\hlExtMeanDropDOFAEnva}{5.4}
\newcommand{\hlExtMeanDropTMEnva}{6.9}
\newcommand{\hlExtMeanDropRNEnva}{12.1}
\newcommand{\hlExtMeanDropEnva}{7.7}
\newcommand{\hlExtCleanEnva}{54.2}
\newcommand{\hlExtTypeRankEnvaOne}{omission}
\newcommand{\hlExtTypeRankEnvaTwo}{boundary}
\newcommand{\hlExtTypeRankEnvaThree}{coarse}
\newcommand{\hlExtTypeRankEnvaFour}{shift}
\newcommand{\hlExtFOneEnvaEst}{\ensuremath{-}1.5}
\newcommand{\hlExtFOneEnvaCILo}{\ensuremath{-}4.5}
\newcommand{\hlExtFOneEnvaCIHi}{1.6}
\newcommand{\hlExtFOneEnvaTostCILo}{\ensuremath{-}3.8}
\newcommand{\hlExtFOneEnvaTostCIHi}{0.9}
\newcommand{\hlExtFOneEnvaMde}{5.1}
\newcommand{\hlExtFOneEnvaPHolm}{1.000}
\newcommand{\hlExtFOneEnvaN}{5}
\newcommand{\hlExtVerdictFOneEnva}{Undetermined, MDE 5.1}
\newcommand{\hlExtFTwoEnvaEst}{\ensuremath{-}5.9}
\newcommand{\hlExtFTwoEnvaCILo}{\ensuremath{-}8.5}
\newcommand{\hlExtFTwoEnvaCIHi}{\ensuremath{-}3.3}
\newcommand{\hlExtFTwoEnvaTostCILo}{\ensuremath{-}7.9}
\newcommand{\hlExtFTwoEnvaTostCIHi}{\ensuremath{-}3.9}
\newcommand{\hlExtFTwoEnvaMde}{4.3}
\newcommand{\hlExtFTwoEnvaPHolm}{0.022}
\newcommand{\hlExtFTwoEnvaN}{5}
\newcommand{\hlExtVerdictFTwoEnva}{\dofa and \tm lose less}
\newcommand{\hlExtNSixEnvaEst}{\ensuremath{-}1.5}
\newcommand{\hlExtNSixEnvaCILo}{\ensuremath{-}4.7}
\newcommand{\hlExtNSixEnvaCIHi}{1.8}
\newcommand{\hlExtNSixEnvaTostCILo}{\ensuremath{-}4.0}
\newcommand{\hlExtNSixEnvaTostCIHi}{1.0}
\newcommand{\hlExtNSixEnvaMde}{5.4}
\newcommand{\hlExtNSixEnvaPHolm}{1.000}
\newcommand{\hlExtNSixEnvaN}{5}
\newcommand{\hlExtVerdictNSixEnva}{Undetermined, MDE 5.4}
\newcommand{\hlExtHFiveEnvaEst}{\ensuremath{-}3.3}
\newcommand{\hlExtHFiveEnvaCILo}{\ensuremath{-}5.0}
\newcommand{\hlExtHFiveEnvaCIHi}{\ensuremath{-}1.7}
\newcommand{\hlExtHFiveEnvaTostCILo}{\ensuremath{-}4.7}
\newcommand{\hlExtHFiveEnvaTostCIHi}{\ensuremath{-}2.0}
\newcommand{\hlExtHFiveEnvaMde}{2.6}
\newcommand{\hlExtHFiveEnvaPHolm}{0.008}
\newcommand{\hlExtHFiveEnvaN}{10}
\newcommand{\hlExtVerdictHFiveEnva}{the other heads lose less}
\newcommand{\hlExtFOneOneEnvaEst}{2.4}
\newcommand{\hlExtFOneOneEnvaCILo}{\ensuremath{-}1.2}
\newcommand{\hlExtFOneOneEnvaCIHi}{5.9}
\newcommand{\hlExtFOneOneEnvaTostCILo}{\ensuremath{-}0.4}
\newcommand{\hlExtFOneOneEnvaTostCIHi}{5.1}
\newcommand{\hlExtFOneOneEnvaMde}{5.9}
\newcommand{\hlExtFOneOneEnvaPHolm}{0.970}
\newcommand{\hlExtFOneOneEnvaN}{5}
\newcommand{\hlExtHFiveSegfEnvaEst}{\ensuremath{-}3.0}
\newcommand{\hlExtHFiveSegfEnvaCILo}{\ensuremath{-}5.1}
\newcommand{\hlExtHFiveSegfEnvaCIHi}{\ensuremath{-}1.0}
\newcommand{\hlExtHFiveSegfEnvaTostCILo}{\ensuremath{-}4.7}
\newcommand{\hlExtHFiveSegfEnvaTostCIHi}{\ensuremath{-}1.3}
\newcommand{\hlExtHFiveSegfEnvaMde}{3.3}
\newcommand{\hlExtHFiveSegfEnvaPHolm}{0.009}
\newcommand{\hlExtHFiveSegfEnvaN}{10}
\newcommand{\hlExtHFiveMtwoFEnvaEst}{\ensuremath{-}2.3}
\newcommand{\hlExtHFiveMtwoFEnvaCILo}{\ensuremath{-}5.2}
\newcommand{\hlExtHFiveMtwoFEnvaCIHi}{0.5}
\newcommand{\hlExtHFiveMtwoFEnvaTostCILo}{\ensuremath{-}4.7}
\newcommand{\hlExtHFiveMtwoFEnvaTostCIHi}{0.0}
\newcommand{\hlExtHFiveMtwoFEnvaMde}{4.6}
\newcommand{\hlExtHFiveMtwoFEnvaPHolm}{0.098}
\newcommand{\hlExtHFiveMtwoFEnvaN}{10}
\newcommand{\hlExtHFiveSamEnvaEst}{\ensuremath{-}4.7}
\newcommand{\hlExtHFiveSamEnvaCILo}{\ensuremath{-}6.5}
\newcommand{\hlExtHFiveSamEnvaCIHi}{\ensuremath{-}2.8}
\newcommand{\hlExtHFiveSamEnvaTostCILo}{\ensuremath{-}6.2}
\newcommand{\hlExtHFiveSamEnvaTostCIHi}{\ensuremath{-}3.2}
\newcommand{\hlExtHFiveSamEnvaMde}{3.0}
\newcommand{\hlExtHFiveSamEnvaPHolm}{\ensuremath{<}0.001}
\newcommand{\hlExtHFiveSamEnvaN}{10}
\newcommand{\hlRealDropSATEnva}{21.8}
\newcommand{\hlRealDropSATEnvaCILo}{19.1}
\newcommand{\hlRealDropSATEnvaCIHi}{24.5}
\newcommand{\hlRealDropLVDEnva}{30.0}
\newcommand{\hlRealDropLVDEnvaCILo}{23.5}
\newcommand{\hlRealDropLVDEnvaCIHi}{36.5}
\newcommand{\hlRealDropDOFAEnva}{20.7}
\newcommand{\hlRealDropDOFAEnvaCILo}{16.6}
\newcommand{\hlRealDropDOFAEnvaCIHi}{24.9}
\newcommand{\hlRealDropTMEnva}{26.1}
\newcommand{\hlRealDropTMEnvaCILo}{22.9}
\newcommand{\hlRealDropTMEnvaCIHi}{29.3}
\newcommand{\hlRealDropRNEnva}{24.4}
\newcommand{\hlRealDropRNEnvaCILo}{17.4}
\newcommand{\hlRealDropRNEnvaCIHi}{31.4}
\newcommand{\hlRealDropEnva}{24.6}
\newcommand{\hlRealDropEnvaCILo}{22.6}
\newcommand{\hlRealDropEnvaCIHi}{26.7}
\newcommand{\hlRealDropEnvaN}{25}
\newcommand{\hlRealMatchedDropEnva}{3.2}
\newcommand{\hlRealVsSynthEnva}{21.4}
\newcommand{\hlRealVsSynthEnvaEst}{21.4}
\newcommand{\hlRealVsSynthEnvaCILo}{19.1}
\newcommand{\hlRealVsSynthEnvaCIHi}{23.7}
\newcommand{\hlRealVsSynthEnvaTostCILo}{19.5}
\newcommand{\hlRealVsSynthEnvaTostCIHi}{23.3}
\newcommand{\hlRealVsSynthEnvaMde}{3.6}
\newcommand{\hlRealVsSynthEnvaPHolm}{\ensuremath{<}0.001}
\newcommand{\hlRealVsSynthEnvaN}{25}
\newcommand{\hlRealVerdictEnva}{Real costs more}
\newcommand{\hlRealMatchedTypeEnva}{coarse}
\newcommand{\hlRealMatchedLevelEnva}{\Ltwo}
\newcommand{\hlRealBaselineEnva}{clean run on the full training subset}
\newcommand{\hlExtMeanDropSATSnTwo}{11.4}
\newcommand{\hlExtMeanDropLVDSnTwo}{10.4}
\newcommand{\hlExtMeanDropDOFASnTwo}{11.8}
\newcommand{\hlExtMeanDropTMSnTwo}{11.7}
\newcommand{\hlExtMeanDropRNSnTwo}{13.8}
\newcommand{\hlExtMeanDropSnTwo}{11.8}
\newcommand{\hlExtCleanSnTwo}{84.2}
\newcommand{\hlExtTypeRankSnTwoOne}{omission}
\newcommand{\hlExtTypeRankSnTwoTwo}{coarse}
\newcommand{\hlExtTypeRankSnTwoThree}{boundary}
\newcommand{\hlExtTypeRankSnTwoFour}{shift}
\newcommand{\hlExtFOneSnTwoEst}{1.1}
\newcommand{\hlExtFOneSnTwoCILo}{0.5}
\newcommand{\hlExtFOneSnTwoCIHi}{1.6}
\newcommand{\hlExtFOneSnTwoTostCILo}{0.7}
\newcommand{\hlExtFOneSnTwoTostCIHi}{1.5}
\newcommand{\hlExtFOneSnTwoMde}{0.9}
\newcommand{\hlExtFOneSnTwoPHolm}{0.034}
\newcommand{\hlExtFOneSnTwoN}{5}
\newcommand{\hlExtVerdictFOneSnTwo}{Equivalent within $\pm$\TostMargin, \lvd loses less}
\newcommand{\hlExtFTwoSnTwoEst}{\ensuremath{-}2.1}
\newcommand{\hlExtFTwoSnTwoCILo}{\ensuremath{-}4.0}
\newcommand{\hlExtFTwoSnTwoCIHi}{\ensuremath{-}0.2}
\newcommand{\hlExtFTwoSnTwoTostCILo}{\ensuremath{-}3.6}
\newcommand{\hlExtFTwoSnTwoTostCIHi}{\ensuremath{-}0.6}
\newcommand{\hlExtFTwoSnTwoMde}{3.2}
\newcommand{\hlExtFTwoSnTwoPHolm}{0.157}
\newcommand{\hlExtFTwoSnTwoN}{5}
\newcommand{\hlExtVerdictFTwoSnTwo}{\dofa and \tm lose less}
\newcommand{\hlExtNSixSnTwoEst}{0.1}
\newcommand{\hlExtNSixSnTwoCILo}{\ensuremath{-}1.4}
\newcommand{\hlExtNSixSnTwoCIHi}{1.6}
\newcommand{\hlExtNSixSnTwoTostCILo}{\ensuremath{-}1.1}
\newcommand{\hlExtNSixSnTwoTostCIHi}{1.3}
\newcommand{\hlExtNSixSnTwoMde}{2.5}
\newcommand{\hlExtNSixSnTwoPHolm}{1.000}
\newcommand{\hlExtNSixSnTwoN}{5}
\newcommand{\hlExtVerdictNSixSnTwo}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlExtHFiveSnTwoEst}{2.9}
\newcommand{\hlExtHFiveSnTwoCILo}{2.2}
\newcommand{\hlExtHFiveSnTwoCIHi}{3.6}
\newcommand{\hlExtHFiveSnTwoTostCILo}{2.3}
\newcommand{\hlExtHFiveSnTwoTostCIHi}{3.4}
\newcommand{\hlExtHFiveSnTwoMde}{1.1}
\newcommand{\hlExtHFiveSnTwoPHolm}{\ensuremath{<}0.001}
\newcommand{\hlExtHFiveSnTwoN}{10}
\newcommand{\hlExtVerdictHFiveSnTwo}{the other heads lose more}
\newcommand{\hlExtFOneOneSnTwoEst}{\ensuremath{-}0.7}
\newcommand{\hlExtFOneOneSnTwoCILo}{\ensuremath{-}3.0}
\newcommand{\hlExtFOneOneSnTwoCIHi}{1.6}
\newcommand{\hlExtFOneOneSnTwoTostCILo}{\ensuremath{-}2.5}
\newcommand{\hlExtFOneOneSnTwoTostCIHi}{1.1}
\newcommand{\hlExtFOneOneSnTwoMde}{3.8}
\newcommand{\hlExtFOneOneSnTwoPHolm}{1.000}
\newcommand{\hlExtFOneOneSnTwoN}{5}
\newcommand{\hlExtHFiveSegfSnTwoEst}{0.4}
\newcommand{\hlExtHFiveSegfSnTwoCILo}{\ensuremath{-}0.7}
\newcommand{\hlExtHFiveSegfSnTwoCIHi}{1.5}
\newcommand{\hlExtHFiveSegfSnTwoTostCILo}{\ensuremath{-}0.5}
\newcommand{\hlExtHFiveSegfSnTwoTostCIHi}{1.3}
\newcommand{\hlExtHFiveSegfSnTwoMde}{1.7}
\newcommand{\hlExtHFiveSegfSnTwoPHolm}{0.436}
\newcommand{\hlExtHFiveSegfSnTwoN}{10}
\newcommand{\hlExtHFiveMtwoFSnTwoEst}{5.5}
\newcommand{\hlExtHFiveMtwoFSnTwoCILo}{2.9}
\newcommand{\hlExtHFiveMtwoFSnTwoCIHi}{8.1}
\newcommand{\hlExtHFiveMtwoFSnTwoTostCILo}{3.4}
\newcommand{\hlExtHFiveMtwoFSnTwoTostCIHi}{7.6}
\newcommand{\hlExtHFiveMtwoFSnTwoMde}{4.2}
\newcommand{\hlExtHFiveMtwoFSnTwoPHolm}{0.001}
\newcommand{\hlExtHFiveMtwoFSnTwoN}{10}
\newcommand{\hlExtHFiveSamSnTwoEst}{2.7}
\newcommand{\hlExtHFiveSamSnTwoCILo}{1.3}
\newcommand{\hlExtHFiveSamSnTwoCIHi}{4.1}
\newcommand{\hlExtHFiveSamSnTwoTostCILo}{1.6}
\newcommand{\hlExtHFiveSamSnTwoTostCIHi}{3.9}
\newcommand{\hlExtHFiveSamSnTwoMde}{2.2}
\newcommand{\hlExtHFiveSamSnTwoPHolm}{0.002}
\newcommand{\hlExtHFiveSamSnTwoN}{10}
\newcommand{\hlExtMeanDropSATKuro}{6.5}
\newcommand{\hlExtMeanDropLVDKuro}{7.4}
\newcommand{\hlExtMeanDropDOFAKuro}{5.1}
\newcommand{\hlExtMeanDropTMKuro}{7.7}
\newcommand{\hlExtMeanDropRNKuro}{0.5}
\newcommand{\hlExtMeanDropKuro}{5.5}
\newcommand{\hlExtCleanKuro}{51.4}
\newcommand{\hlExtTypeRankKuroOne}{omission}
\newcommand{\hlExtTypeRankKuroTwo}{coarse}
\newcommand{\hlExtTypeRankKuroThree}{boundary}
\newcommand{\hlExtTypeRankKuroFour}{shift}
\newcommand{\hlExtFOneKuroEst}{\ensuremath{-}0.9}
\newcommand{\hlExtFOneKuroCILo}{\ensuremath{-}4.3}
\newcommand{\hlExtFOneKuroCIHi}{2.4}
\newcommand{\hlExtFOneKuroTostCILo}{\ensuremath{-}3.5}
\newcommand{\hlExtFOneKuroTostCIHi}{1.6}
\newcommand{\hlExtFOneKuroMde}{5.5}
\newcommand{\hlExtFOneKuroPHolm}{1.000}
\newcommand{\hlExtFOneKuroN}{5}
\newcommand{\hlExtVerdictFOneKuro}{Undetermined, MDE 5.5}
\newcommand{\hlExtFTwoKuroEst}{5.9}
\newcommand{\hlExtFTwoKuroCILo}{1.1}
\newcommand{\hlExtFTwoKuroCIHi}{10.7}
\newcommand{\hlExtFTwoKuroTostCILo}{2.2}
\newcommand{\hlExtFTwoKuroTostCIHi}{9.6}
\newcommand{\hlExtFTwoKuroMde}{8.0}
\newcommand{\hlExtFTwoKuroPHolm}{0.138}
\newcommand{\hlExtFTwoKuroN}{5}
\newcommand{\hlExtVerdictFTwoKuro}{\rn loses less}
\newcommand{\hlExtNSixKuroEst}{\ensuremath{-}1.3}
\newcommand{\hlExtNSixKuroCILo}{\ensuremath{-}3.5}
\newcommand{\hlExtNSixKuroCIHi}{0.8}
\newcommand{\hlExtNSixKuroTostCILo}{\ensuremath{-}3.0}
\newcommand{\hlExtNSixKuroTostCIHi}{0.3}
\newcommand{\hlExtNSixKuroMde}{3.6}
\newcommand{\hlExtNSixKuroPHolm}{1.000}
\newcommand{\hlExtNSixKuroN}{5}
\newcommand{\hlExtVerdictNSixKuro}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlExtHFiveKuroEst}{0.9}
\newcommand{\hlExtHFiveKuroCILo}{\ensuremath{-}1.9}
\newcommand{\hlExtHFiveKuroCIHi}{3.7}
\newcommand{\hlExtHFiveKuroTostCILo}{\ensuremath{-}1.4}
\newcommand{\hlExtHFiveKuroTostCIHi}{3.1}
\newcommand{\hlExtHFiveKuroMde}{4.4}
\newcommand{\hlExtHFiveKuroPHolm}{1.000}
\newcommand{\hlExtHFiveKuroN}{10}
\newcommand{\hlExtVerdictHFiveKuro}{Undetermined, MDE 4.4}
\newcommand{\hlExtFOneOneKuroEst}{\ensuremath{-}1.4}
\newcommand{\hlExtFOneOneKuroCILo}{\ensuremath{-}9.8}
\newcommand{\hlExtFOneOneKuroCIHi}{7.0}
\newcommand{\hlExtFOneOneKuroTostCILo}{\ensuremath{-}7.9}
\newcommand{\hlExtFOneOneKuroTostCIHi}{5.1}
\newcommand{\hlExtFOneOneKuroMde}{13.9}
\newcommand{\hlExtFOneOneKuroPHolm}{1.000}
\newcommand{\hlExtFOneOneKuroN}{5}
\newcommand{\hlExtHFiveSegfKuroEst}{0.2}
\newcommand{\hlExtHFiveSegfKuroCILo}{\ensuremath{-}3.2}
\newcommand{\hlExtHFiveSegfKuroCIHi}{3.6}
\newcommand{\hlExtHFiveSegfKuroTostCILo}{\ensuremath{-}2.5}
\newcommand{\hlExtHFiveSegfKuroTostCIHi}{2.9}
\newcommand{\hlExtHFiveSegfKuroMde}{5.4}
\newcommand{\hlExtHFiveSegfKuroPHolm}{0.892}
\newcommand{\hlExtHFiveSegfKuroN}{10}
\newcommand{\hlExtHFiveMtwoFKuroEst}{0.2}
\newcommand{\hlExtHFiveMtwoFKuroCILo}{\ensuremath{-}3.6}
\newcommand{\hlExtHFiveMtwoFKuroCIHi}{4.0}
\newcommand{\hlExtHFiveMtwoFKuroTostCILo}{\ensuremath{-}2.9}
\newcommand{\hlExtHFiveMtwoFKuroTostCIHi}{3.3}
\newcommand{\hlExtHFiveMtwoFKuroMde}{6.0}
\newcommand{\hlExtHFiveMtwoFKuroPHolm}{0.911}
\newcommand{\hlExtHFiveMtwoFKuroN}{10}
\newcommand{\hlExtHFiveSamKuroEst}{2.2}
\newcommand{\hlExtHFiveSamKuroCILo}{0.0}
\newcommand{\hlExtHFiveSamKuroCIHi}{4.4}
\newcommand{\hlExtHFiveSamKuroTostCILo}{0.4}
\newcommand{\hlExtHFiveSamKuroTostCIHi}{4.0}
\newcommand{\hlExtHFiveSamKuroMde}{3.5}
\newcommand{\hlExtHFiveSamKuroPHolm}{0.048}
\newcommand{\hlExtHFiveSamKuroN}{10}
\newcommand{\hlRealDropSATKuro}{0.3}
\newcommand{\hlRealDropSATKuroCILo}{\ensuremath{-}8.1}
\newcommand{\hlRealDropSATKuroCIHi}{8.6}
\newcommand{\hlRealDropLVDKuro}{2.4}
\newcommand{\hlRealDropLVDKuroCILo}{\ensuremath{-}0.3}
\newcommand{\hlRealDropLVDKuroCIHi}{5.2}
\newcommand{\hlRealDropDOFAKuro}{0.5}
\newcommand{\hlRealDropDOFAKuroCILo}{\ensuremath{-}3.0}
\newcommand{\hlRealDropDOFAKuroCIHi}{4.0}
\newcommand{\hlRealDropTMKuro}{0.7}
\newcommand{\hlRealDropTMKuroCILo}{\ensuremath{-}1.0}
\newcommand{\hlRealDropTMKuroCIHi}{2.5}
\newcommand{\hlRealDropRNKuro}{\ensuremath{-}0.1}
\newcommand{\hlRealDropRNKuroCILo}{\ensuremath{-}0.5}
\newcommand{\hlRealDropRNKuroCIHi}{0.2}
\newcommand{\hlRealDropKuro}{0.8}
\newcommand{\hlRealDropKuroCILo}{\ensuremath{-}0.6}
\newcommand{\hlRealDropKuroCIHi}{2.1}
\newcommand{\hlRealDropKuroN}{25}
\newcommand{\hlRealMatchedDropKuro}{0.1}
\newcommand{\hlRealVsSynthKuro}{0.7}
\newcommand{\hlRealVsSynthKuroEst}{0.7}
\newcommand{\hlRealVsSynthKuroCILo}{\ensuremath{-}1.4}
\newcommand{\hlRealVsSynthKuroCIHi}{2.8}
\newcommand{\hlRealVsSynthKuroTostCILo}{\ensuremath{-}1.0}
\newcommand{\hlRealVsSynthKuroTostCIHi}{2.4}
\newcommand{\hlRealVsSynthKuroMde}{3.3}
\newcommand{\hlRealVsSynthKuroPHolm}{1.000}
\newcommand{\hlRealVsSynthKuroN}{25}
\newcommand{\hlRealVerdictKuro}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlRealMatchedTypeKuro}{coarse}
\newcommand{\hlRealMatchedLevelKuro}{\Lone}
\newcommand{\hlRealBaselineKuro}{clean run on the tiles the real labels cover}
\newcommand{\hlExtMeanDropSATOem}{7.6}
\newcommand{\hlExtMeanDropLVDOem}{6.7}
\newcommand{\hlExtMeanDropDOFAOem}{6.8}
\newcommand{\hlExtMeanDropTMOem}{6.0}
\newcommand{\hlExtMeanDropRNOem}{5.4}
\newcommand{\hlExtMeanDropOem}{6.5}
\newcommand{\hlExtCleanOem}{59.7}
\newcommand{\hlExtTypeRankOemOne}{boundary}
\newcommand{\hlExtTypeRankOemTwo}{omission}
\newcommand{\hlExtTypeRankOemThree}{coarse}
\newcommand{\hlExtTypeRankOemFour}{shift}
\newcommand{\hlExtFOneOemEst}{0.9}
\newcommand{\hlExtFOneOemCILo}{0.1}
\newcommand{\hlExtFOneOemCIHi}{1.6}
\newcommand{\hlExtFOneOemTostCILo}{0.3}
\newcommand{\hlExtFOneOemTostCIHi}{1.4}
\newcommand{\hlExtFOneOemMde}{1.2}
\newcommand{\hlExtFOneOemPHolm}{0.182}
\newcommand{\hlExtFOneOemN}{5}
\newcommand{\hlExtVerdictFOneOem}{Equivalent within $\pm$\TostMargin, \lvd loses less}
\newcommand{\hlExtFTwoOemEst}{1.0}
\newcommand{\hlExtFTwoOemCILo}{\ensuremath{-}0.3}
\newcommand{\hlExtFTwoOemCIHi}{2.3}
\newcommand{\hlExtFTwoOemTostCILo}{0.0}
\newcommand{\hlExtFTwoOemTostCIHi}{2.0}
\newcommand{\hlExtFTwoOemMde}{2.1}
\newcommand{\hlExtFTwoOemPHolm}{0.283}
\newcommand{\hlExtFTwoOemN}{5}
\newcommand{\hlExtVerdictFTwoOem}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlExtNSixOemEst}{\ensuremath{-}0.1}
\newcommand{\hlExtNSixOemCILo}{\ensuremath{-}0.7}
\newcommand{\hlExtNSixOemCIHi}{0.5}
\newcommand{\hlExtNSixOemTostCILo}{\ensuremath{-}0.6}
\newcommand{\hlExtNSixOemTostCIHi}{0.3}
\newcommand{\hlExtNSixOemMde}{1.0}
\newcommand{\hlExtNSixOemPHolm}{1.000}
\newcommand{\hlExtNSixOemN}{5}
\newcommand{\hlExtVerdictNSixOem}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlExtHFiveOemEst}{\ensuremath{-}0.5}
\newcommand{\hlExtHFiveOemCILo}{\ensuremath{-}1.1}
\newcommand{\hlExtHFiveOemCIHi}{0.1}
\newcommand{\hlExtHFiveOemTostCILo}{\ensuremath{-}1.0}
\newcommand{\hlExtHFiveOemTostCIHi}{0.0}
\newcommand{\hlExtHFiveOemMde}{0.9}
\newcommand{\hlExtHFiveOemPHolm}{0.365}
\newcommand{\hlExtHFiveOemN}{10}
\newcommand{\hlExtVerdictHFiveOem}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlExtFOneOneOemEst}{\ensuremath{-}0.2}
\newcommand{\hlExtFOneOneOemCILo}{\ensuremath{-}1.6}
\newcommand{\hlExtFOneOneOemCIHi}{1.3}
\newcommand{\hlExtFOneOneOemTostCILo}{\ensuremath{-}1.3}
\newcommand{\hlExtFOneOneOemTostCIHi}{1.0}
\newcommand{\hlExtFOneOneOemMde}{2.4}
\newcommand{\hlExtFOneOneOemPHolm}{1.000}
\newcommand{\hlExtFOneOneOemN}{5}
\newcommand{\hlExtHFiveSegfOemEst}{\ensuremath{-}0.1}
\newcommand{\hlExtHFiveSegfOemCILo}{\ensuremath{-}1.0}
\newcommand{\hlExtHFiveSegfOemCIHi}{0.7}
\newcommand{\hlExtHFiveSegfOemTostCILo}{\ensuremath{-}0.8}
\newcommand{\hlExtHFiveSegfOemTostCIHi}{0.6}
\newcommand{\hlExtHFiveSegfOemMde}{1.4}
\newcommand{\hlExtHFiveSegfOemPHolm}{0.716}
\newcommand{\hlExtHFiveSegfOemN}{10}
\newcommand{\hlExtHFiveMtwoFOemEst}{\ensuremath{-}0.1}
\newcommand{\hlExtHFiveMtwoFOemCILo}{\ensuremath{-}0.8}
\newcommand{\hlExtHFiveMtwoFOemCIHi}{0.6}
\newcommand{\hlExtHFiveMtwoFOemTostCILo}{\ensuremath{-}0.7}
\newcommand{\hlExtHFiveMtwoFOemTostCIHi}{0.5}
\newcommand{\hlExtHFiveMtwoFOemMde}{1.1}
\newcommand{\hlExtHFiveMtwoFOemPHolm}{0.785}
\newcommand{\hlExtHFiveMtwoFOemN}{10}
\newcommand{\hlExtHFiveSamOemEst}{\ensuremath{-}1.3}
\newcommand{\hlExtHFiveSamOemCILo}{\ensuremath{-}1.9}
\newcommand{\hlExtHFiveSamOemCIHi}{\ensuremath{-}0.7}
\newcommand{\hlExtHFiveSamOemTostCILo}{\ensuremath{-}1.8}
\newcommand{\hlExtHFiveSamOemTostCIHi}{\ensuremath{-}0.8}
\newcommand{\hlExtHFiveSamOemMde}{0.9}
\newcommand{\hlExtHFiveSamOemPHolm}{\ensuremath{<}0.001}
\newcommand{\hlExtHFiveSamOemN}{10}
\newcommand{\hlDsTotal}{9}
\newcommand{\hlDsDone}{9}
\newcommand{\hlDsNSixEquiv}{8}
\newcommand{\hlDsNSixRead}{9}
\newcommand{\hlDsFTwoEquiv}{5}
\newcommand{\hlDsFTwoRead}{9}
\newcommand{\hlDsTotalSubm}{3}
\newcommand{\hlDsNSixEquivSubm}{3}
\newcommand{\hlDsNSixReadSubm}{3}
\newcommand{\hlDsTotalRest}{6}
\newcommand{\hlDsNSixEquivRest}{5}
\newcommand{\hlDsNSixReadRest}{6}
\newcommand{\hlDsShiftLeast}{9}
\newcommand{\hlDsOmissionMost}{3}
\newcommand{\hlDsCoarseMost}{4}
\newcommand{\hlDsTypeRead}{9}
\newcommand{\hlDsRealMore}{4}
\newcommand{\hlDsRealRead}{5}
\newcommand{\hlRunsPlannedNSeven}{550}
\newcommand{\hlRunsDoneNSeven}{550}
\newcommand{\hlBlockStatusNSeven}{Complete}
\newcommand{\hlRunsPlannedNEight}{194}
\newcommand{\hlRunsDoneNEight}{194}
\newcommand{\hlBlockStatusNEight}{Complete}
\newcommand{\hlRunsPlannedNNine}{550}
\newcommand{\hlRunsDoneNNine}{550}
\newcommand{\hlBlockStatusNNine}{Complete}
\newcommand{\hlRunsPlannedNTen}{550}
\newcommand{\hlRunsDoneNTen}{550}
\newcommand{\hlBlockStatusNTen}{Complete}
\newcommand{\hlRunsPlannedNEleven}{550}
\newcommand{\hlRunsDoneNEleven}{550}
\newcommand{\hlBlockStatusNEleven}{Complete}
\newcommand{\hlRunsPlannedNTwelve}{280}
\newcommand{\hlRunsDoneNTwelve}{280}
\newcommand{\hlBlockStatusNTwelve}{Complete}
\newcommand{\hlRunsPlannedNThirteen}{45}
\newcommand{\hlRunsDoneNThirteen}{45}
\newcommand{\hlBlockStatusNThirteen}{Complete}
\newcommand{\hlRunsPlannedNFourteen}{500}
\newcommand{\hlRunsDoneNFourteen}{500}
\newcommand{\hlBlockStatusNFourteen}{Complete}
\newcommand{\hlRunsPlannedNFifteen}{550}
\newcommand{\hlRunsDoneNFifteen}{550}
\newcommand{\hlBlockStatusNFifteen}{Complete}
\newcommand{\hlRunsPlannedDOne}{450}
\newcommand{\hlRunsDoneDOne}{450}
\newcommand{\hlBlockStatusDOne}{Complete}
\newcommand{\hlRunsPlannedDTwo}{450}
\newcommand{\hlRunsDoneDTwo}{450}
\newcommand{\hlBlockStatusDTwo}{Complete}
\newcommand{\hlRunsPlannedDThree}{475}
\newcommand{\hlRunsDoneDThree}{475}
\newcommand{\hlBlockStatusDThree}{Complete}
\newcommand{\hlRunsPlannedDFour}{450}
\newcommand{\hlRunsDoneDFour}{450}
\newcommand{\hlBlockStatusDFour}{Complete}
\newcommand{\hlRunsPlannedDFive}{425}
\newcommand{\hlRunsDoneDFive}{425}
\newcommand{\hlBlockStatusDFive}{Complete}
\newcommand{\hlRunsPlannedDSix}{475}
\newcommand{\hlRunsDoneDSix}{475}
\newcommand{\hlBlockStatusDSix}{Complete}
\newcommand{\hlRunsPlannedDSeven}{425}
\newcommand{\hlRunsDoneDSeven}{425}
\newcommand{\hlBlockStatusDSeven}{Complete}
\newcommand{\hlNCollapsedPostReviewburn}{233}
\newcommand{\hlNCollapsedNSevenburn}{4}
\newcommand{\hlNCollapsedNEightburn}{3}
\newcommand{\hlNCollapsedNNineburn}{60}
\newcommand{\hlNCollapsedNTenburn}{26}
\newcommand{\hlNCollapsedNElevenburn}{30}
\newcommand{\hlNCollapsedNTwelveburn}{24}
\newcommand{\hlNCollapsedNFourteenburn}{3}
\newcommand{\hlNCollapsedNFifteenburn}{83}
\newcommand{\hlMlrDropSATburn}{13.9}
\newcommand{\hlMlrDropLVDburn}{13.8}
\newcommand{\hlMlrDropDiffburn}{\ensuremath{-}0.2}
\newcommand{\hlMlrDropDiffCILoburn}{\ensuremath{-}3.7}
\newcommand{\hlMlrDropDiffCIHiburn}{3.3}
\newcommand{\hlMlrDropNburn}{5}
\newcommand{\hlMlrDropDiffHalfburn}{3.5}
\newcommand{\hlMlrDropTostCILoburn}{\ensuremath{-}2.9}
\newcommand{\hlMlrDropTostCIHiburn}{2.5}
\newcommand{\hlMlrDropTostPburn}{0.044}
\newcommand{\hlMlrDropTostEquivalentburn}{yes}
\newcommand{\hlMlrRetSATburn}{82.9}
\newcommand{\hlMlrRetLVDburn}{83.1}
\newcommand{\hlMlrRetDiffburn}{0.1}
\newcommand{\hlMlrRetDiffCILoburn}{\ensuremath{-}3.7}
\newcommand{\hlMlrRetDiffCIHiburn}{3.9}
\newcommand{\hlMlrRetNburn}{5}
\newcommand{\hlMlrRetDiffHalfburn}{3.8}
\newcommand{\hlMlrRetTostCILoburn}{\ensuremath{-}2.8}
\newcommand{\hlMlrRetTostCIHiburn}{3.0}
\newcommand{\hlMlrRetTostPburn}{0.052}
\newcommand{\hlMlrRetTostEquivalentburn}{no}
\newcommand{\hlMlrDropSATflair}{5.1}
\newcommand{\hlMlrDropLVDflair}{3.5}
\newcommand{\hlMlrDropDiffflair}{1.5}
\newcommand{\hlMlrDropDiffCILoflair}{0.6}
\newcommand{\hlMlrDropDiffCIHiflair}{2.5}
\newcommand{\hlMlrDropNflair}{5}
\newcommand{\hlMlrDropDiffHalfflair}{1.0}
\newcommand{\hlMlrDropTostCILoflair}{0.8}
\newcommand{\hlMlrDropTostCIHiflair}{2.2}
\newcommand{\hlMlrDropTostPflair}{0.006}
\newcommand{\hlMlrDropTostEquivalentflair}{yes}
\newcommand{\hlMlrRetSATflair}{89.9}
\newcommand{\hlMlrRetLVDflair}{93.1}
\newcommand{\hlMlrRetDiffflair}{\ensuremath{-}3.0}
\newcommand{\hlMlrRetDiffCILoflair}{\ensuremath{-}4.9}
\newcommand{\hlMlrRetDiffCIHiflair}{\ensuremath{-}1.2}
\newcommand{\hlMlrRetNflair}{5}
\newcommand{\hlMlrRetDiffHalfflair}{1.8}
\newcommand{\hlMlrRetTostCILoflair}{\ensuremath{-}4.4}
\newcommand{\hlMlrRetTostCIHiflair}{\ensuremath{-}1.7}
\newcommand{\hlMlrRetTostPflair}{0.526}
\newcommand{\hlMlrRetTostEquivalentflair}{no}
\newcommand{\hlSATLrMainburn}{77.5}
\newcommand{\hlSATLrLrThirdburn}{81.9}
\newcommand{\hlSATLrMainflair}{60.9}
\newcommand{\hlSATLrLrThirdflair}{56.7}
\newcommand{\hlSATLrMainsen}{74.5}
\newcommand{\hlMsFractionPct}{20}
\newcommand{\hlMsShareburn}{19}
\newcommand{\hlMsShareflair}{64}
\newcommand{\hlMsShareChes}{29}
\newcommand{\hlMsShareCsTwelve}{45}
\newcommand{\hlMsShareDfc}{130}
\newcommand{\hlMsShareEnva}{39}
\newcommand{\hlMsShareSnTwo}{25}
\newcommand{\hlMsShareKuro}{55}
\newcommand{\hlMsShareOem}{46}
\newcommand{\hlMsShareOverHalf}{3}
\newcommand{\hlMsNSixRead}{9}
\newcommand{\hlMsNSixEquiv}{8}
\newcommand{\hlMsNSixEquivScaled}{4}
\newcommand{\hlMsNSixEquivRet}{5}
\newcommand{\hlMsNSixReadSubm}{3}
\newcommand{\hlMsNSixEquivSubm}{3}
\newcommand{\hlMsNSixEquivScaledSubm}{2}
\newcommand{\hlMsNSixEquivRetSubm}{2}
\newcommand{\hlMsNSixReadRest}{6}
\newcommand{\hlMsNSixEquivRest}{5}
\newcommand{\hlMsNSixEquivScaledRest}{2}
\newcommand{\hlMsNSixEquivRetRest}{3}
\newcommand{\hlMsFOneRead}{9}
\newcommand{\hlMsFOneEquiv}{5}
\newcommand{\hlMsFOneEquivScaled}{2}
\newcommand{\hlMsFOneEquivRet}{3}
\newcommand{\hlMsFTwoRead}{9}
\newcommand{\hlMsFTwoEquiv}{5}
\newcommand{\hlMsFTwoEquivScaled}{1}
\newcommand{\hlMsFTwoEquivRet}{2}
\newcommand{\hlMsVerdictNSixburn}{Undetermined}
\newcommand{\hlMsMarginNSixburn}{2.8}
\newcommand{\hlMsRetVerdictNSixburn}{Equivalent}
\newcommand{\hlMsRetMarginNSixburn}{3.4}
\newcommand{\hlMsRetNSixburnEst}{0.1}
\newcommand{\hlMsRetNSixburnCILo}{\ensuremath{-}2.8}
\newcommand{\hlMsRetNSixburnCIHi}{3.0}
\newcommand{\hlMsVerdictFOneburn}{Differs}
\newcommand{\hlMsMarginFOneburn}{3.0}
\newcommand{\hlMsRetVerdictFOneburn}{Differs}
\newcommand{\hlMsRetMarginFOneburn}{4.0}
\newcommand{\hlMsRetFOneburnEst}{\ensuremath{-}6.6}
\newcommand{\hlMsRetFOneburnCILo}{\ensuremath{-}9.2}
\newcommand{\hlMsRetFOneburnCIHi}{\ensuremath{-}4.0}
\newcommand{\hlMsVerdictFTwoburn}{Equivalent}
\newcommand{\hlMsMarginFTwoburn}{3.0}
\newcommand{\hlMsRetVerdictFTwoburn}{Equivalent}
\newcommand{\hlMsRetMarginFTwoburn}{3.5}
\newcommand{\hlMsRetFTwoburnEst}{\ensuremath{-}0.4}
\newcommand{\hlMsRetFTwoburnCILo}{\ensuremath{-}2.8}
\newcommand{\hlMsRetFTwoburnCIHi}{1.9}
\newcommand{\hlMsVerdictHFiveSegfburn}{Equivalent}
\newcommand{\hlMsMarginHFiveSegfburn}{3.0}
\newcommand{\hlMsVerdictHFiveMtwoFburn}{Undetermined}
\newcommand{\hlMsMarginHFiveMtwoFburn}{3.0}
\newcommand{\hlMsVerdictHFiveSamburn}{Equivalent}
\newcommand{\hlMsMarginHFiveSamburn}{3.0}
\newcommand{\hlMsVerdictHFiveMtwoFFburn}{Equivalent}
\newcommand{\hlMsMarginHFiveMtwoFFburn}{3.0}
\newcommand{\hlMsVerdictHFiveSamPreburn}{Undetermined}
\newcommand{\hlMsMarginHFiveSamPreburn}{3.0}
\newcommand{\hlMsVerdictHSixRqOneOneburn}{Undetermined}
\newcommand{\hlMsMarginHSixRqOneOneburn}{3.0}
\newcommand{\hlMsVerdictHSixRqOneThirdburn}{Undetermined}
\newcommand{\hlMsMarginHSixRqOneThirdburn}{2.8}
\newcommand{\hlMsVerdictHSixFTwoOneburn}{Undetermined}
\newcommand{\hlMsMarginHSixFTwoOneburn}{3.0}
\newcommand{\hlMsVerdictHSixFTwoThirdburn}{Equivalent}
\newcommand{\hlMsMarginHSixFTwoThirdburn}{2.8}
\newcommand{\hlMsVerdictMitGceburn}{Equivalent}
\newcommand{\hlMsMarginMitGceburn}{3.0}
\newcommand{\hlMsVerdictMitBootburn}{Equivalent}
\newcommand{\hlMsMarginMitBootburn}{3.0}
\newcommand{\hlMsVerdictNSixflair}{Differs}
\newcommand{\hlMsMarginNSixflair}{0.9}
\newcommand{\hlMsRetVerdictNSixflair}{Differs}
\newcommand{\hlMsRetMarginNSixflair}{1.7}
\newcommand{\hlMsRetNSixflairEst}{\ensuremath{-}3.0}
\newcommand{\hlMsRetNSixflairCILo}{\ensuremath{-}4.4}
\newcommand{\hlMsRetNSixflairCIHi}{\ensuremath{-}1.7}
\newcommand{\hlMsVerdictFOneflair}{Differs}
\newcommand{\hlMsMarginFOneflair}{1.0}
\newcommand{\hlMsRetVerdictFOneflair}{Differs}
\newcommand{\hlMsRetMarginFOneflair}{1.9}
\newcommand{\hlMsRetFOneflairEst}{\ensuremath{-}5.2}
\newcommand{\hlMsRetFOneflairCILo}{\ensuremath{-}6.7}
\newcommand{\hlMsRetFOneflairCIHi}{\ensuremath{-}3.7}
\newcommand{\hlMsVerdictFTwoflair}{Undetermined}
\newcommand{\hlMsMarginFTwoflair}{0.9}
\newcommand{\hlMsRetVerdictFTwoflair}{Undetermined}
\newcommand{\hlMsRetMarginFTwoflair}{2.0}
\newcommand{\hlMsRetFTwoflairEst}{\ensuremath{-}1.6}
\newcommand{\hlMsRetFTwoflairCILo}{\ensuremath{-}5.7}
\newcommand{\hlMsRetFTwoflairCIHi}{2.5}
\newcommand{\hlMsVerdictHFiveSegfflair}{Equivalent}
\newcommand{\hlMsMarginHFiveSegfflair}{0.9}
\newcommand{\hlMsVerdictHFiveMtwoFflair}{Differs}
\newcommand{\hlMsMarginHFiveMtwoFflair}{1.0}
\newcommand{\hlMsVerdictHFiveSamflair}{Equivalent}
\newcommand{\hlMsMarginHFiveSamflair}{1.0}
\newcommand{\hlMsVerdictHFiveMtwoFFflair}{Equivalent}
\newcommand{\hlMsMarginHFiveMtwoFFflair}{1.0}
\newcommand{\hlMsVerdictHFiveSamPreflair}{Undetermined}
\newcommand{\hlMsMarginHFiveSamPreflair}{1.0}
\newcommand{\hlMsVerdictHSixRqOneOneflair}{Differs}
\newcommand{\hlMsMarginHSixRqOneOneflair}{1.0}
\newcommand{\hlMsVerdictHSixRqOneThirdflair}{Differs}
\newcommand{\hlMsMarginHSixRqOneThirdflair}{0.9}
\newcommand{\hlMsVerdictHSixFTwoOneflair}{Undetermined}
\newcommand{\hlMsMarginHSixFTwoOneflair}{0.9}
\newcommand{\hlMsVerdictHSixFTwoThirdflair}{Undetermined}
\newcommand{\hlMsMarginHSixFTwoThirdflair}{0.8}
\newcommand{\hlMsVerdictMitGceflair}{Equivalent}
\newcommand{\hlMsMarginMitGceflair}{1.0}
\newcommand{\hlMsVerdictMitBootflair}{Equivalent}
\newcommand{\hlMsMarginMitBootflair}{1.0}
\newcommand{\hlMsVerdictNSixChes}{Equivalent}
\newcommand{\hlMsMarginNSixChes}{2.0}
\newcommand{\hlMsRetVerdictNSixChes}{Equivalent}
\newcommand{\hlMsRetMarginNSixChes}{2.5}
\newcommand{\hlMsRetNSixChesEst}{1.0}
\newcommand{\hlMsRetNSixChesCILo}{\ensuremath{-}0.1}
\newcommand{\hlMsRetNSixChesCIHi}{2.1}
\newcommand{\hlMsVerdictFOneChes}{Equivalent}
\newcommand{\hlMsMarginFOneChes}{2.0}
\newcommand{\hlMsRetVerdictFOneChes}{Equivalent}
\newcommand{\hlMsRetMarginFOneChes}{2.5}
\newcommand{\hlMsRetFOneChesEst}{0.4}
\newcommand{\hlMsRetFOneChesCILo}{\ensuremath{-}1.5}
\newcommand{\hlMsRetFOneChesCIHi}{2.2}
\newcommand{\hlMsVerdictFTwoChes}{Differs}
\newcommand{\hlMsMarginFTwoChes}{2.0}
\newcommand{\hlMsRetVerdictFTwoChes}{Differs}
\newcommand{\hlMsRetMarginFTwoChes}{2.4}
\newcommand{\hlMsRetFTwoChesEst}{\ensuremath{-}2.8}
\newcommand{\hlMsRetFTwoChesCILo}{\ensuremath{-}3.7}
\newcommand{\hlMsRetFTwoChesCIHi}{\ensuremath{-}1.8}
\newcommand{\hlMsVerdictHFiveChes}{Equivalent}
\newcommand{\hlMsMarginHFiveChes}{2.1}
\newcommand{\hlMsVerdictNSixCsTwelve}{Equivalent}
\newcommand{\hlMsMarginNSixCsTwelve}{1.3}
\newcommand{\hlMsRetVerdictNSixCsTwelve}{Equivalent}
\newcommand{\hlMsRetMarginNSixCsTwelve}{1.9}
\newcommand{\hlMsRetNSixCsTwelveEst}{\ensuremath{-}0.6}
\newcommand{\hlMsRetNSixCsTwelveCILo}{\ensuremath{-}1.9}
\newcommand{\hlMsRetNSixCsTwelveCIHi}{0.7}
\newcommand{\hlMsVerdictFOneCsTwelve}{Undetermined}
\newcommand{\hlMsMarginFOneCsTwelve}{1.2}
\newcommand{\hlMsRetVerdictFOneCsTwelve}{Undetermined}
\newcommand{\hlMsRetMarginFOneCsTwelve}{1.8}
\newcommand{\hlMsRetFOneCsTwelveEst}{0.4}
\newcommand{\hlMsRetFOneCsTwelveCILo}{\ensuremath{-}1.8}
\newcommand{\hlMsRetFOneCsTwelveCIHi}{2.6}
\newcommand{\hlMsVerdictFTwoCsTwelve}{Undetermined}
\newcommand{\hlMsMarginFTwoCsTwelve}{1.4}
\newcommand{\hlMsRetVerdictFTwoCsTwelve}{Equivalent}
\newcommand{\hlMsRetMarginFTwoCsTwelve}{2.1}
\newcommand{\hlMsRetFTwoCsTwelveEst}{\ensuremath{-}0.1}
\newcommand{\hlMsRetFTwoCsTwelveCILo}{\ensuremath{-}1.6}
\newcommand{\hlMsRetFTwoCsTwelveCIHi}{1.5}
\newcommand{\hlMsVerdictHFiveCsTwelve}{Equivalent}
\newcommand{\hlMsMarginHFiveCsTwelve}{1.3}
\newcommand{\hlMsVerdictNSixDfc}{Undetermined}
\newcommand{\hlMsMarginNSixDfc}{0.6}
\newcommand{\hlMsRetVerdictNSixDfc}{Undetermined}
\newcommand{\hlMsRetMarginNSixDfc}{1.3}
\newcommand{\hlMsRetNSixDfcEst}{\ensuremath{-}1.5}
\newcommand{\hlMsRetNSixDfcCILo}{\ensuremath{-}5.3}
\newcommand{\hlMsRetNSixDfcCIHi}{2.3}
\newcommand{\hlMsVerdictFOneDfc}{Undetermined}
\newcommand{\hlMsMarginFOneDfc}{0.5}
\newcommand{\hlMsRetVerdictFOneDfc}{Undetermined}
\newcommand{\hlMsRetMarginFOneDfc}{1.3}
\newcommand{\hlMsRetFOneDfcEst}{\ensuremath{-}1.4}
\newcommand{\hlMsRetFOneDfcCILo}{\ensuremath{-}3.5}
\newcommand{\hlMsRetFOneDfcCIHi}{0.7}
\newcommand{\hlMsVerdictFTwoDfc}{Undetermined}
\newcommand{\hlMsMarginFTwoDfc}{0.4}
\newcommand{\hlMsRetVerdictFTwoDfc}{Undetermined}
\newcommand{\hlMsRetMarginFTwoDfc}{0.9}
\newcommand{\hlMsRetFTwoDfcEst}{\ensuremath{-}3.3}
\newcommand{\hlMsRetFTwoDfcCILo}{\ensuremath{-}6.8}
\newcommand{\hlMsRetFTwoDfcCIHi}{0.3}
\newcommand{\hlMsVerdictHFiveDfc}{Undetermined}
\newcommand{\hlMsMarginHFiveDfc}{0.5}
\newcommand{\hlMsVerdictNSixEnva}{Undetermined}
\newcommand{\hlMsMarginNSixEnva}{1.4}
\newcommand{\hlMsRetVerdictNSixEnva}{Undetermined}
\newcommand{\hlMsRetMarginNSixEnva}{2.3}
\newcommand{\hlMsRetNSixEnvaEst}{1.6}
\newcommand{\hlMsRetNSixEnvaCILo}{\ensuremath{-}2.5}
\newcommand{\hlMsRetNSixEnvaCIHi}{5.7}
\newcommand{\hlMsVerdictFOneEnva}{Undetermined}
\newcommand{\hlMsMarginFOneEnva}{1.4}
\newcommand{\hlMsRetVerdictFOneEnva}{Undetermined}
\newcommand{\hlMsRetMarginFOneEnva}{2.2}
\newcommand{\hlMsRetFOneEnvaEst}{2.1}
\newcommand{\hlMsRetFOneEnvaCILo}{\ensuremath{-}1.7}
\newcommand{\hlMsRetFOneEnvaCIHi}{6.0}
\newcommand{\hlMsVerdictFTwoEnva}{Differs}
\newcommand{\hlMsMarginFTwoEnva}{1.8}
\newcommand{\hlMsRetVerdictFTwoEnva}{Differs}
\newcommand{\hlMsRetMarginFTwoEnva}{3.7}
\newcommand{\hlMsRetFTwoEnvaEst}{11.9}
\newcommand{\hlMsRetFTwoEnvaCILo}{8.5}
\newcommand{\hlMsRetFTwoEnvaCIHi}{15.2}
\newcommand{\hlMsVerdictHFiveEnva}{Differs}
\newcommand{\hlMsMarginHFiveEnva}{1.1}
\newcommand{\hlMsVerdictNSixSnTwo}{Equivalent}
\newcommand{\hlMsMarginNSixSnTwo}{2.1}
\newcommand{\hlMsRetVerdictNSixSnTwo}{Equivalent}
\newcommand{\hlMsRetMarginNSixSnTwo}{2.4}
\newcommand{\hlMsRetNSixSnTwoEst}{\ensuremath{-}0.4}
\newcommand{\hlMsRetNSixSnTwoCILo}{\ensuremath{-}1.7}
\newcommand{\hlMsRetNSixSnTwoCIHi}{1.0}
\newcommand{\hlMsVerdictFOneSnTwo}{Equivalent}
\newcommand{\hlMsMarginFOneSnTwo}{2.2}
\newcommand{\hlMsRetVerdictFOneSnTwo}{Equivalent}
\newcommand{\hlMsRetMarginFOneSnTwo}{2.5}
\newcommand{\hlMsRetFOneSnTwoEst}{\ensuremath{-}1.3}
\newcommand{\hlMsRetFOneSnTwoCILo}{\ensuremath{-}1.8}
\newcommand{\hlMsRetFOneSnTwoCIHi}{\ensuremath{-}0.8}
\newcommand{\hlMsVerdictFTwoSnTwo}{Differs}
\newcommand{\hlMsMarginFTwoSnTwo}{2.6}
\newcommand{\hlMsRetVerdictFTwoSnTwo}{Differs}
\newcommand{\hlMsRetMarginFTwoSnTwo}{3.1}
\newcommand{\hlMsRetFTwoSnTwoEst}{2.9}
\newcommand{\hlMsRetFTwoSnTwoCILo}{1.3}
\newcommand{\hlMsRetFTwoSnTwoCIHi}{4.5}
\newcommand{\hlMsVerdictHFiveSnTwo}{Differs}
\newcommand{\hlMsMarginHFiveSnTwo}{2.5}
\newcommand{\hlMsVerdictNSixKuro}{Undetermined}
\newcommand{\hlMsMarginNSixKuro}{1.4}
\newcommand{\hlMsRetVerdictNSixKuro}{Undetermined}
\newcommand{\hlMsRetMarginNSixKuro}{2.3}
\newcommand{\hlMsRetNSixKuroEst}{1.9}
\newcommand{\hlMsRetNSixKuroCILo}{\ensuremath{-}0.6}
\newcommand{\hlMsRetNSixKuroCIHi}{4.3}
\newcommand{\hlMsVerdictFOneKuro}{Undetermined}
\newcommand{\hlMsMarginFOneKuro}{1.4}
\newcommand{\hlMsRetVerdictFOneKuro}{Undetermined}
\newcommand{\hlMsRetMarginFOneKuro}{2.4}
\newcommand{\hlMsRetFOneKuroEst}{0.5}
\newcommand{\hlMsRetFOneKuroCILo}{\ensuremath{-}3.8}
\newcommand{\hlMsRetFOneKuroCIHi}{4.9}
\newcommand{\hlMsVerdictFTwoKuro}{Differs}
\newcommand{\hlMsMarginFTwoKuro}{0.7}
\newcommand{\hlMsRetVerdictFTwoKuro}{Undetermined}
\newcommand{\hlMsRetMarginFTwoKuro}{1.2}
\newcommand{\hlMsRetFTwoKuroEst}{\ensuremath{-}10.6}
\newcommand{\hlMsRetFTwoKuroCILo}{\ensuremath{-}21.1}
\newcommand{\hlMsRetFTwoKuroCIHi}{\ensuremath{-}0.2}
\newcommand{\hlMsVerdictHFiveKuro}{Undetermined}
\newcommand{\hlMsMarginHFiveKuro}{1.5}
\newcommand{\hlMsVerdictNSixOem}{Equivalent}
\newcommand{\hlMsMarginNSixOem}{1.3}
\newcommand{\hlMsRetVerdictNSixOem}{Equivalent}
\newcommand{\hlMsRetMarginNSixOem}{2.1}
\newcommand{\hlMsRetNSixOemEst}{\ensuremath{-}0.1}
\newcommand{\hlMsRetNSixOemCILo}{\ensuremath{-}0.8}
\newcommand{\hlMsRetNSixOemCIHi}{0.6}
\newcommand{\hlMsVerdictFOneOem}{Differs}
\newcommand{\hlMsMarginFOneOem}{1.4}
\newcommand{\hlMsRetVerdictFOneOem}{Equivalent}
\newcommand{\hlMsRetMarginFOneOem}{2.3}
\newcommand{\hlMsRetFOneOemEst}{\ensuremath{-}1.3}
\newcommand{\hlMsRetFOneOemCILo}{\ensuremath{-}2.2}
\newcommand{\hlMsRetFOneOemCIHi}{\ensuremath{-}0.5}
\newcommand{\hlMsVerdictFTwoOem}{Undetermined}
\newcommand{\hlMsMarginFTwoOem}{1.2}
\newcommand{\hlMsRetVerdictFTwoOem}{Undetermined}
\newcommand{\hlMsRetMarginFTwoOem}{2.1}
\newcommand{\hlMsRetFTwoOemEst}{\ensuremath{-}1.3}
\newcommand{\hlMsRetFTwoOemCILo}{\ensuremath{-}3.1}
\newcommand{\hlMsRetFTwoOemCIHi}{0.4}
\newcommand{\hlMsVerdictHFiveOem}{Equivalent}
\newcommand{\hlMsMarginHFiveOem}{1.4}
\newcommand{\hlHwCtlNSixburnN}{3}
\newcommand{\hlHwCtlNSixburnEst}{\ensuremath{-}1.2}
\newcommand{\hlHwCtlNSixburnCILo}{\ensuremath{-}5.0}
\newcommand{\hlHwCtlNSixburnCIHi}{2.6}
\newcommand{\hlHwCtlNSixburnVerdict}{Undetermined}
\newcommand{\hlHwCtlNSixburnClass}{RTX PRO 6000}
\newcommand{\hlHwCtlNSixburnSeeds}{3, 4 and 5}
\newcommand{\hlHwCtlSettleNSixburnRuns}{7}
\newcommand{\hlHwCtlSettleNSixburnClass}{RTX PRO 6000}
\newcommand{\hlHwCtlArmNSixburnN}{3}
\newcommand{\hlHwCtlArmNSixburnEst}{\ensuremath{-}1.2}
\newcommand{\hlHwCtlArmNSixburnCILo}{\ensuremath{-}5.0}
\newcommand{\hlHwCtlArmNSixburnCIHi}{2.6}
\newcommand{\hlHwCtlArmNSixburnVerdict}{Undetermined}
\newcommand{\hlHwCtlNSixflairN}{2}
\newcommand{\hlHwCtlNSixflairEst}{2.0}
\newcommand{\hlHwCtlNSixflairCILo}{\ensuremath{-}2.0}
\newcommand{\hlHwCtlNSixflairCIHi}{5.9}
\newcommand{\hlHwCtlNSixflairVerdict}{Undetermined}
\newcommand{\hlHwCtlNSixflairClass}{RTX PRO 6000}
\newcommand{\hlHwCtlNSixflairSeeds}{4 and 5}
\newcommand{\hlHwCtlSettleNSixflairRuns}{12}
\newcommand{\hlHwCtlSettleNSixflairClass}{RTX PRO 6000}
\newcommand{\hlHwCtlArmNSixflairN}{3}
\newcommand{\hlHwCtlArmNSixflairEst}{2.0}
\newcommand{\hlHwCtlArmNSixflairCILo}{0.9}
\newcommand{\hlHwCtlArmNSixflairCIHi}{3.0}
\newcommand{\hlHwCtlArmNSixflairVerdict}{Differs}
\newcommand{\hlHwCtlFTwoburnN}{0}
\newcommand{\hlHwCtlFTwoburnEst}{--}
\newcommand{\hlHwCtlFTwoburnCILo}{--}
\newcommand{\hlHwCtlFTwoburnCIHi}{--}
\newcommand{\hlHwCtlFTwoburnVerdict}{No such subset}
\newcommand{\hlHwCtlFTwoburnClass}{none}
\newcommand{\hlHwCtlFTwoburnSeeds}{none}
\newcommand{\hlHwCtlSettleFTwoburnRuns}{25}
\newcommand{\hlHwCtlSettleFTwoburnClass}{RTX 4090}
\newcommand{\hlHwCtlArmFTwoburnN}{8}
\newcommand{\hlHwCtlArmFTwoburnEst}{0.0}
\newcommand{\hlHwCtlArmFTwoburnCILo}{\ensuremath{-}2.2}
\newcommand{\hlHwCtlArmFTwoburnCIHi}{2.1}
\newcommand{\hlHwCtlArmFTwoburnVerdict}{Equivalent}
\newcommand{\hlHwCtlFTwoflairN}{0}
\newcommand{\hlHwCtlFTwoflairEst}{--}
\newcommand{\hlHwCtlFTwoflairCILo}{--}
\newcommand{\hlHwCtlFTwoflairCIHi}{--}
\newcommand{\hlHwCtlFTwoflairVerdict}{No such subset}
\newcommand{\hlHwCtlFTwoflairClass}{none}
\newcommand{\hlHwCtlFTwoflairSeeds}{none}
\newcommand{\hlHwCtlSettleFTwoflairRuns}{25}
\newcommand{\hlHwCtlSettleFTwoflairClass}{RTX 4090}
\newcommand{\hlHwCtlArmFTwoflairN}{5}
\newcommand{\hlHwCtlArmFTwoflairEst}{0.6}
\newcommand{\hlHwCtlArmFTwoflairCILo}{\ensuremath{-}1.4}
\newcommand{\hlHwCtlArmFTwoflairCIHi}{2.5}
\newcommand{\hlHwCtlArmFTwoflairVerdict}{Equivalent}
\newcommand{\hlHwCtlDupGroups}{7}
\newcommand{\hlHwCtlDupRuns}{59}
\newcommand{\hlHwCtlDupClasses}{7}
\newcommand{\hlHwCtlDupAbsN}{278}
\newcommand{\hlHwCtlDupWithinN}{40}
\newcommand{\hlHwCtlDupSignedN}{118}
\newcommand{\hlHwCtlDupAbs}{2.1}
\newcommand{\hlHwCtlDupWithin}{2.8}
\newcommand{\hlHwCtlDupSigned}{0.4}
\newcommand{\hlHwCtlDupRefClass}{RTX PRO 6000}
\newcommand{\hlHwCtlDupEpochs}{2}
\newcommand{\hlHwCtlDupDropGroups}{0}
\newcommand{\hlHwCtlDupDropAbs}{--}
\newcommand{\hlHwCtlDupDropSigned}{--}
\newcommand{\hlHwCtlReplicateRuns}{20}
\newcommand{\hlRealInterpChesEst}{0.2}
\newcommand{\hlRealInterpChesCILo}{\ensuremath{-}0.8}
\newcommand{\hlRealInterpChesCIHi}{1.1}
\newcommand{\hlRealInterpChesTostCILo}{\ensuremath{-}0.6}
\newcommand{\hlRealInterpChesTostCIHi}{0.9}
\newcommand{\hlRealInterpChesMde}{1.5}
\newcommand{\hlRealInterpChesPHolm}{0.739}
\newcommand{\hlRealInterpChesN}{25}
\newcommand{\hlRealInterpShiftChesEst}{8.8}
\newcommand{\hlRealInterpShiftChesCILo}{7.8}
\newcommand{\hlRealInterpShiftChesCIHi}{9.8}
\newcommand{\hlRealInterpShiftChesSim}{12.6}
\newcommand{\hlRealInterpShiftChesVerdict}{the real label costs more}
\newcommand{\hlRealInterpCoarseChesEst}{0.2}
\newcommand{\hlRealInterpCoarseChesCILo}{\ensuremath{-}0.8}
\newcommand{\hlRealInterpCoarseChesCIHi}{1.1}
\newcommand{\hlRealInterpCoarseChesSim}{21.2}
\newcommand{\hlRealInterpCoarseChesVerdict}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlRealInterpChesSim}{21.2}
\newcommand{\hlRealInterpChesVerdict}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlRealInterpBoundaryChesEst}{3.3}
\newcommand{\hlRealInterpBoundaryChesCILo}{1.6}
\newcommand{\hlRealInterpBoundaryChesCIHi}{4.9}
\newcommand{\hlRealInterpBoundaryChesSim}{18.1}
\newcommand{\hlRealInterpBoundaryChesVerdict}{the real label costs more}
\newcommand{\hlRealInterpOmissionChesEst}{5.0}
\newcommand{\hlRealInterpOmissionChesCILo}{1.8}
\newcommand{\hlRealInterpOmissionChesCIHi}{8.3}
\newcommand{\hlRealInterpOmissionChesSim}{16.3}
\newcommand{\hlRealInterpOmissionChesVerdict}{the real label costs more}
\newcommand{\hlRealInterpMeanChesEst}{4.3}
\newcommand{\hlRealInterpMeanChesCILo}{3.1}
\newcommand{\hlRealInterpMeanChesCIHi}{5.5}
\newcommand{\hlRealInterpMeanChesSim}{17.1}
\newcommand{\hlRealInterpMeanChesVerdict}{the real label costs more}
\newcommand{\hlRealInterpChesFlag}{extrapolated}
\newcommand{\hlRealInterpChesGap}{0.13}
\newcommand{\hlRealInterpChesLabelMiou}{0.571}
\newcommand{\hlRealInterpCsTwelveEst}{9.5}
\newcommand{\hlRealInterpCsTwelveCILo}{7.6}
\newcommand{\hlRealInterpCsTwelveCIHi}{11.3}
\newcommand{\hlRealInterpCsTwelveTostCILo}{8.0}
\newcommand{\hlRealInterpCsTwelveTostCIHi}{11.0}
\newcommand{\hlRealInterpCsTwelveMde}{2.9}
\newcommand{\hlRealInterpCsTwelvePHolm}{\ensuremath{<}0.001}
\newcommand{\hlRealInterpCsTwelveN}{25}
\newcommand{\hlRealInterpShiftCsTwelveEst}{16.7}
\newcommand{\hlRealInterpShiftCsTwelveCILo}{15.1}
\newcommand{\hlRealInterpShiftCsTwelveCIHi}{18.3}
\newcommand{\hlRealInterpShiftCsTwelveSim}{15.7}
\newcommand{\hlRealInterpShiftCsTwelveVerdict}{the real label costs more}
\newcommand{\hlRealInterpCoarseCsTwelveEst}{9.5}
\newcommand{\hlRealInterpCoarseCsTwelveCILo}{7.6}
\newcommand{\hlRealInterpCoarseCsTwelveCIHi}{11.3}
\newcommand{\hlRealInterpCoarseCsTwelveSim}{22.9}
\newcommand{\hlRealInterpCoarseCsTwelveVerdict}{the real label costs more}
\newcommand{\hlRealInterpCsTwelveSim}{22.9}
\newcommand{\hlRealInterpCsTwelveVerdict}{the real label costs more}
\newcommand{\hlRealInterpBoundaryCsTwelveEst}{14.0}
\newcommand{\hlRealInterpBoundaryCsTwelveCILo}{11.4}
\newcommand{\hlRealInterpBoundaryCsTwelveCIHi}{16.7}
\newcommand{\hlRealInterpBoundaryCsTwelveSim}{18.3}
\newcommand{\hlRealInterpBoundaryCsTwelveVerdict}{the real label costs more}
\newcommand{\hlRealInterpOmissionCsTwelveEst}{16.2}
\newcommand{\hlRealInterpOmissionCsTwelveCILo}{14.5}
\newcommand{\hlRealInterpOmissionCsTwelveCIHi}{17.8}
\newcommand{\hlRealInterpOmissionCsTwelveSim}{16.2}
\newcommand{\hlRealInterpOmissionCsTwelveVerdict}{the real label costs more}
\newcommand{\hlRealInterpMeanCsTwelveEst}{14.1}
\newcommand{\hlRealInterpMeanCsTwelveCILo}{12.8}
\newcommand{\hlRealInterpMeanCsTwelveCIHi}{15.4}
\newcommand{\hlRealInterpMeanCsTwelveSim}{18.3}
\newcommand{\hlRealInterpMeanCsTwelveVerdict}{the real label costs more}
\newcommand{\hlRealInterpCsTwelveFlag}{extrapolated}
\newcommand{\hlRealInterpCsTwelveGap}{0.37}
\newcommand{\hlRealInterpCsTwelveLabelMiou}{0.331}
\newcommand{\hlRealInterpDfcEst}{3.2}
\newcommand{\hlRealInterpDfcCILo}{2.0}
\newcommand{\hlRealInterpDfcCIHi}{4.5}
\newcommand{\hlRealInterpDfcTostCILo}{2.2}
\newcommand{\hlRealInterpDfcTostCIHi}{4.3}
\newcommand{\hlRealInterpDfcMde}{2.0}
\newcommand{\hlRealInterpDfcPHolm}{\ensuremath{<}0.001}
\newcommand{\hlRealInterpDfcN}{25}
\newcommand{\hlRealInterpShiftDfcEst}{4.7}
\newcommand{\hlRealInterpShiftDfcCILo}{3.5}
\newcommand{\hlRealInterpShiftDfcCIHi}{5.9}
\newcommand{\hlRealInterpShiftDfcSim}{0.1}
\newcommand{\hlRealInterpShiftDfcVerdict}{the real label costs more}
\newcommand{\hlRealInterpCoarseDfcEst}{3.2}
\newcommand{\hlRealInterpCoarseDfcCILo}{2.0}
\newcommand{\hlRealInterpCoarseDfcCIHi}{4.5}
\newcommand{\hlRealInterpCoarseDfcSim}{1.5}
\newcommand{\hlRealInterpCoarseDfcVerdict}{the real label costs more}
\newcommand{\hlRealInterpDfcSim}{1.5}
\newcommand{\hlRealInterpDfcVerdict}{the real label costs more}
\newcommand{\hlRealInterpBoundaryDfcEst}{0.0}
\newcommand{\hlRealInterpBoundaryDfcCILo}{\ensuremath{-}1.5}
\newcommand{\hlRealInterpBoundaryDfcCIHi}{1.5}
\newcommand{\hlRealInterpBoundaryDfcSim}{4.8}
\newcommand{\hlRealInterpBoundaryDfcVerdict}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlRealInterpOmissionDfcEst}{0.9}
\newcommand{\hlRealInterpOmissionDfcCILo}{\ensuremath{-}0.5}
\newcommand{\hlRealInterpOmissionDfcCIHi}{2.4}
\newcommand{\hlRealInterpOmissionDfcSim}{3.8}
\newcommand{\hlRealInterpOmissionDfcVerdict}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlRealInterpMeanDfcEst}{2.2}
\newcommand{\hlRealInterpMeanDfcCILo}{1.1}
\newcommand{\hlRealInterpMeanDfcCIHi}{3.3}
\newcommand{\hlRealInterpMeanDfcSim}{2.6}
\newcommand{\hlRealInterpMeanDfcVerdict}{the real label costs more}
\newcommand{\hlRealInterpDfcFlag}{extrapolated}
\newcommand{\hlRealInterpDfcGap}{0.03}
\newcommand{\hlRealInterpDfcLabelMiou}{0.675}
\newcommand{\hlRealInterpEnvaEst}{15.4}
\newcommand{\hlRealInterpEnvaCILo}{11.6}
\newcommand{\hlRealInterpEnvaCIHi}{19.2}
\newcommand{\hlRealInterpEnvaTostCILo}{12.2}
\newcommand{\hlRealInterpEnvaTostCIHi}{18.6}
\newcommand{\hlRealInterpEnvaMde}{6.0}
\newcommand{\hlRealInterpEnvaPHolm}{\ensuremath{<}0.001}
\newcommand{\hlRealInterpEnvaN}{25}
\newcommand{\hlRealInterpShiftEnvaEst}{15.9}
\newcommand{\hlRealInterpShiftEnvaCILo}{11.5}
\newcommand{\hlRealInterpShiftEnvaCIHi}{20.4}
\newcommand{\hlRealInterpShiftEnvaSim}{8.7}
\newcommand{\hlRealInterpShiftEnvaVerdict}{the real label costs more}
\newcommand{\hlRealInterpCoarseEnvaEst}{15.4}
\newcommand{\hlRealInterpCoarseEnvaCILo}{11.6}
\newcommand{\hlRealInterpCoarseEnvaCIHi}{19.2}
\newcommand{\hlRealInterpCoarseEnvaSim}{9.2}
\newcommand{\hlRealInterpCoarseEnvaVerdict}{the real label costs more}
\newcommand{\hlRealInterpEnvaSim}{9.2}
\newcommand{\hlRealInterpEnvaVerdict}{the real label costs more}
\newcommand{\hlRealInterpBoundaryEnvaEst}{4.8}
\newcommand{\hlRealInterpBoundaryEnvaCILo}{\ensuremath{-}1.7}
\newcommand{\hlRealInterpBoundaryEnvaCIHi}{11.3}
\newcommand{\hlRealInterpBoundaryEnvaSim}{19.8}
\newcommand{\hlRealInterpBoundaryEnvaVerdict}{Undetermined, MDE 10.3}
\newcommand{\hlRealInterpOmissionEnvaEst}{\ensuremath{-}1.4}
\newcommand{\hlRealInterpOmissionEnvaCILo}{\ensuremath{-}8.6}
\newcommand{\hlRealInterpOmissionEnvaCIHi}{5.8}
\newcommand{\hlRealInterpOmissionEnvaSim}{26.0}
\newcommand{\hlRealInterpOmissionEnvaVerdict}{Undetermined, MDE 11.4}
\newcommand{\hlRealInterpMeanEnvaEst}{8.7}
\newcommand{\hlRealInterpMeanEnvaCILo}{5.6}
\newcommand{\hlRealInterpMeanEnvaCIHi}{11.8}
\newcommand{\hlRealInterpMeanEnvaSim}{15.9}
\newcommand{\hlRealInterpMeanEnvaVerdict}{the real label costs more}
\newcommand{\hlRealInterpEnvaFlag}{extrapolated}
\newcommand{\hlRealInterpEnvaGap}{0.22}
\newcommand{\hlRealInterpEnvaLabelMiou}{0.483}
\newcommand{\hlRealInterpKuroEst}{0.7}
\newcommand{\hlRealInterpKuroCILo}{\ensuremath{-}1.0}
\newcommand{\hlRealInterpKuroCIHi}{2.5}
\newcommand{\hlRealInterpKuroTostCILo}{\ensuremath{-}0.7}
\newcommand{\hlRealInterpKuroTostCIHi}{2.2}
\newcommand{\hlRealInterpKuroMde}{2.8}
\newcommand{\hlRealInterpKuroPHolm}{0.410}
\newcommand{\hlRealInterpKuroN}{25}
\newcommand{\hlRealInterpShiftKuroEst}{\ensuremath{-}0.6}
\newcommand{\hlRealInterpShiftKuroCILo}{\ensuremath{-}2.3}
\newcommand{\hlRealInterpShiftKuroCIHi}{1.1}
\newcommand{\hlRealInterpShiftKuroSim}{1.4}
\newcommand{\hlRealInterpShiftKuroVerdict}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlRealInterpCoarseKuroEst}{0.7}
\newcommand{\hlRealInterpCoarseKuroCILo}{\ensuremath{-}1.0}
\newcommand{\hlRealInterpCoarseKuroCIHi}{2.5}
\newcommand{\hlRealInterpCoarseKuroSim}{0.0}
\newcommand{\hlRealInterpCoarseKuroVerdict}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlRealInterpKuroSim}{0.0}
\newcommand{\hlRealInterpKuroVerdict}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlRealInterpBoundaryKuroEst}{\ensuremath{-}0.2}
\newcommand{\hlRealInterpBoundaryKuroCILo}{\ensuremath{-}1.8}
\newcommand{\hlRealInterpBoundaryKuroCIHi}{1.5}
\newcommand{\hlRealInterpBoundaryKuroSim}{0.9}
\newcommand{\hlRealInterpBoundaryKuroVerdict}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlRealInterpOmissionKuroEst}{\ensuremath{-}1.6}
\newcommand{\hlRealInterpOmissionKuroCILo}{\ensuremath{-}3.3}
\newcommand{\hlRealInterpOmissionKuroCIHi}{0.1}
\newcommand{\hlRealInterpOmissionKuroSim}{2.3}
\newcommand{\hlRealInterpOmissionKuroVerdict}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlRealInterpMeanKuroEst}{\ensuremath{-}0.4}
\newcommand{\hlRealInterpMeanKuroCILo}{\ensuremath{-}2.0}
\newcommand{\hlRealInterpMeanKuroCIHi}{1.2}
\newcommand{\hlRealInterpMeanKuroSim}{1.2}
\newcommand{\hlRealInterpMeanKuroVerdict}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlRealInterpKuroFlag}{interpolated}
\newcommand{\hlRealInterpKuroGap}{0.00}
\newcommand{\hlRealInterpKuroLabelMiou}{0.893}
\newcommand{\hlRankRhoburn}{0.93}
\newcommand{\hlRankRhoCILoburn}{0.82}
\newcommand{\hlRankRhoCIHiburn}{0.97}
\newcommand{\hlRankTauburn}{0.83}
\newcommand{\hlRankTauCILoburn}{0.67}
\newcommand{\hlRankTauCIHiburn}{0.89}
\newcommand{\hlRankSlopeburn}{0.20}
\newcommand{\hlRankSlopeCILoburn}{0.07}
\newcommand{\hlRankSlopeCIHiburn}{0.34}
\newcommand{\hlRankRhoPburn}{\ensuremath{<}0.001}
\newcommand{\hlRankNburn}{9}
\newcommand{\hlRankRhoflair}{0.98}
\newcommand{\hlRankRhoCILoflair}{0.95}
\newcommand{\hlRankRhoCIHiflair}{0.98}
\newcommand{\hlRankTauflair}{0.94}
\newcommand{\hlRankTauCILoflair}{0.83}
\newcommand{\hlRankTauCIHiflair}{0.94}
\newcommand{\hlRankSlopeflair}{0.08}
\newcommand{\hlRankSlopeCILoflair}{0.04}
\newcommand{\hlRankSlopeCIHiflair}{0.11}
\newcommand{\hlRankRhoPflair}{\ensuremath{<}0.001}
\newcommand{\hlRankNflair}{9}
\newcommand{\hlRankRhoChes}{0.40}
\newcommand{\hlRankRhoCILoChes}{0.30}
\newcommand{\hlRankRhoCIHiChes}{0.70}
\newcommand{\hlRankTauChes}{0.40}
\newcommand{\hlRankTauCILoChes}{0.20}
\newcommand{\hlRankTauCIHiChes}{0.60}
\newcommand{\hlRankSlopeChes}{0.13}
\newcommand{\hlRankSlopeCILoChes}{\ensuremath{-}0.12}
\newcommand{\hlRankSlopeCIHiChes}{0.33}
\newcommand{\hlRankRhoPChes}{0.258}
\newcommand{\hlRankNChes}{5}
\newcommand{\hlRankRhoCsTwelve}{1.00}
\newcommand{\hlRankRhoCILoCsTwelve}{0.80}
\newcommand{\hlRankRhoCIHiCsTwelve}{1.00}
\newcommand{\hlRankTauCsTwelve}{1.00}
\newcommand{\hlRankTauCILoCsTwelve}{0.60}
\newcommand{\hlRankTauCIHiCsTwelve}{1.00}
\newcommand{\hlRankSlopeCsTwelve}{0.01}
\newcommand{\hlRankSlopeCILoCsTwelve}{\ensuremath{-}0.11}
\newcommand{\hlRankSlopeCIHiCsTwelve}{0.14}
\newcommand{\hlRankRhoPCsTwelve}{0.008}
\newcommand{\hlRankNCsTwelve}{5}
\newcommand{\hlRankRhoDfc}{0.90}
\newcommand{\hlRankRhoCILoDfc}{0.50}
\newcommand{\hlRankRhoCIHiDfc}{1.00}
\newcommand{\hlRankTauDfc}{0.80}
\newcommand{\hlRankTauCILoDfc}{0.40}
\newcommand{\hlRankTauCIHiDfc}{1.00}
\newcommand{\hlRankSlopeDfc}{0.18}
\newcommand{\hlRankSlopeCILoDfc}{\ensuremath{-}0.04}
\newcommand{\hlRankSlopeCIHiDfc}{0.41}
\newcommand{\hlRankRhoPDfc}{0.042}
\newcommand{\hlRankNDfc}{5}
\newcommand{\hlRankRhoEnva}{0.50}
\newcommand{\hlRankRhoCILoEnva}{0.50}
\newcommand{\hlRankRhoCIHiEnva}{1.00}
\newcommand{\hlRankTauEnva}{0.20}
\newcommand{\hlRankTauCILoEnva}{0.20}
\newcommand{\hlRankTauCIHiEnva}{1.00}
\newcommand{\hlRankSlopeEnva}{\ensuremath{-}0.06}
\newcommand{\hlRankSlopeCILoEnva}{\ensuremath{-}0.18}
\newcommand{\hlRankSlopeCIHiEnva}{0.08}
\newcommand{\hlRankRhoPEnva}{0.225}
\newcommand{\hlRankNEnva}{5}
\newcommand{\hlRankRhoSnTwo}{1.00}
\newcommand{\hlRankRhoCILoSnTwo}{0.90}
\newcommand{\hlRankRhoCIHiSnTwo}{1.00}
\newcommand{\hlRankTauSnTwo}{1.00}
\newcommand{\hlRankTauCILoSnTwo}{0.80}
\newcommand{\hlRankTauCIHiSnTwo}{1.00}
\newcommand{\hlRankSlopeSnTwo}{\ensuremath{-}0.65}
\newcommand{\hlRankSlopeCILoSnTwo}{\ensuremath{-}1.12}
\newcommand{\hlRankSlopeCIHiSnTwo}{\ensuremath{-}0.27}
\newcommand{\hlRankRhoPSnTwo}{0.008}
\newcommand{\hlRankNSnTwo}{5}
\newcommand{\hlRankRhoKuro}{1.00}
\newcommand{\hlRankRhoCILoKuro}{0.90}
\newcommand{\hlRankRhoCIHiKuro}{1.00}
\newcommand{\hlRankTauKuro}{1.00}
\newcommand{\hlRankTauCILoKuro}{0.80}
\newcommand{\hlRankTauCIHiKuro}{1.00}
\newcommand{\hlRankSlopeKuro}{0.26}
\newcommand{\hlRankSlopeCILoKuro}{0.14}
\newcommand{\hlRankSlopeCIHiKuro}{0.35}
\newcommand{\hlRankRhoPKuro}{0.008}
\newcommand{\hlRankNKuro}{5}
\newcommand{\hlRankRhoOem}{0.90}
\newcommand{\hlRankRhoCILoOem}{0.80}
\newcommand{\hlRankRhoCIHiOem}{1.00}
\newcommand{\hlRankTauOem}{0.80}
\newcommand{\hlRankTauCILoOem}{0.60}
\newcommand{\hlRankTauCIHiOem}{1.00}
\newcommand{\hlRankSlopeOem}{0.19}
\newcommand{\hlRankSlopeCILoOem}{0.13}
\newcommand{\hlRankSlopeCIHiOem}{0.25}
\newcommand{\hlRankRhoPOem}{0.042}
\newcommand{\hlRankNOem}{5}
\newcommand{\hlRankRhoCore}{0.96}
\newcommand{\hlRankRhoCILoCore}{0.90}
\newcommand{\hlRankRhoCIHiCore}{0.97}
\newcommand{\hlRankTauCore}{0.89}
\newcommand{\hlRankTauCILoCore}{0.78}
\newcommand{\hlRankTauCIHiCore}{0.92}
\newcommand{\hlRankSlopeCore}{0.14}
\newcommand{\hlRankSlopeCILoCore}{0.07}
\newcommand{\hlRankSlopeCIHiCore}{0.21}
\newcommand{\hlRankNCore}{18}
\newcommand{\hlRankRhoPooled}{0.85}
\newcommand{\hlRankRhoCILoPooled}{0.80}
\newcommand{\hlRankRhoCIHiPooled}{0.92}
\newcommand{\hlRankTauPooled}{0.78}
\newcommand{\hlRankTauCILoPooled}{0.70}
\newcommand{\hlRankTauCIHiPooled}{0.87}
\newcommand{\hlRankSlopePooled}{0.04}
\newcommand{\hlRankSlopeCILoPooled}{\ensuremath{-}0.03}
\newcommand{\hlRankSlopeCIHiPooled}{0.10}
\newcommand{\hlRankNPooled}{53}
\newcommand{\hlRankDsPooled}{9}
\newcommand{\hlRealLmChesEst}{\ensuremath{-}1.4}
\newcommand{\hlRealLmChesCILo}{\ensuremath{-}2.3}
\newcommand{\hlRealLmChesCIHi}{\ensuremath{-}0.4}
\newcommand{\hlRealLmChesTostCILo}{\ensuremath{-}2.2}
\newcommand{\hlRealLmChesTostCIHi}{\ensuremath{-}0.6}
\newcommand{\hlRealLmChesMde}{1.5}
\newcommand{\hlRealLmChesN}{25}
\newcommand{\hlRealLmChesReal}{21.4}
\newcommand{\hlRealLmChesSim}{22.7}
\newcommand{\hlRealLmChesVerdict}{Equivalent within $\pm$\TostMargin, the real label costs less}
\newcommand{\hlRealLmChesType}{coarse}
\newcommand{\hlRealLmChesLabelMiou}{0.574}
\newcommand{\hlRealLmChesLabelMiouLo}{0.571}
\newcommand{\hlRealLmChesLabelMiouHi}{0.576}
\newcommand{\hlRealLmChesRealLabelMiou}{0.571}
\newcommand{\hlRealLmCsTwelveEst}{\ensuremath{-}0.3}
\newcommand{\hlRealLmCsTwelveCILo}{\ensuremath{-}2.4}
\newcommand{\hlRealLmCsTwelveCIHi}{1.7}
\newcommand{\hlRealLmCsTwelveTostCILo}{\ensuremath{-}2.0}
\newcommand{\hlRealLmCsTwelveTostCIHi}{1.4}
\newcommand{\hlRealLmCsTwelveMde}{3.2}
\newcommand{\hlRealLmCsTwelveN}{25}
\newcommand{\hlRealLmCsTwelveReal}{32.4}
\newcommand{\hlRealLmCsTwelveSim}{32.7}
\newcommand{\hlRealLmCsTwelveVerdict}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlRealLmCsTwelveType}{omission}
\newcommand{\hlRealLmCsTwelveLabelMiou}{0.331}
\newcommand{\hlRealLmCsTwelveLabelMiouLo}{0.324}
\newcommand{\hlRealLmCsTwelveLabelMiouHi}{0.348}
\newcommand{\hlRealLmCsTwelveRealLabelMiou}{0.331}
\newcommand{\hlRealLmDfcEst}{3.2}
\newcommand{\hlRealLmDfcCILo}{1.9}
\newcommand{\hlRealLmDfcCIHi}{4.4}
\newcommand{\hlRealLmDfcTostCILo}{2.1}
\newcommand{\hlRealLmDfcTostCIHi}{4.2}
\newcommand{\hlRealLmDfcMde}{2.0}
\newcommand{\hlRealLmDfcN}{25}
\newcommand{\hlRealLmDfcReal}{4.8}
\newcommand{\hlRealLmDfcSim}{1.6}
\newcommand{\hlRealLmDfcVerdict}{the real label costs more}
\newcommand{\hlRealLmDfcType}{coarse}
\newcommand{\hlRealLmDfcLabelMiou}{0.676}
\newcommand{\hlRealLmDfcLabelMiouLo}{0.676}
\newcommand{\hlRealLmDfcLabelMiouHi}{0.676}
\newcommand{\hlRealLmDfcRealLabelMiou}{0.675}
\newcommand{\hlRealLmEnvaEst}{8.8}
\newcommand{\hlRealLmEnvaCILo}{5.7}
\newcommand{\hlRealLmEnvaCIHi}{11.8}
\newcommand{\hlRealLmEnvaTostCILo}{6.2}
\newcommand{\hlRealLmEnvaTostCIHi}{11.3}
\newcommand{\hlRealLmEnvaMde}{4.8}
\newcommand{\hlRealLmEnvaN}{25}
\newcommand{\hlRealLmEnvaReal}{24.6}
\newcommand{\hlRealLmEnvaSim}{15.9}
\newcommand{\hlRealLmEnvaVerdict}{the real label costs more}
\newcommand{\hlRealLmEnvaType}{coarse}
\newcommand{\hlRealLmEnvaLabelMiou}{0.485}
\newcommand{\hlRealLmEnvaLabelMiouLo}{0.483}
\newcommand{\hlRealLmEnvaLabelMiouHi}{0.489}
\newcommand{\hlRealLmEnvaRealLabelMiou}{0.483}
\newcommand{\hlRealLmKuroEst}{\ensuremath{-}0.5}
\newcommand{\hlRealLmKuroCILo}{\ensuremath{-}2.0}
\newcommand{\hlRealLmKuroCIHi}{1.1}
\newcommand{\hlRealLmKuroTostCILo}{\ensuremath{-}1.8}
\newcommand{\hlRealLmKuroTostCIHi}{0.8}
\newcommand{\hlRealLmKuroMde}{2.5}
\newcommand{\hlRealLmKuroN}{25}
\newcommand{\hlRealLmKuroReal}{0.8}
\newcommand{\hlRealLmKuroSim}{1.2}
\newcommand{\hlRealLmKuroVerdict}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlRealLmKuroType}{coarse}
\newcommand{\hlRealLmKuroLabelMiou}{0.898}
\newcommand{\hlRealLmKuroLabelMiouLo}{0.897}
\newcommand{\hlRealLmKuroLabelMiouHi}{0.899}
\newcommand{\hlRealLmKuroRealLabelMiou}{0.893}
\newcommand{\hlRealLmBoundaryKuroEst}{0.3}
\newcommand{\hlRealLmBoundaryKuroCILo}{\ensuremath{-}1.1}
\newcommand{\hlRealLmBoundaryKuroCIHi}{1.7}
\newcommand{\hlRealLmBoundaryKuroTostCILo}{\ensuremath{-}0.8}
\newcommand{\hlRealLmBoundaryKuroTostCIHi}{1.5}
\newcommand{\hlRealLmBoundaryKuroMde}{2.2}
\newcommand{\hlRealLmBoundaryKuroN}{25}
\newcommand{\hlRealLmBoundaryKuroReal}{0.8}
\newcommand{\hlRealLmBoundaryKuroSim}{0.4}
\newcommand{\hlRealLmBoundaryKuroVerdict}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlRealLmBoundaryKuroType}{boundary}
\newcommand{\hlRealLmBoundaryKuroLabelMiou}{0.895}
\newcommand{\hlRealLmBoundaryKuroLabelMiouLo}{0.893}
\newcommand{\hlRealLmBoundaryKuroLabelMiouHi}{0.897}
\newcommand{\hlRealLmBoundaryKuroRealLabelMiou}{0.893}
\newcommand{\hlRealLmRead}{5}
\newcommand{\hlRealLmEquiv}{3}
\newcommand{\hlRealLmRealMore}{2}
\newcommand{\hlRealLmTotal}{5}
\newcommand{\hlHwRepCleanburnSigned}{0.80}
\newcommand{\hlHwRepCleanburnSignedCILo}{\ensuremath{-}0.70}
\newcommand{\hlHwRepCleanburnSignedCIHi}{2.30}
\newcommand{\hlHwRepCleanburnAbs}{0.98}
\newcommand{\hlHwRepCleanburnAbsCILo}{\ensuremath{-}0.38}
\newcommand{\hlHwRepCleanburnAbsCIHi}{2.33}
\newcommand{\hlHwRepCleanburnMax}{2.70}
\newcommand{\hlHwRepCleanburnN}{6}
\newcommand{\hlHwRepNoisyburnSigned}{\ensuremath{-}0.37}
\newcommand{\hlHwRepNoisyburnSignedCILo}{\ensuremath{-}1.51}
\newcommand{\hlHwRepNoisyburnSignedCIHi}{0.77}
\newcommand{\hlHwRepNoisyburnAbs}{2.23}
\newcommand{\hlHwRepNoisyburnAbsCILo}{1.59}
\newcommand{\hlHwRepNoisyburnAbsCIHi}{2.87}
\newcommand{\hlHwRepNoisyburnMax}{5.65}
\newcommand{\hlHwRepNoisyburnN}{24}
\newcommand{\hlHwRepDropburnSigned}{1.17}
\newcommand{\hlHwRepDropburnSignedCILo}{\ensuremath{-}0.04}
\newcommand{\hlHwRepDropburnSignedCIHi}{2.38}
\newcommand{\hlHwRepDropburnAbs}{2.26}
\newcommand{\hlHwRepDropburnAbsCILo}{1.38}
\newcommand{\hlHwRepDropburnAbsCIHi}{3.13}
\newcommand{\hlHwRepDropburnMax}{6.69}
\newcommand{\hlHwRepDropburnN}{24}
\newcommand{\hlHwRepRunsburn}{30}
\newcommand{\hlHwRepPlannedburn}{30}
\newcommand{\hlHwRepNSixburnRep}{0.15}
\newcommand{\hlHwRepNSixburnRepCILo}{\ensuremath{-}0.95}
\newcommand{\hlHwRepNSixburnRepCIHi}{1.25}
\newcommand{\hlHwRepNSixburnRepTostCILo}{\ensuremath{-}0.60}
\newcommand{\hlHwRepNSixburnRepTostCIHi}{0.90}
\newcommand{\hlHwRepNSixburnOrig}{\ensuremath{-}1.22}
\newcommand{\hlHwRepNSixburnOrigCILo}{\ensuremath{-}6.83}
\newcommand{\hlHwRepNSixburnOrigCIHi}{4.38}
\newcommand{\hlHwRepNSixburnOrigTostCILo}{\ensuremath{-}5.03}
\newcommand{\hlHwRepNSixburnOrigTostCIHi}{2.58}
\newcommand{\hlHwRepNSixburnDiff}{1.37}
\newcommand{\hlHwRepNSixburnDiffMax}{3.50}
\newcommand{\hlHwRepNSixburnN}{3}
\newcommand{\hlHwRepNSixburnSeeds}{3, 4, 5}
\newcommand{\hlHwRepCleanflairSigned}{0.14}
\newcommand{\hlHwRepCleanflairSignedCILo}{\ensuremath{-}1.09}
\newcommand{\hlHwRepCleanflairSignedCIHi}{1.38}
\newcommand{\hlHwRepCleanflairAbs}{0.53}
\newcommand{\hlHwRepCleanflairAbsCILo}{\ensuremath{-}0.26}
\newcommand{\hlHwRepCleanflairAbsCIHi}{1.33}
\newcommand{\hlHwRepCleanflairMax}{1.14}
\newcommand{\hlHwRepCleanflairN}{4}
\newcommand{\hlHwRepNoisyflairSigned}{0.27}
\newcommand{\hlHwRepNoisyflairSignedCILo}{\ensuremath{-}0.06}
\newcommand{\hlHwRepNoisyflairSignedCIHi}{0.61}
\newcommand{\hlHwRepNoisyflairAbs}{0.47}
\newcommand{\hlHwRepNoisyflairAbsCILo}{0.21}
\newcommand{\hlHwRepNoisyflairAbsCIHi}{0.73}
\newcommand{\hlHwRepNoisyflairMax}{1.78}
\newcommand{\hlHwRepNoisyflairN}{16}
\newcommand{\hlHwRepDropflairSigned}{\ensuremath{-}0.13}
\newcommand{\hlHwRepDropflairSignedCILo}{\ensuremath{-}0.64}
\newcommand{\hlHwRepDropflairSignedCIHi}{0.38}
\newcommand{\hlHwRepDropflairAbs}{0.74}
\newcommand{\hlHwRepDropflairAbsCILo}{0.42}
\newcommand{\hlHwRepDropflairAbsCIHi}{1.05}
\newcommand{\hlHwRepDropflairMax}{2.50}
\newcommand{\hlHwRepDropflairN}{16}
\newcommand{\hlHwRepRunsflair}{20}
\newcommand{\hlHwRepPlannedflair}{20}
\newcommand{\hlHwRepNSixflairRep}{0.73}
\newcommand{\hlHwRepNSixflairRepCILo}{0.00}
\newcommand{\hlHwRepNSixflairRepCIHi}{1.46}
\newcommand{\hlHwRepNSixflairRepTostCILo}{0.37}
\newcommand{\hlHwRepNSixflairRepTostCIHi}{1.09}
\newcommand{\hlHwRepNSixflairOrig}{1.97}
\newcommand{\hlHwRepNSixflairOrigCILo}{\ensuremath{-}6.01}
\newcommand{\hlHwRepNSixflairOrigCIHi}{9.96}
\newcommand{\hlHwRepNSixflairOrigTostCILo}{\ensuremath{-}1.99}
\newcommand{\hlHwRepNSixflairOrigTostCIHi}{5.94}
\newcommand{\hlHwRepNSixflairDiff}{\ensuremath{-}1.24}
\newcommand{\hlHwRepNSixflairDiffMax}{1.93}
\newcommand{\hlHwRepNSixflairN}{2}
\newcommand{\hlHwRepNSixflairSeeds}{4, 5}
\newcommand{\hlHwRepCleanPooledSigned}{0.54}
\newcommand{\hlHwRepCleanPooledSignedCILo}{\ensuremath{-}0.33}
\newcommand{\hlHwRepCleanPooledSignedCIHi}{1.40}
\newcommand{\hlHwRepCleanPooledAbs}{0.80}
\newcommand{\hlHwRepCleanPooledAbsCILo}{0.06}
\newcommand{\hlHwRepCleanPooledAbsCIHi}{1.54}
\newcommand{\hlHwRepCleanPooledMax}{2.70}
\newcommand{\hlHwRepCleanPooledN}{10}
\newcommand{\hlHwRepNoisyPooledSigned}{\ensuremath{-}0.11}
\newcommand{\hlHwRepNoisyPooledSignedCILo}{\ensuremath{-}0.80}
\newcommand{\hlHwRepNoisyPooledSignedCIHi}{0.57}
\newcommand{\hlHwRepNoisyPooledAbs}{1.53}
\newcommand{\hlHwRepNoisyPooledAbsCILo}{1.05}
\newcommand{\hlHwRepNoisyPooledAbsCIHi}{2.00}
\newcommand{\hlHwRepNoisyPooledMax}{5.65}
\newcommand{\hlHwRepNoisyPooledN}{40}
\newcommand{\hlHwRepDropPooledSigned}{0.65}
\newcommand{\hlHwRepDropPooledSignedCILo}{\ensuremath{-}0.11}
\newcommand{\hlHwRepDropPooledSignedCIHi}{1.40}
\newcommand{\hlHwRepDropPooledAbs}{1.65}
\newcommand{\hlHwRepDropPooledAbsCILo}{1.07}
\newcommand{\hlHwRepDropPooledAbsCIHi}{2.22}
\newcommand{\hlHwRepDropPooledMax}{6.69}
\newcommand{\hlHwRepDropPooledN}{40}
\newcommand{\hlHwRepRunsPooled}{50}
\newcommand{\hlHwRepPlannedPooled}{50}
\newcommand{\hlHwRepClass}{H100 NVL}
\newcommand{\hlHwRepOrigClass}{RTX PRO 6000}
\newcommand{\hlVarShiftFixedburnEst}{1.6}
\newcommand{\hlVarShiftFixedburnCILo}{0.4}
\newcommand{\hlVarShiftFixedburnCIHi}{2.8}
\newcommand{\hlVarShiftFixedburnTostCILo}{0.6}
\newcommand{\hlVarShiftFixedburnTostCIHi}{2.6}
\newcommand{\hlVarShiftFixedburnMde}{1.9}
\newcommand{\hlVarShiftFixedburnN}{25}
\newcommand{\hlVarShiftFixedburnVar}{13.0}
\newcommand{\hlVarShiftFixedburnBase}{11.4}
\newcommand{\hlVarShiftFixedburnVerdict}{Equivalent within $\pm$\TostMargin, the one-sided variant costs more}
\newcommand{\hlVarBoundaryDilateburnEst}{5.4}
\newcommand{\hlVarBoundaryDilateburnCILo}{3.8}
\newcommand{\hlVarBoundaryDilateburnCIHi}{7.1}
\newcommand{\hlVarBoundaryDilateburnTostCILo}{4.1}
\newcommand{\hlVarBoundaryDilateburnTostCIHi}{6.8}
\newcommand{\hlVarBoundaryDilateburnMde}{2.6}
\newcommand{\hlVarBoundaryDilateburnN}{25}
\newcommand{\hlVarBoundaryDilateburnVar}{18.8}
\newcommand{\hlVarBoundaryDilateburnBase}{13.4}
\newcommand{\hlVarBoundaryDilateburnVerdict}{the one-sided variant costs more}
\newcommand{\hlVarRankburnOne}{coarse}
\newcommand{\hlVarRankburnTwo}{omission}
\newcommand{\hlVarRankburnThree}{boundary dilation}
\newcommand{\hlVarRankburnFour}{fixed shift}
\newcommand{\hlVarDropShiftFixedburn}{13.0}
\newcommand{\hlVarDropCoarseburn}{19.1}
\newcommand{\hlVarDropBoundaryDilateburn}{18.8}
\newcommand{\hlVarDropOmissionburn}{19.0}
\newcommand{\hlVarLeastburn}{fixed shift}
\newcommand{\hlVarShiftLeastburn}{yes}
\newcommand{\hlVarBaseLeastburn}{shift}
\newcommand{\hlVarRankSameburn}{yes}
\newcommand{\hlVarGfmLeastburn}{fixed shift}
\newcommand{\hlVarGfmShiftLeastburn}{yes}
\newcommand{\hlVarShiftFixedflairEst}{0.9}
\newcommand{\hlVarShiftFixedflairCILo}{0.4}
\newcommand{\hlVarShiftFixedflairCIHi}{1.4}
\newcommand{\hlVarShiftFixedflairTostCILo}{0.5}
\newcommand{\hlVarShiftFixedflairTostCIHi}{1.3}
\newcommand{\hlVarShiftFixedflairMde}{0.8}
\newcommand{\hlVarShiftFixedflairN}{25}
\newcommand{\hlVarShiftFixedflairVar}{4.2}
\newcommand{\hlVarShiftFixedflairBase}{3.3}
\newcommand{\hlVarShiftFixedflairVerdict}{Equivalent within $\pm$\TostMargin, the one-sided variant costs more}
\newcommand{\hlVarBoundaryDilateflairEst}{\ensuremath{-}0.1}
\newcommand{\hlVarBoundaryDilateflairCILo}{\ensuremath{-}0.7}
\newcommand{\hlVarBoundaryDilateflairCIHi}{0.6}
\newcommand{\hlVarBoundaryDilateflairTostCILo}{\ensuremath{-}0.6}
\newcommand{\hlVarBoundaryDilateflairTostCIHi}{0.5}
\newcommand{\hlVarBoundaryDilateflairMde}{1.0}
\newcommand{\hlVarBoundaryDilateflairN}{25}
\newcommand{\hlVarBoundaryDilateflairVar}{5.1}
\newcommand{\hlVarBoundaryDilateflairBase}{5.2}
\newcommand{\hlVarBoundaryDilateflairVerdict}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlVarRankflairOne}{coarse}
\newcommand{\hlVarRankflairTwo}{boundary dilation}
\newcommand{\hlVarRankflairThree}{omission}
\newcommand{\hlVarRankflairFour}{fixed shift}
\newcommand{\hlVarDropShiftFixedflair}{4.2}
\newcommand{\hlVarDropCoarseflair}{5.5}
\newcommand{\hlVarDropBoundaryDilateflair}{5.1}
\newcommand{\hlVarDropOmissionflair}{5.0}
\newcommand{\hlVarLeastflair}{fixed shift}
\newcommand{\hlVarShiftLeastflair}{yes}
\newcommand{\hlVarBaseLeastflair}{shift}
\newcommand{\hlVarRankSameflair}{yes}
\newcommand{\hlVarGfmLeastflair}{fixed shift}
\newcommand{\hlVarGfmShiftLeastflair}{yes}
\newcommand{\hlVarRankRead}{2}
\newcommand{\hlVarShiftLeastCount}{2}
\newcommand{\hlRankNineChesRho}{0.77}
\newcommand{\hlRankNineChesRhoCILo}{0.72}
\newcommand{\hlRankNineChesRhoCIHi}{0.88}
\newcommand{\hlRankNineChesTau}{0.67}
\newcommand{\hlRankNineChesRhoP}{0.011}
\newcommand{\hlRankNineChesN}{9}
\newcommand{\hlRankNineCsTwelveRho}{1.00}
\newcommand{\hlRankNineCsTwelveRhoCILo}{0.95}
\newcommand{\hlRankNineCsTwelveRhoCIHi}{1.00}
\newcommand{\hlRankNineCsTwelveTau}{1.00}
\newcommand{\hlRankNineCsTwelveRhoP}{\ensuremath{<}0.001}
\newcommand{\hlRankNineCsTwelveN}{9}
\newcommand{\hlRankNineDfcRho}{0.97}
\newcommand{\hlRankNineDfcRhoCILo}{0.83}
\newcommand{\hlRankNineDfcRhoCIHi}{0.98}
\newcommand{\hlRankNineDfcTau}{0.89}
\newcommand{\hlRankNineDfcRhoP}{\ensuremath{<}0.001}
\newcommand{\hlRankNineDfcN}{9}
\newcommand{\hlRankNineEnvaRho}{0.65}
\newcommand{\hlRankNineEnvaRhoCILo}{0.45}
\newcommand{\hlRankNineEnvaRhoCIHi}{0.93}
\newcommand{\hlRankNineEnvaTau}{0.44}
\newcommand{\hlRankNineEnvaRhoP}{0.034}
\newcommand{\hlRankNineEnvaN}{9}
\newcommand{\hlRankNineSnTwoRho}{0.90}
\newcommand{\hlRankNineSnTwoRhoCILo}{0.88}
\newcommand{\hlRankNineSnTwoRhoCIHi}{0.98}
\newcommand{\hlRankNineSnTwoTau}{0.78}
\newcommand{\hlRankNineSnTwoRhoP}{0.002}
\newcommand{\hlRankNineSnTwoN}{9}
\newcommand{\hlRankNineKuroRho}{0.98}
\newcommand{\hlRankNineKuroRhoCILo}{0.88}
\newcommand{\hlRankNineKuroRhoCIHi}{1.00}
\newcommand{\hlRankNineKuroTau}{0.94}
\newcommand{\hlRankNineKuroRhoP}{\ensuremath{<}0.001}
\newcommand{\hlRankNineKuroN}{9}
\newcommand{\hlRankNineOemRho}{0.98}
\newcommand{\hlRankNineOemRhoCILo}{0.95}
\newcommand{\hlRankNineOemRhoCIHi}{1.00}
\newcommand{\hlRankNineOemTau}{0.94}
\newcommand{\hlRankNineOemRhoP}{\ensuremath{<}0.001}
\newcommand{\hlRankNineOemN}{9}
\newcommand{\hlRankNinePooledRho}{0.91}
\newcommand{\hlRankNinePooledRhoCILo}{0.87}
\newcommand{\hlRankNinePooledRhoCIHi}{0.94}
\newcommand{\hlRankNinePooledTau}{0.83}
\newcommand{\hlRankNinePooledN}{9}
\newcommand{\hlRankNineRead}{9}
\newcommand{\hlRankNineSepCount}{9}
\newcommand{\hlRankNineInDomChesRho}{0.77}
\newcommand{\hlRankNineInDomChesRhoCILo}{0.72}
\newcommand{\hlRankNineInDomChesRhoCIHi}{0.88}
\newcommand{\hlRankNineInDomChesTau}{0.67}
\newcommand{\hlRankNineInDomChesRhoP}{0.011}
\newcommand{\hlRankNineInDomChesN}{9}
\newcommand{\hlRankNineInDomChesExcluded}{0}
\newcommand{\hlRankNineInDomCsTwelveRho}{1.00}
\newcommand{\hlRankNineInDomCsTwelveRhoCILo}{0.95}
\newcommand{\hlRankNineInDomCsTwelveRhoCIHi}{1.00}
\newcommand{\hlRankNineInDomCsTwelveTau}{1.00}
\newcommand{\hlRankNineInDomCsTwelveRhoP}{\ensuremath{<}0.001}
\newcommand{\hlRankNineInDomCsTwelveN}{9}
\newcommand{\hlRankNineInDomCsTwelveExcluded}{0}
\newcommand{\hlRankNineInDomDfcRho}{0.97}
\newcommand{\hlRankNineInDomDfcRhoCILo}{0.83}
\newcommand{\hlRankNineInDomDfcRhoCIHi}{0.98}
\newcommand{\hlRankNineInDomDfcTau}{0.89}
\newcommand{\hlRankNineInDomDfcRhoP}{\ensuremath{<}0.001}
\newcommand{\hlRankNineInDomDfcN}{9}
\newcommand{\hlRankNineInDomDfcExcluded}{0}
\newcommand{\hlRankNineInDomEnvaRho}{0.65}
\newcommand{\hlRankNineInDomEnvaRhoCILo}{0.45}
\newcommand{\hlRankNineInDomEnvaRhoCIHi}{0.93}
\newcommand{\hlRankNineInDomEnvaTau}{0.44}
\newcommand{\hlRankNineInDomEnvaRhoP}{0.034}
\newcommand{\hlRankNineInDomEnvaN}{9}
\newcommand{\hlRankNineInDomEnvaExcluded}{0}
\newcommand{\hlRankNineInDomSnTwoRho}{0.90}
\newcommand{\hlRankNineInDomSnTwoRhoCILo}{0.88}
\newcommand{\hlRankNineInDomSnTwoRhoCIHi}{0.98}
\newcommand{\hlRankNineInDomSnTwoTau}{0.78}
\newcommand{\hlRankNineInDomSnTwoRhoP}{0.002}
\newcommand{\hlRankNineInDomSnTwoN}{9}
\newcommand{\hlRankNineInDomSnTwoExcluded}{0}
\newcommand{\hlRankNineInDomKuroRho}{1.00}
\newcommand{\hlRankNineInDomKuroRhoCILo}{0.94}
\newcommand{\hlRankNineInDomKuroRhoCIHi}{1.00}
\newcommand{\hlRankNineInDomKuroTau}{1.00}
\newcommand{\hlRankNineInDomKuroRhoP}{0.001}
\newcommand{\hlRankNineInDomKuroN}{6}
\newcommand{\hlRankNineInDomKuroExcluded}{3}
\newcommand{\hlRankNineInDomOemRho}{0.96}
\newcommand{\hlRankNineInDomOemRhoCILo}{0.93}
\newcommand{\hlRankNineInDomOemRhoCIHi}{1.00}
\newcommand{\hlRankNineInDomOemTau}{0.90}
\newcommand{\hlRankNineInDomOemRhoP}{0.001}
\newcommand{\hlRankNineInDomOemN}{7}
\newcommand{\hlRankNineInDomOemExcluded}{2}
\newcommand{\hlRankNineInDomPooledRho}{0.91}
\newcommand{\hlRankNineInDomPooledRhoCILo}{0.87}
\newcommand{\hlRankNineInDomPooledRhoCIHi}{0.94}
\newcommand{\hlRankNineInDomPooledTau}{0.83}
\newcommand{\hlRankNineInDomPooledN}{9}
\newcommand{\hlRankNineInDomRead}{9}
\newcommand{\hlRankNineInDomSepCount}{9}
\newcommand{\hlRankNineTotal}{9}
\newcommand{\hlSThreeDropDOFAChesEst}{\ensuremath{-}1.4}
\newcommand{\hlSThreeDropDOFAChesCILo}{\ensuremath{-}2.2}
\newcommand{\hlSThreeDropDOFAChesCIHi}{\ensuremath{-}0.6}
\newcommand{\hlSThreeDropDOFAChesTostCILo}{\ensuremath{-}2.0}
\newcommand{\hlSThreeDropDOFAChesTostCIHi}{\ensuremath{-}0.8}
\newcommand{\hlSThreeDropDOFAChesMde}{1.3}
\newcommand{\hlSThreeDropDOFAChesN}{5}
\newcommand{\hlSThreeDropDOFAChesA}{10.6}
\newcommand{\hlSThreeDropDOFAChesB}{12.0}
\newcommand{\hlSThreeDropDOFAChesVerdict}{Equivalent within $\pm$\TostMargin, the extension encoder loses less}
\newcommand{\hlSThreeDropDOFAChesFlag}{partial bands}
\newcommand{\hlSThreeDropDOFACsTwelveEst}{\ensuremath{-}1.2}
\newcommand{\hlSThreeDropDOFACsTwelveCILo}{\ensuremath{-}1.7}
\newcommand{\hlSThreeDropDOFACsTwelveCIHi}{\ensuremath{-}0.6}
\newcommand{\hlSThreeDropDOFACsTwelveTostCILo}{\ensuremath{-}1.6}
\newcommand{\hlSThreeDropDOFACsTwelveTostCIHi}{\ensuremath{-}0.7}
\newcommand{\hlSThreeDropDOFACsTwelveMde}{0.9}
\newcommand{\hlSThreeDropDOFACsTwelveN}{5}
\newcommand{\hlSThreeDropDOFACsTwelveA}{6.0}
\newcommand{\hlSThreeDropDOFACsTwelveB}{7.2}
\newcommand{\hlSThreeDropDOFACsTwelveVerdict}{Equivalent within $\pm$\TostMargin, the extension encoder loses less}
\newcommand{\hlSThreeDropDOFACsTwelveFlag}{in domain}
\newcommand{\hlSThreeDropDOFADfcEst}{1.8}
\newcommand{\hlSThreeDropDOFADfcCILo}{\ensuremath{-}0.7}
\newcommand{\hlSThreeDropDOFADfcCIHi}{4.3}
\newcommand{\hlSThreeDropDOFADfcTostCILo}{\ensuremath{-}0.1}
\newcommand{\hlSThreeDropDOFADfcTostCIHi}{3.8}
\newcommand{\hlSThreeDropDOFADfcMde}{4.1}
\newcommand{\hlSThreeDropDOFADfcN}{5}
\newcommand{\hlSThreeDropDOFADfcA}{3.2}
\newcommand{\hlSThreeDropDOFADfcB}{1.4}
\newcommand{\hlSThreeDropDOFADfcVerdict}{Undetermined, MDE 4.1}
\newcommand{\hlSThreeDropDOFADfcFlag}{in domain}
\newcommand{\hlSThreeDropDOFAEnvaEst}{3.8}
\newcommand{\hlSThreeDropDOFAEnvaCILo}{\ensuremath{-}4.2}
\newcommand{\hlSThreeDropDOFAEnvaCIHi}{11.9}
\newcommand{\hlSThreeDropDOFAEnvaTostCILo}{\ensuremath{-}2.4}
\newcommand{\hlSThreeDropDOFAEnvaTostCIHi}{10.0}
\newcommand{\hlSThreeDropDOFAEnvaMde}{13.3}
\newcommand{\hlSThreeDropDOFAEnvaN}{5}
\newcommand{\hlSThreeDropDOFAEnvaA}{9.3}
\newcommand{\hlSThreeDropDOFAEnvaB}{5.4}
\newcommand{\hlSThreeDropDOFAEnvaVerdict}{Undetermined, MDE 13.3}
\newcommand{\hlSThreeDropDOFAEnvaFlag}{partial bands}
\newcommand{\hlSThreeDropDOFASnTwoEst}{3.0}
\newcommand{\hlSThreeDropDOFASnTwoCILo}{1.2}
\newcommand{\hlSThreeDropDOFASnTwoCIHi}{4.7}
\newcommand{\hlSThreeDropDOFASnTwoTostCILo}{1.6}
\newcommand{\hlSThreeDropDOFASnTwoTostCIHi}{4.3}
\newcommand{\hlSThreeDropDOFASnTwoMde}{2.9}
\newcommand{\hlSThreeDropDOFASnTwoN}{5}
\newcommand{\hlSThreeDropDOFASnTwoA}{14.8}
\newcommand{\hlSThreeDropDOFASnTwoB}{11.8}
\newcommand{\hlSThreeDropDOFASnTwoVerdict}{the extension encoder loses more}
\newcommand{\hlSThreeDropDOFASnTwoFlag}{partial bands}
\newcommand{\hlSThreeDropDOFAKuroEst}{\ensuremath{-}1.3}
\newcommand{\hlSThreeDropDOFAKuroCILo}{\ensuremath{-}5.8}
\newcommand{\hlSThreeDropDOFAKuroCIHi}{3.3}
\newcommand{\hlSThreeDropDOFAKuroTostCILo}{\ensuremath{-}4.7}
\newcommand{\hlSThreeDropDOFAKuroTostCIHi}{2.2}
\newcommand{\hlSThreeDropDOFAKuroMde}{7.4}
\newcommand{\hlSThreeDropDOFAKuroN}{5}
\newcommand{\hlSThreeDropDOFAKuroA}{3.9}
\newcommand{\hlSThreeDropDOFAKuroB}{5.1}
\newcommand{\hlSThreeDropDOFAKuroVerdict}{Undetermined, MDE 7.4}
\newcommand{\hlSThreeDropDOFAKuroFlag}{out of domain}
\newcommand{\hlSThreeDropDOFAOemEst}{\ensuremath{-}0.3}
\newcommand{\hlSThreeDropDOFAOemCILo}{\ensuremath{-}2.4}
\newcommand{\hlSThreeDropDOFAOemCIHi}{1.8}
\newcommand{\hlSThreeDropDOFAOemTostCILo}{\ensuremath{-}1.9}
\newcommand{\hlSThreeDropDOFAOemTostCIHi}{1.3}
\newcommand{\hlSThreeDropDOFAOemMde}{3.5}
\newcommand{\hlSThreeDropDOFAOemN}{5}
\newcommand{\hlSThreeDropDOFAOemA}{6.5}
\newcommand{\hlSThreeDropDOFAOemB}{6.8}
\newcommand{\hlSThreeDropDOFAOemVerdict}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlSThreeDropDOFAOemFlag}{out of domain}
\newcommand{\hlSThreeDropDOFAInDomDatasets}{5}
\newcommand{\hlSThreeDropDOFAInDomRead}{5}
\newcommand{\hlSThreeDropDOFAInDomEquiv}{2}
\newcommand{\hlSThreeDropDOFAInDomDiffer}{1}
\newcommand{\hlSThreeDropDOFAInDomUndet}{2}
\newcommand{\hlSThreeDropDOFAOutDomDatasets}{2}
\newcommand{\hlSThreeDropDOFAOutDomRead}{2}
\newcommand{\hlSThreeDropDOFAOutDomEquiv}{1}
\newcommand{\hlSThreeDropDOFAOutDomDiffer}{0}
\newcommand{\hlSThreeDropDOFAOutDomUndet}{1}
\newcommand{\hlSThreeDropDOFANoPreDatasets}{0}
\newcommand{\hlSThreeDropDOFANoPreRead}{0}
\newcommand{\hlSThreeDropDOFANoPreEquiv}{0}
\newcommand{\hlSThreeDropDOFANoPreDiffer}{0}
\newcommand{\hlSThreeDropDOFANoPreUndet}{0}
\newcommand{\hlSFourDropRNChesEst}{0.8}
\newcommand{\hlSFourDropRNChesCILo}{\ensuremath{-}0.5}
\newcommand{\hlSFourDropRNChesCIHi}{2.0}
\newcommand{\hlSFourDropRNChesTostCILo}{\ensuremath{-}0.2}
\newcommand{\hlSFourDropRNChesTostCIHi}{1.7}
\newcommand{\hlSFourDropRNChesMde}{2.0}
\newcommand{\hlSFourDropRNChesN}{5}
\newcommand{\hlSFourDropRNChesA}{9.5}
\newcommand{\hlSFourDropRNChesB}{8.7}
\newcommand{\hlSFourDropRNChesVerdict}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlSFourDropRNChesFlag}{partial bands}
\newcommand{\hlSFourDropRNCsTwelveEst}{0.2}
\newcommand{\hlSFourDropRNCsTwelveCILo}{\ensuremath{-}1.2}
\newcommand{\hlSFourDropRNCsTwelveCIHi}{1.7}
\newcommand{\hlSFourDropRNCsTwelveTostCILo}{\ensuremath{-}0.8}
\newcommand{\hlSFourDropRNCsTwelveTostCIHi}{1.3}
\newcommand{\hlSFourDropRNCsTwelveMde}{2.3}
\newcommand{\hlSFourDropRNCsTwelveN}{5}
\newcommand{\hlSFourDropRNCsTwelveA}{7.0}
\newcommand{\hlSFourDropRNCsTwelveB}{6.8}
\newcommand{\hlSFourDropRNCsTwelveVerdict}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlSFourDropRNCsTwelveFlag}{in domain}
\newcommand{\hlSFourDropRNDfcEst}{0.4}
\newcommand{\hlSFourDropRNDfcCILo}{\ensuremath{-}3.3}
\newcommand{\hlSFourDropRNDfcCIHi}{4.1}
\newcommand{\hlSFourDropRNDfcTostCILo}{\ensuremath{-}2.5}
\newcommand{\hlSFourDropRNDfcTostCIHi}{3.2}
\newcommand{\hlSFourDropRNDfcMde}{6.1}
\newcommand{\hlSFourDropRNDfcN}{5}
\newcommand{\hlSFourDropRNDfcA}{1.6}
\newcommand{\hlSFourDropRNDfcB}{1.2}
\newcommand{\hlSFourDropRNDfcVerdict}{Undetermined, MDE 6.1}
\newcommand{\hlSFourDropRNDfcFlag}{partial bands}
\newcommand{\hlSFourDropRNEnvaEst}{2.8}
\newcommand{\hlSFourDropRNEnvaCILo}{\ensuremath{-}3.5}
\newcommand{\hlSFourDropRNEnvaCIHi}{9.1}
\newcommand{\hlSFourDropRNEnvaTostCILo}{\ensuremath{-}2.1}
\newcommand{\hlSFourDropRNEnvaTostCIHi}{7.6}
\newcommand{\hlSFourDropRNEnvaMde}{10.4}
\newcommand{\hlSFourDropRNEnvaN}{5}
\newcommand{\hlSFourDropRNEnvaA}{14.8}
\newcommand{\hlSFourDropRNEnvaB}{12.1}
\newcommand{\hlSFourDropRNEnvaVerdict}{Undetermined, MDE 10.4}
\newcommand{\hlSFourDropRNEnvaFlag}{partial bands}
\newcommand{\hlSFourDropRNSnTwoEst}{\ensuremath{-}1.3}
\newcommand{\hlSFourDropRNSnTwoCILo}{\ensuremath{-}3.4}
\newcommand{\hlSFourDropRNSnTwoCIHi}{0.8}
\newcommand{\hlSFourDropRNSnTwoTostCILo}{\ensuremath{-}2.9}
\newcommand{\hlSFourDropRNSnTwoTostCIHi}{0.3}
\newcommand{\hlSFourDropRNSnTwoMde}{3.5}
\newcommand{\hlSFourDropRNSnTwoN}{5}
\newcommand{\hlSFourDropRNSnTwoA}{12.5}
\newcommand{\hlSFourDropRNSnTwoB}{13.8}
\newcommand{\hlSFourDropRNSnTwoVerdict}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlSFourDropRNSnTwoFlag}{partial bands}
\newcommand{\hlSFourDropRNKuroEst}{\ensuremath{-}1.7}
\newcommand{\hlSFourDropRNKuroCILo}{\ensuremath{-}9.7}
\newcommand{\hlSFourDropRNKuroCIHi}{6.4}
\newcommand{\hlSFourDropRNKuroTostCILo}{\ensuremath{-}7.8}
\newcommand{\hlSFourDropRNKuroTostCIHi}{4.5}
\newcommand{\hlSFourDropRNKuroMde}{13.2}
\newcommand{\hlSFourDropRNKuroN}{5}
\newcommand{\hlSFourDropRNKuroA}{\ensuremath{-}1.1}
\newcommand{\hlSFourDropRNKuroB}{0.5}
\newcommand{\hlSFourDropRNKuroVerdict}{Undetermined, MDE 13.2}
\newcommand{\hlSFourDropRNKuroFlag}{out of domain}
\newcommand{\hlSFourDropRNOemEst}{\ensuremath{-}0.7}
\newcommand{\hlSFourDropRNOemCILo}{\ensuremath{-}3.3}
\newcommand{\hlSFourDropRNOemCIHi}{1.8}
\newcommand{\hlSFourDropRNOemTostCILo}{\ensuremath{-}2.7}
\newcommand{\hlSFourDropRNOemTostCIHi}{1.2}
\newcommand{\hlSFourDropRNOemMde}{4.1}
\newcommand{\hlSFourDropRNOemN}{5}
\newcommand{\hlSFourDropRNOemA}{4.6}
\newcommand{\hlSFourDropRNOemB}{5.4}
\newcommand{\hlSFourDropRNOemVerdict}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlSFourDropRNOemFlag}{out of domain}
\newcommand{\hlSFourDropRNInDomDatasets}{5}
\newcommand{\hlSFourDropRNInDomRead}{5}
\newcommand{\hlSFourDropRNInDomEquiv}{3}
\newcommand{\hlSFourDropRNInDomDiffer}{0}
\newcommand{\hlSFourDropRNInDomUndet}{2}
\newcommand{\hlSFourDropRNOutDomDatasets}{2}
\newcommand{\hlSFourDropRNOutDomRead}{2}
\newcommand{\hlSFourDropRNOutDomEquiv}{1}
\newcommand{\hlSFourDropRNOutDomDiffer}{0}
\newcommand{\hlSFourDropRNOutDomUndet}{1}
\newcommand{\hlSFourDropRNNoPreDatasets}{0}
\newcommand{\hlSFourDropRNNoPreRead}{0}
\newcommand{\hlSFourDropRNNoPreEquiv}{0}
\newcommand{\hlSFourDropRNNoPreDiffer}{0}
\newcommand{\hlSFourDropRNNoPreUndet}{0}
\newcommand{\hlSFiveDropSATChesEst}{\ensuremath{-}2.6}
\newcommand{\hlSFiveDropSATChesCILo}{\ensuremath{-}5.6}
\newcommand{\hlSFiveDropSATChesCIHi}{0.3}
\newcommand{\hlSFiveDropSATChesTostCILo}{\ensuremath{-}4.9}
\newcommand{\hlSFiveDropSATChesTostCIHi}{\ensuremath{-}0.3}
\newcommand{\hlSFiveDropSATChesMde}{4.9}
\newcommand{\hlSFiveDropSATChesN}{5}
\newcommand{\hlSFiveDropSATChesA}{7.5}
\newcommand{\hlSFiveDropSATChesB}{10.2}
\newcommand{\hlSFiveDropSATChesVerdict}{Undetermined, MDE 4.9}
\newcommand{\hlSFiveDropSATChesFlag}{no pretraining}
\newcommand{\hlSFiveDropSATCsTwelveEst}{\ensuremath{-}0.1}
\newcommand{\hlSFiveDropSATCsTwelveCILo}{\ensuremath{-}2.9}
\newcommand{\hlSFiveDropSATCsTwelveCIHi}{2.6}
\newcommand{\hlSFiveDropSATCsTwelveTostCILo}{\ensuremath{-}2.2}
\newcommand{\hlSFiveDropSATCsTwelveTostCIHi}{2.0}
\newcommand{\hlSFiveDropSATCsTwelveMde}{4.5}
\newcommand{\hlSFiveDropSATCsTwelveN}{5}
\newcommand{\hlSFiveDropSATCsTwelveA}{5.8}
\newcommand{\hlSFiveDropSATCsTwelveB}{5.9}
\newcommand{\hlSFiveDropSATCsTwelveVerdict}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlSFiveDropSATCsTwelveFlag}{no pretraining}
\newcommand{\hlSFiveDropSATDfcEst}{\ensuremath{-}2.0}
\newcommand{\hlSFiveDropSATDfcCILo}{\ensuremath{-}4.9}
\newcommand{\hlSFiveDropSATDfcCIHi}{0.9}
\newcommand{\hlSFiveDropSATDfcTostCILo}{\ensuremath{-}4.2}
\newcommand{\hlSFiveDropSATDfcTostCIHi}{0.3}
\newcommand{\hlSFiveDropSATDfcMde}{4.8}
\newcommand{\hlSFiveDropSATDfcN}{5}
\newcommand{\hlSFiveDropSATDfcA}{1.0}
\newcommand{\hlSFiveDropSATDfcB}{2.9}
\newcommand{\hlSFiveDropSATDfcVerdict}{Undetermined, MDE 4.8}
\newcommand{\hlSFiveDropSATDfcFlag}{no pretraining}
\newcommand{\hlSFiveDropSATEnvaEst}{1.9}
\newcommand{\hlSFiveDropSATEnvaCILo}{\ensuremath{-}5.9}
\newcommand{\hlSFiveDropSATEnvaCIHi}{9.8}
\newcommand{\hlSFiveDropSATEnvaTostCILo}{\ensuremath{-}4.1}
\newcommand{\hlSFiveDropSATEnvaTostCIHi}{7.9}
\newcommand{\hlSFiveDropSATEnvaMde}{12.9}
\newcommand{\hlSFiveDropSATEnvaN}{5}
\newcommand{\hlSFiveDropSATEnvaA}{8.2}
\newcommand{\hlSFiveDropSATEnvaB}{6.3}
\newcommand{\hlSFiveDropSATEnvaVerdict}{Undetermined, MDE 12.9}
\newcommand{\hlSFiveDropSATEnvaFlag}{no pretraining}
\newcommand{\hlSFiveDropSATSnTwoEst}{0.4}
\newcommand{\hlSFiveDropSATSnTwoCILo}{\ensuremath{-}1.2}
\newcommand{\hlSFiveDropSATSnTwoCIHi}{2.0}
\newcommand{\hlSFiveDropSATSnTwoTostCILo}{\ensuremath{-}0.8}
\newcommand{\hlSFiveDropSATSnTwoTostCIHi}{1.6}
\newcommand{\hlSFiveDropSATSnTwoMde}{2.6}
\newcommand{\hlSFiveDropSATSnTwoN}{5}
\newcommand{\hlSFiveDropSATSnTwoA}{11.9}
\newcommand{\hlSFiveDropSATSnTwoB}{11.4}
\newcommand{\hlSFiveDropSATSnTwoVerdict}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlSFiveDropSATSnTwoFlag}{no pretraining}
\newcommand{\hlSFiveDropSATKuroEst}{\ensuremath{-}6.1}
\newcommand{\hlSFiveDropSATKuroCILo}{\ensuremath{-}9.7}
\newcommand{\hlSFiveDropSATKuroCIHi}{\ensuremath{-}2.4}
\newcommand{\hlSFiveDropSATKuroTostCILo}{\ensuremath{-}8.9}
\newcommand{\hlSFiveDropSATKuroTostCIHi}{\ensuremath{-}3.3}
\newcommand{\hlSFiveDropSATKuroMde}{6.0}
\newcommand{\hlSFiveDropSATKuroN}{5}
\newcommand{\hlSFiveDropSATKuroA}{0.4}
\newcommand{\hlSFiveDropSATKuroB}{6.5}
\newcommand{\hlSFiveDropSATKuroVerdict}{the extension encoder loses less}
\newcommand{\hlSFiveDropSATKuroFlag}{no pretraining}
\newcommand{\hlSFiveDropSATOemEst}{\ensuremath{-}4.1}
\newcommand{\hlSFiveDropSATOemCILo}{\ensuremath{-}5.3}
\newcommand{\hlSFiveDropSATOemCIHi}{\ensuremath{-}2.8}
\newcommand{\hlSFiveDropSATOemTostCILo}{\ensuremath{-}5.0}
\newcommand{\hlSFiveDropSATOemTostCIHi}{\ensuremath{-}3.1}
\newcommand{\hlSFiveDropSATOemMde}{2.0}
\newcommand{\hlSFiveDropSATOemN}{5}
\newcommand{\hlSFiveDropSATOemA}{3.6}
\newcommand{\hlSFiveDropSATOemB}{7.6}
\newcommand{\hlSFiveDropSATOemVerdict}{the extension encoder loses less}
\newcommand{\hlSFiveDropSATOemFlag}{no pretraining}
\newcommand{\hlSFiveDropSATInDomDatasets}{0}
\newcommand{\hlSFiveDropSATInDomRead}{0}
\newcommand{\hlSFiveDropSATInDomEquiv}{0}
\newcommand{\hlSFiveDropSATInDomDiffer}{0}
\newcommand{\hlSFiveDropSATInDomUndet}{0}
\newcommand{\hlSFiveDropSATOutDomDatasets}{0}
\newcommand{\hlSFiveDropSATOutDomRead}{0}
\newcommand{\hlSFiveDropSATOutDomEquiv}{0}
\newcommand{\hlSFiveDropSATOutDomDiffer}{0}
\newcommand{\hlSFiveDropSATOutDomUndet}{0}
\newcommand{\hlSFiveDropSATNoPreDatasets}{7}
\newcommand{\hlSFiveDropSATNoPreRead}{7}
\newcommand{\hlSFiveDropSATNoPreEquiv}{2}
\newcommand{\hlSFiveDropSATNoPreDiffer}{2}
\newcommand{\hlSFiveDropSATNoPreUndet}{3}
\newcommand{\hlSSixDropSATChesEst}{0.5}
\newcommand{\hlSSixDropSATChesCILo}{\ensuremath{-}2.0}
\newcommand{\hlSSixDropSATChesCIHi}{2.9}
\newcommand{\hlSSixDropSATChesTostCILo}{\ensuremath{-}1.4}
\newcommand{\hlSSixDropSATChesTostCIHi}{2.4}
\newcommand{\hlSSixDropSATChesMde}{4.1}
\newcommand{\hlSSixDropSATChesN}{5}
\newcommand{\hlSSixDropSATChesA}{10.6}
\newcommand{\hlSSixDropSATChesB}{10.2}
\newcommand{\hlSSixDropSATChesVerdict}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlSSixDropSATChesFlag}{in domain}
\newcommand{\hlSSixDropSATCsTwelveEst}{0.9}
\newcommand{\hlSSixDropSATCsTwelveCILo}{\ensuremath{-}1.9}
\newcommand{\hlSSixDropSATCsTwelveCIHi}{3.8}
\newcommand{\hlSSixDropSATCsTwelveTostCILo}{\ensuremath{-}1.2}
\newcommand{\hlSSixDropSATCsTwelveTostCIHi}{3.1}
\newcommand{\hlSSixDropSATCsTwelveMde}{4.6}
\newcommand{\hlSSixDropSATCsTwelveN}{5}
\newcommand{\hlSSixDropSATCsTwelveA}{6.8}
\newcommand{\hlSSixDropSATCsTwelveB}{5.9}
\newcommand{\hlSSixDropSATCsTwelveVerdict}{Undetermined, MDE 4.6}
\newcommand{\hlSSixDropSATCsTwelveFlag}{in domain}
\newcommand{\hlSSixDropSATDfcEst}{0.2}
\newcommand{\hlSSixDropSATDfcCILo}{\ensuremath{-}1.4}
\newcommand{\hlSSixDropSATDfcCIHi}{1.7}
\newcommand{\hlSSixDropSATDfcTostCILo}{\ensuremath{-}1.0}
\newcommand{\hlSSixDropSATDfcTostCIHi}{1.4}
\newcommand{\hlSSixDropSATDfcMde}{2.6}
\newcommand{\hlSSixDropSATDfcN}{5}
\newcommand{\hlSSixDropSATDfcA}{3.1}
\newcommand{\hlSSixDropSATDfcB}{2.9}
\newcommand{\hlSSixDropSATDfcVerdict}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlSSixDropSATDfcFlag}{in domain}
\newcommand{\hlSSixDropSATEnvaEst}{\ensuremath{-}9.0}
\newcommand{\hlSSixDropSATEnvaCILo}{\ensuremath{-}15.3}
\newcommand{\hlSSixDropSATEnvaCIHi}{\ensuremath{-}2.7}
\newcommand{\hlSSixDropSATEnvaTostCILo}{\ensuremath{-}13.9}
\newcommand{\hlSSixDropSATEnvaTostCIHi}{\ensuremath{-}4.1}
\newcommand{\hlSSixDropSATEnvaMde}{10.5}
\newcommand{\hlSSixDropSATEnvaN}{5}
\newcommand{\hlSSixDropSATEnvaA}{\ensuremath{-}2.7}
\newcommand{\hlSSixDropSATEnvaB}{6.3}
\newcommand{\hlSSixDropSATEnvaVerdict}{the extension encoder loses less}
\newcommand{\hlSSixDropSATEnvaFlag}{in domain}
\newcommand{\hlSSixDropSATSnTwoEst}{0.5}
\newcommand{\hlSSixDropSATSnTwoCILo}{\ensuremath{-}1.8}
\newcommand{\hlSSixDropSATSnTwoCIHi}{2.8}
\newcommand{\hlSSixDropSATSnTwoTostCILo}{\ensuremath{-}1.3}
\newcommand{\hlSSixDropSATSnTwoTostCIHi}{2.2}
\newcommand{\hlSSixDropSATSnTwoMde}{3.8}
\newcommand{\hlSSixDropSATSnTwoN}{5}
\newcommand{\hlSSixDropSATSnTwoA}{11.9}
\newcommand{\hlSSixDropSATSnTwoB}{11.4}
\newcommand{\hlSSixDropSATSnTwoVerdict}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlSSixDropSATSnTwoFlag}{in domain}
\newcommand{\hlSSixDropSATKuroEst}{2.8}
\newcommand{\hlSSixDropSATKuroCILo}{\ensuremath{-}3.8}
\newcommand{\hlSSixDropSATKuroCIHi}{9.4}
\newcommand{\hlSSixDropSATKuroTostCILo}{\ensuremath{-}2.2}
\newcommand{\hlSSixDropSATKuroTostCIHi}{7.9}
\newcommand{\hlSSixDropSATKuroMde}{10.9}
\newcommand{\hlSSixDropSATKuroN}{5}
\newcommand{\hlSSixDropSATKuroA}{9.3}
\newcommand{\hlSSixDropSATKuroB}{6.5}
\newcommand{\hlSSixDropSATKuroVerdict}{Undetermined, MDE 10.9}
\newcommand{\hlSSixDropSATKuroFlag}{out of domain}
\newcommand{\hlSSixDropSATOemEst}{\ensuremath{-}0.9}
\newcommand{\hlSSixDropSATOemCILo}{\ensuremath{-}2.2}
\newcommand{\hlSSixDropSATOemCIHi}{0.5}
\newcommand{\hlSSixDropSATOemTostCILo}{\ensuremath{-}1.9}
\newcommand{\hlSSixDropSATOemTostCIHi}{0.1}
\newcommand{\hlSSixDropSATOemMde}{2.2}
\newcommand{\hlSSixDropSATOemN}{5}
\newcommand{\hlSSixDropSATOemA}{6.8}
\newcommand{\hlSSixDropSATOemB}{7.6}
\newcommand{\hlSSixDropSATOemVerdict}{Equivalent within $\pm$\TostMargin}
\newcommand{\hlSSixDropSATOemFlag}{in domain}
\newcommand{\hlSSixDropSATInDomDatasets}{6}
\newcommand{\hlSSixDropSATInDomRead}{6}
\newcommand{\hlSSixDropSATInDomEquiv}{4}
\newcommand{\hlSSixDropSATInDomDiffer}{1}
\newcommand{\hlSSixDropSATInDomUndet}{1}
\newcommand{\hlSSixDropSATOutDomDatasets}{1}
\newcommand{\hlSSixDropSATOutDomRead}{1}
\newcommand{\hlSSixDropSATOutDomEquiv}{0}
\newcommand{\hlSSixDropSATOutDomDiffer}{0}
\newcommand{\hlSSixDropSATOutDomUndet}{1}
\newcommand{\hlSSixDropSATNoPreDatasets}{0}
\newcommand{\hlSSixDropSATNoPreRead}{0}
\newcommand{\hlSSixDropSATNoPreEquiv}{0}
\newcommand{\hlSSixDropSATNoPreDiffer}{0}
\newcommand{\hlSSixDropSATNoPreUndet}{0}
\newcommand{\hlNNineteenInDomPairs}{16}
\newcommand{\hlNNineteenInDomRead}{16}
\newcommand{\hlNNineteenInDomEquiv}{9}
\newcommand{\hlNNineteenInDomDiffer}{2}
\newcommand{\hlNNineteenInDomUndet}{5}
\newcommand{\hlNNineteenOutDomPairs}{5}
\newcommand{\hlNNineteenOutDomRead}{5}
\newcommand{\hlNNineteenOutDomEquiv}{2}
\newcommand{\hlNNineteenOutDomDiffer}{0}
\newcommand{\hlNNineteenOutDomUndet}{3}
\newcommand{\hlNNineteenNoPrePairs}{7}
\newcommand{\hlNNineteenNoPreRead}{7}
\newcommand{\hlNNineteenNoPreEquiv}{2}
\newcommand{\hlNNineteenNoPreDiffer}{2}
\newcommand{\hlNNineteenNoPreUndet}{3}
\newcommand{\hlLayDepth}{24}
\newcommand{\hlLayArmSix}{6}
\newcommand{\hlLayParamsSix}{75.6M}
\newcommand{\hlLayArmTwelve}{12}
\newcommand{\hlLayParamsTwelve}{151.1M}
\newcommand{\hlLayParamsAll}{303.1M}
\newcommand{\hlLayRunsPlanned}{216}
\newcommand{\hlLaySeeds}{5}
\newcommand{\hlLaySeedsAll}{3}
\newcommand{\hlLayBandPx}{3}
\newcommand{\hlLayWorstburn}{coarse}
\newcommand{\hlLayWorstflair}{omission}
\newcommand{\hlLayRunsDone}{216}
\newcommand{\hlLayStepSATburnTwentyFourTwelveEst}{\ensuremath{-}0.4}
\newcommand{\hlLayStepSATburnTwentyFourTwelveCILo}{\ensuremath{-}5.0}
\newcommand{\hlLayStepSATburnTwentyFourTwelveCIHi}{4.3}
\newcommand{\hlLayStepSATburnTwelveSixEst}{0.3}
\newcommand{\hlLayStepSATburnTwelveSixCILo}{\ensuremath{-}1.9}
\newcommand{\hlLayStepSATburnTwelveSixCIHi}{2.5}
\newcommand{\hlLayStepSATburnSixZeroEst}{0.3}
\newcommand{\hlLayStepSATburnSixZeroCILo}{\ensuremath{-}2.4}
\newcommand{\hlLayStepSATburnSixZeroCIHi}{3.0}
\newcommand{\hlLayStepLVDburnTwentyFourTwelveEst}{\ensuremath{-}0.1}
\newcommand{\hlLayStepLVDburnTwentyFourTwelveCILo}{\ensuremath{-}4.1}
\newcommand{\hlLayStepLVDburnTwentyFourTwelveCIHi}{3.9}
\newcommand{\hlLayStepLVDburnTwelveSixEst}{0.7}
\newcommand{\hlLayStepLVDburnTwelveSixCILo}{\ensuremath{-}4.4}
\newcommand{\hlLayStepLVDburnTwelveSixCIHi}{5.8}
\newcommand{\hlLayStepLVDburnSixZeroEst}{\ensuremath{-}1.4}
\newcommand{\hlLayStepLVDburnSixZeroCILo}{\ensuremath{-}7.9}
\newcommand{\hlLayStepLVDburnSixZeroCIHi}{5.2}
\newcommand{\hlLayPairburnZeroEst}{\ensuremath{-}1.7}
\newcommand{\hlLayPairburnZeroCILo}{\ensuremath{-}6.4}
\newcommand{\hlLayPairburnZeroCIHi}{3.0}
\newcommand{\hlLayPairburnTwentyFourEst}{\ensuremath{-}0.7}
\newcommand{\hlLayPairburnTwentyFourCILo}{\ensuremath{-}5.5}
\newcommand{\hlLayPairburnTwentyFourCIHi}{4.0}
\newcommand{\hlLayStepSATflairTwentyFourTwelveEst}{0.2}
\newcommand{\hlLayStepSATflairTwentyFourTwelveCILo}{\ensuremath{-}0.7}
\newcommand{\hlLayStepSATflairTwentyFourTwelveCIHi}{1.2}
\newcommand{\hlLayStepSATflairTwelveSixEst}{1.1}
\newcommand{\hlLayStepSATflairTwelveSixCILo}{\ensuremath{-}0.2}
\newcommand{\hlLayStepSATflairTwelveSixCIHi}{2.3}
\newcommand{\hlLayStepSATflairSixZeroEst}{2.0}
\newcommand{\hlLayStepSATflairSixZeroCILo}{\ensuremath{-}0.2}
\newcommand{\hlLayStepSATflairSixZeroCIHi}{4.2}
\newcommand{\hlLayStepLVDflairTwentyFourTwelveEst}{0.3}
\newcommand{\hlLayStepLVDflairTwentyFourTwelveCILo}{\ensuremath{-}1.6}
\newcommand{\hlLayStepLVDflairTwentyFourTwelveCIHi}{2.3}
\newcommand{\hlLayStepLVDflairTwelveSixEst}{\ensuremath{-}0.2}
\newcommand{\hlLayStepLVDflairTwelveSixCILo}{\ensuremath{-}0.8}
\newcommand{\hlLayStepLVDflairTwelveSixCIHi}{0.4}
\newcommand{\hlLayStepLVDflairSixZeroEst}{0.4}
\newcommand{\hlLayStepLVDflairSixZeroCILo}{\ensuremath{-}0.7}
\newcommand{\hlLayStepLVDflairSixZeroCIHi}{1.5}
\newcommand{\hlLayPairflairZeroEst}{\ensuremath{-}0.2}
\newcommand{\hlLayPairflairZeroCILo}{\ensuremath{-}2.2}
\newcommand{\hlLayPairflairZeroCIHi}{1.8}
\newcommand{\hlLayPairflairTwentyFourEst}{2.6}
\newcommand{\hlLayPairflairTwentyFourCILo}{0.9}
\newcommand{\hlLayPairflairTwentyFourCIHi}{4.2}
\newcommand{\hlLayDriftSATburnEst}{1.14}
\newcommand{\hlLayDriftSATburnCILo}{0.20}
\newcommand{\hlLayDriftSATburnCIHi}{2.08}
\newcommand{\hlLayDriftStepSATburn}{1.16}
\newcommand{\hlLayCkaSATburnEst}{0.073}
\newcommand{\hlLayCkaSATburnCILo}{\ensuremath{-}0.152}
\newcommand{\hlLayCkaSATburnCIHi}{0.298}
\newcommand{\hlLayDriftSATburnThird}{early}
\newcommand{\hlLayDriftSATburnThirdEst}{1.25}
\newcommand{\hlLayCkaSATburnThird}{late}
\newcommand{\hlLayEpochSATburnClean}{12.7}
\newcommand{\hlLayEpochSATburnNoisy}{14.0}
\newcommand{\hlLayDriftLVDburnEst}{0.79}
\newcommand{\hlLayDriftLVDburnCILo}{0.09}
\newcommand{\hlLayDriftLVDburnCIHi}{1.49}
\newcommand{\hlLayDriftStepLVDburn}{1.48}
\newcommand{\hlLayCkaLVDburnEst}{0.029}
\newcommand{\hlLayCkaLVDburnCILo}{\ensuremath{-}0.052}
\newcommand{\hlLayCkaLVDburnCIHi}{0.110}
\newcommand{\hlLayDriftLVDburnThird}{middle}
\newcommand{\hlLayDriftLVDburnThirdEst}{0.77}
\newcommand{\hlLayCkaLVDburnThird}{middle}
\newcommand{\hlLayEpochLVDburnClean}{24.0}
\newcommand{\hlLayEpochLVDburnNoisy}{12.7}
\newcommand{\hlLayDriftSATflairEst}{1.06}
\newcommand{\hlLayDriftSATflairCILo}{0.53}
\newcommand{\hlLayDriftSATflairCIHi}{1.60}
\newcommand{\hlLayDriftStepSATflair}{1.00}
\newcommand{\hlLayCkaSATflairEst}{\ensuremath{-}0.008}
\newcommand{\hlLayCkaSATflairCILo}{\ensuremath{-}0.021}
\newcommand{\hlLayCkaSATflairCIHi}{0.006}
\newcommand{\hlLayDriftSATflairThird}{early}
\newcommand{\hlLayDriftSATflairThirdEst}{1.11}
\newcommand{\hlLayCkaSATflairThird}{late}
\newcommand{\hlLayEpochSATflairClean}{37.3}
\newcommand{\hlLayEpochSATflairNoisy}{38.0}
\newcommand{\hlLayDriftLVDflairEst}{0.79}
\newcommand{\hlLayDriftLVDflairCILo}{0.53}
\newcommand{\hlLayDriftLVDflairCIHi}{1.05}
\newcommand{\hlLayDriftStepLVDflair}{1.48}
\newcommand{\hlLayCkaLVDflairEst}{\ensuremath{-}0.005}
\newcommand{\hlLayCkaLVDflairCILo}{\ensuremath{-}0.020}
\newcommand{\hlLayCkaLVDflairCIHi}{0.009}
\newcommand{\hlLayDriftLVDflairThird}{late}
\newcommand{\hlLayDriftLVDflairThirdEst}{0.77}
\newcommand{\hlLayCkaLVDflairThird}{late}
\newcommand{\hlLayEpochLVDflairClean}{32.0}
\newcommand{\hlLayEpochLVDflairNoisy}{16.7}
\newcommand{\hlLayFrozenRuns}{180}
\newcommand{\hlLayFrozenMaxDrift}{0.000}
\newcommand{\hlLayFrozenMinCka}{1.000}
\newcommand{\hlLayShareSATburnShift}{8.1}
\newcommand{\hlLayBandIntSATburnShiftEst}{5.7}
\newcommand{\hlLayBandIntSATburnShiftCILo}{1.0}
\newcommand{\hlLayBandIntSATburnShiftCIHi}{10.5}
\newcommand{\hlLayShareSATburnWorst}{6.0}
\newcommand{\hlLayBandIntSATburnWorstEst}{5.1}
\newcommand{\hlLayBandIntSATburnWorstCILo}{2.4}
\newcommand{\hlLayBandIntSATburnWorstCIHi}{7.8}
\newcommand{\hlLayIntSATburnTwentyFour}{3.2}
\newcommand{\hlLayIntSATburnSix}{2.8}
\newcommand{\hlLayShareLVDburnShift}{10.4}
\newcommand{\hlLayBandIntLVDburnShiftEst}{8.7}
\newcommand{\hlLayBandIntLVDburnShiftCILo}{4.4}
\newcommand{\hlLayBandIntLVDburnShiftCIHi}{13.0}
\newcommand{\hlLayShareLVDburnWorst}{8.0}
\newcommand{\hlLayBandIntLVDburnWorstEst}{8.2}
\newcommand{\hlLayBandIntLVDburnWorstCILo}{5.5}
\newcommand{\hlLayBandIntLVDburnWorstCIHi}{11.0}
\newcommand{\hlLayIntLVDburnTwentyFour}{3.3}
\newcommand{\hlLayIntLVDburnSix}{3.4}
\newcommand{\hlLayBandFracburn}{2.4}
\newcommand{\hlLayShareSATflairShift}{15.7}
\newcommand{\hlLayBandIntSATflairShiftEst}{1.6}
\newcommand{\hlLayBandIntSATflairShiftCILo}{0.4}
\newcommand{\hlLayBandIntSATflairShiftCIHi}{2.8}
\newcommand{\hlLayShareSATflairWorst}{4.8}
\newcommand{\hlLayBandIntSATflairWorstEst}{\ensuremath{-}3.8}
\newcommand{\hlLayBandIntSATflairWorstCILo}{\ensuremath{-}7.6}
\newcommand{\hlLayBandIntSATflairWorstCIHi}{0.0}
\newcommand{\hlLayIntSATflairTwentyFour}{7.3}
\newcommand{\hlLayIntSATflairSix}{4.8}
\newcommand{\hlLayShareLVDflairShift}{18.6}
\newcommand{\hlLayBandIntLVDflairShiftEst}{1.8}
\newcommand{\hlLayBandIntLVDflairShiftCILo}{0.4}
\newcommand{\hlLayBandIntLVDflairShiftCIHi}{3.2}
\newcommand{\hlLayShareLVDflairWorst}{9.4}
\newcommand{\hlLayBandIntLVDflairWorstEst}{\ensuremath{-}0.1}
\newcommand{\hlLayBandIntLVDflairWorstCILo}{\ensuremath{-}0.8}
\newcommand{\hlLayBandIntLVDflairWorstCIHi}{0.7}
\newcommand{\hlLayIntLVDflairTwentyFour}{3.0}
\newcommand{\hlLayIntLVDflairSix}{2.4}
\newcommand{\hlLayBandFracflair}{9.7}
\newcommand{\hlLayReproburnAbs}{2.38}
\newcommand{\hlLayReproburnMax}{4.98}
\newcommand{\hlLayReproburnN}{18}
\newcommand{\hlLayReproflairAbs}{0.75}
\newcommand{\hlLayReproflairMax}{2.32}
\newcommand{\hlLayReproflairN}{18}
\newcommand{\ResultsProvenance}{Analysis of the finished runs}
%
\newcommand{\ProvNSeven}{Analysis of the finished runs}
\newcommand{\ProvNEight}{Analysis of the finished runs}
\newcommand{\ProvNNine}{Analysis of the finished runs}
\newcommand{\ProvNTen}{Analysis of the finished runs}
\newcommand{\ProvNEleven}{Analysis of the finished runs}
\newcommand{\ProvNTwelve}{Analysis of the finished runs}
\newcommand{\ProvNThirteen}{Analysis of the finished runs}
\newcommand{\ProvNFourteen}{Analysis of the finished runs}
\newcommand{\ProvNFifteen}{Analysis of the finished runs}
\newcommand{\ProvDOne}{Analysis of the finished runs}
\newcommand{\ProvDTwo}{Analysis of the finished runs}
\newcommand{\ProvDThree}{Analysis of the finished runs}
\newcommand{\ProvDFour}{Analysis of the finished runs}
\newcommand{\ProvDFive}{Analysis of the finished runs}
\newcommand{\ProvDSix}{Analysis of the finished runs}
\newcommand{\ProvDSeven}{Analysis of the finished runs}
\newcommand{\ProvExtension}{Analysis of the finished runs}
\newcommand{\PlannedProvenance}{Analysis of the finished runs}


==> generated/supp_refs.tex <==
\expandafter\def\csname sref@tab:supp-calibration\endcsname{1}
\expandafter\def\csname sref@sec:supp-calibration\endcsname{A}
\expandafter\def\csname sref@fig:supp-mechanics\endcsname{1}
\expandafter\def\csname sref@tab:supp-realizations\endcsname{2}
\expandafter\def\csname sref@tab:supp-omadj\endcsname{3}
\expandafter\def\csname sref@tab:supp-acceptance\endcsname{4}
\expandafter\def\csname sref@sec:supp-acceptance\endcsname{B}
\expandafter\def\csname sref@sec:supp-grid\endcsname{C}
\expandafter\def\csname sref@sec:supp-collapsed\endcsname{D}
\expandafter\def\csname sref@sec:supp-perclass\endcsname{E}
\expandafter\def\csname sref@sec:supp-boundary\endcsname{F}
\expandafter\def\csname sref@tab:supp-main\endcsname{5}
\expandafter\def\csname sref@fig:supp-dose\endcsname{2}
\expandafter\def\csname sref@sec:supp-ablation\endcsname{G}
\expandafter\def\csname sref@fig:supp-typedrop\endcsname{3}
\expandafter\def\csname sref@sec:supp-budget\endcsname{H}
\expandafter\def\csname sref@tab:supp-grid-burn\endcsname{6}
\expandafter\def\csname sref@tab:supp-grid-flair\endcsname{7}
\expandafter\def\csname sref@tab:supp-collapsed\endcsname{8}
\expandafter\def\csname sref@tab:supp-collapsed-sens\endcsname{9}
\expandafter\def\csname sref@tab:supp-perclass\endcsname{10}
\expandafter\def\csname sref@tab:supp-perclass-drop\endcsname{11}
\expandafter\def\csname sref@tab:supp-boundary\endcsname{12}
\expandafter\def\csname sref@sec:supp-fliprate\endcsname{I}
\expandafter\def\csname sref@sec:supp-stats\endcsname{J}
\expandafter\def\csname sref@tab:supp-mlr\endcsname{13}
\expandafter\def\csname sref@fig:supp-budget\endcsname{4}
\expandafter\def\csname sref@tab:supp-ablation\endcsname{14}
\expandafter\def\csname sref@fig:supp-frozen\endcsname{5}
\expandafter\def\csname sref@tab:supp-frozen\endcsname{15}
\expandafter\def\csname sref@tab:supp-budget\endcsname{16}
\expandafter\def\csname sref@tab:supp-breakeven\endcsname{17}
\expandafter\def\csname sref@tab:mem\endcsname{18}
\expandafter\def\csname sref@fig:supp-er\endcsname{6}
\expandafter\def\csname sref@fig:supp-mem\endcsname{7}
\expandafter\def\csname sref@sec:supp-stretch\endcsname{K}
\expandafter\def\csname sref@tab:supp-sen1floods\endcsname{19}
\expandafter\def\csname sref@sec:supp-hardware\endcsname{L}
\expandafter\def\csname sref@tab:supp-stretch\endcsname{20}
\expandafter\def\csname sref@tab:supp-blocks\endcsname{21}
\expandafter\def\csname sref@fig:supp-roster\endcsname{8}
\expandafter\def\csname sref@tab:supp-models\endcsname{22}
\expandafter\def\csname sref@tab:supp-hardware\endcsname{23}
\expandafter\def\csname sref@tab:supp-manifest\endcsname{24}
\expandafter\def\csname sref@tab:supp-hwmix\endcsname{25}


==> macro_fallbacks.tex <==
%
%
%
\providecommand{\dropCIDOFAChesBoundaryLOne}{\tbd{dropCIDOFAChesBoundaryLOne}}
\providecommand{\dropCIDOFAChesBoundaryLTwo}{\tbd{dropCIDOFAChesBoundaryLTwo}}
\providecommand{\dropCIDOFAChesCoarseLOne}{\tbd{dropCIDOFAChesCoarseLOne}}
\providecommand{\dropCIDOFAChesCoarseLTwo}{\tbd{dropCIDOFAChesCoarseLTwo}}
\providecommand{\dropCIDOFAChesNlcdREAL}{\tbd{dropCIDOFAChesNlcdREAL}}
\providecommand{\dropCIDOFAChesOmissionLOne}{\tbd{dropCIDOFAChesOmissionLOne}}
\providecommand{\dropCIDOFAChesOmissionLTwo}{\tbd{dropCIDOFAChesOmissionLTwo}}
\providecommand{\dropCIDOFAChesShiftLOne}{\tbd{dropCIDOFAChesShiftLOne}}
\providecommand{\dropCIDOFAChesShiftLTwo}{\tbd{dropCIDOFAChesShiftLTwo}}
\providecommand{\dropCIDOFACsTwelveBoundaryLOne}{\tbd{dropCIDOFACsTwelveBoundaryLOne}}
\providecommand{\dropCIDOFACsTwelveBoundaryLTwo}{\tbd{dropCIDOFACsTwelveBoundaryLTwo}}
\providecommand{\dropCIDOFACsTwelveCoarseLOne}{\tbd{dropCIDOFACsTwelveCoarseLOne}}
\providecommand{\dropCIDOFACsTwelveCoarseLTwo}{\tbd{dropCIDOFACsTwelveCoarseLTwo}}
\providecommand{\dropCIDOFACsTwelveOmissionLOne}{\tbd{dropCIDOFACsTwelveOmissionLOne}}
\providecommand{\dropCIDOFACsTwelveOmissionLTwo}{\tbd{dropCIDOFACsTwelveOmissionLTwo}}
\providecommand{\dropCIDOFACsTwelveSTwocloudlessREAL}{\tbd{dropCIDOFACsTwelveSTwocloudlessREAL}}
\providecommand{\dropCIDOFACsTwelveShiftLOne}{\tbd{dropCIDOFACsTwelveShiftLOne}}
\providecommand{\dropCIDOFACsTwelveShiftLTwo}{\tbd{dropCIDOFACsTwelveShiftLTwo}}
\providecommand{\dropCIDOFADfcBoundaryLOne}{\tbd{dropCIDOFADfcBoundaryLOne}}
\providecommand{\dropCIDOFADfcBoundaryLTwo}{\tbd{dropCIDOFADfcBoundaryLTwo}}
\providecommand{\dropCIDOFADfcCoarseLOne}{\tbd{dropCIDOFADfcCoarseLOne}}
\providecommand{\dropCIDOFADfcCoarseLTwo}{\tbd{dropCIDOFADfcCoarseLTwo}}
\providecommand{\dropCIDOFADfcModisREALVarTrainSubsetRealcov}{\tbd{dropCIDOFADfcModisREALVarTrainSubsetRealcov}}
\providecommand{\dropCIDOFADfcOmissionLOne}{\tbd{dropCIDOFADfcOmissionLOne}}
\providecommand{\dropCIDOFADfcOmissionLTwo}{\tbd{dropCIDOFADfcOmissionLTwo}}
\providecommand{\dropCIDOFADfcShiftLOne}{\tbd{dropCIDOFADfcShiftLOne}}
\providecommand{\dropCIDOFADfcShiftLTwo}{\tbd{dropCIDOFADfcShiftLTwo}}
\providecommand{\dropCIDOFAEnvaBoundaryLOne}{\tbd{dropCIDOFAEnvaBoundaryLOne}}
\providecommand{\dropCIDOFAEnvaBoundaryLTwo}{\tbd{dropCIDOFAEnvaBoundaryLTwo}}
\providecommand{\dropCIDOFAEnvaCoarseLOne}{\tbd{dropCIDOFAEnvaCoarseLOne}}
\providecommand{\dropCIDOFAEnvaCoarseLTwo}{\tbd{dropCIDOFAEnvaCoarseLTwo}}
\providecommand{\dropCIDOFAEnvaNlcdREAL}{\tbd{dropCIDOFAEnvaNlcdREAL}}
\providecommand{\dropCIDOFAEnvaOmissionLOne}{\tbd{dropCIDOFAEnvaOmissionLOne}}
\providecommand{\dropCIDOFAEnvaOmissionLTwo}{\tbd{dropCIDOFAEnvaOmissionLTwo}}
\providecommand{\dropCIDOFAEnvaShiftLOne}{\tbd{dropCIDOFAEnvaShiftLOne}}
\providecommand{\dropCIDOFAEnvaShiftLTwo}{\tbd{dropCIDOFAEnvaShiftLTwo}}
\providecommand{\dropCIDOFAKuroBoundaryLOne}{\tbd{dropCIDOFAKuroBoundaryLOne}}
\providecommand{\dropCIDOFAKuroBoundaryLTwo}{\tbd{dropCIDOFAKuroBoundaryLTwo}}
\providecommand{\dropCIDOFAKuroCemsREALVarTrainSubsetRealcov}{\tbd{dropCIDOFAKuroCemsREALVarTrainSubsetRealcov}}
\providecommand{\dropCIDOFAKuroCoarseLOne}{\tbd{dropCIDOFAKuroCoarseLOne}}
\providecommand{\dropCIDOFAKuroCoarseLTwo}{\tbd{dropCIDOFAKuroCoarseLTwo}}
\providecommand{\dropCIDOFAKuroOmissionLOne}{\tbd{dropCIDOFAKuroOmissionLOne}}
\providecommand{\dropCIDOFAKuroOmissionLTwo}{\tbd{dropCIDOFAKuroOmissionLTwo}}
\providecommand{\dropCIDOFAKuroShiftLOne}{\tbd{dropCIDOFAKuroShiftLOne}}
\providecommand{\dropCIDOFAKuroShiftLTwo}{\tbd{dropCIDOFAKuroShiftLTwo}}
\providecommand{\dropCIDOFAOemBoundaryLOne}{\tbd{dropCIDOFAOemBoundaryLOne}}
\providecommand{\dropCIDOFAOemBoundaryLTwo}{\tbd{dropCIDOFAOemBoundaryLTwo}}
\providecommand{\dropCIDOFAOemCoarseLOne}{\tbd{dropCIDOFAOemCoarseLOne}}
\providecommand{\dropCIDOFAOemCoarseLTwo}{\tbd{dropCIDOFAOemCoarseLTwo}}
\providecommand{\dropCIDOFAOemOmissionLOne}{\tbd{dropCIDOFAOemOmissionLOne}}
\providecommand{\dropCIDOFAOemOmissionLTwo}{\tbd{dropCIDOFAOemOmissionLTwo}}
\providecommand{\dropCIDOFAOemShiftLOne}{\tbd{dropCIDOFAOemShiftLOne}}
\providecommand{\dropCIDOFAOemShiftLTwo}{\tbd{dropCIDOFAOemShiftLTwo}}
\providecommand{\dropCIDOFASnTwoBoundaryLOne}{\tbd{dropCIDOFASnTwoBoundaryLOne}}
\providecommand{\dropCIDOFASnTwoBoundaryLTwo}{\tbd{dropCIDOFASnTwoBoundaryLTwo}}
\providecommand{\dropCIDOFASnTwoCoarseLOne}{\tbd{dropCIDOFASnTwoCoarseLOne}}
\providecommand{\dropCIDOFASnTwoCoarseLTwo}{\tbd{dropCIDOFASnTwoCoarseLTwo}}
\providecommand{\dropCIDOFASnTwoOmissionLOne}{\tbd{dropCIDOFASnTwoOmissionLOne}}
\providecommand{\dropCIDOFASnTwoOmissionLTwo}{\tbd{dropCIDOFASnTwoOmissionLTwo}}
\providecommand{\dropCIDOFASnTwoShiftLOne}{\tbd{dropCIDOFASnTwoShiftLOne}}
\providecommand{\dropCIDOFASnTwoShiftLTwo}{\tbd{dropCIDOFASnTwoShiftLTwo}}
\providecommand{\dropCIDOFAburnBoundaryLOne}{\tbd{dropCIDOFAburnBoundaryLOne}}
\providecommand{\dropCIDOFAburnBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{dropCIDOFAburnBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCIDOFAburnBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{dropCIDOFAburnBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCIDOFAburnBoundaryLOneVarDecoderSamLite}{\tbd{dropCIDOFAburnBoundaryLOneVarDecoderSamLite}}
\providecommand{\dropCIDOFAburnBoundaryLOneVarDecoderSamPretrained}{\tbd{dropCIDOFAburnBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\dropCIDOFAburnBoundaryLOneVarDecoderSegformerMlp}{\tbd{dropCIDOFAburnBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\dropCIDOFAburnBoundaryLR}{\tbd{dropCIDOFAburnBoundaryLR}}
\providecommand{\dropCIDOFAburnBoundaryLTwo}{\tbd{dropCIDOFAburnBoundaryLTwo}}
\providecommand{\dropCIDOFAburnBoundaryLTwoVarBandsRgb}{\tbd{dropCIDOFAburnBoundaryLTwoVarBandsRgb}}
\providecommand{\dropCIDOFAburnBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCIDOFAburnBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCIDOFAburnBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCIDOFAburnBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCIDOFAburnBoundaryLTwoVarDecoderSamLite}{\tbd{dropCIDOFAburnBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropCIDOFAburnBoundaryLTwoVarDecoderSamPretrained}{\tbd{dropCIDOFAburnBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\dropCIDOFAburnBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropCIDOFAburnBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCIDOFAburnBoundaryLTwoVarFrozenEncoderTrue}{\tbd{dropCIDOFAburnBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\dropCIDOFAburnBoundaryLTwoVarLossBootstrap}{\tbd{dropCIDOFAburnBoundaryLTwoVarLossBootstrap}}
\providecommand{\dropCIDOFAburnBoundaryLTwoVarLossGce}{\tbd{dropCIDOFAburnBoundaryLTwoVarLossGce}}
\providecommand{\dropCIDOFAburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCIDOFAburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCIDOFAburnBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCIDOFAburnBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCIDOFAburnCoarseLOne}{\tbd{dropCIDOFAburnCoarseLOne}}
\providecommand{\dropCIDOFAburnCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{dropCIDOFAburnCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCIDOFAburnCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{dropCIDOFAburnCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCIDOFAburnCoarseLOneVarDecoderSamLite}{\tbd{dropCIDOFAburnCoarseLOneVarDecoderSamLite}}
\providecommand{\dropCIDOFAburnCoarseLOneVarDecoderSamPretrained}{\tbd{dropCIDOFAburnCoarseLOneVarDecoderSamPretrained}}
\providecommand{\dropCIDOFAburnCoarseLOneVarDecoderSegformerMlp}{\tbd{dropCIDOFAburnCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\dropCIDOFAburnCoarseLR}{\tbd{dropCIDOFAburnCoarseLR}}
\providecommand{\dropCIDOFAburnCoarseLTwo}{\tbd{dropCIDOFAburnCoarseLTwo}}
\providecommand{\dropCIDOFAburnCoarseLTwoVarBandsRgb}{\tbd{dropCIDOFAburnCoarseLTwoVarBandsRgb}}
\providecommand{\dropCIDOFAburnCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCIDOFAburnCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCIDOFAburnCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCIDOFAburnCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCIDOFAburnCoarseLTwoVarDecoderSamLite}{\tbd{dropCIDOFAburnCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropCIDOFAburnCoarseLTwoVarDecoderSamPretrained}{\tbd{dropCIDOFAburnCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\dropCIDOFAburnCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropCIDOFAburnCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCIDOFAburnCoarseLTwoVarFrozenEncoderTrue}{\tbd{dropCIDOFAburnCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\dropCIDOFAburnCoarseLTwoVarLossBootstrap}{\tbd{dropCIDOFAburnCoarseLTwoVarLossBootstrap}}
\providecommand{\dropCIDOFAburnCoarseLTwoVarLossGce}{\tbd{dropCIDOFAburnCoarseLTwoVarLossGce}}
\providecommand{\dropCIDOFAburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCIDOFAburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCIDOFAburnCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCIDOFAburnCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCIDOFAburnOmissionLOne}{\tbd{dropCIDOFAburnOmissionLOne}}
\providecommand{\dropCIDOFAburnOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{dropCIDOFAburnOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCIDOFAburnOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{dropCIDOFAburnOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCIDOFAburnOmissionLOneVarDecoderSamLite}{\tbd{dropCIDOFAburnOmissionLOneVarDecoderSamLite}}
\providecommand{\dropCIDOFAburnOmissionLOneVarDecoderSamPretrained}{\tbd{dropCIDOFAburnOmissionLOneVarDecoderSamPretrained}}
\providecommand{\dropCIDOFAburnOmissionLOneVarDecoderSegformerMlp}{\tbd{dropCIDOFAburnOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\dropCIDOFAburnOmissionLR}{\tbd{dropCIDOFAburnOmissionLR}}
\providecommand{\dropCIDOFAburnOmissionLTwo}{\tbd{dropCIDOFAburnOmissionLTwo}}
\providecommand{\dropCIDOFAburnOmissionLTwoVarBandsRgb}{\tbd{dropCIDOFAburnOmissionLTwoVarBandsRgb}}
\providecommand{\dropCIDOFAburnOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCIDOFAburnOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCIDOFAburnOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCIDOFAburnOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCIDOFAburnOmissionLTwoVarDecoderSamLite}{\tbd{dropCIDOFAburnOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropCIDOFAburnOmissionLTwoVarDecoderSamPretrained}{\tbd{dropCIDOFAburnOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\dropCIDOFAburnOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropCIDOFAburnOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCIDOFAburnOmissionLTwoVarFrozenEncoderTrue}{\tbd{dropCIDOFAburnOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\dropCIDOFAburnOmissionLTwoVarLossBootstrap}{\tbd{dropCIDOFAburnOmissionLTwoVarLossBootstrap}}
\providecommand{\dropCIDOFAburnOmissionLTwoVarLossGce}{\tbd{dropCIDOFAburnOmissionLTwoVarLossGce}}
\providecommand{\dropCIDOFAburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCIDOFAburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCIDOFAburnOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCIDOFAburnOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCIDOFAburnShiftLOne}{\tbd{dropCIDOFAburnShiftLOne}}
\providecommand{\dropCIDOFAburnShiftLOneVarDecoderMaskTwoformerFull}{\tbd{dropCIDOFAburnShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCIDOFAburnShiftLOneVarDecoderMaskTwoformerLite}{\tbd{dropCIDOFAburnShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCIDOFAburnShiftLOneVarDecoderSamLite}{\tbd{dropCIDOFAburnShiftLOneVarDecoderSamLite}}
\providecommand{\dropCIDOFAburnShiftLOneVarDecoderSamPretrained}{\tbd{dropCIDOFAburnShiftLOneVarDecoderSamPretrained}}
\providecommand{\dropCIDOFAburnShiftLOneVarDecoderSegformerMlp}{\tbd{dropCIDOFAburnShiftLOneVarDecoderSegformerMlp}}
\providecommand{\dropCIDOFAburnShiftLR}{\tbd{dropCIDOFAburnShiftLR}}
\providecommand{\dropCIDOFAburnShiftLTwo}{\tbd{dropCIDOFAburnShiftLTwo}}
\providecommand{\dropCIDOFAburnShiftLTwoVarBandsRgb}{\tbd{dropCIDOFAburnShiftLTwoVarBandsRgb}}
\providecommand{\dropCIDOFAburnShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCIDOFAburnShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCIDOFAburnShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCIDOFAburnShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCIDOFAburnShiftLTwoVarDecoderSamLite}{\tbd{dropCIDOFAburnShiftLTwoVarDecoderSamLite}}
\providecommand{\dropCIDOFAburnShiftLTwoVarDecoderSamPretrained}{\tbd{dropCIDOFAburnShiftLTwoVarDecoderSamPretrained}}
\providecommand{\dropCIDOFAburnShiftLTwoVarDecoderSegformerMlp}{\tbd{dropCIDOFAburnShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCIDOFAburnShiftLTwoVarFrozenEncoderTrue}{\tbd{dropCIDOFAburnShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\dropCIDOFAburnShiftLTwoVarLossBootstrap}{\tbd{dropCIDOFAburnShiftLTwoVarLossBootstrap}}
\providecommand{\dropCIDOFAburnShiftLTwoVarLossGce}{\tbd{dropCIDOFAburnShiftLTwoVarLossGce}}
\providecommand{\dropCIDOFAburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCIDOFAburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCIDOFAburnShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCIDOFAburnShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCIDOFAflairBoundaryLOne}{\tbd{dropCIDOFAflairBoundaryLOne}}
\providecommand{\dropCIDOFAflairBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{dropCIDOFAflairBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCIDOFAflairBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{dropCIDOFAflairBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCIDOFAflairBoundaryLOneVarDecoderSamLite}{\tbd{dropCIDOFAflairBoundaryLOneVarDecoderSamLite}}
\providecommand{\dropCIDOFAflairBoundaryLOneVarDecoderSamPretrained}{\tbd{dropCIDOFAflairBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\dropCIDOFAflairBoundaryLOneVarDecoderSegformerMlp}{\tbd{dropCIDOFAflairBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\dropCIDOFAflairBoundaryLR}{\tbd{dropCIDOFAflairBoundaryLR}}
\providecommand{\dropCIDOFAflairBoundaryLTwo}{\tbd{dropCIDOFAflairBoundaryLTwo}}
\providecommand{\dropCIDOFAflairBoundaryLTwoVarBandsRgb}{\tbd{dropCIDOFAflairBoundaryLTwoVarBandsRgb}}
\providecommand{\dropCIDOFAflairBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCIDOFAflairBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCIDOFAflairBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCIDOFAflairBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCIDOFAflairBoundaryLTwoVarDecoderSamLite}{\tbd{dropCIDOFAflairBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropCIDOFAflairBoundaryLTwoVarDecoderSamPretrained}{\tbd{dropCIDOFAflairBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\dropCIDOFAflairBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropCIDOFAflairBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCIDOFAflairBoundaryLTwoVarFrozenEncoderTrue}{\tbd{dropCIDOFAflairBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\dropCIDOFAflairBoundaryLTwoVarLossBootstrap}{\tbd{dropCIDOFAflairBoundaryLTwoVarLossBootstrap}}
\providecommand{\dropCIDOFAflairBoundaryLTwoVarLossGce}{\tbd{dropCIDOFAflairBoundaryLTwoVarLossGce}}
\providecommand{\dropCIDOFAflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCIDOFAflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCIDOFAflairBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCIDOFAflairBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCIDOFAflairCoarseLOne}{\tbd{dropCIDOFAflairCoarseLOne}}
\providecommand{\dropCIDOFAflairCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{dropCIDOFAflairCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCIDOFAflairCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{dropCIDOFAflairCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCIDOFAflairCoarseLOneVarDecoderSamLite}{\tbd{dropCIDOFAflairCoarseLOneVarDecoderSamLite}}
\providecommand{\dropCIDOFAflairCoarseLOneVarDecoderSamPretrained}{\tbd{dropCIDOFAflairCoarseLOneVarDecoderSamPretrained}}
\providecommand{\dropCIDOFAflairCoarseLOneVarDecoderSegformerMlp}{\tbd{dropCIDOFAflairCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\dropCIDOFAflairCoarseLR}{\tbd{dropCIDOFAflairCoarseLR}}
\providecommand{\dropCIDOFAflairCoarseLTwo}{\tbd{dropCIDOFAflairCoarseLTwo}}
\providecommand{\dropCIDOFAflairCoarseLTwoVarBandsRgb}{\tbd{dropCIDOFAflairCoarseLTwoVarBandsRgb}}
\providecommand{\dropCIDOFAflairCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCIDOFAflairCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCIDOFAflairCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCIDOFAflairCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCIDOFAflairCoarseLTwoVarDecoderSamLite}{\tbd{dropCIDOFAflairCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropCIDOFAflairCoarseLTwoVarDecoderSamPretrained}{\tbd{dropCIDOFAflairCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\dropCIDOFAflairCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropCIDOFAflairCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCIDOFAflairCoarseLTwoVarFrozenEncoderTrue}{\tbd{dropCIDOFAflairCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\dropCIDOFAflairCoarseLTwoVarLossBootstrap}{\tbd{dropCIDOFAflairCoarseLTwoVarLossBootstrap}}
\providecommand{\dropCIDOFAflairCoarseLTwoVarLossGce}{\tbd{dropCIDOFAflairCoarseLTwoVarLossGce}}
\providecommand{\dropCIDOFAflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCIDOFAflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCIDOFAflairCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCIDOFAflairCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCIDOFAflairOmissionLOne}{\tbd{dropCIDOFAflairOmissionLOne}}
\providecommand{\dropCIDOFAflairOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{dropCIDOFAflairOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCIDOFAflairOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{dropCIDOFAflairOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCIDOFAflairOmissionLOneVarDecoderSamLite}{\tbd{dropCIDOFAflairOmissionLOneVarDecoderSamLite}}
\providecommand{\dropCIDOFAflairOmissionLOneVarDecoderSamPretrained}{\tbd{dropCIDOFAflairOmissionLOneVarDecoderSamPretrained}}
\providecommand{\dropCIDOFAflairOmissionLOneVarDecoderSegformerMlp}{\tbd{dropCIDOFAflairOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\dropCIDOFAflairOmissionLR}{\tbd{dropCIDOFAflairOmissionLR}}
\providecommand{\dropCIDOFAflairOmissionLTwo}{\tbd{dropCIDOFAflairOmissionLTwo}}
\providecommand{\dropCIDOFAflairOmissionLTwoVarBandsRgb}{\tbd{dropCIDOFAflairOmissionLTwoVarBandsRgb}}
\providecommand{\dropCIDOFAflairOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCIDOFAflairOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCIDOFAflairOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCIDOFAflairOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCIDOFAflairOmissionLTwoVarDecoderSamLite}{\tbd{dropCIDOFAflairOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropCIDOFAflairOmissionLTwoVarDecoderSamPretrained}{\tbd{dropCIDOFAflairOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\dropCIDOFAflairOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropCIDOFAflairOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCIDOFAflairOmissionLTwoVarFrozenEncoderTrue}{\tbd{dropCIDOFAflairOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\dropCIDOFAflairOmissionLTwoVarLossBootstrap}{\tbd{dropCIDOFAflairOmissionLTwoVarLossBootstrap}}
\providecommand{\dropCIDOFAflairOmissionLTwoVarLossGce}{\tbd{dropCIDOFAflairOmissionLTwoVarLossGce}}
\providecommand{\dropCIDOFAflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCIDOFAflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCIDOFAflairOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCIDOFAflairOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCIDOFAflairShiftLOne}{\tbd{dropCIDOFAflairShiftLOne}}
\providecommand{\dropCIDOFAflairShiftLOneVarDecoderMaskTwoformerFull}{\tbd{dropCIDOFAflairShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCIDOFAflairShiftLOneVarDecoderMaskTwoformerLite}{\tbd{dropCIDOFAflairShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCIDOFAflairShiftLOneVarDecoderSamLite}{\tbd{dropCIDOFAflairShiftLOneVarDecoderSamLite}}
\providecommand{\dropCIDOFAflairShiftLOneVarDecoderSamPretrained}{\tbd{dropCIDOFAflairShiftLOneVarDecoderSamPretrained}}
\providecommand{\dropCIDOFAflairShiftLOneVarDecoderSegformerMlp}{\tbd{dropCIDOFAflairShiftLOneVarDecoderSegformerMlp}}
\providecommand{\dropCIDOFAflairShiftLR}{\tbd{dropCIDOFAflairShiftLR}}
\providecommand{\dropCIDOFAflairShiftLTwo}{\tbd{dropCIDOFAflairShiftLTwo}}
\providecommand{\dropCIDOFAflairShiftLTwoVarBandsRgb}{\tbd{dropCIDOFAflairShiftLTwoVarBandsRgb}}
\providecommand{\dropCIDOFAflairShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCIDOFAflairShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCIDOFAflairShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCIDOFAflairShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCIDOFAflairShiftLTwoVarDecoderSamLite}{\tbd{dropCIDOFAflairShiftLTwoVarDecoderSamLite}}
\providecommand{\dropCIDOFAflairShiftLTwoVarDecoderSamPretrained}{\tbd{dropCIDOFAflairShiftLTwoVarDecoderSamPretrained}}
\providecommand{\dropCIDOFAflairShiftLTwoVarDecoderSegformerMlp}{\tbd{dropCIDOFAflairShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCIDOFAflairShiftLTwoVarFrozenEncoderTrue}{\tbd{dropCIDOFAflairShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\dropCIDOFAflairShiftLTwoVarLossBootstrap}{\tbd{dropCIDOFAflairShiftLTwoVarLossBootstrap}}
\providecommand{\dropCIDOFAflairShiftLTwoVarLossGce}{\tbd{dropCIDOFAflairShiftLTwoVarLossGce}}
\providecommand{\dropCIDOFAflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCIDOFAflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCIDOFAflairShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCIDOFAflairShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCIDOFAsenOtsuLTwo}{\tbd{dropCIDOFAsenOtsuLTwo}}
\providecommand{\dropCIDinovThreeConvnextLburnBoundaryLOne}{\tbd{dropCIDinovThreeConvnextLburnBoundaryLOne}}
\providecommand{\dropCIDinovThreeConvnextLburnBoundaryLTwo}{\tbd{dropCIDinovThreeConvnextLburnBoundaryLTwo}}
\providecommand{\dropCIDinovThreeConvnextLburnCoarseLOne}{\tbd{dropCIDinovThreeConvnextLburnCoarseLOne}}
\providecommand{\dropCIDinovThreeConvnextLburnCoarseLTwo}{\tbd{dropCIDinovThreeConvnextLburnCoarseLTwo}}
\providecommand{\dropCIDinovThreeConvnextLburnOmissionLOne}{\tbd{dropCIDinovThreeConvnextLburnOmissionLOne}}
\providecommand{\dropCIDinovThreeConvnextLburnOmissionLTwo}{\tbd{dropCIDinovThreeConvnextLburnOmissionLTwo}}
\providecommand{\dropCIDinovThreeConvnextLburnShiftLOne}{\tbd{dropCIDinovThreeConvnextLburnShiftLOne}}
\providecommand{\dropCIDinovThreeConvnextLburnShiftLTwo}{\tbd{dropCIDinovThreeConvnextLburnShiftLTwo}}
\providecommand{\dropCIDinovThreeConvnextLflairBoundaryLOne}{\tbd{dropCIDinovThreeConvnextLflairBoundaryLOne}}
\providecommand{\dropCIDinovThreeConvnextLflairBoundaryLTwo}{\tbd{dropCIDinovThreeConvnextLflairBoundaryLTwo}}
\providecommand{\dropCIDinovThreeConvnextLflairCoarseLOne}{\tbd{dropCIDinovThreeConvnextLflairCoarseLOne}}
\providecommand{\dropCIDinovThreeConvnextLflairCoarseLTwo}{\tbd{dropCIDinovThreeConvnextLflairCoarseLTwo}}
\providecommand{\dropCIDinovThreeConvnextLflairOmissionLOne}{\tbd{dropCIDinovThreeConvnextLflairOmissionLOne}}
\providecommand{\dropCIDinovThreeConvnextLflairOmissionLTwo}{\tbd{dropCIDinovThreeConvnextLflairOmissionLTwo}}
\providecommand{\dropCIDinovThreeConvnextLflairShiftLOne}{\tbd{dropCIDinovThreeConvnextLflairShiftLOne}}
\providecommand{\dropCIDinovThreeConvnextLflairShiftLTwo}{\tbd{dropCIDinovThreeConvnextLflairShiftLTwo}}
\providecommand{\dropCILVDChesBoundaryLOne}{\tbd{dropCILVDChesBoundaryLOne}}
\providecommand{\dropCILVDChesBoundaryLTwo}{\tbd{dropCILVDChesBoundaryLTwo}}
\providecommand{\dropCILVDChesBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCILVDChesBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDChesBoundaryLTwoVarDecoderSamLite}{\tbd{dropCILVDChesBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropCILVDChesBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropCILVDChesBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCILVDChesBoundaryLTwoVarLrMultOne}{\tbd{dropCILVDChesBoundaryLTwoVarLrMultOne}}
\providecommand{\dropCILVDChesCoarseLOne}{\tbd{dropCILVDChesCoarseLOne}}
\providecommand{\dropCILVDChesCoarseLTwo}{\tbd{dropCILVDChesCoarseLTwo}}
\providecommand{\dropCILVDChesCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCILVDChesCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDChesCoarseLTwoVarDecoderSamLite}{\tbd{dropCILVDChesCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropCILVDChesCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropCILVDChesCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCILVDChesCoarseLTwoVarLrMultOne}{\tbd{dropCILVDChesCoarseLTwoVarLrMultOne}}
\providecommand{\dropCILVDChesNlcdREAL}{\tbd{dropCILVDChesNlcdREAL}}
\providecommand{\dropCILVDChesOmissionLOne}{\tbd{dropCILVDChesOmissionLOne}}
\providecommand{\dropCILVDChesOmissionLTwo}{\tbd{dropCILVDChesOmissionLTwo}}
\providecommand{\dropCILVDChesOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCILVDChesOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDChesOmissionLTwoVarDecoderSamLite}{\tbd{dropCILVDChesOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropCILVDChesOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropCILVDChesOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCILVDChesOmissionLTwoVarLrMultOne}{\tbd{dropCILVDChesOmissionLTwoVarLrMultOne}}
\providecommand{\dropCILVDChesShiftLOne}{\tbd{dropCILVDChesShiftLOne}}
\providecommand{\dropCILVDChesShiftLTwo}{\tbd{dropCILVDChesShiftLTwo}}
\providecommand{\dropCILVDChesShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCILVDChesShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDChesShiftLTwoVarDecoderSamLite}{\tbd{dropCILVDChesShiftLTwoVarDecoderSamLite}}
\providecommand{\dropCILVDChesShiftLTwoVarDecoderSegformerMlp}{\tbd{dropCILVDChesShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCILVDChesShiftLTwoVarLrMultOne}{\tbd{dropCILVDChesShiftLTwoVarLrMultOne}}
\providecommand{\dropCILVDCsTwelveBoundaryLOne}{\tbd{dropCILVDCsTwelveBoundaryLOne}}
\providecommand{\dropCILVDCsTwelveBoundaryLTwo}{\tbd{dropCILVDCsTwelveBoundaryLTwo}}
\providecommand{\dropCILVDCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCILVDCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDCsTwelveBoundaryLTwoVarDecoderSamLite}{\tbd{dropCILVDCsTwelveBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropCILVDCsTwelveBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropCILVDCsTwelveBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCILVDCsTwelveBoundaryLTwoVarLrMultOne}{\tbd{dropCILVDCsTwelveBoundaryLTwoVarLrMultOne}}
\providecommand{\dropCILVDCsTwelveCoarseLOne}{\tbd{dropCILVDCsTwelveCoarseLOne}}
\providecommand{\dropCILVDCsTwelveCoarseLTwo}{\tbd{dropCILVDCsTwelveCoarseLTwo}}
\providecommand{\dropCILVDCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCILVDCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDCsTwelveCoarseLTwoVarDecoderSamLite}{\tbd{dropCILVDCsTwelveCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropCILVDCsTwelveCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropCILVDCsTwelveCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCILVDCsTwelveCoarseLTwoVarLrMultOne}{\tbd{dropCILVDCsTwelveCoarseLTwoVarLrMultOne}}
\providecommand{\dropCILVDCsTwelveOmissionLOne}{\tbd{dropCILVDCsTwelveOmissionLOne}}
\providecommand{\dropCILVDCsTwelveOmissionLTwo}{\tbd{dropCILVDCsTwelveOmissionLTwo}}
\providecommand{\dropCILVDCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCILVDCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDCsTwelveOmissionLTwoVarDecoderSamLite}{\tbd{dropCILVDCsTwelveOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropCILVDCsTwelveOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropCILVDCsTwelveOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCILVDCsTwelveOmissionLTwoVarLrMultOne}{\tbd{dropCILVDCsTwelveOmissionLTwoVarLrMultOne}}
\providecommand{\dropCILVDCsTwelveSTwocloudlessREAL}{\tbd{dropCILVDCsTwelveSTwocloudlessREAL}}
\providecommand{\dropCILVDCsTwelveShiftLOne}{\tbd{dropCILVDCsTwelveShiftLOne}}
\providecommand{\dropCILVDCsTwelveShiftLTwo}{\tbd{dropCILVDCsTwelveShiftLTwo}}
\providecommand{\dropCILVDCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCILVDCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDCsTwelveShiftLTwoVarDecoderSamLite}{\tbd{dropCILVDCsTwelveShiftLTwoVarDecoderSamLite}}
\providecommand{\dropCILVDCsTwelveShiftLTwoVarDecoderSegformerMlp}{\tbd{dropCILVDCsTwelveShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCILVDCsTwelveShiftLTwoVarLrMultOne}{\tbd{dropCILVDCsTwelveShiftLTwoVarLrMultOne}}
\providecommand{\dropCILVDDfcBoundaryLOne}{\tbd{dropCILVDDfcBoundaryLOne}}
\providecommand{\dropCILVDDfcBoundaryLTwo}{\tbd{dropCILVDDfcBoundaryLTwo}}
\providecommand{\dropCILVDDfcBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCILVDDfcBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDDfcBoundaryLTwoVarDecoderSamLite}{\tbd{dropCILVDDfcBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropCILVDDfcBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropCILVDDfcBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCILVDDfcBoundaryLTwoVarLrMultOne}{\tbd{dropCILVDDfcBoundaryLTwoVarLrMultOne}}
\providecommand{\dropCILVDDfcCoarseLOne}{\tbd{dropCILVDDfcCoarseLOne}}
\providecommand{\dropCILVDDfcCoarseLTwo}{\tbd{dropCILVDDfcCoarseLTwo}}
\providecommand{\dropCILVDDfcCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCILVDDfcCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDDfcCoarseLTwoVarDecoderSamLite}{\tbd{dropCILVDDfcCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropCILVDDfcCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropCILVDDfcCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCILVDDfcCoarseLTwoVarLrMultOne}{\tbd{dropCILVDDfcCoarseLTwoVarLrMultOne}}
\providecommand{\dropCILVDDfcModisREALVarTrainSubsetRealcov}{\tbd{dropCILVDDfcModisREALVarTrainSubsetRealcov}}
\providecommand{\dropCILVDDfcOmissionLOne}{\tbd{dropCILVDDfcOmissionLOne}}
\providecommand{\dropCILVDDfcOmissionLTwo}{\tbd{dropCILVDDfcOmissionLTwo}}
\providecommand{\dropCILVDDfcOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCILVDDfcOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDDfcOmissionLTwoVarDecoderSamLite}{\tbd{dropCILVDDfcOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropCILVDDfcOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropCILVDDfcOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCILVDDfcOmissionLTwoVarLrMultOne}{\tbd{dropCILVDDfcOmissionLTwoVarLrMultOne}}
\providecommand{\dropCILVDDfcShiftLOne}{\tbd{dropCILVDDfcShiftLOne}}
\providecommand{\dropCILVDDfcShiftLTwo}{\tbd{dropCILVDDfcShiftLTwo}}
\providecommand{\dropCILVDDfcShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCILVDDfcShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDDfcShiftLTwoVarDecoderSamLite}{\tbd{dropCILVDDfcShiftLTwoVarDecoderSamLite}}
\providecommand{\dropCILVDDfcShiftLTwoVarDecoderSegformerMlp}{\tbd{dropCILVDDfcShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCILVDDfcShiftLTwoVarLrMultOne}{\tbd{dropCILVDDfcShiftLTwoVarLrMultOne}}
\providecommand{\dropCILVDEnvaBoundaryLOne}{\tbd{dropCILVDEnvaBoundaryLOne}}
\providecommand{\dropCILVDEnvaBoundaryLTwo}{\tbd{dropCILVDEnvaBoundaryLTwo}}
\providecommand{\dropCILVDEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCILVDEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDEnvaBoundaryLTwoVarDecoderSamLite}{\tbd{dropCILVDEnvaBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropCILVDEnvaBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropCILVDEnvaBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCILVDEnvaBoundaryLTwoVarLrMultOne}{\tbd{dropCILVDEnvaBoundaryLTwoVarLrMultOne}}
\providecommand{\dropCILVDEnvaCoarseLOne}{\tbd{dropCILVDEnvaCoarseLOne}}
\providecommand{\dropCILVDEnvaCoarseLTwo}{\tbd{dropCILVDEnvaCoarseLTwo}}
\providecommand{\dropCILVDEnvaCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCILVDEnvaCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDEnvaCoarseLTwoVarDecoderSamLite}{\tbd{dropCILVDEnvaCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropCILVDEnvaCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropCILVDEnvaCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCILVDEnvaCoarseLTwoVarLrMultOne}{\tbd{dropCILVDEnvaCoarseLTwoVarLrMultOne}}
\providecommand{\dropCILVDEnvaNlcdREAL}{\tbd{dropCILVDEnvaNlcdREAL}}
\providecommand{\dropCILVDEnvaOmissionLOne}{\tbd{dropCILVDEnvaOmissionLOne}}
\providecommand{\dropCILVDEnvaOmissionLTwo}{\tbd{dropCILVDEnvaOmissionLTwo}}
\providecommand{\dropCILVDEnvaOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCILVDEnvaOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDEnvaOmissionLTwoVarDecoderSamLite}{\tbd{dropCILVDEnvaOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropCILVDEnvaOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropCILVDEnvaOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCILVDEnvaOmissionLTwoVarLrMultOne}{\tbd{dropCILVDEnvaOmissionLTwoVarLrMultOne}}
\providecommand{\dropCILVDEnvaShiftLOne}{\tbd{dropCILVDEnvaShiftLOne}}
\providecommand{\dropCILVDEnvaShiftLTwo}{\tbd{dropCILVDEnvaShiftLTwo}}
\providecommand{\dropCILVDEnvaShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCILVDEnvaShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDEnvaShiftLTwoVarDecoderSamLite}{\tbd{dropCILVDEnvaShiftLTwoVarDecoderSamLite}}
\providecommand{\dropCILVDEnvaShiftLTwoVarDecoderSegformerMlp}{\tbd{dropCILVDEnvaShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCILVDEnvaShiftLTwoVarLrMultOne}{\tbd{dropCILVDEnvaShiftLTwoVarLrMultOne}}
\providecommand{\dropCILVDKuroBoundaryLOne}{\tbd{dropCILVDKuroBoundaryLOne}}
\providecommand{\dropCILVDKuroBoundaryLTwo}{\tbd{dropCILVDKuroBoundaryLTwo}}
\providecommand{\dropCILVDKuroBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCILVDKuroBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDKuroBoundaryLTwoVarDecoderSamLite}{\tbd{dropCILVDKuroBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropCILVDKuroBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropCILVDKuroBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCILVDKuroBoundaryLTwoVarLrMultOne}{\tbd{dropCILVDKuroBoundaryLTwoVarLrMultOne}}
\providecommand{\dropCILVDKuroCemsREALVarTrainSubsetRealcov}{\tbd{dropCILVDKuroCemsREALVarTrainSubsetRealcov}}
\providecommand{\dropCILVDKuroCoarseLOne}{\tbd{dropCILVDKuroCoarseLOne}}
\providecommand{\dropCILVDKuroCoarseLTwo}{\tbd{dropCILVDKuroCoarseLTwo}}
\providecommand{\dropCILVDKuroCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCILVDKuroCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDKuroCoarseLTwoVarDecoderSamLite}{\tbd{dropCILVDKuroCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropCILVDKuroCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropCILVDKuroCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCILVDKuroCoarseLTwoVarLrMultOne}{\tbd{dropCILVDKuroCoarseLTwoVarLrMultOne}}
\providecommand{\dropCILVDKuroOmissionLOne}{\tbd{dropCILVDKuroOmissionLOne}}
\providecommand{\dropCILVDKuroOmissionLTwo}{\tbd{dropCILVDKuroOmissionLTwo}}
\providecommand{\dropCILVDKuroOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCILVDKuroOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDKuroOmissionLTwoVarDecoderSamLite}{\tbd{dropCILVDKuroOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropCILVDKuroOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropCILVDKuroOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCILVDKuroOmissionLTwoVarLrMultOne}{\tbd{dropCILVDKuroOmissionLTwoVarLrMultOne}}
\providecommand{\dropCILVDKuroShiftLOne}{\tbd{dropCILVDKuroShiftLOne}}
\providecommand{\dropCILVDKuroShiftLTwo}{\tbd{dropCILVDKuroShiftLTwo}}
\providecommand{\dropCILVDKuroShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCILVDKuroShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDKuroShiftLTwoVarDecoderSamLite}{\tbd{dropCILVDKuroShiftLTwoVarDecoderSamLite}}
\providecommand{\dropCILVDKuroShiftLTwoVarDecoderSegformerMlp}{\tbd{dropCILVDKuroShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCILVDKuroShiftLTwoVarLrMultOne}{\tbd{dropCILVDKuroShiftLTwoVarLrMultOne}}
\providecommand{\dropCILVDOemBoundaryLOne}{\tbd{dropCILVDOemBoundaryLOne}}
\providecommand{\dropCILVDOemBoundaryLTwo}{\tbd{dropCILVDOemBoundaryLTwo}}
\providecommand{\dropCILVDOemBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCILVDOemBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDOemBoundaryLTwoVarDecoderSamLite}{\tbd{dropCILVDOemBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropCILVDOemBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropCILVDOemBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCILVDOemBoundaryLTwoVarLrMultOne}{\tbd{dropCILVDOemBoundaryLTwoVarLrMultOne}}
\providecommand{\dropCILVDOemCoarseLOne}{\tbd{dropCILVDOemCoarseLOne}}
\providecommand{\dropCILVDOemCoarseLTwo}{\tbd{dropCILVDOemCoarseLTwo}}
\providecommand{\dropCILVDOemCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCILVDOemCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDOemCoarseLTwoVarDecoderSamLite}{\tbd{dropCILVDOemCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropCILVDOemCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropCILVDOemCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCILVDOemCoarseLTwoVarLrMultOne}{\tbd{dropCILVDOemCoarseLTwoVarLrMultOne}}
\providecommand{\dropCILVDOemOmissionLOne}{\tbd{dropCILVDOemOmissionLOne}}
\providecommand{\dropCILVDOemOmissionLTwo}{\tbd{dropCILVDOemOmissionLTwo}}
\providecommand{\dropCILVDOemOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCILVDOemOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDOemOmissionLTwoVarDecoderSamLite}{\tbd{dropCILVDOemOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropCILVDOemOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropCILVDOemOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCILVDOemOmissionLTwoVarLrMultOne}{\tbd{dropCILVDOemOmissionLTwoVarLrMultOne}}
\providecommand{\dropCILVDOemShiftLOne}{\tbd{dropCILVDOemShiftLOne}}
\providecommand{\dropCILVDOemShiftLTwo}{\tbd{dropCILVDOemShiftLTwo}}
\providecommand{\dropCILVDOemShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCILVDOemShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDOemShiftLTwoVarDecoderSamLite}{\tbd{dropCILVDOemShiftLTwoVarDecoderSamLite}}
\providecommand{\dropCILVDOemShiftLTwoVarDecoderSegformerMlp}{\tbd{dropCILVDOemShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCILVDOemShiftLTwoVarLrMultOne}{\tbd{dropCILVDOemShiftLTwoVarLrMultOne}}
\providecommand{\dropCILVDSnTwoBoundaryLOne}{\tbd{dropCILVDSnTwoBoundaryLOne}}
\providecommand{\dropCILVDSnTwoBoundaryLTwo}{\tbd{dropCILVDSnTwoBoundaryLTwo}}
\providecommand{\dropCILVDSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCILVDSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDSnTwoBoundaryLTwoVarDecoderSamLite}{\tbd{dropCILVDSnTwoBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropCILVDSnTwoBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropCILVDSnTwoBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCILVDSnTwoBoundaryLTwoVarLrMultOne}{\tbd{dropCILVDSnTwoBoundaryLTwoVarLrMultOne}}
\providecommand{\dropCILVDSnTwoCoarseLOne}{\tbd{dropCILVDSnTwoCoarseLOne}}
\providecommand{\dropCILVDSnTwoCoarseLTwo}{\tbd{dropCILVDSnTwoCoarseLTwo}}
\providecommand{\dropCILVDSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCILVDSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDSnTwoCoarseLTwoVarDecoderSamLite}{\tbd{dropCILVDSnTwoCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropCILVDSnTwoCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropCILVDSnTwoCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCILVDSnTwoCoarseLTwoVarLrMultOne}{\tbd{dropCILVDSnTwoCoarseLTwoVarLrMultOne}}
\providecommand{\dropCILVDSnTwoOmissionLOne}{\tbd{dropCILVDSnTwoOmissionLOne}}
\providecommand{\dropCILVDSnTwoOmissionLTwo}{\tbd{dropCILVDSnTwoOmissionLTwo}}
\providecommand{\dropCILVDSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCILVDSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDSnTwoOmissionLTwoVarDecoderSamLite}{\tbd{dropCILVDSnTwoOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropCILVDSnTwoOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropCILVDSnTwoOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCILVDSnTwoOmissionLTwoVarLrMultOne}{\tbd{dropCILVDSnTwoOmissionLTwoVarLrMultOne}}
\providecommand{\dropCILVDSnTwoShiftLOne}{\tbd{dropCILVDSnTwoShiftLOne}}
\providecommand{\dropCILVDSnTwoShiftLTwo}{\tbd{dropCILVDSnTwoShiftLTwo}}
\providecommand{\dropCILVDSnTwoShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCILVDSnTwoShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDSnTwoShiftLTwoVarDecoderSamLite}{\tbd{dropCILVDSnTwoShiftLTwoVarDecoderSamLite}}
\providecommand{\dropCILVDSnTwoShiftLTwoVarDecoderSegformerMlp}{\tbd{dropCILVDSnTwoShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCILVDSnTwoShiftLTwoVarLrMultOne}{\tbd{dropCILVDSnTwoShiftLTwoVarLrMultOne}}
\providecommand{\dropCILVDburnBoundaryLOne}{\tbd{dropCILVDburnBoundaryLOne}}
\providecommand{\dropCILVDburnBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{dropCILVDburnBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCILVDburnBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{dropCILVDburnBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDburnBoundaryLOneVarDecoderSamLite}{\tbd{dropCILVDburnBoundaryLOneVarDecoderSamLite}}
\providecommand{\dropCILVDburnBoundaryLOneVarDecoderSamPretrained}{\tbd{dropCILVDburnBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\dropCILVDburnBoundaryLOneVarDecoderSegformerMlp}{\tbd{dropCILVDburnBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\dropCILVDburnBoundaryLR}{\tbd{dropCILVDburnBoundaryLR}}
\providecommand{\dropCILVDburnBoundaryLRVarLrMultOne}{\tbd{dropCILVDburnBoundaryLRVarLrMultOne}}
\providecommand{\dropCILVDburnBoundaryLTwo}{\tbd{dropCILVDburnBoundaryLTwo}}
\providecommand{\dropCILVDburnBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCILVDburnBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCILVDburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{dropCILVDburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\dropCILVDburnBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCILVDburnBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{dropCILVDburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\dropCILVDburnBoundaryLTwoVarDecoderSamLite}{\tbd{dropCILVDburnBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropCILVDburnBoundaryLTwoVarDecoderSamLiteLrMultOne}{\tbd{dropCILVDburnBoundaryLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\dropCILVDburnBoundaryLTwoVarDecoderSamPretrained}{\tbd{dropCILVDburnBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\dropCILVDburnBoundaryLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{dropCILVDburnBoundaryLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\dropCILVDburnBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropCILVDburnBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCILVDburnBoundaryLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{dropCILVDburnBoundaryLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\dropCILVDburnBoundaryLTwoVarLossBootstrap}{\tbd{dropCILVDburnBoundaryLTwoVarLossBootstrap}}
\providecommand{\dropCILVDburnBoundaryLTwoVarLossGce}{\tbd{dropCILVDburnBoundaryLTwoVarLossGce}}
\providecommand{\dropCILVDburnBoundaryLTwoVarLrMultOne}{\tbd{dropCILVDburnBoundaryLTwoVarLrMultOne}}
\providecommand{\dropCILVDburnBoundaryLTwoVarLrMultThree}{\tbd{dropCILVDburnBoundaryLTwoVarLrMultThree}}
\providecommand{\dropCILVDburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCILVDburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCILVDburnBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCILVDburnBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCILVDburnCoarseLOne}{\tbd{dropCILVDburnCoarseLOne}}
\providecommand{\dropCILVDburnCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{dropCILVDburnCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCILVDburnCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{dropCILVDburnCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDburnCoarseLOneVarDecoderSamLite}{\tbd{dropCILVDburnCoarseLOneVarDecoderSamLite}}
\providecommand{\dropCILVDburnCoarseLOneVarDecoderSamPretrained}{\tbd{dropCILVDburnCoarseLOneVarDecoderSamPretrained}}
\providecommand{\dropCILVDburnCoarseLOneVarDecoderSegformerMlp}{\tbd{dropCILVDburnCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\dropCILVDburnCoarseLR}{\tbd{dropCILVDburnCoarseLR}}
\providecommand{\dropCILVDburnCoarseLRVarLrMultOne}{\tbd{dropCILVDburnCoarseLRVarLrMultOne}}
\providecommand{\dropCILVDburnCoarseLTwo}{\tbd{dropCILVDburnCoarseLTwo}}
\providecommand{\dropCILVDburnCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCILVDburnCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCILVDburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{dropCILVDburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\dropCILVDburnCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCILVDburnCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{dropCILVDburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\dropCILVDburnCoarseLTwoVarDecoderSamLite}{\tbd{dropCILVDburnCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropCILVDburnCoarseLTwoVarDecoderSamLiteLrMultOne}{\tbd{dropCILVDburnCoarseLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\dropCILVDburnCoarseLTwoVarDecoderSamPretrained}{\tbd{dropCILVDburnCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\dropCILVDburnCoarseLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{dropCILVDburnCoarseLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\dropCILVDburnCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropCILVDburnCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCILVDburnCoarseLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{dropCILVDburnCoarseLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\dropCILVDburnCoarseLTwoVarLossBootstrap}{\tbd{dropCILVDburnCoarseLTwoVarLossBootstrap}}
\providecommand{\dropCILVDburnCoarseLTwoVarLossGce}{\tbd{dropCILVDburnCoarseLTwoVarLossGce}}
\providecommand{\dropCILVDburnCoarseLTwoVarLrMultOne}{\tbd{dropCILVDburnCoarseLTwoVarLrMultOne}}
\providecommand{\dropCILVDburnCoarseLTwoVarLrMultThree}{\tbd{dropCILVDburnCoarseLTwoVarLrMultThree}}
\providecommand{\dropCILVDburnCoarseLTwoVarLrMultZeroOneOneOneOne}{\tbd{dropCILVDburnCoarseLTwoVarLrMultZeroOneOneOneOne}}
\providecommand{\dropCILVDburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCILVDburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCILVDburnCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCILVDburnCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCILVDburnOmissionLOne}{\tbd{dropCILVDburnOmissionLOne}}
\providecommand{\dropCILVDburnOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{dropCILVDburnOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCILVDburnOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{dropCILVDburnOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDburnOmissionLOneVarDecoderSamLite}{\tbd{dropCILVDburnOmissionLOneVarDecoderSamLite}}
\providecommand{\dropCILVDburnOmissionLOneVarDecoderSamPretrained}{\tbd{dropCILVDburnOmissionLOneVarDecoderSamPretrained}}
\providecommand{\dropCILVDburnOmissionLOneVarDecoderSegformerMlp}{\tbd{dropCILVDburnOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\dropCILVDburnOmissionLR}{\tbd{dropCILVDburnOmissionLR}}
\providecommand{\dropCILVDburnOmissionLRVarLrMultOne}{\tbd{dropCILVDburnOmissionLRVarLrMultOne}}
\providecommand{\dropCILVDburnOmissionLTwo}{\tbd{dropCILVDburnOmissionLTwo}}
\providecommand{\dropCILVDburnOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCILVDburnOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCILVDburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{dropCILVDburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\dropCILVDburnOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCILVDburnOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{dropCILVDburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\dropCILVDburnOmissionLTwoVarDecoderSamLite}{\tbd{dropCILVDburnOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropCILVDburnOmissionLTwoVarDecoderSamLiteLrMultOne}{\tbd{dropCILVDburnOmissionLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\dropCILVDburnOmissionLTwoVarDecoderSamPretrained}{\tbd{dropCILVDburnOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\dropCILVDburnOmissionLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{dropCILVDburnOmissionLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\dropCILVDburnOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropCILVDburnOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCILVDburnOmissionLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{dropCILVDburnOmissionLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\dropCILVDburnOmissionLTwoVarLossBootstrap}{\tbd{dropCILVDburnOmissionLTwoVarLossBootstrap}}
\providecommand{\dropCILVDburnOmissionLTwoVarLossGce}{\tbd{dropCILVDburnOmissionLTwoVarLossGce}}
\providecommand{\dropCILVDburnOmissionLTwoVarLrMultOne}{\tbd{dropCILVDburnOmissionLTwoVarLrMultOne}}
\providecommand{\dropCILVDburnOmissionLTwoVarLrMultThree}{\tbd{dropCILVDburnOmissionLTwoVarLrMultThree}}
\providecommand{\dropCILVDburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCILVDburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCILVDburnOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCILVDburnOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCILVDburnShiftLOne}{\tbd{dropCILVDburnShiftLOne}}
\providecommand{\dropCILVDburnShiftLOneVarDecoderMaskTwoformerFull}{\tbd{dropCILVDburnShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCILVDburnShiftLOneVarDecoderMaskTwoformerLite}{\tbd{dropCILVDburnShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDburnShiftLOneVarDecoderSamLite}{\tbd{dropCILVDburnShiftLOneVarDecoderSamLite}}
\providecommand{\dropCILVDburnShiftLOneVarDecoderSamPretrained}{\tbd{dropCILVDburnShiftLOneVarDecoderSamPretrained}}
\providecommand{\dropCILVDburnShiftLOneVarDecoderSegformerMlp}{\tbd{dropCILVDburnShiftLOneVarDecoderSegformerMlp}}
\providecommand{\dropCILVDburnShiftLR}{\tbd{dropCILVDburnShiftLR}}
\providecommand{\dropCILVDburnShiftLRVarLrMultOne}{\tbd{dropCILVDburnShiftLRVarLrMultOne}}
\providecommand{\dropCILVDburnShiftLTwo}{\tbd{dropCILVDburnShiftLTwo}}
\providecommand{\dropCILVDburnShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCILVDburnShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCILVDburnShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{dropCILVDburnShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\dropCILVDburnShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCILVDburnShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{dropCILVDburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\dropCILVDburnShiftLTwoVarDecoderSamLite}{\tbd{dropCILVDburnShiftLTwoVarDecoderSamLite}}
\providecommand{\dropCILVDburnShiftLTwoVarDecoderSamLiteLrMultOne}{\tbd{dropCILVDburnShiftLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\dropCILVDburnShiftLTwoVarDecoderSamPretrained}{\tbd{dropCILVDburnShiftLTwoVarDecoderSamPretrained}}
\providecommand{\dropCILVDburnShiftLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{dropCILVDburnShiftLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\dropCILVDburnShiftLTwoVarDecoderSegformerMlp}{\tbd{dropCILVDburnShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCILVDburnShiftLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{dropCILVDburnShiftLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\dropCILVDburnShiftLTwoVarLossBootstrap}{\tbd{dropCILVDburnShiftLTwoVarLossBootstrap}}
\providecommand{\dropCILVDburnShiftLTwoVarLossGce}{\tbd{dropCILVDburnShiftLTwoVarLossGce}}
\providecommand{\dropCILVDburnShiftLTwoVarLrMultOne}{\tbd{dropCILVDburnShiftLTwoVarLrMultOne}}
\providecommand{\dropCILVDburnShiftLTwoVarLrMultThree}{\tbd{dropCILVDburnShiftLTwoVarLrMultThree}}
\providecommand{\dropCILVDburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCILVDburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCILVDburnShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCILVDburnShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCILVDflairBoundaryLOne}{\tbd{dropCILVDflairBoundaryLOne}}
\providecommand{\dropCILVDflairBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{dropCILVDflairBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCILVDflairBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{dropCILVDflairBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDflairBoundaryLOneVarDecoderSamLite}{\tbd{dropCILVDflairBoundaryLOneVarDecoderSamLite}}
\providecommand{\dropCILVDflairBoundaryLOneVarDecoderSamPretrained}{\tbd{dropCILVDflairBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\dropCILVDflairBoundaryLOneVarDecoderSegformerMlp}{\tbd{dropCILVDflairBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\dropCILVDflairBoundaryLR}{\tbd{dropCILVDflairBoundaryLR}}
\providecommand{\dropCILVDflairBoundaryLRVarLrMultOne}{\tbd{dropCILVDflairBoundaryLRVarLrMultOne}}
\providecommand{\dropCILVDflairBoundaryLTwo}{\tbd{dropCILVDflairBoundaryLTwo}}
\providecommand{\dropCILVDflairBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCILVDflairBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCILVDflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{dropCILVDflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\dropCILVDflairBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCILVDflairBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{dropCILVDflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\dropCILVDflairBoundaryLTwoVarDecoderSamLite}{\tbd{dropCILVDflairBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropCILVDflairBoundaryLTwoVarDecoderSamLiteLrMultOne}{\tbd{dropCILVDflairBoundaryLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\dropCILVDflairBoundaryLTwoVarDecoderSamPretrained}{\tbd{dropCILVDflairBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\dropCILVDflairBoundaryLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{dropCILVDflairBoundaryLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\dropCILVDflairBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropCILVDflairBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCILVDflairBoundaryLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{dropCILVDflairBoundaryLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\dropCILVDflairBoundaryLTwoVarLossBootstrap}{\tbd{dropCILVDflairBoundaryLTwoVarLossBootstrap}}
\providecommand{\dropCILVDflairBoundaryLTwoVarLossGce}{\tbd{dropCILVDflairBoundaryLTwoVarLossGce}}
\providecommand{\dropCILVDflairBoundaryLTwoVarLrMultOne}{\tbd{dropCILVDflairBoundaryLTwoVarLrMultOne}}
\providecommand{\dropCILVDflairBoundaryLTwoVarLrMultThree}{\tbd{dropCILVDflairBoundaryLTwoVarLrMultThree}}
\providecommand{\dropCILVDflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCILVDflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCILVDflairBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCILVDflairBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCILVDflairCoarseLOne}{\tbd{dropCILVDflairCoarseLOne}}
\providecommand{\dropCILVDflairCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{dropCILVDflairCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCILVDflairCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{dropCILVDflairCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDflairCoarseLOneVarDecoderSamLite}{\tbd{dropCILVDflairCoarseLOneVarDecoderSamLite}}
\providecommand{\dropCILVDflairCoarseLOneVarDecoderSamPretrained}{\tbd{dropCILVDflairCoarseLOneVarDecoderSamPretrained}}
\providecommand{\dropCILVDflairCoarseLOneVarDecoderSegformerMlp}{\tbd{dropCILVDflairCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\dropCILVDflairCoarseLR}{\tbd{dropCILVDflairCoarseLR}}
\providecommand{\dropCILVDflairCoarseLRVarLrMultOne}{\tbd{dropCILVDflairCoarseLRVarLrMultOne}}
\providecommand{\dropCILVDflairCoarseLTwo}{\tbd{dropCILVDflairCoarseLTwo}}
\providecommand{\dropCILVDflairCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCILVDflairCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCILVDflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{dropCILVDflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\dropCILVDflairCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCILVDflairCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{dropCILVDflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\dropCILVDflairCoarseLTwoVarDecoderSamLite}{\tbd{dropCILVDflairCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropCILVDflairCoarseLTwoVarDecoderSamLiteLrMultOne}{\tbd{dropCILVDflairCoarseLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\dropCILVDflairCoarseLTwoVarDecoderSamPretrained}{\tbd{dropCILVDflairCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\dropCILVDflairCoarseLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{dropCILVDflairCoarseLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\dropCILVDflairCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropCILVDflairCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCILVDflairCoarseLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{dropCILVDflairCoarseLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\dropCILVDflairCoarseLTwoVarLossBootstrap}{\tbd{dropCILVDflairCoarseLTwoVarLossBootstrap}}
\providecommand{\dropCILVDflairCoarseLTwoVarLossGce}{\tbd{dropCILVDflairCoarseLTwoVarLossGce}}
\providecommand{\dropCILVDflairCoarseLTwoVarLrMultOne}{\tbd{dropCILVDflairCoarseLTwoVarLrMultOne}}
\providecommand{\dropCILVDflairCoarseLTwoVarLrMultThree}{\tbd{dropCILVDflairCoarseLTwoVarLrMultThree}}
\providecommand{\dropCILVDflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCILVDflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCILVDflairCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCILVDflairCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCILVDflairOmissionLOne}{\tbd{dropCILVDflairOmissionLOne}}
\providecommand{\dropCILVDflairOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{dropCILVDflairOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCILVDflairOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{dropCILVDflairOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDflairOmissionLOneVarDecoderSamLite}{\tbd{dropCILVDflairOmissionLOneVarDecoderSamLite}}
\providecommand{\dropCILVDflairOmissionLOneVarDecoderSamPretrained}{\tbd{dropCILVDflairOmissionLOneVarDecoderSamPretrained}}
\providecommand{\dropCILVDflairOmissionLOneVarDecoderSegformerMlp}{\tbd{dropCILVDflairOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\dropCILVDflairOmissionLR}{\tbd{dropCILVDflairOmissionLR}}
\providecommand{\dropCILVDflairOmissionLRVarLrMultOne}{\tbd{dropCILVDflairOmissionLRVarLrMultOne}}
\providecommand{\dropCILVDflairOmissionLTwo}{\tbd{dropCILVDflairOmissionLTwo}}
\providecommand{\dropCILVDflairOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCILVDflairOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCILVDflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{dropCILVDflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\dropCILVDflairOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCILVDflairOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{dropCILVDflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\dropCILVDflairOmissionLTwoVarDecoderSamLite}{\tbd{dropCILVDflairOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropCILVDflairOmissionLTwoVarDecoderSamLiteLrMultOne}{\tbd{dropCILVDflairOmissionLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\dropCILVDflairOmissionLTwoVarDecoderSamPretrained}{\tbd{dropCILVDflairOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\dropCILVDflairOmissionLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{dropCILVDflairOmissionLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\dropCILVDflairOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropCILVDflairOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCILVDflairOmissionLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{dropCILVDflairOmissionLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\dropCILVDflairOmissionLTwoVarLossBootstrap}{\tbd{dropCILVDflairOmissionLTwoVarLossBootstrap}}
\providecommand{\dropCILVDflairOmissionLTwoVarLossGce}{\tbd{dropCILVDflairOmissionLTwoVarLossGce}}
\providecommand{\dropCILVDflairOmissionLTwoVarLrMultOne}{\tbd{dropCILVDflairOmissionLTwoVarLrMultOne}}
\providecommand{\dropCILVDflairOmissionLTwoVarLrMultThree}{\tbd{dropCILVDflairOmissionLTwoVarLrMultThree}}
\providecommand{\dropCILVDflairOmissionLTwoVarLrMultZeroOneOneOneOne}{\tbd{dropCILVDflairOmissionLTwoVarLrMultZeroOneOneOneOne}}
\providecommand{\dropCILVDflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCILVDflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCILVDflairOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCILVDflairOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCILVDflairShiftLOne}{\tbd{dropCILVDflairShiftLOne}}
\providecommand{\dropCILVDflairShiftLOneVarDecoderMaskTwoformerFull}{\tbd{dropCILVDflairShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCILVDflairShiftLOneVarDecoderMaskTwoformerLite}{\tbd{dropCILVDflairShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDflairShiftLOneVarDecoderSamLite}{\tbd{dropCILVDflairShiftLOneVarDecoderSamLite}}
\providecommand{\dropCILVDflairShiftLOneVarDecoderSamPretrained}{\tbd{dropCILVDflairShiftLOneVarDecoderSamPretrained}}
\providecommand{\dropCILVDflairShiftLOneVarDecoderSegformerMlp}{\tbd{dropCILVDflairShiftLOneVarDecoderSegformerMlp}}
\providecommand{\dropCILVDflairShiftLR}{\tbd{dropCILVDflairShiftLR}}
\providecommand{\dropCILVDflairShiftLRVarLrMultOne}{\tbd{dropCILVDflairShiftLRVarLrMultOne}}
\providecommand{\dropCILVDflairShiftLTwo}{\tbd{dropCILVDflairShiftLTwo}}
\providecommand{\dropCILVDflairShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCILVDflairShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCILVDflairShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{dropCILVDflairShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\dropCILVDflairShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCILVDflairShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCILVDflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{dropCILVDflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\dropCILVDflairShiftLTwoVarDecoderSamLite}{\tbd{dropCILVDflairShiftLTwoVarDecoderSamLite}}
\providecommand{\dropCILVDflairShiftLTwoVarDecoderSamLiteLrMultOne}{\tbd{dropCILVDflairShiftLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\dropCILVDflairShiftLTwoVarDecoderSamPretrained}{\tbd{dropCILVDflairShiftLTwoVarDecoderSamPretrained}}
\providecommand{\dropCILVDflairShiftLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{dropCILVDflairShiftLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\dropCILVDflairShiftLTwoVarDecoderSegformerMlp}{\tbd{dropCILVDflairShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCILVDflairShiftLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{dropCILVDflairShiftLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\dropCILVDflairShiftLTwoVarLossBootstrap}{\tbd{dropCILVDflairShiftLTwoVarLossBootstrap}}
\providecommand{\dropCILVDflairShiftLTwoVarLossGce}{\tbd{dropCILVDflairShiftLTwoVarLossGce}}
\providecommand{\dropCILVDflairShiftLTwoVarLrMultOne}{\tbd{dropCILVDflairShiftLTwoVarLrMultOne}}
\providecommand{\dropCILVDflairShiftLTwoVarLrMultThree}{\tbd{dropCILVDflairShiftLTwoVarLrMultThree}}
\providecommand{\dropCILVDflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCILVDflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCILVDflairShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCILVDflairShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCILVDsenOtsuLTwo}{\tbd{dropCILVDsenOtsuLTwo}}
\providecommand{\dropCIPRIburnBoundaryLOne}{\tbd{dropCIPRIburnBoundaryLOne}}
\providecommand{\dropCIPRIburnBoundaryLTwo}{\tbd{dropCIPRIburnBoundaryLTwo}}
\providecommand{\dropCIPRIburnCoarseLOne}{\tbd{dropCIPRIburnCoarseLOne}}
\providecommand{\dropCIPRIburnCoarseLTwo}{\tbd{dropCIPRIburnCoarseLTwo}}
\providecommand{\dropCIPRIburnOmissionLOne}{\tbd{dropCIPRIburnOmissionLOne}}
\providecommand{\dropCIPRIburnOmissionLTwo}{\tbd{dropCIPRIburnOmissionLTwo}}
\providecommand{\dropCIPRIburnShiftLOne}{\tbd{dropCIPRIburnShiftLOne}}
\providecommand{\dropCIPRIburnShiftLTwo}{\tbd{dropCIPRIburnShiftLTwo}}
\providecommand{\dropCIPRIflairBoundaryLOne}{\tbd{dropCIPRIflairBoundaryLOne}}
\providecommand{\dropCIPRIflairBoundaryLTwo}{\tbd{dropCIPRIflairBoundaryLTwo}}
\providecommand{\dropCIPRIflairCoarseLOne}{\tbd{dropCIPRIflairCoarseLOne}}
\providecommand{\dropCIPRIflairCoarseLTwo}{\tbd{dropCIPRIflairCoarseLTwo}}
\providecommand{\dropCIPRIflairOmissionLOne}{\tbd{dropCIPRIflairOmissionLOne}}
\providecommand{\dropCIPRIflairOmissionLTwo}{\tbd{dropCIPRIflairOmissionLTwo}}
\providecommand{\dropCIPRIflairShiftLOne}{\tbd{dropCIPRIflairShiftLOne}}
\providecommand{\dropCIPRIflairShiftLTwo}{\tbd{dropCIPRIflairShiftLTwo}}
\providecommand{\dropCIRNChesBoundaryLOne}{\tbd{dropCIRNChesBoundaryLOne}}
\providecommand{\dropCIRNChesBoundaryLTwo}{\tbd{dropCIRNChesBoundaryLTwo}}
\providecommand{\dropCIRNChesCoarseLOne}{\tbd{dropCIRNChesCoarseLOne}}
\providecommand{\dropCIRNChesCoarseLTwo}{\tbd{dropCIRNChesCoarseLTwo}}
\providecommand{\dropCIRNChesNlcdREAL}{\tbd{dropCIRNChesNlcdREAL}}
\providecommand{\dropCIRNChesOmissionLOne}{\tbd{dropCIRNChesOmissionLOne}}
\providecommand{\dropCIRNChesOmissionLTwo}{\tbd{dropCIRNChesOmissionLTwo}}
\providecommand{\dropCIRNChesShiftLOne}{\tbd{dropCIRNChesShiftLOne}}
\providecommand{\dropCIRNChesShiftLTwo}{\tbd{dropCIRNChesShiftLTwo}}
\providecommand{\dropCIRNCsTwelveBoundaryLOne}{\tbd{dropCIRNCsTwelveBoundaryLOne}}
\providecommand{\dropCIRNCsTwelveBoundaryLTwo}{\tbd{dropCIRNCsTwelveBoundaryLTwo}}
\providecommand{\dropCIRNCsTwelveCoarseLOne}{\tbd{dropCIRNCsTwelveCoarseLOne}}
\providecommand{\dropCIRNCsTwelveCoarseLTwo}{\tbd{dropCIRNCsTwelveCoarseLTwo}}
\providecommand{\dropCIRNCsTwelveOmissionLOne}{\tbd{dropCIRNCsTwelveOmissionLOne}}
\providecommand{\dropCIRNCsTwelveOmissionLTwo}{\tbd{dropCIRNCsTwelveOmissionLTwo}}
\providecommand{\dropCIRNCsTwelveSTwocloudlessREAL}{\tbd{dropCIRNCsTwelveSTwocloudlessREAL}}
\providecommand{\dropCIRNCsTwelveShiftLOne}{\tbd{dropCIRNCsTwelveShiftLOne}}
\providecommand{\dropCIRNCsTwelveShiftLTwo}{\tbd{dropCIRNCsTwelveShiftLTwo}}
\providecommand{\dropCIRNDfcBoundaryLOne}{\tbd{dropCIRNDfcBoundaryLOne}}
\providecommand{\dropCIRNDfcBoundaryLTwo}{\tbd{dropCIRNDfcBoundaryLTwo}}
\providecommand{\dropCIRNDfcCoarseLOne}{\tbd{dropCIRNDfcCoarseLOne}}
\providecommand{\dropCIRNDfcCoarseLTwo}{\tbd{dropCIRNDfcCoarseLTwo}}
\providecommand{\dropCIRNDfcModisREALVarTrainSubsetRealcov}{\tbd{dropCIRNDfcModisREALVarTrainSubsetRealcov}}
\providecommand{\dropCIRNDfcOmissionLOne}{\tbd{dropCIRNDfcOmissionLOne}}
\providecommand{\dropCIRNDfcOmissionLTwo}{\tbd{dropCIRNDfcOmissionLTwo}}
\providecommand{\dropCIRNDfcShiftLOne}{\tbd{dropCIRNDfcShiftLOne}}
\providecommand{\dropCIRNDfcShiftLTwo}{\tbd{dropCIRNDfcShiftLTwo}}
\providecommand{\dropCIRNEnvaBoundaryLOne}{\tbd{dropCIRNEnvaBoundaryLOne}}
\providecommand{\dropCIRNEnvaBoundaryLTwo}{\tbd{dropCIRNEnvaBoundaryLTwo}}
\providecommand{\dropCIRNEnvaCoarseLOne}{\tbd{dropCIRNEnvaCoarseLOne}}
\providecommand{\dropCIRNEnvaCoarseLTwo}{\tbd{dropCIRNEnvaCoarseLTwo}}
\providecommand{\dropCIRNEnvaNlcdREAL}{\tbd{dropCIRNEnvaNlcdREAL}}
\providecommand{\dropCIRNEnvaOmissionLOne}{\tbd{dropCIRNEnvaOmissionLOne}}
\providecommand{\dropCIRNEnvaOmissionLTwo}{\tbd{dropCIRNEnvaOmissionLTwo}}
\providecommand{\dropCIRNEnvaShiftLOne}{\tbd{dropCIRNEnvaShiftLOne}}
\providecommand{\dropCIRNEnvaShiftLTwo}{\tbd{dropCIRNEnvaShiftLTwo}}
\providecommand{\dropCIRNKuroBoundaryLOne}{\tbd{dropCIRNKuroBoundaryLOne}}
\providecommand{\dropCIRNKuroBoundaryLTwo}{\tbd{dropCIRNKuroBoundaryLTwo}}
\providecommand{\dropCIRNKuroCemsREALVarTrainSubsetRealcov}{\tbd{dropCIRNKuroCemsREALVarTrainSubsetRealcov}}
\providecommand{\dropCIRNKuroCoarseLOne}{\tbd{dropCIRNKuroCoarseLOne}}
\providecommand{\dropCIRNKuroCoarseLTwo}{\tbd{dropCIRNKuroCoarseLTwo}}
\providecommand{\dropCIRNKuroOmissionLOne}{\tbd{dropCIRNKuroOmissionLOne}}
\providecommand{\dropCIRNKuroOmissionLTwo}{\tbd{dropCIRNKuroOmissionLTwo}}
\providecommand{\dropCIRNKuroShiftLOne}{\tbd{dropCIRNKuroShiftLOne}}
\providecommand{\dropCIRNKuroShiftLTwo}{\tbd{dropCIRNKuroShiftLTwo}}
\providecommand{\dropCIRNOemBoundaryLOne}{\tbd{dropCIRNOemBoundaryLOne}}
\providecommand{\dropCIRNOemBoundaryLTwo}{\tbd{dropCIRNOemBoundaryLTwo}}
\providecommand{\dropCIRNOemCoarseLOne}{\tbd{dropCIRNOemCoarseLOne}}
\providecommand{\dropCIRNOemCoarseLTwo}{\tbd{dropCIRNOemCoarseLTwo}}
\providecommand{\dropCIRNOemOmissionLOne}{\tbd{dropCIRNOemOmissionLOne}}
\providecommand{\dropCIRNOemOmissionLTwo}{\tbd{dropCIRNOemOmissionLTwo}}
\providecommand{\dropCIRNOemShiftLOne}{\tbd{dropCIRNOemShiftLOne}}
\providecommand{\dropCIRNOemShiftLTwo}{\tbd{dropCIRNOemShiftLTwo}}
\providecommand{\dropCIRNSnTwoBoundaryLOne}{\tbd{dropCIRNSnTwoBoundaryLOne}}
\providecommand{\dropCIRNSnTwoBoundaryLTwo}{\tbd{dropCIRNSnTwoBoundaryLTwo}}
\providecommand{\dropCIRNSnTwoCoarseLOne}{\tbd{dropCIRNSnTwoCoarseLOne}}
\providecommand{\dropCIRNSnTwoCoarseLTwo}{\tbd{dropCIRNSnTwoCoarseLTwo}}
\providecommand{\dropCIRNSnTwoOmissionLOne}{\tbd{dropCIRNSnTwoOmissionLOne}}
\providecommand{\dropCIRNSnTwoOmissionLTwo}{\tbd{dropCIRNSnTwoOmissionLTwo}}
\providecommand{\dropCIRNSnTwoShiftLOne}{\tbd{dropCIRNSnTwoShiftLOne}}
\providecommand{\dropCIRNSnTwoShiftLTwo}{\tbd{dropCIRNSnTwoShiftLTwo}}
\providecommand{\dropCIRNburnBoundaryLOne}{\tbd{dropCIRNburnBoundaryLOne}}
\providecommand{\dropCIRNburnBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{dropCIRNburnBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCIRNburnBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{dropCIRNburnBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCIRNburnBoundaryLOneVarDecoderSamLite}{\tbd{dropCIRNburnBoundaryLOneVarDecoderSamLite}}
\providecommand{\dropCIRNburnBoundaryLOneVarDecoderSamPretrained}{\tbd{dropCIRNburnBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\dropCIRNburnBoundaryLOneVarDecoderSegformerMlp}{\tbd{dropCIRNburnBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\dropCIRNburnBoundaryLR}{\tbd{dropCIRNburnBoundaryLR}}
\providecommand{\dropCIRNburnBoundaryLTwo}{\tbd{dropCIRNburnBoundaryLTwo}}
\providecommand{\dropCIRNburnBoundaryLTwoVarBandsRgb}{\tbd{dropCIRNburnBoundaryLTwoVarBandsRgb}}
\providecommand{\dropCIRNburnBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCIRNburnBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCIRNburnBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCIRNburnBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCIRNburnBoundaryLTwoVarDecoderSamLite}{\tbd{dropCIRNburnBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropCIRNburnBoundaryLTwoVarDecoderSamPretrained}{\tbd{dropCIRNburnBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\dropCIRNburnBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropCIRNburnBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCIRNburnBoundaryLTwoVarInitRandom}{\tbd{dropCIRNburnBoundaryLTwoVarInitRandom}}
\providecommand{\dropCIRNburnBoundaryLTwoVarLossBootstrap}{\tbd{dropCIRNburnBoundaryLTwoVarLossBootstrap}}
\providecommand{\dropCIRNburnBoundaryLTwoVarLossGce}{\tbd{dropCIRNburnBoundaryLTwoVarLossGce}}
\providecommand{\dropCIRNburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCIRNburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCIRNburnBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCIRNburnBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCIRNburnCoarseLOne}{\tbd{dropCIRNburnCoarseLOne}}
\providecommand{\dropCIRNburnCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{dropCIRNburnCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCIRNburnCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{dropCIRNburnCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCIRNburnCoarseLOneVarDecoderSamLite}{\tbd{dropCIRNburnCoarseLOneVarDecoderSamLite}}
\providecommand{\dropCIRNburnCoarseLOneVarDecoderSamPretrained}{\tbd{dropCIRNburnCoarseLOneVarDecoderSamPretrained}}
\providecommand{\dropCIRNburnCoarseLOneVarDecoderSegformerMlp}{\tbd{dropCIRNburnCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\dropCIRNburnCoarseLR}{\tbd{dropCIRNburnCoarseLR}}
\providecommand{\dropCIRNburnCoarseLTwo}{\tbd{dropCIRNburnCoarseLTwo}}
\providecommand{\dropCIRNburnCoarseLTwoVarBandsRgb}{\tbd{dropCIRNburnCoarseLTwoVarBandsRgb}}
\providecommand{\dropCIRNburnCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCIRNburnCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCIRNburnCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCIRNburnCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCIRNburnCoarseLTwoVarDecoderSamLite}{\tbd{dropCIRNburnCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropCIRNburnCoarseLTwoVarDecoderSamPretrained}{\tbd{dropCIRNburnCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\dropCIRNburnCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropCIRNburnCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCIRNburnCoarseLTwoVarInitRandom}{\tbd{dropCIRNburnCoarseLTwoVarInitRandom}}
\providecommand{\dropCIRNburnCoarseLTwoVarLossBootstrap}{\tbd{dropCIRNburnCoarseLTwoVarLossBootstrap}}
\providecommand{\dropCIRNburnCoarseLTwoVarLossGce}{\tbd{dropCIRNburnCoarseLTwoVarLossGce}}
\providecommand{\dropCIRNburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCIRNburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCIRNburnCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCIRNburnCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCIRNburnOmissionLOne}{\tbd{dropCIRNburnOmissionLOne}}
\providecommand{\dropCIRNburnOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{dropCIRNburnOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCIRNburnOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{dropCIRNburnOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCIRNburnOmissionLOneVarDecoderSamLite}{\tbd{dropCIRNburnOmissionLOneVarDecoderSamLite}}
\providecommand{\dropCIRNburnOmissionLOneVarDecoderSamPretrained}{\tbd{dropCIRNburnOmissionLOneVarDecoderSamPretrained}}
\providecommand{\dropCIRNburnOmissionLOneVarDecoderSegformerMlp}{\tbd{dropCIRNburnOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\dropCIRNburnOmissionLR}{\tbd{dropCIRNburnOmissionLR}}
\providecommand{\dropCIRNburnOmissionLTwo}{\tbd{dropCIRNburnOmissionLTwo}}
\providecommand{\dropCIRNburnOmissionLTwoVarBandsRgb}{\tbd{dropCIRNburnOmissionLTwoVarBandsRgb}}
\providecommand{\dropCIRNburnOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCIRNburnOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCIRNburnOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCIRNburnOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCIRNburnOmissionLTwoVarDecoderSamLite}{\tbd{dropCIRNburnOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropCIRNburnOmissionLTwoVarDecoderSamPretrained}{\tbd{dropCIRNburnOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\dropCIRNburnOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropCIRNburnOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCIRNburnOmissionLTwoVarInitRandom}{\tbd{dropCIRNburnOmissionLTwoVarInitRandom}}
\providecommand{\dropCIRNburnOmissionLTwoVarLossBootstrap}{\tbd{dropCIRNburnOmissionLTwoVarLossBootstrap}}
\providecommand{\dropCIRNburnOmissionLTwoVarLossGce}{\tbd{dropCIRNburnOmissionLTwoVarLossGce}}
\providecommand{\dropCIRNburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCIRNburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCIRNburnOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCIRNburnOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCIRNburnShiftLOne}{\tbd{dropCIRNburnShiftLOne}}
\providecommand{\dropCIRNburnShiftLOneVarDecoderMaskTwoformerFull}{\tbd{dropCIRNburnShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCIRNburnShiftLOneVarDecoderMaskTwoformerLite}{\tbd{dropCIRNburnShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCIRNburnShiftLOneVarDecoderSamLite}{\tbd{dropCIRNburnShiftLOneVarDecoderSamLite}}
\providecommand{\dropCIRNburnShiftLOneVarDecoderSamPretrained}{\tbd{dropCIRNburnShiftLOneVarDecoderSamPretrained}}
\providecommand{\dropCIRNburnShiftLOneVarDecoderSegformerMlp}{\tbd{dropCIRNburnShiftLOneVarDecoderSegformerMlp}}
\providecommand{\dropCIRNburnShiftLR}{\tbd{dropCIRNburnShiftLR}}
\providecommand{\dropCIRNburnShiftLTwo}{\tbd{dropCIRNburnShiftLTwo}}
\providecommand{\dropCIRNburnShiftLTwoVarBandsRgb}{\tbd{dropCIRNburnShiftLTwoVarBandsRgb}}
\providecommand{\dropCIRNburnShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCIRNburnShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCIRNburnShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCIRNburnShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCIRNburnShiftLTwoVarDecoderSamLite}{\tbd{dropCIRNburnShiftLTwoVarDecoderSamLite}}
\providecommand{\dropCIRNburnShiftLTwoVarDecoderSamPretrained}{\tbd{dropCIRNburnShiftLTwoVarDecoderSamPretrained}}
\providecommand{\dropCIRNburnShiftLTwoVarDecoderSegformerMlp}{\tbd{dropCIRNburnShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCIRNburnShiftLTwoVarInitRandom}{\tbd{dropCIRNburnShiftLTwoVarInitRandom}}
\providecommand{\dropCIRNburnShiftLTwoVarLossBootstrap}{\tbd{dropCIRNburnShiftLTwoVarLossBootstrap}}
\providecommand{\dropCIRNburnShiftLTwoVarLossGce}{\tbd{dropCIRNburnShiftLTwoVarLossGce}}
\providecommand{\dropCIRNburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCIRNburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCIRNburnShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCIRNburnShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCIRNflairBoundaryLOne}{\tbd{dropCIRNflairBoundaryLOne}}
\providecommand{\dropCIRNflairBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{dropCIRNflairBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCIRNflairBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{dropCIRNflairBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCIRNflairBoundaryLOneVarDecoderSamLite}{\tbd{dropCIRNflairBoundaryLOneVarDecoderSamLite}}
\providecommand{\dropCIRNflairBoundaryLOneVarDecoderSamPretrained}{\tbd{dropCIRNflairBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\dropCIRNflairBoundaryLOneVarDecoderSegformerMlp}{\tbd{dropCIRNflairBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\dropCIRNflairBoundaryLR}{\tbd{dropCIRNflairBoundaryLR}}
\providecommand{\dropCIRNflairBoundaryLTwo}{\tbd{dropCIRNflairBoundaryLTwo}}
\providecommand{\dropCIRNflairBoundaryLTwoVarBandsRgb}{\tbd{dropCIRNflairBoundaryLTwoVarBandsRgb}}
\providecommand{\dropCIRNflairBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCIRNflairBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCIRNflairBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCIRNflairBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCIRNflairBoundaryLTwoVarDecoderSamLite}{\tbd{dropCIRNflairBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropCIRNflairBoundaryLTwoVarDecoderSamPretrained}{\tbd{dropCIRNflairBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\dropCIRNflairBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropCIRNflairBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCIRNflairBoundaryLTwoVarInitRandom}{\tbd{dropCIRNflairBoundaryLTwoVarInitRandom}}
\providecommand{\dropCIRNflairBoundaryLTwoVarLossBootstrap}{\tbd{dropCIRNflairBoundaryLTwoVarLossBootstrap}}
\providecommand{\dropCIRNflairBoundaryLTwoVarLossGce}{\tbd{dropCIRNflairBoundaryLTwoVarLossGce}}
\providecommand{\dropCIRNflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCIRNflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCIRNflairBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCIRNflairBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCIRNflairCoarseLOne}{\tbd{dropCIRNflairCoarseLOne}}
\providecommand{\dropCIRNflairCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{dropCIRNflairCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCIRNflairCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{dropCIRNflairCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCIRNflairCoarseLOneVarDecoderSamLite}{\tbd{dropCIRNflairCoarseLOneVarDecoderSamLite}}
\providecommand{\dropCIRNflairCoarseLOneVarDecoderSamPretrained}{\tbd{dropCIRNflairCoarseLOneVarDecoderSamPretrained}}
\providecommand{\dropCIRNflairCoarseLOneVarDecoderSegformerMlp}{\tbd{dropCIRNflairCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\dropCIRNflairCoarseLR}{\tbd{dropCIRNflairCoarseLR}}
\providecommand{\dropCIRNflairCoarseLTwo}{\tbd{dropCIRNflairCoarseLTwo}}
\providecommand{\dropCIRNflairCoarseLTwoVarBandsRgb}{\tbd{dropCIRNflairCoarseLTwoVarBandsRgb}}
\providecommand{\dropCIRNflairCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCIRNflairCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCIRNflairCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCIRNflairCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCIRNflairCoarseLTwoVarDecoderSamLite}{\tbd{dropCIRNflairCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropCIRNflairCoarseLTwoVarDecoderSamPretrained}{\tbd{dropCIRNflairCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\dropCIRNflairCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropCIRNflairCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCIRNflairCoarseLTwoVarInitRandom}{\tbd{dropCIRNflairCoarseLTwoVarInitRandom}}
\providecommand{\dropCIRNflairCoarseLTwoVarLossBootstrap}{\tbd{dropCIRNflairCoarseLTwoVarLossBootstrap}}
\providecommand{\dropCIRNflairCoarseLTwoVarLossGce}{\tbd{dropCIRNflairCoarseLTwoVarLossGce}}
\providecommand{\dropCIRNflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCIRNflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCIRNflairCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCIRNflairCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCIRNflairOmissionLOne}{\tbd{dropCIRNflairOmissionLOne}}
\providecommand{\dropCIRNflairOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{dropCIRNflairOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCIRNflairOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{dropCIRNflairOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCIRNflairOmissionLOneVarDecoderSamLite}{\tbd{dropCIRNflairOmissionLOneVarDecoderSamLite}}
\providecommand{\dropCIRNflairOmissionLOneVarDecoderSamPretrained}{\tbd{dropCIRNflairOmissionLOneVarDecoderSamPretrained}}
\providecommand{\dropCIRNflairOmissionLOneVarDecoderSegformerMlp}{\tbd{dropCIRNflairOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\dropCIRNflairOmissionLR}{\tbd{dropCIRNflairOmissionLR}}
\providecommand{\dropCIRNflairOmissionLTwo}{\tbd{dropCIRNflairOmissionLTwo}}
\providecommand{\dropCIRNflairOmissionLTwoVarBandsRgb}{\tbd{dropCIRNflairOmissionLTwoVarBandsRgb}}
\providecommand{\dropCIRNflairOmissionLTwoVarClassWeightedTrue}{\tbd{dropCIRNflairOmissionLTwoVarClassWeightedTrue}}
\providecommand{\dropCIRNflairOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCIRNflairOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCIRNflairOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCIRNflairOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCIRNflairOmissionLTwoVarDecoderSamLite}{\tbd{dropCIRNflairOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropCIRNflairOmissionLTwoVarDecoderSamPretrained}{\tbd{dropCIRNflairOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\dropCIRNflairOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropCIRNflairOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCIRNflairOmissionLTwoVarInitRandom}{\tbd{dropCIRNflairOmissionLTwoVarInitRandom}}
\providecommand{\dropCIRNflairOmissionLTwoVarLossBootstrap}{\tbd{dropCIRNflairOmissionLTwoVarLossBootstrap}}
\providecommand{\dropCIRNflairOmissionLTwoVarLossGce}{\tbd{dropCIRNflairOmissionLTwoVarLossGce}}
\providecommand{\dropCIRNflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCIRNflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCIRNflairOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCIRNflairOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCIRNflairShiftLOne}{\tbd{dropCIRNflairShiftLOne}}
\providecommand{\dropCIRNflairShiftLOneVarDecoderMaskTwoformerFull}{\tbd{dropCIRNflairShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCIRNflairShiftLOneVarDecoderMaskTwoformerLite}{\tbd{dropCIRNflairShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCIRNflairShiftLOneVarDecoderSamLite}{\tbd{dropCIRNflairShiftLOneVarDecoderSamLite}}
\providecommand{\dropCIRNflairShiftLOneVarDecoderSamPretrained}{\tbd{dropCIRNflairShiftLOneVarDecoderSamPretrained}}
\providecommand{\dropCIRNflairShiftLOneVarDecoderSegformerMlp}{\tbd{dropCIRNflairShiftLOneVarDecoderSegformerMlp}}
\providecommand{\dropCIRNflairShiftLR}{\tbd{dropCIRNflairShiftLR}}
\providecommand{\dropCIRNflairShiftLTwo}{\tbd{dropCIRNflairShiftLTwo}}
\providecommand{\dropCIRNflairShiftLTwoVarBandsRgb}{\tbd{dropCIRNflairShiftLTwoVarBandsRgb}}
\providecommand{\dropCIRNflairShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCIRNflairShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCIRNflairShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCIRNflairShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCIRNflairShiftLTwoVarDecoderSamLite}{\tbd{dropCIRNflairShiftLTwoVarDecoderSamLite}}
\providecommand{\dropCIRNflairShiftLTwoVarDecoderSamPretrained}{\tbd{dropCIRNflairShiftLTwoVarDecoderSamPretrained}}
\providecommand{\dropCIRNflairShiftLTwoVarDecoderSegformerMlp}{\tbd{dropCIRNflairShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCIRNflairShiftLTwoVarInitRandom}{\tbd{dropCIRNflairShiftLTwoVarInitRandom}}
\providecommand{\dropCIRNflairShiftLTwoVarLossBootstrap}{\tbd{dropCIRNflairShiftLTwoVarLossBootstrap}}
\providecommand{\dropCIRNflairShiftLTwoVarLossGce}{\tbd{dropCIRNflairShiftLTwoVarLossGce}}
\providecommand{\dropCIRNflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCIRNflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCIRNflairShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCIRNflairShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCIRNsenOtsuLTwo}{\tbd{dropCIRNsenOtsuLTwo}}
\providecommand{\dropCIResnetFiveZeroSslFoureoburnBoundaryLOne}{\tbd{dropCIResnetFiveZeroSslFoureoburnBoundaryLOne}}
\providecommand{\dropCIResnetFiveZeroSslFoureoburnBoundaryLTwo}{\tbd{dropCIResnetFiveZeroSslFoureoburnBoundaryLTwo}}
\providecommand{\dropCIResnetFiveZeroSslFoureoburnCoarseLOne}{\tbd{dropCIResnetFiveZeroSslFoureoburnCoarseLOne}}
\providecommand{\dropCIResnetFiveZeroSslFoureoburnCoarseLTwo}{\tbd{dropCIResnetFiveZeroSslFoureoburnCoarseLTwo}}
\providecommand{\dropCIResnetFiveZeroSslFoureoburnOmissionLOne}{\tbd{dropCIResnetFiveZeroSslFoureoburnOmissionLOne}}
\providecommand{\dropCIResnetFiveZeroSslFoureoburnOmissionLTwo}{\tbd{dropCIResnetFiveZeroSslFoureoburnOmissionLTwo}}
\providecommand{\dropCIResnetFiveZeroSslFoureoburnShiftLOne}{\tbd{dropCIResnetFiveZeroSslFoureoburnShiftLOne}}
\providecommand{\dropCIResnetFiveZeroSslFoureoburnShiftLTwo}{\tbd{dropCIResnetFiveZeroSslFoureoburnShiftLTwo}}
\providecommand{\dropCIResnetFiveZeroSslFoureoflairBoundaryLOne}{\tbd{dropCIResnetFiveZeroSslFoureoflairBoundaryLOne}}
\providecommand{\dropCIResnetFiveZeroSslFoureoflairBoundaryLTwo}{\tbd{dropCIResnetFiveZeroSslFoureoflairBoundaryLTwo}}
\providecommand{\dropCIResnetFiveZeroSslFoureoflairCoarseLOne}{\tbd{dropCIResnetFiveZeroSslFoureoflairCoarseLOne}}
\providecommand{\dropCIResnetFiveZeroSslFoureoflairCoarseLTwo}{\tbd{dropCIResnetFiveZeroSslFoureoflairCoarseLTwo}}
\providecommand{\dropCIResnetFiveZeroSslFoureoflairOmissionLOne}{\tbd{dropCIResnetFiveZeroSslFoureoflairOmissionLOne}}
\providecommand{\dropCIResnetFiveZeroSslFoureoflairOmissionLTwo}{\tbd{dropCIResnetFiveZeroSslFoureoflairOmissionLTwo}}
\providecommand{\dropCIResnetFiveZeroSslFoureoflairShiftLOne}{\tbd{dropCIResnetFiveZeroSslFoureoflairShiftLOne}}
\providecommand{\dropCIResnetFiveZeroSslFoureoflairShiftLTwo}{\tbd{dropCIResnetFiveZeroSslFoureoflairShiftLTwo}}
\providecommand{\dropCISATChesBoundaryLOne}{\tbd{dropCISATChesBoundaryLOne}}
\providecommand{\dropCISATChesBoundaryLTwo}{\tbd{dropCISATChesBoundaryLTwo}}
\providecommand{\dropCISATChesBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCISATChesBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATChesBoundaryLTwoVarDecoderSamLite}{\tbd{dropCISATChesBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropCISATChesBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropCISATChesBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCISATChesBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATChesBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATChesCoarseLOne}{\tbd{dropCISATChesCoarseLOne}}
\providecommand{\dropCISATChesCoarseLTwo}{\tbd{dropCISATChesCoarseLTwo}}
\providecommand{\dropCISATChesCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCISATChesCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATChesCoarseLTwoVarDecoderSamLite}{\tbd{dropCISATChesCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropCISATChesCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropCISATChesCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCISATChesCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATChesCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATChesNlcdREAL}{\tbd{dropCISATChesNlcdREAL}}
\providecommand{\dropCISATChesOmissionLOne}{\tbd{dropCISATChesOmissionLOne}}
\providecommand{\dropCISATChesOmissionLTwo}{\tbd{dropCISATChesOmissionLTwo}}
\providecommand{\dropCISATChesOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCISATChesOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATChesOmissionLTwoVarDecoderSamLite}{\tbd{dropCISATChesOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropCISATChesOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropCISATChesOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCISATChesOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATChesOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATChesShiftLOne}{\tbd{dropCISATChesShiftLOne}}
\providecommand{\dropCISATChesShiftLTwo}{\tbd{dropCISATChesShiftLTwo}}
\providecommand{\dropCISATChesShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCISATChesShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATChesShiftLTwoVarDecoderSamLite}{\tbd{dropCISATChesShiftLTwoVarDecoderSamLite}}
\providecommand{\dropCISATChesShiftLTwoVarDecoderSegformerMlp}{\tbd{dropCISATChesShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCISATChesShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATChesShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATCsTwelveBoundaryLOne}{\tbd{dropCISATCsTwelveBoundaryLOne}}
\providecommand{\dropCISATCsTwelveBoundaryLTwo}{\tbd{dropCISATCsTwelveBoundaryLTwo}}
\providecommand{\dropCISATCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCISATCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATCsTwelveBoundaryLTwoVarDecoderSamLite}{\tbd{dropCISATCsTwelveBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropCISATCsTwelveBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropCISATCsTwelveBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCISATCsTwelveBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATCsTwelveBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATCsTwelveCoarseLOne}{\tbd{dropCISATCsTwelveCoarseLOne}}
\providecommand{\dropCISATCsTwelveCoarseLTwo}{\tbd{dropCISATCsTwelveCoarseLTwo}}
\providecommand{\dropCISATCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCISATCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATCsTwelveCoarseLTwoVarDecoderSamLite}{\tbd{dropCISATCsTwelveCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropCISATCsTwelveCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropCISATCsTwelveCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCISATCsTwelveCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATCsTwelveCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATCsTwelveOmissionLOne}{\tbd{dropCISATCsTwelveOmissionLOne}}
\providecommand{\dropCISATCsTwelveOmissionLTwo}{\tbd{dropCISATCsTwelveOmissionLTwo}}
\providecommand{\dropCISATCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCISATCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATCsTwelveOmissionLTwoVarDecoderSamLite}{\tbd{dropCISATCsTwelveOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropCISATCsTwelveOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropCISATCsTwelveOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCISATCsTwelveOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATCsTwelveOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATCsTwelveSTwocloudlessREAL}{\tbd{dropCISATCsTwelveSTwocloudlessREAL}}
\providecommand{\dropCISATCsTwelveShiftLOne}{\tbd{dropCISATCsTwelveShiftLOne}}
\providecommand{\dropCISATCsTwelveShiftLTwo}{\tbd{dropCISATCsTwelveShiftLTwo}}
\providecommand{\dropCISATCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCISATCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATCsTwelveShiftLTwoVarDecoderSamLite}{\tbd{dropCISATCsTwelveShiftLTwoVarDecoderSamLite}}
\providecommand{\dropCISATCsTwelveShiftLTwoVarDecoderSegformerMlp}{\tbd{dropCISATCsTwelveShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCISATCsTwelveShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATCsTwelveShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATDfcBoundaryLOne}{\tbd{dropCISATDfcBoundaryLOne}}
\providecommand{\dropCISATDfcBoundaryLTwo}{\tbd{dropCISATDfcBoundaryLTwo}}
\providecommand{\dropCISATDfcBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCISATDfcBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATDfcBoundaryLTwoVarDecoderSamLite}{\tbd{dropCISATDfcBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropCISATDfcBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropCISATDfcBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCISATDfcBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATDfcBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATDfcCoarseLOne}{\tbd{dropCISATDfcCoarseLOne}}
\providecommand{\dropCISATDfcCoarseLTwo}{\tbd{dropCISATDfcCoarseLTwo}}
\providecommand{\dropCISATDfcCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCISATDfcCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATDfcCoarseLTwoVarDecoderSamLite}{\tbd{dropCISATDfcCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropCISATDfcCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropCISATDfcCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCISATDfcCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATDfcCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATDfcModisREALVarTrainSubsetRealcov}{\tbd{dropCISATDfcModisREALVarTrainSubsetRealcov}}
\providecommand{\dropCISATDfcOmissionLOne}{\tbd{dropCISATDfcOmissionLOne}}
\providecommand{\dropCISATDfcOmissionLTwo}{\tbd{dropCISATDfcOmissionLTwo}}
\providecommand{\dropCISATDfcOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCISATDfcOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATDfcOmissionLTwoVarDecoderSamLite}{\tbd{dropCISATDfcOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropCISATDfcOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropCISATDfcOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCISATDfcOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATDfcOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATDfcShiftLOne}{\tbd{dropCISATDfcShiftLOne}}
\providecommand{\dropCISATDfcShiftLTwo}{\tbd{dropCISATDfcShiftLTwo}}
\providecommand{\dropCISATDfcShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCISATDfcShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATDfcShiftLTwoVarDecoderSamLite}{\tbd{dropCISATDfcShiftLTwoVarDecoderSamLite}}
\providecommand{\dropCISATDfcShiftLTwoVarDecoderSegformerMlp}{\tbd{dropCISATDfcShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCISATDfcShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATDfcShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATEnvaBoundaryLOne}{\tbd{dropCISATEnvaBoundaryLOne}}
\providecommand{\dropCISATEnvaBoundaryLTwo}{\tbd{dropCISATEnvaBoundaryLTwo}}
\providecommand{\dropCISATEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCISATEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATEnvaBoundaryLTwoVarDecoderSamLite}{\tbd{dropCISATEnvaBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropCISATEnvaBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropCISATEnvaBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCISATEnvaBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATEnvaBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATEnvaCoarseLOne}{\tbd{dropCISATEnvaCoarseLOne}}
\providecommand{\dropCISATEnvaCoarseLTwo}{\tbd{dropCISATEnvaCoarseLTwo}}
\providecommand{\dropCISATEnvaCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCISATEnvaCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATEnvaCoarseLTwoVarDecoderSamLite}{\tbd{dropCISATEnvaCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropCISATEnvaCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropCISATEnvaCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCISATEnvaCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATEnvaCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATEnvaNlcdREAL}{\tbd{dropCISATEnvaNlcdREAL}}
\providecommand{\dropCISATEnvaOmissionLOne}{\tbd{dropCISATEnvaOmissionLOne}}
\providecommand{\dropCISATEnvaOmissionLTwo}{\tbd{dropCISATEnvaOmissionLTwo}}
\providecommand{\dropCISATEnvaOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCISATEnvaOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATEnvaOmissionLTwoVarDecoderSamLite}{\tbd{dropCISATEnvaOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropCISATEnvaOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropCISATEnvaOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCISATEnvaOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATEnvaOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATEnvaShiftLOne}{\tbd{dropCISATEnvaShiftLOne}}
\providecommand{\dropCISATEnvaShiftLTwo}{\tbd{dropCISATEnvaShiftLTwo}}
\providecommand{\dropCISATEnvaShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCISATEnvaShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATEnvaShiftLTwoVarDecoderSamLite}{\tbd{dropCISATEnvaShiftLTwoVarDecoderSamLite}}
\providecommand{\dropCISATEnvaShiftLTwoVarDecoderSegformerMlp}{\tbd{dropCISATEnvaShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCISATEnvaShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATEnvaShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATKuroBoundaryLOne}{\tbd{dropCISATKuroBoundaryLOne}}
\providecommand{\dropCISATKuroBoundaryLTwo}{\tbd{dropCISATKuroBoundaryLTwo}}
\providecommand{\dropCISATKuroBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCISATKuroBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATKuroBoundaryLTwoVarDecoderSamLite}{\tbd{dropCISATKuroBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropCISATKuroBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropCISATKuroBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCISATKuroBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATKuroBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATKuroCemsREALVarTrainSubsetRealcov}{\tbd{dropCISATKuroCemsREALVarTrainSubsetRealcov}}
\providecommand{\dropCISATKuroCoarseLOne}{\tbd{dropCISATKuroCoarseLOne}}
\providecommand{\dropCISATKuroCoarseLTwo}{\tbd{dropCISATKuroCoarseLTwo}}
\providecommand{\dropCISATKuroCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCISATKuroCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATKuroCoarseLTwoVarDecoderSamLite}{\tbd{dropCISATKuroCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropCISATKuroCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropCISATKuroCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCISATKuroCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATKuroCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATKuroOmissionLOne}{\tbd{dropCISATKuroOmissionLOne}}
\providecommand{\dropCISATKuroOmissionLTwo}{\tbd{dropCISATKuroOmissionLTwo}}
\providecommand{\dropCISATKuroOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCISATKuroOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATKuroOmissionLTwoVarDecoderSamLite}{\tbd{dropCISATKuroOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropCISATKuroOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropCISATKuroOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCISATKuroOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATKuroOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATKuroShiftLOne}{\tbd{dropCISATKuroShiftLOne}}
\providecommand{\dropCISATKuroShiftLTwo}{\tbd{dropCISATKuroShiftLTwo}}
\providecommand{\dropCISATKuroShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCISATKuroShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATKuroShiftLTwoVarDecoderSamLite}{\tbd{dropCISATKuroShiftLTwoVarDecoderSamLite}}
\providecommand{\dropCISATKuroShiftLTwoVarDecoderSegformerMlp}{\tbd{dropCISATKuroShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCISATKuroShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATKuroShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATOemBoundaryLOne}{\tbd{dropCISATOemBoundaryLOne}}
\providecommand{\dropCISATOemBoundaryLTwo}{\tbd{dropCISATOemBoundaryLTwo}}
\providecommand{\dropCISATOemBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCISATOemBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATOemBoundaryLTwoVarDecoderSamLite}{\tbd{dropCISATOemBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropCISATOemBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropCISATOemBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCISATOemBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATOemBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATOemCoarseLOne}{\tbd{dropCISATOemCoarseLOne}}
\providecommand{\dropCISATOemCoarseLTwo}{\tbd{dropCISATOemCoarseLTwo}}
\providecommand{\dropCISATOemCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCISATOemCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATOemCoarseLTwoVarDecoderSamLite}{\tbd{dropCISATOemCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropCISATOemCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropCISATOemCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCISATOemCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATOemCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATOemOmissionLOne}{\tbd{dropCISATOemOmissionLOne}}
\providecommand{\dropCISATOemOmissionLTwo}{\tbd{dropCISATOemOmissionLTwo}}
\providecommand{\dropCISATOemOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCISATOemOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATOemOmissionLTwoVarDecoderSamLite}{\tbd{dropCISATOemOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropCISATOemOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropCISATOemOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCISATOemOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATOemOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATOemShiftLOne}{\tbd{dropCISATOemShiftLOne}}
\providecommand{\dropCISATOemShiftLTwo}{\tbd{dropCISATOemShiftLTwo}}
\providecommand{\dropCISATOemShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCISATOemShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATOemShiftLTwoVarDecoderSamLite}{\tbd{dropCISATOemShiftLTwoVarDecoderSamLite}}
\providecommand{\dropCISATOemShiftLTwoVarDecoderSegformerMlp}{\tbd{dropCISATOemShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCISATOemShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATOemShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATSnTwoBoundaryLOne}{\tbd{dropCISATSnTwoBoundaryLOne}}
\providecommand{\dropCISATSnTwoBoundaryLTwo}{\tbd{dropCISATSnTwoBoundaryLTwo}}
\providecommand{\dropCISATSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCISATSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATSnTwoBoundaryLTwoVarDecoderSamLite}{\tbd{dropCISATSnTwoBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropCISATSnTwoBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropCISATSnTwoBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCISATSnTwoBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATSnTwoBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATSnTwoCoarseLOne}{\tbd{dropCISATSnTwoCoarseLOne}}
\providecommand{\dropCISATSnTwoCoarseLTwo}{\tbd{dropCISATSnTwoCoarseLTwo}}
\providecommand{\dropCISATSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCISATSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATSnTwoCoarseLTwoVarDecoderSamLite}{\tbd{dropCISATSnTwoCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropCISATSnTwoCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropCISATSnTwoCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCISATSnTwoCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATSnTwoCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATSnTwoOmissionLOne}{\tbd{dropCISATSnTwoOmissionLOne}}
\providecommand{\dropCISATSnTwoOmissionLTwo}{\tbd{dropCISATSnTwoOmissionLTwo}}
\providecommand{\dropCISATSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCISATSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATSnTwoOmissionLTwoVarDecoderSamLite}{\tbd{dropCISATSnTwoOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropCISATSnTwoOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropCISATSnTwoOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCISATSnTwoOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATSnTwoOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATSnTwoShiftLOne}{\tbd{dropCISATSnTwoShiftLOne}}
\providecommand{\dropCISATSnTwoShiftLTwo}{\tbd{dropCISATSnTwoShiftLTwo}}
\providecommand{\dropCISATSnTwoShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCISATSnTwoShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATSnTwoShiftLTwoVarDecoderSamLite}{\tbd{dropCISATSnTwoShiftLTwoVarDecoderSamLite}}
\providecommand{\dropCISATSnTwoShiftLTwoVarDecoderSegformerMlp}{\tbd{dropCISATSnTwoShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCISATSnTwoShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATSnTwoShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATburnBoundaryLOne}{\tbd{dropCISATburnBoundaryLOne}}
\providecommand{\dropCISATburnBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{dropCISATburnBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCISATburnBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{dropCISATburnBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATburnBoundaryLOneVarDecoderSamLite}{\tbd{dropCISATburnBoundaryLOneVarDecoderSamLite}}
\providecommand{\dropCISATburnBoundaryLOneVarDecoderSamPretrained}{\tbd{dropCISATburnBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\dropCISATburnBoundaryLOneVarDecoderSegformerMlp}{\tbd{dropCISATburnBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\dropCISATburnBoundaryLR}{\tbd{dropCISATburnBoundaryLR}}
\providecommand{\dropCISATburnBoundaryLRVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATburnBoundaryLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATburnBoundaryLTwo}{\tbd{dropCISATburnBoundaryLTwo}}
\providecommand{\dropCISATburnBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCISATburnBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCISATburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATburnBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCISATburnBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATburnBoundaryLTwoVarDecoderSamLite}{\tbd{dropCISATburnBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropCISATburnBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATburnBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATburnBoundaryLTwoVarDecoderSamPretrained}{\tbd{dropCISATburnBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\dropCISATburnBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATburnBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATburnBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropCISATburnBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCISATburnBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATburnBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATburnBoundaryLTwoVarFrozenEncoderTrue}{\tbd{dropCISATburnBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\dropCISATburnBoundaryLTwoVarLossBootstrap}{\tbd{dropCISATburnBoundaryLTwoVarLossBootstrap}}
\providecommand{\dropCISATburnBoundaryLTwoVarLossGce}{\tbd{dropCISATburnBoundaryLTwoVarLossGce}}
\providecommand{\dropCISATburnBoundaryLTwoVarLrMultThree}{\tbd{dropCISATburnBoundaryLTwoVarLrMultThree}}
\providecommand{\dropCISATburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATburnBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCISATburnBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCISATburnBoundaryLTwoVarValLabelsClean}{\tbd{dropCISATburnBoundaryLTwoVarValLabelsClean}}
\providecommand{\dropCISATburnCoarseLOne}{\tbd{dropCISATburnCoarseLOne}}
\providecommand{\dropCISATburnCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{dropCISATburnCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCISATburnCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{dropCISATburnCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATburnCoarseLOneVarDecoderSamLite}{\tbd{dropCISATburnCoarseLOneVarDecoderSamLite}}
\providecommand{\dropCISATburnCoarseLOneVarDecoderSamPretrained}{\tbd{dropCISATburnCoarseLOneVarDecoderSamPretrained}}
\providecommand{\dropCISATburnCoarseLOneVarDecoderSegformerMlp}{\tbd{dropCISATburnCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\dropCISATburnCoarseLR}{\tbd{dropCISATburnCoarseLR}}
\providecommand{\dropCISATburnCoarseLRVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATburnCoarseLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATburnCoarseLTwo}{\tbd{dropCISATburnCoarseLTwo}}
\providecommand{\dropCISATburnCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCISATburnCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCISATburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATburnCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCISATburnCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATburnCoarseLTwoVarDecoderSamLite}{\tbd{dropCISATburnCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropCISATburnCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATburnCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATburnCoarseLTwoVarDecoderSamPretrained}{\tbd{dropCISATburnCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\dropCISATburnCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATburnCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATburnCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropCISATburnCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCISATburnCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATburnCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATburnCoarseLTwoVarEarlyStoppingFalse}{\tbd{dropCISATburnCoarseLTwoVarEarlyStoppingFalse}}
\providecommand{\dropCISATburnCoarseLTwoVarEarlyStoppingFalseFrozenEncoderTrue}{\tbd{dropCISATburnCoarseLTwoVarEarlyStoppingFalseFrozenEncoderTrue}}
\providecommand{\dropCISATburnCoarseLTwoVarFrozenEncoderTrue}{\tbd{dropCISATburnCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\dropCISATburnCoarseLTwoVarLossBootstrap}{\tbd{dropCISATburnCoarseLTwoVarLossBootstrap}}
\providecommand{\dropCISATburnCoarseLTwoVarLossGce}{\tbd{dropCISATburnCoarseLTwoVarLossGce}}
\providecommand{\dropCISATburnCoarseLTwoVarLrMultThree}{\tbd{dropCISATburnCoarseLTwoVarLrMultThree}}
\providecommand{\dropCISATburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATburnCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCISATburnCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCISATburnCoarseLTwoVarValLabelsClean}{\tbd{dropCISATburnCoarseLTwoVarValLabelsClean}}
\providecommand{\dropCISATburnOmissionLOne}{\tbd{dropCISATburnOmissionLOne}}
\providecommand{\dropCISATburnOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{dropCISATburnOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCISATburnOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{dropCISATburnOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATburnOmissionLOneVarDecoderSamLite}{\tbd{dropCISATburnOmissionLOneVarDecoderSamLite}}
\providecommand{\dropCISATburnOmissionLOneVarDecoderSamPretrained}{\tbd{dropCISATburnOmissionLOneVarDecoderSamPretrained}}
\providecommand{\dropCISATburnOmissionLOneVarDecoderSegformerMlp}{\tbd{dropCISATburnOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\dropCISATburnOmissionLR}{\tbd{dropCISATburnOmissionLR}}
\providecommand{\dropCISATburnOmissionLRVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATburnOmissionLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATburnOmissionLTwo}{\tbd{dropCISATburnOmissionLTwo}}
\providecommand{\dropCISATburnOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCISATburnOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCISATburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATburnOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCISATburnOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATburnOmissionLTwoVarDecoderSamLite}{\tbd{dropCISATburnOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropCISATburnOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATburnOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATburnOmissionLTwoVarDecoderSamPretrained}{\tbd{dropCISATburnOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\dropCISATburnOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATburnOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATburnOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropCISATburnOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCISATburnOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATburnOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATburnOmissionLTwoVarFrozenEncoderTrue}{\tbd{dropCISATburnOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\dropCISATburnOmissionLTwoVarLossBootstrap}{\tbd{dropCISATburnOmissionLTwoVarLossBootstrap}}
\providecommand{\dropCISATburnOmissionLTwoVarLossGce}{\tbd{dropCISATburnOmissionLTwoVarLossGce}}
\providecommand{\dropCISATburnOmissionLTwoVarLrMultThree}{\tbd{dropCISATburnOmissionLTwoVarLrMultThree}}
\providecommand{\dropCISATburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATburnOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCISATburnOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCISATburnOmissionLTwoVarValLabelsClean}{\tbd{dropCISATburnOmissionLTwoVarValLabelsClean}}
\providecommand{\dropCISATburnShiftLOne}{\tbd{dropCISATburnShiftLOne}}
\providecommand{\dropCISATburnShiftLOneVarDecoderMaskTwoformerFull}{\tbd{dropCISATburnShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCISATburnShiftLOneVarDecoderMaskTwoformerLite}{\tbd{dropCISATburnShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATburnShiftLOneVarDecoderSamLite}{\tbd{dropCISATburnShiftLOneVarDecoderSamLite}}
\providecommand{\dropCISATburnShiftLOneVarDecoderSamPretrained}{\tbd{dropCISATburnShiftLOneVarDecoderSamPretrained}}
\providecommand{\dropCISATburnShiftLOneVarDecoderSegformerMlp}{\tbd{dropCISATburnShiftLOneVarDecoderSegformerMlp}}
\providecommand{\dropCISATburnShiftLR}{\tbd{dropCISATburnShiftLR}}
\providecommand{\dropCISATburnShiftLRVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATburnShiftLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATburnShiftLTwo}{\tbd{dropCISATburnShiftLTwo}}
\providecommand{\dropCISATburnShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCISATburnShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCISATburnShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATburnShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATburnShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCISATburnShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATburnShiftLTwoVarDecoderSamLite}{\tbd{dropCISATburnShiftLTwoVarDecoderSamLite}}
\providecommand{\dropCISATburnShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATburnShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATburnShiftLTwoVarDecoderSamPretrained}{\tbd{dropCISATburnShiftLTwoVarDecoderSamPretrained}}
\providecommand{\dropCISATburnShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATburnShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATburnShiftLTwoVarDecoderSegformerMlp}{\tbd{dropCISATburnShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCISATburnShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATburnShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATburnShiftLTwoVarFrozenEncoderTrue}{\tbd{dropCISATburnShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\dropCISATburnShiftLTwoVarLossBootstrap}{\tbd{dropCISATburnShiftLTwoVarLossBootstrap}}
\providecommand{\dropCISATburnShiftLTwoVarLossGce}{\tbd{dropCISATburnShiftLTwoVarLossGce}}
\providecommand{\dropCISATburnShiftLTwoVarLrMultThree}{\tbd{dropCISATburnShiftLTwoVarLrMultThree}}
\providecommand{\dropCISATburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATburnShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCISATburnShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCISATburnShiftLTwoVarValLabelsClean}{\tbd{dropCISATburnShiftLTwoVarValLabelsClean}}
\providecommand{\dropCISATflairBoundaryLOne}{\tbd{dropCISATflairBoundaryLOne}}
\providecommand{\dropCISATflairBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{dropCISATflairBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCISATflairBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{dropCISATflairBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATflairBoundaryLOneVarDecoderSamLite}{\tbd{dropCISATflairBoundaryLOneVarDecoderSamLite}}
\providecommand{\dropCISATflairBoundaryLOneVarDecoderSamPretrained}{\tbd{dropCISATflairBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\dropCISATflairBoundaryLOneVarDecoderSegformerMlp}{\tbd{dropCISATflairBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\dropCISATflairBoundaryLR}{\tbd{dropCISATflairBoundaryLR}}
\providecommand{\dropCISATflairBoundaryLRVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATflairBoundaryLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATflairBoundaryLTwo}{\tbd{dropCISATflairBoundaryLTwo}}
\providecommand{\dropCISATflairBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCISATflairBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCISATflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATflairBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCISATflairBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATflairBoundaryLTwoVarDecoderSamLite}{\tbd{dropCISATflairBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropCISATflairBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATflairBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATflairBoundaryLTwoVarDecoderSamPretrained}{\tbd{dropCISATflairBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\dropCISATflairBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATflairBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATflairBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropCISATflairBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCISATflairBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATflairBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATflairBoundaryLTwoVarFrozenEncoderTrue}{\tbd{dropCISATflairBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\dropCISATflairBoundaryLTwoVarLossBootstrap}{\tbd{dropCISATflairBoundaryLTwoVarLossBootstrap}}
\providecommand{\dropCISATflairBoundaryLTwoVarLossGce}{\tbd{dropCISATflairBoundaryLTwoVarLossGce}}
\providecommand{\dropCISATflairBoundaryLTwoVarLrMultThree}{\tbd{dropCISATflairBoundaryLTwoVarLrMultThree}}
\providecommand{\dropCISATflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATflairBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCISATflairBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCISATflairBoundaryLTwoVarValLabelsClean}{\tbd{dropCISATflairBoundaryLTwoVarValLabelsClean}}
\providecommand{\dropCISATflairCoarseLOne}{\tbd{dropCISATflairCoarseLOne}}
\providecommand{\dropCISATflairCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{dropCISATflairCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCISATflairCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{dropCISATflairCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATflairCoarseLOneVarDecoderSamLite}{\tbd{dropCISATflairCoarseLOneVarDecoderSamLite}}
\providecommand{\dropCISATflairCoarseLOneVarDecoderSamPretrained}{\tbd{dropCISATflairCoarseLOneVarDecoderSamPretrained}}
\providecommand{\dropCISATflairCoarseLOneVarDecoderSegformerMlp}{\tbd{dropCISATflairCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\dropCISATflairCoarseLR}{\tbd{dropCISATflairCoarseLR}}
\providecommand{\dropCISATflairCoarseLRVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATflairCoarseLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATflairCoarseLTwo}{\tbd{dropCISATflairCoarseLTwo}}
\providecommand{\dropCISATflairCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCISATflairCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCISATflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATflairCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCISATflairCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATflairCoarseLTwoVarDecoderSamLite}{\tbd{dropCISATflairCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropCISATflairCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATflairCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATflairCoarseLTwoVarDecoderSamPretrained}{\tbd{dropCISATflairCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\dropCISATflairCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATflairCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATflairCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropCISATflairCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCISATflairCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATflairCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATflairCoarseLTwoVarFrozenEncoderTrue}{\tbd{dropCISATflairCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\dropCISATflairCoarseLTwoVarLossBootstrap}{\tbd{dropCISATflairCoarseLTwoVarLossBootstrap}}
\providecommand{\dropCISATflairCoarseLTwoVarLossGce}{\tbd{dropCISATflairCoarseLTwoVarLossGce}}
\providecommand{\dropCISATflairCoarseLTwoVarLrMultThree}{\tbd{dropCISATflairCoarseLTwoVarLrMultThree}}
\providecommand{\dropCISATflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATflairCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCISATflairCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCISATflairCoarseLTwoVarValLabelsClean}{\tbd{dropCISATflairCoarseLTwoVarValLabelsClean}}
\providecommand{\dropCISATflairOmissionLOne}{\tbd{dropCISATflairOmissionLOne}}
\providecommand{\dropCISATflairOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{dropCISATflairOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCISATflairOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{dropCISATflairOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATflairOmissionLOneVarDecoderSamLite}{\tbd{dropCISATflairOmissionLOneVarDecoderSamLite}}
\providecommand{\dropCISATflairOmissionLOneVarDecoderSamPretrained}{\tbd{dropCISATflairOmissionLOneVarDecoderSamPretrained}}
\providecommand{\dropCISATflairOmissionLOneVarDecoderSegformerMlp}{\tbd{dropCISATflairOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\dropCISATflairOmissionLR}{\tbd{dropCISATflairOmissionLR}}
\providecommand{\dropCISATflairOmissionLRVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATflairOmissionLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATflairOmissionLTwo}{\tbd{dropCISATflairOmissionLTwo}}
\providecommand{\dropCISATflairOmissionLTwoVarClassWeightedTrue}{\tbd{dropCISATflairOmissionLTwoVarClassWeightedTrue}}
\providecommand{\dropCISATflairOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCISATflairOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCISATflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATflairOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCISATflairOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATflairOmissionLTwoVarDecoderSamLite}{\tbd{dropCISATflairOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropCISATflairOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATflairOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATflairOmissionLTwoVarDecoderSamPretrained}{\tbd{dropCISATflairOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\dropCISATflairOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATflairOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATflairOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropCISATflairOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCISATflairOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATflairOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATflairOmissionLTwoVarEarlyStoppingFalse}{\tbd{dropCISATflairOmissionLTwoVarEarlyStoppingFalse}}
\providecommand{\dropCISATflairOmissionLTwoVarEarlyStoppingFalseFrozenEncoderTrue}{\tbd{dropCISATflairOmissionLTwoVarEarlyStoppingFalseFrozenEncoderTrue}}
\providecommand{\dropCISATflairOmissionLTwoVarFrozenEncoderTrue}{\tbd{dropCISATflairOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\dropCISATflairOmissionLTwoVarLossBootstrap}{\tbd{dropCISATflairOmissionLTwoVarLossBootstrap}}
\providecommand{\dropCISATflairOmissionLTwoVarLossGce}{\tbd{dropCISATflairOmissionLTwoVarLossGce}}
\providecommand{\dropCISATflairOmissionLTwoVarLrMultThree}{\tbd{dropCISATflairOmissionLTwoVarLrMultThree}}
\providecommand{\dropCISATflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATflairOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCISATflairOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCISATflairOmissionLTwoVarValLabelsClean}{\tbd{dropCISATflairOmissionLTwoVarValLabelsClean}}
\providecommand{\dropCISATflairShiftLOne}{\tbd{dropCISATflairShiftLOne}}
\providecommand{\dropCISATflairShiftLOneVarDecoderMaskTwoformerFull}{\tbd{dropCISATflairShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCISATflairShiftLOneVarDecoderMaskTwoformerLite}{\tbd{dropCISATflairShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATflairShiftLOneVarDecoderSamLite}{\tbd{dropCISATflairShiftLOneVarDecoderSamLite}}
\providecommand{\dropCISATflairShiftLOneVarDecoderSamPretrained}{\tbd{dropCISATflairShiftLOneVarDecoderSamPretrained}}
\providecommand{\dropCISATflairShiftLOneVarDecoderSegformerMlp}{\tbd{dropCISATflairShiftLOneVarDecoderSegformerMlp}}
\providecommand{\dropCISATflairShiftLR}{\tbd{dropCISATflairShiftLR}}
\providecommand{\dropCISATflairShiftLRVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATflairShiftLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATflairShiftLTwo}{\tbd{dropCISATflairShiftLTwo}}
\providecommand{\dropCISATflairShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCISATflairShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCISATflairShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATflairShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATflairShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCISATflairShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCISATflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATflairShiftLTwoVarDecoderSamLite}{\tbd{dropCISATflairShiftLTwoVarDecoderSamLite}}
\providecommand{\dropCISATflairShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATflairShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATflairShiftLTwoVarDecoderSamPretrained}{\tbd{dropCISATflairShiftLTwoVarDecoderSamPretrained}}
\providecommand{\dropCISATflairShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATflairShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATflairShiftLTwoVarDecoderSegformerMlp}{\tbd{dropCISATflairShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCISATflairShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATflairShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATflairShiftLTwoVarFrozenEncoderTrue}{\tbd{dropCISATflairShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\dropCISATflairShiftLTwoVarLossBootstrap}{\tbd{dropCISATflairShiftLTwoVarLossBootstrap}}
\providecommand{\dropCISATflairShiftLTwoVarLossGce}{\tbd{dropCISATflairShiftLTwoVarLossGce}}
\providecommand{\dropCISATflairShiftLTwoVarLrMultThree}{\tbd{dropCISATflairShiftLTwoVarLrMultThree}}
\providecommand{\dropCISATflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCISATflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCISATflairShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCISATflairShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCISATflairShiftLTwoVarValLabelsClean}{\tbd{dropCISATflairShiftLTwoVarValLabelsClean}}
\providecommand{\dropCISATsenOtsuLTwo}{\tbd{dropCISATsenOtsuLTwo}}
\providecommand{\dropCITMChesBoundaryLOne}{\tbd{dropCITMChesBoundaryLOne}}
\providecommand{\dropCITMChesBoundaryLTwo}{\tbd{dropCITMChesBoundaryLTwo}}
\providecommand{\dropCITMChesCoarseLOne}{\tbd{dropCITMChesCoarseLOne}}
\providecommand{\dropCITMChesCoarseLTwo}{\tbd{dropCITMChesCoarseLTwo}}
\providecommand{\dropCITMChesNlcdREAL}{\tbd{dropCITMChesNlcdREAL}}
\providecommand{\dropCITMChesOmissionLOne}{\tbd{dropCITMChesOmissionLOne}}
\providecommand{\dropCITMChesOmissionLTwo}{\tbd{dropCITMChesOmissionLTwo}}
\providecommand{\dropCITMChesShiftLOne}{\tbd{dropCITMChesShiftLOne}}
\providecommand{\dropCITMChesShiftLTwo}{\tbd{dropCITMChesShiftLTwo}}
\providecommand{\dropCITMCsTwelveBoundaryLOne}{\tbd{dropCITMCsTwelveBoundaryLOne}}
\providecommand{\dropCITMCsTwelveBoundaryLTwo}{\tbd{dropCITMCsTwelveBoundaryLTwo}}
\providecommand{\dropCITMCsTwelveCoarseLOne}{\tbd{dropCITMCsTwelveCoarseLOne}}
\providecommand{\dropCITMCsTwelveCoarseLTwo}{\tbd{dropCITMCsTwelveCoarseLTwo}}
\providecommand{\dropCITMCsTwelveOmissionLOne}{\tbd{dropCITMCsTwelveOmissionLOne}}
\providecommand{\dropCITMCsTwelveOmissionLTwo}{\tbd{dropCITMCsTwelveOmissionLTwo}}
\providecommand{\dropCITMCsTwelveSTwocloudlessREAL}{\tbd{dropCITMCsTwelveSTwocloudlessREAL}}
\providecommand{\dropCITMCsTwelveShiftLOne}{\tbd{dropCITMCsTwelveShiftLOne}}
\providecommand{\dropCITMCsTwelveShiftLTwo}{\tbd{dropCITMCsTwelveShiftLTwo}}
\providecommand{\dropCITMDfcBoundaryLOne}{\tbd{dropCITMDfcBoundaryLOne}}
\providecommand{\dropCITMDfcBoundaryLTwo}{\tbd{dropCITMDfcBoundaryLTwo}}
\providecommand{\dropCITMDfcCoarseLOne}{\tbd{dropCITMDfcCoarseLOne}}
\providecommand{\dropCITMDfcCoarseLTwo}{\tbd{dropCITMDfcCoarseLTwo}}
\providecommand{\dropCITMDfcModisREALVarTrainSubsetRealcov}{\tbd{dropCITMDfcModisREALVarTrainSubsetRealcov}}
\providecommand{\dropCITMDfcOmissionLOne}{\tbd{dropCITMDfcOmissionLOne}}
\providecommand{\dropCITMDfcOmissionLTwo}{\tbd{dropCITMDfcOmissionLTwo}}
\providecommand{\dropCITMDfcShiftLOne}{\tbd{dropCITMDfcShiftLOne}}
\providecommand{\dropCITMDfcShiftLTwo}{\tbd{dropCITMDfcShiftLTwo}}
\providecommand{\dropCITMEnvaBoundaryLOne}{\tbd{dropCITMEnvaBoundaryLOne}}
\providecommand{\dropCITMEnvaBoundaryLTwo}{\tbd{dropCITMEnvaBoundaryLTwo}}
\providecommand{\dropCITMEnvaCoarseLOne}{\tbd{dropCITMEnvaCoarseLOne}}
\providecommand{\dropCITMEnvaCoarseLTwo}{\tbd{dropCITMEnvaCoarseLTwo}}
\providecommand{\dropCITMEnvaNlcdREAL}{\tbd{dropCITMEnvaNlcdREAL}}
\providecommand{\dropCITMEnvaOmissionLOne}{\tbd{dropCITMEnvaOmissionLOne}}
\providecommand{\dropCITMEnvaOmissionLTwo}{\tbd{dropCITMEnvaOmissionLTwo}}
\providecommand{\dropCITMEnvaShiftLOne}{\tbd{dropCITMEnvaShiftLOne}}
\providecommand{\dropCITMEnvaShiftLTwo}{\tbd{dropCITMEnvaShiftLTwo}}
\providecommand{\dropCITMKuroBoundaryLOne}{\tbd{dropCITMKuroBoundaryLOne}}
\providecommand{\dropCITMKuroBoundaryLTwo}{\tbd{dropCITMKuroBoundaryLTwo}}
\providecommand{\dropCITMKuroCemsREALVarTrainSubsetRealcov}{\tbd{dropCITMKuroCemsREALVarTrainSubsetRealcov}}
\providecommand{\dropCITMKuroCoarseLOne}{\tbd{dropCITMKuroCoarseLOne}}
\providecommand{\dropCITMKuroCoarseLTwo}{\tbd{dropCITMKuroCoarseLTwo}}
\providecommand{\dropCITMKuroOmissionLOne}{\tbd{dropCITMKuroOmissionLOne}}
\providecommand{\dropCITMKuroOmissionLTwo}{\tbd{dropCITMKuroOmissionLTwo}}
\providecommand{\dropCITMKuroShiftLOne}{\tbd{dropCITMKuroShiftLOne}}
\providecommand{\dropCITMKuroShiftLTwo}{\tbd{dropCITMKuroShiftLTwo}}
\providecommand{\dropCITMOemBoundaryLOne}{\tbd{dropCITMOemBoundaryLOne}}
\providecommand{\dropCITMOemBoundaryLTwo}{\tbd{dropCITMOemBoundaryLTwo}}
\providecommand{\dropCITMOemCoarseLOne}{\tbd{dropCITMOemCoarseLOne}}
\providecommand{\dropCITMOemCoarseLTwo}{\tbd{dropCITMOemCoarseLTwo}}
\providecommand{\dropCITMOemOmissionLOne}{\tbd{dropCITMOemOmissionLOne}}
\providecommand{\dropCITMOemOmissionLTwo}{\tbd{dropCITMOemOmissionLTwo}}
\providecommand{\dropCITMOemShiftLOne}{\tbd{dropCITMOemShiftLOne}}
\providecommand{\dropCITMOemShiftLTwo}{\tbd{dropCITMOemShiftLTwo}}
\providecommand{\dropCITMSnTwoBoundaryLOne}{\tbd{dropCITMSnTwoBoundaryLOne}}
\providecommand{\dropCITMSnTwoBoundaryLTwo}{\tbd{dropCITMSnTwoBoundaryLTwo}}
\providecommand{\dropCITMSnTwoCoarseLOne}{\tbd{dropCITMSnTwoCoarseLOne}}
\providecommand{\dropCITMSnTwoCoarseLTwo}{\tbd{dropCITMSnTwoCoarseLTwo}}
\providecommand{\dropCITMSnTwoOmissionLOne}{\tbd{dropCITMSnTwoOmissionLOne}}
\providecommand{\dropCITMSnTwoOmissionLTwo}{\tbd{dropCITMSnTwoOmissionLTwo}}
\providecommand{\dropCITMSnTwoShiftLOne}{\tbd{dropCITMSnTwoShiftLOne}}
\providecommand{\dropCITMSnTwoShiftLTwo}{\tbd{dropCITMSnTwoShiftLTwo}}
\providecommand{\dropCITMburnBoundaryLOne}{\tbd{dropCITMburnBoundaryLOne}}
\providecommand{\dropCITMburnBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{dropCITMburnBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCITMburnBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{dropCITMburnBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCITMburnBoundaryLOneVarDecoderSamLite}{\tbd{dropCITMburnBoundaryLOneVarDecoderSamLite}}
\providecommand{\dropCITMburnBoundaryLOneVarDecoderSamPretrained}{\tbd{dropCITMburnBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\dropCITMburnBoundaryLOneVarDecoderSegformerMlp}{\tbd{dropCITMburnBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\dropCITMburnBoundaryLR}{\tbd{dropCITMburnBoundaryLR}}
\providecommand{\dropCITMburnBoundaryLTwo}{\tbd{dropCITMburnBoundaryLTwo}}
\providecommand{\dropCITMburnBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCITMburnBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCITMburnBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCITMburnBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCITMburnBoundaryLTwoVarDecoderSamLite}{\tbd{dropCITMburnBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropCITMburnBoundaryLTwoVarDecoderSamPretrained}{\tbd{dropCITMburnBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\dropCITMburnBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropCITMburnBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCITMburnBoundaryLTwoVarFrozenEncoderTrue}{\tbd{dropCITMburnBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\dropCITMburnBoundaryLTwoVarLossBootstrap}{\tbd{dropCITMburnBoundaryLTwoVarLossBootstrap}}
\providecommand{\dropCITMburnBoundaryLTwoVarLossGce}{\tbd{dropCITMburnBoundaryLTwoVarLossGce}}
\providecommand{\dropCITMburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCITMburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCITMburnBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCITMburnBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCITMburnCoarseLOne}{\tbd{dropCITMburnCoarseLOne}}
\providecommand{\dropCITMburnCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{dropCITMburnCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCITMburnCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{dropCITMburnCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCITMburnCoarseLOneVarDecoderSamLite}{\tbd{dropCITMburnCoarseLOneVarDecoderSamLite}}
\providecommand{\dropCITMburnCoarseLOneVarDecoderSamPretrained}{\tbd{dropCITMburnCoarseLOneVarDecoderSamPretrained}}
\providecommand{\dropCITMburnCoarseLOneVarDecoderSegformerMlp}{\tbd{dropCITMburnCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\dropCITMburnCoarseLR}{\tbd{dropCITMburnCoarseLR}}
\providecommand{\dropCITMburnCoarseLTwo}{\tbd{dropCITMburnCoarseLTwo}}
\providecommand{\dropCITMburnCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCITMburnCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCITMburnCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCITMburnCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCITMburnCoarseLTwoVarDecoderSamLite}{\tbd{dropCITMburnCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropCITMburnCoarseLTwoVarDecoderSamPretrained}{\tbd{dropCITMburnCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\dropCITMburnCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropCITMburnCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCITMburnCoarseLTwoVarFrozenEncoderTrue}{\tbd{dropCITMburnCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\dropCITMburnCoarseLTwoVarLossBootstrap}{\tbd{dropCITMburnCoarseLTwoVarLossBootstrap}}
\providecommand{\dropCITMburnCoarseLTwoVarLossGce}{\tbd{dropCITMburnCoarseLTwoVarLossGce}}
\providecommand{\dropCITMburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCITMburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCITMburnCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCITMburnCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCITMburnOmissionLOne}{\tbd{dropCITMburnOmissionLOne}}
\providecommand{\dropCITMburnOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{dropCITMburnOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCITMburnOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{dropCITMburnOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCITMburnOmissionLOneVarDecoderSamLite}{\tbd{dropCITMburnOmissionLOneVarDecoderSamLite}}
\providecommand{\dropCITMburnOmissionLOneVarDecoderSamPretrained}{\tbd{dropCITMburnOmissionLOneVarDecoderSamPretrained}}
\providecommand{\dropCITMburnOmissionLOneVarDecoderSegformerMlp}{\tbd{dropCITMburnOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\dropCITMburnOmissionLR}{\tbd{dropCITMburnOmissionLR}}
\providecommand{\dropCITMburnOmissionLTwo}{\tbd{dropCITMburnOmissionLTwo}}
\providecommand{\dropCITMburnOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCITMburnOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCITMburnOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCITMburnOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCITMburnOmissionLTwoVarDecoderSamLite}{\tbd{dropCITMburnOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropCITMburnOmissionLTwoVarDecoderSamPretrained}{\tbd{dropCITMburnOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\dropCITMburnOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropCITMburnOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCITMburnOmissionLTwoVarFrozenEncoderTrue}{\tbd{dropCITMburnOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\dropCITMburnOmissionLTwoVarLossBootstrap}{\tbd{dropCITMburnOmissionLTwoVarLossBootstrap}}
\providecommand{\dropCITMburnOmissionLTwoVarLossGce}{\tbd{dropCITMburnOmissionLTwoVarLossGce}}
\providecommand{\dropCITMburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCITMburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCITMburnOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCITMburnOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCITMburnShiftLOne}{\tbd{dropCITMburnShiftLOne}}
\providecommand{\dropCITMburnShiftLOneVarDecoderMaskTwoformerFull}{\tbd{dropCITMburnShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCITMburnShiftLOneVarDecoderMaskTwoformerLite}{\tbd{dropCITMburnShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCITMburnShiftLOneVarDecoderSamLite}{\tbd{dropCITMburnShiftLOneVarDecoderSamLite}}
\providecommand{\dropCITMburnShiftLOneVarDecoderSamPretrained}{\tbd{dropCITMburnShiftLOneVarDecoderSamPretrained}}
\providecommand{\dropCITMburnShiftLOneVarDecoderSegformerMlp}{\tbd{dropCITMburnShiftLOneVarDecoderSegformerMlp}}
\providecommand{\dropCITMburnShiftLR}{\tbd{dropCITMburnShiftLR}}
\providecommand{\dropCITMburnShiftLTwo}{\tbd{dropCITMburnShiftLTwo}}
\providecommand{\dropCITMburnShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCITMburnShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCITMburnShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCITMburnShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCITMburnShiftLTwoVarDecoderSamLite}{\tbd{dropCITMburnShiftLTwoVarDecoderSamLite}}
\providecommand{\dropCITMburnShiftLTwoVarDecoderSamPretrained}{\tbd{dropCITMburnShiftLTwoVarDecoderSamPretrained}}
\providecommand{\dropCITMburnShiftLTwoVarDecoderSegformerMlp}{\tbd{dropCITMburnShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCITMburnShiftLTwoVarFrozenEncoderTrue}{\tbd{dropCITMburnShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\dropCITMburnShiftLTwoVarLossBootstrap}{\tbd{dropCITMburnShiftLTwoVarLossBootstrap}}
\providecommand{\dropCITMburnShiftLTwoVarLossGce}{\tbd{dropCITMburnShiftLTwoVarLossGce}}
\providecommand{\dropCITMburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCITMburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCITMburnShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCITMburnShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCITMflairBoundaryLOne}{\tbd{dropCITMflairBoundaryLOne}}
\providecommand{\dropCITMflairBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{dropCITMflairBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCITMflairBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{dropCITMflairBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCITMflairBoundaryLOneVarDecoderSamLite}{\tbd{dropCITMflairBoundaryLOneVarDecoderSamLite}}
\providecommand{\dropCITMflairBoundaryLOneVarDecoderSamPretrained}{\tbd{dropCITMflairBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\dropCITMflairBoundaryLOneVarDecoderSegformerMlp}{\tbd{dropCITMflairBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\dropCITMflairBoundaryLR}{\tbd{dropCITMflairBoundaryLR}}
\providecommand{\dropCITMflairBoundaryLTwo}{\tbd{dropCITMflairBoundaryLTwo}}
\providecommand{\dropCITMflairBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCITMflairBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCITMflairBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCITMflairBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCITMflairBoundaryLTwoVarDecoderSamLite}{\tbd{dropCITMflairBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropCITMflairBoundaryLTwoVarDecoderSamPretrained}{\tbd{dropCITMflairBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\dropCITMflairBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropCITMflairBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCITMflairBoundaryLTwoVarFrozenEncoderTrue}{\tbd{dropCITMflairBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\dropCITMflairBoundaryLTwoVarLossBootstrap}{\tbd{dropCITMflairBoundaryLTwoVarLossBootstrap}}
\providecommand{\dropCITMflairBoundaryLTwoVarLossGce}{\tbd{dropCITMflairBoundaryLTwoVarLossGce}}
\providecommand{\dropCITMflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCITMflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCITMflairBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCITMflairBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCITMflairCoarseLOne}{\tbd{dropCITMflairCoarseLOne}}
\providecommand{\dropCITMflairCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{dropCITMflairCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCITMflairCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{dropCITMflairCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCITMflairCoarseLOneVarDecoderSamLite}{\tbd{dropCITMflairCoarseLOneVarDecoderSamLite}}
\providecommand{\dropCITMflairCoarseLOneVarDecoderSamPretrained}{\tbd{dropCITMflairCoarseLOneVarDecoderSamPretrained}}
\providecommand{\dropCITMflairCoarseLOneVarDecoderSegformerMlp}{\tbd{dropCITMflairCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\dropCITMflairCoarseLR}{\tbd{dropCITMflairCoarseLR}}
\providecommand{\dropCITMflairCoarseLTwo}{\tbd{dropCITMflairCoarseLTwo}}
\providecommand{\dropCITMflairCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCITMflairCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCITMflairCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCITMflairCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCITMflairCoarseLTwoVarDecoderSamLite}{\tbd{dropCITMflairCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropCITMflairCoarseLTwoVarDecoderSamPretrained}{\tbd{dropCITMflairCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\dropCITMflairCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropCITMflairCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCITMflairCoarseLTwoVarFrozenEncoderTrue}{\tbd{dropCITMflairCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\dropCITMflairCoarseLTwoVarLossBootstrap}{\tbd{dropCITMflairCoarseLTwoVarLossBootstrap}}
\providecommand{\dropCITMflairCoarseLTwoVarLossGce}{\tbd{dropCITMflairCoarseLTwoVarLossGce}}
\providecommand{\dropCITMflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCITMflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCITMflairCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCITMflairCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCITMflairOmissionLOne}{\tbd{dropCITMflairOmissionLOne}}
\providecommand{\dropCITMflairOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{dropCITMflairOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCITMflairOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{dropCITMflairOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCITMflairOmissionLOneVarDecoderSamLite}{\tbd{dropCITMflairOmissionLOneVarDecoderSamLite}}
\providecommand{\dropCITMflairOmissionLOneVarDecoderSamPretrained}{\tbd{dropCITMflairOmissionLOneVarDecoderSamPretrained}}
\providecommand{\dropCITMflairOmissionLOneVarDecoderSegformerMlp}{\tbd{dropCITMflairOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\dropCITMflairOmissionLR}{\tbd{dropCITMflairOmissionLR}}
\providecommand{\dropCITMflairOmissionLTwo}{\tbd{dropCITMflairOmissionLTwo}}
\providecommand{\dropCITMflairOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCITMflairOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCITMflairOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCITMflairOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCITMflairOmissionLTwoVarDecoderSamLite}{\tbd{dropCITMflairOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropCITMflairOmissionLTwoVarDecoderSamPretrained}{\tbd{dropCITMflairOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\dropCITMflairOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropCITMflairOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCITMflairOmissionLTwoVarFrozenEncoderTrue}{\tbd{dropCITMflairOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\dropCITMflairOmissionLTwoVarLossBootstrap}{\tbd{dropCITMflairOmissionLTwoVarLossBootstrap}}
\providecommand{\dropCITMflairOmissionLTwoVarLossGce}{\tbd{dropCITMflairOmissionLTwoVarLossGce}}
\providecommand{\dropCITMflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCITMflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCITMflairOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCITMflairOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCITMflairShiftLOne}{\tbd{dropCITMflairShiftLOne}}
\providecommand{\dropCITMflairShiftLOneVarDecoderMaskTwoformerFull}{\tbd{dropCITMflairShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropCITMflairShiftLOneVarDecoderMaskTwoformerLite}{\tbd{dropCITMflairShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropCITMflairShiftLOneVarDecoderSamLite}{\tbd{dropCITMflairShiftLOneVarDecoderSamLite}}
\providecommand{\dropCITMflairShiftLOneVarDecoderSamPretrained}{\tbd{dropCITMflairShiftLOneVarDecoderSamPretrained}}
\providecommand{\dropCITMflairShiftLOneVarDecoderSegformerMlp}{\tbd{dropCITMflairShiftLOneVarDecoderSegformerMlp}}
\providecommand{\dropCITMflairShiftLR}{\tbd{dropCITMflairShiftLR}}
\providecommand{\dropCITMflairShiftLTwo}{\tbd{dropCITMflairShiftLTwo}}
\providecommand{\dropCITMflairShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{dropCITMflairShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropCITMflairShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropCITMflairShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropCITMflairShiftLTwoVarDecoderSamLite}{\tbd{dropCITMflairShiftLTwoVarDecoderSamLite}}
\providecommand{\dropCITMflairShiftLTwoVarDecoderSamPretrained}{\tbd{dropCITMflairShiftLTwoVarDecoderSamPretrained}}
\providecommand{\dropCITMflairShiftLTwoVarDecoderSegformerMlp}{\tbd{dropCITMflairShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropCITMflairShiftLTwoVarFrozenEncoderTrue}{\tbd{dropCITMflairShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\dropCITMflairShiftLTwoVarLossBootstrap}{\tbd{dropCITMflairShiftLTwoVarLossBootstrap}}
\providecommand{\dropCITMflairShiftLTwoVarLossGce}{\tbd{dropCITMflairShiftLTwoVarLossGce}}
\providecommand{\dropCITMflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropCITMflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropCITMflairShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropCITMflairShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropCITMsenOtsuLTwo}{\tbd{dropCITMsenOtsuLTwo}}
\providecommand{\dropCIVitlRandomburnBoundaryLOneVarInitRandom}{\tbd{dropCIVitlRandomburnBoundaryLOneVarInitRandom}}
\providecommand{\dropCIVitlRandomburnBoundaryLTwoVarInitRandom}{\tbd{dropCIVitlRandomburnBoundaryLTwoVarInitRandom}}
\providecommand{\dropCIVitlRandomburnCoarseLOneVarInitRandom}{\tbd{dropCIVitlRandomburnCoarseLOneVarInitRandom}}
\providecommand{\dropCIVitlRandomburnCoarseLTwoVarInitRandom}{\tbd{dropCIVitlRandomburnCoarseLTwoVarInitRandom}}
\providecommand{\dropCIVitlRandomburnOmissionLOneVarInitRandom}{\tbd{dropCIVitlRandomburnOmissionLOneVarInitRandom}}
\providecommand{\dropCIVitlRandomburnOmissionLTwoVarInitRandom}{\tbd{dropCIVitlRandomburnOmissionLTwoVarInitRandom}}
\providecommand{\dropCIVitlRandomburnShiftLOneVarInitRandom}{\tbd{dropCIVitlRandomburnShiftLOneVarInitRandom}}
\providecommand{\dropCIVitlRandomburnShiftLTwoVarInitRandom}{\tbd{dropCIVitlRandomburnShiftLTwoVarInitRandom}}
\providecommand{\dropCIVitlRandomflairBoundaryLOneVarInitRandom}{\tbd{dropCIVitlRandomflairBoundaryLOneVarInitRandom}}
\providecommand{\dropCIVitlRandomflairBoundaryLTwoVarInitRandom}{\tbd{dropCIVitlRandomflairBoundaryLTwoVarInitRandom}}
\providecommand{\dropCIVitlRandomflairCoarseLOneVarInitRandom}{\tbd{dropCIVitlRandomflairCoarseLOneVarInitRandom}}
\providecommand{\dropCIVitlRandomflairCoarseLTwoVarInitRandom}{\tbd{dropCIVitlRandomflairCoarseLTwoVarInitRandom}}
\providecommand{\dropCIVitlRandomflairOmissionLOneVarInitRandom}{\tbd{dropCIVitlRandomflairOmissionLOneVarInitRandom}}
\providecommand{\dropCIVitlRandomflairOmissionLTwoVarInitRandom}{\tbd{dropCIVitlRandomflairOmissionLTwoVarInitRandom}}
\providecommand{\dropCIVitlRandomflairShiftLOneVarInitRandom}{\tbd{dropCIVitlRandomflairShiftLOneVarInitRandom}}
\providecommand{\dropCIVitlRandomflairShiftLTwoVarInitRandom}{\tbd{dropCIVitlRandomflairShiftLTwoVarInitRandom}}
\providecommand{\dropDOFAChesBoundaryLOne}{\tbd{dropDOFAChesBoundaryLOne}}
\providecommand{\dropDOFAChesBoundaryLTwo}{\tbd{dropDOFAChesBoundaryLTwo}}
\providecommand{\dropDOFAChesCoarseLOne}{\tbd{dropDOFAChesCoarseLOne}}
\providecommand{\dropDOFAChesCoarseLTwo}{\tbd{dropDOFAChesCoarseLTwo}}
\providecommand{\dropDOFAChesNlcdREAL}{\tbd{dropDOFAChesNlcdREAL}}
\providecommand{\dropDOFAChesOmissionLOne}{\tbd{dropDOFAChesOmissionLOne}}
\providecommand{\dropDOFAChesOmissionLTwo}{\tbd{dropDOFAChesOmissionLTwo}}
\providecommand{\dropDOFAChesShiftLOne}{\tbd{dropDOFAChesShiftLOne}}
\providecommand{\dropDOFAChesShiftLTwo}{\tbd{dropDOFAChesShiftLTwo}}
\providecommand{\dropDOFACsTwelveBoundaryLOne}{\tbd{dropDOFACsTwelveBoundaryLOne}}
\providecommand{\dropDOFACsTwelveBoundaryLTwo}{\tbd{dropDOFACsTwelveBoundaryLTwo}}
\providecommand{\dropDOFACsTwelveCoarseLOne}{\tbd{dropDOFACsTwelveCoarseLOne}}
\providecommand{\dropDOFACsTwelveCoarseLTwo}{\tbd{dropDOFACsTwelveCoarseLTwo}}
\providecommand{\dropDOFACsTwelveOmissionLOne}{\tbd{dropDOFACsTwelveOmissionLOne}}
\providecommand{\dropDOFACsTwelveOmissionLTwo}{\tbd{dropDOFACsTwelveOmissionLTwo}}
\providecommand{\dropDOFACsTwelveSTwocloudlessREAL}{\tbd{dropDOFACsTwelveSTwocloudlessREAL}}
\providecommand{\dropDOFACsTwelveShiftLOne}{\tbd{dropDOFACsTwelveShiftLOne}}
\providecommand{\dropDOFACsTwelveShiftLTwo}{\tbd{dropDOFACsTwelveShiftLTwo}}
\providecommand{\dropDOFADfcBoundaryLOne}{\tbd{dropDOFADfcBoundaryLOne}}
\providecommand{\dropDOFADfcBoundaryLTwo}{\tbd{dropDOFADfcBoundaryLTwo}}
\providecommand{\dropDOFADfcCoarseLOne}{\tbd{dropDOFADfcCoarseLOne}}
\providecommand{\dropDOFADfcCoarseLTwo}{\tbd{dropDOFADfcCoarseLTwo}}
\providecommand{\dropDOFADfcModisREALVarTrainSubsetRealcov}{\tbd{dropDOFADfcModisREALVarTrainSubsetRealcov}}
\providecommand{\dropDOFADfcOmissionLOne}{\tbd{dropDOFADfcOmissionLOne}}
\providecommand{\dropDOFADfcOmissionLTwo}{\tbd{dropDOFADfcOmissionLTwo}}
\providecommand{\dropDOFADfcShiftLOne}{\tbd{dropDOFADfcShiftLOne}}
\providecommand{\dropDOFADfcShiftLTwo}{\tbd{dropDOFADfcShiftLTwo}}
\providecommand{\dropDOFAEnvaBoundaryLOne}{\tbd{dropDOFAEnvaBoundaryLOne}}
\providecommand{\dropDOFAEnvaBoundaryLTwo}{\tbd{dropDOFAEnvaBoundaryLTwo}}
\providecommand{\dropDOFAEnvaCoarseLOne}{\tbd{dropDOFAEnvaCoarseLOne}}
\providecommand{\dropDOFAEnvaCoarseLTwo}{\tbd{dropDOFAEnvaCoarseLTwo}}
\providecommand{\dropDOFAEnvaNlcdREAL}{\tbd{dropDOFAEnvaNlcdREAL}}
\providecommand{\dropDOFAEnvaOmissionLOne}{\tbd{dropDOFAEnvaOmissionLOne}}
\providecommand{\dropDOFAEnvaOmissionLTwo}{\tbd{dropDOFAEnvaOmissionLTwo}}
\providecommand{\dropDOFAEnvaShiftLOne}{\tbd{dropDOFAEnvaShiftLOne}}
\providecommand{\dropDOFAEnvaShiftLTwo}{\tbd{dropDOFAEnvaShiftLTwo}}
\providecommand{\dropDOFAKuroBoundaryLOne}{\tbd{dropDOFAKuroBoundaryLOne}}
\providecommand{\dropDOFAKuroBoundaryLTwo}{\tbd{dropDOFAKuroBoundaryLTwo}}
\providecommand{\dropDOFAKuroCemsREALVarTrainSubsetRealcov}{\tbd{dropDOFAKuroCemsREALVarTrainSubsetRealcov}}
\providecommand{\dropDOFAKuroCoarseLOne}{\tbd{dropDOFAKuroCoarseLOne}}
\providecommand{\dropDOFAKuroCoarseLTwo}{\tbd{dropDOFAKuroCoarseLTwo}}
\providecommand{\dropDOFAKuroOmissionLOne}{\tbd{dropDOFAKuroOmissionLOne}}
\providecommand{\dropDOFAKuroOmissionLTwo}{\tbd{dropDOFAKuroOmissionLTwo}}
\providecommand{\dropDOFAKuroShiftLOne}{\tbd{dropDOFAKuroShiftLOne}}
\providecommand{\dropDOFAKuroShiftLTwo}{\tbd{dropDOFAKuroShiftLTwo}}
\providecommand{\dropDOFAOemBoundaryLOne}{\tbd{dropDOFAOemBoundaryLOne}}
\providecommand{\dropDOFAOemBoundaryLTwo}{\tbd{dropDOFAOemBoundaryLTwo}}
\providecommand{\dropDOFAOemCoarseLOne}{\tbd{dropDOFAOemCoarseLOne}}
\providecommand{\dropDOFAOemCoarseLTwo}{\tbd{dropDOFAOemCoarseLTwo}}
\providecommand{\dropDOFAOemOmissionLOne}{\tbd{dropDOFAOemOmissionLOne}}
\providecommand{\dropDOFAOemOmissionLTwo}{\tbd{dropDOFAOemOmissionLTwo}}
\providecommand{\dropDOFAOemShiftLOne}{\tbd{dropDOFAOemShiftLOne}}
\providecommand{\dropDOFAOemShiftLTwo}{\tbd{dropDOFAOemShiftLTwo}}
\providecommand{\dropDOFASnTwoBoundaryLOne}{\tbd{dropDOFASnTwoBoundaryLOne}}
\providecommand{\dropDOFASnTwoBoundaryLTwo}{\tbd{dropDOFASnTwoBoundaryLTwo}}
\providecommand{\dropDOFASnTwoCoarseLOne}{\tbd{dropDOFASnTwoCoarseLOne}}
\providecommand{\dropDOFASnTwoCoarseLTwo}{\tbd{dropDOFASnTwoCoarseLTwo}}
\providecommand{\dropDOFASnTwoOmissionLOne}{\tbd{dropDOFASnTwoOmissionLOne}}
\providecommand{\dropDOFASnTwoOmissionLTwo}{\tbd{dropDOFASnTwoOmissionLTwo}}
\providecommand{\dropDOFASnTwoShiftLOne}{\tbd{dropDOFASnTwoShiftLOne}}
\providecommand{\dropDOFASnTwoShiftLTwo}{\tbd{dropDOFASnTwoShiftLTwo}}
\providecommand{\dropDOFAburnBoundaryLOne}{\tbd{dropDOFAburnBoundaryLOne}}
\providecommand{\dropDOFAburnBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{dropDOFAburnBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropDOFAburnBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{dropDOFAburnBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropDOFAburnBoundaryLOneVarDecoderSamLite}{\tbd{dropDOFAburnBoundaryLOneVarDecoderSamLite}}
\providecommand{\dropDOFAburnBoundaryLOneVarDecoderSamPretrained}{\tbd{dropDOFAburnBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\dropDOFAburnBoundaryLOneVarDecoderSegformerMlp}{\tbd{dropDOFAburnBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\dropDOFAburnBoundaryLR}{\tbd{dropDOFAburnBoundaryLR}}
\providecommand{\dropDOFAburnBoundaryLTwo}{\tbd{dropDOFAburnBoundaryLTwo}}
\providecommand{\dropDOFAburnBoundaryLTwoVarBandsRgb}{\tbd{dropDOFAburnBoundaryLTwoVarBandsRgb}}
\providecommand{\dropDOFAburnBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{dropDOFAburnBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropDOFAburnBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropDOFAburnBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropDOFAburnBoundaryLTwoVarDecoderSamLite}{\tbd{dropDOFAburnBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropDOFAburnBoundaryLTwoVarDecoderSamPretrained}{\tbd{dropDOFAburnBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\dropDOFAburnBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropDOFAburnBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropDOFAburnBoundaryLTwoVarFrozenEncoderTrue}{\tbd{dropDOFAburnBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\dropDOFAburnBoundaryLTwoVarLossBootstrap}{\tbd{dropDOFAburnBoundaryLTwoVarLossBootstrap}}
\providecommand{\dropDOFAburnBoundaryLTwoVarLossGce}{\tbd{dropDOFAburnBoundaryLTwoVarLossGce}}
\providecommand{\dropDOFAburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropDOFAburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropDOFAburnBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropDOFAburnBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropDOFAburnCoarseLOne}{\tbd{dropDOFAburnCoarseLOne}}
\providecommand{\dropDOFAburnCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{dropDOFAburnCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropDOFAburnCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{dropDOFAburnCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropDOFAburnCoarseLOneVarDecoderSamLite}{\tbd{dropDOFAburnCoarseLOneVarDecoderSamLite}}
\providecommand{\dropDOFAburnCoarseLOneVarDecoderSamPretrained}{\tbd{dropDOFAburnCoarseLOneVarDecoderSamPretrained}}
\providecommand{\dropDOFAburnCoarseLOneVarDecoderSegformerMlp}{\tbd{dropDOFAburnCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\dropDOFAburnCoarseLR}{\tbd{dropDOFAburnCoarseLR}}
\providecommand{\dropDOFAburnCoarseLTwo}{\tbd{dropDOFAburnCoarseLTwo}}
\providecommand{\dropDOFAburnCoarseLTwoVarBandsRgb}{\tbd{dropDOFAburnCoarseLTwoVarBandsRgb}}
\providecommand{\dropDOFAburnCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{dropDOFAburnCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropDOFAburnCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropDOFAburnCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropDOFAburnCoarseLTwoVarDecoderSamLite}{\tbd{dropDOFAburnCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropDOFAburnCoarseLTwoVarDecoderSamPretrained}{\tbd{dropDOFAburnCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\dropDOFAburnCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropDOFAburnCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropDOFAburnCoarseLTwoVarFrozenEncoderTrue}{\tbd{dropDOFAburnCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\dropDOFAburnCoarseLTwoVarLossBootstrap}{\tbd{dropDOFAburnCoarseLTwoVarLossBootstrap}}
\providecommand{\dropDOFAburnCoarseLTwoVarLossGce}{\tbd{dropDOFAburnCoarseLTwoVarLossGce}}
\providecommand{\dropDOFAburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropDOFAburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropDOFAburnCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropDOFAburnCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropDOFAburnOmissionLOne}{\tbd{dropDOFAburnOmissionLOne}}
\providecommand{\dropDOFAburnOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{dropDOFAburnOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropDOFAburnOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{dropDOFAburnOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropDOFAburnOmissionLOneVarDecoderSamLite}{\tbd{dropDOFAburnOmissionLOneVarDecoderSamLite}}
\providecommand{\dropDOFAburnOmissionLOneVarDecoderSamPretrained}{\tbd{dropDOFAburnOmissionLOneVarDecoderSamPretrained}}
\providecommand{\dropDOFAburnOmissionLOneVarDecoderSegformerMlp}{\tbd{dropDOFAburnOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\dropDOFAburnOmissionLR}{\tbd{dropDOFAburnOmissionLR}}
\providecommand{\dropDOFAburnOmissionLTwo}{\tbd{dropDOFAburnOmissionLTwo}}
\providecommand{\dropDOFAburnOmissionLTwoVarBandsRgb}{\tbd{dropDOFAburnOmissionLTwoVarBandsRgb}}
\providecommand{\dropDOFAburnOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{dropDOFAburnOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropDOFAburnOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropDOFAburnOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropDOFAburnOmissionLTwoVarDecoderSamLite}{\tbd{dropDOFAburnOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropDOFAburnOmissionLTwoVarDecoderSamPretrained}{\tbd{dropDOFAburnOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\dropDOFAburnOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropDOFAburnOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropDOFAburnOmissionLTwoVarFrozenEncoderTrue}{\tbd{dropDOFAburnOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\dropDOFAburnOmissionLTwoVarLossBootstrap}{\tbd{dropDOFAburnOmissionLTwoVarLossBootstrap}}
\providecommand{\dropDOFAburnOmissionLTwoVarLossGce}{\tbd{dropDOFAburnOmissionLTwoVarLossGce}}
\providecommand{\dropDOFAburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropDOFAburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropDOFAburnOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropDOFAburnOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropDOFAburnShiftLOne}{\tbd{dropDOFAburnShiftLOne}}
\providecommand{\dropDOFAburnShiftLOneVarDecoderMaskTwoformerFull}{\tbd{dropDOFAburnShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropDOFAburnShiftLOneVarDecoderMaskTwoformerLite}{\tbd{dropDOFAburnShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropDOFAburnShiftLOneVarDecoderSamLite}{\tbd{dropDOFAburnShiftLOneVarDecoderSamLite}}
\providecommand{\dropDOFAburnShiftLOneVarDecoderSamPretrained}{\tbd{dropDOFAburnShiftLOneVarDecoderSamPretrained}}
\providecommand{\dropDOFAburnShiftLOneVarDecoderSegformerMlp}{\tbd{dropDOFAburnShiftLOneVarDecoderSegformerMlp}}
\providecommand{\dropDOFAburnShiftLR}{\tbd{dropDOFAburnShiftLR}}
\providecommand{\dropDOFAburnShiftLTwo}{\tbd{dropDOFAburnShiftLTwo}}
\providecommand{\dropDOFAburnShiftLTwoVarBandsRgb}{\tbd{dropDOFAburnShiftLTwoVarBandsRgb}}
\providecommand{\dropDOFAburnShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{dropDOFAburnShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropDOFAburnShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropDOFAburnShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropDOFAburnShiftLTwoVarDecoderSamLite}{\tbd{dropDOFAburnShiftLTwoVarDecoderSamLite}}
\providecommand{\dropDOFAburnShiftLTwoVarDecoderSamPretrained}{\tbd{dropDOFAburnShiftLTwoVarDecoderSamPretrained}}
\providecommand{\dropDOFAburnShiftLTwoVarDecoderSegformerMlp}{\tbd{dropDOFAburnShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropDOFAburnShiftLTwoVarFrozenEncoderTrue}{\tbd{dropDOFAburnShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\dropDOFAburnShiftLTwoVarLossBootstrap}{\tbd{dropDOFAburnShiftLTwoVarLossBootstrap}}
\providecommand{\dropDOFAburnShiftLTwoVarLossGce}{\tbd{dropDOFAburnShiftLTwoVarLossGce}}
\providecommand{\dropDOFAburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropDOFAburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropDOFAburnShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropDOFAburnShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropDOFAflairBoundaryLOne}{\tbd{dropDOFAflairBoundaryLOne}}
\providecommand{\dropDOFAflairBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{dropDOFAflairBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropDOFAflairBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{dropDOFAflairBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropDOFAflairBoundaryLOneVarDecoderSamLite}{\tbd{dropDOFAflairBoundaryLOneVarDecoderSamLite}}
\providecommand{\dropDOFAflairBoundaryLOneVarDecoderSamPretrained}{\tbd{dropDOFAflairBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\dropDOFAflairBoundaryLOneVarDecoderSegformerMlp}{\tbd{dropDOFAflairBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\dropDOFAflairBoundaryLR}{\tbd{dropDOFAflairBoundaryLR}}
\providecommand{\dropDOFAflairBoundaryLTwo}{\tbd{dropDOFAflairBoundaryLTwo}}
\providecommand{\dropDOFAflairBoundaryLTwoVarBandsRgb}{\tbd{dropDOFAflairBoundaryLTwoVarBandsRgb}}
\providecommand{\dropDOFAflairBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{dropDOFAflairBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropDOFAflairBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropDOFAflairBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropDOFAflairBoundaryLTwoVarDecoderSamLite}{\tbd{dropDOFAflairBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropDOFAflairBoundaryLTwoVarDecoderSamPretrained}{\tbd{dropDOFAflairBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\dropDOFAflairBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropDOFAflairBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropDOFAflairBoundaryLTwoVarFrozenEncoderTrue}{\tbd{dropDOFAflairBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\dropDOFAflairBoundaryLTwoVarLossBootstrap}{\tbd{dropDOFAflairBoundaryLTwoVarLossBootstrap}}
\providecommand{\dropDOFAflairBoundaryLTwoVarLossGce}{\tbd{dropDOFAflairBoundaryLTwoVarLossGce}}
\providecommand{\dropDOFAflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropDOFAflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropDOFAflairBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropDOFAflairBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropDOFAflairCoarseLOne}{\tbd{dropDOFAflairCoarseLOne}}
\providecommand{\dropDOFAflairCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{dropDOFAflairCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropDOFAflairCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{dropDOFAflairCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropDOFAflairCoarseLOneVarDecoderSamLite}{\tbd{dropDOFAflairCoarseLOneVarDecoderSamLite}}
\providecommand{\dropDOFAflairCoarseLOneVarDecoderSamPretrained}{\tbd{dropDOFAflairCoarseLOneVarDecoderSamPretrained}}
\providecommand{\dropDOFAflairCoarseLOneVarDecoderSegformerMlp}{\tbd{dropDOFAflairCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\dropDOFAflairCoarseLR}{\tbd{dropDOFAflairCoarseLR}}
\providecommand{\dropDOFAflairCoarseLTwo}{\tbd{dropDOFAflairCoarseLTwo}}
\providecommand{\dropDOFAflairCoarseLTwoVarBandsRgb}{\tbd{dropDOFAflairCoarseLTwoVarBandsRgb}}
\providecommand{\dropDOFAflairCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{dropDOFAflairCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropDOFAflairCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropDOFAflairCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropDOFAflairCoarseLTwoVarDecoderSamLite}{\tbd{dropDOFAflairCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropDOFAflairCoarseLTwoVarDecoderSamPretrained}{\tbd{dropDOFAflairCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\dropDOFAflairCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropDOFAflairCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropDOFAflairCoarseLTwoVarFrozenEncoderTrue}{\tbd{dropDOFAflairCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\dropDOFAflairCoarseLTwoVarLossBootstrap}{\tbd{dropDOFAflairCoarseLTwoVarLossBootstrap}}
\providecommand{\dropDOFAflairCoarseLTwoVarLossGce}{\tbd{dropDOFAflairCoarseLTwoVarLossGce}}
\providecommand{\dropDOFAflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropDOFAflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropDOFAflairCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropDOFAflairCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropDOFAflairOmissionLOne}{\tbd{dropDOFAflairOmissionLOne}}
\providecommand{\dropDOFAflairOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{dropDOFAflairOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropDOFAflairOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{dropDOFAflairOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropDOFAflairOmissionLOneVarDecoderSamLite}{\tbd{dropDOFAflairOmissionLOneVarDecoderSamLite}}
\providecommand{\dropDOFAflairOmissionLOneVarDecoderSamPretrained}{\tbd{dropDOFAflairOmissionLOneVarDecoderSamPretrained}}
\providecommand{\dropDOFAflairOmissionLOneVarDecoderSegformerMlp}{\tbd{dropDOFAflairOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\dropDOFAflairOmissionLR}{\tbd{dropDOFAflairOmissionLR}}
\providecommand{\dropDOFAflairOmissionLTwo}{\tbd{dropDOFAflairOmissionLTwo}}
\providecommand{\dropDOFAflairOmissionLTwoVarBandsRgb}{\tbd{dropDOFAflairOmissionLTwoVarBandsRgb}}
\providecommand{\dropDOFAflairOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{dropDOFAflairOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropDOFAflairOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropDOFAflairOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropDOFAflairOmissionLTwoVarDecoderSamLite}{\tbd{dropDOFAflairOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropDOFAflairOmissionLTwoVarDecoderSamPretrained}{\tbd{dropDOFAflairOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\dropDOFAflairOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropDOFAflairOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropDOFAflairOmissionLTwoVarFrozenEncoderTrue}{\tbd{dropDOFAflairOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\dropDOFAflairOmissionLTwoVarLossBootstrap}{\tbd{dropDOFAflairOmissionLTwoVarLossBootstrap}}
\providecommand{\dropDOFAflairOmissionLTwoVarLossGce}{\tbd{dropDOFAflairOmissionLTwoVarLossGce}}
\providecommand{\dropDOFAflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropDOFAflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropDOFAflairOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropDOFAflairOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropDOFAflairShiftLOne}{\tbd{dropDOFAflairShiftLOne}}
\providecommand{\dropDOFAflairShiftLOneVarDecoderMaskTwoformerFull}{\tbd{dropDOFAflairShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropDOFAflairShiftLOneVarDecoderMaskTwoformerLite}{\tbd{dropDOFAflairShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropDOFAflairShiftLOneVarDecoderSamLite}{\tbd{dropDOFAflairShiftLOneVarDecoderSamLite}}
\providecommand{\dropDOFAflairShiftLOneVarDecoderSamPretrained}{\tbd{dropDOFAflairShiftLOneVarDecoderSamPretrained}}
\providecommand{\dropDOFAflairShiftLOneVarDecoderSegformerMlp}{\tbd{dropDOFAflairShiftLOneVarDecoderSegformerMlp}}
\providecommand{\dropDOFAflairShiftLR}{\tbd{dropDOFAflairShiftLR}}
\providecommand{\dropDOFAflairShiftLTwo}{\tbd{dropDOFAflairShiftLTwo}}
\providecommand{\dropDOFAflairShiftLTwoVarBandsRgb}{\tbd{dropDOFAflairShiftLTwoVarBandsRgb}}
\providecommand{\dropDOFAflairShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{dropDOFAflairShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropDOFAflairShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropDOFAflairShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropDOFAflairShiftLTwoVarDecoderSamLite}{\tbd{dropDOFAflairShiftLTwoVarDecoderSamLite}}
\providecommand{\dropDOFAflairShiftLTwoVarDecoderSamPretrained}{\tbd{dropDOFAflairShiftLTwoVarDecoderSamPretrained}}
\providecommand{\dropDOFAflairShiftLTwoVarDecoderSegformerMlp}{\tbd{dropDOFAflairShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropDOFAflairShiftLTwoVarFrozenEncoderTrue}{\tbd{dropDOFAflairShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\dropDOFAflairShiftLTwoVarLossBootstrap}{\tbd{dropDOFAflairShiftLTwoVarLossBootstrap}}
\providecommand{\dropDOFAflairShiftLTwoVarLossGce}{\tbd{dropDOFAflairShiftLTwoVarLossGce}}
\providecommand{\dropDOFAflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropDOFAflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropDOFAflairShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropDOFAflairShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropDOFAsenOtsuLTwo}{\tbd{dropDOFAsenOtsuLTwo}}
\providecommand{\dropDinovThreeConvnextLburnBoundaryLOne}{\tbd{dropDinovThreeConvnextLburnBoundaryLOne}}
\providecommand{\dropDinovThreeConvnextLburnBoundaryLTwo}{\tbd{dropDinovThreeConvnextLburnBoundaryLTwo}}
\providecommand{\dropDinovThreeConvnextLburnCoarseLOne}{\tbd{dropDinovThreeConvnextLburnCoarseLOne}}
\providecommand{\dropDinovThreeConvnextLburnCoarseLTwo}{\tbd{dropDinovThreeConvnextLburnCoarseLTwo}}
\providecommand{\dropDinovThreeConvnextLburnOmissionLOne}{\tbd{dropDinovThreeConvnextLburnOmissionLOne}}
\providecommand{\dropDinovThreeConvnextLburnOmissionLTwo}{\tbd{dropDinovThreeConvnextLburnOmissionLTwo}}
\providecommand{\dropDinovThreeConvnextLburnShiftLOne}{\tbd{dropDinovThreeConvnextLburnShiftLOne}}
\providecommand{\dropDinovThreeConvnextLburnShiftLTwo}{\tbd{dropDinovThreeConvnextLburnShiftLTwo}}
\providecommand{\dropDinovThreeConvnextLflairBoundaryLOne}{\tbd{dropDinovThreeConvnextLflairBoundaryLOne}}
\providecommand{\dropDinovThreeConvnextLflairBoundaryLTwo}{\tbd{dropDinovThreeConvnextLflairBoundaryLTwo}}
\providecommand{\dropDinovThreeConvnextLflairCoarseLOne}{\tbd{dropDinovThreeConvnextLflairCoarseLOne}}
\providecommand{\dropDinovThreeConvnextLflairCoarseLTwo}{\tbd{dropDinovThreeConvnextLflairCoarseLTwo}}
\providecommand{\dropDinovThreeConvnextLflairOmissionLOne}{\tbd{dropDinovThreeConvnextLflairOmissionLOne}}
\providecommand{\dropDinovThreeConvnextLflairOmissionLTwo}{\tbd{dropDinovThreeConvnextLflairOmissionLTwo}}
\providecommand{\dropDinovThreeConvnextLflairShiftLOne}{\tbd{dropDinovThreeConvnextLflairShiftLOne}}
\providecommand{\dropDinovThreeConvnextLflairShiftLTwo}{\tbd{dropDinovThreeConvnextLflairShiftLTwo}}
\providecommand{\dropLVDChesBoundaryLOne}{\tbd{dropLVDChesBoundaryLOne}}
\providecommand{\dropLVDChesBoundaryLTwo}{\tbd{dropLVDChesBoundaryLTwo}}
\providecommand{\dropLVDChesBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropLVDChesBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDChesBoundaryLTwoVarDecoderSamLite}{\tbd{dropLVDChesBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropLVDChesBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropLVDChesBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropLVDChesBoundaryLTwoVarLrMultOne}{\tbd{dropLVDChesBoundaryLTwoVarLrMultOne}}
\providecommand{\dropLVDChesCoarseLOne}{\tbd{dropLVDChesCoarseLOne}}
\providecommand{\dropLVDChesCoarseLTwo}{\tbd{dropLVDChesCoarseLTwo}}
\providecommand{\dropLVDChesCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropLVDChesCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDChesCoarseLTwoVarDecoderSamLite}{\tbd{dropLVDChesCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropLVDChesCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropLVDChesCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropLVDChesCoarseLTwoVarLrMultOne}{\tbd{dropLVDChesCoarseLTwoVarLrMultOne}}
\providecommand{\dropLVDChesNlcdREAL}{\tbd{dropLVDChesNlcdREAL}}
\providecommand{\dropLVDChesOmissionLOne}{\tbd{dropLVDChesOmissionLOne}}
\providecommand{\dropLVDChesOmissionLTwo}{\tbd{dropLVDChesOmissionLTwo}}
\providecommand{\dropLVDChesOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropLVDChesOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDChesOmissionLTwoVarDecoderSamLite}{\tbd{dropLVDChesOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropLVDChesOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropLVDChesOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropLVDChesOmissionLTwoVarLrMultOne}{\tbd{dropLVDChesOmissionLTwoVarLrMultOne}}
\providecommand{\dropLVDChesShiftLOne}{\tbd{dropLVDChesShiftLOne}}
\providecommand{\dropLVDChesShiftLTwo}{\tbd{dropLVDChesShiftLTwo}}
\providecommand{\dropLVDChesShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropLVDChesShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDChesShiftLTwoVarDecoderSamLite}{\tbd{dropLVDChesShiftLTwoVarDecoderSamLite}}
\providecommand{\dropLVDChesShiftLTwoVarDecoderSegformerMlp}{\tbd{dropLVDChesShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropLVDChesShiftLTwoVarLrMultOne}{\tbd{dropLVDChesShiftLTwoVarLrMultOne}}
\providecommand{\dropLVDCsTwelveBoundaryLOne}{\tbd{dropLVDCsTwelveBoundaryLOne}}
\providecommand{\dropLVDCsTwelveBoundaryLTwo}{\tbd{dropLVDCsTwelveBoundaryLTwo}}
\providecommand{\dropLVDCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropLVDCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDCsTwelveBoundaryLTwoVarDecoderSamLite}{\tbd{dropLVDCsTwelveBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropLVDCsTwelveBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropLVDCsTwelveBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropLVDCsTwelveBoundaryLTwoVarLrMultOne}{\tbd{dropLVDCsTwelveBoundaryLTwoVarLrMultOne}}
\providecommand{\dropLVDCsTwelveCoarseLOne}{\tbd{dropLVDCsTwelveCoarseLOne}}
\providecommand{\dropLVDCsTwelveCoarseLTwo}{\tbd{dropLVDCsTwelveCoarseLTwo}}
\providecommand{\dropLVDCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropLVDCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDCsTwelveCoarseLTwoVarDecoderSamLite}{\tbd{dropLVDCsTwelveCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropLVDCsTwelveCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropLVDCsTwelveCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropLVDCsTwelveCoarseLTwoVarLrMultOne}{\tbd{dropLVDCsTwelveCoarseLTwoVarLrMultOne}}
\providecommand{\dropLVDCsTwelveOmissionLOne}{\tbd{dropLVDCsTwelveOmissionLOne}}
\providecommand{\dropLVDCsTwelveOmissionLTwo}{\tbd{dropLVDCsTwelveOmissionLTwo}}
\providecommand{\dropLVDCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropLVDCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDCsTwelveOmissionLTwoVarDecoderSamLite}{\tbd{dropLVDCsTwelveOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropLVDCsTwelveOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropLVDCsTwelveOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropLVDCsTwelveOmissionLTwoVarLrMultOne}{\tbd{dropLVDCsTwelveOmissionLTwoVarLrMultOne}}
\providecommand{\dropLVDCsTwelveSTwocloudlessREAL}{\tbd{dropLVDCsTwelveSTwocloudlessREAL}}
\providecommand{\dropLVDCsTwelveShiftLOne}{\tbd{dropLVDCsTwelveShiftLOne}}
\providecommand{\dropLVDCsTwelveShiftLTwo}{\tbd{dropLVDCsTwelveShiftLTwo}}
\providecommand{\dropLVDCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropLVDCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDCsTwelveShiftLTwoVarDecoderSamLite}{\tbd{dropLVDCsTwelveShiftLTwoVarDecoderSamLite}}
\providecommand{\dropLVDCsTwelveShiftLTwoVarDecoderSegformerMlp}{\tbd{dropLVDCsTwelveShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropLVDCsTwelveShiftLTwoVarLrMultOne}{\tbd{dropLVDCsTwelveShiftLTwoVarLrMultOne}}
\providecommand{\dropLVDDfcBoundaryLOne}{\tbd{dropLVDDfcBoundaryLOne}}
\providecommand{\dropLVDDfcBoundaryLTwo}{\tbd{dropLVDDfcBoundaryLTwo}}
\providecommand{\dropLVDDfcBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropLVDDfcBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDDfcBoundaryLTwoVarDecoderSamLite}{\tbd{dropLVDDfcBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropLVDDfcBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropLVDDfcBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropLVDDfcBoundaryLTwoVarLrMultOne}{\tbd{dropLVDDfcBoundaryLTwoVarLrMultOne}}
\providecommand{\dropLVDDfcCoarseLOne}{\tbd{dropLVDDfcCoarseLOne}}
\providecommand{\dropLVDDfcCoarseLTwo}{\tbd{dropLVDDfcCoarseLTwo}}
\providecommand{\dropLVDDfcCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropLVDDfcCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDDfcCoarseLTwoVarDecoderSamLite}{\tbd{dropLVDDfcCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropLVDDfcCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropLVDDfcCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropLVDDfcCoarseLTwoVarLrMultOne}{\tbd{dropLVDDfcCoarseLTwoVarLrMultOne}}
\providecommand{\dropLVDDfcModisREALVarTrainSubsetRealcov}{\tbd{dropLVDDfcModisREALVarTrainSubsetRealcov}}
\providecommand{\dropLVDDfcOmissionLOne}{\tbd{dropLVDDfcOmissionLOne}}
\providecommand{\dropLVDDfcOmissionLTwo}{\tbd{dropLVDDfcOmissionLTwo}}
\providecommand{\dropLVDDfcOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropLVDDfcOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDDfcOmissionLTwoVarDecoderSamLite}{\tbd{dropLVDDfcOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropLVDDfcOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropLVDDfcOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropLVDDfcOmissionLTwoVarLrMultOne}{\tbd{dropLVDDfcOmissionLTwoVarLrMultOne}}
\providecommand{\dropLVDDfcShiftLOne}{\tbd{dropLVDDfcShiftLOne}}
\providecommand{\dropLVDDfcShiftLTwo}{\tbd{dropLVDDfcShiftLTwo}}
\providecommand{\dropLVDDfcShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropLVDDfcShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDDfcShiftLTwoVarDecoderSamLite}{\tbd{dropLVDDfcShiftLTwoVarDecoderSamLite}}
\providecommand{\dropLVDDfcShiftLTwoVarDecoderSegformerMlp}{\tbd{dropLVDDfcShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropLVDDfcShiftLTwoVarLrMultOne}{\tbd{dropLVDDfcShiftLTwoVarLrMultOne}}
\providecommand{\dropLVDEnvaBoundaryLOne}{\tbd{dropLVDEnvaBoundaryLOne}}
\providecommand{\dropLVDEnvaBoundaryLTwo}{\tbd{dropLVDEnvaBoundaryLTwo}}
\providecommand{\dropLVDEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropLVDEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDEnvaBoundaryLTwoVarDecoderSamLite}{\tbd{dropLVDEnvaBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropLVDEnvaBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropLVDEnvaBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropLVDEnvaBoundaryLTwoVarLrMultOne}{\tbd{dropLVDEnvaBoundaryLTwoVarLrMultOne}}
\providecommand{\dropLVDEnvaCoarseLOne}{\tbd{dropLVDEnvaCoarseLOne}}
\providecommand{\dropLVDEnvaCoarseLTwo}{\tbd{dropLVDEnvaCoarseLTwo}}
\providecommand{\dropLVDEnvaCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropLVDEnvaCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDEnvaCoarseLTwoVarDecoderSamLite}{\tbd{dropLVDEnvaCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropLVDEnvaCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropLVDEnvaCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropLVDEnvaCoarseLTwoVarLrMultOne}{\tbd{dropLVDEnvaCoarseLTwoVarLrMultOne}}
\providecommand{\dropLVDEnvaNlcdREAL}{\tbd{dropLVDEnvaNlcdREAL}}
\providecommand{\dropLVDEnvaOmissionLOne}{\tbd{dropLVDEnvaOmissionLOne}}
\providecommand{\dropLVDEnvaOmissionLTwo}{\tbd{dropLVDEnvaOmissionLTwo}}
\providecommand{\dropLVDEnvaOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropLVDEnvaOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDEnvaOmissionLTwoVarDecoderSamLite}{\tbd{dropLVDEnvaOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropLVDEnvaOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropLVDEnvaOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropLVDEnvaOmissionLTwoVarLrMultOne}{\tbd{dropLVDEnvaOmissionLTwoVarLrMultOne}}
\providecommand{\dropLVDEnvaShiftLOne}{\tbd{dropLVDEnvaShiftLOne}}
\providecommand{\dropLVDEnvaShiftLTwo}{\tbd{dropLVDEnvaShiftLTwo}}
\providecommand{\dropLVDEnvaShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropLVDEnvaShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDEnvaShiftLTwoVarDecoderSamLite}{\tbd{dropLVDEnvaShiftLTwoVarDecoderSamLite}}
\providecommand{\dropLVDEnvaShiftLTwoVarDecoderSegformerMlp}{\tbd{dropLVDEnvaShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropLVDEnvaShiftLTwoVarLrMultOne}{\tbd{dropLVDEnvaShiftLTwoVarLrMultOne}}
\providecommand{\dropLVDKuroBoundaryLOne}{\tbd{dropLVDKuroBoundaryLOne}}
\providecommand{\dropLVDKuroBoundaryLTwo}{\tbd{dropLVDKuroBoundaryLTwo}}
\providecommand{\dropLVDKuroBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropLVDKuroBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDKuroBoundaryLTwoVarDecoderSamLite}{\tbd{dropLVDKuroBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropLVDKuroBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropLVDKuroBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropLVDKuroBoundaryLTwoVarLrMultOne}{\tbd{dropLVDKuroBoundaryLTwoVarLrMultOne}}
\providecommand{\dropLVDKuroCemsREALVarTrainSubsetRealcov}{\tbd{dropLVDKuroCemsREALVarTrainSubsetRealcov}}
\providecommand{\dropLVDKuroCoarseLOne}{\tbd{dropLVDKuroCoarseLOne}}
\providecommand{\dropLVDKuroCoarseLTwo}{\tbd{dropLVDKuroCoarseLTwo}}
\providecommand{\dropLVDKuroCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropLVDKuroCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDKuroCoarseLTwoVarDecoderSamLite}{\tbd{dropLVDKuroCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropLVDKuroCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropLVDKuroCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropLVDKuroCoarseLTwoVarLrMultOne}{\tbd{dropLVDKuroCoarseLTwoVarLrMultOne}}
\providecommand{\dropLVDKuroOmissionLOne}{\tbd{dropLVDKuroOmissionLOne}}
\providecommand{\dropLVDKuroOmissionLTwo}{\tbd{dropLVDKuroOmissionLTwo}}
\providecommand{\dropLVDKuroOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropLVDKuroOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDKuroOmissionLTwoVarDecoderSamLite}{\tbd{dropLVDKuroOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropLVDKuroOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropLVDKuroOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropLVDKuroOmissionLTwoVarLrMultOne}{\tbd{dropLVDKuroOmissionLTwoVarLrMultOne}}
\providecommand{\dropLVDKuroShiftLOne}{\tbd{dropLVDKuroShiftLOne}}
\providecommand{\dropLVDKuroShiftLTwo}{\tbd{dropLVDKuroShiftLTwo}}
\providecommand{\dropLVDKuroShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropLVDKuroShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDKuroShiftLTwoVarDecoderSamLite}{\tbd{dropLVDKuroShiftLTwoVarDecoderSamLite}}
\providecommand{\dropLVDKuroShiftLTwoVarDecoderSegformerMlp}{\tbd{dropLVDKuroShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropLVDKuroShiftLTwoVarLrMultOne}{\tbd{dropLVDKuroShiftLTwoVarLrMultOne}}
\providecommand{\dropLVDOemBoundaryLOne}{\tbd{dropLVDOemBoundaryLOne}}
\providecommand{\dropLVDOemBoundaryLTwo}{\tbd{dropLVDOemBoundaryLTwo}}
\providecommand{\dropLVDOemBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropLVDOemBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDOemBoundaryLTwoVarDecoderSamLite}{\tbd{dropLVDOemBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropLVDOemBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropLVDOemBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropLVDOemBoundaryLTwoVarLrMultOne}{\tbd{dropLVDOemBoundaryLTwoVarLrMultOne}}
\providecommand{\dropLVDOemCoarseLOne}{\tbd{dropLVDOemCoarseLOne}}
\providecommand{\dropLVDOemCoarseLTwo}{\tbd{dropLVDOemCoarseLTwo}}
\providecommand{\dropLVDOemCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropLVDOemCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDOemCoarseLTwoVarDecoderSamLite}{\tbd{dropLVDOemCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropLVDOemCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropLVDOemCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropLVDOemCoarseLTwoVarLrMultOne}{\tbd{dropLVDOemCoarseLTwoVarLrMultOne}}
\providecommand{\dropLVDOemOmissionLOne}{\tbd{dropLVDOemOmissionLOne}}
\providecommand{\dropLVDOemOmissionLTwo}{\tbd{dropLVDOemOmissionLTwo}}
\providecommand{\dropLVDOemOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropLVDOemOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDOemOmissionLTwoVarDecoderSamLite}{\tbd{dropLVDOemOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropLVDOemOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropLVDOemOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropLVDOemOmissionLTwoVarLrMultOne}{\tbd{dropLVDOemOmissionLTwoVarLrMultOne}}
\providecommand{\dropLVDOemShiftLOne}{\tbd{dropLVDOemShiftLOne}}
\providecommand{\dropLVDOemShiftLTwo}{\tbd{dropLVDOemShiftLTwo}}
\providecommand{\dropLVDOemShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropLVDOemShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDOemShiftLTwoVarDecoderSamLite}{\tbd{dropLVDOemShiftLTwoVarDecoderSamLite}}
\providecommand{\dropLVDOemShiftLTwoVarDecoderSegformerMlp}{\tbd{dropLVDOemShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropLVDOemShiftLTwoVarLrMultOne}{\tbd{dropLVDOemShiftLTwoVarLrMultOne}}
\providecommand{\dropLVDSnTwoBoundaryLOne}{\tbd{dropLVDSnTwoBoundaryLOne}}
\providecommand{\dropLVDSnTwoBoundaryLTwo}{\tbd{dropLVDSnTwoBoundaryLTwo}}
\providecommand{\dropLVDSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropLVDSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDSnTwoBoundaryLTwoVarDecoderSamLite}{\tbd{dropLVDSnTwoBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropLVDSnTwoBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropLVDSnTwoBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropLVDSnTwoBoundaryLTwoVarLrMultOne}{\tbd{dropLVDSnTwoBoundaryLTwoVarLrMultOne}}
\providecommand{\dropLVDSnTwoCoarseLOne}{\tbd{dropLVDSnTwoCoarseLOne}}
\providecommand{\dropLVDSnTwoCoarseLTwo}{\tbd{dropLVDSnTwoCoarseLTwo}}
\providecommand{\dropLVDSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropLVDSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDSnTwoCoarseLTwoVarDecoderSamLite}{\tbd{dropLVDSnTwoCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropLVDSnTwoCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropLVDSnTwoCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropLVDSnTwoCoarseLTwoVarLrMultOne}{\tbd{dropLVDSnTwoCoarseLTwoVarLrMultOne}}
\providecommand{\dropLVDSnTwoOmissionLOne}{\tbd{dropLVDSnTwoOmissionLOne}}
\providecommand{\dropLVDSnTwoOmissionLTwo}{\tbd{dropLVDSnTwoOmissionLTwo}}
\providecommand{\dropLVDSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropLVDSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDSnTwoOmissionLTwoVarDecoderSamLite}{\tbd{dropLVDSnTwoOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropLVDSnTwoOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropLVDSnTwoOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropLVDSnTwoOmissionLTwoVarLrMultOne}{\tbd{dropLVDSnTwoOmissionLTwoVarLrMultOne}}
\providecommand{\dropLVDSnTwoShiftLOne}{\tbd{dropLVDSnTwoShiftLOne}}
\providecommand{\dropLVDSnTwoShiftLTwo}{\tbd{dropLVDSnTwoShiftLTwo}}
\providecommand{\dropLVDSnTwoShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropLVDSnTwoShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDSnTwoShiftLTwoVarDecoderSamLite}{\tbd{dropLVDSnTwoShiftLTwoVarDecoderSamLite}}
\providecommand{\dropLVDSnTwoShiftLTwoVarDecoderSegformerMlp}{\tbd{dropLVDSnTwoShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropLVDSnTwoShiftLTwoVarLrMultOne}{\tbd{dropLVDSnTwoShiftLTwoVarLrMultOne}}
\providecommand{\dropLVDburnBoundaryLOne}{\tbd{dropLVDburnBoundaryLOne}}
\providecommand{\dropLVDburnBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{dropLVDburnBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropLVDburnBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{dropLVDburnBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDburnBoundaryLOneVarDecoderSamLite}{\tbd{dropLVDburnBoundaryLOneVarDecoderSamLite}}
\providecommand{\dropLVDburnBoundaryLOneVarDecoderSamPretrained}{\tbd{dropLVDburnBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\dropLVDburnBoundaryLOneVarDecoderSegformerMlp}{\tbd{dropLVDburnBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\dropLVDburnBoundaryLR}{\tbd{dropLVDburnBoundaryLR}}
\providecommand{\dropLVDburnBoundaryLRVarLrMultOne}{\tbd{dropLVDburnBoundaryLRVarLrMultOne}}
\providecommand{\dropLVDburnBoundaryLTwo}{\tbd{dropLVDburnBoundaryLTwo}}
\providecommand{\dropLVDburnBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{dropLVDburnBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropLVDburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{dropLVDburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\dropLVDburnBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropLVDburnBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{dropLVDburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\dropLVDburnBoundaryLTwoVarDecoderSamLite}{\tbd{dropLVDburnBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropLVDburnBoundaryLTwoVarDecoderSamLiteLrMultOne}{\tbd{dropLVDburnBoundaryLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\dropLVDburnBoundaryLTwoVarDecoderSamPretrained}{\tbd{dropLVDburnBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\dropLVDburnBoundaryLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{dropLVDburnBoundaryLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\dropLVDburnBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropLVDburnBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropLVDburnBoundaryLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{dropLVDburnBoundaryLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\dropLVDburnBoundaryLTwoVarLossBootstrap}{\tbd{dropLVDburnBoundaryLTwoVarLossBootstrap}}
\providecommand{\dropLVDburnBoundaryLTwoVarLossGce}{\tbd{dropLVDburnBoundaryLTwoVarLossGce}}
\providecommand{\dropLVDburnBoundaryLTwoVarLrMultOne}{\tbd{dropLVDburnBoundaryLTwoVarLrMultOne}}
\providecommand{\dropLVDburnBoundaryLTwoVarLrMultThree}{\tbd{dropLVDburnBoundaryLTwoVarLrMultThree}}
\providecommand{\dropLVDburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropLVDburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropLVDburnBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropLVDburnBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropLVDburnCoarseLOne}{\tbd{dropLVDburnCoarseLOne}}
\providecommand{\dropLVDburnCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{dropLVDburnCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropLVDburnCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{dropLVDburnCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDburnCoarseLOneVarDecoderSamLite}{\tbd{dropLVDburnCoarseLOneVarDecoderSamLite}}
\providecommand{\dropLVDburnCoarseLOneVarDecoderSamPretrained}{\tbd{dropLVDburnCoarseLOneVarDecoderSamPretrained}}
\providecommand{\dropLVDburnCoarseLOneVarDecoderSegformerMlp}{\tbd{dropLVDburnCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\dropLVDburnCoarseLR}{\tbd{dropLVDburnCoarseLR}}
\providecommand{\dropLVDburnCoarseLRVarLrMultOne}{\tbd{dropLVDburnCoarseLRVarLrMultOne}}
\providecommand{\dropLVDburnCoarseLTwo}{\tbd{dropLVDburnCoarseLTwo}}
\providecommand{\dropLVDburnCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{dropLVDburnCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropLVDburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{dropLVDburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\dropLVDburnCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropLVDburnCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{dropLVDburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\dropLVDburnCoarseLTwoVarDecoderSamLite}{\tbd{dropLVDburnCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropLVDburnCoarseLTwoVarDecoderSamLiteLrMultOne}{\tbd{dropLVDburnCoarseLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\dropLVDburnCoarseLTwoVarDecoderSamPretrained}{\tbd{dropLVDburnCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\dropLVDburnCoarseLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{dropLVDburnCoarseLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\dropLVDburnCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropLVDburnCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropLVDburnCoarseLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{dropLVDburnCoarseLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\dropLVDburnCoarseLTwoVarLossBootstrap}{\tbd{dropLVDburnCoarseLTwoVarLossBootstrap}}
\providecommand{\dropLVDburnCoarseLTwoVarLossGce}{\tbd{dropLVDburnCoarseLTwoVarLossGce}}
\providecommand{\dropLVDburnCoarseLTwoVarLrMultOne}{\tbd{dropLVDburnCoarseLTwoVarLrMultOne}}
\providecommand{\dropLVDburnCoarseLTwoVarLrMultThree}{\tbd{dropLVDburnCoarseLTwoVarLrMultThree}}
\providecommand{\dropLVDburnCoarseLTwoVarLrMultZeroOneOneOneOne}{\tbd{dropLVDburnCoarseLTwoVarLrMultZeroOneOneOneOne}}
\providecommand{\dropLVDburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropLVDburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropLVDburnCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropLVDburnCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropLVDburnOmissionLOne}{\tbd{dropLVDburnOmissionLOne}}
\providecommand{\dropLVDburnOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{dropLVDburnOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropLVDburnOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{dropLVDburnOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDburnOmissionLOneVarDecoderSamLite}{\tbd{dropLVDburnOmissionLOneVarDecoderSamLite}}
\providecommand{\dropLVDburnOmissionLOneVarDecoderSamPretrained}{\tbd{dropLVDburnOmissionLOneVarDecoderSamPretrained}}
\providecommand{\dropLVDburnOmissionLOneVarDecoderSegformerMlp}{\tbd{dropLVDburnOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\dropLVDburnOmissionLR}{\tbd{dropLVDburnOmissionLR}}
\providecommand{\dropLVDburnOmissionLRVarLrMultOne}{\tbd{dropLVDburnOmissionLRVarLrMultOne}}
\providecommand{\dropLVDburnOmissionLTwo}{\tbd{dropLVDburnOmissionLTwo}}
\providecommand{\dropLVDburnOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{dropLVDburnOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropLVDburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{dropLVDburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\dropLVDburnOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropLVDburnOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{dropLVDburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\dropLVDburnOmissionLTwoVarDecoderSamLite}{\tbd{dropLVDburnOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropLVDburnOmissionLTwoVarDecoderSamLiteLrMultOne}{\tbd{dropLVDburnOmissionLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\dropLVDburnOmissionLTwoVarDecoderSamPretrained}{\tbd{dropLVDburnOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\dropLVDburnOmissionLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{dropLVDburnOmissionLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\dropLVDburnOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropLVDburnOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropLVDburnOmissionLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{dropLVDburnOmissionLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\dropLVDburnOmissionLTwoVarLossBootstrap}{\tbd{dropLVDburnOmissionLTwoVarLossBootstrap}}
\providecommand{\dropLVDburnOmissionLTwoVarLossGce}{\tbd{dropLVDburnOmissionLTwoVarLossGce}}
\providecommand{\dropLVDburnOmissionLTwoVarLrMultOne}{\tbd{dropLVDburnOmissionLTwoVarLrMultOne}}
\providecommand{\dropLVDburnOmissionLTwoVarLrMultThree}{\tbd{dropLVDburnOmissionLTwoVarLrMultThree}}
\providecommand{\dropLVDburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropLVDburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropLVDburnOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropLVDburnOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropLVDburnShiftLOne}{\tbd{dropLVDburnShiftLOne}}
\providecommand{\dropLVDburnShiftLOneVarDecoderMaskTwoformerFull}{\tbd{dropLVDburnShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropLVDburnShiftLOneVarDecoderMaskTwoformerLite}{\tbd{dropLVDburnShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDburnShiftLOneVarDecoderSamLite}{\tbd{dropLVDburnShiftLOneVarDecoderSamLite}}
\providecommand{\dropLVDburnShiftLOneVarDecoderSamPretrained}{\tbd{dropLVDburnShiftLOneVarDecoderSamPretrained}}
\providecommand{\dropLVDburnShiftLOneVarDecoderSegformerMlp}{\tbd{dropLVDburnShiftLOneVarDecoderSegformerMlp}}
\providecommand{\dropLVDburnShiftLR}{\tbd{dropLVDburnShiftLR}}
\providecommand{\dropLVDburnShiftLRVarLrMultOne}{\tbd{dropLVDburnShiftLRVarLrMultOne}}
\providecommand{\dropLVDburnShiftLTwo}{\tbd{dropLVDburnShiftLTwo}}
\providecommand{\dropLVDburnShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{dropLVDburnShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropLVDburnShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{dropLVDburnShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\dropLVDburnShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropLVDburnShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{dropLVDburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\dropLVDburnShiftLTwoVarDecoderSamLite}{\tbd{dropLVDburnShiftLTwoVarDecoderSamLite}}
\providecommand{\dropLVDburnShiftLTwoVarDecoderSamLiteLrMultOne}{\tbd{dropLVDburnShiftLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\dropLVDburnShiftLTwoVarDecoderSamPretrained}{\tbd{dropLVDburnShiftLTwoVarDecoderSamPretrained}}
\providecommand{\dropLVDburnShiftLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{dropLVDburnShiftLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\dropLVDburnShiftLTwoVarDecoderSegformerMlp}{\tbd{dropLVDburnShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropLVDburnShiftLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{dropLVDburnShiftLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\dropLVDburnShiftLTwoVarLossBootstrap}{\tbd{dropLVDburnShiftLTwoVarLossBootstrap}}
\providecommand{\dropLVDburnShiftLTwoVarLossGce}{\tbd{dropLVDburnShiftLTwoVarLossGce}}
\providecommand{\dropLVDburnShiftLTwoVarLrMultOne}{\tbd{dropLVDburnShiftLTwoVarLrMultOne}}
\providecommand{\dropLVDburnShiftLTwoVarLrMultThree}{\tbd{dropLVDburnShiftLTwoVarLrMultThree}}
\providecommand{\dropLVDburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropLVDburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropLVDburnShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropLVDburnShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropLVDflairBoundaryLOne}{\tbd{dropLVDflairBoundaryLOne}}
\providecommand{\dropLVDflairBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{dropLVDflairBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropLVDflairBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{dropLVDflairBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDflairBoundaryLOneVarDecoderSamLite}{\tbd{dropLVDflairBoundaryLOneVarDecoderSamLite}}
\providecommand{\dropLVDflairBoundaryLOneVarDecoderSamPretrained}{\tbd{dropLVDflairBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\dropLVDflairBoundaryLOneVarDecoderSegformerMlp}{\tbd{dropLVDflairBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\dropLVDflairBoundaryLR}{\tbd{dropLVDflairBoundaryLR}}
\providecommand{\dropLVDflairBoundaryLRVarLrMultOne}{\tbd{dropLVDflairBoundaryLRVarLrMultOne}}
\providecommand{\dropLVDflairBoundaryLTwo}{\tbd{dropLVDflairBoundaryLTwo}}
\providecommand{\dropLVDflairBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{dropLVDflairBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropLVDflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{dropLVDflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\dropLVDflairBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropLVDflairBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{dropLVDflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\dropLVDflairBoundaryLTwoVarDecoderSamLite}{\tbd{dropLVDflairBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropLVDflairBoundaryLTwoVarDecoderSamLiteLrMultOne}{\tbd{dropLVDflairBoundaryLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\dropLVDflairBoundaryLTwoVarDecoderSamPretrained}{\tbd{dropLVDflairBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\dropLVDflairBoundaryLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{dropLVDflairBoundaryLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\dropLVDflairBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropLVDflairBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropLVDflairBoundaryLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{dropLVDflairBoundaryLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\dropLVDflairBoundaryLTwoVarLossBootstrap}{\tbd{dropLVDflairBoundaryLTwoVarLossBootstrap}}
\providecommand{\dropLVDflairBoundaryLTwoVarLossGce}{\tbd{dropLVDflairBoundaryLTwoVarLossGce}}
\providecommand{\dropLVDflairBoundaryLTwoVarLrMultOne}{\tbd{dropLVDflairBoundaryLTwoVarLrMultOne}}
\providecommand{\dropLVDflairBoundaryLTwoVarLrMultThree}{\tbd{dropLVDflairBoundaryLTwoVarLrMultThree}}
\providecommand{\dropLVDflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropLVDflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropLVDflairBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropLVDflairBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropLVDflairCoarseLOne}{\tbd{dropLVDflairCoarseLOne}}
\providecommand{\dropLVDflairCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{dropLVDflairCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropLVDflairCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{dropLVDflairCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDflairCoarseLOneVarDecoderSamLite}{\tbd{dropLVDflairCoarseLOneVarDecoderSamLite}}
\providecommand{\dropLVDflairCoarseLOneVarDecoderSamPretrained}{\tbd{dropLVDflairCoarseLOneVarDecoderSamPretrained}}
\providecommand{\dropLVDflairCoarseLOneVarDecoderSegformerMlp}{\tbd{dropLVDflairCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\dropLVDflairCoarseLR}{\tbd{dropLVDflairCoarseLR}}
\providecommand{\dropLVDflairCoarseLRVarLrMultOne}{\tbd{dropLVDflairCoarseLRVarLrMultOne}}
\providecommand{\dropLVDflairCoarseLTwo}{\tbd{dropLVDflairCoarseLTwo}}
\providecommand{\dropLVDflairCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{dropLVDflairCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropLVDflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{dropLVDflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\dropLVDflairCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropLVDflairCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{dropLVDflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\dropLVDflairCoarseLTwoVarDecoderSamLite}{\tbd{dropLVDflairCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropLVDflairCoarseLTwoVarDecoderSamLiteLrMultOne}{\tbd{dropLVDflairCoarseLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\dropLVDflairCoarseLTwoVarDecoderSamPretrained}{\tbd{dropLVDflairCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\dropLVDflairCoarseLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{dropLVDflairCoarseLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\dropLVDflairCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropLVDflairCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropLVDflairCoarseLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{dropLVDflairCoarseLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\dropLVDflairCoarseLTwoVarLossBootstrap}{\tbd{dropLVDflairCoarseLTwoVarLossBootstrap}}
\providecommand{\dropLVDflairCoarseLTwoVarLossGce}{\tbd{dropLVDflairCoarseLTwoVarLossGce}}
\providecommand{\dropLVDflairCoarseLTwoVarLrMultOne}{\tbd{dropLVDflairCoarseLTwoVarLrMultOne}}
\providecommand{\dropLVDflairCoarseLTwoVarLrMultThree}{\tbd{dropLVDflairCoarseLTwoVarLrMultThree}}
\providecommand{\dropLVDflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropLVDflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropLVDflairCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropLVDflairCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropLVDflairOmissionLOne}{\tbd{dropLVDflairOmissionLOne}}
\providecommand{\dropLVDflairOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{dropLVDflairOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropLVDflairOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{dropLVDflairOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDflairOmissionLOneVarDecoderSamLite}{\tbd{dropLVDflairOmissionLOneVarDecoderSamLite}}
\providecommand{\dropLVDflairOmissionLOneVarDecoderSamPretrained}{\tbd{dropLVDflairOmissionLOneVarDecoderSamPretrained}}
\providecommand{\dropLVDflairOmissionLOneVarDecoderSegformerMlp}{\tbd{dropLVDflairOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\dropLVDflairOmissionLR}{\tbd{dropLVDflairOmissionLR}}
\providecommand{\dropLVDflairOmissionLRVarLrMultOne}{\tbd{dropLVDflairOmissionLRVarLrMultOne}}
\providecommand{\dropLVDflairOmissionLTwo}{\tbd{dropLVDflairOmissionLTwo}}
\providecommand{\dropLVDflairOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{dropLVDflairOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropLVDflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{dropLVDflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\dropLVDflairOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropLVDflairOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{dropLVDflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\dropLVDflairOmissionLTwoVarDecoderSamLite}{\tbd{dropLVDflairOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropLVDflairOmissionLTwoVarDecoderSamLiteLrMultOne}{\tbd{dropLVDflairOmissionLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\dropLVDflairOmissionLTwoVarDecoderSamPretrained}{\tbd{dropLVDflairOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\dropLVDflairOmissionLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{dropLVDflairOmissionLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\dropLVDflairOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropLVDflairOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropLVDflairOmissionLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{dropLVDflairOmissionLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\dropLVDflairOmissionLTwoVarLossBootstrap}{\tbd{dropLVDflairOmissionLTwoVarLossBootstrap}}
\providecommand{\dropLVDflairOmissionLTwoVarLossGce}{\tbd{dropLVDflairOmissionLTwoVarLossGce}}
\providecommand{\dropLVDflairOmissionLTwoVarLrMultOne}{\tbd{dropLVDflairOmissionLTwoVarLrMultOne}}
\providecommand{\dropLVDflairOmissionLTwoVarLrMultThree}{\tbd{dropLVDflairOmissionLTwoVarLrMultThree}}
\providecommand{\dropLVDflairOmissionLTwoVarLrMultZeroOneOneOneOne}{\tbd{dropLVDflairOmissionLTwoVarLrMultZeroOneOneOneOne}}
\providecommand{\dropLVDflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropLVDflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropLVDflairOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropLVDflairOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropLVDflairShiftLOne}{\tbd{dropLVDflairShiftLOne}}
\providecommand{\dropLVDflairShiftLOneVarDecoderMaskTwoformerFull}{\tbd{dropLVDflairShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropLVDflairShiftLOneVarDecoderMaskTwoformerLite}{\tbd{dropLVDflairShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDflairShiftLOneVarDecoderSamLite}{\tbd{dropLVDflairShiftLOneVarDecoderSamLite}}
\providecommand{\dropLVDflairShiftLOneVarDecoderSamPretrained}{\tbd{dropLVDflairShiftLOneVarDecoderSamPretrained}}
\providecommand{\dropLVDflairShiftLOneVarDecoderSegformerMlp}{\tbd{dropLVDflairShiftLOneVarDecoderSegformerMlp}}
\providecommand{\dropLVDflairShiftLR}{\tbd{dropLVDflairShiftLR}}
\providecommand{\dropLVDflairShiftLRVarLrMultOne}{\tbd{dropLVDflairShiftLRVarLrMultOne}}
\providecommand{\dropLVDflairShiftLTwo}{\tbd{dropLVDflairShiftLTwo}}
\providecommand{\dropLVDflairShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{dropLVDflairShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropLVDflairShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{dropLVDflairShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\dropLVDflairShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropLVDflairShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropLVDflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{dropLVDflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\dropLVDflairShiftLTwoVarDecoderSamLite}{\tbd{dropLVDflairShiftLTwoVarDecoderSamLite}}
\providecommand{\dropLVDflairShiftLTwoVarDecoderSamLiteLrMultOne}{\tbd{dropLVDflairShiftLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\dropLVDflairShiftLTwoVarDecoderSamPretrained}{\tbd{dropLVDflairShiftLTwoVarDecoderSamPretrained}}
\providecommand{\dropLVDflairShiftLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{dropLVDflairShiftLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\dropLVDflairShiftLTwoVarDecoderSegformerMlp}{\tbd{dropLVDflairShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropLVDflairShiftLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{dropLVDflairShiftLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\dropLVDflairShiftLTwoVarLossBootstrap}{\tbd{dropLVDflairShiftLTwoVarLossBootstrap}}
\providecommand{\dropLVDflairShiftLTwoVarLossGce}{\tbd{dropLVDflairShiftLTwoVarLossGce}}
\providecommand{\dropLVDflairShiftLTwoVarLrMultOne}{\tbd{dropLVDflairShiftLTwoVarLrMultOne}}
\providecommand{\dropLVDflairShiftLTwoVarLrMultThree}{\tbd{dropLVDflairShiftLTwoVarLrMultThree}}
\providecommand{\dropLVDflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropLVDflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropLVDflairShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropLVDflairShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropLVDsenOtsuLTwo}{\tbd{dropLVDsenOtsuLTwo}}
\providecommand{\dropPRIburnBoundaryLOne}{\tbd{dropPRIburnBoundaryLOne}}
\providecommand{\dropPRIburnBoundaryLTwo}{\tbd{dropPRIburnBoundaryLTwo}}
\providecommand{\dropPRIburnCoarseLOne}{\tbd{dropPRIburnCoarseLOne}}
\providecommand{\dropPRIburnCoarseLTwo}{\tbd{dropPRIburnCoarseLTwo}}
\providecommand{\dropPRIburnOmissionLOne}{\tbd{dropPRIburnOmissionLOne}}
\providecommand{\dropPRIburnOmissionLTwo}{\tbd{dropPRIburnOmissionLTwo}}
\providecommand{\dropPRIburnShiftLOne}{\tbd{dropPRIburnShiftLOne}}
\providecommand{\dropPRIburnShiftLTwo}{\tbd{dropPRIburnShiftLTwo}}
\providecommand{\dropPRIflairBoundaryLOne}{\tbd{dropPRIflairBoundaryLOne}}
\providecommand{\dropPRIflairBoundaryLTwo}{\tbd{dropPRIflairBoundaryLTwo}}
\providecommand{\dropPRIflairCoarseLOne}{\tbd{dropPRIflairCoarseLOne}}
\providecommand{\dropPRIflairCoarseLTwo}{\tbd{dropPRIflairCoarseLTwo}}
\providecommand{\dropPRIflairOmissionLOne}{\tbd{dropPRIflairOmissionLOne}}
\providecommand{\dropPRIflairOmissionLTwo}{\tbd{dropPRIflairOmissionLTwo}}
\providecommand{\dropPRIflairShiftLOne}{\tbd{dropPRIflairShiftLOne}}
\providecommand{\dropPRIflairShiftLTwo}{\tbd{dropPRIflairShiftLTwo}}
\providecommand{\dropRNChesBoundaryLOne}{\tbd{dropRNChesBoundaryLOne}}
\providecommand{\dropRNChesBoundaryLTwo}{\tbd{dropRNChesBoundaryLTwo}}
\providecommand{\dropRNChesCoarseLOne}{\tbd{dropRNChesCoarseLOne}}
\providecommand{\dropRNChesCoarseLTwo}{\tbd{dropRNChesCoarseLTwo}}
\providecommand{\dropRNChesNlcdREAL}{\tbd{dropRNChesNlcdREAL}}
\providecommand{\dropRNChesOmissionLOne}{\tbd{dropRNChesOmissionLOne}}
\providecommand{\dropRNChesOmissionLTwo}{\tbd{dropRNChesOmissionLTwo}}
\providecommand{\dropRNChesShiftLOne}{\tbd{dropRNChesShiftLOne}}
\providecommand{\dropRNChesShiftLTwo}{\tbd{dropRNChesShiftLTwo}}
\providecommand{\dropRNCsTwelveBoundaryLOne}{\tbd{dropRNCsTwelveBoundaryLOne}}
\providecommand{\dropRNCsTwelveBoundaryLTwo}{\tbd{dropRNCsTwelveBoundaryLTwo}}
\providecommand{\dropRNCsTwelveCoarseLOne}{\tbd{dropRNCsTwelveCoarseLOne}}
\providecommand{\dropRNCsTwelveCoarseLTwo}{\tbd{dropRNCsTwelveCoarseLTwo}}
\providecommand{\dropRNCsTwelveOmissionLOne}{\tbd{dropRNCsTwelveOmissionLOne}}
\providecommand{\dropRNCsTwelveOmissionLTwo}{\tbd{dropRNCsTwelveOmissionLTwo}}
\providecommand{\dropRNCsTwelveSTwocloudlessREAL}{\tbd{dropRNCsTwelveSTwocloudlessREAL}}
\providecommand{\dropRNCsTwelveShiftLOne}{\tbd{dropRNCsTwelveShiftLOne}}
\providecommand{\dropRNCsTwelveShiftLTwo}{\tbd{dropRNCsTwelveShiftLTwo}}
\providecommand{\dropRNDfcBoundaryLOne}{\tbd{dropRNDfcBoundaryLOne}}
\providecommand{\dropRNDfcBoundaryLTwo}{\tbd{dropRNDfcBoundaryLTwo}}
\providecommand{\dropRNDfcCoarseLOne}{\tbd{dropRNDfcCoarseLOne}}
\providecommand{\dropRNDfcCoarseLTwo}{\tbd{dropRNDfcCoarseLTwo}}
\providecommand{\dropRNDfcModisREALVarTrainSubsetRealcov}{\tbd{dropRNDfcModisREALVarTrainSubsetRealcov}}
\providecommand{\dropRNDfcOmissionLOne}{\tbd{dropRNDfcOmissionLOne}}
\providecommand{\dropRNDfcOmissionLTwo}{\tbd{dropRNDfcOmissionLTwo}}
\providecommand{\dropRNDfcShiftLOne}{\tbd{dropRNDfcShiftLOne}}
\providecommand{\dropRNDfcShiftLTwo}{\tbd{dropRNDfcShiftLTwo}}
\providecommand{\dropRNEnvaBoundaryLOne}{\tbd{dropRNEnvaBoundaryLOne}}
\providecommand{\dropRNEnvaBoundaryLTwo}{\tbd{dropRNEnvaBoundaryLTwo}}
\providecommand{\dropRNEnvaCoarseLOne}{\tbd{dropRNEnvaCoarseLOne}}
\providecommand{\dropRNEnvaCoarseLTwo}{\tbd{dropRNEnvaCoarseLTwo}}
\providecommand{\dropRNEnvaNlcdREAL}{\tbd{dropRNEnvaNlcdREAL}}
\providecommand{\dropRNEnvaOmissionLOne}{\tbd{dropRNEnvaOmissionLOne}}
\providecommand{\dropRNEnvaOmissionLTwo}{\tbd{dropRNEnvaOmissionLTwo}}
\providecommand{\dropRNEnvaShiftLOne}{\tbd{dropRNEnvaShiftLOne}}
\providecommand{\dropRNEnvaShiftLTwo}{\tbd{dropRNEnvaShiftLTwo}}
\providecommand{\dropRNKuroBoundaryLOne}{\tbd{dropRNKuroBoundaryLOne}}
\providecommand{\dropRNKuroBoundaryLTwo}{\tbd{dropRNKuroBoundaryLTwo}}
\providecommand{\dropRNKuroCemsREALVarTrainSubsetRealcov}{\tbd{dropRNKuroCemsREALVarTrainSubsetRealcov}}
\providecommand{\dropRNKuroCoarseLOne}{\tbd{dropRNKuroCoarseLOne}}
\providecommand{\dropRNKuroCoarseLTwo}{\tbd{dropRNKuroCoarseLTwo}}
\providecommand{\dropRNKuroOmissionLOne}{\tbd{dropRNKuroOmissionLOne}}
\providecommand{\dropRNKuroOmissionLTwo}{\tbd{dropRNKuroOmissionLTwo}}
\providecommand{\dropRNKuroShiftLOne}{\tbd{dropRNKuroShiftLOne}}
\providecommand{\dropRNKuroShiftLTwo}{\tbd{dropRNKuroShiftLTwo}}
\providecommand{\dropRNOemBoundaryLOne}{\tbd{dropRNOemBoundaryLOne}}
\providecommand{\dropRNOemBoundaryLTwo}{\tbd{dropRNOemBoundaryLTwo}}
\providecommand{\dropRNOemCoarseLOne}{\tbd{dropRNOemCoarseLOne}}
\providecommand{\dropRNOemCoarseLTwo}{\tbd{dropRNOemCoarseLTwo}}
\providecommand{\dropRNOemOmissionLOne}{\tbd{dropRNOemOmissionLOne}}
\providecommand{\dropRNOemOmissionLTwo}{\tbd{dropRNOemOmissionLTwo}}
\providecommand{\dropRNOemShiftLOne}{\tbd{dropRNOemShiftLOne}}
\providecommand{\dropRNOemShiftLTwo}{\tbd{dropRNOemShiftLTwo}}
\providecommand{\dropRNSnTwoBoundaryLOne}{\tbd{dropRNSnTwoBoundaryLOne}}
\providecommand{\dropRNSnTwoBoundaryLTwo}{\tbd{dropRNSnTwoBoundaryLTwo}}
\providecommand{\dropRNSnTwoCoarseLOne}{\tbd{dropRNSnTwoCoarseLOne}}
\providecommand{\dropRNSnTwoCoarseLTwo}{\tbd{dropRNSnTwoCoarseLTwo}}
\providecommand{\dropRNSnTwoOmissionLOne}{\tbd{dropRNSnTwoOmissionLOne}}
\providecommand{\dropRNSnTwoOmissionLTwo}{\tbd{dropRNSnTwoOmissionLTwo}}
\providecommand{\dropRNSnTwoShiftLOne}{\tbd{dropRNSnTwoShiftLOne}}
\providecommand{\dropRNSnTwoShiftLTwo}{\tbd{dropRNSnTwoShiftLTwo}}
\providecommand{\dropRNburnBoundaryLOne}{\tbd{dropRNburnBoundaryLOne}}
\providecommand{\dropRNburnBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{dropRNburnBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropRNburnBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{dropRNburnBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropRNburnBoundaryLOneVarDecoderSamLite}{\tbd{dropRNburnBoundaryLOneVarDecoderSamLite}}
\providecommand{\dropRNburnBoundaryLOneVarDecoderSamPretrained}{\tbd{dropRNburnBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\dropRNburnBoundaryLOneVarDecoderSegformerMlp}{\tbd{dropRNburnBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\dropRNburnBoundaryLR}{\tbd{dropRNburnBoundaryLR}}
\providecommand{\dropRNburnBoundaryLTwo}{\tbd{dropRNburnBoundaryLTwo}}
\providecommand{\dropRNburnBoundaryLTwoVarBandsRgb}{\tbd{dropRNburnBoundaryLTwoVarBandsRgb}}
\providecommand{\dropRNburnBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{dropRNburnBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropRNburnBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropRNburnBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropRNburnBoundaryLTwoVarDecoderSamLite}{\tbd{dropRNburnBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropRNburnBoundaryLTwoVarDecoderSamPretrained}{\tbd{dropRNburnBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\dropRNburnBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropRNburnBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropRNburnBoundaryLTwoVarInitRandom}{\tbd{dropRNburnBoundaryLTwoVarInitRandom}}
\providecommand{\dropRNburnBoundaryLTwoVarLossBootstrap}{\tbd{dropRNburnBoundaryLTwoVarLossBootstrap}}
\providecommand{\dropRNburnBoundaryLTwoVarLossGce}{\tbd{dropRNburnBoundaryLTwoVarLossGce}}
\providecommand{\dropRNburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropRNburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropRNburnBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropRNburnBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropRNburnCoarseLOne}{\tbd{dropRNburnCoarseLOne}}
\providecommand{\dropRNburnCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{dropRNburnCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropRNburnCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{dropRNburnCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropRNburnCoarseLOneVarDecoderSamLite}{\tbd{dropRNburnCoarseLOneVarDecoderSamLite}}
\providecommand{\dropRNburnCoarseLOneVarDecoderSamPretrained}{\tbd{dropRNburnCoarseLOneVarDecoderSamPretrained}}
\providecommand{\dropRNburnCoarseLOneVarDecoderSegformerMlp}{\tbd{dropRNburnCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\dropRNburnCoarseLR}{\tbd{dropRNburnCoarseLR}}
\providecommand{\dropRNburnCoarseLTwo}{\tbd{dropRNburnCoarseLTwo}}
\providecommand{\dropRNburnCoarseLTwoVarBandsRgb}{\tbd{dropRNburnCoarseLTwoVarBandsRgb}}
\providecommand{\dropRNburnCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{dropRNburnCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropRNburnCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropRNburnCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropRNburnCoarseLTwoVarDecoderSamLite}{\tbd{dropRNburnCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropRNburnCoarseLTwoVarDecoderSamPretrained}{\tbd{dropRNburnCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\dropRNburnCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropRNburnCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropRNburnCoarseLTwoVarInitRandom}{\tbd{dropRNburnCoarseLTwoVarInitRandom}}
\providecommand{\dropRNburnCoarseLTwoVarLossBootstrap}{\tbd{dropRNburnCoarseLTwoVarLossBootstrap}}
\providecommand{\dropRNburnCoarseLTwoVarLossGce}{\tbd{dropRNburnCoarseLTwoVarLossGce}}
\providecommand{\dropRNburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropRNburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropRNburnCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropRNburnCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropRNburnOmissionLOne}{\tbd{dropRNburnOmissionLOne}}
\providecommand{\dropRNburnOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{dropRNburnOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropRNburnOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{dropRNburnOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropRNburnOmissionLOneVarDecoderSamLite}{\tbd{dropRNburnOmissionLOneVarDecoderSamLite}}
\providecommand{\dropRNburnOmissionLOneVarDecoderSamPretrained}{\tbd{dropRNburnOmissionLOneVarDecoderSamPretrained}}
\providecommand{\dropRNburnOmissionLOneVarDecoderSegformerMlp}{\tbd{dropRNburnOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\dropRNburnOmissionLR}{\tbd{dropRNburnOmissionLR}}
\providecommand{\dropRNburnOmissionLTwo}{\tbd{dropRNburnOmissionLTwo}}
\providecommand{\dropRNburnOmissionLTwoVarBandsRgb}{\tbd{dropRNburnOmissionLTwoVarBandsRgb}}
\providecommand{\dropRNburnOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{dropRNburnOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropRNburnOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropRNburnOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropRNburnOmissionLTwoVarDecoderSamLite}{\tbd{dropRNburnOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropRNburnOmissionLTwoVarDecoderSamPretrained}{\tbd{dropRNburnOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\dropRNburnOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropRNburnOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropRNburnOmissionLTwoVarInitRandom}{\tbd{dropRNburnOmissionLTwoVarInitRandom}}
\providecommand{\dropRNburnOmissionLTwoVarLossBootstrap}{\tbd{dropRNburnOmissionLTwoVarLossBootstrap}}
\providecommand{\dropRNburnOmissionLTwoVarLossGce}{\tbd{dropRNburnOmissionLTwoVarLossGce}}
\providecommand{\dropRNburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropRNburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropRNburnOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropRNburnOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropRNburnShiftLOne}{\tbd{dropRNburnShiftLOne}}
\providecommand{\dropRNburnShiftLOneVarDecoderMaskTwoformerFull}{\tbd{dropRNburnShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropRNburnShiftLOneVarDecoderMaskTwoformerLite}{\tbd{dropRNburnShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropRNburnShiftLOneVarDecoderSamLite}{\tbd{dropRNburnShiftLOneVarDecoderSamLite}}
\providecommand{\dropRNburnShiftLOneVarDecoderSamPretrained}{\tbd{dropRNburnShiftLOneVarDecoderSamPretrained}}
\providecommand{\dropRNburnShiftLOneVarDecoderSegformerMlp}{\tbd{dropRNburnShiftLOneVarDecoderSegformerMlp}}
\providecommand{\dropRNburnShiftLR}{\tbd{dropRNburnShiftLR}}
\providecommand{\dropRNburnShiftLTwo}{\tbd{dropRNburnShiftLTwo}}
\providecommand{\dropRNburnShiftLTwoVarBandsRgb}{\tbd{dropRNburnShiftLTwoVarBandsRgb}}
\providecommand{\dropRNburnShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{dropRNburnShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropRNburnShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropRNburnShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropRNburnShiftLTwoVarDecoderSamLite}{\tbd{dropRNburnShiftLTwoVarDecoderSamLite}}
\providecommand{\dropRNburnShiftLTwoVarDecoderSamPretrained}{\tbd{dropRNburnShiftLTwoVarDecoderSamPretrained}}
\providecommand{\dropRNburnShiftLTwoVarDecoderSegformerMlp}{\tbd{dropRNburnShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropRNburnShiftLTwoVarInitRandom}{\tbd{dropRNburnShiftLTwoVarInitRandom}}
\providecommand{\dropRNburnShiftLTwoVarLossBootstrap}{\tbd{dropRNburnShiftLTwoVarLossBootstrap}}
\providecommand{\dropRNburnShiftLTwoVarLossGce}{\tbd{dropRNburnShiftLTwoVarLossGce}}
\providecommand{\dropRNburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropRNburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropRNburnShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropRNburnShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropRNflairBoundaryLOne}{\tbd{dropRNflairBoundaryLOne}}
\providecommand{\dropRNflairBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{dropRNflairBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropRNflairBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{dropRNflairBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropRNflairBoundaryLOneVarDecoderSamLite}{\tbd{dropRNflairBoundaryLOneVarDecoderSamLite}}
\providecommand{\dropRNflairBoundaryLOneVarDecoderSamPretrained}{\tbd{dropRNflairBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\dropRNflairBoundaryLOneVarDecoderSegformerMlp}{\tbd{dropRNflairBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\dropRNflairBoundaryLR}{\tbd{dropRNflairBoundaryLR}}
\providecommand{\dropRNflairBoundaryLTwo}{\tbd{dropRNflairBoundaryLTwo}}
\providecommand{\dropRNflairBoundaryLTwoVarBandsRgb}{\tbd{dropRNflairBoundaryLTwoVarBandsRgb}}
\providecommand{\dropRNflairBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{dropRNflairBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropRNflairBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropRNflairBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropRNflairBoundaryLTwoVarDecoderSamLite}{\tbd{dropRNflairBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropRNflairBoundaryLTwoVarDecoderSamPretrained}{\tbd{dropRNflairBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\dropRNflairBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropRNflairBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropRNflairBoundaryLTwoVarInitRandom}{\tbd{dropRNflairBoundaryLTwoVarInitRandom}}
\providecommand{\dropRNflairBoundaryLTwoVarLossBootstrap}{\tbd{dropRNflairBoundaryLTwoVarLossBootstrap}}
\providecommand{\dropRNflairBoundaryLTwoVarLossGce}{\tbd{dropRNflairBoundaryLTwoVarLossGce}}
\providecommand{\dropRNflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropRNflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropRNflairBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropRNflairBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropRNflairCoarseLOne}{\tbd{dropRNflairCoarseLOne}}
\providecommand{\dropRNflairCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{dropRNflairCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropRNflairCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{dropRNflairCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropRNflairCoarseLOneVarDecoderSamLite}{\tbd{dropRNflairCoarseLOneVarDecoderSamLite}}
\providecommand{\dropRNflairCoarseLOneVarDecoderSamPretrained}{\tbd{dropRNflairCoarseLOneVarDecoderSamPretrained}}
\providecommand{\dropRNflairCoarseLOneVarDecoderSegformerMlp}{\tbd{dropRNflairCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\dropRNflairCoarseLR}{\tbd{dropRNflairCoarseLR}}
\providecommand{\dropRNflairCoarseLTwo}{\tbd{dropRNflairCoarseLTwo}}
\providecommand{\dropRNflairCoarseLTwoVarBandsRgb}{\tbd{dropRNflairCoarseLTwoVarBandsRgb}}
\providecommand{\dropRNflairCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{dropRNflairCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropRNflairCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropRNflairCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropRNflairCoarseLTwoVarDecoderSamLite}{\tbd{dropRNflairCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropRNflairCoarseLTwoVarDecoderSamPretrained}{\tbd{dropRNflairCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\dropRNflairCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropRNflairCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropRNflairCoarseLTwoVarInitRandom}{\tbd{dropRNflairCoarseLTwoVarInitRandom}}
\providecommand{\dropRNflairCoarseLTwoVarLossBootstrap}{\tbd{dropRNflairCoarseLTwoVarLossBootstrap}}
\providecommand{\dropRNflairCoarseLTwoVarLossGce}{\tbd{dropRNflairCoarseLTwoVarLossGce}}
\providecommand{\dropRNflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropRNflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropRNflairCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropRNflairCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropRNflairOmissionLOne}{\tbd{dropRNflairOmissionLOne}}
\providecommand{\dropRNflairOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{dropRNflairOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropRNflairOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{dropRNflairOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropRNflairOmissionLOneVarDecoderSamLite}{\tbd{dropRNflairOmissionLOneVarDecoderSamLite}}
\providecommand{\dropRNflairOmissionLOneVarDecoderSamPretrained}{\tbd{dropRNflairOmissionLOneVarDecoderSamPretrained}}
\providecommand{\dropRNflairOmissionLOneVarDecoderSegformerMlp}{\tbd{dropRNflairOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\dropRNflairOmissionLR}{\tbd{dropRNflairOmissionLR}}
\providecommand{\dropRNflairOmissionLTwo}{\tbd{dropRNflairOmissionLTwo}}
\providecommand{\dropRNflairOmissionLTwoVarBandsRgb}{\tbd{dropRNflairOmissionLTwoVarBandsRgb}}
\providecommand{\dropRNflairOmissionLTwoVarClassWeightedTrue}{\tbd{dropRNflairOmissionLTwoVarClassWeightedTrue}}
\providecommand{\dropRNflairOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{dropRNflairOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropRNflairOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropRNflairOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropRNflairOmissionLTwoVarDecoderSamLite}{\tbd{dropRNflairOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropRNflairOmissionLTwoVarDecoderSamPretrained}{\tbd{dropRNflairOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\dropRNflairOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropRNflairOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropRNflairOmissionLTwoVarInitRandom}{\tbd{dropRNflairOmissionLTwoVarInitRandom}}
\providecommand{\dropRNflairOmissionLTwoVarLossBootstrap}{\tbd{dropRNflairOmissionLTwoVarLossBootstrap}}
\providecommand{\dropRNflairOmissionLTwoVarLossGce}{\tbd{dropRNflairOmissionLTwoVarLossGce}}
\providecommand{\dropRNflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropRNflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropRNflairOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropRNflairOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropRNflairShiftLOne}{\tbd{dropRNflairShiftLOne}}
\providecommand{\dropRNflairShiftLOneVarDecoderMaskTwoformerFull}{\tbd{dropRNflairShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropRNflairShiftLOneVarDecoderMaskTwoformerLite}{\tbd{dropRNflairShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropRNflairShiftLOneVarDecoderSamLite}{\tbd{dropRNflairShiftLOneVarDecoderSamLite}}
\providecommand{\dropRNflairShiftLOneVarDecoderSamPretrained}{\tbd{dropRNflairShiftLOneVarDecoderSamPretrained}}
\providecommand{\dropRNflairShiftLOneVarDecoderSegformerMlp}{\tbd{dropRNflairShiftLOneVarDecoderSegformerMlp}}
\providecommand{\dropRNflairShiftLR}{\tbd{dropRNflairShiftLR}}
\providecommand{\dropRNflairShiftLTwo}{\tbd{dropRNflairShiftLTwo}}
\providecommand{\dropRNflairShiftLTwoVarBandsRgb}{\tbd{dropRNflairShiftLTwoVarBandsRgb}}
\providecommand{\dropRNflairShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{dropRNflairShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropRNflairShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropRNflairShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropRNflairShiftLTwoVarDecoderSamLite}{\tbd{dropRNflairShiftLTwoVarDecoderSamLite}}
\providecommand{\dropRNflairShiftLTwoVarDecoderSamPretrained}{\tbd{dropRNflairShiftLTwoVarDecoderSamPretrained}}
\providecommand{\dropRNflairShiftLTwoVarDecoderSegformerMlp}{\tbd{dropRNflairShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropRNflairShiftLTwoVarInitRandom}{\tbd{dropRNflairShiftLTwoVarInitRandom}}
\providecommand{\dropRNflairShiftLTwoVarLossBootstrap}{\tbd{dropRNflairShiftLTwoVarLossBootstrap}}
\providecommand{\dropRNflairShiftLTwoVarLossGce}{\tbd{dropRNflairShiftLTwoVarLossGce}}
\providecommand{\dropRNflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropRNflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropRNflairShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropRNflairShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropRNsenOtsuLTwo}{\tbd{dropRNsenOtsuLTwo}}
\providecommand{\dropResnetFiveZeroSslFoureoburnBoundaryLOne}{\tbd{dropResnetFiveZeroSslFoureoburnBoundaryLOne}}
\providecommand{\dropResnetFiveZeroSslFoureoburnBoundaryLTwo}{\tbd{dropResnetFiveZeroSslFoureoburnBoundaryLTwo}}
\providecommand{\dropResnetFiveZeroSslFoureoburnCoarseLOne}{\tbd{dropResnetFiveZeroSslFoureoburnCoarseLOne}}
\providecommand{\dropResnetFiveZeroSslFoureoburnCoarseLTwo}{\tbd{dropResnetFiveZeroSslFoureoburnCoarseLTwo}}
\providecommand{\dropResnetFiveZeroSslFoureoburnOmissionLOne}{\tbd{dropResnetFiveZeroSslFoureoburnOmissionLOne}}
\providecommand{\dropResnetFiveZeroSslFoureoburnOmissionLTwo}{\tbd{dropResnetFiveZeroSslFoureoburnOmissionLTwo}}
\providecommand{\dropResnetFiveZeroSslFoureoburnShiftLOne}{\tbd{dropResnetFiveZeroSslFoureoburnShiftLOne}}
\providecommand{\dropResnetFiveZeroSslFoureoburnShiftLTwo}{\tbd{dropResnetFiveZeroSslFoureoburnShiftLTwo}}
\providecommand{\dropResnetFiveZeroSslFoureoflairBoundaryLOne}{\tbd{dropResnetFiveZeroSslFoureoflairBoundaryLOne}}
\providecommand{\dropResnetFiveZeroSslFoureoflairBoundaryLTwo}{\tbd{dropResnetFiveZeroSslFoureoflairBoundaryLTwo}}
\providecommand{\dropResnetFiveZeroSslFoureoflairCoarseLOne}{\tbd{dropResnetFiveZeroSslFoureoflairCoarseLOne}}
\providecommand{\dropResnetFiveZeroSslFoureoflairCoarseLTwo}{\tbd{dropResnetFiveZeroSslFoureoflairCoarseLTwo}}
\providecommand{\dropResnetFiveZeroSslFoureoflairOmissionLOne}{\tbd{dropResnetFiveZeroSslFoureoflairOmissionLOne}}
\providecommand{\dropResnetFiveZeroSslFoureoflairOmissionLTwo}{\tbd{dropResnetFiveZeroSslFoureoflairOmissionLTwo}}
\providecommand{\dropResnetFiveZeroSslFoureoflairShiftLOne}{\tbd{dropResnetFiveZeroSslFoureoflairShiftLOne}}
\providecommand{\dropResnetFiveZeroSslFoureoflairShiftLTwo}{\tbd{dropResnetFiveZeroSslFoureoflairShiftLTwo}}
\providecommand{\dropSATChesBoundaryLOne}{\tbd{dropSATChesBoundaryLOne}}
\providecommand{\dropSATChesBoundaryLTwo}{\tbd{dropSATChesBoundaryLTwo}}
\providecommand{\dropSATChesBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropSATChesBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATChesBoundaryLTwoVarDecoderSamLite}{\tbd{dropSATChesBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropSATChesBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropSATChesBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropSATChesBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATChesBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATChesCoarseLOne}{\tbd{dropSATChesCoarseLOne}}
\providecommand{\dropSATChesCoarseLTwo}{\tbd{dropSATChesCoarseLTwo}}
\providecommand{\dropSATChesCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropSATChesCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATChesCoarseLTwoVarDecoderSamLite}{\tbd{dropSATChesCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropSATChesCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropSATChesCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropSATChesCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATChesCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATChesNlcdREAL}{\tbd{dropSATChesNlcdREAL}}
\providecommand{\dropSATChesOmissionLOne}{\tbd{dropSATChesOmissionLOne}}
\providecommand{\dropSATChesOmissionLTwo}{\tbd{dropSATChesOmissionLTwo}}
\providecommand{\dropSATChesOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropSATChesOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATChesOmissionLTwoVarDecoderSamLite}{\tbd{dropSATChesOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropSATChesOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropSATChesOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropSATChesOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATChesOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATChesShiftLOne}{\tbd{dropSATChesShiftLOne}}
\providecommand{\dropSATChesShiftLTwo}{\tbd{dropSATChesShiftLTwo}}
\providecommand{\dropSATChesShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropSATChesShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATChesShiftLTwoVarDecoderSamLite}{\tbd{dropSATChesShiftLTwoVarDecoderSamLite}}
\providecommand{\dropSATChesShiftLTwoVarDecoderSegformerMlp}{\tbd{dropSATChesShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropSATChesShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATChesShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATCsTwelveBoundaryLOne}{\tbd{dropSATCsTwelveBoundaryLOne}}
\providecommand{\dropSATCsTwelveBoundaryLTwo}{\tbd{dropSATCsTwelveBoundaryLTwo}}
\providecommand{\dropSATCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropSATCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATCsTwelveBoundaryLTwoVarDecoderSamLite}{\tbd{dropSATCsTwelveBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropSATCsTwelveBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropSATCsTwelveBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropSATCsTwelveBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATCsTwelveBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATCsTwelveCoarseLOne}{\tbd{dropSATCsTwelveCoarseLOne}}
\providecommand{\dropSATCsTwelveCoarseLTwo}{\tbd{dropSATCsTwelveCoarseLTwo}}
\providecommand{\dropSATCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropSATCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATCsTwelveCoarseLTwoVarDecoderSamLite}{\tbd{dropSATCsTwelveCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropSATCsTwelveCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropSATCsTwelveCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropSATCsTwelveCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATCsTwelveCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATCsTwelveOmissionLOne}{\tbd{dropSATCsTwelveOmissionLOne}}
\providecommand{\dropSATCsTwelveOmissionLTwo}{\tbd{dropSATCsTwelveOmissionLTwo}}
\providecommand{\dropSATCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropSATCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATCsTwelveOmissionLTwoVarDecoderSamLite}{\tbd{dropSATCsTwelveOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropSATCsTwelveOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropSATCsTwelveOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropSATCsTwelveOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATCsTwelveOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATCsTwelveSTwocloudlessREAL}{\tbd{dropSATCsTwelveSTwocloudlessREAL}}
\providecommand{\dropSATCsTwelveShiftLOne}{\tbd{dropSATCsTwelveShiftLOne}}
\providecommand{\dropSATCsTwelveShiftLTwo}{\tbd{dropSATCsTwelveShiftLTwo}}
\providecommand{\dropSATCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropSATCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATCsTwelveShiftLTwoVarDecoderSamLite}{\tbd{dropSATCsTwelveShiftLTwoVarDecoderSamLite}}
\providecommand{\dropSATCsTwelveShiftLTwoVarDecoderSegformerMlp}{\tbd{dropSATCsTwelveShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropSATCsTwelveShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATCsTwelveShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATDfcBoundaryLOne}{\tbd{dropSATDfcBoundaryLOne}}
\providecommand{\dropSATDfcBoundaryLTwo}{\tbd{dropSATDfcBoundaryLTwo}}
\providecommand{\dropSATDfcBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropSATDfcBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATDfcBoundaryLTwoVarDecoderSamLite}{\tbd{dropSATDfcBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropSATDfcBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropSATDfcBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropSATDfcBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATDfcBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATDfcCoarseLOne}{\tbd{dropSATDfcCoarseLOne}}
\providecommand{\dropSATDfcCoarseLTwo}{\tbd{dropSATDfcCoarseLTwo}}
\providecommand{\dropSATDfcCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropSATDfcCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATDfcCoarseLTwoVarDecoderSamLite}{\tbd{dropSATDfcCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropSATDfcCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropSATDfcCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropSATDfcCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATDfcCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATDfcModisREALVarTrainSubsetRealcov}{\tbd{dropSATDfcModisREALVarTrainSubsetRealcov}}
\providecommand{\dropSATDfcOmissionLOne}{\tbd{dropSATDfcOmissionLOne}}
\providecommand{\dropSATDfcOmissionLTwo}{\tbd{dropSATDfcOmissionLTwo}}
\providecommand{\dropSATDfcOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropSATDfcOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATDfcOmissionLTwoVarDecoderSamLite}{\tbd{dropSATDfcOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropSATDfcOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropSATDfcOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropSATDfcOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATDfcOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATDfcShiftLOne}{\tbd{dropSATDfcShiftLOne}}
\providecommand{\dropSATDfcShiftLTwo}{\tbd{dropSATDfcShiftLTwo}}
\providecommand{\dropSATDfcShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropSATDfcShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATDfcShiftLTwoVarDecoderSamLite}{\tbd{dropSATDfcShiftLTwoVarDecoderSamLite}}
\providecommand{\dropSATDfcShiftLTwoVarDecoderSegformerMlp}{\tbd{dropSATDfcShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropSATDfcShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATDfcShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATEnvaBoundaryLOne}{\tbd{dropSATEnvaBoundaryLOne}}
\providecommand{\dropSATEnvaBoundaryLTwo}{\tbd{dropSATEnvaBoundaryLTwo}}
\providecommand{\dropSATEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropSATEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATEnvaBoundaryLTwoVarDecoderSamLite}{\tbd{dropSATEnvaBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropSATEnvaBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropSATEnvaBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropSATEnvaBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATEnvaBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATEnvaCoarseLOne}{\tbd{dropSATEnvaCoarseLOne}}
\providecommand{\dropSATEnvaCoarseLTwo}{\tbd{dropSATEnvaCoarseLTwo}}
\providecommand{\dropSATEnvaCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropSATEnvaCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATEnvaCoarseLTwoVarDecoderSamLite}{\tbd{dropSATEnvaCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropSATEnvaCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropSATEnvaCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropSATEnvaCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATEnvaCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATEnvaNlcdREAL}{\tbd{dropSATEnvaNlcdREAL}}
\providecommand{\dropSATEnvaOmissionLOne}{\tbd{dropSATEnvaOmissionLOne}}
\providecommand{\dropSATEnvaOmissionLTwo}{\tbd{dropSATEnvaOmissionLTwo}}
\providecommand{\dropSATEnvaOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropSATEnvaOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATEnvaOmissionLTwoVarDecoderSamLite}{\tbd{dropSATEnvaOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropSATEnvaOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropSATEnvaOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropSATEnvaOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATEnvaOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATEnvaShiftLOne}{\tbd{dropSATEnvaShiftLOne}}
\providecommand{\dropSATEnvaShiftLTwo}{\tbd{dropSATEnvaShiftLTwo}}
\providecommand{\dropSATEnvaShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropSATEnvaShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATEnvaShiftLTwoVarDecoderSamLite}{\tbd{dropSATEnvaShiftLTwoVarDecoderSamLite}}
\providecommand{\dropSATEnvaShiftLTwoVarDecoderSegformerMlp}{\tbd{dropSATEnvaShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropSATEnvaShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATEnvaShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATKuroBoundaryLOne}{\tbd{dropSATKuroBoundaryLOne}}
\providecommand{\dropSATKuroBoundaryLTwo}{\tbd{dropSATKuroBoundaryLTwo}}
\providecommand{\dropSATKuroBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropSATKuroBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATKuroBoundaryLTwoVarDecoderSamLite}{\tbd{dropSATKuroBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropSATKuroBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropSATKuroBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropSATKuroBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATKuroBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATKuroCemsREALVarTrainSubsetRealcov}{\tbd{dropSATKuroCemsREALVarTrainSubsetRealcov}}
\providecommand{\dropSATKuroCoarseLOne}{\tbd{dropSATKuroCoarseLOne}}
\providecommand{\dropSATKuroCoarseLTwo}{\tbd{dropSATKuroCoarseLTwo}}
\providecommand{\dropSATKuroCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropSATKuroCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATKuroCoarseLTwoVarDecoderSamLite}{\tbd{dropSATKuroCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropSATKuroCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropSATKuroCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropSATKuroCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATKuroCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATKuroOmissionLOne}{\tbd{dropSATKuroOmissionLOne}}
\providecommand{\dropSATKuroOmissionLTwo}{\tbd{dropSATKuroOmissionLTwo}}
\providecommand{\dropSATKuroOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropSATKuroOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATKuroOmissionLTwoVarDecoderSamLite}{\tbd{dropSATKuroOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropSATKuroOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropSATKuroOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropSATKuroOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATKuroOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATKuroShiftLOne}{\tbd{dropSATKuroShiftLOne}}
\providecommand{\dropSATKuroShiftLTwo}{\tbd{dropSATKuroShiftLTwo}}
\providecommand{\dropSATKuroShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropSATKuroShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATKuroShiftLTwoVarDecoderSamLite}{\tbd{dropSATKuroShiftLTwoVarDecoderSamLite}}
\providecommand{\dropSATKuroShiftLTwoVarDecoderSegformerMlp}{\tbd{dropSATKuroShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropSATKuroShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATKuroShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATOemBoundaryLOne}{\tbd{dropSATOemBoundaryLOne}}
\providecommand{\dropSATOemBoundaryLTwo}{\tbd{dropSATOemBoundaryLTwo}}
\providecommand{\dropSATOemBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropSATOemBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATOemBoundaryLTwoVarDecoderSamLite}{\tbd{dropSATOemBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropSATOemBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropSATOemBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropSATOemBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATOemBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATOemCoarseLOne}{\tbd{dropSATOemCoarseLOne}}
\providecommand{\dropSATOemCoarseLTwo}{\tbd{dropSATOemCoarseLTwo}}
\providecommand{\dropSATOemCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropSATOemCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATOemCoarseLTwoVarDecoderSamLite}{\tbd{dropSATOemCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropSATOemCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropSATOemCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropSATOemCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATOemCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATOemOmissionLOne}{\tbd{dropSATOemOmissionLOne}}
\providecommand{\dropSATOemOmissionLTwo}{\tbd{dropSATOemOmissionLTwo}}
\providecommand{\dropSATOemOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropSATOemOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATOemOmissionLTwoVarDecoderSamLite}{\tbd{dropSATOemOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropSATOemOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropSATOemOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropSATOemOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATOemOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATOemShiftLOne}{\tbd{dropSATOemShiftLOne}}
\providecommand{\dropSATOemShiftLTwo}{\tbd{dropSATOemShiftLTwo}}
\providecommand{\dropSATOemShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropSATOemShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATOemShiftLTwoVarDecoderSamLite}{\tbd{dropSATOemShiftLTwoVarDecoderSamLite}}
\providecommand{\dropSATOemShiftLTwoVarDecoderSegformerMlp}{\tbd{dropSATOemShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropSATOemShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATOemShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATSnTwoBoundaryLOne}{\tbd{dropSATSnTwoBoundaryLOne}}
\providecommand{\dropSATSnTwoBoundaryLTwo}{\tbd{dropSATSnTwoBoundaryLTwo}}
\providecommand{\dropSATSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropSATSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATSnTwoBoundaryLTwoVarDecoderSamLite}{\tbd{dropSATSnTwoBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropSATSnTwoBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropSATSnTwoBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropSATSnTwoBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATSnTwoBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATSnTwoCoarseLOne}{\tbd{dropSATSnTwoCoarseLOne}}
\providecommand{\dropSATSnTwoCoarseLTwo}{\tbd{dropSATSnTwoCoarseLTwo}}
\providecommand{\dropSATSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropSATSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATSnTwoCoarseLTwoVarDecoderSamLite}{\tbd{dropSATSnTwoCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropSATSnTwoCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropSATSnTwoCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropSATSnTwoCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATSnTwoCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATSnTwoOmissionLOne}{\tbd{dropSATSnTwoOmissionLOne}}
\providecommand{\dropSATSnTwoOmissionLTwo}{\tbd{dropSATSnTwoOmissionLTwo}}
\providecommand{\dropSATSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropSATSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATSnTwoOmissionLTwoVarDecoderSamLite}{\tbd{dropSATSnTwoOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropSATSnTwoOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropSATSnTwoOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropSATSnTwoOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATSnTwoOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATSnTwoShiftLOne}{\tbd{dropSATSnTwoShiftLOne}}
\providecommand{\dropSATSnTwoShiftLTwo}{\tbd{dropSATSnTwoShiftLTwo}}
\providecommand{\dropSATSnTwoShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropSATSnTwoShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATSnTwoShiftLTwoVarDecoderSamLite}{\tbd{dropSATSnTwoShiftLTwoVarDecoderSamLite}}
\providecommand{\dropSATSnTwoShiftLTwoVarDecoderSegformerMlp}{\tbd{dropSATSnTwoShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropSATSnTwoShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATSnTwoShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATburnBoundaryLOne}{\tbd{dropSATburnBoundaryLOne}}
\providecommand{\dropSATburnBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{dropSATburnBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropSATburnBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{dropSATburnBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATburnBoundaryLOneVarDecoderSamLite}{\tbd{dropSATburnBoundaryLOneVarDecoderSamLite}}
\providecommand{\dropSATburnBoundaryLOneVarDecoderSamPretrained}{\tbd{dropSATburnBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\dropSATburnBoundaryLOneVarDecoderSegformerMlp}{\tbd{dropSATburnBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\dropSATburnBoundaryLR}{\tbd{dropSATburnBoundaryLR}}
\providecommand{\dropSATburnBoundaryLRVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATburnBoundaryLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATburnBoundaryLTwo}{\tbd{dropSATburnBoundaryLTwo}}
\providecommand{\dropSATburnBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{dropSATburnBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropSATburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{dropSATburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATburnBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropSATburnBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{dropSATburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATburnBoundaryLTwoVarDecoderSamLite}{\tbd{dropSATburnBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropSATburnBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{dropSATburnBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATburnBoundaryLTwoVarDecoderSamPretrained}{\tbd{dropSATburnBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\dropSATburnBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{dropSATburnBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATburnBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropSATburnBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropSATburnBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{dropSATburnBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATburnBoundaryLTwoVarFrozenEncoderTrue}{\tbd{dropSATburnBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\dropSATburnBoundaryLTwoVarLossBootstrap}{\tbd{dropSATburnBoundaryLTwoVarLossBootstrap}}
\providecommand{\dropSATburnBoundaryLTwoVarLossGce}{\tbd{dropSATburnBoundaryLTwoVarLossGce}}
\providecommand{\dropSATburnBoundaryLTwoVarLrMultThree}{\tbd{dropSATburnBoundaryLTwoVarLrMultThree}}
\providecommand{\dropSATburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATburnBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropSATburnBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropSATburnBoundaryLTwoVarValLabelsClean}{\tbd{dropSATburnBoundaryLTwoVarValLabelsClean}}
\providecommand{\dropSATburnCoarseLOne}{\tbd{dropSATburnCoarseLOne}}
\providecommand{\dropSATburnCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{dropSATburnCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropSATburnCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{dropSATburnCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATburnCoarseLOneVarDecoderSamLite}{\tbd{dropSATburnCoarseLOneVarDecoderSamLite}}
\providecommand{\dropSATburnCoarseLOneVarDecoderSamPretrained}{\tbd{dropSATburnCoarseLOneVarDecoderSamPretrained}}
\providecommand{\dropSATburnCoarseLOneVarDecoderSegformerMlp}{\tbd{dropSATburnCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\dropSATburnCoarseLR}{\tbd{dropSATburnCoarseLR}}
\providecommand{\dropSATburnCoarseLRVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATburnCoarseLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATburnCoarseLTwo}{\tbd{dropSATburnCoarseLTwo}}
\providecommand{\dropSATburnCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{dropSATburnCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropSATburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{dropSATburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATburnCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropSATburnCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{dropSATburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATburnCoarseLTwoVarDecoderSamLite}{\tbd{dropSATburnCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropSATburnCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{dropSATburnCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATburnCoarseLTwoVarDecoderSamPretrained}{\tbd{dropSATburnCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\dropSATburnCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{dropSATburnCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATburnCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropSATburnCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropSATburnCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{dropSATburnCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATburnCoarseLTwoVarEarlyStoppingFalse}{\tbd{dropSATburnCoarseLTwoVarEarlyStoppingFalse}}
\providecommand{\dropSATburnCoarseLTwoVarEarlyStoppingFalseFrozenEncoderTrue}{\tbd{dropSATburnCoarseLTwoVarEarlyStoppingFalseFrozenEncoderTrue}}
\providecommand{\dropSATburnCoarseLTwoVarFrozenEncoderTrue}{\tbd{dropSATburnCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\dropSATburnCoarseLTwoVarLossBootstrap}{\tbd{dropSATburnCoarseLTwoVarLossBootstrap}}
\providecommand{\dropSATburnCoarseLTwoVarLossGce}{\tbd{dropSATburnCoarseLTwoVarLossGce}}
\providecommand{\dropSATburnCoarseLTwoVarLrMultThree}{\tbd{dropSATburnCoarseLTwoVarLrMultThree}}
\providecommand{\dropSATburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATburnCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropSATburnCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropSATburnCoarseLTwoVarValLabelsClean}{\tbd{dropSATburnCoarseLTwoVarValLabelsClean}}
\providecommand{\dropSATburnOmissionLOne}{\tbd{dropSATburnOmissionLOne}}
\providecommand{\dropSATburnOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{dropSATburnOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropSATburnOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{dropSATburnOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATburnOmissionLOneVarDecoderSamLite}{\tbd{dropSATburnOmissionLOneVarDecoderSamLite}}
\providecommand{\dropSATburnOmissionLOneVarDecoderSamPretrained}{\tbd{dropSATburnOmissionLOneVarDecoderSamPretrained}}
\providecommand{\dropSATburnOmissionLOneVarDecoderSegformerMlp}{\tbd{dropSATburnOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\dropSATburnOmissionLR}{\tbd{dropSATburnOmissionLR}}
\providecommand{\dropSATburnOmissionLRVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATburnOmissionLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATburnOmissionLTwo}{\tbd{dropSATburnOmissionLTwo}}
\providecommand{\dropSATburnOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{dropSATburnOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropSATburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{dropSATburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATburnOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropSATburnOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{dropSATburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATburnOmissionLTwoVarDecoderSamLite}{\tbd{dropSATburnOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropSATburnOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{dropSATburnOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATburnOmissionLTwoVarDecoderSamPretrained}{\tbd{dropSATburnOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\dropSATburnOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{dropSATburnOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATburnOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropSATburnOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropSATburnOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{dropSATburnOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATburnOmissionLTwoVarFrozenEncoderTrue}{\tbd{dropSATburnOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\dropSATburnOmissionLTwoVarLossBootstrap}{\tbd{dropSATburnOmissionLTwoVarLossBootstrap}}
\providecommand{\dropSATburnOmissionLTwoVarLossGce}{\tbd{dropSATburnOmissionLTwoVarLossGce}}
\providecommand{\dropSATburnOmissionLTwoVarLrMultThree}{\tbd{dropSATburnOmissionLTwoVarLrMultThree}}
\providecommand{\dropSATburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATburnOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropSATburnOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropSATburnOmissionLTwoVarValLabelsClean}{\tbd{dropSATburnOmissionLTwoVarValLabelsClean}}
\providecommand{\dropSATburnShiftLOne}{\tbd{dropSATburnShiftLOne}}
\providecommand{\dropSATburnShiftLOneVarDecoderMaskTwoformerFull}{\tbd{dropSATburnShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropSATburnShiftLOneVarDecoderMaskTwoformerLite}{\tbd{dropSATburnShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATburnShiftLOneVarDecoderSamLite}{\tbd{dropSATburnShiftLOneVarDecoderSamLite}}
\providecommand{\dropSATburnShiftLOneVarDecoderSamPretrained}{\tbd{dropSATburnShiftLOneVarDecoderSamPretrained}}
\providecommand{\dropSATburnShiftLOneVarDecoderSegformerMlp}{\tbd{dropSATburnShiftLOneVarDecoderSegformerMlp}}
\providecommand{\dropSATburnShiftLR}{\tbd{dropSATburnShiftLR}}
\providecommand{\dropSATburnShiftLRVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATburnShiftLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATburnShiftLTwo}{\tbd{dropSATburnShiftLTwo}}
\providecommand{\dropSATburnShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{dropSATburnShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropSATburnShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{dropSATburnShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATburnShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropSATburnShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{dropSATburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATburnShiftLTwoVarDecoderSamLite}{\tbd{dropSATburnShiftLTwoVarDecoderSamLite}}
\providecommand{\dropSATburnShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{dropSATburnShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATburnShiftLTwoVarDecoderSamPretrained}{\tbd{dropSATburnShiftLTwoVarDecoderSamPretrained}}
\providecommand{\dropSATburnShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{dropSATburnShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATburnShiftLTwoVarDecoderSegformerMlp}{\tbd{dropSATburnShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropSATburnShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{dropSATburnShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATburnShiftLTwoVarFrozenEncoderTrue}{\tbd{dropSATburnShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\dropSATburnShiftLTwoVarLossBootstrap}{\tbd{dropSATburnShiftLTwoVarLossBootstrap}}
\providecommand{\dropSATburnShiftLTwoVarLossGce}{\tbd{dropSATburnShiftLTwoVarLossGce}}
\providecommand{\dropSATburnShiftLTwoVarLrMultThree}{\tbd{dropSATburnShiftLTwoVarLrMultThree}}
\providecommand{\dropSATburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATburnShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropSATburnShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropSATburnShiftLTwoVarValLabelsClean}{\tbd{dropSATburnShiftLTwoVarValLabelsClean}}
\providecommand{\dropSATflairBoundaryLOne}{\tbd{dropSATflairBoundaryLOne}}
\providecommand{\dropSATflairBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{dropSATflairBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropSATflairBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{dropSATflairBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATflairBoundaryLOneVarDecoderSamLite}{\tbd{dropSATflairBoundaryLOneVarDecoderSamLite}}
\providecommand{\dropSATflairBoundaryLOneVarDecoderSamPretrained}{\tbd{dropSATflairBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\dropSATflairBoundaryLOneVarDecoderSegformerMlp}{\tbd{dropSATflairBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\dropSATflairBoundaryLR}{\tbd{dropSATflairBoundaryLR}}
\providecommand{\dropSATflairBoundaryLRVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATflairBoundaryLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATflairBoundaryLTwo}{\tbd{dropSATflairBoundaryLTwo}}
\providecommand{\dropSATflairBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{dropSATflairBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropSATflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{dropSATflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATflairBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropSATflairBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{dropSATflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATflairBoundaryLTwoVarDecoderSamLite}{\tbd{dropSATflairBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropSATflairBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{dropSATflairBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATflairBoundaryLTwoVarDecoderSamPretrained}{\tbd{dropSATflairBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\dropSATflairBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{dropSATflairBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATflairBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropSATflairBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropSATflairBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{dropSATflairBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATflairBoundaryLTwoVarFrozenEncoderTrue}{\tbd{dropSATflairBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\dropSATflairBoundaryLTwoVarLossBootstrap}{\tbd{dropSATflairBoundaryLTwoVarLossBootstrap}}
\providecommand{\dropSATflairBoundaryLTwoVarLossGce}{\tbd{dropSATflairBoundaryLTwoVarLossGce}}
\providecommand{\dropSATflairBoundaryLTwoVarLrMultThree}{\tbd{dropSATflairBoundaryLTwoVarLrMultThree}}
\providecommand{\dropSATflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATflairBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropSATflairBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropSATflairBoundaryLTwoVarValLabelsClean}{\tbd{dropSATflairBoundaryLTwoVarValLabelsClean}}
\providecommand{\dropSATflairCoarseLOne}{\tbd{dropSATflairCoarseLOne}}
\providecommand{\dropSATflairCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{dropSATflairCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropSATflairCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{dropSATflairCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATflairCoarseLOneVarDecoderSamLite}{\tbd{dropSATflairCoarseLOneVarDecoderSamLite}}
\providecommand{\dropSATflairCoarseLOneVarDecoderSamPretrained}{\tbd{dropSATflairCoarseLOneVarDecoderSamPretrained}}
\providecommand{\dropSATflairCoarseLOneVarDecoderSegformerMlp}{\tbd{dropSATflairCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\dropSATflairCoarseLR}{\tbd{dropSATflairCoarseLR}}
\providecommand{\dropSATflairCoarseLRVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATflairCoarseLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATflairCoarseLTwo}{\tbd{dropSATflairCoarseLTwo}}
\providecommand{\dropSATflairCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{dropSATflairCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropSATflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{dropSATflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATflairCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropSATflairCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{dropSATflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATflairCoarseLTwoVarDecoderSamLite}{\tbd{dropSATflairCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropSATflairCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{dropSATflairCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATflairCoarseLTwoVarDecoderSamPretrained}{\tbd{dropSATflairCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\dropSATflairCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{dropSATflairCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATflairCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropSATflairCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropSATflairCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{dropSATflairCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATflairCoarseLTwoVarFrozenEncoderTrue}{\tbd{dropSATflairCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\dropSATflairCoarseLTwoVarLossBootstrap}{\tbd{dropSATflairCoarseLTwoVarLossBootstrap}}
\providecommand{\dropSATflairCoarseLTwoVarLossGce}{\tbd{dropSATflairCoarseLTwoVarLossGce}}
\providecommand{\dropSATflairCoarseLTwoVarLrMultThree}{\tbd{dropSATflairCoarseLTwoVarLrMultThree}}
\providecommand{\dropSATflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATflairCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropSATflairCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropSATflairCoarseLTwoVarValLabelsClean}{\tbd{dropSATflairCoarseLTwoVarValLabelsClean}}
\providecommand{\dropSATflairOmissionLOne}{\tbd{dropSATflairOmissionLOne}}
\providecommand{\dropSATflairOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{dropSATflairOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropSATflairOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{dropSATflairOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATflairOmissionLOneVarDecoderSamLite}{\tbd{dropSATflairOmissionLOneVarDecoderSamLite}}
\providecommand{\dropSATflairOmissionLOneVarDecoderSamPretrained}{\tbd{dropSATflairOmissionLOneVarDecoderSamPretrained}}
\providecommand{\dropSATflairOmissionLOneVarDecoderSegformerMlp}{\tbd{dropSATflairOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\dropSATflairOmissionLR}{\tbd{dropSATflairOmissionLR}}
\providecommand{\dropSATflairOmissionLRVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATflairOmissionLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATflairOmissionLTwo}{\tbd{dropSATflairOmissionLTwo}}
\providecommand{\dropSATflairOmissionLTwoVarClassWeightedTrue}{\tbd{dropSATflairOmissionLTwoVarClassWeightedTrue}}
\providecommand{\dropSATflairOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{dropSATflairOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropSATflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{dropSATflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATflairOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropSATflairOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{dropSATflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATflairOmissionLTwoVarDecoderSamLite}{\tbd{dropSATflairOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropSATflairOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{dropSATflairOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATflairOmissionLTwoVarDecoderSamPretrained}{\tbd{dropSATflairOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\dropSATflairOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{dropSATflairOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATflairOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropSATflairOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropSATflairOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{dropSATflairOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATflairOmissionLTwoVarEarlyStoppingFalse}{\tbd{dropSATflairOmissionLTwoVarEarlyStoppingFalse}}
\providecommand{\dropSATflairOmissionLTwoVarEarlyStoppingFalseFrozenEncoderTrue}{\tbd{dropSATflairOmissionLTwoVarEarlyStoppingFalseFrozenEncoderTrue}}
\providecommand{\dropSATflairOmissionLTwoVarFrozenEncoderTrue}{\tbd{dropSATflairOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\dropSATflairOmissionLTwoVarLossBootstrap}{\tbd{dropSATflairOmissionLTwoVarLossBootstrap}}
\providecommand{\dropSATflairOmissionLTwoVarLossGce}{\tbd{dropSATflairOmissionLTwoVarLossGce}}
\providecommand{\dropSATflairOmissionLTwoVarLrMultThree}{\tbd{dropSATflairOmissionLTwoVarLrMultThree}}
\providecommand{\dropSATflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATflairOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropSATflairOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropSATflairOmissionLTwoVarValLabelsClean}{\tbd{dropSATflairOmissionLTwoVarValLabelsClean}}
\providecommand{\dropSATflairShiftLOne}{\tbd{dropSATflairShiftLOne}}
\providecommand{\dropSATflairShiftLOneVarDecoderMaskTwoformerFull}{\tbd{dropSATflairShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropSATflairShiftLOneVarDecoderMaskTwoformerLite}{\tbd{dropSATflairShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATflairShiftLOneVarDecoderSamLite}{\tbd{dropSATflairShiftLOneVarDecoderSamLite}}
\providecommand{\dropSATflairShiftLOneVarDecoderSamPretrained}{\tbd{dropSATflairShiftLOneVarDecoderSamPretrained}}
\providecommand{\dropSATflairShiftLOneVarDecoderSegformerMlp}{\tbd{dropSATflairShiftLOneVarDecoderSegformerMlp}}
\providecommand{\dropSATflairShiftLR}{\tbd{dropSATflairShiftLR}}
\providecommand{\dropSATflairShiftLRVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATflairShiftLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATflairShiftLTwo}{\tbd{dropSATflairShiftLTwo}}
\providecommand{\dropSATflairShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{dropSATflairShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropSATflairShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{dropSATflairShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATflairShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropSATflairShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropSATflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{dropSATflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATflairShiftLTwoVarDecoderSamLite}{\tbd{dropSATflairShiftLTwoVarDecoderSamLite}}
\providecommand{\dropSATflairShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{dropSATflairShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATflairShiftLTwoVarDecoderSamPretrained}{\tbd{dropSATflairShiftLTwoVarDecoderSamPretrained}}
\providecommand{\dropSATflairShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{dropSATflairShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATflairShiftLTwoVarDecoderSegformerMlp}{\tbd{dropSATflairShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropSATflairShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{dropSATflairShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATflairShiftLTwoVarFrozenEncoderTrue}{\tbd{dropSATflairShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\dropSATflairShiftLTwoVarLossBootstrap}{\tbd{dropSATflairShiftLTwoVarLossBootstrap}}
\providecommand{\dropSATflairShiftLTwoVarLossGce}{\tbd{dropSATflairShiftLTwoVarLossGce}}
\providecommand{\dropSATflairShiftLTwoVarLrMultThree}{\tbd{dropSATflairShiftLTwoVarLrMultThree}}
\providecommand{\dropSATflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropSATflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropSATflairShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropSATflairShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropSATflairShiftLTwoVarValLabelsClean}{\tbd{dropSATflairShiftLTwoVarValLabelsClean}}
\providecommand{\dropSATsenOtsuLTwo}{\tbd{dropSATsenOtsuLTwo}}
\providecommand{\dropTMChesBoundaryLOne}{\tbd{dropTMChesBoundaryLOne}}
\providecommand{\dropTMChesBoundaryLTwo}{\tbd{dropTMChesBoundaryLTwo}}
\providecommand{\dropTMChesCoarseLOne}{\tbd{dropTMChesCoarseLOne}}
\providecommand{\dropTMChesCoarseLTwo}{\tbd{dropTMChesCoarseLTwo}}
\providecommand{\dropTMChesNlcdREAL}{\tbd{dropTMChesNlcdREAL}}
\providecommand{\dropTMChesOmissionLOne}{\tbd{dropTMChesOmissionLOne}}
\providecommand{\dropTMChesOmissionLTwo}{\tbd{dropTMChesOmissionLTwo}}
\providecommand{\dropTMChesShiftLOne}{\tbd{dropTMChesShiftLOne}}
\providecommand{\dropTMChesShiftLTwo}{\tbd{dropTMChesShiftLTwo}}
\providecommand{\dropTMCsTwelveBoundaryLOne}{\tbd{dropTMCsTwelveBoundaryLOne}}
\providecommand{\dropTMCsTwelveBoundaryLTwo}{\tbd{dropTMCsTwelveBoundaryLTwo}}
\providecommand{\dropTMCsTwelveCoarseLOne}{\tbd{dropTMCsTwelveCoarseLOne}}
\providecommand{\dropTMCsTwelveCoarseLTwo}{\tbd{dropTMCsTwelveCoarseLTwo}}
\providecommand{\dropTMCsTwelveOmissionLOne}{\tbd{dropTMCsTwelveOmissionLOne}}
\providecommand{\dropTMCsTwelveOmissionLTwo}{\tbd{dropTMCsTwelveOmissionLTwo}}
\providecommand{\dropTMCsTwelveSTwocloudlessREAL}{\tbd{dropTMCsTwelveSTwocloudlessREAL}}
\providecommand{\dropTMCsTwelveShiftLOne}{\tbd{dropTMCsTwelveShiftLOne}}
\providecommand{\dropTMCsTwelveShiftLTwo}{\tbd{dropTMCsTwelveShiftLTwo}}
\providecommand{\dropTMDfcBoundaryLOne}{\tbd{dropTMDfcBoundaryLOne}}
\providecommand{\dropTMDfcBoundaryLTwo}{\tbd{dropTMDfcBoundaryLTwo}}
\providecommand{\dropTMDfcCoarseLOne}{\tbd{dropTMDfcCoarseLOne}}
\providecommand{\dropTMDfcCoarseLTwo}{\tbd{dropTMDfcCoarseLTwo}}
\providecommand{\dropTMDfcModisREALVarTrainSubsetRealcov}{\tbd{dropTMDfcModisREALVarTrainSubsetRealcov}}
\providecommand{\dropTMDfcOmissionLOne}{\tbd{dropTMDfcOmissionLOne}}
\providecommand{\dropTMDfcOmissionLTwo}{\tbd{dropTMDfcOmissionLTwo}}
\providecommand{\dropTMDfcShiftLOne}{\tbd{dropTMDfcShiftLOne}}
\providecommand{\dropTMDfcShiftLTwo}{\tbd{dropTMDfcShiftLTwo}}
\providecommand{\dropTMEnvaBoundaryLOne}{\tbd{dropTMEnvaBoundaryLOne}}
\providecommand{\dropTMEnvaBoundaryLTwo}{\tbd{dropTMEnvaBoundaryLTwo}}
\providecommand{\dropTMEnvaCoarseLOne}{\tbd{dropTMEnvaCoarseLOne}}
\providecommand{\dropTMEnvaCoarseLTwo}{\tbd{dropTMEnvaCoarseLTwo}}
\providecommand{\dropTMEnvaNlcdREAL}{\tbd{dropTMEnvaNlcdREAL}}
\providecommand{\dropTMEnvaOmissionLOne}{\tbd{dropTMEnvaOmissionLOne}}
\providecommand{\dropTMEnvaOmissionLTwo}{\tbd{dropTMEnvaOmissionLTwo}}
\providecommand{\dropTMEnvaShiftLOne}{\tbd{dropTMEnvaShiftLOne}}
\providecommand{\dropTMEnvaShiftLTwo}{\tbd{dropTMEnvaShiftLTwo}}
\providecommand{\dropTMKuroBoundaryLOne}{\tbd{dropTMKuroBoundaryLOne}}
\providecommand{\dropTMKuroBoundaryLTwo}{\tbd{dropTMKuroBoundaryLTwo}}
\providecommand{\dropTMKuroCemsREALVarTrainSubsetRealcov}{\tbd{dropTMKuroCemsREALVarTrainSubsetRealcov}}
\providecommand{\dropTMKuroCoarseLOne}{\tbd{dropTMKuroCoarseLOne}}
\providecommand{\dropTMKuroCoarseLTwo}{\tbd{dropTMKuroCoarseLTwo}}
\providecommand{\dropTMKuroOmissionLOne}{\tbd{dropTMKuroOmissionLOne}}
\providecommand{\dropTMKuroOmissionLTwo}{\tbd{dropTMKuroOmissionLTwo}}
\providecommand{\dropTMKuroShiftLOne}{\tbd{dropTMKuroShiftLOne}}
\providecommand{\dropTMKuroShiftLTwo}{\tbd{dropTMKuroShiftLTwo}}
\providecommand{\dropTMOemBoundaryLOne}{\tbd{dropTMOemBoundaryLOne}}
\providecommand{\dropTMOemBoundaryLTwo}{\tbd{dropTMOemBoundaryLTwo}}
\providecommand{\dropTMOemCoarseLOne}{\tbd{dropTMOemCoarseLOne}}
\providecommand{\dropTMOemCoarseLTwo}{\tbd{dropTMOemCoarseLTwo}}
\providecommand{\dropTMOemOmissionLOne}{\tbd{dropTMOemOmissionLOne}}
\providecommand{\dropTMOemOmissionLTwo}{\tbd{dropTMOemOmissionLTwo}}
\providecommand{\dropTMOemShiftLOne}{\tbd{dropTMOemShiftLOne}}
\providecommand{\dropTMOemShiftLTwo}{\tbd{dropTMOemShiftLTwo}}
\providecommand{\dropTMSnTwoBoundaryLOne}{\tbd{dropTMSnTwoBoundaryLOne}}
\providecommand{\dropTMSnTwoBoundaryLTwo}{\tbd{dropTMSnTwoBoundaryLTwo}}
\providecommand{\dropTMSnTwoCoarseLOne}{\tbd{dropTMSnTwoCoarseLOne}}
\providecommand{\dropTMSnTwoCoarseLTwo}{\tbd{dropTMSnTwoCoarseLTwo}}
\providecommand{\dropTMSnTwoOmissionLOne}{\tbd{dropTMSnTwoOmissionLOne}}
\providecommand{\dropTMSnTwoOmissionLTwo}{\tbd{dropTMSnTwoOmissionLTwo}}
\providecommand{\dropTMSnTwoShiftLOne}{\tbd{dropTMSnTwoShiftLOne}}
\providecommand{\dropTMSnTwoShiftLTwo}{\tbd{dropTMSnTwoShiftLTwo}}
\providecommand{\dropTMburnBoundaryLOne}{\tbd{dropTMburnBoundaryLOne}}
\providecommand{\dropTMburnBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{dropTMburnBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropTMburnBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{dropTMburnBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropTMburnBoundaryLOneVarDecoderSamLite}{\tbd{dropTMburnBoundaryLOneVarDecoderSamLite}}
\providecommand{\dropTMburnBoundaryLOneVarDecoderSamPretrained}{\tbd{dropTMburnBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\dropTMburnBoundaryLOneVarDecoderSegformerMlp}{\tbd{dropTMburnBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\dropTMburnBoundaryLR}{\tbd{dropTMburnBoundaryLR}}
\providecommand{\dropTMburnBoundaryLTwo}{\tbd{dropTMburnBoundaryLTwo}}
\providecommand{\dropTMburnBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{dropTMburnBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropTMburnBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropTMburnBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropTMburnBoundaryLTwoVarDecoderSamLite}{\tbd{dropTMburnBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropTMburnBoundaryLTwoVarDecoderSamPretrained}{\tbd{dropTMburnBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\dropTMburnBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropTMburnBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropTMburnBoundaryLTwoVarFrozenEncoderTrue}{\tbd{dropTMburnBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\dropTMburnBoundaryLTwoVarLossBootstrap}{\tbd{dropTMburnBoundaryLTwoVarLossBootstrap}}
\providecommand{\dropTMburnBoundaryLTwoVarLossGce}{\tbd{dropTMburnBoundaryLTwoVarLossGce}}
\providecommand{\dropTMburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropTMburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropTMburnBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropTMburnBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropTMburnCoarseLOne}{\tbd{dropTMburnCoarseLOne}}
\providecommand{\dropTMburnCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{dropTMburnCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropTMburnCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{dropTMburnCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropTMburnCoarseLOneVarDecoderSamLite}{\tbd{dropTMburnCoarseLOneVarDecoderSamLite}}
\providecommand{\dropTMburnCoarseLOneVarDecoderSamPretrained}{\tbd{dropTMburnCoarseLOneVarDecoderSamPretrained}}
\providecommand{\dropTMburnCoarseLOneVarDecoderSegformerMlp}{\tbd{dropTMburnCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\dropTMburnCoarseLR}{\tbd{dropTMburnCoarseLR}}
\providecommand{\dropTMburnCoarseLTwo}{\tbd{dropTMburnCoarseLTwo}}
\providecommand{\dropTMburnCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{dropTMburnCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropTMburnCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropTMburnCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropTMburnCoarseLTwoVarDecoderSamLite}{\tbd{dropTMburnCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropTMburnCoarseLTwoVarDecoderSamPretrained}{\tbd{dropTMburnCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\dropTMburnCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropTMburnCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropTMburnCoarseLTwoVarFrozenEncoderTrue}{\tbd{dropTMburnCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\dropTMburnCoarseLTwoVarLossBootstrap}{\tbd{dropTMburnCoarseLTwoVarLossBootstrap}}
\providecommand{\dropTMburnCoarseLTwoVarLossGce}{\tbd{dropTMburnCoarseLTwoVarLossGce}}
\providecommand{\dropTMburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropTMburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropTMburnCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropTMburnCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropTMburnOmissionLOne}{\tbd{dropTMburnOmissionLOne}}
\providecommand{\dropTMburnOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{dropTMburnOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropTMburnOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{dropTMburnOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropTMburnOmissionLOneVarDecoderSamLite}{\tbd{dropTMburnOmissionLOneVarDecoderSamLite}}
\providecommand{\dropTMburnOmissionLOneVarDecoderSamPretrained}{\tbd{dropTMburnOmissionLOneVarDecoderSamPretrained}}
\providecommand{\dropTMburnOmissionLOneVarDecoderSegformerMlp}{\tbd{dropTMburnOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\dropTMburnOmissionLR}{\tbd{dropTMburnOmissionLR}}
\providecommand{\dropTMburnOmissionLTwo}{\tbd{dropTMburnOmissionLTwo}}
\providecommand{\dropTMburnOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{dropTMburnOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropTMburnOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropTMburnOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropTMburnOmissionLTwoVarDecoderSamLite}{\tbd{dropTMburnOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropTMburnOmissionLTwoVarDecoderSamPretrained}{\tbd{dropTMburnOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\dropTMburnOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropTMburnOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropTMburnOmissionLTwoVarFrozenEncoderTrue}{\tbd{dropTMburnOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\dropTMburnOmissionLTwoVarLossBootstrap}{\tbd{dropTMburnOmissionLTwoVarLossBootstrap}}
\providecommand{\dropTMburnOmissionLTwoVarLossGce}{\tbd{dropTMburnOmissionLTwoVarLossGce}}
\providecommand{\dropTMburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropTMburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropTMburnOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropTMburnOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropTMburnShiftLOne}{\tbd{dropTMburnShiftLOne}}
\providecommand{\dropTMburnShiftLOneVarDecoderMaskTwoformerFull}{\tbd{dropTMburnShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropTMburnShiftLOneVarDecoderMaskTwoformerLite}{\tbd{dropTMburnShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropTMburnShiftLOneVarDecoderSamLite}{\tbd{dropTMburnShiftLOneVarDecoderSamLite}}
\providecommand{\dropTMburnShiftLOneVarDecoderSamPretrained}{\tbd{dropTMburnShiftLOneVarDecoderSamPretrained}}
\providecommand{\dropTMburnShiftLOneVarDecoderSegformerMlp}{\tbd{dropTMburnShiftLOneVarDecoderSegformerMlp}}
\providecommand{\dropTMburnShiftLR}{\tbd{dropTMburnShiftLR}}
\providecommand{\dropTMburnShiftLTwo}{\tbd{dropTMburnShiftLTwo}}
\providecommand{\dropTMburnShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{dropTMburnShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropTMburnShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropTMburnShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropTMburnShiftLTwoVarDecoderSamLite}{\tbd{dropTMburnShiftLTwoVarDecoderSamLite}}
\providecommand{\dropTMburnShiftLTwoVarDecoderSamPretrained}{\tbd{dropTMburnShiftLTwoVarDecoderSamPretrained}}
\providecommand{\dropTMburnShiftLTwoVarDecoderSegformerMlp}{\tbd{dropTMburnShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropTMburnShiftLTwoVarFrozenEncoderTrue}{\tbd{dropTMburnShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\dropTMburnShiftLTwoVarLossBootstrap}{\tbd{dropTMburnShiftLTwoVarLossBootstrap}}
\providecommand{\dropTMburnShiftLTwoVarLossGce}{\tbd{dropTMburnShiftLTwoVarLossGce}}
\providecommand{\dropTMburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropTMburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropTMburnShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropTMburnShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropTMflairBoundaryLOne}{\tbd{dropTMflairBoundaryLOne}}
\providecommand{\dropTMflairBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{dropTMflairBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropTMflairBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{dropTMflairBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropTMflairBoundaryLOneVarDecoderSamLite}{\tbd{dropTMflairBoundaryLOneVarDecoderSamLite}}
\providecommand{\dropTMflairBoundaryLOneVarDecoderSamPretrained}{\tbd{dropTMflairBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\dropTMflairBoundaryLOneVarDecoderSegformerMlp}{\tbd{dropTMflairBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\dropTMflairBoundaryLR}{\tbd{dropTMflairBoundaryLR}}
\providecommand{\dropTMflairBoundaryLTwo}{\tbd{dropTMflairBoundaryLTwo}}
\providecommand{\dropTMflairBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{dropTMflairBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropTMflairBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{dropTMflairBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropTMflairBoundaryLTwoVarDecoderSamLite}{\tbd{dropTMflairBoundaryLTwoVarDecoderSamLite}}
\providecommand{\dropTMflairBoundaryLTwoVarDecoderSamPretrained}{\tbd{dropTMflairBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\dropTMflairBoundaryLTwoVarDecoderSegformerMlp}{\tbd{dropTMflairBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\dropTMflairBoundaryLTwoVarFrozenEncoderTrue}{\tbd{dropTMflairBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\dropTMflairBoundaryLTwoVarLossBootstrap}{\tbd{dropTMflairBoundaryLTwoVarLossBootstrap}}
\providecommand{\dropTMflairBoundaryLTwoVarLossGce}{\tbd{dropTMflairBoundaryLTwoVarLossGce}}
\providecommand{\dropTMflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropTMflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropTMflairBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropTMflairBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropTMflairCoarseLOne}{\tbd{dropTMflairCoarseLOne}}
\providecommand{\dropTMflairCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{dropTMflairCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropTMflairCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{dropTMflairCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropTMflairCoarseLOneVarDecoderSamLite}{\tbd{dropTMflairCoarseLOneVarDecoderSamLite}}
\providecommand{\dropTMflairCoarseLOneVarDecoderSamPretrained}{\tbd{dropTMflairCoarseLOneVarDecoderSamPretrained}}
\providecommand{\dropTMflairCoarseLOneVarDecoderSegformerMlp}{\tbd{dropTMflairCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\dropTMflairCoarseLR}{\tbd{dropTMflairCoarseLR}}
\providecommand{\dropTMflairCoarseLTwo}{\tbd{dropTMflairCoarseLTwo}}
\providecommand{\dropTMflairCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{dropTMflairCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropTMflairCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{dropTMflairCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropTMflairCoarseLTwoVarDecoderSamLite}{\tbd{dropTMflairCoarseLTwoVarDecoderSamLite}}
\providecommand{\dropTMflairCoarseLTwoVarDecoderSamPretrained}{\tbd{dropTMflairCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\dropTMflairCoarseLTwoVarDecoderSegformerMlp}{\tbd{dropTMflairCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\dropTMflairCoarseLTwoVarFrozenEncoderTrue}{\tbd{dropTMflairCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\dropTMflairCoarseLTwoVarLossBootstrap}{\tbd{dropTMflairCoarseLTwoVarLossBootstrap}}
\providecommand{\dropTMflairCoarseLTwoVarLossGce}{\tbd{dropTMflairCoarseLTwoVarLossGce}}
\providecommand{\dropTMflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropTMflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropTMflairCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropTMflairCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropTMflairOmissionLOne}{\tbd{dropTMflairOmissionLOne}}
\providecommand{\dropTMflairOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{dropTMflairOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropTMflairOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{dropTMflairOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropTMflairOmissionLOneVarDecoderSamLite}{\tbd{dropTMflairOmissionLOneVarDecoderSamLite}}
\providecommand{\dropTMflairOmissionLOneVarDecoderSamPretrained}{\tbd{dropTMflairOmissionLOneVarDecoderSamPretrained}}
\providecommand{\dropTMflairOmissionLOneVarDecoderSegformerMlp}{\tbd{dropTMflairOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\dropTMflairOmissionLR}{\tbd{dropTMflairOmissionLR}}
\providecommand{\dropTMflairOmissionLTwo}{\tbd{dropTMflairOmissionLTwo}}
\providecommand{\dropTMflairOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{dropTMflairOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropTMflairOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{dropTMflairOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropTMflairOmissionLTwoVarDecoderSamLite}{\tbd{dropTMflairOmissionLTwoVarDecoderSamLite}}
\providecommand{\dropTMflairOmissionLTwoVarDecoderSamPretrained}{\tbd{dropTMflairOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\dropTMflairOmissionLTwoVarDecoderSegformerMlp}{\tbd{dropTMflairOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\dropTMflairOmissionLTwoVarFrozenEncoderTrue}{\tbd{dropTMflairOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\dropTMflairOmissionLTwoVarLossBootstrap}{\tbd{dropTMflairOmissionLTwoVarLossBootstrap}}
\providecommand{\dropTMflairOmissionLTwoVarLossGce}{\tbd{dropTMflairOmissionLTwoVarLossGce}}
\providecommand{\dropTMflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropTMflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropTMflairOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropTMflairOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropTMflairShiftLOne}{\tbd{dropTMflairShiftLOne}}
\providecommand{\dropTMflairShiftLOneVarDecoderMaskTwoformerFull}{\tbd{dropTMflairShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\dropTMflairShiftLOneVarDecoderMaskTwoformerLite}{\tbd{dropTMflairShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\dropTMflairShiftLOneVarDecoderSamLite}{\tbd{dropTMflairShiftLOneVarDecoderSamLite}}
\providecommand{\dropTMflairShiftLOneVarDecoderSamPretrained}{\tbd{dropTMflairShiftLOneVarDecoderSamPretrained}}
\providecommand{\dropTMflairShiftLOneVarDecoderSegformerMlp}{\tbd{dropTMflairShiftLOneVarDecoderSegformerMlp}}
\providecommand{\dropTMflairShiftLR}{\tbd{dropTMflairShiftLR}}
\providecommand{\dropTMflairShiftLTwo}{\tbd{dropTMflairShiftLTwo}}
\providecommand{\dropTMflairShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{dropTMflairShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\dropTMflairShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{dropTMflairShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\dropTMflairShiftLTwoVarDecoderSamLite}{\tbd{dropTMflairShiftLTwoVarDecoderSamLite}}
\providecommand{\dropTMflairShiftLTwoVarDecoderSamPretrained}{\tbd{dropTMflairShiftLTwoVarDecoderSamPretrained}}
\providecommand{\dropTMflairShiftLTwoVarDecoderSegformerMlp}{\tbd{dropTMflairShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\dropTMflairShiftLTwoVarFrozenEncoderTrue}{\tbd{dropTMflairShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\dropTMflairShiftLTwoVarLossBootstrap}{\tbd{dropTMflairShiftLTwoVarLossBootstrap}}
\providecommand{\dropTMflairShiftLTwoVarLossGce}{\tbd{dropTMflairShiftLTwoVarLossGce}}
\providecommand{\dropTMflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{dropTMflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\dropTMflairShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{dropTMflairShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\dropTMsenOtsuLTwo}{\tbd{dropTMsenOtsuLTwo}}
\providecommand{\dropVitlRandomburnBoundaryLOneVarInitRandom}{\tbd{dropVitlRandomburnBoundaryLOneVarInitRandom}}
\providecommand{\dropVitlRandomburnBoundaryLTwoVarInitRandom}{\tbd{dropVitlRandomburnBoundaryLTwoVarInitRandom}}
\providecommand{\dropVitlRandomburnCoarseLOneVarInitRandom}{\tbd{dropVitlRandomburnCoarseLOneVarInitRandom}}
\providecommand{\dropVitlRandomburnCoarseLTwoVarInitRandom}{\tbd{dropVitlRandomburnCoarseLTwoVarInitRandom}}
\providecommand{\dropVitlRandomburnOmissionLOneVarInitRandom}{\tbd{dropVitlRandomburnOmissionLOneVarInitRandom}}
\providecommand{\dropVitlRandomburnOmissionLTwoVarInitRandom}{\tbd{dropVitlRandomburnOmissionLTwoVarInitRandom}}
\providecommand{\dropVitlRandomburnShiftLOneVarInitRandom}{\tbd{dropVitlRandomburnShiftLOneVarInitRandom}}
\providecommand{\dropVitlRandomburnShiftLTwoVarInitRandom}{\tbd{dropVitlRandomburnShiftLTwoVarInitRandom}}
\providecommand{\dropVitlRandomflairBoundaryLOneVarInitRandom}{\tbd{dropVitlRandomflairBoundaryLOneVarInitRandom}}
\providecommand{\dropVitlRandomflairBoundaryLTwoVarInitRandom}{\tbd{dropVitlRandomflairBoundaryLTwoVarInitRandom}}
\providecommand{\dropVitlRandomflairCoarseLOneVarInitRandom}{\tbd{dropVitlRandomflairCoarseLOneVarInitRandom}}
\providecommand{\dropVitlRandomflairCoarseLTwoVarInitRandom}{\tbd{dropVitlRandomflairCoarseLTwoVarInitRandom}}
\providecommand{\dropVitlRandomflairOmissionLOneVarInitRandom}{\tbd{dropVitlRandomflairOmissionLOneVarInitRandom}}
\providecommand{\dropVitlRandomflairOmissionLTwoVarInitRandom}{\tbd{dropVitlRandomflairOmissionLTwoVarInitRandom}}
\providecommand{\dropVitlRandomflairShiftLOneVarInitRandom}{\tbd{dropVitlRandomflairShiftLOneVarInitRandom}}
\providecommand{\dropVitlRandomflairShiftLTwoVarInitRandom}{\tbd{dropVitlRandomflairShiftLTwoVarInitRandom}}
\providecommand{\hlAblContrastAFiveburnCIHi}{\tbd{hlAblContrastAFiveburnCIHi}}
\providecommand{\hlAblContrastAFiveburnCILo}{\tbd{hlAblContrastAFiveburnCILo}}
\providecommand{\hlAblContrastAFiveburnEst}{\tbd{hlAblContrastAFiveburnEst}}
\providecommand{\hlAblContrastAFiveburnN}{\tbd{hlAblContrastAFiveburnN}}
\providecommand{\hlAblContrastAFiveflairCIHi}{\tbd{hlAblContrastAFiveflairCIHi}}
\providecommand{\hlAblContrastAFiveflairCILo}{\tbd{hlAblContrastAFiveflairCILo}}
\providecommand{\hlAblContrastAFiveflairEst}{\tbd{hlAblContrastAFiveflairEst}}
\providecommand{\hlAblContrastAFiveflairN}{\tbd{hlAblContrastAFiveflairN}}
\providecommand{\hlAblContrastAFourburnCIHi}{\tbd{hlAblContrastAFourburnCIHi}}
\providecommand{\hlAblContrastAFourburnCILo}{\tbd{hlAblContrastAFourburnCILo}}
\providecommand{\hlAblContrastAFourburnEst}{\tbd{hlAblContrastAFourburnEst}}
\providecommand{\hlAblContrastAFourburnN}{\tbd{hlAblContrastAFourburnN}}
\providecommand{\hlAblContrastAFourflairCIHi}{\tbd{hlAblContrastAFourflairCIHi}}
\providecommand{\hlAblContrastAFourflairCILo}{\tbd{hlAblContrastAFourflairCILo}}
\providecommand{\hlAblContrastAFourflairEst}{\tbd{hlAblContrastAFourflairEst}}
\providecommand{\hlAblContrastAFourflairN}{\tbd{hlAblContrastAFourflairN}}
\providecommand{\hlAblContrastASixburnCIHi}{\tbd{hlAblContrastASixburnCIHi}}
\providecommand{\hlAblContrastASixburnCILo}{\tbd{hlAblContrastASixburnCILo}}
\providecommand{\hlAblContrastASixburnEst}{\tbd{hlAblContrastASixburnEst}}
\providecommand{\hlAblContrastASixburnN}{\tbd{hlAblContrastASixburnN}}
\providecommand{\hlAblContrastASixflairCIHi}{\tbd{hlAblContrastASixflairCIHi}}
\providecommand{\hlAblContrastASixflairCILo}{\tbd{hlAblContrastASixflairCILo}}
\providecommand{\hlAblContrastASixflairEst}{\tbd{hlAblContrastASixflairEst}}
\providecommand{\hlAblContrastASixflairN}{\tbd{hlAblContrastASixflairN}}
\providecommand{\hlAblContrastAThreeburnCIHi}{\tbd{hlAblContrastAThreeburnCIHi}}
\providecommand{\hlAblContrastAThreeburnCILo}{\tbd{hlAblContrastAThreeburnCILo}}
\providecommand{\hlAblContrastAThreeburnEst}{\tbd{hlAblContrastAThreeburnEst}}
\providecommand{\hlAblContrastAThreeburnN}{\tbd{hlAblContrastAThreeburnN}}
\providecommand{\hlAblContrastAThreeflairCIHi}{\tbd{hlAblContrastAThreeflairCIHi}}
\providecommand{\hlAblContrastAThreeflairCILo}{\tbd{hlAblContrastAThreeflairCILo}}
\providecommand{\hlAblContrastAThreeflairEst}{\tbd{hlAblContrastAThreeflairEst}}
\providecommand{\hlAblContrastAThreeflairN}{\tbd{hlAblContrastAThreeflairN}}
\providecommand{\hlAblContrastNSixburnCIHi}{\tbd{hlAblContrastNSixburnCIHi}}
\providecommand{\hlAblContrastNSixburnCILo}{\tbd{hlAblContrastNSixburnCILo}}
\providecommand{\hlAblContrastNSixburnEst}{\tbd{hlAblContrastNSixburnEst}}
\providecommand{\hlAblContrastNSixburnN}{\tbd{hlAblContrastNSixburnN}}
\providecommand{\hlAblContrastNSixflairCIHi}{\tbd{hlAblContrastNSixflairCIHi}}
\providecommand{\hlAblContrastNSixflairCILo}{\tbd{hlAblContrastNSixflairCILo}}
\providecommand{\hlAblContrastNSixflairEst}{\tbd{hlAblContrastNSixflairEst}}
\providecommand{\hlAblContrastNSixflairN}{\tbd{hlAblContrastNSixflairN}}
\providecommand{\hlBdropGapBoundaryNarrowburn}{\tbd{hlBdropGapBoundaryNarrowburn}}
\providecommand{\hlBdropGapBoundaryNarrowburnCIHi}{\tbd{hlBdropGapBoundaryNarrowburnCIHi}}
\providecommand{\hlBdropGapBoundaryNarrowburnCILo}{\tbd{hlBdropGapBoundaryNarrowburnCILo}}
\providecommand{\hlBdropGapBoundaryNarrowburnN}{\tbd{hlBdropGapBoundaryNarrowburnN}}
\providecommand{\hlBdropGapBoundaryNarrowflair}{\tbd{hlBdropGapBoundaryNarrowflair}}
\providecommand{\hlBdropGapBoundaryNarrowflairCIHi}{\tbd{hlBdropGapBoundaryNarrowflairCIHi}}
\providecommand{\hlBdropGapBoundaryNarrowflairCILo}{\tbd{hlBdropGapBoundaryNarrowflairCILo}}
\providecommand{\hlBdropGapBoundaryNarrowflairN}{\tbd{hlBdropGapBoundaryNarrowflairN}}
\providecommand{\hlBdropGapBoundaryWideburn}{\tbd{hlBdropGapBoundaryWideburn}}
\providecommand{\hlBdropGapBoundaryWideburnCIHi}{\tbd{hlBdropGapBoundaryWideburnCIHi}}
\providecommand{\hlBdropGapBoundaryWideburnCILo}{\tbd{hlBdropGapBoundaryWideburnCILo}}
\providecommand{\hlBdropGapBoundaryWideburnN}{\tbd{hlBdropGapBoundaryWideburnN}}
\providecommand{\hlBdropGapBoundaryWideflair}{\tbd{hlBdropGapBoundaryWideflair}}
\providecommand{\hlBdropGapBoundaryWideflairCIHi}{\tbd{hlBdropGapBoundaryWideflairCIHi}}
\providecommand{\hlBdropGapBoundaryWideflairCILo}{\tbd{hlBdropGapBoundaryWideflairCILo}}
\providecommand{\hlBdropGapBoundaryWideflairN}{\tbd{hlBdropGapBoundaryWideflairN}}
\providecommand{\hlBdropGapOmissionNarrowburn}{\tbd{hlBdropGapOmissionNarrowburn}}
\providecommand{\hlBdropGapOmissionNarrowburnCIHi}{\tbd{hlBdropGapOmissionNarrowburnCIHi}}
\providecommand{\hlBdropGapOmissionNarrowburnCILo}{\tbd{hlBdropGapOmissionNarrowburnCILo}}
\providecommand{\hlBdropGapOmissionNarrowburnN}{\tbd{hlBdropGapOmissionNarrowburnN}}
\providecommand{\hlBdropGapOmissionNarrowflair}{\tbd{hlBdropGapOmissionNarrowflair}}
\providecommand{\hlBdropGapOmissionNarrowflairCIHi}{\tbd{hlBdropGapOmissionNarrowflairCIHi}}
\providecommand{\hlBdropGapOmissionNarrowflairCILo}{\tbd{hlBdropGapOmissionNarrowflairCILo}}
\providecommand{\hlBdropGapOmissionNarrowflairN}{\tbd{hlBdropGapOmissionNarrowflairN}}
\providecommand{\hlBdropGapOmissionWideburn}{\tbd{hlBdropGapOmissionWideburn}}
\providecommand{\hlBdropGapOmissionWideburnCIHi}{\tbd{hlBdropGapOmissionWideburnCIHi}}
\providecommand{\hlBdropGapOmissionWideburnCILo}{\tbd{hlBdropGapOmissionWideburnCILo}}
\providecommand{\hlBdropGapOmissionWideburnN}{\tbd{hlBdropGapOmissionWideburnN}}
\providecommand{\hlBdropGapOmissionWideflair}{\tbd{hlBdropGapOmissionWideflair}}
\providecommand{\hlBdropGapOmissionWideflairCIHi}{\tbd{hlBdropGapOmissionWideflairCIHi}}
\providecommand{\hlBdropGapOmissionWideflairCILo}{\tbd{hlBdropGapOmissionWideflairCILo}}
\providecommand{\hlBdropGapOmissionWideflairN}{\tbd{hlBdropGapOmissionWideflairN}}
\providecommand{\hlBdropGapShiftCIHiNarrowburn}{\tbd{hlBdropGapShiftCIHiNarrowburn}}
\providecommand{\hlBdropGapShiftCIHiNarrowflair}{\tbd{hlBdropGapShiftCIHiNarrowflair}}
\providecommand{\hlBdropGapShiftCIHiWideburn}{\tbd{hlBdropGapShiftCIHiWideburn}}
\providecommand{\hlBdropGapShiftCIHiWideflair}{\tbd{hlBdropGapShiftCIHiWideflair}}
\providecommand{\hlBdropGapShiftCILoNarrowburn}{\tbd{hlBdropGapShiftCILoNarrowburn}}
\providecommand{\hlBdropGapShiftCILoNarrowflair}{\tbd{hlBdropGapShiftCILoNarrowflair}}
\providecommand{\hlBdropGapShiftCILoWideburn}{\tbd{hlBdropGapShiftCILoWideburn}}
\providecommand{\hlBdropGapShiftCILoWideflair}{\tbd{hlBdropGapShiftCILoWideflair}}
\providecommand{\hlBdropGapShiftNarrowburn}{\tbd{hlBdropGapShiftNarrowburn}}
\providecommand{\hlBdropGapShiftNarrowflair}{\tbd{hlBdropGapShiftNarrowflair}}
\providecommand{\hlBdropGapShiftTypeNarrowburn}{\tbd{hlBdropGapShiftTypeNarrowburn}}
\providecommand{\hlBdropGapShiftTypeNarrowflair}{\tbd{hlBdropGapShiftTypeNarrowflair}}
\providecommand{\hlBdropGapShiftTypeWideburn}{\tbd{hlBdropGapShiftTypeWideburn}}
\providecommand{\hlBdropGapShiftTypeWideflair}{\tbd{hlBdropGapShiftTypeWideflair}}
\providecommand{\hlBdropGapShiftWideburn}{\tbd{hlBdropGapShiftWideburn}}
\providecommand{\hlBdropGapShiftWideflair}{\tbd{hlBdropGapShiftWideflair}}
\providecommand{\hlBdropNarrowburnBoundary}{\tbd{hlBdropNarrowburnBoundary}}
\providecommand{\hlBdropNarrowburnCoarse}{\tbd{hlBdropNarrowburnCoarse}}
\providecommand{\hlBdropNarrowburnOmission}{\tbd{hlBdropNarrowburnOmission}}
\providecommand{\hlBdropNarrowburnShift}{\tbd{hlBdropNarrowburnShift}}
\providecommand{\hlBdropNarrowflairBoundary}{\tbd{hlBdropNarrowflairBoundary}}
\providecommand{\hlBdropNarrowflairCoarse}{\tbd{hlBdropNarrowflairCoarse}}
\providecommand{\hlBdropNarrowflairOmission}{\tbd{hlBdropNarrowflairOmission}}
\providecommand{\hlBdropNarrowflairShift}{\tbd{hlBdropNarrowflairShift}}
\providecommand{\hlBdropRankNarrowburn}{\tbd{hlBdropRankNarrowburn}}
\providecommand{\hlBdropRankNarrowflair}{\tbd{hlBdropRankNarrowflair}}
\providecommand{\hlBdropRankWideburn}{\tbd{hlBdropRankWideburn}}
\providecommand{\hlBdropRankWideflair}{\tbd{hlBdropRankWideflair}}
\providecommand{\hlBdropShiftLastNarrowburn}{\tbd{hlBdropShiftLastNarrowburn}}
\providecommand{\hlBdropShiftLastNarrowflair}{\tbd{hlBdropShiftLastNarrowflair}}
\providecommand{\hlBdropShiftLastWideburn}{\tbd{hlBdropShiftLastWideburn}}
\providecommand{\hlBdropShiftLastWideflair}{\tbd{hlBdropShiftLastWideflair}}
\providecommand{\hlBdropWideburnBoundary}{\tbd{hlBdropWideburnBoundary}}
\providecommand{\hlBdropWideburnCoarse}{\tbd{hlBdropWideburnCoarse}}
\providecommand{\hlBdropWideburnOmission}{\tbd{hlBdropWideburnOmission}}
\providecommand{\hlBdropWideburnShift}{\tbd{hlBdropWideburnShift}}
\providecommand{\hlBdropWideflairBoundary}{\tbd{hlBdropWideflairBoundary}}
\providecommand{\hlBdropWideflairCoarse}{\tbd{hlBdropWideflairCoarse}}
\providecommand{\hlBdropWideflairOmission}{\tbd{hlBdropWideflairOmission}}
\providecommand{\hlBdropWideflairShift}{\tbd{hlBdropWideflairShift}}
\providecommand{\hlBlockStatusDFive}{\tbd{hlBlockStatusDFive}}
\providecommand{\hlBlockStatusDFour}{\tbd{hlBlockStatusDFour}}
\providecommand{\hlBlockStatusDOne}{\tbd{hlBlockStatusDOne}}
\providecommand{\hlBlockStatusDSeven}{\tbd{hlBlockStatusDSeven}}
\providecommand{\hlBlockStatusDSix}{\tbd{hlBlockStatusDSix}}
\providecommand{\hlBlockStatusDThree}{\tbd{hlBlockStatusDThree}}
\providecommand{\hlBlockStatusDTwo}{\tbd{hlBlockStatusDTwo}}
\providecommand{\hlBlockStatusNEight}{\tbd{hlBlockStatusNEight}}
\providecommand{\hlBlockStatusNEleven}{\tbd{hlBlockStatusNEleven}}
\providecommand{\hlBlockStatusNFifteen}{\tbd{hlBlockStatusNFifteen}}
\providecommand{\hlBlockStatusNFourteen}{\tbd{hlBlockStatusNFourteen}}
\providecommand{\hlBlockStatusNNine}{\tbd{hlBlockStatusNNine}}
\providecommand{\hlBlockStatusNSeven}{\tbd{hlBlockStatusNSeven}}
\providecommand{\hlBlockStatusNTen}{\tbd{hlBlockStatusNTen}}
\providecommand{\hlBlockStatusNThirteen}{\tbd{hlBlockStatusNThirteen}}
\providecommand{\hlBlockStatusNTwelve}{\tbd{hlBlockStatusNTwelve}}
\providecommand{\hlBreakEvenDOFAburn}{\tbd{hlBreakEvenDOFAburn}}
\providecommand{\hlBreakEvenDOFAflair}{\tbd{hlBreakEvenDOFAflair}}
\providecommand{\hlBreakEvenExtrapolatedburn}{\tbd{hlBreakEvenExtrapolatedburn}}
\providecommand{\hlBreakEvenExtrapolatedflair}{\tbd{hlBreakEvenExtrapolatedflair}}
\providecommand{\hlBreakEvenFStarburn}{\tbd{hlBreakEvenFStarburn}}
\providecommand{\hlBreakEvenFStarflair}{\tbd{hlBreakEvenFStarflair}}
\providecommand{\hlBreakEvenLVDburn}{\tbd{hlBreakEvenLVDburn}}
\providecommand{\hlBreakEvenLVDflair}{\tbd{hlBreakEvenLVDflair}}
\providecommand{\hlBreakEvenModelAboveburn}{\tbd{hlBreakEvenModelAboveburn}}
\providecommand{\hlBreakEvenModelAboveflair}{\tbd{hlBreakEvenModelAboveflair}}
\providecommand{\hlBreakEvenModelMaxburn}{\tbd{hlBreakEvenModelMaxburn}}
\providecommand{\hlBreakEvenModelMaxflair}{\tbd{hlBreakEvenModelMaxflair}}
\providecommand{\hlBreakEvenModelMinburn}{\tbd{hlBreakEvenModelMinburn}}
\providecommand{\hlBreakEvenModelMinflair}{\tbd{hlBreakEvenModelMinflair}}
\providecommand{\hlBreakEvenModelNburn}{\tbd{hlBreakEvenModelNburn}}
\providecommand{\hlBreakEvenModelNflair}{\tbd{hlBreakEvenModelNflair}}
\providecommand{\hlBreakEvenRNburn}{\tbd{hlBreakEvenRNburn}}
\providecommand{\hlBreakEvenRNflair}{\tbd{hlBreakEvenRNflair}}
\providecommand{\hlBreakEvenSATburn}{\tbd{hlBreakEvenSATburn}}
\providecommand{\hlBreakEvenSATflair}{\tbd{hlBreakEvenSATflair}}
\providecommand{\hlBreakEvenSeedAboveburn}{\tbd{hlBreakEvenSeedAboveburn}}
\providecommand{\hlBreakEvenSeedAboveflair}{\tbd{hlBreakEvenSeedAboveflair}}
\providecommand{\hlBreakEvenSeedMaxburn}{\tbd{hlBreakEvenSeedMaxburn}}
\providecommand{\hlBreakEvenSeedMaxflair}{\tbd{hlBreakEvenSeedMaxflair}}
\providecommand{\hlBreakEvenSeedMinburn}{\tbd{hlBreakEvenSeedMinburn}}
\providecommand{\hlBreakEvenSeedMinflair}{\tbd{hlBreakEvenSeedMinflair}}
\providecommand{\hlBreakEvenSeedNburn}{\tbd{hlBreakEvenSeedNburn}}
\providecommand{\hlBreakEvenSeedNflair}{\tbd{hlBreakEvenSeedNflair}}
\providecommand{\hlBreakEvenTMburn}{\tbd{hlBreakEvenTMburn}}
\providecommand{\hlBreakEvenTMflair}{\tbd{hlBreakEvenTMflair}}
\providecommand{\hlBreakEvenburn}{\tbd{hlBreakEvenburn}}
\providecommand{\hlBreakEvenflair}{\tbd{hlBreakEvenflair}}
\providecommand{\hlCElevenWorstburn}{\tbd{hlCElevenWorstburn}}
\providecommand{\hlCElevenWorstflair}{\tbd{hlCElevenWorstflair}}
\providecommand{\hlCollFFourAllCIHi}{\tbd{hlCollFFourAllCIHi}}
\providecommand{\hlCollFFourAllCILo}{\tbd{hlCollFFourAllCILo}}
\providecommand{\hlCollFFourAllEst}{\tbd{hlCollFFourAllEst}}
\providecommand{\hlCollFFourAllN}{\tbd{hlCollFFourAllN}}
\providecommand{\hlCollFFourWithoutCIHi}{\tbd{hlCollFFourWithoutCIHi}}
\providecommand{\hlCollFFourWithoutCILo}{\tbd{hlCollFFourWithoutCILo}}
\providecommand{\hlCollFFourWithoutEst}{\tbd{hlCollFFourWithoutEst}}
\providecommand{\hlCollFFourWithoutN}{\tbd{hlCollFFourWithoutN}}
\providecommand{\hlCollFOneAllCIHi}{\tbd{hlCollFOneAllCIHi}}
\providecommand{\hlCollFOneAllCILo}{\tbd{hlCollFOneAllCILo}}
\providecommand{\hlCollFOneAllEst}{\tbd{hlCollFOneAllEst}}
\providecommand{\hlCollFOneAllN}{\tbd{hlCollFOneAllN}}
\providecommand{\hlCollFOneWithoutCIHi}{\tbd{hlCollFOneWithoutCIHi}}
\providecommand{\hlCollFOneWithoutCILo}{\tbd{hlCollFOneWithoutCILo}}
\providecommand{\hlCollFOneWithoutEst}{\tbd{hlCollFOneWithoutEst}}
\providecommand{\hlCollFOneWithoutN}{\tbd{hlCollFOneWithoutN}}
\providecommand{\hlCollFThreeAllCIHi}{\tbd{hlCollFThreeAllCIHi}}
\providecommand{\hlCollFThreeAllCILo}{\tbd{hlCollFThreeAllCILo}}
\providecommand{\hlCollFThreeAllEst}{\tbd{hlCollFThreeAllEst}}
\providecommand{\hlCollFThreeAllN}{\tbd{hlCollFThreeAllN}}
\providecommand{\hlCollFThreeWithoutCIHi}{\tbd{hlCollFThreeWithoutCIHi}}
\providecommand{\hlCollFThreeWithoutCILo}{\tbd{hlCollFThreeWithoutCILo}}
\providecommand{\hlCollFThreeWithoutEst}{\tbd{hlCollFThreeWithoutEst}}
\providecommand{\hlCollFThreeWithoutN}{\tbd{hlCollFThreeWithoutN}}
\providecommand{\hlCollFTwoAllCIHi}{\tbd{hlCollFTwoAllCIHi}}
\providecommand{\hlCollFTwoAllCILo}{\tbd{hlCollFTwoAllCILo}}
\providecommand{\hlCollFTwoAllEst}{\tbd{hlCollFTwoAllEst}}
\providecommand{\hlCollFTwoAllN}{\tbd{hlCollFTwoAllN}}
\providecommand{\hlCollFTwoWithoutCIHi}{\tbd{hlCollFTwoWithoutCIHi}}
\providecommand{\hlCollFTwoWithoutCILo}{\tbd{hlCollFTwoWithoutCILo}}
\providecommand{\hlCollFTwoWithoutEst}{\tbd{hlCollFTwoWithoutEst}}
\providecommand{\hlCollFTwoWithoutN}{\tbd{hlCollFTwoWithoutN}}
\providecommand{\hlCollHTwoAllCIHi}{\tbd{hlCollHTwoAllCIHi}}
\providecommand{\hlCollHTwoAllCILo}{\tbd{hlCollHTwoAllCILo}}
\providecommand{\hlCollHTwoAllEst}{\tbd{hlCollHTwoAllEst}}
\providecommand{\hlCollHTwoAllN}{\tbd{hlCollHTwoAllN}}
\providecommand{\hlCollHTwoWithoutCIHi}{\tbd{hlCollHTwoWithoutCIHi}}
\providecommand{\hlCollHTwoWithoutCILo}{\tbd{hlCollHTwoWithoutCILo}}
\providecommand{\hlCollHTwoWithoutEst}{\tbd{hlCollHTwoWithoutEst}}
\providecommand{\hlCollHTwoWithoutN}{\tbd{hlCollHTwoWithoutN}}
\providecommand{\hlCollTypeMeanBoundaryAll}{\tbd{hlCollTypeMeanBoundaryAll}}
\providecommand{\hlCollTypeMeanBoundaryWithout}{\tbd{hlCollTypeMeanBoundaryWithout}}
\providecommand{\hlCollTypeMeanCoarseAll}{\tbd{hlCollTypeMeanCoarseAll}}
\providecommand{\hlCollTypeMeanCoarseWithout}{\tbd{hlCollTypeMeanCoarseWithout}}
\providecommand{\hlCollTypeMeanOmissionAll}{\tbd{hlCollTypeMeanOmissionAll}}
\providecommand{\hlCollTypeMeanOmissionWithout}{\tbd{hlCollTypeMeanOmissionWithout}}
\providecommand{\hlCollTypeMeanShiftAll}{\tbd{hlCollTypeMeanShiftAll}}
\providecommand{\hlCollTypeMeanShiftWithout}{\tbd{hlCollTypeMeanShiftWithout}}
\providecommand{\hlCollapsedEpochMax}{\tbd{hlCollapsedEpochMax}}
\providecommand{\hlCollapsedEpochMin}{\tbd{hlCollapsedEpochMin}}
\providecommand{\hlCollapsedExtList}{\tbd{hlCollapsedExtList}}
\providecommand{\hlCollapsedExtModelsN}{\tbd{hlCollapsedExtModelsN}}
\providecommand{\hlCollapsedExtN}{\tbd{hlCollapsedExtN}}
\providecommand{\hlCollapsedExtSThreeN}{\tbd{hlCollapsedExtSThreeN}}
\providecommand{\hlCollapsedExtTypes}{\tbd{hlCollapsedExtTypes}}
\providecommand{\hlCollapsedIoUMax}{\tbd{hlCollapsedIoUMax}}
\providecommand{\hlCollapsedMainGridN}{\tbd{hlCollapsedMainGridN}}
\providecommand{\hlDecCleanMtwoFFburn}{\tbd{hlDecCleanMtwoFFburn}}
\providecommand{\hlDecCleanMtwoFFflair}{\tbd{hlDecCleanMtwoFFflair}}
\providecommand{\hlDecCleanMtwoFburn}{\tbd{hlDecCleanMtwoFburn}}
\providecommand{\hlDecCleanMtwoFflair}{\tbd{hlDecCleanMtwoFflair}}
\providecommand{\hlDecCleanSamPreburn}{\tbd{hlDecCleanSamPreburn}}
\providecommand{\hlDecCleanSamPreflair}{\tbd{hlDecCleanSamPreflair}}
\providecommand{\hlDecCleanSamburn}{\tbd{hlDecCleanSamburn}}
\providecommand{\hlDecCleanSamflair}{\tbd{hlDecCleanSamflair}}
\providecommand{\hlDecCleanSegfburn}{\tbd{hlDecCleanSegfburn}}
\providecommand{\hlDecCleanSegfflair}{\tbd{hlDecCleanSegfflair}}
\providecommand{\hlDecCleanUNetburn}{\tbd{hlDecCleanUNetburn}}
\providecommand{\hlDecCleanUNetflair}{\tbd{hlDecCleanUNetflair}}
\providecommand{\hlDecFOneMtwoFFburnCIHi}{\tbd{hlDecFOneMtwoFFburnCIHi}}
\providecommand{\hlDecFOneMtwoFFburnCILo}{\tbd{hlDecFOneMtwoFFburnCILo}}
\providecommand{\hlDecFOneMtwoFFburnEst}{\tbd{hlDecFOneMtwoFFburnEst}}
\providecommand{\hlDecFOneMtwoFFburnMde}{\tbd{hlDecFOneMtwoFFburnMde}}
\providecommand{\hlDecFOneMtwoFFburnN}{\tbd{hlDecFOneMtwoFFburnN}}
\providecommand{\hlDecFOneMtwoFFburnPHolm}{\tbd{hlDecFOneMtwoFFburnPHolm}}
\providecommand{\hlDecFOneMtwoFFburnTostCIHi}{\tbd{hlDecFOneMtwoFFburnTostCIHi}}
\providecommand{\hlDecFOneMtwoFFburnTostCILo}{\tbd{hlDecFOneMtwoFFburnTostCILo}}
\providecommand{\hlDecFOneMtwoFFflairCIHi}{\tbd{hlDecFOneMtwoFFflairCIHi}}
\providecommand{\hlDecFOneMtwoFFflairCILo}{\tbd{hlDecFOneMtwoFFflairCILo}}
\providecommand{\hlDecFOneMtwoFFflairEst}{\tbd{hlDecFOneMtwoFFflairEst}}
\providecommand{\hlDecFOneMtwoFFflairMde}{\tbd{hlDecFOneMtwoFFflairMde}}
\providecommand{\hlDecFOneMtwoFFflairN}{\tbd{hlDecFOneMtwoFFflairN}}
\providecommand{\hlDecFOneMtwoFFflairPHolm}{\tbd{hlDecFOneMtwoFFflairPHolm}}
\providecommand{\hlDecFOneMtwoFFflairTostCIHi}{\tbd{hlDecFOneMtwoFFflairTostCIHi}}
\providecommand{\hlDecFOneMtwoFFflairTostCILo}{\tbd{hlDecFOneMtwoFFflairTostCILo}}
\providecommand{\hlDecFOneMtwoFburnCIHi}{\tbd{hlDecFOneMtwoFburnCIHi}}
\providecommand{\hlDecFOneMtwoFburnCILo}{\tbd{hlDecFOneMtwoFburnCILo}}
\providecommand{\hlDecFOneMtwoFburnEst}{\tbd{hlDecFOneMtwoFburnEst}}
\providecommand{\hlDecFOneMtwoFburnMde}{\tbd{hlDecFOneMtwoFburnMde}}
\providecommand{\hlDecFOneMtwoFburnN}{\tbd{hlDecFOneMtwoFburnN}}
\providecommand{\hlDecFOneMtwoFburnPHolm}{\tbd{hlDecFOneMtwoFburnPHolm}}
\providecommand{\hlDecFOneMtwoFburnTostCIHi}{\tbd{hlDecFOneMtwoFburnTostCIHi}}
\providecommand{\hlDecFOneMtwoFburnTostCILo}{\tbd{hlDecFOneMtwoFburnTostCILo}}
\providecommand{\hlDecFOneMtwoFflairCIHi}{\tbd{hlDecFOneMtwoFflairCIHi}}
\providecommand{\hlDecFOneMtwoFflairCILo}{\tbd{hlDecFOneMtwoFflairCILo}}
\providecommand{\hlDecFOneMtwoFflairEst}{\tbd{hlDecFOneMtwoFflairEst}}
\providecommand{\hlDecFOneMtwoFflairMde}{\tbd{hlDecFOneMtwoFflairMde}}
\providecommand{\hlDecFOneMtwoFflairN}{\tbd{hlDecFOneMtwoFflairN}}
\providecommand{\hlDecFOneMtwoFflairPHolm}{\tbd{hlDecFOneMtwoFflairPHolm}}
\providecommand{\hlDecFOneMtwoFflairTostCIHi}{\tbd{hlDecFOneMtwoFflairTostCIHi}}
\providecommand{\hlDecFOneMtwoFflairTostCILo}{\tbd{hlDecFOneMtwoFflairTostCILo}}
\providecommand{\hlDecFOneOneMtwoFFburnCIHi}{\tbd{hlDecFOneOneMtwoFFburnCIHi}}
\providecommand{\hlDecFOneOneMtwoFFburnCILo}{\tbd{hlDecFOneOneMtwoFFburnCILo}}
\providecommand{\hlDecFOneOneMtwoFFburnEst}{\tbd{hlDecFOneOneMtwoFFburnEst}}
\providecommand{\hlDecFOneOneMtwoFFburnMde}{\tbd{hlDecFOneOneMtwoFFburnMde}}
\providecommand{\hlDecFOneOneMtwoFFburnN}{\tbd{hlDecFOneOneMtwoFFburnN}}
\providecommand{\hlDecFOneOneMtwoFFburnPHolm}{\tbd{hlDecFOneOneMtwoFFburnPHolm}}
\providecommand{\hlDecFOneOneMtwoFFburnTostCIHi}{\tbd{hlDecFOneOneMtwoFFburnTostCIHi}}
\providecommand{\hlDecFOneOneMtwoFFburnTostCILo}{\tbd{hlDecFOneOneMtwoFFburnTostCILo}}
\providecommand{\hlDecFOneOneMtwoFFflairCIHi}{\tbd{hlDecFOneOneMtwoFFflairCIHi}}
\providecommand{\hlDecFOneOneMtwoFFflairCILo}{\tbd{hlDecFOneOneMtwoFFflairCILo}}
\providecommand{\hlDecFOneOneMtwoFFflairEst}{\tbd{hlDecFOneOneMtwoFFflairEst}}
\providecommand{\hlDecFOneOneMtwoFFflairMde}{\tbd{hlDecFOneOneMtwoFFflairMde}}
\providecommand{\hlDecFOneOneMtwoFFflairN}{\tbd{hlDecFOneOneMtwoFFflairN}}
\providecommand{\hlDecFOneOneMtwoFFflairPHolm}{\tbd{hlDecFOneOneMtwoFFflairPHolm}}
\providecommand{\hlDecFOneOneMtwoFFflairTostCIHi}{\tbd{hlDecFOneOneMtwoFFflairTostCIHi}}
\providecommand{\hlDecFOneOneMtwoFFflairTostCILo}{\tbd{hlDecFOneOneMtwoFFflairTostCILo}}
\providecommand{\hlDecFOneOneMtwoFburnCIHi}{\tbd{hlDecFOneOneMtwoFburnCIHi}}
\providecommand{\hlDecFOneOneMtwoFburnCILo}{\tbd{hlDecFOneOneMtwoFburnCILo}}
\providecommand{\hlDecFOneOneMtwoFburnEst}{\tbd{hlDecFOneOneMtwoFburnEst}}
\providecommand{\hlDecFOneOneMtwoFburnMde}{\tbd{hlDecFOneOneMtwoFburnMde}}
\providecommand{\hlDecFOneOneMtwoFburnN}{\tbd{hlDecFOneOneMtwoFburnN}}
\providecommand{\hlDecFOneOneMtwoFburnPHolm}{\tbd{hlDecFOneOneMtwoFburnPHolm}}
\providecommand{\hlDecFOneOneMtwoFburnTostCIHi}{\tbd{hlDecFOneOneMtwoFburnTostCIHi}}
\providecommand{\hlDecFOneOneMtwoFburnTostCILo}{\tbd{hlDecFOneOneMtwoFburnTostCILo}}
\providecommand{\hlDecFOneOneMtwoFflairCIHi}{\tbd{hlDecFOneOneMtwoFflairCIHi}}
\providecommand{\hlDecFOneOneMtwoFflairCILo}{\tbd{hlDecFOneOneMtwoFflairCILo}}
\providecommand{\hlDecFOneOneMtwoFflairEst}{\tbd{hlDecFOneOneMtwoFflairEst}}
\providecommand{\hlDecFOneOneMtwoFflairMde}{\tbd{hlDecFOneOneMtwoFflairMde}}
\providecommand{\hlDecFOneOneMtwoFflairN}{\tbd{hlDecFOneOneMtwoFflairN}}
\providecommand{\hlDecFOneOneMtwoFflairPHolm}{\tbd{hlDecFOneOneMtwoFflairPHolm}}
\providecommand{\hlDecFOneOneMtwoFflairTostCIHi}{\tbd{hlDecFOneOneMtwoFflairTostCIHi}}
\providecommand{\hlDecFOneOneMtwoFflairTostCILo}{\tbd{hlDecFOneOneMtwoFflairTostCILo}}
\providecommand{\hlDecFOneOneSamPreburnCIHi}{\tbd{hlDecFOneOneSamPreburnCIHi}}
\providecommand{\hlDecFOneOneSamPreburnCILo}{\tbd{hlDecFOneOneSamPreburnCILo}}
\providecommand{\hlDecFOneOneSamPreburnEst}{\tbd{hlDecFOneOneSamPreburnEst}}
\providecommand{\hlDecFOneOneSamPreburnMde}{\tbd{hlDecFOneOneSamPreburnMde}}
\providecommand{\hlDecFOneOneSamPreburnN}{\tbd{hlDecFOneOneSamPreburnN}}
\providecommand{\hlDecFOneOneSamPreburnPHolm}{\tbd{hlDecFOneOneSamPreburnPHolm}}
\providecommand{\hlDecFOneOneSamPreburnTostCIHi}{\tbd{hlDecFOneOneSamPreburnTostCIHi}}
\providecommand{\hlDecFOneOneSamPreburnTostCILo}{\tbd{hlDecFOneOneSamPreburnTostCILo}}
\providecommand{\hlDecFOneOneSamPreflairCIHi}{\tbd{hlDecFOneOneSamPreflairCIHi}}
\providecommand{\hlDecFOneOneSamPreflairCILo}{\tbd{hlDecFOneOneSamPreflairCILo}}
\providecommand{\hlDecFOneOneSamPreflairEst}{\tbd{hlDecFOneOneSamPreflairEst}}
\providecommand{\hlDecFOneOneSamPreflairMde}{\tbd{hlDecFOneOneSamPreflairMde}}
\providecommand{\hlDecFOneOneSamPreflairN}{\tbd{hlDecFOneOneSamPreflairN}}
\providecommand{\hlDecFOneOneSamPreflairPHolm}{\tbd{hlDecFOneOneSamPreflairPHolm}}
\providecommand{\hlDecFOneOneSamPreflairTostCIHi}{\tbd{hlDecFOneOneSamPreflairTostCIHi}}
\providecommand{\hlDecFOneOneSamPreflairTostCILo}{\tbd{hlDecFOneOneSamPreflairTostCILo}}
\providecommand{\hlDecFOneOneSamburnCIHi}{\tbd{hlDecFOneOneSamburnCIHi}}
\providecommand{\hlDecFOneOneSamburnCILo}{\tbd{hlDecFOneOneSamburnCILo}}
\providecommand{\hlDecFOneOneSamburnEst}{\tbd{hlDecFOneOneSamburnEst}}
\providecommand{\hlDecFOneOneSamburnMde}{\tbd{hlDecFOneOneSamburnMde}}
\providecommand{\hlDecFOneOneSamburnN}{\tbd{hlDecFOneOneSamburnN}}
\providecommand{\hlDecFOneOneSamburnPHolm}{\tbd{hlDecFOneOneSamburnPHolm}}
\providecommand{\hlDecFOneOneSamburnTostCIHi}{\tbd{hlDecFOneOneSamburnTostCIHi}}
\providecommand{\hlDecFOneOneSamburnTostCILo}{\tbd{hlDecFOneOneSamburnTostCILo}}
\providecommand{\hlDecFOneOneSamflairCIHi}{\tbd{hlDecFOneOneSamflairCIHi}}
\providecommand{\hlDecFOneOneSamflairCILo}{\tbd{hlDecFOneOneSamflairCILo}}
\providecommand{\hlDecFOneOneSamflairEst}{\tbd{hlDecFOneOneSamflairEst}}
\providecommand{\hlDecFOneOneSamflairMde}{\tbd{hlDecFOneOneSamflairMde}}
\providecommand{\hlDecFOneOneSamflairN}{\tbd{hlDecFOneOneSamflairN}}
\providecommand{\hlDecFOneOneSamflairPHolm}{\tbd{hlDecFOneOneSamflairPHolm}}
\providecommand{\hlDecFOneOneSamflairTostCIHi}{\tbd{hlDecFOneOneSamflairTostCIHi}}
\providecommand{\hlDecFOneOneSamflairTostCILo}{\tbd{hlDecFOneOneSamflairTostCILo}}
\providecommand{\hlDecFOneOneSegfburnCIHi}{\tbd{hlDecFOneOneSegfburnCIHi}}
\providecommand{\hlDecFOneOneSegfburnCILo}{\tbd{hlDecFOneOneSegfburnCILo}}
\providecommand{\hlDecFOneOneSegfburnEst}{\tbd{hlDecFOneOneSegfburnEst}}
\providecommand{\hlDecFOneOneSegfburnMde}{\tbd{hlDecFOneOneSegfburnMde}}
\providecommand{\hlDecFOneOneSegfburnN}{\tbd{hlDecFOneOneSegfburnN}}
\providecommand{\hlDecFOneOneSegfburnPHolm}{\tbd{hlDecFOneOneSegfburnPHolm}}
\providecommand{\hlDecFOneOneSegfburnTostCIHi}{\tbd{hlDecFOneOneSegfburnTostCIHi}}
\providecommand{\hlDecFOneOneSegfburnTostCILo}{\tbd{hlDecFOneOneSegfburnTostCILo}}
\providecommand{\hlDecFOneOneSegfflairCIHi}{\tbd{hlDecFOneOneSegfflairCIHi}}
\providecommand{\hlDecFOneOneSegfflairCILo}{\tbd{hlDecFOneOneSegfflairCILo}}
\providecommand{\hlDecFOneOneSegfflairEst}{\tbd{hlDecFOneOneSegfflairEst}}
\providecommand{\hlDecFOneOneSegfflairMde}{\tbd{hlDecFOneOneSegfflairMde}}
\providecommand{\hlDecFOneOneSegfflairN}{\tbd{hlDecFOneOneSegfflairN}}
\providecommand{\hlDecFOneOneSegfflairPHolm}{\tbd{hlDecFOneOneSegfflairPHolm}}
\providecommand{\hlDecFOneOneSegfflairTostCIHi}{\tbd{hlDecFOneOneSegfflairTostCIHi}}
\providecommand{\hlDecFOneOneSegfflairTostCILo}{\tbd{hlDecFOneOneSegfflairTostCILo}}
\providecommand{\hlDecFOneOneburnCIHi}{\tbd{hlDecFOneOneburnCIHi}}
\providecommand{\hlDecFOneOneburnCILo}{\tbd{hlDecFOneOneburnCILo}}
\providecommand{\hlDecFOneOneburnEst}{\tbd{hlDecFOneOneburnEst}}
\providecommand{\hlDecFOneOneburnMde}{\tbd{hlDecFOneOneburnMde}}
\providecommand{\hlDecFOneOneburnN}{\tbd{hlDecFOneOneburnN}}
\providecommand{\hlDecFOneOneburnPHolm}{\tbd{hlDecFOneOneburnPHolm}}
\providecommand{\hlDecFOneOneburnTostCIHi}{\tbd{hlDecFOneOneburnTostCIHi}}
\providecommand{\hlDecFOneOneburnTostCILo}{\tbd{hlDecFOneOneburnTostCILo}}
\providecommand{\hlDecFOneOneflairCIHi}{\tbd{hlDecFOneOneflairCIHi}}
\providecommand{\hlDecFOneOneflairCILo}{\tbd{hlDecFOneOneflairCILo}}
\providecommand{\hlDecFOneOneflairEst}{\tbd{hlDecFOneOneflairEst}}
\providecommand{\hlDecFOneOneflairMde}{\tbd{hlDecFOneOneflairMde}}
\providecommand{\hlDecFOneOneflairN}{\tbd{hlDecFOneOneflairN}}
\providecommand{\hlDecFOneOneflairPHolm}{\tbd{hlDecFOneOneflairPHolm}}
\providecommand{\hlDecFOneOneflairTostCIHi}{\tbd{hlDecFOneOneflairTostCIHi}}
\providecommand{\hlDecFOneOneflairTostCILo}{\tbd{hlDecFOneOneflairTostCILo}}
\providecommand{\hlDecFOneSamPreburnCIHi}{\tbd{hlDecFOneSamPreburnCIHi}}
\providecommand{\hlDecFOneSamPreburnCILo}{\tbd{hlDecFOneSamPreburnCILo}}
\providecommand{\hlDecFOneSamPreburnEst}{\tbd{hlDecFOneSamPreburnEst}}
\providecommand{\hlDecFOneSamPreburnMde}{\tbd{hlDecFOneSamPreburnMde}}
\providecommand{\hlDecFOneSamPreburnN}{\tbd{hlDecFOneSamPreburnN}}
\providecommand{\hlDecFOneSamPreburnPHolm}{\tbd{hlDecFOneSamPreburnPHolm}}
\providecommand{\hlDecFOneSamPreburnTostCIHi}{\tbd{hlDecFOneSamPreburnTostCIHi}}
\providecommand{\hlDecFOneSamPreburnTostCILo}{\tbd{hlDecFOneSamPreburnTostCILo}}
\providecommand{\hlDecFOneSamPreflairCIHi}{\tbd{hlDecFOneSamPreflairCIHi}}
\providecommand{\hlDecFOneSamPreflairCILo}{\tbd{hlDecFOneSamPreflairCILo}}
\providecommand{\hlDecFOneSamPreflairEst}{\tbd{hlDecFOneSamPreflairEst}}
\providecommand{\hlDecFOneSamPreflairMde}{\tbd{hlDecFOneSamPreflairMde}}
\providecommand{\hlDecFOneSamPreflairN}{\tbd{hlDecFOneSamPreflairN}}
\providecommand{\hlDecFOneSamPreflairPHolm}{\tbd{hlDecFOneSamPreflairPHolm}}
\providecommand{\hlDecFOneSamPreflairTostCIHi}{\tbd{hlDecFOneSamPreflairTostCIHi}}
\providecommand{\hlDecFOneSamPreflairTostCILo}{\tbd{hlDecFOneSamPreflairTostCILo}}
\providecommand{\hlDecFOneSamburnCIHi}{\tbd{hlDecFOneSamburnCIHi}}
\providecommand{\hlDecFOneSamburnCILo}{\tbd{hlDecFOneSamburnCILo}}
\providecommand{\hlDecFOneSamburnEst}{\tbd{hlDecFOneSamburnEst}}
\providecommand{\hlDecFOneSamburnMde}{\tbd{hlDecFOneSamburnMde}}
\providecommand{\hlDecFOneSamburnN}{\tbd{hlDecFOneSamburnN}}
\providecommand{\hlDecFOneSamburnPHolm}{\tbd{hlDecFOneSamburnPHolm}}
\providecommand{\hlDecFOneSamburnTostCIHi}{\tbd{hlDecFOneSamburnTostCIHi}}
\providecommand{\hlDecFOneSamburnTostCILo}{\tbd{hlDecFOneSamburnTostCILo}}
\providecommand{\hlDecFOneSamflairCIHi}{\tbd{hlDecFOneSamflairCIHi}}
\providecommand{\hlDecFOneSamflairCILo}{\tbd{hlDecFOneSamflairCILo}}
\providecommand{\hlDecFOneSamflairEst}{\tbd{hlDecFOneSamflairEst}}
\providecommand{\hlDecFOneSamflairMde}{\tbd{hlDecFOneSamflairMde}}
\providecommand{\hlDecFOneSamflairN}{\tbd{hlDecFOneSamflairN}}
\providecommand{\hlDecFOneSamflairPHolm}{\tbd{hlDecFOneSamflairPHolm}}
\providecommand{\hlDecFOneSamflairTostCIHi}{\tbd{hlDecFOneSamflairTostCIHi}}
\providecommand{\hlDecFOneSamflairTostCILo}{\tbd{hlDecFOneSamflairTostCILo}}
\providecommand{\hlDecFOneSegfburnCIHi}{\tbd{hlDecFOneSegfburnCIHi}}
\providecommand{\hlDecFOneSegfburnCILo}{\tbd{hlDecFOneSegfburnCILo}}
\providecommand{\hlDecFOneSegfburnEst}{\tbd{hlDecFOneSegfburnEst}}
\providecommand{\hlDecFOneSegfburnMde}{\tbd{hlDecFOneSegfburnMde}}
\providecommand{\hlDecFOneSegfburnN}{\tbd{hlDecFOneSegfburnN}}
\providecommand{\hlDecFOneSegfburnPHolm}{\tbd{hlDecFOneSegfburnPHolm}}
\providecommand{\hlDecFOneSegfburnTostCIHi}{\tbd{hlDecFOneSegfburnTostCIHi}}
\providecommand{\hlDecFOneSegfburnTostCILo}{\tbd{hlDecFOneSegfburnTostCILo}}
\providecommand{\hlDecFOneSegfflairCIHi}{\tbd{hlDecFOneSegfflairCIHi}}
\providecommand{\hlDecFOneSegfflairCILo}{\tbd{hlDecFOneSegfflairCILo}}
\providecommand{\hlDecFOneSegfflairEst}{\tbd{hlDecFOneSegfflairEst}}
\providecommand{\hlDecFOneSegfflairMde}{\tbd{hlDecFOneSegfflairMde}}
\providecommand{\hlDecFOneSegfflairN}{\tbd{hlDecFOneSegfflairN}}
\providecommand{\hlDecFOneSegfflairPHolm}{\tbd{hlDecFOneSegfflairPHolm}}
\providecommand{\hlDecFOneSegfflairTostCIHi}{\tbd{hlDecFOneSegfflairTostCIHi}}
\providecommand{\hlDecFOneSegfflairTostCILo}{\tbd{hlDecFOneSegfflairTostCILo}}
\providecommand{\hlDecFOneburnCIHi}{\tbd{hlDecFOneburnCIHi}}
\providecommand{\hlDecFOneburnCILo}{\tbd{hlDecFOneburnCILo}}
\providecommand{\hlDecFOneburnEst}{\tbd{hlDecFOneburnEst}}
\providecommand{\hlDecFOneburnMde}{\tbd{hlDecFOneburnMde}}
\providecommand{\hlDecFOneburnN}{\tbd{hlDecFOneburnN}}
\providecommand{\hlDecFOneburnPHolm}{\tbd{hlDecFOneburnPHolm}}
\providecommand{\hlDecFOneburnTostCIHi}{\tbd{hlDecFOneburnTostCIHi}}
\providecommand{\hlDecFOneburnTostCILo}{\tbd{hlDecFOneburnTostCILo}}
\providecommand{\hlDecFOneflairCIHi}{\tbd{hlDecFOneflairCIHi}}
\providecommand{\hlDecFOneflairCILo}{\tbd{hlDecFOneflairCILo}}
\providecommand{\hlDecFOneflairEst}{\tbd{hlDecFOneflairEst}}
\providecommand{\hlDecFOneflairMde}{\tbd{hlDecFOneflairMde}}
\providecommand{\hlDecFOneflairN}{\tbd{hlDecFOneflairN}}
\providecommand{\hlDecFOneflairPHolm}{\tbd{hlDecFOneflairPHolm}}
\providecommand{\hlDecFOneflairTostCIHi}{\tbd{hlDecFOneflairTostCIHi}}
\providecommand{\hlDecFOneflairTostCILo}{\tbd{hlDecFOneflairTostCILo}}
\providecommand{\hlDecFTwoMtwoFFburnCIHi}{\tbd{hlDecFTwoMtwoFFburnCIHi}}
\providecommand{\hlDecFTwoMtwoFFburnCILo}{\tbd{hlDecFTwoMtwoFFburnCILo}}
\providecommand{\hlDecFTwoMtwoFFburnEst}{\tbd{hlDecFTwoMtwoFFburnEst}}
\providecommand{\hlDecFTwoMtwoFFburnMde}{\tbd{hlDecFTwoMtwoFFburnMde}}
\providecommand{\hlDecFTwoMtwoFFburnN}{\tbd{hlDecFTwoMtwoFFburnN}}
\providecommand{\hlDecFTwoMtwoFFburnPHolm}{\tbd{hlDecFTwoMtwoFFburnPHolm}}
\providecommand{\hlDecFTwoMtwoFFburnTostCIHi}{\tbd{hlDecFTwoMtwoFFburnTostCIHi}}
\providecommand{\hlDecFTwoMtwoFFburnTostCILo}{\tbd{hlDecFTwoMtwoFFburnTostCILo}}
\providecommand{\hlDecFTwoMtwoFFflairCIHi}{\tbd{hlDecFTwoMtwoFFflairCIHi}}
\providecommand{\hlDecFTwoMtwoFFflairCILo}{\tbd{hlDecFTwoMtwoFFflairCILo}}
\providecommand{\hlDecFTwoMtwoFFflairEst}{\tbd{hlDecFTwoMtwoFFflairEst}}
\providecommand{\hlDecFTwoMtwoFFflairMde}{\tbd{hlDecFTwoMtwoFFflairMde}}
\providecommand{\hlDecFTwoMtwoFFflairN}{\tbd{hlDecFTwoMtwoFFflairN}}
\providecommand{\hlDecFTwoMtwoFFflairPHolm}{\tbd{hlDecFTwoMtwoFFflairPHolm}}
\providecommand{\hlDecFTwoMtwoFFflairTostCIHi}{\tbd{hlDecFTwoMtwoFFflairTostCIHi}}
\providecommand{\hlDecFTwoMtwoFFflairTostCILo}{\tbd{hlDecFTwoMtwoFFflairTostCILo}}
\providecommand{\hlDecFTwoMtwoFburnCIHi}{\tbd{hlDecFTwoMtwoFburnCIHi}}
\providecommand{\hlDecFTwoMtwoFburnCILo}{\tbd{hlDecFTwoMtwoFburnCILo}}
\providecommand{\hlDecFTwoMtwoFburnEst}{\tbd{hlDecFTwoMtwoFburnEst}}
\providecommand{\hlDecFTwoMtwoFburnMde}{\tbd{hlDecFTwoMtwoFburnMde}}
\providecommand{\hlDecFTwoMtwoFburnN}{\tbd{hlDecFTwoMtwoFburnN}}
\providecommand{\hlDecFTwoMtwoFburnPHolm}{\tbd{hlDecFTwoMtwoFburnPHolm}}
\providecommand{\hlDecFTwoMtwoFburnTostCIHi}{\tbd{hlDecFTwoMtwoFburnTostCIHi}}
\providecommand{\hlDecFTwoMtwoFburnTostCILo}{\tbd{hlDecFTwoMtwoFburnTostCILo}}
\providecommand{\hlDecFTwoMtwoFflairCIHi}{\tbd{hlDecFTwoMtwoFflairCIHi}}
\providecommand{\hlDecFTwoMtwoFflairCILo}{\tbd{hlDecFTwoMtwoFflairCILo}}
\providecommand{\hlDecFTwoMtwoFflairEst}{\tbd{hlDecFTwoMtwoFflairEst}}
\providecommand{\hlDecFTwoMtwoFflairMde}{\tbd{hlDecFTwoMtwoFflairMde}}
\providecommand{\hlDecFTwoMtwoFflairN}{\tbd{hlDecFTwoMtwoFflairN}}
\providecommand{\hlDecFTwoMtwoFflairPHolm}{\tbd{hlDecFTwoMtwoFflairPHolm}}
\providecommand{\hlDecFTwoMtwoFflairTostCIHi}{\tbd{hlDecFTwoMtwoFflairTostCIHi}}
\providecommand{\hlDecFTwoMtwoFflairTostCILo}{\tbd{hlDecFTwoMtwoFflairTostCILo}}
\providecommand{\hlDecFTwoSamPreburnCIHi}{\tbd{hlDecFTwoSamPreburnCIHi}}
\providecommand{\hlDecFTwoSamPreburnCILo}{\tbd{hlDecFTwoSamPreburnCILo}}
\providecommand{\hlDecFTwoSamPreburnEst}{\tbd{hlDecFTwoSamPreburnEst}}
\providecommand{\hlDecFTwoSamPreburnMde}{\tbd{hlDecFTwoSamPreburnMde}}
\providecommand{\hlDecFTwoSamPreburnN}{\tbd{hlDecFTwoSamPreburnN}}
\providecommand{\hlDecFTwoSamPreburnPHolm}{\tbd{hlDecFTwoSamPreburnPHolm}}
\providecommand{\hlDecFTwoSamPreburnTostCIHi}{\tbd{hlDecFTwoSamPreburnTostCIHi}}
\providecommand{\hlDecFTwoSamPreburnTostCILo}{\tbd{hlDecFTwoSamPreburnTostCILo}}
\providecommand{\hlDecFTwoSamPreflairCIHi}{\tbd{hlDecFTwoSamPreflairCIHi}}
\providecommand{\hlDecFTwoSamPreflairCILo}{\tbd{hlDecFTwoSamPreflairCILo}}
\providecommand{\hlDecFTwoSamPreflairEst}{\tbd{hlDecFTwoSamPreflairEst}}
\providecommand{\hlDecFTwoSamPreflairMde}{\tbd{hlDecFTwoSamPreflairMde}}
\providecommand{\hlDecFTwoSamPreflairN}{\tbd{hlDecFTwoSamPreflairN}}
\providecommand{\hlDecFTwoSamPreflairPHolm}{\tbd{hlDecFTwoSamPreflairPHolm}}
\providecommand{\hlDecFTwoSamPreflairTostCIHi}{\tbd{hlDecFTwoSamPreflairTostCIHi}}
\providecommand{\hlDecFTwoSamPreflairTostCILo}{\tbd{hlDecFTwoSamPreflairTostCILo}}
\providecommand{\hlDecFTwoSamburnCIHi}{\tbd{hlDecFTwoSamburnCIHi}}
\providecommand{\hlDecFTwoSamburnCILo}{\tbd{hlDecFTwoSamburnCILo}}
\providecommand{\hlDecFTwoSamburnEst}{\tbd{hlDecFTwoSamburnEst}}
\providecommand{\hlDecFTwoSamburnMde}{\tbd{hlDecFTwoSamburnMde}}
\providecommand{\hlDecFTwoSamburnN}{\tbd{hlDecFTwoSamburnN}}
\providecommand{\hlDecFTwoSamburnPHolm}{\tbd{hlDecFTwoSamburnPHolm}}
\providecommand{\hlDecFTwoSamburnTostCIHi}{\tbd{hlDecFTwoSamburnTostCIHi}}
\providecommand{\hlDecFTwoSamburnTostCILo}{\tbd{hlDecFTwoSamburnTostCILo}}
\providecommand{\hlDecFTwoSamflairCIHi}{\tbd{hlDecFTwoSamflairCIHi}}
\providecommand{\hlDecFTwoSamflairCILo}{\tbd{hlDecFTwoSamflairCILo}}
\providecommand{\hlDecFTwoSamflairEst}{\tbd{hlDecFTwoSamflairEst}}
\providecommand{\hlDecFTwoSamflairMde}{\tbd{hlDecFTwoSamflairMde}}
\providecommand{\hlDecFTwoSamflairN}{\tbd{hlDecFTwoSamflairN}}
\providecommand{\hlDecFTwoSamflairPHolm}{\tbd{hlDecFTwoSamflairPHolm}}
\providecommand{\hlDecFTwoSamflairTostCIHi}{\tbd{hlDecFTwoSamflairTostCIHi}}
\providecommand{\hlDecFTwoSamflairTostCILo}{\tbd{hlDecFTwoSamflairTostCILo}}
\providecommand{\hlDecFTwoSegfburnCIHi}{\tbd{hlDecFTwoSegfburnCIHi}}
\providecommand{\hlDecFTwoSegfburnCILo}{\tbd{hlDecFTwoSegfburnCILo}}
\providecommand{\hlDecFTwoSegfburnEst}{\tbd{hlDecFTwoSegfburnEst}}
\providecommand{\hlDecFTwoSegfburnMde}{\tbd{hlDecFTwoSegfburnMde}}
\providecommand{\hlDecFTwoSegfburnN}{\tbd{hlDecFTwoSegfburnN}}
\providecommand{\hlDecFTwoSegfburnPHolm}{\tbd{hlDecFTwoSegfburnPHolm}}
\providecommand{\hlDecFTwoSegfburnTostCIHi}{\tbd{hlDecFTwoSegfburnTostCIHi}}
\providecommand{\hlDecFTwoSegfburnTostCILo}{\tbd{hlDecFTwoSegfburnTostCILo}}
\providecommand{\hlDecFTwoSegfflairCIHi}{\tbd{hlDecFTwoSegfflairCIHi}}
\providecommand{\hlDecFTwoSegfflairCILo}{\tbd{hlDecFTwoSegfflairCILo}}
\providecommand{\hlDecFTwoSegfflairEst}{\tbd{hlDecFTwoSegfflairEst}}
\providecommand{\hlDecFTwoSegfflairMde}{\tbd{hlDecFTwoSegfflairMde}}
\providecommand{\hlDecFTwoSegfflairN}{\tbd{hlDecFTwoSegfflairN}}
\providecommand{\hlDecFTwoSegfflairPHolm}{\tbd{hlDecFTwoSegfflairPHolm}}
\providecommand{\hlDecFTwoSegfflairTostCIHi}{\tbd{hlDecFTwoSegfflairTostCIHi}}
\providecommand{\hlDecFTwoSegfflairTostCILo}{\tbd{hlDecFTwoSegfflairTostCILo}}
\providecommand{\hlDecFTwoburnCIHi}{\tbd{hlDecFTwoburnCIHi}}
\providecommand{\hlDecFTwoburnCILo}{\tbd{hlDecFTwoburnCILo}}
\providecommand{\hlDecFTwoburnEst}{\tbd{hlDecFTwoburnEst}}
\providecommand{\hlDecFTwoburnMde}{\tbd{hlDecFTwoburnMde}}
\providecommand{\hlDecFTwoburnN}{\tbd{hlDecFTwoburnN}}
\providecommand{\hlDecFTwoburnPHolm}{\tbd{hlDecFTwoburnPHolm}}
\providecommand{\hlDecFTwoburnTostCIHi}{\tbd{hlDecFTwoburnTostCIHi}}
\providecommand{\hlDecFTwoburnTostCILo}{\tbd{hlDecFTwoburnTostCILo}}
\providecommand{\hlDecFTwoflairCIHi}{\tbd{hlDecFTwoflairCIHi}}
\providecommand{\hlDecFTwoflairCILo}{\tbd{hlDecFTwoflairCILo}}
\providecommand{\hlDecFTwoflairEst}{\tbd{hlDecFTwoflairEst}}
\providecommand{\hlDecFTwoflairMde}{\tbd{hlDecFTwoflairMde}}
\providecommand{\hlDecFTwoflairN}{\tbd{hlDecFTwoflairN}}
\providecommand{\hlDecFTwoflairPHolm}{\tbd{hlDecFTwoflairPHolm}}
\providecommand{\hlDecFTwoflairTostCIHi}{\tbd{hlDecFTwoflairTostCIHi}}
\providecommand{\hlDecFTwoflairTostCILo}{\tbd{hlDecFTwoflairTostCILo}}
\providecommand{\hlDecFullVsLiteburnCIHi}{\tbd{hlDecFullVsLiteburnCIHi}}
\providecommand{\hlDecFullVsLiteburnCILo}{\tbd{hlDecFullVsLiteburnCILo}}
\providecommand{\hlDecFullVsLiteburnEst}{\tbd{hlDecFullVsLiteburnEst}}
\providecommand{\hlDecFullVsLiteburnMde}{\tbd{hlDecFullVsLiteburnMde}}
\providecommand{\hlDecFullVsLiteburnN}{\tbd{hlDecFullVsLiteburnN}}
\providecommand{\hlDecFullVsLiteburnPHolm}{\tbd{hlDecFullVsLiteburnPHolm}}
\providecommand{\hlDecFullVsLiteburnTostCIHi}{\tbd{hlDecFullVsLiteburnTostCIHi}}
\providecommand{\hlDecFullVsLiteburnTostCILo}{\tbd{hlDecFullVsLiteburnTostCILo}}
\providecommand{\hlDecFullVsLiteflairCIHi}{\tbd{hlDecFullVsLiteflairCIHi}}
\providecommand{\hlDecFullVsLiteflairCILo}{\tbd{hlDecFullVsLiteflairCILo}}
\providecommand{\hlDecFullVsLiteflairEst}{\tbd{hlDecFullVsLiteflairEst}}
\providecommand{\hlDecFullVsLiteflairMde}{\tbd{hlDecFullVsLiteflairMde}}
\providecommand{\hlDecFullVsLiteflairN}{\tbd{hlDecFullVsLiteflairN}}
\providecommand{\hlDecFullVsLiteflairPHolm}{\tbd{hlDecFullVsLiteflairPHolm}}
\providecommand{\hlDecFullVsLiteflairTostCIHi}{\tbd{hlDecFullVsLiteflairTostCIHi}}
\providecommand{\hlDecFullVsLiteflairTostCILo}{\tbd{hlDecFullVsLiteflairTostCILo}}
\providecommand{\hlDecInvDOFAburnCIHi}{\tbd{hlDecInvDOFAburnCIHi}}
\providecommand{\hlDecInvDOFAburnCILo}{\tbd{hlDecInvDOFAburnCILo}}
\providecommand{\hlDecInvDOFAburnEst}{\tbd{hlDecInvDOFAburnEst}}
\providecommand{\hlDecInvDOFAflairCIHi}{\tbd{hlDecInvDOFAflairCIHi}}
\providecommand{\hlDecInvDOFAflairCILo}{\tbd{hlDecInvDOFAflairCILo}}
\providecommand{\hlDecInvDOFAflairEst}{\tbd{hlDecInvDOFAflairEst}}
\providecommand{\hlDecInvLVDburnCIHi}{\tbd{hlDecInvLVDburnCIHi}}
\providecommand{\hlDecInvLVDburnCILo}{\tbd{hlDecInvLVDburnCILo}}
\providecommand{\hlDecInvLVDburnEst}{\tbd{hlDecInvLVDburnEst}}
\providecommand{\hlDecInvLVDflairCIHi}{\tbd{hlDecInvLVDflairCIHi}}
\providecommand{\hlDecInvLVDflairCILo}{\tbd{hlDecInvLVDflairCILo}}
\providecommand{\hlDecInvLVDflairEst}{\tbd{hlDecInvLVDflairEst}}
\providecommand{\hlDecInvMtwoFDOFAburnCIHi}{\tbd{hlDecInvMtwoFDOFAburnCIHi}}
\providecommand{\hlDecInvMtwoFDOFAburnCILo}{\tbd{hlDecInvMtwoFDOFAburnCILo}}
\providecommand{\hlDecInvMtwoFDOFAburnEst}{\tbd{hlDecInvMtwoFDOFAburnEst}}
\providecommand{\hlDecInvMtwoFDOFAflairCIHi}{\tbd{hlDecInvMtwoFDOFAflairCIHi}}
\providecommand{\hlDecInvMtwoFDOFAflairCILo}{\tbd{hlDecInvMtwoFDOFAflairCILo}}
\providecommand{\hlDecInvMtwoFDOFAflairEst}{\tbd{hlDecInvMtwoFDOFAflairEst}}
\providecommand{\hlDecInvMtwoFFDOFAburnCIHi}{\tbd{hlDecInvMtwoFFDOFAburnCIHi}}
\providecommand{\hlDecInvMtwoFFDOFAburnCILo}{\tbd{hlDecInvMtwoFFDOFAburnCILo}}
\providecommand{\hlDecInvMtwoFFDOFAburnEst}{\tbd{hlDecInvMtwoFFDOFAburnEst}}
\providecommand{\hlDecInvMtwoFFDOFAflairCIHi}{\tbd{hlDecInvMtwoFFDOFAflairCIHi}}
\providecommand{\hlDecInvMtwoFFDOFAflairCILo}{\tbd{hlDecInvMtwoFFDOFAflairCILo}}
\providecommand{\hlDecInvMtwoFFDOFAflairEst}{\tbd{hlDecInvMtwoFFDOFAflairEst}}
\providecommand{\hlDecInvMtwoFFLVDburnCIHi}{\tbd{hlDecInvMtwoFFLVDburnCIHi}}
\providecommand{\hlDecInvMtwoFFLVDburnCILo}{\tbd{hlDecInvMtwoFFLVDburnCILo}}
\providecommand{\hlDecInvMtwoFFLVDburnEst}{\tbd{hlDecInvMtwoFFLVDburnEst}}
\providecommand{\hlDecInvMtwoFFLVDflairCIHi}{\tbd{hlDecInvMtwoFFLVDflairCIHi}}
\providecommand{\hlDecInvMtwoFFLVDflairCILo}{\tbd{hlDecInvMtwoFFLVDflairCILo}}
\providecommand{\hlDecInvMtwoFFLVDflairEst}{\tbd{hlDecInvMtwoFFLVDflairEst}}
\providecommand{\hlDecInvMtwoFFRNburnCIHi}{\tbd{hlDecInvMtwoFFRNburnCIHi}}
\providecommand{\hlDecInvMtwoFFRNburnCILo}{\tbd{hlDecInvMtwoFFRNburnCILo}}
\providecommand{\hlDecInvMtwoFFRNburnEst}{\tbd{hlDecInvMtwoFFRNburnEst}}
\providecommand{\hlDecInvMtwoFFRNflairCIHi}{\tbd{hlDecInvMtwoFFRNflairCIHi}}
\providecommand{\hlDecInvMtwoFFRNflairCILo}{\tbd{hlDecInvMtwoFFRNflairCILo}}
\providecommand{\hlDecInvMtwoFFRNflairEst}{\tbd{hlDecInvMtwoFFRNflairEst}}
\providecommand{\hlDecInvMtwoFFSATburnCIHi}{\tbd{hlDecInvMtwoFFSATburnCIHi}}
\providecommand{\hlDecInvMtwoFFSATburnCILo}{\tbd{hlDecInvMtwoFFSATburnCILo}}
\providecommand{\hlDecInvMtwoFFSATburnEst}{\tbd{hlDecInvMtwoFFSATburnEst}}
\providecommand{\hlDecInvMtwoFFSATflairCIHi}{\tbd{hlDecInvMtwoFFSATflairCIHi}}
\providecommand{\hlDecInvMtwoFFSATflairCILo}{\tbd{hlDecInvMtwoFFSATflairCILo}}
\providecommand{\hlDecInvMtwoFFSATflairEst}{\tbd{hlDecInvMtwoFFSATflairEst}}
\providecommand{\hlDecInvMtwoFFTMburnCIHi}{\tbd{hlDecInvMtwoFFTMburnCIHi}}
\providecommand{\hlDecInvMtwoFFTMburnCILo}{\tbd{hlDecInvMtwoFFTMburnCILo}}
\providecommand{\hlDecInvMtwoFFTMburnEst}{\tbd{hlDecInvMtwoFFTMburnEst}}
\providecommand{\hlDecInvMtwoFFTMflairCIHi}{\tbd{hlDecInvMtwoFFTMflairCIHi}}
\providecommand{\hlDecInvMtwoFFTMflairCILo}{\tbd{hlDecInvMtwoFFTMflairCILo}}
\providecommand{\hlDecInvMtwoFFTMflairEst}{\tbd{hlDecInvMtwoFFTMflairEst}}
\providecommand{\hlDecInvMtwoFFburnCIHi}{\tbd{hlDecInvMtwoFFburnCIHi}}
\providecommand{\hlDecInvMtwoFFburnCILo}{\tbd{hlDecInvMtwoFFburnCILo}}
\providecommand{\hlDecInvMtwoFFburnEst}{\tbd{hlDecInvMtwoFFburnEst}}
\providecommand{\hlDecInvMtwoFFburnMde}{\tbd{hlDecInvMtwoFFburnMde}}
\providecommand{\hlDecInvMtwoFFburnN}{\tbd{hlDecInvMtwoFFburnN}}
\providecommand{\hlDecInvMtwoFFburnPHolm}{\tbd{hlDecInvMtwoFFburnPHolm}}
\providecommand{\hlDecInvMtwoFFburnTostCIHi}{\tbd{hlDecInvMtwoFFburnTostCIHi}}
\providecommand{\hlDecInvMtwoFFburnTostCILo}{\tbd{hlDecInvMtwoFFburnTostCILo}}
\providecommand{\hlDecInvMtwoFFflairCIHi}{\tbd{hlDecInvMtwoFFflairCIHi}}
\providecommand{\hlDecInvMtwoFFflairCILo}{\tbd{hlDecInvMtwoFFflairCILo}}
\providecommand{\hlDecInvMtwoFFflairEst}{\tbd{hlDecInvMtwoFFflairEst}}
\providecommand{\hlDecInvMtwoFFflairMde}{\tbd{hlDecInvMtwoFFflairMde}}
\providecommand{\hlDecInvMtwoFFflairN}{\tbd{hlDecInvMtwoFFflairN}}
\providecommand{\hlDecInvMtwoFFflairPHolm}{\tbd{hlDecInvMtwoFFflairPHolm}}
\providecommand{\hlDecInvMtwoFFflairTostCIHi}{\tbd{hlDecInvMtwoFFflairTostCIHi}}
\providecommand{\hlDecInvMtwoFFflairTostCILo}{\tbd{hlDecInvMtwoFFflairTostCILo}}
\providecommand{\hlDecInvMtwoFLVDburnCIHi}{\tbd{hlDecInvMtwoFLVDburnCIHi}}
\providecommand{\hlDecInvMtwoFLVDburnCILo}{\tbd{hlDecInvMtwoFLVDburnCILo}}
\providecommand{\hlDecInvMtwoFLVDburnEst}{\tbd{hlDecInvMtwoFLVDburnEst}}
\providecommand{\hlDecInvMtwoFLVDflairCIHi}{\tbd{hlDecInvMtwoFLVDflairCIHi}}
\providecommand{\hlDecInvMtwoFLVDflairCILo}{\tbd{hlDecInvMtwoFLVDflairCILo}}
\providecommand{\hlDecInvMtwoFLVDflairEst}{\tbd{hlDecInvMtwoFLVDflairEst}}
\providecommand{\hlDecInvMtwoFRNburnCIHi}{\tbd{hlDecInvMtwoFRNburnCIHi}}
\providecommand{\hlDecInvMtwoFRNburnCILo}{\tbd{hlDecInvMtwoFRNburnCILo}}
\providecommand{\hlDecInvMtwoFRNburnEst}{\tbd{hlDecInvMtwoFRNburnEst}}
\providecommand{\hlDecInvMtwoFRNflairCIHi}{\tbd{hlDecInvMtwoFRNflairCIHi}}
\providecommand{\hlDecInvMtwoFRNflairCILo}{\tbd{hlDecInvMtwoFRNflairCILo}}
\providecommand{\hlDecInvMtwoFRNflairEst}{\tbd{hlDecInvMtwoFRNflairEst}}
\providecommand{\hlDecInvMtwoFSATburnCIHi}{\tbd{hlDecInvMtwoFSATburnCIHi}}
\providecommand{\hlDecInvMtwoFSATburnCILo}{\tbd{hlDecInvMtwoFSATburnCILo}}
\providecommand{\hlDecInvMtwoFSATburnEst}{\tbd{hlDecInvMtwoFSATburnEst}}
\providecommand{\hlDecInvMtwoFSATflairCIHi}{\tbd{hlDecInvMtwoFSATflairCIHi}}
\providecommand{\hlDecInvMtwoFSATflairCILo}{\tbd{hlDecInvMtwoFSATflairCILo}}
\providecommand{\hlDecInvMtwoFSATflairEst}{\tbd{hlDecInvMtwoFSATflairEst}}
\providecommand{\hlDecInvMtwoFTMburnCIHi}{\tbd{hlDecInvMtwoFTMburnCIHi}}
\providecommand{\hlDecInvMtwoFTMburnCILo}{\tbd{hlDecInvMtwoFTMburnCILo}}
\providecommand{\hlDecInvMtwoFTMburnEst}{\tbd{hlDecInvMtwoFTMburnEst}}
\providecommand{\hlDecInvMtwoFTMflairCIHi}{\tbd{hlDecInvMtwoFTMflairCIHi}}
\providecommand{\hlDecInvMtwoFTMflairCILo}{\tbd{hlDecInvMtwoFTMflairCILo}}
\providecommand{\hlDecInvMtwoFTMflairEst}{\tbd{hlDecInvMtwoFTMflairEst}}
\providecommand{\hlDecInvMtwoFburnCIHi}{\tbd{hlDecInvMtwoFburnCIHi}}
\providecommand{\hlDecInvMtwoFburnCILo}{\tbd{hlDecInvMtwoFburnCILo}}
\providecommand{\hlDecInvMtwoFburnEst}{\tbd{hlDecInvMtwoFburnEst}}
\providecommand{\hlDecInvMtwoFburnMde}{\tbd{hlDecInvMtwoFburnMde}}
\providecommand{\hlDecInvMtwoFburnN}{\tbd{hlDecInvMtwoFburnN}}
\providecommand{\hlDecInvMtwoFburnPHolm}{\tbd{hlDecInvMtwoFburnPHolm}}
\providecommand{\hlDecInvMtwoFburnTostCIHi}{\tbd{hlDecInvMtwoFburnTostCIHi}}
\providecommand{\hlDecInvMtwoFburnTostCILo}{\tbd{hlDecInvMtwoFburnTostCILo}}
\providecommand{\hlDecInvMtwoFflairCIHi}{\tbd{hlDecInvMtwoFflairCIHi}}
\providecommand{\hlDecInvMtwoFflairCILo}{\tbd{hlDecInvMtwoFflairCILo}}
\providecommand{\hlDecInvMtwoFflairEst}{\tbd{hlDecInvMtwoFflairEst}}
\providecommand{\hlDecInvMtwoFflairMde}{\tbd{hlDecInvMtwoFflairMde}}
\providecommand{\hlDecInvMtwoFflairN}{\tbd{hlDecInvMtwoFflairN}}
\providecommand{\hlDecInvMtwoFflairPHolm}{\tbd{hlDecInvMtwoFflairPHolm}}
\providecommand{\hlDecInvMtwoFflairTostCIHi}{\tbd{hlDecInvMtwoFflairTostCIHi}}
\providecommand{\hlDecInvMtwoFflairTostCILo}{\tbd{hlDecInvMtwoFflairTostCILo}}
\providecommand{\hlDecInvRNburnCIHi}{\tbd{hlDecInvRNburnCIHi}}
\providecommand{\hlDecInvRNburnCILo}{\tbd{hlDecInvRNburnCILo}}
\providecommand{\hlDecInvRNburnEst}{\tbd{hlDecInvRNburnEst}}
\providecommand{\hlDecInvRNflairCIHi}{\tbd{hlDecInvRNflairCIHi}}
\providecommand{\hlDecInvRNflairCILo}{\tbd{hlDecInvRNflairCILo}}
\providecommand{\hlDecInvRNflairEst}{\tbd{hlDecInvRNflairEst}}
\providecommand{\hlDecInvSATburnCIHi}{\tbd{hlDecInvSATburnCIHi}}
\providecommand{\hlDecInvSATburnCILo}{\tbd{hlDecInvSATburnCILo}}
\providecommand{\hlDecInvSATburnEst}{\tbd{hlDecInvSATburnEst}}
\providecommand{\hlDecInvSATflairCIHi}{\tbd{hlDecInvSATflairCIHi}}
\providecommand{\hlDecInvSATflairCILo}{\tbd{hlDecInvSATflairCILo}}
\providecommand{\hlDecInvSATflairEst}{\tbd{hlDecInvSATflairEst}}
\providecommand{\hlDecInvSamDOFAburnCIHi}{\tbd{hlDecInvSamDOFAburnCIHi}}
\providecommand{\hlDecInvSamDOFAburnCILo}{\tbd{hlDecInvSamDOFAburnCILo}}
\providecommand{\hlDecInvSamDOFAburnEst}{\tbd{hlDecInvSamDOFAburnEst}}
\providecommand{\hlDecInvSamDOFAflairCIHi}{\tbd{hlDecInvSamDOFAflairCIHi}}
\providecommand{\hlDecInvSamDOFAflairCILo}{\tbd{hlDecInvSamDOFAflairCILo}}
\providecommand{\hlDecInvSamDOFAflairEst}{\tbd{hlDecInvSamDOFAflairEst}}
\providecommand{\hlDecInvSamLVDburnCIHi}{\tbd{hlDecInvSamLVDburnCIHi}}
\providecommand{\hlDecInvSamLVDburnCILo}{\tbd{hlDecInvSamLVDburnCILo}}
\providecommand{\hlDecInvSamLVDburnEst}{\tbd{hlDecInvSamLVDburnEst}}
\providecommand{\hlDecInvSamLVDflairCIHi}{\tbd{hlDecInvSamLVDflairCIHi}}
\providecommand{\hlDecInvSamLVDflairCILo}{\tbd{hlDecInvSamLVDflairCILo}}
\providecommand{\hlDecInvSamLVDflairEst}{\tbd{hlDecInvSamLVDflairEst}}
\providecommand{\hlDecInvSamPreDOFAburnCIHi}{\tbd{hlDecInvSamPreDOFAburnCIHi}}
\providecommand{\hlDecInvSamPreDOFAburnCILo}{\tbd{hlDecInvSamPreDOFAburnCILo}}
\providecommand{\hlDecInvSamPreDOFAburnEst}{\tbd{hlDecInvSamPreDOFAburnEst}}
\providecommand{\hlDecInvSamPreDOFAflairCIHi}{\tbd{hlDecInvSamPreDOFAflairCIHi}}
\providecommand{\hlDecInvSamPreDOFAflairCILo}{\tbd{hlDecInvSamPreDOFAflairCILo}}
\providecommand{\hlDecInvSamPreDOFAflairEst}{\tbd{hlDecInvSamPreDOFAflairEst}}
\providecommand{\hlDecInvSamPreLVDburnCIHi}{\tbd{hlDecInvSamPreLVDburnCIHi}}
\providecommand{\hlDecInvSamPreLVDburnCILo}{\tbd{hlDecInvSamPreLVDburnCILo}}
\providecommand{\hlDecInvSamPreLVDburnEst}{\tbd{hlDecInvSamPreLVDburnEst}}
\providecommand{\hlDecInvSamPreLVDflairCIHi}{\tbd{hlDecInvSamPreLVDflairCIHi}}
\providecommand{\hlDecInvSamPreLVDflairCILo}{\tbd{hlDecInvSamPreLVDflairCILo}}
\providecommand{\hlDecInvSamPreLVDflairEst}{\tbd{hlDecInvSamPreLVDflairEst}}
\providecommand{\hlDecInvSamPreRNburnCIHi}{\tbd{hlDecInvSamPreRNburnCIHi}}
\providecommand{\hlDecInvSamPreRNburnCILo}{\tbd{hlDecInvSamPreRNburnCILo}}
\providecommand{\hlDecInvSamPreRNburnEst}{\tbd{hlDecInvSamPreRNburnEst}}
\providecommand{\hlDecInvSamPreRNflairCIHi}{\tbd{hlDecInvSamPreRNflairCIHi}}
\providecommand{\hlDecInvSamPreRNflairCILo}{\tbd{hlDecInvSamPreRNflairCILo}}
\providecommand{\hlDecInvSamPreRNflairEst}{\tbd{hlDecInvSamPreRNflairEst}}
\providecommand{\hlDecInvSamPreSATburnCIHi}{\tbd{hlDecInvSamPreSATburnCIHi}}
\providecommand{\hlDecInvSamPreSATburnCILo}{\tbd{hlDecInvSamPreSATburnCILo}}
\providecommand{\hlDecInvSamPreSATburnEst}{\tbd{hlDecInvSamPreSATburnEst}}
\providecommand{\hlDecInvSamPreSATflairCIHi}{\tbd{hlDecInvSamPreSATflairCIHi}}
\providecommand{\hlDecInvSamPreSATflairCILo}{\tbd{hlDecInvSamPreSATflairCILo}}
\providecommand{\hlDecInvSamPreSATflairEst}{\tbd{hlDecInvSamPreSATflairEst}}
\providecommand{\hlDecInvSamPreTMburnCIHi}{\tbd{hlDecInvSamPreTMburnCIHi}}
\providecommand{\hlDecInvSamPreTMburnCILo}{\tbd{hlDecInvSamPreTMburnCILo}}
\providecommand{\hlDecInvSamPreTMburnEst}{\tbd{hlDecInvSamPreTMburnEst}}
\providecommand{\hlDecInvSamPreTMflairCIHi}{\tbd{hlDecInvSamPreTMflairCIHi}}
\providecommand{\hlDecInvSamPreTMflairCILo}{\tbd{hlDecInvSamPreTMflairCILo}}
\providecommand{\hlDecInvSamPreTMflairEst}{\tbd{hlDecInvSamPreTMflairEst}}
\providecommand{\hlDecInvSamPreburnCIHi}{\tbd{hlDecInvSamPreburnCIHi}}
\providecommand{\hlDecInvSamPreburnCILo}{\tbd{hlDecInvSamPreburnCILo}}
\providecommand{\hlDecInvSamPreburnEst}{\tbd{hlDecInvSamPreburnEst}}
\providecommand{\hlDecInvSamPreburnMde}{\tbd{hlDecInvSamPreburnMde}}
\providecommand{\hlDecInvSamPreburnN}{\tbd{hlDecInvSamPreburnN}}
\providecommand{\hlDecInvSamPreburnPHolm}{\tbd{hlDecInvSamPreburnPHolm}}
\providecommand{\hlDecInvSamPreburnTostCIHi}{\tbd{hlDecInvSamPreburnTostCIHi}}
\providecommand{\hlDecInvSamPreburnTostCILo}{\tbd{hlDecInvSamPreburnTostCILo}}
\providecommand{\hlDecInvSamPreflairCIHi}{\tbd{hlDecInvSamPreflairCIHi}}
\providecommand{\hlDecInvSamPreflairCILo}{\tbd{hlDecInvSamPreflairCILo}}
\providecommand{\hlDecInvSamPreflairEst}{\tbd{hlDecInvSamPreflairEst}}
\providecommand{\hlDecInvSamPreflairMde}{\tbd{hlDecInvSamPreflairMde}}
\providecommand{\hlDecInvSamPreflairN}{\tbd{hlDecInvSamPreflairN}}
\providecommand{\hlDecInvSamPreflairPHolm}{\tbd{hlDecInvSamPreflairPHolm}}
\providecommand{\hlDecInvSamPreflairTostCIHi}{\tbd{hlDecInvSamPreflairTostCIHi}}
\providecommand{\hlDecInvSamPreflairTostCILo}{\tbd{hlDecInvSamPreflairTostCILo}}
\providecommand{\hlDecInvSamRNburnCIHi}{\tbd{hlDecInvSamRNburnCIHi}}
\providecommand{\hlDecInvSamRNburnCILo}{\tbd{hlDecInvSamRNburnCILo}}
\providecommand{\hlDecInvSamRNburnEst}{\tbd{hlDecInvSamRNburnEst}}
\providecommand{\hlDecInvSamRNflairCIHi}{\tbd{hlDecInvSamRNflairCIHi}}
\providecommand{\hlDecInvSamRNflairCILo}{\tbd{hlDecInvSamRNflairCILo}}
\providecommand{\hlDecInvSamRNflairEst}{\tbd{hlDecInvSamRNflairEst}}
\providecommand{\hlDecInvSamSATburnCIHi}{\tbd{hlDecInvSamSATburnCIHi}}
\providecommand{\hlDecInvSamSATburnCILo}{\tbd{hlDecInvSamSATburnCILo}}
\providecommand{\hlDecInvSamSATburnEst}{\tbd{hlDecInvSamSATburnEst}}
\providecommand{\hlDecInvSamSATflairCIHi}{\tbd{hlDecInvSamSATflairCIHi}}
\providecommand{\hlDecInvSamSATflairCILo}{\tbd{hlDecInvSamSATflairCILo}}
\providecommand{\hlDecInvSamSATflairEst}{\tbd{hlDecInvSamSATflairEst}}
\providecommand{\hlDecInvSamTMburnCIHi}{\tbd{hlDecInvSamTMburnCIHi}}
\providecommand{\hlDecInvSamTMburnCILo}{\tbd{hlDecInvSamTMburnCILo}}
\providecommand{\hlDecInvSamTMburnEst}{\tbd{hlDecInvSamTMburnEst}}
\providecommand{\hlDecInvSamTMflairCIHi}{\tbd{hlDecInvSamTMflairCIHi}}
\providecommand{\hlDecInvSamTMflairCILo}{\tbd{hlDecInvSamTMflairCILo}}
\providecommand{\hlDecInvSamTMflairEst}{\tbd{hlDecInvSamTMflairEst}}
\providecommand{\hlDecInvSamburnCIHi}{\tbd{hlDecInvSamburnCIHi}}
\providecommand{\hlDecInvSamburnCILo}{\tbd{hlDecInvSamburnCILo}}
\providecommand{\hlDecInvSamburnEst}{\tbd{hlDecInvSamburnEst}}
\providecommand{\hlDecInvSamburnMde}{\tbd{hlDecInvSamburnMde}}
\providecommand{\hlDecInvSamburnN}{\tbd{hlDecInvSamburnN}}
\providecommand{\hlDecInvSamburnPHolm}{\tbd{hlDecInvSamburnPHolm}}
\providecommand{\hlDecInvSamburnTostCIHi}{\tbd{hlDecInvSamburnTostCIHi}}
\providecommand{\hlDecInvSamburnTostCILo}{\tbd{hlDecInvSamburnTostCILo}}
\providecommand{\hlDecInvSamflairCIHi}{\tbd{hlDecInvSamflairCIHi}}
\providecommand{\hlDecInvSamflairCILo}{\tbd{hlDecInvSamflairCILo}}
\providecommand{\hlDecInvSamflairEst}{\tbd{hlDecInvSamflairEst}}
\providecommand{\hlDecInvSamflairMde}{\tbd{hlDecInvSamflairMde}}
\providecommand{\hlDecInvSamflairN}{\tbd{hlDecInvSamflairN}}
\providecommand{\hlDecInvSamflairPHolm}{\tbd{hlDecInvSamflairPHolm}}
\providecommand{\hlDecInvSamflairTostCIHi}{\tbd{hlDecInvSamflairTostCIHi}}
\providecommand{\hlDecInvSamflairTostCILo}{\tbd{hlDecInvSamflairTostCILo}}
\providecommand{\hlDecInvSegfDOFAburnCIHi}{\tbd{hlDecInvSegfDOFAburnCIHi}}
\providecommand{\hlDecInvSegfDOFAburnCILo}{\tbd{hlDecInvSegfDOFAburnCILo}}
\providecommand{\hlDecInvSegfDOFAburnEst}{\tbd{hlDecInvSegfDOFAburnEst}}
\providecommand{\hlDecInvSegfDOFAflairCIHi}{\tbd{hlDecInvSegfDOFAflairCIHi}}
\providecommand{\hlDecInvSegfDOFAflairCILo}{\tbd{hlDecInvSegfDOFAflairCILo}}
\providecommand{\hlDecInvSegfDOFAflairEst}{\tbd{hlDecInvSegfDOFAflairEst}}
\providecommand{\hlDecInvSegfLVDburnCIHi}{\tbd{hlDecInvSegfLVDburnCIHi}}
\providecommand{\hlDecInvSegfLVDburnCILo}{\tbd{hlDecInvSegfLVDburnCILo}}
\providecommand{\hlDecInvSegfLVDburnEst}{\tbd{hlDecInvSegfLVDburnEst}}
\providecommand{\hlDecInvSegfLVDflairCIHi}{\tbd{hlDecInvSegfLVDflairCIHi}}
\providecommand{\hlDecInvSegfLVDflairCILo}{\tbd{hlDecInvSegfLVDflairCILo}}
\providecommand{\hlDecInvSegfLVDflairEst}{\tbd{hlDecInvSegfLVDflairEst}}
\providecommand{\hlDecInvSegfRNburnCIHi}{\tbd{hlDecInvSegfRNburnCIHi}}
\providecommand{\hlDecInvSegfRNburnCILo}{\tbd{hlDecInvSegfRNburnCILo}}
\providecommand{\hlDecInvSegfRNburnEst}{\tbd{hlDecInvSegfRNburnEst}}
\providecommand{\hlDecInvSegfRNflairCIHi}{\tbd{hlDecInvSegfRNflairCIHi}}
\providecommand{\hlDecInvSegfRNflairCILo}{\tbd{hlDecInvSegfRNflairCILo}}
\providecommand{\hlDecInvSegfRNflairEst}{\tbd{hlDecInvSegfRNflairEst}}
\providecommand{\hlDecInvSegfSATburnCIHi}{\tbd{hlDecInvSegfSATburnCIHi}}
\providecommand{\hlDecInvSegfSATburnCILo}{\tbd{hlDecInvSegfSATburnCILo}}
\providecommand{\hlDecInvSegfSATburnEst}{\tbd{hlDecInvSegfSATburnEst}}
\providecommand{\hlDecInvSegfSATflairCIHi}{\tbd{hlDecInvSegfSATflairCIHi}}
\providecommand{\hlDecInvSegfSATflairCILo}{\tbd{hlDecInvSegfSATflairCILo}}
\providecommand{\hlDecInvSegfSATflairEst}{\tbd{hlDecInvSegfSATflairEst}}
\providecommand{\hlDecInvSegfTMburnCIHi}{\tbd{hlDecInvSegfTMburnCIHi}}
\providecommand{\hlDecInvSegfTMburnCILo}{\tbd{hlDecInvSegfTMburnCILo}}
\providecommand{\hlDecInvSegfTMburnEst}{\tbd{hlDecInvSegfTMburnEst}}
\providecommand{\hlDecInvSegfTMflairCIHi}{\tbd{hlDecInvSegfTMflairCIHi}}
\providecommand{\hlDecInvSegfTMflairCILo}{\tbd{hlDecInvSegfTMflairCILo}}
\providecommand{\hlDecInvSegfTMflairEst}{\tbd{hlDecInvSegfTMflairEst}}
\providecommand{\hlDecInvSegfburnCIHi}{\tbd{hlDecInvSegfburnCIHi}}
\providecommand{\hlDecInvSegfburnCILo}{\tbd{hlDecInvSegfburnCILo}}
\providecommand{\hlDecInvSegfburnEst}{\tbd{hlDecInvSegfburnEst}}
\providecommand{\hlDecInvSegfburnMde}{\tbd{hlDecInvSegfburnMde}}
\providecommand{\hlDecInvSegfburnN}{\tbd{hlDecInvSegfburnN}}
\providecommand{\hlDecInvSegfburnPHolm}{\tbd{hlDecInvSegfburnPHolm}}
\providecommand{\hlDecInvSegfburnTostCIHi}{\tbd{hlDecInvSegfburnTostCIHi}}
\providecommand{\hlDecInvSegfburnTostCILo}{\tbd{hlDecInvSegfburnTostCILo}}
\providecommand{\hlDecInvSegfflairCIHi}{\tbd{hlDecInvSegfflairCIHi}}
\providecommand{\hlDecInvSegfflairCILo}{\tbd{hlDecInvSegfflairCILo}}
\providecommand{\hlDecInvSegfflairEst}{\tbd{hlDecInvSegfflairEst}}
\providecommand{\hlDecInvSegfflairMde}{\tbd{hlDecInvSegfflairMde}}
\providecommand{\hlDecInvSegfflairN}{\tbd{hlDecInvSegfflairN}}
\providecommand{\hlDecInvSegfflairPHolm}{\tbd{hlDecInvSegfflairPHolm}}
\providecommand{\hlDecInvSegfflairTostCIHi}{\tbd{hlDecInvSegfflairTostCIHi}}
\providecommand{\hlDecInvSegfflairTostCILo}{\tbd{hlDecInvSegfflairTostCILo}}
\providecommand{\hlDecInvTMburnCIHi}{\tbd{hlDecInvTMburnCIHi}}
\providecommand{\hlDecInvTMburnCILo}{\tbd{hlDecInvTMburnCILo}}
\providecommand{\hlDecInvTMburnEst}{\tbd{hlDecInvTMburnEst}}
\providecommand{\hlDecInvTMflairCIHi}{\tbd{hlDecInvTMflairCIHi}}
\providecommand{\hlDecInvTMflairCILo}{\tbd{hlDecInvTMflairCILo}}
\providecommand{\hlDecInvTMflairEst}{\tbd{hlDecInvTMflairEst}}
\providecommand{\hlDecInvburnCIHi}{\tbd{hlDecInvburnCIHi}}
\providecommand{\hlDecInvburnCILo}{\tbd{hlDecInvburnCILo}}
\providecommand{\hlDecInvburnEst}{\tbd{hlDecInvburnEst}}
\providecommand{\hlDecInvburnMde}{\tbd{hlDecInvburnMde}}
\providecommand{\hlDecInvburnN}{\tbd{hlDecInvburnN}}
\providecommand{\hlDecInvburnPHolm}{\tbd{hlDecInvburnPHolm}}
\providecommand{\hlDecInvburnTostCIHi}{\tbd{hlDecInvburnTostCIHi}}
\providecommand{\hlDecInvburnTostCILo}{\tbd{hlDecInvburnTostCILo}}
\providecommand{\hlDecInvflairCIHi}{\tbd{hlDecInvflairCIHi}}
\providecommand{\hlDecInvflairCILo}{\tbd{hlDecInvflairCILo}}
\providecommand{\hlDecInvflairEst}{\tbd{hlDecInvflairEst}}
\providecommand{\hlDecInvflairMde}{\tbd{hlDecInvflairMde}}
\providecommand{\hlDecInvflairN}{\tbd{hlDecInvflairN}}
\providecommand{\hlDecInvflairPHolm}{\tbd{hlDecInvflairPHolm}}
\providecommand{\hlDecInvflairTostCIHi}{\tbd{hlDecInvflairTostCIHi}}
\providecommand{\hlDecInvflairTostCILo}{\tbd{hlDecInvflairTostCILo}}
\providecommand{\hlDecMeanDropMtwoFFburn}{\tbd{hlDecMeanDropMtwoFFburn}}
\providecommand{\hlDecMeanDropMtwoFFflair}{\tbd{hlDecMeanDropMtwoFFflair}}
\providecommand{\hlDecMeanDropMtwoFburn}{\tbd{hlDecMeanDropMtwoFburn}}
\providecommand{\hlDecMeanDropMtwoFflair}{\tbd{hlDecMeanDropMtwoFflair}}
\providecommand{\hlDecMeanDropSamPreburn}{\tbd{hlDecMeanDropSamPreburn}}
\providecommand{\hlDecMeanDropSamPreflair}{\tbd{hlDecMeanDropSamPreflair}}
\providecommand{\hlDecMeanDropSamburn}{\tbd{hlDecMeanDropSamburn}}
\providecommand{\hlDecMeanDropSamflair}{\tbd{hlDecMeanDropSamflair}}
\providecommand{\hlDecMeanDropSegfburn}{\tbd{hlDecMeanDropSegfburn}}
\providecommand{\hlDecMeanDropSegfflair}{\tbd{hlDecMeanDropSegfflair}}
\providecommand{\hlDecMeanDropUNetburn}{\tbd{hlDecMeanDropUNetburn}}
\providecommand{\hlDecMeanDropUNetflair}{\tbd{hlDecMeanDropUNetflair}}
\providecommand{\hlDecNSixMtwoFFburnCIHi}{\tbd{hlDecNSixMtwoFFburnCIHi}}
\providecommand{\hlDecNSixMtwoFFburnCILo}{\tbd{hlDecNSixMtwoFFburnCILo}}
\providecommand{\hlDecNSixMtwoFFburnEst}{\tbd{hlDecNSixMtwoFFburnEst}}
\providecommand{\hlDecNSixMtwoFFburnMde}{\tbd{hlDecNSixMtwoFFburnMde}}
\providecommand{\hlDecNSixMtwoFFburnN}{\tbd{hlDecNSixMtwoFFburnN}}
\providecommand{\hlDecNSixMtwoFFburnPHolm}{\tbd{hlDecNSixMtwoFFburnPHolm}}
\providecommand{\hlDecNSixMtwoFFburnTostCIHi}{\tbd{hlDecNSixMtwoFFburnTostCIHi}}
\providecommand{\hlDecNSixMtwoFFburnTostCILo}{\tbd{hlDecNSixMtwoFFburnTostCILo}}
\providecommand{\hlDecNSixMtwoFFflairCIHi}{\tbd{hlDecNSixMtwoFFflairCIHi}}
\providecommand{\hlDecNSixMtwoFFflairCILo}{\tbd{hlDecNSixMtwoFFflairCILo}}
\providecommand{\hlDecNSixMtwoFFflairEst}{\tbd{hlDecNSixMtwoFFflairEst}}
\providecommand{\hlDecNSixMtwoFFflairMde}{\tbd{hlDecNSixMtwoFFflairMde}}
\providecommand{\hlDecNSixMtwoFFflairN}{\tbd{hlDecNSixMtwoFFflairN}}
\providecommand{\hlDecNSixMtwoFFflairPHolm}{\tbd{hlDecNSixMtwoFFflairPHolm}}
\providecommand{\hlDecNSixMtwoFFflairTostCIHi}{\tbd{hlDecNSixMtwoFFflairTostCIHi}}
\providecommand{\hlDecNSixMtwoFFflairTostCILo}{\tbd{hlDecNSixMtwoFFflairTostCILo}}
\providecommand{\hlDecNSixMtwoFburnCIHi}{\tbd{hlDecNSixMtwoFburnCIHi}}
\providecommand{\hlDecNSixMtwoFburnCILo}{\tbd{hlDecNSixMtwoFburnCILo}}
\providecommand{\hlDecNSixMtwoFburnEst}{\tbd{hlDecNSixMtwoFburnEst}}
\providecommand{\hlDecNSixMtwoFburnMde}{\tbd{hlDecNSixMtwoFburnMde}}
\providecommand{\hlDecNSixMtwoFburnN}{\tbd{hlDecNSixMtwoFburnN}}
\providecommand{\hlDecNSixMtwoFburnPHolm}{\tbd{hlDecNSixMtwoFburnPHolm}}
\providecommand{\hlDecNSixMtwoFburnTostCIHi}{\tbd{hlDecNSixMtwoFburnTostCIHi}}
\providecommand{\hlDecNSixMtwoFburnTostCILo}{\tbd{hlDecNSixMtwoFburnTostCILo}}
\providecommand{\hlDecNSixMtwoFflairCIHi}{\tbd{hlDecNSixMtwoFflairCIHi}}
\providecommand{\hlDecNSixMtwoFflairCILo}{\tbd{hlDecNSixMtwoFflairCILo}}
\providecommand{\hlDecNSixMtwoFflairEst}{\tbd{hlDecNSixMtwoFflairEst}}
\providecommand{\hlDecNSixMtwoFflairMde}{\tbd{hlDecNSixMtwoFflairMde}}
\providecommand{\hlDecNSixMtwoFflairN}{\tbd{hlDecNSixMtwoFflairN}}
\providecommand{\hlDecNSixMtwoFflairPHolm}{\tbd{hlDecNSixMtwoFflairPHolm}}
\providecommand{\hlDecNSixMtwoFflairTostCIHi}{\tbd{hlDecNSixMtwoFflairTostCIHi}}
\providecommand{\hlDecNSixMtwoFflairTostCILo}{\tbd{hlDecNSixMtwoFflairTostCILo}}
\providecommand{\hlDecNSixSamPreburnCIHi}{\tbd{hlDecNSixSamPreburnCIHi}}
\providecommand{\hlDecNSixSamPreburnCILo}{\tbd{hlDecNSixSamPreburnCILo}}
\providecommand{\hlDecNSixSamPreburnEst}{\tbd{hlDecNSixSamPreburnEst}}
\providecommand{\hlDecNSixSamPreburnMde}{\tbd{hlDecNSixSamPreburnMde}}
\providecommand{\hlDecNSixSamPreburnN}{\tbd{hlDecNSixSamPreburnN}}
\providecommand{\hlDecNSixSamPreburnPHolm}{\tbd{hlDecNSixSamPreburnPHolm}}
\providecommand{\hlDecNSixSamPreburnTostCIHi}{\tbd{hlDecNSixSamPreburnTostCIHi}}
\providecommand{\hlDecNSixSamPreburnTostCILo}{\tbd{hlDecNSixSamPreburnTostCILo}}
\providecommand{\hlDecNSixSamPreflairCIHi}{\tbd{hlDecNSixSamPreflairCIHi}}
\providecommand{\hlDecNSixSamPreflairCILo}{\tbd{hlDecNSixSamPreflairCILo}}
\providecommand{\hlDecNSixSamPreflairEst}{\tbd{hlDecNSixSamPreflairEst}}
\providecommand{\hlDecNSixSamPreflairMde}{\tbd{hlDecNSixSamPreflairMde}}
\providecommand{\hlDecNSixSamPreflairN}{\tbd{hlDecNSixSamPreflairN}}
\providecommand{\hlDecNSixSamPreflairPHolm}{\tbd{hlDecNSixSamPreflairPHolm}}
\providecommand{\hlDecNSixSamPreflairTostCIHi}{\tbd{hlDecNSixSamPreflairTostCIHi}}
\providecommand{\hlDecNSixSamPreflairTostCILo}{\tbd{hlDecNSixSamPreflairTostCILo}}
\providecommand{\hlDecNSixSamburnCIHi}{\tbd{hlDecNSixSamburnCIHi}}
\providecommand{\hlDecNSixSamburnCILo}{\tbd{hlDecNSixSamburnCILo}}
\providecommand{\hlDecNSixSamburnEst}{\tbd{hlDecNSixSamburnEst}}
\providecommand{\hlDecNSixSamburnMde}{\tbd{hlDecNSixSamburnMde}}
\providecommand{\hlDecNSixSamburnN}{\tbd{hlDecNSixSamburnN}}
\providecommand{\hlDecNSixSamburnPHolm}{\tbd{hlDecNSixSamburnPHolm}}
\providecommand{\hlDecNSixSamburnTostCIHi}{\tbd{hlDecNSixSamburnTostCIHi}}
\providecommand{\hlDecNSixSamburnTostCILo}{\tbd{hlDecNSixSamburnTostCILo}}
\providecommand{\hlDecNSixSamflairCIHi}{\tbd{hlDecNSixSamflairCIHi}}
\providecommand{\hlDecNSixSamflairCILo}{\tbd{hlDecNSixSamflairCILo}}
\providecommand{\hlDecNSixSamflairEst}{\tbd{hlDecNSixSamflairEst}}
\providecommand{\hlDecNSixSamflairMde}{\tbd{hlDecNSixSamflairMde}}
\providecommand{\hlDecNSixSamflairN}{\tbd{hlDecNSixSamflairN}}
\providecommand{\hlDecNSixSamflairPHolm}{\tbd{hlDecNSixSamflairPHolm}}
\providecommand{\hlDecNSixSamflairTostCIHi}{\tbd{hlDecNSixSamflairTostCIHi}}
\providecommand{\hlDecNSixSamflairTostCILo}{\tbd{hlDecNSixSamflairTostCILo}}
\providecommand{\hlDecNSixSegfburnCIHi}{\tbd{hlDecNSixSegfburnCIHi}}
\providecommand{\hlDecNSixSegfburnCILo}{\tbd{hlDecNSixSegfburnCILo}}
\providecommand{\hlDecNSixSegfburnEst}{\tbd{hlDecNSixSegfburnEst}}
\providecommand{\hlDecNSixSegfburnMde}{\tbd{hlDecNSixSegfburnMde}}
\providecommand{\hlDecNSixSegfburnN}{\tbd{hlDecNSixSegfburnN}}
\providecommand{\hlDecNSixSegfburnPHolm}{\tbd{hlDecNSixSegfburnPHolm}}
\providecommand{\hlDecNSixSegfburnTostCIHi}{\tbd{hlDecNSixSegfburnTostCIHi}}
\providecommand{\hlDecNSixSegfburnTostCILo}{\tbd{hlDecNSixSegfburnTostCILo}}
\providecommand{\hlDecNSixSegfflairCIHi}{\tbd{hlDecNSixSegfflairCIHi}}
\providecommand{\hlDecNSixSegfflairCILo}{\tbd{hlDecNSixSegfflairCILo}}
\providecommand{\hlDecNSixSegfflairEst}{\tbd{hlDecNSixSegfflairEst}}
\providecommand{\hlDecNSixSegfflairMde}{\tbd{hlDecNSixSegfflairMde}}
\providecommand{\hlDecNSixSegfflairN}{\tbd{hlDecNSixSegfflairN}}
\providecommand{\hlDecNSixSegfflairPHolm}{\tbd{hlDecNSixSegfflairPHolm}}
\providecommand{\hlDecNSixSegfflairTostCIHi}{\tbd{hlDecNSixSegfflairTostCIHi}}
\providecommand{\hlDecNSixSegfflairTostCILo}{\tbd{hlDecNSixSegfflairTostCILo}}
\providecommand{\hlDecNSixburnCIHi}{\tbd{hlDecNSixburnCIHi}}
\providecommand{\hlDecNSixburnCILo}{\tbd{hlDecNSixburnCILo}}
\providecommand{\hlDecNSixburnEst}{\tbd{hlDecNSixburnEst}}
\providecommand{\hlDecNSixburnMde}{\tbd{hlDecNSixburnMde}}
\providecommand{\hlDecNSixburnN}{\tbd{hlDecNSixburnN}}
\providecommand{\hlDecNSixburnPHolm}{\tbd{hlDecNSixburnPHolm}}
\providecommand{\hlDecNSixburnTostCIHi}{\tbd{hlDecNSixburnTostCIHi}}
\providecommand{\hlDecNSixburnTostCILo}{\tbd{hlDecNSixburnTostCILo}}
\providecommand{\hlDecNSixflairCIHi}{\tbd{hlDecNSixflairCIHi}}
\providecommand{\hlDecNSixflairCILo}{\tbd{hlDecNSixflairCILo}}
\providecommand{\hlDecNSixflairEst}{\tbd{hlDecNSixflairEst}}
\providecommand{\hlDecNSixflairMde}{\tbd{hlDecNSixflairMde}}
\providecommand{\hlDecNSixflairN}{\tbd{hlDecNSixflairN}}
\providecommand{\hlDecNSixflairPHolm}{\tbd{hlDecNSixflairPHolm}}
\providecommand{\hlDecNSixflairTostCIHi}{\tbd{hlDecNSixflairTostCIHi}}
\providecommand{\hlDecNSixflairTostCILo}{\tbd{hlDecNSixflairTostCILo}}
\providecommand{\hlDecPretrainedVsScratchburnCIHi}{\tbd{hlDecPretrainedVsScratchburnCIHi}}
\providecommand{\hlDecPretrainedVsScratchburnCILo}{\tbd{hlDecPretrainedVsScratchburnCILo}}
\providecommand{\hlDecPretrainedVsScratchburnEst}{\tbd{hlDecPretrainedVsScratchburnEst}}
\providecommand{\hlDecPretrainedVsScratchburnMde}{\tbd{hlDecPretrainedVsScratchburnMde}}
\providecommand{\hlDecPretrainedVsScratchburnN}{\tbd{hlDecPretrainedVsScratchburnN}}
\providecommand{\hlDecPretrainedVsScratchburnPHolm}{\tbd{hlDecPretrainedVsScratchburnPHolm}}
\providecommand{\hlDecPretrainedVsScratchburnTostCIHi}{\tbd{hlDecPretrainedVsScratchburnTostCIHi}}
\providecommand{\hlDecPretrainedVsScratchburnTostCILo}{\tbd{hlDecPretrainedVsScratchburnTostCILo}}
\providecommand{\hlDecPretrainedVsScratchflairCIHi}{\tbd{hlDecPretrainedVsScratchflairCIHi}}
\providecommand{\hlDecPretrainedVsScratchflairCILo}{\tbd{hlDecPretrainedVsScratchflairCILo}}
\providecommand{\hlDecPretrainedVsScratchflairEst}{\tbd{hlDecPretrainedVsScratchflairEst}}
\providecommand{\hlDecPretrainedVsScratchflairMde}{\tbd{hlDecPretrainedVsScratchflairMde}}
\providecommand{\hlDecPretrainedVsScratchflairN}{\tbd{hlDecPretrainedVsScratchflairN}}
\providecommand{\hlDecPretrainedVsScratchflairPHolm}{\tbd{hlDecPretrainedVsScratchflairPHolm}}
\providecommand{\hlDecPretrainedVsScratchflairTostCIHi}{\tbd{hlDecPretrainedVsScratchflairTostCIHi}}
\providecommand{\hlDecPretrainedVsScratchflairTostCILo}{\tbd{hlDecPretrainedVsScratchflairTostCILo}}
\providecommand{\hlDecTypeRankMtwoFFburnFour}{\tbd{hlDecTypeRankMtwoFFburnFour}}
\providecommand{\hlDecTypeRankMtwoFFburnOne}{\tbd{hlDecTypeRankMtwoFFburnOne}}
\providecommand{\hlDecTypeRankMtwoFFburnThree}{\tbd{hlDecTypeRankMtwoFFburnThree}}
\providecommand{\hlDecTypeRankMtwoFFburnTwo}{\tbd{hlDecTypeRankMtwoFFburnTwo}}
\providecommand{\hlDecTypeRankMtwoFFflairFour}{\tbd{hlDecTypeRankMtwoFFflairFour}}
\providecommand{\hlDecTypeRankMtwoFFflairOne}{\tbd{hlDecTypeRankMtwoFFflairOne}}
\providecommand{\hlDecTypeRankMtwoFFflairThree}{\tbd{hlDecTypeRankMtwoFFflairThree}}
\providecommand{\hlDecTypeRankMtwoFFflairTwo}{\tbd{hlDecTypeRankMtwoFFflairTwo}}
\providecommand{\hlDecTypeRankMtwoFburnFour}{\tbd{hlDecTypeRankMtwoFburnFour}}
\providecommand{\hlDecTypeRankMtwoFburnOne}{\tbd{hlDecTypeRankMtwoFburnOne}}
\providecommand{\hlDecTypeRankMtwoFburnThree}{\tbd{hlDecTypeRankMtwoFburnThree}}
\providecommand{\hlDecTypeRankMtwoFburnTwo}{\tbd{hlDecTypeRankMtwoFburnTwo}}
\providecommand{\hlDecTypeRankMtwoFflairFour}{\tbd{hlDecTypeRankMtwoFflairFour}}
\providecommand{\hlDecTypeRankMtwoFflairOne}{\tbd{hlDecTypeRankMtwoFflairOne}}
\providecommand{\hlDecTypeRankMtwoFflairThree}{\tbd{hlDecTypeRankMtwoFflairThree}}
\providecommand{\hlDecTypeRankMtwoFflairTwo}{\tbd{hlDecTypeRankMtwoFflairTwo}}
\providecommand{\hlDecTypeRankSamPreburnFour}{\tbd{hlDecTypeRankSamPreburnFour}}
\providecommand{\hlDecTypeRankSamPreburnOne}{\tbd{hlDecTypeRankSamPreburnOne}}
\providecommand{\hlDecTypeRankSamPreburnThree}{\tbd{hlDecTypeRankSamPreburnThree}}
\providecommand{\hlDecTypeRankSamPreburnTwo}{\tbd{hlDecTypeRankSamPreburnTwo}}
\providecommand{\hlDecTypeRankSamPreflairFour}{\tbd{hlDecTypeRankSamPreflairFour}}
\providecommand{\hlDecTypeRankSamPreflairOne}{\tbd{hlDecTypeRankSamPreflairOne}}
\providecommand{\hlDecTypeRankSamPreflairThree}{\tbd{hlDecTypeRankSamPreflairThree}}
\providecommand{\hlDecTypeRankSamPreflairTwo}{\tbd{hlDecTypeRankSamPreflairTwo}}
\providecommand{\hlDecTypeRankSamburnFour}{\tbd{hlDecTypeRankSamburnFour}}
\providecommand{\hlDecTypeRankSamburnOne}{\tbd{hlDecTypeRankSamburnOne}}
\providecommand{\hlDecTypeRankSamburnThree}{\tbd{hlDecTypeRankSamburnThree}}
\providecommand{\hlDecTypeRankSamburnTwo}{\tbd{hlDecTypeRankSamburnTwo}}
\providecommand{\hlDecTypeRankSamflairFour}{\tbd{hlDecTypeRankSamflairFour}}
\providecommand{\hlDecTypeRankSamflairOne}{\tbd{hlDecTypeRankSamflairOne}}
\providecommand{\hlDecTypeRankSamflairThree}{\tbd{hlDecTypeRankSamflairThree}}
\providecommand{\hlDecTypeRankSamflairTwo}{\tbd{hlDecTypeRankSamflairTwo}}
\providecommand{\hlDecTypeRankSegfburnFour}{\tbd{hlDecTypeRankSegfburnFour}}
\providecommand{\hlDecTypeRankSegfburnOne}{\tbd{hlDecTypeRankSegfburnOne}}
\providecommand{\hlDecTypeRankSegfburnThree}{\tbd{hlDecTypeRankSegfburnThree}}
\providecommand{\hlDecTypeRankSegfburnTwo}{\tbd{hlDecTypeRankSegfburnTwo}}
\providecommand{\hlDecTypeRankSegfflairFour}{\tbd{hlDecTypeRankSegfflairFour}}
\providecommand{\hlDecTypeRankSegfflairOne}{\tbd{hlDecTypeRankSegfflairOne}}
\providecommand{\hlDecTypeRankSegfflairThree}{\tbd{hlDecTypeRankSegfflairThree}}
\providecommand{\hlDecTypeRankSegfflairTwo}{\tbd{hlDecTypeRankSegfflairTwo}}
\providecommand{\hlDecTypeRankburnFour}{\tbd{hlDecTypeRankburnFour}}
\providecommand{\hlDecTypeRankburnOne}{\tbd{hlDecTypeRankburnOne}}
\providecommand{\hlDecTypeRankburnThree}{\tbd{hlDecTypeRankburnThree}}
\providecommand{\hlDecTypeRankburnTwo}{\tbd{hlDecTypeRankburnTwo}}
\providecommand{\hlDecTypeRankflairFour}{\tbd{hlDecTypeRankflairFour}}
\providecommand{\hlDecTypeRankflairOne}{\tbd{hlDecTypeRankflairOne}}
\providecommand{\hlDecTypeRankflairThree}{\tbd{hlDecTypeRankflairThree}}
\providecommand{\hlDecTypeRankflairTwo}{\tbd{hlDecTypeRankflairTwo}}
\providecommand{\hlDecVerdictFTwoMtwoFFburn}{\tbd{hlDecVerdictFTwoMtwoFFburn}}
\providecommand{\hlDecVerdictFTwoMtwoFFflair}{\tbd{hlDecVerdictFTwoMtwoFFflair}}
\providecommand{\hlDecVerdictFTwoMtwoFburn}{\tbd{hlDecVerdictFTwoMtwoFburn}}
\providecommand{\hlDecVerdictFTwoMtwoFflair}{\tbd{hlDecVerdictFTwoMtwoFflair}}
\providecommand{\hlDecVerdictFTwoSamPreburn}{\tbd{hlDecVerdictFTwoSamPreburn}}
\providecommand{\hlDecVerdictFTwoSamPreflair}{\tbd{hlDecVerdictFTwoSamPreflair}}
\providecommand{\hlDecVerdictFTwoSamburn}{\tbd{hlDecVerdictFTwoSamburn}}
\providecommand{\hlDecVerdictFTwoSamflair}{\tbd{hlDecVerdictFTwoSamflair}}
\providecommand{\hlDecVerdictFTwoSegfburn}{\tbd{hlDecVerdictFTwoSegfburn}}
\providecommand{\hlDecVerdictFTwoSegfflair}{\tbd{hlDecVerdictFTwoSegfflair}}
\providecommand{\hlDecVerdictFTwoburn}{\tbd{hlDecVerdictFTwoburn}}
\providecommand{\hlDecVerdictFTwoflair}{\tbd{hlDecVerdictFTwoflair}}
\providecommand{\hlDecVerdictFullVsLiteburn}{\tbd{hlDecVerdictFullVsLiteburn}}
\providecommand{\hlDecVerdictFullVsLiteflair}{\tbd{hlDecVerdictFullVsLiteflair}}
\providecommand{\hlDecVerdictMtwoFFburn}{\tbd{hlDecVerdictMtwoFFburn}}
\providecommand{\hlDecVerdictMtwoFFflair}{\tbd{hlDecVerdictMtwoFFflair}}
\providecommand{\hlDecVerdictMtwoFburn}{\tbd{hlDecVerdictMtwoFburn}}
\providecommand{\hlDecVerdictMtwoFflair}{\tbd{hlDecVerdictMtwoFflair}}
\providecommand{\hlDecVerdictNSixMtwoFFburn}{\tbd{hlDecVerdictNSixMtwoFFburn}}
\providecommand{\hlDecVerdictNSixMtwoFFflair}{\tbd{hlDecVerdictNSixMtwoFFflair}}
\providecommand{\hlDecVerdictNSixMtwoFburn}{\tbd{hlDecVerdictNSixMtwoFburn}}
\providecommand{\hlDecVerdictNSixMtwoFflair}{\tbd{hlDecVerdictNSixMtwoFflair}}
\providecommand{\hlDecVerdictNSixSamPreburn}{\tbd{hlDecVerdictNSixSamPreburn}}
\providecommand{\hlDecVerdictNSixSamPreflair}{\tbd{hlDecVerdictNSixSamPreflair}}
\providecommand{\hlDecVerdictNSixSamburn}{\tbd{hlDecVerdictNSixSamburn}}
\providecommand{\hlDecVerdictNSixSamflair}{\tbd{hlDecVerdictNSixSamflair}}
\providecommand{\hlDecVerdictNSixSegfburn}{\tbd{hlDecVerdictNSixSegfburn}}
\providecommand{\hlDecVerdictNSixSegfflair}{\tbd{hlDecVerdictNSixSegfflair}}
\providecommand{\hlDecVerdictNSixburn}{\tbd{hlDecVerdictNSixburn}}
\providecommand{\hlDecVerdictNSixflair}{\tbd{hlDecVerdictNSixflair}}
\providecommand{\hlDecVerdictPretrainedVsScratchburn}{\tbd{hlDecVerdictPretrainedVsScratchburn}}
\providecommand{\hlDecVerdictPretrainedVsScratchflair}{\tbd{hlDecVerdictPretrainedVsScratchflair}}
\providecommand{\hlDecVerdictSamPreburn}{\tbd{hlDecVerdictSamPreburn}}
\providecommand{\hlDecVerdictSamPreflair}{\tbd{hlDecVerdictSamPreflair}}
\providecommand{\hlDecVerdictSamburn}{\tbd{hlDecVerdictSamburn}}
\providecommand{\hlDecVerdictSamflair}{\tbd{hlDecVerdictSamflair}}
\providecommand{\hlDecVerdictSegfburn}{\tbd{hlDecVerdictSegfburn}}
\providecommand{\hlDecVerdictSegfflair}{\tbd{hlDecVerdictSegfflair}}
\providecommand{\hlDecVerdictburn}{\tbd{hlDecVerdictburn}}
\providecommand{\hlDecVerdictflair}{\tbd{hlDecVerdictflair}}
\providecommand{\hlDsCoarseMost}{\tbd{hlDsCoarseMost}}
\providecommand{\hlDsDone}{\tbd{hlDsDone}}
\providecommand{\hlDsFTwoEquiv}{\tbd{hlDsFTwoEquiv}}
\providecommand{\hlDsFTwoRead}{\tbd{hlDsFTwoRead}}
\providecommand{\hlDsNSixEquiv}{\tbd{hlDsNSixEquiv}}
\providecommand{\hlDsNSixEquivRest}{\tbd{hlDsNSixEquivRest}}
\providecommand{\hlDsNSixEquivSubm}{\tbd{hlDsNSixEquivSubm}}
\providecommand{\hlDsNSixRead}{\tbd{hlDsNSixRead}}
\providecommand{\hlDsNSixReadRest}{\tbd{hlDsNSixReadRest}}
\providecommand{\hlDsNSixReadSubm}{\tbd{hlDsNSixReadSubm}}
\providecommand{\hlDsOmissionMost}{\tbd{hlDsOmissionMost}}
\providecommand{\hlDsRealMore}{\tbd{hlDsRealMore}}
\providecommand{\hlDsRealRead}{\tbd{hlDsRealRead}}
\providecommand{\hlDsShiftLeast}{\tbd{hlDsShiftLeast}}
\providecommand{\hlDsTotal}{\tbd{hlDsTotal}}
\providecommand{\hlDsTotalRest}{\tbd{hlDsTotalRest}}
\providecommand{\hlDsTotalSubm}{\tbd{hlDsTotalSubm}}
\providecommand{\hlDsTypeRead}{\tbd{hlDsTypeRead}}
\providecommand{\hlExtCleanChes}{\tbd{hlExtCleanChes}}
\providecommand{\hlExtCleanCsTwelve}{\tbd{hlExtCleanCsTwelve}}
\providecommand{\hlExtCleanDfc}{\tbd{hlExtCleanDfc}}
\providecommand{\hlExtCleanEnva}{\tbd{hlExtCleanEnva}}
\providecommand{\hlExtCleanKuro}{\tbd{hlExtCleanKuro}}
\providecommand{\hlExtCleanOem}{\tbd{hlExtCleanOem}}
\providecommand{\hlExtCleanSnTwo}{\tbd{hlExtCleanSnTwo}}
\providecommand{\hlExtFOneChesCIHi}{\tbd{hlExtFOneChesCIHi}}
\providecommand{\hlExtFOneChesCILo}{\tbd{hlExtFOneChesCILo}}
\providecommand{\hlExtFOneChesEst}{\tbd{hlExtFOneChesEst}}
\providecommand{\hlExtFOneChesMde}{\tbd{hlExtFOneChesMde}}
\providecommand{\hlExtFOneChesN}{\tbd{hlExtFOneChesN}}
\providecommand{\hlExtFOneChesPHolm}{\tbd{hlExtFOneChesPHolm}}
\providecommand{\hlExtFOneChesTostCIHi}{\tbd{hlExtFOneChesTostCIHi}}
\providecommand{\hlExtFOneChesTostCILo}{\tbd{hlExtFOneChesTostCILo}}
\providecommand{\hlExtFOneCsTwelveCIHi}{\tbd{hlExtFOneCsTwelveCIHi}}
\providecommand{\hlExtFOneCsTwelveCILo}{\tbd{hlExtFOneCsTwelveCILo}}
\providecommand{\hlExtFOneCsTwelveEst}{\tbd{hlExtFOneCsTwelveEst}}
\providecommand{\hlExtFOneCsTwelveMde}{\tbd{hlExtFOneCsTwelveMde}}
\providecommand{\hlExtFOneCsTwelveN}{\tbd{hlExtFOneCsTwelveN}}
\providecommand{\hlExtFOneCsTwelvePHolm}{\tbd{hlExtFOneCsTwelvePHolm}}
\providecommand{\hlExtFOneCsTwelveTostCIHi}{\tbd{hlExtFOneCsTwelveTostCIHi}}
\providecommand{\hlExtFOneCsTwelveTostCILo}{\tbd{hlExtFOneCsTwelveTostCILo}}
\providecommand{\hlExtFOneDfcCIHi}{\tbd{hlExtFOneDfcCIHi}}
\providecommand{\hlExtFOneDfcCILo}{\tbd{hlExtFOneDfcCILo}}
\providecommand{\hlExtFOneDfcEst}{\tbd{hlExtFOneDfcEst}}
\providecommand{\hlExtFOneDfcMde}{\tbd{hlExtFOneDfcMde}}
\providecommand{\hlExtFOneDfcN}{\tbd{hlExtFOneDfcN}}
\providecommand{\hlExtFOneDfcPHolm}{\tbd{hlExtFOneDfcPHolm}}
\providecommand{\hlExtFOneDfcTostCIHi}{\tbd{hlExtFOneDfcTostCIHi}}
\providecommand{\hlExtFOneDfcTostCILo}{\tbd{hlExtFOneDfcTostCILo}}
\providecommand{\hlExtFOneEnvaCIHi}{\tbd{hlExtFOneEnvaCIHi}}
\providecommand{\hlExtFOneEnvaCILo}{\tbd{hlExtFOneEnvaCILo}}
\providecommand{\hlExtFOneEnvaEst}{\tbd{hlExtFOneEnvaEst}}
\providecommand{\hlExtFOneEnvaMde}{\tbd{hlExtFOneEnvaMde}}
\providecommand{\hlExtFOneEnvaN}{\tbd{hlExtFOneEnvaN}}
\providecommand{\hlExtFOneEnvaPHolm}{\tbd{hlExtFOneEnvaPHolm}}
\providecommand{\hlExtFOneEnvaTostCIHi}{\tbd{hlExtFOneEnvaTostCIHi}}
\providecommand{\hlExtFOneEnvaTostCILo}{\tbd{hlExtFOneEnvaTostCILo}}
\providecommand{\hlExtFOneKuroCIHi}{\tbd{hlExtFOneKuroCIHi}}
\providecommand{\hlExtFOneKuroCILo}{\tbd{hlExtFOneKuroCILo}}
\providecommand{\hlExtFOneKuroEst}{\tbd{hlExtFOneKuroEst}}
\providecommand{\hlExtFOneKuroMde}{\tbd{hlExtFOneKuroMde}}
\providecommand{\hlExtFOneKuroN}{\tbd{hlExtFOneKuroN}}
\providecommand{\hlExtFOneKuroPHolm}{\tbd{hlExtFOneKuroPHolm}}
\providecommand{\hlExtFOneKuroTostCIHi}{\tbd{hlExtFOneKuroTostCIHi}}
\providecommand{\hlExtFOneKuroTostCILo}{\tbd{hlExtFOneKuroTostCILo}}
\providecommand{\hlExtFOneOemCIHi}{\tbd{hlExtFOneOemCIHi}}
\providecommand{\hlExtFOneOemCILo}{\tbd{hlExtFOneOemCILo}}
\providecommand{\hlExtFOneOemEst}{\tbd{hlExtFOneOemEst}}
\providecommand{\hlExtFOneOemMde}{\tbd{hlExtFOneOemMde}}
\providecommand{\hlExtFOneOemN}{\tbd{hlExtFOneOemN}}
\providecommand{\hlExtFOneOemPHolm}{\tbd{hlExtFOneOemPHolm}}
\providecommand{\hlExtFOneOemTostCIHi}{\tbd{hlExtFOneOemTostCIHi}}
\providecommand{\hlExtFOneOemTostCILo}{\tbd{hlExtFOneOemTostCILo}}
\providecommand{\hlExtFOneOneChesCIHi}{\tbd{hlExtFOneOneChesCIHi}}
\providecommand{\hlExtFOneOneChesCILo}{\tbd{hlExtFOneOneChesCILo}}
\providecommand{\hlExtFOneOneChesEst}{\tbd{hlExtFOneOneChesEst}}
\providecommand{\hlExtFOneOneChesMde}{\tbd{hlExtFOneOneChesMde}}
\providecommand{\hlExtFOneOneChesN}{\tbd{hlExtFOneOneChesN}}
\providecommand{\hlExtFOneOneChesPHolm}{\tbd{hlExtFOneOneChesPHolm}}
\providecommand{\hlExtFOneOneChesTostCIHi}{\tbd{hlExtFOneOneChesTostCIHi}}
\providecommand{\hlExtFOneOneChesTostCILo}{\tbd{hlExtFOneOneChesTostCILo}}
\providecommand{\hlExtFOneOneCsTwelveCIHi}{\tbd{hlExtFOneOneCsTwelveCIHi}}
\providecommand{\hlExtFOneOneCsTwelveCILo}{\tbd{hlExtFOneOneCsTwelveCILo}}
\providecommand{\hlExtFOneOneCsTwelveEst}{\tbd{hlExtFOneOneCsTwelveEst}}
\providecommand{\hlExtFOneOneCsTwelveMde}{\tbd{hlExtFOneOneCsTwelveMde}}
\providecommand{\hlExtFOneOneCsTwelveN}{\tbd{hlExtFOneOneCsTwelveN}}
\providecommand{\hlExtFOneOneCsTwelvePHolm}{\tbd{hlExtFOneOneCsTwelvePHolm}}
\providecommand{\hlExtFOneOneCsTwelveTostCIHi}{\tbd{hlExtFOneOneCsTwelveTostCIHi}}
\providecommand{\hlExtFOneOneCsTwelveTostCILo}{\tbd{hlExtFOneOneCsTwelveTostCILo}}
\providecommand{\hlExtFOneOneDfcCIHi}{\tbd{hlExtFOneOneDfcCIHi}}
\providecommand{\hlExtFOneOneDfcCILo}{\tbd{hlExtFOneOneDfcCILo}}
\providecommand{\hlExtFOneOneDfcEst}{\tbd{hlExtFOneOneDfcEst}}
\providecommand{\hlExtFOneOneDfcMde}{\tbd{hlExtFOneOneDfcMde}}
\providecommand{\hlExtFOneOneDfcN}{\tbd{hlExtFOneOneDfcN}}
\providecommand{\hlExtFOneOneDfcPHolm}{\tbd{hlExtFOneOneDfcPHolm}}
\providecommand{\hlExtFOneOneDfcTostCIHi}{\tbd{hlExtFOneOneDfcTostCIHi}}
\providecommand{\hlExtFOneOneDfcTostCILo}{\tbd{hlExtFOneOneDfcTostCILo}}
\providecommand{\hlExtFOneOneEnvaCIHi}{\tbd{hlExtFOneOneEnvaCIHi}}
\providecommand{\hlExtFOneOneEnvaCILo}{\tbd{hlExtFOneOneEnvaCILo}}
\providecommand{\hlExtFOneOneEnvaEst}{\tbd{hlExtFOneOneEnvaEst}}
\providecommand{\hlExtFOneOneEnvaMde}{\tbd{hlExtFOneOneEnvaMde}}
\providecommand{\hlExtFOneOneEnvaN}{\tbd{hlExtFOneOneEnvaN}}
\providecommand{\hlExtFOneOneEnvaPHolm}{\tbd{hlExtFOneOneEnvaPHolm}}
\providecommand{\hlExtFOneOneEnvaTostCIHi}{\tbd{hlExtFOneOneEnvaTostCIHi}}
\providecommand{\hlExtFOneOneEnvaTostCILo}{\tbd{hlExtFOneOneEnvaTostCILo}}
\providecommand{\hlExtFOneOneKuroCIHi}{\tbd{hlExtFOneOneKuroCIHi}}
\providecommand{\hlExtFOneOneKuroCILo}{\tbd{hlExtFOneOneKuroCILo}}
\providecommand{\hlExtFOneOneKuroEst}{\tbd{hlExtFOneOneKuroEst}}
\providecommand{\hlExtFOneOneKuroMde}{\tbd{hlExtFOneOneKuroMde}}
\providecommand{\hlExtFOneOneKuroN}{\tbd{hlExtFOneOneKuroN}}
\providecommand{\hlExtFOneOneKuroPHolm}{\tbd{hlExtFOneOneKuroPHolm}}
\providecommand{\hlExtFOneOneKuroTostCIHi}{\tbd{hlExtFOneOneKuroTostCIHi}}
\providecommand{\hlExtFOneOneKuroTostCILo}{\tbd{hlExtFOneOneKuroTostCILo}}
\providecommand{\hlExtFOneOneOemCIHi}{\tbd{hlExtFOneOneOemCIHi}}
\providecommand{\hlExtFOneOneOemCILo}{\tbd{hlExtFOneOneOemCILo}}
\providecommand{\hlExtFOneOneOemEst}{\tbd{hlExtFOneOneOemEst}}
\providecommand{\hlExtFOneOneOemMde}{\tbd{hlExtFOneOneOemMde}}
\providecommand{\hlExtFOneOneOemN}{\tbd{hlExtFOneOneOemN}}
\providecommand{\hlExtFOneOneOemPHolm}{\tbd{hlExtFOneOneOemPHolm}}
\providecommand{\hlExtFOneOneOemTostCIHi}{\tbd{hlExtFOneOneOemTostCIHi}}
\providecommand{\hlExtFOneOneOemTostCILo}{\tbd{hlExtFOneOneOemTostCILo}}
\providecommand{\hlExtFOneOneSnTwoCIHi}{\tbd{hlExtFOneOneSnTwoCIHi}}
\providecommand{\hlExtFOneOneSnTwoCILo}{\tbd{hlExtFOneOneSnTwoCILo}}
\providecommand{\hlExtFOneOneSnTwoEst}{\tbd{hlExtFOneOneSnTwoEst}}
\providecommand{\hlExtFOneOneSnTwoMde}{\tbd{hlExtFOneOneSnTwoMde}}
\providecommand{\hlExtFOneOneSnTwoN}{\tbd{hlExtFOneOneSnTwoN}}
\providecommand{\hlExtFOneOneSnTwoPHolm}{\tbd{hlExtFOneOneSnTwoPHolm}}
\providecommand{\hlExtFOneOneSnTwoTostCIHi}{\tbd{hlExtFOneOneSnTwoTostCIHi}}
\providecommand{\hlExtFOneOneSnTwoTostCILo}{\tbd{hlExtFOneOneSnTwoTostCILo}}
\providecommand{\hlExtFOneSnTwoCIHi}{\tbd{hlExtFOneSnTwoCIHi}}
\providecommand{\hlExtFOneSnTwoCILo}{\tbd{hlExtFOneSnTwoCILo}}
\providecommand{\hlExtFOneSnTwoEst}{\tbd{hlExtFOneSnTwoEst}}
\providecommand{\hlExtFOneSnTwoMde}{\tbd{hlExtFOneSnTwoMde}}
\providecommand{\hlExtFOneSnTwoN}{\tbd{hlExtFOneSnTwoN}}
\providecommand{\hlExtFOneSnTwoPHolm}{\tbd{hlExtFOneSnTwoPHolm}}
\providecommand{\hlExtFOneSnTwoTostCIHi}{\tbd{hlExtFOneSnTwoTostCIHi}}
\providecommand{\hlExtFOneSnTwoTostCILo}{\tbd{hlExtFOneSnTwoTostCILo}}
\providecommand{\hlExtFTwoChesCIHi}{\tbd{hlExtFTwoChesCIHi}}
\providecommand{\hlExtFTwoChesCILo}{\tbd{hlExtFTwoChesCILo}}
\providecommand{\hlExtFTwoChesEst}{\tbd{hlExtFTwoChesEst}}
\providecommand{\hlExtFTwoChesMde}{\tbd{hlExtFTwoChesMde}}
\providecommand{\hlExtFTwoChesN}{\tbd{hlExtFTwoChesN}}
\providecommand{\hlExtFTwoChesPHolm}{\tbd{hlExtFTwoChesPHolm}}
\providecommand{\hlExtFTwoChesTostCIHi}{\tbd{hlExtFTwoChesTostCIHi}}
\providecommand{\hlExtFTwoChesTostCILo}{\tbd{hlExtFTwoChesTostCILo}}
\providecommand{\hlExtFTwoCsTwelveCIHi}{\tbd{hlExtFTwoCsTwelveCIHi}}
\providecommand{\hlExtFTwoCsTwelveCILo}{\tbd{hlExtFTwoCsTwelveCILo}}
\providecommand{\hlExtFTwoCsTwelveEst}{\tbd{hlExtFTwoCsTwelveEst}}
\providecommand{\hlExtFTwoCsTwelveMde}{\tbd{hlExtFTwoCsTwelveMde}}
\providecommand{\hlExtFTwoCsTwelveN}{\tbd{hlExtFTwoCsTwelveN}}
\providecommand{\hlExtFTwoCsTwelvePHolm}{\tbd{hlExtFTwoCsTwelvePHolm}}
\providecommand{\hlExtFTwoCsTwelveTostCIHi}{\tbd{hlExtFTwoCsTwelveTostCIHi}}
\providecommand{\hlExtFTwoCsTwelveTostCILo}{\tbd{hlExtFTwoCsTwelveTostCILo}}
\providecommand{\hlExtFTwoDfcCIHi}{\tbd{hlExtFTwoDfcCIHi}}
\providecommand{\hlExtFTwoDfcCILo}{\tbd{hlExtFTwoDfcCILo}}
\providecommand{\hlExtFTwoDfcEst}{\tbd{hlExtFTwoDfcEst}}
\providecommand{\hlExtFTwoDfcMde}{\tbd{hlExtFTwoDfcMde}}
\providecommand{\hlExtFTwoDfcN}{\tbd{hlExtFTwoDfcN}}
\providecommand{\hlExtFTwoDfcPHolm}{\tbd{hlExtFTwoDfcPHolm}}
\providecommand{\hlExtFTwoDfcTostCIHi}{\tbd{hlExtFTwoDfcTostCIHi}}
\providecommand{\hlExtFTwoDfcTostCILo}{\tbd{hlExtFTwoDfcTostCILo}}
\providecommand{\hlExtFTwoEnvaCIHi}{\tbd{hlExtFTwoEnvaCIHi}}
\providecommand{\hlExtFTwoEnvaCILo}{\tbd{hlExtFTwoEnvaCILo}}
\providecommand{\hlExtFTwoEnvaEst}{\tbd{hlExtFTwoEnvaEst}}
\providecommand{\hlExtFTwoEnvaMde}{\tbd{hlExtFTwoEnvaMde}}
\providecommand{\hlExtFTwoEnvaN}{\tbd{hlExtFTwoEnvaN}}
\providecommand{\hlExtFTwoEnvaPHolm}{\tbd{hlExtFTwoEnvaPHolm}}
\providecommand{\hlExtFTwoEnvaTostCIHi}{\tbd{hlExtFTwoEnvaTostCIHi}}
\providecommand{\hlExtFTwoEnvaTostCILo}{\tbd{hlExtFTwoEnvaTostCILo}}
\providecommand{\hlExtFTwoKuroCIHi}{\tbd{hlExtFTwoKuroCIHi}}
\providecommand{\hlExtFTwoKuroCILo}{\tbd{hlExtFTwoKuroCILo}}
\providecommand{\hlExtFTwoKuroEst}{\tbd{hlExtFTwoKuroEst}}
\providecommand{\hlExtFTwoKuroMde}{\tbd{hlExtFTwoKuroMde}}
\providecommand{\hlExtFTwoKuroN}{\tbd{hlExtFTwoKuroN}}
\providecommand{\hlExtFTwoKuroPHolm}{\tbd{hlExtFTwoKuroPHolm}}
\providecommand{\hlExtFTwoKuroTostCIHi}{\tbd{hlExtFTwoKuroTostCIHi}}
\providecommand{\hlExtFTwoKuroTostCILo}{\tbd{hlExtFTwoKuroTostCILo}}
\providecommand{\hlExtFTwoOemCIHi}{\tbd{hlExtFTwoOemCIHi}}
\providecommand{\hlExtFTwoOemCILo}{\tbd{hlExtFTwoOemCILo}}
\providecommand{\hlExtFTwoOemEst}{\tbd{hlExtFTwoOemEst}}
\providecommand{\hlExtFTwoOemMde}{\tbd{hlExtFTwoOemMde}}
\providecommand{\hlExtFTwoOemN}{\tbd{hlExtFTwoOemN}}
\providecommand{\hlExtFTwoOemPHolm}{\tbd{hlExtFTwoOemPHolm}}
\providecommand{\hlExtFTwoOemTostCIHi}{\tbd{hlExtFTwoOemTostCIHi}}
\providecommand{\hlExtFTwoOemTostCILo}{\tbd{hlExtFTwoOemTostCILo}}
\providecommand{\hlExtFTwoSnTwoCIHi}{\tbd{hlExtFTwoSnTwoCIHi}}
\providecommand{\hlExtFTwoSnTwoCILo}{\tbd{hlExtFTwoSnTwoCILo}}
\providecommand{\hlExtFTwoSnTwoEst}{\tbd{hlExtFTwoSnTwoEst}}
\providecommand{\hlExtFTwoSnTwoMde}{\tbd{hlExtFTwoSnTwoMde}}
\providecommand{\hlExtFTwoSnTwoN}{\tbd{hlExtFTwoSnTwoN}}
\providecommand{\hlExtFTwoSnTwoPHolm}{\tbd{hlExtFTwoSnTwoPHolm}}
\providecommand{\hlExtFTwoSnTwoTostCIHi}{\tbd{hlExtFTwoSnTwoTostCIHi}}
\providecommand{\hlExtFTwoSnTwoTostCILo}{\tbd{hlExtFTwoSnTwoTostCILo}}
\providecommand{\hlExtHFiveChesCIHi}{\tbd{hlExtHFiveChesCIHi}}
\providecommand{\hlExtHFiveChesCILo}{\tbd{hlExtHFiveChesCILo}}
\providecommand{\hlExtHFiveChesEst}{\tbd{hlExtHFiveChesEst}}
\providecommand{\hlExtHFiveChesMde}{\tbd{hlExtHFiveChesMde}}
\providecommand{\hlExtHFiveChesN}{\tbd{hlExtHFiveChesN}}
\providecommand{\hlExtHFiveChesPHolm}{\tbd{hlExtHFiveChesPHolm}}
\providecommand{\hlExtHFiveChesTostCIHi}{\tbd{hlExtHFiveChesTostCIHi}}
\providecommand{\hlExtHFiveChesTostCILo}{\tbd{hlExtHFiveChesTostCILo}}
\providecommand{\hlExtHFiveCsTwelveCIHi}{\tbd{hlExtHFiveCsTwelveCIHi}}
\providecommand{\hlExtHFiveCsTwelveCILo}{\tbd{hlExtHFiveCsTwelveCILo}}
\providecommand{\hlExtHFiveCsTwelveEst}{\tbd{hlExtHFiveCsTwelveEst}}
\providecommand{\hlExtHFiveCsTwelveMde}{\tbd{hlExtHFiveCsTwelveMde}}
\providecommand{\hlExtHFiveCsTwelveN}{\tbd{hlExtHFiveCsTwelveN}}
\providecommand{\hlExtHFiveCsTwelvePHolm}{\tbd{hlExtHFiveCsTwelvePHolm}}
\providecommand{\hlExtHFiveCsTwelveTostCIHi}{\tbd{hlExtHFiveCsTwelveTostCIHi}}
\providecommand{\hlExtHFiveCsTwelveTostCILo}{\tbd{hlExtHFiveCsTwelveTostCILo}}
\providecommand{\hlExtHFiveDfcCIHi}{\tbd{hlExtHFiveDfcCIHi}}
\providecommand{\hlExtHFiveDfcCILo}{\tbd{hlExtHFiveDfcCILo}}
\providecommand{\hlExtHFiveDfcEst}{\tbd{hlExtHFiveDfcEst}}
\providecommand{\hlExtHFiveDfcMde}{\tbd{hlExtHFiveDfcMde}}
\providecommand{\hlExtHFiveDfcN}{\tbd{hlExtHFiveDfcN}}
\providecommand{\hlExtHFiveDfcPHolm}{\tbd{hlExtHFiveDfcPHolm}}
\providecommand{\hlExtHFiveDfcTostCIHi}{\tbd{hlExtHFiveDfcTostCIHi}}
\providecommand{\hlExtHFiveDfcTostCILo}{\tbd{hlExtHFiveDfcTostCILo}}
\providecommand{\hlExtHFiveEnvaCIHi}{\tbd{hlExtHFiveEnvaCIHi}}
\providecommand{\hlExtHFiveEnvaCILo}{\tbd{hlExtHFiveEnvaCILo}}
\providecommand{\hlExtHFiveEnvaEst}{\tbd{hlExtHFiveEnvaEst}}
\providecommand{\hlExtHFiveEnvaMde}{\tbd{hlExtHFiveEnvaMde}}
\providecommand{\hlExtHFiveEnvaN}{\tbd{hlExtHFiveEnvaN}}
\providecommand{\hlExtHFiveEnvaPHolm}{\tbd{hlExtHFiveEnvaPHolm}}
\providecommand{\hlExtHFiveEnvaTostCIHi}{\tbd{hlExtHFiveEnvaTostCIHi}}
\providecommand{\hlExtHFiveEnvaTostCILo}{\tbd{hlExtHFiveEnvaTostCILo}}
\providecommand{\hlExtHFiveKuroCIHi}{\tbd{hlExtHFiveKuroCIHi}}
\providecommand{\hlExtHFiveKuroCILo}{\tbd{hlExtHFiveKuroCILo}}
\providecommand{\hlExtHFiveKuroEst}{\tbd{hlExtHFiveKuroEst}}
\providecommand{\hlExtHFiveKuroMde}{\tbd{hlExtHFiveKuroMde}}
\providecommand{\hlExtHFiveKuroN}{\tbd{hlExtHFiveKuroN}}
\providecommand{\hlExtHFiveKuroPHolm}{\tbd{hlExtHFiveKuroPHolm}}
\providecommand{\hlExtHFiveKuroTostCIHi}{\tbd{hlExtHFiveKuroTostCIHi}}
\providecommand{\hlExtHFiveKuroTostCILo}{\tbd{hlExtHFiveKuroTostCILo}}
\providecommand{\hlExtHFiveMtwoFChesCIHi}{\tbd{hlExtHFiveMtwoFChesCIHi}}
\providecommand{\hlExtHFiveMtwoFChesCILo}{\tbd{hlExtHFiveMtwoFChesCILo}}
\providecommand{\hlExtHFiveMtwoFChesEst}{\tbd{hlExtHFiveMtwoFChesEst}}
\providecommand{\hlExtHFiveMtwoFChesMde}{\tbd{hlExtHFiveMtwoFChesMde}}
\providecommand{\hlExtHFiveMtwoFChesN}{\tbd{hlExtHFiveMtwoFChesN}}
\providecommand{\hlExtHFiveMtwoFChesPHolm}{\tbd{hlExtHFiveMtwoFChesPHolm}}
\providecommand{\hlExtHFiveMtwoFChesTostCIHi}{\tbd{hlExtHFiveMtwoFChesTostCIHi}}
\providecommand{\hlExtHFiveMtwoFChesTostCILo}{\tbd{hlExtHFiveMtwoFChesTostCILo}}
\providecommand{\hlExtHFiveMtwoFCsTwelveCIHi}{\tbd{hlExtHFiveMtwoFCsTwelveCIHi}}
\providecommand{\hlExtHFiveMtwoFCsTwelveCILo}{\tbd{hlExtHFiveMtwoFCsTwelveCILo}}
\providecommand{\hlExtHFiveMtwoFCsTwelveEst}{\tbd{hlExtHFiveMtwoFCsTwelveEst}}
\providecommand{\hlExtHFiveMtwoFCsTwelveMde}{\tbd{hlExtHFiveMtwoFCsTwelveMde}}
\providecommand{\hlExtHFiveMtwoFCsTwelveN}{\tbd{hlExtHFiveMtwoFCsTwelveN}}
\providecommand{\hlExtHFiveMtwoFCsTwelvePHolm}{\tbd{hlExtHFiveMtwoFCsTwelvePHolm}}
\providecommand{\hlExtHFiveMtwoFCsTwelveTostCIHi}{\tbd{hlExtHFiveMtwoFCsTwelveTostCIHi}}
\providecommand{\hlExtHFiveMtwoFCsTwelveTostCILo}{\tbd{hlExtHFiveMtwoFCsTwelveTostCILo}}
\providecommand{\hlExtHFiveMtwoFDfcCIHi}{\tbd{hlExtHFiveMtwoFDfcCIHi}}
\providecommand{\hlExtHFiveMtwoFDfcCILo}{\tbd{hlExtHFiveMtwoFDfcCILo}}
\providecommand{\hlExtHFiveMtwoFDfcEst}{\tbd{hlExtHFiveMtwoFDfcEst}}
\providecommand{\hlExtHFiveMtwoFDfcMde}{\tbd{hlExtHFiveMtwoFDfcMde}}
\providecommand{\hlExtHFiveMtwoFDfcN}{\tbd{hlExtHFiveMtwoFDfcN}}
\providecommand{\hlExtHFiveMtwoFDfcPHolm}{\tbd{hlExtHFiveMtwoFDfcPHolm}}
\providecommand{\hlExtHFiveMtwoFDfcTostCIHi}{\tbd{hlExtHFiveMtwoFDfcTostCIHi}}
\providecommand{\hlExtHFiveMtwoFDfcTostCILo}{\tbd{hlExtHFiveMtwoFDfcTostCILo}}
\providecommand{\hlExtHFiveMtwoFEnvaCIHi}{\tbd{hlExtHFiveMtwoFEnvaCIHi}}
\providecommand{\hlExtHFiveMtwoFEnvaCILo}{\tbd{hlExtHFiveMtwoFEnvaCILo}}
\providecommand{\hlExtHFiveMtwoFEnvaEst}{\tbd{hlExtHFiveMtwoFEnvaEst}}
\providecommand{\hlExtHFiveMtwoFEnvaMde}{\tbd{hlExtHFiveMtwoFEnvaMde}}
\providecommand{\hlExtHFiveMtwoFEnvaN}{\tbd{hlExtHFiveMtwoFEnvaN}}
\providecommand{\hlExtHFiveMtwoFEnvaPHolm}{\tbd{hlExtHFiveMtwoFEnvaPHolm}}
\providecommand{\hlExtHFiveMtwoFEnvaTostCIHi}{\tbd{hlExtHFiveMtwoFEnvaTostCIHi}}
\providecommand{\hlExtHFiveMtwoFEnvaTostCILo}{\tbd{hlExtHFiveMtwoFEnvaTostCILo}}
\providecommand{\hlExtHFiveMtwoFKuroCIHi}{\tbd{hlExtHFiveMtwoFKuroCIHi}}
\providecommand{\hlExtHFiveMtwoFKuroCILo}{\tbd{hlExtHFiveMtwoFKuroCILo}}
\providecommand{\hlExtHFiveMtwoFKuroEst}{\tbd{hlExtHFiveMtwoFKuroEst}}
\providecommand{\hlExtHFiveMtwoFKuroMde}{\tbd{hlExtHFiveMtwoFKuroMde}}
\providecommand{\hlExtHFiveMtwoFKuroN}{\tbd{hlExtHFiveMtwoFKuroN}}
\providecommand{\hlExtHFiveMtwoFKuroPHolm}{\tbd{hlExtHFiveMtwoFKuroPHolm}}
\providecommand{\hlExtHFiveMtwoFKuroTostCIHi}{\tbd{hlExtHFiveMtwoFKuroTostCIHi}}
\providecommand{\hlExtHFiveMtwoFKuroTostCILo}{\tbd{hlExtHFiveMtwoFKuroTostCILo}}
\providecommand{\hlExtHFiveMtwoFOemCIHi}{\tbd{hlExtHFiveMtwoFOemCIHi}}
\providecommand{\hlExtHFiveMtwoFOemCILo}{\tbd{hlExtHFiveMtwoFOemCILo}}
\providecommand{\hlExtHFiveMtwoFOemEst}{\tbd{hlExtHFiveMtwoFOemEst}}
\providecommand{\hlExtHFiveMtwoFOemMde}{\tbd{hlExtHFiveMtwoFOemMde}}
\providecommand{\hlExtHFiveMtwoFOemN}{\tbd{hlExtHFiveMtwoFOemN}}
\providecommand{\hlExtHFiveMtwoFOemPHolm}{\tbd{hlExtHFiveMtwoFOemPHolm}}
\providecommand{\hlExtHFiveMtwoFOemTostCIHi}{\tbd{hlExtHFiveMtwoFOemTostCIHi}}
\providecommand{\hlExtHFiveMtwoFOemTostCILo}{\tbd{hlExtHFiveMtwoFOemTostCILo}}
\providecommand{\hlExtHFiveMtwoFSnTwoCIHi}{\tbd{hlExtHFiveMtwoFSnTwoCIHi}}
\providecommand{\hlExtHFiveMtwoFSnTwoCILo}{\tbd{hlExtHFiveMtwoFSnTwoCILo}}
\providecommand{\hlExtHFiveMtwoFSnTwoEst}{\tbd{hlExtHFiveMtwoFSnTwoEst}}
\providecommand{\hlExtHFiveMtwoFSnTwoMde}{\tbd{hlExtHFiveMtwoFSnTwoMde}}
\providecommand{\hlExtHFiveMtwoFSnTwoN}{\tbd{hlExtHFiveMtwoFSnTwoN}}
\providecommand{\hlExtHFiveMtwoFSnTwoPHolm}{\tbd{hlExtHFiveMtwoFSnTwoPHolm}}
\providecommand{\hlExtHFiveMtwoFSnTwoTostCIHi}{\tbd{hlExtHFiveMtwoFSnTwoTostCIHi}}
\providecommand{\hlExtHFiveMtwoFSnTwoTostCILo}{\tbd{hlExtHFiveMtwoFSnTwoTostCILo}}
\providecommand{\hlExtHFiveOemCIHi}{\tbd{hlExtHFiveOemCIHi}}
\providecommand{\hlExtHFiveOemCILo}{\tbd{hlExtHFiveOemCILo}}
\providecommand{\hlExtHFiveOemEst}{\tbd{hlExtHFiveOemEst}}
\providecommand{\hlExtHFiveOemMde}{\tbd{hlExtHFiveOemMde}}
\providecommand{\hlExtHFiveOemN}{\tbd{hlExtHFiveOemN}}
\providecommand{\hlExtHFiveOemPHolm}{\tbd{hlExtHFiveOemPHolm}}
\providecommand{\hlExtHFiveOemTostCIHi}{\tbd{hlExtHFiveOemTostCIHi}}
\providecommand{\hlExtHFiveOemTostCILo}{\tbd{hlExtHFiveOemTostCILo}}
\providecommand{\hlExtHFiveSamChesCIHi}{\tbd{hlExtHFiveSamChesCIHi}}
\providecommand{\hlExtHFiveSamChesCILo}{\tbd{hlExtHFiveSamChesCILo}}
\providecommand{\hlExtHFiveSamChesEst}{\tbd{hlExtHFiveSamChesEst}}
\providecommand{\hlExtHFiveSamChesMde}{\tbd{hlExtHFiveSamChesMde}}
\providecommand{\hlExtHFiveSamChesN}{\tbd{hlExtHFiveSamChesN}}
\providecommand{\hlExtHFiveSamChesPHolm}{\tbd{hlExtHFiveSamChesPHolm}}
\providecommand{\hlExtHFiveSamChesTostCIHi}{\tbd{hlExtHFiveSamChesTostCIHi}}
\providecommand{\hlExtHFiveSamChesTostCILo}{\tbd{hlExtHFiveSamChesTostCILo}}
\providecommand{\hlExtHFiveSamCsTwelveCIHi}{\tbd{hlExtHFiveSamCsTwelveCIHi}}
\providecommand{\hlExtHFiveSamCsTwelveCILo}{\tbd{hlExtHFiveSamCsTwelveCILo}}
\providecommand{\hlExtHFiveSamCsTwelveEst}{\tbd{hlExtHFiveSamCsTwelveEst}}
\providecommand{\hlExtHFiveSamCsTwelveMde}{\tbd{hlExtHFiveSamCsTwelveMde}}
\providecommand{\hlExtHFiveSamCsTwelveN}{\tbd{hlExtHFiveSamCsTwelveN}}
\providecommand{\hlExtHFiveSamCsTwelvePHolm}{\tbd{hlExtHFiveSamCsTwelvePHolm}}
\providecommand{\hlExtHFiveSamCsTwelveTostCIHi}{\tbd{hlExtHFiveSamCsTwelveTostCIHi}}
\providecommand{\hlExtHFiveSamCsTwelveTostCILo}{\tbd{hlExtHFiveSamCsTwelveTostCILo}}
\providecommand{\hlExtHFiveSamDfcCIHi}{\tbd{hlExtHFiveSamDfcCIHi}}
\providecommand{\hlExtHFiveSamDfcCILo}{\tbd{hlExtHFiveSamDfcCILo}}
\providecommand{\hlExtHFiveSamDfcEst}{\tbd{hlExtHFiveSamDfcEst}}
\providecommand{\hlExtHFiveSamDfcMde}{\tbd{hlExtHFiveSamDfcMde}}
\providecommand{\hlExtHFiveSamDfcN}{\tbd{hlExtHFiveSamDfcN}}
\providecommand{\hlExtHFiveSamDfcPHolm}{\tbd{hlExtHFiveSamDfcPHolm}}
\providecommand{\hlExtHFiveSamDfcTostCIHi}{\tbd{hlExtHFiveSamDfcTostCIHi}}
\providecommand{\hlExtHFiveSamDfcTostCILo}{\tbd{hlExtHFiveSamDfcTostCILo}}
\providecommand{\hlExtHFiveSamEnvaCIHi}{\tbd{hlExtHFiveSamEnvaCIHi}}
\providecommand{\hlExtHFiveSamEnvaCILo}{\tbd{hlExtHFiveSamEnvaCILo}}
\providecommand{\hlExtHFiveSamEnvaEst}{\tbd{hlExtHFiveSamEnvaEst}}
\providecommand{\hlExtHFiveSamEnvaMde}{\tbd{hlExtHFiveSamEnvaMde}}
\providecommand{\hlExtHFiveSamEnvaN}{\tbd{hlExtHFiveSamEnvaN}}
\providecommand{\hlExtHFiveSamEnvaPHolm}{\tbd{hlExtHFiveSamEnvaPHolm}}
\providecommand{\hlExtHFiveSamEnvaTostCIHi}{\tbd{hlExtHFiveSamEnvaTostCIHi}}
\providecommand{\hlExtHFiveSamEnvaTostCILo}{\tbd{hlExtHFiveSamEnvaTostCILo}}
\providecommand{\hlExtHFiveSamKuroCIHi}{\tbd{hlExtHFiveSamKuroCIHi}}
\providecommand{\hlExtHFiveSamKuroCILo}{\tbd{hlExtHFiveSamKuroCILo}}
\providecommand{\hlExtHFiveSamKuroEst}{\tbd{hlExtHFiveSamKuroEst}}
\providecommand{\hlExtHFiveSamKuroMde}{\tbd{hlExtHFiveSamKuroMde}}
\providecommand{\hlExtHFiveSamKuroN}{\tbd{hlExtHFiveSamKuroN}}
\providecommand{\hlExtHFiveSamKuroPHolm}{\tbd{hlExtHFiveSamKuroPHolm}}
\providecommand{\hlExtHFiveSamKuroTostCIHi}{\tbd{hlExtHFiveSamKuroTostCIHi}}
\providecommand{\hlExtHFiveSamKuroTostCILo}{\tbd{hlExtHFiveSamKuroTostCILo}}
\providecommand{\hlExtHFiveSamOemCIHi}{\tbd{hlExtHFiveSamOemCIHi}}
\providecommand{\hlExtHFiveSamOemCILo}{\tbd{hlExtHFiveSamOemCILo}}
\providecommand{\hlExtHFiveSamOemEst}{\tbd{hlExtHFiveSamOemEst}}
\providecommand{\hlExtHFiveSamOemMde}{\tbd{hlExtHFiveSamOemMde}}
\providecommand{\hlExtHFiveSamOemN}{\tbd{hlExtHFiveSamOemN}}
\providecommand{\hlExtHFiveSamOemPHolm}{\tbd{hlExtHFiveSamOemPHolm}}
\providecommand{\hlExtHFiveSamOemTostCIHi}{\tbd{hlExtHFiveSamOemTostCIHi}}
\providecommand{\hlExtHFiveSamOemTostCILo}{\tbd{hlExtHFiveSamOemTostCILo}}
\providecommand{\hlExtHFiveSamSnTwoCIHi}{\tbd{hlExtHFiveSamSnTwoCIHi}}
\providecommand{\hlExtHFiveSamSnTwoCILo}{\tbd{hlExtHFiveSamSnTwoCILo}}
\providecommand{\hlExtHFiveSamSnTwoEst}{\tbd{hlExtHFiveSamSnTwoEst}}
\providecommand{\hlExtHFiveSamSnTwoMde}{\tbd{hlExtHFiveSamSnTwoMde}}
\providecommand{\hlExtHFiveSamSnTwoN}{\tbd{hlExtHFiveSamSnTwoN}}
\providecommand{\hlExtHFiveSamSnTwoPHolm}{\tbd{hlExtHFiveSamSnTwoPHolm}}
\providecommand{\hlExtHFiveSamSnTwoTostCIHi}{\tbd{hlExtHFiveSamSnTwoTostCIHi}}
\providecommand{\hlExtHFiveSamSnTwoTostCILo}{\tbd{hlExtHFiveSamSnTwoTostCILo}}
\providecommand{\hlExtHFiveSegfChesCIHi}{\tbd{hlExtHFiveSegfChesCIHi}}
\providecommand{\hlExtHFiveSegfChesCILo}{\tbd{hlExtHFiveSegfChesCILo}}
\providecommand{\hlExtHFiveSegfChesEst}{\tbd{hlExtHFiveSegfChesEst}}
\providecommand{\hlExtHFiveSegfChesMde}{\tbd{hlExtHFiveSegfChesMde}}
\providecommand{\hlExtHFiveSegfChesN}{\tbd{hlExtHFiveSegfChesN}}
\providecommand{\hlExtHFiveSegfChesPHolm}{\tbd{hlExtHFiveSegfChesPHolm}}
\providecommand{\hlExtHFiveSegfChesTostCIHi}{\tbd{hlExtHFiveSegfChesTostCIHi}}
\providecommand{\hlExtHFiveSegfChesTostCILo}{\tbd{hlExtHFiveSegfChesTostCILo}}
\providecommand{\hlExtHFiveSegfCsTwelveCIHi}{\tbd{hlExtHFiveSegfCsTwelveCIHi}}
\providecommand{\hlExtHFiveSegfCsTwelveCILo}{\tbd{hlExtHFiveSegfCsTwelveCILo}}
\providecommand{\hlExtHFiveSegfCsTwelveEst}{\tbd{hlExtHFiveSegfCsTwelveEst}}
\providecommand{\hlExtHFiveSegfCsTwelveMde}{\tbd{hlExtHFiveSegfCsTwelveMde}}
\providecommand{\hlExtHFiveSegfCsTwelveN}{\tbd{hlExtHFiveSegfCsTwelveN}}
\providecommand{\hlExtHFiveSegfCsTwelvePHolm}{\tbd{hlExtHFiveSegfCsTwelvePHolm}}
\providecommand{\hlExtHFiveSegfCsTwelveTostCIHi}{\tbd{hlExtHFiveSegfCsTwelveTostCIHi}}
\providecommand{\hlExtHFiveSegfCsTwelveTostCILo}{\tbd{hlExtHFiveSegfCsTwelveTostCILo}}
\providecommand{\hlExtHFiveSegfDfcCIHi}{\tbd{hlExtHFiveSegfDfcCIHi}}
\providecommand{\hlExtHFiveSegfDfcCILo}{\tbd{hlExtHFiveSegfDfcCILo}}
\providecommand{\hlExtHFiveSegfDfcEst}{\tbd{hlExtHFiveSegfDfcEst}}
\providecommand{\hlExtHFiveSegfDfcMde}{\tbd{hlExtHFiveSegfDfcMde}}
\providecommand{\hlExtHFiveSegfDfcN}{\tbd{hlExtHFiveSegfDfcN}}
\providecommand{\hlExtHFiveSegfDfcPHolm}{\tbd{hlExtHFiveSegfDfcPHolm}}
\providecommand{\hlExtHFiveSegfDfcTostCIHi}{\tbd{hlExtHFiveSegfDfcTostCIHi}}
\providecommand{\hlExtHFiveSegfDfcTostCILo}{\tbd{hlExtHFiveSegfDfcTostCILo}}
\providecommand{\hlExtHFiveSegfEnvaCIHi}{\tbd{hlExtHFiveSegfEnvaCIHi}}
\providecommand{\hlExtHFiveSegfEnvaCILo}{\tbd{hlExtHFiveSegfEnvaCILo}}
\providecommand{\hlExtHFiveSegfEnvaEst}{\tbd{hlExtHFiveSegfEnvaEst}}
\providecommand{\hlExtHFiveSegfEnvaMde}{\tbd{hlExtHFiveSegfEnvaMde}}
\providecommand{\hlExtHFiveSegfEnvaN}{\tbd{hlExtHFiveSegfEnvaN}}
\providecommand{\hlExtHFiveSegfEnvaPHolm}{\tbd{hlExtHFiveSegfEnvaPHolm}}
\providecommand{\hlExtHFiveSegfEnvaTostCIHi}{\tbd{hlExtHFiveSegfEnvaTostCIHi}}
\providecommand{\hlExtHFiveSegfEnvaTostCILo}{\tbd{hlExtHFiveSegfEnvaTostCILo}}
\providecommand{\hlExtHFiveSegfKuroCIHi}{\tbd{hlExtHFiveSegfKuroCIHi}}
\providecommand{\hlExtHFiveSegfKuroCILo}{\tbd{hlExtHFiveSegfKuroCILo}}
\providecommand{\hlExtHFiveSegfKuroEst}{\tbd{hlExtHFiveSegfKuroEst}}
\providecommand{\hlExtHFiveSegfKuroMde}{\tbd{hlExtHFiveSegfKuroMde}}
\providecommand{\hlExtHFiveSegfKuroN}{\tbd{hlExtHFiveSegfKuroN}}
\providecommand{\hlExtHFiveSegfKuroPHolm}{\tbd{hlExtHFiveSegfKuroPHolm}}
\providecommand{\hlExtHFiveSegfKuroTostCIHi}{\tbd{hlExtHFiveSegfKuroTostCIHi}}
\providecommand{\hlExtHFiveSegfKuroTostCILo}{\tbd{hlExtHFiveSegfKuroTostCILo}}
\providecommand{\hlExtHFiveSegfOemCIHi}{\tbd{hlExtHFiveSegfOemCIHi}}
\providecommand{\hlExtHFiveSegfOemCILo}{\tbd{hlExtHFiveSegfOemCILo}}
\providecommand{\hlExtHFiveSegfOemEst}{\tbd{hlExtHFiveSegfOemEst}}
\providecommand{\hlExtHFiveSegfOemMde}{\tbd{hlExtHFiveSegfOemMde}}
\providecommand{\hlExtHFiveSegfOemN}{\tbd{hlExtHFiveSegfOemN}}
\providecommand{\hlExtHFiveSegfOemPHolm}{\tbd{hlExtHFiveSegfOemPHolm}}
\providecommand{\hlExtHFiveSegfOemTostCIHi}{\tbd{hlExtHFiveSegfOemTostCIHi}}
\providecommand{\hlExtHFiveSegfOemTostCILo}{\tbd{hlExtHFiveSegfOemTostCILo}}
\providecommand{\hlExtHFiveSegfSnTwoCIHi}{\tbd{hlExtHFiveSegfSnTwoCIHi}}
\providecommand{\hlExtHFiveSegfSnTwoCILo}{\tbd{hlExtHFiveSegfSnTwoCILo}}
\providecommand{\hlExtHFiveSegfSnTwoEst}{\tbd{hlExtHFiveSegfSnTwoEst}}
\providecommand{\hlExtHFiveSegfSnTwoMde}{\tbd{hlExtHFiveSegfSnTwoMde}}
\providecommand{\hlExtHFiveSegfSnTwoN}{\tbd{hlExtHFiveSegfSnTwoN}}
\providecommand{\hlExtHFiveSegfSnTwoPHolm}{\tbd{hlExtHFiveSegfSnTwoPHolm}}
\providecommand{\hlExtHFiveSegfSnTwoTostCIHi}{\tbd{hlExtHFiveSegfSnTwoTostCIHi}}
\providecommand{\hlExtHFiveSegfSnTwoTostCILo}{\tbd{hlExtHFiveSegfSnTwoTostCILo}}
\providecommand{\hlExtHFiveSnTwoCIHi}{\tbd{hlExtHFiveSnTwoCIHi}}
\providecommand{\hlExtHFiveSnTwoCILo}{\tbd{hlExtHFiveSnTwoCILo}}
\providecommand{\hlExtHFiveSnTwoEst}{\tbd{hlExtHFiveSnTwoEst}}
\providecommand{\hlExtHFiveSnTwoMde}{\tbd{hlExtHFiveSnTwoMde}}
\providecommand{\hlExtHFiveSnTwoN}{\tbd{hlExtHFiveSnTwoN}}
\providecommand{\hlExtHFiveSnTwoPHolm}{\tbd{hlExtHFiveSnTwoPHolm}}
\providecommand{\hlExtHFiveSnTwoTostCIHi}{\tbd{hlExtHFiveSnTwoTostCIHi}}
\providecommand{\hlExtHFiveSnTwoTostCILo}{\tbd{hlExtHFiveSnTwoTostCILo}}
\providecommand{\hlExtMeanDropChes}{\tbd{hlExtMeanDropChes}}
\providecommand{\hlExtMeanDropCsTwelve}{\tbd{hlExtMeanDropCsTwelve}}
\providecommand{\hlExtMeanDropDOFAChes}{\tbd{hlExtMeanDropDOFAChes}}
\providecommand{\hlExtMeanDropDOFACsTwelve}{\tbd{hlExtMeanDropDOFACsTwelve}}
\providecommand{\hlExtMeanDropDOFADfc}{\tbd{hlExtMeanDropDOFADfc}}
\providecommand{\hlExtMeanDropDOFAEnva}{\tbd{hlExtMeanDropDOFAEnva}}
\providecommand{\hlExtMeanDropDOFAKuro}{\tbd{hlExtMeanDropDOFAKuro}}
\providecommand{\hlExtMeanDropDOFAOem}{\tbd{hlExtMeanDropDOFAOem}}
\providecommand{\hlExtMeanDropDOFASnTwo}{\tbd{hlExtMeanDropDOFASnTwo}}
\providecommand{\hlExtMeanDropDfc}{\tbd{hlExtMeanDropDfc}}
\providecommand{\hlExtMeanDropEnva}{\tbd{hlExtMeanDropEnva}}
\providecommand{\hlExtMeanDropKuro}{\tbd{hlExtMeanDropKuro}}
\providecommand{\hlExtMeanDropLVDChes}{\tbd{hlExtMeanDropLVDChes}}
\providecommand{\hlExtMeanDropLVDCsTwelve}{\tbd{hlExtMeanDropLVDCsTwelve}}
\providecommand{\hlExtMeanDropLVDDfc}{\tbd{hlExtMeanDropLVDDfc}}
\providecommand{\hlExtMeanDropLVDEnva}{\tbd{hlExtMeanDropLVDEnva}}
\providecommand{\hlExtMeanDropLVDKuro}{\tbd{hlExtMeanDropLVDKuro}}
\providecommand{\hlExtMeanDropLVDOem}{\tbd{hlExtMeanDropLVDOem}}
\providecommand{\hlExtMeanDropLVDSnTwo}{\tbd{hlExtMeanDropLVDSnTwo}}
\providecommand{\hlExtMeanDropOem}{\tbd{hlExtMeanDropOem}}
\providecommand{\hlExtMeanDropRNChes}{\tbd{hlExtMeanDropRNChes}}
\providecommand{\hlExtMeanDropRNCsTwelve}{\tbd{hlExtMeanDropRNCsTwelve}}
\providecommand{\hlExtMeanDropRNDfc}{\tbd{hlExtMeanDropRNDfc}}
\providecommand{\hlExtMeanDropRNEnva}{\tbd{hlExtMeanDropRNEnva}}
\providecommand{\hlExtMeanDropRNKuro}{\tbd{hlExtMeanDropRNKuro}}
\providecommand{\hlExtMeanDropRNOem}{\tbd{hlExtMeanDropRNOem}}
\providecommand{\hlExtMeanDropRNSnTwo}{\tbd{hlExtMeanDropRNSnTwo}}
\providecommand{\hlExtMeanDropSATChes}{\tbd{hlExtMeanDropSATChes}}
\providecommand{\hlExtMeanDropSATCsTwelve}{\tbd{hlExtMeanDropSATCsTwelve}}
\providecommand{\hlExtMeanDropSATDfc}{\tbd{hlExtMeanDropSATDfc}}
\providecommand{\hlExtMeanDropSATEnva}{\tbd{hlExtMeanDropSATEnva}}
\providecommand{\hlExtMeanDropSATKuro}{\tbd{hlExtMeanDropSATKuro}}
\providecommand{\hlExtMeanDropSATOem}{\tbd{hlExtMeanDropSATOem}}
\providecommand{\hlExtMeanDropSATSnTwo}{\tbd{hlExtMeanDropSATSnTwo}}
\providecommand{\hlExtMeanDropSnTwo}{\tbd{hlExtMeanDropSnTwo}}
\providecommand{\hlExtMeanDropTMChes}{\tbd{hlExtMeanDropTMChes}}
\providecommand{\hlExtMeanDropTMCsTwelve}{\tbd{hlExtMeanDropTMCsTwelve}}
\providecommand{\hlExtMeanDropTMDfc}{\tbd{hlExtMeanDropTMDfc}}
\providecommand{\hlExtMeanDropTMEnva}{\tbd{hlExtMeanDropTMEnva}}
\providecommand{\hlExtMeanDropTMKuro}{\tbd{hlExtMeanDropTMKuro}}
\providecommand{\hlExtMeanDropTMOem}{\tbd{hlExtMeanDropTMOem}}
\providecommand{\hlExtMeanDropTMSnTwo}{\tbd{hlExtMeanDropTMSnTwo}}
\providecommand{\hlExtNSixChesCIHi}{\tbd{hlExtNSixChesCIHi}}
\providecommand{\hlExtNSixChesCILo}{\tbd{hlExtNSixChesCILo}}
\providecommand{\hlExtNSixChesEst}{\tbd{hlExtNSixChesEst}}
\providecommand{\hlExtNSixChesMde}{\tbd{hlExtNSixChesMde}}
\providecommand{\hlExtNSixChesN}{\tbd{hlExtNSixChesN}}
\providecommand{\hlExtNSixChesPHolm}{\tbd{hlExtNSixChesPHolm}}
\providecommand{\hlExtNSixChesTostCIHi}{\tbd{hlExtNSixChesTostCIHi}}
\providecommand{\hlExtNSixChesTostCILo}{\tbd{hlExtNSixChesTostCILo}}
\providecommand{\hlExtNSixCsTwelveCIHi}{\tbd{hlExtNSixCsTwelveCIHi}}
\providecommand{\hlExtNSixCsTwelveCILo}{\tbd{hlExtNSixCsTwelveCILo}}
\providecommand{\hlExtNSixCsTwelveEst}{\tbd{hlExtNSixCsTwelveEst}}
\providecommand{\hlExtNSixCsTwelveMde}{\tbd{hlExtNSixCsTwelveMde}}
\providecommand{\hlExtNSixCsTwelveN}{\tbd{hlExtNSixCsTwelveN}}
\providecommand{\hlExtNSixCsTwelvePHolm}{\tbd{hlExtNSixCsTwelvePHolm}}
\providecommand{\hlExtNSixCsTwelveTostCIHi}{\tbd{hlExtNSixCsTwelveTostCIHi}}
\providecommand{\hlExtNSixCsTwelveTostCILo}{\tbd{hlExtNSixCsTwelveTostCILo}}
\providecommand{\hlExtNSixDfcCIHi}{\tbd{hlExtNSixDfcCIHi}}
\providecommand{\hlExtNSixDfcCILo}{\tbd{hlExtNSixDfcCILo}}
\providecommand{\hlExtNSixDfcEst}{\tbd{hlExtNSixDfcEst}}
\providecommand{\hlExtNSixDfcMde}{\tbd{hlExtNSixDfcMde}}
\providecommand{\hlExtNSixDfcN}{\tbd{hlExtNSixDfcN}}
\providecommand{\hlExtNSixDfcPHolm}{\tbd{hlExtNSixDfcPHolm}}
\providecommand{\hlExtNSixDfcTostCIHi}{\tbd{hlExtNSixDfcTostCIHi}}
\providecommand{\hlExtNSixDfcTostCILo}{\tbd{hlExtNSixDfcTostCILo}}
\providecommand{\hlExtNSixEnvaCIHi}{\tbd{hlExtNSixEnvaCIHi}}
\providecommand{\hlExtNSixEnvaCILo}{\tbd{hlExtNSixEnvaCILo}}
\providecommand{\hlExtNSixEnvaEst}{\tbd{hlExtNSixEnvaEst}}
\providecommand{\hlExtNSixEnvaMde}{\tbd{hlExtNSixEnvaMde}}
\providecommand{\hlExtNSixEnvaN}{\tbd{hlExtNSixEnvaN}}
\providecommand{\hlExtNSixEnvaPHolm}{\tbd{hlExtNSixEnvaPHolm}}
\providecommand{\hlExtNSixEnvaTostCIHi}{\tbd{hlExtNSixEnvaTostCIHi}}
\providecommand{\hlExtNSixEnvaTostCILo}{\tbd{hlExtNSixEnvaTostCILo}}
\providecommand{\hlExtNSixKuroCIHi}{\tbd{hlExtNSixKuroCIHi}}
\providecommand{\hlExtNSixKuroCILo}{\tbd{hlExtNSixKuroCILo}}
\providecommand{\hlExtNSixKuroEst}{\tbd{hlExtNSixKuroEst}}
\providecommand{\hlExtNSixKuroMde}{\tbd{hlExtNSixKuroMde}}
\providecommand{\hlExtNSixKuroN}{\tbd{hlExtNSixKuroN}}
\providecommand{\hlExtNSixKuroPHolm}{\tbd{hlExtNSixKuroPHolm}}
\providecommand{\hlExtNSixKuroTostCIHi}{\tbd{hlExtNSixKuroTostCIHi}}
\providecommand{\hlExtNSixKuroTostCILo}{\tbd{hlExtNSixKuroTostCILo}}
\providecommand{\hlExtNSixOemCIHi}{\tbd{hlExtNSixOemCIHi}}
\providecommand{\hlExtNSixOemCILo}{\tbd{hlExtNSixOemCILo}}
\providecommand{\hlExtNSixOemEst}{\tbd{hlExtNSixOemEst}}
\providecommand{\hlExtNSixOemMde}{\tbd{hlExtNSixOemMde}}
\providecommand{\hlExtNSixOemN}{\tbd{hlExtNSixOemN}}
\providecommand{\hlExtNSixOemPHolm}{\tbd{hlExtNSixOemPHolm}}
\providecommand{\hlExtNSixOemTostCIHi}{\tbd{hlExtNSixOemTostCIHi}}
\providecommand{\hlExtNSixOemTostCILo}{\tbd{hlExtNSixOemTostCILo}}
\providecommand{\hlExtNSixSnTwoCIHi}{\tbd{hlExtNSixSnTwoCIHi}}
\providecommand{\hlExtNSixSnTwoCILo}{\tbd{hlExtNSixSnTwoCILo}}
\providecommand{\hlExtNSixSnTwoEst}{\tbd{hlExtNSixSnTwoEst}}
\providecommand{\hlExtNSixSnTwoMde}{\tbd{hlExtNSixSnTwoMde}}
\providecommand{\hlExtNSixSnTwoN}{\tbd{hlExtNSixSnTwoN}}
\providecommand{\hlExtNSixSnTwoPHolm}{\tbd{hlExtNSixSnTwoPHolm}}
\providecommand{\hlExtNSixSnTwoTostCIHi}{\tbd{hlExtNSixSnTwoTostCIHi}}
\providecommand{\hlExtNSixSnTwoTostCILo}{\tbd{hlExtNSixSnTwoTostCILo}}
\providecommand{\hlExtTypeRankChesFour}{\tbd{hlExtTypeRankChesFour}}
\providecommand{\hlExtTypeRankChesOne}{\tbd{hlExtTypeRankChesOne}}
\providecommand{\hlExtTypeRankChesThree}{\tbd{hlExtTypeRankChesThree}}
\providecommand{\hlExtTypeRankChesTwo}{\tbd{hlExtTypeRankChesTwo}}
\providecommand{\hlExtTypeRankCsTwelveFour}{\tbd{hlExtTypeRankCsTwelveFour}}
\providecommand{\hlExtTypeRankCsTwelveOne}{\tbd{hlExtTypeRankCsTwelveOne}}
\providecommand{\hlExtTypeRankCsTwelveThree}{\tbd{hlExtTypeRankCsTwelveThree}}
\providecommand{\hlExtTypeRankCsTwelveTwo}{\tbd{hlExtTypeRankCsTwelveTwo}}
\providecommand{\hlExtTypeRankDfcFour}{\tbd{hlExtTypeRankDfcFour}}
\providecommand{\hlExtTypeRankDfcOne}{\tbd{hlExtTypeRankDfcOne}}
\providecommand{\hlExtTypeRankDfcThree}{\tbd{hlExtTypeRankDfcThree}}
\providecommand{\hlExtTypeRankDfcTwo}{\tbd{hlExtTypeRankDfcTwo}}
\providecommand{\hlExtTypeRankEnvaFour}{\tbd{hlExtTypeRankEnvaFour}}
\providecommand{\hlExtTypeRankEnvaOne}{\tbd{hlExtTypeRankEnvaOne}}
\providecommand{\hlExtTypeRankEnvaThree}{\tbd{hlExtTypeRankEnvaThree}}
\providecommand{\hlExtTypeRankEnvaTwo}{\tbd{hlExtTypeRankEnvaTwo}}
\providecommand{\hlExtTypeRankKuroFour}{\tbd{hlExtTypeRankKuroFour}}
\providecommand{\hlExtTypeRankKuroOne}{\tbd{hlExtTypeRankKuroOne}}
\providecommand{\hlExtTypeRankKuroThree}{\tbd{hlExtTypeRankKuroThree}}
\providecommand{\hlExtTypeRankKuroTwo}{\tbd{hlExtTypeRankKuroTwo}}
\providecommand{\hlExtTypeRankOemFour}{\tbd{hlExtTypeRankOemFour}}
\providecommand{\hlExtTypeRankOemOne}{\tbd{hlExtTypeRankOemOne}}
\providecommand{\hlExtTypeRankOemThree}{\tbd{hlExtTypeRankOemThree}}
\providecommand{\hlExtTypeRankOemTwo}{\tbd{hlExtTypeRankOemTwo}}
\providecommand{\hlExtTypeRankSnTwoFour}{\tbd{hlExtTypeRankSnTwoFour}}
\providecommand{\hlExtTypeRankSnTwoOne}{\tbd{hlExtTypeRankSnTwoOne}}
\providecommand{\hlExtTypeRankSnTwoThree}{\tbd{hlExtTypeRankSnTwoThree}}
\providecommand{\hlExtTypeRankSnTwoTwo}{\tbd{hlExtTypeRankSnTwoTwo}}
\providecommand{\hlExtVerdictFOneChes}{\tbd{hlExtVerdictFOneChes}}
\providecommand{\hlExtVerdictFOneCsTwelve}{\tbd{hlExtVerdictFOneCsTwelve}}
\providecommand{\hlExtVerdictFOneDfc}{\tbd{hlExtVerdictFOneDfc}}
\providecommand{\hlExtVerdictFOneEnva}{\tbd{hlExtVerdictFOneEnva}}
\providecommand{\hlExtVerdictFOneKuro}{\tbd{hlExtVerdictFOneKuro}}
\providecommand{\hlExtVerdictFOneOem}{\tbd{hlExtVerdictFOneOem}}
\providecommand{\hlExtVerdictFOneSnTwo}{\tbd{hlExtVerdictFOneSnTwo}}
\providecommand{\hlExtVerdictFTwoChes}{\tbd{hlExtVerdictFTwoChes}}
\providecommand{\hlExtVerdictFTwoCsTwelve}{\tbd{hlExtVerdictFTwoCsTwelve}}
\providecommand{\hlExtVerdictFTwoDfc}{\tbd{hlExtVerdictFTwoDfc}}
\providecommand{\hlExtVerdictFTwoEnva}{\tbd{hlExtVerdictFTwoEnva}}
\providecommand{\hlExtVerdictFTwoKuro}{\tbd{hlExtVerdictFTwoKuro}}
\providecommand{\hlExtVerdictFTwoOem}{\tbd{hlExtVerdictFTwoOem}}
\providecommand{\hlExtVerdictFTwoSnTwo}{\tbd{hlExtVerdictFTwoSnTwo}}
\providecommand{\hlExtVerdictHFiveChes}{\tbd{hlExtVerdictHFiveChes}}
\providecommand{\hlExtVerdictHFiveCsTwelve}{\tbd{hlExtVerdictHFiveCsTwelve}}
\providecommand{\hlExtVerdictHFiveDfc}{\tbd{hlExtVerdictHFiveDfc}}
\providecommand{\hlExtVerdictHFiveEnva}{\tbd{hlExtVerdictHFiveEnva}}
\providecommand{\hlExtVerdictHFiveKuro}{\tbd{hlExtVerdictHFiveKuro}}
\providecommand{\hlExtVerdictHFiveOem}{\tbd{hlExtVerdictHFiveOem}}
\providecommand{\hlExtVerdictHFiveSnTwo}{\tbd{hlExtVerdictHFiveSnTwo}}
\providecommand{\hlExtVerdictNSixChes}{\tbd{hlExtVerdictNSixChes}}
\providecommand{\hlExtVerdictNSixCsTwelve}{\tbd{hlExtVerdictNSixCsTwelve}}
\providecommand{\hlExtVerdictNSixDfc}{\tbd{hlExtVerdictNSixDfc}}
\providecommand{\hlExtVerdictNSixEnva}{\tbd{hlExtVerdictNSixEnva}}
\providecommand{\hlExtVerdictNSixKuro}{\tbd{hlExtVerdictNSixKuro}}
\providecommand{\hlExtVerdictNSixOem}{\tbd{hlExtVerdictNSixOem}}
\providecommand{\hlExtVerdictNSixSnTwo}{\tbd{hlExtVerdictNSixSnTwo}}
\providecommand{\hlFFourAdjflairCIHi}{\tbd{hlFFourAdjflairCIHi}}
\providecommand{\hlFFourAdjflairCILo}{\tbd{hlFFourAdjflairCILo}}
\providecommand{\hlFFourAdjflairEst}{\tbd{hlFFourAdjflairEst}}
\providecommand{\hlFFourAdjflairIncludesZero}{\tbd{hlFFourAdjflairIncludesZero}}
\providecommand{\hlFFourAdjflairN}{\tbd{hlFFourAdjflairN}}
\providecommand{\hlFFourAdjflairP}{\tbd{hlFFourAdjflairP}}
\providecommand{\hlFFourAdjflairPHolm}{\tbd{hlFFourAdjflairPHolm}}
\providecommand{\hlFFourAdjflairVerdict}{\tbd{hlFFourAdjflairVerdict}}
\providecommand{\hlFFourRawflairCIHi}{\tbd{hlFFourRawflairCIHi}}
\providecommand{\hlFFourRawflairCILo}{\tbd{hlFFourRawflairCILo}}
\providecommand{\hlFFourRawflairEst}{\tbd{hlFFourRawflairEst}}
\providecommand{\hlFFourRawflairN}{\tbd{hlFFourRawflairN}}
\providecommand{\hlFFourRawflairP}{\tbd{hlFFourRawflairP}}
\providecommand{\hlFFourRawflairPHolm}{\tbd{hlFFourRawflairPHolm}}
\providecommand{\hlFOneExtFiveVerdictburn}{\tbd{hlFOneExtFiveVerdictburn}}
\providecommand{\hlFOneExtFiveVerdictflair}{\tbd{hlFOneExtFiveVerdictflair}}
\providecommand{\hlFOneExtFiveburnCIHi}{\tbd{hlFOneExtFiveburnCIHi}}
\providecommand{\hlFOneExtFiveburnCILo}{\tbd{hlFOneExtFiveburnCILo}}
\providecommand{\hlFOneExtFiveburnEst}{\tbd{hlFOneExtFiveburnEst}}
\providecommand{\hlFOneExtFiveburnMde}{\tbd{hlFOneExtFiveburnMde}}
\providecommand{\hlFOneExtFiveburnN}{\tbd{hlFOneExtFiveburnN}}
\providecommand{\hlFOneExtFiveburnPHolm}{\tbd{hlFOneExtFiveburnPHolm}}
\providecommand{\hlFOneExtFiveburnTostCIHi}{\tbd{hlFOneExtFiveburnTostCIHi}}
\providecommand{\hlFOneExtFiveburnTostCILo}{\tbd{hlFOneExtFiveburnTostCILo}}
\providecommand{\hlFOneExtFiveflairCIHi}{\tbd{hlFOneExtFiveflairCIHi}}
\providecommand{\hlFOneExtFiveflairCILo}{\tbd{hlFOneExtFiveflairCILo}}
\providecommand{\hlFOneExtFiveflairEst}{\tbd{hlFOneExtFiveflairEst}}
\providecommand{\hlFOneExtFiveflairMde}{\tbd{hlFOneExtFiveflairMde}}
\providecommand{\hlFOneExtFiveflairN}{\tbd{hlFOneExtFiveflairN}}
\providecommand{\hlFOneExtFiveflairPHolm}{\tbd{hlFOneExtFiveflairPHolm}}
\providecommand{\hlFOneExtFiveflairTostCIHi}{\tbd{hlFOneExtFiveflairTostCIHi}}
\providecommand{\hlFOneExtFiveflairTostCILo}{\tbd{hlFOneExtFiveflairTostCILo}}
\providecommand{\hlFOneExtVerdictburn}{\tbd{hlFOneExtVerdictburn}}
\providecommand{\hlFOneExtVerdictflair}{\tbd{hlFOneExtVerdictflair}}
\providecommand{\hlFOneExtburnCIHi}{\tbd{hlFOneExtburnCIHi}}
\providecommand{\hlFOneExtburnCILo}{\tbd{hlFOneExtburnCILo}}
\providecommand{\hlFOneExtburnEst}{\tbd{hlFOneExtburnEst}}
\providecommand{\hlFOneExtburnMde}{\tbd{hlFOneExtburnMde}}
\providecommand{\hlFOneExtburnN}{\tbd{hlFOneExtburnN}}
\providecommand{\hlFOneExtburnPHolm}{\tbd{hlFOneExtburnPHolm}}
\providecommand{\hlFOneExtburnTostCIHi}{\tbd{hlFOneExtburnTostCIHi}}
\providecommand{\hlFOneExtburnTostCILo}{\tbd{hlFOneExtburnTostCILo}}
\providecommand{\hlFOneExtflairCIHi}{\tbd{hlFOneExtflairCIHi}}
\providecommand{\hlFOneExtflairCILo}{\tbd{hlFOneExtflairCILo}}
\providecommand{\hlFOneExtflairEst}{\tbd{hlFOneExtflairEst}}
\providecommand{\hlFOneExtflairMde}{\tbd{hlFOneExtflairMde}}
\providecommand{\hlFOneExtflairN}{\tbd{hlFOneExtflairN}}
\providecommand{\hlFOneExtflairPHolm}{\tbd{hlFOneExtflairPHolm}}
\providecommand{\hlFOneExtflairTostCIHi}{\tbd{hlFOneExtflairTostCIHi}}
\providecommand{\hlFOneExtflairTostCILo}{\tbd{hlFOneExtflairTostCILo}}
\providecommand{\hlFThreeAdjflairCIHi}{\tbd{hlFThreeAdjflairCIHi}}
\providecommand{\hlFThreeAdjflairCILo}{\tbd{hlFThreeAdjflairCILo}}
\providecommand{\hlFThreeAdjflairEst}{\tbd{hlFThreeAdjflairEst}}
\providecommand{\hlFThreeAdjflairIncludesZero}{\tbd{hlFThreeAdjflairIncludesZero}}
\providecommand{\hlFThreeAdjflairN}{\tbd{hlFThreeAdjflairN}}
\providecommand{\hlFThreeAdjflairP}{\tbd{hlFThreeAdjflairP}}
\providecommand{\hlFThreeAdjflairPHolm}{\tbd{hlFThreeAdjflairPHolm}}
\providecommand{\hlFThreeAdjflairSlopeArm}{\tbd{hlFThreeAdjflairSlopeArm}}
\providecommand{\hlFThreeAdjflairVerdict}{\tbd{hlFThreeAdjflairVerdict}}
\providecommand{\hlFThreeRawflairCIHi}{\tbd{hlFThreeRawflairCIHi}}
\providecommand{\hlFThreeRawflairCILo}{\tbd{hlFThreeRawflairCILo}}
\providecommand{\hlFThreeRawflairEst}{\tbd{hlFThreeRawflairEst}}
\providecommand{\hlFThreeRawflairN}{\tbd{hlFThreeRawflairN}}
\providecommand{\hlFThreeRawflairP}{\tbd{hlFThreeRawflairP}}
\providecommand{\hlFThreeRawflairPHolm}{\tbd{hlFThreeRawflairPHolm}}
\providecommand{\hlFTwoExtFiveVerdictburn}{\tbd{hlFTwoExtFiveVerdictburn}}
\providecommand{\hlFTwoExtFiveVerdictflair}{\tbd{hlFTwoExtFiveVerdictflair}}
\providecommand{\hlFTwoExtFiveburnCIHi}{\tbd{hlFTwoExtFiveburnCIHi}}
\providecommand{\hlFTwoExtFiveburnCILo}{\tbd{hlFTwoExtFiveburnCILo}}
\providecommand{\hlFTwoExtFiveburnEst}{\tbd{hlFTwoExtFiveburnEst}}
\providecommand{\hlFTwoExtFiveburnMde}{\tbd{hlFTwoExtFiveburnMde}}
\providecommand{\hlFTwoExtFiveburnN}{\tbd{hlFTwoExtFiveburnN}}
\providecommand{\hlFTwoExtFiveburnPHolm}{\tbd{hlFTwoExtFiveburnPHolm}}
\providecommand{\hlFTwoExtFiveburnTostCIHi}{\tbd{hlFTwoExtFiveburnTostCIHi}}
\providecommand{\hlFTwoExtFiveburnTostCILo}{\tbd{hlFTwoExtFiveburnTostCILo}}
\providecommand{\hlFTwoExtFiveflairCIHi}{\tbd{hlFTwoExtFiveflairCIHi}}
\providecommand{\hlFTwoExtFiveflairCILo}{\tbd{hlFTwoExtFiveflairCILo}}
\providecommand{\hlFTwoExtFiveflairEst}{\tbd{hlFTwoExtFiveflairEst}}
\providecommand{\hlFTwoExtFiveflairMde}{\tbd{hlFTwoExtFiveflairMde}}
\providecommand{\hlFTwoExtFiveflairN}{\tbd{hlFTwoExtFiveflairN}}
\providecommand{\hlFTwoExtFiveflairPHolm}{\tbd{hlFTwoExtFiveflairPHolm}}
\providecommand{\hlFTwoExtFiveflairTostCIHi}{\tbd{hlFTwoExtFiveflairTostCIHi}}
\providecommand{\hlFTwoExtFiveflairTostCILo}{\tbd{hlFTwoExtFiveflairTostCILo}}
\providecommand{\hlFTwoExtVerdictburn}{\tbd{hlFTwoExtVerdictburn}}
\providecommand{\hlFTwoExtVerdictflair}{\tbd{hlFTwoExtVerdictflair}}
\providecommand{\hlFTwoExtburnCIHi}{\tbd{hlFTwoExtburnCIHi}}
\providecommand{\hlFTwoExtburnCILo}{\tbd{hlFTwoExtburnCILo}}
\providecommand{\hlFTwoExtburnEst}{\tbd{hlFTwoExtburnEst}}
\providecommand{\hlFTwoExtburnMde}{\tbd{hlFTwoExtburnMde}}
\providecommand{\hlFTwoExtburnN}{\tbd{hlFTwoExtburnN}}
\providecommand{\hlFTwoExtburnPHolm}{\tbd{hlFTwoExtburnPHolm}}
\providecommand{\hlFTwoExtburnTostCIHi}{\tbd{hlFTwoExtburnTostCIHi}}
\providecommand{\hlFTwoExtburnTostCILo}{\tbd{hlFTwoExtburnTostCILo}}
\providecommand{\hlFTwoExtflairCIHi}{\tbd{hlFTwoExtflairCIHi}}
\providecommand{\hlFTwoExtflairCILo}{\tbd{hlFTwoExtflairCILo}}
\providecommand{\hlFTwoExtflairEst}{\tbd{hlFTwoExtflairEst}}
\providecommand{\hlFTwoExtflairMde}{\tbd{hlFTwoExtflairMde}}
\providecommand{\hlFTwoExtflairN}{\tbd{hlFTwoExtflairN}}
\providecommand{\hlFTwoExtflairPHolm}{\tbd{hlFTwoExtflairPHolm}}
\providecommand{\hlFTwoExtflairTostCIHi}{\tbd{hlFTwoExtflairTostCIHi}}
\providecommand{\hlFTwoExtflairTostCILo}{\tbd{hlFTwoExtflairTostCILo}}
\providecommand{\hlFamilySeedsAllFive}{\tbd{hlFamilySeedsAllFive}}
\providecommand{\hlFlipRankChangedburn}{\tbd{hlFlipRankChangedburn}}
\providecommand{\hlFlipRankChangedflair}{\tbd{hlFlipRankChangedflair}}
\providecommand{\hlFlipRankCommonPctburn}{\tbd{hlFlipRankCommonPctburn}}
\providecommand{\hlFlipRankCommonPctflair}{\tbd{hlFlipRankCommonPctflair}}
\providecommand{\hlFlipRankburn}{\tbd{hlFlipRankburn}}
\providecommand{\hlFlipRankflair}{\tbd{hlFlipRankflair}}
\providecommand{\hlGpuHours}{\tbd{hlGpuHours}}
\providecommand{\hlGpuHoursCore}{\tbd{hlGpuHoursCore}}
\providecommand{\hlHOneSeedburnCIHi}{\tbd{hlHOneSeedburnCIHi}}
\providecommand{\hlHOneSeedburnCILo}{\tbd{hlHOneSeedburnCILo}}
\providecommand{\hlHOneSeedburnEst}{\tbd{hlHOneSeedburnEst}}
\providecommand{\hlHOneSeedburnIncludesZero}{\tbd{hlHOneSeedburnIncludesZero}}
\providecommand{\hlHOneSeedburnN}{\tbd{hlHOneSeedburnN}}
\providecommand{\hlHOneSeedflairCIHi}{\tbd{hlHOneSeedflairCIHi}}
\providecommand{\hlHOneSeedflairCILo}{\tbd{hlHOneSeedflairCILo}}
\providecommand{\hlHOneSeedflairEst}{\tbd{hlHOneSeedflairEst}}
\providecommand{\hlHOneSeedflairIncludesZero}{\tbd{hlHOneSeedflairIncludesZero}}
\providecommand{\hlHOneSeedflairN}{\tbd{hlHOneSeedflairN}}
\providecommand{\hlHTwoAdjCIHiburn}{\tbd{hlHTwoAdjCIHiburn}}
\providecommand{\hlHTwoAdjCIHiflair}{\tbd{hlHTwoAdjCIHiflair}}
\providecommand{\hlHTwoAdjCILoburn}{\tbd{hlHTwoAdjCILoburn}}
\providecommand{\hlHTwoAdjCILoflair}{\tbd{hlHTwoAdjCILoflair}}
\providecommand{\hlHTwoAdjSeedburnCIHi}{\tbd{hlHTwoAdjSeedburnCIHi}}
\providecommand{\hlHTwoAdjSeedburnCILo}{\tbd{hlHTwoAdjSeedburnCILo}}
\providecommand{\hlHTwoAdjSeedburnEst}{\tbd{hlHTwoAdjSeedburnEst}}
\providecommand{\hlHTwoAdjSeedburnIncludesZero}{\tbd{hlHTwoAdjSeedburnIncludesZero}}
\providecommand{\hlHTwoAdjSeedburnN}{\tbd{hlHTwoAdjSeedburnN}}
\providecommand{\hlHTwoAdjSeedflairCIHi}{\tbd{hlHTwoAdjSeedflairCIHi}}
\providecommand{\hlHTwoAdjSeedflairCILo}{\tbd{hlHTwoAdjSeedflairCILo}}
\providecommand{\hlHTwoAdjSeedflairEst}{\tbd{hlHTwoAdjSeedflairEst}}
\providecommand{\hlHTwoAdjSeedflairIncludesZero}{\tbd{hlHTwoAdjSeedflairIncludesZero}}
\providecommand{\hlHTwoAdjSeedflairN}{\tbd{hlHTwoAdjSeedflairN}}
\providecommand{\hlHTwoAdjburn}{\tbd{hlHTwoAdjburn}}
\providecommand{\hlHTwoAdjflair}{\tbd{hlHTwoAdjflair}}
\providecommand{\hlHTwoDiffCIHiChes}{\tbd{hlHTwoDiffCIHiChes}}
\providecommand{\hlHTwoDiffCIHiCsTwelve}{\tbd{hlHTwoDiffCIHiCsTwelve}}
\providecommand{\hlHTwoDiffCIHiDfc}{\tbd{hlHTwoDiffCIHiDfc}}
\providecommand{\hlHTwoDiffCIHiEnva}{\tbd{hlHTwoDiffCIHiEnva}}
\providecommand{\hlHTwoDiffCIHiKuro}{\tbd{hlHTwoDiffCIHiKuro}}
\providecommand{\hlHTwoDiffCIHiOem}{\tbd{hlHTwoDiffCIHiOem}}
\providecommand{\hlHTwoDiffCIHiSnTwo}{\tbd{hlHTwoDiffCIHiSnTwo}}
\providecommand{\hlHTwoDiffCIHiburn}{\tbd{hlHTwoDiffCIHiburn}}
\providecommand{\hlHTwoDiffCIHiflair}{\tbd{hlHTwoDiffCIHiflair}}
\providecommand{\hlHTwoDiffCILoChes}{\tbd{hlHTwoDiffCILoChes}}
\providecommand{\hlHTwoDiffCILoCsTwelve}{\tbd{hlHTwoDiffCILoCsTwelve}}
\providecommand{\hlHTwoDiffCILoDfc}{\tbd{hlHTwoDiffCILoDfc}}
\providecommand{\hlHTwoDiffCILoEnva}{\tbd{hlHTwoDiffCILoEnva}}
\providecommand{\hlHTwoDiffCILoKuro}{\tbd{hlHTwoDiffCILoKuro}}
\providecommand{\hlHTwoDiffCILoOem}{\tbd{hlHTwoDiffCILoOem}}
\providecommand{\hlHTwoDiffCILoSnTwo}{\tbd{hlHTwoDiffCILoSnTwo}}
\providecommand{\hlHTwoDiffCILoburn}{\tbd{hlHTwoDiffCILoburn}}
\providecommand{\hlHTwoDiffCILoflair}{\tbd{hlHTwoDiffCILoflair}}
\providecommand{\hlHTwoDiffChes}{\tbd{hlHTwoDiffChes}}
\providecommand{\hlHTwoDiffCsTwelve}{\tbd{hlHTwoDiffCsTwelve}}
\providecommand{\hlHTwoDiffDfc}{\tbd{hlHTwoDiffDfc}}
\providecommand{\hlHTwoDiffEnva}{\tbd{hlHTwoDiffEnva}}
\providecommand{\hlHTwoDiffKuro}{\tbd{hlHTwoDiffKuro}}
\providecommand{\hlHTwoDiffNChes}{\tbd{hlHTwoDiffNChes}}
\providecommand{\hlHTwoDiffNCsTwelve}{\tbd{hlHTwoDiffNCsTwelve}}
\providecommand{\hlHTwoDiffNDfc}{\tbd{hlHTwoDiffNDfc}}
\providecommand{\hlHTwoDiffNEnva}{\tbd{hlHTwoDiffNEnva}}
\providecommand{\hlHTwoDiffNKuro}{\tbd{hlHTwoDiffNKuro}}
\providecommand{\hlHTwoDiffNOem}{\tbd{hlHTwoDiffNOem}}
\providecommand{\hlHTwoDiffNSnTwo}{\tbd{hlHTwoDiffNSnTwo}}
\providecommand{\hlHTwoDiffNburn}{\tbd{hlHTwoDiffNburn}}
\providecommand{\hlHTwoDiffNflair}{\tbd{hlHTwoDiffNflair}}
\providecommand{\hlHTwoDiffOem}{\tbd{hlHTwoDiffOem}}
\providecommand{\hlHTwoDiffSnTwo}{\tbd{hlHTwoDiffSnTwo}}
\providecommand{\hlHTwoDiffburn}{\tbd{hlHTwoDiffburn}}
\providecommand{\hlHTwoDiffflair}{\tbd{hlHTwoDiffflair}}
\providecommand{\hlHTwoSeedburnCIHi}{\tbd{hlHTwoSeedburnCIHi}}
\providecommand{\hlHTwoSeedburnCILo}{\tbd{hlHTwoSeedburnCILo}}
\providecommand{\hlHTwoSeedburnEst}{\tbd{hlHTwoSeedburnEst}}
\providecommand{\hlHTwoSeedburnIncludesZero}{\tbd{hlHTwoSeedburnIncludesZero}}
\providecommand{\hlHTwoSeedburnN}{\tbd{hlHTwoSeedburnN}}
\providecommand{\hlHTwoSeedflairCIHi}{\tbd{hlHTwoSeedflairCIHi}}
\providecommand{\hlHTwoSeedflairCILo}{\tbd{hlHTwoSeedflairCILo}}
\providecommand{\hlHTwoSeedflairEst}{\tbd{hlHTwoSeedflairEst}}
\providecommand{\hlHTwoSeedflairIncludesZero}{\tbd{hlHTwoSeedflairIncludesZero}}
\providecommand{\hlHTwoSeedflairN}{\tbd{hlHTwoSeedflairN}}
\providecommand{\hlHwBlockClassesSFive}{\tbd{hlHwBlockClassesSFive}}
\providecommand{\hlHwBlockClassesSFour}{\tbd{hlHwBlockClassesSFour}}
\providecommand{\hlHwBlockClassesSOne}{\tbd{hlHwBlockClassesSOne}}
\providecommand{\hlHwBlockClassesSSix}{\tbd{hlHwBlockClassesSSix}}
\providecommand{\hlHwBlockClassesSThree}{\tbd{hlHwBlockClassesSThree}}
\providecommand{\hlHwBlockClassesSTwo}{\tbd{hlHwBlockClassesSTwo}}
\providecommand{\hlHwBlockMainClassSFive}{\tbd{hlHwBlockMainClassSFive}}
\providecommand{\hlHwBlockMainClassSFour}{\tbd{hlHwBlockMainClassSFour}}
\providecommand{\hlHwBlockMainClassSOne}{\tbd{hlHwBlockMainClassSOne}}
\providecommand{\hlHwBlockMainClassSSix}{\tbd{hlHwBlockMainClassSSix}}
\providecommand{\hlHwBlockMainClassSThree}{\tbd{hlHwBlockMainClassSThree}}
\providecommand{\hlHwBlockMainClassSTwo}{\tbd{hlHwBlockMainClassSTwo}}
\providecommand{\hlHwBlockNClassesSFive}{\tbd{hlHwBlockNClassesSFive}}
\providecommand{\hlHwBlockNClassesSFour}{\tbd{hlHwBlockNClassesSFour}}
\providecommand{\hlHwBlockNClassesSOne}{\tbd{hlHwBlockNClassesSOne}}
\providecommand{\hlHwBlockNClassesSSix}{\tbd{hlHwBlockNClassesSSix}}
\providecommand{\hlHwBlockNClassesSThree}{\tbd{hlHwBlockNClassesSThree}}
\providecommand{\hlHwBlockNClassesSTwo}{\tbd{hlHwBlockNClassesSTwo}}
\providecommand{\hlHwCleanDiffMaxburn}{\tbd{hlHwCleanDiffMaxburn}}
\providecommand{\hlHwCleanDiffMaxflair}{\tbd{hlHwCleanDiffMaxflair}}
\providecommand{\hlHwCtlArmFTwoburnCIHi}{\tbd{hlHwCtlArmFTwoburnCIHi}}
\providecommand{\hlHwCtlArmFTwoburnCILo}{\tbd{hlHwCtlArmFTwoburnCILo}}
\providecommand{\hlHwCtlArmFTwoburnEst}{\tbd{hlHwCtlArmFTwoburnEst}}
\providecommand{\hlHwCtlArmFTwoburnN}{\tbd{hlHwCtlArmFTwoburnN}}
\providecommand{\hlHwCtlArmFTwoburnVerdict}{\tbd{hlHwCtlArmFTwoburnVerdict}}
\providecommand{\hlHwCtlArmFTwoflairCIHi}{\tbd{hlHwCtlArmFTwoflairCIHi}}
\providecommand{\hlHwCtlArmFTwoflairCILo}{\tbd{hlHwCtlArmFTwoflairCILo}}
\providecommand{\hlHwCtlArmFTwoflairEst}{\tbd{hlHwCtlArmFTwoflairEst}}
\providecommand{\hlHwCtlArmFTwoflairN}{\tbd{hlHwCtlArmFTwoflairN}}
\providecommand{\hlHwCtlArmFTwoflairVerdict}{\tbd{hlHwCtlArmFTwoflairVerdict}}
\providecommand{\hlHwCtlArmNSixburnCIHi}{\tbd{hlHwCtlArmNSixburnCIHi}}
\providecommand{\hlHwCtlArmNSixburnCILo}{\tbd{hlHwCtlArmNSixburnCILo}}
\providecommand{\hlHwCtlArmNSixburnEst}{\tbd{hlHwCtlArmNSixburnEst}}
\providecommand{\hlHwCtlArmNSixburnN}{\tbd{hlHwCtlArmNSixburnN}}
\providecommand{\hlHwCtlArmNSixburnVerdict}{\tbd{hlHwCtlArmNSixburnVerdict}}
\providecommand{\hlHwCtlArmNSixflairCIHi}{\tbd{hlHwCtlArmNSixflairCIHi}}
\providecommand{\hlHwCtlArmNSixflairCILo}{\tbd{hlHwCtlArmNSixflairCILo}}
\providecommand{\hlHwCtlArmNSixflairEst}{\tbd{hlHwCtlArmNSixflairEst}}
\providecommand{\hlHwCtlArmNSixflairN}{\tbd{hlHwCtlArmNSixflairN}}
\providecommand{\hlHwCtlArmNSixflairVerdict}{\tbd{hlHwCtlArmNSixflairVerdict}}
\providecommand{\hlHwCtlDupAbs}{\tbd{hlHwCtlDupAbs}}
\providecommand{\hlHwCtlDupAbsN}{\tbd{hlHwCtlDupAbsN}}
\providecommand{\hlHwCtlDupClasses}{\tbd{hlHwCtlDupClasses}}
\providecommand{\hlHwCtlDupDropAbs}{\tbd{hlHwCtlDupDropAbs}}
\providecommand{\hlHwCtlDupDropGroups}{\tbd{hlHwCtlDupDropGroups}}
\providecommand{\hlHwCtlDupDropSigned}{\tbd{hlHwCtlDupDropSigned}}
\providecommand{\hlHwCtlDupEpochs}{\tbd{hlHwCtlDupEpochs}}
\providecommand{\hlHwCtlDupGroups}{\tbd{hlHwCtlDupGroups}}
\providecommand{\hlHwCtlDupRefClass}{\tbd{hlHwCtlDupRefClass}}
\providecommand{\hlHwCtlDupRuns}{\tbd{hlHwCtlDupRuns}}
\providecommand{\hlHwCtlDupSigned}{\tbd{hlHwCtlDupSigned}}
\providecommand{\hlHwCtlDupSignedN}{\tbd{hlHwCtlDupSignedN}}
\providecommand{\hlHwCtlDupWithin}{\tbd{hlHwCtlDupWithin}}
\providecommand{\hlHwCtlDupWithinN}{\tbd{hlHwCtlDupWithinN}}
\providecommand{\hlHwCtlFTwoburnCIHi}{\tbd{hlHwCtlFTwoburnCIHi}}
\providecommand{\hlHwCtlFTwoburnCILo}{\tbd{hlHwCtlFTwoburnCILo}}
\providecommand{\hlHwCtlFTwoburnClass}{\tbd{hlHwCtlFTwoburnClass}}
\providecommand{\hlHwCtlFTwoburnEst}{\tbd{hlHwCtlFTwoburnEst}}
\providecommand{\hlHwCtlFTwoburnN}{\tbd{hlHwCtlFTwoburnN}}
\providecommand{\hlHwCtlFTwoburnSeeds}{\tbd{hlHwCtlFTwoburnSeeds}}
\providecommand{\hlHwCtlFTwoburnVerdict}{\tbd{hlHwCtlFTwoburnVerdict}}
\providecommand{\hlHwCtlFTwoflairCIHi}{\tbd{hlHwCtlFTwoflairCIHi}}
\providecommand{\hlHwCtlFTwoflairCILo}{\tbd{hlHwCtlFTwoflairCILo}}
\providecommand{\hlHwCtlFTwoflairClass}{\tbd{hlHwCtlFTwoflairClass}}
\providecommand{\hlHwCtlFTwoflairEst}{\tbd{hlHwCtlFTwoflairEst}}
\providecommand{\hlHwCtlFTwoflairN}{\tbd{hlHwCtlFTwoflairN}}
\providecommand{\hlHwCtlFTwoflairSeeds}{\tbd{hlHwCtlFTwoflairSeeds}}
\providecommand{\hlHwCtlFTwoflairVerdict}{\tbd{hlHwCtlFTwoflairVerdict}}
\providecommand{\hlHwCtlNSixburnCIHi}{\tbd{hlHwCtlNSixburnCIHi}}
\providecommand{\hlHwCtlNSixburnCILo}{\tbd{hlHwCtlNSixburnCILo}}
\providecommand{\hlHwCtlNSixburnClass}{\tbd{hlHwCtlNSixburnClass}}
\providecommand{\hlHwCtlNSixburnEst}{\tbd{hlHwCtlNSixburnEst}}
\providecommand{\hlHwCtlNSixburnN}{\tbd{hlHwCtlNSixburnN}}
\providecommand{\hlHwCtlNSixburnSeeds}{\tbd{hlHwCtlNSixburnSeeds}}
\providecommand{\hlHwCtlNSixburnVerdict}{\tbd{hlHwCtlNSixburnVerdict}}
\providecommand{\hlHwCtlNSixflairCIHi}{\tbd{hlHwCtlNSixflairCIHi}}
\providecommand{\hlHwCtlNSixflairCILo}{\tbd{hlHwCtlNSixflairCILo}}
\providecommand{\hlHwCtlNSixflairClass}{\tbd{hlHwCtlNSixflairClass}}
\providecommand{\hlHwCtlNSixflairEst}{\tbd{hlHwCtlNSixflairEst}}
\providecommand{\hlHwCtlNSixflairN}{\tbd{hlHwCtlNSixflairN}}
\providecommand{\hlHwCtlNSixflairSeeds}{\tbd{hlHwCtlNSixflairSeeds}}
\providecommand{\hlHwCtlNSixflairVerdict}{\tbd{hlHwCtlNSixflairVerdict}}
\providecommand{\hlHwCtlReplicateRuns}{\tbd{hlHwCtlReplicateRuns}}
\providecommand{\hlHwCtlSettleFTwoburnClass}{\tbd{hlHwCtlSettleFTwoburnClass}}
\providecommand{\hlHwCtlSettleFTwoburnRuns}{\tbd{hlHwCtlSettleFTwoburnRuns}}
\providecommand{\hlHwCtlSettleFTwoflairClass}{\tbd{hlHwCtlSettleFTwoflairClass}}
\providecommand{\hlHwCtlSettleFTwoflairRuns}{\tbd{hlHwCtlSettleFTwoflairRuns}}
\providecommand{\hlHwCtlSettleNSixburnClass}{\tbd{hlHwCtlSettleNSixburnClass}}
\providecommand{\hlHwCtlSettleNSixburnRuns}{\tbd{hlHwCtlSettleNSixburnRuns}}
\providecommand{\hlHwCtlSettleNSixflairClass}{\tbd{hlHwCtlSettleNSixflairClass}}
\providecommand{\hlHwCtlSettleNSixflairRuns}{\tbd{hlHwCtlSettleNSixflairRuns}}
\providecommand{\hlHwDropDiffMaxburn}{\tbd{hlHwDropDiffMaxburn}}
\providecommand{\hlHwDropDiffMaxflair}{\tbd{hlHwDropDiffMaxflair}}
\providecommand{\hlHwDropDiffMeanburn}{\tbd{hlHwDropDiffMeanburn}}
\providecommand{\hlHwDropDiffMeanflair}{\tbd{hlHwDropDiffMeanflair}}
\providecommand{\hlHwDropDiffSignedMeanburn}{\tbd{hlHwDropDiffSignedMeanburn}}
\providecommand{\hlHwDropDiffSignedMeanflair}{\tbd{hlHwDropDiffSignedMeanflair}}
\providecommand{\hlHwMixedAOneLOneNburn}{\tbd{hlHwMixedAOneLOneNburn}}
\providecommand{\hlHwMixedAOneLOneNflair}{\tbd{hlHwMixedAOneLOneNflair}}
\providecommand{\hlHwMixedAOneNburn}{\tbd{hlHwMixedAOneNburn}}
\providecommand{\hlHwMixedAOneNflair}{\tbd{hlHwMixedAOneNflair}}
\providecommand{\hlHwMixedNburn}{\tbd{hlHwMixedNburn}}
\providecommand{\hlHwMixedNflair}{\tbd{hlHwMixedNflair}}
\providecommand{\hlHwNSixCellsNburn}{\tbd{hlHwNSixCellsNburn}}
\providecommand{\hlHwNSixCellsNflair}{\tbd{hlHwNSixCellsNflair}}
\providecommand{\hlHwNSixCellsburn}{\tbd{hlHwNSixCellsburn}}
\providecommand{\hlHwNSixCellsflair}{\tbd{hlHwNSixCellsflair}}
\providecommand{\hlHwNSixDropDiffMaxburn}{\tbd{hlHwNSixDropDiffMaxburn}}
\providecommand{\hlHwNSixDropDiffMaxflair}{\tbd{hlHwNSixDropDiffMaxflair}}
\providecommand{\hlHwRepClass}{\tbd{hlHwRepClass}}
\providecommand{\hlHwRepCleanPooledAbs}{\tbd{hlHwRepCleanPooledAbs}}
\providecommand{\hlHwRepCleanPooledAbsCIHi}{\tbd{hlHwRepCleanPooledAbsCIHi}}
\providecommand{\hlHwRepCleanPooledAbsCILo}{\tbd{hlHwRepCleanPooledAbsCILo}}
\providecommand{\hlHwRepCleanPooledMax}{\tbd{hlHwRepCleanPooledMax}}
\providecommand{\hlHwRepCleanPooledN}{\tbd{hlHwRepCleanPooledN}}
\providecommand{\hlHwRepCleanPooledSigned}{\tbd{hlHwRepCleanPooledSigned}}
\providecommand{\hlHwRepCleanPooledSignedCIHi}{\tbd{hlHwRepCleanPooledSignedCIHi}}
\providecommand{\hlHwRepCleanPooledSignedCILo}{\tbd{hlHwRepCleanPooledSignedCILo}}
\providecommand{\hlHwRepCleanburnAbs}{\tbd{hlHwRepCleanburnAbs}}
\providecommand{\hlHwRepCleanburnAbsCIHi}{\tbd{hlHwRepCleanburnAbsCIHi}}
\providecommand{\hlHwRepCleanburnAbsCILo}{\tbd{hlHwRepCleanburnAbsCILo}}
\providecommand{\hlHwRepCleanburnMax}{\tbd{hlHwRepCleanburnMax}}
\providecommand{\hlHwRepCleanburnN}{\tbd{hlHwRepCleanburnN}}
\providecommand{\hlHwRepCleanburnSigned}{\tbd{hlHwRepCleanburnSigned}}
\providecommand{\hlHwRepCleanburnSignedCIHi}{\tbd{hlHwRepCleanburnSignedCIHi}}
\providecommand{\hlHwRepCleanburnSignedCILo}{\tbd{hlHwRepCleanburnSignedCILo}}
\providecommand{\hlHwRepCleanflairAbs}{\tbd{hlHwRepCleanflairAbs}}
\providecommand{\hlHwRepCleanflairAbsCIHi}{\tbd{hlHwRepCleanflairAbsCIHi}}
\providecommand{\hlHwRepCleanflairAbsCILo}{\tbd{hlHwRepCleanflairAbsCILo}}
\providecommand{\hlHwRepCleanflairMax}{\tbd{hlHwRepCleanflairMax}}
\providecommand{\hlHwRepCleanflairN}{\tbd{hlHwRepCleanflairN}}
\providecommand{\hlHwRepCleanflairSigned}{\tbd{hlHwRepCleanflairSigned}}
\providecommand{\hlHwRepCleanflairSignedCIHi}{\tbd{hlHwRepCleanflairSignedCIHi}}
\providecommand{\hlHwRepCleanflairSignedCILo}{\tbd{hlHwRepCleanflairSignedCILo}}
\providecommand{\hlHwRepDropPooledAbs}{\tbd{hlHwRepDropPooledAbs}}
\providecommand{\hlHwRepDropPooledAbsCIHi}{\tbd{hlHwRepDropPooledAbsCIHi}}
\providecommand{\hlHwRepDropPooledAbsCILo}{\tbd{hlHwRepDropPooledAbsCILo}}
\providecommand{\hlHwRepDropPooledMax}{\tbd{hlHwRepDropPooledMax}}
\providecommand{\hlHwRepDropPooledN}{\tbd{hlHwRepDropPooledN}}
\providecommand{\hlHwRepDropPooledSigned}{\tbd{hlHwRepDropPooledSigned}}
\providecommand{\hlHwRepDropPooledSignedCIHi}{\tbd{hlHwRepDropPooledSignedCIHi}}
\providecommand{\hlHwRepDropPooledSignedCILo}{\tbd{hlHwRepDropPooledSignedCILo}}
\providecommand{\hlHwRepDropburnAbs}{\tbd{hlHwRepDropburnAbs}}
\providecommand{\hlHwRepDropburnAbsCIHi}{\tbd{hlHwRepDropburnAbsCIHi}}
\providecommand{\hlHwRepDropburnAbsCILo}{\tbd{hlHwRepDropburnAbsCILo}}
\providecommand{\hlHwRepDropburnMax}{\tbd{hlHwRepDropburnMax}}
\providecommand{\hlHwRepDropburnN}{\tbd{hlHwRepDropburnN}}
\providecommand{\hlHwRepDropburnSigned}{\tbd{hlHwRepDropburnSigned}}
\providecommand{\hlHwRepDropburnSignedCIHi}{\tbd{hlHwRepDropburnSignedCIHi}}
\providecommand{\hlHwRepDropburnSignedCILo}{\tbd{hlHwRepDropburnSignedCILo}}
\providecommand{\hlHwRepDropflairAbs}{\tbd{hlHwRepDropflairAbs}}
\providecommand{\hlHwRepDropflairAbsCIHi}{\tbd{hlHwRepDropflairAbsCIHi}}
\providecommand{\hlHwRepDropflairAbsCILo}{\tbd{hlHwRepDropflairAbsCILo}}
\providecommand{\hlHwRepDropflairMax}{\tbd{hlHwRepDropflairMax}}
\providecommand{\hlHwRepDropflairN}{\tbd{hlHwRepDropflairN}}
\providecommand{\hlHwRepDropflairSigned}{\tbd{hlHwRepDropflairSigned}}
\providecommand{\hlHwRepDropflairSignedCIHi}{\tbd{hlHwRepDropflairSignedCIHi}}
\providecommand{\hlHwRepDropflairSignedCILo}{\tbd{hlHwRepDropflairSignedCILo}}
\providecommand{\hlHwRepNSixburnDiff}{\tbd{hlHwRepNSixburnDiff}}
\providecommand{\hlHwRepNSixburnDiffMax}{\tbd{hlHwRepNSixburnDiffMax}}
\providecommand{\hlHwRepNSixburnN}{\tbd{hlHwRepNSixburnN}}
\providecommand{\hlHwRepNSixburnOrig}{\tbd{hlHwRepNSixburnOrig}}
\providecommand{\hlHwRepNSixburnOrigCIHi}{\tbd{hlHwRepNSixburnOrigCIHi}}
\providecommand{\hlHwRepNSixburnOrigCILo}{\tbd{hlHwRepNSixburnOrigCILo}}
\providecommand{\hlHwRepNSixburnOrigTostCIHi}{\tbd{hlHwRepNSixburnOrigTostCIHi}}
\providecommand{\hlHwRepNSixburnOrigTostCILo}{\tbd{hlHwRepNSixburnOrigTostCILo}}
\providecommand{\hlHwRepNSixburnRep}{\tbd{hlHwRepNSixburnRep}}
\providecommand{\hlHwRepNSixburnRepCIHi}{\tbd{hlHwRepNSixburnRepCIHi}}
\providecommand{\hlHwRepNSixburnRepCILo}{\tbd{hlHwRepNSixburnRepCILo}}
\providecommand{\hlHwRepNSixburnRepTostCIHi}{\tbd{hlHwRepNSixburnRepTostCIHi}}
\providecommand{\hlHwRepNSixburnRepTostCILo}{\tbd{hlHwRepNSixburnRepTostCILo}}
\providecommand{\hlHwRepNSixburnSeeds}{\tbd{hlHwRepNSixburnSeeds}}
\providecommand{\hlHwRepNSixflairDiff}{\tbd{hlHwRepNSixflairDiff}}
\providecommand{\hlHwRepNSixflairDiffMax}{\tbd{hlHwRepNSixflairDiffMax}}
\providecommand{\hlHwRepNSixflairN}{\tbd{hlHwRepNSixflairN}}
\providecommand{\hlHwRepNSixflairOrig}{\tbd{hlHwRepNSixflairOrig}}
\providecommand{\hlHwRepNSixflairOrigCIHi}{\tbd{hlHwRepNSixflairOrigCIHi}}
\providecommand{\hlHwRepNSixflairOrigCILo}{\tbd{hlHwRepNSixflairOrigCILo}}
\providecommand{\hlHwRepNSixflairOrigTostCIHi}{\tbd{hlHwRepNSixflairOrigTostCIHi}}
\providecommand{\hlHwRepNSixflairOrigTostCILo}{\tbd{hlHwRepNSixflairOrigTostCILo}}
\providecommand{\hlHwRepNSixflairRep}{\tbd{hlHwRepNSixflairRep}}
\providecommand{\hlHwRepNSixflairRepCIHi}{\tbd{hlHwRepNSixflairRepCIHi}}
\providecommand{\hlHwRepNSixflairRepCILo}{\tbd{hlHwRepNSixflairRepCILo}}
\providecommand{\hlHwRepNSixflairRepTostCIHi}{\tbd{hlHwRepNSixflairRepTostCIHi}}
\providecommand{\hlHwRepNSixflairRepTostCILo}{\tbd{hlHwRepNSixflairRepTostCILo}}
\providecommand{\hlHwRepNSixflairSeeds}{\tbd{hlHwRepNSixflairSeeds}}
\providecommand{\hlHwRepNoisyPooledAbs}{\tbd{hlHwRepNoisyPooledAbs}}
\providecommand{\hlHwRepNoisyPooledAbsCIHi}{\tbd{hlHwRepNoisyPooledAbsCIHi}}
\providecommand{\hlHwRepNoisyPooledAbsCILo}{\tbd{hlHwRepNoisyPooledAbsCILo}}
\providecommand{\hlHwRepNoisyPooledMax}{\tbd{hlHwRepNoisyPooledMax}}
\providecommand{\hlHwRepNoisyPooledN}{\tbd{hlHwRepNoisyPooledN}}
\providecommand{\hlHwRepNoisyPooledSigned}{\tbd{hlHwRepNoisyPooledSigned}}
\providecommand{\hlHwRepNoisyPooledSignedCIHi}{\tbd{hlHwRepNoisyPooledSignedCIHi}}
\providecommand{\hlHwRepNoisyPooledSignedCILo}{\tbd{hlHwRepNoisyPooledSignedCILo}}
\providecommand{\hlHwRepNoisyburnAbs}{\tbd{hlHwRepNoisyburnAbs}}
\providecommand{\hlHwRepNoisyburnAbsCIHi}{\tbd{hlHwRepNoisyburnAbsCIHi}}
\providecommand{\hlHwRepNoisyburnAbsCILo}{\tbd{hlHwRepNoisyburnAbsCILo}}
\providecommand{\hlHwRepNoisyburnMax}{\tbd{hlHwRepNoisyburnMax}}
\providecommand{\hlHwRepNoisyburnN}{\tbd{hlHwRepNoisyburnN}}
\providecommand{\hlHwRepNoisyburnSigned}{\tbd{hlHwRepNoisyburnSigned}}
\providecommand{\hlHwRepNoisyburnSignedCIHi}{\tbd{hlHwRepNoisyburnSignedCIHi}}
\providecommand{\hlHwRepNoisyburnSignedCILo}{\tbd{hlHwRepNoisyburnSignedCILo}}
\providecommand{\hlHwRepNoisyflairAbs}{\tbd{hlHwRepNoisyflairAbs}}
\providecommand{\hlHwRepNoisyflairAbsCIHi}{\tbd{hlHwRepNoisyflairAbsCIHi}}
\providecommand{\hlHwRepNoisyflairAbsCILo}{\tbd{hlHwRepNoisyflairAbsCILo}}
\providecommand{\hlHwRepNoisyflairMax}{\tbd{hlHwRepNoisyflairMax}}
\providecommand{\hlHwRepNoisyflairN}{\tbd{hlHwRepNoisyflairN}}
\providecommand{\hlHwRepNoisyflairSigned}{\tbd{hlHwRepNoisyflairSigned}}
\providecommand{\hlHwRepNoisyflairSignedCIHi}{\tbd{hlHwRepNoisyflairSignedCIHi}}
\providecommand{\hlHwRepNoisyflairSignedCILo}{\tbd{hlHwRepNoisyflairSignedCILo}}
\providecommand{\hlHwRepOrigClass}{\tbd{hlHwRepOrigClass}}
\providecommand{\hlHwRepPlannedPooled}{\tbd{hlHwRepPlannedPooled}}
\providecommand{\hlHwRepPlannedburn}{\tbd{hlHwRepPlannedburn}}
\providecommand{\hlHwRepPlannedflair}{\tbd{hlHwRepPlannedflair}}
\providecommand{\hlHwRepRunsPooled}{\tbd{hlHwRepRunsPooled}}
\providecommand{\hlHwRepRunsburn}{\tbd{hlHwRepRunsburn}}
\providecommand{\hlHwRepRunsflair}{\tbd{hlHwRepRunsflair}}
\providecommand{\hlHwSThreeCellsNburn}{\tbd{hlHwSThreeCellsNburn}}
\providecommand{\hlHwSThreeCellsNflair}{\tbd{hlHwSThreeCellsNflair}}
\providecommand{\hlHwSThreeNClassesburn}{\tbd{hlHwSThreeNClassesburn}}
\providecommand{\hlHwSThreeNClassesflair}{\tbd{hlHwSThreeNClassesflair}}
\providecommand{\hlHwSThreeRangeMaxLTwoburn}{\tbd{hlHwSThreeRangeMaxLTwoburn}}
\providecommand{\hlHwSThreeRangeMaxLTwoflair}{\tbd{hlHwSThreeRangeMaxLTwoflair}}
\providecommand{\hlHwSThreeRangeMaxTypeLTwoburn}{\tbd{hlHwSThreeRangeMaxTypeLTwoburn}}
\providecommand{\hlHwSThreeRangeMaxTypeLTwoflair}{\tbd{hlHwSThreeRangeMaxTypeLTwoflair}}
\providecommand{\hlHwSThreeRangeMeanLTwoburn}{\tbd{hlHwSThreeRangeMeanLTwoburn}}
\providecommand{\hlHwSThreeRangeMeanLTwoflair}{\tbd{hlHwSThreeRangeMeanLTwoflair}}
\providecommand{\hlHwSThreeRangeMinLTwoburn}{\tbd{hlHwSThreeRangeMinLTwoburn}}
\providecommand{\hlHwSThreeRangeMinLTwoflair}{\tbd{hlHwSThreeRangeMinLTwoflair}}
\providecommand{\hlLayArmSix}{\tbd{hlLayArmSix}}
\providecommand{\hlLayArmTwelve}{\tbd{hlLayArmTwelve}}
\providecommand{\hlLayBandFracburn}{\tbd{hlLayBandFracburn}}
\providecommand{\hlLayBandFracflair}{\tbd{hlLayBandFracflair}}
\providecommand{\hlLayBandIntLVDburnShiftCIHi}{\tbd{hlLayBandIntLVDburnShiftCIHi}}
\providecommand{\hlLayBandIntLVDburnShiftCILo}{\tbd{hlLayBandIntLVDburnShiftCILo}}
\providecommand{\hlLayBandIntLVDburnShiftEst}{\tbd{hlLayBandIntLVDburnShiftEst}}
\providecommand{\hlLayBandIntLVDburnWorstCIHi}{\tbd{hlLayBandIntLVDburnWorstCIHi}}
\providecommand{\hlLayBandIntLVDburnWorstCILo}{\tbd{hlLayBandIntLVDburnWorstCILo}}
\providecommand{\hlLayBandIntLVDburnWorstEst}{\tbd{hlLayBandIntLVDburnWorstEst}}
\providecommand{\hlLayBandIntLVDflairShiftCIHi}{\tbd{hlLayBandIntLVDflairShiftCIHi}}
\providecommand{\hlLayBandIntLVDflairShiftCILo}{\tbd{hlLayBandIntLVDflairShiftCILo}}
\providecommand{\hlLayBandIntLVDflairShiftEst}{\tbd{hlLayBandIntLVDflairShiftEst}}
\providecommand{\hlLayBandIntLVDflairWorstCIHi}{\tbd{hlLayBandIntLVDflairWorstCIHi}}
\providecommand{\hlLayBandIntLVDflairWorstCILo}{\tbd{hlLayBandIntLVDflairWorstCILo}}
\providecommand{\hlLayBandIntLVDflairWorstEst}{\tbd{hlLayBandIntLVDflairWorstEst}}
\providecommand{\hlLayBandIntSATburnShiftCIHi}{\tbd{hlLayBandIntSATburnShiftCIHi}}
\providecommand{\hlLayBandIntSATburnShiftCILo}{\tbd{hlLayBandIntSATburnShiftCILo}}
\providecommand{\hlLayBandIntSATburnShiftEst}{\tbd{hlLayBandIntSATburnShiftEst}}
\providecommand{\hlLayBandIntSATburnWorstCIHi}{\tbd{hlLayBandIntSATburnWorstCIHi}}
\providecommand{\hlLayBandIntSATburnWorstCILo}{\tbd{hlLayBandIntSATburnWorstCILo}}
\providecommand{\hlLayBandIntSATburnWorstEst}{\tbd{hlLayBandIntSATburnWorstEst}}
\providecommand{\hlLayBandIntSATflairShiftCIHi}{\tbd{hlLayBandIntSATflairShiftCIHi}}
\providecommand{\hlLayBandIntSATflairShiftCILo}{\tbd{hlLayBandIntSATflairShiftCILo}}
\providecommand{\hlLayBandIntSATflairShiftEst}{\tbd{hlLayBandIntSATflairShiftEst}}
\providecommand{\hlLayBandIntSATflairWorstCIHi}{\tbd{hlLayBandIntSATflairWorstCIHi}}
\providecommand{\hlLayBandIntSATflairWorstCILo}{\tbd{hlLayBandIntSATflairWorstCILo}}
\providecommand{\hlLayBandIntSATflairWorstEst}{\tbd{hlLayBandIntSATflairWorstEst}}
\providecommand{\hlLayBandPx}{\tbd{hlLayBandPx}}
\providecommand{\hlLayCkaLVDburnCIHi}{\tbd{hlLayCkaLVDburnCIHi}}
\providecommand{\hlLayCkaLVDburnCILo}{\tbd{hlLayCkaLVDburnCILo}}
\providecommand{\hlLayCkaLVDburnEst}{\tbd{hlLayCkaLVDburnEst}}
\providecommand{\hlLayCkaLVDburnThird}{\tbd{hlLayCkaLVDburnThird}}
\providecommand{\hlLayCkaLVDflairCIHi}{\tbd{hlLayCkaLVDflairCIHi}}
\providecommand{\hlLayCkaLVDflairCILo}{\tbd{hlLayCkaLVDflairCILo}}
\providecommand{\hlLayCkaLVDflairEst}{\tbd{hlLayCkaLVDflairEst}}
\providecommand{\hlLayCkaLVDflairThird}{\tbd{hlLayCkaLVDflairThird}}
\providecommand{\hlLayCkaSATburnCIHi}{\tbd{hlLayCkaSATburnCIHi}}
\providecommand{\hlLayCkaSATburnCILo}{\tbd{hlLayCkaSATburnCILo}}
\providecommand{\hlLayCkaSATburnEst}{\tbd{hlLayCkaSATburnEst}}
\providecommand{\hlLayCkaSATburnThird}{\tbd{hlLayCkaSATburnThird}}
\providecommand{\hlLayCkaSATflairCIHi}{\tbd{hlLayCkaSATflairCIHi}}
\providecommand{\hlLayCkaSATflairCILo}{\tbd{hlLayCkaSATflairCILo}}
\providecommand{\hlLayCkaSATflairEst}{\tbd{hlLayCkaSATflairEst}}
\providecommand{\hlLayCkaSATflairThird}{\tbd{hlLayCkaSATflairThird}}
\providecommand{\hlLayDepth}{\tbd{hlLayDepth}}
\providecommand{\hlLayDriftLVDburnCIHi}{\tbd{hlLayDriftLVDburnCIHi}}
\providecommand{\hlLayDriftLVDburnCILo}{\tbd{hlLayDriftLVDburnCILo}}
\providecommand{\hlLayDriftLVDburnEst}{\tbd{hlLayDriftLVDburnEst}}
\providecommand{\hlLayDriftLVDburnThird}{\tbd{hlLayDriftLVDburnThird}}
\providecommand{\hlLayDriftLVDburnThirdEst}{\tbd{hlLayDriftLVDburnThirdEst}}
\providecommand{\hlLayDriftLVDflairCIHi}{\tbd{hlLayDriftLVDflairCIHi}}
\providecommand{\hlLayDriftLVDflairCILo}{\tbd{hlLayDriftLVDflairCILo}}
\providecommand{\hlLayDriftLVDflairEst}{\tbd{hlLayDriftLVDflairEst}}
\providecommand{\hlLayDriftLVDflairThird}{\tbd{hlLayDriftLVDflairThird}}
\providecommand{\hlLayDriftLVDflairThirdEst}{\tbd{hlLayDriftLVDflairThirdEst}}
\providecommand{\hlLayDriftSATburnCIHi}{\tbd{hlLayDriftSATburnCIHi}}
\providecommand{\hlLayDriftSATburnCILo}{\tbd{hlLayDriftSATburnCILo}}
\providecommand{\hlLayDriftSATburnEst}{\tbd{hlLayDriftSATburnEst}}
\providecommand{\hlLayDriftSATburnThird}{\tbd{hlLayDriftSATburnThird}}
\providecommand{\hlLayDriftSATburnThirdEst}{\tbd{hlLayDriftSATburnThirdEst}}
\providecommand{\hlLayDriftSATflairCIHi}{\tbd{hlLayDriftSATflairCIHi}}
\providecommand{\hlLayDriftSATflairCILo}{\tbd{hlLayDriftSATflairCILo}}
\providecommand{\hlLayDriftSATflairEst}{\tbd{hlLayDriftSATflairEst}}
\providecommand{\hlLayDriftSATflairThird}{\tbd{hlLayDriftSATflairThird}}
\providecommand{\hlLayDriftSATflairThirdEst}{\tbd{hlLayDriftSATflairThirdEst}}
\providecommand{\hlLayDriftStepLVDburn}{\tbd{hlLayDriftStepLVDburn}}
\providecommand{\hlLayDriftStepLVDflair}{\tbd{hlLayDriftStepLVDflair}}
\providecommand{\hlLayDriftStepSATburn}{\tbd{hlLayDriftStepSATburn}}
\providecommand{\hlLayDriftStepSATflair}{\tbd{hlLayDriftStepSATflair}}
\providecommand{\hlLayEpochLVDburnClean}{\tbd{hlLayEpochLVDburnClean}}
\providecommand{\hlLayEpochLVDburnNoisy}{\tbd{hlLayEpochLVDburnNoisy}}
\providecommand{\hlLayEpochLVDflairClean}{\tbd{hlLayEpochLVDflairClean}}
\providecommand{\hlLayEpochLVDflairNoisy}{\tbd{hlLayEpochLVDflairNoisy}}
\providecommand{\hlLayEpochSATburnClean}{\tbd{hlLayEpochSATburnClean}}
\providecommand{\hlLayEpochSATburnNoisy}{\tbd{hlLayEpochSATburnNoisy}}
\providecommand{\hlLayEpochSATflairClean}{\tbd{hlLayEpochSATflairClean}}
\providecommand{\hlLayEpochSATflairNoisy}{\tbd{hlLayEpochSATflairNoisy}}
\providecommand{\hlLayFrozenMaxDrift}{\tbd{hlLayFrozenMaxDrift}}
\providecommand{\hlLayFrozenMinCka}{\tbd{hlLayFrozenMinCka}}
\providecommand{\hlLayFrozenRuns}{\tbd{hlLayFrozenRuns}}
\providecommand{\hlLayIntLVDburnSix}{\tbd{hlLayIntLVDburnSix}}
\providecommand{\hlLayIntLVDburnTwentyFour}{\tbd{hlLayIntLVDburnTwentyFour}}
\providecommand{\hlLayIntLVDflairSix}{\tbd{hlLayIntLVDflairSix}}
\providecommand{\hlLayIntLVDflairTwentyFour}{\tbd{hlLayIntLVDflairTwentyFour}}
\providecommand{\hlLayIntSATburnSix}{\tbd{hlLayIntSATburnSix}}
\providecommand{\hlLayIntSATburnTwentyFour}{\tbd{hlLayIntSATburnTwentyFour}}
\providecommand{\hlLayIntSATflairSix}{\tbd{hlLayIntSATflairSix}}
\providecommand{\hlLayIntSATflairTwentyFour}{\tbd{hlLayIntSATflairTwentyFour}}
\providecommand{\hlLayPairburnTwentyFourCIHi}{\tbd{hlLayPairburnTwentyFourCIHi}}
\providecommand{\hlLayPairburnTwentyFourCILo}{\tbd{hlLayPairburnTwentyFourCILo}}
\providecommand{\hlLayPairburnTwentyFourEst}{\tbd{hlLayPairburnTwentyFourEst}}
\providecommand{\hlLayPairburnZeroCIHi}{\tbd{hlLayPairburnZeroCIHi}}
\providecommand{\hlLayPairburnZeroCILo}{\tbd{hlLayPairburnZeroCILo}}
\providecommand{\hlLayPairburnZeroEst}{\tbd{hlLayPairburnZeroEst}}
\providecommand{\hlLayPairflairTwentyFourCIHi}{\tbd{hlLayPairflairTwentyFourCIHi}}
\providecommand{\hlLayPairflairTwentyFourCILo}{\tbd{hlLayPairflairTwentyFourCILo}}
\providecommand{\hlLayPairflairTwentyFourEst}{\tbd{hlLayPairflairTwentyFourEst}}
\providecommand{\hlLayPairflairZeroCIHi}{\tbd{hlLayPairflairZeroCIHi}}
\providecommand{\hlLayPairflairZeroCILo}{\tbd{hlLayPairflairZeroCILo}}
\providecommand{\hlLayPairflairZeroEst}{\tbd{hlLayPairflairZeroEst}}
\providecommand{\hlLayParamsAll}{\tbd{hlLayParamsAll}}
\providecommand{\hlLayParamsSix}{\tbd{hlLayParamsSix}}
\providecommand{\hlLayParamsTwelve}{\tbd{hlLayParamsTwelve}}
\providecommand{\hlLayReproburnAbs}{\tbd{hlLayReproburnAbs}}
\providecommand{\hlLayReproburnMax}{\tbd{hlLayReproburnMax}}
\providecommand{\hlLayReproburnN}{\tbd{hlLayReproburnN}}
\providecommand{\hlLayReproflairAbs}{\tbd{hlLayReproflairAbs}}
\providecommand{\hlLayReproflairMax}{\tbd{hlLayReproflairMax}}
\providecommand{\hlLayReproflairN}{\tbd{hlLayReproflairN}}
\providecommand{\hlLayRunsDone}{\tbd{hlLayRunsDone}}
\providecommand{\hlLayRunsPlanned}{\tbd{hlLayRunsPlanned}}
\providecommand{\hlLaySeeds}{\tbd{hlLaySeeds}}
\providecommand{\hlLaySeedsAll}{\tbd{hlLaySeedsAll}}
\providecommand{\hlLayShareLVDburnShift}{\tbd{hlLayShareLVDburnShift}}
\providecommand{\hlLayShareLVDburnWorst}{\tbd{hlLayShareLVDburnWorst}}
\providecommand{\hlLayShareLVDflairShift}{\tbd{hlLayShareLVDflairShift}}
\providecommand{\hlLayShareLVDflairWorst}{\tbd{hlLayShareLVDflairWorst}}
\providecommand{\hlLayShareSATburnShift}{\tbd{hlLayShareSATburnShift}}
\providecommand{\hlLayShareSATburnWorst}{\tbd{hlLayShareSATburnWorst}}
\providecommand{\hlLayShareSATflairShift}{\tbd{hlLayShareSATflairShift}}
\providecommand{\hlLayShareSATflairWorst}{\tbd{hlLayShareSATflairWorst}}
\providecommand{\hlLayStepLVDburnSixZeroCIHi}{\tbd{hlLayStepLVDburnSixZeroCIHi}}
\providecommand{\hlLayStepLVDburnSixZeroCILo}{\tbd{hlLayStepLVDburnSixZeroCILo}}
\providecommand{\hlLayStepLVDburnSixZeroEst}{\tbd{hlLayStepLVDburnSixZeroEst}}
\providecommand{\hlLayStepLVDburnTwelveSixCIHi}{\tbd{hlLayStepLVDburnTwelveSixCIHi}}
\providecommand{\hlLayStepLVDburnTwelveSixCILo}{\tbd{hlLayStepLVDburnTwelveSixCILo}}
\providecommand{\hlLayStepLVDburnTwelveSixEst}{\tbd{hlLayStepLVDburnTwelveSixEst}}
\providecommand{\hlLayStepLVDburnTwentyFourTwelveCIHi}{\tbd{hlLayStepLVDburnTwentyFourTwelveCIHi}}
\providecommand{\hlLayStepLVDburnTwentyFourTwelveCILo}{\tbd{hlLayStepLVDburnTwentyFourTwelveCILo}}
\providecommand{\hlLayStepLVDburnTwentyFourTwelveEst}{\tbd{hlLayStepLVDburnTwentyFourTwelveEst}}
\providecommand{\hlLayStepLVDflairSixZeroCIHi}{\tbd{hlLayStepLVDflairSixZeroCIHi}}
\providecommand{\hlLayStepLVDflairSixZeroCILo}{\tbd{hlLayStepLVDflairSixZeroCILo}}
\providecommand{\hlLayStepLVDflairSixZeroEst}{\tbd{hlLayStepLVDflairSixZeroEst}}
\providecommand{\hlLayStepLVDflairTwelveSixCIHi}{\tbd{hlLayStepLVDflairTwelveSixCIHi}}
\providecommand{\hlLayStepLVDflairTwelveSixCILo}{\tbd{hlLayStepLVDflairTwelveSixCILo}}
\providecommand{\hlLayStepLVDflairTwelveSixEst}{\tbd{hlLayStepLVDflairTwelveSixEst}}
\providecommand{\hlLayStepLVDflairTwentyFourTwelveCIHi}{\tbd{hlLayStepLVDflairTwentyFourTwelveCIHi}}
\providecommand{\hlLayStepLVDflairTwentyFourTwelveCILo}{\tbd{hlLayStepLVDflairTwentyFourTwelveCILo}}
\providecommand{\hlLayStepLVDflairTwentyFourTwelveEst}{\tbd{hlLayStepLVDflairTwentyFourTwelveEst}}
\providecommand{\hlLayStepSATburnSixZeroCIHi}{\tbd{hlLayStepSATburnSixZeroCIHi}}
\providecommand{\hlLayStepSATburnSixZeroCILo}{\tbd{hlLayStepSATburnSixZeroCILo}}
\providecommand{\hlLayStepSATburnSixZeroEst}{\tbd{hlLayStepSATburnSixZeroEst}}
\providecommand{\hlLayStepSATburnTwelveSixCIHi}{\tbd{hlLayStepSATburnTwelveSixCIHi}}
\providecommand{\hlLayStepSATburnTwelveSixCILo}{\tbd{hlLayStepSATburnTwelveSixCILo}}
\providecommand{\hlLayStepSATburnTwelveSixEst}{\tbd{hlLayStepSATburnTwelveSixEst}}
\providecommand{\hlLayStepSATburnTwentyFourTwelveCIHi}{\tbd{hlLayStepSATburnTwentyFourTwelveCIHi}}
\providecommand{\hlLayStepSATburnTwentyFourTwelveCILo}{\tbd{hlLayStepSATburnTwentyFourTwelveCILo}}
\providecommand{\hlLayStepSATburnTwentyFourTwelveEst}{\tbd{hlLayStepSATburnTwentyFourTwelveEst}}
\providecommand{\hlLayStepSATflairSixZeroCIHi}{\tbd{hlLayStepSATflairSixZeroCIHi}}
\providecommand{\hlLayStepSATflairSixZeroCILo}{\tbd{hlLayStepSATflairSixZeroCILo}}
\providecommand{\hlLayStepSATflairSixZeroEst}{\tbd{hlLayStepSATflairSixZeroEst}}
\providecommand{\hlLayStepSATflairTwelveSixCIHi}{\tbd{hlLayStepSATflairTwelveSixCIHi}}
\providecommand{\hlLayStepSATflairTwelveSixCILo}{\tbd{hlLayStepSATflairTwelveSixCILo}}
\providecommand{\hlLayStepSATflairTwelveSixEst}{\tbd{hlLayStepSATflairTwelveSixEst}}
\providecommand{\hlLayStepSATflairTwentyFourTwelveCIHi}{\tbd{hlLayStepSATflairTwentyFourTwelveCIHi}}
\providecommand{\hlLayStepSATflairTwentyFourTwelveCILo}{\tbd{hlLayStepSATflairTwentyFourTwelveCILo}}
\providecommand{\hlLayStepSATflairTwentyFourTwelveEst}{\tbd{hlLayStepSATflairTwentyFourTwelveEst}}
\providecommand{\hlLayWorstburn}{\tbd{hlLayWorstburn}}
\providecommand{\hlLayWorstflair}{\tbd{hlLayWorstflair}}
\providecommand{\hlLossCleanBootDOFAburn}{\tbd{hlLossCleanBootDOFAburn}}
\providecommand{\hlLossCleanBootDOFAflair}{\tbd{hlLossCleanBootDOFAflair}}
\providecommand{\hlLossCleanBootLVDburn}{\tbd{hlLossCleanBootLVDburn}}
\providecommand{\hlLossCleanBootLVDflair}{\tbd{hlLossCleanBootLVDflair}}
\providecommand{\hlLossCleanBootRNburn}{\tbd{hlLossCleanBootRNburn}}
\providecommand{\hlLossCleanBootRNflair}{\tbd{hlLossCleanBootRNflair}}
\providecommand{\hlLossCleanBootSATburn}{\tbd{hlLossCleanBootSATburn}}
\providecommand{\hlLossCleanBootSATflair}{\tbd{hlLossCleanBootSATflair}}
\providecommand{\hlLossCleanBootTMburn}{\tbd{hlLossCleanBootTMburn}}
\providecommand{\hlLossCleanBootTMflair}{\tbd{hlLossCleanBootTMflair}}
\providecommand{\hlLossCleanBootburn}{\tbd{hlLossCleanBootburn}}
\providecommand{\hlLossCleanBootflair}{\tbd{hlLossCleanBootflair}}
\providecommand{\hlLossCleanCEDOFAburn}{\tbd{hlLossCleanCEDOFAburn}}
\providecommand{\hlLossCleanCEDOFAflair}{\tbd{hlLossCleanCEDOFAflair}}
\providecommand{\hlLossCleanCELVDburn}{\tbd{hlLossCleanCELVDburn}}
\providecommand{\hlLossCleanCELVDflair}{\tbd{hlLossCleanCELVDflair}}
\providecommand{\hlLossCleanCERNburn}{\tbd{hlLossCleanCERNburn}}
\providecommand{\hlLossCleanCERNflair}{\tbd{hlLossCleanCERNflair}}
\providecommand{\hlLossCleanCESATburn}{\tbd{hlLossCleanCESATburn}}
\providecommand{\hlLossCleanCESATflair}{\tbd{hlLossCleanCESATflair}}
\providecommand{\hlLossCleanCETMburn}{\tbd{hlLossCleanCETMburn}}
\providecommand{\hlLossCleanCETMflair}{\tbd{hlLossCleanCETMflair}}
\providecommand{\hlLossCleanCEburn}{\tbd{hlLossCleanCEburn}}
\providecommand{\hlLossCleanCEflair}{\tbd{hlLossCleanCEflair}}
\providecommand{\hlLossCleanGceDOFAburn}{\tbd{hlLossCleanGceDOFAburn}}
\providecommand{\hlLossCleanGceDOFAflair}{\tbd{hlLossCleanGceDOFAflair}}
\providecommand{\hlLossCleanGceLVDburn}{\tbd{hlLossCleanGceLVDburn}}
\providecommand{\hlLossCleanGceLVDflair}{\tbd{hlLossCleanGceLVDflair}}
\providecommand{\hlLossCleanGceRNburn}{\tbd{hlLossCleanGceRNburn}}
\providecommand{\hlLossCleanGceRNflair}{\tbd{hlLossCleanGceRNflair}}
\providecommand{\hlLossCleanGceSATburn}{\tbd{hlLossCleanGceSATburn}}
\providecommand{\hlLossCleanGceSATflair}{\tbd{hlLossCleanGceSATflair}}
\providecommand{\hlLossCleanGceTMburn}{\tbd{hlLossCleanGceTMburn}}
\providecommand{\hlLossCleanGceTMflair}{\tbd{hlLossCleanGceTMflair}}
\providecommand{\hlLossCleanGceburn}{\tbd{hlLossCleanGceburn}}
\providecommand{\hlLossCleanGceflair}{\tbd{hlLossCleanGceflair}}
\providecommand{\hlLossCleanInvBootburnCIHi}{\tbd{hlLossCleanInvBootburnCIHi}}
\providecommand{\hlLossCleanInvBootburnCILo}{\tbd{hlLossCleanInvBootburnCILo}}
\providecommand{\hlLossCleanInvBootburnEst}{\tbd{hlLossCleanInvBootburnEst}}
\providecommand{\hlLossCleanInvBootburnMde}{\tbd{hlLossCleanInvBootburnMde}}
\providecommand{\hlLossCleanInvBootburnN}{\tbd{hlLossCleanInvBootburnN}}
\providecommand{\hlLossCleanInvBootburnPHolm}{\tbd{hlLossCleanInvBootburnPHolm}}
\providecommand{\hlLossCleanInvBootburnTostCIHi}{\tbd{hlLossCleanInvBootburnTostCIHi}}
\providecommand{\hlLossCleanInvBootburnTostCILo}{\tbd{hlLossCleanInvBootburnTostCILo}}
\providecommand{\hlLossCleanInvBootflairCIHi}{\tbd{hlLossCleanInvBootflairCIHi}}
\providecommand{\hlLossCleanInvBootflairCILo}{\tbd{hlLossCleanInvBootflairCILo}}
\providecommand{\hlLossCleanInvBootflairEst}{\tbd{hlLossCleanInvBootflairEst}}
\providecommand{\hlLossCleanInvBootflairMde}{\tbd{hlLossCleanInvBootflairMde}}
\providecommand{\hlLossCleanInvBootflairN}{\tbd{hlLossCleanInvBootflairN}}
\providecommand{\hlLossCleanInvBootflairPHolm}{\tbd{hlLossCleanInvBootflairPHolm}}
\providecommand{\hlLossCleanInvBootflairTostCIHi}{\tbd{hlLossCleanInvBootflairTostCIHi}}
\providecommand{\hlLossCleanInvBootflairTostCILo}{\tbd{hlLossCleanInvBootflairTostCILo}}
\providecommand{\hlLossCleanInvGceburnCIHi}{\tbd{hlLossCleanInvGceburnCIHi}}
\providecommand{\hlLossCleanInvGceburnCILo}{\tbd{hlLossCleanInvGceburnCILo}}
\providecommand{\hlLossCleanInvGceburnEst}{\tbd{hlLossCleanInvGceburnEst}}
\providecommand{\hlLossCleanInvGceburnMde}{\tbd{hlLossCleanInvGceburnMde}}
\providecommand{\hlLossCleanInvGceburnN}{\tbd{hlLossCleanInvGceburnN}}
\providecommand{\hlLossCleanInvGceburnPHolm}{\tbd{hlLossCleanInvGceburnPHolm}}
\providecommand{\hlLossCleanInvGceburnTostCIHi}{\tbd{hlLossCleanInvGceburnTostCIHi}}
\providecommand{\hlLossCleanInvGceburnTostCILo}{\tbd{hlLossCleanInvGceburnTostCILo}}
\providecommand{\hlLossCleanInvGceflairCIHi}{\tbd{hlLossCleanInvGceflairCIHi}}
\providecommand{\hlLossCleanInvGceflairCILo}{\tbd{hlLossCleanInvGceflairCILo}}
\providecommand{\hlLossCleanInvGceflairEst}{\tbd{hlLossCleanInvGceflairEst}}
\providecommand{\hlLossCleanInvGceflairMde}{\tbd{hlLossCleanInvGceflairMde}}
\providecommand{\hlLossCleanInvGceflairN}{\tbd{hlLossCleanInvGceflairN}}
\providecommand{\hlLossCleanInvGceflairPHolm}{\tbd{hlLossCleanInvGceflairPHolm}}
\providecommand{\hlLossCleanInvGceflairTostCIHi}{\tbd{hlLossCleanInvGceflairTostCIHi}}
\providecommand{\hlLossCleanInvGceflairTostCILo}{\tbd{hlLossCleanInvGceflairTostCILo}}
\providecommand{\hlLossDropBootDOFAburn}{\tbd{hlLossDropBootDOFAburn}}
\providecommand{\hlLossDropBootDOFAflair}{\tbd{hlLossDropBootDOFAflair}}
\providecommand{\hlLossDropBootLVDburn}{\tbd{hlLossDropBootLVDburn}}
\providecommand{\hlLossDropBootLVDflair}{\tbd{hlLossDropBootLVDflair}}
\providecommand{\hlLossDropBootRNburn}{\tbd{hlLossDropBootRNburn}}
\providecommand{\hlLossDropBootRNflair}{\tbd{hlLossDropBootRNflair}}
\providecommand{\hlLossDropBootSATburn}{\tbd{hlLossDropBootSATburn}}
\providecommand{\hlLossDropBootSATflair}{\tbd{hlLossDropBootSATflair}}
\providecommand{\hlLossDropBootTMburn}{\tbd{hlLossDropBootTMburn}}
\providecommand{\hlLossDropBootTMflair}{\tbd{hlLossDropBootTMflair}}
\providecommand{\hlLossDropBootburn}{\tbd{hlLossDropBootburn}}
\providecommand{\hlLossDropBootflair}{\tbd{hlLossDropBootflair}}
\providecommand{\hlLossDropCEDOFAburn}{\tbd{hlLossDropCEDOFAburn}}
\providecommand{\hlLossDropCEDOFAflair}{\tbd{hlLossDropCEDOFAflair}}
\providecommand{\hlLossDropCELVDburn}{\tbd{hlLossDropCELVDburn}}
\providecommand{\hlLossDropCELVDflair}{\tbd{hlLossDropCELVDflair}}
\providecommand{\hlLossDropCERNburn}{\tbd{hlLossDropCERNburn}}
\providecommand{\hlLossDropCERNflair}{\tbd{hlLossDropCERNflair}}
\providecommand{\hlLossDropCESATburn}{\tbd{hlLossDropCESATburn}}
\providecommand{\hlLossDropCESATflair}{\tbd{hlLossDropCESATflair}}
\providecommand{\hlLossDropCETMburn}{\tbd{hlLossDropCETMburn}}
\providecommand{\hlLossDropCETMflair}{\tbd{hlLossDropCETMflair}}
\providecommand{\hlLossDropCEburn}{\tbd{hlLossDropCEburn}}
\providecommand{\hlLossDropCEflair}{\tbd{hlLossDropCEflair}}
\providecommand{\hlLossDropGceDOFAburn}{\tbd{hlLossDropGceDOFAburn}}
\providecommand{\hlLossDropGceDOFAflair}{\tbd{hlLossDropGceDOFAflair}}
\providecommand{\hlLossDropGceLVDburn}{\tbd{hlLossDropGceLVDburn}}
\providecommand{\hlLossDropGceLVDflair}{\tbd{hlLossDropGceLVDflair}}
\providecommand{\hlLossDropGceRNburn}{\tbd{hlLossDropGceRNburn}}
\providecommand{\hlLossDropGceRNflair}{\tbd{hlLossDropGceRNflair}}
\providecommand{\hlLossDropGceSATburn}{\tbd{hlLossDropGceSATburn}}
\providecommand{\hlLossDropGceSATflair}{\tbd{hlLossDropGceSATflair}}
\providecommand{\hlLossDropGceTMburn}{\tbd{hlLossDropGceTMburn}}
\providecommand{\hlLossDropGceTMflair}{\tbd{hlLossDropGceTMflair}}
\providecommand{\hlLossDropGceburn}{\tbd{hlLossDropGceburn}}
\providecommand{\hlLossDropGceflair}{\tbd{hlLossDropGceflair}}
\providecommand{\hlLossInvBootDOFAburnCIHi}{\tbd{hlLossInvBootDOFAburnCIHi}}
\providecommand{\hlLossInvBootDOFAburnCILo}{\tbd{hlLossInvBootDOFAburnCILo}}
\providecommand{\hlLossInvBootDOFAburnEst}{\tbd{hlLossInvBootDOFAburnEst}}
\providecommand{\hlLossInvBootDOFAburnMde}{\tbd{hlLossInvBootDOFAburnMde}}
\providecommand{\hlLossInvBootDOFAburnN}{\tbd{hlLossInvBootDOFAburnN}}
\providecommand{\hlLossInvBootDOFAburnPHolm}{\tbd{hlLossInvBootDOFAburnPHolm}}
\providecommand{\hlLossInvBootDOFAburnTostCIHi}{\tbd{hlLossInvBootDOFAburnTostCIHi}}
\providecommand{\hlLossInvBootDOFAburnTostCILo}{\tbd{hlLossInvBootDOFAburnTostCILo}}
\providecommand{\hlLossInvBootDOFAflairCIHi}{\tbd{hlLossInvBootDOFAflairCIHi}}
\providecommand{\hlLossInvBootDOFAflairCILo}{\tbd{hlLossInvBootDOFAflairCILo}}
\providecommand{\hlLossInvBootDOFAflairEst}{\tbd{hlLossInvBootDOFAflairEst}}
\providecommand{\hlLossInvBootDOFAflairMde}{\tbd{hlLossInvBootDOFAflairMde}}
\providecommand{\hlLossInvBootDOFAflairN}{\tbd{hlLossInvBootDOFAflairN}}
\providecommand{\hlLossInvBootDOFAflairPHolm}{\tbd{hlLossInvBootDOFAflairPHolm}}
\providecommand{\hlLossInvBootDOFAflairTostCIHi}{\tbd{hlLossInvBootDOFAflairTostCIHi}}
\providecommand{\hlLossInvBootDOFAflairTostCILo}{\tbd{hlLossInvBootDOFAflairTostCILo}}
\providecommand{\hlLossInvBootLVDburnCIHi}{\tbd{hlLossInvBootLVDburnCIHi}}
\providecommand{\hlLossInvBootLVDburnCILo}{\tbd{hlLossInvBootLVDburnCILo}}
\providecommand{\hlLossInvBootLVDburnEst}{\tbd{hlLossInvBootLVDburnEst}}
\providecommand{\hlLossInvBootLVDburnMde}{\tbd{hlLossInvBootLVDburnMde}}
\providecommand{\hlLossInvBootLVDburnN}{\tbd{hlLossInvBootLVDburnN}}
\providecommand{\hlLossInvBootLVDburnPHolm}{\tbd{hlLossInvBootLVDburnPHolm}}
\providecommand{\hlLossInvBootLVDburnTostCIHi}{\tbd{hlLossInvBootLVDburnTostCIHi}}
\providecommand{\hlLossInvBootLVDburnTostCILo}{\tbd{hlLossInvBootLVDburnTostCILo}}
\providecommand{\hlLossInvBootLVDflairCIHi}{\tbd{hlLossInvBootLVDflairCIHi}}
\providecommand{\hlLossInvBootLVDflairCILo}{\tbd{hlLossInvBootLVDflairCILo}}
\providecommand{\hlLossInvBootLVDflairEst}{\tbd{hlLossInvBootLVDflairEst}}
\providecommand{\hlLossInvBootLVDflairMde}{\tbd{hlLossInvBootLVDflairMde}}
\providecommand{\hlLossInvBootLVDflairN}{\tbd{hlLossInvBootLVDflairN}}
\providecommand{\hlLossInvBootLVDflairPHolm}{\tbd{hlLossInvBootLVDflairPHolm}}
\providecommand{\hlLossInvBootLVDflairTostCIHi}{\tbd{hlLossInvBootLVDflairTostCIHi}}
\providecommand{\hlLossInvBootLVDflairTostCILo}{\tbd{hlLossInvBootLVDflairTostCILo}}
\providecommand{\hlLossInvBootRNburnCIHi}{\tbd{hlLossInvBootRNburnCIHi}}
\providecommand{\hlLossInvBootRNburnCILo}{\tbd{hlLossInvBootRNburnCILo}}
\providecommand{\hlLossInvBootRNburnEst}{\tbd{hlLossInvBootRNburnEst}}
\providecommand{\hlLossInvBootRNburnMde}{\tbd{hlLossInvBootRNburnMde}}
\providecommand{\hlLossInvBootRNburnN}{\tbd{hlLossInvBootRNburnN}}
\providecommand{\hlLossInvBootRNburnPHolm}{\tbd{hlLossInvBootRNburnPHolm}}
\providecommand{\hlLossInvBootRNburnTostCIHi}{\tbd{hlLossInvBootRNburnTostCIHi}}
\providecommand{\hlLossInvBootRNburnTostCILo}{\tbd{hlLossInvBootRNburnTostCILo}}
\providecommand{\hlLossInvBootRNflairCIHi}{\tbd{hlLossInvBootRNflairCIHi}}
\providecommand{\hlLossInvBootRNflairCILo}{\tbd{hlLossInvBootRNflairCILo}}
\providecommand{\hlLossInvBootRNflairEst}{\tbd{hlLossInvBootRNflairEst}}
\providecommand{\hlLossInvBootRNflairMde}{\tbd{hlLossInvBootRNflairMde}}
\providecommand{\hlLossInvBootRNflairN}{\tbd{hlLossInvBootRNflairN}}
\providecommand{\hlLossInvBootRNflairPHolm}{\tbd{hlLossInvBootRNflairPHolm}}
\providecommand{\hlLossInvBootRNflairTostCIHi}{\tbd{hlLossInvBootRNflairTostCIHi}}
\providecommand{\hlLossInvBootRNflairTostCILo}{\tbd{hlLossInvBootRNflairTostCILo}}
\providecommand{\hlLossInvBootSATburnCIHi}{\tbd{hlLossInvBootSATburnCIHi}}
\providecommand{\hlLossInvBootSATburnCILo}{\tbd{hlLossInvBootSATburnCILo}}
\providecommand{\hlLossInvBootSATburnEst}{\tbd{hlLossInvBootSATburnEst}}
\providecommand{\hlLossInvBootSATburnMde}{\tbd{hlLossInvBootSATburnMde}}
\providecommand{\hlLossInvBootSATburnN}{\tbd{hlLossInvBootSATburnN}}
\providecommand{\hlLossInvBootSATburnPHolm}{\tbd{hlLossInvBootSATburnPHolm}}
\providecommand{\hlLossInvBootSATburnTostCIHi}{\tbd{hlLossInvBootSATburnTostCIHi}}
\providecommand{\hlLossInvBootSATburnTostCILo}{\tbd{hlLossInvBootSATburnTostCILo}}
\providecommand{\hlLossInvBootSATflairCIHi}{\tbd{hlLossInvBootSATflairCIHi}}
\providecommand{\hlLossInvBootSATflairCILo}{\tbd{hlLossInvBootSATflairCILo}}
\providecommand{\hlLossInvBootSATflairEst}{\tbd{hlLossInvBootSATflairEst}}
\providecommand{\hlLossInvBootSATflairMde}{\tbd{hlLossInvBootSATflairMde}}
\providecommand{\hlLossInvBootSATflairN}{\tbd{hlLossInvBootSATflairN}}
\providecommand{\hlLossInvBootSATflairPHolm}{\tbd{hlLossInvBootSATflairPHolm}}
\providecommand{\hlLossInvBootSATflairTostCIHi}{\tbd{hlLossInvBootSATflairTostCIHi}}
\providecommand{\hlLossInvBootSATflairTostCILo}{\tbd{hlLossInvBootSATflairTostCILo}}
\providecommand{\hlLossInvBootTMburnCIHi}{\tbd{hlLossInvBootTMburnCIHi}}
\providecommand{\hlLossInvBootTMburnCILo}{\tbd{hlLossInvBootTMburnCILo}}
\providecommand{\hlLossInvBootTMburnEst}{\tbd{hlLossInvBootTMburnEst}}
\providecommand{\hlLossInvBootTMburnMde}{\tbd{hlLossInvBootTMburnMde}}
\providecommand{\hlLossInvBootTMburnN}{\tbd{hlLossInvBootTMburnN}}
\providecommand{\hlLossInvBootTMburnPHolm}{\tbd{hlLossInvBootTMburnPHolm}}
\providecommand{\hlLossInvBootTMburnTostCIHi}{\tbd{hlLossInvBootTMburnTostCIHi}}
\providecommand{\hlLossInvBootTMburnTostCILo}{\tbd{hlLossInvBootTMburnTostCILo}}
\providecommand{\hlLossInvBootTMflairCIHi}{\tbd{hlLossInvBootTMflairCIHi}}
\providecommand{\hlLossInvBootTMflairCILo}{\tbd{hlLossInvBootTMflairCILo}}
\providecommand{\hlLossInvBootTMflairEst}{\tbd{hlLossInvBootTMflairEst}}
\providecommand{\hlLossInvBootTMflairMde}{\tbd{hlLossInvBootTMflairMde}}
\providecommand{\hlLossInvBootTMflairN}{\tbd{hlLossInvBootTMflairN}}
\providecommand{\hlLossInvBootTMflairPHolm}{\tbd{hlLossInvBootTMflairPHolm}}
\providecommand{\hlLossInvBootTMflairTostCIHi}{\tbd{hlLossInvBootTMflairTostCIHi}}
\providecommand{\hlLossInvBootTMflairTostCILo}{\tbd{hlLossInvBootTMflairTostCILo}}
\providecommand{\hlLossInvBootburnCIHi}{\tbd{hlLossInvBootburnCIHi}}
\providecommand{\hlLossInvBootburnCILo}{\tbd{hlLossInvBootburnCILo}}
\providecommand{\hlLossInvBootburnEst}{\tbd{hlLossInvBootburnEst}}
\providecommand{\hlLossInvBootburnMde}{\tbd{hlLossInvBootburnMde}}
\providecommand{\hlLossInvBootburnN}{\tbd{hlLossInvBootburnN}}
\providecommand{\hlLossInvBootburnPHolm}{\tbd{hlLossInvBootburnPHolm}}
\providecommand{\hlLossInvBootburnTostCIHi}{\tbd{hlLossInvBootburnTostCIHi}}
\providecommand{\hlLossInvBootburnTostCILo}{\tbd{hlLossInvBootburnTostCILo}}
\providecommand{\hlLossInvBootflairCIHi}{\tbd{hlLossInvBootflairCIHi}}
\providecommand{\hlLossInvBootflairCILo}{\tbd{hlLossInvBootflairCILo}}
\providecommand{\hlLossInvBootflairEst}{\tbd{hlLossInvBootflairEst}}
\providecommand{\hlLossInvBootflairMde}{\tbd{hlLossInvBootflairMde}}
\providecommand{\hlLossInvBootflairN}{\tbd{hlLossInvBootflairN}}
\providecommand{\hlLossInvBootflairPHolm}{\tbd{hlLossInvBootflairPHolm}}
\providecommand{\hlLossInvBootflairTostCIHi}{\tbd{hlLossInvBootflairTostCIHi}}
\providecommand{\hlLossInvBootflairTostCILo}{\tbd{hlLossInvBootflairTostCILo}}
\providecommand{\hlLossInvGceDOFAburnCIHi}{\tbd{hlLossInvGceDOFAburnCIHi}}
\providecommand{\hlLossInvGceDOFAburnCILo}{\tbd{hlLossInvGceDOFAburnCILo}}
\providecommand{\hlLossInvGceDOFAburnEst}{\tbd{hlLossInvGceDOFAburnEst}}
\providecommand{\hlLossInvGceDOFAburnMde}{\tbd{hlLossInvGceDOFAburnMde}}
\providecommand{\hlLossInvGceDOFAburnN}{\tbd{hlLossInvGceDOFAburnN}}
\providecommand{\hlLossInvGceDOFAburnPHolm}{\tbd{hlLossInvGceDOFAburnPHolm}}
\providecommand{\hlLossInvGceDOFAburnTostCIHi}{\tbd{hlLossInvGceDOFAburnTostCIHi}}
\providecommand{\hlLossInvGceDOFAburnTostCILo}{\tbd{hlLossInvGceDOFAburnTostCILo}}
\providecommand{\hlLossInvGceDOFAflairCIHi}{\tbd{hlLossInvGceDOFAflairCIHi}}
\providecommand{\hlLossInvGceDOFAflairCILo}{\tbd{hlLossInvGceDOFAflairCILo}}
\providecommand{\hlLossInvGceDOFAflairEst}{\tbd{hlLossInvGceDOFAflairEst}}
\providecommand{\hlLossInvGceDOFAflairMde}{\tbd{hlLossInvGceDOFAflairMde}}
\providecommand{\hlLossInvGceDOFAflairN}{\tbd{hlLossInvGceDOFAflairN}}
\providecommand{\hlLossInvGceDOFAflairPHolm}{\tbd{hlLossInvGceDOFAflairPHolm}}
\providecommand{\hlLossInvGceDOFAflairTostCIHi}{\tbd{hlLossInvGceDOFAflairTostCIHi}}
\providecommand{\hlLossInvGceDOFAflairTostCILo}{\tbd{hlLossInvGceDOFAflairTostCILo}}
\providecommand{\hlLossInvGceLVDburnCIHi}{\tbd{hlLossInvGceLVDburnCIHi}}
\providecommand{\hlLossInvGceLVDburnCILo}{\tbd{hlLossInvGceLVDburnCILo}}
\providecommand{\hlLossInvGceLVDburnEst}{\tbd{hlLossInvGceLVDburnEst}}
\providecommand{\hlLossInvGceLVDburnMde}{\tbd{hlLossInvGceLVDburnMde}}
\providecommand{\hlLossInvGceLVDburnN}{\tbd{hlLossInvGceLVDburnN}}
\providecommand{\hlLossInvGceLVDburnPHolm}{\tbd{hlLossInvGceLVDburnPHolm}}
\providecommand{\hlLossInvGceLVDburnTostCIHi}{\tbd{hlLossInvGceLVDburnTostCIHi}}
\providecommand{\hlLossInvGceLVDburnTostCILo}{\tbd{hlLossInvGceLVDburnTostCILo}}
\providecommand{\hlLossInvGceLVDflairCIHi}{\tbd{hlLossInvGceLVDflairCIHi}}
\providecommand{\hlLossInvGceLVDflairCILo}{\tbd{hlLossInvGceLVDflairCILo}}
\providecommand{\hlLossInvGceLVDflairEst}{\tbd{hlLossInvGceLVDflairEst}}
\providecommand{\hlLossInvGceLVDflairMde}{\tbd{hlLossInvGceLVDflairMde}}
\providecommand{\hlLossInvGceLVDflairN}{\tbd{hlLossInvGceLVDflairN}}
\providecommand{\hlLossInvGceLVDflairPHolm}{\tbd{hlLossInvGceLVDflairPHolm}}
\providecommand{\hlLossInvGceLVDflairTostCIHi}{\tbd{hlLossInvGceLVDflairTostCIHi}}
\providecommand{\hlLossInvGceLVDflairTostCILo}{\tbd{hlLossInvGceLVDflairTostCILo}}
\providecommand{\hlLossInvGceRNburnCIHi}{\tbd{hlLossInvGceRNburnCIHi}}
\providecommand{\hlLossInvGceRNburnCILo}{\tbd{hlLossInvGceRNburnCILo}}
\providecommand{\hlLossInvGceRNburnEst}{\tbd{hlLossInvGceRNburnEst}}
\providecommand{\hlLossInvGceRNburnMde}{\tbd{hlLossInvGceRNburnMde}}
\providecommand{\hlLossInvGceRNburnN}{\tbd{hlLossInvGceRNburnN}}
\providecommand{\hlLossInvGceRNburnPHolm}{\tbd{hlLossInvGceRNburnPHolm}}
\providecommand{\hlLossInvGceRNburnTostCIHi}{\tbd{hlLossInvGceRNburnTostCIHi}}
\providecommand{\hlLossInvGceRNburnTostCILo}{\tbd{hlLossInvGceRNburnTostCILo}}
\providecommand{\hlLossInvGceRNflairCIHi}{\tbd{hlLossInvGceRNflairCIHi}}
\providecommand{\hlLossInvGceRNflairCILo}{\tbd{hlLossInvGceRNflairCILo}}
\providecommand{\hlLossInvGceRNflairEst}{\tbd{hlLossInvGceRNflairEst}}
\providecommand{\hlLossInvGceRNflairMde}{\tbd{hlLossInvGceRNflairMde}}
\providecommand{\hlLossInvGceRNflairN}{\tbd{hlLossInvGceRNflairN}}
\providecommand{\hlLossInvGceRNflairPHolm}{\tbd{hlLossInvGceRNflairPHolm}}
\providecommand{\hlLossInvGceRNflairTostCIHi}{\tbd{hlLossInvGceRNflairTostCIHi}}
\providecommand{\hlLossInvGceRNflairTostCILo}{\tbd{hlLossInvGceRNflairTostCILo}}
\providecommand{\hlLossInvGceSATburnCIHi}{\tbd{hlLossInvGceSATburnCIHi}}
\providecommand{\hlLossInvGceSATburnCILo}{\tbd{hlLossInvGceSATburnCILo}}
\providecommand{\hlLossInvGceSATburnEst}{\tbd{hlLossInvGceSATburnEst}}
\providecommand{\hlLossInvGceSATburnMde}{\tbd{hlLossInvGceSATburnMde}}
\providecommand{\hlLossInvGceSATburnN}{\tbd{hlLossInvGceSATburnN}}
\providecommand{\hlLossInvGceSATburnPHolm}{\tbd{hlLossInvGceSATburnPHolm}}
\providecommand{\hlLossInvGceSATburnTostCIHi}{\tbd{hlLossInvGceSATburnTostCIHi}}
\providecommand{\hlLossInvGceSATburnTostCILo}{\tbd{hlLossInvGceSATburnTostCILo}}
\providecommand{\hlLossInvGceSATflairCIHi}{\tbd{hlLossInvGceSATflairCIHi}}
\providecommand{\hlLossInvGceSATflairCILo}{\tbd{hlLossInvGceSATflairCILo}}
\providecommand{\hlLossInvGceSATflairEst}{\tbd{hlLossInvGceSATflairEst}}
\providecommand{\hlLossInvGceSATflairMde}{\tbd{hlLossInvGceSATflairMde}}
\providecommand{\hlLossInvGceSATflairN}{\tbd{hlLossInvGceSATflairN}}
\providecommand{\hlLossInvGceSATflairPHolm}{\tbd{hlLossInvGceSATflairPHolm}}
\providecommand{\hlLossInvGceSATflairTostCIHi}{\tbd{hlLossInvGceSATflairTostCIHi}}
\providecommand{\hlLossInvGceSATflairTostCILo}{\tbd{hlLossInvGceSATflairTostCILo}}
\providecommand{\hlLossInvGceTMburnCIHi}{\tbd{hlLossInvGceTMburnCIHi}}
\providecommand{\hlLossInvGceTMburnCILo}{\tbd{hlLossInvGceTMburnCILo}}
\providecommand{\hlLossInvGceTMburnEst}{\tbd{hlLossInvGceTMburnEst}}
\providecommand{\hlLossInvGceTMburnMde}{\tbd{hlLossInvGceTMburnMde}}
\providecommand{\hlLossInvGceTMburnN}{\tbd{hlLossInvGceTMburnN}}
\providecommand{\hlLossInvGceTMburnPHolm}{\tbd{hlLossInvGceTMburnPHolm}}
\providecommand{\hlLossInvGceTMburnTostCIHi}{\tbd{hlLossInvGceTMburnTostCIHi}}
\providecommand{\hlLossInvGceTMburnTostCILo}{\tbd{hlLossInvGceTMburnTostCILo}}
\providecommand{\hlLossInvGceTMflairCIHi}{\tbd{hlLossInvGceTMflairCIHi}}
\providecommand{\hlLossInvGceTMflairCILo}{\tbd{hlLossInvGceTMflairCILo}}
\providecommand{\hlLossInvGceTMflairEst}{\tbd{hlLossInvGceTMflairEst}}
\providecommand{\hlLossInvGceTMflairMde}{\tbd{hlLossInvGceTMflairMde}}
\providecommand{\hlLossInvGceTMflairN}{\tbd{hlLossInvGceTMflairN}}
\providecommand{\hlLossInvGceTMflairPHolm}{\tbd{hlLossInvGceTMflairPHolm}}
\providecommand{\hlLossInvGceTMflairTostCIHi}{\tbd{hlLossInvGceTMflairTostCIHi}}
\providecommand{\hlLossInvGceTMflairTostCILo}{\tbd{hlLossInvGceTMflairTostCILo}}
\providecommand{\hlLossInvGceburnCIHi}{\tbd{hlLossInvGceburnCIHi}}
\providecommand{\hlLossInvGceburnCILo}{\tbd{hlLossInvGceburnCILo}}
\providecommand{\hlLossInvGceburnEst}{\tbd{hlLossInvGceburnEst}}
\providecommand{\hlLossInvGceburnMde}{\tbd{hlLossInvGceburnMde}}
\providecommand{\hlLossInvGceburnN}{\tbd{hlLossInvGceburnN}}
\providecommand{\hlLossInvGceburnPHolm}{\tbd{hlLossInvGceburnPHolm}}
\providecommand{\hlLossInvGceburnTostCIHi}{\tbd{hlLossInvGceburnTostCIHi}}
\providecommand{\hlLossInvGceburnTostCILo}{\tbd{hlLossInvGceburnTostCILo}}
\providecommand{\hlLossInvGceflairCIHi}{\tbd{hlLossInvGceflairCIHi}}
\providecommand{\hlLossInvGceflairCILo}{\tbd{hlLossInvGceflairCILo}}
\providecommand{\hlLossInvGceflairEst}{\tbd{hlLossInvGceflairEst}}
\providecommand{\hlLossInvGceflairMde}{\tbd{hlLossInvGceflairMde}}
\providecommand{\hlLossInvGceflairN}{\tbd{hlLossInvGceflairN}}
\providecommand{\hlLossInvGceflairPHolm}{\tbd{hlLossInvGceflairPHolm}}
\providecommand{\hlLossInvGceflairTostCIHi}{\tbd{hlLossInvGceflairTostCIHi}}
\providecommand{\hlLossInvGceflairTostCILo}{\tbd{hlLossInvGceflairTostCILo}}
\providecommand{\hlLossVerdictBootburn}{\tbd{hlLossVerdictBootburn}}
\providecommand{\hlLossVerdictBootflair}{\tbd{hlLossVerdictBootflair}}
\providecommand{\hlLossVerdictGceburn}{\tbd{hlLossVerdictGceburn}}
\providecommand{\hlLossVerdictGceflair}{\tbd{hlLossVerdictGceflair}}
\providecommand{\hlLrDropDOFAburnBoundary}{\tbd{hlLrDropDOFAburnBoundary}}
\providecommand{\hlLrDropDOFAburnBoundaryCIHi}{\tbd{hlLrDropDOFAburnBoundaryCIHi}}
\providecommand{\hlLrDropDOFAburnBoundaryCILo}{\tbd{hlLrDropDOFAburnBoundaryCILo}}
\providecommand{\hlLrDropDOFAburnCoarse}{\tbd{hlLrDropDOFAburnCoarse}}
\providecommand{\hlLrDropDOFAburnCoarseCIHi}{\tbd{hlLrDropDOFAburnCoarseCIHi}}
\providecommand{\hlLrDropDOFAburnCoarseCILo}{\tbd{hlLrDropDOFAburnCoarseCILo}}
\providecommand{\hlLrDropDOFAburnOmission}{\tbd{hlLrDropDOFAburnOmission}}
\providecommand{\hlLrDropDOFAburnOmissionCIHi}{\tbd{hlLrDropDOFAburnOmissionCIHi}}
\providecommand{\hlLrDropDOFAburnOmissionCILo}{\tbd{hlLrDropDOFAburnOmissionCILo}}
\providecommand{\hlLrDropDOFAburnShift}{\tbd{hlLrDropDOFAburnShift}}
\providecommand{\hlLrDropDOFAburnShiftCIHi}{\tbd{hlLrDropDOFAburnShiftCIHi}}
\providecommand{\hlLrDropDOFAburnShiftCILo}{\tbd{hlLrDropDOFAburnShiftCILo}}
\providecommand{\hlLrDropDOFAflairBoundary}{\tbd{hlLrDropDOFAflairBoundary}}
\providecommand{\hlLrDropDOFAflairBoundaryCIHi}{\tbd{hlLrDropDOFAflairBoundaryCIHi}}
\providecommand{\hlLrDropDOFAflairBoundaryCILo}{\tbd{hlLrDropDOFAflairBoundaryCILo}}
\providecommand{\hlLrDropDOFAflairCoarse}{\tbd{hlLrDropDOFAflairCoarse}}
\providecommand{\hlLrDropDOFAflairCoarseCIHi}{\tbd{hlLrDropDOFAflairCoarseCIHi}}
\providecommand{\hlLrDropDOFAflairCoarseCILo}{\tbd{hlLrDropDOFAflairCoarseCILo}}
\providecommand{\hlLrDropDOFAflairOmission}{\tbd{hlLrDropDOFAflairOmission}}
\providecommand{\hlLrDropDOFAflairOmissionCIHi}{\tbd{hlLrDropDOFAflairOmissionCIHi}}
\providecommand{\hlLrDropDOFAflairOmissionCILo}{\tbd{hlLrDropDOFAflairOmissionCILo}}
\providecommand{\hlLrDropDOFAflairShift}{\tbd{hlLrDropDOFAflairShift}}
\providecommand{\hlLrDropDOFAflairShiftCIHi}{\tbd{hlLrDropDOFAflairShiftCIHi}}
\providecommand{\hlLrDropDOFAflairShiftCILo}{\tbd{hlLrDropDOFAflairShiftCILo}}
\providecommand{\hlLrDropLVDburnBoundary}{\tbd{hlLrDropLVDburnBoundary}}
\providecommand{\hlLrDropLVDburnBoundaryCIHi}{\tbd{hlLrDropLVDburnBoundaryCIHi}}
\providecommand{\hlLrDropLVDburnBoundaryCILo}{\tbd{hlLrDropLVDburnBoundaryCILo}}
\providecommand{\hlLrDropLVDburnCoarse}{\tbd{hlLrDropLVDburnCoarse}}
\providecommand{\hlLrDropLVDburnCoarseCIHi}{\tbd{hlLrDropLVDburnCoarseCIHi}}
\providecommand{\hlLrDropLVDburnCoarseCILo}{\tbd{hlLrDropLVDburnCoarseCILo}}
\providecommand{\hlLrDropLVDburnOmission}{\tbd{hlLrDropLVDburnOmission}}
\providecommand{\hlLrDropLVDburnOmissionCIHi}{\tbd{hlLrDropLVDburnOmissionCIHi}}
\providecommand{\hlLrDropLVDburnOmissionCILo}{\tbd{hlLrDropLVDburnOmissionCILo}}
\providecommand{\hlLrDropLVDburnShift}{\tbd{hlLrDropLVDburnShift}}
\providecommand{\hlLrDropLVDburnShiftCIHi}{\tbd{hlLrDropLVDburnShiftCIHi}}
\providecommand{\hlLrDropLVDburnShiftCILo}{\tbd{hlLrDropLVDburnShiftCILo}}
\providecommand{\hlLrDropLVDflairBoundary}{\tbd{hlLrDropLVDflairBoundary}}
\providecommand{\hlLrDropLVDflairBoundaryCIHi}{\tbd{hlLrDropLVDflairBoundaryCIHi}}
\providecommand{\hlLrDropLVDflairBoundaryCILo}{\tbd{hlLrDropLVDflairBoundaryCILo}}
\providecommand{\hlLrDropLVDflairCoarse}{\tbd{hlLrDropLVDflairCoarse}}
\providecommand{\hlLrDropLVDflairCoarseCIHi}{\tbd{hlLrDropLVDflairCoarseCIHi}}
\providecommand{\hlLrDropLVDflairCoarseCILo}{\tbd{hlLrDropLVDflairCoarseCILo}}
\providecommand{\hlLrDropLVDflairOmission}{\tbd{hlLrDropLVDflairOmission}}
\providecommand{\hlLrDropLVDflairOmissionCIHi}{\tbd{hlLrDropLVDflairOmissionCIHi}}
\providecommand{\hlLrDropLVDflairOmissionCILo}{\tbd{hlLrDropLVDflairOmissionCILo}}
\providecommand{\hlLrDropLVDflairShift}{\tbd{hlLrDropLVDflairShift}}
\providecommand{\hlLrDropLVDflairShiftCIHi}{\tbd{hlLrDropLVDflairShiftCIHi}}
\providecommand{\hlLrDropLVDflairShiftCILo}{\tbd{hlLrDropLVDflairShiftCILo}}
\providecommand{\hlLrDropRNburnBoundary}{\tbd{hlLrDropRNburnBoundary}}
\providecommand{\hlLrDropRNburnBoundaryCIHi}{\tbd{hlLrDropRNburnBoundaryCIHi}}
\providecommand{\hlLrDropRNburnBoundaryCILo}{\tbd{hlLrDropRNburnBoundaryCILo}}
\providecommand{\hlLrDropRNburnCoarse}{\tbd{hlLrDropRNburnCoarse}}
\providecommand{\hlLrDropRNburnCoarseCIHi}{\tbd{hlLrDropRNburnCoarseCIHi}}
\providecommand{\hlLrDropRNburnCoarseCILo}{\tbd{hlLrDropRNburnCoarseCILo}}
\providecommand{\hlLrDropRNburnOmission}{\tbd{hlLrDropRNburnOmission}}
\providecommand{\hlLrDropRNburnOmissionCIHi}{\tbd{hlLrDropRNburnOmissionCIHi}}
\providecommand{\hlLrDropRNburnOmissionCILo}{\tbd{hlLrDropRNburnOmissionCILo}}
\providecommand{\hlLrDropRNburnShift}{\tbd{hlLrDropRNburnShift}}
\providecommand{\hlLrDropRNburnShiftCIHi}{\tbd{hlLrDropRNburnShiftCIHi}}
\providecommand{\hlLrDropRNburnShiftCILo}{\tbd{hlLrDropRNburnShiftCILo}}
\providecommand{\hlLrDropRNflairBoundary}{\tbd{hlLrDropRNflairBoundary}}
\providecommand{\hlLrDropRNflairBoundaryCIHi}{\tbd{hlLrDropRNflairBoundaryCIHi}}
\providecommand{\hlLrDropRNflairBoundaryCILo}{\tbd{hlLrDropRNflairBoundaryCILo}}
\providecommand{\hlLrDropRNflairCoarse}{\tbd{hlLrDropRNflairCoarse}}
\providecommand{\hlLrDropRNflairCoarseCIHi}{\tbd{hlLrDropRNflairCoarseCIHi}}
\providecommand{\hlLrDropRNflairCoarseCILo}{\tbd{hlLrDropRNflairCoarseCILo}}
\providecommand{\hlLrDropRNflairOmission}{\tbd{hlLrDropRNflairOmission}}
\providecommand{\hlLrDropRNflairOmissionCIHi}{\tbd{hlLrDropRNflairOmissionCIHi}}
\providecommand{\hlLrDropRNflairOmissionCILo}{\tbd{hlLrDropRNflairOmissionCILo}}
\providecommand{\hlLrDropRNflairShift}{\tbd{hlLrDropRNflairShift}}
\providecommand{\hlLrDropRNflairShiftCIHi}{\tbd{hlLrDropRNflairShiftCIHi}}
\providecommand{\hlLrDropRNflairShiftCILo}{\tbd{hlLrDropRNflairShiftCILo}}
\providecommand{\hlLrDropSATburnBoundary}{\tbd{hlLrDropSATburnBoundary}}
\providecommand{\hlLrDropSATburnBoundaryCIHi}{\tbd{hlLrDropSATburnBoundaryCIHi}}
\providecommand{\hlLrDropSATburnBoundaryCILo}{\tbd{hlLrDropSATburnBoundaryCILo}}
\providecommand{\hlLrDropSATburnCoarse}{\tbd{hlLrDropSATburnCoarse}}
\providecommand{\hlLrDropSATburnCoarseCIHi}{\tbd{hlLrDropSATburnCoarseCIHi}}
\providecommand{\hlLrDropSATburnCoarseCILo}{\tbd{hlLrDropSATburnCoarseCILo}}
\providecommand{\hlLrDropSATburnOmission}{\tbd{hlLrDropSATburnOmission}}
\providecommand{\hlLrDropSATburnOmissionCIHi}{\tbd{hlLrDropSATburnOmissionCIHi}}
\providecommand{\hlLrDropSATburnOmissionCILo}{\tbd{hlLrDropSATburnOmissionCILo}}
\providecommand{\hlLrDropSATburnShift}{\tbd{hlLrDropSATburnShift}}
\providecommand{\hlLrDropSATburnShiftCIHi}{\tbd{hlLrDropSATburnShiftCIHi}}
\providecommand{\hlLrDropSATburnShiftCILo}{\tbd{hlLrDropSATburnShiftCILo}}
\providecommand{\hlLrDropSATflairBoundary}{\tbd{hlLrDropSATflairBoundary}}
\providecommand{\hlLrDropSATflairBoundaryCIHi}{\tbd{hlLrDropSATflairBoundaryCIHi}}
\providecommand{\hlLrDropSATflairBoundaryCILo}{\tbd{hlLrDropSATflairBoundaryCILo}}
\providecommand{\hlLrDropSATflairCoarse}{\tbd{hlLrDropSATflairCoarse}}
\providecommand{\hlLrDropSATflairCoarseCIHi}{\tbd{hlLrDropSATflairCoarseCIHi}}
\providecommand{\hlLrDropSATflairCoarseCILo}{\tbd{hlLrDropSATflairCoarseCILo}}
\providecommand{\hlLrDropSATflairOmission}{\tbd{hlLrDropSATflairOmission}}
\providecommand{\hlLrDropSATflairOmissionCIHi}{\tbd{hlLrDropSATflairOmissionCIHi}}
\providecommand{\hlLrDropSATflairOmissionCILo}{\tbd{hlLrDropSATflairOmissionCILo}}
\providecommand{\hlLrDropSATflairShift}{\tbd{hlLrDropSATflairShift}}
\providecommand{\hlLrDropSATflairShiftCIHi}{\tbd{hlLrDropSATflairShiftCIHi}}
\providecommand{\hlLrDropSATflairShiftCILo}{\tbd{hlLrDropSATflairShiftCILo}}
\providecommand{\hlLrDropTMburnBoundary}{\tbd{hlLrDropTMburnBoundary}}
\providecommand{\hlLrDropTMburnBoundaryCIHi}{\tbd{hlLrDropTMburnBoundaryCIHi}}
\providecommand{\hlLrDropTMburnBoundaryCILo}{\tbd{hlLrDropTMburnBoundaryCILo}}
\providecommand{\hlLrDropTMburnCoarse}{\tbd{hlLrDropTMburnCoarse}}
\providecommand{\hlLrDropTMburnCoarseCIHi}{\tbd{hlLrDropTMburnCoarseCIHi}}
\providecommand{\hlLrDropTMburnCoarseCILo}{\tbd{hlLrDropTMburnCoarseCILo}}
\providecommand{\hlLrDropTMburnOmission}{\tbd{hlLrDropTMburnOmission}}
\providecommand{\hlLrDropTMburnOmissionCIHi}{\tbd{hlLrDropTMburnOmissionCIHi}}
\providecommand{\hlLrDropTMburnOmissionCILo}{\tbd{hlLrDropTMburnOmissionCILo}}
\providecommand{\hlLrDropTMburnShift}{\tbd{hlLrDropTMburnShift}}
\providecommand{\hlLrDropTMburnShiftCIHi}{\tbd{hlLrDropTMburnShiftCIHi}}
\providecommand{\hlLrDropTMburnShiftCILo}{\tbd{hlLrDropTMburnShiftCILo}}
\providecommand{\hlLrDropTMflairBoundary}{\tbd{hlLrDropTMflairBoundary}}
\providecommand{\hlLrDropTMflairBoundaryCIHi}{\tbd{hlLrDropTMflairBoundaryCIHi}}
\providecommand{\hlLrDropTMflairBoundaryCILo}{\tbd{hlLrDropTMflairBoundaryCILo}}
\providecommand{\hlLrDropTMflairCoarse}{\tbd{hlLrDropTMflairCoarse}}
\providecommand{\hlLrDropTMflairCoarseCIHi}{\tbd{hlLrDropTMflairCoarseCIHi}}
\providecommand{\hlLrDropTMflairCoarseCILo}{\tbd{hlLrDropTMflairCoarseCILo}}
\providecommand{\hlLrDropTMflairOmission}{\tbd{hlLrDropTMflairOmission}}
\providecommand{\hlLrDropTMflairOmissionCIHi}{\tbd{hlLrDropTMflairOmissionCIHi}}
\providecommand{\hlLrDropTMflairOmissionCILo}{\tbd{hlLrDropTMflairOmissionCILo}}
\providecommand{\hlLrDropTMflairShift}{\tbd{hlLrDropTMflairShift}}
\providecommand{\hlLrDropTMflairShiftCIHi}{\tbd{hlLrDropTMflairShiftCIHi}}
\providecommand{\hlLrDropTMflairShiftCILo}{\tbd{hlLrDropTMflairShiftCILo}}
\providecommand{\hlLrFOneOneburnCIHi}{\tbd{hlLrFOneOneburnCIHi}}
\providecommand{\hlLrFOneOneburnCILo}{\tbd{hlLrFOneOneburnCILo}}
\providecommand{\hlLrFOneOneburnEst}{\tbd{hlLrFOneOneburnEst}}
\providecommand{\hlLrFOneOneburnMde}{\tbd{hlLrFOneOneburnMde}}
\providecommand{\hlLrFOneOneburnN}{\tbd{hlLrFOneOneburnN}}
\providecommand{\hlLrFOneOneburnPHolm}{\tbd{hlLrFOneOneburnPHolm}}
\providecommand{\hlLrFOneOneburnTostCIHi}{\tbd{hlLrFOneOneburnTostCIHi}}
\providecommand{\hlLrFOneOneburnTostCILo}{\tbd{hlLrFOneOneburnTostCILo}}
\providecommand{\hlLrFOneOneflairCIHi}{\tbd{hlLrFOneOneflairCIHi}}
\providecommand{\hlLrFOneOneflairCILo}{\tbd{hlLrFOneOneflairCILo}}
\providecommand{\hlLrFOneOneflairEst}{\tbd{hlLrFOneOneflairEst}}
\providecommand{\hlLrFOneOneflairMde}{\tbd{hlLrFOneOneflairMde}}
\providecommand{\hlLrFOneOneflairN}{\tbd{hlLrFOneOneflairN}}
\providecommand{\hlLrFOneOneflairPHolm}{\tbd{hlLrFOneOneflairPHolm}}
\providecommand{\hlLrFOneOneflairTostCIHi}{\tbd{hlLrFOneOneflairTostCIHi}}
\providecommand{\hlLrFOneOneflairTostCILo}{\tbd{hlLrFOneOneflairTostCILo}}
\providecommand{\hlLrFOneburnCIHi}{\tbd{hlLrFOneburnCIHi}}
\providecommand{\hlLrFOneburnCILo}{\tbd{hlLrFOneburnCILo}}
\providecommand{\hlLrFOneburnEst}{\tbd{hlLrFOneburnEst}}
\providecommand{\hlLrFOneburnMde}{\tbd{hlLrFOneburnMde}}
\providecommand{\hlLrFOneburnN}{\tbd{hlLrFOneburnN}}
\providecommand{\hlLrFOneburnPHolm}{\tbd{hlLrFOneburnPHolm}}
\providecommand{\hlLrFOneburnTostCIHi}{\tbd{hlLrFOneburnTostCIHi}}
\providecommand{\hlLrFOneburnTostCILo}{\tbd{hlLrFOneburnTostCILo}}
\providecommand{\hlLrFOneflairCIHi}{\tbd{hlLrFOneflairCIHi}}
\providecommand{\hlLrFOneflairCILo}{\tbd{hlLrFOneflairCILo}}
\providecommand{\hlLrFOneflairEst}{\tbd{hlLrFOneflairEst}}
\providecommand{\hlLrFOneflairMde}{\tbd{hlLrFOneflairMde}}
\providecommand{\hlLrFOneflairN}{\tbd{hlLrFOneflairN}}
\providecommand{\hlLrFOneflairPHolm}{\tbd{hlLrFOneflairPHolm}}
\providecommand{\hlLrFOneflairTostCIHi}{\tbd{hlLrFOneflairTostCIHi}}
\providecommand{\hlLrFOneflairTostCILo}{\tbd{hlLrFOneflairTostCILo}}
\providecommand{\hlLrFTwoburnCIHi}{\tbd{hlLrFTwoburnCIHi}}
\providecommand{\hlLrFTwoburnCILo}{\tbd{hlLrFTwoburnCILo}}
\providecommand{\hlLrFTwoburnEst}{\tbd{hlLrFTwoburnEst}}
\providecommand{\hlLrFTwoburnMde}{\tbd{hlLrFTwoburnMde}}
\providecommand{\hlLrFTwoburnN}{\tbd{hlLrFTwoburnN}}
\providecommand{\hlLrFTwoburnPHolm}{\tbd{hlLrFTwoburnPHolm}}
\providecommand{\hlLrFTwoburnTostCIHi}{\tbd{hlLrFTwoburnTostCIHi}}
\providecommand{\hlLrFTwoburnTostCILo}{\tbd{hlLrFTwoburnTostCILo}}
\providecommand{\hlLrFTwoflairCIHi}{\tbd{hlLrFTwoflairCIHi}}
\providecommand{\hlLrFTwoflairCILo}{\tbd{hlLrFTwoflairCILo}}
\providecommand{\hlLrFTwoflairEst}{\tbd{hlLrFTwoflairEst}}
\providecommand{\hlLrFTwoflairMde}{\tbd{hlLrFTwoflairMde}}
\providecommand{\hlLrFTwoflairN}{\tbd{hlLrFTwoflairN}}
\providecommand{\hlLrFTwoflairPHolm}{\tbd{hlLrFTwoflairPHolm}}
\providecommand{\hlLrFTwoflairTostCIHi}{\tbd{hlLrFTwoflairTostCIHi}}
\providecommand{\hlLrFTwoflairTostCILo}{\tbd{hlLrFTwoflairTostCILo}}
\providecommand{\hlLrMeanDropDOFAburn}{\tbd{hlLrMeanDropDOFAburn}}
\providecommand{\hlLrMeanDropDOFAflair}{\tbd{hlLrMeanDropDOFAflair}}
\providecommand{\hlLrMeanDropLVDburn}{\tbd{hlLrMeanDropLVDburn}}
\providecommand{\hlLrMeanDropLVDflair}{\tbd{hlLrMeanDropLVDflair}}
\providecommand{\hlLrMeanDropRNburn}{\tbd{hlLrMeanDropRNburn}}
\providecommand{\hlLrMeanDropRNflair}{\tbd{hlLrMeanDropRNflair}}
\providecommand{\hlLrMeanDropSATburn}{\tbd{hlLrMeanDropSATburn}}
\providecommand{\hlLrMeanDropSATflair}{\tbd{hlLrMeanDropSATflair}}
\providecommand{\hlLrMeanDropTMburn}{\tbd{hlLrMeanDropTMburn}}
\providecommand{\hlLrMeanDropTMflair}{\tbd{hlLrMeanDropTMflair}}
\providecommand{\hlLrMeanDropburn}{\tbd{hlLrMeanDropburn}}
\providecommand{\hlLrMeanDropflair}{\tbd{hlLrMeanDropflair}}
\providecommand{\hlLrMinusLOneburnCIHi}{\tbd{hlLrMinusLOneburnCIHi}}
\providecommand{\hlLrMinusLOneburnCILo}{\tbd{hlLrMinusLOneburnCILo}}
\providecommand{\hlLrMinusLOneburnEst}{\tbd{hlLrMinusLOneburnEst}}
\providecommand{\hlLrMinusLOneburnMde}{\tbd{hlLrMinusLOneburnMde}}
\providecommand{\hlLrMinusLOneburnN}{\tbd{hlLrMinusLOneburnN}}
\providecommand{\hlLrMinusLOneburnPHolm}{\tbd{hlLrMinusLOneburnPHolm}}
\providecommand{\hlLrMinusLOneburnTostCIHi}{\tbd{hlLrMinusLOneburnTostCIHi}}
\providecommand{\hlLrMinusLOneburnTostCILo}{\tbd{hlLrMinusLOneburnTostCILo}}
\providecommand{\hlLrMinusLOneflairCIHi}{\tbd{hlLrMinusLOneflairCIHi}}
\providecommand{\hlLrMinusLOneflairCILo}{\tbd{hlLrMinusLOneflairCILo}}
\providecommand{\hlLrMinusLOneflairEst}{\tbd{hlLrMinusLOneflairEst}}
\providecommand{\hlLrMinusLOneflairMde}{\tbd{hlLrMinusLOneflairMde}}
\providecommand{\hlLrMinusLOneflairN}{\tbd{hlLrMinusLOneflairN}}
\providecommand{\hlLrMinusLOneflairPHolm}{\tbd{hlLrMinusLOneflairPHolm}}
\providecommand{\hlLrMinusLOneflairTostCIHi}{\tbd{hlLrMinusLOneflairTostCIHi}}
\providecommand{\hlLrMinusLOneflairTostCILo}{\tbd{hlLrMinusLOneflairTostCILo}}
\providecommand{\hlLrMinusLTwoburnCIHi}{\tbd{hlLrMinusLTwoburnCIHi}}
\providecommand{\hlLrMinusLTwoburnCILo}{\tbd{hlLrMinusLTwoburnCILo}}
\providecommand{\hlLrMinusLTwoburnEst}{\tbd{hlLrMinusLTwoburnEst}}
\providecommand{\hlLrMinusLTwoburnMde}{\tbd{hlLrMinusLTwoburnMde}}
\providecommand{\hlLrMinusLTwoburnN}{\tbd{hlLrMinusLTwoburnN}}
\providecommand{\hlLrMinusLTwoburnPHolm}{\tbd{hlLrMinusLTwoburnPHolm}}
\providecommand{\hlLrMinusLTwoburnTostCIHi}{\tbd{hlLrMinusLTwoburnTostCIHi}}
\providecommand{\hlLrMinusLTwoburnTostCILo}{\tbd{hlLrMinusLTwoburnTostCILo}}
\providecommand{\hlLrMinusLTwoflairCIHi}{\tbd{hlLrMinusLTwoflairCIHi}}
\providecommand{\hlLrMinusLTwoflairCILo}{\tbd{hlLrMinusLTwoflairCILo}}
\providecommand{\hlLrMinusLTwoflairEst}{\tbd{hlLrMinusLTwoflairEst}}
\providecommand{\hlLrMinusLTwoflairMde}{\tbd{hlLrMinusLTwoflairMde}}
\providecommand{\hlLrMinusLTwoflairN}{\tbd{hlLrMinusLTwoflairN}}
\providecommand{\hlLrMinusLTwoflairPHolm}{\tbd{hlLrMinusLTwoflairPHolm}}
\providecommand{\hlLrMinusLTwoflairTostCIHi}{\tbd{hlLrMinusLTwoflairTostCIHi}}
\providecommand{\hlLrMinusLTwoflairTostCILo}{\tbd{hlLrMinusLTwoflairTostCILo}}
\providecommand{\hlLrNSixburnCIHi}{\tbd{hlLrNSixburnCIHi}}
\providecommand{\hlLrNSixburnCILo}{\tbd{hlLrNSixburnCILo}}
\providecommand{\hlLrNSixburnEst}{\tbd{hlLrNSixburnEst}}
\providecommand{\hlLrNSixburnMde}{\tbd{hlLrNSixburnMde}}
\providecommand{\hlLrNSixburnN}{\tbd{hlLrNSixburnN}}
\providecommand{\hlLrNSixburnPHolm}{\tbd{hlLrNSixburnPHolm}}
\providecommand{\hlLrNSixburnTostCIHi}{\tbd{hlLrNSixburnTostCIHi}}
\providecommand{\hlLrNSixburnTostCILo}{\tbd{hlLrNSixburnTostCILo}}
\providecommand{\hlLrNSixflairCIHi}{\tbd{hlLrNSixflairCIHi}}
\providecommand{\hlLrNSixflairCILo}{\tbd{hlLrNSixflairCILo}}
\providecommand{\hlLrNSixflairEst}{\tbd{hlLrNSixflairEst}}
\providecommand{\hlLrNSixflairMde}{\tbd{hlLrNSixflairMde}}
\providecommand{\hlLrNSixflairN}{\tbd{hlLrNSixflairN}}
\providecommand{\hlLrNSixflairPHolm}{\tbd{hlLrNSixflairPHolm}}
\providecommand{\hlLrNSixflairTostCIHi}{\tbd{hlLrNSixflairTostCIHi}}
\providecommand{\hlLrNSixflairTostCILo}{\tbd{hlLrNSixflairTostCILo}}
\providecommand{\hlLrRankSameburn}{\tbd{hlLrRankSameburn}}
\providecommand{\hlLrRankSameflair}{\tbd{hlLrRankSameflair}}
\providecommand{\hlLrRankVerdictburn}{\tbd{hlLrRankVerdictburn}}
\providecommand{\hlLrRankVerdictflair}{\tbd{hlLrRankVerdictflair}}
\providecommand{\hlLrRefDropDOFAburnLOne}{\tbd{hlLrRefDropDOFAburnLOne}}
\providecommand{\hlLrRefDropDOFAburnLTwo}{\tbd{hlLrRefDropDOFAburnLTwo}}
\providecommand{\hlLrRefDropDOFAflairLOne}{\tbd{hlLrRefDropDOFAflairLOne}}
\providecommand{\hlLrRefDropDOFAflairLTwo}{\tbd{hlLrRefDropDOFAflairLTwo}}
\providecommand{\hlLrRefDropLVDburnLOne}{\tbd{hlLrRefDropLVDburnLOne}}
\providecommand{\hlLrRefDropLVDburnLTwo}{\tbd{hlLrRefDropLVDburnLTwo}}
\providecommand{\hlLrRefDropLVDflairLOne}{\tbd{hlLrRefDropLVDflairLOne}}
\providecommand{\hlLrRefDropLVDflairLTwo}{\tbd{hlLrRefDropLVDflairLTwo}}
\providecommand{\hlLrRefDropRNburnLOne}{\tbd{hlLrRefDropRNburnLOne}}
\providecommand{\hlLrRefDropRNburnLTwo}{\tbd{hlLrRefDropRNburnLTwo}}
\providecommand{\hlLrRefDropRNflairLOne}{\tbd{hlLrRefDropRNflairLOne}}
\providecommand{\hlLrRefDropRNflairLTwo}{\tbd{hlLrRefDropRNflairLTwo}}
\providecommand{\hlLrRefDropSATburnLOne}{\tbd{hlLrRefDropSATburnLOne}}
\providecommand{\hlLrRefDropSATburnLTwo}{\tbd{hlLrRefDropSATburnLTwo}}
\providecommand{\hlLrRefDropSATflairLOne}{\tbd{hlLrRefDropSATflairLOne}}
\providecommand{\hlLrRefDropSATflairLTwo}{\tbd{hlLrRefDropSATflairLTwo}}
\providecommand{\hlLrRefDropTMburnLOne}{\tbd{hlLrRefDropTMburnLOne}}
\providecommand{\hlLrRefDropTMburnLTwo}{\tbd{hlLrRefDropTMburnLTwo}}
\providecommand{\hlLrRefDropTMflairLOne}{\tbd{hlLrRefDropTMflairLOne}}
\providecommand{\hlLrRefDropTMflairLTwo}{\tbd{hlLrRefDropTMflairLTwo}}
\providecommand{\hlLrRefDropburnLOne}{\tbd{hlLrRefDropburnLOne}}
\providecommand{\hlLrRefDropburnLTwo}{\tbd{hlLrRefDropburnLTwo}}
\providecommand{\hlLrRefDropflairLOne}{\tbd{hlLrRefDropflairLOne}}
\providecommand{\hlLrRefDropflairLTwo}{\tbd{hlLrRefDropflairLTwo}}
\providecommand{\hlLrTypeRankburnFour}{\tbd{hlLrTypeRankburnFour}}
\providecommand{\hlLrTypeRankburnOne}{\tbd{hlLrTypeRankburnOne}}
\providecommand{\hlLrTypeRankburnThree}{\tbd{hlLrTypeRankburnThree}}
\providecommand{\hlLrTypeRankburnTwo}{\tbd{hlLrTypeRankburnTwo}}
\providecommand{\hlLrTypeRankflairFour}{\tbd{hlLrTypeRankflairFour}}
\providecommand{\hlLrTypeRankflairOne}{\tbd{hlLrTypeRankflairOne}}
\providecommand{\hlLrTypeRankflairThree}{\tbd{hlLrTypeRankflairThree}}
\providecommand{\hlLrTypeRankflairTwo}{\tbd{hlLrTypeRankflairTwo}}
\providecommand{\hlLrVerdictFTwoburn}{\tbd{hlLrVerdictFTwoburn}}
\providecommand{\hlLrVerdictFTwoflair}{\tbd{hlLrVerdictFTwoflair}}
\providecommand{\hlLrVerdictNSixburn}{\tbd{hlLrVerdictNSixburn}}
\providecommand{\hlLrVerdictNSixflair}{\tbd{hlLrVerdictNSixflair}}
\providecommand{\hlLrVerdictburn}{\tbd{hlLrVerdictburn}}
\providecommand{\hlLrVerdictflair}{\tbd{hlLrVerdictflair}}
\providecommand{\hlMeanDropLTwoCNXLburn}{\tbd{hlMeanDropLTwoCNXLburn}}
\providecommand{\hlMeanDropLTwoCNXLflair}{\tbd{hlMeanDropLTwoCNXLflair}}
\providecommand{\hlMeanDropLTwoDOFAburn}{\tbd{hlMeanDropLTwoDOFAburn}}
\providecommand{\hlMeanDropLTwoDOFAflair}{\tbd{hlMeanDropLTwoDOFAflair}}
\providecommand{\hlMeanDropLTwoLVDburn}{\tbd{hlMeanDropLTwoLVDburn}}
\providecommand{\hlMeanDropLTwoLVDflair}{\tbd{hlMeanDropLTwoLVDflair}}
\providecommand{\hlMeanDropLTwoPRIburn}{\tbd{hlMeanDropLTwoPRIburn}}
\providecommand{\hlMeanDropLTwoPRIflair}{\tbd{hlMeanDropLTwoPRIflair}}
\providecommand{\hlMeanDropLTwoRNSSLburn}{\tbd{hlMeanDropLTwoRNSSLburn}}
\providecommand{\hlMeanDropLTwoRNSSLflair}{\tbd{hlMeanDropLTwoRNSSLflair}}
\providecommand{\hlMeanDropLTwoRNburn}{\tbd{hlMeanDropLTwoRNburn}}
\providecommand{\hlMeanDropLTwoRNflair}{\tbd{hlMeanDropLTwoRNflair}}
\providecommand{\hlMeanDropLTwoSATburn}{\tbd{hlMeanDropLTwoSATburn}}
\providecommand{\hlMeanDropLTwoSATflair}{\tbd{hlMeanDropLTwoSATflair}}
\providecommand{\hlMeanDropLTwoTMburn}{\tbd{hlMeanDropLTwoTMburn}}
\providecommand{\hlMeanDropLTwoTMflair}{\tbd{hlMeanDropLTwoTMflair}}
\providecommand{\hlMeanDropLTwoVITRburn}{\tbd{hlMeanDropLTwoVITRburn}}
\providecommand{\hlMeanDropLTwoVITRflair}{\tbd{hlMeanDropLTwoVITRflair}}
\providecommand{\hlMemPerClassDOFAburnBackground}{\tbd{hlMemPerClassDOFAburnBackground}}
\providecommand{\hlMemPerClassDOFAburnBackgroundCI}{\tbd{hlMemPerClassDOFAburnBackgroundCI}}
\providecommand{\hlMemPerClassDOFAburnBurnScar}{\tbd{hlMemPerClassDOFAburnBurnScar}}
\providecommand{\hlMemPerClassDOFAburnBurnScarCI}{\tbd{hlMemPerClassDOFAburnBurnScarCI}}
\providecommand{\hlMemPerClassLVDburnBackground}{\tbd{hlMemPerClassLVDburnBackground}}
\providecommand{\hlMemPerClassLVDburnBackgroundCI}{\tbd{hlMemPerClassLVDburnBackgroundCI}}
\providecommand{\hlMemPerClassLVDburnBurnScar}{\tbd{hlMemPerClassLVDburnBurnScar}}
\providecommand{\hlMemPerClassLVDburnBurnScarCI}{\tbd{hlMemPerClassLVDburnBurnScarCI}}
\providecommand{\hlMemPerClassRNburnBackground}{\tbd{hlMemPerClassRNburnBackground}}
\providecommand{\hlMemPerClassRNburnBackgroundCI}{\tbd{hlMemPerClassRNburnBackgroundCI}}
\providecommand{\hlMemPerClassRNburnBurnScar}{\tbd{hlMemPerClassRNburnBurnScar}}
\providecommand{\hlMemPerClassRNburnBurnScarCI}{\tbd{hlMemPerClassRNburnBurnScarCI}}
\providecommand{\hlMemPerClassSATNSixburnBackground}{\tbd{hlMemPerClassSATNSixburnBackground}}
\providecommand{\hlMemPerClassSATNSixburnBackgroundCI}{\tbd{hlMemPerClassSATNSixburnBackgroundCI}}
\providecommand{\hlMemPerClassSATNSixburnBurnScar}{\tbd{hlMemPerClassSATNSixburnBurnScar}}
\providecommand{\hlMemPerClassSATNSixburnBurnScarCI}{\tbd{hlMemPerClassSATNSixburnBurnScarCI}}
\providecommand{\hlMemPerClassSATburnBackground}{\tbd{hlMemPerClassSATburnBackground}}
\providecommand{\hlMemPerClassSATburnBackgroundCI}{\tbd{hlMemPerClassSATburnBackgroundCI}}
\providecommand{\hlMemPerClassSATburnBurnScar}{\tbd{hlMemPerClassSATburnBurnScar}}
\providecommand{\hlMemPerClassSATburnBurnScarCI}{\tbd{hlMemPerClassSATburnBurnScarCI}}
\providecommand{\hlMemPerClassTMburnBackground}{\tbd{hlMemPerClassTMburnBackground}}
\providecommand{\hlMemPerClassTMburnBackgroundCI}{\tbd{hlMemPerClassTMburnBackgroundCI}}
\providecommand{\hlMemPerClassTMburnBurnScar}{\tbd{hlMemPerClassTMburnBurnScar}}
\providecommand{\hlMemPerClassTMburnBurnScarCI}{\tbd{hlMemPerClassTMburnBurnScarCI}}
\providecommand{\hlMemRateCIDOFAburn}{\tbd{hlMemRateCIDOFAburn}}
\providecommand{\hlMemRateCIDOFAflair}{\tbd{hlMemRateCIDOFAflair}}
\providecommand{\hlMemRateCILVDburn}{\tbd{hlMemRateCILVDburn}}
\providecommand{\hlMemRateCILVDflair}{\tbd{hlMemRateCILVDflair}}
\providecommand{\hlMemRateCIRNburn}{\tbd{hlMemRateCIRNburn}}
\providecommand{\hlMemRateCIRNflair}{\tbd{hlMemRateCIRNflair}}
\providecommand{\hlMemRateCISATNSixburn}{\tbd{hlMemRateCISATNSixburn}}
\providecommand{\hlMemRateCISATNSixflair}{\tbd{hlMemRateCISATNSixflair}}
\providecommand{\hlMemRateCISATburn}{\tbd{hlMemRateCISATburn}}
\providecommand{\hlMemRateCISATflair}{\tbd{hlMemRateCISATflair}}
\providecommand{\hlMemRateCITMburn}{\tbd{hlMemRateCITMburn}}
\providecommand{\hlMemRateCITMflair}{\tbd{hlMemRateCITMflair}}
\providecommand{\hlMemRateDOFAburn}{\tbd{hlMemRateDOFAburn}}
\providecommand{\hlMemRateDOFAflair}{\tbd{hlMemRateDOFAflair}}
\providecommand{\hlMemRateLVDburn}{\tbd{hlMemRateLVDburn}}
\providecommand{\hlMemRateLVDflair}{\tbd{hlMemRateLVDflair}}
\providecommand{\hlMemRateRNburn}{\tbd{hlMemRateRNburn}}
\providecommand{\hlMemRateRNflair}{\tbd{hlMemRateRNflair}}
\providecommand{\hlMemRateSATNSixburn}{\tbd{hlMemRateSATNSixburn}}
\providecommand{\hlMemRateSATNSixflair}{\tbd{hlMemRateSATNSixflair}}
\providecommand{\hlMemRateSATburn}{\tbd{hlMemRateSATburn}}
\providecommand{\hlMemRateSATflair}{\tbd{hlMemRateSATflair}}
\providecommand{\hlMemRateTMburn}{\tbd{hlMemRateTMburn}}
\providecommand{\hlMemRateTMflair}{\tbd{hlMemRateTMflair}}
\providecommand{\hlMitBootBoundaryburnCIHi}{\tbd{hlMitBootBoundaryburnCIHi}}
\providecommand{\hlMitBootBoundaryburnCILo}{\tbd{hlMitBootBoundaryburnCILo}}
\providecommand{\hlMitBootBoundaryburnEst}{\tbd{hlMitBootBoundaryburnEst}}
\providecommand{\hlMitBootBoundaryflairCIHi}{\tbd{hlMitBootBoundaryflairCIHi}}
\providecommand{\hlMitBootBoundaryflairCILo}{\tbd{hlMitBootBoundaryflairCILo}}
\providecommand{\hlMitBootBoundaryflairEst}{\tbd{hlMitBootBoundaryflairEst}}
\providecommand{\hlMitBootCleanCostburnCIHi}{\tbd{hlMitBootCleanCostburnCIHi}}
\providecommand{\hlMitBootCleanCostburnCILo}{\tbd{hlMitBootCleanCostburnCILo}}
\providecommand{\hlMitBootCleanCostburnEst}{\tbd{hlMitBootCleanCostburnEst}}
\providecommand{\hlMitBootCleanCostflairCIHi}{\tbd{hlMitBootCleanCostflairCIHi}}
\providecommand{\hlMitBootCleanCostflairCILo}{\tbd{hlMitBootCleanCostflairCILo}}
\providecommand{\hlMitBootCleanCostflairEst}{\tbd{hlMitBootCleanCostflairEst}}
\providecommand{\hlMitBootCleanDOFAburn}{\tbd{hlMitBootCleanDOFAburn}}
\providecommand{\hlMitBootCleanDOFAflair}{\tbd{hlMitBootCleanDOFAflair}}
\providecommand{\hlMitBootCleanLVDburn}{\tbd{hlMitBootCleanLVDburn}}
\providecommand{\hlMitBootCleanLVDflair}{\tbd{hlMitBootCleanLVDflair}}
\providecommand{\hlMitBootCleanRNburn}{\tbd{hlMitBootCleanRNburn}}
\providecommand{\hlMitBootCleanRNflair}{\tbd{hlMitBootCleanRNflair}}
\providecommand{\hlMitBootCleanSATburn}{\tbd{hlMitBootCleanSATburn}}
\providecommand{\hlMitBootCleanSATflair}{\tbd{hlMitBootCleanSATflair}}
\providecommand{\hlMitBootCleanTMburn}{\tbd{hlMitBootCleanTMburn}}
\providecommand{\hlMitBootCleanTMflair}{\tbd{hlMitBootCleanTMflair}}
\providecommand{\hlMitBootCoarseburnCIHi}{\tbd{hlMitBootCoarseburnCIHi}}
\providecommand{\hlMitBootCoarseburnCILo}{\tbd{hlMitBootCoarseburnCILo}}
\providecommand{\hlMitBootCoarseburnEst}{\tbd{hlMitBootCoarseburnEst}}
\providecommand{\hlMitBootCoarseflairCIHi}{\tbd{hlMitBootCoarseflairCIHi}}
\providecommand{\hlMitBootCoarseflairCILo}{\tbd{hlMitBootCoarseflairCILo}}
\providecommand{\hlMitBootCoarseflairEst}{\tbd{hlMitBootCoarseflairEst}}
\providecommand{\hlMitBootDOFAburnCIHi}{\tbd{hlMitBootDOFAburnCIHi}}
\providecommand{\hlMitBootDOFAburnCILo}{\tbd{hlMitBootDOFAburnCILo}}
\providecommand{\hlMitBootDOFAburnEst}{\tbd{hlMitBootDOFAburnEst}}
\providecommand{\hlMitBootDOFAflairCIHi}{\tbd{hlMitBootDOFAflairCIHi}}
\providecommand{\hlMitBootDOFAflairCILo}{\tbd{hlMitBootDOFAflairCILo}}
\providecommand{\hlMitBootDOFAflairEst}{\tbd{hlMitBootDOFAflairEst}}
\providecommand{\hlMitBootDropDOFAburn}{\tbd{hlMitBootDropDOFAburn}}
\providecommand{\hlMitBootDropDOFAflair}{\tbd{hlMitBootDropDOFAflair}}
\providecommand{\hlMitBootDropLVDburn}{\tbd{hlMitBootDropLVDburn}}
\providecommand{\hlMitBootDropLVDflair}{\tbd{hlMitBootDropLVDflair}}
\providecommand{\hlMitBootDropRNburn}{\tbd{hlMitBootDropRNburn}}
\providecommand{\hlMitBootDropRNflair}{\tbd{hlMitBootDropRNflair}}
\providecommand{\hlMitBootDropSATburn}{\tbd{hlMitBootDropSATburn}}
\providecommand{\hlMitBootDropSATflair}{\tbd{hlMitBootDropSATflair}}
\providecommand{\hlMitBootDropTMburn}{\tbd{hlMitBootDropTMburn}}
\providecommand{\hlMitBootDropTMflair}{\tbd{hlMitBootDropTMflair}}
\providecommand{\hlMitBootLVDburnCIHi}{\tbd{hlMitBootLVDburnCIHi}}
\providecommand{\hlMitBootLVDburnCILo}{\tbd{hlMitBootLVDburnCILo}}
\providecommand{\hlMitBootLVDburnEst}{\tbd{hlMitBootLVDburnEst}}
\providecommand{\hlMitBootLVDflairCIHi}{\tbd{hlMitBootLVDflairCIHi}}
\providecommand{\hlMitBootLVDflairCILo}{\tbd{hlMitBootLVDflairCILo}}
\providecommand{\hlMitBootLVDflairEst}{\tbd{hlMitBootLVDflairEst}}
\providecommand{\hlMitBootOmissionburnCIHi}{\tbd{hlMitBootOmissionburnCIHi}}
\providecommand{\hlMitBootOmissionburnCILo}{\tbd{hlMitBootOmissionburnCILo}}
\providecommand{\hlMitBootOmissionburnEst}{\tbd{hlMitBootOmissionburnEst}}
\providecommand{\hlMitBootOmissionflairCIHi}{\tbd{hlMitBootOmissionflairCIHi}}
\providecommand{\hlMitBootOmissionflairCILo}{\tbd{hlMitBootOmissionflairCILo}}
\providecommand{\hlMitBootOmissionflairEst}{\tbd{hlMitBootOmissionflairEst}}
\providecommand{\hlMitBootRNburnCIHi}{\tbd{hlMitBootRNburnCIHi}}
\providecommand{\hlMitBootRNburnCILo}{\tbd{hlMitBootRNburnCILo}}
\providecommand{\hlMitBootRNburnEst}{\tbd{hlMitBootRNburnEst}}
\providecommand{\hlMitBootRNflairCIHi}{\tbd{hlMitBootRNflairCIHi}}
\providecommand{\hlMitBootRNflairCILo}{\tbd{hlMitBootRNflairCILo}}
\providecommand{\hlMitBootRNflairEst}{\tbd{hlMitBootRNflairEst}}
\providecommand{\hlMitBootSATburnCIHi}{\tbd{hlMitBootSATburnCIHi}}
\providecommand{\hlMitBootSATburnCILo}{\tbd{hlMitBootSATburnCILo}}
\providecommand{\hlMitBootSATburnEst}{\tbd{hlMitBootSATburnEst}}
\providecommand{\hlMitBootSATflairCIHi}{\tbd{hlMitBootSATflairCIHi}}
\providecommand{\hlMitBootSATflairCILo}{\tbd{hlMitBootSATflairCILo}}
\providecommand{\hlMitBootSATflairEst}{\tbd{hlMitBootSATflairEst}}
\providecommand{\hlMitBootShiftburnCIHi}{\tbd{hlMitBootShiftburnCIHi}}
\providecommand{\hlMitBootShiftburnCILo}{\tbd{hlMitBootShiftburnCILo}}
\providecommand{\hlMitBootShiftburnEst}{\tbd{hlMitBootShiftburnEst}}
\providecommand{\hlMitBootShiftflairCIHi}{\tbd{hlMitBootShiftflairCIHi}}
\providecommand{\hlMitBootShiftflairCILo}{\tbd{hlMitBootShiftflairCILo}}
\providecommand{\hlMitBootShiftflairEst}{\tbd{hlMitBootShiftflairEst}}
\providecommand{\hlMitBootTMburnCIHi}{\tbd{hlMitBootTMburnCIHi}}
\providecommand{\hlMitBootTMburnCILo}{\tbd{hlMitBootTMburnCILo}}
\providecommand{\hlMitBootTMburnEst}{\tbd{hlMitBootTMburnEst}}
\providecommand{\hlMitBootTMflairCIHi}{\tbd{hlMitBootTMflairCIHi}}
\providecommand{\hlMitBootTMflairCILo}{\tbd{hlMitBootTMflairCILo}}
\providecommand{\hlMitBootTMflairEst}{\tbd{hlMitBootTMflairEst}}
\providecommand{\hlMitBootburnCIHi}{\tbd{hlMitBootburnCIHi}}
\providecommand{\hlMitBootburnCILo}{\tbd{hlMitBootburnCILo}}
\providecommand{\hlMitBootburnEst}{\tbd{hlMitBootburnEst}}
\providecommand{\hlMitBootburnMde}{\tbd{hlMitBootburnMde}}
\providecommand{\hlMitBootburnN}{\tbd{hlMitBootburnN}}
\providecommand{\hlMitBootburnPHolm}{\tbd{hlMitBootburnPHolm}}
\providecommand{\hlMitBootburnTostCIHi}{\tbd{hlMitBootburnTostCIHi}}
\providecommand{\hlMitBootburnTostCILo}{\tbd{hlMitBootburnTostCILo}}
\providecommand{\hlMitBootflairCIHi}{\tbd{hlMitBootflairCIHi}}
\providecommand{\hlMitBootflairCILo}{\tbd{hlMitBootflairCILo}}
\providecommand{\hlMitBootflairEst}{\tbd{hlMitBootflairEst}}
\providecommand{\hlMitBootflairMde}{\tbd{hlMitBootflairMde}}
\providecommand{\hlMitBootflairN}{\tbd{hlMitBootflairN}}
\providecommand{\hlMitBootflairPHolm}{\tbd{hlMitBootflairPHolm}}
\providecommand{\hlMitBootflairTostCIHi}{\tbd{hlMitBootflairTostCIHi}}
\providecommand{\hlMitBootflairTostCILo}{\tbd{hlMitBootflairTostCILo}}
\providecommand{\hlMitGceBoundaryburnCIHi}{\tbd{hlMitGceBoundaryburnCIHi}}
\providecommand{\hlMitGceBoundaryburnCILo}{\tbd{hlMitGceBoundaryburnCILo}}
\providecommand{\hlMitGceBoundaryburnEst}{\tbd{hlMitGceBoundaryburnEst}}
\providecommand{\hlMitGceBoundaryflairCIHi}{\tbd{hlMitGceBoundaryflairCIHi}}
\providecommand{\hlMitGceBoundaryflairCILo}{\tbd{hlMitGceBoundaryflairCILo}}
\providecommand{\hlMitGceBoundaryflairEst}{\tbd{hlMitGceBoundaryflairEst}}
\providecommand{\hlMitGceCleanCostburnCIHi}{\tbd{hlMitGceCleanCostburnCIHi}}
\providecommand{\hlMitGceCleanCostburnCILo}{\tbd{hlMitGceCleanCostburnCILo}}
\providecommand{\hlMitGceCleanCostburnEst}{\tbd{hlMitGceCleanCostburnEst}}
\providecommand{\hlMitGceCleanCostflairCIHi}{\tbd{hlMitGceCleanCostflairCIHi}}
\providecommand{\hlMitGceCleanCostflairCILo}{\tbd{hlMitGceCleanCostflairCILo}}
\providecommand{\hlMitGceCleanCostflairEst}{\tbd{hlMitGceCleanCostflairEst}}
\providecommand{\hlMitGceCleanDOFAburn}{\tbd{hlMitGceCleanDOFAburn}}
\providecommand{\hlMitGceCleanDOFAflair}{\tbd{hlMitGceCleanDOFAflair}}
\providecommand{\hlMitGceCleanLVDburn}{\tbd{hlMitGceCleanLVDburn}}
\providecommand{\hlMitGceCleanLVDflair}{\tbd{hlMitGceCleanLVDflair}}
\providecommand{\hlMitGceCleanRNburn}{\tbd{hlMitGceCleanRNburn}}
\providecommand{\hlMitGceCleanRNflair}{\tbd{hlMitGceCleanRNflair}}
\providecommand{\hlMitGceCleanSATburn}{\tbd{hlMitGceCleanSATburn}}
\providecommand{\hlMitGceCleanSATflair}{\tbd{hlMitGceCleanSATflair}}
\providecommand{\hlMitGceCleanTMburn}{\tbd{hlMitGceCleanTMburn}}
\providecommand{\hlMitGceCleanTMflair}{\tbd{hlMitGceCleanTMflair}}
\providecommand{\hlMitGceCoarseburnCIHi}{\tbd{hlMitGceCoarseburnCIHi}}
\providecommand{\hlMitGceCoarseburnCILo}{\tbd{hlMitGceCoarseburnCILo}}
\providecommand{\hlMitGceCoarseburnEst}{\tbd{hlMitGceCoarseburnEst}}
\providecommand{\hlMitGceCoarseflairCIHi}{\tbd{hlMitGceCoarseflairCIHi}}
\providecommand{\hlMitGceCoarseflairCILo}{\tbd{hlMitGceCoarseflairCILo}}
\providecommand{\hlMitGceCoarseflairEst}{\tbd{hlMitGceCoarseflairEst}}
\providecommand{\hlMitGceDOFAburnCIHi}{\tbd{hlMitGceDOFAburnCIHi}}
\providecommand{\hlMitGceDOFAburnCILo}{\tbd{hlMitGceDOFAburnCILo}}
\providecommand{\hlMitGceDOFAburnEst}{\tbd{hlMitGceDOFAburnEst}}
\providecommand{\hlMitGceDOFAflairCIHi}{\tbd{hlMitGceDOFAflairCIHi}}
\providecommand{\hlMitGceDOFAflairCILo}{\tbd{hlMitGceDOFAflairCILo}}
\providecommand{\hlMitGceDOFAflairEst}{\tbd{hlMitGceDOFAflairEst}}
\providecommand{\hlMitGceDropDOFAburn}{\tbd{hlMitGceDropDOFAburn}}
\providecommand{\hlMitGceDropDOFAflair}{\tbd{hlMitGceDropDOFAflair}}
\providecommand{\hlMitGceDropLVDburn}{\tbd{hlMitGceDropLVDburn}}
\providecommand{\hlMitGceDropLVDflair}{\tbd{hlMitGceDropLVDflair}}
\providecommand{\hlMitGceDropRNburn}{\tbd{hlMitGceDropRNburn}}
\providecommand{\hlMitGceDropRNflair}{\tbd{hlMitGceDropRNflair}}
\providecommand{\hlMitGceDropSATburn}{\tbd{hlMitGceDropSATburn}}
\providecommand{\hlMitGceDropSATflair}{\tbd{hlMitGceDropSATflair}}
\providecommand{\hlMitGceDropTMburn}{\tbd{hlMitGceDropTMburn}}
\providecommand{\hlMitGceDropTMflair}{\tbd{hlMitGceDropTMflair}}
\providecommand{\hlMitGceLVDburnCIHi}{\tbd{hlMitGceLVDburnCIHi}}
\providecommand{\hlMitGceLVDburnCILo}{\tbd{hlMitGceLVDburnCILo}}
\providecommand{\hlMitGceLVDburnEst}{\tbd{hlMitGceLVDburnEst}}
\providecommand{\hlMitGceLVDflairCIHi}{\tbd{hlMitGceLVDflairCIHi}}
\providecommand{\hlMitGceLVDflairCILo}{\tbd{hlMitGceLVDflairCILo}}
\providecommand{\hlMitGceLVDflairEst}{\tbd{hlMitGceLVDflairEst}}
\providecommand{\hlMitGceOmissionburnCIHi}{\tbd{hlMitGceOmissionburnCIHi}}
\providecommand{\hlMitGceOmissionburnCILo}{\tbd{hlMitGceOmissionburnCILo}}
\providecommand{\hlMitGceOmissionburnEst}{\tbd{hlMitGceOmissionburnEst}}
\providecommand{\hlMitGceOmissionflairCIHi}{\tbd{hlMitGceOmissionflairCIHi}}
\providecommand{\hlMitGceOmissionflairCILo}{\tbd{hlMitGceOmissionflairCILo}}
\providecommand{\hlMitGceOmissionflairEst}{\tbd{hlMitGceOmissionflairEst}}
\providecommand{\hlMitGceRNburnCIHi}{\tbd{hlMitGceRNburnCIHi}}
\providecommand{\hlMitGceRNburnCILo}{\tbd{hlMitGceRNburnCILo}}
\providecommand{\hlMitGceRNburnEst}{\tbd{hlMitGceRNburnEst}}
\providecommand{\hlMitGceRNflairCIHi}{\tbd{hlMitGceRNflairCIHi}}
\providecommand{\hlMitGceRNflairCILo}{\tbd{hlMitGceRNflairCILo}}
\providecommand{\hlMitGceRNflairEst}{\tbd{hlMitGceRNflairEst}}
\providecommand{\hlMitGceSATburnCIHi}{\tbd{hlMitGceSATburnCIHi}}
\providecommand{\hlMitGceSATburnCILo}{\tbd{hlMitGceSATburnCILo}}
\providecommand{\hlMitGceSATburnEst}{\tbd{hlMitGceSATburnEst}}
\providecommand{\hlMitGceSATflairCIHi}{\tbd{hlMitGceSATflairCIHi}}
\providecommand{\hlMitGceSATflairCILo}{\tbd{hlMitGceSATflairCILo}}
\providecommand{\hlMitGceSATflairEst}{\tbd{hlMitGceSATflairEst}}
\providecommand{\hlMitGceShiftburnCIHi}{\tbd{hlMitGceShiftburnCIHi}}
\providecommand{\hlMitGceShiftburnCILo}{\tbd{hlMitGceShiftburnCILo}}
\providecommand{\hlMitGceShiftburnEst}{\tbd{hlMitGceShiftburnEst}}
\providecommand{\hlMitGceShiftflairCIHi}{\tbd{hlMitGceShiftflairCIHi}}
\providecommand{\hlMitGceShiftflairCILo}{\tbd{hlMitGceShiftflairCILo}}
\providecommand{\hlMitGceShiftflairEst}{\tbd{hlMitGceShiftflairEst}}
\providecommand{\hlMitGceTMburnCIHi}{\tbd{hlMitGceTMburnCIHi}}
\providecommand{\hlMitGceTMburnCILo}{\tbd{hlMitGceTMburnCILo}}
\providecommand{\hlMitGceTMburnEst}{\tbd{hlMitGceTMburnEst}}
\providecommand{\hlMitGceTMflairCIHi}{\tbd{hlMitGceTMflairCIHi}}
\providecommand{\hlMitGceTMflairCILo}{\tbd{hlMitGceTMflairCILo}}
\providecommand{\hlMitGceTMflairEst}{\tbd{hlMitGceTMflairEst}}
\providecommand{\hlMitGceburnCIHi}{\tbd{hlMitGceburnCIHi}}
\providecommand{\hlMitGceburnCILo}{\tbd{hlMitGceburnCILo}}
\providecommand{\hlMitGceburnEst}{\tbd{hlMitGceburnEst}}
\providecommand{\hlMitGceburnMde}{\tbd{hlMitGceburnMde}}
\providecommand{\hlMitGceburnN}{\tbd{hlMitGceburnN}}
\providecommand{\hlMitGceburnPHolm}{\tbd{hlMitGceburnPHolm}}
\providecommand{\hlMitGceburnTostCIHi}{\tbd{hlMitGceburnTostCIHi}}
\providecommand{\hlMitGceburnTostCILo}{\tbd{hlMitGceburnTostCILo}}
\providecommand{\hlMitGceflairCIHi}{\tbd{hlMitGceflairCIHi}}
\providecommand{\hlMitGceflairCILo}{\tbd{hlMitGceflairCILo}}
\providecommand{\hlMitGceflairEst}{\tbd{hlMitGceflairEst}}
\providecommand{\hlMitGceflairMde}{\tbd{hlMitGceflairMde}}
\providecommand{\hlMitGceflairN}{\tbd{hlMitGceflairN}}
\providecommand{\hlMitGceflairPHolm}{\tbd{hlMitGceflairPHolm}}
\providecommand{\hlMitGceflairTostCIHi}{\tbd{hlMitGceflairTostCIHi}}
\providecommand{\hlMitGceflairTostCILo}{\tbd{hlMitGceflairTostCILo}}
\providecommand{\hlMitVerdictBootburn}{\tbd{hlMitVerdictBootburn}}
\providecommand{\hlMitVerdictBootflair}{\tbd{hlMitVerdictBootflair}}
\providecommand{\hlMitVerdictGceburn}{\tbd{hlMitVerdictGceburn}}
\providecommand{\hlMitVerdictGceflair}{\tbd{hlMitVerdictGceflair}}
\providecommand{\hlMixedCoefburnCoarse}{\tbd{hlMixedCoefburnCoarse}}
\providecommand{\hlMixedCoefburnOmission}{\tbd{hlMixedCoefburnOmission}}
\providecommand{\hlMixedCoefburnShift}{\tbd{hlMixedCoefburnShift}}
\providecommand{\hlMixedCoefflairCoarse}{\tbd{hlMixedCoefflairCoarse}}
\providecommand{\hlMixedCoefflairOmission}{\tbd{hlMixedCoefflairOmission}}
\providecommand{\hlMixedCoefflairShift}{\tbd{hlMixedCoefflairShift}}
\providecommand{\hlMixedConvergedburn}{\tbd{hlMixedConvergedburn}}
\providecommand{\hlMixedConvergedflair}{\tbd{hlMixedConvergedflair}}
\providecommand{\hlMixedSEburnCoarse}{\tbd{hlMixedSEburnCoarse}}
\providecommand{\hlMixedSEburnOmission}{\tbd{hlMixedSEburnOmission}}
\providecommand{\hlMixedSEburnShift}{\tbd{hlMixedSEburnShift}}
\providecommand{\hlMixedSEflairCoarse}{\tbd{hlMixedSEflairCoarse}}
\providecommand{\hlMixedSEflairOmission}{\tbd{hlMixedSEflairOmission}}
\providecommand{\hlMixedSEflairShift}{\tbd{hlMixedSEflairShift}}
\providecommand{\hlMixedUsableburn}{\tbd{hlMixedUsableburn}}
\providecommand{\hlMixedUsableflair}{\tbd{hlMixedUsableflair}}
\providecommand{\hlMlrDropDiffCIHiburn}{\tbd{hlMlrDropDiffCIHiburn}}
\providecommand{\hlMlrDropDiffCIHiflair}{\tbd{hlMlrDropDiffCIHiflair}}
\providecommand{\hlMlrDropDiffCILoburn}{\tbd{hlMlrDropDiffCILoburn}}
\providecommand{\hlMlrDropDiffCILoflair}{\tbd{hlMlrDropDiffCILoflair}}
\providecommand{\hlMlrDropDiffHalfburn}{\tbd{hlMlrDropDiffHalfburn}}
\providecommand{\hlMlrDropDiffHalfflair}{\tbd{hlMlrDropDiffHalfflair}}
\providecommand{\hlMlrDropDiffburn}{\tbd{hlMlrDropDiffburn}}
\providecommand{\hlMlrDropDiffflair}{\tbd{hlMlrDropDiffflair}}
\providecommand{\hlMlrDropLVDburn}{\tbd{hlMlrDropLVDburn}}
\providecommand{\hlMlrDropLVDflair}{\tbd{hlMlrDropLVDflair}}
\providecommand{\hlMlrDropNburn}{\tbd{hlMlrDropNburn}}
\providecommand{\hlMlrDropNflair}{\tbd{hlMlrDropNflair}}
\providecommand{\hlMlrDropSATburn}{\tbd{hlMlrDropSATburn}}
\providecommand{\hlMlrDropSATflair}{\tbd{hlMlrDropSATflair}}
\providecommand{\hlMlrDropTostCIHiburn}{\tbd{hlMlrDropTostCIHiburn}}
\providecommand{\hlMlrDropTostCIHiflair}{\tbd{hlMlrDropTostCIHiflair}}
\providecommand{\hlMlrDropTostCILoburn}{\tbd{hlMlrDropTostCILoburn}}
\providecommand{\hlMlrDropTostCILoflair}{\tbd{hlMlrDropTostCILoflair}}
\providecommand{\hlMlrDropTostEquivalentburn}{\tbd{hlMlrDropTostEquivalentburn}}
\providecommand{\hlMlrDropTostEquivalentflair}{\tbd{hlMlrDropTostEquivalentflair}}
\providecommand{\hlMlrDropTostPburn}{\tbd{hlMlrDropTostPburn}}
\providecommand{\hlMlrDropTostPflair}{\tbd{hlMlrDropTostPflair}}
\providecommand{\hlMlrRetDiffCIHiburn}{\tbd{hlMlrRetDiffCIHiburn}}
\providecommand{\hlMlrRetDiffCIHiflair}{\tbd{hlMlrRetDiffCIHiflair}}
\providecommand{\hlMlrRetDiffCILoburn}{\tbd{hlMlrRetDiffCILoburn}}
\providecommand{\hlMlrRetDiffCILoflair}{\tbd{hlMlrRetDiffCILoflair}}
\providecommand{\hlMlrRetDiffHalfburn}{\tbd{hlMlrRetDiffHalfburn}}
\providecommand{\hlMlrRetDiffHalfflair}{\tbd{hlMlrRetDiffHalfflair}}
\providecommand{\hlMlrRetDiffburn}{\tbd{hlMlrRetDiffburn}}
\providecommand{\hlMlrRetDiffflair}{\tbd{hlMlrRetDiffflair}}
\providecommand{\hlMlrRetLVDburn}{\tbd{hlMlrRetLVDburn}}
\providecommand{\hlMlrRetLVDflair}{\tbd{hlMlrRetLVDflair}}
\providecommand{\hlMlrRetNburn}{\tbd{hlMlrRetNburn}}
\providecommand{\hlMlrRetNflair}{\tbd{hlMlrRetNflair}}
\providecommand{\hlMlrRetSATburn}{\tbd{hlMlrRetSATburn}}
\providecommand{\hlMlrRetSATflair}{\tbd{hlMlrRetSATflair}}
\providecommand{\hlMlrRetTostCIHiburn}{\tbd{hlMlrRetTostCIHiburn}}
\providecommand{\hlMlrRetTostCIHiflair}{\tbd{hlMlrRetTostCIHiflair}}
\providecommand{\hlMlrRetTostCILoburn}{\tbd{hlMlrRetTostCILoburn}}
\providecommand{\hlMlrRetTostCILoflair}{\tbd{hlMlrRetTostCILoflair}}
\providecommand{\hlMlrRetTostEquivalentburn}{\tbd{hlMlrRetTostEquivalentburn}}
\providecommand{\hlMlrRetTostEquivalentflair}{\tbd{hlMlrRetTostEquivalentflair}}
\providecommand{\hlMlrRetTostPburn}{\tbd{hlMlrRetTostPburn}}
\providecommand{\hlMlrRetTostPflair}{\tbd{hlMlrRetTostPflair}}
\providecommand{\hlMraBestRateDOFAburn}{\tbd{hlMraBestRateDOFAburn}}
\providecommand{\hlMraBestRateDOFAflair}{\tbd{hlMraBestRateDOFAflair}}
\providecommand{\hlMraBestRateLVDburn}{\tbd{hlMraBestRateLVDburn}}
\providecommand{\hlMraBestRateLVDflair}{\tbd{hlMraBestRateLVDflair}}
\providecommand{\hlMraBestRateRNburn}{\tbd{hlMraBestRateRNburn}}
\providecommand{\hlMraBestRateRNflair}{\tbd{hlMraBestRateRNflair}}
\providecommand{\hlMraBestRateSATburn}{\tbd{hlMraBestRateSATburn}}
\providecommand{\hlMraBestRateSATflair}{\tbd{hlMraBestRateSATflair}}
\providecommand{\hlMraBestRateTMburn}{\tbd{hlMraBestRateTMburn}}
\providecommand{\hlMraBestRateTMflair}{\tbd{hlMraBestRateTMflair}}
\providecommand{\hlMraCleanDOFAOneburn}{\tbd{hlMraCleanDOFAOneburn}}
\providecommand{\hlMraCleanDOFAOneflair}{\tbd{hlMraCleanDOFAOneflair}}
\providecommand{\hlMraCleanDOFAThirdburn}{\tbd{hlMraCleanDOFAThirdburn}}
\providecommand{\hlMraCleanDOFAThirdflair}{\tbd{hlMraCleanDOFAThirdflair}}
\providecommand{\hlMraCleanLVDOneburn}{\tbd{hlMraCleanLVDOneburn}}
\providecommand{\hlMraCleanLVDOneflair}{\tbd{hlMraCleanLVDOneflair}}
\providecommand{\hlMraCleanLVDThirdburn}{\tbd{hlMraCleanLVDThirdburn}}
\providecommand{\hlMraCleanLVDThirdflair}{\tbd{hlMraCleanLVDThirdflair}}
\providecommand{\hlMraCleanRNOneburn}{\tbd{hlMraCleanRNOneburn}}
\providecommand{\hlMraCleanRNOneflair}{\tbd{hlMraCleanRNOneflair}}
\providecommand{\hlMraCleanRNThirdburn}{\tbd{hlMraCleanRNThirdburn}}
\providecommand{\hlMraCleanRNThirdflair}{\tbd{hlMraCleanRNThirdflair}}
\providecommand{\hlMraCleanSATOneburn}{\tbd{hlMraCleanSATOneburn}}
\providecommand{\hlMraCleanSATOneflair}{\tbd{hlMraCleanSATOneflair}}
\providecommand{\hlMraCleanSATThirdburn}{\tbd{hlMraCleanSATThirdburn}}
\providecommand{\hlMraCleanSATThirdflair}{\tbd{hlMraCleanSATThirdflair}}
\providecommand{\hlMraCleanTMOneburn}{\tbd{hlMraCleanTMOneburn}}
\providecommand{\hlMraCleanTMOneflair}{\tbd{hlMraCleanTMOneflair}}
\providecommand{\hlMraCleanTMThirdburn}{\tbd{hlMraCleanTMThirdburn}}
\providecommand{\hlMraCleanTMThirdflair}{\tbd{hlMraCleanTMThirdflair}}
\providecommand{\hlMraDropDOFAOneburn}{\tbd{hlMraDropDOFAOneburn}}
\providecommand{\hlMraDropDOFAOneflair}{\tbd{hlMraDropDOFAOneflair}}
\providecommand{\hlMraDropDOFAThirdburn}{\tbd{hlMraDropDOFAThirdburn}}
\providecommand{\hlMraDropDOFAThirdflair}{\tbd{hlMraDropDOFAThirdflair}}
\providecommand{\hlMraDropLVDOneburn}{\tbd{hlMraDropLVDOneburn}}
\providecommand{\hlMraDropLVDOneflair}{\tbd{hlMraDropLVDOneflair}}
\providecommand{\hlMraDropLVDThirdburn}{\tbd{hlMraDropLVDThirdburn}}
\providecommand{\hlMraDropLVDThirdflair}{\tbd{hlMraDropLVDThirdflair}}
\providecommand{\hlMraDropRNOneburn}{\tbd{hlMraDropRNOneburn}}
\providecommand{\hlMraDropRNOneflair}{\tbd{hlMraDropRNOneflair}}
\providecommand{\hlMraDropRNThirdburn}{\tbd{hlMraDropRNThirdburn}}
\providecommand{\hlMraDropRNThirdflair}{\tbd{hlMraDropRNThirdflair}}
\providecommand{\hlMraDropSATOneburn}{\tbd{hlMraDropSATOneburn}}
\providecommand{\hlMraDropSATOneflair}{\tbd{hlMraDropSATOneflair}}
\providecommand{\hlMraDropSATThirdburn}{\tbd{hlMraDropSATThirdburn}}
\providecommand{\hlMraDropSATThirdflair}{\tbd{hlMraDropSATThirdflair}}
\providecommand{\hlMraDropTMOneburn}{\tbd{hlMraDropTMOneburn}}
\providecommand{\hlMraDropTMOneflair}{\tbd{hlMraDropTMOneflair}}
\providecommand{\hlMraDropTMThirdburn}{\tbd{hlMraDropTMThirdburn}}
\providecommand{\hlMraDropTMThirdflair}{\tbd{hlMraDropTMThirdflair}}
\providecommand{\hlMraFOneOneburnCIHi}{\tbd{hlMraFOneOneburnCIHi}}
\providecommand{\hlMraFOneOneburnCILo}{\tbd{hlMraFOneOneburnCILo}}
\providecommand{\hlMraFOneOneburnEst}{\tbd{hlMraFOneOneburnEst}}
\providecommand{\hlMraFOneOneburnMde}{\tbd{hlMraFOneOneburnMde}}
\providecommand{\hlMraFOneOneburnN}{\tbd{hlMraFOneOneburnN}}
\providecommand{\hlMraFOneOneburnPHolm}{\tbd{hlMraFOneOneburnPHolm}}
\providecommand{\hlMraFOneOneburnTostCIHi}{\tbd{hlMraFOneOneburnTostCIHi}}
\providecommand{\hlMraFOneOneburnTostCILo}{\tbd{hlMraFOneOneburnTostCILo}}
\providecommand{\hlMraFOneOneflairCIHi}{\tbd{hlMraFOneOneflairCIHi}}
\providecommand{\hlMraFOneOneflairCILo}{\tbd{hlMraFOneOneflairCILo}}
\providecommand{\hlMraFOneOneflairEst}{\tbd{hlMraFOneOneflairEst}}
\providecommand{\hlMraFOneOneflairMde}{\tbd{hlMraFOneOneflairMde}}
\providecommand{\hlMraFOneOneflairN}{\tbd{hlMraFOneOneflairN}}
\providecommand{\hlMraFOneOneflairPHolm}{\tbd{hlMraFOneOneflairPHolm}}
\providecommand{\hlMraFOneOneflairTostCIHi}{\tbd{hlMraFOneOneflairTostCIHi}}
\providecommand{\hlMraFOneOneflairTostCILo}{\tbd{hlMraFOneOneflairTostCILo}}
\providecommand{\hlMraFTwoThirdburnCIHi}{\tbd{hlMraFTwoThirdburnCIHi}}
\providecommand{\hlMraFTwoThirdburnCILo}{\tbd{hlMraFTwoThirdburnCILo}}
\providecommand{\hlMraFTwoThirdburnEst}{\tbd{hlMraFTwoThirdburnEst}}
\providecommand{\hlMraFTwoThirdburnMde}{\tbd{hlMraFTwoThirdburnMde}}
\providecommand{\hlMraFTwoThirdburnN}{\tbd{hlMraFTwoThirdburnN}}
\providecommand{\hlMraFTwoThirdburnPHolm}{\tbd{hlMraFTwoThirdburnPHolm}}
\providecommand{\hlMraFTwoThirdburnTostCIHi}{\tbd{hlMraFTwoThirdburnTostCIHi}}
\providecommand{\hlMraFTwoThirdburnTostCILo}{\tbd{hlMraFTwoThirdburnTostCILo}}
\providecommand{\hlMraFTwoThirdflairCIHi}{\tbd{hlMraFTwoThirdflairCIHi}}
\providecommand{\hlMraFTwoThirdflairCILo}{\tbd{hlMraFTwoThirdflairCILo}}
\providecommand{\hlMraFTwoThirdflairEst}{\tbd{hlMraFTwoThirdflairEst}}
\providecommand{\hlMraFTwoThirdflairMde}{\tbd{hlMraFTwoThirdflairMde}}
\providecommand{\hlMraFTwoThirdflairN}{\tbd{hlMraFTwoThirdflairN}}
\providecommand{\hlMraFTwoThirdflairPHolm}{\tbd{hlMraFTwoThirdflairPHolm}}
\providecommand{\hlMraFTwoThirdflairTostCIHi}{\tbd{hlMraFTwoThirdflairTostCIHi}}
\providecommand{\hlMraFTwoThirdflairTostCILo}{\tbd{hlMraFTwoThirdflairTostCILo}}
\providecommand{\hlMraRateDiffDOFAburnCIHi}{\tbd{hlMraRateDiffDOFAburnCIHi}}
\providecommand{\hlMraRateDiffDOFAburnCILo}{\tbd{hlMraRateDiffDOFAburnCILo}}
\providecommand{\hlMraRateDiffDOFAburnEst}{\tbd{hlMraRateDiffDOFAburnEst}}
\providecommand{\hlMraRateDiffDOFAflairCIHi}{\tbd{hlMraRateDiffDOFAflairCIHi}}
\providecommand{\hlMraRateDiffDOFAflairCILo}{\tbd{hlMraRateDiffDOFAflairCILo}}
\providecommand{\hlMraRateDiffDOFAflairEst}{\tbd{hlMraRateDiffDOFAflairEst}}
\providecommand{\hlMraRateDiffLVDburnCIHi}{\tbd{hlMraRateDiffLVDburnCIHi}}
\providecommand{\hlMraRateDiffLVDburnCILo}{\tbd{hlMraRateDiffLVDburnCILo}}
\providecommand{\hlMraRateDiffLVDburnEst}{\tbd{hlMraRateDiffLVDburnEst}}
\providecommand{\hlMraRateDiffLVDflairCIHi}{\tbd{hlMraRateDiffLVDflairCIHi}}
\providecommand{\hlMraRateDiffLVDflairCILo}{\tbd{hlMraRateDiffLVDflairCILo}}
\providecommand{\hlMraRateDiffLVDflairEst}{\tbd{hlMraRateDiffLVDflairEst}}
\providecommand{\hlMraRateDiffRNburnCIHi}{\tbd{hlMraRateDiffRNburnCIHi}}
\providecommand{\hlMraRateDiffRNburnCILo}{\tbd{hlMraRateDiffRNburnCILo}}
\providecommand{\hlMraRateDiffRNburnEst}{\tbd{hlMraRateDiffRNburnEst}}
\providecommand{\hlMraRateDiffRNflairCIHi}{\tbd{hlMraRateDiffRNflairCIHi}}
\providecommand{\hlMraRateDiffRNflairCILo}{\tbd{hlMraRateDiffRNflairCILo}}
\providecommand{\hlMraRateDiffRNflairEst}{\tbd{hlMraRateDiffRNflairEst}}
\providecommand{\hlMraRateDiffSATburnCIHi}{\tbd{hlMraRateDiffSATburnCIHi}}
\providecommand{\hlMraRateDiffSATburnCILo}{\tbd{hlMraRateDiffSATburnCILo}}
\providecommand{\hlMraRateDiffSATburnEst}{\tbd{hlMraRateDiffSATburnEst}}
\providecommand{\hlMraRateDiffSATflairCIHi}{\tbd{hlMraRateDiffSATflairCIHi}}
\providecommand{\hlMraRateDiffSATflairCILo}{\tbd{hlMraRateDiffSATflairCILo}}
\providecommand{\hlMraRateDiffSATflairEst}{\tbd{hlMraRateDiffSATflairEst}}
\providecommand{\hlMraRateDiffTMburnCIHi}{\tbd{hlMraRateDiffTMburnCIHi}}
\providecommand{\hlMraRateDiffTMburnCILo}{\tbd{hlMraRateDiffTMburnCILo}}
\providecommand{\hlMraRateDiffTMburnEst}{\tbd{hlMraRateDiffTMburnEst}}
\providecommand{\hlMraRateDiffTMflairCIHi}{\tbd{hlMraRateDiffTMflairCIHi}}
\providecommand{\hlMraRateDiffTMflairCILo}{\tbd{hlMraRateDiffTMflairCILo}}
\providecommand{\hlMraRateDiffTMflairEst}{\tbd{hlMraRateDiffTMflairEst}}
\providecommand{\hlMraRetDOFAOneburn}{\tbd{hlMraRetDOFAOneburn}}
\providecommand{\hlMraRetDOFAOneflair}{\tbd{hlMraRetDOFAOneflair}}
\providecommand{\hlMraRetDOFAThirdburn}{\tbd{hlMraRetDOFAThirdburn}}
\providecommand{\hlMraRetDOFAThirdflair}{\tbd{hlMraRetDOFAThirdflair}}
\providecommand{\hlMraRetLVDOneburn}{\tbd{hlMraRetLVDOneburn}}
\providecommand{\hlMraRetLVDOneflair}{\tbd{hlMraRetLVDOneflair}}
\providecommand{\hlMraRetLVDThirdburn}{\tbd{hlMraRetLVDThirdburn}}
\providecommand{\hlMraRetLVDThirdflair}{\tbd{hlMraRetLVDThirdflair}}
\providecommand{\hlMraRetRNOneburn}{\tbd{hlMraRetRNOneburn}}
\providecommand{\hlMraRetRNOneflair}{\tbd{hlMraRetRNOneflair}}
\providecommand{\hlMraRetRNThirdburn}{\tbd{hlMraRetRNThirdburn}}
\providecommand{\hlMraRetRNThirdflair}{\tbd{hlMraRetRNThirdflair}}
\providecommand{\hlMraRetSATOneburn}{\tbd{hlMraRetSATOneburn}}
\providecommand{\hlMraRetSATOneflair}{\tbd{hlMraRetSATOneflair}}
\providecommand{\hlMraRetSATThirdburn}{\tbd{hlMraRetSATThirdburn}}
\providecommand{\hlMraRetSATThirdflair}{\tbd{hlMraRetSATThirdflair}}
\providecommand{\hlMraRetTMOneburn}{\tbd{hlMraRetTMOneburn}}
\providecommand{\hlMraRetTMOneflair}{\tbd{hlMraRetTMOneflair}}
\providecommand{\hlMraRetTMThirdburn}{\tbd{hlMraRetTMThirdburn}}
\providecommand{\hlMraRetTMThirdflair}{\tbd{hlMraRetTMThirdflair}}
\providecommand{\hlMraVerdictFOneburn}{\tbd{hlMraVerdictFOneburn}}
\providecommand{\hlMraVerdictFOneflair}{\tbd{hlMraVerdictFOneflair}}
\providecommand{\hlMraVerdictburn}{\tbd{hlMraVerdictburn}}
\providecommand{\hlMraVerdictflair}{\tbd{hlMraVerdictflair}}
\providecommand{\hlMsFOneEquiv}{\tbd{hlMsFOneEquiv}}
\providecommand{\hlMsFOneEquivRet}{\tbd{hlMsFOneEquivRet}}
\providecommand{\hlMsFOneEquivScaled}{\tbd{hlMsFOneEquivScaled}}
\providecommand{\hlMsFOneRead}{\tbd{hlMsFOneRead}}
\providecommand{\hlMsFTwoEquiv}{\tbd{hlMsFTwoEquiv}}
\providecommand{\hlMsFTwoEquivRet}{\tbd{hlMsFTwoEquivRet}}
\providecommand{\hlMsFTwoEquivScaled}{\tbd{hlMsFTwoEquivScaled}}
\providecommand{\hlMsFTwoRead}{\tbd{hlMsFTwoRead}}
\providecommand{\hlMsFractionPct}{\tbd{hlMsFractionPct}}
\providecommand{\hlMsMarginFOneChes}{\tbd{hlMsMarginFOneChes}}
\providecommand{\hlMsMarginFOneCsTwelve}{\tbd{hlMsMarginFOneCsTwelve}}
\providecommand{\hlMsMarginFOneDfc}{\tbd{hlMsMarginFOneDfc}}
\providecommand{\hlMsMarginFOneEnva}{\tbd{hlMsMarginFOneEnva}}
\providecommand{\hlMsMarginFOneKuro}{\tbd{hlMsMarginFOneKuro}}
\providecommand{\hlMsMarginFOneOem}{\tbd{hlMsMarginFOneOem}}
\providecommand{\hlMsMarginFOneSnTwo}{\tbd{hlMsMarginFOneSnTwo}}
\providecommand{\hlMsMarginFOneburn}{\tbd{hlMsMarginFOneburn}}
\providecommand{\hlMsMarginFOneflair}{\tbd{hlMsMarginFOneflair}}
\providecommand{\hlMsMarginFTwoChes}{\tbd{hlMsMarginFTwoChes}}
\providecommand{\hlMsMarginFTwoCsTwelve}{\tbd{hlMsMarginFTwoCsTwelve}}
\providecommand{\hlMsMarginFTwoDfc}{\tbd{hlMsMarginFTwoDfc}}
\providecommand{\hlMsMarginFTwoEnva}{\tbd{hlMsMarginFTwoEnva}}
\providecommand{\hlMsMarginFTwoKuro}{\tbd{hlMsMarginFTwoKuro}}
\providecommand{\hlMsMarginFTwoOem}{\tbd{hlMsMarginFTwoOem}}
\providecommand{\hlMsMarginFTwoSnTwo}{\tbd{hlMsMarginFTwoSnTwo}}
\providecommand{\hlMsMarginFTwoburn}{\tbd{hlMsMarginFTwoburn}}
\providecommand{\hlMsMarginFTwoflair}{\tbd{hlMsMarginFTwoflair}}
\providecommand{\hlMsMarginHFiveChes}{\tbd{hlMsMarginHFiveChes}}
\providecommand{\hlMsMarginHFiveCsTwelve}{\tbd{hlMsMarginHFiveCsTwelve}}
\providecommand{\hlMsMarginHFiveDfc}{\tbd{hlMsMarginHFiveDfc}}
\providecommand{\hlMsMarginHFiveEnva}{\tbd{hlMsMarginHFiveEnva}}
\providecommand{\hlMsMarginHFiveKuro}{\tbd{hlMsMarginHFiveKuro}}
\providecommand{\hlMsMarginHFiveMtwoFFburn}{\tbd{hlMsMarginHFiveMtwoFFburn}}
\providecommand{\hlMsMarginHFiveMtwoFFflair}{\tbd{hlMsMarginHFiveMtwoFFflair}}
\providecommand{\hlMsMarginHFiveMtwoFburn}{\tbd{hlMsMarginHFiveMtwoFburn}}
\providecommand{\hlMsMarginHFiveMtwoFflair}{\tbd{hlMsMarginHFiveMtwoFflair}}
\providecommand{\hlMsMarginHFiveOem}{\tbd{hlMsMarginHFiveOem}}
\providecommand{\hlMsMarginHFiveSamPreburn}{\tbd{hlMsMarginHFiveSamPreburn}}
\providecommand{\hlMsMarginHFiveSamPreflair}{\tbd{hlMsMarginHFiveSamPreflair}}
\providecommand{\hlMsMarginHFiveSamburn}{\tbd{hlMsMarginHFiveSamburn}}
\providecommand{\hlMsMarginHFiveSamflair}{\tbd{hlMsMarginHFiveSamflair}}
\providecommand{\hlMsMarginHFiveSegfburn}{\tbd{hlMsMarginHFiveSegfburn}}
\providecommand{\hlMsMarginHFiveSegfflair}{\tbd{hlMsMarginHFiveSegfflair}}
\providecommand{\hlMsMarginHFiveSnTwo}{\tbd{hlMsMarginHFiveSnTwo}}
\providecommand{\hlMsMarginHSixFTwoOneburn}{\tbd{hlMsMarginHSixFTwoOneburn}}
\providecommand{\hlMsMarginHSixFTwoOneflair}{\tbd{hlMsMarginHSixFTwoOneflair}}
\providecommand{\hlMsMarginHSixFTwoThirdburn}{\tbd{hlMsMarginHSixFTwoThirdburn}}
\providecommand{\hlMsMarginHSixFTwoThirdflair}{\tbd{hlMsMarginHSixFTwoThirdflair}}
\providecommand{\hlMsMarginHSixRqOneOneburn}{\tbd{hlMsMarginHSixRqOneOneburn}}
\providecommand{\hlMsMarginHSixRqOneOneflair}{\tbd{hlMsMarginHSixRqOneOneflair}}
\providecommand{\hlMsMarginHSixRqOneThirdburn}{\tbd{hlMsMarginHSixRqOneThirdburn}}
\providecommand{\hlMsMarginHSixRqOneThirdflair}{\tbd{hlMsMarginHSixRqOneThirdflair}}
\providecommand{\hlMsMarginMitBootburn}{\tbd{hlMsMarginMitBootburn}}
\providecommand{\hlMsMarginMitBootflair}{\tbd{hlMsMarginMitBootflair}}
\providecommand{\hlMsMarginMitGceburn}{\tbd{hlMsMarginMitGceburn}}
\providecommand{\hlMsMarginMitGceflair}{\tbd{hlMsMarginMitGceflair}}
\providecommand{\hlMsMarginNSixChes}{\tbd{hlMsMarginNSixChes}}
\providecommand{\hlMsMarginNSixCsTwelve}{\tbd{hlMsMarginNSixCsTwelve}}
\providecommand{\hlMsMarginNSixDfc}{\tbd{hlMsMarginNSixDfc}}
\providecommand{\hlMsMarginNSixEnva}{\tbd{hlMsMarginNSixEnva}}
\providecommand{\hlMsMarginNSixKuro}{\tbd{hlMsMarginNSixKuro}}
\providecommand{\hlMsMarginNSixOem}{\tbd{hlMsMarginNSixOem}}
\providecommand{\hlMsMarginNSixSnTwo}{\tbd{hlMsMarginNSixSnTwo}}
\providecommand{\hlMsMarginNSixburn}{\tbd{hlMsMarginNSixburn}}
\providecommand{\hlMsMarginNSixflair}{\tbd{hlMsMarginNSixflair}}
\providecommand{\hlMsNSixEquiv}{\tbd{hlMsNSixEquiv}}
\providecommand{\hlMsNSixEquivRest}{\tbd{hlMsNSixEquivRest}}
\providecommand{\hlMsNSixEquivRet}{\tbd{hlMsNSixEquivRet}}
\providecommand{\hlMsNSixEquivRetRest}{\tbd{hlMsNSixEquivRetRest}}
\providecommand{\hlMsNSixEquivRetSubm}{\tbd{hlMsNSixEquivRetSubm}}
\providecommand{\hlMsNSixEquivScaled}{\tbd{hlMsNSixEquivScaled}}
\providecommand{\hlMsNSixEquivScaledRest}{\tbd{hlMsNSixEquivScaledRest}}
\providecommand{\hlMsNSixEquivScaledSubm}{\tbd{hlMsNSixEquivScaledSubm}}
\providecommand{\hlMsNSixEquivSubm}{\tbd{hlMsNSixEquivSubm}}
\providecommand{\hlMsNSixRead}{\tbd{hlMsNSixRead}}
\providecommand{\hlMsNSixReadRest}{\tbd{hlMsNSixReadRest}}
\providecommand{\hlMsNSixReadSubm}{\tbd{hlMsNSixReadSubm}}
\providecommand{\hlMsRetFOneChesCIHi}{\tbd{hlMsRetFOneChesCIHi}}
\providecommand{\hlMsRetFOneChesCILo}{\tbd{hlMsRetFOneChesCILo}}
\providecommand{\hlMsRetFOneChesEst}{\tbd{hlMsRetFOneChesEst}}
\providecommand{\hlMsRetFOneCsTwelveCIHi}{\tbd{hlMsRetFOneCsTwelveCIHi}}
\providecommand{\hlMsRetFOneCsTwelveCILo}{\tbd{hlMsRetFOneCsTwelveCILo}}
\providecommand{\hlMsRetFOneCsTwelveEst}{\tbd{hlMsRetFOneCsTwelveEst}}
\providecommand{\hlMsRetFOneDfcCIHi}{\tbd{hlMsRetFOneDfcCIHi}}
\providecommand{\hlMsRetFOneDfcCILo}{\tbd{hlMsRetFOneDfcCILo}}
\providecommand{\hlMsRetFOneDfcEst}{\tbd{hlMsRetFOneDfcEst}}
\providecommand{\hlMsRetFOneEnvaCIHi}{\tbd{hlMsRetFOneEnvaCIHi}}
\providecommand{\hlMsRetFOneEnvaCILo}{\tbd{hlMsRetFOneEnvaCILo}}
\providecommand{\hlMsRetFOneEnvaEst}{\tbd{hlMsRetFOneEnvaEst}}
\providecommand{\hlMsRetFOneKuroCIHi}{\tbd{hlMsRetFOneKuroCIHi}}
\providecommand{\hlMsRetFOneKuroCILo}{\tbd{hlMsRetFOneKuroCILo}}
\providecommand{\hlMsRetFOneKuroEst}{\tbd{hlMsRetFOneKuroEst}}
\providecommand{\hlMsRetFOneOemCIHi}{\tbd{hlMsRetFOneOemCIHi}}
\providecommand{\hlMsRetFOneOemCILo}{\tbd{hlMsRetFOneOemCILo}}
\providecommand{\hlMsRetFOneOemEst}{\tbd{hlMsRetFOneOemEst}}
\providecommand{\hlMsRetFOneSnTwoCIHi}{\tbd{hlMsRetFOneSnTwoCIHi}}
\providecommand{\hlMsRetFOneSnTwoCILo}{\tbd{hlMsRetFOneSnTwoCILo}}
\providecommand{\hlMsRetFOneSnTwoEst}{\tbd{hlMsRetFOneSnTwoEst}}
\providecommand{\hlMsRetFOneburnCIHi}{\tbd{hlMsRetFOneburnCIHi}}
\providecommand{\hlMsRetFOneburnCILo}{\tbd{hlMsRetFOneburnCILo}}
\providecommand{\hlMsRetFOneburnEst}{\tbd{hlMsRetFOneburnEst}}
\providecommand{\hlMsRetFOneflairCIHi}{\tbd{hlMsRetFOneflairCIHi}}
\providecommand{\hlMsRetFOneflairCILo}{\tbd{hlMsRetFOneflairCILo}}
\providecommand{\hlMsRetFOneflairEst}{\tbd{hlMsRetFOneflairEst}}
\providecommand{\hlMsRetFTwoChesCIHi}{\tbd{hlMsRetFTwoChesCIHi}}
\providecommand{\hlMsRetFTwoChesCILo}{\tbd{hlMsRetFTwoChesCILo}}
\providecommand{\hlMsRetFTwoChesEst}{\tbd{hlMsRetFTwoChesEst}}
\providecommand{\hlMsRetFTwoCsTwelveCIHi}{\tbd{hlMsRetFTwoCsTwelveCIHi}}
\providecommand{\hlMsRetFTwoCsTwelveCILo}{\tbd{hlMsRetFTwoCsTwelveCILo}}
\providecommand{\hlMsRetFTwoCsTwelveEst}{\tbd{hlMsRetFTwoCsTwelveEst}}
\providecommand{\hlMsRetFTwoDfcCIHi}{\tbd{hlMsRetFTwoDfcCIHi}}
\providecommand{\hlMsRetFTwoDfcCILo}{\tbd{hlMsRetFTwoDfcCILo}}
\providecommand{\hlMsRetFTwoDfcEst}{\tbd{hlMsRetFTwoDfcEst}}
\providecommand{\hlMsRetFTwoEnvaCIHi}{\tbd{hlMsRetFTwoEnvaCIHi}}
\providecommand{\hlMsRetFTwoEnvaCILo}{\tbd{hlMsRetFTwoEnvaCILo}}
\providecommand{\hlMsRetFTwoEnvaEst}{\tbd{hlMsRetFTwoEnvaEst}}
\providecommand{\hlMsRetFTwoKuroCIHi}{\tbd{hlMsRetFTwoKuroCIHi}}
\providecommand{\hlMsRetFTwoKuroCILo}{\tbd{hlMsRetFTwoKuroCILo}}
\providecommand{\hlMsRetFTwoKuroEst}{\tbd{hlMsRetFTwoKuroEst}}
\providecommand{\hlMsRetFTwoOemCIHi}{\tbd{hlMsRetFTwoOemCIHi}}
\providecommand{\hlMsRetFTwoOemCILo}{\tbd{hlMsRetFTwoOemCILo}}
\providecommand{\hlMsRetFTwoOemEst}{\tbd{hlMsRetFTwoOemEst}}
\providecommand{\hlMsRetFTwoSnTwoCIHi}{\tbd{hlMsRetFTwoSnTwoCIHi}}
\providecommand{\hlMsRetFTwoSnTwoCILo}{\tbd{hlMsRetFTwoSnTwoCILo}}
\providecommand{\hlMsRetFTwoSnTwoEst}{\tbd{hlMsRetFTwoSnTwoEst}}
\providecommand{\hlMsRetFTwoburnCIHi}{\tbd{hlMsRetFTwoburnCIHi}}
\providecommand{\hlMsRetFTwoburnCILo}{\tbd{hlMsRetFTwoburnCILo}}
\providecommand{\hlMsRetFTwoburnEst}{\tbd{hlMsRetFTwoburnEst}}
\providecommand{\hlMsRetFTwoflairCIHi}{\tbd{hlMsRetFTwoflairCIHi}}
\providecommand{\hlMsRetFTwoflairCILo}{\tbd{hlMsRetFTwoflairCILo}}
\providecommand{\hlMsRetFTwoflairEst}{\tbd{hlMsRetFTwoflairEst}}
\providecommand{\hlMsRetMarginFOneChes}{\tbd{hlMsRetMarginFOneChes}}
\providecommand{\hlMsRetMarginFOneCsTwelve}{\tbd{hlMsRetMarginFOneCsTwelve}}
\providecommand{\hlMsRetMarginFOneDfc}{\tbd{hlMsRetMarginFOneDfc}}
\providecommand{\hlMsRetMarginFOneEnva}{\tbd{hlMsRetMarginFOneEnva}}
\providecommand{\hlMsRetMarginFOneKuro}{\tbd{hlMsRetMarginFOneKuro}}
\providecommand{\hlMsRetMarginFOneOem}{\tbd{hlMsRetMarginFOneOem}}
\providecommand{\hlMsRetMarginFOneSnTwo}{\tbd{hlMsRetMarginFOneSnTwo}}
\providecommand{\hlMsRetMarginFOneburn}{\tbd{hlMsRetMarginFOneburn}}
\providecommand{\hlMsRetMarginFOneflair}{\tbd{hlMsRetMarginFOneflair}}
\providecommand{\hlMsRetMarginFTwoChes}{\tbd{hlMsRetMarginFTwoChes}}
\providecommand{\hlMsRetMarginFTwoCsTwelve}{\tbd{hlMsRetMarginFTwoCsTwelve}}
\providecommand{\hlMsRetMarginFTwoDfc}{\tbd{hlMsRetMarginFTwoDfc}}
\providecommand{\hlMsRetMarginFTwoEnva}{\tbd{hlMsRetMarginFTwoEnva}}
\providecommand{\hlMsRetMarginFTwoKuro}{\tbd{hlMsRetMarginFTwoKuro}}
\providecommand{\hlMsRetMarginFTwoOem}{\tbd{hlMsRetMarginFTwoOem}}
\providecommand{\hlMsRetMarginFTwoSnTwo}{\tbd{hlMsRetMarginFTwoSnTwo}}
\providecommand{\hlMsRetMarginFTwoburn}{\tbd{hlMsRetMarginFTwoburn}}
\providecommand{\hlMsRetMarginFTwoflair}{\tbd{hlMsRetMarginFTwoflair}}
\providecommand{\hlMsRetMarginNSixChes}{\tbd{hlMsRetMarginNSixChes}}
\providecommand{\hlMsRetMarginNSixCsTwelve}{\tbd{hlMsRetMarginNSixCsTwelve}}
\providecommand{\hlMsRetMarginNSixDfc}{\tbd{hlMsRetMarginNSixDfc}}
\providecommand{\hlMsRetMarginNSixEnva}{\tbd{hlMsRetMarginNSixEnva}}
\providecommand{\hlMsRetMarginNSixKuro}{\tbd{hlMsRetMarginNSixKuro}}
\providecommand{\hlMsRetMarginNSixOem}{\tbd{hlMsRetMarginNSixOem}}
\providecommand{\hlMsRetMarginNSixSnTwo}{\tbd{hlMsRetMarginNSixSnTwo}}
\providecommand{\hlMsRetMarginNSixburn}{\tbd{hlMsRetMarginNSixburn}}
\providecommand{\hlMsRetMarginNSixflair}{\tbd{hlMsRetMarginNSixflair}}
\providecommand{\hlMsRetNSixChesCIHi}{\tbd{hlMsRetNSixChesCIHi}}
\providecommand{\hlMsRetNSixChesCILo}{\tbd{hlMsRetNSixChesCILo}}
\providecommand{\hlMsRetNSixChesEst}{\tbd{hlMsRetNSixChesEst}}
\providecommand{\hlMsRetNSixCsTwelveCIHi}{\tbd{hlMsRetNSixCsTwelveCIHi}}
\providecommand{\hlMsRetNSixCsTwelveCILo}{\tbd{hlMsRetNSixCsTwelveCILo}}
\providecommand{\hlMsRetNSixCsTwelveEst}{\tbd{hlMsRetNSixCsTwelveEst}}
\providecommand{\hlMsRetNSixDfcCIHi}{\tbd{hlMsRetNSixDfcCIHi}}
\providecommand{\hlMsRetNSixDfcCILo}{\tbd{hlMsRetNSixDfcCILo}}
\providecommand{\hlMsRetNSixDfcEst}{\tbd{hlMsRetNSixDfcEst}}
\providecommand{\hlMsRetNSixEnvaCIHi}{\tbd{hlMsRetNSixEnvaCIHi}}
\providecommand{\hlMsRetNSixEnvaCILo}{\tbd{hlMsRetNSixEnvaCILo}}
\providecommand{\hlMsRetNSixEnvaEst}{\tbd{hlMsRetNSixEnvaEst}}
\providecommand{\hlMsRetNSixKuroCIHi}{\tbd{hlMsRetNSixKuroCIHi}}
\providecommand{\hlMsRetNSixKuroCILo}{\tbd{hlMsRetNSixKuroCILo}}
\providecommand{\hlMsRetNSixKuroEst}{\tbd{hlMsRetNSixKuroEst}}
\providecommand{\hlMsRetNSixOemCIHi}{\tbd{hlMsRetNSixOemCIHi}}
\providecommand{\hlMsRetNSixOemCILo}{\tbd{hlMsRetNSixOemCILo}}
\providecommand{\hlMsRetNSixOemEst}{\tbd{hlMsRetNSixOemEst}}
\providecommand{\hlMsRetNSixSnTwoCIHi}{\tbd{hlMsRetNSixSnTwoCIHi}}
\providecommand{\hlMsRetNSixSnTwoCILo}{\tbd{hlMsRetNSixSnTwoCILo}}
\providecommand{\hlMsRetNSixSnTwoEst}{\tbd{hlMsRetNSixSnTwoEst}}
\providecommand{\hlMsRetNSixburnCIHi}{\tbd{hlMsRetNSixburnCIHi}}
\providecommand{\hlMsRetNSixburnCILo}{\tbd{hlMsRetNSixburnCILo}}
\providecommand{\hlMsRetNSixburnEst}{\tbd{hlMsRetNSixburnEst}}
\providecommand{\hlMsRetNSixflairCIHi}{\tbd{hlMsRetNSixflairCIHi}}
\providecommand{\hlMsRetNSixflairCILo}{\tbd{hlMsRetNSixflairCILo}}
\providecommand{\hlMsRetNSixflairEst}{\tbd{hlMsRetNSixflairEst}}
\providecommand{\hlMsRetVerdictFOneChes}{\tbd{hlMsRetVerdictFOneChes}}
\providecommand{\hlMsRetVerdictFOneCsTwelve}{\tbd{hlMsRetVerdictFOneCsTwelve}}
\providecommand{\hlMsRetVerdictFOneDfc}{\tbd{hlMsRetVerdictFOneDfc}}
\providecommand{\hlMsRetVerdictFOneEnva}{\tbd{hlMsRetVerdictFOneEnva}}
\providecommand{\hlMsRetVerdictFOneKuro}{\tbd{hlMsRetVerdictFOneKuro}}
\providecommand{\hlMsRetVerdictFOneOem}{\tbd{hlMsRetVerdictFOneOem}}
\providecommand{\hlMsRetVerdictFOneSnTwo}{\tbd{hlMsRetVerdictFOneSnTwo}}
\providecommand{\hlMsRetVerdictFOneburn}{\tbd{hlMsRetVerdictFOneburn}}
\providecommand{\hlMsRetVerdictFOneflair}{\tbd{hlMsRetVerdictFOneflair}}
\providecommand{\hlMsRetVerdictFTwoChes}{\tbd{hlMsRetVerdictFTwoChes}}
\providecommand{\hlMsRetVerdictFTwoCsTwelve}{\tbd{hlMsRetVerdictFTwoCsTwelve}}
\providecommand{\hlMsRetVerdictFTwoDfc}{\tbd{hlMsRetVerdictFTwoDfc}}
\providecommand{\hlMsRetVerdictFTwoEnva}{\tbd{hlMsRetVerdictFTwoEnva}}
\providecommand{\hlMsRetVerdictFTwoKuro}{\tbd{hlMsRetVerdictFTwoKuro}}
\providecommand{\hlMsRetVerdictFTwoOem}{\tbd{hlMsRetVerdictFTwoOem}}
\providecommand{\hlMsRetVerdictFTwoSnTwo}{\tbd{hlMsRetVerdictFTwoSnTwo}}
\providecommand{\hlMsRetVerdictFTwoburn}{\tbd{hlMsRetVerdictFTwoburn}}
\providecommand{\hlMsRetVerdictFTwoflair}{\tbd{hlMsRetVerdictFTwoflair}}
\providecommand{\hlMsRetVerdictNSixChes}{\tbd{hlMsRetVerdictNSixChes}}
\providecommand{\hlMsRetVerdictNSixCsTwelve}{\tbd{hlMsRetVerdictNSixCsTwelve}}
\providecommand{\hlMsRetVerdictNSixDfc}{\tbd{hlMsRetVerdictNSixDfc}}
\providecommand{\hlMsRetVerdictNSixEnva}{\tbd{hlMsRetVerdictNSixEnva}}
\providecommand{\hlMsRetVerdictNSixKuro}{\tbd{hlMsRetVerdictNSixKuro}}
\providecommand{\hlMsRetVerdictNSixOem}{\tbd{hlMsRetVerdictNSixOem}}
\providecommand{\hlMsRetVerdictNSixSnTwo}{\tbd{hlMsRetVerdictNSixSnTwo}}
\providecommand{\hlMsRetVerdictNSixburn}{\tbd{hlMsRetVerdictNSixburn}}
\providecommand{\hlMsRetVerdictNSixflair}{\tbd{hlMsRetVerdictNSixflair}}
\providecommand{\hlMsShareChes}{\tbd{hlMsShareChes}}
\providecommand{\hlMsShareCsTwelve}{\tbd{hlMsShareCsTwelve}}
\providecommand{\hlMsShareDfc}{\tbd{hlMsShareDfc}}
\providecommand{\hlMsShareEnva}{\tbd{hlMsShareEnva}}
\providecommand{\hlMsShareKuro}{\tbd{hlMsShareKuro}}
\providecommand{\hlMsShareOem}{\tbd{hlMsShareOem}}
\providecommand{\hlMsShareOverHalf}{\tbd{hlMsShareOverHalf}}
\providecommand{\hlMsShareSnTwo}{\tbd{hlMsShareSnTwo}}
\providecommand{\hlMsShareburn}{\tbd{hlMsShareburn}}
\providecommand{\hlMsShareflair}{\tbd{hlMsShareflair}}
\providecommand{\hlMsVerdictFOneChes}{\tbd{hlMsVerdictFOneChes}}
\providecommand{\hlMsVerdictFOneCsTwelve}{\tbd{hlMsVerdictFOneCsTwelve}}
\providecommand{\hlMsVerdictFOneDfc}{\tbd{hlMsVerdictFOneDfc}}
\providecommand{\hlMsVerdictFOneEnva}{\tbd{hlMsVerdictFOneEnva}}
\providecommand{\hlMsVerdictFOneKuro}{\tbd{hlMsVerdictFOneKuro}}
\providecommand{\hlMsVerdictFOneOem}{\tbd{hlMsVerdictFOneOem}}
\providecommand{\hlMsVerdictFOneSnTwo}{\tbd{hlMsVerdictFOneSnTwo}}
\providecommand{\hlMsVerdictFOneburn}{\tbd{hlMsVerdictFOneburn}}
\providecommand{\hlMsVerdictFOneflair}{\tbd{hlMsVerdictFOneflair}}
\providecommand{\hlMsVerdictFTwoChes}{\tbd{hlMsVerdictFTwoChes}}
\providecommand{\hlMsVerdictFTwoCsTwelve}{\tbd{hlMsVerdictFTwoCsTwelve}}
\providecommand{\hlMsVerdictFTwoDfc}{\tbd{hlMsVerdictFTwoDfc}}
\providecommand{\hlMsVerdictFTwoEnva}{\tbd{hlMsVerdictFTwoEnva}}
\providecommand{\hlMsVerdictFTwoKuro}{\tbd{hlMsVerdictFTwoKuro}}
\providecommand{\hlMsVerdictFTwoOem}{\tbd{hlMsVerdictFTwoOem}}
\providecommand{\hlMsVerdictFTwoSnTwo}{\tbd{hlMsVerdictFTwoSnTwo}}
\providecommand{\hlMsVerdictFTwoburn}{\tbd{hlMsVerdictFTwoburn}}
\providecommand{\hlMsVerdictFTwoflair}{\tbd{hlMsVerdictFTwoflair}}
\providecommand{\hlMsVerdictHFiveChes}{\tbd{hlMsVerdictHFiveChes}}
\providecommand{\hlMsVerdictHFiveCsTwelve}{\tbd{hlMsVerdictHFiveCsTwelve}}
\providecommand{\hlMsVerdictHFiveDfc}{\tbd{hlMsVerdictHFiveDfc}}
\providecommand{\hlMsVerdictHFiveEnva}{\tbd{hlMsVerdictHFiveEnva}}
\providecommand{\hlMsVerdictHFiveKuro}{\tbd{hlMsVerdictHFiveKuro}}
\providecommand{\hlMsVerdictHFiveMtwoFFburn}{\tbd{hlMsVerdictHFiveMtwoFFburn}}
\providecommand{\hlMsVerdictHFiveMtwoFFflair}{\tbd{hlMsVerdictHFiveMtwoFFflair}}
\providecommand{\hlMsVerdictHFiveMtwoFburn}{\tbd{hlMsVerdictHFiveMtwoFburn}}
\providecommand{\hlMsVerdictHFiveMtwoFflair}{\tbd{hlMsVerdictHFiveMtwoFflair}}
\providecommand{\hlMsVerdictHFiveOem}{\tbd{hlMsVerdictHFiveOem}}
\providecommand{\hlMsVerdictHFiveSamPreburn}{\tbd{hlMsVerdictHFiveSamPreburn}}
\providecommand{\hlMsVerdictHFiveSamPreflair}{\tbd{hlMsVerdictHFiveSamPreflair}}
\providecommand{\hlMsVerdictHFiveSamburn}{\tbd{hlMsVerdictHFiveSamburn}}
\providecommand{\hlMsVerdictHFiveSamflair}{\tbd{hlMsVerdictHFiveSamflair}}
\providecommand{\hlMsVerdictHFiveSegfburn}{\tbd{hlMsVerdictHFiveSegfburn}}
\providecommand{\hlMsVerdictHFiveSegfflair}{\tbd{hlMsVerdictHFiveSegfflair}}
\providecommand{\hlMsVerdictHFiveSnTwo}{\tbd{hlMsVerdictHFiveSnTwo}}
\providecommand{\hlMsVerdictHSixFTwoOneburn}{\tbd{hlMsVerdictHSixFTwoOneburn}}
\providecommand{\hlMsVerdictHSixFTwoOneflair}{\tbd{hlMsVerdictHSixFTwoOneflair}}
\providecommand{\hlMsVerdictHSixFTwoThirdburn}{\tbd{hlMsVerdictHSixFTwoThirdburn}}
\providecommand{\hlMsVerdictHSixFTwoThirdflair}{\tbd{hlMsVerdictHSixFTwoThirdflair}}
\providecommand{\hlMsVerdictHSixRqOneOneburn}{\tbd{hlMsVerdictHSixRqOneOneburn}}
\providecommand{\hlMsVerdictHSixRqOneOneflair}{\tbd{hlMsVerdictHSixRqOneOneflair}}
\providecommand{\hlMsVerdictHSixRqOneThirdburn}{\tbd{hlMsVerdictHSixRqOneThirdburn}}
\providecommand{\hlMsVerdictHSixRqOneThirdflair}{\tbd{hlMsVerdictHSixRqOneThirdflair}}
\providecommand{\hlMsVerdictMitBootburn}{\tbd{hlMsVerdictMitBootburn}}
\providecommand{\hlMsVerdictMitBootflair}{\tbd{hlMsVerdictMitBootflair}}
\providecommand{\hlMsVerdictMitGceburn}{\tbd{hlMsVerdictMitGceburn}}
\providecommand{\hlMsVerdictMitGceflair}{\tbd{hlMsVerdictMitGceflair}}
\providecommand{\hlMsVerdictNSixChes}{\tbd{hlMsVerdictNSixChes}}
\providecommand{\hlMsVerdictNSixCsTwelve}{\tbd{hlMsVerdictNSixCsTwelve}}
\providecommand{\hlMsVerdictNSixDfc}{\tbd{hlMsVerdictNSixDfc}}
\providecommand{\hlMsVerdictNSixEnva}{\tbd{hlMsVerdictNSixEnva}}
\providecommand{\hlMsVerdictNSixKuro}{\tbd{hlMsVerdictNSixKuro}}
\providecommand{\hlMsVerdictNSixOem}{\tbd{hlMsVerdictNSixOem}}
\providecommand{\hlMsVerdictNSixSnTwo}{\tbd{hlMsVerdictNSixSnTwo}}
\providecommand{\hlMsVerdictNSixburn}{\tbd{hlMsVerdictNSixburn}}
\providecommand{\hlMsVerdictNSixflair}{\tbd{hlMsVerdictNSixflair}}
\providecommand{\hlNCells}{\tbd{hlNCells}}
\providecommand{\hlNCellsComplete}{\tbd{hlNCellsComplete}}
\providecommand{\hlNCollapsedNEightburn}{\tbd{hlNCollapsedNEightburn}}
\providecommand{\hlNCollapsedNElevenburn}{\tbd{hlNCollapsedNElevenburn}}
\providecommand{\hlNCollapsedNFifteenburn}{\tbd{hlNCollapsedNFifteenburn}}
\providecommand{\hlNCollapsedNFourteenburn}{\tbd{hlNCollapsedNFourteenburn}}
\providecommand{\hlNCollapsedNNineburn}{\tbd{hlNCollapsedNNineburn}}
\providecommand{\hlNCollapsedNSevenburn}{\tbd{hlNCollapsedNSevenburn}}
\providecommand{\hlNCollapsedNTenburn}{\tbd{hlNCollapsedNTenburn}}
\providecommand{\hlNCollapsedNTwelveburn}{\tbd{hlNCollapsedNTwelveburn}}
\providecommand{\hlNCollapsedPostReviewburn}{\tbd{hlNCollapsedPostReviewburn}}
\providecommand{\hlNCollapsedburn}{\tbd{hlNCollapsedburn}}
\providecommand{\hlNNineteenInDomDiffer}{\tbd{hlNNineteenInDomDiffer}}
\providecommand{\hlNNineteenInDomEquiv}{\tbd{hlNNineteenInDomEquiv}}
\providecommand{\hlNNineteenInDomPairs}{\tbd{hlNNineteenInDomPairs}}
\providecommand{\hlNNineteenInDomRead}{\tbd{hlNNineteenInDomRead}}
\providecommand{\hlNNineteenInDomUndet}{\tbd{hlNNineteenInDomUndet}}
\providecommand{\hlNNineteenNoPreDiffer}{\tbd{hlNNineteenNoPreDiffer}}
\providecommand{\hlNNineteenNoPreEquiv}{\tbd{hlNNineteenNoPreEquiv}}
\providecommand{\hlNNineteenNoPrePairs}{\tbd{hlNNineteenNoPrePairs}}
\providecommand{\hlNNineteenNoPreRead}{\tbd{hlNNineteenNoPreRead}}
\providecommand{\hlNNineteenNoPreUndet}{\tbd{hlNNineteenNoPreUndet}}
\providecommand{\hlNNineteenOutDomDiffer}{\tbd{hlNNineteenOutDomDiffer}}
\providecommand{\hlNNineteenOutDomEquiv}{\tbd{hlNNineteenOutDomEquiv}}
\providecommand{\hlNNineteenOutDomPairs}{\tbd{hlNNineteenOutDomPairs}}
\providecommand{\hlNNineteenOutDomRead}{\tbd{hlNNineteenOutDomRead}}
\providecommand{\hlNNineteenOutDomUndet}{\tbd{hlNNineteenOutDomUndet}}
\providecommand{\hlNRunsAnalysed}{\tbd{hlNRunsAnalysed}}
\providecommand{\hlNRunsCoreAnalysed}{\tbd{hlNRunsCoreAnalysed}}
\providecommand{\hlNRunsDuplicate}{\tbd{hlNRunsDuplicate}}
\providecommand{\hlNRunsExcluded}{\tbd{hlNRunsExcluded}}
\providecommand{\hlNRunsExcludedBlocks}{\tbd{hlNRunsExcludedBlocks}}
\providecommand{\hlNRunsExtAnalysed}{\tbd{hlNRunsExtAnalysed}}
\providecommand{\hlNRunsExtDatasetsAnalysed}{\tbd{hlNRunsExtDatasetsAnalysed}}
\providecommand{\hlNRunsGpu}{\tbd{hlNRunsGpu}}
\providecommand{\hlNRunsGpuCore}{\tbd{hlNRunsGpuCore}}
\providecommand{\hlNRunsGpuExt}{\tbd{hlNRunsGpuExt}}
\providecommand{\hlNRunsNSix}{\tbd{hlNRunsNSix}}
\providecommand{\hlNRunsPostReviewAnalysed}{\tbd{hlNRunsPostReviewAnalysed}}
\providecommand{\hlNRunsReviewAnalysed}{\tbd{hlNRunsReviewAnalysed}}
\providecommand{\hlNRunsTotal}{\tbd{hlNRunsTotal}}
\providecommand{\hlOmAdjDOFAburn}{\tbd{hlOmAdjDOFAburn}}
\providecommand{\hlOmAdjDOFAflair}{\tbd{hlOmAdjDOFAflair}}
\providecommand{\hlOmAdjLVDburn}{\tbd{hlOmAdjLVDburn}}
\providecommand{\hlOmAdjLVDflair}{\tbd{hlOmAdjLVDflair}}
\providecommand{\hlOmAdjMeanburn}{\tbd{hlOmAdjMeanburn}}
\providecommand{\hlOmAdjMeanflair}{\tbd{hlOmAdjMeanflair}}
\providecommand{\hlOmAdjRNburn}{\tbd{hlOmAdjRNburn}}
\providecommand{\hlOmAdjRNflair}{\tbd{hlOmAdjRNflair}}
\providecommand{\hlOmAdjRankburn}{\tbd{hlOmAdjRankburn}}
\providecommand{\hlOmAdjRankflair}{\tbd{hlOmAdjRankflair}}
\providecommand{\hlOmAdjSATburn}{\tbd{hlOmAdjSATburn}}
\providecommand{\hlOmAdjSATflair}{\tbd{hlOmAdjSATflair}}
\providecommand{\hlOmAdjTMburn}{\tbd{hlOmAdjTMburn}}
\providecommand{\hlOmAdjTMflair}{\tbd{hlOmAdjTMflair}}
\providecommand{\hlOmRawDOFAburn}{\tbd{hlOmRawDOFAburn}}
\providecommand{\hlOmRawDOFAflair}{\tbd{hlOmRawDOFAflair}}
\providecommand{\hlOmRawLVDburn}{\tbd{hlOmRawLVDburn}}
\providecommand{\hlOmRawLVDflair}{\tbd{hlOmRawLVDflair}}
\providecommand{\hlOmRawMeanburn}{\tbd{hlOmRawMeanburn}}
\providecommand{\hlOmRawMeanflair}{\tbd{hlOmRawMeanflair}}
\providecommand{\hlOmRawRNburn}{\tbd{hlOmRawRNburn}}
\providecommand{\hlOmRawRNflair}{\tbd{hlOmRawRNflair}}
\providecommand{\hlOmRawRankburn}{\tbd{hlOmRawRankburn}}
\providecommand{\hlOmRawRankflair}{\tbd{hlOmRawRankflair}}
\providecommand{\hlOmRawSATburn}{\tbd{hlOmRawSATburn}}
\providecommand{\hlOmRawSATflair}{\tbd{hlOmRawSATflair}}
\providecommand{\hlOmRawTMburn}{\tbd{hlOmRawTMburn}}
\providecommand{\hlOmRawTMflair}{\tbd{hlOmRawTMflair}}
\providecommand{\hlOtsuFlipRateAll}{\tbd{hlOtsuFlipRateAll}}
\providecommand{\hlOtsuFlipRateTrain}{\tbd{hlOtsuFlipRateTrain}}
\providecommand{\hlOtsuFlipRateVal}{\tbd{hlOtsuFlipRateVal}}
\providecommand{\hlOtsuIoUNotWaterAll}{\tbd{hlOtsuIoUNotWaterAll}}
\providecommand{\hlOtsuIoUNotWaterTrain}{\tbd{hlOtsuIoUNotWaterTrain}}
\providecommand{\hlOtsuIoUNotWaterVal}{\tbd{hlOtsuIoUNotWaterVal}}
\providecommand{\hlOtsuIoUWaterAll}{\tbd{hlOtsuIoUWaterAll}}
\providecommand{\hlOtsuIoUWaterTrain}{\tbd{hlOtsuIoUWaterTrain}}
\providecommand{\hlOtsuIoUWaterVal}{\tbd{hlOtsuIoUWaterVal}}
\providecommand{\hlOtsuLabelMiouAll}{\tbd{hlOtsuLabelMiouAll}}
\providecommand{\hlOtsuLabelMiouFracAll}{\tbd{hlOtsuLabelMiouFracAll}}
\providecommand{\hlOtsuLabelMiouFracTrain}{\tbd{hlOtsuLabelMiouFracTrain}}
\providecommand{\hlOtsuLabelMiouFracVal}{\tbd{hlOtsuLabelMiouFracVal}}
\providecommand{\hlOtsuLabelMiouTrain}{\tbd{hlOtsuLabelMiouTrain}}
\providecommand{\hlOtsuLabelMiouVal}{\tbd{hlOtsuLabelMiouVal}}
\providecommand{\hlOtsuNTilesAll}{\tbd{hlOtsuNTilesAll}}
\providecommand{\hlOtsuNTilesTrain}{\tbd{hlOtsuNTilesTrain}}
\providecommand{\hlOtsuNTilesVal}{\tbd{hlOtsuNTilesVal}}
\providecommand{\hlPcDropAgriculturalBoundary}{\tbd{hlPcDropAgriculturalBoundary}}
\providecommand{\hlPcDropAgriculturalCoarse}{\tbd{hlPcDropAgriculturalCoarse}}
\providecommand{\hlPcDropAgriculturalOmission}{\tbd{hlPcDropAgriculturalOmission}}
\providecommand{\hlPcDropAgriculturalShift}{\tbd{hlPcDropAgriculturalShift}}
\providecommand{\hlPcDropBareSoilBoundary}{\tbd{hlPcDropBareSoilBoundary}}
\providecommand{\hlPcDropBareSoilCoarse}{\tbd{hlPcDropBareSoilCoarse}}
\providecommand{\hlPcDropBareSoilOmission}{\tbd{hlPcDropBareSoilOmission}}
\providecommand{\hlPcDropBareSoilShift}{\tbd{hlPcDropBareSoilShift}}
\providecommand{\hlPcDropBrushwoodBoundary}{\tbd{hlPcDropBrushwoodBoundary}}
\providecommand{\hlPcDropBrushwoodCoarse}{\tbd{hlPcDropBrushwoodCoarse}}
\providecommand{\hlPcDropBrushwoodOmission}{\tbd{hlPcDropBrushwoodOmission}}
\providecommand{\hlPcDropBrushwoodShift}{\tbd{hlPcDropBrushwoodShift}}
\providecommand{\hlPcDropBuildingBoundary}{\tbd{hlPcDropBuildingBoundary}}
\providecommand{\hlPcDropBuildingCoarse}{\tbd{hlPcDropBuildingCoarse}}
\providecommand{\hlPcDropBuildingOmission}{\tbd{hlPcDropBuildingOmission}}
\providecommand{\hlPcDropBuildingShift}{\tbd{hlPcDropBuildingShift}}
\providecommand{\hlPcDropCIHiAgriculturalBoundary}{\tbd{hlPcDropCIHiAgriculturalBoundary}}
\providecommand{\hlPcDropCIHiAgriculturalCoarse}{\tbd{hlPcDropCIHiAgriculturalCoarse}}
\providecommand{\hlPcDropCIHiAgriculturalOmission}{\tbd{hlPcDropCIHiAgriculturalOmission}}
\providecommand{\hlPcDropCIHiAgriculturalShift}{\tbd{hlPcDropCIHiAgriculturalShift}}
\providecommand{\hlPcDropCIHiBareSoilBoundary}{\tbd{hlPcDropCIHiBareSoilBoundary}}
\providecommand{\hlPcDropCIHiBareSoilCoarse}{\tbd{hlPcDropCIHiBareSoilCoarse}}
\providecommand{\hlPcDropCIHiBareSoilOmission}{\tbd{hlPcDropCIHiBareSoilOmission}}
\providecommand{\hlPcDropCIHiBareSoilShift}{\tbd{hlPcDropCIHiBareSoilShift}}
\providecommand{\hlPcDropCIHiBrushwoodBoundary}{\tbd{hlPcDropCIHiBrushwoodBoundary}}
\providecommand{\hlPcDropCIHiBrushwoodCoarse}{\tbd{hlPcDropCIHiBrushwoodCoarse}}
\providecommand{\hlPcDropCIHiBrushwoodOmission}{\tbd{hlPcDropCIHiBrushwoodOmission}}
\providecommand{\hlPcDropCIHiBrushwoodShift}{\tbd{hlPcDropCIHiBrushwoodShift}}
\providecommand{\hlPcDropCIHiBuildingBoundary}{\tbd{hlPcDropCIHiBuildingBoundary}}
\providecommand{\hlPcDropCIHiBuildingCoarse}{\tbd{hlPcDropCIHiBuildingCoarse}}
\providecommand{\hlPcDropCIHiBuildingOmission}{\tbd{hlPcDropCIHiBuildingOmission}}
\providecommand{\hlPcDropCIHiBuildingShift}{\tbd{hlPcDropCIHiBuildingShift}}
\providecommand{\hlPcDropCIHiConiferousBoundary}{\tbd{hlPcDropCIHiConiferousBoundary}}
\providecommand{\hlPcDropCIHiConiferousCoarse}{\tbd{hlPcDropCIHiConiferousCoarse}}
\providecommand{\hlPcDropCIHiConiferousOmission}{\tbd{hlPcDropCIHiConiferousOmission}}
\providecommand{\hlPcDropCIHiConiferousShift}{\tbd{hlPcDropCIHiConiferousShift}}
\providecommand{\hlPcDropCIHiDeciduousBoundary}{\tbd{hlPcDropCIHiDeciduousBoundary}}
\providecommand{\hlPcDropCIHiDeciduousCoarse}{\tbd{hlPcDropCIHiDeciduousCoarse}}
\providecommand{\hlPcDropCIHiDeciduousOmission}{\tbd{hlPcDropCIHiDeciduousOmission}}
\providecommand{\hlPcDropCIHiDeciduousShift}{\tbd{hlPcDropCIHiDeciduousShift}}
\providecommand{\hlPcDropCIHiHerbaceousBoundary}{\tbd{hlPcDropCIHiHerbaceousBoundary}}
\providecommand{\hlPcDropCIHiHerbaceousCoarse}{\tbd{hlPcDropCIHiHerbaceousCoarse}}
\providecommand{\hlPcDropCIHiHerbaceousOmission}{\tbd{hlPcDropCIHiHerbaceousOmission}}
\providecommand{\hlPcDropCIHiHerbaceousShift}{\tbd{hlPcDropCIHiHerbaceousShift}}
\providecommand{\hlPcDropCIHiImperviousBoundary}{\tbd{hlPcDropCIHiImperviousBoundary}}
\providecommand{\hlPcDropCIHiImperviousCoarse}{\tbd{hlPcDropCIHiImperviousCoarse}}
\providecommand{\hlPcDropCIHiImperviousOmission}{\tbd{hlPcDropCIHiImperviousOmission}}
\providecommand{\hlPcDropCIHiImperviousShift}{\tbd{hlPcDropCIHiImperviousShift}}
\providecommand{\hlPcDropCIHiOtherBoundary}{\tbd{hlPcDropCIHiOtherBoundary}}
\providecommand{\hlPcDropCIHiOtherCoarse}{\tbd{hlPcDropCIHiOtherCoarse}}
\providecommand{\hlPcDropCIHiOtherOmission}{\tbd{hlPcDropCIHiOtherOmission}}
\providecommand{\hlPcDropCIHiOtherShift}{\tbd{hlPcDropCIHiOtherShift}}
\providecommand{\hlPcDropCIHiPerviousBoundary}{\tbd{hlPcDropCIHiPerviousBoundary}}
\providecommand{\hlPcDropCIHiPerviousCoarse}{\tbd{hlPcDropCIHiPerviousCoarse}}
\providecommand{\hlPcDropCIHiPerviousOmission}{\tbd{hlPcDropCIHiPerviousOmission}}
\providecommand{\hlPcDropCIHiPerviousShift}{\tbd{hlPcDropCIHiPerviousShift}}
\providecommand{\hlPcDropCIHiPlowedBoundary}{\tbd{hlPcDropCIHiPlowedBoundary}}
\providecommand{\hlPcDropCIHiPlowedCoarse}{\tbd{hlPcDropCIHiPlowedCoarse}}
\providecommand{\hlPcDropCIHiPlowedOmission}{\tbd{hlPcDropCIHiPlowedOmission}}
\providecommand{\hlPcDropCIHiPlowedShift}{\tbd{hlPcDropCIHiPlowedShift}}
\providecommand{\hlPcDropCIHiVineyardBoundary}{\tbd{hlPcDropCIHiVineyardBoundary}}
\providecommand{\hlPcDropCIHiVineyardCoarse}{\tbd{hlPcDropCIHiVineyardCoarse}}
\providecommand{\hlPcDropCIHiVineyardOmission}{\tbd{hlPcDropCIHiVineyardOmission}}
\providecommand{\hlPcDropCIHiVineyardShift}{\tbd{hlPcDropCIHiVineyardShift}}
\providecommand{\hlPcDropCIHiWaterBoundary}{\tbd{hlPcDropCIHiWaterBoundary}}
\providecommand{\hlPcDropCIHiWaterCoarse}{\tbd{hlPcDropCIHiWaterCoarse}}
\providecommand{\hlPcDropCIHiWaterOmission}{\tbd{hlPcDropCIHiWaterOmission}}
\providecommand{\hlPcDropCIHiWaterShift}{\tbd{hlPcDropCIHiWaterShift}}
\providecommand{\hlPcDropCILoAgriculturalBoundary}{\tbd{hlPcDropCILoAgriculturalBoundary}}
\providecommand{\hlPcDropCILoAgriculturalCoarse}{\tbd{hlPcDropCILoAgriculturalCoarse}}
\providecommand{\hlPcDropCILoAgriculturalOmission}{\tbd{hlPcDropCILoAgriculturalOmission}}
\providecommand{\hlPcDropCILoAgriculturalShift}{\tbd{hlPcDropCILoAgriculturalShift}}
\providecommand{\hlPcDropCILoBareSoilBoundary}{\tbd{hlPcDropCILoBareSoilBoundary}}
\providecommand{\hlPcDropCILoBareSoilCoarse}{\tbd{hlPcDropCILoBareSoilCoarse}}
\providecommand{\hlPcDropCILoBareSoilOmission}{\tbd{hlPcDropCILoBareSoilOmission}}
\providecommand{\hlPcDropCILoBareSoilShift}{\tbd{hlPcDropCILoBareSoilShift}}
\providecommand{\hlPcDropCILoBrushwoodBoundary}{\tbd{hlPcDropCILoBrushwoodBoundary}}
\providecommand{\hlPcDropCILoBrushwoodCoarse}{\tbd{hlPcDropCILoBrushwoodCoarse}}
\providecommand{\hlPcDropCILoBrushwoodOmission}{\tbd{hlPcDropCILoBrushwoodOmission}}
\providecommand{\hlPcDropCILoBrushwoodShift}{\tbd{hlPcDropCILoBrushwoodShift}}
\providecommand{\hlPcDropCILoBuildingBoundary}{\tbd{hlPcDropCILoBuildingBoundary}}
\providecommand{\hlPcDropCILoBuildingCoarse}{\tbd{hlPcDropCILoBuildingCoarse}}
\providecommand{\hlPcDropCILoBuildingOmission}{\tbd{hlPcDropCILoBuildingOmission}}
\providecommand{\hlPcDropCILoBuildingShift}{\tbd{hlPcDropCILoBuildingShift}}
\providecommand{\hlPcDropCILoConiferousBoundary}{\tbd{hlPcDropCILoConiferousBoundary}}
\providecommand{\hlPcDropCILoConiferousCoarse}{\tbd{hlPcDropCILoConiferousCoarse}}
\providecommand{\hlPcDropCILoConiferousOmission}{\tbd{hlPcDropCILoConiferousOmission}}
\providecommand{\hlPcDropCILoConiferousShift}{\tbd{hlPcDropCILoConiferousShift}}
\providecommand{\hlPcDropCILoDeciduousBoundary}{\tbd{hlPcDropCILoDeciduousBoundary}}
\providecommand{\hlPcDropCILoDeciduousCoarse}{\tbd{hlPcDropCILoDeciduousCoarse}}
\providecommand{\hlPcDropCILoDeciduousOmission}{\tbd{hlPcDropCILoDeciduousOmission}}
\providecommand{\hlPcDropCILoDeciduousShift}{\tbd{hlPcDropCILoDeciduousShift}}
\providecommand{\hlPcDropCILoHerbaceousBoundary}{\tbd{hlPcDropCILoHerbaceousBoundary}}
\providecommand{\hlPcDropCILoHerbaceousCoarse}{\tbd{hlPcDropCILoHerbaceousCoarse}}
\providecommand{\hlPcDropCILoHerbaceousOmission}{\tbd{hlPcDropCILoHerbaceousOmission}}
\providecommand{\hlPcDropCILoHerbaceousShift}{\tbd{hlPcDropCILoHerbaceousShift}}
\providecommand{\hlPcDropCILoImperviousBoundary}{\tbd{hlPcDropCILoImperviousBoundary}}
\providecommand{\hlPcDropCILoImperviousCoarse}{\tbd{hlPcDropCILoImperviousCoarse}}
\providecommand{\hlPcDropCILoImperviousOmission}{\tbd{hlPcDropCILoImperviousOmission}}
\providecommand{\hlPcDropCILoImperviousShift}{\tbd{hlPcDropCILoImperviousShift}}
\providecommand{\hlPcDropCILoOtherBoundary}{\tbd{hlPcDropCILoOtherBoundary}}
\providecommand{\hlPcDropCILoOtherCoarse}{\tbd{hlPcDropCILoOtherCoarse}}
\providecommand{\hlPcDropCILoOtherOmission}{\tbd{hlPcDropCILoOtherOmission}}
\providecommand{\hlPcDropCILoOtherShift}{\tbd{hlPcDropCILoOtherShift}}
\providecommand{\hlPcDropCILoPerviousBoundary}{\tbd{hlPcDropCILoPerviousBoundary}}
\providecommand{\hlPcDropCILoPerviousCoarse}{\tbd{hlPcDropCILoPerviousCoarse}}
\providecommand{\hlPcDropCILoPerviousOmission}{\tbd{hlPcDropCILoPerviousOmission}}
\providecommand{\hlPcDropCILoPerviousShift}{\tbd{hlPcDropCILoPerviousShift}}
\providecommand{\hlPcDropCILoPlowedBoundary}{\tbd{hlPcDropCILoPlowedBoundary}}
\providecommand{\hlPcDropCILoPlowedCoarse}{\tbd{hlPcDropCILoPlowedCoarse}}
\providecommand{\hlPcDropCILoPlowedOmission}{\tbd{hlPcDropCILoPlowedOmission}}
\providecommand{\hlPcDropCILoPlowedShift}{\tbd{hlPcDropCILoPlowedShift}}
\providecommand{\hlPcDropCILoVineyardBoundary}{\tbd{hlPcDropCILoVineyardBoundary}}
\providecommand{\hlPcDropCILoVineyardCoarse}{\tbd{hlPcDropCILoVineyardCoarse}}
\providecommand{\hlPcDropCILoVineyardOmission}{\tbd{hlPcDropCILoVineyardOmission}}
\providecommand{\hlPcDropCILoVineyardShift}{\tbd{hlPcDropCILoVineyardShift}}
\providecommand{\hlPcDropCILoWaterBoundary}{\tbd{hlPcDropCILoWaterBoundary}}
\providecommand{\hlPcDropCILoWaterCoarse}{\tbd{hlPcDropCILoWaterCoarse}}
\providecommand{\hlPcDropCILoWaterOmission}{\tbd{hlPcDropCILoWaterOmission}}
\providecommand{\hlPcDropCILoWaterShift}{\tbd{hlPcDropCILoWaterShift}}
\providecommand{\hlPcDropConiferousBoundary}{\tbd{hlPcDropConiferousBoundary}}
\providecommand{\hlPcDropConiferousCoarse}{\tbd{hlPcDropConiferousCoarse}}
\providecommand{\hlPcDropConiferousOmission}{\tbd{hlPcDropConiferousOmission}}
\providecommand{\hlPcDropConiferousShift}{\tbd{hlPcDropConiferousShift}}
\providecommand{\hlPcDropDeciduousBoundary}{\tbd{hlPcDropDeciduousBoundary}}
\providecommand{\hlPcDropDeciduousCoarse}{\tbd{hlPcDropDeciduousCoarse}}
\providecommand{\hlPcDropDeciduousOmission}{\tbd{hlPcDropDeciduousOmission}}
\providecommand{\hlPcDropDeciduousShift}{\tbd{hlPcDropDeciduousShift}}
\providecommand{\hlPcDropHerbaceousBoundary}{\tbd{hlPcDropHerbaceousBoundary}}
\providecommand{\hlPcDropHerbaceousCoarse}{\tbd{hlPcDropHerbaceousCoarse}}
\providecommand{\hlPcDropHerbaceousOmission}{\tbd{hlPcDropHerbaceousOmission}}
\providecommand{\hlPcDropHerbaceousShift}{\tbd{hlPcDropHerbaceousShift}}
\providecommand{\hlPcDropImperviousBoundary}{\tbd{hlPcDropImperviousBoundary}}
\providecommand{\hlPcDropImperviousCoarse}{\tbd{hlPcDropImperviousCoarse}}
\providecommand{\hlPcDropImperviousOmission}{\tbd{hlPcDropImperviousOmission}}
\providecommand{\hlPcDropImperviousShift}{\tbd{hlPcDropImperviousShift}}
\providecommand{\hlPcDropOtherBoundary}{\tbd{hlPcDropOtherBoundary}}
\providecommand{\hlPcDropOtherCoarse}{\tbd{hlPcDropOtherCoarse}}
\providecommand{\hlPcDropOtherOmission}{\tbd{hlPcDropOtherOmission}}
\providecommand{\hlPcDropOtherShift}{\tbd{hlPcDropOtherShift}}
\providecommand{\hlPcDropPerviousBoundary}{\tbd{hlPcDropPerviousBoundary}}
\providecommand{\hlPcDropPerviousCoarse}{\tbd{hlPcDropPerviousCoarse}}
\providecommand{\hlPcDropPerviousOmission}{\tbd{hlPcDropPerviousOmission}}
\providecommand{\hlPcDropPerviousShift}{\tbd{hlPcDropPerviousShift}}
\providecommand{\hlPcDropPlowedBoundary}{\tbd{hlPcDropPlowedBoundary}}
\providecommand{\hlPcDropPlowedCoarse}{\tbd{hlPcDropPlowedCoarse}}
\providecommand{\hlPcDropPlowedOmission}{\tbd{hlPcDropPlowedOmission}}
\providecommand{\hlPcDropPlowedShift}{\tbd{hlPcDropPlowedShift}}
\providecommand{\hlPcDropVineyardBoundary}{\tbd{hlPcDropVineyardBoundary}}
\providecommand{\hlPcDropVineyardCoarse}{\tbd{hlPcDropVineyardCoarse}}
\providecommand{\hlPcDropVineyardOmission}{\tbd{hlPcDropVineyardOmission}}
\providecommand{\hlPcDropVineyardShift}{\tbd{hlPcDropVineyardShift}}
\providecommand{\hlPcDropWaterBoundary}{\tbd{hlPcDropWaterBoundary}}
\providecommand{\hlPcDropWaterCoarse}{\tbd{hlPcDropWaterCoarse}}
\providecommand{\hlPcDropWaterOmission}{\tbd{hlPcDropWaterOmission}}
\providecommand{\hlPcDropWaterShift}{\tbd{hlPcDropWaterShift}}
\providecommand{\hlRNRGBburn}{\tbd{hlRNRGBburn}}
\providecommand{\hlRNRGBburnN}{\tbd{hlRNRGBburnN}}
\providecommand{\hlRNRGBflair}{\tbd{hlRNRGBflair}}
\providecommand{\hlRankDsPooled}{\tbd{hlRankDsPooled}}
\providecommand{\hlRankNChes}{\tbd{hlRankNChes}}
\providecommand{\hlRankNCore}{\tbd{hlRankNCore}}
\providecommand{\hlRankNCsTwelve}{\tbd{hlRankNCsTwelve}}
\providecommand{\hlRankNDfc}{\tbd{hlRankNDfc}}
\providecommand{\hlRankNEnva}{\tbd{hlRankNEnva}}
\providecommand{\hlRankNKuro}{\tbd{hlRankNKuro}}
\providecommand{\hlRankNOem}{\tbd{hlRankNOem}}
\providecommand{\hlRankNPooled}{\tbd{hlRankNPooled}}
\providecommand{\hlRankNSnTwo}{\tbd{hlRankNSnTwo}}
\providecommand{\hlRankNburn}{\tbd{hlRankNburn}}
\providecommand{\hlRankNflair}{\tbd{hlRankNflair}}
\providecommand{\hlRankNineChesN}{\tbd{hlRankNineChesN}}
\providecommand{\hlRankNineChesRho}{\tbd{hlRankNineChesRho}}
\providecommand{\hlRankNineChesRhoCIHi}{\tbd{hlRankNineChesRhoCIHi}}
\providecommand{\hlRankNineChesRhoCILo}{\tbd{hlRankNineChesRhoCILo}}
\providecommand{\hlRankNineChesRhoP}{\tbd{hlRankNineChesRhoP}}
\providecommand{\hlRankNineChesTau}{\tbd{hlRankNineChesTau}}
\providecommand{\hlRankNineCsTwelveN}{\tbd{hlRankNineCsTwelveN}}
\providecommand{\hlRankNineCsTwelveRho}{\tbd{hlRankNineCsTwelveRho}}
\providecommand{\hlRankNineCsTwelveRhoCIHi}{\tbd{hlRankNineCsTwelveRhoCIHi}}
\providecommand{\hlRankNineCsTwelveRhoCILo}{\tbd{hlRankNineCsTwelveRhoCILo}}
\providecommand{\hlRankNineCsTwelveRhoP}{\tbd{hlRankNineCsTwelveRhoP}}
\providecommand{\hlRankNineCsTwelveTau}{\tbd{hlRankNineCsTwelveTau}}
\providecommand{\hlRankNineDfcN}{\tbd{hlRankNineDfcN}}
\providecommand{\hlRankNineDfcRho}{\tbd{hlRankNineDfcRho}}
\providecommand{\hlRankNineDfcRhoCIHi}{\tbd{hlRankNineDfcRhoCIHi}}
\providecommand{\hlRankNineDfcRhoCILo}{\tbd{hlRankNineDfcRhoCILo}}
\providecommand{\hlRankNineDfcRhoP}{\tbd{hlRankNineDfcRhoP}}
\providecommand{\hlRankNineDfcTau}{\tbd{hlRankNineDfcTau}}
\providecommand{\hlRankNineEnvaN}{\tbd{hlRankNineEnvaN}}
\providecommand{\hlRankNineEnvaRho}{\tbd{hlRankNineEnvaRho}}
\providecommand{\hlRankNineEnvaRhoCIHi}{\tbd{hlRankNineEnvaRhoCIHi}}
\providecommand{\hlRankNineEnvaRhoCILo}{\tbd{hlRankNineEnvaRhoCILo}}
\providecommand{\hlRankNineEnvaRhoP}{\tbd{hlRankNineEnvaRhoP}}
\providecommand{\hlRankNineEnvaTau}{\tbd{hlRankNineEnvaTau}}
\providecommand{\hlRankNineInDomChesExcluded}{\tbd{hlRankNineInDomChesExcluded}}
\providecommand{\hlRankNineInDomChesN}{\tbd{hlRankNineInDomChesN}}
\providecommand{\hlRankNineInDomChesRho}{\tbd{hlRankNineInDomChesRho}}
\providecommand{\hlRankNineInDomChesRhoCIHi}{\tbd{hlRankNineInDomChesRhoCIHi}}
\providecommand{\hlRankNineInDomChesRhoCILo}{\tbd{hlRankNineInDomChesRhoCILo}}
\providecommand{\hlRankNineInDomChesRhoP}{\tbd{hlRankNineInDomChesRhoP}}
\providecommand{\hlRankNineInDomChesTau}{\tbd{hlRankNineInDomChesTau}}
\providecommand{\hlRankNineInDomCsTwelveExcluded}{\tbd{hlRankNineInDomCsTwelveExcluded}}
\providecommand{\hlRankNineInDomCsTwelveN}{\tbd{hlRankNineInDomCsTwelveN}}
\providecommand{\hlRankNineInDomCsTwelveRho}{\tbd{hlRankNineInDomCsTwelveRho}}
\providecommand{\hlRankNineInDomCsTwelveRhoCIHi}{\tbd{hlRankNineInDomCsTwelveRhoCIHi}}
\providecommand{\hlRankNineInDomCsTwelveRhoCILo}{\tbd{hlRankNineInDomCsTwelveRhoCILo}}
\providecommand{\hlRankNineInDomCsTwelveRhoP}{\tbd{hlRankNineInDomCsTwelveRhoP}}
\providecommand{\hlRankNineInDomCsTwelveTau}{\tbd{hlRankNineInDomCsTwelveTau}}
\providecommand{\hlRankNineInDomDfcExcluded}{\tbd{hlRankNineInDomDfcExcluded}}
\providecommand{\hlRankNineInDomDfcN}{\tbd{hlRankNineInDomDfcN}}
\providecommand{\hlRankNineInDomDfcRho}{\tbd{hlRankNineInDomDfcRho}}
\providecommand{\hlRankNineInDomDfcRhoCIHi}{\tbd{hlRankNineInDomDfcRhoCIHi}}
\providecommand{\hlRankNineInDomDfcRhoCILo}{\tbd{hlRankNineInDomDfcRhoCILo}}
\providecommand{\hlRankNineInDomDfcRhoP}{\tbd{hlRankNineInDomDfcRhoP}}
\providecommand{\hlRankNineInDomDfcTau}{\tbd{hlRankNineInDomDfcTau}}
\providecommand{\hlRankNineInDomEnvaExcluded}{\tbd{hlRankNineInDomEnvaExcluded}}
\providecommand{\hlRankNineInDomEnvaN}{\tbd{hlRankNineInDomEnvaN}}
\providecommand{\hlRankNineInDomEnvaRho}{\tbd{hlRankNineInDomEnvaRho}}
\providecommand{\hlRankNineInDomEnvaRhoCIHi}{\tbd{hlRankNineInDomEnvaRhoCIHi}}
\providecommand{\hlRankNineInDomEnvaRhoCILo}{\tbd{hlRankNineInDomEnvaRhoCILo}}
\providecommand{\hlRankNineInDomEnvaRhoP}{\tbd{hlRankNineInDomEnvaRhoP}}
\providecommand{\hlRankNineInDomEnvaTau}{\tbd{hlRankNineInDomEnvaTau}}
\providecommand{\hlRankNineInDomKuroExcluded}{\tbd{hlRankNineInDomKuroExcluded}}
\providecommand{\hlRankNineInDomKuroN}{\tbd{hlRankNineInDomKuroN}}
\providecommand{\hlRankNineInDomKuroRho}{\tbd{hlRankNineInDomKuroRho}}
\providecommand{\hlRankNineInDomKuroRhoCIHi}{\tbd{hlRankNineInDomKuroRhoCIHi}}
\providecommand{\hlRankNineInDomKuroRhoCILo}{\tbd{hlRankNineInDomKuroRhoCILo}}
\providecommand{\hlRankNineInDomKuroRhoP}{\tbd{hlRankNineInDomKuroRhoP}}
\providecommand{\hlRankNineInDomKuroTau}{\tbd{hlRankNineInDomKuroTau}}
\providecommand{\hlRankNineInDomOemExcluded}{\tbd{hlRankNineInDomOemExcluded}}
\providecommand{\hlRankNineInDomOemN}{\tbd{hlRankNineInDomOemN}}
\providecommand{\hlRankNineInDomOemRho}{\tbd{hlRankNineInDomOemRho}}
\providecommand{\hlRankNineInDomOemRhoCIHi}{\tbd{hlRankNineInDomOemRhoCIHi}}
\providecommand{\hlRankNineInDomOemRhoCILo}{\tbd{hlRankNineInDomOemRhoCILo}}
\providecommand{\hlRankNineInDomOemRhoP}{\tbd{hlRankNineInDomOemRhoP}}
\providecommand{\hlRankNineInDomOemTau}{\tbd{hlRankNineInDomOemTau}}
\providecommand{\hlRankNineInDomPooledN}{\tbd{hlRankNineInDomPooledN}}
\providecommand{\hlRankNineInDomPooledRho}{\tbd{hlRankNineInDomPooledRho}}
\providecommand{\hlRankNineInDomPooledRhoCIHi}{\tbd{hlRankNineInDomPooledRhoCIHi}}
\providecommand{\hlRankNineInDomPooledRhoCILo}{\tbd{hlRankNineInDomPooledRhoCILo}}
\providecommand{\hlRankNineInDomPooledTau}{\tbd{hlRankNineInDomPooledTau}}
\providecommand{\hlRankNineInDomRead}{\tbd{hlRankNineInDomRead}}
\providecommand{\hlRankNineInDomSepCount}{\tbd{hlRankNineInDomSepCount}}
\providecommand{\hlRankNineInDomSnTwoExcluded}{\tbd{hlRankNineInDomSnTwoExcluded}}
\providecommand{\hlRankNineInDomSnTwoN}{\tbd{hlRankNineInDomSnTwoN}}
\providecommand{\hlRankNineInDomSnTwoRho}{\tbd{hlRankNineInDomSnTwoRho}}
\providecommand{\hlRankNineInDomSnTwoRhoCIHi}{\tbd{hlRankNineInDomSnTwoRhoCIHi}}
\providecommand{\hlRankNineInDomSnTwoRhoCILo}{\tbd{hlRankNineInDomSnTwoRhoCILo}}
\providecommand{\hlRankNineInDomSnTwoRhoP}{\tbd{hlRankNineInDomSnTwoRhoP}}
\providecommand{\hlRankNineInDomSnTwoTau}{\tbd{hlRankNineInDomSnTwoTau}}
\providecommand{\hlRankNineKuroN}{\tbd{hlRankNineKuroN}}
\providecommand{\hlRankNineKuroRho}{\tbd{hlRankNineKuroRho}}
\providecommand{\hlRankNineKuroRhoCIHi}{\tbd{hlRankNineKuroRhoCIHi}}
\providecommand{\hlRankNineKuroRhoCILo}{\tbd{hlRankNineKuroRhoCILo}}
\providecommand{\hlRankNineKuroRhoP}{\tbd{hlRankNineKuroRhoP}}
\providecommand{\hlRankNineKuroTau}{\tbd{hlRankNineKuroTau}}
\providecommand{\hlRankNineOemN}{\tbd{hlRankNineOemN}}
\providecommand{\hlRankNineOemRho}{\tbd{hlRankNineOemRho}}
\providecommand{\hlRankNineOemRhoCIHi}{\tbd{hlRankNineOemRhoCIHi}}
\providecommand{\hlRankNineOemRhoCILo}{\tbd{hlRankNineOemRhoCILo}}
\providecommand{\hlRankNineOemRhoP}{\tbd{hlRankNineOemRhoP}}
\providecommand{\hlRankNineOemTau}{\tbd{hlRankNineOemTau}}
\providecommand{\hlRankNinePooledN}{\tbd{hlRankNinePooledN}}
\providecommand{\hlRankNinePooledRho}{\tbd{hlRankNinePooledRho}}
\providecommand{\hlRankNinePooledRhoCIHi}{\tbd{hlRankNinePooledRhoCIHi}}
\providecommand{\hlRankNinePooledRhoCILo}{\tbd{hlRankNinePooledRhoCILo}}
\providecommand{\hlRankNinePooledTau}{\tbd{hlRankNinePooledTau}}
\providecommand{\hlRankNineRead}{\tbd{hlRankNineRead}}
\providecommand{\hlRankNineSepCount}{\tbd{hlRankNineSepCount}}
\providecommand{\hlRankNineSnTwoN}{\tbd{hlRankNineSnTwoN}}
\providecommand{\hlRankNineSnTwoRho}{\tbd{hlRankNineSnTwoRho}}
\providecommand{\hlRankNineSnTwoRhoCIHi}{\tbd{hlRankNineSnTwoRhoCIHi}}
\providecommand{\hlRankNineSnTwoRhoCILo}{\tbd{hlRankNineSnTwoRhoCILo}}
\providecommand{\hlRankNineSnTwoRhoP}{\tbd{hlRankNineSnTwoRhoP}}
\providecommand{\hlRankNineSnTwoTau}{\tbd{hlRankNineSnTwoTau}}
\providecommand{\hlRankNineTotal}{\tbd{hlRankNineTotal}}
\providecommand{\hlRankRhoCIHiChes}{\tbd{hlRankRhoCIHiChes}}
\providecommand{\hlRankRhoCIHiCore}{\tbd{hlRankRhoCIHiCore}}
\providecommand{\hlRankRhoCIHiCsTwelve}{\tbd{hlRankRhoCIHiCsTwelve}}
\providecommand{\hlRankRhoCIHiDfc}{\tbd{hlRankRhoCIHiDfc}}
\providecommand{\hlRankRhoCIHiEnva}{\tbd{hlRankRhoCIHiEnva}}
\providecommand{\hlRankRhoCIHiKuro}{\tbd{hlRankRhoCIHiKuro}}
\providecommand{\hlRankRhoCIHiOem}{\tbd{hlRankRhoCIHiOem}}
\providecommand{\hlRankRhoCIHiPooled}{\tbd{hlRankRhoCIHiPooled}}
\providecommand{\hlRankRhoCIHiSnTwo}{\tbd{hlRankRhoCIHiSnTwo}}
\providecommand{\hlRankRhoCIHiburn}{\tbd{hlRankRhoCIHiburn}}
\providecommand{\hlRankRhoCIHiflair}{\tbd{hlRankRhoCIHiflair}}
\providecommand{\hlRankRhoCILoChes}{\tbd{hlRankRhoCILoChes}}
\providecommand{\hlRankRhoCILoCore}{\tbd{hlRankRhoCILoCore}}
\providecommand{\hlRankRhoCILoCsTwelve}{\tbd{hlRankRhoCILoCsTwelve}}
\providecommand{\hlRankRhoCILoDfc}{\tbd{hlRankRhoCILoDfc}}
\providecommand{\hlRankRhoCILoEnva}{\tbd{hlRankRhoCILoEnva}}
\providecommand{\hlRankRhoCILoKuro}{\tbd{hlRankRhoCILoKuro}}
\providecommand{\hlRankRhoCILoOem}{\tbd{hlRankRhoCILoOem}}
\providecommand{\hlRankRhoCILoPooled}{\tbd{hlRankRhoCILoPooled}}
\providecommand{\hlRankRhoCILoSnTwo}{\tbd{hlRankRhoCILoSnTwo}}
\providecommand{\hlRankRhoCILoburn}{\tbd{hlRankRhoCILoburn}}
\providecommand{\hlRankRhoCILoflair}{\tbd{hlRankRhoCILoflair}}
\providecommand{\hlRankRhoChes}{\tbd{hlRankRhoChes}}
\providecommand{\hlRankRhoCore}{\tbd{hlRankRhoCore}}
\providecommand{\hlRankRhoCsTwelve}{\tbd{hlRankRhoCsTwelve}}
\providecommand{\hlRankRhoDfc}{\tbd{hlRankRhoDfc}}
\providecommand{\hlRankRhoEnva}{\tbd{hlRankRhoEnva}}
\providecommand{\hlRankRhoKuro}{\tbd{hlRankRhoKuro}}
\providecommand{\hlRankRhoOem}{\tbd{hlRankRhoOem}}
\providecommand{\hlRankRhoPChes}{\tbd{hlRankRhoPChes}}
\providecommand{\hlRankRhoPCsTwelve}{\tbd{hlRankRhoPCsTwelve}}
\providecommand{\hlRankRhoPDfc}{\tbd{hlRankRhoPDfc}}
\providecommand{\hlRankRhoPEnva}{\tbd{hlRankRhoPEnva}}
\providecommand{\hlRankRhoPKuro}{\tbd{hlRankRhoPKuro}}
\providecommand{\hlRankRhoPOem}{\tbd{hlRankRhoPOem}}
\providecommand{\hlRankRhoPSnTwo}{\tbd{hlRankRhoPSnTwo}}
\providecommand{\hlRankRhoPburn}{\tbd{hlRankRhoPburn}}
\providecommand{\hlRankRhoPflair}{\tbd{hlRankRhoPflair}}
\providecommand{\hlRankRhoPooled}{\tbd{hlRankRhoPooled}}
\providecommand{\hlRankRhoSnTwo}{\tbd{hlRankRhoSnTwo}}
\providecommand{\hlRankRhoburn}{\tbd{hlRankRhoburn}}
\providecommand{\hlRankRhoflair}{\tbd{hlRankRhoflair}}
\providecommand{\hlRankSlopeCIHiChes}{\tbd{hlRankSlopeCIHiChes}}
\providecommand{\hlRankSlopeCIHiCore}{\tbd{hlRankSlopeCIHiCore}}
\providecommand{\hlRankSlopeCIHiCsTwelve}{\tbd{hlRankSlopeCIHiCsTwelve}}
\providecommand{\hlRankSlopeCIHiDfc}{\tbd{hlRankSlopeCIHiDfc}}
\providecommand{\hlRankSlopeCIHiEnva}{\tbd{hlRankSlopeCIHiEnva}}
\providecommand{\hlRankSlopeCIHiKuro}{\tbd{hlRankSlopeCIHiKuro}}
\providecommand{\hlRankSlopeCIHiOem}{\tbd{hlRankSlopeCIHiOem}}
\providecommand{\hlRankSlopeCIHiPooled}{\tbd{hlRankSlopeCIHiPooled}}
\providecommand{\hlRankSlopeCIHiSnTwo}{\tbd{hlRankSlopeCIHiSnTwo}}
\providecommand{\hlRankSlopeCIHiburn}{\tbd{hlRankSlopeCIHiburn}}
\providecommand{\hlRankSlopeCIHiflair}{\tbd{hlRankSlopeCIHiflair}}
\providecommand{\hlRankSlopeCILoChes}{\tbd{hlRankSlopeCILoChes}}
\providecommand{\hlRankSlopeCILoCore}{\tbd{hlRankSlopeCILoCore}}
\providecommand{\hlRankSlopeCILoCsTwelve}{\tbd{hlRankSlopeCILoCsTwelve}}
\providecommand{\hlRankSlopeCILoDfc}{\tbd{hlRankSlopeCILoDfc}}
\providecommand{\hlRankSlopeCILoEnva}{\tbd{hlRankSlopeCILoEnva}}
\providecommand{\hlRankSlopeCILoKuro}{\tbd{hlRankSlopeCILoKuro}}
\providecommand{\hlRankSlopeCILoOem}{\tbd{hlRankSlopeCILoOem}}
\providecommand{\hlRankSlopeCILoPooled}{\tbd{hlRankSlopeCILoPooled}}
\providecommand{\hlRankSlopeCILoSnTwo}{\tbd{hlRankSlopeCILoSnTwo}}
\providecommand{\hlRankSlopeCILoburn}{\tbd{hlRankSlopeCILoburn}}
\providecommand{\hlRankSlopeCILoflair}{\tbd{hlRankSlopeCILoflair}}
\providecommand{\hlRankSlopeChes}{\tbd{hlRankSlopeChes}}
\providecommand{\hlRankSlopeCore}{\tbd{hlRankSlopeCore}}
\providecommand{\hlRankSlopeCsTwelve}{\tbd{hlRankSlopeCsTwelve}}
\providecommand{\hlRankSlopeDfc}{\tbd{hlRankSlopeDfc}}
\providecommand{\hlRankSlopeEnva}{\tbd{hlRankSlopeEnva}}
\providecommand{\hlRankSlopeKuro}{\tbd{hlRankSlopeKuro}}
\providecommand{\hlRankSlopeOem}{\tbd{hlRankSlopeOem}}
\providecommand{\hlRankSlopePooled}{\tbd{hlRankSlopePooled}}
\providecommand{\hlRankSlopeSnTwo}{\tbd{hlRankSlopeSnTwo}}
\providecommand{\hlRankSlopeburn}{\tbd{hlRankSlopeburn}}
\providecommand{\hlRankSlopeflair}{\tbd{hlRankSlopeflair}}
\providecommand{\hlRankTauCIHiChes}{\tbd{hlRankTauCIHiChes}}
\providecommand{\hlRankTauCIHiCore}{\tbd{hlRankTauCIHiCore}}
\providecommand{\hlRankTauCIHiCsTwelve}{\tbd{hlRankTauCIHiCsTwelve}}
\providecommand{\hlRankTauCIHiDfc}{\tbd{hlRankTauCIHiDfc}}
\providecommand{\hlRankTauCIHiEnva}{\tbd{hlRankTauCIHiEnva}}
\providecommand{\hlRankTauCIHiKuro}{\tbd{hlRankTauCIHiKuro}}
\providecommand{\hlRankTauCIHiOem}{\tbd{hlRankTauCIHiOem}}
\providecommand{\hlRankTauCIHiPooled}{\tbd{hlRankTauCIHiPooled}}
\providecommand{\hlRankTauCIHiSnTwo}{\tbd{hlRankTauCIHiSnTwo}}
\providecommand{\hlRankTauCIHiburn}{\tbd{hlRankTauCIHiburn}}
\providecommand{\hlRankTauCIHiflair}{\tbd{hlRankTauCIHiflair}}
\providecommand{\hlRankTauCILoChes}{\tbd{hlRankTauCILoChes}}
\providecommand{\hlRankTauCILoCore}{\tbd{hlRankTauCILoCore}}
\providecommand{\hlRankTauCILoCsTwelve}{\tbd{hlRankTauCILoCsTwelve}}
\providecommand{\hlRankTauCILoDfc}{\tbd{hlRankTauCILoDfc}}
\providecommand{\hlRankTauCILoEnva}{\tbd{hlRankTauCILoEnva}}
\providecommand{\hlRankTauCILoKuro}{\tbd{hlRankTauCILoKuro}}
\providecommand{\hlRankTauCILoOem}{\tbd{hlRankTauCILoOem}}
\providecommand{\hlRankTauCILoPooled}{\tbd{hlRankTauCILoPooled}}
\providecommand{\hlRankTauCILoSnTwo}{\tbd{hlRankTauCILoSnTwo}}
\providecommand{\hlRankTauCILoburn}{\tbd{hlRankTauCILoburn}}
\providecommand{\hlRankTauCILoflair}{\tbd{hlRankTauCILoflair}}
\providecommand{\hlRankTauChes}{\tbd{hlRankTauChes}}
\providecommand{\hlRankTauCore}{\tbd{hlRankTauCore}}
\providecommand{\hlRankTauCsTwelve}{\tbd{hlRankTauCsTwelve}}
\providecommand{\hlRankTauDfc}{\tbd{hlRankTauDfc}}
\providecommand{\hlRankTauEnva}{\tbd{hlRankTauEnva}}
\providecommand{\hlRankTauKuro}{\tbd{hlRankTauKuro}}
\providecommand{\hlRankTauOem}{\tbd{hlRankTauOem}}
\providecommand{\hlRankTauPooled}{\tbd{hlRankTauPooled}}
\providecommand{\hlRankTauSnTwo}{\tbd{hlRankTauSnTwo}}
\providecommand{\hlRankTauburn}{\tbd{hlRankTauburn}}
\providecommand{\hlRankTauflair}{\tbd{hlRankTauflair}}
\providecommand{\hlRealBaselineChes}{\tbd{hlRealBaselineChes}}
\providecommand{\hlRealBaselineCsTwelve}{\tbd{hlRealBaselineCsTwelve}}
\providecommand{\hlRealBaselineDfc}{\tbd{hlRealBaselineDfc}}
\providecommand{\hlRealBaselineEnva}{\tbd{hlRealBaselineEnva}}
\providecommand{\hlRealBaselineKuro}{\tbd{hlRealBaselineKuro}}
\providecommand{\hlRealDropChes}{\tbd{hlRealDropChes}}
\providecommand{\hlRealDropChesCIHi}{\tbd{hlRealDropChesCIHi}}
\providecommand{\hlRealDropChesCILo}{\tbd{hlRealDropChesCILo}}
\providecommand{\hlRealDropChesN}{\tbd{hlRealDropChesN}}
\providecommand{\hlRealDropCsTwelve}{\tbd{hlRealDropCsTwelve}}
\providecommand{\hlRealDropCsTwelveCIHi}{\tbd{hlRealDropCsTwelveCIHi}}
\providecommand{\hlRealDropCsTwelveCILo}{\tbd{hlRealDropCsTwelveCILo}}
\providecommand{\hlRealDropCsTwelveN}{\tbd{hlRealDropCsTwelveN}}
\providecommand{\hlRealDropDOFAChes}{\tbd{hlRealDropDOFAChes}}
\providecommand{\hlRealDropDOFAChesCIHi}{\tbd{hlRealDropDOFAChesCIHi}}
\providecommand{\hlRealDropDOFAChesCILo}{\tbd{hlRealDropDOFAChesCILo}}
\providecommand{\hlRealDropDOFACsTwelve}{\tbd{hlRealDropDOFACsTwelve}}
\providecommand{\hlRealDropDOFACsTwelveCIHi}{\tbd{hlRealDropDOFACsTwelveCIHi}}
\providecommand{\hlRealDropDOFACsTwelveCILo}{\tbd{hlRealDropDOFACsTwelveCILo}}
\providecommand{\hlRealDropDOFADfc}{\tbd{hlRealDropDOFADfc}}
\providecommand{\hlRealDropDOFADfcCIHi}{\tbd{hlRealDropDOFADfcCIHi}}
\providecommand{\hlRealDropDOFADfcCILo}{\tbd{hlRealDropDOFADfcCILo}}
\providecommand{\hlRealDropDOFAEnva}{\tbd{hlRealDropDOFAEnva}}
\providecommand{\hlRealDropDOFAEnvaCIHi}{\tbd{hlRealDropDOFAEnvaCIHi}}
\providecommand{\hlRealDropDOFAEnvaCILo}{\tbd{hlRealDropDOFAEnvaCILo}}
\providecommand{\hlRealDropDOFAKuro}{\tbd{hlRealDropDOFAKuro}}
\providecommand{\hlRealDropDOFAKuroCIHi}{\tbd{hlRealDropDOFAKuroCIHi}}
\providecommand{\hlRealDropDOFAKuroCILo}{\tbd{hlRealDropDOFAKuroCILo}}
\providecommand{\hlRealDropDfc}{\tbd{hlRealDropDfc}}
\providecommand{\hlRealDropDfcCIHi}{\tbd{hlRealDropDfcCIHi}}
\providecommand{\hlRealDropDfcCILo}{\tbd{hlRealDropDfcCILo}}
\providecommand{\hlRealDropDfcN}{\tbd{hlRealDropDfcN}}
\providecommand{\hlRealDropEnva}{\tbd{hlRealDropEnva}}
\providecommand{\hlRealDropEnvaCIHi}{\tbd{hlRealDropEnvaCIHi}}
\providecommand{\hlRealDropEnvaCILo}{\tbd{hlRealDropEnvaCILo}}
\providecommand{\hlRealDropEnvaN}{\tbd{hlRealDropEnvaN}}
\providecommand{\hlRealDropKuro}{\tbd{hlRealDropKuro}}
\providecommand{\hlRealDropKuroCIHi}{\tbd{hlRealDropKuroCIHi}}
\providecommand{\hlRealDropKuroCILo}{\tbd{hlRealDropKuroCILo}}
\providecommand{\hlRealDropKuroN}{\tbd{hlRealDropKuroN}}
\providecommand{\hlRealDropLVDChes}{\tbd{hlRealDropLVDChes}}
\providecommand{\hlRealDropLVDChesCIHi}{\tbd{hlRealDropLVDChesCIHi}}
\providecommand{\hlRealDropLVDChesCILo}{\tbd{hlRealDropLVDChesCILo}}
\providecommand{\hlRealDropLVDCsTwelve}{\tbd{hlRealDropLVDCsTwelve}}
\providecommand{\hlRealDropLVDCsTwelveCIHi}{\tbd{hlRealDropLVDCsTwelveCIHi}}
\providecommand{\hlRealDropLVDCsTwelveCILo}{\tbd{hlRealDropLVDCsTwelveCILo}}
\providecommand{\hlRealDropLVDDfc}{\tbd{hlRealDropLVDDfc}}
\providecommand{\hlRealDropLVDDfcCIHi}{\tbd{hlRealDropLVDDfcCIHi}}
\providecommand{\hlRealDropLVDDfcCILo}{\tbd{hlRealDropLVDDfcCILo}}
\providecommand{\hlRealDropLVDEnva}{\tbd{hlRealDropLVDEnva}}
\providecommand{\hlRealDropLVDEnvaCIHi}{\tbd{hlRealDropLVDEnvaCIHi}}
\providecommand{\hlRealDropLVDEnvaCILo}{\tbd{hlRealDropLVDEnvaCILo}}
\providecommand{\hlRealDropLVDKuro}{\tbd{hlRealDropLVDKuro}}
\providecommand{\hlRealDropLVDKuroCIHi}{\tbd{hlRealDropLVDKuroCIHi}}
\providecommand{\hlRealDropLVDKuroCILo}{\tbd{hlRealDropLVDKuroCILo}}
\providecommand{\hlRealDropRNChes}{\tbd{hlRealDropRNChes}}
\providecommand{\hlRealDropRNChesCIHi}{\tbd{hlRealDropRNChesCIHi}}
\providecommand{\hlRealDropRNChesCILo}{\tbd{hlRealDropRNChesCILo}}
\providecommand{\hlRealDropRNCsTwelve}{\tbd{hlRealDropRNCsTwelve}}
\providecommand{\hlRealDropRNCsTwelveCIHi}{\tbd{hlRealDropRNCsTwelveCIHi}}
\providecommand{\hlRealDropRNCsTwelveCILo}{\tbd{hlRealDropRNCsTwelveCILo}}
\providecommand{\hlRealDropRNDfc}{\tbd{hlRealDropRNDfc}}
\providecommand{\hlRealDropRNDfcCIHi}{\tbd{hlRealDropRNDfcCIHi}}
\providecommand{\hlRealDropRNDfcCILo}{\tbd{hlRealDropRNDfcCILo}}
\providecommand{\hlRealDropRNEnva}{\tbd{hlRealDropRNEnva}}
\providecommand{\hlRealDropRNEnvaCIHi}{\tbd{hlRealDropRNEnvaCIHi}}
\providecommand{\hlRealDropRNEnvaCILo}{\tbd{hlRealDropRNEnvaCILo}}
\providecommand{\hlRealDropRNKuro}{\tbd{hlRealDropRNKuro}}
\providecommand{\hlRealDropRNKuroCIHi}{\tbd{hlRealDropRNKuroCIHi}}
\providecommand{\hlRealDropRNKuroCILo}{\tbd{hlRealDropRNKuroCILo}}
\providecommand{\hlRealDropSATChes}{\tbd{hlRealDropSATChes}}
\providecommand{\hlRealDropSATChesCIHi}{\tbd{hlRealDropSATChesCIHi}}
\providecommand{\hlRealDropSATChesCILo}{\tbd{hlRealDropSATChesCILo}}
\providecommand{\hlRealDropSATCsTwelve}{\tbd{hlRealDropSATCsTwelve}}
\providecommand{\hlRealDropSATCsTwelveCIHi}{\tbd{hlRealDropSATCsTwelveCIHi}}
\providecommand{\hlRealDropSATCsTwelveCILo}{\tbd{hlRealDropSATCsTwelveCILo}}
\providecommand{\hlRealDropSATDfc}{\tbd{hlRealDropSATDfc}}
\providecommand{\hlRealDropSATDfcCIHi}{\tbd{hlRealDropSATDfcCIHi}}
\providecommand{\hlRealDropSATDfcCILo}{\tbd{hlRealDropSATDfcCILo}}
\providecommand{\hlRealDropSATEnva}{\tbd{hlRealDropSATEnva}}
\providecommand{\hlRealDropSATEnvaCIHi}{\tbd{hlRealDropSATEnvaCIHi}}
\providecommand{\hlRealDropSATEnvaCILo}{\tbd{hlRealDropSATEnvaCILo}}
\providecommand{\hlRealDropSATKuro}{\tbd{hlRealDropSATKuro}}
\providecommand{\hlRealDropSATKuroCIHi}{\tbd{hlRealDropSATKuroCIHi}}
\providecommand{\hlRealDropSATKuroCILo}{\tbd{hlRealDropSATKuroCILo}}
\providecommand{\hlRealDropTMChes}{\tbd{hlRealDropTMChes}}
\providecommand{\hlRealDropTMChesCIHi}{\tbd{hlRealDropTMChesCIHi}}
\providecommand{\hlRealDropTMChesCILo}{\tbd{hlRealDropTMChesCILo}}
\providecommand{\hlRealDropTMCsTwelve}{\tbd{hlRealDropTMCsTwelve}}
\providecommand{\hlRealDropTMCsTwelveCIHi}{\tbd{hlRealDropTMCsTwelveCIHi}}
\providecommand{\hlRealDropTMCsTwelveCILo}{\tbd{hlRealDropTMCsTwelveCILo}}
\providecommand{\hlRealDropTMDfc}{\tbd{hlRealDropTMDfc}}
\providecommand{\hlRealDropTMDfcCIHi}{\tbd{hlRealDropTMDfcCIHi}}
\providecommand{\hlRealDropTMDfcCILo}{\tbd{hlRealDropTMDfcCILo}}
\providecommand{\hlRealDropTMEnva}{\tbd{hlRealDropTMEnva}}
\providecommand{\hlRealDropTMEnvaCIHi}{\tbd{hlRealDropTMEnvaCIHi}}
\providecommand{\hlRealDropTMEnvaCILo}{\tbd{hlRealDropTMEnvaCILo}}
\providecommand{\hlRealDropTMKuro}{\tbd{hlRealDropTMKuro}}
\providecommand{\hlRealDropTMKuroCIHi}{\tbd{hlRealDropTMKuroCIHi}}
\providecommand{\hlRealDropTMKuroCILo}{\tbd{hlRealDropTMKuroCILo}}
\providecommand{\hlRealInterpBoundaryChesCIHi}{\tbd{hlRealInterpBoundaryChesCIHi}}
\providecommand{\hlRealInterpBoundaryChesCILo}{\tbd{hlRealInterpBoundaryChesCILo}}
\providecommand{\hlRealInterpBoundaryChesEst}{\tbd{hlRealInterpBoundaryChesEst}}
\providecommand{\hlRealInterpBoundaryChesSim}{\tbd{hlRealInterpBoundaryChesSim}}
\providecommand{\hlRealInterpBoundaryChesVerdict}{\tbd{hlRealInterpBoundaryChesVerdict}}
\providecommand{\hlRealInterpBoundaryCsTwelveCIHi}{\tbd{hlRealInterpBoundaryCsTwelveCIHi}}
\providecommand{\hlRealInterpBoundaryCsTwelveCILo}{\tbd{hlRealInterpBoundaryCsTwelveCILo}}
\providecommand{\hlRealInterpBoundaryCsTwelveEst}{\tbd{hlRealInterpBoundaryCsTwelveEst}}
\providecommand{\hlRealInterpBoundaryCsTwelveSim}{\tbd{hlRealInterpBoundaryCsTwelveSim}}
\providecommand{\hlRealInterpBoundaryCsTwelveVerdict}{\tbd{hlRealInterpBoundaryCsTwelveVerdict}}
\providecommand{\hlRealInterpBoundaryDfcCIHi}{\tbd{hlRealInterpBoundaryDfcCIHi}}
\providecommand{\hlRealInterpBoundaryDfcCILo}{\tbd{hlRealInterpBoundaryDfcCILo}}
\providecommand{\hlRealInterpBoundaryDfcEst}{\tbd{hlRealInterpBoundaryDfcEst}}
\providecommand{\hlRealInterpBoundaryDfcSim}{\tbd{hlRealInterpBoundaryDfcSim}}
\providecommand{\hlRealInterpBoundaryDfcVerdict}{\tbd{hlRealInterpBoundaryDfcVerdict}}
\providecommand{\hlRealInterpBoundaryEnvaCIHi}{\tbd{hlRealInterpBoundaryEnvaCIHi}}
\providecommand{\hlRealInterpBoundaryEnvaCILo}{\tbd{hlRealInterpBoundaryEnvaCILo}}
\providecommand{\hlRealInterpBoundaryEnvaEst}{\tbd{hlRealInterpBoundaryEnvaEst}}
\providecommand{\hlRealInterpBoundaryEnvaSim}{\tbd{hlRealInterpBoundaryEnvaSim}}
\providecommand{\hlRealInterpBoundaryEnvaVerdict}{\tbd{hlRealInterpBoundaryEnvaVerdict}}
\providecommand{\hlRealInterpBoundaryKuroCIHi}{\tbd{hlRealInterpBoundaryKuroCIHi}}
\providecommand{\hlRealInterpBoundaryKuroCILo}{\tbd{hlRealInterpBoundaryKuroCILo}}
\providecommand{\hlRealInterpBoundaryKuroEst}{\tbd{hlRealInterpBoundaryKuroEst}}
\providecommand{\hlRealInterpBoundaryKuroSim}{\tbd{hlRealInterpBoundaryKuroSim}}
\providecommand{\hlRealInterpBoundaryKuroVerdict}{\tbd{hlRealInterpBoundaryKuroVerdict}}
\providecommand{\hlRealInterpChesCIHi}{\tbd{hlRealInterpChesCIHi}}
\providecommand{\hlRealInterpChesCILo}{\tbd{hlRealInterpChesCILo}}
\providecommand{\hlRealInterpChesEst}{\tbd{hlRealInterpChesEst}}
\providecommand{\hlRealInterpChesFlag}{\tbd{hlRealInterpChesFlag}}
\providecommand{\hlRealInterpChesGap}{\tbd{hlRealInterpChesGap}}
\providecommand{\hlRealInterpChesLabelMiou}{\tbd{hlRealInterpChesLabelMiou}}
\providecommand{\hlRealInterpChesMde}{\tbd{hlRealInterpChesMde}}
\providecommand{\hlRealInterpChesN}{\tbd{hlRealInterpChesN}}
\providecommand{\hlRealInterpChesPHolm}{\tbd{hlRealInterpChesPHolm}}
\providecommand{\hlRealInterpChesSim}{\tbd{hlRealInterpChesSim}}
\providecommand{\hlRealInterpChesTostCIHi}{\tbd{hlRealInterpChesTostCIHi}}
\providecommand{\hlRealInterpChesTostCILo}{\tbd{hlRealInterpChesTostCILo}}
\providecommand{\hlRealInterpChesVerdict}{\tbd{hlRealInterpChesVerdict}}
\providecommand{\hlRealInterpCoarseChesCIHi}{\tbd{hlRealInterpCoarseChesCIHi}}
\providecommand{\hlRealInterpCoarseChesCILo}{\tbd{hlRealInterpCoarseChesCILo}}
\providecommand{\hlRealInterpCoarseChesEst}{\tbd{hlRealInterpCoarseChesEst}}
\providecommand{\hlRealInterpCoarseChesSim}{\tbd{hlRealInterpCoarseChesSim}}
\providecommand{\hlRealInterpCoarseChesVerdict}{\tbd{hlRealInterpCoarseChesVerdict}}
\providecommand{\hlRealInterpCoarseCsTwelveCIHi}{\tbd{hlRealInterpCoarseCsTwelveCIHi}}
\providecommand{\hlRealInterpCoarseCsTwelveCILo}{\tbd{hlRealInterpCoarseCsTwelveCILo}}
\providecommand{\hlRealInterpCoarseCsTwelveEst}{\tbd{hlRealInterpCoarseCsTwelveEst}}
\providecommand{\hlRealInterpCoarseCsTwelveSim}{\tbd{hlRealInterpCoarseCsTwelveSim}}
\providecommand{\hlRealInterpCoarseCsTwelveVerdict}{\tbd{hlRealInterpCoarseCsTwelveVerdict}}
\providecommand{\hlRealInterpCoarseDfcCIHi}{\tbd{hlRealInterpCoarseDfcCIHi}}
\providecommand{\hlRealInterpCoarseDfcCILo}{\tbd{hlRealInterpCoarseDfcCILo}}
\providecommand{\hlRealInterpCoarseDfcEst}{\tbd{hlRealInterpCoarseDfcEst}}
\providecommand{\hlRealInterpCoarseDfcSim}{\tbd{hlRealInterpCoarseDfcSim}}
\providecommand{\hlRealInterpCoarseDfcVerdict}{\tbd{hlRealInterpCoarseDfcVerdict}}
\providecommand{\hlRealInterpCoarseEnvaCIHi}{\tbd{hlRealInterpCoarseEnvaCIHi}}
\providecommand{\hlRealInterpCoarseEnvaCILo}{\tbd{hlRealInterpCoarseEnvaCILo}}
\providecommand{\hlRealInterpCoarseEnvaEst}{\tbd{hlRealInterpCoarseEnvaEst}}
\providecommand{\hlRealInterpCoarseEnvaSim}{\tbd{hlRealInterpCoarseEnvaSim}}
\providecommand{\hlRealInterpCoarseEnvaVerdict}{\tbd{hlRealInterpCoarseEnvaVerdict}}
\providecommand{\hlRealInterpCoarseKuroCIHi}{\tbd{hlRealInterpCoarseKuroCIHi}}
\providecommand{\hlRealInterpCoarseKuroCILo}{\tbd{hlRealInterpCoarseKuroCILo}}
\providecommand{\hlRealInterpCoarseKuroEst}{\tbd{hlRealInterpCoarseKuroEst}}
\providecommand{\hlRealInterpCoarseKuroSim}{\tbd{hlRealInterpCoarseKuroSim}}
\providecommand{\hlRealInterpCoarseKuroVerdict}{\tbd{hlRealInterpCoarseKuroVerdict}}
\providecommand{\hlRealInterpCsTwelveCIHi}{\tbd{hlRealInterpCsTwelveCIHi}}
\providecommand{\hlRealInterpCsTwelveCILo}{\tbd{hlRealInterpCsTwelveCILo}}
\providecommand{\hlRealInterpCsTwelveEst}{\tbd{hlRealInterpCsTwelveEst}}
\providecommand{\hlRealInterpCsTwelveFlag}{\tbd{hlRealInterpCsTwelveFlag}}
\providecommand{\hlRealInterpCsTwelveGap}{\tbd{hlRealInterpCsTwelveGap}}
\providecommand{\hlRealInterpCsTwelveLabelMiou}{\tbd{hlRealInterpCsTwelveLabelMiou}}
\providecommand{\hlRealInterpCsTwelveMde}{\tbd{hlRealInterpCsTwelveMde}}
\providecommand{\hlRealInterpCsTwelveN}{\tbd{hlRealInterpCsTwelveN}}
\providecommand{\hlRealInterpCsTwelvePHolm}{\tbd{hlRealInterpCsTwelvePHolm}}
\providecommand{\hlRealInterpCsTwelveSim}{\tbd{hlRealInterpCsTwelveSim}}
\providecommand{\hlRealInterpCsTwelveTostCIHi}{\tbd{hlRealInterpCsTwelveTostCIHi}}
\providecommand{\hlRealInterpCsTwelveTostCILo}{\tbd{hlRealInterpCsTwelveTostCILo}}
\providecommand{\hlRealInterpCsTwelveVerdict}{\tbd{hlRealInterpCsTwelveVerdict}}
\providecommand{\hlRealInterpDfcCIHi}{\tbd{hlRealInterpDfcCIHi}}
\providecommand{\hlRealInterpDfcCILo}{\tbd{hlRealInterpDfcCILo}}
\providecommand{\hlRealInterpDfcEst}{\tbd{hlRealInterpDfcEst}}
\providecommand{\hlRealInterpDfcFlag}{\tbd{hlRealInterpDfcFlag}}
\providecommand{\hlRealInterpDfcGap}{\tbd{hlRealInterpDfcGap}}
\providecommand{\hlRealInterpDfcLabelMiou}{\tbd{hlRealInterpDfcLabelMiou}}
\providecommand{\hlRealInterpDfcMde}{\tbd{hlRealInterpDfcMde}}
\providecommand{\hlRealInterpDfcN}{\tbd{hlRealInterpDfcN}}
\providecommand{\hlRealInterpDfcPHolm}{\tbd{hlRealInterpDfcPHolm}}
\providecommand{\hlRealInterpDfcSim}{\tbd{hlRealInterpDfcSim}}
\providecommand{\hlRealInterpDfcTostCIHi}{\tbd{hlRealInterpDfcTostCIHi}}
\providecommand{\hlRealInterpDfcTostCILo}{\tbd{hlRealInterpDfcTostCILo}}
\providecommand{\hlRealInterpDfcVerdict}{\tbd{hlRealInterpDfcVerdict}}
\providecommand{\hlRealInterpEnvaCIHi}{\tbd{hlRealInterpEnvaCIHi}}
\providecommand{\hlRealInterpEnvaCILo}{\tbd{hlRealInterpEnvaCILo}}
\providecommand{\hlRealInterpEnvaEst}{\tbd{hlRealInterpEnvaEst}}
\providecommand{\hlRealInterpEnvaFlag}{\tbd{hlRealInterpEnvaFlag}}
\providecommand{\hlRealInterpEnvaGap}{\tbd{hlRealInterpEnvaGap}}
\providecommand{\hlRealInterpEnvaLabelMiou}{\tbd{hlRealInterpEnvaLabelMiou}}
\providecommand{\hlRealInterpEnvaMde}{\tbd{hlRealInterpEnvaMde}}
\providecommand{\hlRealInterpEnvaN}{\tbd{hlRealInterpEnvaN}}
\providecommand{\hlRealInterpEnvaPHolm}{\tbd{hlRealInterpEnvaPHolm}}
\providecommand{\hlRealInterpEnvaSim}{\tbd{hlRealInterpEnvaSim}}
\providecommand{\hlRealInterpEnvaTostCIHi}{\tbd{hlRealInterpEnvaTostCIHi}}
\providecommand{\hlRealInterpEnvaTostCILo}{\tbd{hlRealInterpEnvaTostCILo}}
\providecommand{\hlRealInterpEnvaVerdict}{\tbd{hlRealInterpEnvaVerdict}}
\providecommand{\hlRealInterpKuroCIHi}{\tbd{hlRealInterpKuroCIHi}}
\providecommand{\hlRealInterpKuroCILo}{\tbd{hlRealInterpKuroCILo}}
\providecommand{\hlRealInterpKuroEst}{\tbd{hlRealInterpKuroEst}}
\providecommand{\hlRealInterpKuroFlag}{\tbd{hlRealInterpKuroFlag}}
\providecommand{\hlRealInterpKuroGap}{\tbd{hlRealInterpKuroGap}}
\providecommand{\hlRealInterpKuroLabelMiou}{\tbd{hlRealInterpKuroLabelMiou}}
\providecommand{\hlRealInterpKuroMde}{\tbd{hlRealInterpKuroMde}}
\providecommand{\hlRealInterpKuroN}{\tbd{hlRealInterpKuroN}}
\providecommand{\hlRealInterpKuroPHolm}{\tbd{hlRealInterpKuroPHolm}}
\providecommand{\hlRealInterpKuroSim}{\tbd{hlRealInterpKuroSim}}
\providecommand{\hlRealInterpKuroTostCIHi}{\tbd{hlRealInterpKuroTostCIHi}}
\providecommand{\hlRealInterpKuroTostCILo}{\tbd{hlRealInterpKuroTostCILo}}
\providecommand{\hlRealInterpKuroVerdict}{\tbd{hlRealInterpKuroVerdict}}
\providecommand{\hlRealInterpMeanChesCIHi}{\tbd{hlRealInterpMeanChesCIHi}}
\providecommand{\hlRealInterpMeanChesCILo}{\tbd{hlRealInterpMeanChesCILo}}
\providecommand{\hlRealInterpMeanChesEst}{\tbd{hlRealInterpMeanChesEst}}
\providecommand{\hlRealInterpMeanChesSim}{\tbd{hlRealInterpMeanChesSim}}
\providecommand{\hlRealInterpMeanChesVerdict}{\tbd{hlRealInterpMeanChesVerdict}}
\providecommand{\hlRealInterpMeanCsTwelveCIHi}{\tbd{hlRealInterpMeanCsTwelveCIHi}}
\providecommand{\hlRealInterpMeanCsTwelveCILo}{\tbd{hlRealInterpMeanCsTwelveCILo}}
\providecommand{\hlRealInterpMeanCsTwelveEst}{\tbd{hlRealInterpMeanCsTwelveEst}}
\providecommand{\hlRealInterpMeanCsTwelveSim}{\tbd{hlRealInterpMeanCsTwelveSim}}
\providecommand{\hlRealInterpMeanCsTwelveVerdict}{\tbd{hlRealInterpMeanCsTwelveVerdict}}
\providecommand{\hlRealInterpMeanDfcCIHi}{\tbd{hlRealInterpMeanDfcCIHi}}
\providecommand{\hlRealInterpMeanDfcCILo}{\tbd{hlRealInterpMeanDfcCILo}}
\providecommand{\hlRealInterpMeanDfcEst}{\tbd{hlRealInterpMeanDfcEst}}
\providecommand{\hlRealInterpMeanDfcSim}{\tbd{hlRealInterpMeanDfcSim}}
\providecommand{\hlRealInterpMeanDfcVerdict}{\tbd{hlRealInterpMeanDfcVerdict}}
\providecommand{\hlRealInterpMeanEnvaCIHi}{\tbd{hlRealInterpMeanEnvaCIHi}}
\providecommand{\hlRealInterpMeanEnvaCILo}{\tbd{hlRealInterpMeanEnvaCILo}}
\providecommand{\hlRealInterpMeanEnvaEst}{\tbd{hlRealInterpMeanEnvaEst}}
\providecommand{\hlRealInterpMeanEnvaSim}{\tbd{hlRealInterpMeanEnvaSim}}
\providecommand{\hlRealInterpMeanEnvaVerdict}{\tbd{hlRealInterpMeanEnvaVerdict}}
\providecommand{\hlRealInterpMeanKuroCIHi}{\tbd{hlRealInterpMeanKuroCIHi}}
\providecommand{\hlRealInterpMeanKuroCILo}{\tbd{hlRealInterpMeanKuroCILo}}
\providecommand{\hlRealInterpMeanKuroEst}{\tbd{hlRealInterpMeanKuroEst}}
\providecommand{\hlRealInterpMeanKuroSim}{\tbd{hlRealInterpMeanKuroSim}}
\providecommand{\hlRealInterpMeanKuroVerdict}{\tbd{hlRealInterpMeanKuroVerdict}}
\providecommand{\hlRealInterpOmissionChesCIHi}{\tbd{hlRealInterpOmissionChesCIHi}}
\providecommand{\hlRealInterpOmissionChesCILo}{\tbd{hlRealInterpOmissionChesCILo}}
\providecommand{\hlRealInterpOmissionChesEst}{\tbd{hlRealInterpOmissionChesEst}}
\providecommand{\hlRealInterpOmissionChesSim}{\tbd{hlRealInterpOmissionChesSim}}
\providecommand{\hlRealInterpOmissionChesVerdict}{\tbd{hlRealInterpOmissionChesVerdict}}
\providecommand{\hlRealInterpOmissionCsTwelveCIHi}{\tbd{hlRealInterpOmissionCsTwelveCIHi}}
\providecommand{\hlRealInterpOmissionCsTwelveCILo}{\tbd{hlRealInterpOmissionCsTwelveCILo}}
\providecommand{\hlRealInterpOmissionCsTwelveEst}{\tbd{hlRealInterpOmissionCsTwelveEst}}
\providecommand{\hlRealInterpOmissionCsTwelveSim}{\tbd{hlRealInterpOmissionCsTwelveSim}}
\providecommand{\hlRealInterpOmissionCsTwelveVerdict}{\tbd{hlRealInterpOmissionCsTwelveVerdict}}
\providecommand{\hlRealInterpOmissionDfcCIHi}{\tbd{hlRealInterpOmissionDfcCIHi}}
\providecommand{\hlRealInterpOmissionDfcCILo}{\tbd{hlRealInterpOmissionDfcCILo}}
\providecommand{\hlRealInterpOmissionDfcEst}{\tbd{hlRealInterpOmissionDfcEst}}
\providecommand{\hlRealInterpOmissionDfcSim}{\tbd{hlRealInterpOmissionDfcSim}}
\providecommand{\hlRealInterpOmissionDfcVerdict}{\tbd{hlRealInterpOmissionDfcVerdict}}
\providecommand{\hlRealInterpOmissionEnvaCIHi}{\tbd{hlRealInterpOmissionEnvaCIHi}}
\providecommand{\hlRealInterpOmissionEnvaCILo}{\tbd{hlRealInterpOmissionEnvaCILo}}
\providecommand{\hlRealInterpOmissionEnvaEst}{\tbd{hlRealInterpOmissionEnvaEst}}
\providecommand{\hlRealInterpOmissionEnvaSim}{\tbd{hlRealInterpOmissionEnvaSim}}
\providecommand{\hlRealInterpOmissionEnvaVerdict}{\tbd{hlRealInterpOmissionEnvaVerdict}}
\providecommand{\hlRealInterpOmissionKuroCIHi}{\tbd{hlRealInterpOmissionKuroCIHi}}
\providecommand{\hlRealInterpOmissionKuroCILo}{\tbd{hlRealInterpOmissionKuroCILo}}
\providecommand{\hlRealInterpOmissionKuroEst}{\tbd{hlRealInterpOmissionKuroEst}}
\providecommand{\hlRealInterpOmissionKuroSim}{\tbd{hlRealInterpOmissionKuroSim}}
\providecommand{\hlRealInterpOmissionKuroVerdict}{\tbd{hlRealInterpOmissionKuroVerdict}}
\providecommand{\hlRealInterpShiftChesCIHi}{\tbd{hlRealInterpShiftChesCIHi}}
\providecommand{\hlRealInterpShiftChesCILo}{\tbd{hlRealInterpShiftChesCILo}}
\providecommand{\hlRealInterpShiftChesEst}{\tbd{hlRealInterpShiftChesEst}}
\providecommand{\hlRealInterpShiftChesSim}{\tbd{hlRealInterpShiftChesSim}}
\providecommand{\hlRealInterpShiftChesVerdict}{\tbd{hlRealInterpShiftChesVerdict}}
\providecommand{\hlRealInterpShiftCsTwelveCIHi}{\tbd{hlRealInterpShiftCsTwelveCIHi}}
\providecommand{\hlRealInterpShiftCsTwelveCILo}{\tbd{hlRealInterpShiftCsTwelveCILo}}
\providecommand{\hlRealInterpShiftCsTwelveEst}{\tbd{hlRealInterpShiftCsTwelveEst}}
\providecommand{\hlRealInterpShiftCsTwelveSim}{\tbd{hlRealInterpShiftCsTwelveSim}}
\providecommand{\hlRealInterpShiftCsTwelveVerdict}{\tbd{hlRealInterpShiftCsTwelveVerdict}}
\providecommand{\hlRealInterpShiftDfcCIHi}{\tbd{hlRealInterpShiftDfcCIHi}}
\providecommand{\hlRealInterpShiftDfcCILo}{\tbd{hlRealInterpShiftDfcCILo}}
\providecommand{\hlRealInterpShiftDfcEst}{\tbd{hlRealInterpShiftDfcEst}}
\providecommand{\hlRealInterpShiftDfcSim}{\tbd{hlRealInterpShiftDfcSim}}
\providecommand{\hlRealInterpShiftDfcVerdict}{\tbd{hlRealInterpShiftDfcVerdict}}
\providecommand{\hlRealInterpShiftEnvaCIHi}{\tbd{hlRealInterpShiftEnvaCIHi}}
\providecommand{\hlRealInterpShiftEnvaCILo}{\tbd{hlRealInterpShiftEnvaCILo}}
\providecommand{\hlRealInterpShiftEnvaEst}{\tbd{hlRealInterpShiftEnvaEst}}
\providecommand{\hlRealInterpShiftEnvaSim}{\tbd{hlRealInterpShiftEnvaSim}}
\providecommand{\hlRealInterpShiftEnvaVerdict}{\tbd{hlRealInterpShiftEnvaVerdict}}
\providecommand{\hlRealInterpShiftKuroCIHi}{\tbd{hlRealInterpShiftKuroCIHi}}
\providecommand{\hlRealInterpShiftKuroCILo}{\tbd{hlRealInterpShiftKuroCILo}}
\providecommand{\hlRealInterpShiftKuroEst}{\tbd{hlRealInterpShiftKuroEst}}
\providecommand{\hlRealInterpShiftKuroSim}{\tbd{hlRealInterpShiftKuroSim}}
\providecommand{\hlRealInterpShiftKuroVerdict}{\tbd{hlRealInterpShiftKuroVerdict}}
\providecommand{\hlRealLmBoundaryKuroCIHi}{\tbd{hlRealLmBoundaryKuroCIHi}}
\providecommand{\hlRealLmBoundaryKuroCILo}{\tbd{hlRealLmBoundaryKuroCILo}}
\providecommand{\hlRealLmBoundaryKuroEst}{\tbd{hlRealLmBoundaryKuroEst}}
\providecommand{\hlRealLmBoundaryKuroLabelMiou}{\tbd{hlRealLmBoundaryKuroLabelMiou}}
\providecommand{\hlRealLmBoundaryKuroLabelMiouHi}{\tbd{hlRealLmBoundaryKuroLabelMiouHi}}
\providecommand{\hlRealLmBoundaryKuroLabelMiouLo}{\tbd{hlRealLmBoundaryKuroLabelMiouLo}}
\providecommand{\hlRealLmBoundaryKuroMde}{\tbd{hlRealLmBoundaryKuroMde}}
\providecommand{\hlRealLmBoundaryKuroN}{\tbd{hlRealLmBoundaryKuroN}}
\providecommand{\hlRealLmBoundaryKuroReal}{\tbd{hlRealLmBoundaryKuroReal}}
\providecommand{\hlRealLmBoundaryKuroRealLabelMiou}{\tbd{hlRealLmBoundaryKuroRealLabelMiou}}
\providecommand{\hlRealLmBoundaryKuroSim}{\tbd{hlRealLmBoundaryKuroSim}}
\providecommand{\hlRealLmBoundaryKuroTostCIHi}{\tbd{hlRealLmBoundaryKuroTostCIHi}}
\providecommand{\hlRealLmBoundaryKuroTostCILo}{\tbd{hlRealLmBoundaryKuroTostCILo}}
\providecommand{\hlRealLmBoundaryKuroType}{\tbd{hlRealLmBoundaryKuroType}}
\providecommand{\hlRealLmBoundaryKuroVerdict}{\tbd{hlRealLmBoundaryKuroVerdict}}
\providecommand{\hlRealLmChesCIHi}{\tbd{hlRealLmChesCIHi}}
\providecommand{\hlRealLmChesCILo}{\tbd{hlRealLmChesCILo}}
\providecommand{\hlRealLmChesEst}{\tbd{hlRealLmChesEst}}
\providecommand{\hlRealLmChesLabelMiou}{\tbd{hlRealLmChesLabelMiou}}
\providecommand{\hlRealLmChesLabelMiouHi}{\tbd{hlRealLmChesLabelMiouHi}}
\providecommand{\hlRealLmChesLabelMiouLo}{\tbd{hlRealLmChesLabelMiouLo}}
\providecommand{\hlRealLmChesMde}{\tbd{hlRealLmChesMde}}
\providecommand{\hlRealLmChesN}{\tbd{hlRealLmChesN}}
\providecommand{\hlRealLmChesReal}{\tbd{hlRealLmChesReal}}
\providecommand{\hlRealLmChesRealLabelMiou}{\tbd{hlRealLmChesRealLabelMiou}}
\providecommand{\hlRealLmChesSim}{\tbd{hlRealLmChesSim}}
\providecommand{\hlRealLmChesTostCIHi}{\tbd{hlRealLmChesTostCIHi}}
\providecommand{\hlRealLmChesTostCILo}{\tbd{hlRealLmChesTostCILo}}
\providecommand{\hlRealLmChesType}{\tbd{hlRealLmChesType}}
\providecommand{\hlRealLmChesVerdict}{\tbd{hlRealLmChesVerdict}}
\providecommand{\hlRealLmCsTwelveCIHi}{\tbd{hlRealLmCsTwelveCIHi}}
\providecommand{\hlRealLmCsTwelveCILo}{\tbd{hlRealLmCsTwelveCILo}}
\providecommand{\hlRealLmCsTwelveEst}{\tbd{hlRealLmCsTwelveEst}}
\providecommand{\hlRealLmCsTwelveLabelMiou}{\tbd{hlRealLmCsTwelveLabelMiou}}
\providecommand{\hlRealLmCsTwelveLabelMiouHi}{\tbd{hlRealLmCsTwelveLabelMiouHi}}
\providecommand{\hlRealLmCsTwelveLabelMiouLo}{\tbd{hlRealLmCsTwelveLabelMiouLo}}
\providecommand{\hlRealLmCsTwelveMde}{\tbd{hlRealLmCsTwelveMde}}
\providecommand{\hlRealLmCsTwelveN}{\tbd{hlRealLmCsTwelveN}}
\providecommand{\hlRealLmCsTwelveReal}{\tbd{hlRealLmCsTwelveReal}}
\providecommand{\hlRealLmCsTwelveRealLabelMiou}{\tbd{hlRealLmCsTwelveRealLabelMiou}}
\providecommand{\hlRealLmCsTwelveSim}{\tbd{hlRealLmCsTwelveSim}}
\providecommand{\hlRealLmCsTwelveTostCIHi}{\tbd{hlRealLmCsTwelveTostCIHi}}
\providecommand{\hlRealLmCsTwelveTostCILo}{\tbd{hlRealLmCsTwelveTostCILo}}
\providecommand{\hlRealLmCsTwelveType}{\tbd{hlRealLmCsTwelveType}}
\providecommand{\hlRealLmCsTwelveVerdict}{\tbd{hlRealLmCsTwelveVerdict}}
\providecommand{\hlRealLmDfcCIHi}{\tbd{hlRealLmDfcCIHi}}
\providecommand{\hlRealLmDfcCILo}{\tbd{hlRealLmDfcCILo}}
\providecommand{\hlRealLmDfcEst}{\tbd{hlRealLmDfcEst}}
\providecommand{\hlRealLmDfcLabelMiou}{\tbd{hlRealLmDfcLabelMiou}}
\providecommand{\hlRealLmDfcLabelMiouHi}{\tbd{hlRealLmDfcLabelMiouHi}}
\providecommand{\hlRealLmDfcLabelMiouLo}{\tbd{hlRealLmDfcLabelMiouLo}}
\providecommand{\hlRealLmDfcMde}{\tbd{hlRealLmDfcMde}}
\providecommand{\hlRealLmDfcN}{\tbd{hlRealLmDfcN}}
\providecommand{\hlRealLmDfcReal}{\tbd{hlRealLmDfcReal}}
\providecommand{\hlRealLmDfcRealLabelMiou}{\tbd{hlRealLmDfcRealLabelMiou}}
\providecommand{\hlRealLmDfcSim}{\tbd{hlRealLmDfcSim}}
\providecommand{\hlRealLmDfcTostCIHi}{\tbd{hlRealLmDfcTostCIHi}}
\providecommand{\hlRealLmDfcTostCILo}{\tbd{hlRealLmDfcTostCILo}}
\providecommand{\hlRealLmDfcType}{\tbd{hlRealLmDfcType}}
\providecommand{\hlRealLmDfcVerdict}{\tbd{hlRealLmDfcVerdict}}
\providecommand{\hlRealLmEnvaCIHi}{\tbd{hlRealLmEnvaCIHi}}
\providecommand{\hlRealLmEnvaCILo}{\tbd{hlRealLmEnvaCILo}}
\providecommand{\hlRealLmEnvaEst}{\tbd{hlRealLmEnvaEst}}
\providecommand{\hlRealLmEnvaLabelMiou}{\tbd{hlRealLmEnvaLabelMiou}}
\providecommand{\hlRealLmEnvaLabelMiouHi}{\tbd{hlRealLmEnvaLabelMiouHi}}
\providecommand{\hlRealLmEnvaLabelMiouLo}{\tbd{hlRealLmEnvaLabelMiouLo}}
\providecommand{\hlRealLmEnvaMde}{\tbd{hlRealLmEnvaMde}}
\providecommand{\hlRealLmEnvaN}{\tbd{hlRealLmEnvaN}}
\providecommand{\hlRealLmEnvaReal}{\tbd{hlRealLmEnvaReal}}
\providecommand{\hlRealLmEnvaRealLabelMiou}{\tbd{hlRealLmEnvaRealLabelMiou}}
\providecommand{\hlRealLmEnvaSim}{\tbd{hlRealLmEnvaSim}}
\providecommand{\hlRealLmEnvaTostCIHi}{\tbd{hlRealLmEnvaTostCIHi}}
\providecommand{\hlRealLmEnvaTostCILo}{\tbd{hlRealLmEnvaTostCILo}}
\providecommand{\hlRealLmEnvaType}{\tbd{hlRealLmEnvaType}}
\providecommand{\hlRealLmEnvaVerdict}{\tbd{hlRealLmEnvaVerdict}}
\providecommand{\hlRealLmEquiv}{\tbd{hlRealLmEquiv}}
\providecommand{\hlRealLmKuroCIHi}{\tbd{hlRealLmKuroCIHi}}
\providecommand{\hlRealLmKuroCILo}{\tbd{hlRealLmKuroCILo}}
\providecommand{\hlRealLmKuroEst}{\tbd{hlRealLmKuroEst}}
\providecommand{\hlRealLmKuroLabelMiou}{\tbd{hlRealLmKuroLabelMiou}}
\providecommand{\hlRealLmKuroLabelMiouHi}{\tbd{hlRealLmKuroLabelMiouHi}}
\providecommand{\hlRealLmKuroLabelMiouLo}{\tbd{hlRealLmKuroLabelMiouLo}}
\providecommand{\hlRealLmKuroMde}{\tbd{hlRealLmKuroMde}}
\providecommand{\hlRealLmKuroN}{\tbd{hlRealLmKuroN}}
\providecommand{\hlRealLmKuroReal}{\tbd{hlRealLmKuroReal}}
\providecommand{\hlRealLmKuroRealLabelMiou}{\tbd{hlRealLmKuroRealLabelMiou}}
\providecommand{\hlRealLmKuroSim}{\tbd{hlRealLmKuroSim}}
\providecommand{\hlRealLmKuroTostCIHi}{\tbd{hlRealLmKuroTostCIHi}}
\providecommand{\hlRealLmKuroTostCILo}{\tbd{hlRealLmKuroTostCILo}}
\providecommand{\hlRealLmKuroType}{\tbd{hlRealLmKuroType}}
\providecommand{\hlRealLmKuroVerdict}{\tbd{hlRealLmKuroVerdict}}
\providecommand{\hlRealLmRead}{\tbd{hlRealLmRead}}
\providecommand{\hlRealLmRealMore}{\tbd{hlRealLmRealMore}}
\providecommand{\hlRealLmTotal}{\tbd{hlRealLmTotal}}
\providecommand{\hlRealMatchedDropChes}{\tbd{hlRealMatchedDropChes}}
\providecommand{\hlRealMatchedDropCsTwelve}{\tbd{hlRealMatchedDropCsTwelve}}
\providecommand{\hlRealMatchedDropDfc}{\tbd{hlRealMatchedDropDfc}}
\providecommand{\hlRealMatchedDropEnva}{\tbd{hlRealMatchedDropEnva}}
\providecommand{\hlRealMatchedDropKuro}{\tbd{hlRealMatchedDropKuro}}
\providecommand{\hlRealMatchedLevelChes}{\tbd{hlRealMatchedLevelChes}}
\providecommand{\hlRealMatchedLevelCsTwelve}{\tbd{hlRealMatchedLevelCsTwelve}}
\providecommand{\hlRealMatchedLevelDfc}{\tbd{hlRealMatchedLevelDfc}}
\providecommand{\hlRealMatchedLevelEnva}{\tbd{hlRealMatchedLevelEnva}}
\providecommand{\hlRealMatchedLevelKuro}{\tbd{hlRealMatchedLevelKuro}}
\providecommand{\hlRealMatchedTypeChes}{\tbd{hlRealMatchedTypeChes}}
\providecommand{\hlRealMatchedTypeCsTwelve}{\tbd{hlRealMatchedTypeCsTwelve}}
\providecommand{\hlRealMatchedTypeDfc}{\tbd{hlRealMatchedTypeDfc}}
\providecommand{\hlRealMatchedTypeEnva}{\tbd{hlRealMatchedTypeEnva}}
\providecommand{\hlRealMatchedTypeKuro}{\tbd{hlRealMatchedTypeKuro}}
\providecommand{\hlRealSlopeburnOmission}{\tbd{hlRealSlopeburnOmission}}
\providecommand{\hlRealSlopeflairOmission}{\tbd{hlRealSlopeflairOmission}}
\providecommand{\hlRealVerdictChes}{\tbd{hlRealVerdictChes}}
\providecommand{\hlRealVerdictCsTwelve}{\tbd{hlRealVerdictCsTwelve}}
\providecommand{\hlRealVerdictDfc}{\tbd{hlRealVerdictDfc}}
\providecommand{\hlRealVerdictEnva}{\tbd{hlRealVerdictEnva}}
\providecommand{\hlRealVerdictKuro}{\tbd{hlRealVerdictKuro}}
\providecommand{\hlRealVsSynthChes}{\tbd{hlRealVsSynthChes}}
\providecommand{\hlRealVsSynthChesCIHi}{\tbd{hlRealVsSynthChesCIHi}}
\providecommand{\hlRealVsSynthChesCILo}{\tbd{hlRealVsSynthChesCILo}}
\providecommand{\hlRealVsSynthChesEst}{\tbd{hlRealVsSynthChesEst}}
\providecommand{\hlRealVsSynthChesMde}{\tbd{hlRealVsSynthChesMde}}
\providecommand{\hlRealVsSynthChesN}{\tbd{hlRealVsSynthChesN}}
\providecommand{\hlRealVsSynthChesPHolm}{\tbd{hlRealVsSynthChesPHolm}}
\providecommand{\hlRealVsSynthChesTostCIHi}{\tbd{hlRealVsSynthChesTostCIHi}}
\providecommand{\hlRealVsSynthChesTostCILo}{\tbd{hlRealVsSynthChesTostCILo}}
\providecommand{\hlRealVsSynthCsTwelve}{\tbd{hlRealVsSynthCsTwelve}}
\providecommand{\hlRealVsSynthCsTwelveCIHi}{\tbd{hlRealVsSynthCsTwelveCIHi}}
\providecommand{\hlRealVsSynthCsTwelveCILo}{\tbd{hlRealVsSynthCsTwelveCILo}}
\providecommand{\hlRealVsSynthCsTwelveEst}{\tbd{hlRealVsSynthCsTwelveEst}}
\providecommand{\hlRealVsSynthCsTwelveMde}{\tbd{hlRealVsSynthCsTwelveMde}}
\providecommand{\hlRealVsSynthCsTwelveN}{\tbd{hlRealVsSynthCsTwelveN}}
\providecommand{\hlRealVsSynthCsTwelvePHolm}{\tbd{hlRealVsSynthCsTwelvePHolm}}
\providecommand{\hlRealVsSynthCsTwelveTostCIHi}{\tbd{hlRealVsSynthCsTwelveTostCIHi}}
\providecommand{\hlRealVsSynthCsTwelveTostCILo}{\tbd{hlRealVsSynthCsTwelveTostCILo}}
\providecommand{\hlRealVsSynthDfc}{\tbd{hlRealVsSynthDfc}}
\providecommand{\hlRealVsSynthDfcCIHi}{\tbd{hlRealVsSynthDfcCIHi}}
\providecommand{\hlRealVsSynthDfcCILo}{\tbd{hlRealVsSynthDfcCILo}}
\providecommand{\hlRealVsSynthDfcEst}{\tbd{hlRealVsSynthDfcEst}}
\providecommand{\hlRealVsSynthDfcMde}{\tbd{hlRealVsSynthDfcMde}}
\providecommand{\hlRealVsSynthDfcN}{\tbd{hlRealVsSynthDfcN}}
\providecommand{\hlRealVsSynthDfcPHolm}{\tbd{hlRealVsSynthDfcPHolm}}
\providecommand{\hlRealVsSynthDfcTostCIHi}{\tbd{hlRealVsSynthDfcTostCIHi}}
\providecommand{\hlRealVsSynthDfcTostCILo}{\tbd{hlRealVsSynthDfcTostCILo}}
\providecommand{\hlRealVsSynthEnva}{\tbd{hlRealVsSynthEnva}}
\providecommand{\hlRealVsSynthEnvaCIHi}{\tbd{hlRealVsSynthEnvaCIHi}}
\providecommand{\hlRealVsSynthEnvaCILo}{\tbd{hlRealVsSynthEnvaCILo}}
\providecommand{\hlRealVsSynthEnvaEst}{\tbd{hlRealVsSynthEnvaEst}}
\providecommand{\hlRealVsSynthEnvaMde}{\tbd{hlRealVsSynthEnvaMde}}
\providecommand{\hlRealVsSynthEnvaN}{\tbd{hlRealVsSynthEnvaN}}
\providecommand{\hlRealVsSynthEnvaPHolm}{\tbd{hlRealVsSynthEnvaPHolm}}
\providecommand{\hlRealVsSynthEnvaTostCIHi}{\tbd{hlRealVsSynthEnvaTostCIHi}}
\providecommand{\hlRealVsSynthEnvaTostCILo}{\tbd{hlRealVsSynthEnvaTostCILo}}
\providecommand{\hlRealVsSynthKuro}{\tbd{hlRealVsSynthKuro}}
\providecommand{\hlRealVsSynthKuroCIHi}{\tbd{hlRealVsSynthKuroCIHi}}
\providecommand{\hlRealVsSynthKuroCILo}{\tbd{hlRealVsSynthKuroCILo}}
\providecommand{\hlRealVsSynthKuroEst}{\tbd{hlRealVsSynthKuroEst}}
\providecommand{\hlRealVsSynthKuroMde}{\tbd{hlRealVsSynthKuroMde}}
\providecommand{\hlRealVsSynthKuroN}{\tbd{hlRealVsSynthKuroN}}
\providecommand{\hlRealVsSynthKuroPHolm}{\tbd{hlRealVsSynthKuroPHolm}}
\providecommand{\hlRealVsSynthKuroTostCIHi}{\tbd{hlRealVsSynthKuroTostCIHi}}
\providecommand{\hlRealVsSynthKuroTostCILo}{\tbd{hlRealVsSynthKuroTostCILo}}
\providecommand{\hlRetDiffCIHiburn}{\tbd{hlRetDiffCIHiburn}}
\providecommand{\hlRetDiffCIHiflair}{\tbd{hlRetDiffCIHiflair}}
\providecommand{\hlRetDiffCILoburn}{\tbd{hlRetDiffCILoburn}}
\providecommand{\hlRetDiffCILoflair}{\tbd{hlRetDiffCILoflair}}
\providecommand{\hlRetDiffNburn}{\tbd{hlRetDiffNburn}}
\providecommand{\hlRetDiffNflair}{\tbd{hlRetDiffNflair}}
\providecommand{\hlRetDiffburn}{\tbd{hlRetDiffburn}}
\providecommand{\hlRetDiffflair}{\tbd{hlRetDiffflair}}
\providecommand{\hlRetDsDiffCIHiDOFA}{\tbd{hlRetDsDiffCIHiDOFA}}
\providecommand{\hlRetDsDiffCIHiLVD}{\tbd{hlRetDsDiffCIHiLVD}}
\providecommand{\hlRetDsDiffCIHiRN}{\tbd{hlRetDsDiffCIHiRN}}
\providecommand{\hlRetDsDiffCIHiSAT}{\tbd{hlRetDsDiffCIHiSAT}}
\providecommand{\hlRetDsDiffCIHiTM}{\tbd{hlRetDsDiffCIHiTM}}
\providecommand{\hlRetDsDiffCILoDOFA}{\tbd{hlRetDsDiffCILoDOFA}}
\providecommand{\hlRetDsDiffCILoLVD}{\tbd{hlRetDsDiffCILoLVD}}
\providecommand{\hlRetDsDiffCILoRN}{\tbd{hlRetDsDiffCILoRN}}
\providecommand{\hlRetDsDiffCILoSAT}{\tbd{hlRetDsDiffCILoSAT}}
\providecommand{\hlRetDsDiffCILoTM}{\tbd{hlRetDsDiffCILoTM}}
\providecommand{\hlRetDsDiffDOFA}{\tbd{hlRetDsDiffDOFA}}
\providecommand{\hlRetDsDiffLVD}{\tbd{hlRetDsDiffLVD}}
\providecommand{\hlRetDsDiffRN}{\tbd{hlRetDsDiffRN}}
\providecommand{\hlRetDsDiffSAT}{\tbd{hlRetDsDiffSAT}}
\providecommand{\hlRetDsDiffTM}{\tbd{hlRetDsDiffTM}}
\providecommand{\hlRetLVDburn}{\tbd{hlRetLVDburn}}
\providecommand{\hlRetLVDflair}{\tbd{hlRetLVDflair}}
\providecommand{\hlRetMeanDOFAburn}{\tbd{hlRetMeanDOFAburn}}
\providecommand{\hlRetMeanDOFAflair}{\tbd{hlRetMeanDOFAflair}}
\providecommand{\hlRetMeanLVDburn}{\tbd{hlRetMeanLVDburn}}
\providecommand{\hlRetMeanLVDflair}{\tbd{hlRetMeanLVDflair}}
\providecommand{\hlRetMeanRNburn}{\tbd{hlRetMeanRNburn}}
\providecommand{\hlRetMeanRNflair}{\tbd{hlRetMeanRNflair}}
\providecommand{\hlRetMeanSATburn}{\tbd{hlRetMeanSATburn}}
\providecommand{\hlRetMeanSATflair}{\tbd{hlRetMeanSATflair}}
\providecommand{\hlRetMeanTMburn}{\tbd{hlRetMeanTMburn}}
\providecommand{\hlRetMeanTMflair}{\tbd{hlRetMeanTMflair}}
\providecommand{\hlRetSATburn}{\tbd{hlRetSATburn}}
\providecommand{\hlRetSATflair}{\tbd{hlRetSATflair}}
\providecommand{\hlRunsDoneDFive}{\tbd{hlRunsDoneDFive}}
\providecommand{\hlRunsDoneDFour}{\tbd{hlRunsDoneDFour}}
\providecommand{\hlRunsDoneDOne}{\tbd{hlRunsDoneDOne}}
\providecommand{\hlRunsDoneDSeven}{\tbd{hlRunsDoneDSeven}}
\providecommand{\hlRunsDoneDSix}{\tbd{hlRunsDoneDSix}}
\providecommand{\hlRunsDoneDThree}{\tbd{hlRunsDoneDThree}}
\providecommand{\hlRunsDoneDTwo}{\tbd{hlRunsDoneDTwo}}
\providecommand{\hlRunsDoneNEight}{\tbd{hlRunsDoneNEight}}
\providecommand{\hlRunsDoneNEleven}{\tbd{hlRunsDoneNEleven}}
\providecommand{\hlRunsDoneNFifteen}{\tbd{hlRunsDoneNFifteen}}
\providecommand{\hlRunsDoneNFourteen}{\tbd{hlRunsDoneNFourteen}}
\providecommand{\hlRunsDoneNNine}{\tbd{hlRunsDoneNNine}}
\providecommand{\hlRunsDoneNSeven}{\tbd{hlRunsDoneNSeven}}
\providecommand{\hlRunsDoneNTen}{\tbd{hlRunsDoneNTen}}
\providecommand{\hlRunsDoneNThirteen}{\tbd{hlRunsDoneNThirteen}}
\providecommand{\hlRunsDoneNTwelve}{\tbd{hlRunsDoneNTwelve}}
\providecommand{\hlRunsPlannedDFive}{\tbd{hlRunsPlannedDFive}}
\providecommand{\hlRunsPlannedDFour}{\tbd{hlRunsPlannedDFour}}
\providecommand{\hlRunsPlannedDOne}{\tbd{hlRunsPlannedDOne}}
\providecommand{\hlRunsPlannedDSeven}{\tbd{hlRunsPlannedDSeven}}
\providecommand{\hlRunsPlannedDSix}{\tbd{hlRunsPlannedDSix}}
\providecommand{\hlRunsPlannedDThree}{\tbd{hlRunsPlannedDThree}}
\providecommand{\hlRunsPlannedDTwo}{\tbd{hlRunsPlannedDTwo}}
\providecommand{\hlRunsPlannedNEight}{\tbd{hlRunsPlannedNEight}}
\providecommand{\hlRunsPlannedNEleven}{\tbd{hlRunsPlannedNEleven}}
\providecommand{\hlRunsPlannedNFifteen}{\tbd{hlRunsPlannedNFifteen}}
\providecommand{\hlRunsPlannedNFourteen}{\tbd{hlRunsPlannedNFourteen}}
\providecommand{\hlRunsPlannedNNine}{\tbd{hlRunsPlannedNNine}}
\providecommand{\hlRunsPlannedNSeven}{\tbd{hlRunsPlannedNSeven}}
\providecommand{\hlRunsPlannedNTen}{\tbd{hlRunsPlannedNTen}}
\providecommand{\hlRunsPlannedNThirteen}{\tbd{hlRunsPlannedNThirteen}}
\providecommand{\hlRunsPlannedNTwelve}{\tbd{hlRunsPlannedNTwelve}}
\providecommand{\hlSATLrLrThirdburn}{\tbd{hlSATLrLrThirdburn}}
\providecommand{\hlSATLrLrThirdflair}{\tbd{hlSATLrLrThirdflair}}
\providecommand{\hlSATLrMainburn}{\tbd{hlSATLrMainburn}}
\providecommand{\hlSATLrMainflair}{\tbd{hlSATLrMainflair}}
\providecommand{\hlSATLrMainsen}{\tbd{hlSATLrMainsen}}
\providecommand{\hlSFiveBudgetburnA}{\tbd{hlSFiveBudgetburnA}}
\providecommand{\hlSFiveBudgetburnB}{\tbd{hlSFiveBudgetburnB}}
\providecommand{\hlSFiveBudgetburnCIHi}{\tbd{hlSFiveBudgetburnCIHi}}
\providecommand{\hlSFiveBudgetburnCILo}{\tbd{hlSFiveBudgetburnCILo}}
\providecommand{\hlSFiveBudgetburnEst}{\tbd{hlSFiveBudgetburnEst}}
\providecommand{\hlSFiveBudgetburnN}{\tbd{hlSFiveBudgetburnN}}
\providecommand{\hlSFiveBudgetflairA}{\tbd{hlSFiveBudgetflairA}}
\providecommand{\hlSFiveBudgetflairB}{\tbd{hlSFiveBudgetflairB}}
\providecommand{\hlSFiveBudgetflairCIHi}{\tbd{hlSFiveBudgetflairCIHi}}
\providecommand{\hlSFiveBudgetflairCILo}{\tbd{hlSFiveBudgetflairCILo}}
\providecommand{\hlSFiveBudgetflairEst}{\tbd{hlSFiveBudgetflairEst}}
\providecommand{\hlSFiveBudgetflairN}{\tbd{hlSFiveBudgetflairN}}
\providecommand{\hlSFiveDropLVDburnA}{\tbd{hlSFiveDropLVDburnA}}
\providecommand{\hlSFiveDropLVDburnB}{\tbd{hlSFiveDropLVDburnB}}
\providecommand{\hlSFiveDropLVDburnCIHi}{\tbd{hlSFiveDropLVDburnCIHi}}
\providecommand{\hlSFiveDropLVDburnCILo}{\tbd{hlSFiveDropLVDburnCILo}}
\providecommand{\hlSFiveDropLVDburnEst}{\tbd{hlSFiveDropLVDburnEst}}
\providecommand{\hlSFiveDropLVDburnN}{\tbd{hlSFiveDropLVDburnN}}
\providecommand{\hlSFiveDropLVDflairA}{\tbd{hlSFiveDropLVDflairA}}
\providecommand{\hlSFiveDropLVDflairB}{\tbd{hlSFiveDropLVDflairB}}
\providecommand{\hlSFiveDropLVDflairCIHi}{\tbd{hlSFiveDropLVDflairCIHi}}
\providecommand{\hlSFiveDropLVDflairCILo}{\tbd{hlSFiveDropLVDflairCILo}}
\providecommand{\hlSFiveDropLVDflairEst}{\tbd{hlSFiveDropLVDflairEst}}
\providecommand{\hlSFiveDropLVDflairN}{\tbd{hlSFiveDropLVDflairN}}
\providecommand{\hlSFiveDropSATChesA}{\tbd{hlSFiveDropSATChesA}}
\providecommand{\hlSFiveDropSATChesB}{\tbd{hlSFiveDropSATChesB}}
\providecommand{\hlSFiveDropSATChesCIHi}{\tbd{hlSFiveDropSATChesCIHi}}
\providecommand{\hlSFiveDropSATChesCILo}{\tbd{hlSFiveDropSATChesCILo}}
\providecommand{\hlSFiveDropSATChesEst}{\tbd{hlSFiveDropSATChesEst}}
\providecommand{\hlSFiveDropSATChesFlag}{\tbd{hlSFiveDropSATChesFlag}}
\providecommand{\hlSFiveDropSATChesMde}{\tbd{hlSFiveDropSATChesMde}}
\providecommand{\hlSFiveDropSATChesN}{\tbd{hlSFiveDropSATChesN}}
\providecommand{\hlSFiveDropSATChesTostCIHi}{\tbd{hlSFiveDropSATChesTostCIHi}}
\providecommand{\hlSFiveDropSATChesTostCILo}{\tbd{hlSFiveDropSATChesTostCILo}}
\providecommand{\hlSFiveDropSATChesVerdict}{\tbd{hlSFiveDropSATChesVerdict}}
\providecommand{\hlSFiveDropSATCsTwelveA}{\tbd{hlSFiveDropSATCsTwelveA}}
\providecommand{\hlSFiveDropSATCsTwelveB}{\tbd{hlSFiveDropSATCsTwelveB}}
\providecommand{\hlSFiveDropSATCsTwelveCIHi}{\tbd{hlSFiveDropSATCsTwelveCIHi}}
\providecommand{\hlSFiveDropSATCsTwelveCILo}{\tbd{hlSFiveDropSATCsTwelveCILo}}
\providecommand{\hlSFiveDropSATCsTwelveEst}{\tbd{hlSFiveDropSATCsTwelveEst}}
\providecommand{\hlSFiveDropSATCsTwelveFlag}{\tbd{hlSFiveDropSATCsTwelveFlag}}
\providecommand{\hlSFiveDropSATCsTwelveMde}{\tbd{hlSFiveDropSATCsTwelveMde}}
\providecommand{\hlSFiveDropSATCsTwelveN}{\tbd{hlSFiveDropSATCsTwelveN}}
\providecommand{\hlSFiveDropSATCsTwelveTostCIHi}{\tbd{hlSFiveDropSATCsTwelveTostCIHi}}
\providecommand{\hlSFiveDropSATCsTwelveTostCILo}{\tbd{hlSFiveDropSATCsTwelveTostCILo}}
\providecommand{\hlSFiveDropSATCsTwelveVerdict}{\tbd{hlSFiveDropSATCsTwelveVerdict}}
\providecommand{\hlSFiveDropSATDfcA}{\tbd{hlSFiveDropSATDfcA}}
\providecommand{\hlSFiveDropSATDfcB}{\tbd{hlSFiveDropSATDfcB}}
\providecommand{\hlSFiveDropSATDfcCIHi}{\tbd{hlSFiveDropSATDfcCIHi}}
\providecommand{\hlSFiveDropSATDfcCILo}{\tbd{hlSFiveDropSATDfcCILo}}
\providecommand{\hlSFiveDropSATDfcEst}{\tbd{hlSFiveDropSATDfcEst}}
\providecommand{\hlSFiveDropSATDfcFlag}{\tbd{hlSFiveDropSATDfcFlag}}
\providecommand{\hlSFiveDropSATDfcMde}{\tbd{hlSFiveDropSATDfcMde}}
\providecommand{\hlSFiveDropSATDfcN}{\tbd{hlSFiveDropSATDfcN}}
\providecommand{\hlSFiveDropSATDfcTostCIHi}{\tbd{hlSFiveDropSATDfcTostCIHi}}
\providecommand{\hlSFiveDropSATDfcTostCILo}{\tbd{hlSFiveDropSATDfcTostCILo}}
\providecommand{\hlSFiveDropSATDfcVerdict}{\tbd{hlSFiveDropSATDfcVerdict}}
\providecommand{\hlSFiveDropSATEnvaA}{\tbd{hlSFiveDropSATEnvaA}}
\providecommand{\hlSFiveDropSATEnvaB}{\tbd{hlSFiveDropSATEnvaB}}
\providecommand{\hlSFiveDropSATEnvaCIHi}{\tbd{hlSFiveDropSATEnvaCIHi}}
\providecommand{\hlSFiveDropSATEnvaCILo}{\tbd{hlSFiveDropSATEnvaCILo}}
\providecommand{\hlSFiveDropSATEnvaEst}{\tbd{hlSFiveDropSATEnvaEst}}
\providecommand{\hlSFiveDropSATEnvaFlag}{\tbd{hlSFiveDropSATEnvaFlag}}
\providecommand{\hlSFiveDropSATEnvaMde}{\tbd{hlSFiveDropSATEnvaMde}}
\providecommand{\hlSFiveDropSATEnvaN}{\tbd{hlSFiveDropSATEnvaN}}
\providecommand{\hlSFiveDropSATEnvaTostCIHi}{\tbd{hlSFiveDropSATEnvaTostCIHi}}
\providecommand{\hlSFiveDropSATEnvaTostCILo}{\tbd{hlSFiveDropSATEnvaTostCILo}}
\providecommand{\hlSFiveDropSATEnvaVerdict}{\tbd{hlSFiveDropSATEnvaVerdict}}
\providecommand{\hlSFiveDropSATInDomDatasets}{\tbd{hlSFiveDropSATInDomDatasets}}
\providecommand{\hlSFiveDropSATInDomDiffer}{\tbd{hlSFiveDropSATInDomDiffer}}
\providecommand{\hlSFiveDropSATInDomEquiv}{\tbd{hlSFiveDropSATInDomEquiv}}
\providecommand{\hlSFiveDropSATInDomRead}{\tbd{hlSFiveDropSATInDomRead}}
\providecommand{\hlSFiveDropSATInDomUndet}{\tbd{hlSFiveDropSATInDomUndet}}
\providecommand{\hlSFiveDropSATKuroA}{\tbd{hlSFiveDropSATKuroA}}
\providecommand{\hlSFiveDropSATKuroB}{\tbd{hlSFiveDropSATKuroB}}
\providecommand{\hlSFiveDropSATKuroCIHi}{\tbd{hlSFiveDropSATKuroCIHi}}
\providecommand{\hlSFiveDropSATKuroCILo}{\tbd{hlSFiveDropSATKuroCILo}}
\providecommand{\hlSFiveDropSATKuroEst}{\tbd{hlSFiveDropSATKuroEst}}
\providecommand{\hlSFiveDropSATKuroFlag}{\tbd{hlSFiveDropSATKuroFlag}}
\providecommand{\hlSFiveDropSATKuroMde}{\tbd{hlSFiveDropSATKuroMde}}
\providecommand{\hlSFiveDropSATKuroN}{\tbd{hlSFiveDropSATKuroN}}
\providecommand{\hlSFiveDropSATKuroTostCIHi}{\tbd{hlSFiveDropSATKuroTostCIHi}}
\providecommand{\hlSFiveDropSATKuroTostCILo}{\tbd{hlSFiveDropSATKuroTostCILo}}
\providecommand{\hlSFiveDropSATKuroVerdict}{\tbd{hlSFiveDropSATKuroVerdict}}
\providecommand{\hlSFiveDropSATNoPreDatasets}{\tbd{hlSFiveDropSATNoPreDatasets}}
\providecommand{\hlSFiveDropSATNoPreDiffer}{\tbd{hlSFiveDropSATNoPreDiffer}}
\providecommand{\hlSFiveDropSATNoPreEquiv}{\tbd{hlSFiveDropSATNoPreEquiv}}
\providecommand{\hlSFiveDropSATNoPreRead}{\tbd{hlSFiveDropSATNoPreRead}}
\providecommand{\hlSFiveDropSATNoPreUndet}{\tbd{hlSFiveDropSATNoPreUndet}}
\providecommand{\hlSFiveDropSATOemA}{\tbd{hlSFiveDropSATOemA}}
\providecommand{\hlSFiveDropSATOemB}{\tbd{hlSFiveDropSATOemB}}
\providecommand{\hlSFiveDropSATOemCIHi}{\tbd{hlSFiveDropSATOemCIHi}}
\providecommand{\hlSFiveDropSATOemCILo}{\tbd{hlSFiveDropSATOemCILo}}
\providecommand{\hlSFiveDropSATOemEst}{\tbd{hlSFiveDropSATOemEst}}
\providecommand{\hlSFiveDropSATOemFlag}{\tbd{hlSFiveDropSATOemFlag}}
\providecommand{\hlSFiveDropSATOemMde}{\tbd{hlSFiveDropSATOemMde}}
\providecommand{\hlSFiveDropSATOemN}{\tbd{hlSFiveDropSATOemN}}
\providecommand{\hlSFiveDropSATOemTostCIHi}{\tbd{hlSFiveDropSATOemTostCIHi}}
\providecommand{\hlSFiveDropSATOemTostCILo}{\tbd{hlSFiveDropSATOemTostCILo}}
\providecommand{\hlSFiveDropSATOemVerdict}{\tbd{hlSFiveDropSATOemVerdict}}
\providecommand{\hlSFiveDropSATOutDomDatasets}{\tbd{hlSFiveDropSATOutDomDatasets}}
\providecommand{\hlSFiveDropSATOutDomDiffer}{\tbd{hlSFiveDropSATOutDomDiffer}}
\providecommand{\hlSFiveDropSATOutDomEquiv}{\tbd{hlSFiveDropSATOutDomEquiv}}
\providecommand{\hlSFiveDropSATOutDomRead}{\tbd{hlSFiveDropSATOutDomRead}}
\providecommand{\hlSFiveDropSATOutDomUndet}{\tbd{hlSFiveDropSATOutDomUndet}}
\providecommand{\hlSFiveDropSATSnTwoA}{\tbd{hlSFiveDropSATSnTwoA}}
\providecommand{\hlSFiveDropSATSnTwoB}{\tbd{hlSFiveDropSATSnTwoB}}
\providecommand{\hlSFiveDropSATSnTwoCIHi}{\tbd{hlSFiveDropSATSnTwoCIHi}}
\providecommand{\hlSFiveDropSATSnTwoCILo}{\tbd{hlSFiveDropSATSnTwoCILo}}
\providecommand{\hlSFiveDropSATSnTwoEst}{\tbd{hlSFiveDropSATSnTwoEst}}
\providecommand{\hlSFiveDropSATSnTwoFlag}{\tbd{hlSFiveDropSATSnTwoFlag}}
\providecommand{\hlSFiveDropSATSnTwoMde}{\tbd{hlSFiveDropSATSnTwoMde}}
\providecommand{\hlSFiveDropSATSnTwoN}{\tbd{hlSFiveDropSATSnTwoN}}
\providecommand{\hlSFiveDropSATSnTwoTostCIHi}{\tbd{hlSFiveDropSATSnTwoTostCIHi}}
\providecommand{\hlSFiveDropSATSnTwoTostCILo}{\tbd{hlSFiveDropSATSnTwoTostCILo}}
\providecommand{\hlSFiveDropSATSnTwoVerdict}{\tbd{hlSFiveDropSATSnTwoVerdict}}
\providecommand{\hlSFiveDropSATburnA}{\tbd{hlSFiveDropSATburnA}}
\providecommand{\hlSFiveDropSATburnB}{\tbd{hlSFiveDropSATburnB}}
\providecommand{\hlSFiveDropSATburnCIHi}{\tbd{hlSFiveDropSATburnCIHi}}
\providecommand{\hlSFiveDropSATburnCILo}{\tbd{hlSFiveDropSATburnCILo}}
\providecommand{\hlSFiveDropSATburnEst}{\tbd{hlSFiveDropSATburnEst}}
\providecommand{\hlSFiveDropSATburnN}{\tbd{hlSFiveDropSATburnN}}
\providecommand{\hlSFiveDropSATflairA}{\tbd{hlSFiveDropSATflairA}}
\providecommand{\hlSFiveDropSATflairB}{\tbd{hlSFiveDropSATflairB}}
\providecommand{\hlSFiveDropSATflairCIHi}{\tbd{hlSFiveDropSATflairCIHi}}
\providecommand{\hlSFiveDropSATflairCILo}{\tbd{hlSFiveDropSATflairCILo}}
\providecommand{\hlSFiveDropSATflairEst}{\tbd{hlSFiveDropSATflairEst}}
\providecommand{\hlSFiveDropSATflairN}{\tbd{hlSFiveDropSATflairN}}
\providecommand{\hlSFiveRetLVDburnA}{\tbd{hlSFiveRetLVDburnA}}
\providecommand{\hlSFiveRetLVDburnB}{\tbd{hlSFiveRetLVDburnB}}
\providecommand{\hlSFiveRetLVDburnCIHi}{\tbd{hlSFiveRetLVDburnCIHi}}
\providecommand{\hlSFiveRetLVDburnCILo}{\tbd{hlSFiveRetLVDburnCILo}}
\providecommand{\hlSFiveRetLVDburnEst}{\tbd{hlSFiveRetLVDburnEst}}
\providecommand{\hlSFiveRetLVDburnN}{\tbd{hlSFiveRetLVDburnN}}
\providecommand{\hlSFiveRetLVDflairA}{\tbd{hlSFiveRetLVDflairA}}
\providecommand{\hlSFiveRetLVDflairB}{\tbd{hlSFiveRetLVDflairB}}
\providecommand{\hlSFiveRetLVDflairCIHi}{\tbd{hlSFiveRetLVDflairCIHi}}
\providecommand{\hlSFiveRetLVDflairCILo}{\tbd{hlSFiveRetLVDflairCILo}}
\providecommand{\hlSFiveRetLVDflairEst}{\tbd{hlSFiveRetLVDflairEst}}
\providecommand{\hlSFiveRetLVDflairN}{\tbd{hlSFiveRetLVDflairN}}
\providecommand{\hlSFiveRetSATburnA}{\tbd{hlSFiveRetSATburnA}}
\providecommand{\hlSFiveRetSATburnB}{\tbd{hlSFiveRetSATburnB}}
\providecommand{\hlSFiveRetSATburnCIHi}{\tbd{hlSFiveRetSATburnCIHi}}
\providecommand{\hlSFiveRetSATburnCILo}{\tbd{hlSFiveRetSATburnCILo}}
\providecommand{\hlSFiveRetSATburnEst}{\tbd{hlSFiveRetSATburnEst}}
\providecommand{\hlSFiveRetSATburnN}{\tbd{hlSFiveRetSATburnN}}
\providecommand{\hlSFiveRetSATflairA}{\tbd{hlSFiveRetSATflairA}}
\providecommand{\hlSFiveRetSATflairB}{\tbd{hlSFiveRetSATflairB}}
\providecommand{\hlSFiveRetSATflairCIHi}{\tbd{hlSFiveRetSATflairCIHi}}
\providecommand{\hlSFiveRetSATflairCILo}{\tbd{hlSFiveRetSATflairCILo}}
\providecommand{\hlSFiveRetSATflairEst}{\tbd{hlSFiveRetSATflairEst}}
\providecommand{\hlSFiveRetSATflairN}{\tbd{hlSFiveRetSATflairN}}
\providecommand{\hlSFourBudgetburnA}{\tbd{hlSFourBudgetburnA}}
\providecommand{\hlSFourBudgetburnB}{\tbd{hlSFourBudgetburnB}}
\providecommand{\hlSFourBudgetburnCIHi}{\tbd{hlSFourBudgetburnCIHi}}
\providecommand{\hlSFourBudgetburnCILo}{\tbd{hlSFourBudgetburnCILo}}
\providecommand{\hlSFourBudgetburnEst}{\tbd{hlSFourBudgetburnEst}}
\providecommand{\hlSFourBudgetburnN}{\tbd{hlSFourBudgetburnN}}
\providecommand{\hlSFourBudgetflairA}{\tbd{hlSFourBudgetflairA}}
\providecommand{\hlSFourBudgetflairB}{\tbd{hlSFourBudgetflairB}}
\providecommand{\hlSFourBudgetflairCIHi}{\tbd{hlSFourBudgetflairCIHi}}
\providecommand{\hlSFourBudgetflairCILo}{\tbd{hlSFourBudgetflairCILo}}
\providecommand{\hlSFourBudgetflairEst}{\tbd{hlSFourBudgetflairEst}}
\providecommand{\hlSFourBudgetflairN}{\tbd{hlSFourBudgetflairN}}
\providecommand{\hlSFourDropRNChesA}{\tbd{hlSFourDropRNChesA}}
\providecommand{\hlSFourDropRNChesB}{\tbd{hlSFourDropRNChesB}}
\providecommand{\hlSFourDropRNChesCIHi}{\tbd{hlSFourDropRNChesCIHi}}
\providecommand{\hlSFourDropRNChesCILo}{\tbd{hlSFourDropRNChesCILo}}
\providecommand{\hlSFourDropRNChesEst}{\tbd{hlSFourDropRNChesEst}}
\providecommand{\hlSFourDropRNChesFlag}{\tbd{hlSFourDropRNChesFlag}}
\providecommand{\hlSFourDropRNChesMde}{\tbd{hlSFourDropRNChesMde}}
\providecommand{\hlSFourDropRNChesN}{\tbd{hlSFourDropRNChesN}}
\providecommand{\hlSFourDropRNChesTostCIHi}{\tbd{hlSFourDropRNChesTostCIHi}}
\providecommand{\hlSFourDropRNChesTostCILo}{\tbd{hlSFourDropRNChesTostCILo}}
\providecommand{\hlSFourDropRNChesVerdict}{\tbd{hlSFourDropRNChesVerdict}}
\providecommand{\hlSFourDropRNCsTwelveA}{\tbd{hlSFourDropRNCsTwelveA}}
\providecommand{\hlSFourDropRNCsTwelveB}{\tbd{hlSFourDropRNCsTwelveB}}
\providecommand{\hlSFourDropRNCsTwelveCIHi}{\tbd{hlSFourDropRNCsTwelveCIHi}}
\providecommand{\hlSFourDropRNCsTwelveCILo}{\tbd{hlSFourDropRNCsTwelveCILo}}
\providecommand{\hlSFourDropRNCsTwelveEst}{\tbd{hlSFourDropRNCsTwelveEst}}
\providecommand{\hlSFourDropRNCsTwelveFlag}{\tbd{hlSFourDropRNCsTwelveFlag}}
\providecommand{\hlSFourDropRNCsTwelveMde}{\tbd{hlSFourDropRNCsTwelveMde}}
\providecommand{\hlSFourDropRNCsTwelveN}{\tbd{hlSFourDropRNCsTwelveN}}
\providecommand{\hlSFourDropRNCsTwelveTostCIHi}{\tbd{hlSFourDropRNCsTwelveTostCIHi}}
\providecommand{\hlSFourDropRNCsTwelveTostCILo}{\tbd{hlSFourDropRNCsTwelveTostCILo}}
\providecommand{\hlSFourDropRNCsTwelveVerdict}{\tbd{hlSFourDropRNCsTwelveVerdict}}
\providecommand{\hlSFourDropRNDfcA}{\tbd{hlSFourDropRNDfcA}}
\providecommand{\hlSFourDropRNDfcB}{\tbd{hlSFourDropRNDfcB}}
\providecommand{\hlSFourDropRNDfcCIHi}{\tbd{hlSFourDropRNDfcCIHi}}
\providecommand{\hlSFourDropRNDfcCILo}{\tbd{hlSFourDropRNDfcCILo}}
\providecommand{\hlSFourDropRNDfcEst}{\tbd{hlSFourDropRNDfcEst}}
\providecommand{\hlSFourDropRNDfcFlag}{\tbd{hlSFourDropRNDfcFlag}}
\providecommand{\hlSFourDropRNDfcMde}{\tbd{hlSFourDropRNDfcMde}}
\providecommand{\hlSFourDropRNDfcN}{\tbd{hlSFourDropRNDfcN}}
\providecommand{\hlSFourDropRNDfcTostCIHi}{\tbd{hlSFourDropRNDfcTostCIHi}}
\providecommand{\hlSFourDropRNDfcTostCILo}{\tbd{hlSFourDropRNDfcTostCILo}}
\providecommand{\hlSFourDropRNDfcVerdict}{\tbd{hlSFourDropRNDfcVerdict}}
\providecommand{\hlSFourDropRNEnvaA}{\tbd{hlSFourDropRNEnvaA}}
\providecommand{\hlSFourDropRNEnvaB}{\tbd{hlSFourDropRNEnvaB}}
\providecommand{\hlSFourDropRNEnvaCIHi}{\tbd{hlSFourDropRNEnvaCIHi}}
\providecommand{\hlSFourDropRNEnvaCILo}{\tbd{hlSFourDropRNEnvaCILo}}
\providecommand{\hlSFourDropRNEnvaEst}{\tbd{hlSFourDropRNEnvaEst}}
\providecommand{\hlSFourDropRNEnvaFlag}{\tbd{hlSFourDropRNEnvaFlag}}
\providecommand{\hlSFourDropRNEnvaMde}{\tbd{hlSFourDropRNEnvaMde}}
\providecommand{\hlSFourDropRNEnvaN}{\tbd{hlSFourDropRNEnvaN}}
\providecommand{\hlSFourDropRNEnvaTostCIHi}{\tbd{hlSFourDropRNEnvaTostCIHi}}
\providecommand{\hlSFourDropRNEnvaTostCILo}{\tbd{hlSFourDropRNEnvaTostCILo}}
\providecommand{\hlSFourDropRNEnvaVerdict}{\tbd{hlSFourDropRNEnvaVerdict}}
\providecommand{\hlSFourDropRNInDomDatasets}{\tbd{hlSFourDropRNInDomDatasets}}
\providecommand{\hlSFourDropRNInDomDiffer}{\tbd{hlSFourDropRNInDomDiffer}}
\providecommand{\hlSFourDropRNInDomEquiv}{\tbd{hlSFourDropRNInDomEquiv}}
\providecommand{\hlSFourDropRNInDomRead}{\tbd{hlSFourDropRNInDomRead}}
\providecommand{\hlSFourDropRNInDomUndet}{\tbd{hlSFourDropRNInDomUndet}}
\providecommand{\hlSFourDropRNKuroA}{\tbd{hlSFourDropRNKuroA}}
\providecommand{\hlSFourDropRNKuroB}{\tbd{hlSFourDropRNKuroB}}
\providecommand{\hlSFourDropRNKuroCIHi}{\tbd{hlSFourDropRNKuroCIHi}}
\providecommand{\hlSFourDropRNKuroCILo}{\tbd{hlSFourDropRNKuroCILo}}
\providecommand{\hlSFourDropRNKuroEst}{\tbd{hlSFourDropRNKuroEst}}
\providecommand{\hlSFourDropRNKuroFlag}{\tbd{hlSFourDropRNKuroFlag}}
\providecommand{\hlSFourDropRNKuroMde}{\tbd{hlSFourDropRNKuroMde}}
\providecommand{\hlSFourDropRNKuroN}{\tbd{hlSFourDropRNKuroN}}
\providecommand{\hlSFourDropRNKuroTostCIHi}{\tbd{hlSFourDropRNKuroTostCIHi}}
\providecommand{\hlSFourDropRNKuroTostCILo}{\tbd{hlSFourDropRNKuroTostCILo}}
\providecommand{\hlSFourDropRNKuroVerdict}{\tbd{hlSFourDropRNKuroVerdict}}
\providecommand{\hlSFourDropRNNoPreDatasets}{\tbd{hlSFourDropRNNoPreDatasets}}
\providecommand{\hlSFourDropRNNoPreDiffer}{\tbd{hlSFourDropRNNoPreDiffer}}
\providecommand{\hlSFourDropRNNoPreEquiv}{\tbd{hlSFourDropRNNoPreEquiv}}
\providecommand{\hlSFourDropRNNoPreRead}{\tbd{hlSFourDropRNNoPreRead}}
\providecommand{\hlSFourDropRNNoPreUndet}{\tbd{hlSFourDropRNNoPreUndet}}
\providecommand{\hlSFourDropRNOemA}{\tbd{hlSFourDropRNOemA}}
\providecommand{\hlSFourDropRNOemB}{\tbd{hlSFourDropRNOemB}}
\providecommand{\hlSFourDropRNOemCIHi}{\tbd{hlSFourDropRNOemCIHi}}
\providecommand{\hlSFourDropRNOemCILo}{\tbd{hlSFourDropRNOemCILo}}
\providecommand{\hlSFourDropRNOemEst}{\tbd{hlSFourDropRNOemEst}}
\providecommand{\hlSFourDropRNOemFlag}{\tbd{hlSFourDropRNOemFlag}}
\providecommand{\hlSFourDropRNOemMde}{\tbd{hlSFourDropRNOemMde}}
\providecommand{\hlSFourDropRNOemN}{\tbd{hlSFourDropRNOemN}}
\providecommand{\hlSFourDropRNOemTostCIHi}{\tbd{hlSFourDropRNOemTostCIHi}}
\providecommand{\hlSFourDropRNOemTostCILo}{\tbd{hlSFourDropRNOemTostCILo}}
\providecommand{\hlSFourDropRNOemVerdict}{\tbd{hlSFourDropRNOemVerdict}}
\providecommand{\hlSFourDropRNOutDomDatasets}{\tbd{hlSFourDropRNOutDomDatasets}}
\providecommand{\hlSFourDropRNOutDomDiffer}{\tbd{hlSFourDropRNOutDomDiffer}}
\providecommand{\hlSFourDropRNOutDomEquiv}{\tbd{hlSFourDropRNOutDomEquiv}}
\providecommand{\hlSFourDropRNOutDomRead}{\tbd{hlSFourDropRNOutDomRead}}
\providecommand{\hlSFourDropRNOutDomUndet}{\tbd{hlSFourDropRNOutDomUndet}}
\providecommand{\hlSFourDropRNSnTwoA}{\tbd{hlSFourDropRNSnTwoA}}
\providecommand{\hlSFourDropRNSnTwoB}{\tbd{hlSFourDropRNSnTwoB}}
\providecommand{\hlSFourDropRNSnTwoCIHi}{\tbd{hlSFourDropRNSnTwoCIHi}}
\providecommand{\hlSFourDropRNSnTwoCILo}{\tbd{hlSFourDropRNSnTwoCILo}}
\providecommand{\hlSFourDropRNSnTwoEst}{\tbd{hlSFourDropRNSnTwoEst}}
\providecommand{\hlSFourDropRNSnTwoFlag}{\tbd{hlSFourDropRNSnTwoFlag}}
\providecommand{\hlSFourDropRNSnTwoMde}{\tbd{hlSFourDropRNSnTwoMde}}
\providecommand{\hlSFourDropRNSnTwoN}{\tbd{hlSFourDropRNSnTwoN}}
\providecommand{\hlSFourDropRNSnTwoTostCIHi}{\tbd{hlSFourDropRNSnTwoTostCIHi}}
\providecommand{\hlSFourDropRNSnTwoTostCILo}{\tbd{hlSFourDropRNSnTwoTostCILo}}
\providecommand{\hlSFourDropRNSnTwoVerdict}{\tbd{hlSFourDropRNSnTwoVerdict}}
\providecommand{\hlSFourDropRNburnA}{\tbd{hlSFourDropRNburnA}}
\providecommand{\hlSFourDropRNburnB}{\tbd{hlSFourDropRNburnB}}
\providecommand{\hlSFourDropRNburnCIHi}{\tbd{hlSFourDropRNburnCIHi}}
\providecommand{\hlSFourDropRNburnCILo}{\tbd{hlSFourDropRNburnCILo}}
\providecommand{\hlSFourDropRNburnEst}{\tbd{hlSFourDropRNburnEst}}
\providecommand{\hlSFourDropRNburnN}{\tbd{hlSFourDropRNburnN}}
\providecommand{\hlSFourDropRNflairA}{\tbd{hlSFourDropRNflairA}}
\providecommand{\hlSFourDropRNflairB}{\tbd{hlSFourDropRNflairB}}
\providecommand{\hlSFourDropRNflairCIHi}{\tbd{hlSFourDropRNflairCIHi}}
\providecommand{\hlSFourDropRNflairCILo}{\tbd{hlSFourDropRNflairCILo}}
\providecommand{\hlSFourDropRNflairEst}{\tbd{hlSFourDropRNflairEst}}
\providecommand{\hlSFourDropRNflairN}{\tbd{hlSFourDropRNflairN}}
\providecommand{\hlSFourRetRNburnA}{\tbd{hlSFourRetRNburnA}}
\providecommand{\hlSFourRetRNburnB}{\tbd{hlSFourRetRNburnB}}
\providecommand{\hlSFourRetRNburnCIHi}{\tbd{hlSFourRetRNburnCIHi}}
\providecommand{\hlSFourRetRNburnCILo}{\tbd{hlSFourRetRNburnCILo}}
\providecommand{\hlSFourRetRNburnEst}{\tbd{hlSFourRetRNburnEst}}
\providecommand{\hlSFourRetRNburnN}{\tbd{hlSFourRetRNburnN}}
\providecommand{\hlSFourRetRNflairA}{\tbd{hlSFourRetRNflairA}}
\providecommand{\hlSFourRetRNflairB}{\tbd{hlSFourRetRNflairB}}
\providecommand{\hlSFourRetRNflairCIHi}{\tbd{hlSFourRetRNflairCIHi}}
\providecommand{\hlSFourRetRNflairCILo}{\tbd{hlSFourRetRNflairCILo}}
\providecommand{\hlSFourRetRNflairEst}{\tbd{hlSFourRetRNflairEst}}
\providecommand{\hlSFourRetRNflairN}{\tbd{hlSFourRetRNflairN}}
\providecommand{\hlSOneDropDOFAsenA}{\tbd{hlSOneDropDOFAsenA}}
\providecommand{\hlSOneDropDOFAsenB}{\tbd{hlSOneDropDOFAsenB}}
\providecommand{\hlSOneDropDOFAsenCIHi}{\tbd{hlSOneDropDOFAsenCIHi}}
\providecommand{\hlSOneDropDOFAsenCILo}{\tbd{hlSOneDropDOFAsenCILo}}
\providecommand{\hlSOneDropDOFAsenEst}{\tbd{hlSOneDropDOFAsenEst}}
\providecommand{\hlSOneDropDOFAsenN}{\tbd{hlSOneDropDOFAsenN}}
\providecommand{\hlSOneDropLVDsenA}{\tbd{hlSOneDropLVDsenA}}
\providecommand{\hlSOneDropLVDsenB}{\tbd{hlSOneDropLVDsenB}}
\providecommand{\hlSOneDropLVDsenCIHi}{\tbd{hlSOneDropLVDsenCIHi}}
\providecommand{\hlSOneDropLVDsenCILo}{\tbd{hlSOneDropLVDsenCILo}}
\providecommand{\hlSOneDropLVDsenEst}{\tbd{hlSOneDropLVDsenEst}}
\providecommand{\hlSOneDropLVDsenN}{\tbd{hlSOneDropLVDsenN}}
\providecommand{\hlSOneDropMeansenA}{\tbd{hlSOneDropMeansenA}}
\providecommand{\hlSOneDropMeansenB}{\tbd{hlSOneDropMeansenB}}
\providecommand{\hlSOneDropMeansenCIHi}{\tbd{hlSOneDropMeansenCIHi}}
\providecommand{\hlSOneDropMeansenCILo}{\tbd{hlSOneDropMeansenCILo}}
\providecommand{\hlSOneDropMeansenEst}{\tbd{hlSOneDropMeansenEst}}
\providecommand{\hlSOneDropMeansenN}{\tbd{hlSOneDropMeansenN}}
\providecommand{\hlSOneDropRNsenA}{\tbd{hlSOneDropRNsenA}}
\providecommand{\hlSOneDropRNsenB}{\tbd{hlSOneDropRNsenB}}
\providecommand{\hlSOneDropRNsenCIHi}{\tbd{hlSOneDropRNsenCIHi}}
\providecommand{\hlSOneDropRNsenCILo}{\tbd{hlSOneDropRNsenCILo}}
\providecommand{\hlSOneDropRNsenEst}{\tbd{hlSOneDropRNsenEst}}
\providecommand{\hlSOneDropRNsenN}{\tbd{hlSOneDropRNsenN}}
\providecommand{\hlSOneDropSATsenA}{\tbd{hlSOneDropSATsenA}}
\providecommand{\hlSOneDropSATsenB}{\tbd{hlSOneDropSATsenB}}
\providecommand{\hlSOneDropSATsenCIHi}{\tbd{hlSOneDropSATsenCIHi}}
\providecommand{\hlSOneDropSATsenCILo}{\tbd{hlSOneDropSATsenCILo}}
\providecommand{\hlSOneDropSATsenEst}{\tbd{hlSOneDropSATsenEst}}
\providecommand{\hlSOneDropSATsenN}{\tbd{hlSOneDropSATsenN}}
\providecommand{\hlSOneDropTMsenA}{\tbd{hlSOneDropTMsenA}}
\providecommand{\hlSOneDropTMsenB}{\tbd{hlSOneDropTMsenB}}
\providecommand{\hlSOneDropTMsenCIHi}{\tbd{hlSOneDropTMsenCIHi}}
\providecommand{\hlSOneDropTMsenCILo}{\tbd{hlSOneDropTMsenCILo}}
\providecommand{\hlSOneDropTMsenEst}{\tbd{hlSOneDropTMsenEst}}
\providecommand{\hlSOneDropTMsenN}{\tbd{hlSOneDropTMsenN}}
\providecommand{\hlSSixBudgetburnA}{\tbd{hlSSixBudgetburnA}}
\providecommand{\hlSSixBudgetburnB}{\tbd{hlSSixBudgetburnB}}
\providecommand{\hlSSixBudgetburnCIHi}{\tbd{hlSSixBudgetburnCIHi}}
\providecommand{\hlSSixBudgetburnCILo}{\tbd{hlSSixBudgetburnCILo}}
\providecommand{\hlSSixBudgetburnEst}{\tbd{hlSSixBudgetburnEst}}
\providecommand{\hlSSixBudgetburnN}{\tbd{hlSSixBudgetburnN}}
\providecommand{\hlSSixBudgetflairA}{\tbd{hlSSixBudgetflairA}}
\providecommand{\hlSSixBudgetflairB}{\tbd{hlSSixBudgetflairB}}
\providecommand{\hlSSixBudgetflairCIHi}{\tbd{hlSSixBudgetflairCIHi}}
\providecommand{\hlSSixBudgetflairCILo}{\tbd{hlSSixBudgetflairCILo}}
\providecommand{\hlSSixBudgetflairEst}{\tbd{hlSSixBudgetflairEst}}
\providecommand{\hlSSixBudgetflairN}{\tbd{hlSSixBudgetflairN}}
\providecommand{\hlSSixDropLVDburnA}{\tbd{hlSSixDropLVDburnA}}
\providecommand{\hlSSixDropLVDburnB}{\tbd{hlSSixDropLVDburnB}}
\providecommand{\hlSSixDropLVDburnCIHi}{\tbd{hlSSixDropLVDburnCIHi}}
\providecommand{\hlSSixDropLVDburnCILo}{\tbd{hlSSixDropLVDburnCILo}}
\providecommand{\hlSSixDropLVDburnEst}{\tbd{hlSSixDropLVDburnEst}}
\providecommand{\hlSSixDropLVDburnN}{\tbd{hlSSixDropLVDburnN}}
\providecommand{\hlSSixDropLVDflairA}{\tbd{hlSSixDropLVDflairA}}
\providecommand{\hlSSixDropLVDflairB}{\tbd{hlSSixDropLVDflairB}}
\providecommand{\hlSSixDropLVDflairCIHi}{\tbd{hlSSixDropLVDflairCIHi}}
\providecommand{\hlSSixDropLVDflairCILo}{\tbd{hlSSixDropLVDflairCILo}}
\providecommand{\hlSSixDropLVDflairEst}{\tbd{hlSSixDropLVDflairEst}}
\providecommand{\hlSSixDropLVDflairN}{\tbd{hlSSixDropLVDflairN}}
\providecommand{\hlSSixDropSATChesA}{\tbd{hlSSixDropSATChesA}}
\providecommand{\hlSSixDropSATChesB}{\tbd{hlSSixDropSATChesB}}
\providecommand{\hlSSixDropSATChesCIHi}{\tbd{hlSSixDropSATChesCIHi}}
\providecommand{\hlSSixDropSATChesCILo}{\tbd{hlSSixDropSATChesCILo}}
\providecommand{\hlSSixDropSATChesEst}{\tbd{hlSSixDropSATChesEst}}
\providecommand{\hlSSixDropSATChesFlag}{\tbd{hlSSixDropSATChesFlag}}
\providecommand{\hlSSixDropSATChesMde}{\tbd{hlSSixDropSATChesMde}}
\providecommand{\hlSSixDropSATChesN}{\tbd{hlSSixDropSATChesN}}
\providecommand{\hlSSixDropSATChesTostCIHi}{\tbd{hlSSixDropSATChesTostCIHi}}
\providecommand{\hlSSixDropSATChesTostCILo}{\tbd{hlSSixDropSATChesTostCILo}}
\providecommand{\hlSSixDropSATChesVerdict}{\tbd{hlSSixDropSATChesVerdict}}
\providecommand{\hlSSixDropSATCsTwelveA}{\tbd{hlSSixDropSATCsTwelveA}}
\providecommand{\hlSSixDropSATCsTwelveB}{\tbd{hlSSixDropSATCsTwelveB}}
\providecommand{\hlSSixDropSATCsTwelveCIHi}{\tbd{hlSSixDropSATCsTwelveCIHi}}
\providecommand{\hlSSixDropSATCsTwelveCILo}{\tbd{hlSSixDropSATCsTwelveCILo}}
\providecommand{\hlSSixDropSATCsTwelveEst}{\tbd{hlSSixDropSATCsTwelveEst}}
\providecommand{\hlSSixDropSATCsTwelveFlag}{\tbd{hlSSixDropSATCsTwelveFlag}}
\providecommand{\hlSSixDropSATCsTwelveMde}{\tbd{hlSSixDropSATCsTwelveMde}}
\providecommand{\hlSSixDropSATCsTwelveN}{\tbd{hlSSixDropSATCsTwelveN}}
\providecommand{\hlSSixDropSATCsTwelveTostCIHi}{\tbd{hlSSixDropSATCsTwelveTostCIHi}}
\providecommand{\hlSSixDropSATCsTwelveTostCILo}{\tbd{hlSSixDropSATCsTwelveTostCILo}}
\providecommand{\hlSSixDropSATCsTwelveVerdict}{\tbd{hlSSixDropSATCsTwelveVerdict}}
\providecommand{\hlSSixDropSATDfcA}{\tbd{hlSSixDropSATDfcA}}
\providecommand{\hlSSixDropSATDfcB}{\tbd{hlSSixDropSATDfcB}}
\providecommand{\hlSSixDropSATDfcCIHi}{\tbd{hlSSixDropSATDfcCIHi}}
\providecommand{\hlSSixDropSATDfcCILo}{\tbd{hlSSixDropSATDfcCILo}}
\providecommand{\hlSSixDropSATDfcEst}{\tbd{hlSSixDropSATDfcEst}}
\providecommand{\hlSSixDropSATDfcFlag}{\tbd{hlSSixDropSATDfcFlag}}
\providecommand{\hlSSixDropSATDfcMde}{\tbd{hlSSixDropSATDfcMde}}
\providecommand{\hlSSixDropSATDfcN}{\tbd{hlSSixDropSATDfcN}}
\providecommand{\hlSSixDropSATDfcTostCIHi}{\tbd{hlSSixDropSATDfcTostCIHi}}
\providecommand{\hlSSixDropSATDfcTostCILo}{\tbd{hlSSixDropSATDfcTostCILo}}
\providecommand{\hlSSixDropSATDfcVerdict}{\tbd{hlSSixDropSATDfcVerdict}}
\providecommand{\hlSSixDropSATEnvaA}{\tbd{hlSSixDropSATEnvaA}}
\providecommand{\hlSSixDropSATEnvaB}{\tbd{hlSSixDropSATEnvaB}}
\providecommand{\hlSSixDropSATEnvaCIHi}{\tbd{hlSSixDropSATEnvaCIHi}}
\providecommand{\hlSSixDropSATEnvaCILo}{\tbd{hlSSixDropSATEnvaCILo}}
\providecommand{\hlSSixDropSATEnvaEst}{\tbd{hlSSixDropSATEnvaEst}}
\providecommand{\hlSSixDropSATEnvaFlag}{\tbd{hlSSixDropSATEnvaFlag}}
\providecommand{\hlSSixDropSATEnvaMde}{\tbd{hlSSixDropSATEnvaMde}}
\providecommand{\hlSSixDropSATEnvaN}{\tbd{hlSSixDropSATEnvaN}}
\providecommand{\hlSSixDropSATEnvaTostCIHi}{\tbd{hlSSixDropSATEnvaTostCIHi}}
\providecommand{\hlSSixDropSATEnvaTostCILo}{\tbd{hlSSixDropSATEnvaTostCILo}}
\providecommand{\hlSSixDropSATEnvaVerdict}{\tbd{hlSSixDropSATEnvaVerdict}}
\providecommand{\hlSSixDropSATInDomDatasets}{\tbd{hlSSixDropSATInDomDatasets}}
\providecommand{\hlSSixDropSATInDomDiffer}{\tbd{hlSSixDropSATInDomDiffer}}
\providecommand{\hlSSixDropSATInDomEquiv}{\tbd{hlSSixDropSATInDomEquiv}}
\providecommand{\hlSSixDropSATInDomRead}{\tbd{hlSSixDropSATInDomRead}}
\providecommand{\hlSSixDropSATInDomUndet}{\tbd{hlSSixDropSATInDomUndet}}
\providecommand{\hlSSixDropSATKuroA}{\tbd{hlSSixDropSATKuroA}}
\providecommand{\hlSSixDropSATKuroB}{\tbd{hlSSixDropSATKuroB}}
\providecommand{\hlSSixDropSATKuroCIHi}{\tbd{hlSSixDropSATKuroCIHi}}
\providecommand{\hlSSixDropSATKuroCILo}{\tbd{hlSSixDropSATKuroCILo}}
\providecommand{\hlSSixDropSATKuroEst}{\tbd{hlSSixDropSATKuroEst}}
\providecommand{\hlSSixDropSATKuroFlag}{\tbd{hlSSixDropSATKuroFlag}}
\providecommand{\hlSSixDropSATKuroMde}{\tbd{hlSSixDropSATKuroMde}}
\providecommand{\hlSSixDropSATKuroN}{\tbd{hlSSixDropSATKuroN}}
\providecommand{\hlSSixDropSATKuroTostCIHi}{\tbd{hlSSixDropSATKuroTostCIHi}}
\providecommand{\hlSSixDropSATKuroTostCILo}{\tbd{hlSSixDropSATKuroTostCILo}}
\providecommand{\hlSSixDropSATKuroVerdict}{\tbd{hlSSixDropSATKuroVerdict}}
\providecommand{\hlSSixDropSATNoPreDatasets}{\tbd{hlSSixDropSATNoPreDatasets}}
\providecommand{\hlSSixDropSATNoPreDiffer}{\tbd{hlSSixDropSATNoPreDiffer}}
\providecommand{\hlSSixDropSATNoPreEquiv}{\tbd{hlSSixDropSATNoPreEquiv}}
\providecommand{\hlSSixDropSATNoPreRead}{\tbd{hlSSixDropSATNoPreRead}}
\providecommand{\hlSSixDropSATNoPreUndet}{\tbd{hlSSixDropSATNoPreUndet}}
\providecommand{\hlSSixDropSATOemA}{\tbd{hlSSixDropSATOemA}}
\providecommand{\hlSSixDropSATOemB}{\tbd{hlSSixDropSATOemB}}
\providecommand{\hlSSixDropSATOemCIHi}{\tbd{hlSSixDropSATOemCIHi}}
\providecommand{\hlSSixDropSATOemCILo}{\tbd{hlSSixDropSATOemCILo}}
\providecommand{\hlSSixDropSATOemEst}{\tbd{hlSSixDropSATOemEst}}
\providecommand{\hlSSixDropSATOemFlag}{\tbd{hlSSixDropSATOemFlag}}
\providecommand{\hlSSixDropSATOemMde}{\tbd{hlSSixDropSATOemMde}}
\providecommand{\hlSSixDropSATOemN}{\tbd{hlSSixDropSATOemN}}
\providecommand{\hlSSixDropSATOemTostCIHi}{\tbd{hlSSixDropSATOemTostCIHi}}
\providecommand{\hlSSixDropSATOemTostCILo}{\tbd{hlSSixDropSATOemTostCILo}}
\providecommand{\hlSSixDropSATOemVerdict}{\tbd{hlSSixDropSATOemVerdict}}
\providecommand{\hlSSixDropSATOutDomDatasets}{\tbd{hlSSixDropSATOutDomDatasets}}
\providecommand{\hlSSixDropSATOutDomDiffer}{\tbd{hlSSixDropSATOutDomDiffer}}
\providecommand{\hlSSixDropSATOutDomEquiv}{\tbd{hlSSixDropSATOutDomEquiv}}
\providecommand{\hlSSixDropSATOutDomRead}{\tbd{hlSSixDropSATOutDomRead}}
\providecommand{\hlSSixDropSATOutDomUndet}{\tbd{hlSSixDropSATOutDomUndet}}
\providecommand{\hlSSixDropSATSnTwoA}{\tbd{hlSSixDropSATSnTwoA}}
\providecommand{\hlSSixDropSATSnTwoB}{\tbd{hlSSixDropSATSnTwoB}}
\providecommand{\hlSSixDropSATSnTwoCIHi}{\tbd{hlSSixDropSATSnTwoCIHi}}
\providecommand{\hlSSixDropSATSnTwoCILo}{\tbd{hlSSixDropSATSnTwoCILo}}
\providecommand{\hlSSixDropSATSnTwoEst}{\tbd{hlSSixDropSATSnTwoEst}}
\providecommand{\hlSSixDropSATSnTwoFlag}{\tbd{hlSSixDropSATSnTwoFlag}}
\providecommand{\hlSSixDropSATSnTwoMde}{\tbd{hlSSixDropSATSnTwoMde}}
\providecommand{\hlSSixDropSATSnTwoN}{\tbd{hlSSixDropSATSnTwoN}}
\providecommand{\hlSSixDropSATSnTwoTostCIHi}{\tbd{hlSSixDropSATSnTwoTostCIHi}}
\providecommand{\hlSSixDropSATSnTwoTostCILo}{\tbd{hlSSixDropSATSnTwoTostCILo}}
\providecommand{\hlSSixDropSATSnTwoVerdict}{\tbd{hlSSixDropSATSnTwoVerdict}}
\providecommand{\hlSSixDropSATburnA}{\tbd{hlSSixDropSATburnA}}
\providecommand{\hlSSixDropSATburnB}{\tbd{hlSSixDropSATburnB}}
\providecommand{\hlSSixDropSATburnCIHi}{\tbd{hlSSixDropSATburnCIHi}}
\providecommand{\hlSSixDropSATburnCILo}{\tbd{hlSSixDropSATburnCILo}}
\providecommand{\hlSSixDropSATburnEst}{\tbd{hlSSixDropSATburnEst}}
\providecommand{\hlSSixDropSATburnN}{\tbd{hlSSixDropSATburnN}}
\providecommand{\hlSSixDropSATflairA}{\tbd{hlSSixDropSATflairA}}
\providecommand{\hlSSixDropSATflairB}{\tbd{hlSSixDropSATflairB}}
\providecommand{\hlSSixDropSATflairCIHi}{\tbd{hlSSixDropSATflairCIHi}}
\providecommand{\hlSSixDropSATflairCILo}{\tbd{hlSSixDropSATflairCILo}}
\providecommand{\hlSSixDropSATflairEst}{\tbd{hlSSixDropSATflairEst}}
\providecommand{\hlSSixDropSATflairN}{\tbd{hlSSixDropSATflairN}}
\providecommand{\hlSSixRetLVDburnA}{\tbd{hlSSixRetLVDburnA}}
\providecommand{\hlSSixRetLVDburnB}{\tbd{hlSSixRetLVDburnB}}
\providecommand{\hlSSixRetLVDburnCIHi}{\tbd{hlSSixRetLVDburnCIHi}}
\providecommand{\hlSSixRetLVDburnCILo}{\tbd{hlSSixRetLVDburnCILo}}
\providecommand{\hlSSixRetLVDburnEst}{\tbd{hlSSixRetLVDburnEst}}
\providecommand{\hlSSixRetLVDburnN}{\tbd{hlSSixRetLVDburnN}}
\providecommand{\hlSSixRetLVDflairA}{\tbd{hlSSixRetLVDflairA}}
\providecommand{\hlSSixRetLVDflairB}{\tbd{hlSSixRetLVDflairB}}
\providecommand{\hlSSixRetLVDflairCIHi}{\tbd{hlSSixRetLVDflairCIHi}}
\providecommand{\hlSSixRetLVDflairCILo}{\tbd{hlSSixRetLVDflairCILo}}
\providecommand{\hlSSixRetLVDflairEst}{\tbd{hlSSixRetLVDflairEst}}
\providecommand{\hlSSixRetLVDflairN}{\tbd{hlSSixRetLVDflairN}}
\providecommand{\hlSSixRetSATburnA}{\tbd{hlSSixRetSATburnA}}
\providecommand{\hlSSixRetSATburnB}{\tbd{hlSSixRetSATburnB}}
\providecommand{\hlSSixRetSATburnCIHi}{\tbd{hlSSixRetSATburnCIHi}}
\providecommand{\hlSSixRetSATburnCILo}{\tbd{hlSSixRetSATburnCILo}}
\providecommand{\hlSSixRetSATburnEst}{\tbd{hlSSixRetSATburnEst}}
\providecommand{\hlSSixRetSATburnN}{\tbd{hlSSixRetSATburnN}}
\providecommand{\hlSSixRetSATflairA}{\tbd{hlSSixRetSATflairA}}
\providecommand{\hlSSixRetSATflairB}{\tbd{hlSSixRetSATflairB}}
\providecommand{\hlSSixRetSATflairCIHi}{\tbd{hlSSixRetSATflairCIHi}}
\providecommand{\hlSSixRetSATflairCILo}{\tbd{hlSSixRetSATflairCILo}}
\providecommand{\hlSSixRetSATflairEst}{\tbd{hlSSixRetSATflairEst}}
\providecommand{\hlSSixRetSATflairN}{\tbd{hlSSixRetSATflairN}}
\providecommand{\hlSThreeBudgetburnA}{\tbd{hlSThreeBudgetburnA}}
\providecommand{\hlSThreeBudgetburnB}{\tbd{hlSThreeBudgetburnB}}
\providecommand{\hlSThreeBudgetburnCIHi}{\tbd{hlSThreeBudgetburnCIHi}}
\providecommand{\hlSThreeBudgetburnCILo}{\tbd{hlSThreeBudgetburnCILo}}
\providecommand{\hlSThreeBudgetburnEst}{\tbd{hlSThreeBudgetburnEst}}
\providecommand{\hlSThreeBudgetburnN}{\tbd{hlSThreeBudgetburnN}}
\providecommand{\hlSThreeBudgetflairA}{\tbd{hlSThreeBudgetflairA}}
\providecommand{\hlSThreeBudgetflairB}{\tbd{hlSThreeBudgetflairB}}
\providecommand{\hlSThreeBudgetflairCIHi}{\tbd{hlSThreeBudgetflairCIHi}}
\providecommand{\hlSThreeBudgetflairCILo}{\tbd{hlSThreeBudgetflairCILo}}
\providecommand{\hlSThreeBudgetflairEst}{\tbd{hlSThreeBudgetflairEst}}
\providecommand{\hlSThreeBudgetflairN}{\tbd{hlSThreeBudgetflairN}}
\providecommand{\hlSThreeDropDOFAChesA}{\tbd{hlSThreeDropDOFAChesA}}
\providecommand{\hlSThreeDropDOFAChesB}{\tbd{hlSThreeDropDOFAChesB}}
\providecommand{\hlSThreeDropDOFAChesCIHi}{\tbd{hlSThreeDropDOFAChesCIHi}}
\providecommand{\hlSThreeDropDOFAChesCILo}{\tbd{hlSThreeDropDOFAChesCILo}}
\providecommand{\hlSThreeDropDOFAChesEst}{\tbd{hlSThreeDropDOFAChesEst}}
\providecommand{\hlSThreeDropDOFAChesFlag}{\tbd{hlSThreeDropDOFAChesFlag}}
\providecommand{\hlSThreeDropDOFAChesMde}{\tbd{hlSThreeDropDOFAChesMde}}
\providecommand{\hlSThreeDropDOFAChesN}{\tbd{hlSThreeDropDOFAChesN}}
\providecommand{\hlSThreeDropDOFAChesTostCIHi}{\tbd{hlSThreeDropDOFAChesTostCIHi}}
\providecommand{\hlSThreeDropDOFAChesTostCILo}{\tbd{hlSThreeDropDOFAChesTostCILo}}
\providecommand{\hlSThreeDropDOFAChesVerdict}{\tbd{hlSThreeDropDOFAChesVerdict}}
\providecommand{\hlSThreeDropDOFACsTwelveA}{\tbd{hlSThreeDropDOFACsTwelveA}}
\providecommand{\hlSThreeDropDOFACsTwelveB}{\tbd{hlSThreeDropDOFACsTwelveB}}
\providecommand{\hlSThreeDropDOFACsTwelveCIHi}{\tbd{hlSThreeDropDOFACsTwelveCIHi}}
\providecommand{\hlSThreeDropDOFACsTwelveCILo}{\tbd{hlSThreeDropDOFACsTwelveCILo}}
\providecommand{\hlSThreeDropDOFACsTwelveEst}{\tbd{hlSThreeDropDOFACsTwelveEst}}
\providecommand{\hlSThreeDropDOFACsTwelveFlag}{\tbd{hlSThreeDropDOFACsTwelveFlag}}
\providecommand{\hlSThreeDropDOFACsTwelveMde}{\tbd{hlSThreeDropDOFACsTwelveMde}}
\providecommand{\hlSThreeDropDOFACsTwelveN}{\tbd{hlSThreeDropDOFACsTwelveN}}
\providecommand{\hlSThreeDropDOFACsTwelveTostCIHi}{\tbd{hlSThreeDropDOFACsTwelveTostCIHi}}
\providecommand{\hlSThreeDropDOFACsTwelveTostCILo}{\tbd{hlSThreeDropDOFACsTwelveTostCILo}}
\providecommand{\hlSThreeDropDOFACsTwelveVerdict}{\tbd{hlSThreeDropDOFACsTwelveVerdict}}
\providecommand{\hlSThreeDropDOFADfcA}{\tbd{hlSThreeDropDOFADfcA}}
\providecommand{\hlSThreeDropDOFADfcB}{\tbd{hlSThreeDropDOFADfcB}}
\providecommand{\hlSThreeDropDOFADfcCIHi}{\tbd{hlSThreeDropDOFADfcCIHi}}
\providecommand{\hlSThreeDropDOFADfcCILo}{\tbd{hlSThreeDropDOFADfcCILo}}
\providecommand{\hlSThreeDropDOFADfcEst}{\tbd{hlSThreeDropDOFADfcEst}}
\providecommand{\hlSThreeDropDOFADfcFlag}{\tbd{hlSThreeDropDOFADfcFlag}}
\providecommand{\hlSThreeDropDOFADfcMde}{\tbd{hlSThreeDropDOFADfcMde}}
\providecommand{\hlSThreeDropDOFADfcN}{\tbd{hlSThreeDropDOFADfcN}}
\providecommand{\hlSThreeDropDOFADfcTostCIHi}{\tbd{hlSThreeDropDOFADfcTostCIHi}}
\providecommand{\hlSThreeDropDOFADfcTostCILo}{\tbd{hlSThreeDropDOFADfcTostCILo}}
\providecommand{\hlSThreeDropDOFADfcVerdict}{\tbd{hlSThreeDropDOFADfcVerdict}}
\providecommand{\hlSThreeDropDOFAEnvaA}{\tbd{hlSThreeDropDOFAEnvaA}}
\providecommand{\hlSThreeDropDOFAEnvaB}{\tbd{hlSThreeDropDOFAEnvaB}}
\providecommand{\hlSThreeDropDOFAEnvaCIHi}{\tbd{hlSThreeDropDOFAEnvaCIHi}}
\providecommand{\hlSThreeDropDOFAEnvaCILo}{\tbd{hlSThreeDropDOFAEnvaCILo}}
\providecommand{\hlSThreeDropDOFAEnvaEst}{\tbd{hlSThreeDropDOFAEnvaEst}}
\providecommand{\hlSThreeDropDOFAEnvaFlag}{\tbd{hlSThreeDropDOFAEnvaFlag}}
\providecommand{\hlSThreeDropDOFAEnvaMde}{\tbd{hlSThreeDropDOFAEnvaMde}}
\providecommand{\hlSThreeDropDOFAEnvaN}{\tbd{hlSThreeDropDOFAEnvaN}}
\providecommand{\hlSThreeDropDOFAEnvaTostCIHi}{\tbd{hlSThreeDropDOFAEnvaTostCIHi}}
\providecommand{\hlSThreeDropDOFAEnvaTostCILo}{\tbd{hlSThreeDropDOFAEnvaTostCILo}}
\providecommand{\hlSThreeDropDOFAEnvaVerdict}{\tbd{hlSThreeDropDOFAEnvaVerdict}}
\providecommand{\hlSThreeDropDOFAInDomDatasets}{\tbd{hlSThreeDropDOFAInDomDatasets}}
\providecommand{\hlSThreeDropDOFAInDomDiffer}{\tbd{hlSThreeDropDOFAInDomDiffer}}
\providecommand{\hlSThreeDropDOFAInDomEquiv}{\tbd{hlSThreeDropDOFAInDomEquiv}}
\providecommand{\hlSThreeDropDOFAInDomRead}{\tbd{hlSThreeDropDOFAInDomRead}}
\providecommand{\hlSThreeDropDOFAInDomUndet}{\tbd{hlSThreeDropDOFAInDomUndet}}
\providecommand{\hlSThreeDropDOFAKuroA}{\tbd{hlSThreeDropDOFAKuroA}}
\providecommand{\hlSThreeDropDOFAKuroB}{\tbd{hlSThreeDropDOFAKuroB}}
\providecommand{\hlSThreeDropDOFAKuroCIHi}{\tbd{hlSThreeDropDOFAKuroCIHi}}
\providecommand{\hlSThreeDropDOFAKuroCILo}{\tbd{hlSThreeDropDOFAKuroCILo}}
\providecommand{\hlSThreeDropDOFAKuroEst}{\tbd{hlSThreeDropDOFAKuroEst}}
\providecommand{\hlSThreeDropDOFAKuroFlag}{\tbd{hlSThreeDropDOFAKuroFlag}}
\providecommand{\hlSThreeDropDOFAKuroMde}{\tbd{hlSThreeDropDOFAKuroMde}}
\providecommand{\hlSThreeDropDOFAKuroN}{\tbd{hlSThreeDropDOFAKuroN}}
\providecommand{\hlSThreeDropDOFAKuroTostCIHi}{\tbd{hlSThreeDropDOFAKuroTostCIHi}}
\providecommand{\hlSThreeDropDOFAKuroTostCILo}{\tbd{hlSThreeDropDOFAKuroTostCILo}}
\providecommand{\hlSThreeDropDOFAKuroVerdict}{\tbd{hlSThreeDropDOFAKuroVerdict}}
\providecommand{\hlSThreeDropDOFANoPreDatasets}{\tbd{hlSThreeDropDOFANoPreDatasets}}
\providecommand{\hlSThreeDropDOFANoPreDiffer}{\tbd{hlSThreeDropDOFANoPreDiffer}}
\providecommand{\hlSThreeDropDOFANoPreEquiv}{\tbd{hlSThreeDropDOFANoPreEquiv}}
\providecommand{\hlSThreeDropDOFANoPreRead}{\tbd{hlSThreeDropDOFANoPreRead}}
\providecommand{\hlSThreeDropDOFANoPreUndet}{\tbd{hlSThreeDropDOFANoPreUndet}}
\providecommand{\hlSThreeDropDOFAOemA}{\tbd{hlSThreeDropDOFAOemA}}
\providecommand{\hlSThreeDropDOFAOemB}{\tbd{hlSThreeDropDOFAOemB}}
\providecommand{\hlSThreeDropDOFAOemCIHi}{\tbd{hlSThreeDropDOFAOemCIHi}}
\providecommand{\hlSThreeDropDOFAOemCILo}{\tbd{hlSThreeDropDOFAOemCILo}}
\providecommand{\hlSThreeDropDOFAOemEst}{\tbd{hlSThreeDropDOFAOemEst}}
\providecommand{\hlSThreeDropDOFAOemFlag}{\tbd{hlSThreeDropDOFAOemFlag}}
\providecommand{\hlSThreeDropDOFAOemMde}{\tbd{hlSThreeDropDOFAOemMde}}
\providecommand{\hlSThreeDropDOFAOemN}{\tbd{hlSThreeDropDOFAOemN}}
\providecommand{\hlSThreeDropDOFAOemTostCIHi}{\tbd{hlSThreeDropDOFAOemTostCIHi}}
\providecommand{\hlSThreeDropDOFAOemTostCILo}{\tbd{hlSThreeDropDOFAOemTostCILo}}
\providecommand{\hlSThreeDropDOFAOemVerdict}{\tbd{hlSThreeDropDOFAOemVerdict}}
\providecommand{\hlSThreeDropDOFAOutDomDatasets}{\tbd{hlSThreeDropDOFAOutDomDatasets}}
\providecommand{\hlSThreeDropDOFAOutDomDiffer}{\tbd{hlSThreeDropDOFAOutDomDiffer}}
\providecommand{\hlSThreeDropDOFAOutDomEquiv}{\tbd{hlSThreeDropDOFAOutDomEquiv}}
\providecommand{\hlSThreeDropDOFAOutDomRead}{\tbd{hlSThreeDropDOFAOutDomRead}}
\providecommand{\hlSThreeDropDOFAOutDomUndet}{\tbd{hlSThreeDropDOFAOutDomUndet}}
\providecommand{\hlSThreeDropDOFASnTwoA}{\tbd{hlSThreeDropDOFASnTwoA}}
\providecommand{\hlSThreeDropDOFASnTwoB}{\tbd{hlSThreeDropDOFASnTwoB}}
\providecommand{\hlSThreeDropDOFASnTwoCIHi}{\tbd{hlSThreeDropDOFASnTwoCIHi}}
\providecommand{\hlSThreeDropDOFASnTwoCILo}{\tbd{hlSThreeDropDOFASnTwoCILo}}
\providecommand{\hlSThreeDropDOFASnTwoEst}{\tbd{hlSThreeDropDOFASnTwoEst}}
\providecommand{\hlSThreeDropDOFASnTwoFlag}{\tbd{hlSThreeDropDOFASnTwoFlag}}
\providecommand{\hlSThreeDropDOFASnTwoMde}{\tbd{hlSThreeDropDOFASnTwoMde}}
\providecommand{\hlSThreeDropDOFASnTwoN}{\tbd{hlSThreeDropDOFASnTwoN}}
\providecommand{\hlSThreeDropDOFASnTwoTostCIHi}{\tbd{hlSThreeDropDOFASnTwoTostCIHi}}
\providecommand{\hlSThreeDropDOFASnTwoTostCILo}{\tbd{hlSThreeDropDOFASnTwoTostCILo}}
\providecommand{\hlSThreeDropDOFASnTwoVerdict}{\tbd{hlSThreeDropDOFASnTwoVerdict}}
\providecommand{\hlSThreeDropDOFAburnA}{\tbd{hlSThreeDropDOFAburnA}}
\providecommand{\hlSThreeDropDOFAburnB}{\tbd{hlSThreeDropDOFAburnB}}
\providecommand{\hlSThreeDropDOFAburnCIHi}{\tbd{hlSThreeDropDOFAburnCIHi}}
\providecommand{\hlSThreeDropDOFAburnCILo}{\tbd{hlSThreeDropDOFAburnCILo}}
\providecommand{\hlSThreeDropDOFAburnEst}{\tbd{hlSThreeDropDOFAburnEst}}
\providecommand{\hlSThreeDropDOFAburnN}{\tbd{hlSThreeDropDOFAburnN}}
\providecommand{\hlSThreeDropDOFAflairA}{\tbd{hlSThreeDropDOFAflairA}}
\providecommand{\hlSThreeDropDOFAflairB}{\tbd{hlSThreeDropDOFAflairB}}
\providecommand{\hlSThreeDropDOFAflairCIHi}{\tbd{hlSThreeDropDOFAflairCIHi}}
\providecommand{\hlSThreeDropDOFAflairCILo}{\tbd{hlSThreeDropDOFAflairCILo}}
\providecommand{\hlSThreeDropDOFAflairEst}{\tbd{hlSThreeDropDOFAflairEst}}
\providecommand{\hlSThreeDropDOFAflairN}{\tbd{hlSThreeDropDOFAflairN}}
\providecommand{\hlSThreeRetDOFAburnA}{\tbd{hlSThreeRetDOFAburnA}}
\providecommand{\hlSThreeRetDOFAburnB}{\tbd{hlSThreeRetDOFAburnB}}
\providecommand{\hlSThreeRetDOFAburnCIHi}{\tbd{hlSThreeRetDOFAburnCIHi}}
\providecommand{\hlSThreeRetDOFAburnCILo}{\tbd{hlSThreeRetDOFAburnCILo}}
\providecommand{\hlSThreeRetDOFAburnEst}{\tbd{hlSThreeRetDOFAburnEst}}
\providecommand{\hlSThreeRetDOFAburnN}{\tbd{hlSThreeRetDOFAburnN}}
\providecommand{\hlSThreeRetDOFAflairA}{\tbd{hlSThreeRetDOFAflairA}}
\providecommand{\hlSThreeRetDOFAflairB}{\tbd{hlSThreeRetDOFAflairB}}
\providecommand{\hlSThreeRetDOFAflairCIHi}{\tbd{hlSThreeRetDOFAflairCIHi}}
\providecommand{\hlSThreeRetDOFAflairCILo}{\tbd{hlSThreeRetDOFAflairCILo}}
\providecommand{\hlSThreeRetDOFAflairEst}{\tbd{hlSThreeRetDOFAflairEst}}
\providecommand{\hlSThreeRetDOFAflairN}{\tbd{hlSThreeRetDOFAflairN}}
\providecommand{\hlSTwoDeltaRNflairA}{\tbd{hlSTwoDeltaRNflairA}}
\providecommand{\hlSTwoDeltaRNflairB}{\tbd{hlSTwoDeltaRNflairB}}
\providecommand{\hlSTwoDeltaRNflairCIHi}{\tbd{hlSTwoDeltaRNflairCIHi}}
\providecommand{\hlSTwoDeltaRNflairCILo}{\tbd{hlSTwoDeltaRNflairCILo}}
\providecommand{\hlSTwoDeltaRNflairEst}{\tbd{hlSTwoDeltaRNflairEst}}
\providecommand{\hlSTwoDeltaRNflairN}{\tbd{hlSTwoDeltaRNflairN}}
\providecommand{\hlSTwoDeltaSATflairA}{\tbd{hlSTwoDeltaSATflairA}}
\providecommand{\hlSTwoDeltaSATflairB}{\tbd{hlSTwoDeltaSATflairB}}
\providecommand{\hlSTwoDeltaSATflairCIHi}{\tbd{hlSTwoDeltaSATflairCIHi}}
\providecommand{\hlSTwoDeltaSATflairCILo}{\tbd{hlSTwoDeltaSATflairCILo}}
\providecommand{\hlSTwoDeltaSATflairEst}{\tbd{hlSTwoDeltaSATflairEst}}
\providecommand{\hlSTwoDeltaSATflairN}{\tbd{hlSTwoDeltaSATflairN}}
\providecommand{\hlSeedExtFOneAllburnCIHi}{\tbd{hlSeedExtFOneAllburnCIHi}}
\providecommand{\hlSeedExtFOneAllburnCILo}{\tbd{hlSeedExtFOneAllburnCILo}}
\providecommand{\hlSeedExtFOneAllburnEst}{\tbd{hlSeedExtFOneAllburnEst}}
\providecommand{\hlSeedExtFOneAllburnMde}{\tbd{hlSeedExtFOneAllburnMde}}
\providecommand{\hlSeedExtFOneAllburnN}{\tbd{hlSeedExtFOneAllburnN}}
\providecommand{\hlSeedExtFOneAllburnPHolm}{\tbd{hlSeedExtFOneAllburnPHolm}}
\providecommand{\hlSeedExtFOneAllburnTostCIHi}{\tbd{hlSeedExtFOneAllburnTostCIHi}}
\providecommand{\hlSeedExtFOneAllburnTostCILo}{\tbd{hlSeedExtFOneAllburnTostCILo}}
\providecommand{\hlSeedExtFOneAllflairCIHi}{\tbd{hlSeedExtFOneAllflairCIHi}}
\providecommand{\hlSeedExtFOneAllflairCILo}{\tbd{hlSeedExtFOneAllflairCILo}}
\providecommand{\hlSeedExtFOneAllflairEst}{\tbd{hlSeedExtFOneAllflairEst}}
\providecommand{\hlSeedExtFOneAllflairMde}{\tbd{hlSeedExtFOneAllflairMde}}
\providecommand{\hlSeedExtFOneAllflairN}{\tbd{hlSeedExtFOneAllflairN}}
\providecommand{\hlSeedExtFOneAllflairPHolm}{\tbd{hlSeedExtFOneAllflairPHolm}}
\providecommand{\hlSeedExtFOneAllflairTostCIHi}{\tbd{hlSeedExtFOneAllflairTostCIHi}}
\providecommand{\hlSeedExtFOneAllflairTostCILo}{\tbd{hlSeedExtFOneAllflairTostCILo}}
\providecommand{\hlSeedExtFOneFiveburnCIHi}{\tbd{hlSeedExtFOneFiveburnCIHi}}
\providecommand{\hlSeedExtFOneFiveburnCILo}{\tbd{hlSeedExtFOneFiveburnCILo}}
\providecommand{\hlSeedExtFOneFiveburnEst}{\tbd{hlSeedExtFOneFiveburnEst}}
\providecommand{\hlSeedExtFOneFiveburnMde}{\tbd{hlSeedExtFOneFiveburnMde}}
\providecommand{\hlSeedExtFOneFiveburnN}{\tbd{hlSeedExtFOneFiveburnN}}
\providecommand{\hlSeedExtFOneFiveburnPHolm}{\tbd{hlSeedExtFOneFiveburnPHolm}}
\providecommand{\hlSeedExtFOneFiveburnTostCIHi}{\tbd{hlSeedExtFOneFiveburnTostCIHi}}
\providecommand{\hlSeedExtFOneFiveburnTostCILo}{\tbd{hlSeedExtFOneFiveburnTostCILo}}
\providecommand{\hlSeedExtFOneFiveflairCIHi}{\tbd{hlSeedExtFOneFiveflairCIHi}}
\providecommand{\hlSeedExtFOneFiveflairCILo}{\tbd{hlSeedExtFOneFiveflairCILo}}
\providecommand{\hlSeedExtFOneFiveflairEst}{\tbd{hlSeedExtFOneFiveflairEst}}
\providecommand{\hlSeedExtFOneFiveflairMde}{\tbd{hlSeedExtFOneFiveflairMde}}
\providecommand{\hlSeedExtFOneFiveflairN}{\tbd{hlSeedExtFOneFiveflairN}}
\providecommand{\hlSeedExtFOneFiveflairPHolm}{\tbd{hlSeedExtFOneFiveflairPHolm}}
\providecommand{\hlSeedExtFOneFiveflairTostCIHi}{\tbd{hlSeedExtFOneFiveflairTostCIHi}}
\providecommand{\hlSeedExtFOneFiveflairTostCILo}{\tbd{hlSeedExtFOneFiveflairTostCILo}}
\providecommand{\hlSeedExtFTwoAllburnCIHi}{\tbd{hlSeedExtFTwoAllburnCIHi}}
\providecommand{\hlSeedExtFTwoAllburnCILo}{\tbd{hlSeedExtFTwoAllburnCILo}}
\providecommand{\hlSeedExtFTwoAllburnEst}{\tbd{hlSeedExtFTwoAllburnEst}}
\providecommand{\hlSeedExtFTwoAllburnMde}{\tbd{hlSeedExtFTwoAllburnMde}}
\providecommand{\hlSeedExtFTwoAllburnN}{\tbd{hlSeedExtFTwoAllburnN}}
\providecommand{\hlSeedExtFTwoAllburnPHolm}{\tbd{hlSeedExtFTwoAllburnPHolm}}
\providecommand{\hlSeedExtFTwoAllburnTostCIHi}{\tbd{hlSeedExtFTwoAllburnTostCIHi}}
\providecommand{\hlSeedExtFTwoAllburnTostCILo}{\tbd{hlSeedExtFTwoAllburnTostCILo}}
\providecommand{\hlSeedExtFTwoAllflairCIHi}{\tbd{hlSeedExtFTwoAllflairCIHi}}
\providecommand{\hlSeedExtFTwoAllflairCILo}{\tbd{hlSeedExtFTwoAllflairCILo}}
\providecommand{\hlSeedExtFTwoAllflairEst}{\tbd{hlSeedExtFTwoAllflairEst}}
\providecommand{\hlSeedExtFTwoAllflairMde}{\tbd{hlSeedExtFTwoAllflairMde}}
\providecommand{\hlSeedExtFTwoAllflairN}{\tbd{hlSeedExtFTwoAllflairN}}
\providecommand{\hlSeedExtFTwoAllflairPHolm}{\tbd{hlSeedExtFTwoAllflairPHolm}}
\providecommand{\hlSeedExtFTwoAllflairTostCIHi}{\tbd{hlSeedExtFTwoAllflairTostCIHi}}
\providecommand{\hlSeedExtFTwoAllflairTostCILo}{\tbd{hlSeedExtFTwoAllflairTostCILo}}
\providecommand{\hlSeedExtFTwoFiveburnCIHi}{\tbd{hlSeedExtFTwoFiveburnCIHi}}
\providecommand{\hlSeedExtFTwoFiveburnCILo}{\tbd{hlSeedExtFTwoFiveburnCILo}}
\providecommand{\hlSeedExtFTwoFiveburnEst}{\tbd{hlSeedExtFTwoFiveburnEst}}
\providecommand{\hlSeedExtFTwoFiveburnMde}{\tbd{hlSeedExtFTwoFiveburnMde}}
\providecommand{\hlSeedExtFTwoFiveburnN}{\tbd{hlSeedExtFTwoFiveburnN}}
\providecommand{\hlSeedExtFTwoFiveburnPHolm}{\tbd{hlSeedExtFTwoFiveburnPHolm}}
\providecommand{\hlSeedExtFTwoFiveburnTostCIHi}{\tbd{hlSeedExtFTwoFiveburnTostCIHi}}
\providecommand{\hlSeedExtFTwoFiveburnTostCILo}{\tbd{hlSeedExtFTwoFiveburnTostCILo}}
\providecommand{\hlSeedExtFTwoFiveflairCIHi}{\tbd{hlSeedExtFTwoFiveflairCIHi}}
\providecommand{\hlSeedExtFTwoFiveflairCILo}{\tbd{hlSeedExtFTwoFiveflairCILo}}
\providecommand{\hlSeedExtFTwoFiveflairEst}{\tbd{hlSeedExtFTwoFiveflairEst}}
\providecommand{\hlSeedExtFTwoFiveflairMde}{\tbd{hlSeedExtFTwoFiveflairMde}}
\providecommand{\hlSeedExtFTwoFiveflairN}{\tbd{hlSeedExtFTwoFiveflairN}}
\providecommand{\hlSeedExtFTwoFiveflairPHolm}{\tbd{hlSeedExtFTwoFiveflairPHolm}}
\providecommand{\hlSeedExtFTwoFiveflairTostCIHi}{\tbd{hlSeedExtFTwoFiveflairTostCIHi}}
\providecommand{\hlSeedExtFTwoFiveflairTostCILo}{\tbd{hlSeedExtFTwoFiveflairTostCILo}}
\providecommand{\hlSeedExtNDOFAburn}{\tbd{hlSeedExtNDOFAburn}}
\providecommand{\hlSeedExtNDOFAflair}{\tbd{hlSeedExtNDOFAflair}}
\providecommand{\hlSeedExtNLVDburn}{\tbd{hlSeedExtNLVDburn}}
\providecommand{\hlSeedExtNLVDflair}{\tbd{hlSeedExtNLVDflair}}
\providecommand{\hlSeedExtNRNburn}{\tbd{hlSeedExtNRNburn}}
\providecommand{\hlSeedExtNRNflair}{\tbd{hlSeedExtNRNflair}}
\providecommand{\hlSeedExtNSATburn}{\tbd{hlSeedExtNSATburn}}
\providecommand{\hlSeedExtNSATflair}{\tbd{hlSeedExtNSATflair}}
\providecommand{\hlSeedExtNTMburn}{\tbd{hlSeedExtNTMburn}}
\providecommand{\hlSeedExtNTMflair}{\tbd{hlSeedExtNTMflair}}
\providecommand{\hlSeedExtraBlocks}{\tbd{hlSeedExtraBlocks}}
\providecommand{\hlSeedExtraCellsN}{\tbd{hlSeedExtraCellsN}}
\providecommand{\hlSeedExtraCellsburn}{\tbd{hlSeedExtraCellsburn}}
\providecommand{\hlSeedExtraCellsflair}{\tbd{hlSeedExtraCellsflair}}
\providecommand{\hlSeedExtraSeeds}{\tbd{hlSeedExtraSeeds}}
\providecommand{\hlTypeRankChesFour}{\tbd{hlTypeRankChesFour}}
\providecommand{\hlTypeRankChesOne}{\tbd{hlTypeRankChesOne}}
\providecommand{\hlTypeRankChesThree}{\tbd{hlTypeRankChesThree}}
\providecommand{\hlTypeRankChesTwo}{\tbd{hlTypeRankChesTwo}}
\providecommand{\hlTypeRankCsTwelveFour}{\tbd{hlTypeRankCsTwelveFour}}
\providecommand{\hlTypeRankCsTwelveOne}{\tbd{hlTypeRankCsTwelveOne}}
\providecommand{\hlTypeRankCsTwelveThree}{\tbd{hlTypeRankCsTwelveThree}}
\providecommand{\hlTypeRankCsTwelveTwo}{\tbd{hlTypeRankCsTwelveTwo}}
\providecommand{\hlTypeRankDfcFour}{\tbd{hlTypeRankDfcFour}}
\providecommand{\hlTypeRankDfcOne}{\tbd{hlTypeRankDfcOne}}
\providecommand{\hlTypeRankDfcThree}{\tbd{hlTypeRankDfcThree}}
\providecommand{\hlTypeRankDfcTwo}{\tbd{hlTypeRankDfcTwo}}
\providecommand{\hlTypeRankDiffCIHiChesOne}{\tbd{hlTypeRankDiffCIHiChesOne}}
\providecommand{\hlTypeRankDiffCIHiChesThree}{\tbd{hlTypeRankDiffCIHiChesThree}}
\providecommand{\hlTypeRankDiffCIHiChesTwo}{\tbd{hlTypeRankDiffCIHiChesTwo}}
\providecommand{\hlTypeRankDiffCIHiCsTwelveOne}{\tbd{hlTypeRankDiffCIHiCsTwelveOne}}
\providecommand{\hlTypeRankDiffCIHiCsTwelveThree}{\tbd{hlTypeRankDiffCIHiCsTwelveThree}}
\providecommand{\hlTypeRankDiffCIHiCsTwelveTwo}{\tbd{hlTypeRankDiffCIHiCsTwelveTwo}}
\providecommand{\hlTypeRankDiffCIHiDfcOne}{\tbd{hlTypeRankDiffCIHiDfcOne}}
\providecommand{\hlTypeRankDiffCIHiDfcThree}{\tbd{hlTypeRankDiffCIHiDfcThree}}
\providecommand{\hlTypeRankDiffCIHiDfcTwo}{\tbd{hlTypeRankDiffCIHiDfcTwo}}
\providecommand{\hlTypeRankDiffCIHiEnvaOne}{\tbd{hlTypeRankDiffCIHiEnvaOne}}
\providecommand{\hlTypeRankDiffCIHiEnvaThree}{\tbd{hlTypeRankDiffCIHiEnvaThree}}
\providecommand{\hlTypeRankDiffCIHiEnvaTwo}{\tbd{hlTypeRankDiffCIHiEnvaTwo}}
\providecommand{\hlTypeRankDiffCIHiKuroOne}{\tbd{hlTypeRankDiffCIHiKuroOne}}
\providecommand{\hlTypeRankDiffCIHiKuroThree}{\tbd{hlTypeRankDiffCIHiKuroThree}}
\providecommand{\hlTypeRankDiffCIHiKuroTwo}{\tbd{hlTypeRankDiffCIHiKuroTwo}}
\providecommand{\hlTypeRankDiffCIHiOemOne}{\tbd{hlTypeRankDiffCIHiOemOne}}
\providecommand{\hlTypeRankDiffCIHiOemThree}{\tbd{hlTypeRankDiffCIHiOemThree}}
\providecommand{\hlTypeRankDiffCIHiOemTwo}{\tbd{hlTypeRankDiffCIHiOemTwo}}
\providecommand{\hlTypeRankDiffCIHiSnTwoOne}{\tbd{hlTypeRankDiffCIHiSnTwoOne}}
\providecommand{\hlTypeRankDiffCIHiSnTwoThree}{\tbd{hlTypeRankDiffCIHiSnTwoThree}}
\providecommand{\hlTypeRankDiffCIHiSnTwoTwo}{\tbd{hlTypeRankDiffCIHiSnTwoTwo}}
\providecommand{\hlTypeRankDiffCIHiburnOne}{\tbd{hlTypeRankDiffCIHiburnOne}}
\providecommand{\hlTypeRankDiffCIHiburnThree}{\tbd{hlTypeRankDiffCIHiburnThree}}
\providecommand{\hlTypeRankDiffCIHiburnTwo}{\tbd{hlTypeRankDiffCIHiburnTwo}}
\providecommand{\hlTypeRankDiffCIHiflairOne}{\tbd{hlTypeRankDiffCIHiflairOne}}
\providecommand{\hlTypeRankDiffCIHiflairThree}{\tbd{hlTypeRankDiffCIHiflairThree}}
\providecommand{\hlTypeRankDiffCIHiflairTwo}{\tbd{hlTypeRankDiffCIHiflairTwo}}
\providecommand{\hlTypeRankDiffCILoChesOne}{\tbd{hlTypeRankDiffCILoChesOne}}
\providecommand{\hlTypeRankDiffCILoChesThree}{\tbd{hlTypeRankDiffCILoChesThree}}
\providecommand{\hlTypeRankDiffCILoChesTwo}{\tbd{hlTypeRankDiffCILoChesTwo}}
\providecommand{\hlTypeRankDiffCILoCsTwelveOne}{\tbd{hlTypeRankDiffCILoCsTwelveOne}}
\providecommand{\hlTypeRankDiffCILoCsTwelveThree}{\tbd{hlTypeRankDiffCILoCsTwelveThree}}
\providecommand{\hlTypeRankDiffCILoCsTwelveTwo}{\tbd{hlTypeRankDiffCILoCsTwelveTwo}}
\providecommand{\hlTypeRankDiffCILoDfcOne}{\tbd{hlTypeRankDiffCILoDfcOne}}
\providecommand{\hlTypeRankDiffCILoDfcThree}{\tbd{hlTypeRankDiffCILoDfcThree}}
\providecommand{\hlTypeRankDiffCILoDfcTwo}{\tbd{hlTypeRankDiffCILoDfcTwo}}
\providecommand{\hlTypeRankDiffCILoEnvaOne}{\tbd{hlTypeRankDiffCILoEnvaOne}}
\providecommand{\hlTypeRankDiffCILoEnvaThree}{\tbd{hlTypeRankDiffCILoEnvaThree}}
\providecommand{\hlTypeRankDiffCILoEnvaTwo}{\tbd{hlTypeRankDiffCILoEnvaTwo}}
\providecommand{\hlTypeRankDiffCILoKuroOne}{\tbd{hlTypeRankDiffCILoKuroOne}}
\providecommand{\hlTypeRankDiffCILoKuroThree}{\tbd{hlTypeRankDiffCILoKuroThree}}
\providecommand{\hlTypeRankDiffCILoKuroTwo}{\tbd{hlTypeRankDiffCILoKuroTwo}}
\providecommand{\hlTypeRankDiffCILoOemOne}{\tbd{hlTypeRankDiffCILoOemOne}}
\providecommand{\hlTypeRankDiffCILoOemThree}{\tbd{hlTypeRankDiffCILoOemThree}}
\providecommand{\hlTypeRankDiffCILoOemTwo}{\tbd{hlTypeRankDiffCILoOemTwo}}
\providecommand{\hlTypeRankDiffCILoSnTwoOne}{\tbd{hlTypeRankDiffCILoSnTwoOne}}
\providecommand{\hlTypeRankDiffCILoSnTwoThree}{\tbd{hlTypeRankDiffCILoSnTwoThree}}
\providecommand{\hlTypeRankDiffCILoSnTwoTwo}{\tbd{hlTypeRankDiffCILoSnTwoTwo}}
\providecommand{\hlTypeRankDiffCILoburnOne}{\tbd{hlTypeRankDiffCILoburnOne}}
\providecommand{\hlTypeRankDiffCILoburnThree}{\tbd{hlTypeRankDiffCILoburnThree}}
\providecommand{\hlTypeRankDiffCILoburnTwo}{\tbd{hlTypeRankDiffCILoburnTwo}}
\providecommand{\hlTypeRankDiffCILoflairOne}{\tbd{hlTypeRankDiffCILoflairOne}}
\providecommand{\hlTypeRankDiffCILoflairThree}{\tbd{hlTypeRankDiffCILoflairThree}}
\providecommand{\hlTypeRankDiffCILoflairTwo}{\tbd{hlTypeRankDiffCILoflairTwo}}
\providecommand{\hlTypeRankDiffChesOne}{\tbd{hlTypeRankDiffChesOne}}
\providecommand{\hlTypeRankDiffChesThree}{\tbd{hlTypeRankDiffChesThree}}
\providecommand{\hlTypeRankDiffChesTwo}{\tbd{hlTypeRankDiffChesTwo}}
\providecommand{\hlTypeRankDiffCsTwelveOne}{\tbd{hlTypeRankDiffCsTwelveOne}}
\providecommand{\hlTypeRankDiffCsTwelveThree}{\tbd{hlTypeRankDiffCsTwelveThree}}
\providecommand{\hlTypeRankDiffCsTwelveTwo}{\tbd{hlTypeRankDiffCsTwelveTwo}}
\providecommand{\hlTypeRankDiffDfcOne}{\tbd{hlTypeRankDiffDfcOne}}
\providecommand{\hlTypeRankDiffDfcThree}{\tbd{hlTypeRankDiffDfcThree}}
\providecommand{\hlTypeRankDiffDfcTwo}{\tbd{hlTypeRankDiffDfcTwo}}
\providecommand{\hlTypeRankDiffEnvaOne}{\tbd{hlTypeRankDiffEnvaOne}}
\providecommand{\hlTypeRankDiffEnvaThree}{\tbd{hlTypeRankDiffEnvaThree}}
\providecommand{\hlTypeRankDiffEnvaTwo}{\tbd{hlTypeRankDiffEnvaTwo}}
\providecommand{\hlTypeRankDiffKuroOne}{\tbd{hlTypeRankDiffKuroOne}}
\providecommand{\hlTypeRankDiffKuroThree}{\tbd{hlTypeRankDiffKuroThree}}
\providecommand{\hlTypeRankDiffKuroTwo}{\tbd{hlTypeRankDiffKuroTwo}}
\providecommand{\hlTypeRankDiffOemOne}{\tbd{hlTypeRankDiffOemOne}}
\providecommand{\hlTypeRankDiffOemThree}{\tbd{hlTypeRankDiffOemThree}}
\providecommand{\hlTypeRankDiffOemTwo}{\tbd{hlTypeRankDiffOemTwo}}
\providecommand{\hlTypeRankDiffSnTwoOne}{\tbd{hlTypeRankDiffSnTwoOne}}
\providecommand{\hlTypeRankDiffSnTwoThree}{\tbd{hlTypeRankDiffSnTwoThree}}
\providecommand{\hlTypeRankDiffSnTwoTwo}{\tbd{hlTypeRankDiffSnTwoTwo}}
\providecommand{\hlTypeRankDiffburnOne}{\tbd{hlTypeRankDiffburnOne}}
\providecommand{\hlTypeRankDiffburnThree}{\tbd{hlTypeRankDiffburnThree}}
\providecommand{\hlTypeRankDiffburnTwo}{\tbd{hlTypeRankDiffburnTwo}}
\providecommand{\hlTypeRankDiffflairOne}{\tbd{hlTypeRankDiffflairOne}}
\providecommand{\hlTypeRankDiffflairThree}{\tbd{hlTypeRankDiffflairThree}}
\providecommand{\hlTypeRankDiffflairTwo}{\tbd{hlTypeRankDiffflairTwo}}
\providecommand{\hlTypeRankDropChesFour}{\tbd{hlTypeRankDropChesFour}}
\providecommand{\hlTypeRankDropChesOne}{\tbd{hlTypeRankDropChesOne}}
\providecommand{\hlTypeRankDropChesThree}{\tbd{hlTypeRankDropChesThree}}
\providecommand{\hlTypeRankDropChesTwo}{\tbd{hlTypeRankDropChesTwo}}
\providecommand{\hlTypeRankDropCsTwelveFour}{\tbd{hlTypeRankDropCsTwelveFour}}
\providecommand{\hlTypeRankDropCsTwelveOne}{\tbd{hlTypeRankDropCsTwelveOne}}
\providecommand{\hlTypeRankDropCsTwelveThree}{\tbd{hlTypeRankDropCsTwelveThree}}
\providecommand{\hlTypeRankDropCsTwelveTwo}{\tbd{hlTypeRankDropCsTwelveTwo}}
\providecommand{\hlTypeRankDropDfcFour}{\tbd{hlTypeRankDropDfcFour}}
\providecommand{\hlTypeRankDropDfcOne}{\tbd{hlTypeRankDropDfcOne}}
\providecommand{\hlTypeRankDropDfcThree}{\tbd{hlTypeRankDropDfcThree}}
\providecommand{\hlTypeRankDropDfcTwo}{\tbd{hlTypeRankDropDfcTwo}}
\providecommand{\hlTypeRankDropEnvaFour}{\tbd{hlTypeRankDropEnvaFour}}
\providecommand{\hlTypeRankDropEnvaOne}{\tbd{hlTypeRankDropEnvaOne}}
\providecommand{\hlTypeRankDropEnvaThree}{\tbd{hlTypeRankDropEnvaThree}}
\providecommand{\hlTypeRankDropEnvaTwo}{\tbd{hlTypeRankDropEnvaTwo}}
\providecommand{\hlTypeRankDropKuroFour}{\tbd{hlTypeRankDropKuroFour}}
\providecommand{\hlTypeRankDropKuroOne}{\tbd{hlTypeRankDropKuroOne}}
\providecommand{\hlTypeRankDropKuroThree}{\tbd{hlTypeRankDropKuroThree}}
\providecommand{\hlTypeRankDropKuroTwo}{\tbd{hlTypeRankDropKuroTwo}}
\providecommand{\hlTypeRankDropOemFour}{\tbd{hlTypeRankDropOemFour}}
\providecommand{\hlTypeRankDropOemOne}{\tbd{hlTypeRankDropOemOne}}
\providecommand{\hlTypeRankDropOemThree}{\tbd{hlTypeRankDropOemThree}}
\providecommand{\hlTypeRankDropOemTwo}{\tbd{hlTypeRankDropOemTwo}}
\providecommand{\hlTypeRankDropSnTwoFour}{\tbd{hlTypeRankDropSnTwoFour}}
\providecommand{\hlTypeRankDropSnTwoOne}{\tbd{hlTypeRankDropSnTwoOne}}
\providecommand{\hlTypeRankDropSnTwoThree}{\tbd{hlTypeRankDropSnTwoThree}}
\providecommand{\hlTypeRankDropSnTwoTwo}{\tbd{hlTypeRankDropSnTwoTwo}}
\providecommand{\hlTypeRankDropburnFour}{\tbd{hlTypeRankDropburnFour}}
\providecommand{\hlTypeRankDropburnOne}{\tbd{hlTypeRankDropburnOne}}
\providecommand{\hlTypeRankDropburnThree}{\tbd{hlTypeRankDropburnThree}}
\providecommand{\hlTypeRankDropburnTwo}{\tbd{hlTypeRankDropburnTwo}}
\providecommand{\hlTypeRankDropflairFour}{\tbd{hlTypeRankDropflairFour}}
\providecommand{\hlTypeRankDropflairOne}{\tbd{hlTypeRankDropflairOne}}
\providecommand{\hlTypeRankDropflairThree}{\tbd{hlTypeRankDropflairThree}}
\providecommand{\hlTypeRankDropflairTwo}{\tbd{hlTypeRankDropflairTwo}}
\providecommand{\hlTypeRankEnvaFour}{\tbd{hlTypeRankEnvaFour}}
\providecommand{\hlTypeRankEnvaOne}{\tbd{hlTypeRankEnvaOne}}
\providecommand{\hlTypeRankEnvaThree}{\tbd{hlTypeRankEnvaThree}}
\providecommand{\hlTypeRankEnvaTwo}{\tbd{hlTypeRankEnvaTwo}}
\providecommand{\hlTypeRankKuroFour}{\tbd{hlTypeRankKuroFour}}
\providecommand{\hlTypeRankKuroOne}{\tbd{hlTypeRankKuroOne}}
\providecommand{\hlTypeRankKuroThree}{\tbd{hlTypeRankKuroThree}}
\providecommand{\hlTypeRankKuroTwo}{\tbd{hlTypeRankKuroTwo}}
\providecommand{\hlTypeRankLOneChesFour}{\tbd{hlTypeRankLOneChesFour}}
\providecommand{\hlTypeRankLOneChesOne}{\tbd{hlTypeRankLOneChesOne}}
\providecommand{\hlTypeRankLOneChesThree}{\tbd{hlTypeRankLOneChesThree}}
\providecommand{\hlTypeRankLOneChesTwo}{\tbd{hlTypeRankLOneChesTwo}}
\providecommand{\hlTypeRankLOneCsTwelveFour}{\tbd{hlTypeRankLOneCsTwelveFour}}
\providecommand{\hlTypeRankLOneCsTwelveOne}{\tbd{hlTypeRankLOneCsTwelveOne}}
\providecommand{\hlTypeRankLOneCsTwelveThree}{\tbd{hlTypeRankLOneCsTwelveThree}}
\providecommand{\hlTypeRankLOneCsTwelveTwo}{\tbd{hlTypeRankLOneCsTwelveTwo}}
\providecommand{\hlTypeRankLOneDfcFour}{\tbd{hlTypeRankLOneDfcFour}}
\providecommand{\hlTypeRankLOneDfcOne}{\tbd{hlTypeRankLOneDfcOne}}
\providecommand{\hlTypeRankLOneDfcThree}{\tbd{hlTypeRankLOneDfcThree}}
\providecommand{\hlTypeRankLOneDfcTwo}{\tbd{hlTypeRankLOneDfcTwo}}
\providecommand{\hlTypeRankLOneEnvaFour}{\tbd{hlTypeRankLOneEnvaFour}}
\providecommand{\hlTypeRankLOneEnvaOne}{\tbd{hlTypeRankLOneEnvaOne}}
\providecommand{\hlTypeRankLOneEnvaThree}{\tbd{hlTypeRankLOneEnvaThree}}
\providecommand{\hlTypeRankLOneEnvaTwo}{\tbd{hlTypeRankLOneEnvaTwo}}
\providecommand{\hlTypeRankLOneKuroFour}{\tbd{hlTypeRankLOneKuroFour}}
\providecommand{\hlTypeRankLOneKuroOne}{\tbd{hlTypeRankLOneKuroOne}}
\providecommand{\hlTypeRankLOneKuroThree}{\tbd{hlTypeRankLOneKuroThree}}
\providecommand{\hlTypeRankLOneKuroTwo}{\tbd{hlTypeRankLOneKuroTwo}}
\providecommand{\hlTypeRankLOneOemFour}{\tbd{hlTypeRankLOneOemFour}}
\providecommand{\hlTypeRankLOneOemOne}{\tbd{hlTypeRankLOneOemOne}}
\providecommand{\hlTypeRankLOneOemThree}{\tbd{hlTypeRankLOneOemThree}}
\providecommand{\hlTypeRankLOneOemTwo}{\tbd{hlTypeRankLOneOemTwo}}
\providecommand{\hlTypeRankLOneSnTwoFour}{\tbd{hlTypeRankLOneSnTwoFour}}
\providecommand{\hlTypeRankLOneSnTwoOne}{\tbd{hlTypeRankLOneSnTwoOne}}
\providecommand{\hlTypeRankLOneSnTwoThree}{\tbd{hlTypeRankLOneSnTwoThree}}
\providecommand{\hlTypeRankLOneSnTwoTwo}{\tbd{hlTypeRankLOneSnTwoTwo}}
\providecommand{\hlTypeRankLOneburnFour}{\tbd{hlTypeRankLOneburnFour}}
\providecommand{\hlTypeRankLOneburnOne}{\tbd{hlTypeRankLOneburnOne}}
\providecommand{\hlTypeRankLOneburnThree}{\tbd{hlTypeRankLOneburnThree}}
\providecommand{\hlTypeRankLOneburnTwo}{\tbd{hlTypeRankLOneburnTwo}}
\providecommand{\hlTypeRankLOneflairFour}{\tbd{hlTypeRankLOneflairFour}}
\providecommand{\hlTypeRankLOneflairOne}{\tbd{hlTypeRankLOneflairOne}}
\providecommand{\hlTypeRankLOneflairThree}{\tbd{hlTypeRankLOneflairThree}}
\providecommand{\hlTypeRankLOneflairTwo}{\tbd{hlTypeRankLOneflairTwo}}
\providecommand{\hlTypeRankOemFour}{\tbd{hlTypeRankOemFour}}
\providecommand{\hlTypeRankOemOne}{\tbd{hlTypeRankOemOne}}
\providecommand{\hlTypeRankOemThree}{\tbd{hlTypeRankOemThree}}
\providecommand{\hlTypeRankOemTwo}{\tbd{hlTypeRankOemTwo}}
\providecommand{\hlTypeRankSnTwoFour}{\tbd{hlTypeRankSnTwoFour}}
\providecommand{\hlTypeRankSnTwoOne}{\tbd{hlTypeRankSnTwoOne}}
\providecommand{\hlTypeRankSnTwoThree}{\tbd{hlTypeRankSnTwoThree}}
\providecommand{\hlTypeRankSnTwoTwo}{\tbd{hlTypeRankSnTwoTwo}}
\providecommand{\hlTypeRankburnFour}{\tbd{hlTypeRankburnFour}}
\providecommand{\hlTypeRankburnOne}{\tbd{hlTypeRankburnOne}}
\providecommand{\hlTypeRankburnThree}{\tbd{hlTypeRankburnThree}}
\providecommand{\hlTypeRankburnTwo}{\tbd{hlTypeRankburnTwo}}
\providecommand{\hlTypeRankflairFour}{\tbd{hlTypeRankflairFour}}
\providecommand{\hlTypeRankflairOne}{\tbd{hlTypeRankflairOne}}
\providecommand{\hlTypeRankflairThree}{\tbd{hlTypeRankflairThree}}
\providecommand{\hlTypeRankflairTwo}{\tbd{hlTypeRankflairTwo}}
\providecommand{\hlVarBaseLeastburn}{\tbd{hlVarBaseLeastburn}}
\providecommand{\hlVarBaseLeastflair}{\tbd{hlVarBaseLeastflair}}
\providecommand{\hlVarBoundaryDilateburnBase}{\tbd{hlVarBoundaryDilateburnBase}}
\providecommand{\hlVarBoundaryDilateburnCIHi}{\tbd{hlVarBoundaryDilateburnCIHi}}
\providecommand{\hlVarBoundaryDilateburnCILo}{\tbd{hlVarBoundaryDilateburnCILo}}
\providecommand{\hlVarBoundaryDilateburnEst}{\tbd{hlVarBoundaryDilateburnEst}}
\providecommand{\hlVarBoundaryDilateburnMde}{\tbd{hlVarBoundaryDilateburnMde}}
\providecommand{\hlVarBoundaryDilateburnN}{\tbd{hlVarBoundaryDilateburnN}}
\providecommand{\hlVarBoundaryDilateburnTostCIHi}{\tbd{hlVarBoundaryDilateburnTostCIHi}}
\providecommand{\hlVarBoundaryDilateburnTostCILo}{\tbd{hlVarBoundaryDilateburnTostCILo}}
\providecommand{\hlVarBoundaryDilateburnVar}{\tbd{hlVarBoundaryDilateburnVar}}
\providecommand{\hlVarBoundaryDilateburnVerdict}{\tbd{hlVarBoundaryDilateburnVerdict}}
\providecommand{\hlVarBoundaryDilateflairBase}{\tbd{hlVarBoundaryDilateflairBase}}
\providecommand{\hlVarBoundaryDilateflairCIHi}{\tbd{hlVarBoundaryDilateflairCIHi}}
\providecommand{\hlVarBoundaryDilateflairCILo}{\tbd{hlVarBoundaryDilateflairCILo}}
\providecommand{\hlVarBoundaryDilateflairEst}{\tbd{hlVarBoundaryDilateflairEst}}
\providecommand{\hlVarBoundaryDilateflairMde}{\tbd{hlVarBoundaryDilateflairMde}}
\providecommand{\hlVarBoundaryDilateflairN}{\tbd{hlVarBoundaryDilateflairN}}
\providecommand{\hlVarBoundaryDilateflairTostCIHi}{\tbd{hlVarBoundaryDilateflairTostCIHi}}
\providecommand{\hlVarBoundaryDilateflairTostCILo}{\tbd{hlVarBoundaryDilateflairTostCILo}}
\providecommand{\hlVarBoundaryDilateflairVar}{\tbd{hlVarBoundaryDilateflairVar}}
\providecommand{\hlVarBoundaryDilateflairVerdict}{\tbd{hlVarBoundaryDilateflairVerdict}}
\providecommand{\hlVarDropBoundaryDilateburn}{\tbd{hlVarDropBoundaryDilateburn}}
\providecommand{\hlVarDropBoundaryDilateflair}{\tbd{hlVarDropBoundaryDilateflair}}
\providecommand{\hlVarDropCoarseburn}{\tbd{hlVarDropCoarseburn}}
\providecommand{\hlVarDropCoarseflair}{\tbd{hlVarDropCoarseflair}}
\providecommand{\hlVarDropOmissionburn}{\tbd{hlVarDropOmissionburn}}
\providecommand{\hlVarDropOmissionflair}{\tbd{hlVarDropOmissionflair}}
\providecommand{\hlVarDropShiftFixedburn}{\tbd{hlVarDropShiftFixedburn}}
\providecommand{\hlVarDropShiftFixedflair}{\tbd{hlVarDropShiftFixedflair}}
\providecommand{\hlVarGfmLeastburn}{\tbd{hlVarGfmLeastburn}}
\providecommand{\hlVarGfmLeastflair}{\tbd{hlVarGfmLeastflair}}
\providecommand{\hlVarGfmShiftLeastburn}{\tbd{hlVarGfmShiftLeastburn}}
\providecommand{\hlVarGfmShiftLeastflair}{\tbd{hlVarGfmShiftLeastflair}}
\providecommand{\hlVarLeastburn}{\tbd{hlVarLeastburn}}
\providecommand{\hlVarLeastflair}{\tbd{hlVarLeastflair}}
\providecommand{\hlVarRankRead}{\tbd{hlVarRankRead}}
\providecommand{\hlVarRankSameburn}{\tbd{hlVarRankSameburn}}
\providecommand{\hlVarRankSameflair}{\tbd{hlVarRankSameflair}}
\providecommand{\hlVarRankburnFour}{\tbd{hlVarRankburnFour}}
\providecommand{\hlVarRankburnOne}{\tbd{hlVarRankburnOne}}
\providecommand{\hlVarRankburnThree}{\tbd{hlVarRankburnThree}}
\providecommand{\hlVarRankburnTwo}{\tbd{hlVarRankburnTwo}}
\providecommand{\hlVarRankflairFour}{\tbd{hlVarRankflairFour}}
\providecommand{\hlVarRankflairOne}{\tbd{hlVarRankflairOne}}
\providecommand{\hlVarRankflairThree}{\tbd{hlVarRankflairThree}}
\providecommand{\hlVarRankflairTwo}{\tbd{hlVarRankflairTwo}}
\providecommand{\hlVarShiftFixedburnBase}{\tbd{hlVarShiftFixedburnBase}}
\providecommand{\hlVarShiftFixedburnCIHi}{\tbd{hlVarShiftFixedburnCIHi}}
\providecommand{\hlVarShiftFixedburnCILo}{\tbd{hlVarShiftFixedburnCILo}}
\providecommand{\hlVarShiftFixedburnEst}{\tbd{hlVarShiftFixedburnEst}}
\providecommand{\hlVarShiftFixedburnMde}{\tbd{hlVarShiftFixedburnMde}}
\providecommand{\hlVarShiftFixedburnN}{\tbd{hlVarShiftFixedburnN}}
\providecommand{\hlVarShiftFixedburnTostCIHi}{\tbd{hlVarShiftFixedburnTostCIHi}}
\providecommand{\hlVarShiftFixedburnTostCILo}{\tbd{hlVarShiftFixedburnTostCILo}}
\providecommand{\hlVarShiftFixedburnVar}{\tbd{hlVarShiftFixedburnVar}}
\providecommand{\hlVarShiftFixedburnVerdict}{\tbd{hlVarShiftFixedburnVerdict}}
\providecommand{\hlVarShiftFixedflairBase}{\tbd{hlVarShiftFixedflairBase}}
\providecommand{\hlVarShiftFixedflairCIHi}{\tbd{hlVarShiftFixedflairCIHi}}
\providecommand{\hlVarShiftFixedflairCILo}{\tbd{hlVarShiftFixedflairCILo}}
\providecommand{\hlVarShiftFixedflairEst}{\tbd{hlVarShiftFixedflairEst}}
\providecommand{\hlVarShiftFixedflairMde}{\tbd{hlVarShiftFixedflairMde}}
\providecommand{\hlVarShiftFixedflairN}{\tbd{hlVarShiftFixedflairN}}
\providecommand{\hlVarShiftFixedflairTostCIHi}{\tbd{hlVarShiftFixedflairTostCIHi}}
\providecommand{\hlVarShiftFixedflairTostCILo}{\tbd{hlVarShiftFixedflairTostCILo}}
\providecommand{\hlVarShiftFixedflairVar}{\tbd{hlVarShiftFixedflairVar}}
\providecommand{\hlVarShiftFixedflairVerdict}{\tbd{hlVarShiftFixedflairVerdict}}
\providecommand{\hlVarShiftLeastCount}{\tbd{hlVarShiftLeastCount}}
\providecommand{\hlVarShiftLeastburn}{\tbd{hlVarShiftLeastburn}}
\providecommand{\hlVarShiftLeastflair}{\tbd{hlVarShiftLeastflair}}
\providecommand{\hlVeDOFARNburnCIHi}{\tbd{hlVeDOFARNburnCIHi}}
\providecommand{\hlVeDOFARNburnCILo}{\tbd{hlVeDOFARNburnCILo}}
\providecommand{\hlVeDOFARNburnEst}{\tbd{hlVeDOFARNburnEst}}
\providecommand{\hlVeDOFARNburnN}{\tbd{hlVeDOFARNburnN}}
\providecommand{\hlVeDOFARNburnP}{\tbd{hlVeDOFARNburnP}}
\providecommand{\hlVeDOFARNflairCIHi}{\tbd{hlVeDOFARNflairCIHi}}
\providecommand{\hlVeDOFARNflairCILo}{\tbd{hlVeDOFARNflairCILo}}
\providecommand{\hlVeDOFARNflairEst}{\tbd{hlVeDOFARNflairEst}}
\providecommand{\hlVeDOFARNflairN}{\tbd{hlVeDOFARNflairN}}
\providecommand{\hlVeDOFARNflairP}{\tbd{hlVeDOFARNflairP}}
\providecommand{\hlVeFFourLOneburnCIHi}{\tbd{hlVeFFourLOneburnCIHi}}
\providecommand{\hlVeFFourLOneburnCILo}{\tbd{hlVeFFourLOneburnCILo}}
\providecommand{\hlVeFFourLOneburnEst}{\tbd{hlVeFFourLOneburnEst}}
\providecommand{\hlVeFFourLOneburnN}{\tbd{hlVeFFourLOneburnN}}
\providecommand{\hlVeFFourLOneburnP}{\tbd{hlVeFFourLOneburnP}}
\providecommand{\hlVeFFourLOneflairCIHi}{\tbd{hlVeFFourLOneflairCIHi}}
\providecommand{\hlVeFFourLOneflairCILo}{\tbd{hlVeFFourLOneflairCILo}}
\providecommand{\hlVeFFourLOneflairEst}{\tbd{hlVeFFourLOneflairEst}}
\providecommand{\hlVeFFourLOneflairN}{\tbd{hlVeFFourLOneflairN}}
\providecommand{\hlVeFFourLOneflairP}{\tbd{hlVeFFourLOneflairP}}
\providecommand{\hlVeFOneFiveburnCIHi}{\tbd{hlVeFOneFiveburnCIHi}}
\providecommand{\hlVeFOneFiveburnCILo}{\tbd{hlVeFOneFiveburnCILo}}
\providecommand{\hlVeFOneFiveburnEst}{\tbd{hlVeFOneFiveburnEst}}
\providecommand{\hlVeFOneFiveburnN}{\tbd{hlVeFOneFiveburnN}}
\providecommand{\hlVeFOneFiveburnP}{\tbd{hlVeFOneFiveburnP}}
\providecommand{\hlVeFOneFiveflairCIHi}{\tbd{hlVeFOneFiveflairCIHi}}
\providecommand{\hlVeFOneFiveflairCILo}{\tbd{hlVeFOneFiveflairCILo}}
\providecommand{\hlVeFOneFiveflairEst}{\tbd{hlVeFOneFiveflairEst}}
\providecommand{\hlVeFOneFiveflairN}{\tbd{hlVeFOneFiveflairN}}
\providecommand{\hlVeFOneFiveflairP}{\tbd{hlVeFOneFiveflairP}}
\providecommand{\hlVeFOneSignFlipburnEst}{\tbd{hlVeFOneSignFlipburnEst}}
\providecommand{\hlVeFOneSignFlipburnFloorFive}{\tbd{hlVeFOneSignFlipburnFloorFive}}
\providecommand{\hlVeFOneSignFlipburnN}{\tbd{hlVeFOneSignFlipburnN}}
\providecommand{\hlVeFOneSignFlipburnP}{\tbd{hlVeFOneSignFlipburnP}}
\providecommand{\hlVeFOneSignFlipflairEst}{\tbd{hlVeFOneSignFlipflairEst}}
\providecommand{\hlVeFOneSignFlipflairFloorFive}{\tbd{hlVeFOneSignFlipflairFloorFive}}
\providecommand{\hlVeFOneSignFlipflairN}{\tbd{hlVeFOneSignFlipflairN}}
\providecommand{\hlVeFOneSignFlipflairP}{\tbd{hlVeFOneSignFlipflairP}}
\providecommand{\hlVeFTwoCollTostburnCIHi}{\tbd{hlVeFTwoCollTostburnCIHi}}
\providecommand{\hlVeFTwoCollTostburnCILo}{\tbd{hlVeFTwoCollTostburnCILo}}
\providecommand{\hlVeFTwoCollTostburnEquivalent}{\tbd{hlVeFTwoCollTostburnEquivalent}}
\providecommand{\hlVeFTwoCollTostburnEst}{\tbd{hlVeFTwoCollTostburnEst}}
\providecommand{\hlVeFTwoCollTostburnN}{\tbd{hlVeFTwoCollTostburnN}}
\providecommand{\hlVeFTwoCollTostburnP}{\tbd{hlVeFTwoCollTostburnP}}
\providecommand{\hlVeFrozenDOFAburnCIHi}{\tbd{hlVeFrozenDOFAburnCIHi}}
\providecommand{\hlVeFrozenDOFAburnCILo}{\tbd{hlVeFrozenDOFAburnCILo}}
\providecommand{\hlVeFrozenDOFAburnEst}{\tbd{hlVeFrozenDOFAburnEst}}
\providecommand{\hlVeFrozenDOFAburnN}{\tbd{hlVeFrozenDOFAburnN}}
\providecommand{\hlVeFrozenDOFAburnP}{\tbd{hlVeFrozenDOFAburnP}}
\providecommand{\hlVeFrozenDOFAflairCIHi}{\tbd{hlVeFrozenDOFAflairCIHi}}
\providecommand{\hlVeFrozenDOFAflairCILo}{\tbd{hlVeFrozenDOFAflairCILo}}
\providecommand{\hlVeFrozenDOFAflairEst}{\tbd{hlVeFrozenDOFAflairEst}}
\providecommand{\hlVeFrozenDOFAflairN}{\tbd{hlVeFrozenDOFAflairN}}
\providecommand{\hlVeFrozenDOFAflairP}{\tbd{hlVeFrozenDOFAflairP}}
\providecommand{\hlVeFrozenSATNSixburnCIHi}{\tbd{hlVeFrozenSATNSixburnCIHi}}
\providecommand{\hlVeFrozenSATNSixburnCILo}{\tbd{hlVeFrozenSATNSixburnCILo}}
\providecommand{\hlVeFrozenSATNSixburnEst}{\tbd{hlVeFrozenSATNSixburnEst}}
\providecommand{\hlVeFrozenSATNSixburnN}{\tbd{hlVeFrozenSATNSixburnN}}
\providecommand{\hlVeFrozenSATNSixburnP}{\tbd{hlVeFrozenSATNSixburnP}}
\providecommand{\hlVeFrozenSATNSixflairCIHi}{\tbd{hlVeFrozenSATNSixflairCIHi}}
\providecommand{\hlVeFrozenSATNSixflairCILo}{\tbd{hlVeFrozenSATNSixflairCILo}}
\providecommand{\hlVeFrozenSATNSixflairEst}{\tbd{hlVeFrozenSATNSixflairEst}}
\providecommand{\hlVeFrozenSATNSixflairN}{\tbd{hlVeFrozenSATNSixflairN}}
\providecommand{\hlVeFrozenSATNSixflairP}{\tbd{hlVeFrozenSATNSixflairP}}
\providecommand{\hlVeFrozenSATburnCIHi}{\tbd{hlVeFrozenSATburnCIHi}}
\providecommand{\hlVeFrozenSATburnCILo}{\tbd{hlVeFrozenSATburnCILo}}
\providecommand{\hlVeFrozenSATburnEst}{\tbd{hlVeFrozenSATburnEst}}
\providecommand{\hlVeFrozenSATburnN}{\tbd{hlVeFrozenSATburnN}}
\providecommand{\hlVeFrozenSATburnP}{\tbd{hlVeFrozenSATburnP}}
\providecommand{\hlVeFrozenSATflairCIHi}{\tbd{hlVeFrozenSATflairCIHi}}
\providecommand{\hlVeFrozenSATflairCILo}{\tbd{hlVeFrozenSATflairCILo}}
\providecommand{\hlVeFrozenSATflairEst}{\tbd{hlVeFrozenSATflairEst}}
\providecommand{\hlVeFrozenSATflairN}{\tbd{hlVeFrozenSATflairN}}
\providecommand{\hlVeFrozenSATflairP}{\tbd{hlVeFrozenSATflairP}}
\providecommand{\hlVeFrozenTMburnCIHi}{\tbd{hlVeFrozenTMburnCIHi}}
\providecommand{\hlVeFrozenTMburnCILo}{\tbd{hlVeFrozenTMburnCILo}}
\providecommand{\hlVeFrozenTMburnEst}{\tbd{hlVeFrozenTMburnEst}}
\providecommand{\hlVeFrozenTMburnN}{\tbd{hlVeFrozenTMburnN}}
\providecommand{\hlVeFrozenTMburnP}{\tbd{hlVeFrozenTMburnP}}
\providecommand{\hlVeFrozenTMflairCIHi}{\tbd{hlVeFrozenTMflairCIHi}}
\providecommand{\hlVeFrozenTMflairCILo}{\tbd{hlVeFrozenTMflairCILo}}
\providecommand{\hlVeFrozenTMflairEst}{\tbd{hlVeFrozenTMflairEst}}
\providecommand{\hlVeFrozenTMflairN}{\tbd{hlVeFrozenTMflairN}}
\providecommand{\hlVeFrozenTMflairP}{\tbd{hlVeFrozenTMflairP}}
\providecommand{\hlVeMemSATLVDburnCIHi}{\tbd{hlVeMemSATLVDburnCIHi}}
\providecommand{\hlVeMemSATLVDburnCILo}{\tbd{hlVeMemSATLVDburnCILo}}
\providecommand{\hlVeMemSATLVDburnEst}{\tbd{hlVeMemSATLVDburnEst}}
\providecommand{\hlVeMemSATLVDburnN}{\tbd{hlVeMemSATLVDburnN}}
\providecommand{\hlVeMemSATLVDburnP}{\tbd{hlVeMemSATLVDburnP}}
\providecommand{\hlVeMemSATLVDflairCIHi}{\tbd{hlVeMemSATLVDflairCIHi}}
\providecommand{\hlVeMemSATLVDflairCILo}{\tbd{hlVeMemSATLVDflairCILo}}
\providecommand{\hlVeMemSATLVDflairEst}{\tbd{hlVeMemSATLVDflairEst}}
\providecommand{\hlVeMemSATLVDflairN}{\tbd{hlVeMemSATLVDflairN}}
\providecommand{\hlVeMemSATLVDflairP}{\tbd{hlVeMemSATLVDflairP}}
\providecommand{\hlVeNFiveMdeFiveburnEst}{\tbd{hlVeNFiveMdeFiveburnEst}}
\providecommand{\hlVeNFiveMdeFiveburnN}{\tbd{hlVeNFiveMdeFiveburnN}}
\providecommand{\hlVeNFiveMdeFiveburnP}{\tbd{hlVeNFiveMdeFiveburnP}}
\providecommand{\hlVeNFiveMdeFiveflairEst}{\tbd{hlVeNFiveMdeFiveflairEst}}
\providecommand{\hlVeNFiveMdeFiveflairN}{\tbd{hlVeNFiveMdeFiveflairN}}
\providecommand{\hlVeNFiveMdeFiveflairP}{\tbd{hlVeNFiveMdeFiveflairP}}
\providecommand{\hlVeNFiveMdeThreeburnEst}{\tbd{hlVeNFiveMdeThreeburnEst}}
\providecommand{\hlVeNFiveMdeThreeburnN}{\tbd{hlVeNFiveMdeThreeburnN}}
\providecommand{\hlVeNFiveMdeThreeburnP}{\tbd{hlVeNFiveMdeThreeburnP}}
\providecommand{\hlVeNFiveMdeThreeflairEst}{\tbd{hlVeNFiveMdeThreeflairEst}}
\providecommand{\hlVeNFiveMdeThreeflairN}{\tbd{hlVeNFiveMdeThreeflairN}}
\providecommand{\hlVeNFiveMdeThreeflairP}{\tbd{hlVeNFiveMdeThreeflairP}}
\providecommand{\hlVeNSixMdeburnEst}{\tbd{hlVeNSixMdeburnEst}}
\providecommand{\hlVeNSixMdeburnN}{\tbd{hlVeNSixMdeburnN}}
\providecommand{\hlVeNSixMdeburnP}{\tbd{hlVeNSixMdeburnP}}
\providecommand{\hlVeNSixMdeflairEst}{\tbd{hlVeNSixMdeflairEst}}
\providecommand{\hlVeNSixMdeflairN}{\tbd{hlVeNSixMdeflairN}}
\providecommand{\hlVeNSixMdeflairP}{\tbd{hlVeNSixMdeflairP}}
\providecommand{\hlVeNSixTostburnCIHi}{\tbd{hlVeNSixTostburnCIHi}}
\providecommand{\hlVeNSixTostburnCILo}{\tbd{hlVeNSixTostburnCILo}}
\providecommand{\hlVeNSixTostburnEquivalent}{\tbd{hlVeNSixTostburnEquivalent}}
\providecommand{\hlVeNSixTostburnEst}{\tbd{hlVeNSixTostburnEst}}
\providecommand{\hlVeNSixTostburnN}{\tbd{hlVeNSixTostburnN}}
\providecommand{\hlVeNSixTostburnP}{\tbd{hlVeNSixTostburnP}}
\providecommand{\hlVeNSixTostflairCIHi}{\tbd{hlVeNSixTostflairCIHi}}
\providecommand{\hlVeNSixTostflairCILo}{\tbd{hlVeNSixTostflairCILo}}
\providecommand{\hlVeNSixTostflairEquivalent}{\tbd{hlVeNSixTostflairEquivalent}}
\providecommand{\hlVeNSixTostflairEst}{\tbd{hlVeNSixTostflairEst}}
\providecommand{\hlVeNSixTostflairN}{\tbd{hlVeNSixTostflairN}}
\providecommand{\hlVeNSixTostflairP}{\tbd{hlVeNSixTostflairP}}
\providecommand{\hlVeNoisyLVDSATNSixburnCIHi}{\tbd{hlVeNoisyLVDSATNSixburnCIHi}}
\providecommand{\hlVeNoisyLVDSATNSixburnCILo}{\tbd{hlVeNoisyLVDSATNSixburnCILo}}
\providecommand{\hlVeNoisyLVDSATNSixburnEst}{\tbd{hlVeNoisyLVDSATNSixburnEst}}
\providecommand{\hlVeNoisyLVDSATNSixburnN}{\tbd{hlVeNoisyLVDSATNSixburnN}}
\providecommand{\hlVeNoisyLVDSATNSixburnP}{\tbd{hlVeNoisyLVDSATNSixburnP}}
\providecommand{\hlVeNoisyLVDSATNSixflairCIHi}{\tbd{hlVeNoisyLVDSATNSixflairCIHi}}
\providecommand{\hlVeNoisyLVDSATNSixflairCILo}{\tbd{hlVeNoisyLVDSATNSixflairCILo}}
\providecommand{\hlVeNoisyLVDSATNSixflairEst}{\tbd{hlVeNoisyLVDSATNSixflairEst}}
\providecommand{\hlVeNoisyLVDSATNSixflairN}{\tbd{hlVeNoisyLVDSATNSixflairN}}
\providecommand{\hlVeNoisyLVDSATNSixflairP}{\tbd{hlVeNoisyLVDSATNSixflairP}}
\providecommand{\hlVeNoisyLVDSATburnCIHi}{\tbd{hlVeNoisyLVDSATburnCIHi}}
\providecommand{\hlVeNoisyLVDSATburnCILo}{\tbd{hlVeNoisyLVDSATburnCILo}}
\providecommand{\hlVeNoisyLVDSATburnEst}{\tbd{hlVeNoisyLVDSATburnEst}}
\providecommand{\hlVeNoisyLVDSATburnN}{\tbd{hlVeNoisyLVDSATburnN}}
\providecommand{\hlVeNoisyLVDSATburnP}{\tbd{hlVeNoisyLVDSATburnP}}
\providecommand{\hlVeNoisyLVDSATflairCIHi}{\tbd{hlVeNoisyLVDSATflairCIHi}}
\providecommand{\hlVeNoisyLVDSATflairCILo}{\tbd{hlVeNoisyLVDSATflairCILo}}
\providecommand{\hlVeNoisyLVDSATflairEst}{\tbd{hlVeNoisyLVDSATflairEst}}
\providecommand{\hlVeNoisyLVDSATflairN}{\tbd{hlVeNoisyLVDSATflairN}}
\providecommand{\hlVeNoisyLVDSATflairP}{\tbd{hlVeNoisyLVDSATflairP}}
\providecommand{\hlVeSThreeTMburnCIHi}{\tbd{hlVeSThreeTMburnCIHi}}
\providecommand{\hlVeSThreeTMburnCILo}{\tbd{hlVeSThreeTMburnCILo}}
\providecommand{\hlVeSThreeTMburnEst}{\tbd{hlVeSThreeTMburnEst}}
\providecommand{\hlVeSThreeTMburnN}{\tbd{hlVeSThreeTMburnN}}
\providecommand{\hlVeSThreeTMburnP}{\tbd{hlVeSThreeTMburnP}}
\providecommand{\hlVeSThreeTMflairCIHi}{\tbd{hlVeSThreeTMflairCIHi}}
\providecommand{\hlVeSThreeTMflairCILo}{\tbd{hlVeSThreeTMflairCILo}}
\providecommand{\hlVeSThreeTMflairEst}{\tbd{hlVeSThreeTMflairEst}}
\providecommand{\hlVeSThreeTMflairN}{\tbd{hlVeSThreeTMflairN}}
\providecommand{\hlVeSThreeTMflairP}{\tbd{hlVeSThreeTMflairP}}
\providecommand{\hlVeTMRNburnCIHi}{\tbd{hlVeTMRNburnCIHi}}
\providecommand{\hlVeTMRNburnCILo}{\tbd{hlVeTMRNburnCILo}}
\providecommand{\hlVeTMRNburnEst}{\tbd{hlVeTMRNburnEst}}
\providecommand{\hlVeTMRNburnN}{\tbd{hlVeTMRNburnN}}
\providecommand{\hlVeTMRNburnP}{\tbd{hlVeTMRNburnP}}
\providecommand{\hlVeTMRNflairCIHi}{\tbd{hlVeTMRNflairCIHi}}
\providecommand{\hlVeTMRNflairCILo}{\tbd{hlVeTMRNflairCILo}}
\providecommand{\hlVeTMRNflairEst}{\tbd{hlVeTMRNflairEst}}
\providecommand{\hlVeTMRNflairN}{\tbd{hlVeTMRNflairN}}
\providecommand{\hlVeTMRNflairP}{\tbd{hlVeTMRNflairP}}
\providecommand{\hlWinnersCurseAFiveburnCIHi}{\tbd{hlWinnersCurseAFiveburnCIHi}}
\providecommand{\hlWinnersCurseAFiveburnCILo}{\tbd{hlWinnersCurseAFiveburnCILo}}
\providecommand{\hlWinnersCurseAFiveburnEst}{\tbd{hlWinnersCurseAFiveburnEst}}
\providecommand{\hlWinnersCurseAFiveburnN}{\tbd{hlWinnersCurseAFiveburnN}}
\providecommand{\hlWinnersCurseAFiveflairCIHi}{\tbd{hlWinnersCurseAFiveflairCIHi}}
\providecommand{\hlWinnersCurseAFiveflairCILo}{\tbd{hlWinnersCurseAFiveflairCILo}}
\providecommand{\hlWinnersCurseAFiveflairEst}{\tbd{hlWinnersCurseAFiveflairEst}}
\providecommand{\hlWinnersCurseAFiveflairN}{\tbd{hlWinnersCurseAFiveflairN}}
\providecommand{\hlWinnersCurseAFourburnCIHi}{\tbd{hlWinnersCurseAFourburnCIHi}}
\providecommand{\hlWinnersCurseAFourburnCILo}{\tbd{hlWinnersCurseAFourburnCILo}}
\providecommand{\hlWinnersCurseAFourburnEst}{\tbd{hlWinnersCurseAFourburnEst}}
\providecommand{\hlWinnersCurseAFourburnN}{\tbd{hlWinnersCurseAFourburnN}}
\providecommand{\hlWinnersCurseAFourflairCIHi}{\tbd{hlWinnersCurseAFourflairCIHi}}
\providecommand{\hlWinnersCurseAFourflairCILo}{\tbd{hlWinnersCurseAFourflairCILo}}
\providecommand{\hlWinnersCurseAFourflairEst}{\tbd{hlWinnersCurseAFourflairEst}}
\providecommand{\hlWinnersCurseAFourflairN}{\tbd{hlWinnersCurseAFourflairN}}
\providecommand{\hlWinnersCurseASixburnCIHi}{\tbd{hlWinnersCurseASixburnCIHi}}
\providecommand{\hlWinnersCurseASixburnCILo}{\tbd{hlWinnersCurseASixburnCILo}}
\providecommand{\hlWinnersCurseASixburnEst}{\tbd{hlWinnersCurseASixburnEst}}
\providecommand{\hlWinnersCurseASixburnN}{\tbd{hlWinnersCurseASixburnN}}
\providecommand{\hlWinnersCurseASixflairCIHi}{\tbd{hlWinnersCurseASixflairCIHi}}
\providecommand{\hlWinnersCurseASixflairCILo}{\tbd{hlWinnersCurseASixflairCILo}}
\providecommand{\hlWinnersCurseASixflairEst}{\tbd{hlWinnersCurseASixflairEst}}
\providecommand{\hlWinnersCurseASixflairN}{\tbd{hlWinnersCurseASixflairN}}
\providecommand{\hlWinnersCurseAThreeburnCIHi}{\tbd{hlWinnersCurseAThreeburnCIHi}}
\providecommand{\hlWinnersCurseAThreeburnCILo}{\tbd{hlWinnersCurseAThreeburnCILo}}
\providecommand{\hlWinnersCurseAThreeburnEst}{\tbd{hlWinnersCurseAThreeburnEst}}
\providecommand{\hlWinnersCurseAThreeburnN}{\tbd{hlWinnersCurseAThreeburnN}}
\providecommand{\hlWinnersCurseAThreeflairCIHi}{\tbd{hlWinnersCurseAThreeflairCIHi}}
\providecommand{\hlWinnersCurseAThreeflairCILo}{\tbd{hlWinnersCurseAThreeflairCILo}}
\providecommand{\hlWinnersCurseAThreeflairEst}{\tbd{hlWinnersCurseAThreeflairEst}}
\providecommand{\hlWinnersCurseAThreeflairN}{\tbd{hlWinnersCurseAThreeflairN}}
\providecommand{\hlWinnersCurseNSixburnCIHi}{\tbd{hlWinnersCurseNSixburnCIHi}}
\providecommand{\hlWinnersCurseNSixburnCILo}{\tbd{hlWinnersCurseNSixburnCILo}}
\providecommand{\hlWinnersCurseNSixburnEst}{\tbd{hlWinnersCurseNSixburnEst}}
\providecommand{\hlWinnersCurseNSixburnN}{\tbd{hlWinnersCurseNSixburnN}}
\providecommand{\hlWinnersCurseNSixflairCIHi}{\tbd{hlWinnersCurseNSixflairCIHi}}
\providecommand{\hlWinnersCurseNSixflairCILo}{\tbd{hlWinnersCurseNSixflairCILo}}
\providecommand{\hlWinnersCurseNSixflairEst}{\tbd{hlWinnersCurseNSixflairEst}}
\providecommand{\hlWinnersCurseNSixflairN}{\tbd{hlWinnersCurseNSixflairN}}
\providecommand{\hlWorstTypeChes}{\tbd{hlWorstTypeChes}}
\providecommand{\hlWorstTypeCsTwelve}{\tbd{hlWorstTypeCsTwelve}}
\providecommand{\hlWorstTypeDfc}{\tbd{hlWorstTypeDfc}}
\providecommand{\hlWorstTypeDropChes}{\tbd{hlWorstTypeDropChes}}
\providecommand{\hlWorstTypeDropCsTwelve}{\tbd{hlWorstTypeDropCsTwelve}}
\providecommand{\hlWorstTypeDropDfc}{\tbd{hlWorstTypeDropDfc}}
\providecommand{\hlWorstTypeDropEnva}{\tbd{hlWorstTypeDropEnva}}
\providecommand{\hlWorstTypeDropKuro}{\tbd{hlWorstTypeDropKuro}}
\providecommand{\hlWorstTypeDropOem}{\tbd{hlWorstTypeDropOem}}
\providecommand{\hlWorstTypeDropSnTwo}{\tbd{hlWorstTypeDropSnTwo}}
\providecommand{\hlWorstTypeDropburn}{\tbd{hlWorstTypeDropburn}}
\providecommand{\hlWorstTypeDropflair}{\tbd{hlWorstTypeDropflair}}
\providecommand{\hlWorstTypeEnva}{\tbd{hlWorstTypeEnva}}
\providecommand{\hlWorstTypeKuro}{\tbd{hlWorstTypeKuro}}
\providecommand{\hlWorstTypeOem}{\tbd{hlWorstTypeOem}}
\providecommand{\hlWorstTypeSnTwo}{\tbd{hlWorstTypeSnTwo}}
\providecommand{\hlWorstTypeburn}{\tbd{hlWorstTypeburn}}
\providecommand{\hlWorstTypeflair}{\tbd{hlWorstTypeflair}}
\providecommand{\miouCIDOFAChesBoundaryLOne}{\tbd{miouCIDOFAChesBoundaryLOne}}
\providecommand{\miouCIDOFAChesBoundaryLTwo}{\tbd{miouCIDOFAChesBoundaryLTwo}}
\providecommand{\miouCIDOFAChesClean}{\tbd{miouCIDOFAChesClean}}
\providecommand{\miouCIDOFAChesCoarseLOne}{\tbd{miouCIDOFAChesCoarseLOne}}
\providecommand{\miouCIDOFAChesCoarseLTwo}{\tbd{miouCIDOFAChesCoarseLTwo}}
\providecommand{\miouCIDOFAChesNlcdREAL}{\tbd{miouCIDOFAChesNlcdREAL}}
\providecommand{\miouCIDOFAChesOmissionLOne}{\tbd{miouCIDOFAChesOmissionLOne}}
\providecommand{\miouCIDOFAChesOmissionLTwo}{\tbd{miouCIDOFAChesOmissionLTwo}}
\providecommand{\miouCIDOFAChesShiftLOne}{\tbd{miouCIDOFAChesShiftLOne}}
\providecommand{\miouCIDOFAChesShiftLTwo}{\tbd{miouCIDOFAChesShiftLTwo}}
\providecommand{\miouCIDOFACsTwelveBoundaryLOne}{\tbd{miouCIDOFACsTwelveBoundaryLOne}}
\providecommand{\miouCIDOFACsTwelveBoundaryLTwo}{\tbd{miouCIDOFACsTwelveBoundaryLTwo}}
\providecommand{\miouCIDOFACsTwelveClean}{\tbd{miouCIDOFACsTwelveClean}}
\providecommand{\miouCIDOFACsTwelveCoarseLOne}{\tbd{miouCIDOFACsTwelveCoarseLOne}}
\providecommand{\miouCIDOFACsTwelveCoarseLTwo}{\tbd{miouCIDOFACsTwelveCoarseLTwo}}
\providecommand{\miouCIDOFACsTwelveOmissionLOne}{\tbd{miouCIDOFACsTwelveOmissionLOne}}
\providecommand{\miouCIDOFACsTwelveOmissionLTwo}{\tbd{miouCIDOFACsTwelveOmissionLTwo}}
\providecommand{\miouCIDOFACsTwelveSTwocloudlessREAL}{\tbd{miouCIDOFACsTwelveSTwocloudlessREAL}}
\providecommand{\miouCIDOFACsTwelveShiftLOne}{\tbd{miouCIDOFACsTwelveShiftLOne}}
\providecommand{\miouCIDOFACsTwelveShiftLTwo}{\tbd{miouCIDOFACsTwelveShiftLTwo}}
\providecommand{\miouCIDOFADfcBoundaryLOne}{\tbd{miouCIDOFADfcBoundaryLOne}}
\providecommand{\miouCIDOFADfcBoundaryLTwo}{\tbd{miouCIDOFADfcBoundaryLTwo}}
\providecommand{\miouCIDOFADfcClean}{\tbd{miouCIDOFADfcClean}}
\providecommand{\miouCIDOFADfcCleanVarTrainSubsetRealcov}{\tbd{miouCIDOFADfcCleanVarTrainSubsetRealcov}}
\providecommand{\miouCIDOFADfcCoarseLOne}{\tbd{miouCIDOFADfcCoarseLOne}}
\providecommand{\miouCIDOFADfcCoarseLTwo}{\tbd{miouCIDOFADfcCoarseLTwo}}
\providecommand{\miouCIDOFADfcModisREALVarTrainSubsetRealcov}{\tbd{miouCIDOFADfcModisREALVarTrainSubsetRealcov}}
\providecommand{\miouCIDOFADfcOmissionLOne}{\tbd{miouCIDOFADfcOmissionLOne}}
\providecommand{\miouCIDOFADfcOmissionLTwo}{\tbd{miouCIDOFADfcOmissionLTwo}}
\providecommand{\miouCIDOFADfcShiftLOne}{\tbd{miouCIDOFADfcShiftLOne}}
\providecommand{\miouCIDOFADfcShiftLTwo}{\tbd{miouCIDOFADfcShiftLTwo}}
\providecommand{\miouCIDOFAEnvaBoundaryLOne}{\tbd{miouCIDOFAEnvaBoundaryLOne}}
\providecommand{\miouCIDOFAEnvaBoundaryLTwo}{\tbd{miouCIDOFAEnvaBoundaryLTwo}}
\providecommand{\miouCIDOFAEnvaClean}{\tbd{miouCIDOFAEnvaClean}}
\providecommand{\miouCIDOFAEnvaCoarseLOne}{\tbd{miouCIDOFAEnvaCoarseLOne}}
\providecommand{\miouCIDOFAEnvaCoarseLTwo}{\tbd{miouCIDOFAEnvaCoarseLTwo}}
\providecommand{\miouCIDOFAEnvaNlcdREAL}{\tbd{miouCIDOFAEnvaNlcdREAL}}
\providecommand{\miouCIDOFAEnvaOmissionLOne}{\tbd{miouCIDOFAEnvaOmissionLOne}}
\providecommand{\miouCIDOFAEnvaOmissionLTwo}{\tbd{miouCIDOFAEnvaOmissionLTwo}}
\providecommand{\miouCIDOFAEnvaShiftLOne}{\tbd{miouCIDOFAEnvaShiftLOne}}
\providecommand{\miouCIDOFAEnvaShiftLTwo}{\tbd{miouCIDOFAEnvaShiftLTwo}}
\providecommand{\miouCIDOFAKuroBoundaryLOne}{\tbd{miouCIDOFAKuroBoundaryLOne}}
\providecommand{\miouCIDOFAKuroBoundaryLTwo}{\tbd{miouCIDOFAKuroBoundaryLTwo}}
\providecommand{\miouCIDOFAKuroCemsREALVarTrainSubsetRealcov}{\tbd{miouCIDOFAKuroCemsREALVarTrainSubsetRealcov}}
\providecommand{\miouCIDOFAKuroClean}{\tbd{miouCIDOFAKuroClean}}
\providecommand{\miouCIDOFAKuroCleanVarTrainSubsetRealcov}{\tbd{miouCIDOFAKuroCleanVarTrainSubsetRealcov}}
\providecommand{\miouCIDOFAKuroCoarseLOne}{\tbd{miouCIDOFAKuroCoarseLOne}}
\providecommand{\miouCIDOFAKuroCoarseLTwo}{\tbd{miouCIDOFAKuroCoarseLTwo}}
\providecommand{\miouCIDOFAKuroOmissionLOne}{\tbd{miouCIDOFAKuroOmissionLOne}}
\providecommand{\miouCIDOFAKuroOmissionLTwo}{\tbd{miouCIDOFAKuroOmissionLTwo}}
\providecommand{\miouCIDOFAKuroShiftLOne}{\tbd{miouCIDOFAKuroShiftLOne}}
\providecommand{\miouCIDOFAKuroShiftLTwo}{\tbd{miouCIDOFAKuroShiftLTwo}}
\providecommand{\miouCIDOFAOemBoundaryLOne}{\tbd{miouCIDOFAOemBoundaryLOne}}
\providecommand{\miouCIDOFAOemBoundaryLTwo}{\tbd{miouCIDOFAOemBoundaryLTwo}}
\providecommand{\miouCIDOFAOemClean}{\tbd{miouCIDOFAOemClean}}
\providecommand{\miouCIDOFAOemCoarseLOne}{\tbd{miouCIDOFAOemCoarseLOne}}
\providecommand{\miouCIDOFAOemCoarseLTwo}{\tbd{miouCIDOFAOemCoarseLTwo}}
\providecommand{\miouCIDOFAOemOmissionLOne}{\tbd{miouCIDOFAOemOmissionLOne}}
\providecommand{\miouCIDOFAOemOmissionLTwo}{\tbd{miouCIDOFAOemOmissionLTwo}}
\providecommand{\miouCIDOFAOemShiftLOne}{\tbd{miouCIDOFAOemShiftLOne}}
\providecommand{\miouCIDOFAOemShiftLTwo}{\tbd{miouCIDOFAOemShiftLTwo}}
\providecommand{\miouCIDOFASnTwoBoundaryLOne}{\tbd{miouCIDOFASnTwoBoundaryLOne}}
\providecommand{\miouCIDOFASnTwoBoundaryLTwo}{\tbd{miouCIDOFASnTwoBoundaryLTwo}}
\providecommand{\miouCIDOFASnTwoClean}{\tbd{miouCIDOFASnTwoClean}}
\providecommand{\miouCIDOFASnTwoCoarseLOne}{\tbd{miouCIDOFASnTwoCoarseLOne}}
\providecommand{\miouCIDOFASnTwoCoarseLTwo}{\tbd{miouCIDOFASnTwoCoarseLTwo}}
\providecommand{\miouCIDOFASnTwoOmissionLOne}{\tbd{miouCIDOFASnTwoOmissionLOne}}
\providecommand{\miouCIDOFASnTwoOmissionLTwo}{\tbd{miouCIDOFASnTwoOmissionLTwo}}
\providecommand{\miouCIDOFASnTwoShiftLOne}{\tbd{miouCIDOFASnTwoShiftLOne}}
\providecommand{\miouCIDOFASnTwoShiftLTwo}{\tbd{miouCIDOFASnTwoShiftLTwo}}
\providecommand{\miouCIDOFAburnBoundaryLOne}{\tbd{miouCIDOFAburnBoundaryLOne}}
\providecommand{\miouCIDOFAburnBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{miouCIDOFAburnBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCIDOFAburnBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{miouCIDOFAburnBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCIDOFAburnBoundaryLOneVarDecoderSamLite}{\tbd{miouCIDOFAburnBoundaryLOneVarDecoderSamLite}}
\providecommand{\miouCIDOFAburnBoundaryLOneVarDecoderSamPretrained}{\tbd{miouCIDOFAburnBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\miouCIDOFAburnBoundaryLOneVarDecoderSegformerMlp}{\tbd{miouCIDOFAburnBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\miouCIDOFAburnBoundaryLR}{\tbd{miouCIDOFAburnBoundaryLR}}
\providecommand{\miouCIDOFAburnBoundaryLTwo}{\tbd{miouCIDOFAburnBoundaryLTwo}}
\providecommand{\miouCIDOFAburnBoundaryLTwoVarBandsRgb}{\tbd{miouCIDOFAburnBoundaryLTwoVarBandsRgb}}
\providecommand{\miouCIDOFAburnBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCIDOFAburnBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCIDOFAburnBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCIDOFAburnBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCIDOFAburnBoundaryLTwoVarDecoderSamLite}{\tbd{miouCIDOFAburnBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouCIDOFAburnBoundaryLTwoVarDecoderSamPretrained}{\tbd{miouCIDOFAburnBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\miouCIDOFAburnBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouCIDOFAburnBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCIDOFAburnBoundaryLTwoVarFrozenEncoderTrue}{\tbd{miouCIDOFAburnBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\miouCIDOFAburnBoundaryLTwoVarLossBootstrap}{\tbd{miouCIDOFAburnBoundaryLTwoVarLossBootstrap}}
\providecommand{\miouCIDOFAburnBoundaryLTwoVarLossGce}{\tbd{miouCIDOFAburnBoundaryLTwoVarLossGce}}
\providecommand{\miouCIDOFAburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCIDOFAburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCIDOFAburnBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCIDOFAburnBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCIDOFAburnClean}{\tbd{miouCIDOFAburnClean}}
\providecommand{\miouCIDOFAburnCleanVarBandsRgb}{\tbd{miouCIDOFAburnCleanVarBandsRgb}}
\providecommand{\miouCIDOFAburnCleanVarDecoderMaskTwoformerFull}{\tbd{miouCIDOFAburnCleanVarDecoderMaskTwoformerFull}}
\providecommand{\miouCIDOFAburnCleanVarDecoderMaskTwoformerLite}{\tbd{miouCIDOFAburnCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouCIDOFAburnCleanVarDecoderSamLite}{\tbd{miouCIDOFAburnCleanVarDecoderSamLite}}
\providecommand{\miouCIDOFAburnCleanVarDecoderSamPretrained}{\tbd{miouCIDOFAburnCleanVarDecoderSamPretrained}}
\providecommand{\miouCIDOFAburnCleanVarDecoderSegformerMlp}{\tbd{miouCIDOFAburnCleanVarDecoderSegformerMlp}}
\providecommand{\miouCIDOFAburnCleanVarFrozenEncoderTrue}{\tbd{miouCIDOFAburnCleanVarFrozenEncoderTrue}}
\providecommand{\miouCIDOFAburnCleanVarLossBootstrap}{\tbd{miouCIDOFAburnCleanVarLossBootstrap}}
\providecommand{\miouCIDOFAburnCleanVarLossGce}{\tbd{miouCIDOFAburnCleanVarLossGce}}
\providecommand{\miouCIDOFAburnCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCIDOFAburnCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCIDOFAburnCleanVarTrainSubsetCleanTwoFive}{\tbd{miouCIDOFAburnCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCIDOFAburnCoarseLOne}{\tbd{miouCIDOFAburnCoarseLOne}}
\providecommand{\miouCIDOFAburnCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{miouCIDOFAburnCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCIDOFAburnCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{miouCIDOFAburnCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCIDOFAburnCoarseLOneVarDecoderSamLite}{\tbd{miouCIDOFAburnCoarseLOneVarDecoderSamLite}}
\providecommand{\miouCIDOFAburnCoarseLOneVarDecoderSamPretrained}{\tbd{miouCIDOFAburnCoarseLOneVarDecoderSamPretrained}}
\providecommand{\miouCIDOFAburnCoarseLOneVarDecoderSegformerMlp}{\tbd{miouCIDOFAburnCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\miouCIDOFAburnCoarseLR}{\tbd{miouCIDOFAburnCoarseLR}}
\providecommand{\miouCIDOFAburnCoarseLTwo}{\tbd{miouCIDOFAburnCoarseLTwo}}
\providecommand{\miouCIDOFAburnCoarseLTwoVarBandsRgb}{\tbd{miouCIDOFAburnCoarseLTwoVarBandsRgb}}
\providecommand{\miouCIDOFAburnCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCIDOFAburnCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCIDOFAburnCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCIDOFAburnCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCIDOFAburnCoarseLTwoVarDecoderSamLite}{\tbd{miouCIDOFAburnCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouCIDOFAburnCoarseLTwoVarDecoderSamPretrained}{\tbd{miouCIDOFAburnCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\miouCIDOFAburnCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouCIDOFAburnCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCIDOFAburnCoarseLTwoVarFrozenEncoderTrue}{\tbd{miouCIDOFAburnCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\miouCIDOFAburnCoarseLTwoVarLossBootstrap}{\tbd{miouCIDOFAburnCoarseLTwoVarLossBootstrap}}
\providecommand{\miouCIDOFAburnCoarseLTwoVarLossGce}{\tbd{miouCIDOFAburnCoarseLTwoVarLossGce}}
\providecommand{\miouCIDOFAburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCIDOFAburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCIDOFAburnCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCIDOFAburnCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCIDOFAburnOmissionLOne}{\tbd{miouCIDOFAburnOmissionLOne}}
\providecommand{\miouCIDOFAburnOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{miouCIDOFAburnOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCIDOFAburnOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{miouCIDOFAburnOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCIDOFAburnOmissionLOneVarDecoderSamLite}{\tbd{miouCIDOFAburnOmissionLOneVarDecoderSamLite}}
\providecommand{\miouCIDOFAburnOmissionLOneVarDecoderSamPretrained}{\tbd{miouCIDOFAburnOmissionLOneVarDecoderSamPretrained}}
\providecommand{\miouCIDOFAburnOmissionLOneVarDecoderSegformerMlp}{\tbd{miouCIDOFAburnOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\miouCIDOFAburnOmissionLR}{\tbd{miouCIDOFAburnOmissionLR}}
\providecommand{\miouCIDOFAburnOmissionLTwo}{\tbd{miouCIDOFAburnOmissionLTwo}}
\providecommand{\miouCIDOFAburnOmissionLTwoVarBandsRgb}{\tbd{miouCIDOFAburnOmissionLTwoVarBandsRgb}}
\providecommand{\miouCIDOFAburnOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCIDOFAburnOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCIDOFAburnOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCIDOFAburnOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCIDOFAburnOmissionLTwoVarDecoderSamLite}{\tbd{miouCIDOFAburnOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouCIDOFAburnOmissionLTwoVarDecoderSamPretrained}{\tbd{miouCIDOFAburnOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\miouCIDOFAburnOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouCIDOFAburnOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCIDOFAburnOmissionLTwoVarFrozenEncoderTrue}{\tbd{miouCIDOFAburnOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\miouCIDOFAburnOmissionLTwoVarLossBootstrap}{\tbd{miouCIDOFAburnOmissionLTwoVarLossBootstrap}}
\providecommand{\miouCIDOFAburnOmissionLTwoVarLossGce}{\tbd{miouCIDOFAburnOmissionLTwoVarLossGce}}
\providecommand{\miouCIDOFAburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCIDOFAburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCIDOFAburnOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCIDOFAburnOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCIDOFAburnShiftLOne}{\tbd{miouCIDOFAburnShiftLOne}}
\providecommand{\miouCIDOFAburnShiftLOneVarDecoderMaskTwoformerFull}{\tbd{miouCIDOFAburnShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCIDOFAburnShiftLOneVarDecoderMaskTwoformerLite}{\tbd{miouCIDOFAburnShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCIDOFAburnShiftLOneVarDecoderSamLite}{\tbd{miouCIDOFAburnShiftLOneVarDecoderSamLite}}
\providecommand{\miouCIDOFAburnShiftLOneVarDecoderSamPretrained}{\tbd{miouCIDOFAburnShiftLOneVarDecoderSamPretrained}}
\providecommand{\miouCIDOFAburnShiftLOneVarDecoderSegformerMlp}{\tbd{miouCIDOFAburnShiftLOneVarDecoderSegformerMlp}}
\providecommand{\miouCIDOFAburnShiftLR}{\tbd{miouCIDOFAburnShiftLR}}
\providecommand{\miouCIDOFAburnShiftLTwo}{\tbd{miouCIDOFAburnShiftLTwo}}
\providecommand{\miouCIDOFAburnShiftLTwoVarBandsRgb}{\tbd{miouCIDOFAburnShiftLTwoVarBandsRgb}}
\providecommand{\miouCIDOFAburnShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCIDOFAburnShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCIDOFAburnShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCIDOFAburnShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCIDOFAburnShiftLTwoVarDecoderSamLite}{\tbd{miouCIDOFAburnShiftLTwoVarDecoderSamLite}}
\providecommand{\miouCIDOFAburnShiftLTwoVarDecoderSamPretrained}{\tbd{miouCIDOFAburnShiftLTwoVarDecoderSamPretrained}}
\providecommand{\miouCIDOFAburnShiftLTwoVarDecoderSegformerMlp}{\tbd{miouCIDOFAburnShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCIDOFAburnShiftLTwoVarFrozenEncoderTrue}{\tbd{miouCIDOFAburnShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\miouCIDOFAburnShiftLTwoVarLossBootstrap}{\tbd{miouCIDOFAburnShiftLTwoVarLossBootstrap}}
\providecommand{\miouCIDOFAburnShiftLTwoVarLossGce}{\tbd{miouCIDOFAburnShiftLTwoVarLossGce}}
\providecommand{\miouCIDOFAburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCIDOFAburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCIDOFAburnShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCIDOFAburnShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCIDOFAflairBoundaryLOne}{\tbd{miouCIDOFAflairBoundaryLOne}}
\providecommand{\miouCIDOFAflairBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{miouCIDOFAflairBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCIDOFAflairBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{miouCIDOFAflairBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCIDOFAflairBoundaryLOneVarDecoderSamLite}{\tbd{miouCIDOFAflairBoundaryLOneVarDecoderSamLite}}
\providecommand{\miouCIDOFAflairBoundaryLOneVarDecoderSamPretrained}{\tbd{miouCIDOFAflairBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\miouCIDOFAflairBoundaryLOneVarDecoderSegformerMlp}{\tbd{miouCIDOFAflairBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\miouCIDOFAflairBoundaryLR}{\tbd{miouCIDOFAflairBoundaryLR}}
\providecommand{\miouCIDOFAflairBoundaryLTwo}{\tbd{miouCIDOFAflairBoundaryLTwo}}
\providecommand{\miouCIDOFAflairBoundaryLTwoVarBandsRgb}{\tbd{miouCIDOFAflairBoundaryLTwoVarBandsRgb}}
\providecommand{\miouCIDOFAflairBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCIDOFAflairBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCIDOFAflairBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCIDOFAflairBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCIDOFAflairBoundaryLTwoVarDecoderSamLite}{\tbd{miouCIDOFAflairBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouCIDOFAflairBoundaryLTwoVarDecoderSamPretrained}{\tbd{miouCIDOFAflairBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\miouCIDOFAflairBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouCIDOFAflairBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCIDOFAflairBoundaryLTwoVarFrozenEncoderTrue}{\tbd{miouCIDOFAflairBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\miouCIDOFAflairBoundaryLTwoVarLossBootstrap}{\tbd{miouCIDOFAflairBoundaryLTwoVarLossBootstrap}}
\providecommand{\miouCIDOFAflairBoundaryLTwoVarLossGce}{\tbd{miouCIDOFAflairBoundaryLTwoVarLossGce}}
\providecommand{\miouCIDOFAflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCIDOFAflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCIDOFAflairBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCIDOFAflairBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCIDOFAflairClean}{\tbd{miouCIDOFAflairClean}}
\providecommand{\miouCIDOFAflairCleanVarBandsRgb}{\tbd{miouCIDOFAflairCleanVarBandsRgb}}
\providecommand{\miouCIDOFAflairCleanVarDecoderMaskTwoformerFull}{\tbd{miouCIDOFAflairCleanVarDecoderMaskTwoformerFull}}
\providecommand{\miouCIDOFAflairCleanVarDecoderMaskTwoformerLite}{\tbd{miouCIDOFAflairCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouCIDOFAflairCleanVarDecoderSamLite}{\tbd{miouCIDOFAflairCleanVarDecoderSamLite}}
\providecommand{\miouCIDOFAflairCleanVarDecoderSamPretrained}{\tbd{miouCIDOFAflairCleanVarDecoderSamPretrained}}
\providecommand{\miouCIDOFAflairCleanVarDecoderSegformerMlp}{\tbd{miouCIDOFAflairCleanVarDecoderSegformerMlp}}
\providecommand{\miouCIDOFAflairCleanVarFrozenEncoderTrue}{\tbd{miouCIDOFAflairCleanVarFrozenEncoderTrue}}
\providecommand{\miouCIDOFAflairCleanVarLossBootstrap}{\tbd{miouCIDOFAflairCleanVarLossBootstrap}}
\providecommand{\miouCIDOFAflairCleanVarLossGce}{\tbd{miouCIDOFAflairCleanVarLossGce}}
\providecommand{\miouCIDOFAflairCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCIDOFAflairCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCIDOFAflairCleanVarTrainSubsetCleanTwoFive}{\tbd{miouCIDOFAflairCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCIDOFAflairCoarseLOne}{\tbd{miouCIDOFAflairCoarseLOne}}
\providecommand{\miouCIDOFAflairCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{miouCIDOFAflairCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCIDOFAflairCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{miouCIDOFAflairCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCIDOFAflairCoarseLOneVarDecoderSamLite}{\tbd{miouCIDOFAflairCoarseLOneVarDecoderSamLite}}
\providecommand{\miouCIDOFAflairCoarseLOneVarDecoderSamPretrained}{\tbd{miouCIDOFAflairCoarseLOneVarDecoderSamPretrained}}
\providecommand{\miouCIDOFAflairCoarseLOneVarDecoderSegformerMlp}{\tbd{miouCIDOFAflairCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\miouCIDOFAflairCoarseLR}{\tbd{miouCIDOFAflairCoarseLR}}
\providecommand{\miouCIDOFAflairCoarseLTwo}{\tbd{miouCIDOFAflairCoarseLTwo}}
\providecommand{\miouCIDOFAflairCoarseLTwoVarBandsRgb}{\tbd{miouCIDOFAflairCoarseLTwoVarBandsRgb}}
\providecommand{\miouCIDOFAflairCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCIDOFAflairCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCIDOFAflairCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCIDOFAflairCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCIDOFAflairCoarseLTwoVarDecoderSamLite}{\tbd{miouCIDOFAflairCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouCIDOFAflairCoarseLTwoVarDecoderSamPretrained}{\tbd{miouCIDOFAflairCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\miouCIDOFAflairCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouCIDOFAflairCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCIDOFAflairCoarseLTwoVarFrozenEncoderTrue}{\tbd{miouCIDOFAflairCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\miouCIDOFAflairCoarseLTwoVarLossBootstrap}{\tbd{miouCIDOFAflairCoarseLTwoVarLossBootstrap}}
\providecommand{\miouCIDOFAflairCoarseLTwoVarLossGce}{\tbd{miouCIDOFAflairCoarseLTwoVarLossGce}}
\providecommand{\miouCIDOFAflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCIDOFAflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCIDOFAflairCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCIDOFAflairCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCIDOFAflairOmissionLOne}{\tbd{miouCIDOFAflairOmissionLOne}}
\providecommand{\miouCIDOFAflairOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{miouCIDOFAflairOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCIDOFAflairOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{miouCIDOFAflairOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCIDOFAflairOmissionLOneVarDecoderSamLite}{\tbd{miouCIDOFAflairOmissionLOneVarDecoderSamLite}}
\providecommand{\miouCIDOFAflairOmissionLOneVarDecoderSamPretrained}{\tbd{miouCIDOFAflairOmissionLOneVarDecoderSamPretrained}}
\providecommand{\miouCIDOFAflairOmissionLOneVarDecoderSegformerMlp}{\tbd{miouCIDOFAflairOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\miouCIDOFAflairOmissionLR}{\tbd{miouCIDOFAflairOmissionLR}}
\providecommand{\miouCIDOFAflairOmissionLTwo}{\tbd{miouCIDOFAflairOmissionLTwo}}
\providecommand{\miouCIDOFAflairOmissionLTwoVarBandsRgb}{\tbd{miouCIDOFAflairOmissionLTwoVarBandsRgb}}
\providecommand{\miouCIDOFAflairOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCIDOFAflairOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCIDOFAflairOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCIDOFAflairOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCIDOFAflairOmissionLTwoVarDecoderSamLite}{\tbd{miouCIDOFAflairOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouCIDOFAflairOmissionLTwoVarDecoderSamPretrained}{\tbd{miouCIDOFAflairOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\miouCIDOFAflairOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouCIDOFAflairOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCIDOFAflairOmissionLTwoVarFrozenEncoderTrue}{\tbd{miouCIDOFAflairOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\miouCIDOFAflairOmissionLTwoVarLossBootstrap}{\tbd{miouCIDOFAflairOmissionLTwoVarLossBootstrap}}
\providecommand{\miouCIDOFAflairOmissionLTwoVarLossGce}{\tbd{miouCIDOFAflairOmissionLTwoVarLossGce}}
\providecommand{\miouCIDOFAflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCIDOFAflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCIDOFAflairOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCIDOFAflairOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCIDOFAflairShiftLOne}{\tbd{miouCIDOFAflairShiftLOne}}
\providecommand{\miouCIDOFAflairShiftLOneVarDecoderMaskTwoformerFull}{\tbd{miouCIDOFAflairShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCIDOFAflairShiftLOneVarDecoderMaskTwoformerLite}{\tbd{miouCIDOFAflairShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCIDOFAflairShiftLOneVarDecoderSamLite}{\tbd{miouCIDOFAflairShiftLOneVarDecoderSamLite}}
\providecommand{\miouCIDOFAflairShiftLOneVarDecoderSamPretrained}{\tbd{miouCIDOFAflairShiftLOneVarDecoderSamPretrained}}
\providecommand{\miouCIDOFAflairShiftLOneVarDecoderSegformerMlp}{\tbd{miouCIDOFAflairShiftLOneVarDecoderSegformerMlp}}
\providecommand{\miouCIDOFAflairShiftLR}{\tbd{miouCIDOFAflairShiftLR}}
\providecommand{\miouCIDOFAflairShiftLTwo}{\tbd{miouCIDOFAflairShiftLTwo}}
\providecommand{\miouCIDOFAflairShiftLTwoVarBandsRgb}{\tbd{miouCIDOFAflairShiftLTwoVarBandsRgb}}
\providecommand{\miouCIDOFAflairShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCIDOFAflairShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCIDOFAflairShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCIDOFAflairShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCIDOFAflairShiftLTwoVarDecoderSamLite}{\tbd{miouCIDOFAflairShiftLTwoVarDecoderSamLite}}
\providecommand{\miouCIDOFAflairShiftLTwoVarDecoderSamPretrained}{\tbd{miouCIDOFAflairShiftLTwoVarDecoderSamPretrained}}
\providecommand{\miouCIDOFAflairShiftLTwoVarDecoderSegformerMlp}{\tbd{miouCIDOFAflairShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCIDOFAflairShiftLTwoVarFrozenEncoderTrue}{\tbd{miouCIDOFAflairShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\miouCIDOFAflairShiftLTwoVarLossBootstrap}{\tbd{miouCIDOFAflairShiftLTwoVarLossBootstrap}}
\providecommand{\miouCIDOFAflairShiftLTwoVarLossGce}{\tbd{miouCIDOFAflairShiftLTwoVarLossGce}}
\providecommand{\miouCIDOFAflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCIDOFAflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCIDOFAflairShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCIDOFAflairShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCIDOFAsenClean}{\tbd{miouCIDOFAsenClean}}
\providecommand{\miouCIDOFAsenOtsuLTwo}{\tbd{miouCIDOFAsenOtsuLTwo}}
\providecommand{\miouCIDinovThreeConvnextLburnBoundaryLOne}{\tbd{miouCIDinovThreeConvnextLburnBoundaryLOne}}
\providecommand{\miouCIDinovThreeConvnextLburnBoundaryLTwo}{\tbd{miouCIDinovThreeConvnextLburnBoundaryLTwo}}
\providecommand{\miouCIDinovThreeConvnextLburnClean}{\tbd{miouCIDinovThreeConvnextLburnClean}}
\providecommand{\miouCIDinovThreeConvnextLburnCleanVarTrainSubsetCleanTwoFive}{\tbd{miouCIDinovThreeConvnextLburnCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCIDinovThreeConvnextLburnCoarseLOne}{\tbd{miouCIDinovThreeConvnextLburnCoarseLOne}}
\providecommand{\miouCIDinovThreeConvnextLburnCoarseLTwo}{\tbd{miouCIDinovThreeConvnextLburnCoarseLTwo}}
\providecommand{\miouCIDinovThreeConvnextLburnOmissionLOne}{\tbd{miouCIDinovThreeConvnextLburnOmissionLOne}}
\providecommand{\miouCIDinovThreeConvnextLburnOmissionLTwo}{\tbd{miouCIDinovThreeConvnextLburnOmissionLTwo}}
\providecommand{\miouCIDinovThreeConvnextLburnShiftLOne}{\tbd{miouCIDinovThreeConvnextLburnShiftLOne}}
\providecommand{\miouCIDinovThreeConvnextLburnShiftLTwo}{\tbd{miouCIDinovThreeConvnextLburnShiftLTwo}}
\providecommand{\miouCIDinovThreeConvnextLflairBoundaryLOne}{\tbd{miouCIDinovThreeConvnextLflairBoundaryLOne}}
\providecommand{\miouCIDinovThreeConvnextLflairBoundaryLTwo}{\tbd{miouCIDinovThreeConvnextLflairBoundaryLTwo}}
\providecommand{\miouCIDinovThreeConvnextLflairClean}{\tbd{miouCIDinovThreeConvnextLflairClean}}
\providecommand{\miouCIDinovThreeConvnextLflairCleanVarTrainSubsetCleanTwoFive}{\tbd{miouCIDinovThreeConvnextLflairCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCIDinovThreeConvnextLflairCoarseLOne}{\tbd{miouCIDinovThreeConvnextLflairCoarseLOne}}
\providecommand{\miouCIDinovThreeConvnextLflairCoarseLTwo}{\tbd{miouCIDinovThreeConvnextLflairCoarseLTwo}}
\providecommand{\miouCIDinovThreeConvnextLflairOmissionLOne}{\tbd{miouCIDinovThreeConvnextLflairOmissionLOne}}
\providecommand{\miouCIDinovThreeConvnextLflairOmissionLTwo}{\tbd{miouCIDinovThreeConvnextLflairOmissionLTwo}}
\providecommand{\miouCIDinovThreeConvnextLflairShiftLOne}{\tbd{miouCIDinovThreeConvnextLflairShiftLOne}}
\providecommand{\miouCIDinovThreeConvnextLflairShiftLTwo}{\tbd{miouCIDinovThreeConvnextLflairShiftLTwo}}
\providecommand{\miouCILVDChesBoundaryLOne}{\tbd{miouCILVDChesBoundaryLOne}}
\providecommand{\miouCILVDChesBoundaryLTwo}{\tbd{miouCILVDChesBoundaryLTwo}}
\providecommand{\miouCILVDChesBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCILVDChesBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDChesBoundaryLTwoVarDecoderSamLite}{\tbd{miouCILVDChesBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouCILVDChesBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouCILVDChesBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCILVDChesBoundaryLTwoVarLrMultOne}{\tbd{miouCILVDChesBoundaryLTwoVarLrMultOne}}
\providecommand{\miouCILVDChesClean}{\tbd{miouCILVDChesClean}}
\providecommand{\miouCILVDChesCleanVarDecoderMaskTwoformerLite}{\tbd{miouCILVDChesCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDChesCleanVarDecoderSamLite}{\tbd{miouCILVDChesCleanVarDecoderSamLite}}
\providecommand{\miouCILVDChesCleanVarDecoderSegformerMlp}{\tbd{miouCILVDChesCleanVarDecoderSegformerMlp}}
\providecommand{\miouCILVDChesCleanVarLrMultOne}{\tbd{miouCILVDChesCleanVarLrMultOne}}
\providecommand{\miouCILVDChesCoarseLOne}{\tbd{miouCILVDChesCoarseLOne}}
\providecommand{\miouCILVDChesCoarseLTwo}{\tbd{miouCILVDChesCoarseLTwo}}
\providecommand{\miouCILVDChesCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCILVDChesCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDChesCoarseLTwoVarDecoderSamLite}{\tbd{miouCILVDChesCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouCILVDChesCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouCILVDChesCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCILVDChesCoarseLTwoVarLrMultOne}{\tbd{miouCILVDChesCoarseLTwoVarLrMultOne}}
\providecommand{\miouCILVDChesNlcdREAL}{\tbd{miouCILVDChesNlcdREAL}}
\providecommand{\miouCILVDChesOmissionLOne}{\tbd{miouCILVDChesOmissionLOne}}
\providecommand{\miouCILVDChesOmissionLTwo}{\tbd{miouCILVDChesOmissionLTwo}}
\providecommand{\miouCILVDChesOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCILVDChesOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDChesOmissionLTwoVarDecoderSamLite}{\tbd{miouCILVDChesOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouCILVDChesOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouCILVDChesOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCILVDChesOmissionLTwoVarLrMultOne}{\tbd{miouCILVDChesOmissionLTwoVarLrMultOne}}
\providecommand{\miouCILVDChesShiftLOne}{\tbd{miouCILVDChesShiftLOne}}
\providecommand{\miouCILVDChesShiftLTwo}{\tbd{miouCILVDChesShiftLTwo}}
\providecommand{\miouCILVDChesShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCILVDChesShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDChesShiftLTwoVarDecoderSamLite}{\tbd{miouCILVDChesShiftLTwoVarDecoderSamLite}}
\providecommand{\miouCILVDChesShiftLTwoVarDecoderSegformerMlp}{\tbd{miouCILVDChesShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCILVDChesShiftLTwoVarLrMultOne}{\tbd{miouCILVDChesShiftLTwoVarLrMultOne}}
\providecommand{\miouCILVDCsTwelveBoundaryLOne}{\tbd{miouCILVDCsTwelveBoundaryLOne}}
\providecommand{\miouCILVDCsTwelveBoundaryLTwo}{\tbd{miouCILVDCsTwelveBoundaryLTwo}}
\providecommand{\miouCILVDCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCILVDCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDCsTwelveBoundaryLTwoVarDecoderSamLite}{\tbd{miouCILVDCsTwelveBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouCILVDCsTwelveBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouCILVDCsTwelveBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCILVDCsTwelveBoundaryLTwoVarLrMultOne}{\tbd{miouCILVDCsTwelveBoundaryLTwoVarLrMultOne}}
\providecommand{\miouCILVDCsTwelveClean}{\tbd{miouCILVDCsTwelveClean}}
\providecommand{\miouCILVDCsTwelveCleanVarDecoderMaskTwoformerLite}{\tbd{miouCILVDCsTwelveCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDCsTwelveCleanVarDecoderSamLite}{\tbd{miouCILVDCsTwelveCleanVarDecoderSamLite}}
\providecommand{\miouCILVDCsTwelveCleanVarDecoderSegformerMlp}{\tbd{miouCILVDCsTwelveCleanVarDecoderSegformerMlp}}
\providecommand{\miouCILVDCsTwelveCleanVarLrMultOne}{\tbd{miouCILVDCsTwelveCleanVarLrMultOne}}
\providecommand{\miouCILVDCsTwelveCoarseLOne}{\tbd{miouCILVDCsTwelveCoarseLOne}}
\providecommand{\miouCILVDCsTwelveCoarseLTwo}{\tbd{miouCILVDCsTwelveCoarseLTwo}}
\providecommand{\miouCILVDCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCILVDCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDCsTwelveCoarseLTwoVarDecoderSamLite}{\tbd{miouCILVDCsTwelveCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouCILVDCsTwelveCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouCILVDCsTwelveCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCILVDCsTwelveCoarseLTwoVarLrMultOne}{\tbd{miouCILVDCsTwelveCoarseLTwoVarLrMultOne}}
\providecommand{\miouCILVDCsTwelveOmissionLOne}{\tbd{miouCILVDCsTwelveOmissionLOne}}
\providecommand{\miouCILVDCsTwelveOmissionLTwo}{\tbd{miouCILVDCsTwelveOmissionLTwo}}
\providecommand{\miouCILVDCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCILVDCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDCsTwelveOmissionLTwoVarDecoderSamLite}{\tbd{miouCILVDCsTwelveOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouCILVDCsTwelveOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouCILVDCsTwelveOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCILVDCsTwelveOmissionLTwoVarLrMultOne}{\tbd{miouCILVDCsTwelveOmissionLTwoVarLrMultOne}}
\providecommand{\miouCILVDCsTwelveSTwocloudlessREAL}{\tbd{miouCILVDCsTwelveSTwocloudlessREAL}}
\providecommand{\miouCILVDCsTwelveShiftLOne}{\tbd{miouCILVDCsTwelveShiftLOne}}
\providecommand{\miouCILVDCsTwelveShiftLTwo}{\tbd{miouCILVDCsTwelveShiftLTwo}}
\providecommand{\miouCILVDCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCILVDCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDCsTwelveShiftLTwoVarDecoderSamLite}{\tbd{miouCILVDCsTwelveShiftLTwoVarDecoderSamLite}}
\providecommand{\miouCILVDCsTwelveShiftLTwoVarDecoderSegformerMlp}{\tbd{miouCILVDCsTwelveShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCILVDCsTwelveShiftLTwoVarLrMultOne}{\tbd{miouCILVDCsTwelveShiftLTwoVarLrMultOne}}
\providecommand{\miouCILVDDfcBoundaryLOne}{\tbd{miouCILVDDfcBoundaryLOne}}
\providecommand{\miouCILVDDfcBoundaryLTwo}{\tbd{miouCILVDDfcBoundaryLTwo}}
\providecommand{\miouCILVDDfcBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCILVDDfcBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDDfcBoundaryLTwoVarDecoderSamLite}{\tbd{miouCILVDDfcBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouCILVDDfcBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouCILVDDfcBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCILVDDfcBoundaryLTwoVarLrMultOne}{\tbd{miouCILVDDfcBoundaryLTwoVarLrMultOne}}
\providecommand{\miouCILVDDfcClean}{\tbd{miouCILVDDfcClean}}
\providecommand{\miouCILVDDfcCleanVarDecoderMaskTwoformerLite}{\tbd{miouCILVDDfcCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDDfcCleanVarDecoderSamLite}{\tbd{miouCILVDDfcCleanVarDecoderSamLite}}
\providecommand{\miouCILVDDfcCleanVarDecoderSegformerMlp}{\tbd{miouCILVDDfcCleanVarDecoderSegformerMlp}}
\providecommand{\miouCILVDDfcCleanVarLrMultOne}{\tbd{miouCILVDDfcCleanVarLrMultOne}}
\providecommand{\miouCILVDDfcCleanVarTrainSubsetRealcov}{\tbd{miouCILVDDfcCleanVarTrainSubsetRealcov}}
\providecommand{\miouCILVDDfcCoarseLOne}{\tbd{miouCILVDDfcCoarseLOne}}
\providecommand{\miouCILVDDfcCoarseLTwo}{\tbd{miouCILVDDfcCoarseLTwo}}
\providecommand{\miouCILVDDfcCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCILVDDfcCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDDfcCoarseLTwoVarDecoderSamLite}{\tbd{miouCILVDDfcCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouCILVDDfcCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouCILVDDfcCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCILVDDfcCoarseLTwoVarLrMultOne}{\tbd{miouCILVDDfcCoarseLTwoVarLrMultOne}}
\providecommand{\miouCILVDDfcModisREALVarTrainSubsetRealcov}{\tbd{miouCILVDDfcModisREALVarTrainSubsetRealcov}}
\providecommand{\miouCILVDDfcOmissionLOne}{\tbd{miouCILVDDfcOmissionLOne}}
\providecommand{\miouCILVDDfcOmissionLTwo}{\tbd{miouCILVDDfcOmissionLTwo}}
\providecommand{\miouCILVDDfcOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCILVDDfcOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDDfcOmissionLTwoVarDecoderSamLite}{\tbd{miouCILVDDfcOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouCILVDDfcOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouCILVDDfcOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCILVDDfcOmissionLTwoVarLrMultOne}{\tbd{miouCILVDDfcOmissionLTwoVarLrMultOne}}
\providecommand{\miouCILVDDfcShiftLOne}{\tbd{miouCILVDDfcShiftLOne}}
\providecommand{\miouCILVDDfcShiftLTwo}{\tbd{miouCILVDDfcShiftLTwo}}
\providecommand{\miouCILVDDfcShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCILVDDfcShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDDfcShiftLTwoVarDecoderSamLite}{\tbd{miouCILVDDfcShiftLTwoVarDecoderSamLite}}
\providecommand{\miouCILVDDfcShiftLTwoVarDecoderSegformerMlp}{\tbd{miouCILVDDfcShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCILVDDfcShiftLTwoVarLrMultOne}{\tbd{miouCILVDDfcShiftLTwoVarLrMultOne}}
\providecommand{\miouCILVDEnvaBoundaryLOne}{\tbd{miouCILVDEnvaBoundaryLOne}}
\providecommand{\miouCILVDEnvaBoundaryLTwo}{\tbd{miouCILVDEnvaBoundaryLTwo}}
\providecommand{\miouCILVDEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCILVDEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDEnvaBoundaryLTwoVarDecoderSamLite}{\tbd{miouCILVDEnvaBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouCILVDEnvaBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouCILVDEnvaBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCILVDEnvaBoundaryLTwoVarLrMultOne}{\tbd{miouCILVDEnvaBoundaryLTwoVarLrMultOne}}
\providecommand{\miouCILVDEnvaClean}{\tbd{miouCILVDEnvaClean}}
\providecommand{\miouCILVDEnvaCleanVarDecoderMaskTwoformerLite}{\tbd{miouCILVDEnvaCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDEnvaCleanVarDecoderSamLite}{\tbd{miouCILVDEnvaCleanVarDecoderSamLite}}
\providecommand{\miouCILVDEnvaCleanVarDecoderSegformerMlp}{\tbd{miouCILVDEnvaCleanVarDecoderSegformerMlp}}
\providecommand{\miouCILVDEnvaCleanVarLrMultOne}{\tbd{miouCILVDEnvaCleanVarLrMultOne}}
\providecommand{\miouCILVDEnvaCoarseLOne}{\tbd{miouCILVDEnvaCoarseLOne}}
\providecommand{\miouCILVDEnvaCoarseLTwo}{\tbd{miouCILVDEnvaCoarseLTwo}}
\providecommand{\miouCILVDEnvaCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCILVDEnvaCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDEnvaCoarseLTwoVarDecoderSamLite}{\tbd{miouCILVDEnvaCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouCILVDEnvaCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouCILVDEnvaCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCILVDEnvaCoarseLTwoVarLrMultOne}{\tbd{miouCILVDEnvaCoarseLTwoVarLrMultOne}}
\providecommand{\miouCILVDEnvaNlcdREAL}{\tbd{miouCILVDEnvaNlcdREAL}}
\providecommand{\miouCILVDEnvaOmissionLOne}{\tbd{miouCILVDEnvaOmissionLOne}}
\providecommand{\miouCILVDEnvaOmissionLTwo}{\tbd{miouCILVDEnvaOmissionLTwo}}
\providecommand{\miouCILVDEnvaOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCILVDEnvaOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDEnvaOmissionLTwoVarDecoderSamLite}{\tbd{miouCILVDEnvaOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouCILVDEnvaOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouCILVDEnvaOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCILVDEnvaOmissionLTwoVarLrMultOne}{\tbd{miouCILVDEnvaOmissionLTwoVarLrMultOne}}
\providecommand{\miouCILVDEnvaShiftLOne}{\tbd{miouCILVDEnvaShiftLOne}}
\providecommand{\miouCILVDEnvaShiftLTwo}{\tbd{miouCILVDEnvaShiftLTwo}}
\providecommand{\miouCILVDEnvaShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCILVDEnvaShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDEnvaShiftLTwoVarDecoderSamLite}{\tbd{miouCILVDEnvaShiftLTwoVarDecoderSamLite}}
\providecommand{\miouCILVDEnvaShiftLTwoVarDecoderSegformerMlp}{\tbd{miouCILVDEnvaShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCILVDEnvaShiftLTwoVarLrMultOne}{\tbd{miouCILVDEnvaShiftLTwoVarLrMultOne}}
\providecommand{\miouCILVDKuroBoundaryLOne}{\tbd{miouCILVDKuroBoundaryLOne}}
\providecommand{\miouCILVDKuroBoundaryLTwo}{\tbd{miouCILVDKuroBoundaryLTwo}}
\providecommand{\miouCILVDKuroBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCILVDKuroBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDKuroBoundaryLTwoVarDecoderSamLite}{\tbd{miouCILVDKuroBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouCILVDKuroBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouCILVDKuroBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCILVDKuroBoundaryLTwoVarLrMultOne}{\tbd{miouCILVDKuroBoundaryLTwoVarLrMultOne}}
\providecommand{\miouCILVDKuroCemsREALVarTrainSubsetRealcov}{\tbd{miouCILVDKuroCemsREALVarTrainSubsetRealcov}}
\providecommand{\miouCILVDKuroClean}{\tbd{miouCILVDKuroClean}}
\providecommand{\miouCILVDKuroCleanVarDecoderMaskTwoformerLite}{\tbd{miouCILVDKuroCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDKuroCleanVarDecoderSamLite}{\tbd{miouCILVDKuroCleanVarDecoderSamLite}}
\providecommand{\miouCILVDKuroCleanVarDecoderSegformerMlp}{\tbd{miouCILVDKuroCleanVarDecoderSegformerMlp}}
\providecommand{\miouCILVDKuroCleanVarLrMultOne}{\tbd{miouCILVDKuroCleanVarLrMultOne}}
\providecommand{\miouCILVDKuroCleanVarTrainSubsetRealcov}{\tbd{miouCILVDKuroCleanVarTrainSubsetRealcov}}
\providecommand{\miouCILVDKuroCoarseLOne}{\tbd{miouCILVDKuroCoarseLOne}}
\providecommand{\miouCILVDKuroCoarseLTwo}{\tbd{miouCILVDKuroCoarseLTwo}}
\providecommand{\miouCILVDKuroCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCILVDKuroCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDKuroCoarseLTwoVarDecoderSamLite}{\tbd{miouCILVDKuroCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouCILVDKuroCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouCILVDKuroCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCILVDKuroCoarseLTwoVarLrMultOne}{\tbd{miouCILVDKuroCoarseLTwoVarLrMultOne}}
\providecommand{\miouCILVDKuroOmissionLOne}{\tbd{miouCILVDKuroOmissionLOne}}
\providecommand{\miouCILVDKuroOmissionLTwo}{\tbd{miouCILVDKuroOmissionLTwo}}
\providecommand{\miouCILVDKuroOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCILVDKuroOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDKuroOmissionLTwoVarDecoderSamLite}{\tbd{miouCILVDKuroOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouCILVDKuroOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouCILVDKuroOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCILVDKuroOmissionLTwoVarLrMultOne}{\tbd{miouCILVDKuroOmissionLTwoVarLrMultOne}}
\providecommand{\miouCILVDKuroShiftLOne}{\tbd{miouCILVDKuroShiftLOne}}
\providecommand{\miouCILVDKuroShiftLTwo}{\tbd{miouCILVDKuroShiftLTwo}}
\providecommand{\miouCILVDKuroShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCILVDKuroShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDKuroShiftLTwoVarDecoderSamLite}{\tbd{miouCILVDKuroShiftLTwoVarDecoderSamLite}}
\providecommand{\miouCILVDKuroShiftLTwoVarDecoderSegformerMlp}{\tbd{miouCILVDKuroShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCILVDKuroShiftLTwoVarLrMultOne}{\tbd{miouCILVDKuroShiftLTwoVarLrMultOne}}
\providecommand{\miouCILVDOemBoundaryLOne}{\tbd{miouCILVDOemBoundaryLOne}}
\providecommand{\miouCILVDOemBoundaryLTwo}{\tbd{miouCILVDOemBoundaryLTwo}}
\providecommand{\miouCILVDOemBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCILVDOemBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDOemBoundaryLTwoVarDecoderSamLite}{\tbd{miouCILVDOemBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouCILVDOemBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouCILVDOemBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCILVDOemBoundaryLTwoVarLrMultOne}{\tbd{miouCILVDOemBoundaryLTwoVarLrMultOne}}
\providecommand{\miouCILVDOemClean}{\tbd{miouCILVDOemClean}}
\providecommand{\miouCILVDOemCleanVarDecoderMaskTwoformerLite}{\tbd{miouCILVDOemCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDOemCleanVarDecoderSamLite}{\tbd{miouCILVDOemCleanVarDecoderSamLite}}
\providecommand{\miouCILVDOemCleanVarDecoderSegformerMlp}{\tbd{miouCILVDOemCleanVarDecoderSegformerMlp}}
\providecommand{\miouCILVDOemCleanVarLrMultOne}{\tbd{miouCILVDOemCleanVarLrMultOne}}
\providecommand{\miouCILVDOemCoarseLOne}{\tbd{miouCILVDOemCoarseLOne}}
\providecommand{\miouCILVDOemCoarseLTwo}{\tbd{miouCILVDOemCoarseLTwo}}
\providecommand{\miouCILVDOemCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCILVDOemCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDOemCoarseLTwoVarDecoderSamLite}{\tbd{miouCILVDOemCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouCILVDOemCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouCILVDOemCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCILVDOemCoarseLTwoVarLrMultOne}{\tbd{miouCILVDOemCoarseLTwoVarLrMultOne}}
\providecommand{\miouCILVDOemOmissionLOne}{\tbd{miouCILVDOemOmissionLOne}}
\providecommand{\miouCILVDOemOmissionLTwo}{\tbd{miouCILVDOemOmissionLTwo}}
\providecommand{\miouCILVDOemOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCILVDOemOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDOemOmissionLTwoVarDecoderSamLite}{\tbd{miouCILVDOemOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouCILVDOemOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouCILVDOemOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCILVDOemOmissionLTwoVarLrMultOne}{\tbd{miouCILVDOemOmissionLTwoVarLrMultOne}}
\providecommand{\miouCILVDOemShiftLOne}{\tbd{miouCILVDOemShiftLOne}}
\providecommand{\miouCILVDOemShiftLTwo}{\tbd{miouCILVDOemShiftLTwo}}
\providecommand{\miouCILVDOemShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCILVDOemShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDOemShiftLTwoVarDecoderSamLite}{\tbd{miouCILVDOemShiftLTwoVarDecoderSamLite}}
\providecommand{\miouCILVDOemShiftLTwoVarDecoderSegformerMlp}{\tbd{miouCILVDOemShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCILVDOemShiftLTwoVarLrMultOne}{\tbd{miouCILVDOemShiftLTwoVarLrMultOne}}
\providecommand{\miouCILVDSnTwoBoundaryLOne}{\tbd{miouCILVDSnTwoBoundaryLOne}}
\providecommand{\miouCILVDSnTwoBoundaryLTwo}{\tbd{miouCILVDSnTwoBoundaryLTwo}}
\providecommand{\miouCILVDSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCILVDSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDSnTwoBoundaryLTwoVarDecoderSamLite}{\tbd{miouCILVDSnTwoBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouCILVDSnTwoBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouCILVDSnTwoBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCILVDSnTwoBoundaryLTwoVarLrMultOne}{\tbd{miouCILVDSnTwoBoundaryLTwoVarLrMultOne}}
\providecommand{\miouCILVDSnTwoClean}{\tbd{miouCILVDSnTwoClean}}
\providecommand{\miouCILVDSnTwoCleanVarDecoderMaskTwoformerLite}{\tbd{miouCILVDSnTwoCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDSnTwoCleanVarDecoderSamLite}{\tbd{miouCILVDSnTwoCleanVarDecoderSamLite}}
\providecommand{\miouCILVDSnTwoCleanVarDecoderSegformerMlp}{\tbd{miouCILVDSnTwoCleanVarDecoderSegformerMlp}}
\providecommand{\miouCILVDSnTwoCleanVarLrMultOne}{\tbd{miouCILVDSnTwoCleanVarLrMultOne}}
\providecommand{\miouCILVDSnTwoCoarseLOne}{\tbd{miouCILVDSnTwoCoarseLOne}}
\providecommand{\miouCILVDSnTwoCoarseLTwo}{\tbd{miouCILVDSnTwoCoarseLTwo}}
\providecommand{\miouCILVDSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCILVDSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDSnTwoCoarseLTwoVarDecoderSamLite}{\tbd{miouCILVDSnTwoCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouCILVDSnTwoCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouCILVDSnTwoCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCILVDSnTwoCoarseLTwoVarLrMultOne}{\tbd{miouCILVDSnTwoCoarseLTwoVarLrMultOne}}
\providecommand{\miouCILVDSnTwoOmissionLOne}{\tbd{miouCILVDSnTwoOmissionLOne}}
\providecommand{\miouCILVDSnTwoOmissionLTwo}{\tbd{miouCILVDSnTwoOmissionLTwo}}
\providecommand{\miouCILVDSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCILVDSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDSnTwoOmissionLTwoVarDecoderSamLite}{\tbd{miouCILVDSnTwoOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouCILVDSnTwoOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouCILVDSnTwoOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCILVDSnTwoOmissionLTwoVarLrMultOne}{\tbd{miouCILVDSnTwoOmissionLTwoVarLrMultOne}}
\providecommand{\miouCILVDSnTwoShiftLOne}{\tbd{miouCILVDSnTwoShiftLOne}}
\providecommand{\miouCILVDSnTwoShiftLTwo}{\tbd{miouCILVDSnTwoShiftLTwo}}
\providecommand{\miouCILVDSnTwoShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCILVDSnTwoShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDSnTwoShiftLTwoVarDecoderSamLite}{\tbd{miouCILVDSnTwoShiftLTwoVarDecoderSamLite}}
\providecommand{\miouCILVDSnTwoShiftLTwoVarDecoderSegformerMlp}{\tbd{miouCILVDSnTwoShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCILVDSnTwoShiftLTwoVarLrMultOne}{\tbd{miouCILVDSnTwoShiftLTwoVarLrMultOne}}
\providecommand{\miouCILVDburnBoundaryLOne}{\tbd{miouCILVDburnBoundaryLOne}}
\providecommand{\miouCILVDburnBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{miouCILVDburnBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCILVDburnBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{miouCILVDburnBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDburnBoundaryLOneVarDecoderSamLite}{\tbd{miouCILVDburnBoundaryLOneVarDecoderSamLite}}
\providecommand{\miouCILVDburnBoundaryLOneVarDecoderSamPretrained}{\tbd{miouCILVDburnBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\miouCILVDburnBoundaryLOneVarDecoderSegformerMlp}{\tbd{miouCILVDburnBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\miouCILVDburnBoundaryLR}{\tbd{miouCILVDburnBoundaryLR}}
\providecommand{\miouCILVDburnBoundaryLRVarLrMultOne}{\tbd{miouCILVDburnBoundaryLRVarLrMultOne}}
\providecommand{\miouCILVDburnBoundaryLTwo}{\tbd{miouCILVDburnBoundaryLTwo}}
\providecommand{\miouCILVDburnBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCILVDburnBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCILVDburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{miouCILVDburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\miouCILVDburnBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCILVDburnBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{miouCILVDburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\miouCILVDburnBoundaryLTwoVarDecoderSamLite}{\tbd{miouCILVDburnBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouCILVDburnBoundaryLTwoVarDecoderSamLiteLrMultOne}{\tbd{miouCILVDburnBoundaryLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\miouCILVDburnBoundaryLTwoVarDecoderSamPretrained}{\tbd{miouCILVDburnBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\miouCILVDburnBoundaryLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{miouCILVDburnBoundaryLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\miouCILVDburnBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouCILVDburnBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCILVDburnBoundaryLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{miouCILVDburnBoundaryLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\miouCILVDburnBoundaryLTwoVarLossBootstrap}{\tbd{miouCILVDburnBoundaryLTwoVarLossBootstrap}}
\providecommand{\miouCILVDburnBoundaryLTwoVarLossGce}{\tbd{miouCILVDburnBoundaryLTwoVarLossGce}}
\providecommand{\miouCILVDburnBoundaryLTwoVarLrMultOne}{\tbd{miouCILVDburnBoundaryLTwoVarLrMultOne}}
\providecommand{\miouCILVDburnBoundaryLTwoVarLrMultThree}{\tbd{miouCILVDburnBoundaryLTwoVarLrMultThree}}
\providecommand{\miouCILVDburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCILVDburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCILVDburnBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCILVDburnBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCILVDburnClean}{\tbd{miouCILVDburnClean}}
\providecommand{\miouCILVDburnCleanVarDecoderMaskTwoformerFull}{\tbd{miouCILVDburnCleanVarDecoderMaskTwoformerFull}}
\providecommand{\miouCILVDburnCleanVarDecoderMaskTwoformerFullLrMultOne}{\tbd{miouCILVDburnCleanVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\miouCILVDburnCleanVarDecoderMaskTwoformerLite}{\tbd{miouCILVDburnCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDburnCleanVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{miouCILVDburnCleanVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\miouCILVDburnCleanVarDecoderSamLite}{\tbd{miouCILVDburnCleanVarDecoderSamLite}}
\providecommand{\miouCILVDburnCleanVarDecoderSamLiteLrMultOne}{\tbd{miouCILVDburnCleanVarDecoderSamLiteLrMultOne}}
\providecommand{\miouCILVDburnCleanVarDecoderSamPretrained}{\tbd{miouCILVDburnCleanVarDecoderSamPretrained}}
\providecommand{\miouCILVDburnCleanVarDecoderSamPretrainedLrMultOne}{\tbd{miouCILVDburnCleanVarDecoderSamPretrainedLrMultOne}}
\providecommand{\miouCILVDburnCleanVarDecoderSegformerMlp}{\tbd{miouCILVDburnCleanVarDecoderSegformerMlp}}
\providecommand{\miouCILVDburnCleanVarDecoderSegformerMlpLrMultOne}{\tbd{miouCILVDburnCleanVarDecoderSegformerMlpLrMultOne}}
\providecommand{\miouCILVDburnCleanVarLossBootstrap}{\tbd{miouCILVDburnCleanVarLossBootstrap}}
\providecommand{\miouCILVDburnCleanVarLossGce}{\tbd{miouCILVDburnCleanVarLossGce}}
\providecommand{\miouCILVDburnCleanVarLrMultOne}{\tbd{miouCILVDburnCleanVarLrMultOne}}
\providecommand{\miouCILVDburnCleanVarLrMultThree}{\tbd{miouCILVDburnCleanVarLrMultThree}}
\providecommand{\miouCILVDburnCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCILVDburnCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCILVDburnCleanVarTrainSubsetCleanTwoFive}{\tbd{miouCILVDburnCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCILVDburnCoarseLOne}{\tbd{miouCILVDburnCoarseLOne}}
\providecommand{\miouCILVDburnCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{miouCILVDburnCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCILVDburnCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{miouCILVDburnCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDburnCoarseLOneVarDecoderSamLite}{\tbd{miouCILVDburnCoarseLOneVarDecoderSamLite}}
\providecommand{\miouCILVDburnCoarseLOneVarDecoderSamPretrained}{\tbd{miouCILVDburnCoarseLOneVarDecoderSamPretrained}}
\providecommand{\miouCILVDburnCoarseLOneVarDecoderSegformerMlp}{\tbd{miouCILVDburnCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\miouCILVDburnCoarseLR}{\tbd{miouCILVDburnCoarseLR}}
\providecommand{\miouCILVDburnCoarseLRVarLrMultOne}{\tbd{miouCILVDburnCoarseLRVarLrMultOne}}
\providecommand{\miouCILVDburnCoarseLTwo}{\tbd{miouCILVDburnCoarseLTwo}}
\providecommand{\miouCILVDburnCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCILVDburnCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCILVDburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{miouCILVDburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\miouCILVDburnCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCILVDburnCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{miouCILVDburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\miouCILVDburnCoarseLTwoVarDecoderSamLite}{\tbd{miouCILVDburnCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouCILVDburnCoarseLTwoVarDecoderSamLiteLrMultOne}{\tbd{miouCILVDburnCoarseLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\miouCILVDburnCoarseLTwoVarDecoderSamPretrained}{\tbd{miouCILVDburnCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\miouCILVDburnCoarseLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{miouCILVDburnCoarseLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\miouCILVDburnCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouCILVDburnCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCILVDburnCoarseLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{miouCILVDburnCoarseLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\miouCILVDburnCoarseLTwoVarLossBootstrap}{\tbd{miouCILVDburnCoarseLTwoVarLossBootstrap}}
\providecommand{\miouCILVDburnCoarseLTwoVarLossGce}{\tbd{miouCILVDburnCoarseLTwoVarLossGce}}
\providecommand{\miouCILVDburnCoarseLTwoVarLrMultOne}{\tbd{miouCILVDburnCoarseLTwoVarLrMultOne}}
\providecommand{\miouCILVDburnCoarseLTwoVarLrMultThree}{\tbd{miouCILVDburnCoarseLTwoVarLrMultThree}}
\providecommand{\miouCILVDburnCoarseLTwoVarLrMultZeroOneOneOneOne}{\tbd{miouCILVDburnCoarseLTwoVarLrMultZeroOneOneOneOne}}
\providecommand{\miouCILVDburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCILVDburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCILVDburnCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCILVDburnCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCILVDburnOmissionLOne}{\tbd{miouCILVDburnOmissionLOne}}
\providecommand{\miouCILVDburnOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{miouCILVDburnOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCILVDburnOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{miouCILVDburnOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDburnOmissionLOneVarDecoderSamLite}{\tbd{miouCILVDburnOmissionLOneVarDecoderSamLite}}
\providecommand{\miouCILVDburnOmissionLOneVarDecoderSamPretrained}{\tbd{miouCILVDburnOmissionLOneVarDecoderSamPretrained}}
\providecommand{\miouCILVDburnOmissionLOneVarDecoderSegformerMlp}{\tbd{miouCILVDburnOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\miouCILVDburnOmissionLR}{\tbd{miouCILVDburnOmissionLR}}
\providecommand{\miouCILVDburnOmissionLRVarLrMultOne}{\tbd{miouCILVDburnOmissionLRVarLrMultOne}}
\providecommand{\miouCILVDburnOmissionLTwo}{\tbd{miouCILVDburnOmissionLTwo}}
\providecommand{\miouCILVDburnOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCILVDburnOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCILVDburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{miouCILVDburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\miouCILVDburnOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCILVDburnOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{miouCILVDburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\miouCILVDburnOmissionLTwoVarDecoderSamLite}{\tbd{miouCILVDburnOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouCILVDburnOmissionLTwoVarDecoderSamLiteLrMultOne}{\tbd{miouCILVDburnOmissionLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\miouCILVDburnOmissionLTwoVarDecoderSamPretrained}{\tbd{miouCILVDburnOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\miouCILVDburnOmissionLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{miouCILVDburnOmissionLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\miouCILVDburnOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouCILVDburnOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCILVDburnOmissionLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{miouCILVDburnOmissionLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\miouCILVDburnOmissionLTwoVarLossBootstrap}{\tbd{miouCILVDburnOmissionLTwoVarLossBootstrap}}
\providecommand{\miouCILVDburnOmissionLTwoVarLossGce}{\tbd{miouCILVDburnOmissionLTwoVarLossGce}}
\providecommand{\miouCILVDburnOmissionLTwoVarLrMultOne}{\tbd{miouCILVDburnOmissionLTwoVarLrMultOne}}
\providecommand{\miouCILVDburnOmissionLTwoVarLrMultThree}{\tbd{miouCILVDburnOmissionLTwoVarLrMultThree}}
\providecommand{\miouCILVDburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCILVDburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCILVDburnOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCILVDburnOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCILVDburnShiftLOne}{\tbd{miouCILVDburnShiftLOne}}
\providecommand{\miouCILVDburnShiftLOneVarDecoderMaskTwoformerFull}{\tbd{miouCILVDburnShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCILVDburnShiftLOneVarDecoderMaskTwoformerLite}{\tbd{miouCILVDburnShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDburnShiftLOneVarDecoderSamLite}{\tbd{miouCILVDburnShiftLOneVarDecoderSamLite}}
\providecommand{\miouCILVDburnShiftLOneVarDecoderSamPretrained}{\tbd{miouCILVDburnShiftLOneVarDecoderSamPretrained}}
\providecommand{\miouCILVDburnShiftLOneVarDecoderSegformerMlp}{\tbd{miouCILVDburnShiftLOneVarDecoderSegformerMlp}}
\providecommand{\miouCILVDburnShiftLR}{\tbd{miouCILVDburnShiftLR}}
\providecommand{\miouCILVDburnShiftLRVarLrMultOne}{\tbd{miouCILVDburnShiftLRVarLrMultOne}}
\providecommand{\miouCILVDburnShiftLTwo}{\tbd{miouCILVDburnShiftLTwo}}
\providecommand{\miouCILVDburnShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCILVDburnShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCILVDburnShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{miouCILVDburnShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\miouCILVDburnShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCILVDburnShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{miouCILVDburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\miouCILVDburnShiftLTwoVarDecoderSamLite}{\tbd{miouCILVDburnShiftLTwoVarDecoderSamLite}}
\providecommand{\miouCILVDburnShiftLTwoVarDecoderSamLiteLrMultOne}{\tbd{miouCILVDburnShiftLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\miouCILVDburnShiftLTwoVarDecoderSamPretrained}{\tbd{miouCILVDburnShiftLTwoVarDecoderSamPretrained}}
\providecommand{\miouCILVDburnShiftLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{miouCILVDburnShiftLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\miouCILVDburnShiftLTwoVarDecoderSegformerMlp}{\tbd{miouCILVDburnShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCILVDburnShiftLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{miouCILVDburnShiftLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\miouCILVDburnShiftLTwoVarLossBootstrap}{\tbd{miouCILVDburnShiftLTwoVarLossBootstrap}}
\providecommand{\miouCILVDburnShiftLTwoVarLossGce}{\tbd{miouCILVDburnShiftLTwoVarLossGce}}
\providecommand{\miouCILVDburnShiftLTwoVarLrMultOne}{\tbd{miouCILVDburnShiftLTwoVarLrMultOne}}
\providecommand{\miouCILVDburnShiftLTwoVarLrMultThree}{\tbd{miouCILVDburnShiftLTwoVarLrMultThree}}
\providecommand{\miouCILVDburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCILVDburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCILVDburnShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCILVDburnShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCILVDflairBoundaryLOne}{\tbd{miouCILVDflairBoundaryLOne}}
\providecommand{\miouCILVDflairBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{miouCILVDflairBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCILVDflairBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{miouCILVDflairBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDflairBoundaryLOneVarDecoderSamLite}{\tbd{miouCILVDflairBoundaryLOneVarDecoderSamLite}}
\providecommand{\miouCILVDflairBoundaryLOneVarDecoderSamPretrained}{\tbd{miouCILVDflairBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\miouCILVDflairBoundaryLOneVarDecoderSegformerMlp}{\tbd{miouCILVDflairBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\miouCILVDflairBoundaryLR}{\tbd{miouCILVDflairBoundaryLR}}
\providecommand{\miouCILVDflairBoundaryLRVarLrMultOne}{\tbd{miouCILVDflairBoundaryLRVarLrMultOne}}
\providecommand{\miouCILVDflairBoundaryLTwo}{\tbd{miouCILVDflairBoundaryLTwo}}
\providecommand{\miouCILVDflairBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCILVDflairBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCILVDflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{miouCILVDflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\miouCILVDflairBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCILVDflairBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{miouCILVDflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\miouCILVDflairBoundaryLTwoVarDecoderSamLite}{\tbd{miouCILVDflairBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouCILVDflairBoundaryLTwoVarDecoderSamLiteLrMultOne}{\tbd{miouCILVDflairBoundaryLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\miouCILVDflairBoundaryLTwoVarDecoderSamPretrained}{\tbd{miouCILVDflairBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\miouCILVDflairBoundaryLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{miouCILVDflairBoundaryLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\miouCILVDflairBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouCILVDflairBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCILVDflairBoundaryLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{miouCILVDflairBoundaryLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\miouCILVDflairBoundaryLTwoVarLossBootstrap}{\tbd{miouCILVDflairBoundaryLTwoVarLossBootstrap}}
\providecommand{\miouCILVDflairBoundaryLTwoVarLossGce}{\tbd{miouCILVDflairBoundaryLTwoVarLossGce}}
\providecommand{\miouCILVDflairBoundaryLTwoVarLrMultOne}{\tbd{miouCILVDflairBoundaryLTwoVarLrMultOne}}
\providecommand{\miouCILVDflairBoundaryLTwoVarLrMultThree}{\tbd{miouCILVDflairBoundaryLTwoVarLrMultThree}}
\providecommand{\miouCILVDflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCILVDflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCILVDflairBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCILVDflairBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCILVDflairClean}{\tbd{miouCILVDflairClean}}
\providecommand{\miouCILVDflairCleanVarDecoderMaskTwoformerFull}{\tbd{miouCILVDflairCleanVarDecoderMaskTwoformerFull}}
\providecommand{\miouCILVDflairCleanVarDecoderMaskTwoformerFullLrMultOne}{\tbd{miouCILVDflairCleanVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\miouCILVDflairCleanVarDecoderMaskTwoformerLite}{\tbd{miouCILVDflairCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDflairCleanVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{miouCILVDflairCleanVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\miouCILVDflairCleanVarDecoderSamLite}{\tbd{miouCILVDflairCleanVarDecoderSamLite}}
\providecommand{\miouCILVDflairCleanVarDecoderSamLiteLrMultOne}{\tbd{miouCILVDflairCleanVarDecoderSamLiteLrMultOne}}
\providecommand{\miouCILVDflairCleanVarDecoderSamPretrained}{\tbd{miouCILVDflairCleanVarDecoderSamPretrained}}
\providecommand{\miouCILVDflairCleanVarDecoderSamPretrainedLrMultOne}{\tbd{miouCILVDflairCleanVarDecoderSamPretrainedLrMultOne}}
\providecommand{\miouCILVDflairCleanVarDecoderSegformerMlp}{\tbd{miouCILVDflairCleanVarDecoderSegformerMlp}}
\providecommand{\miouCILVDflairCleanVarDecoderSegformerMlpLrMultOne}{\tbd{miouCILVDflairCleanVarDecoderSegformerMlpLrMultOne}}
\providecommand{\miouCILVDflairCleanVarLossBootstrap}{\tbd{miouCILVDflairCleanVarLossBootstrap}}
\providecommand{\miouCILVDflairCleanVarLossGce}{\tbd{miouCILVDflairCleanVarLossGce}}
\providecommand{\miouCILVDflairCleanVarLrMultOne}{\tbd{miouCILVDflairCleanVarLrMultOne}}
\providecommand{\miouCILVDflairCleanVarLrMultThree}{\tbd{miouCILVDflairCleanVarLrMultThree}}
\providecommand{\miouCILVDflairCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCILVDflairCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCILVDflairCleanVarTrainSubsetCleanTwoFive}{\tbd{miouCILVDflairCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCILVDflairCoarseLOne}{\tbd{miouCILVDflairCoarseLOne}}
\providecommand{\miouCILVDflairCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{miouCILVDflairCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCILVDflairCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{miouCILVDflairCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDflairCoarseLOneVarDecoderSamLite}{\tbd{miouCILVDflairCoarseLOneVarDecoderSamLite}}
\providecommand{\miouCILVDflairCoarseLOneVarDecoderSamPretrained}{\tbd{miouCILVDflairCoarseLOneVarDecoderSamPretrained}}
\providecommand{\miouCILVDflairCoarseLOneVarDecoderSegformerMlp}{\tbd{miouCILVDflairCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\miouCILVDflairCoarseLR}{\tbd{miouCILVDflairCoarseLR}}
\providecommand{\miouCILVDflairCoarseLRVarLrMultOne}{\tbd{miouCILVDflairCoarseLRVarLrMultOne}}
\providecommand{\miouCILVDflairCoarseLTwo}{\tbd{miouCILVDflairCoarseLTwo}}
\providecommand{\miouCILVDflairCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCILVDflairCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCILVDflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{miouCILVDflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\miouCILVDflairCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCILVDflairCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{miouCILVDflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\miouCILVDflairCoarseLTwoVarDecoderSamLite}{\tbd{miouCILVDflairCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouCILVDflairCoarseLTwoVarDecoderSamLiteLrMultOne}{\tbd{miouCILVDflairCoarseLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\miouCILVDflairCoarseLTwoVarDecoderSamPretrained}{\tbd{miouCILVDflairCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\miouCILVDflairCoarseLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{miouCILVDflairCoarseLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\miouCILVDflairCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouCILVDflairCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCILVDflairCoarseLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{miouCILVDflairCoarseLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\miouCILVDflairCoarseLTwoVarLossBootstrap}{\tbd{miouCILVDflairCoarseLTwoVarLossBootstrap}}
\providecommand{\miouCILVDflairCoarseLTwoVarLossGce}{\tbd{miouCILVDflairCoarseLTwoVarLossGce}}
\providecommand{\miouCILVDflairCoarseLTwoVarLrMultOne}{\tbd{miouCILVDflairCoarseLTwoVarLrMultOne}}
\providecommand{\miouCILVDflairCoarseLTwoVarLrMultThree}{\tbd{miouCILVDflairCoarseLTwoVarLrMultThree}}
\providecommand{\miouCILVDflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCILVDflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCILVDflairCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCILVDflairCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCILVDflairOmissionLOne}{\tbd{miouCILVDflairOmissionLOne}}
\providecommand{\miouCILVDflairOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{miouCILVDflairOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCILVDflairOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{miouCILVDflairOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDflairOmissionLOneVarDecoderSamLite}{\tbd{miouCILVDflairOmissionLOneVarDecoderSamLite}}
\providecommand{\miouCILVDflairOmissionLOneVarDecoderSamPretrained}{\tbd{miouCILVDflairOmissionLOneVarDecoderSamPretrained}}
\providecommand{\miouCILVDflairOmissionLOneVarDecoderSegformerMlp}{\tbd{miouCILVDflairOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\miouCILVDflairOmissionLR}{\tbd{miouCILVDflairOmissionLR}}
\providecommand{\miouCILVDflairOmissionLRVarLrMultOne}{\tbd{miouCILVDflairOmissionLRVarLrMultOne}}
\providecommand{\miouCILVDflairOmissionLTwo}{\tbd{miouCILVDflairOmissionLTwo}}
\providecommand{\miouCILVDflairOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCILVDflairOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCILVDflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{miouCILVDflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\miouCILVDflairOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCILVDflairOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{miouCILVDflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\miouCILVDflairOmissionLTwoVarDecoderSamLite}{\tbd{miouCILVDflairOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouCILVDflairOmissionLTwoVarDecoderSamLiteLrMultOne}{\tbd{miouCILVDflairOmissionLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\miouCILVDflairOmissionLTwoVarDecoderSamPretrained}{\tbd{miouCILVDflairOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\miouCILVDflairOmissionLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{miouCILVDflairOmissionLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\miouCILVDflairOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouCILVDflairOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCILVDflairOmissionLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{miouCILVDflairOmissionLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\miouCILVDflairOmissionLTwoVarLossBootstrap}{\tbd{miouCILVDflairOmissionLTwoVarLossBootstrap}}
\providecommand{\miouCILVDflairOmissionLTwoVarLossGce}{\tbd{miouCILVDflairOmissionLTwoVarLossGce}}
\providecommand{\miouCILVDflairOmissionLTwoVarLrMultOne}{\tbd{miouCILVDflairOmissionLTwoVarLrMultOne}}
\providecommand{\miouCILVDflairOmissionLTwoVarLrMultThree}{\tbd{miouCILVDflairOmissionLTwoVarLrMultThree}}
\providecommand{\miouCILVDflairOmissionLTwoVarLrMultZeroOneOneOneOne}{\tbd{miouCILVDflairOmissionLTwoVarLrMultZeroOneOneOneOne}}
\providecommand{\miouCILVDflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCILVDflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCILVDflairOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCILVDflairOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCILVDflairShiftLOne}{\tbd{miouCILVDflairShiftLOne}}
\providecommand{\miouCILVDflairShiftLOneVarDecoderMaskTwoformerFull}{\tbd{miouCILVDflairShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCILVDflairShiftLOneVarDecoderMaskTwoformerLite}{\tbd{miouCILVDflairShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDflairShiftLOneVarDecoderSamLite}{\tbd{miouCILVDflairShiftLOneVarDecoderSamLite}}
\providecommand{\miouCILVDflairShiftLOneVarDecoderSamPretrained}{\tbd{miouCILVDflairShiftLOneVarDecoderSamPretrained}}
\providecommand{\miouCILVDflairShiftLOneVarDecoderSegformerMlp}{\tbd{miouCILVDflairShiftLOneVarDecoderSegformerMlp}}
\providecommand{\miouCILVDflairShiftLR}{\tbd{miouCILVDflairShiftLR}}
\providecommand{\miouCILVDflairShiftLRVarLrMultOne}{\tbd{miouCILVDflairShiftLRVarLrMultOne}}
\providecommand{\miouCILVDflairShiftLTwo}{\tbd{miouCILVDflairShiftLTwo}}
\providecommand{\miouCILVDflairShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCILVDflairShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCILVDflairShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{miouCILVDflairShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\miouCILVDflairShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCILVDflairShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCILVDflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{miouCILVDflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\miouCILVDflairShiftLTwoVarDecoderSamLite}{\tbd{miouCILVDflairShiftLTwoVarDecoderSamLite}}
\providecommand{\miouCILVDflairShiftLTwoVarDecoderSamLiteLrMultOne}{\tbd{miouCILVDflairShiftLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\miouCILVDflairShiftLTwoVarDecoderSamPretrained}{\tbd{miouCILVDflairShiftLTwoVarDecoderSamPretrained}}
\providecommand{\miouCILVDflairShiftLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{miouCILVDflairShiftLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\miouCILVDflairShiftLTwoVarDecoderSegformerMlp}{\tbd{miouCILVDflairShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCILVDflairShiftLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{miouCILVDflairShiftLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\miouCILVDflairShiftLTwoVarLossBootstrap}{\tbd{miouCILVDflairShiftLTwoVarLossBootstrap}}
\providecommand{\miouCILVDflairShiftLTwoVarLossGce}{\tbd{miouCILVDflairShiftLTwoVarLossGce}}
\providecommand{\miouCILVDflairShiftLTwoVarLrMultOne}{\tbd{miouCILVDflairShiftLTwoVarLrMultOne}}
\providecommand{\miouCILVDflairShiftLTwoVarLrMultThree}{\tbd{miouCILVDflairShiftLTwoVarLrMultThree}}
\providecommand{\miouCILVDflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCILVDflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCILVDflairShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCILVDflairShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCILVDsenClean}{\tbd{miouCILVDsenClean}}
\providecommand{\miouCILVDsenOtsuLTwo}{\tbd{miouCILVDsenOtsuLTwo}}
\providecommand{\miouCIPRIburnBoundaryLOne}{\tbd{miouCIPRIburnBoundaryLOne}}
\providecommand{\miouCIPRIburnBoundaryLTwo}{\tbd{miouCIPRIburnBoundaryLTwo}}
\providecommand{\miouCIPRIburnClean}{\tbd{miouCIPRIburnClean}}
\providecommand{\miouCIPRIburnCleanVarTrainSubsetCleanTwoFive}{\tbd{miouCIPRIburnCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCIPRIburnCoarseLOne}{\tbd{miouCIPRIburnCoarseLOne}}
\providecommand{\miouCIPRIburnCoarseLTwo}{\tbd{miouCIPRIburnCoarseLTwo}}
\providecommand{\miouCIPRIburnOmissionLOne}{\tbd{miouCIPRIburnOmissionLOne}}
\providecommand{\miouCIPRIburnOmissionLTwo}{\tbd{miouCIPRIburnOmissionLTwo}}
\providecommand{\miouCIPRIburnShiftLOne}{\tbd{miouCIPRIburnShiftLOne}}
\providecommand{\miouCIPRIburnShiftLTwo}{\tbd{miouCIPRIburnShiftLTwo}}
\providecommand{\miouCIPRIflairBoundaryLOne}{\tbd{miouCIPRIflairBoundaryLOne}}
\providecommand{\miouCIPRIflairBoundaryLTwo}{\tbd{miouCIPRIflairBoundaryLTwo}}
\providecommand{\miouCIPRIflairClean}{\tbd{miouCIPRIflairClean}}
\providecommand{\miouCIPRIflairCleanVarTrainSubsetCleanTwoFive}{\tbd{miouCIPRIflairCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCIPRIflairCoarseLOne}{\tbd{miouCIPRIflairCoarseLOne}}
\providecommand{\miouCIPRIflairCoarseLTwo}{\tbd{miouCIPRIflairCoarseLTwo}}
\providecommand{\miouCIPRIflairOmissionLOne}{\tbd{miouCIPRIflairOmissionLOne}}
\providecommand{\miouCIPRIflairOmissionLTwo}{\tbd{miouCIPRIflairOmissionLTwo}}
\providecommand{\miouCIPRIflairShiftLOne}{\tbd{miouCIPRIflairShiftLOne}}
\providecommand{\miouCIPRIflairShiftLTwo}{\tbd{miouCIPRIflairShiftLTwo}}
\providecommand{\miouCIRNChesBoundaryLOne}{\tbd{miouCIRNChesBoundaryLOne}}
\providecommand{\miouCIRNChesBoundaryLTwo}{\tbd{miouCIRNChesBoundaryLTwo}}
\providecommand{\miouCIRNChesClean}{\tbd{miouCIRNChesClean}}
\providecommand{\miouCIRNChesCoarseLOne}{\tbd{miouCIRNChesCoarseLOne}}
\providecommand{\miouCIRNChesCoarseLTwo}{\tbd{miouCIRNChesCoarseLTwo}}
\providecommand{\miouCIRNChesNlcdREAL}{\tbd{miouCIRNChesNlcdREAL}}
\providecommand{\miouCIRNChesOmissionLOne}{\tbd{miouCIRNChesOmissionLOne}}
\providecommand{\miouCIRNChesOmissionLTwo}{\tbd{miouCIRNChesOmissionLTwo}}
\providecommand{\miouCIRNChesShiftLOne}{\tbd{miouCIRNChesShiftLOne}}
\providecommand{\miouCIRNChesShiftLTwo}{\tbd{miouCIRNChesShiftLTwo}}
\providecommand{\miouCIRNCsTwelveBoundaryLOne}{\tbd{miouCIRNCsTwelveBoundaryLOne}}
\providecommand{\miouCIRNCsTwelveBoundaryLTwo}{\tbd{miouCIRNCsTwelveBoundaryLTwo}}
\providecommand{\miouCIRNCsTwelveClean}{\tbd{miouCIRNCsTwelveClean}}
\providecommand{\miouCIRNCsTwelveCoarseLOne}{\tbd{miouCIRNCsTwelveCoarseLOne}}
\providecommand{\miouCIRNCsTwelveCoarseLTwo}{\tbd{miouCIRNCsTwelveCoarseLTwo}}
\providecommand{\miouCIRNCsTwelveOmissionLOne}{\tbd{miouCIRNCsTwelveOmissionLOne}}
\providecommand{\miouCIRNCsTwelveOmissionLTwo}{\tbd{miouCIRNCsTwelveOmissionLTwo}}
\providecommand{\miouCIRNCsTwelveSTwocloudlessREAL}{\tbd{miouCIRNCsTwelveSTwocloudlessREAL}}
\providecommand{\miouCIRNCsTwelveShiftLOne}{\tbd{miouCIRNCsTwelveShiftLOne}}
\providecommand{\miouCIRNCsTwelveShiftLTwo}{\tbd{miouCIRNCsTwelveShiftLTwo}}
\providecommand{\miouCIRNDfcBoundaryLOne}{\tbd{miouCIRNDfcBoundaryLOne}}
\providecommand{\miouCIRNDfcBoundaryLTwo}{\tbd{miouCIRNDfcBoundaryLTwo}}
\providecommand{\miouCIRNDfcClean}{\tbd{miouCIRNDfcClean}}
\providecommand{\miouCIRNDfcCleanVarTrainSubsetRealcov}{\tbd{miouCIRNDfcCleanVarTrainSubsetRealcov}}
\providecommand{\miouCIRNDfcCoarseLOne}{\tbd{miouCIRNDfcCoarseLOne}}
\providecommand{\miouCIRNDfcCoarseLTwo}{\tbd{miouCIRNDfcCoarseLTwo}}
\providecommand{\miouCIRNDfcModisREALVarTrainSubsetRealcov}{\tbd{miouCIRNDfcModisREALVarTrainSubsetRealcov}}
\providecommand{\miouCIRNDfcOmissionLOne}{\tbd{miouCIRNDfcOmissionLOne}}
\providecommand{\miouCIRNDfcOmissionLTwo}{\tbd{miouCIRNDfcOmissionLTwo}}
\providecommand{\miouCIRNDfcShiftLOne}{\tbd{miouCIRNDfcShiftLOne}}
\providecommand{\miouCIRNDfcShiftLTwo}{\tbd{miouCIRNDfcShiftLTwo}}
\providecommand{\miouCIRNEnvaBoundaryLOne}{\tbd{miouCIRNEnvaBoundaryLOne}}
\providecommand{\miouCIRNEnvaBoundaryLTwo}{\tbd{miouCIRNEnvaBoundaryLTwo}}
\providecommand{\miouCIRNEnvaClean}{\tbd{miouCIRNEnvaClean}}
\providecommand{\miouCIRNEnvaCoarseLOne}{\tbd{miouCIRNEnvaCoarseLOne}}
\providecommand{\miouCIRNEnvaCoarseLTwo}{\tbd{miouCIRNEnvaCoarseLTwo}}
\providecommand{\miouCIRNEnvaNlcdREAL}{\tbd{miouCIRNEnvaNlcdREAL}}
\providecommand{\miouCIRNEnvaOmissionLOne}{\tbd{miouCIRNEnvaOmissionLOne}}
\providecommand{\miouCIRNEnvaOmissionLTwo}{\tbd{miouCIRNEnvaOmissionLTwo}}
\providecommand{\miouCIRNEnvaShiftLOne}{\tbd{miouCIRNEnvaShiftLOne}}
\providecommand{\miouCIRNEnvaShiftLTwo}{\tbd{miouCIRNEnvaShiftLTwo}}
\providecommand{\miouCIRNKuroBoundaryLOne}{\tbd{miouCIRNKuroBoundaryLOne}}
\providecommand{\miouCIRNKuroBoundaryLTwo}{\tbd{miouCIRNKuroBoundaryLTwo}}
\providecommand{\miouCIRNKuroCemsREALVarTrainSubsetRealcov}{\tbd{miouCIRNKuroCemsREALVarTrainSubsetRealcov}}
\providecommand{\miouCIRNKuroClean}{\tbd{miouCIRNKuroClean}}
\providecommand{\miouCIRNKuroCleanVarTrainSubsetRealcov}{\tbd{miouCIRNKuroCleanVarTrainSubsetRealcov}}
\providecommand{\miouCIRNKuroCoarseLOne}{\tbd{miouCIRNKuroCoarseLOne}}
\providecommand{\miouCIRNKuroCoarseLTwo}{\tbd{miouCIRNKuroCoarseLTwo}}
\providecommand{\miouCIRNKuroOmissionLOne}{\tbd{miouCIRNKuroOmissionLOne}}
\providecommand{\miouCIRNKuroOmissionLTwo}{\tbd{miouCIRNKuroOmissionLTwo}}
\providecommand{\miouCIRNKuroShiftLOne}{\tbd{miouCIRNKuroShiftLOne}}
\providecommand{\miouCIRNKuroShiftLTwo}{\tbd{miouCIRNKuroShiftLTwo}}
\providecommand{\miouCIRNOemBoundaryLOne}{\tbd{miouCIRNOemBoundaryLOne}}
\providecommand{\miouCIRNOemBoundaryLTwo}{\tbd{miouCIRNOemBoundaryLTwo}}
\providecommand{\miouCIRNOemClean}{\tbd{miouCIRNOemClean}}
\providecommand{\miouCIRNOemCoarseLOne}{\tbd{miouCIRNOemCoarseLOne}}
\providecommand{\miouCIRNOemCoarseLTwo}{\tbd{miouCIRNOemCoarseLTwo}}
\providecommand{\miouCIRNOemOmissionLOne}{\tbd{miouCIRNOemOmissionLOne}}
\providecommand{\miouCIRNOemOmissionLTwo}{\tbd{miouCIRNOemOmissionLTwo}}
\providecommand{\miouCIRNOemShiftLOne}{\tbd{miouCIRNOemShiftLOne}}
\providecommand{\miouCIRNOemShiftLTwo}{\tbd{miouCIRNOemShiftLTwo}}
\providecommand{\miouCIRNSnTwoBoundaryLOne}{\tbd{miouCIRNSnTwoBoundaryLOne}}
\providecommand{\miouCIRNSnTwoBoundaryLTwo}{\tbd{miouCIRNSnTwoBoundaryLTwo}}
\providecommand{\miouCIRNSnTwoClean}{\tbd{miouCIRNSnTwoClean}}
\providecommand{\miouCIRNSnTwoCoarseLOne}{\tbd{miouCIRNSnTwoCoarseLOne}}
\providecommand{\miouCIRNSnTwoCoarseLTwo}{\tbd{miouCIRNSnTwoCoarseLTwo}}
\providecommand{\miouCIRNSnTwoOmissionLOne}{\tbd{miouCIRNSnTwoOmissionLOne}}
\providecommand{\miouCIRNSnTwoOmissionLTwo}{\tbd{miouCIRNSnTwoOmissionLTwo}}
\providecommand{\miouCIRNSnTwoShiftLOne}{\tbd{miouCIRNSnTwoShiftLOne}}
\providecommand{\miouCIRNSnTwoShiftLTwo}{\tbd{miouCIRNSnTwoShiftLTwo}}
\providecommand{\miouCIRNburnBoundaryLOne}{\tbd{miouCIRNburnBoundaryLOne}}
\providecommand{\miouCIRNburnBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{miouCIRNburnBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCIRNburnBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{miouCIRNburnBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCIRNburnBoundaryLOneVarDecoderSamLite}{\tbd{miouCIRNburnBoundaryLOneVarDecoderSamLite}}
\providecommand{\miouCIRNburnBoundaryLOneVarDecoderSamPretrained}{\tbd{miouCIRNburnBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\miouCIRNburnBoundaryLOneVarDecoderSegformerMlp}{\tbd{miouCIRNburnBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\miouCIRNburnBoundaryLR}{\tbd{miouCIRNburnBoundaryLR}}
\providecommand{\miouCIRNburnBoundaryLTwo}{\tbd{miouCIRNburnBoundaryLTwo}}
\providecommand{\miouCIRNburnBoundaryLTwoVarBandsRgb}{\tbd{miouCIRNburnBoundaryLTwoVarBandsRgb}}
\providecommand{\miouCIRNburnBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCIRNburnBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCIRNburnBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCIRNburnBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCIRNburnBoundaryLTwoVarDecoderSamLite}{\tbd{miouCIRNburnBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouCIRNburnBoundaryLTwoVarDecoderSamPretrained}{\tbd{miouCIRNburnBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\miouCIRNburnBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouCIRNburnBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCIRNburnBoundaryLTwoVarInitRandom}{\tbd{miouCIRNburnBoundaryLTwoVarInitRandom}}
\providecommand{\miouCIRNburnBoundaryLTwoVarLossBootstrap}{\tbd{miouCIRNburnBoundaryLTwoVarLossBootstrap}}
\providecommand{\miouCIRNburnBoundaryLTwoVarLossGce}{\tbd{miouCIRNburnBoundaryLTwoVarLossGce}}
\providecommand{\miouCIRNburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCIRNburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCIRNburnBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCIRNburnBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCIRNburnClean}{\tbd{miouCIRNburnClean}}
\providecommand{\miouCIRNburnCleanVarBandsRgb}{\tbd{miouCIRNburnCleanVarBandsRgb}}
\providecommand{\miouCIRNburnCleanVarDecoderMaskTwoformerFull}{\tbd{miouCIRNburnCleanVarDecoderMaskTwoformerFull}}
\providecommand{\miouCIRNburnCleanVarDecoderMaskTwoformerLite}{\tbd{miouCIRNburnCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouCIRNburnCleanVarDecoderSamLite}{\tbd{miouCIRNburnCleanVarDecoderSamLite}}
\providecommand{\miouCIRNburnCleanVarDecoderSamPretrained}{\tbd{miouCIRNburnCleanVarDecoderSamPretrained}}
\providecommand{\miouCIRNburnCleanVarDecoderSegformerMlp}{\tbd{miouCIRNburnCleanVarDecoderSegformerMlp}}
\providecommand{\miouCIRNburnCleanVarInitRandom}{\tbd{miouCIRNburnCleanVarInitRandom}}
\providecommand{\miouCIRNburnCleanVarInitRandomLrMultThree}{\tbd{miouCIRNburnCleanVarInitRandomLrMultThree}}
\providecommand{\miouCIRNburnCleanVarLossBootstrap}{\tbd{miouCIRNburnCleanVarLossBootstrap}}
\providecommand{\miouCIRNburnCleanVarLossGce}{\tbd{miouCIRNburnCleanVarLossGce}}
\providecommand{\miouCIRNburnCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCIRNburnCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCIRNburnCleanVarTrainSubsetCleanTwoFive}{\tbd{miouCIRNburnCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCIRNburnCoarseLOne}{\tbd{miouCIRNburnCoarseLOne}}
\providecommand{\miouCIRNburnCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{miouCIRNburnCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCIRNburnCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{miouCIRNburnCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCIRNburnCoarseLOneVarDecoderSamLite}{\tbd{miouCIRNburnCoarseLOneVarDecoderSamLite}}
\providecommand{\miouCIRNburnCoarseLOneVarDecoderSamPretrained}{\tbd{miouCIRNburnCoarseLOneVarDecoderSamPretrained}}
\providecommand{\miouCIRNburnCoarseLOneVarDecoderSegformerMlp}{\tbd{miouCIRNburnCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\miouCIRNburnCoarseLR}{\tbd{miouCIRNburnCoarseLR}}
\providecommand{\miouCIRNburnCoarseLTwo}{\tbd{miouCIRNburnCoarseLTwo}}
\providecommand{\miouCIRNburnCoarseLTwoVarBandsRgb}{\tbd{miouCIRNburnCoarseLTwoVarBandsRgb}}
\providecommand{\miouCIRNburnCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCIRNburnCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCIRNburnCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCIRNburnCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCIRNburnCoarseLTwoVarDecoderSamLite}{\tbd{miouCIRNburnCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouCIRNburnCoarseLTwoVarDecoderSamPretrained}{\tbd{miouCIRNburnCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\miouCIRNburnCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouCIRNburnCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCIRNburnCoarseLTwoVarInitRandom}{\tbd{miouCIRNburnCoarseLTwoVarInitRandom}}
\providecommand{\miouCIRNburnCoarseLTwoVarLossBootstrap}{\tbd{miouCIRNburnCoarseLTwoVarLossBootstrap}}
\providecommand{\miouCIRNburnCoarseLTwoVarLossGce}{\tbd{miouCIRNburnCoarseLTwoVarLossGce}}
\providecommand{\miouCIRNburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCIRNburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCIRNburnCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCIRNburnCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCIRNburnOmissionLOne}{\tbd{miouCIRNburnOmissionLOne}}
\providecommand{\miouCIRNburnOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{miouCIRNburnOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCIRNburnOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{miouCIRNburnOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCIRNburnOmissionLOneVarDecoderSamLite}{\tbd{miouCIRNburnOmissionLOneVarDecoderSamLite}}
\providecommand{\miouCIRNburnOmissionLOneVarDecoderSamPretrained}{\tbd{miouCIRNburnOmissionLOneVarDecoderSamPretrained}}
\providecommand{\miouCIRNburnOmissionLOneVarDecoderSegformerMlp}{\tbd{miouCIRNburnOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\miouCIRNburnOmissionLR}{\tbd{miouCIRNburnOmissionLR}}
\providecommand{\miouCIRNburnOmissionLTwo}{\tbd{miouCIRNburnOmissionLTwo}}
\providecommand{\miouCIRNburnOmissionLTwoVarBandsRgb}{\tbd{miouCIRNburnOmissionLTwoVarBandsRgb}}
\providecommand{\miouCIRNburnOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCIRNburnOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCIRNburnOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCIRNburnOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCIRNburnOmissionLTwoVarDecoderSamLite}{\tbd{miouCIRNburnOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouCIRNburnOmissionLTwoVarDecoderSamPretrained}{\tbd{miouCIRNburnOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\miouCIRNburnOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouCIRNburnOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCIRNburnOmissionLTwoVarInitRandom}{\tbd{miouCIRNburnOmissionLTwoVarInitRandom}}
\providecommand{\miouCIRNburnOmissionLTwoVarLossBootstrap}{\tbd{miouCIRNburnOmissionLTwoVarLossBootstrap}}
\providecommand{\miouCIRNburnOmissionLTwoVarLossGce}{\tbd{miouCIRNburnOmissionLTwoVarLossGce}}
\providecommand{\miouCIRNburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCIRNburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCIRNburnOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCIRNburnOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCIRNburnShiftLOne}{\tbd{miouCIRNburnShiftLOne}}
\providecommand{\miouCIRNburnShiftLOneVarDecoderMaskTwoformerFull}{\tbd{miouCIRNburnShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCIRNburnShiftLOneVarDecoderMaskTwoformerLite}{\tbd{miouCIRNburnShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCIRNburnShiftLOneVarDecoderSamLite}{\tbd{miouCIRNburnShiftLOneVarDecoderSamLite}}
\providecommand{\miouCIRNburnShiftLOneVarDecoderSamPretrained}{\tbd{miouCIRNburnShiftLOneVarDecoderSamPretrained}}
\providecommand{\miouCIRNburnShiftLOneVarDecoderSegformerMlp}{\tbd{miouCIRNburnShiftLOneVarDecoderSegformerMlp}}
\providecommand{\miouCIRNburnShiftLR}{\tbd{miouCIRNburnShiftLR}}
\providecommand{\miouCIRNburnShiftLTwo}{\tbd{miouCIRNburnShiftLTwo}}
\providecommand{\miouCIRNburnShiftLTwoVarBandsRgb}{\tbd{miouCIRNburnShiftLTwoVarBandsRgb}}
\providecommand{\miouCIRNburnShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCIRNburnShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCIRNburnShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCIRNburnShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCIRNburnShiftLTwoVarDecoderSamLite}{\tbd{miouCIRNburnShiftLTwoVarDecoderSamLite}}
\providecommand{\miouCIRNburnShiftLTwoVarDecoderSamPretrained}{\tbd{miouCIRNburnShiftLTwoVarDecoderSamPretrained}}
\providecommand{\miouCIRNburnShiftLTwoVarDecoderSegformerMlp}{\tbd{miouCIRNburnShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCIRNburnShiftLTwoVarInitRandom}{\tbd{miouCIRNburnShiftLTwoVarInitRandom}}
\providecommand{\miouCIRNburnShiftLTwoVarLossBootstrap}{\tbd{miouCIRNburnShiftLTwoVarLossBootstrap}}
\providecommand{\miouCIRNburnShiftLTwoVarLossGce}{\tbd{miouCIRNburnShiftLTwoVarLossGce}}
\providecommand{\miouCIRNburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCIRNburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCIRNburnShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCIRNburnShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCIRNflairBoundaryLOne}{\tbd{miouCIRNflairBoundaryLOne}}
\providecommand{\miouCIRNflairBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{miouCIRNflairBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCIRNflairBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{miouCIRNflairBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCIRNflairBoundaryLOneVarDecoderSamLite}{\tbd{miouCIRNflairBoundaryLOneVarDecoderSamLite}}
\providecommand{\miouCIRNflairBoundaryLOneVarDecoderSamPretrained}{\tbd{miouCIRNflairBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\miouCIRNflairBoundaryLOneVarDecoderSegformerMlp}{\tbd{miouCIRNflairBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\miouCIRNflairBoundaryLR}{\tbd{miouCIRNflairBoundaryLR}}
\providecommand{\miouCIRNflairBoundaryLTwo}{\tbd{miouCIRNflairBoundaryLTwo}}
\providecommand{\miouCIRNflairBoundaryLTwoVarBandsRgb}{\tbd{miouCIRNflairBoundaryLTwoVarBandsRgb}}
\providecommand{\miouCIRNflairBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCIRNflairBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCIRNflairBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCIRNflairBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCIRNflairBoundaryLTwoVarDecoderSamLite}{\tbd{miouCIRNflairBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouCIRNflairBoundaryLTwoVarDecoderSamPretrained}{\tbd{miouCIRNflairBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\miouCIRNflairBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouCIRNflairBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCIRNflairBoundaryLTwoVarInitRandom}{\tbd{miouCIRNflairBoundaryLTwoVarInitRandom}}
\providecommand{\miouCIRNflairBoundaryLTwoVarLossBootstrap}{\tbd{miouCIRNflairBoundaryLTwoVarLossBootstrap}}
\providecommand{\miouCIRNflairBoundaryLTwoVarLossGce}{\tbd{miouCIRNflairBoundaryLTwoVarLossGce}}
\providecommand{\miouCIRNflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCIRNflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCIRNflairBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCIRNflairBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCIRNflairClean}{\tbd{miouCIRNflairClean}}
\providecommand{\miouCIRNflairCleanVarBandsRgb}{\tbd{miouCIRNflairCleanVarBandsRgb}}
\providecommand{\miouCIRNflairCleanVarClassWeightedTrue}{\tbd{miouCIRNflairCleanVarClassWeightedTrue}}
\providecommand{\miouCIRNflairCleanVarDecoderMaskTwoformerFull}{\tbd{miouCIRNflairCleanVarDecoderMaskTwoformerFull}}
\providecommand{\miouCIRNflairCleanVarDecoderMaskTwoformerLite}{\tbd{miouCIRNflairCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouCIRNflairCleanVarDecoderSamLite}{\tbd{miouCIRNflairCleanVarDecoderSamLite}}
\providecommand{\miouCIRNflairCleanVarDecoderSamPretrained}{\tbd{miouCIRNflairCleanVarDecoderSamPretrained}}
\providecommand{\miouCIRNflairCleanVarDecoderSegformerMlp}{\tbd{miouCIRNflairCleanVarDecoderSegformerMlp}}
\providecommand{\miouCIRNflairCleanVarInitRandom}{\tbd{miouCIRNflairCleanVarInitRandom}}
\providecommand{\miouCIRNflairCleanVarInitRandomLrMultThree}{\tbd{miouCIRNflairCleanVarInitRandomLrMultThree}}
\providecommand{\miouCIRNflairCleanVarLossBootstrap}{\tbd{miouCIRNflairCleanVarLossBootstrap}}
\providecommand{\miouCIRNflairCleanVarLossGce}{\tbd{miouCIRNflairCleanVarLossGce}}
\providecommand{\miouCIRNflairCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCIRNflairCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCIRNflairCleanVarTrainSubsetCleanTwoFive}{\tbd{miouCIRNflairCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCIRNflairCoarseLOne}{\tbd{miouCIRNflairCoarseLOne}}
\providecommand{\miouCIRNflairCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{miouCIRNflairCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCIRNflairCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{miouCIRNflairCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCIRNflairCoarseLOneVarDecoderSamLite}{\tbd{miouCIRNflairCoarseLOneVarDecoderSamLite}}
\providecommand{\miouCIRNflairCoarseLOneVarDecoderSamPretrained}{\tbd{miouCIRNflairCoarseLOneVarDecoderSamPretrained}}
\providecommand{\miouCIRNflairCoarseLOneVarDecoderSegformerMlp}{\tbd{miouCIRNflairCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\miouCIRNflairCoarseLR}{\tbd{miouCIRNflairCoarseLR}}
\providecommand{\miouCIRNflairCoarseLTwo}{\tbd{miouCIRNflairCoarseLTwo}}
\providecommand{\miouCIRNflairCoarseLTwoVarBandsRgb}{\tbd{miouCIRNflairCoarseLTwoVarBandsRgb}}
\providecommand{\miouCIRNflairCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCIRNflairCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCIRNflairCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCIRNflairCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCIRNflairCoarseLTwoVarDecoderSamLite}{\tbd{miouCIRNflairCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouCIRNflairCoarseLTwoVarDecoderSamPretrained}{\tbd{miouCIRNflairCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\miouCIRNflairCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouCIRNflairCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCIRNflairCoarseLTwoVarInitRandom}{\tbd{miouCIRNflairCoarseLTwoVarInitRandom}}
\providecommand{\miouCIRNflairCoarseLTwoVarLossBootstrap}{\tbd{miouCIRNflairCoarseLTwoVarLossBootstrap}}
\providecommand{\miouCIRNflairCoarseLTwoVarLossGce}{\tbd{miouCIRNflairCoarseLTwoVarLossGce}}
\providecommand{\miouCIRNflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCIRNflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCIRNflairCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCIRNflairCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCIRNflairOmissionLOne}{\tbd{miouCIRNflairOmissionLOne}}
\providecommand{\miouCIRNflairOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{miouCIRNflairOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCIRNflairOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{miouCIRNflairOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCIRNflairOmissionLOneVarDecoderSamLite}{\tbd{miouCIRNflairOmissionLOneVarDecoderSamLite}}
\providecommand{\miouCIRNflairOmissionLOneVarDecoderSamPretrained}{\tbd{miouCIRNflairOmissionLOneVarDecoderSamPretrained}}
\providecommand{\miouCIRNflairOmissionLOneVarDecoderSegformerMlp}{\tbd{miouCIRNflairOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\miouCIRNflairOmissionLR}{\tbd{miouCIRNflairOmissionLR}}
\providecommand{\miouCIRNflairOmissionLTwo}{\tbd{miouCIRNflairOmissionLTwo}}
\providecommand{\miouCIRNflairOmissionLTwoVarBandsRgb}{\tbd{miouCIRNflairOmissionLTwoVarBandsRgb}}
\providecommand{\miouCIRNflairOmissionLTwoVarClassWeightedTrue}{\tbd{miouCIRNflairOmissionLTwoVarClassWeightedTrue}}
\providecommand{\miouCIRNflairOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCIRNflairOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCIRNflairOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCIRNflairOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCIRNflairOmissionLTwoVarDecoderSamLite}{\tbd{miouCIRNflairOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouCIRNflairOmissionLTwoVarDecoderSamPretrained}{\tbd{miouCIRNflairOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\miouCIRNflairOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouCIRNflairOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCIRNflairOmissionLTwoVarInitRandom}{\tbd{miouCIRNflairOmissionLTwoVarInitRandom}}
\providecommand{\miouCIRNflairOmissionLTwoVarLossBootstrap}{\tbd{miouCIRNflairOmissionLTwoVarLossBootstrap}}
\providecommand{\miouCIRNflairOmissionLTwoVarLossGce}{\tbd{miouCIRNflairOmissionLTwoVarLossGce}}
\providecommand{\miouCIRNflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCIRNflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCIRNflairOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCIRNflairOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCIRNflairShiftLOne}{\tbd{miouCIRNflairShiftLOne}}
\providecommand{\miouCIRNflairShiftLOneVarDecoderMaskTwoformerFull}{\tbd{miouCIRNflairShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCIRNflairShiftLOneVarDecoderMaskTwoformerLite}{\tbd{miouCIRNflairShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCIRNflairShiftLOneVarDecoderSamLite}{\tbd{miouCIRNflairShiftLOneVarDecoderSamLite}}
\providecommand{\miouCIRNflairShiftLOneVarDecoderSamPretrained}{\tbd{miouCIRNflairShiftLOneVarDecoderSamPretrained}}
\providecommand{\miouCIRNflairShiftLOneVarDecoderSegformerMlp}{\tbd{miouCIRNflairShiftLOneVarDecoderSegformerMlp}}
\providecommand{\miouCIRNflairShiftLR}{\tbd{miouCIRNflairShiftLR}}
\providecommand{\miouCIRNflairShiftLTwo}{\tbd{miouCIRNflairShiftLTwo}}
\providecommand{\miouCIRNflairShiftLTwoVarBandsRgb}{\tbd{miouCIRNflairShiftLTwoVarBandsRgb}}
\providecommand{\miouCIRNflairShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCIRNflairShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCIRNflairShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCIRNflairShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCIRNflairShiftLTwoVarDecoderSamLite}{\tbd{miouCIRNflairShiftLTwoVarDecoderSamLite}}
\providecommand{\miouCIRNflairShiftLTwoVarDecoderSamPretrained}{\tbd{miouCIRNflairShiftLTwoVarDecoderSamPretrained}}
\providecommand{\miouCIRNflairShiftLTwoVarDecoderSegformerMlp}{\tbd{miouCIRNflairShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCIRNflairShiftLTwoVarInitRandom}{\tbd{miouCIRNflairShiftLTwoVarInitRandom}}
\providecommand{\miouCIRNflairShiftLTwoVarLossBootstrap}{\tbd{miouCIRNflairShiftLTwoVarLossBootstrap}}
\providecommand{\miouCIRNflairShiftLTwoVarLossGce}{\tbd{miouCIRNflairShiftLTwoVarLossGce}}
\providecommand{\miouCIRNflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCIRNflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCIRNflairShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCIRNflairShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCIRNsenClean}{\tbd{miouCIRNsenClean}}
\providecommand{\miouCIRNsenOtsuLTwo}{\tbd{miouCIRNsenOtsuLTwo}}
\providecommand{\miouCIResnetFiveZeroSslFoureoburnBoundaryLOne}{\tbd{miouCIResnetFiveZeroSslFoureoburnBoundaryLOne}}
\providecommand{\miouCIResnetFiveZeroSslFoureoburnBoundaryLTwo}{\tbd{miouCIResnetFiveZeroSslFoureoburnBoundaryLTwo}}
\providecommand{\miouCIResnetFiveZeroSslFoureoburnClean}{\tbd{miouCIResnetFiveZeroSslFoureoburnClean}}
\providecommand{\miouCIResnetFiveZeroSslFoureoburnCleanVarTrainSubsetCleanTwoFive}{\tbd{miouCIResnetFiveZeroSslFoureoburnCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCIResnetFiveZeroSslFoureoburnCoarseLOne}{\tbd{miouCIResnetFiveZeroSslFoureoburnCoarseLOne}}
\providecommand{\miouCIResnetFiveZeroSslFoureoburnCoarseLTwo}{\tbd{miouCIResnetFiveZeroSslFoureoburnCoarseLTwo}}
\providecommand{\miouCIResnetFiveZeroSslFoureoburnOmissionLOne}{\tbd{miouCIResnetFiveZeroSslFoureoburnOmissionLOne}}
\providecommand{\miouCIResnetFiveZeroSslFoureoburnOmissionLTwo}{\tbd{miouCIResnetFiveZeroSslFoureoburnOmissionLTwo}}
\providecommand{\miouCIResnetFiveZeroSslFoureoburnShiftLOne}{\tbd{miouCIResnetFiveZeroSslFoureoburnShiftLOne}}
\providecommand{\miouCIResnetFiveZeroSslFoureoburnShiftLTwo}{\tbd{miouCIResnetFiveZeroSslFoureoburnShiftLTwo}}
\providecommand{\miouCIResnetFiveZeroSslFoureoflairBoundaryLOne}{\tbd{miouCIResnetFiveZeroSslFoureoflairBoundaryLOne}}
\providecommand{\miouCIResnetFiveZeroSslFoureoflairBoundaryLTwo}{\tbd{miouCIResnetFiveZeroSslFoureoflairBoundaryLTwo}}
\providecommand{\miouCIResnetFiveZeroSslFoureoflairClean}{\tbd{miouCIResnetFiveZeroSslFoureoflairClean}}
\providecommand{\miouCIResnetFiveZeroSslFoureoflairCleanVarTrainSubsetCleanTwoFive}{\tbd{miouCIResnetFiveZeroSslFoureoflairCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCIResnetFiveZeroSslFoureoflairCoarseLOne}{\tbd{miouCIResnetFiveZeroSslFoureoflairCoarseLOne}}
\providecommand{\miouCIResnetFiveZeroSslFoureoflairCoarseLTwo}{\tbd{miouCIResnetFiveZeroSslFoureoflairCoarseLTwo}}
\providecommand{\miouCIResnetFiveZeroSslFoureoflairOmissionLOne}{\tbd{miouCIResnetFiveZeroSslFoureoflairOmissionLOne}}
\providecommand{\miouCIResnetFiveZeroSslFoureoflairOmissionLTwo}{\tbd{miouCIResnetFiveZeroSslFoureoflairOmissionLTwo}}
\providecommand{\miouCIResnetFiveZeroSslFoureoflairShiftLOne}{\tbd{miouCIResnetFiveZeroSslFoureoflairShiftLOne}}
\providecommand{\miouCIResnetFiveZeroSslFoureoflairShiftLTwo}{\tbd{miouCIResnetFiveZeroSslFoureoflairShiftLTwo}}
\providecommand{\miouCISATChesBoundaryLOne}{\tbd{miouCISATChesBoundaryLOne}}
\providecommand{\miouCISATChesBoundaryLTwo}{\tbd{miouCISATChesBoundaryLTwo}}
\providecommand{\miouCISATChesBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCISATChesBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATChesBoundaryLTwoVarDecoderSamLite}{\tbd{miouCISATChesBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouCISATChesBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouCISATChesBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCISATChesBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATChesBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATChesClean}{\tbd{miouCISATChesClean}}
\providecommand{\miouCISATChesCleanVarDecoderMaskTwoformerLite}{\tbd{miouCISATChesCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATChesCleanVarDecoderSamLite}{\tbd{miouCISATChesCleanVarDecoderSamLite}}
\providecommand{\miouCISATChesCleanVarDecoderSegformerMlp}{\tbd{miouCISATChesCleanVarDecoderSegformerMlp}}
\providecommand{\miouCISATChesCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATChesCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATChesCoarseLOne}{\tbd{miouCISATChesCoarseLOne}}
\providecommand{\miouCISATChesCoarseLTwo}{\tbd{miouCISATChesCoarseLTwo}}
\providecommand{\miouCISATChesCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCISATChesCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATChesCoarseLTwoVarDecoderSamLite}{\tbd{miouCISATChesCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouCISATChesCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouCISATChesCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCISATChesCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATChesCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATChesNlcdREAL}{\tbd{miouCISATChesNlcdREAL}}
\providecommand{\miouCISATChesOmissionLOne}{\tbd{miouCISATChesOmissionLOne}}
\providecommand{\miouCISATChesOmissionLTwo}{\tbd{miouCISATChesOmissionLTwo}}
\providecommand{\miouCISATChesOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCISATChesOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATChesOmissionLTwoVarDecoderSamLite}{\tbd{miouCISATChesOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouCISATChesOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouCISATChesOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCISATChesOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATChesOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATChesShiftLOne}{\tbd{miouCISATChesShiftLOne}}
\providecommand{\miouCISATChesShiftLTwo}{\tbd{miouCISATChesShiftLTwo}}
\providecommand{\miouCISATChesShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCISATChesShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATChesShiftLTwoVarDecoderSamLite}{\tbd{miouCISATChesShiftLTwoVarDecoderSamLite}}
\providecommand{\miouCISATChesShiftLTwoVarDecoderSegformerMlp}{\tbd{miouCISATChesShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCISATChesShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATChesShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATCsTwelveBoundaryLOne}{\tbd{miouCISATCsTwelveBoundaryLOne}}
\providecommand{\miouCISATCsTwelveBoundaryLTwo}{\tbd{miouCISATCsTwelveBoundaryLTwo}}
\providecommand{\miouCISATCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCISATCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATCsTwelveBoundaryLTwoVarDecoderSamLite}{\tbd{miouCISATCsTwelveBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouCISATCsTwelveBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouCISATCsTwelveBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCISATCsTwelveBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATCsTwelveBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATCsTwelveClean}{\tbd{miouCISATCsTwelveClean}}
\providecommand{\miouCISATCsTwelveCleanVarDecoderMaskTwoformerLite}{\tbd{miouCISATCsTwelveCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATCsTwelveCleanVarDecoderSamLite}{\tbd{miouCISATCsTwelveCleanVarDecoderSamLite}}
\providecommand{\miouCISATCsTwelveCleanVarDecoderSegformerMlp}{\tbd{miouCISATCsTwelveCleanVarDecoderSegformerMlp}}
\providecommand{\miouCISATCsTwelveCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATCsTwelveCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATCsTwelveCoarseLOne}{\tbd{miouCISATCsTwelveCoarseLOne}}
\providecommand{\miouCISATCsTwelveCoarseLTwo}{\tbd{miouCISATCsTwelveCoarseLTwo}}
\providecommand{\miouCISATCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCISATCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATCsTwelveCoarseLTwoVarDecoderSamLite}{\tbd{miouCISATCsTwelveCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouCISATCsTwelveCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouCISATCsTwelveCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCISATCsTwelveCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATCsTwelveCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATCsTwelveOmissionLOne}{\tbd{miouCISATCsTwelveOmissionLOne}}
\providecommand{\miouCISATCsTwelveOmissionLTwo}{\tbd{miouCISATCsTwelveOmissionLTwo}}
\providecommand{\miouCISATCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCISATCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATCsTwelveOmissionLTwoVarDecoderSamLite}{\tbd{miouCISATCsTwelveOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouCISATCsTwelveOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouCISATCsTwelveOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCISATCsTwelveOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATCsTwelveOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATCsTwelveSTwocloudlessREAL}{\tbd{miouCISATCsTwelveSTwocloudlessREAL}}
\providecommand{\miouCISATCsTwelveShiftLOne}{\tbd{miouCISATCsTwelveShiftLOne}}
\providecommand{\miouCISATCsTwelveShiftLTwo}{\tbd{miouCISATCsTwelveShiftLTwo}}
\providecommand{\miouCISATCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCISATCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATCsTwelveShiftLTwoVarDecoderSamLite}{\tbd{miouCISATCsTwelveShiftLTwoVarDecoderSamLite}}
\providecommand{\miouCISATCsTwelveShiftLTwoVarDecoderSegformerMlp}{\tbd{miouCISATCsTwelveShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCISATCsTwelveShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATCsTwelveShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATDfcBoundaryLOne}{\tbd{miouCISATDfcBoundaryLOne}}
\providecommand{\miouCISATDfcBoundaryLTwo}{\tbd{miouCISATDfcBoundaryLTwo}}
\providecommand{\miouCISATDfcBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCISATDfcBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATDfcBoundaryLTwoVarDecoderSamLite}{\tbd{miouCISATDfcBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouCISATDfcBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouCISATDfcBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCISATDfcBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATDfcBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATDfcClean}{\tbd{miouCISATDfcClean}}
\providecommand{\miouCISATDfcCleanVarDecoderMaskTwoformerLite}{\tbd{miouCISATDfcCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATDfcCleanVarDecoderSamLite}{\tbd{miouCISATDfcCleanVarDecoderSamLite}}
\providecommand{\miouCISATDfcCleanVarDecoderSegformerMlp}{\tbd{miouCISATDfcCleanVarDecoderSegformerMlp}}
\providecommand{\miouCISATDfcCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATDfcCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATDfcCleanVarTrainSubsetRealcov}{\tbd{miouCISATDfcCleanVarTrainSubsetRealcov}}
\providecommand{\miouCISATDfcCoarseLOne}{\tbd{miouCISATDfcCoarseLOne}}
\providecommand{\miouCISATDfcCoarseLTwo}{\tbd{miouCISATDfcCoarseLTwo}}
\providecommand{\miouCISATDfcCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCISATDfcCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATDfcCoarseLTwoVarDecoderSamLite}{\tbd{miouCISATDfcCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouCISATDfcCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouCISATDfcCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCISATDfcCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATDfcCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATDfcModisREALVarTrainSubsetRealcov}{\tbd{miouCISATDfcModisREALVarTrainSubsetRealcov}}
\providecommand{\miouCISATDfcOmissionLOne}{\tbd{miouCISATDfcOmissionLOne}}
\providecommand{\miouCISATDfcOmissionLTwo}{\tbd{miouCISATDfcOmissionLTwo}}
\providecommand{\miouCISATDfcOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCISATDfcOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATDfcOmissionLTwoVarDecoderSamLite}{\tbd{miouCISATDfcOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouCISATDfcOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouCISATDfcOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCISATDfcOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATDfcOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATDfcShiftLOne}{\tbd{miouCISATDfcShiftLOne}}
\providecommand{\miouCISATDfcShiftLTwo}{\tbd{miouCISATDfcShiftLTwo}}
\providecommand{\miouCISATDfcShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCISATDfcShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATDfcShiftLTwoVarDecoderSamLite}{\tbd{miouCISATDfcShiftLTwoVarDecoderSamLite}}
\providecommand{\miouCISATDfcShiftLTwoVarDecoderSegformerMlp}{\tbd{miouCISATDfcShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCISATDfcShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATDfcShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATEnvaBoundaryLOne}{\tbd{miouCISATEnvaBoundaryLOne}}
\providecommand{\miouCISATEnvaBoundaryLTwo}{\tbd{miouCISATEnvaBoundaryLTwo}}
\providecommand{\miouCISATEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCISATEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATEnvaBoundaryLTwoVarDecoderSamLite}{\tbd{miouCISATEnvaBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouCISATEnvaBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouCISATEnvaBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCISATEnvaBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATEnvaBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATEnvaClean}{\tbd{miouCISATEnvaClean}}
\providecommand{\miouCISATEnvaCleanVarDecoderMaskTwoformerLite}{\tbd{miouCISATEnvaCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATEnvaCleanVarDecoderSamLite}{\tbd{miouCISATEnvaCleanVarDecoderSamLite}}
\providecommand{\miouCISATEnvaCleanVarDecoderSegformerMlp}{\tbd{miouCISATEnvaCleanVarDecoderSegformerMlp}}
\providecommand{\miouCISATEnvaCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATEnvaCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATEnvaCoarseLOne}{\tbd{miouCISATEnvaCoarseLOne}}
\providecommand{\miouCISATEnvaCoarseLTwo}{\tbd{miouCISATEnvaCoarseLTwo}}
\providecommand{\miouCISATEnvaCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCISATEnvaCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATEnvaCoarseLTwoVarDecoderSamLite}{\tbd{miouCISATEnvaCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouCISATEnvaCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouCISATEnvaCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCISATEnvaCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATEnvaCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATEnvaNlcdREAL}{\tbd{miouCISATEnvaNlcdREAL}}
\providecommand{\miouCISATEnvaOmissionLOne}{\tbd{miouCISATEnvaOmissionLOne}}
\providecommand{\miouCISATEnvaOmissionLTwo}{\tbd{miouCISATEnvaOmissionLTwo}}
\providecommand{\miouCISATEnvaOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCISATEnvaOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATEnvaOmissionLTwoVarDecoderSamLite}{\tbd{miouCISATEnvaOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouCISATEnvaOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouCISATEnvaOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCISATEnvaOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATEnvaOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATEnvaShiftLOne}{\tbd{miouCISATEnvaShiftLOne}}
\providecommand{\miouCISATEnvaShiftLTwo}{\tbd{miouCISATEnvaShiftLTwo}}
\providecommand{\miouCISATEnvaShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCISATEnvaShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATEnvaShiftLTwoVarDecoderSamLite}{\tbd{miouCISATEnvaShiftLTwoVarDecoderSamLite}}
\providecommand{\miouCISATEnvaShiftLTwoVarDecoderSegformerMlp}{\tbd{miouCISATEnvaShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCISATEnvaShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATEnvaShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATKuroBoundaryLOne}{\tbd{miouCISATKuroBoundaryLOne}}
\providecommand{\miouCISATKuroBoundaryLTwo}{\tbd{miouCISATKuroBoundaryLTwo}}
\providecommand{\miouCISATKuroBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCISATKuroBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATKuroBoundaryLTwoVarDecoderSamLite}{\tbd{miouCISATKuroBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouCISATKuroBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouCISATKuroBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCISATKuroBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATKuroBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATKuroCemsREALVarTrainSubsetRealcov}{\tbd{miouCISATKuroCemsREALVarTrainSubsetRealcov}}
\providecommand{\miouCISATKuroClean}{\tbd{miouCISATKuroClean}}
\providecommand{\miouCISATKuroCleanVarDecoderMaskTwoformerLite}{\tbd{miouCISATKuroCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATKuroCleanVarDecoderSamLite}{\tbd{miouCISATKuroCleanVarDecoderSamLite}}
\providecommand{\miouCISATKuroCleanVarDecoderSegformerMlp}{\tbd{miouCISATKuroCleanVarDecoderSegformerMlp}}
\providecommand{\miouCISATKuroCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATKuroCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATKuroCleanVarTrainSubsetRealcov}{\tbd{miouCISATKuroCleanVarTrainSubsetRealcov}}
\providecommand{\miouCISATKuroCoarseLOne}{\tbd{miouCISATKuroCoarseLOne}}
\providecommand{\miouCISATKuroCoarseLTwo}{\tbd{miouCISATKuroCoarseLTwo}}
\providecommand{\miouCISATKuroCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCISATKuroCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATKuroCoarseLTwoVarDecoderSamLite}{\tbd{miouCISATKuroCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouCISATKuroCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouCISATKuroCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCISATKuroCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATKuroCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATKuroOmissionLOne}{\tbd{miouCISATKuroOmissionLOne}}
\providecommand{\miouCISATKuroOmissionLTwo}{\tbd{miouCISATKuroOmissionLTwo}}
\providecommand{\miouCISATKuroOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCISATKuroOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATKuroOmissionLTwoVarDecoderSamLite}{\tbd{miouCISATKuroOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouCISATKuroOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouCISATKuroOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCISATKuroOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATKuroOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATKuroShiftLOne}{\tbd{miouCISATKuroShiftLOne}}
\providecommand{\miouCISATKuroShiftLTwo}{\tbd{miouCISATKuroShiftLTwo}}
\providecommand{\miouCISATKuroShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCISATKuroShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATKuroShiftLTwoVarDecoderSamLite}{\tbd{miouCISATKuroShiftLTwoVarDecoderSamLite}}
\providecommand{\miouCISATKuroShiftLTwoVarDecoderSegformerMlp}{\tbd{miouCISATKuroShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCISATKuroShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATKuroShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATOemBoundaryLOne}{\tbd{miouCISATOemBoundaryLOne}}
\providecommand{\miouCISATOemBoundaryLTwo}{\tbd{miouCISATOemBoundaryLTwo}}
\providecommand{\miouCISATOemBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCISATOemBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATOemBoundaryLTwoVarDecoderSamLite}{\tbd{miouCISATOemBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouCISATOemBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouCISATOemBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCISATOemBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATOemBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATOemClean}{\tbd{miouCISATOemClean}}
\providecommand{\miouCISATOemCleanVarDecoderMaskTwoformerLite}{\tbd{miouCISATOemCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATOemCleanVarDecoderSamLite}{\tbd{miouCISATOemCleanVarDecoderSamLite}}
\providecommand{\miouCISATOemCleanVarDecoderSegformerMlp}{\tbd{miouCISATOemCleanVarDecoderSegformerMlp}}
\providecommand{\miouCISATOemCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATOemCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATOemCoarseLOne}{\tbd{miouCISATOemCoarseLOne}}
\providecommand{\miouCISATOemCoarseLTwo}{\tbd{miouCISATOemCoarseLTwo}}
\providecommand{\miouCISATOemCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCISATOemCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATOemCoarseLTwoVarDecoderSamLite}{\tbd{miouCISATOemCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouCISATOemCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouCISATOemCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCISATOemCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATOemCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATOemOmissionLOne}{\tbd{miouCISATOemOmissionLOne}}
\providecommand{\miouCISATOemOmissionLTwo}{\tbd{miouCISATOemOmissionLTwo}}
\providecommand{\miouCISATOemOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCISATOemOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATOemOmissionLTwoVarDecoderSamLite}{\tbd{miouCISATOemOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouCISATOemOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouCISATOemOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCISATOemOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATOemOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATOemShiftLOne}{\tbd{miouCISATOemShiftLOne}}
\providecommand{\miouCISATOemShiftLTwo}{\tbd{miouCISATOemShiftLTwo}}
\providecommand{\miouCISATOemShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCISATOemShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATOemShiftLTwoVarDecoderSamLite}{\tbd{miouCISATOemShiftLTwoVarDecoderSamLite}}
\providecommand{\miouCISATOemShiftLTwoVarDecoderSegformerMlp}{\tbd{miouCISATOemShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCISATOemShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATOemShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATSnTwoBoundaryLOne}{\tbd{miouCISATSnTwoBoundaryLOne}}
\providecommand{\miouCISATSnTwoBoundaryLTwo}{\tbd{miouCISATSnTwoBoundaryLTwo}}
\providecommand{\miouCISATSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCISATSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATSnTwoBoundaryLTwoVarDecoderSamLite}{\tbd{miouCISATSnTwoBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouCISATSnTwoBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouCISATSnTwoBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCISATSnTwoBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATSnTwoBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATSnTwoClean}{\tbd{miouCISATSnTwoClean}}
\providecommand{\miouCISATSnTwoCleanVarDecoderMaskTwoformerLite}{\tbd{miouCISATSnTwoCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATSnTwoCleanVarDecoderSamLite}{\tbd{miouCISATSnTwoCleanVarDecoderSamLite}}
\providecommand{\miouCISATSnTwoCleanVarDecoderSegformerMlp}{\tbd{miouCISATSnTwoCleanVarDecoderSegformerMlp}}
\providecommand{\miouCISATSnTwoCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATSnTwoCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATSnTwoCoarseLOne}{\tbd{miouCISATSnTwoCoarseLOne}}
\providecommand{\miouCISATSnTwoCoarseLTwo}{\tbd{miouCISATSnTwoCoarseLTwo}}
\providecommand{\miouCISATSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCISATSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATSnTwoCoarseLTwoVarDecoderSamLite}{\tbd{miouCISATSnTwoCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouCISATSnTwoCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouCISATSnTwoCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCISATSnTwoCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATSnTwoCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATSnTwoOmissionLOne}{\tbd{miouCISATSnTwoOmissionLOne}}
\providecommand{\miouCISATSnTwoOmissionLTwo}{\tbd{miouCISATSnTwoOmissionLTwo}}
\providecommand{\miouCISATSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCISATSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATSnTwoOmissionLTwoVarDecoderSamLite}{\tbd{miouCISATSnTwoOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouCISATSnTwoOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouCISATSnTwoOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCISATSnTwoOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATSnTwoOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATSnTwoShiftLOne}{\tbd{miouCISATSnTwoShiftLOne}}
\providecommand{\miouCISATSnTwoShiftLTwo}{\tbd{miouCISATSnTwoShiftLTwo}}
\providecommand{\miouCISATSnTwoShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCISATSnTwoShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATSnTwoShiftLTwoVarDecoderSamLite}{\tbd{miouCISATSnTwoShiftLTwoVarDecoderSamLite}}
\providecommand{\miouCISATSnTwoShiftLTwoVarDecoderSegformerMlp}{\tbd{miouCISATSnTwoShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCISATSnTwoShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATSnTwoShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATburnBoundaryLOne}{\tbd{miouCISATburnBoundaryLOne}}
\providecommand{\miouCISATburnBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{miouCISATburnBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCISATburnBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{miouCISATburnBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATburnBoundaryLOneVarDecoderSamLite}{\tbd{miouCISATburnBoundaryLOneVarDecoderSamLite}}
\providecommand{\miouCISATburnBoundaryLOneVarDecoderSamPretrained}{\tbd{miouCISATburnBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\miouCISATburnBoundaryLOneVarDecoderSegformerMlp}{\tbd{miouCISATburnBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\miouCISATburnBoundaryLR}{\tbd{miouCISATburnBoundaryLR}}
\providecommand{\miouCISATburnBoundaryLRVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATburnBoundaryLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATburnBoundaryLTwo}{\tbd{miouCISATburnBoundaryLTwo}}
\providecommand{\miouCISATburnBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCISATburnBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCISATburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATburnBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCISATburnBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATburnBoundaryLTwoVarDecoderSamLite}{\tbd{miouCISATburnBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouCISATburnBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATburnBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATburnBoundaryLTwoVarDecoderSamPretrained}{\tbd{miouCISATburnBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\miouCISATburnBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATburnBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATburnBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouCISATburnBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCISATburnBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATburnBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATburnBoundaryLTwoVarFrozenEncoderTrue}{\tbd{miouCISATburnBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\miouCISATburnBoundaryLTwoVarLossBootstrap}{\tbd{miouCISATburnBoundaryLTwoVarLossBootstrap}}
\providecommand{\miouCISATburnBoundaryLTwoVarLossGce}{\tbd{miouCISATburnBoundaryLTwoVarLossGce}}
\providecommand{\miouCISATburnBoundaryLTwoVarLrMultThree}{\tbd{miouCISATburnBoundaryLTwoVarLrMultThree}}
\providecommand{\miouCISATburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATburnBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCISATburnBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCISATburnBoundaryLTwoVarValLabelsClean}{\tbd{miouCISATburnBoundaryLTwoVarValLabelsClean}}
\providecommand{\miouCISATburnClean}{\tbd{miouCISATburnClean}}
\providecommand{\miouCISATburnCleanVarDecoderMaskTwoformerFull}{\tbd{miouCISATburnCleanVarDecoderMaskTwoformerFull}}
\providecommand{\miouCISATburnCleanVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATburnCleanVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATburnCleanVarDecoderMaskTwoformerLite}{\tbd{miouCISATburnCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATburnCleanVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATburnCleanVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATburnCleanVarDecoderSamLite}{\tbd{miouCISATburnCleanVarDecoderSamLite}}
\providecommand{\miouCISATburnCleanVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATburnCleanVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATburnCleanVarDecoderSamPretrained}{\tbd{miouCISATburnCleanVarDecoderSamPretrained}}
\providecommand{\miouCISATburnCleanVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATburnCleanVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATburnCleanVarDecoderSegformerMlp}{\tbd{miouCISATburnCleanVarDecoderSegformerMlp}}
\providecommand{\miouCISATburnCleanVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATburnCleanVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATburnCleanVarFrozenEncoderTrue}{\tbd{miouCISATburnCleanVarFrozenEncoderTrue}}
\providecommand{\miouCISATburnCleanVarLossBootstrap}{\tbd{miouCISATburnCleanVarLossBootstrap}}
\providecommand{\miouCISATburnCleanVarLossGce}{\tbd{miouCISATburnCleanVarLossGce}}
\providecommand{\miouCISATburnCleanVarLrMultThree}{\tbd{miouCISATburnCleanVarLrMultThree}}
\providecommand{\miouCISATburnCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATburnCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATburnCleanVarTrainSubsetCleanTwoFive}{\tbd{miouCISATburnCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCISATburnCleanVarValLabelsClean}{\tbd{miouCISATburnCleanVarValLabelsClean}}
\providecommand{\miouCISATburnCoarseLOne}{\tbd{miouCISATburnCoarseLOne}}
\providecommand{\miouCISATburnCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{miouCISATburnCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCISATburnCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{miouCISATburnCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATburnCoarseLOneVarDecoderSamLite}{\tbd{miouCISATburnCoarseLOneVarDecoderSamLite}}
\providecommand{\miouCISATburnCoarseLOneVarDecoderSamPretrained}{\tbd{miouCISATburnCoarseLOneVarDecoderSamPretrained}}
\providecommand{\miouCISATburnCoarseLOneVarDecoderSegformerMlp}{\tbd{miouCISATburnCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\miouCISATburnCoarseLR}{\tbd{miouCISATburnCoarseLR}}
\providecommand{\miouCISATburnCoarseLRVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATburnCoarseLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATburnCoarseLTwo}{\tbd{miouCISATburnCoarseLTwo}}
\providecommand{\miouCISATburnCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCISATburnCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCISATburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATburnCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCISATburnCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATburnCoarseLTwoVarDecoderSamLite}{\tbd{miouCISATburnCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouCISATburnCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATburnCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATburnCoarseLTwoVarDecoderSamPretrained}{\tbd{miouCISATburnCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\miouCISATburnCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATburnCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATburnCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouCISATburnCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCISATburnCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATburnCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATburnCoarseLTwoVarEarlyStoppingFalse}{\tbd{miouCISATburnCoarseLTwoVarEarlyStoppingFalse}}
\providecommand{\miouCISATburnCoarseLTwoVarEarlyStoppingFalseFrozenEncoderTrue}{\tbd{miouCISATburnCoarseLTwoVarEarlyStoppingFalseFrozenEncoderTrue}}
\providecommand{\miouCISATburnCoarseLTwoVarFrozenEncoderTrue}{\tbd{miouCISATburnCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\miouCISATburnCoarseLTwoVarLossBootstrap}{\tbd{miouCISATburnCoarseLTwoVarLossBootstrap}}
\providecommand{\miouCISATburnCoarseLTwoVarLossGce}{\tbd{miouCISATburnCoarseLTwoVarLossGce}}
\providecommand{\miouCISATburnCoarseLTwoVarLrMultThree}{\tbd{miouCISATburnCoarseLTwoVarLrMultThree}}
\providecommand{\miouCISATburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATburnCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCISATburnCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCISATburnCoarseLTwoVarValLabelsClean}{\tbd{miouCISATburnCoarseLTwoVarValLabelsClean}}
\providecommand{\miouCISATburnOmissionLOne}{\tbd{miouCISATburnOmissionLOne}}
\providecommand{\miouCISATburnOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{miouCISATburnOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCISATburnOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{miouCISATburnOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATburnOmissionLOneVarDecoderSamLite}{\tbd{miouCISATburnOmissionLOneVarDecoderSamLite}}
\providecommand{\miouCISATburnOmissionLOneVarDecoderSamPretrained}{\tbd{miouCISATburnOmissionLOneVarDecoderSamPretrained}}
\providecommand{\miouCISATburnOmissionLOneVarDecoderSegformerMlp}{\tbd{miouCISATburnOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\miouCISATburnOmissionLR}{\tbd{miouCISATburnOmissionLR}}
\providecommand{\miouCISATburnOmissionLRVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATburnOmissionLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATburnOmissionLTwo}{\tbd{miouCISATburnOmissionLTwo}}
\providecommand{\miouCISATburnOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCISATburnOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCISATburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATburnOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCISATburnOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATburnOmissionLTwoVarDecoderSamLite}{\tbd{miouCISATburnOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouCISATburnOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATburnOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATburnOmissionLTwoVarDecoderSamPretrained}{\tbd{miouCISATburnOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\miouCISATburnOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATburnOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATburnOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouCISATburnOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCISATburnOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATburnOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATburnOmissionLTwoVarFrozenEncoderTrue}{\tbd{miouCISATburnOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\miouCISATburnOmissionLTwoVarLossBootstrap}{\tbd{miouCISATburnOmissionLTwoVarLossBootstrap}}
\providecommand{\miouCISATburnOmissionLTwoVarLossGce}{\tbd{miouCISATburnOmissionLTwoVarLossGce}}
\providecommand{\miouCISATburnOmissionLTwoVarLrMultThree}{\tbd{miouCISATburnOmissionLTwoVarLrMultThree}}
\providecommand{\miouCISATburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATburnOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCISATburnOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCISATburnOmissionLTwoVarValLabelsClean}{\tbd{miouCISATburnOmissionLTwoVarValLabelsClean}}
\providecommand{\miouCISATburnShiftLOne}{\tbd{miouCISATburnShiftLOne}}
\providecommand{\miouCISATburnShiftLOneVarDecoderMaskTwoformerFull}{\tbd{miouCISATburnShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCISATburnShiftLOneVarDecoderMaskTwoformerLite}{\tbd{miouCISATburnShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATburnShiftLOneVarDecoderSamLite}{\tbd{miouCISATburnShiftLOneVarDecoderSamLite}}
\providecommand{\miouCISATburnShiftLOneVarDecoderSamPretrained}{\tbd{miouCISATburnShiftLOneVarDecoderSamPretrained}}
\providecommand{\miouCISATburnShiftLOneVarDecoderSegformerMlp}{\tbd{miouCISATburnShiftLOneVarDecoderSegformerMlp}}
\providecommand{\miouCISATburnShiftLR}{\tbd{miouCISATburnShiftLR}}
\providecommand{\miouCISATburnShiftLRVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATburnShiftLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATburnShiftLTwo}{\tbd{miouCISATburnShiftLTwo}}
\providecommand{\miouCISATburnShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCISATburnShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCISATburnShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATburnShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATburnShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCISATburnShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATburnShiftLTwoVarDecoderSamLite}{\tbd{miouCISATburnShiftLTwoVarDecoderSamLite}}
\providecommand{\miouCISATburnShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATburnShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATburnShiftLTwoVarDecoderSamPretrained}{\tbd{miouCISATburnShiftLTwoVarDecoderSamPretrained}}
\providecommand{\miouCISATburnShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATburnShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATburnShiftLTwoVarDecoderSegformerMlp}{\tbd{miouCISATburnShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCISATburnShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATburnShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATburnShiftLTwoVarFrozenEncoderTrue}{\tbd{miouCISATburnShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\miouCISATburnShiftLTwoVarLossBootstrap}{\tbd{miouCISATburnShiftLTwoVarLossBootstrap}}
\providecommand{\miouCISATburnShiftLTwoVarLossGce}{\tbd{miouCISATburnShiftLTwoVarLossGce}}
\providecommand{\miouCISATburnShiftLTwoVarLrMultThree}{\tbd{miouCISATburnShiftLTwoVarLrMultThree}}
\providecommand{\miouCISATburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATburnShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCISATburnShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCISATburnShiftLTwoVarValLabelsClean}{\tbd{miouCISATburnShiftLTwoVarValLabelsClean}}
\providecommand{\miouCISATflairBoundaryLOne}{\tbd{miouCISATflairBoundaryLOne}}
\providecommand{\miouCISATflairBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{miouCISATflairBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCISATflairBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{miouCISATflairBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATflairBoundaryLOneVarDecoderSamLite}{\tbd{miouCISATflairBoundaryLOneVarDecoderSamLite}}
\providecommand{\miouCISATflairBoundaryLOneVarDecoderSamPretrained}{\tbd{miouCISATflairBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\miouCISATflairBoundaryLOneVarDecoderSegformerMlp}{\tbd{miouCISATflairBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\miouCISATflairBoundaryLR}{\tbd{miouCISATflairBoundaryLR}}
\providecommand{\miouCISATflairBoundaryLRVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATflairBoundaryLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATflairBoundaryLTwo}{\tbd{miouCISATflairBoundaryLTwo}}
\providecommand{\miouCISATflairBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCISATflairBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCISATflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATflairBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCISATflairBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATflairBoundaryLTwoVarDecoderSamLite}{\tbd{miouCISATflairBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouCISATflairBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATflairBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATflairBoundaryLTwoVarDecoderSamPretrained}{\tbd{miouCISATflairBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\miouCISATflairBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATflairBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATflairBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouCISATflairBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCISATflairBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATflairBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATflairBoundaryLTwoVarFrozenEncoderTrue}{\tbd{miouCISATflairBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\miouCISATflairBoundaryLTwoVarLossBootstrap}{\tbd{miouCISATflairBoundaryLTwoVarLossBootstrap}}
\providecommand{\miouCISATflairBoundaryLTwoVarLossGce}{\tbd{miouCISATflairBoundaryLTwoVarLossGce}}
\providecommand{\miouCISATflairBoundaryLTwoVarLrMultThree}{\tbd{miouCISATflairBoundaryLTwoVarLrMultThree}}
\providecommand{\miouCISATflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATflairBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCISATflairBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCISATflairBoundaryLTwoVarValLabelsClean}{\tbd{miouCISATflairBoundaryLTwoVarValLabelsClean}}
\providecommand{\miouCISATflairClean}{\tbd{miouCISATflairClean}}
\providecommand{\miouCISATflairCleanVarClassWeightedTrue}{\tbd{miouCISATflairCleanVarClassWeightedTrue}}
\providecommand{\miouCISATflairCleanVarDecoderMaskTwoformerFull}{\tbd{miouCISATflairCleanVarDecoderMaskTwoformerFull}}
\providecommand{\miouCISATflairCleanVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATflairCleanVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATflairCleanVarDecoderMaskTwoformerLite}{\tbd{miouCISATflairCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATflairCleanVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATflairCleanVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATflairCleanVarDecoderSamLite}{\tbd{miouCISATflairCleanVarDecoderSamLite}}
\providecommand{\miouCISATflairCleanVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATflairCleanVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATflairCleanVarDecoderSamPretrained}{\tbd{miouCISATflairCleanVarDecoderSamPretrained}}
\providecommand{\miouCISATflairCleanVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATflairCleanVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATflairCleanVarDecoderSegformerMlp}{\tbd{miouCISATflairCleanVarDecoderSegformerMlp}}
\providecommand{\miouCISATflairCleanVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATflairCleanVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATflairCleanVarFrozenEncoderTrue}{\tbd{miouCISATflairCleanVarFrozenEncoderTrue}}
\providecommand{\miouCISATflairCleanVarLossBootstrap}{\tbd{miouCISATflairCleanVarLossBootstrap}}
\providecommand{\miouCISATflairCleanVarLossGce}{\tbd{miouCISATflairCleanVarLossGce}}
\providecommand{\miouCISATflairCleanVarLrMultThree}{\tbd{miouCISATflairCleanVarLrMultThree}}
\providecommand{\miouCISATflairCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATflairCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATflairCleanVarTrainSubsetCleanTwoFive}{\tbd{miouCISATflairCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCISATflairCleanVarValLabelsClean}{\tbd{miouCISATflairCleanVarValLabelsClean}}
\providecommand{\miouCISATflairCoarseLOne}{\tbd{miouCISATflairCoarseLOne}}
\providecommand{\miouCISATflairCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{miouCISATflairCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCISATflairCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{miouCISATflairCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATflairCoarseLOneVarDecoderSamLite}{\tbd{miouCISATflairCoarseLOneVarDecoderSamLite}}
\providecommand{\miouCISATflairCoarseLOneVarDecoderSamPretrained}{\tbd{miouCISATflairCoarseLOneVarDecoderSamPretrained}}
\providecommand{\miouCISATflairCoarseLOneVarDecoderSegformerMlp}{\tbd{miouCISATflairCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\miouCISATflairCoarseLR}{\tbd{miouCISATflairCoarseLR}}
\providecommand{\miouCISATflairCoarseLRVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATflairCoarseLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATflairCoarseLTwo}{\tbd{miouCISATflairCoarseLTwo}}
\providecommand{\miouCISATflairCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCISATflairCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCISATflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATflairCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCISATflairCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATflairCoarseLTwoVarDecoderSamLite}{\tbd{miouCISATflairCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouCISATflairCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATflairCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATflairCoarseLTwoVarDecoderSamPretrained}{\tbd{miouCISATflairCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\miouCISATflairCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATflairCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATflairCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouCISATflairCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCISATflairCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATflairCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATflairCoarseLTwoVarFrozenEncoderTrue}{\tbd{miouCISATflairCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\miouCISATflairCoarseLTwoVarLossBootstrap}{\tbd{miouCISATflairCoarseLTwoVarLossBootstrap}}
\providecommand{\miouCISATflairCoarseLTwoVarLossGce}{\tbd{miouCISATflairCoarseLTwoVarLossGce}}
\providecommand{\miouCISATflairCoarseLTwoVarLrMultThree}{\tbd{miouCISATflairCoarseLTwoVarLrMultThree}}
\providecommand{\miouCISATflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATflairCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCISATflairCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCISATflairCoarseLTwoVarValLabelsClean}{\tbd{miouCISATflairCoarseLTwoVarValLabelsClean}}
\providecommand{\miouCISATflairOmissionLOne}{\tbd{miouCISATflairOmissionLOne}}
\providecommand{\miouCISATflairOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{miouCISATflairOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCISATflairOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{miouCISATflairOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATflairOmissionLOneVarDecoderSamLite}{\tbd{miouCISATflairOmissionLOneVarDecoderSamLite}}
\providecommand{\miouCISATflairOmissionLOneVarDecoderSamPretrained}{\tbd{miouCISATflairOmissionLOneVarDecoderSamPretrained}}
\providecommand{\miouCISATflairOmissionLOneVarDecoderSegformerMlp}{\tbd{miouCISATflairOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\miouCISATflairOmissionLR}{\tbd{miouCISATflairOmissionLR}}
\providecommand{\miouCISATflairOmissionLRVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATflairOmissionLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATflairOmissionLTwo}{\tbd{miouCISATflairOmissionLTwo}}
\providecommand{\miouCISATflairOmissionLTwoVarClassWeightedTrue}{\tbd{miouCISATflairOmissionLTwoVarClassWeightedTrue}}
\providecommand{\miouCISATflairOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCISATflairOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCISATflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATflairOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCISATflairOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATflairOmissionLTwoVarDecoderSamLite}{\tbd{miouCISATflairOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouCISATflairOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATflairOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATflairOmissionLTwoVarDecoderSamPretrained}{\tbd{miouCISATflairOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\miouCISATflairOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATflairOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATflairOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouCISATflairOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCISATflairOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATflairOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATflairOmissionLTwoVarEarlyStoppingFalse}{\tbd{miouCISATflairOmissionLTwoVarEarlyStoppingFalse}}
\providecommand{\miouCISATflairOmissionLTwoVarEarlyStoppingFalseFrozenEncoderTrue}{\tbd{miouCISATflairOmissionLTwoVarEarlyStoppingFalseFrozenEncoderTrue}}
\providecommand{\miouCISATflairOmissionLTwoVarFrozenEncoderTrue}{\tbd{miouCISATflairOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\miouCISATflairOmissionLTwoVarLossBootstrap}{\tbd{miouCISATflairOmissionLTwoVarLossBootstrap}}
\providecommand{\miouCISATflairOmissionLTwoVarLossGce}{\tbd{miouCISATflairOmissionLTwoVarLossGce}}
\providecommand{\miouCISATflairOmissionLTwoVarLrMultThree}{\tbd{miouCISATflairOmissionLTwoVarLrMultThree}}
\providecommand{\miouCISATflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATflairOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCISATflairOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCISATflairOmissionLTwoVarValLabelsClean}{\tbd{miouCISATflairOmissionLTwoVarValLabelsClean}}
\providecommand{\miouCISATflairShiftLOne}{\tbd{miouCISATflairShiftLOne}}
\providecommand{\miouCISATflairShiftLOneVarDecoderMaskTwoformerFull}{\tbd{miouCISATflairShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCISATflairShiftLOneVarDecoderMaskTwoformerLite}{\tbd{miouCISATflairShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATflairShiftLOneVarDecoderSamLite}{\tbd{miouCISATflairShiftLOneVarDecoderSamLite}}
\providecommand{\miouCISATflairShiftLOneVarDecoderSamPretrained}{\tbd{miouCISATflairShiftLOneVarDecoderSamPretrained}}
\providecommand{\miouCISATflairShiftLOneVarDecoderSegformerMlp}{\tbd{miouCISATflairShiftLOneVarDecoderSegformerMlp}}
\providecommand{\miouCISATflairShiftLR}{\tbd{miouCISATflairShiftLR}}
\providecommand{\miouCISATflairShiftLRVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATflairShiftLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATflairShiftLTwo}{\tbd{miouCISATflairShiftLTwo}}
\providecommand{\miouCISATflairShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCISATflairShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCISATflairShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATflairShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATflairShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCISATflairShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCISATflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATflairShiftLTwoVarDecoderSamLite}{\tbd{miouCISATflairShiftLTwoVarDecoderSamLite}}
\providecommand{\miouCISATflairShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATflairShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATflairShiftLTwoVarDecoderSamPretrained}{\tbd{miouCISATflairShiftLTwoVarDecoderSamPretrained}}
\providecommand{\miouCISATflairShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATflairShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATflairShiftLTwoVarDecoderSegformerMlp}{\tbd{miouCISATflairShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCISATflairShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATflairShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATflairShiftLTwoVarFrozenEncoderTrue}{\tbd{miouCISATflairShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\miouCISATflairShiftLTwoVarLossBootstrap}{\tbd{miouCISATflairShiftLTwoVarLossBootstrap}}
\providecommand{\miouCISATflairShiftLTwoVarLossGce}{\tbd{miouCISATflairShiftLTwoVarLossGce}}
\providecommand{\miouCISATflairShiftLTwoVarLrMultThree}{\tbd{miouCISATflairShiftLTwoVarLrMultThree}}
\providecommand{\miouCISATflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCISATflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCISATflairShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCISATflairShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCISATflairShiftLTwoVarValLabelsClean}{\tbd{miouCISATflairShiftLTwoVarValLabelsClean}}
\providecommand{\miouCISATsenClean}{\tbd{miouCISATsenClean}}
\providecommand{\miouCISATsenOtsuLTwo}{\tbd{miouCISATsenOtsuLTwo}}
\providecommand{\miouCITMChesBoundaryLOne}{\tbd{miouCITMChesBoundaryLOne}}
\providecommand{\miouCITMChesBoundaryLTwo}{\tbd{miouCITMChesBoundaryLTwo}}
\providecommand{\miouCITMChesClean}{\tbd{miouCITMChesClean}}
\providecommand{\miouCITMChesCoarseLOne}{\tbd{miouCITMChesCoarseLOne}}
\providecommand{\miouCITMChesCoarseLTwo}{\tbd{miouCITMChesCoarseLTwo}}
\providecommand{\miouCITMChesNlcdREAL}{\tbd{miouCITMChesNlcdREAL}}
\providecommand{\miouCITMChesOmissionLOne}{\tbd{miouCITMChesOmissionLOne}}
\providecommand{\miouCITMChesOmissionLTwo}{\tbd{miouCITMChesOmissionLTwo}}
\providecommand{\miouCITMChesShiftLOne}{\tbd{miouCITMChesShiftLOne}}
\providecommand{\miouCITMChesShiftLTwo}{\tbd{miouCITMChesShiftLTwo}}
\providecommand{\miouCITMCsTwelveBoundaryLOne}{\tbd{miouCITMCsTwelveBoundaryLOne}}
\providecommand{\miouCITMCsTwelveBoundaryLTwo}{\tbd{miouCITMCsTwelveBoundaryLTwo}}
\providecommand{\miouCITMCsTwelveClean}{\tbd{miouCITMCsTwelveClean}}
\providecommand{\miouCITMCsTwelveCoarseLOne}{\tbd{miouCITMCsTwelveCoarseLOne}}
\providecommand{\miouCITMCsTwelveCoarseLTwo}{\tbd{miouCITMCsTwelveCoarseLTwo}}
\providecommand{\miouCITMCsTwelveOmissionLOne}{\tbd{miouCITMCsTwelveOmissionLOne}}
\providecommand{\miouCITMCsTwelveOmissionLTwo}{\tbd{miouCITMCsTwelveOmissionLTwo}}
\providecommand{\miouCITMCsTwelveSTwocloudlessREAL}{\tbd{miouCITMCsTwelveSTwocloudlessREAL}}
\providecommand{\miouCITMCsTwelveShiftLOne}{\tbd{miouCITMCsTwelveShiftLOne}}
\providecommand{\miouCITMCsTwelveShiftLTwo}{\tbd{miouCITMCsTwelveShiftLTwo}}
\providecommand{\miouCITMDfcBoundaryLOne}{\tbd{miouCITMDfcBoundaryLOne}}
\providecommand{\miouCITMDfcBoundaryLTwo}{\tbd{miouCITMDfcBoundaryLTwo}}
\providecommand{\miouCITMDfcClean}{\tbd{miouCITMDfcClean}}
\providecommand{\miouCITMDfcCleanVarTrainSubsetRealcov}{\tbd{miouCITMDfcCleanVarTrainSubsetRealcov}}
\providecommand{\miouCITMDfcCoarseLOne}{\tbd{miouCITMDfcCoarseLOne}}
\providecommand{\miouCITMDfcCoarseLTwo}{\tbd{miouCITMDfcCoarseLTwo}}
\providecommand{\miouCITMDfcModisREALVarTrainSubsetRealcov}{\tbd{miouCITMDfcModisREALVarTrainSubsetRealcov}}
\providecommand{\miouCITMDfcOmissionLOne}{\tbd{miouCITMDfcOmissionLOne}}
\providecommand{\miouCITMDfcOmissionLTwo}{\tbd{miouCITMDfcOmissionLTwo}}
\providecommand{\miouCITMDfcShiftLOne}{\tbd{miouCITMDfcShiftLOne}}
\providecommand{\miouCITMDfcShiftLTwo}{\tbd{miouCITMDfcShiftLTwo}}
\providecommand{\miouCITMEnvaBoundaryLOne}{\tbd{miouCITMEnvaBoundaryLOne}}
\providecommand{\miouCITMEnvaBoundaryLTwo}{\tbd{miouCITMEnvaBoundaryLTwo}}
\providecommand{\miouCITMEnvaClean}{\tbd{miouCITMEnvaClean}}
\providecommand{\miouCITMEnvaCoarseLOne}{\tbd{miouCITMEnvaCoarseLOne}}
\providecommand{\miouCITMEnvaCoarseLTwo}{\tbd{miouCITMEnvaCoarseLTwo}}
\providecommand{\miouCITMEnvaNlcdREAL}{\tbd{miouCITMEnvaNlcdREAL}}
\providecommand{\miouCITMEnvaOmissionLOne}{\tbd{miouCITMEnvaOmissionLOne}}
\providecommand{\miouCITMEnvaOmissionLTwo}{\tbd{miouCITMEnvaOmissionLTwo}}
\providecommand{\miouCITMEnvaShiftLOne}{\tbd{miouCITMEnvaShiftLOne}}
\providecommand{\miouCITMEnvaShiftLTwo}{\tbd{miouCITMEnvaShiftLTwo}}
\providecommand{\miouCITMKuroBoundaryLOne}{\tbd{miouCITMKuroBoundaryLOne}}
\providecommand{\miouCITMKuroBoundaryLTwo}{\tbd{miouCITMKuroBoundaryLTwo}}
\providecommand{\miouCITMKuroCemsREALVarTrainSubsetRealcov}{\tbd{miouCITMKuroCemsREALVarTrainSubsetRealcov}}
\providecommand{\miouCITMKuroClean}{\tbd{miouCITMKuroClean}}
\providecommand{\miouCITMKuroCleanVarTrainSubsetRealcov}{\tbd{miouCITMKuroCleanVarTrainSubsetRealcov}}
\providecommand{\miouCITMKuroCoarseLOne}{\tbd{miouCITMKuroCoarseLOne}}
\providecommand{\miouCITMKuroCoarseLTwo}{\tbd{miouCITMKuroCoarseLTwo}}
\providecommand{\miouCITMKuroOmissionLOne}{\tbd{miouCITMKuroOmissionLOne}}
\providecommand{\miouCITMKuroOmissionLTwo}{\tbd{miouCITMKuroOmissionLTwo}}
\providecommand{\miouCITMKuroShiftLOne}{\tbd{miouCITMKuroShiftLOne}}
\providecommand{\miouCITMKuroShiftLTwo}{\tbd{miouCITMKuroShiftLTwo}}
\providecommand{\miouCITMOemBoundaryLOne}{\tbd{miouCITMOemBoundaryLOne}}
\providecommand{\miouCITMOemBoundaryLTwo}{\tbd{miouCITMOemBoundaryLTwo}}
\providecommand{\miouCITMOemClean}{\tbd{miouCITMOemClean}}
\providecommand{\miouCITMOemCoarseLOne}{\tbd{miouCITMOemCoarseLOne}}
\providecommand{\miouCITMOemCoarseLTwo}{\tbd{miouCITMOemCoarseLTwo}}
\providecommand{\miouCITMOemOmissionLOne}{\tbd{miouCITMOemOmissionLOne}}
\providecommand{\miouCITMOemOmissionLTwo}{\tbd{miouCITMOemOmissionLTwo}}
\providecommand{\miouCITMOemShiftLOne}{\tbd{miouCITMOemShiftLOne}}
\providecommand{\miouCITMOemShiftLTwo}{\tbd{miouCITMOemShiftLTwo}}
\providecommand{\miouCITMSnTwoBoundaryLOne}{\tbd{miouCITMSnTwoBoundaryLOne}}
\providecommand{\miouCITMSnTwoBoundaryLTwo}{\tbd{miouCITMSnTwoBoundaryLTwo}}
\providecommand{\miouCITMSnTwoClean}{\tbd{miouCITMSnTwoClean}}
\providecommand{\miouCITMSnTwoCoarseLOne}{\tbd{miouCITMSnTwoCoarseLOne}}
\providecommand{\miouCITMSnTwoCoarseLTwo}{\tbd{miouCITMSnTwoCoarseLTwo}}
\providecommand{\miouCITMSnTwoOmissionLOne}{\tbd{miouCITMSnTwoOmissionLOne}}
\providecommand{\miouCITMSnTwoOmissionLTwo}{\tbd{miouCITMSnTwoOmissionLTwo}}
\providecommand{\miouCITMSnTwoShiftLOne}{\tbd{miouCITMSnTwoShiftLOne}}
\providecommand{\miouCITMSnTwoShiftLTwo}{\tbd{miouCITMSnTwoShiftLTwo}}
\providecommand{\miouCITMburnBoundaryLOne}{\tbd{miouCITMburnBoundaryLOne}}
\providecommand{\miouCITMburnBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{miouCITMburnBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCITMburnBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{miouCITMburnBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCITMburnBoundaryLOneVarDecoderSamLite}{\tbd{miouCITMburnBoundaryLOneVarDecoderSamLite}}
\providecommand{\miouCITMburnBoundaryLOneVarDecoderSamPretrained}{\tbd{miouCITMburnBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\miouCITMburnBoundaryLOneVarDecoderSegformerMlp}{\tbd{miouCITMburnBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\miouCITMburnBoundaryLR}{\tbd{miouCITMburnBoundaryLR}}
\providecommand{\miouCITMburnBoundaryLTwo}{\tbd{miouCITMburnBoundaryLTwo}}
\providecommand{\miouCITMburnBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCITMburnBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCITMburnBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCITMburnBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCITMburnBoundaryLTwoVarDecoderSamLite}{\tbd{miouCITMburnBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouCITMburnBoundaryLTwoVarDecoderSamPretrained}{\tbd{miouCITMburnBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\miouCITMburnBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouCITMburnBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCITMburnBoundaryLTwoVarFrozenEncoderTrue}{\tbd{miouCITMburnBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\miouCITMburnBoundaryLTwoVarLossBootstrap}{\tbd{miouCITMburnBoundaryLTwoVarLossBootstrap}}
\providecommand{\miouCITMburnBoundaryLTwoVarLossGce}{\tbd{miouCITMburnBoundaryLTwoVarLossGce}}
\providecommand{\miouCITMburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCITMburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCITMburnBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCITMburnBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCITMburnClean}{\tbd{miouCITMburnClean}}
\providecommand{\miouCITMburnCleanVarDecoderMaskTwoformerFull}{\tbd{miouCITMburnCleanVarDecoderMaskTwoformerFull}}
\providecommand{\miouCITMburnCleanVarDecoderMaskTwoformerLite}{\tbd{miouCITMburnCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouCITMburnCleanVarDecoderSamLite}{\tbd{miouCITMburnCleanVarDecoderSamLite}}
\providecommand{\miouCITMburnCleanVarDecoderSamPretrained}{\tbd{miouCITMburnCleanVarDecoderSamPretrained}}
\providecommand{\miouCITMburnCleanVarDecoderSegformerMlp}{\tbd{miouCITMburnCleanVarDecoderSegformerMlp}}
\providecommand{\miouCITMburnCleanVarFrozenEncoderTrue}{\tbd{miouCITMburnCleanVarFrozenEncoderTrue}}
\providecommand{\miouCITMburnCleanVarLossBootstrap}{\tbd{miouCITMburnCleanVarLossBootstrap}}
\providecommand{\miouCITMburnCleanVarLossGce}{\tbd{miouCITMburnCleanVarLossGce}}
\providecommand{\miouCITMburnCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCITMburnCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCITMburnCleanVarTrainSubsetCleanTwoFive}{\tbd{miouCITMburnCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCITMburnCoarseLOne}{\tbd{miouCITMburnCoarseLOne}}
\providecommand{\miouCITMburnCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{miouCITMburnCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCITMburnCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{miouCITMburnCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCITMburnCoarseLOneVarDecoderSamLite}{\tbd{miouCITMburnCoarseLOneVarDecoderSamLite}}
\providecommand{\miouCITMburnCoarseLOneVarDecoderSamPretrained}{\tbd{miouCITMburnCoarseLOneVarDecoderSamPretrained}}
\providecommand{\miouCITMburnCoarseLOneVarDecoderSegformerMlp}{\tbd{miouCITMburnCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\miouCITMburnCoarseLR}{\tbd{miouCITMburnCoarseLR}}
\providecommand{\miouCITMburnCoarseLTwo}{\tbd{miouCITMburnCoarseLTwo}}
\providecommand{\miouCITMburnCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCITMburnCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCITMburnCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCITMburnCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCITMburnCoarseLTwoVarDecoderSamLite}{\tbd{miouCITMburnCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouCITMburnCoarseLTwoVarDecoderSamPretrained}{\tbd{miouCITMburnCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\miouCITMburnCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouCITMburnCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCITMburnCoarseLTwoVarFrozenEncoderTrue}{\tbd{miouCITMburnCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\miouCITMburnCoarseLTwoVarLossBootstrap}{\tbd{miouCITMburnCoarseLTwoVarLossBootstrap}}
\providecommand{\miouCITMburnCoarseLTwoVarLossGce}{\tbd{miouCITMburnCoarseLTwoVarLossGce}}
\providecommand{\miouCITMburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCITMburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCITMburnCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCITMburnCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCITMburnOmissionLOne}{\tbd{miouCITMburnOmissionLOne}}
\providecommand{\miouCITMburnOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{miouCITMburnOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCITMburnOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{miouCITMburnOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCITMburnOmissionLOneVarDecoderSamLite}{\tbd{miouCITMburnOmissionLOneVarDecoderSamLite}}
\providecommand{\miouCITMburnOmissionLOneVarDecoderSamPretrained}{\tbd{miouCITMburnOmissionLOneVarDecoderSamPretrained}}
\providecommand{\miouCITMburnOmissionLOneVarDecoderSegformerMlp}{\tbd{miouCITMburnOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\miouCITMburnOmissionLR}{\tbd{miouCITMburnOmissionLR}}
\providecommand{\miouCITMburnOmissionLTwo}{\tbd{miouCITMburnOmissionLTwo}}
\providecommand{\miouCITMburnOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCITMburnOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCITMburnOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCITMburnOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCITMburnOmissionLTwoVarDecoderSamLite}{\tbd{miouCITMburnOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouCITMburnOmissionLTwoVarDecoderSamPretrained}{\tbd{miouCITMburnOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\miouCITMburnOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouCITMburnOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCITMburnOmissionLTwoVarFrozenEncoderTrue}{\tbd{miouCITMburnOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\miouCITMburnOmissionLTwoVarLossBootstrap}{\tbd{miouCITMburnOmissionLTwoVarLossBootstrap}}
\providecommand{\miouCITMburnOmissionLTwoVarLossGce}{\tbd{miouCITMburnOmissionLTwoVarLossGce}}
\providecommand{\miouCITMburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCITMburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCITMburnOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCITMburnOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCITMburnShiftLOne}{\tbd{miouCITMburnShiftLOne}}
\providecommand{\miouCITMburnShiftLOneVarDecoderMaskTwoformerFull}{\tbd{miouCITMburnShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCITMburnShiftLOneVarDecoderMaskTwoformerLite}{\tbd{miouCITMburnShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCITMburnShiftLOneVarDecoderSamLite}{\tbd{miouCITMburnShiftLOneVarDecoderSamLite}}
\providecommand{\miouCITMburnShiftLOneVarDecoderSamPretrained}{\tbd{miouCITMburnShiftLOneVarDecoderSamPretrained}}
\providecommand{\miouCITMburnShiftLOneVarDecoderSegformerMlp}{\tbd{miouCITMburnShiftLOneVarDecoderSegformerMlp}}
\providecommand{\miouCITMburnShiftLR}{\tbd{miouCITMburnShiftLR}}
\providecommand{\miouCITMburnShiftLTwo}{\tbd{miouCITMburnShiftLTwo}}
\providecommand{\miouCITMburnShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCITMburnShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCITMburnShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCITMburnShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCITMburnShiftLTwoVarDecoderSamLite}{\tbd{miouCITMburnShiftLTwoVarDecoderSamLite}}
\providecommand{\miouCITMburnShiftLTwoVarDecoderSamPretrained}{\tbd{miouCITMburnShiftLTwoVarDecoderSamPretrained}}
\providecommand{\miouCITMburnShiftLTwoVarDecoderSegformerMlp}{\tbd{miouCITMburnShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCITMburnShiftLTwoVarFrozenEncoderTrue}{\tbd{miouCITMburnShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\miouCITMburnShiftLTwoVarLossBootstrap}{\tbd{miouCITMburnShiftLTwoVarLossBootstrap}}
\providecommand{\miouCITMburnShiftLTwoVarLossGce}{\tbd{miouCITMburnShiftLTwoVarLossGce}}
\providecommand{\miouCITMburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCITMburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCITMburnShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCITMburnShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCITMflairBoundaryLOne}{\tbd{miouCITMflairBoundaryLOne}}
\providecommand{\miouCITMflairBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{miouCITMflairBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCITMflairBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{miouCITMflairBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCITMflairBoundaryLOneVarDecoderSamLite}{\tbd{miouCITMflairBoundaryLOneVarDecoderSamLite}}
\providecommand{\miouCITMflairBoundaryLOneVarDecoderSamPretrained}{\tbd{miouCITMflairBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\miouCITMflairBoundaryLOneVarDecoderSegformerMlp}{\tbd{miouCITMflairBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\miouCITMflairBoundaryLR}{\tbd{miouCITMflairBoundaryLR}}
\providecommand{\miouCITMflairBoundaryLTwo}{\tbd{miouCITMflairBoundaryLTwo}}
\providecommand{\miouCITMflairBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCITMflairBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCITMflairBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCITMflairBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCITMflairBoundaryLTwoVarDecoderSamLite}{\tbd{miouCITMflairBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouCITMflairBoundaryLTwoVarDecoderSamPretrained}{\tbd{miouCITMflairBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\miouCITMflairBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouCITMflairBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCITMflairBoundaryLTwoVarFrozenEncoderTrue}{\tbd{miouCITMflairBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\miouCITMflairBoundaryLTwoVarLossBootstrap}{\tbd{miouCITMflairBoundaryLTwoVarLossBootstrap}}
\providecommand{\miouCITMflairBoundaryLTwoVarLossGce}{\tbd{miouCITMflairBoundaryLTwoVarLossGce}}
\providecommand{\miouCITMflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCITMflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCITMflairBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCITMflairBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCITMflairClean}{\tbd{miouCITMflairClean}}
\providecommand{\miouCITMflairCleanVarDecoderMaskTwoformerFull}{\tbd{miouCITMflairCleanVarDecoderMaskTwoformerFull}}
\providecommand{\miouCITMflairCleanVarDecoderMaskTwoformerLite}{\tbd{miouCITMflairCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouCITMflairCleanVarDecoderSamLite}{\tbd{miouCITMflairCleanVarDecoderSamLite}}
\providecommand{\miouCITMflairCleanVarDecoderSamPretrained}{\tbd{miouCITMflairCleanVarDecoderSamPretrained}}
\providecommand{\miouCITMflairCleanVarDecoderSegformerMlp}{\tbd{miouCITMflairCleanVarDecoderSegformerMlp}}
\providecommand{\miouCITMflairCleanVarFrozenEncoderTrue}{\tbd{miouCITMflairCleanVarFrozenEncoderTrue}}
\providecommand{\miouCITMflairCleanVarLossBootstrap}{\tbd{miouCITMflairCleanVarLossBootstrap}}
\providecommand{\miouCITMflairCleanVarLossGce}{\tbd{miouCITMflairCleanVarLossGce}}
\providecommand{\miouCITMflairCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCITMflairCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCITMflairCleanVarTrainSubsetCleanTwoFive}{\tbd{miouCITMflairCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCITMflairCoarseLOne}{\tbd{miouCITMflairCoarseLOne}}
\providecommand{\miouCITMflairCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{miouCITMflairCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCITMflairCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{miouCITMflairCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCITMflairCoarseLOneVarDecoderSamLite}{\tbd{miouCITMflairCoarseLOneVarDecoderSamLite}}
\providecommand{\miouCITMflairCoarseLOneVarDecoderSamPretrained}{\tbd{miouCITMflairCoarseLOneVarDecoderSamPretrained}}
\providecommand{\miouCITMflairCoarseLOneVarDecoderSegformerMlp}{\tbd{miouCITMflairCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\miouCITMflairCoarseLR}{\tbd{miouCITMflairCoarseLR}}
\providecommand{\miouCITMflairCoarseLTwo}{\tbd{miouCITMflairCoarseLTwo}}
\providecommand{\miouCITMflairCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCITMflairCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCITMflairCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCITMflairCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCITMflairCoarseLTwoVarDecoderSamLite}{\tbd{miouCITMflairCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouCITMflairCoarseLTwoVarDecoderSamPretrained}{\tbd{miouCITMflairCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\miouCITMflairCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouCITMflairCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCITMflairCoarseLTwoVarFrozenEncoderTrue}{\tbd{miouCITMflairCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\miouCITMflairCoarseLTwoVarLossBootstrap}{\tbd{miouCITMflairCoarseLTwoVarLossBootstrap}}
\providecommand{\miouCITMflairCoarseLTwoVarLossGce}{\tbd{miouCITMflairCoarseLTwoVarLossGce}}
\providecommand{\miouCITMflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCITMflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCITMflairCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCITMflairCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCITMflairOmissionLOne}{\tbd{miouCITMflairOmissionLOne}}
\providecommand{\miouCITMflairOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{miouCITMflairOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCITMflairOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{miouCITMflairOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCITMflairOmissionLOneVarDecoderSamLite}{\tbd{miouCITMflairOmissionLOneVarDecoderSamLite}}
\providecommand{\miouCITMflairOmissionLOneVarDecoderSamPretrained}{\tbd{miouCITMflairOmissionLOneVarDecoderSamPretrained}}
\providecommand{\miouCITMflairOmissionLOneVarDecoderSegformerMlp}{\tbd{miouCITMflairOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\miouCITMflairOmissionLR}{\tbd{miouCITMflairOmissionLR}}
\providecommand{\miouCITMflairOmissionLTwo}{\tbd{miouCITMflairOmissionLTwo}}
\providecommand{\miouCITMflairOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCITMflairOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCITMflairOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCITMflairOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCITMflairOmissionLTwoVarDecoderSamLite}{\tbd{miouCITMflairOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouCITMflairOmissionLTwoVarDecoderSamPretrained}{\tbd{miouCITMflairOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\miouCITMflairOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouCITMflairOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCITMflairOmissionLTwoVarFrozenEncoderTrue}{\tbd{miouCITMflairOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\miouCITMflairOmissionLTwoVarLossBootstrap}{\tbd{miouCITMflairOmissionLTwoVarLossBootstrap}}
\providecommand{\miouCITMflairOmissionLTwoVarLossGce}{\tbd{miouCITMflairOmissionLTwoVarLossGce}}
\providecommand{\miouCITMflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCITMflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCITMflairOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCITMflairOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCITMflairShiftLOne}{\tbd{miouCITMflairShiftLOne}}
\providecommand{\miouCITMflairShiftLOneVarDecoderMaskTwoformerFull}{\tbd{miouCITMflairShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouCITMflairShiftLOneVarDecoderMaskTwoformerLite}{\tbd{miouCITMflairShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouCITMflairShiftLOneVarDecoderSamLite}{\tbd{miouCITMflairShiftLOneVarDecoderSamLite}}
\providecommand{\miouCITMflairShiftLOneVarDecoderSamPretrained}{\tbd{miouCITMflairShiftLOneVarDecoderSamPretrained}}
\providecommand{\miouCITMflairShiftLOneVarDecoderSegformerMlp}{\tbd{miouCITMflairShiftLOneVarDecoderSegformerMlp}}
\providecommand{\miouCITMflairShiftLR}{\tbd{miouCITMflairShiftLR}}
\providecommand{\miouCITMflairShiftLTwo}{\tbd{miouCITMflairShiftLTwo}}
\providecommand{\miouCITMflairShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{miouCITMflairShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouCITMflairShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouCITMflairShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouCITMflairShiftLTwoVarDecoderSamLite}{\tbd{miouCITMflairShiftLTwoVarDecoderSamLite}}
\providecommand{\miouCITMflairShiftLTwoVarDecoderSamPretrained}{\tbd{miouCITMflairShiftLTwoVarDecoderSamPretrained}}
\providecommand{\miouCITMflairShiftLTwoVarDecoderSegformerMlp}{\tbd{miouCITMflairShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouCITMflairShiftLTwoVarFrozenEncoderTrue}{\tbd{miouCITMflairShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\miouCITMflairShiftLTwoVarLossBootstrap}{\tbd{miouCITMflairShiftLTwoVarLossBootstrap}}
\providecommand{\miouCITMflairShiftLTwoVarLossGce}{\tbd{miouCITMflairShiftLTwoVarLossGce}}
\providecommand{\miouCITMflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouCITMflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouCITMflairShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouCITMflairShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouCITMsenClean}{\tbd{miouCITMsenClean}}
\providecommand{\miouCITMsenOtsuLTwo}{\tbd{miouCITMsenOtsuLTwo}}
\providecommand{\miouCIVitlRandomburnBoundaryLOneVarInitRandom}{\tbd{miouCIVitlRandomburnBoundaryLOneVarInitRandom}}
\providecommand{\miouCIVitlRandomburnBoundaryLTwoVarInitRandom}{\tbd{miouCIVitlRandomburnBoundaryLTwoVarInitRandom}}
\providecommand{\miouCIVitlRandomburnCleanVarInitRandom}{\tbd{miouCIVitlRandomburnCleanVarInitRandom}}
\providecommand{\miouCIVitlRandomburnCleanVarInitRandomLrMultOneZero}{\tbd{miouCIVitlRandomburnCleanVarInitRandomLrMultOneZero}}
\providecommand{\miouCIVitlRandomburnCleanVarInitRandomLrMultThree}{\tbd{miouCIVitlRandomburnCleanVarInitRandomLrMultThree}}
\providecommand{\miouCIVitlRandomburnCleanVarInitRandomTrainSubsetCleanTwoFive}{\tbd{miouCIVitlRandomburnCleanVarInitRandomTrainSubsetCleanTwoFive}}
\providecommand{\miouCIVitlRandomburnCoarseLOneVarInitRandom}{\tbd{miouCIVitlRandomburnCoarseLOneVarInitRandom}}
\providecommand{\miouCIVitlRandomburnCoarseLTwoVarInitRandom}{\tbd{miouCIVitlRandomburnCoarseLTwoVarInitRandom}}
\providecommand{\miouCIVitlRandomburnOmissionLOneVarInitRandom}{\tbd{miouCIVitlRandomburnOmissionLOneVarInitRandom}}
\providecommand{\miouCIVitlRandomburnOmissionLTwoVarInitRandom}{\tbd{miouCIVitlRandomburnOmissionLTwoVarInitRandom}}
\providecommand{\miouCIVitlRandomburnShiftLOneVarInitRandom}{\tbd{miouCIVitlRandomburnShiftLOneVarInitRandom}}
\providecommand{\miouCIVitlRandomburnShiftLTwoVarInitRandom}{\tbd{miouCIVitlRandomburnShiftLTwoVarInitRandom}}
\providecommand{\miouCIVitlRandomflairBoundaryLOneVarInitRandom}{\tbd{miouCIVitlRandomflairBoundaryLOneVarInitRandom}}
\providecommand{\miouCIVitlRandomflairBoundaryLTwoVarInitRandom}{\tbd{miouCIVitlRandomflairBoundaryLTwoVarInitRandom}}
\providecommand{\miouCIVitlRandomflairCleanVarInitRandom}{\tbd{miouCIVitlRandomflairCleanVarInitRandom}}
\providecommand{\miouCIVitlRandomflairCleanVarInitRandomLrMultOne}{\tbd{miouCIVitlRandomflairCleanVarInitRandomLrMultOne}}
\providecommand{\miouCIVitlRandomflairCleanVarInitRandomLrMultOneZero}{\tbd{miouCIVitlRandomflairCleanVarInitRandomLrMultOneZero}}
\providecommand{\miouCIVitlRandomflairCleanVarInitRandomTrainSubsetCleanTwoFive}{\tbd{miouCIVitlRandomflairCleanVarInitRandomTrainSubsetCleanTwoFive}}
\providecommand{\miouCIVitlRandomflairCoarseLOneVarInitRandom}{\tbd{miouCIVitlRandomflairCoarseLOneVarInitRandom}}
\providecommand{\miouCIVitlRandomflairCoarseLTwoVarInitRandom}{\tbd{miouCIVitlRandomflairCoarseLTwoVarInitRandom}}
\providecommand{\miouCIVitlRandomflairOmissionLOneVarInitRandom}{\tbd{miouCIVitlRandomflairOmissionLOneVarInitRandom}}
\providecommand{\miouCIVitlRandomflairOmissionLTwoVarInitRandom}{\tbd{miouCIVitlRandomflairOmissionLTwoVarInitRandom}}
\providecommand{\miouCIVitlRandomflairShiftLOneVarInitRandom}{\tbd{miouCIVitlRandomflairShiftLOneVarInitRandom}}
\providecommand{\miouCIVitlRandomflairShiftLTwoVarInitRandom}{\tbd{miouCIVitlRandomflairShiftLTwoVarInitRandom}}
\providecommand{\miouCNXLburnClean}{\tbd{miouCNXLburnClean}}
\providecommand{\miouCNXLflairClean}{\tbd{miouCNXLflairClean}}
\providecommand{\miouDOFAChesBoundaryLOne}{\tbd{miouDOFAChesBoundaryLOne}}
\providecommand{\miouDOFAChesBoundaryLTwo}{\tbd{miouDOFAChesBoundaryLTwo}}
\providecommand{\miouDOFAChesClean}{\tbd{miouDOFAChesClean}}
\providecommand{\miouDOFAChesCoarseLOne}{\tbd{miouDOFAChesCoarseLOne}}
\providecommand{\miouDOFAChesCoarseLTwo}{\tbd{miouDOFAChesCoarseLTwo}}
\providecommand{\miouDOFAChesNlcdREAL}{\tbd{miouDOFAChesNlcdREAL}}
\providecommand{\miouDOFAChesOmissionLOne}{\tbd{miouDOFAChesOmissionLOne}}
\providecommand{\miouDOFAChesOmissionLTwo}{\tbd{miouDOFAChesOmissionLTwo}}
\providecommand{\miouDOFAChesShiftLOne}{\tbd{miouDOFAChesShiftLOne}}
\providecommand{\miouDOFAChesShiftLTwo}{\tbd{miouDOFAChesShiftLTwo}}
\providecommand{\miouDOFACsTwelveBoundaryLOne}{\tbd{miouDOFACsTwelveBoundaryLOne}}
\providecommand{\miouDOFACsTwelveBoundaryLTwo}{\tbd{miouDOFACsTwelveBoundaryLTwo}}
\providecommand{\miouDOFACsTwelveClean}{\tbd{miouDOFACsTwelveClean}}
\providecommand{\miouDOFACsTwelveCoarseLOne}{\tbd{miouDOFACsTwelveCoarseLOne}}
\providecommand{\miouDOFACsTwelveCoarseLTwo}{\tbd{miouDOFACsTwelveCoarseLTwo}}
\providecommand{\miouDOFACsTwelveOmissionLOne}{\tbd{miouDOFACsTwelveOmissionLOne}}
\providecommand{\miouDOFACsTwelveOmissionLTwo}{\tbd{miouDOFACsTwelveOmissionLTwo}}
\providecommand{\miouDOFACsTwelveSTwocloudlessREAL}{\tbd{miouDOFACsTwelveSTwocloudlessREAL}}
\providecommand{\miouDOFACsTwelveShiftLOne}{\tbd{miouDOFACsTwelveShiftLOne}}
\providecommand{\miouDOFACsTwelveShiftLTwo}{\tbd{miouDOFACsTwelveShiftLTwo}}
\providecommand{\miouDOFADfcBoundaryLOne}{\tbd{miouDOFADfcBoundaryLOne}}
\providecommand{\miouDOFADfcBoundaryLTwo}{\tbd{miouDOFADfcBoundaryLTwo}}
\providecommand{\miouDOFADfcClean}{\tbd{miouDOFADfcClean}}
\providecommand{\miouDOFADfcCleanVarTrainSubsetRealcov}{\tbd{miouDOFADfcCleanVarTrainSubsetRealcov}}
\providecommand{\miouDOFADfcCoarseLOne}{\tbd{miouDOFADfcCoarseLOne}}
\providecommand{\miouDOFADfcCoarseLTwo}{\tbd{miouDOFADfcCoarseLTwo}}
\providecommand{\miouDOFADfcModisREALVarTrainSubsetRealcov}{\tbd{miouDOFADfcModisREALVarTrainSubsetRealcov}}
\providecommand{\miouDOFADfcOmissionLOne}{\tbd{miouDOFADfcOmissionLOne}}
\providecommand{\miouDOFADfcOmissionLTwo}{\tbd{miouDOFADfcOmissionLTwo}}
\providecommand{\miouDOFADfcShiftLOne}{\tbd{miouDOFADfcShiftLOne}}
\providecommand{\miouDOFADfcShiftLTwo}{\tbd{miouDOFADfcShiftLTwo}}
\providecommand{\miouDOFAEnvaBoundaryLOne}{\tbd{miouDOFAEnvaBoundaryLOne}}
\providecommand{\miouDOFAEnvaBoundaryLTwo}{\tbd{miouDOFAEnvaBoundaryLTwo}}
\providecommand{\miouDOFAEnvaClean}{\tbd{miouDOFAEnvaClean}}
\providecommand{\miouDOFAEnvaCoarseLOne}{\tbd{miouDOFAEnvaCoarseLOne}}
\providecommand{\miouDOFAEnvaCoarseLTwo}{\tbd{miouDOFAEnvaCoarseLTwo}}
\providecommand{\miouDOFAEnvaNlcdREAL}{\tbd{miouDOFAEnvaNlcdREAL}}
\providecommand{\miouDOFAEnvaOmissionLOne}{\tbd{miouDOFAEnvaOmissionLOne}}
\providecommand{\miouDOFAEnvaOmissionLTwo}{\tbd{miouDOFAEnvaOmissionLTwo}}
\providecommand{\miouDOFAEnvaShiftLOne}{\tbd{miouDOFAEnvaShiftLOne}}
\providecommand{\miouDOFAEnvaShiftLTwo}{\tbd{miouDOFAEnvaShiftLTwo}}
\providecommand{\miouDOFAKuroBoundaryLOne}{\tbd{miouDOFAKuroBoundaryLOne}}
\providecommand{\miouDOFAKuroBoundaryLTwo}{\tbd{miouDOFAKuroBoundaryLTwo}}
\providecommand{\miouDOFAKuroCemsREALVarTrainSubsetRealcov}{\tbd{miouDOFAKuroCemsREALVarTrainSubsetRealcov}}
\providecommand{\miouDOFAKuroClean}{\tbd{miouDOFAKuroClean}}
\providecommand{\miouDOFAKuroCleanVarTrainSubsetRealcov}{\tbd{miouDOFAKuroCleanVarTrainSubsetRealcov}}
\providecommand{\miouDOFAKuroCoarseLOne}{\tbd{miouDOFAKuroCoarseLOne}}
\providecommand{\miouDOFAKuroCoarseLTwo}{\tbd{miouDOFAKuroCoarseLTwo}}
\providecommand{\miouDOFAKuroOmissionLOne}{\tbd{miouDOFAKuroOmissionLOne}}
\providecommand{\miouDOFAKuroOmissionLTwo}{\tbd{miouDOFAKuroOmissionLTwo}}
\providecommand{\miouDOFAKuroShiftLOne}{\tbd{miouDOFAKuroShiftLOne}}
\providecommand{\miouDOFAKuroShiftLTwo}{\tbd{miouDOFAKuroShiftLTwo}}
\providecommand{\miouDOFAOemBoundaryLOne}{\tbd{miouDOFAOemBoundaryLOne}}
\providecommand{\miouDOFAOemBoundaryLTwo}{\tbd{miouDOFAOemBoundaryLTwo}}
\providecommand{\miouDOFAOemClean}{\tbd{miouDOFAOemClean}}
\providecommand{\miouDOFAOemCoarseLOne}{\tbd{miouDOFAOemCoarseLOne}}
\providecommand{\miouDOFAOemCoarseLTwo}{\tbd{miouDOFAOemCoarseLTwo}}
\providecommand{\miouDOFAOemOmissionLOne}{\tbd{miouDOFAOemOmissionLOne}}
\providecommand{\miouDOFAOemOmissionLTwo}{\tbd{miouDOFAOemOmissionLTwo}}
\providecommand{\miouDOFAOemShiftLOne}{\tbd{miouDOFAOemShiftLOne}}
\providecommand{\miouDOFAOemShiftLTwo}{\tbd{miouDOFAOemShiftLTwo}}
\providecommand{\miouDOFASnTwoBoundaryLOne}{\tbd{miouDOFASnTwoBoundaryLOne}}
\providecommand{\miouDOFASnTwoBoundaryLTwo}{\tbd{miouDOFASnTwoBoundaryLTwo}}
\providecommand{\miouDOFASnTwoClean}{\tbd{miouDOFASnTwoClean}}
\providecommand{\miouDOFASnTwoCoarseLOne}{\tbd{miouDOFASnTwoCoarseLOne}}
\providecommand{\miouDOFASnTwoCoarseLTwo}{\tbd{miouDOFASnTwoCoarseLTwo}}
\providecommand{\miouDOFASnTwoOmissionLOne}{\tbd{miouDOFASnTwoOmissionLOne}}
\providecommand{\miouDOFASnTwoOmissionLTwo}{\tbd{miouDOFASnTwoOmissionLTwo}}
\providecommand{\miouDOFASnTwoShiftLOne}{\tbd{miouDOFASnTwoShiftLOne}}
\providecommand{\miouDOFASnTwoShiftLTwo}{\tbd{miouDOFASnTwoShiftLTwo}}
\providecommand{\miouDOFAburnBoundaryLOne}{\tbd{miouDOFAburnBoundaryLOne}}
\providecommand{\miouDOFAburnBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{miouDOFAburnBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouDOFAburnBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{miouDOFAburnBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouDOFAburnBoundaryLOneVarDecoderSamLite}{\tbd{miouDOFAburnBoundaryLOneVarDecoderSamLite}}
\providecommand{\miouDOFAburnBoundaryLOneVarDecoderSamPretrained}{\tbd{miouDOFAburnBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\miouDOFAburnBoundaryLOneVarDecoderSegformerMlp}{\tbd{miouDOFAburnBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\miouDOFAburnBoundaryLR}{\tbd{miouDOFAburnBoundaryLR}}
\providecommand{\miouDOFAburnBoundaryLTwo}{\tbd{miouDOFAburnBoundaryLTwo}}
\providecommand{\miouDOFAburnBoundaryLTwoVarBandsRgb}{\tbd{miouDOFAburnBoundaryLTwoVarBandsRgb}}
\providecommand{\miouDOFAburnBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{miouDOFAburnBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouDOFAburnBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouDOFAburnBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouDOFAburnBoundaryLTwoVarDecoderSamLite}{\tbd{miouDOFAburnBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouDOFAburnBoundaryLTwoVarDecoderSamPretrained}{\tbd{miouDOFAburnBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\miouDOFAburnBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouDOFAburnBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouDOFAburnBoundaryLTwoVarFrozenEncoderTrue}{\tbd{miouDOFAburnBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\miouDOFAburnBoundaryLTwoVarLossBootstrap}{\tbd{miouDOFAburnBoundaryLTwoVarLossBootstrap}}
\providecommand{\miouDOFAburnBoundaryLTwoVarLossGce}{\tbd{miouDOFAburnBoundaryLTwoVarLossGce}}
\providecommand{\miouDOFAburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouDOFAburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouDOFAburnBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouDOFAburnBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouDOFAburnClean}{\tbd{miouDOFAburnClean}}
\providecommand{\miouDOFAburnCleanVarBandsRgb}{\tbd{miouDOFAburnCleanVarBandsRgb}}
\providecommand{\miouDOFAburnCleanVarDecoderMaskTwoformerFull}{\tbd{miouDOFAburnCleanVarDecoderMaskTwoformerFull}}
\providecommand{\miouDOFAburnCleanVarDecoderMaskTwoformerLite}{\tbd{miouDOFAburnCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouDOFAburnCleanVarDecoderSamLite}{\tbd{miouDOFAburnCleanVarDecoderSamLite}}
\providecommand{\miouDOFAburnCleanVarDecoderSamPretrained}{\tbd{miouDOFAburnCleanVarDecoderSamPretrained}}
\providecommand{\miouDOFAburnCleanVarDecoderSegformerMlp}{\tbd{miouDOFAburnCleanVarDecoderSegformerMlp}}
\providecommand{\miouDOFAburnCleanVarFrozenEncoderTrue}{\tbd{miouDOFAburnCleanVarFrozenEncoderTrue}}
\providecommand{\miouDOFAburnCleanVarLossBootstrap}{\tbd{miouDOFAburnCleanVarLossBootstrap}}
\providecommand{\miouDOFAburnCleanVarLossGce}{\tbd{miouDOFAburnCleanVarLossGce}}
\providecommand{\miouDOFAburnCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{miouDOFAburnCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouDOFAburnCleanVarTrainSubsetCleanTwoFive}{\tbd{miouDOFAburnCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\miouDOFAburnCoarseLOne}{\tbd{miouDOFAburnCoarseLOne}}
\providecommand{\miouDOFAburnCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{miouDOFAburnCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouDOFAburnCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{miouDOFAburnCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouDOFAburnCoarseLOneVarDecoderSamLite}{\tbd{miouDOFAburnCoarseLOneVarDecoderSamLite}}
\providecommand{\miouDOFAburnCoarseLOneVarDecoderSamPretrained}{\tbd{miouDOFAburnCoarseLOneVarDecoderSamPretrained}}
\providecommand{\miouDOFAburnCoarseLOneVarDecoderSegformerMlp}{\tbd{miouDOFAburnCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\miouDOFAburnCoarseLR}{\tbd{miouDOFAburnCoarseLR}}
\providecommand{\miouDOFAburnCoarseLTwo}{\tbd{miouDOFAburnCoarseLTwo}}
\providecommand{\miouDOFAburnCoarseLTwoVarBandsRgb}{\tbd{miouDOFAburnCoarseLTwoVarBandsRgb}}
\providecommand{\miouDOFAburnCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{miouDOFAburnCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouDOFAburnCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouDOFAburnCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouDOFAburnCoarseLTwoVarDecoderSamLite}{\tbd{miouDOFAburnCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouDOFAburnCoarseLTwoVarDecoderSamPretrained}{\tbd{miouDOFAburnCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\miouDOFAburnCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouDOFAburnCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouDOFAburnCoarseLTwoVarFrozenEncoderTrue}{\tbd{miouDOFAburnCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\miouDOFAburnCoarseLTwoVarLossBootstrap}{\tbd{miouDOFAburnCoarseLTwoVarLossBootstrap}}
\providecommand{\miouDOFAburnCoarseLTwoVarLossGce}{\tbd{miouDOFAburnCoarseLTwoVarLossGce}}
\providecommand{\miouDOFAburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouDOFAburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouDOFAburnCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouDOFAburnCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouDOFAburnOmissionLOne}{\tbd{miouDOFAburnOmissionLOne}}
\providecommand{\miouDOFAburnOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{miouDOFAburnOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouDOFAburnOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{miouDOFAburnOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouDOFAburnOmissionLOneVarDecoderSamLite}{\tbd{miouDOFAburnOmissionLOneVarDecoderSamLite}}
\providecommand{\miouDOFAburnOmissionLOneVarDecoderSamPretrained}{\tbd{miouDOFAburnOmissionLOneVarDecoderSamPretrained}}
\providecommand{\miouDOFAburnOmissionLOneVarDecoderSegformerMlp}{\tbd{miouDOFAburnOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\miouDOFAburnOmissionLR}{\tbd{miouDOFAburnOmissionLR}}
\providecommand{\miouDOFAburnOmissionLTwo}{\tbd{miouDOFAburnOmissionLTwo}}
\providecommand{\miouDOFAburnOmissionLTwoVarBandsRgb}{\tbd{miouDOFAburnOmissionLTwoVarBandsRgb}}
\providecommand{\miouDOFAburnOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{miouDOFAburnOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouDOFAburnOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouDOFAburnOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouDOFAburnOmissionLTwoVarDecoderSamLite}{\tbd{miouDOFAburnOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouDOFAburnOmissionLTwoVarDecoderSamPretrained}{\tbd{miouDOFAburnOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\miouDOFAburnOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouDOFAburnOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouDOFAburnOmissionLTwoVarFrozenEncoderTrue}{\tbd{miouDOFAburnOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\miouDOFAburnOmissionLTwoVarLossBootstrap}{\tbd{miouDOFAburnOmissionLTwoVarLossBootstrap}}
\providecommand{\miouDOFAburnOmissionLTwoVarLossGce}{\tbd{miouDOFAburnOmissionLTwoVarLossGce}}
\providecommand{\miouDOFAburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouDOFAburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouDOFAburnOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouDOFAburnOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouDOFAburnShiftLOne}{\tbd{miouDOFAburnShiftLOne}}
\providecommand{\miouDOFAburnShiftLOneVarDecoderMaskTwoformerFull}{\tbd{miouDOFAburnShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouDOFAburnShiftLOneVarDecoderMaskTwoformerLite}{\tbd{miouDOFAburnShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouDOFAburnShiftLOneVarDecoderSamLite}{\tbd{miouDOFAburnShiftLOneVarDecoderSamLite}}
\providecommand{\miouDOFAburnShiftLOneVarDecoderSamPretrained}{\tbd{miouDOFAburnShiftLOneVarDecoderSamPretrained}}
\providecommand{\miouDOFAburnShiftLOneVarDecoderSegformerMlp}{\tbd{miouDOFAburnShiftLOneVarDecoderSegformerMlp}}
\providecommand{\miouDOFAburnShiftLR}{\tbd{miouDOFAburnShiftLR}}
\providecommand{\miouDOFAburnShiftLTwo}{\tbd{miouDOFAburnShiftLTwo}}
\providecommand{\miouDOFAburnShiftLTwoVarBandsRgb}{\tbd{miouDOFAburnShiftLTwoVarBandsRgb}}
\providecommand{\miouDOFAburnShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{miouDOFAburnShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouDOFAburnShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouDOFAburnShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouDOFAburnShiftLTwoVarDecoderSamLite}{\tbd{miouDOFAburnShiftLTwoVarDecoderSamLite}}
\providecommand{\miouDOFAburnShiftLTwoVarDecoderSamPretrained}{\tbd{miouDOFAburnShiftLTwoVarDecoderSamPretrained}}
\providecommand{\miouDOFAburnShiftLTwoVarDecoderSegformerMlp}{\tbd{miouDOFAburnShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouDOFAburnShiftLTwoVarFrozenEncoderTrue}{\tbd{miouDOFAburnShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\miouDOFAburnShiftLTwoVarLossBootstrap}{\tbd{miouDOFAburnShiftLTwoVarLossBootstrap}}
\providecommand{\miouDOFAburnShiftLTwoVarLossGce}{\tbd{miouDOFAburnShiftLTwoVarLossGce}}
\providecommand{\miouDOFAburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouDOFAburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouDOFAburnShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouDOFAburnShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouDOFAflairBoundaryLOne}{\tbd{miouDOFAflairBoundaryLOne}}
\providecommand{\miouDOFAflairBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{miouDOFAflairBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouDOFAflairBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{miouDOFAflairBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouDOFAflairBoundaryLOneVarDecoderSamLite}{\tbd{miouDOFAflairBoundaryLOneVarDecoderSamLite}}
\providecommand{\miouDOFAflairBoundaryLOneVarDecoderSamPretrained}{\tbd{miouDOFAflairBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\miouDOFAflairBoundaryLOneVarDecoderSegformerMlp}{\tbd{miouDOFAflairBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\miouDOFAflairBoundaryLR}{\tbd{miouDOFAflairBoundaryLR}}
\providecommand{\miouDOFAflairBoundaryLTwo}{\tbd{miouDOFAflairBoundaryLTwo}}
\providecommand{\miouDOFAflairBoundaryLTwoVarBandsRgb}{\tbd{miouDOFAflairBoundaryLTwoVarBandsRgb}}
\providecommand{\miouDOFAflairBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{miouDOFAflairBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouDOFAflairBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouDOFAflairBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouDOFAflairBoundaryLTwoVarDecoderSamLite}{\tbd{miouDOFAflairBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouDOFAflairBoundaryLTwoVarDecoderSamPretrained}{\tbd{miouDOFAflairBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\miouDOFAflairBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouDOFAflairBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouDOFAflairBoundaryLTwoVarFrozenEncoderTrue}{\tbd{miouDOFAflairBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\miouDOFAflairBoundaryLTwoVarLossBootstrap}{\tbd{miouDOFAflairBoundaryLTwoVarLossBootstrap}}
\providecommand{\miouDOFAflairBoundaryLTwoVarLossGce}{\tbd{miouDOFAflairBoundaryLTwoVarLossGce}}
\providecommand{\miouDOFAflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouDOFAflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouDOFAflairBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouDOFAflairBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouDOFAflairClean}{\tbd{miouDOFAflairClean}}
\providecommand{\miouDOFAflairCleanVarBandsRgb}{\tbd{miouDOFAflairCleanVarBandsRgb}}
\providecommand{\miouDOFAflairCleanVarDecoderMaskTwoformerFull}{\tbd{miouDOFAflairCleanVarDecoderMaskTwoformerFull}}
\providecommand{\miouDOFAflairCleanVarDecoderMaskTwoformerLite}{\tbd{miouDOFAflairCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouDOFAflairCleanVarDecoderSamLite}{\tbd{miouDOFAflairCleanVarDecoderSamLite}}
\providecommand{\miouDOFAflairCleanVarDecoderSamPretrained}{\tbd{miouDOFAflairCleanVarDecoderSamPretrained}}
\providecommand{\miouDOFAflairCleanVarDecoderSegformerMlp}{\tbd{miouDOFAflairCleanVarDecoderSegformerMlp}}
\providecommand{\miouDOFAflairCleanVarFrozenEncoderTrue}{\tbd{miouDOFAflairCleanVarFrozenEncoderTrue}}
\providecommand{\miouDOFAflairCleanVarLossBootstrap}{\tbd{miouDOFAflairCleanVarLossBootstrap}}
\providecommand{\miouDOFAflairCleanVarLossGce}{\tbd{miouDOFAflairCleanVarLossGce}}
\providecommand{\miouDOFAflairCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{miouDOFAflairCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouDOFAflairCleanVarTrainSubsetCleanTwoFive}{\tbd{miouDOFAflairCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\miouDOFAflairCoarseLOne}{\tbd{miouDOFAflairCoarseLOne}}
\providecommand{\miouDOFAflairCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{miouDOFAflairCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouDOFAflairCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{miouDOFAflairCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouDOFAflairCoarseLOneVarDecoderSamLite}{\tbd{miouDOFAflairCoarseLOneVarDecoderSamLite}}
\providecommand{\miouDOFAflairCoarseLOneVarDecoderSamPretrained}{\tbd{miouDOFAflairCoarseLOneVarDecoderSamPretrained}}
\providecommand{\miouDOFAflairCoarseLOneVarDecoderSegformerMlp}{\tbd{miouDOFAflairCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\miouDOFAflairCoarseLR}{\tbd{miouDOFAflairCoarseLR}}
\providecommand{\miouDOFAflairCoarseLTwo}{\tbd{miouDOFAflairCoarseLTwo}}
\providecommand{\miouDOFAflairCoarseLTwoVarBandsRgb}{\tbd{miouDOFAflairCoarseLTwoVarBandsRgb}}
\providecommand{\miouDOFAflairCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{miouDOFAflairCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouDOFAflairCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouDOFAflairCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouDOFAflairCoarseLTwoVarDecoderSamLite}{\tbd{miouDOFAflairCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouDOFAflairCoarseLTwoVarDecoderSamPretrained}{\tbd{miouDOFAflairCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\miouDOFAflairCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouDOFAflairCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouDOFAflairCoarseLTwoVarFrozenEncoderTrue}{\tbd{miouDOFAflairCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\miouDOFAflairCoarseLTwoVarLossBootstrap}{\tbd{miouDOFAflairCoarseLTwoVarLossBootstrap}}
\providecommand{\miouDOFAflairCoarseLTwoVarLossGce}{\tbd{miouDOFAflairCoarseLTwoVarLossGce}}
\providecommand{\miouDOFAflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouDOFAflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouDOFAflairCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouDOFAflairCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouDOFAflairOmissionLOne}{\tbd{miouDOFAflairOmissionLOne}}
\providecommand{\miouDOFAflairOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{miouDOFAflairOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouDOFAflairOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{miouDOFAflairOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouDOFAflairOmissionLOneVarDecoderSamLite}{\tbd{miouDOFAflairOmissionLOneVarDecoderSamLite}}
\providecommand{\miouDOFAflairOmissionLOneVarDecoderSamPretrained}{\tbd{miouDOFAflairOmissionLOneVarDecoderSamPretrained}}
\providecommand{\miouDOFAflairOmissionLOneVarDecoderSegformerMlp}{\tbd{miouDOFAflairOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\miouDOFAflairOmissionLR}{\tbd{miouDOFAflairOmissionLR}}
\providecommand{\miouDOFAflairOmissionLTwo}{\tbd{miouDOFAflairOmissionLTwo}}
\providecommand{\miouDOFAflairOmissionLTwoVarBandsRgb}{\tbd{miouDOFAflairOmissionLTwoVarBandsRgb}}
\providecommand{\miouDOFAflairOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{miouDOFAflairOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouDOFAflairOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouDOFAflairOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouDOFAflairOmissionLTwoVarDecoderSamLite}{\tbd{miouDOFAflairOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouDOFAflairOmissionLTwoVarDecoderSamPretrained}{\tbd{miouDOFAflairOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\miouDOFAflairOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouDOFAflairOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouDOFAflairOmissionLTwoVarFrozenEncoderTrue}{\tbd{miouDOFAflairOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\miouDOFAflairOmissionLTwoVarLossBootstrap}{\tbd{miouDOFAflairOmissionLTwoVarLossBootstrap}}
\providecommand{\miouDOFAflairOmissionLTwoVarLossGce}{\tbd{miouDOFAflairOmissionLTwoVarLossGce}}
\providecommand{\miouDOFAflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouDOFAflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouDOFAflairOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouDOFAflairOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouDOFAflairShiftLOne}{\tbd{miouDOFAflairShiftLOne}}
\providecommand{\miouDOFAflairShiftLOneVarDecoderMaskTwoformerFull}{\tbd{miouDOFAflairShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouDOFAflairShiftLOneVarDecoderMaskTwoformerLite}{\tbd{miouDOFAflairShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouDOFAflairShiftLOneVarDecoderSamLite}{\tbd{miouDOFAflairShiftLOneVarDecoderSamLite}}
\providecommand{\miouDOFAflairShiftLOneVarDecoderSamPretrained}{\tbd{miouDOFAflairShiftLOneVarDecoderSamPretrained}}
\providecommand{\miouDOFAflairShiftLOneVarDecoderSegformerMlp}{\tbd{miouDOFAflairShiftLOneVarDecoderSegformerMlp}}
\providecommand{\miouDOFAflairShiftLR}{\tbd{miouDOFAflairShiftLR}}
\providecommand{\miouDOFAflairShiftLTwo}{\tbd{miouDOFAflairShiftLTwo}}
\providecommand{\miouDOFAflairShiftLTwoVarBandsRgb}{\tbd{miouDOFAflairShiftLTwoVarBandsRgb}}
\providecommand{\miouDOFAflairShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{miouDOFAflairShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouDOFAflairShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouDOFAflairShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouDOFAflairShiftLTwoVarDecoderSamLite}{\tbd{miouDOFAflairShiftLTwoVarDecoderSamLite}}
\providecommand{\miouDOFAflairShiftLTwoVarDecoderSamPretrained}{\tbd{miouDOFAflairShiftLTwoVarDecoderSamPretrained}}
\providecommand{\miouDOFAflairShiftLTwoVarDecoderSegformerMlp}{\tbd{miouDOFAflairShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouDOFAflairShiftLTwoVarFrozenEncoderTrue}{\tbd{miouDOFAflairShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\miouDOFAflairShiftLTwoVarLossBootstrap}{\tbd{miouDOFAflairShiftLTwoVarLossBootstrap}}
\providecommand{\miouDOFAflairShiftLTwoVarLossGce}{\tbd{miouDOFAflairShiftLTwoVarLossGce}}
\providecommand{\miouDOFAflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouDOFAflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouDOFAflairShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouDOFAflairShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouDOFAsenClean}{\tbd{miouDOFAsenClean}}
\providecommand{\miouDOFAsenOtsuLTwo}{\tbd{miouDOFAsenOtsuLTwo}}
\providecommand{\miouDinovThreeConvnextLburnBoundaryLOne}{\tbd{miouDinovThreeConvnextLburnBoundaryLOne}}
\providecommand{\miouDinovThreeConvnextLburnBoundaryLTwo}{\tbd{miouDinovThreeConvnextLburnBoundaryLTwo}}
\providecommand{\miouDinovThreeConvnextLburnClean}{\tbd{miouDinovThreeConvnextLburnClean}}
\providecommand{\miouDinovThreeConvnextLburnCleanVarTrainSubsetCleanTwoFive}{\tbd{miouDinovThreeConvnextLburnCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\miouDinovThreeConvnextLburnCoarseLOne}{\tbd{miouDinovThreeConvnextLburnCoarseLOne}}
\providecommand{\miouDinovThreeConvnextLburnCoarseLTwo}{\tbd{miouDinovThreeConvnextLburnCoarseLTwo}}
\providecommand{\miouDinovThreeConvnextLburnOmissionLOne}{\tbd{miouDinovThreeConvnextLburnOmissionLOne}}
\providecommand{\miouDinovThreeConvnextLburnOmissionLTwo}{\tbd{miouDinovThreeConvnextLburnOmissionLTwo}}
\providecommand{\miouDinovThreeConvnextLburnShiftLOne}{\tbd{miouDinovThreeConvnextLburnShiftLOne}}
\providecommand{\miouDinovThreeConvnextLburnShiftLTwo}{\tbd{miouDinovThreeConvnextLburnShiftLTwo}}
\providecommand{\miouDinovThreeConvnextLflairBoundaryLOne}{\tbd{miouDinovThreeConvnextLflairBoundaryLOne}}
\providecommand{\miouDinovThreeConvnextLflairBoundaryLTwo}{\tbd{miouDinovThreeConvnextLflairBoundaryLTwo}}
\providecommand{\miouDinovThreeConvnextLflairClean}{\tbd{miouDinovThreeConvnextLflairClean}}
\providecommand{\miouDinovThreeConvnextLflairCleanVarTrainSubsetCleanTwoFive}{\tbd{miouDinovThreeConvnextLflairCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\miouDinovThreeConvnextLflairCoarseLOne}{\tbd{miouDinovThreeConvnextLflairCoarseLOne}}
\providecommand{\miouDinovThreeConvnextLflairCoarseLTwo}{\tbd{miouDinovThreeConvnextLflairCoarseLTwo}}
\providecommand{\miouDinovThreeConvnextLflairOmissionLOne}{\tbd{miouDinovThreeConvnextLflairOmissionLOne}}
\providecommand{\miouDinovThreeConvnextLflairOmissionLTwo}{\tbd{miouDinovThreeConvnextLflairOmissionLTwo}}
\providecommand{\miouDinovThreeConvnextLflairShiftLOne}{\tbd{miouDinovThreeConvnextLflairShiftLOne}}
\providecommand{\miouDinovThreeConvnextLflairShiftLTwo}{\tbd{miouDinovThreeConvnextLflairShiftLTwo}}
\providecommand{\miouLVDChesBoundaryLOne}{\tbd{miouLVDChesBoundaryLOne}}
\providecommand{\miouLVDChesBoundaryLTwo}{\tbd{miouLVDChesBoundaryLTwo}}
\providecommand{\miouLVDChesBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouLVDChesBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDChesBoundaryLTwoVarDecoderSamLite}{\tbd{miouLVDChesBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouLVDChesBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouLVDChesBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouLVDChesBoundaryLTwoVarLrMultOne}{\tbd{miouLVDChesBoundaryLTwoVarLrMultOne}}
\providecommand{\miouLVDChesClean}{\tbd{miouLVDChesClean}}
\providecommand{\miouLVDChesCleanVarDecoderMaskTwoformerLite}{\tbd{miouLVDChesCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDChesCleanVarDecoderSamLite}{\tbd{miouLVDChesCleanVarDecoderSamLite}}
\providecommand{\miouLVDChesCleanVarDecoderSegformerMlp}{\tbd{miouLVDChesCleanVarDecoderSegformerMlp}}
\providecommand{\miouLVDChesCleanVarLrMultOne}{\tbd{miouLVDChesCleanVarLrMultOne}}
\providecommand{\miouLVDChesCoarseLOne}{\tbd{miouLVDChesCoarseLOne}}
\providecommand{\miouLVDChesCoarseLTwo}{\tbd{miouLVDChesCoarseLTwo}}
\providecommand{\miouLVDChesCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouLVDChesCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDChesCoarseLTwoVarDecoderSamLite}{\tbd{miouLVDChesCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouLVDChesCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouLVDChesCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouLVDChesCoarseLTwoVarLrMultOne}{\tbd{miouLVDChesCoarseLTwoVarLrMultOne}}
\providecommand{\miouLVDChesNlcdREAL}{\tbd{miouLVDChesNlcdREAL}}
\providecommand{\miouLVDChesOmissionLOne}{\tbd{miouLVDChesOmissionLOne}}
\providecommand{\miouLVDChesOmissionLTwo}{\tbd{miouLVDChesOmissionLTwo}}
\providecommand{\miouLVDChesOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouLVDChesOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDChesOmissionLTwoVarDecoderSamLite}{\tbd{miouLVDChesOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouLVDChesOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouLVDChesOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouLVDChesOmissionLTwoVarLrMultOne}{\tbd{miouLVDChesOmissionLTwoVarLrMultOne}}
\providecommand{\miouLVDChesShiftLOne}{\tbd{miouLVDChesShiftLOne}}
\providecommand{\miouLVDChesShiftLTwo}{\tbd{miouLVDChesShiftLTwo}}
\providecommand{\miouLVDChesShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouLVDChesShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDChesShiftLTwoVarDecoderSamLite}{\tbd{miouLVDChesShiftLTwoVarDecoderSamLite}}
\providecommand{\miouLVDChesShiftLTwoVarDecoderSegformerMlp}{\tbd{miouLVDChesShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouLVDChesShiftLTwoVarLrMultOne}{\tbd{miouLVDChesShiftLTwoVarLrMultOne}}
\providecommand{\miouLVDCsTwelveBoundaryLOne}{\tbd{miouLVDCsTwelveBoundaryLOne}}
\providecommand{\miouLVDCsTwelveBoundaryLTwo}{\tbd{miouLVDCsTwelveBoundaryLTwo}}
\providecommand{\miouLVDCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouLVDCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDCsTwelveBoundaryLTwoVarDecoderSamLite}{\tbd{miouLVDCsTwelveBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouLVDCsTwelveBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouLVDCsTwelveBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouLVDCsTwelveBoundaryLTwoVarLrMultOne}{\tbd{miouLVDCsTwelveBoundaryLTwoVarLrMultOne}}
\providecommand{\miouLVDCsTwelveClean}{\tbd{miouLVDCsTwelveClean}}
\providecommand{\miouLVDCsTwelveCleanVarDecoderMaskTwoformerLite}{\tbd{miouLVDCsTwelveCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDCsTwelveCleanVarDecoderSamLite}{\tbd{miouLVDCsTwelveCleanVarDecoderSamLite}}
\providecommand{\miouLVDCsTwelveCleanVarDecoderSegformerMlp}{\tbd{miouLVDCsTwelveCleanVarDecoderSegformerMlp}}
\providecommand{\miouLVDCsTwelveCleanVarLrMultOne}{\tbd{miouLVDCsTwelveCleanVarLrMultOne}}
\providecommand{\miouLVDCsTwelveCoarseLOne}{\tbd{miouLVDCsTwelveCoarseLOne}}
\providecommand{\miouLVDCsTwelveCoarseLTwo}{\tbd{miouLVDCsTwelveCoarseLTwo}}
\providecommand{\miouLVDCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouLVDCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDCsTwelveCoarseLTwoVarDecoderSamLite}{\tbd{miouLVDCsTwelveCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouLVDCsTwelveCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouLVDCsTwelveCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouLVDCsTwelveCoarseLTwoVarLrMultOne}{\tbd{miouLVDCsTwelveCoarseLTwoVarLrMultOne}}
\providecommand{\miouLVDCsTwelveOmissionLOne}{\tbd{miouLVDCsTwelveOmissionLOne}}
\providecommand{\miouLVDCsTwelveOmissionLTwo}{\tbd{miouLVDCsTwelveOmissionLTwo}}
\providecommand{\miouLVDCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouLVDCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDCsTwelveOmissionLTwoVarDecoderSamLite}{\tbd{miouLVDCsTwelveOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouLVDCsTwelveOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouLVDCsTwelveOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouLVDCsTwelveOmissionLTwoVarLrMultOne}{\tbd{miouLVDCsTwelveOmissionLTwoVarLrMultOne}}
\providecommand{\miouLVDCsTwelveSTwocloudlessREAL}{\tbd{miouLVDCsTwelveSTwocloudlessREAL}}
\providecommand{\miouLVDCsTwelveShiftLOne}{\tbd{miouLVDCsTwelveShiftLOne}}
\providecommand{\miouLVDCsTwelveShiftLTwo}{\tbd{miouLVDCsTwelveShiftLTwo}}
\providecommand{\miouLVDCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouLVDCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDCsTwelveShiftLTwoVarDecoderSamLite}{\tbd{miouLVDCsTwelveShiftLTwoVarDecoderSamLite}}
\providecommand{\miouLVDCsTwelveShiftLTwoVarDecoderSegformerMlp}{\tbd{miouLVDCsTwelveShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouLVDCsTwelveShiftLTwoVarLrMultOne}{\tbd{miouLVDCsTwelveShiftLTwoVarLrMultOne}}
\providecommand{\miouLVDDfcBoundaryLOne}{\tbd{miouLVDDfcBoundaryLOne}}
\providecommand{\miouLVDDfcBoundaryLTwo}{\tbd{miouLVDDfcBoundaryLTwo}}
\providecommand{\miouLVDDfcBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouLVDDfcBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDDfcBoundaryLTwoVarDecoderSamLite}{\tbd{miouLVDDfcBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouLVDDfcBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouLVDDfcBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouLVDDfcBoundaryLTwoVarLrMultOne}{\tbd{miouLVDDfcBoundaryLTwoVarLrMultOne}}
\providecommand{\miouLVDDfcClean}{\tbd{miouLVDDfcClean}}
\providecommand{\miouLVDDfcCleanVarDecoderMaskTwoformerLite}{\tbd{miouLVDDfcCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDDfcCleanVarDecoderSamLite}{\tbd{miouLVDDfcCleanVarDecoderSamLite}}
\providecommand{\miouLVDDfcCleanVarDecoderSegformerMlp}{\tbd{miouLVDDfcCleanVarDecoderSegformerMlp}}
\providecommand{\miouLVDDfcCleanVarLrMultOne}{\tbd{miouLVDDfcCleanVarLrMultOne}}
\providecommand{\miouLVDDfcCleanVarTrainSubsetRealcov}{\tbd{miouLVDDfcCleanVarTrainSubsetRealcov}}
\providecommand{\miouLVDDfcCoarseLOne}{\tbd{miouLVDDfcCoarseLOne}}
\providecommand{\miouLVDDfcCoarseLTwo}{\tbd{miouLVDDfcCoarseLTwo}}
\providecommand{\miouLVDDfcCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouLVDDfcCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDDfcCoarseLTwoVarDecoderSamLite}{\tbd{miouLVDDfcCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouLVDDfcCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouLVDDfcCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouLVDDfcCoarseLTwoVarLrMultOne}{\tbd{miouLVDDfcCoarseLTwoVarLrMultOne}}
\providecommand{\miouLVDDfcModisREALVarTrainSubsetRealcov}{\tbd{miouLVDDfcModisREALVarTrainSubsetRealcov}}
\providecommand{\miouLVDDfcOmissionLOne}{\tbd{miouLVDDfcOmissionLOne}}
\providecommand{\miouLVDDfcOmissionLTwo}{\tbd{miouLVDDfcOmissionLTwo}}
\providecommand{\miouLVDDfcOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouLVDDfcOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDDfcOmissionLTwoVarDecoderSamLite}{\tbd{miouLVDDfcOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouLVDDfcOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouLVDDfcOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouLVDDfcOmissionLTwoVarLrMultOne}{\tbd{miouLVDDfcOmissionLTwoVarLrMultOne}}
\providecommand{\miouLVDDfcShiftLOne}{\tbd{miouLVDDfcShiftLOne}}
\providecommand{\miouLVDDfcShiftLTwo}{\tbd{miouLVDDfcShiftLTwo}}
\providecommand{\miouLVDDfcShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouLVDDfcShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDDfcShiftLTwoVarDecoderSamLite}{\tbd{miouLVDDfcShiftLTwoVarDecoderSamLite}}
\providecommand{\miouLVDDfcShiftLTwoVarDecoderSegformerMlp}{\tbd{miouLVDDfcShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouLVDDfcShiftLTwoVarLrMultOne}{\tbd{miouLVDDfcShiftLTwoVarLrMultOne}}
\providecommand{\miouLVDEnvaBoundaryLOne}{\tbd{miouLVDEnvaBoundaryLOne}}
\providecommand{\miouLVDEnvaBoundaryLTwo}{\tbd{miouLVDEnvaBoundaryLTwo}}
\providecommand{\miouLVDEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouLVDEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDEnvaBoundaryLTwoVarDecoderSamLite}{\tbd{miouLVDEnvaBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouLVDEnvaBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouLVDEnvaBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouLVDEnvaBoundaryLTwoVarLrMultOne}{\tbd{miouLVDEnvaBoundaryLTwoVarLrMultOne}}
\providecommand{\miouLVDEnvaClean}{\tbd{miouLVDEnvaClean}}
\providecommand{\miouLVDEnvaCleanVarDecoderMaskTwoformerLite}{\tbd{miouLVDEnvaCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDEnvaCleanVarDecoderSamLite}{\tbd{miouLVDEnvaCleanVarDecoderSamLite}}
\providecommand{\miouLVDEnvaCleanVarDecoderSegformerMlp}{\tbd{miouLVDEnvaCleanVarDecoderSegformerMlp}}
\providecommand{\miouLVDEnvaCleanVarLrMultOne}{\tbd{miouLVDEnvaCleanVarLrMultOne}}
\providecommand{\miouLVDEnvaCoarseLOne}{\tbd{miouLVDEnvaCoarseLOne}}
\providecommand{\miouLVDEnvaCoarseLTwo}{\tbd{miouLVDEnvaCoarseLTwo}}
\providecommand{\miouLVDEnvaCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouLVDEnvaCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDEnvaCoarseLTwoVarDecoderSamLite}{\tbd{miouLVDEnvaCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouLVDEnvaCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouLVDEnvaCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouLVDEnvaCoarseLTwoVarLrMultOne}{\tbd{miouLVDEnvaCoarseLTwoVarLrMultOne}}
\providecommand{\miouLVDEnvaNlcdREAL}{\tbd{miouLVDEnvaNlcdREAL}}
\providecommand{\miouLVDEnvaOmissionLOne}{\tbd{miouLVDEnvaOmissionLOne}}
\providecommand{\miouLVDEnvaOmissionLTwo}{\tbd{miouLVDEnvaOmissionLTwo}}
\providecommand{\miouLVDEnvaOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouLVDEnvaOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDEnvaOmissionLTwoVarDecoderSamLite}{\tbd{miouLVDEnvaOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouLVDEnvaOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouLVDEnvaOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouLVDEnvaOmissionLTwoVarLrMultOne}{\tbd{miouLVDEnvaOmissionLTwoVarLrMultOne}}
\providecommand{\miouLVDEnvaShiftLOne}{\tbd{miouLVDEnvaShiftLOne}}
\providecommand{\miouLVDEnvaShiftLTwo}{\tbd{miouLVDEnvaShiftLTwo}}
\providecommand{\miouLVDEnvaShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouLVDEnvaShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDEnvaShiftLTwoVarDecoderSamLite}{\tbd{miouLVDEnvaShiftLTwoVarDecoderSamLite}}
\providecommand{\miouLVDEnvaShiftLTwoVarDecoderSegformerMlp}{\tbd{miouLVDEnvaShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouLVDEnvaShiftLTwoVarLrMultOne}{\tbd{miouLVDEnvaShiftLTwoVarLrMultOne}}
\providecommand{\miouLVDKuroBoundaryLOne}{\tbd{miouLVDKuroBoundaryLOne}}
\providecommand{\miouLVDKuroBoundaryLTwo}{\tbd{miouLVDKuroBoundaryLTwo}}
\providecommand{\miouLVDKuroBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouLVDKuroBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDKuroBoundaryLTwoVarDecoderSamLite}{\tbd{miouLVDKuroBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouLVDKuroBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouLVDKuroBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouLVDKuroBoundaryLTwoVarLrMultOne}{\tbd{miouLVDKuroBoundaryLTwoVarLrMultOne}}
\providecommand{\miouLVDKuroCemsREALVarTrainSubsetRealcov}{\tbd{miouLVDKuroCemsREALVarTrainSubsetRealcov}}
\providecommand{\miouLVDKuroClean}{\tbd{miouLVDKuroClean}}
\providecommand{\miouLVDKuroCleanVarDecoderMaskTwoformerLite}{\tbd{miouLVDKuroCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDKuroCleanVarDecoderSamLite}{\tbd{miouLVDKuroCleanVarDecoderSamLite}}
\providecommand{\miouLVDKuroCleanVarDecoderSegformerMlp}{\tbd{miouLVDKuroCleanVarDecoderSegformerMlp}}
\providecommand{\miouLVDKuroCleanVarLrMultOne}{\tbd{miouLVDKuroCleanVarLrMultOne}}
\providecommand{\miouLVDKuroCleanVarTrainSubsetRealcov}{\tbd{miouLVDKuroCleanVarTrainSubsetRealcov}}
\providecommand{\miouLVDKuroCoarseLOne}{\tbd{miouLVDKuroCoarseLOne}}
\providecommand{\miouLVDKuroCoarseLTwo}{\tbd{miouLVDKuroCoarseLTwo}}
\providecommand{\miouLVDKuroCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouLVDKuroCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDKuroCoarseLTwoVarDecoderSamLite}{\tbd{miouLVDKuroCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouLVDKuroCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouLVDKuroCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouLVDKuroCoarseLTwoVarLrMultOne}{\tbd{miouLVDKuroCoarseLTwoVarLrMultOne}}
\providecommand{\miouLVDKuroOmissionLOne}{\tbd{miouLVDKuroOmissionLOne}}
\providecommand{\miouLVDKuroOmissionLTwo}{\tbd{miouLVDKuroOmissionLTwo}}
\providecommand{\miouLVDKuroOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouLVDKuroOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDKuroOmissionLTwoVarDecoderSamLite}{\tbd{miouLVDKuroOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouLVDKuroOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouLVDKuroOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouLVDKuroOmissionLTwoVarLrMultOne}{\tbd{miouLVDKuroOmissionLTwoVarLrMultOne}}
\providecommand{\miouLVDKuroShiftLOne}{\tbd{miouLVDKuroShiftLOne}}
\providecommand{\miouLVDKuroShiftLTwo}{\tbd{miouLVDKuroShiftLTwo}}
\providecommand{\miouLVDKuroShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouLVDKuroShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDKuroShiftLTwoVarDecoderSamLite}{\tbd{miouLVDKuroShiftLTwoVarDecoderSamLite}}
\providecommand{\miouLVDKuroShiftLTwoVarDecoderSegformerMlp}{\tbd{miouLVDKuroShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouLVDKuroShiftLTwoVarLrMultOne}{\tbd{miouLVDKuroShiftLTwoVarLrMultOne}}
\providecommand{\miouLVDOemBoundaryLOne}{\tbd{miouLVDOemBoundaryLOne}}
\providecommand{\miouLVDOemBoundaryLTwo}{\tbd{miouLVDOemBoundaryLTwo}}
\providecommand{\miouLVDOemBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouLVDOemBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDOemBoundaryLTwoVarDecoderSamLite}{\tbd{miouLVDOemBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouLVDOemBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouLVDOemBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouLVDOemBoundaryLTwoVarLrMultOne}{\tbd{miouLVDOemBoundaryLTwoVarLrMultOne}}
\providecommand{\miouLVDOemClean}{\tbd{miouLVDOemClean}}
\providecommand{\miouLVDOemCleanVarDecoderMaskTwoformerLite}{\tbd{miouLVDOemCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDOemCleanVarDecoderSamLite}{\tbd{miouLVDOemCleanVarDecoderSamLite}}
\providecommand{\miouLVDOemCleanVarDecoderSegformerMlp}{\tbd{miouLVDOemCleanVarDecoderSegformerMlp}}
\providecommand{\miouLVDOemCleanVarLrMultOne}{\tbd{miouLVDOemCleanVarLrMultOne}}
\providecommand{\miouLVDOemCoarseLOne}{\tbd{miouLVDOemCoarseLOne}}
\providecommand{\miouLVDOemCoarseLTwo}{\tbd{miouLVDOemCoarseLTwo}}
\providecommand{\miouLVDOemCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouLVDOemCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDOemCoarseLTwoVarDecoderSamLite}{\tbd{miouLVDOemCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouLVDOemCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouLVDOemCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouLVDOemCoarseLTwoVarLrMultOne}{\tbd{miouLVDOemCoarseLTwoVarLrMultOne}}
\providecommand{\miouLVDOemOmissionLOne}{\tbd{miouLVDOemOmissionLOne}}
\providecommand{\miouLVDOemOmissionLTwo}{\tbd{miouLVDOemOmissionLTwo}}
\providecommand{\miouLVDOemOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouLVDOemOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDOemOmissionLTwoVarDecoderSamLite}{\tbd{miouLVDOemOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouLVDOemOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouLVDOemOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouLVDOemOmissionLTwoVarLrMultOne}{\tbd{miouLVDOemOmissionLTwoVarLrMultOne}}
\providecommand{\miouLVDOemShiftLOne}{\tbd{miouLVDOemShiftLOne}}
\providecommand{\miouLVDOemShiftLTwo}{\tbd{miouLVDOemShiftLTwo}}
\providecommand{\miouLVDOemShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouLVDOemShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDOemShiftLTwoVarDecoderSamLite}{\tbd{miouLVDOemShiftLTwoVarDecoderSamLite}}
\providecommand{\miouLVDOemShiftLTwoVarDecoderSegformerMlp}{\tbd{miouLVDOemShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouLVDOemShiftLTwoVarLrMultOne}{\tbd{miouLVDOemShiftLTwoVarLrMultOne}}
\providecommand{\miouLVDSnTwoBoundaryLOne}{\tbd{miouLVDSnTwoBoundaryLOne}}
\providecommand{\miouLVDSnTwoBoundaryLTwo}{\tbd{miouLVDSnTwoBoundaryLTwo}}
\providecommand{\miouLVDSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouLVDSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDSnTwoBoundaryLTwoVarDecoderSamLite}{\tbd{miouLVDSnTwoBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouLVDSnTwoBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouLVDSnTwoBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouLVDSnTwoBoundaryLTwoVarLrMultOne}{\tbd{miouLVDSnTwoBoundaryLTwoVarLrMultOne}}
\providecommand{\miouLVDSnTwoClean}{\tbd{miouLVDSnTwoClean}}
\providecommand{\miouLVDSnTwoCleanVarDecoderMaskTwoformerLite}{\tbd{miouLVDSnTwoCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDSnTwoCleanVarDecoderSamLite}{\tbd{miouLVDSnTwoCleanVarDecoderSamLite}}
\providecommand{\miouLVDSnTwoCleanVarDecoderSegformerMlp}{\tbd{miouLVDSnTwoCleanVarDecoderSegformerMlp}}
\providecommand{\miouLVDSnTwoCleanVarLrMultOne}{\tbd{miouLVDSnTwoCleanVarLrMultOne}}
\providecommand{\miouLVDSnTwoCoarseLOne}{\tbd{miouLVDSnTwoCoarseLOne}}
\providecommand{\miouLVDSnTwoCoarseLTwo}{\tbd{miouLVDSnTwoCoarseLTwo}}
\providecommand{\miouLVDSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouLVDSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDSnTwoCoarseLTwoVarDecoderSamLite}{\tbd{miouLVDSnTwoCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouLVDSnTwoCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouLVDSnTwoCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouLVDSnTwoCoarseLTwoVarLrMultOne}{\tbd{miouLVDSnTwoCoarseLTwoVarLrMultOne}}
\providecommand{\miouLVDSnTwoOmissionLOne}{\tbd{miouLVDSnTwoOmissionLOne}}
\providecommand{\miouLVDSnTwoOmissionLTwo}{\tbd{miouLVDSnTwoOmissionLTwo}}
\providecommand{\miouLVDSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouLVDSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDSnTwoOmissionLTwoVarDecoderSamLite}{\tbd{miouLVDSnTwoOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouLVDSnTwoOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouLVDSnTwoOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouLVDSnTwoOmissionLTwoVarLrMultOne}{\tbd{miouLVDSnTwoOmissionLTwoVarLrMultOne}}
\providecommand{\miouLVDSnTwoShiftLOne}{\tbd{miouLVDSnTwoShiftLOne}}
\providecommand{\miouLVDSnTwoShiftLTwo}{\tbd{miouLVDSnTwoShiftLTwo}}
\providecommand{\miouLVDSnTwoShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouLVDSnTwoShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDSnTwoShiftLTwoVarDecoderSamLite}{\tbd{miouLVDSnTwoShiftLTwoVarDecoderSamLite}}
\providecommand{\miouLVDSnTwoShiftLTwoVarDecoderSegformerMlp}{\tbd{miouLVDSnTwoShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouLVDSnTwoShiftLTwoVarLrMultOne}{\tbd{miouLVDSnTwoShiftLTwoVarLrMultOne}}
\providecommand{\miouLVDburnBoundaryLOne}{\tbd{miouLVDburnBoundaryLOne}}
\providecommand{\miouLVDburnBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{miouLVDburnBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouLVDburnBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{miouLVDburnBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDburnBoundaryLOneVarDecoderSamLite}{\tbd{miouLVDburnBoundaryLOneVarDecoderSamLite}}
\providecommand{\miouLVDburnBoundaryLOneVarDecoderSamPretrained}{\tbd{miouLVDburnBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\miouLVDburnBoundaryLOneVarDecoderSegformerMlp}{\tbd{miouLVDburnBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\miouLVDburnBoundaryLR}{\tbd{miouLVDburnBoundaryLR}}
\providecommand{\miouLVDburnBoundaryLRVarLrMultOne}{\tbd{miouLVDburnBoundaryLRVarLrMultOne}}
\providecommand{\miouLVDburnBoundaryLTwo}{\tbd{miouLVDburnBoundaryLTwo}}
\providecommand{\miouLVDburnBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{miouLVDburnBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouLVDburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{miouLVDburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\miouLVDburnBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouLVDburnBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{miouLVDburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\miouLVDburnBoundaryLTwoVarDecoderSamLite}{\tbd{miouLVDburnBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouLVDburnBoundaryLTwoVarDecoderSamLiteLrMultOne}{\tbd{miouLVDburnBoundaryLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\miouLVDburnBoundaryLTwoVarDecoderSamPretrained}{\tbd{miouLVDburnBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\miouLVDburnBoundaryLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{miouLVDburnBoundaryLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\miouLVDburnBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouLVDburnBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouLVDburnBoundaryLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{miouLVDburnBoundaryLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\miouLVDburnBoundaryLTwoVarLossBootstrap}{\tbd{miouLVDburnBoundaryLTwoVarLossBootstrap}}
\providecommand{\miouLVDburnBoundaryLTwoVarLossGce}{\tbd{miouLVDburnBoundaryLTwoVarLossGce}}
\providecommand{\miouLVDburnBoundaryLTwoVarLrMultOne}{\tbd{miouLVDburnBoundaryLTwoVarLrMultOne}}
\providecommand{\miouLVDburnBoundaryLTwoVarLrMultThree}{\tbd{miouLVDburnBoundaryLTwoVarLrMultThree}}
\providecommand{\miouLVDburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouLVDburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouLVDburnBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouLVDburnBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouLVDburnClean}{\tbd{miouLVDburnClean}}
\providecommand{\miouLVDburnCleanVarDecoderMaskTwoformerFull}{\tbd{miouLVDburnCleanVarDecoderMaskTwoformerFull}}
\providecommand{\miouLVDburnCleanVarDecoderMaskTwoformerFullLrMultOne}{\tbd{miouLVDburnCleanVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\miouLVDburnCleanVarDecoderMaskTwoformerLite}{\tbd{miouLVDburnCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDburnCleanVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{miouLVDburnCleanVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\miouLVDburnCleanVarDecoderSamLite}{\tbd{miouLVDburnCleanVarDecoderSamLite}}
\providecommand{\miouLVDburnCleanVarDecoderSamLiteLrMultOne}{\tbd{miouLVDburnCleanVarDecoderSamLiteLrMultOne}}
\providecommand{\miouLVDburnCleanVarDecoderSamPretrained}{\tbd{miouLVDburnCleanVarDecoderSamPretrained}}
\providecommand{\miouLVDburnCleanVarDecoderSamPretrainedLrMultOne}{\tbd{miouLVDburnCleanVarDecoderSamPretrainedLrMultOne}}
\providecommand{\miouLVDburnCleanVarDecoderSegformerMlp}{\tbd{miouLVDburnCleanVarDecoderSegformerMlp}}
\providecommand{\miouLVDburnCleanVarDecoderSegformerMlpLrMultOne}{\tbd{miouLVDburnCleanVarDecoderSegformerMlpLrMultOne}}
\providecommand{\miouLVDburnCleanVarLossBootstrap}{\tbd{miouLVDburnCleanVarLossBootstrap}}
\providecommand{\miouLVDburnCleanVarLossGce}{\tbd{miouLVDburnCleanVarLossGce}}
\providecommand{\miouLVDburnCleanVarLrMultOne}{\tbd{miouLVDburnCleanVarLrMultOne}}
\providecommand{\miouLVDburnCleanVarLrMultThree}{\tbd{miouLVDburnCleanVarLrMultThree}}
\providecommand{\miouLVDburnCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{miouLVDburnCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouLVDburnCleanVarTrainSubsetCleanTwoFive}{\tbd{miouLVDburnCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\miouLVDburnCoarseLOne}{\tbd{miouLVDburnCoarseLOne}}
\providecommand{\miouLVDburnCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{miouLVDburnCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouLVDburnCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{miouLVDburnCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDburnCoarseLOneVarDecoderSamLite}{\tbd{miouLVDburnCoarseLOneVarDecoderSamLite}}
\providecommand{\miouLVDburnCoarseLOneVarDecoderSamPretrained}{\tbd{miouLVDburnCoarseLOneVarDecoderSamPretrained}}
\providecommand{\miouLVDburnCoarseLOneVarDecoderSegformerMlp}{\tbd{miouLVDburnCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\miouLVDburnCoarseLR}{\tbd{miouLVDburnCoarseLR}}
\providecommand{\miouLVDburnCoarseLRVarLrMultOne}{\tbd{miouLVDburnCoarseLRVarLrMultOne}}
\providecommand{\miouLVDburnCoarseLTwo}{\tbd{miouLVDburnCoarseLTwo}}
\providecommand{\miouLVDburnCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{miouLVDburnCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouLVDburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{miouLVDburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\miouLVDburnCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouLVDburnCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{miouLVDburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\miouLVDburnCoarseLTwoVarDecoderSamLite}{\tbd{miouLVDburnCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouLVDburnCoarseLTwoVarDecoderSamLiteLrMultOne}{\tbd{miouLVDburnCoarseLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\miouLVDburnCoarseLTwoVarDecoderSamPretrained}{\tbd{miouLVDburnCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\miouLVDburnCoarseLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{miouLVDburnCoarseLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\miouLVDburnCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouLVDburnCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouLVDburnCoarseLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{miouLVDburnCoarseLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\miouLVDburnCoarseLTwoVarLossBootstrap}{\tbd{miouLVDburnCoarseLTwoVarLossBootstrap}}
\providecommand{\miouLVDburnCoarseLTwoVarLossGce}{\tbd{miouLVDburnCoarseLTwoVarLossGce}}
\providecommand{\miouLVDburnCoarseLTwoVarLrMultOne}{\tbd{miouLVDburnCoarseLTwoVarLrMultOne}}
\providecommand{\miouLVDburnCoarseLTwoVarLrMultThree}{\tbd{miouLVDburnCoarseLTwoVarLrMultThree}}
\providecommand{\miouLVDburnCoarseLTwoVarLrMultZeroOneOneOneOne}{\tbd{miouLVDburnCoarseLTwoVarLrMultZeroOneOneOneOne}}
\providecommand{\miouLVDburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouLVDburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouLVDburnCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouLVDburnCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouLVDburnOmissionLOne}{\tbd{miouLVDburnOmissionLOne}}
\providecommand{\miouLVDburnOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{miouLVDburnOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouLVDburnOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{miouLVDburnOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDburnOmissionLOneVarDecoderSamLite}{\tbd{miouLVDburnOmissionLOneVarDecoderSamLite}}
\providecommand{\miouLVDburnOmissionLOneVarDecoderSamPretrained}{\tbd{miouLVDburnOmissionLOneVarDecoderSamPretrained}}
\providecommand{\miouLVDburnOmissionLOneVarDecoderSegformerMlp}{\tbd{miouLVDburnOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\miouLVDburnOmissionLR}{\tbd{miouLVDburnOmissionLR}}
\providecommand{\miouLVDburnOmissionLRVarLrMultOne}{\tbd{miouLVDburnOmissionLRVarLrMultOne}}
\providecommand{\miouLVDburnOmissionLTwo}{\tbd{miouLVDburnOmissionLTwo}}
\providecommand{\miouLVDburnOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{miouLVDburnOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouLVDburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{miouLVDburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\miouLVDburnOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouLVDburnOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{miouLVDburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\miouLVDburnOmissionLTwoVarDecoderSamLite}{\tbd{miouLVDburnOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouLVDburnOmissionLTwoVarDecoderSamLiteLrMultOne}{\tbd{miouLVDburnOmissionLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\miouLVDburnOmissionLTwoVarDecoderSamPretrained}{\tbd{miouLVDburnOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\miouLVDburnOmissionLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{miouLVDburnOmissionLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\miouLVDburnOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouLVDburnOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouLVDburnOmissionLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{miouLVDburnOmissionLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\miouLVDburnOmissionLTwoVarLossBootstrap}{\tbd{miouLVDburnOmissionLTwoVarLossBootstrap}}
\providecommand{\miouLVDburnOmissionLTwoVarLossGce}{\tbd{miouLVDburnOmissionLTwoVarLossGce}}
\providecommand{\miouLVDburnOmissionLTwoVarLrMultOne}{\tbd{miouLVDburnOmissionLTwoVarLrMultOne}}
\providecommand{\miouLVDburnOmissionLTwoVarLrMultThree}{\tbd{miouLVDburnOmissionLTwoVarLrMultThree}}
\providecommand{\miouLVDburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouLVDburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouLVDburnOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouLVDburnOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouLVDburnShiftLOne}{\tbd{miouLVDburnShiftLOne}}
\providecommand{\miouLVDburnShiftLOneVarDecoderMaskTwoformerFull}{\tbd{miouLVDburnShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouLVDburnShiftLOneVarDecoderMaskTwoformerLite}{\tbd{miouLVDburnShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDburnShiftLOneVarDecoderSamLite}{\tbd{miouLVDburnShiftLOneVarDecoderSamLite}}
\providecommand{\miouLVDburnShiftLOneVarDecoderSamPretrained}{\tbd{miouLVDburnShiftLOneVarDecoderSamPretrained}}
\providecommand{\miouLVDburnShiftLOneVarDecoderSegformerMlp}{\tbd{miouLVDburnShiftLOneVarDecoderSegformerMlp}}
\providecommand{\miouLVDburnShiftLR}{\tbd{miouLVDburnShiftLR}}
\providecommand{\miouLVDburnShiftLRVarLrMultOne}{\tbd{miouLVDburnShiftLRVarLrMultOne}}
\providecommand{\miouLVDburnShiftLTwo}{\tbd{miouLVDburnShiftLTwo}}
\providecommand{\miouLVDburnShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{miouLVDburnShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouLVDburnShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{miouLVDburnShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\miouLVDburnShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouLVDburnShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{miouLVDburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\miouLVDburnShiftLTwoVarDecoderSamLite}{\tbd{miouLVDburnShiftLTwoVarDecoderSamLite}}
\providecommand{\miouLVDburnShiftLTwoVarDecoderSamLiteLrMultOne}{\tbd{miouLVDburnShiftLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\miouLVDburnShiftLTwoVarDecoderSamPretrained}{\tbd{miouLVDburnShiftLTwoVarDecoderSamPretrained}}
\providecommand{\miouLVDburnShiftLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{miouLVDburnShiftLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\miouLVDburnShiftLTwoVarDecoderSegformerMlp}{\tbd{miouLVDburnShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouLVDburnShiftLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{miouLVDburnShiftLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\miouLVDburnShiftLTwoVarLossBootstrap}{\tbd{miouLVDburnShiftLTwoVarLossBootstrap}}
\providecommand{\miouLVDburnShiftLTwoVarLossGce}{\tbd{miouLVDburnShiftLTwoVarLossGce}}
\providecommand{\miouLVDburnShiftLTwoVarLrMultOne}{\tbd{miouLVDburnShiftLTwoVarLrMultOne}}
\providecommand{\miouLVDburnShiftLTwoVarLrMultThree}{\tbd{miouLVDburnShiftLTwoVarLrMultThree}}
\providecommand{\miouLVDburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouLVDburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouLVDburnShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouLVDburnShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouLVDflairBoundaryLOne}{\tbd{miouLVDflairBoundaryLOne}}
\providecommand{\miouLVDflairBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{miouLVDflairBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouLVDflairBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{miouLVDflairBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDflairBoundaryLOneVarDecoderSamLite}{\tbd{miouLVDflairBoundaryLOneVarDecoderSamLite}}
\providecommand{\miouLVDflairBoundaryLOneVarDecoderSamPretrained}{\tbd{miouLVDflairBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\miouLVDflairBoundaryLOneVarDecoderSegformerMlp}{\tbd{miouLVDflairBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\miouLVDflairBoundaryLR}{\tbd{miouLVDflairBoundaryLR}}
\providecommand{\miouLVDflairBoundaryLRVarLrMultOne}{\tbd{miouLVDflairBoundaryLRVarLrMultOne}}
\providecommand{\miouLVDflairBoundaryLTwo}{\tbd{miouLVDflairBoundaryLTwo}}
\providecommand{\miouLVDflairBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{miouLVDflairBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouLVDflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{miouLVDflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\miouLVDflairBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouLVDflairBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{miouLVDflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\miouLVDflairBoundaryLTwoVarDecoderSamLite}{\tbd{miouLVDflairBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouLVDflairBoundaryLTwoVarDecoderSamLiteLrMultOne}{\tbd{miouLVDflairBoundaryLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\miouLVDflairBoundaryLTwoVarDecoderSamPretrained}{\tbd{miouLVDflairBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\miouLVDflairBoundaryLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{miouLVDflairBoundaryLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\miouLVDflairBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouLVDflairBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouLVDflairBoundaryLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{miouLVDflairBoundaryLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\miouLVDflairBoundaryLTwoVarLossBootstrap}{\tbd{miouLVDflairBoundaryLTwoVarLossBootstrap}}
\providecommand{\miouLVDflairBoundaryLTwoVarLossGce}{\tbd{miouLVDflairBoundaryLTwoVarLossGce}}
\providecommand{\miouLVDflairBoundaryLTwoVarLrMultOne}{\tbd{miouLVDflairBoundaryLTwoVarLrMultOne}}
\providecommand{\miouLVDflairBoundaryLTwoVarLrMultThree}{\tbd{miouLVDflairBoundaryLTwoVarLrMultThree}}
\providecommand{\miouLVDflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouLVDflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouLVDflairBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouLVDflairBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouLVDflairClean}{\tbd{miouLVDflairClean}}
\providecommand{\miouLVDflairCleanVarDecoderMaskTwoformerFull}{\tbd{miouLVDflairCleanVarDecoderMaskTwoformerFull}}
\providecommand{\miouLVDflairCleanVarDecoderMaskTwoformerFullLrMultOne}{\tbd{miouLVDflairCleanVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\miouLVDflairCleanVarDecoderMaskTwoformerLite}{\tbd{miouLVDflairCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDflairCleanVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{miouLVDflairCleanVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\miouLVDflairCleanVarDecoderSamLite}{\tbd{miouLVDflairCleanVarDecoderSamLite}}
\providecommand{\miouLVDflairCleanVarDecoderSamLiteLrMultOne}{\tbd{miouLVDflairCleanVarDecoderSamLiteLrMultOne}}
\providecommand{\miouLVDflairCleanVarDecoderSamPretrained}{\tbd{miouLVDflairCleanVarDecoderSamPretrained}}
\providecommand{\miouLVDflairCleanVarDecoderSamPretrainedLrMultOne}{\tbd{miouLVDflairCleanVarDecoderSamPretrainedLrMultOne}}
\providecommand{\miouLVDflairCleanVarDecoderSegformerMlp}{\tbd{miouLVDflairCleanVarDecoderSegformerMlp}}
\providecommand{\miouLVDflairCleanVarDecoderSegformerMlpLrMultOne}{\tbd{miouLVDflairCleanVarDecoderSegformerMlpLrMultOne}}
\providecommand{\miouLVDflairCleanVarLossBootstrap}{\tbd{miouLVDflairCleanVarLossBootstrap}}
\providecommand{\miouLVDflairCleanVarLossGce}{\tbd{miouLVDflairCleanVarLossGce}}
\providecommand{\miouLVDflairCleanVarLrMultOne}{\tbd{miouLVDflairCleanVarLrMultOne}}
\providecommand{\miouLVDflairCleanVarLrMultThree}{\tbd{miouLVDflairCleanVarLrMultThree}}
\providecommand{\miouLVDflairCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{miouLVDflairCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouLVDflairCleanVarTrainSubsetCleanTwoFive}{\tbd{miouLVDflairCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\miouLVDflairCoarseLOne}{\tbd{miouLVDflairCoarseLOne}}
\providecommand{\miouLVDflairCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{miouLVDflairCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouLVDflairCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{miouLVDflairCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDflairCoarseLOneVarDecoderSamLite}{\tbd{miouLVDflairCoarseLOneVarDecoderSamLite}}
\providecommand{\miouLVDflairCoarseLOneVarDecoderSamPretrained}{\tbd{miouLVDflairCoarseLOneVarDecoderSamPretrained}}
\providecommand{\miouLVDflairCoarseLOneVarDecoderSegformerMlp}{\tbd{miouLVDflairCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\miouLVDflairCoarseLR}{\tbd{miouLVDflairCoarseLR}}
\providecommand{\miouLVDflairCoarseLRVarLrMultOne}{\tbd{miouLVDflairCoarseLRVarLrMultOne}}
\providecommand{\miouLVDflairCoarseLTwo}{\tbd{miouLVDflairCoarseLTwo}}
\providecommand{\miouLVDflairCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{miouLVDflairCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouLVDflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{miouLVDflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\miouLVDflairCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouLVDflairCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{miouLVDflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\miouLVDflairCoarseLTwoVarDecoderSamLite}{\tbd{miouLVDflairCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouLVDflairCoarseLTwoVarDecoderSamLiteLrMultOne}{\tbd{miouLVDflairCoarseLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\miouLVDflairCoarseLTwoVarDecoderSamPretrained}{\tbd{miouLVDflairCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\miouLVDflairCoarseLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{miouLVDflairCoarseLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\miouLVDflairCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouLVDflairCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouLVDflairCoarseLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{miouLVDflairCoarseLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\miouLVDflairCoarseLTwoVarLossBootstrap}{\tbd{miouLVDflairCoarseLTwoVarLossBootstrap}}
\providecommand{\miouLVDflairCoarseLTwoVarLossGce}{\tbd{miouLVDflairCoarseLTwoVarLossGce}}
\providecommand{\miouLVDflairCoarseLTwoVarLrMultOne}{\tbd{miouLVDflairCoarseLTwoVarLrMultOne}}
\providecommand{\miouLVDflairCoarseLTwoVarLrMultThree}{\tbd{miouLVDflairCoarseLTwoVarLrMultThree}}
\providecommand{\miouLVDflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouLVDflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouLVDflairCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouLVDflairCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouLVDflairOmissionLOne}{\tbd{miouLVDflairOmissionLOne}}
\providecommand{\miouLVDflairOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{miouLVDflairOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouLVDflairOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{miouLVDflairOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDflairOmissionLOneVarDecoderSamLite}{\tbd{miouLVDflairOmissionLOneVarDecoderSamLite}}
\providecommand{\miouLVDflairOmissionLOneVarDecoderSamPretrained}{\tbd{miouLVDflairOmissionLOneVarDecoderSamPretrained}}
\providecommand{\miouLVDflairOmissionLOneVarDecoderSegformerMlp}{\tbd{miouLVDflairOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\miouLVDflairOmissionLR}{\tbd{miouLVDflairOmissionLR}}
\providecommand{\miouLVDflairOmissionLRVarLrMultOne}{\tbd{miouLVDflairOmissionLRVarLrMultOne}}
\providecommand{\miouLVDflairOmissionLTwo}{\tbd{miouLVDflairOmissionLTwo}}
\providecommand{\miouLVDflairOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{miouLVDflairOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouLVDflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{miouLVDflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\miouLVDflairOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouLVDflairOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{miouLVDflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\miouLVDflairOmissionLTwoVarDecoderSamLite}{\tbd{miouLVDflairOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouLVDflairOmissionLTwoVarDecoderSamLiteLrMultOne}{\tbd{miouLVDflairOmissionLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\miouLVDflairOmissionLTwoVarDecoderSamPretrained}{\tbd{miouLVDflairOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\miouLVDflairOmissionLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{miouLVDflairOmissionLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\miouLVDflairOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouLVDflairOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouLVDflairOmissionLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{miouLVDflairOmissionLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\miouLVDflairOmissionLTwoVarLossBootstrap}{\tbd{miouLVDflairOmissionLTwoVarLossBootstrap}}
\providecommand{\miouLVDflairOmissionLTwoVarLossGce}{\tbd{miouLVDflairOmissionLTwoVarLossGce}}
\providecommand{\miouLVDflairOmissionLTwoVarLrMultOne}{\tbd{miouLVDflairOmissionLTwoVarLrMultOne}}
\providecommand{\miouLVDflairOmissionLTwoVarLrMultThree}{\tbd{miouLVDflairOmissionLTwoVarLrMultThree}}
\providecommand{\miouLVDflairOmissionLTwoVarLrMultZeroOneOneOneOne}{\tbd{miouLVDflairOmissionLTwoVarLrMultZeroOneOneOneOne}}
\providecommand{\miouLVDflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouLVDflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouLVDflairOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouLVDflairOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouLVDflairShiftLOne}{\tbd{miouLVDflairShiftLOne}}
\providecommand{\miouLVDflairShiftLOneVarDecoderMaskTwoformerFull}{\tbd{miouLVDflairShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouLVDflairShiftLOneVarDecoderMaskTwoformerLite}{\tbd{miouLVDflairShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDflairShiftLOneVarDecoderSamLite}{\tbd{miouLVDflairShiftLOneVarDecoderSamLite}}
\providecommand{\miouLVDflairShiftLOneVarDecoderSamPretrained}{\tbd{miouLVDflairShiftLOneVarDecoderSamPretrained}}
\providecommand{\miouLVDflairShiftLOneVarDecoderSegformerMlp}{\tbd{miouLVDflairShiftLOneVarDecoderSegformerMlp}}
\providecommand{\miouLVDflairShiftLR}{\tbd{miouLVDflairShiftLR}}
\providecommand{\miouLVDflairShiftLRVarLrMultOne}{\tbd{miouLVDflairShiftLRVarLrMultOne}}
\providecommand{\miouLVDflairShiftLTwo}{\tbd{miouLVDflairShiftLTwo}}
\providecommand{\miouLVDflairShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{miouLVDflairShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouLVDflairShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{miouLVDflairShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\miouLVDflairShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouLVDflairShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouLVDflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{miouLVDflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\miouLVDflairShiftLTwoVarDecoderSamLite}{\tbd{miouLVDflairShiftLTwoVarDecoderSamLite}}
\providecommand{\miouLVDflairShiftLTwoVarDecoderSamLiteLrMultOne}{\tbd{miouLVDflairShiftLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\miouLVDflairShiftLTwoVarDecoderSamPretrained}{\tbd{miouLVDflairShiftLTwoVarDecoderSamPretrained}}
\providecommand{\miouLVDflairShiftLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{miouLVDflairShiftLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\miouLVDflairShiftLTwoVarDecoderSegformerMlp}{\tbd{miouLVDflairShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouLVDflairShiftLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{miouLVDflairShiftLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\miouLVDflairShiftLTwoVarLossBootstrap}{\tbd{miouLVDflairShiftLTwoVarLossBootstrap}}
\providecommand{\miouLVDflairShiftLTwoVarLossGce}{\tbd{miouLVDflairShiftLTwoVarLossGce}}
\providecommand{\miouLVDflairShiftLTwoVarLrMultOne}{\tbd{miouLVDflairShiftLTwoVarLrMultOne}}
\providecommand{\miouLVDflairShiftLTwoVarLrMultThree}{\tbd{miouLVDflairShiftLTwoVarLrMultThree}}
\providecommand{\miouLVDflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouLVDflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouLVDflairShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouLVDflairShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouLVDsenClean}{\tbd{miouLVDsenClean}}
\providecommand{\miouLVDsenOtsuLTwo}{\tbd{miouLVDsenOtsuLTwo}}
\providecommand{\miouPRIburnBoundaryLOne}{\tbd{miouPRIburnBoundaryLOne}}
\providecommand{\miouPRIburnBoundaryLTwo}{\tbd{miouPRIburnBoundaryLTwo}}
\providecommand{\miouPRIburnClean}{\tbd{miouPRIburnClean}}
\providecommand{\miouPRIburnCleanVarTrainSubsetCleanTwoFive}{\tbd{miouPRIburnCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\miouPRIburnCoarseLOne}{\tbd{miouPRIburnCoarseLOne}}
\providecommand{\miouPRIburnCoarseLTwo}{\tbd{miouPRIburnCoarseLTwo}}
\providecommand{\miouPRIburnOmissionLOne}{\tbd{miouPRIburnOmissionLOne}}
\providecommand{\miouPRIburnOmissionLTwo}{\tbd{miouPRIburnOmissionLTwo}}
\providecommand{\miouPRIburnShiftLOne}{\tbd{miouPRIburnShiftLOne}}
\providecommand{\miouPRIburnShiftLTwo}{\tbd{miouPRIburnShiftLTwo}}
\providecommand{\miouPRIflairBoundaryLOne}{\tbd{miouPRIflairBoundaryLOne}}
\providecommand{\miouPRIflairBoundaryLTwo}{\tbd{miouPRIflairBoundaryLTwo}}
\providecommand{\miouPRIflairClean}{\tbd{miouPRIflairClean}}
\providecommand{\miouPRIflairCleanVarTrainSubsetCleanTwoFive}{\tbd{miouPRIflairCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\miouPRIflairCoarseLOne}{\tbd{miouPRIflairCoarseLOne}}
\providecommand{\miouPRIflairCoarseLTwo}{\tbd{miouPRIflairCoarseLTwo}}
\providecommand{\miouPRIflairOmissionLOne}{\tbd{miouPRIflairOmissionLOne}}
\providecommand{\miouPRIflairOmissionLTwo}{\tbd{miouPRIflairOmissionLTwo}}
\providecommand{\miouPRIflairShiftLOne}{\tbd{miouPRIflairShiftLOne}}
\providecommand{\miouPRIflairShiftLTwo}{\tbd{miouPRIflairShiftLTwo}}
\providecommand{\miouRNChesBoundaryLOne}{\tbd{miouRNChesBoundaryLOne}}
\providecommand{\miouRNChesBoundaryLTwo}{\tbd{miouRNChesBoundaryLTwo}}
\providecommand{\miouRNChesClean}{\tbd{miouRNChesClean}}
\providecommand{\miouRNChesCoarseLOne}{\tbd{miouRNChesCoarseLOne}}
\providecommand{\miouRNChesCoarseLTwo}{\tbd{miouRNChesCoarseLTwo}}
\providecommand{\miouRNChesNlcdREAL}{\tbd{miouRNChesNlcdREAL}}
\providecommand{\miouRNChesOmissionLOne}{\tbd{miouRNChesOmissionLOne}}
\providecommand{\miouRNChesOmissionLTwo}{\tbd{miouRNChesOmissionLTwo}}
\providecommand{\miouRNChesShiftLOne}{\tbd{miouRNChesShiftLOne}}
\providecommand{\miouRNChesShiftLTwo}{\tbd{miouRNChesShiftLTwo}}
\providecommand{\miouRNCsTwelveBoundaryLOne}{\tbd{miouRNCsTwelveBoundaryLOne}}
\providecommand{\miouRNCsTwelveBoundaryLTwo}{\tbd{miouRNCsTwelveBoundaryLTwo}}
\providecommand{\miouRNCsTwelveClean}{\tbd{miouRNCsTwelveClean}}
\providecommand{\miouRNCsTwelveCoarseLOne}{\tbd{miouRNCsTwelveCoarseLOne}}
\providecommand{\miouRNCsTwelveCoarseLTwo}{\tbd{miouRNCsTwelveCoarseLTwo}}
\providecommand{\miouRNCsTwelveOmissionLOne}{\tbd{miouRNCsTwelveOmissionLOne}}
\providecommand{\miouRNCsTwelveOmissionLTwo}{\tbd{miouRNCsTwelveOmissionLTwo}}
\providecommand{\miouRNCsTwelveSTwocloudlessREAL}{\tbd{miouRNCsTwelveSTwocloudlessREAL}}
\providecommand{\miouRNCsTwelveShiftLOne}{\tbd{miouRNCsTwelveShiftLOne}}
\providecommand{\miouRNCsTwelveShiftLTwo}{\tbd{miouRNCsTwelveShiftLTwo}}
\providecommand{\miouRNDfcBoundaryLOne}{\tbd{miouRNDfcBoundaryLOne}}
\providecommand{\miouRNDfcBoundaryLTwo}{\tbd{miouRNDfcBoundaryLTwo}}
\providecommand{\miouRNDfcClean}{\tbd{miouRNDfcClean}}
\providecommand{\miouRNDfcCleanVarTrainSubsetRealcov}{\tbd{miouRNDfcCleanVarTrainSubsetRealcov}}
\providecommand{\miouRNDfcCoarseLOne}{\tbd{miouRNDfcCoarseLOne}}
\providecommand{\miouRNDfcCoarseLTwo}{\tbd{miouRNDfcCoarseLTwo}}
\providecommand{\miouRNDfcModisREALVarTrainSubsetRealcov}{\tbd{miouRNDfcModisREALVarTrainSubsetRealcov}}
\providecommand{\miouRNDfcOmissionLOne}{\tbd{miouRNDfcOmissionLOne}}
\providecommand{\miouRNDfcOmissionLTwo}{\tbd{miouRNDfcOmissionLTwo}}
\providecommand{\miouRNDfcShiftLOne}{\tbd{miouRNDfcShiftLOne}}
\providecommand{\miouRNDfcShiftLTwo}{\tbd{miouRNDfcShiftLTwo}}
\providecommand{\miouRNEnvaBoundaryLOne}{\tbd{miouRNEnvaBoundaryLOne}}
\providecommand{\miouRNEnvaBoundaryLTwo}{\tbd{miouRNEnvaBoundaryLTwo}}
\providecommand{\miouRNEnvaClean}{\tbd{miouRNEnvaClean}}
\providecommand{\miouRNEnvaCoarseLOne}{\tbd{miouRNEnvaCoarseLOne}}
\providecommand{\miouRNEnvaCoarseLTwo}{\tbd{miouRNEnvaCoarseLTwo}}
\providecommand{\miouRNEnvaNlcdREAL}{\tbd{miouRNEnvaNlcdREAL}}
\providecommand{\miouRNEnvaOmissionLOne}{\tbd{miouRNEnvaOmissionLOne}}
\providecommand{\miouRNEnvaOmissionLTwo}{\tbd{miouRNEnvaOmissionLTwo}}
\providecommand{\miouRNEnvaShiftLOne}{\tbd{miouRNEnvaShiftLOne}}
\providecommand{\miouRNEnvaShiftLTwo}{\tbd{miouRNEnvaShiftLTwo}}
\providecommand{\miouRNKuroBoundaryLOne}{\tbd{miouRNKuroBoundaryLOne}}
\providecommand{\miouRNKuroBoundaryLTwo}{\tbd{miouRNKuroBoundaryLTwo}}
\providecommand{\miouRNKuroCemsREALVarTrainSubsetRealcov}{\tbd{miouRNKuroCemsREALVarTrainSubsetRealcov}}
\providecommand{\miouRNKuroClean}{\tbd{miouRNKuroClean}}
\providecommand{\miouRNKuroCleanVarTrainSubsetRealcov}{\tbd{miouRNKuroCleanVarTrainSubsetRealcov}}
\providecommand{\miouRNKuroCoarseLOne}{\tbd{miouRNKuroCoarseLOne}}
\providecommand{\miouRNKuroCoarseLTwo}{\tbd{miouRNKuroCoarseLTwo}}
\providecommand{\miouRNKuroOmissionLOne}{\tbd{miouRNKuroOmissionLOne}}
\providecommand{\miouRNKuroOmissionLTwo}{\tbd{miouRNKuroOmissionLTwo}}
\providecommand{\miouRNKuroShiftLOne}{\tbd{miouRNKuroShiftLOne}}
\providecommand{\miouRNKuroShiftLTwo}{\tbd{miouRNKuroShiftLTwo}}
\providecommand{\miouRNOemBoundaryLOne}{\tbd{miouRNOemBoundaryLOne}}
\providecommand{\miouRNOemBoundaryLTwo}{\tbd{miouRNOemBoundaryLTwo}}
\providecommand{\miouRNOemClean}{\tbd{miouRNOemClean}}
\providecommand{\miouRNOemCoarseLOne}{\tbd{miouRNOemCoarseLOne}}
\providecommand{\miouRNOemCoarseLTwo}{\tbd{miouRNOemCoarseLTwo}}
\providecommand{\miouRNOemOmissionLOne}{\tbd{miouRNOemOmissionLOne}}
\providecommand{\miouRNOemOmissionLTwo}{\tbd{miouRNOemOmissionLTwo}}
\providecommand{\miouRNOemShiftLOne}{\tbd{miouRNOemShiftLOne}}
\providecommand{\miouRNOemShiftLTwo}{\tbd{miouRNOemShiftLTwo}}
\providecommand{\miouRNSSLburnClean}{\tbd{miouRNSSLburnClean}}
\providecommand{\miouRNSSLflairClean}{\tbd{miouRNSSLflairClean}}
\providecommand{\miouRNSnTwoBoundaryLOne}{\tbd{miouRNSnTwoBoundaryLOne}}
\providecommand{\miouRNSnTwoBoundaryLTwo}{\tbd{miouRNSnTwoBoundaryLTwo}}
\providecommand{\miouRNSnTwoClean}{\tbd{miouRNSnTwoClean}}
\providecommand{\miouRNSnTwoCoarseLOne}{\tbd{miouRNSnTwoCoarseLOne}}
\providecommand{\miouRNSnTwoCoarseLTwo}{\tbd{miouRNSnTwoCoarseLTwo}}
\providecommand{\miouRNSnTwoOmissionLOne}{\tbd{miouRNSnTwoOmissionLOne}}
\providecommand{\miouRNSnTwoOmissionLTwo}{\tbd{miouRNSnTwoOmissionLTwo}}
\providecommand{\miouRNSnTwoShiftLOne}{\tbd{miouRNSnTwoShiftLOne}}
\providecommand{\miouRNSnTwoShiftLTwo}{\tbd{miouRNSnTwoShiftLTwo}}
\providecommand{\miouRNburnBoundaryLOne}{\tbd{miouRNburnBoundaryLOne}}
\providecommand{\miouRNburnBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{miouRNburnBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouRNburnBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{miouRNburnBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouRNburnBoundaryLOneVarDecoderSamLite}{\tbd{miouRNburnBoundaryLOneVarDecoderSamLite}}
\providecommand{\miouRNburnBoundaryLOneVarDecoderSamPretrained}{\tbd{miouRNburnBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\miouRNburnBoundaryLOneVarDecoderSegformerMlp}{\tbd{miouRNburnBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\miouRNburnBoundaryLR}{\tbd{miouRNburnBoundaryLR}}
\providecommand{\miouRNburnBoundaryLTwo}{\tbd{miouRNburnBoundaryLTwo}}
\providecommand{\miouRNburnBoundaryLTwoVarBandsRgb}{\tbd{miouRNburnBoundaryLTwoVarBandsRgb}}
\providecommand{\miouRNburnBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{miouRNburnBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouRNburnBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouRNburnBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouRNburnBoundaryLTwoVarDecoderSamLite}{\tbd{miouRNburnBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouRNburnBoundaryLTwoVarDecoderSamPretrained}{\tbd{miouRNburnBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\miouRNburnBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouRNburnBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouRNburnBoundaryLTwoVarInitRandom}{\tbd{miouRNburnBoundaryLTwoVarInitRandom}}
\providecommand{\miouRNburnBoundaryLTwoVarLossBootstrap}{\tbd{miouRNburnBoundaryLTwoVarLossBootstrap}}
\providecommand{\miouRNburnBoundaryLTwoVarLossGce}{\tbd{miouRNburnBoundaryLTwoVarLossGce}}
\providecommand{\miouRNburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouRNburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouRNburnBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouRNburnBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouRNburnClean}{\tbd{miouRNburnClean}}
\providecommand{\miouRNburnCleanVarBandsRgb}{\tbd{miouRNburnCleanVarBandsRgb}}
\providecommand{\miouRNburnCleanVarDecoderMaskTwoformerFull}{\tbd{miouRNburnCleanVarDecoderMaskTwoformerFull}}
\providecommand{\miouRNburnCleanVarDecoderMaskTwoformerLite}{\tbd{miouRNburnCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouRNburnCleanVarDecoderSamLite}{\tbd{miouRNburnCleanVarDecoderSamLite}}
\providecommand{\miouRNburnCleanVarDecoderSamPretrained}{\tbd{miouRNburnCleanVarDecoderSamPretrained}}
\providecommand{\miouRNburnCleanVarDecoderSegformerMlp}{\tbd{miouRNburnCleanVarDecoderSegformerMlp}}
\providecommand{\miouRNburnCleanVarInitRandom}{\tbd{miouRNburnCleanVarInitRandom}}
\providecommand{\miouRNburnCleanVarInitRandomLrMultThree}{\tbd{miouRNburnCleanVarInitRandomLrMultThree}}
\providecommand{\miouRNburnCleanVarLossBootstrap}{\tbd{miouRNburnCleanVarLossBootstrap}}
\providecommand{\miouRNburnCleanVarLossGce}{\tbd{miouRNburnCleanVarLossGce}}
\providecommand{\miouRNburnCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{miouRNburnCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouRNburnCleanVarTrainSubsetCleanTwoFive}{\tbd{miouRNburnCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\miouRNburnCoarseLOne}{\tbd{miouRNburnCoarseLOne}}
\providecommand{\miouRNburnCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{miouRNburnCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouRNburnCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{miouRNburnCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouRNburnCoarseLOneVarDecoderSamLite}{\tbd{miouRNburnCoarseLOneVarDecoderSamLite}}
\providecommand{\miouRNburnCoarseLOneVarDecoderSamPretrained}{\tbd{miouRNburnCoarseLOneVarDecoderSamPretrained}}
\providecommand{\miouRNburnCoarseLOneVarDecoderSegformerMlp}{\tbd{miouRNburnCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\miouRNburnCoarseLR}{\tbd{miouRNburnCoarseLR}}
\providecommand{\miouRNburnCoarseLTwo}{\tbd{miouRNburnCoarseLTwo}}
\providecommand{\miouRNburnCoarseLTwoVarBandsRgb}{\tbd{miouRNburnCoarseLTwoVarBandsRgb}}
\providecommand{\miouRNburnCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{miouRNburnCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouRNburnCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouRNburnCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouRNburnCoarseLTwoVarDecoderSamLite}{\tbd{miouRNburnCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouRNburnCoarseLTwoVarDecoderSamPretrained}{\tbd{miouRNburnCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\miouRNburnCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouRNburnCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouRNburnCoarseLTwoVarInitRandom}{\tbd{miouRNburnCoarseLTwoVarInitRandom}}
\providecommand{\miouRNburnCoarseLTwoVarLossBootstrap}{\tbd{miouRNburnCoarseLTwoVarLossBootstrap}}
\providecommand{\miouRNburnCoarseLTwoVarLossGce}{\tbd{miouRNburnCoarseLTwoVarLossGce}}
\providecommand{\miouRNburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouRNburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouRNburnCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouRNburnCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouRNburnOmissionLOne}{\tbd{miouRNburnOmissionLOne}}
\providecommand{\miouRNburnOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{miouRNburnOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouRNburnOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{miouRNburnOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouRNburnOmissionLOneVarDecoderSamLite}{\tbd{miouRNburnOmissionLOneVarDecoderSamLite}}
\providecommand{\miouRNburnOmissionLOneVarDecoderSamPretrained}{\tbd{miouRNburnOmissionLOneVarDecoderSamPretrained}}
\providecommand{\miouRNburnOmissionLOneVarDecoderSegformerMlp}{\tbd{miouRNburnOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\miouRNburnOmissionLR}{\tbd{miouRNburnOmissionLR}}
\providecommand{\miouRNburnOmissionLTwo}{\tbd{miouRNburnOmissionLTwo}}
\providecommand{\miouRNburnOmissionLTwoVarBandsRgb}{\tbd{miouRNburnOmissionLTwoVarBandsRgb}}
\providecommand{\miouRNburnOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{miouRNburnOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouRNburnOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouRNburnOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouRNburnOmissionLTwoVarDecoderSamLite}{\tbd{miouRNburnOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouRNburnOmissionLTwoVarDecoderSamPretrained}{\tbd{miouRNburnOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\miouRNburnOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouRNburnOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouRNburnOmissionLTwoVarInitRandom}{\tbd{miouRNburnOmissionLTwoVarInitRandom}}
\providecommand{\miouRNburnOmissionLTwoVarLossBootstrap}{\tbd{miouRNburnOmissionLTwoVarLossBootstrap}}
\providecommand{\miouRNburnOmissionLTwoVarLossGce}{\tbd{miouRNburnOmissionLTwoVarLossGce}}
\providecommand{\miouRNburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouRNburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouRNburnOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouRNburnOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouRNburnShiftLOne}{\tbd{miouRNburnShiftLOne}}
\providecommand{\miouRNburnShiftLOneVarDecoderMaskTwoformerFull}{\tbd{miouRNburnShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouRNburnShiftLOneVarDecoderMaskTwoformerLite}{\tbd{miouRNburnShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouRNburnShiftLOneVarDecoderSamLite}{\tbd{miouRNburnShiftLOneVarDecoderSamLite}}
\providecommand{\miouRNburnShiftLOneVarDecoderSamPretrained}{\tbd{miouRNburnShiftLOneVarDecoderSamPretrained}}
\providecommand{\miouRNburnShiftLOneVarDecoderSegformerMlp}{\tbd{miouRNburnShiftLOneVarDecoderSegformerMlp}}
\providecommand{\miouRNburnShiftLR}{\tbd{miouRNburnShiftLR}}
\providecommand{\miouRNburnShiftLTwo}{\tbd{miouRNburnShiftLTwo}}
\providecommand{\miouRNburnShiftLTwoVarBandsRgb}{\tbd{miouRNburnShiftLTwoVarBandsRgb}}
\providecommand{\miouRNburnShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{miouRNburnShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouRNburnShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouRNburnShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouRNburnShiftLTwoVarDecoderSamLite}{\tbd{miouRNburnShiftLTwoVarDecoderSamLite}}
\providecommand{\miouRNburnShiftLTwoVarDecoderSamPretrained}{\tbd{miouRNburnShiftLTwoVarDecoderSamPretrained}}
\providecommand{\miouRNburnShiftLTwoVarDecoderSegformerMlp}{\tbd{miouRNburnShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouRNburnShiftLTwoVarInitRandom}{\tbd{miouRNburnShiftLTwoVarInitRandom}}
\providecommand{\miouRNburnShiftLTwoVarLossBootstrap}{\tbd{miouRNburnShiftLTwoVarLossBootstrap}}
\providecommand{\miouRNburnShiftLTwoVarLossGce}{\tbd{miouRNburnShiftLTwoVarLossGce}}
\providecommand{\miouRNburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouRNburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouRNburnShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouRNburnShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouRNflairBoundaryLOne}{\tbd{miouRNflairBoundaryLOne}}
\providecommand{\miouRNflairBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{miouRNflairBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouRNflairBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{miouRNflairBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouRNflairBoundaryLOneVarDecoderSamLite}{\tbd{miouRNflairBoundaryLOneVarDecoderSamLite}}
\providecommand{\miouRNflairBoundaryLOneVarDecoderSamPretrained}{\tbd{miouRNflairBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\miouRNflairBoundaryLOneVarDecoderSegformerMlp}{\tbd{miouRNflairBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\miouRNflairBoundaryLR}{\tbd{miouRNflairBoundaryLR}}
\providecommand{\miouRNflairBoundaryLTwo}{\tbd{miouRNflairBoundaryLTwo}}
\providecommand{\miouRNflairBoundaryLTwoVarBandsRgb}{\tbd{miouRNflairBoundaryLTwoVarBandsRgb}}
\providecommand{\miouRNflairBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{miouRNflairBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouRNflairBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouRNflairBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouRNflairBoundaryLTwoVarDecoderSamLite}{\tbd{miouRNflairBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouRNflairBoundaryLTwoVarDecoderSamPretrained}{\tbd{miouRNflairBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\miouRNflairBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouRNflairBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouRNflairBoundaryLTwoVarInitRandom}{\tbd{miouRNflairBoundaryLTwoVarInitRandom}}
\providecommand{\miouRNflairBoundaryLTwoVarLossBootstrap}{\tbd{miouRNflairBoundaryLTwoVarLossBootstrap}}
\providecommand{\miouRNflairBoundaryLTwoVarLossGce}{\tbd{miouRNflairBoundaryLTwoVarLossGce}}
\providecommand{\miouRNflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouRNflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouRNflairBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouRNflairBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouRNflairClean}{\tbd{miouRNflairClean}}
\providecommand{\miouRNflairCleanVarBandsRgb}{\tbd{miouRNflairCleanVarBandsRgb}}
\providecommand{\miouRNflairCleanVarClassWeightedTrue}{\tbd{miouRNflairCleanVarClassWeightedTrue}}
\providecommand{\miouRNflairCleanVarDecoderMaskTwoformerFull}{\tbd{miouRNflairCleanVarDecoderMaskTwoformerFull}}
\providecommand{\miouRNflairCleanVarDecoderMaskTwoformerLite}{\tbd{miouRNflairCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouRNflairCleanVarDecoderSamLite}{\tbd{miouRNflairCleanVarDecoderSamLite}}
\providecommand{\miouRNflairCleanVarDecoderSamPretrained}{\tbd{miouRNflairCleanVarDecoderSamPretrained}}
\providecommand{\miouRNflairCleanVarDecoderSegformerMlp}{\tbd{miouRNflairCleanVarDecoderSegformerMlp}}
\providecommand{\miouRNflairCleanVarInitRandom}{\tbd{miouRNflairCleanVarInitRandom}}
\providecommand{\miouRNflairCleanVarInitRandomLrMultThree}{\tbd{miouRNflairCleanVarInitRandomLrMultThree}}
\providecommand{\miouRNflairCleanVarLossBootstrap}{\tbd{miouRNflairCleanVarLossBootstrap}}
\providecommand{\miouRNflairCleanVarLossGce}{\tbd{miouRNflairCleanVarLossGce}}
\providecommand{\miouRNflairCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{miouRNflairCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouRNflairCleanVarTrainSubsetCleanTwoFive}{\tbd{miouRNflairCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\miouRNflairCoarseLOne}{\tbd{miouRNflairCoarseLOne}}
\providecommand{\miouRNflairCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{miouRNflairCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouRNflairCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{miouRNflairCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouRNflairCoarseLOneVarDecoderSamLite}{\tbd{miouRNflairCoarseLOneVarDecoderSamLite}}
\providecommand{\miouRNflairCoarseLOneVarDecoderSamPretrained}{\tbd{miouRNflairCoarseLOneVarDecoderSamPretrained}}
\providecommand{\miouRNflairCoarseLOneVarDecoderSegformerMlp}{\tbd{miouRNflairCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\miouRNflairCoarseLR}{\tbd{miouRNflairCoarseLR}}
\providecommand{\miouRNflairCoarseLTwo}{\tbd{miouRNflairCoarseLTwo}}
\providecommand{\miouRNflairCoarseLTwoVarBandsRgb}{\tbd{miouRNflairCoarseLTwoVarBandsRgb}}
\providecommand{\miouRNflairCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{miouRNflairCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouRNflairCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouRNflairCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouRNflairCoarseLTwoVarDecoderSamLite}{\tbd{miouRNflairCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouRNflairCoarseLTwoVarDecoderSamPretrained}{\tbd{miouRNflairCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\miouRNflairCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouRNflairCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouRNflairCoarseLTwoVarInitRandom}{\tbd{miouRNflairCoarseLTwoVarInitRandom}}
\providecommand{\miouRNflairCoarseLTwoVarLossBootstrap}{\tbd{miouRNflairCoarseLTwoVarLossBootstrap}}
\providecommand{\miouRNflairCoarseLTwoVarLossGce}{\tbd{miouRNflairCoarseLTwoVarLossGce}}
\providecommand{\miouRNflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouRNflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouRNflairCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouRNflairCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouRNflairOmissionLOne}{\tbd{miouRNflairOmissionLOne}}
\providecommand{\miouRNflairOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{miouRNflairOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouRNflairOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{miouRNflairOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouRNflairOmissionLOneVarDecoderSamLite}{\tbd{miouRNflairOmissionLOneVarDecoderSamLite}}
\providecommand{\miouRNflairOmissionLOneVarDecoderSamPretrained}{\tbd{miouRNflairOmissionLOneVarDecoderSamPretrained}}
\providecommand{\miouRNflairOmissionLOneVarDecoderSegformerMlp}{\tbd{miouRNflairOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\miouRNflairOmissionLR}{\tbd{miouRNflairOmissionLR}}
\providecommand{\miouRNflairOmissionLTwo}{\tbd{miouRNflairOmissionLTwo}}
\providecommand{\miouRNflairOmissionLTwoVarBandsRgb}{\tbd{miouRNflairOmissionLTwoVarBandsRgb}}
\providecommand{\miouRNflairOmissionLTwoVarClassWeightedTrue}{\tbd{miouRNflairOmissionLTwoVarClassWeightedTrue}}
\providecommand{\miouRNflairOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{miouRNflairOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouRNflairOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouRNflairOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouRNflairOmissionLTwoVarDecoderSamLite}{\tbd{miouRNflairOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouRNflairOmissionLTwoVarDecoderSamPretrained}{\tbd{miouRNflairOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\miouRNflairOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouRNflairOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouRNflairOmissionLTwoVarInitRandom}{\tbd{miouRNflairOmissionLTwoVarInitRandom}}
\providecommand{\miouRNflairOmissionLTwoVarLossBootstrap}{\tbd{miouRNflairOmissionLTwoVarLossBootstrap}}
\providecommand{\miouRNflairOmissionLTwoVarLossGce}{\tbd{miouRNflairOmissionLTwoVarLossGce}}
\providecommand{\miouRNflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouRNflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouRNflairOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouRNflairOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouRNflairShiftLOne}{\tbd{miouRNflairShiftLOne}}
\providecommand{\miouRNflairShiftLOneVarDecoderMaskTwoformerFull}{\tbd{miouRNflairShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouRNflairShiftLOneVarDecoderMaskTwoformerLite}{\tbd{miouRNflairShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouRNflairShiftLOneVarDecoderSamLite}{\tbd{miouRNflairShiftLOneVarDecoderSamLite}}
\providecommand{\miouRNflairShiftLOneVarDecoderSamPretrained}{\tbd{miouRNflairShiftLOneVarDecoderSamPretrained}}
\providecommand{\miouRNflairShiftLOneVarDecoderSegformerMlp}{\tbd{miouRNflairShiftLOneVarDecoderSegformerMlp}}
\providecommand{\miouRNflairShiftLR}{\tbd{miouRNflairShiftLR}}
\providecommand{\miouRNflairShiftLTwo}{\tbd{miouRNflairShiftLTwo}}
\providecommand{\miouRNflairShiftLTwoVarBandsRgb}{\tbd{miouRNflairShiftLTwoVarBandsRgb}}
\providecommand{\miouRNflairShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{miouRNflairShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouRNflairShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouRNflairShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouRNflairShiftLTwoVarDecoderSamLite}{\tbd{miouRNflairShiftLTwoVarDecoderSamLite}}
\providecommand{\miouRNflairShiftLTwoVarDecoderSamPretrained}{\tbd{miouRNflairShiftLTwoVarDecoderSamPretrained}}
\providecommand{\miouRNflairShiftLTwoVarDecoderSegformerMlp}{\tbd{miouRNflairShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouRNflairShiftLTwoVarInitRandom}{\tbd{miouRNflairShiftLTwoVarInitRandom}}
\providecommand{\miouRNflairShiftLTwoVarLossBootstrap}{\tbd{miouRNflairShiftLTwoVarLossBootstrap}}
\providecommand{\miouRNflairShiftLTwoVarLossGce}{\tbd{miouRNflairShiftLTwoVarLossGce}}
\providecommand{\miouRNflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouRNflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouRNflairShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouRNflairShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouRNsenClean}{\tbd{miouRNsenClean}}
\providecommand{\miouRNsenOtsuLTwo}{\tbd{miouRNsenOtsuLTwo}}
\providecommand{\miouResnetFiveZeroSslFoureoburnBoundaryLOne}{\tbd{miouResnetFiveZeroSslFoureoburnBoundaryLOne}}
\providecommand{\miouResnetFiveZeroSslFoureoburnBoundaryLTwo}{\tbd{miouResnetFiveZeroSslFoureoburnBoundaryLTwo}}
\providecommand{\miouResnetFiveZeroSslFoureoburnClean}{\tbd{miouResnetFiveZeroSslFoureoburnClean}}
\providecommand{\miouResnetFiveZeroSslFoureoburnCleanVarTrainSubsetCleanTwoFive}{\tbd{miouResnetFiveZeroSslFoureoburnCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\miouResnetFiveZeroSslFoureoburnCoarseLOne}{\tbd{miouResnetFiveZeroSslFoureoburnCoarseLOne}}
\providecommand{\miouResnetFiveZeroSslFoureoburnCoarseLTwo}{\tbd{miouResnetFiveZeroSslFoureoburnCoarseLTwo}}
\providecommand{\miouResnetFiveZeroSslFoureoburnOmissionLOne}{\tbd{miouResnetFiveZeroSslFoureoburnOmissionLOne}}
\providecommand{\miouResnetFiveZeroSslFoureoburnOmissionLTwo}{\tbd{miouResnetFiveZeroSslFoureoburnOmissionLTwo}}
\providecommand{\miouResnetFiveZeroSslFoureoburnShiftLOne}{\tbd{miouResnetFiveZeroSslFoureoburnShiftLOne}}
\providecommand{\miouResnetFiveZeroSslFoureoburnShiftLTwo}{\tbd{miouResnetFiveZeroSslFoureoburnShiftLTwo}}
\providecommand{\miouResnetFiveZeroSslFoureoflairBoundaryLOne}{\tbd{miouResnetFiveZeroSslFoureoflairBoundaryLOne}}
\providecommand{\miouResnetFiveZeroSslFoureoflairBoundaryLTwo}{\tbd{miouResnetFiveZeroSslFoureoflairBoundaryLTwo}}
\providecommand{\miouResnetFiveZeroSslFoureoflairClean}{\tbd{miouResnetFiveZeroSslFoureoflairClean}}
\providecommand{\miouResnetFiveZeroSslFoureoflairCleanVarTrainSubsetCleanTwoFive}{\tbd{miouResnetFiveZeroSslFoureoflairCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\miouResnetFiveZeroSslFoureoflairCoarseLOne}{\tbd{miouResnetFiveZeroSslFoureoflairCoarseLOne}}
\providecommand{\miouResnetFiveZeroSslFoureoflairCoarseLTwo}{\tbd{miouResnetFiveZeroSslFoureoflairCoarseLTwo}}
\providecommand{\miouResnetFiveZeroSslFoureoflairOmissionLOne}{\tbd{miouResnetFiveZeroSslFoureoflairOmissionLOne}}
\providecommand{\miouResnetFiveZeroSslFoureoflairOmissionLTwo}{\tbd{miouResnetFiveZeroSslFoureoflairOmissionLTwo}}
\providecommand{\miouResnetFiveZeroSslFoureoflairShiftLOne}{\tbd{miouResnetFiveZeroSslFoureoflairShiftLOne}}
\providecommand{\miouResnetFiveZeroSslFoureoflairShiftLTwo}{\tbd{miouResnetFiveZeroSslFoureoflairShiftLTwo}}
\providecommand{\miouSATChesBoundaryLOne}{\tbd{miouSATChesBoundaryLOne}}
\providecommand{\miouSATChesBoundaryLTwo}{\tbd{miouSATChesBoundaryLTwo}}
\providecommand{\miouSATChesBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouSATChesBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATChesBoundaryLTwoVarDecoderSamLite}{\tbd{miouSATChesBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouSATChesBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouSATChesBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouSATChesBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATChesBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATChesClean}{\tbd{miouSATChesClean}}
\providecommand{\miouSATChesCleanVarDecoderMaskTwoformerLite}{\tbd{miouSATChesCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATChesCleanVarDecoderSamLite}{\tbd{miouSATChesCleanVarDecoderSamLite}}
\providecommand{\miouSATChesCleanVarDecoderSegformerMlp}{\tbd{miouSATChesCleanVarDecoderSegformerMlp}}
\providecommand{\miouSATChesCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATChesCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATChesCoarseLOne}{\tbd{miouSATChesCoarseLOne}}
\providecommand{\miouSATChesCoarseLTwo}{\tbd{miouSATChesCoarseLTwo}}
\providecommand{\miouSATChesCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouSATChesCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATChesCoarseLTwoVarDecoderSamLite}{\tbd{miouSATChesCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouSATChesCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouSATChesCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouSATChesCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATChesCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATChesNlcdREAL}{\tbd{miouSATChesNlcdREAL}}
\providecommand{\miouSATChesOmissionLOne}{\tbd{miouSATChesOmissionLOne}}
\providecommand{\miouSATChesOmissionLTwo}{\tbd{miouSATChesOmissionLTwo}}
\providecommand{\miouSATChesOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouSATChesOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATChesOmissionLTwoVarDecoderSamLite}{\tbd{miouSATChesOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouSATChesOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouSATChesOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouSATChesOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATChesOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATChesShiftLOne}{\tbd{miouSATChesShiftLOne}}
\providecommand{\miouSATChesShiftLTwo}{\tbd{miouSATChesShiftLTwo}}
\providecommand{\miouSATChesShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouSATChesShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATChesShiftLTwoVarDecoderSamLite}{\tbd{miouSATChesShiftLTwoVarDecoderSamLite}}
\providecommand{\miouSATChesShiftLTwoVarDecoderSegformerMlp}{\tbd{miouSATChesShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouSATChesShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATChesShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATCsTwelveBoundaryLOne}{\tbd{miouSATCsTwelveBoundaryLOne}}
\providecommand{\miouSATCsTwelveBoundaryLTwo}{\tbd{miouSATCsTwelveBoundaryLTwo}}
\providecommand{\miouSATCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouSATCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATCsTwelveBoundaryLTwoVarDecoderSamLite}{\tbd{miouSATCsTwelveBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouSATCsTwelveBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouSATCsTwelveBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouSATCsTwelveBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATCsTwelveBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATCsTwelveClean}{\tbd{miouSATCsTwelveClean}}
\providecommand{\miouSATCsTwelveCleanVarDecoderMaskTwoformerLite}{\tbd{miouSATCsTwelveCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATCsTwelveCleanVarDecoderSamLite}{\tbd{miouSATCsTwelveCleanVarDecoderSamLite}}
\providecommand{\miouSATCsTwelveCleanVarDecoderSegformerMlp}{\tbd{miouSATCsTwelveCleanVarDecoderSegformerMlp}}
\providecommand{\miouSATCsTwelveCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATCsTwelveCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATCsTwelveCoarseLOne}{\tbd{miouSATCsTwelveCoarseLOne}}
\providecommand{\miouSATCsTwelveCoarseLTwo}{\tbd{miouSATCsTwelveCoarseLTwo}}
\providecommand{\miouSATCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouSATCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATCsTwelveCoarseLTwoVarDecoderSamLite}{\tbd{miouSATCsTwelveCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouSATCsTwelveCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouSATCsTwelveCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouSATCsTwelveCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATCsTwelveCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATCsTwelveOmissionLOne}{\tbd{miouSATCsTwelveOmissionLOne}}
\providecommand{\miouSATCsTwelveOmissionLTwo}{\tbd{miouSATCsTwelveOmissionLTwo}}
\providecommand{\miouSATCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouSATCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATCsTwelveOmissionLTwoVarDecoderSamLite}{\tbd{miouSATCsTwelveOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouSATCsTwelveOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouSATCsTwelveOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouSATCsTwelveOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATCsTwelveOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATCsTwelveSTwocloudlessREAL}{\tbd{miouSATCsTwelveSTwocloudlessREAL}}
\providecommand{\miouSATCsTwelveShiftLOne}{\tbd{miouSATCsTwelveShiftLOne}}
\providecommand{\miouSATCsTwelveShiftLTwo}{\tbd{miouSATCsTwelveShiftLTwo}}
\providecommand{\miouSATCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouSATCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATCsTwelveShiftLTwoVarDecoderSamLite}{\tbd{miouSATCsTwelveShiftLTwoVarDecoderSamLite}}
\providecommand{\miouSATCsTwelveShiftLTwoVarDecoderSegformerMlp}{\tbd{miouSATCsTwelveShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouSATCsTwelveShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATCsTwelveShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATDfcBoundaryLOne}{\tbd{miouSATDfcBoundaryLOne}}
\providecommand{\miouSATDfcBoundaryLTwo}{\tbd{miouSATDfcBoundaryLTwo}}
\providecommand{\miouSATDfcBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouSATDfcBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATDfcBoundaryLTwoVarDecoderSamLite}{\tbd{miouSATDfcBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouSATDfcBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouSATDfcBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouSATDfcBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATDfcBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATDfcClean}{\tbd{miouSATDfcClean}}
\providecommand{\miouSATDfcCleanVarDecoderMaskTwoformerLite}{\tbd{miouSATDfcCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATDfcCleanVarDecoderSamLite}{\tbd{miouSATDfcCleanVarDecoderSamLite}}
\providecommand{\miouSATDfcCleanVarDecoderSegformerMlp}{\tbd{miouSATDfcCleanVarDecoderSegformerMlp}}
\providecommand{\miouSATDfcCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATDfcCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATDfcCleanVarTrainSubsetRealcov}{\tbd{miouSATDfcCleanVarTrainSubsetRealcov}}
\providecommand{\miouSATDfcCoarseLOne}{\tbd{miouSATDfcCoarseLOne}}
\providecommand{\miouSATDfcCoarseLTwo}{\tbd{miouSATDfcCoarseLTwo}}
\providecommand{\miouSATDfcCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouSATDfcCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATDfcCoarseLTwoVarDecoderSamLite}{\tbd{miouSATDfcCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouSATDfcCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouSATDfcCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouSATDfcCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATDfcCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATDfcModisREALVarTrainSubsetRealcov}{\tbd{miouSATDfcModisREALVarTrainSubsetRealcov}}
\providecommand{\miouSATDfcOmissionLOne}{\tbd{miouSATDfcOmissionLOne}}
\providecommand{\miouSATDfcOmissionLTwo}{\tbd{miouSATDfcOmissionLTwo}}
\providecommand{\miouSATDfcOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouSATDfcOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATDfcOmissionLTwoVarDecoderSamLite}{\tbd{miouSATDfcOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouSATDfcOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouSATDfcOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouSATDfcOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATDfcOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATDfcShiftLOne}{\tbd{miouSATDfcShiftLOne}}
\providecommand{\miouSATDfcShiftLTwo}{\tbd{miouSATDfcShiftLTwo}}
\providecommand{\miouSATDfcShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouSATDfcShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATDfcShiftLTwoVarDecoderSamLite}{\tbd{miouSATDfcShiftLTwoVarDecoderSamLite}}
\providecommand{\miouSATDfcShiftLTwoVarDecoderSegformerMlp}{\tbd{miouSATDfcShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouSATDfcShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATDfcShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATEnvaBoundaryLOne}{\tbd{miouSATEnvaBoundaryLOne}}
\providecommand{\miouSATEnvaBoundaryLTwo}{\tbd{miouSATEnvaBoundaryLTwo}}
\providecommand{\miouSATEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouSATEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATEnvaBoundaryLTwoVarDecoderSamLite}{\tbd{miouSATEnvaBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouSATEnvaBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouSATEnvaBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouSATEnvaBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATEnvaBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATEnvaClean}{\tbd{miouSATEnvaClean}}
\providecommand{\miouSATEnvaCleanVarDecoderMaskTwoformerLite}{\tbd{miouSATEnvaCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATEnvaCleanVarDecoderSamLite}{\tbd{miouSATEnvaCleanVarDecoderSamLite}}
\providecommand{\miouSATEnvaCleanVarDecoderSegformerMlp}{\tbd{miouSATEnvaCleanVarDecoderSegformerMlp}}
\providecommand{\miouSATEnvaCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATEnvaCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATEnvaCoarseLOne}{\tbd{miouSATEnvaCoarseLOne}}
\providecommand{\miouSATEnvaCoarseLTwo}{\tbd{miouSATEnvaCoarseLTwo}}
\providecommand{\miouSATEnvaCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouSATEnvaCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATEnvaCoarseLTwoVarDecoderSamLite}{\tbd{miouSATEnvaCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouSATEnvaCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouSATEnvaCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouSATEnvaCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATEnvaCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATEnvaNlcdREAL}{\tbd{miouSATEnvaNlcdREAL}}
\providecommand{\miouSATEnvaOmissionLOne}{\tbd{miouSATEnvaOmissionLOne}}
\providecommand{\miouSATEnvaOmissionLTwo}{\tbd{miouSATEnvaOmissionLTwo}}
\providecommand{\miouSATEnvaOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouSATEnvaOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATEnvaOmissionLTwoVarDecoderSamLite}{\tbd{miouSATEnvaOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouSATEnvaOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouSATEnvaOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouSATEnvaOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATEnvaOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATEnvaShiftLOne}{\tbd{miouSATEnvaShiftLOne}}
\providecommand{\miouSATEnvaShiftLTwo}{\tbd{miouSATEnvaShiftLTwo}}
\providecommand{\miouSATEnvaShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouSATEnvaShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATEnvaShiftLTwoVarDecoderSamLite}{\tbd{miouSATEnvaShiftLTwoVarDecoderSamLite}}
\providecommand{\miouSATEnvaShiftLTwoVarDecoderSegformerMlp}{\tbd{miouSATEnvaShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouSATEnvaShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATEnvaShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATKuroBoundaryLOne}{\tbd{miouSATKuroBoundaryLOne}}
\providecommand{\miouSATKuroBoundaryLTwo}{\tbd{miouSATKuroBoundaryLTwo}}
\providecommand{\miouSATKuroBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouSATKuroBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATKuroBoundaryLTwoVarDecoderSamLite}{\tbd{miouSATKuroBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouSATKuroBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouSATKuroBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouSATKuroBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATKuroBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATKuroCemsREALVarTrainSubsetRealcov}{\tbd{miouSATKuroCemsREALVarTrainSubsetRealcov}}
\providecommand{\miouSATKuroClean}{\tbd{miouSATKuroClean}}
\providecommand{\miouSATKuroCleanVarDecoderMaskTwoformerLite}{\tbd{miouSATKuroCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATKuroCleanVarDecoderSamLite}{\tbd{miouSATKuroCleanVarDecoderSamLite}}
\providecommand{\miouSATKuroCleanVarDecoderSegformerMlp}{\tbd{miouSATKuroCleanVarDecoderSegformerMlp}}
\providecommand{\miouSATKuroCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATKuroCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATKuroCleanVarTrainSubsetRealcov}{\tbd{miouSATKuroCleanVarTrainSubsetRealcov}}
\providecommand{\miouSATKuroCoarseLOne}{\tbd{miouSATKuroCoarseLOne}}
\providecommand{\miouSATKuroCoarseLTwo}{\tbd{miouSATKuroCoarseLTwo}}
\providecommand{\miouSATKuroCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouSATKuroCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATKuroCoarseLTwoVarDecoderSamLite}{\tbd{miouSATKuroCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouSATKuroCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouSATKuroCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouSATKuroCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATKuroCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATKuroOmissionLOne}{\tbd{miouSATKuroOmissionLOne}}
\providecommand{\miouSATKuroOmissionLTwo}{\tbd{miouSATKuroOmissionLTwo}}
\providecommand{\miouSATKuroOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouSATKuroOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATKuroOmissionLTwoVarDecoderSamLite}{\tbd{miouSATKuroOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouSATKuroOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouSATKuroOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouSATKuroOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATKuroOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATKuroShiftLOne}{\tbd{miouSATKuroShiftLOne}}
\providecommand{\miouSATKuroShiftLTwo}{\tbd{miouSATKuroShiftLTwo}}
\providecommand{\miouSATKuroShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouSATKuroShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATKuroShiftLTwoVarDecoderSamLite}{\tbd{miouSATKuroShiftLTwoVarDecoderSamLite}}
\providecommand{\miouSATKuroShiftLTwoVarDecoderSegformerMlp}{\tbd{miouSATKuroShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouSATKuroShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATKuroShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATOemBoundaryLOne}{\tbd{miouSATOemBoundaryLOne}}
\providecommand{\miouSATOemBoundaryLTwo}{\tbd{miouSATOemBoundaryLTwo}}
\providecommand{\miouSATOemBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouSATOemBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATOemBoundaryLTwoVarDecoderSamLite}{\tbd{miouSATOemBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouSATOemBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouSATOemBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouSATOemBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATOemBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATOemClean}{\tbd{miouSATOemClean}}
\providecommand{\miouSATOemCleanVarDecoderMaskTwoformerLite}{\tbd{miouSATOemCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATOemCleanVarDecoderSamLite}{\tbd{miouSATOemCleanVarDecoderSamLite}}
\providecommand{\miouSATOemCleanVarDecoderSegformerMlp}{\tbd{miouSATOemCleanVarDecoderSegformerMlp}}
\providecommand{\miouSATOemCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATOemCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATOemCoarseLOne}{\tbd{miouSATOemCoarseLOne}}
\providecommand{\miouSATOemCoarseLTwo}{\tbd{miouSATOemCoarseLTwo}}
\providecommand{\miouSATOemCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouSATOemCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATOemCoarseLTwoVarDecoderSamLite}{\tbd{miouSATOemCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouSATOemCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouSATOemCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouSATOemCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATOemCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATOemOmissionLOne}{\tbd{miouSATOemOmissionLOne}}
\providecommand{\miouSATOemOmissionLTwo}{\tbd{miouSATOemOmissionLTwo}}
\providecommand{\miouSATOemOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouSATOemOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATOemOmissionLTwoVarDecoderSamLite}{\tbd{miouSATOemOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouSATOemOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouSATOemOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouSATOemOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATOemOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATOemShiftLOne}{\tbd{miouSATOemShiftLOne}}
\providecommand{\miouSATOemShiftLTwo}{\tbd{miouSATOemShiftLTwo}}
\providecommand{\miouSATOemShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouSATOemShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATOemShiftLTwoVarDecoderSamLite}{\tbd{miouSATOemShiftLTwoVarDecoderSamLite}}
\providecommand{\miouSATOemShiftLTwoVarDecoderSegformerMlp}{\tbd{miouSATOemShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouSATOemShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATOemShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATSnTwoBoundaryLOne}{\tbd{miouSATSnTwoBoundaryLOne}}
\providecommand{\miouSATSnTwoBoundaryLTwo}{\tbd{miouSATSnTwoBoundaryLTwo}}
\providecommand{\miouSATSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouSATSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATSnTwoBoundaryLTwoVarDecoderSamLite}{\tbd{miouSATSnTwoBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouSATSnTwoBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouSATSnTwoBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouSATSnTwoBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATSnTwoBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATSnTwoClean}{\tbd{miouSATSnTwoClean}}
\providecommand{\miouSATSnTwoCleanVarDecoderMaskTwoformerLite}{\tbd{miouSATSnTwoCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATSnTwoCleanVarDecoderSamLite}{\tbd{miouSATSnTwoCleanVarDecoderSamLite}}
\providecommand{\miouSATSnTwoCleanVarDecoderSegformerMlp}{\tbd{miouSATSnTwoCleanVarDecoderSegformerMlp}}
\providecommand{\miouSATSnTwoCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATSnTwoCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATSnTwoCoarseLOne}{\tbd{miouSATSnTwoCoarseLOne}}
\providecommand{\miouSATSnTwoCoarseLTwo}{\tbd{miouSATSnTwoCoarseLTwo}}
\providecommand{\miouSATSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouSATSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATSnTwoCoarseLTwoVarDecoderSamLite}{\tbd{miouSATSnTwoCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouSATSnTwoCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouSATSnTwoCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouSATSnTwoCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATSnTwoCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATSnTwoOmissionLOne}{\tbd{miouSATSnTwoOmissionLOne}}
\providecommand{\miouSATSnTwoOmissionLTwo}{\tbd{miouSATSnTwoOmissionLTwo}}
\providecommand{\miouSATSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouSATSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATSnTwoOmissionLTwoVarDecoderSamLite}{\tbd{miouSATSnTwoOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouSATSnTwoOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouSATSnTwoOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouSATSnTwoOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATSnTwoOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATSnTwoShiftLOne}{\tbd{miouSATSnTwoShiftLOne}}
\providecommand{\miouSATSnTwoShiftLTwo}{\tbd{miouSATSnTwoShiftLTwo}}
\providecommand{\miouSATSnTwoShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouSATSnTwoShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATSnTwoShiftLTwoVarDecoderSamLite}{\tbd{miouSATSnTwoShiftLTwoVarDecoderSamLite}}
\providecommand{\miouSATSnTwoShiftLTwoVarDecoderSegformerMlp}{\tbd{miouSATSnTwoShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouSATSnTwoShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATSnTwoShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATburnBoundaryLOne}{\tbd{miouSATburnBoundaryLOne}}
\providecommand{\miouSATburnBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{miouSATburnBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouSATburnBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{miouSATburnBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATburnBoundaryLOneVarDecoderSamLite}{\tbd{miouSATburnBoundaryLOneVarDecoderSamLite}}
\providecommand{\miouSATburnBoundaryLOneVarDecoderSamPretrained}{\tbd{miouSATburnBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\miouSATburnBoundaryLOneVarDecoderSegformerMlp}{\tbd{miouSATburnBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\miouSATburnBoundaryLR}{\tbd{miouSATburnBoundaryLR}}
\providecommand{\miouSATburnBoundaryLRVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATburnBoundaryLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATburnBoundaryLTwo}{\tbd{miouSATburnBoundaryLTwo}}
\providecommand{\miouSATburnBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{miouSATburnBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouSATburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{miouSATburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATburnBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouSATburnBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouSATburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATburnBoundaryLTwoVarDecoderSamLite}{\tbd{miouSATburnBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouSATburnBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouSATburnBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATburnBoundaryLTwoVarDecoderSamPretrained}{\tbd{miouSATburnBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\miouSATburnBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{miouSATburnBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATburnBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouSATburnBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouSATburnBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{miouSATburnBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATburnBoundaryLTwoVarFrozenEncoderTrue}{\tbd{miouSATburnBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\miouSATburnBoundaryLTwoVarLossBootstrap}{\tbd{miouSATburnBoundaryLTwoVarLossBootstrap}}
\providecommand{\miouSATburnBoundaryLTwoVarLossGce}{\tbd{miouSATburnBoundaryLTwoVarLossGce}}
\providecommand{\miouSATburnBoundaryLTwoVarLrMultThree}{\tbd{miouSATburnBoundaryLTwoVarLrMultThree}}
\providecommand{\miouSATburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATburnBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouSATburnBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouSATburnBoundaryLTwoVarValLabelsClean}{\tbd{miouSATburnBoundaryLTwoVarValLabelsClean}}
\providecommand{\miouSATburnClean}{\tbd{miouSATburnClean}}
\providecommand{\miouSATburnCleanVarDecoderMaskTwoformerFull}{\tbd{miouSATburnCleanVarDecoderMaskTwoformerFull}}
\providecommand{\miouSATburnCleanVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{miouSATburnCleanVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATburnCleanVarDecoderMaskTwoformerLite}{\tbd{miouSATburnCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATburnCleanVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouSATburnCleanVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATburnCleanVarDecoderSamLite}{\tbd{miouSATburnCleanVarDecoderSamLite}}
\providecommand{\miouSATburnCleanVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouSATburnCleanVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATburnCleanVarDecoderSamPretrained}{\tbd{miouSATburnCleanVarDecoderSamPretrained}}
\providecommand{\miouSATburnCleanVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{miouSATburnCleanVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATburnCleanVarDecoderSegformerMlp}{\tbd{miouSATburnCleanVarDecoderSegformerMlp}}
\providecommand{\miouSATburnCleanVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{miouSATburnCleanVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATburnCleanVarFrozenEncoderTrue}{\tbd{miouSATburnCleanVarFrozenEncoderTrue}}
\providecommand{\miouSATburnCleanVarLossBootstrap}{\tbd{miouSATburnCleanVarLossBootstrap}}
\providecommand{\miouSATburnCleanVarLossGce}{\tbd{miouSATburnCleanVarLossGce}}
\providecommand{\miouSATburnCleanVarLrMultThree}{\tbd{miouSATburnCleanVarLrMultThree}}
\providecommand{\miouSATburnCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATburnCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATburnCleanVarTrainSubsetCleanTwoFive}{\tbd{miouSATburnCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\miouSATburnCleanVarValLabelsClean}{\tbd{miouSATburnCleanVarValLabelsClean}}
\providecommand{\miouSATburnCoarseLOne}{\tbd{miouSATburnCoarseLOne}}
\providecommand{\miouSATburnCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{miouSATburnCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouSATburnCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{miouSATburnCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATburnCoarseLOneVarDecoderSamLite}{\tbd{miouSATburnCoarseLOneVarDecoderSamLite}}
\providecommand{\miouSATburnCoarseLOneVarDecoderSamPretrained}{\tbd{miouSATburnCoarseLOneVarDecoderSamPretrained}}
\providecommand{\miouSATburnCoarseLOneVarDecoderSegformerMlp}{\tbd{miouSATburnCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\miouSATburnCoarseLR}{\tbd{miouSATburnCoarseLR}}
\providecommand{\miouSATburnCoarseLRVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATburnCoarseLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATburnCoarseLTwo}{\tbd{miouSATburnCoarseLTwo}}
\providecommand{\miouSATburnCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{miouSATburnCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouSATburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{miouSATburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATburnCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouSATburnCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouSATburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATburnCoarseLTwoVarDecoderSamLite}{\tbd{miouSATburnCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouSATburnCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouSATburnCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATburnCoarseLTwoVarDecoderSamPretrained}{\tbd{miouSATburnCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\miouSATburnCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{miouSATburnCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATburnCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouSATburnCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouSATburnCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{miouSATburnCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATburnCoarseLTwoVarEarlyStoppingFalse}{\tbd{miouSATburnCoarseLTwoVarEarlyStoppingFalse}}
\providecommand{\miouSATburnCoarseLTwoVarEarlyStoppingFalseFrozenEncoderTrue}{\tbd{miouSATburnCoarseLTwoVarEarlyStoppingFalseFrozenEncoderTrue}}
\providecommand{\miouSATburnCoarseLTwoVarFrozenEncoderTrue}{\tbd{miouSATburnCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\miouSATburnCoarseLTwoVarLossBootstrap}{\tbd{miouSATburnCoarseLTwoVarLossBootstrap}}
\providecommand{\miouSATburnCoarseLTwoVarLossGce}{\tbd{miouSATburnCoarseLTwoVarLossGce}}
\providecommand{\miouSATburnCoarseLTwoVarLrMultThree}{\tbd{miouSATburnCoarseLTwoVarLrMultThree}}
\providecommand{\miouSATburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATburnCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouSATburnCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouSATburnCoarseLTwoVarValLabelsClean}{\tbd{miouSATburnCoarseLTwoVarValLabelsClean}}
\providecommand{\miouSATburnOmissionLOne}{\tbd{miouSATburnOmissionLOne}}
\providecommand{\miouSATburnOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{miouSATburnOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouSATburnOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{miouSATburnOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATburnOmissionLOneVarDecoderSamLite}{\tbd{miouSATburnOmissionLOneVarDecoderSamLite}}
\providecommand{\miouSATburnOmissionLOneVarDecoderSamPretrained}{\tbd{miouSATburnOmissionLOneVarDecoderSamPretrained}}
\providecommand{\miouSATburnOmissionLOneVarDecoderSegformerMlp}{\tbd{miouSATburnOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\miouSATburnOmissionLR}{\tbd{miouSATburnOmissionLR}}
\providecommand{\miouSATburnOmissionLRVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATburnOmissionLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATburnOmissionLTwo}{\tbd{miouSATburnOmissionLTwo}}
\providecommand{\miouSATburnOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{miouSATburnOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouSATburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{miouSATburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATburnOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouSATburnOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouSATburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATburnOmissionLTwoVarDecoderSamLite}{\tbd{miouSATburnOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouSATburnOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouSATburnOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATburnOmissionLTwoVarDecoderSamPretrained}{\tbd{miouSATburnOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\miouSATburnOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{miouSATburnOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATburnOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouSATburnOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouSATburnOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{miouSATburnOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATburnOmissionLTwoVarFrozenEncoderTrue}{\tbd{miouSATburnOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\miouSATburnOmissionLTwoVarLossBootstrap}{\tbd{miouSATburnOmissionLTwoVarLossBootstrap}}
\providecommand{\miouSATburnOmissionLTwoVarLossGce}{\tbd{miouSATburnOmissionLTwoVarLossGce}}
\providecommand{\miouSATburnOmissionLTwoVarLrMultThree}{\tbd{miouSATburnOmissionLTwoVarLrMultThree}}
\providecommand{\miouSATburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATburnOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouSATburnOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouSATburnOmissionLTwoVarValLabelsClean}{\tbd{miouSATburnOmissionLTwoVarValLabelsClean}}
\providecommand{\miouSATburnShiftLOne}{\tbd{miouSATburnShiftLOne}}
\providecommand{\miouSATburnShiftLOneVarDecoderMaskTwoformerFull}{\tbd{miouSATburnShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouSATburnShiftLOneVarDecoderMaskTwoformerLite}{\tbd{miouSATburnShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATburnShiftLOneVarDecoderSamLite}{\tbd{miouSATburnShiftLOneVarDecoderSamLite}}
\providecommand{\miouSATburnShiftLOneVarDecoderSamPretrained}{\tbd{miouSATburnShiftLOneVarDecoderSamPretrained}}
\providecommand{\miouSATburnShiftLOneVarDecoderSegformerMlp}{\tbd{miouSATburnShiftLOneVarDecoderSegformerMlp}}
\providecommand{\miouSATburnShiftLR}{\tbd{miouSATburnShiftLR}}
\providecommand{\miouSATburnShiftLRVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATburnShiftLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATburnShiftLTwo}{\tbd{miouSATburnShiftLTwo}}
\providecommand{\miouSATburnShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{miouSATburnShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouSATburnShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{miouSATburnShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATburnShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouSATburnShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouSATburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATburnShiftLTwoVarDecoderSamLite}{\tbd{miouSATburnShiftLTwoVarDecoderSamLite}}
\providecommand{\miouSATburnShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouSATburnShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATburnShiftLTwoVarDecoderSamPretrained}{\tbd{miouSATburnShiftLTwoVarDecoderSamPretrained}}
\providecommand{\miouSATburnShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{miouSATburnShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATburnShiftLTwoVarDecoderSegformerMlp}{\tbd{miouSATburnShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouSATburnShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{miouSATburnShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATburnShiftLTwoVarFrozenEncoderTrue}{\tbd{miouSATburnShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\miouSATburnShiftLTwoVarLossBootstrap}{\tbd{miouSATburnShiftLTwoVarLossBootstrap}}
\providecommand{\miouSATburnShiftLTwoVarLossGce}{\tbd{miouSATburnShiftLTwoVarLossGce}}
\providecommand{\miouSATburnShiftLTwoVarLrMultThree}{\tbd{miouSATburnShiftLTwoVarLrMultThree}}
\providecommand{\miouSATburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATburnShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouSATburnShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouSATburnShiftLTwoVarValLabelsClean}{\tbd{miouSATburnShiftLTwoVarValLabelsClean}}
\providecommand{\miouSATflairBoundaryLOne}{\tbd{miouSATflairBoundaryLOne}}
\providecommand{\miouSATflairBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{miouSATflairBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouSATflairBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{miouSATflairBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATflairBoundaryLOneVarDecoderSamLite}{\tbd{miouSATflairBoundaryLOneVarDecoderSamLite}}
\providecommand{\miouSATflairBoundaryLOneVarDecoderSamPretrained}{\tbd{miouSATflairBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\miouSATflairBoundaryLOneVarDecoderSegformerMlp}{\tbd{miouSATflairBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\miouSATflairBoundaryLR}{\tbd{miouSATflairBoundaryLR}}
\providecommand{\miouSATflairBoundaryLRVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATflairBoundaryLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATflairBoundaryLTwo}{\tbd{miouSATflairBoundaryLTwo}}
\providecommand{\miouSATflairBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{miouSATflairBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouSATflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{miouSATflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATflairBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouSATflairBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouSATflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATflairBoundaryLTwoVarDecoderSamLite}{\tbd{miouSATflairBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouSATflairBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouSATflairBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATflairBoundaryLTwoVarDecoderSamPretrained}{\tbd{miouSATflairBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\miouSATflairBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{miouSATflairBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATflairBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouSATflairBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouSATflairBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{miouSATflairBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATflairBoundaryLTwoVarFrozenEncoderTrue}{\tbd{miouSATflairBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\miouSATflairBoundaryLTwoVarLossBootstrap}{\tbd{miouSATflairBoundaryLTwoVarLossBootstrap}}
\providecommand{\miouSATflairBoundaryLTwoVarLossGce}{\tbd{miouSATflairBoundaryLTwoVarLossGce}}
\providecommand{\miouSATflairBoundaryLTwoVarLrMultThree}{\tbd{miouSATflairBoundaryLTwoVarLrMultThree}}
\providecommand{\miouSATflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATflairBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouSATflairBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouSATflairBoundaryLTwoVarValLabelsClean}{\tbd{miouSATflairBoundaryLTwoVarValLabelsClean}}
\providecommand{\miouSATflairClean}{\tbd{miouSATflairClean}}
\providecommand{\miouSATflairCleanVarClassWeightedTrue}{\tbd{miouSATflairCleanVarClassWeightedTrue}}
\providecommand{\miouSATflairCleanVarDecoderMaskTwoformerFull}{\tbd{miouSATflairCleanVarDecoderMaskTwoformerFull}}
\providecommand{\miouSATflairCleanVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{miouSATflairCleanVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATflairCleanVarDecoderMaskTwoformerLite}{\tbd{miouSATflairCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATflairCleanVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouSATflairCleanVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATflairCleanVarDecoderSamLite}{\tbd{miouSATflairCleanVarDecoderSamLite}}
\providecommand{\miouSATflairCleanVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouSATflairCleanVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATflairCleanVarDecoderSamPretrained}{\tbd{miouSATflairCleanVarDecoderSamPretrained}}
\providecommand{\miouSATflairCleanVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{miouSATflairCleanVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATflairCleanVarDecoderSegformerMlp}{\tbd{miouSATflairCleanVarDecoderSegformerMlp}}
\providecommand{\miouSATflairCleanVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{miouSATflairCleanVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATflairCleanVarFrozenEncoderTrue}{\tbd{miouSATflairCleanVarFrozenEncoderTrue}}
\providecommand{\miouSATflairCleanVarLossBootstrap}{\tbd{miouSATflairCleanVarLossBootstrap}}
\providecommand{\miouSATflairCleanVarLossGce}{\tbd{miouSATflairCleanVarLossGce}}
\providecommand{\miouSATflairCleanVarLrMultThree}{\tbd{miouSATflairCleanVarLrMultThree}}
\providecommand{\miouSATflairCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATflairCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATflairCleanVarTrainSubsetCleanTwoFive}{\tbd{miouSATflairCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\miouSATflairCleanVarValLabelsClean}{\tbd{miouSATflairCleanVarValLabelsClean}}
\providecommand{\miouSATflairCoarseLOne}{\tbd{miouSATflairCoarseLOne}}
\providecommand{\miouSATflairCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{miouSATflairCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouSATflairCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{miouSATflairCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATflairCoarseLOneVarDecoderSamLite}{\tbd{miouSATflairCoarseLOneVarDecoderSamLite}}
\providecommand{\miouSATflairCoarseLOneVarDecoderSamPretrained}{\tbd{miouSATflairCoarseLOneVarDecoderSamPretrained}}
\providecommand{\miouSATflairCoarseLOneVarDecoderSegformerMlp}{\tbd{miouSATflairCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\miouSATflairCoarseLR}{\tbd{miouSATflairCoarseLR}}
\providecommand{\miouSATflairCoarseLRVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATflairCoarseLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATflairCoarseLTwo}{\tbd{miouSATflairCoarseLTwo}}
\providecommand{\miouSATflairCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{miouSATflairCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouSATflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{miouSATflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATflairCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouSATflairCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouSATflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATflairCoarseLTwoVarDecoderSamLite}{\tbd{miouSATflairCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouSATflairCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouSATflairCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATflairCoarseLTwoVarDecoderSamPretrained}{\tbd{miouSATflairCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\miouSATflairCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{miouSATflairCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATflairCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouSATflairCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouSATflairCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{miouSATflairCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATflairCoarseLTwoVarFrozenEncoderTrue}{\tbd{miouSATflairCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\miouSATflairCoarseLTwoVarLossBootstrap}{\tbd{miouSATflairCoarseLTwoVarLossBootstrap}}
\providecommand{\miouSATflairCoarseLTwoVarLossGce}{\tbd{miouSATflairCoarseLTwoVarLossGce}}
\providecommand{\miouSATflairCoarseLTwoVarLrMultThree}{\tbd{miouSATflairCoarseLTwoVarLrMultThree}}
\providecommand{\miouSATflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATflairCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouSATflairCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouSATflairCoarseLTwoVarValLabelsClean}{\tbd{miouSATflairCoarseLTwoVarValLabelsClean}}
\providecommand{\miouSATflairOmissionLOne}{\tbd{miouSATflairOmissionLOne}}
\providecommand{\miouSATflairOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{miouSATflairOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouSATflairOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{miouSATflairOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATflairOmissionLOneVarDecoderSamLite}{\tbd{miouSATflairOmissionLOneVarDecoderSamLite}}
\providecommand{\miouSATflairOmissionLOneVarDecoderSamPretrained}{\tbd{miouSATflairOmissionLOneVarDecoderSamPretrained}}
\providecommand{\miouSATflairOmissionLOneVarDecoderSegformerMlp}{\tbd{miouSATflairOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\miouSATflairOmissionLR}{\tbd{miouSATflairOmissionLR}}
\providecommand{\miouSATflairOmissionLRVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATflairOmissionLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATflairOmissionLTwo}{\tbd{miouSATflairOmissionLTwo}}
\providecommand{\miouSATflairOmissionLTwoVarClassWeightedTrue}{\tbd{miouSATflairOmissionLTwoVarClassWeightedTrue}}
\providecommand{\miouSATflairOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{miouSATflairOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouSATflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{miouSATflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATflairOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouSATflairOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouSATflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATflairOmissionLTwoVarDecoderSamLite}{\tbd{miouSATflairOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouSATflairOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouSATflairOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATflairOmissionLTwoVarDecoderSamPretrained}{\tbd{miouSATflairOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\miouSATflairOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{miouSATflairOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATflairOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouSATflairOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouSATflairOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{miouSATflairOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATflairOmissionLTwoVarEarlyStoppingFalse}{\tbd{miouSATflairOmissionLTwoVarEarlyStoppingFalse}}
\providecommand{\miouSATflairOmissionLTwoVarEarlyStoppingFalseFrozenEncoderTrue}{\tbd{miouSATflairOmissionLTwoVarEarlyStoppingFalseFrozenEncoderTrue}}
\providecommand{\miouSATflairOmissionLTwoVarFrozenEncoderTrue}{\tbd{miouSATflairOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\miouSATflairOmissionLTwoVarLossBootstrap}{\tbd{miouSATflairOmissionLTwoVarLossBootstrap}}
\providecommand{\miouSATflairOmissionLTwoVarLossGce}{\tbd{miouSATflairOmissionLTwoVarLossGce}}
\providecommand{\miouSATflairOmissionLTwoVarLrMultThree}{\tbd{miouSATflairOmissionLTwoVarLrMultThree}}
\providecommand{\miouSATflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATflairOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouSATflairOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouSATflairOmissionLTwoVarValLabelsClean}{\tbd{miouSATflairOmissionLTwoVarValLabelsClean}}
\providecommand{\miouSATflairShiftLOne}{\tbd{miouSATflairShiftLOne}}
\providecommand{\miouSATflairShiftLOneVarDecoderMaskTwoformerFull}{\tbd{miouSATflairShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouSATflairShiftLOneVarDecoderMaskTwoformerLite}{\tbd{miouSATflairShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATflairShiftLOneVarDecoderSamLite}{\tbd{miouSATflairShiftLOneVarDecoderSamLite}}
\providecommand{\miouSATflairShiftLOneVarDecoderSamPretrained}{\tbd{miouSATflairShiftLOneVarDecoderSamPretrained}}
\providecommand{\miouSATflairShiftLOneVarDecoderSegformerMlp}{\tbd{miouSATflairShiftLOneVarDecoderSegformerMlp}}
\providecommand{\miouSATflairShiftLR}{\tbd{miouSATflairShiftLR}}
\providecommand{\miouSATflairShiftLRVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATflairShiftLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATflairShiftLTwo}{\tbd{miouSATflairShiftLTwo}}
\providecommand{\miouSATflairShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{miouSATflairShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouSATflairShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{miouSATflairShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATflairShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouSATflairShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouSATflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouSATflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATflairShiftLTwoVarDecoderSamLite}{\tbd{miouSATflairShiftLTwoVarDecoderSamLite}}
\providecommand{\miouSATflairShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{miouSATflairShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATflairShiftLTwoVarDecoderSamPretrained}{\tbd{miouSATflairShiftLTwoVarDecoderSamPretrained}}
\providecommand{\miouSATflairShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{miouSATflairShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATflairShiftLTwoVarDecoderSegformerMlp}{\tbd{miouSATflairShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouSATflairShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{miouSATflairShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATflairShiftLTwoVarFrozenEncoderTrue}{\tbd{miouSATflairShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\miouSATflairShiftLTwoVarLossBootstrap}{\tbd{miouSATflairShiftLTwoVarLossBootstrap}}
\providecommand{\miouSATflairShiftLTwoVarLossGce}{\tbd{miouSATflairShiftLTwoVarLossGce}}
\providecommand{\miouSATflairShiftLTwoVarLrMultThree}{\tbd{miouSATflairShiftLTwoVarLrMultThree}}
\providecommand{\miouSATflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouSATflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouSATflairShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouSATflairShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouSATflairShiftLTwoVarValLabelsClean}{\tbd{miouSATflairShiftLTwoVarValLabelsClean}}
\providecommand{\miouSATsenClean}{\tbd{miouSATsenClean}}
\providecommand{\miouSATsenOtsuLTwo}{\tbd{miouSATsenOtsuLTwo}}
\providecommand{\miouTMChesBoundaryLOne}{\tbd{miouTMChesBoundaryLOne}}
\providecommand{\miouTMChesBoundaryLTwo}{\tbd{miouTMChesBoundaryLTwo}}
\providecommand{\miouTMChesClean}{\tbd{miouTMChesClean}}
\providecommand{\miouTMChesCoarseLOne}{\tbd{miouTMChesCoarseLOne}}
\providecommand{\miouTMChesCoarseLTwo}{\tbd{miouTMChesCoarseLTwo}}
\providecommand{\miouTMChesNlcdREAL}{\tbd{miouTMChesNlcdREAL}}
\providecommand{\miouTMChesOmissionLOne}{\tbd{miouTMChesOmissionLOne}}
\providecommand{\miouTMChesOmissionLTwo}{\tbd{miouTMChesOmissionLTwo}}
\providecommand{\miouTMChesShiftLOne}{\tbd{miouTMChesShiftLOne}}
\providecommand{\miouTMChesShiftLTwo}{\tbd{miouTMChesShiftLTwo}}
\providecommand{\miouTMCsTwelveBoundaryLOne}{\tbd{miouTMCsTwelveBoundaryLOne}}
\providecommand{\miouTMCsTwelveBoundaryLTwo}{\tbd{miouTMCsTwelveBoundaryLTwo}}
\providecommand{\miouTMCsTwelveClean}{\tbd{miouTMCsTwelveClean}}
\providecommand{\miouTMCsTwelveCoarseLOne}{\tbd{miouTMCsTwelveCoarseLOne}}
\providecommand{\miouTMCsTwelveCoarseLTwo}{\tbd{miouTMCsTwelveCoarseLTwo}}
\providecommand{\miouTMCsTwelveOmissionLOne}{\tbd{miouTMCsTwelveOmissionLOne}}
\providecommand{\miouTMCsTwelveOmissionLTwo}{\tbd{miouTMCsTwelveOmissionLTwo}}
\providecommand{\miouTMCsTwelveSTwocloudlessREAL}{\tbd{miouTMCsTwelveSTwocloudlessREAL}}
\providecommand{\miouTMCsTwelveShiftLOne}{\tbd{miouTMCsTwelveShiftLOne}}
\providecommand{\miouTMCsTwelveShiftLTwo}{\tbd{miouTMCsTwelveShiftLTwo}}
\providecommand{\miouTMDfcBoundaryLOne}{\tbd{miouTMDfcBoundaryLOne}}
\providecommand{\miouTMDfcBoundaryLTwo}{\tbd{miouTMDfcBoundaryLTwo}}
\providecommand{\miouTMDfcClean}{\tbd{miouTMDfcClean}}
\providecommand{\miouTMDfcCleanVarTrainSubsetRealcov}{\tbd{miouTMDfcCleanVarTrainSubsetRealcov}}
\providecommand{\miouTMDfcCoarseLOne}{\tbd{miouTMDfcCoarseLOne}}
\providecommand{\miouTMDfcCoarseLTwo}{\tbd{miouTMDfcCoarseLTwo}}
\providecommand{\miouTMDfcModisREALVarTrainSubsetRealcov}{\tbd{miouTMDfcModisREALVarTrainSubsetRealcov}}
\providecommand{\miouTMDfcOmissionLOne}{\tbd{miouTMDfcOmissionLOne}}
\providecommand{\miouTMDfcOmissionLTwo}{\tbd{miouTMDfcOmissionLTwo}}
\providecommand{\miouTMDfcShiftLOne}{\tbd{miouTMDfcShiftLOne}}
\providecommand{\miouTMDfcShiftLTwo}{\tbd{miouTMDfcShiftLTwo}}
\providecommand{\miouTMEnvaBoundaryLOne}{\tbd{miouTMEnvaBoundaryLOne}}
\providecommand{\miouTMEnvaBoundaryLTwo}{\tbd{miouTMEnvaBoundaryLTwo}}
\providecommand{\miouTMEnvaClean}{\tbd{miouTMEnvaClean}}
\providecommand{\miouTMEnvaCoarseLOne}{\tbd{miouTMEnvaCoarseLOne}}
\providecommand{\miouTMEnvaCoarseLTwo}{\tbd{miouTMEnvaCoarseLTwo}}
\providecommand{\miouTMEnvaNlcdREAL}{\tbd{miouTMEnvaNlcdREAL}}
\providecommand{\miouTMEnvaOmissionLOne}{\tbd{miouTMEnvaOmissionLOne}}
\providecommand{\miouTMEnvaOmissionLTwo}{\tbd{miouTMEnvaOmissionLTwo}}
\providecommand{\miouTMEnvaShiftLOne}{\tbd{miouTMEnvaShiftLOne}}
\providecommand{\miouTMEnvaShiftLTwo}{\tbd{miouTMEnvaShiftLTwo}}
\providecommand{\miouTMKuroBoundaryLOne}{\tbd{miouTMKuroBoundaryLOne}}
\providecommand{\miouTMKuroBoundaryLTwo}{\tbd{miouTMKuroBoundaryLTwo}}
\providecommand{\miouTMKuroCemsREALVarTrainSubsetRealcov}{\tbd{miouTMKuroCemsREALVarTrainSubsetRealcov}}
\providecommand{\miouTMKuroClean}{\tbd{miouTMKuroClean}}
\providecommand{\miouTMKuroCleanVarTrainSubsetRealcov}{\tbd{miouTMKuroCleanVarTrainSubsetRealcov}}
\providecommand{\miouTMKuroCoarseLOne}{\tbd{miouTMKuroCoarseLOne}}
\providecommand{\miouTMKuroCoarseLTwo}{\tbd{miouTMKuroCoarseLTwo}}
\providecommand{\miouTMKuroOmissionLOne}{\tbd{miouTMKuroOmissionLOne}}
\providecommand{\miouTMKuroOmissionLTwo}{\tbd{miouTMKuroOmissionLTwo}}
\providecommand{\miouTMKuroShiftLOne}{\tbd{miouTMKuroShiftLOne}}
\providecommand{\miouTMKuroShiftLTwo}{\tbd{miouTMKuroShiftLTwo}}
\providecommand{\miouTMOemBoundaryLOne}{\tbd{miouTMOemBoundaryLOne}}
\providecommand{\miouTMOemBoundaryLTwo}{\tbd{miouTMOemBoundaryLTwo}}
\providecommand{\miouTMOemClean}{\tbd{miouTMOemClean}}
\providecommand{\miouTMOemCoarseLOne}{\tbd{miouTMOemCoarseLOne}}
\providecommand{\miouTMOemCoarseLTwo}{\tbd{miouTMOemCoarseLTwo}}
\providecommand{\miouTMOemOmissionLOne}{\tbd{miouTMOemOmissionLOne}}
\providecommand{\miouTMOemOmissionLTwo}{\tbd{miouTMOemOmissionLTwo}}
\providecommand{\miouTMOemShiftLOne}{\tbd{miouTMOemShiftLOne}}
\providecommand{\miouTMOemShiftLTwo}{\tbd{miouTMOemShiftLTwo}}
\providecommand{\miouTMSnTwoBoundaryLOne}{\tbd{miouTMSnTwoBoundaryLOne}}
\providecommand{\miouTMSnTwoBoundaryLTwo}{\tbd{miouTMSnTwoBoundaryLTwo}}
\providecommand{\miouTMSnTwoClean}{\tbd{miouTMSnTwoClean}}
\providecommand{\miouTMSnTwoCoarseLOne}{\tbd{miouTMSnTwoCoarseLOne}}
\providecommand{\miouTMSnTwoCoarseLTwo}{\tbd{miouTMSnTwoCoarseLTwo}}
\providecommand{\miouTMSnTwoOmissionLOne}{\tbd{miouTMSnTwoOmissionLOne}}
\providecommand{\miouTMSnTwoOmissionLTwo}{\tbd{miouTMSnTwoOmissionLTwo}}
\providecommand{\miouTMSnTwoShiftLOne}{\tbd{miouTMSnTwoShiftLOne}}
\providecommand{\miouTMSnTwoShiftLTwo}{\tbd{miouTMSnTwoShiftLTwo}}
\providecommand{\miouTMburnBoundaryLOne}{\tbd{miouTMburnBoundaryLOne}}
\providecommand{\miouTMburnBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{miouTMburnBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouTMburnBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{miouTMburnBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouTMburnBoundaryLOneVarDecoderSamLite}{\tbd{miouTMburnBoundaryLOneVarDecoderSamLite}}
\providecommand{\miouTMburnBoundaryLOneVarDecoderSamPretrained}{\tbd{miouTMburnBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\miouTMburnBoundaryLOneVarDecoderSegformerMlp}{\tbd{miouTMburnBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\miouTMburnBoundaryLR}{\tbd{miouTMburnBoundaryLR}}
\providecommand{\miouTMburnBoundaryLTwo}{\tbd{miouTMburnBoundaryLTwo}}
\providecommand{\miouTMburnBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{miouTMburnBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouTMburnBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouTMburnBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouTMburnBoundaryLTwoVarDecoderSamLite}{\tbd{miouTMburnBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouTMburnBoundaryLTwoVarDecoderSamPretrained}{\tbd{miouTMburnBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\miouTMburnBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouTMburnBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouTMburnBoundaryLTwoVarFrozenEncoderTrue}{\tbd{miouTMburnBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\miouTMburnBoundaryLTwoVarLossBootstrap}{\tbd{miouTMburnBoundaryLTwoVarLossBootstrap}}
\providecommand{\miouTMburnBoundaryLTwoVarLossGce}{\tbd{miouTMburnBoundaryLTwoVarLossGce}}
\providecommand{\miouTMburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouTMburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouTMburnBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouTMburnBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouTMburnClean}{\tbd{miouTMburnClean}}
\providecommand{\miouTMburnCleanVarDecoderMaskTwoformerFull}{\tbd{miouTMburnCleanVarDecoderMaskTwoformerFull}}
\providecommand{\miouTMburnCleanVarDecoderMaskTwoformerLite}{\tbd{miouTMburnCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouTMburnCleanVarDecoderSamLite}{\tbd{miouTMburnCleanVarDecoderSamLite}}
\providecommand{\miouTMburnCleanVarDecoderSamPretrained}{\tbd{miouTMburnCleanVarDecoderSamPretrained}}
\providecommand{\miouTMburnCleanVarDecoderSegformerMlp}{\tbd{miouTMburnCleanVarDecoderSegformerMlp}}
\providecommand{\miouTMburnCleanVarFrozenEncoderTrue}{\tbd{miouTMburnCleanVarFrozenEncoderTrue}}
\providecommand{\miouTMburnCleanVarLossBootstrap}{\tbd{miouTMburnCleanVarLossBootstrap}}
\providecommand{\miouTMburnCleanVarLossGce}{\tbd{miouTMburnCleanVarLossGce}}
\providecommand{\miouTMburnCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{miouTMburnCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouTMburnCleanVarTrainSubsetCleanTwoFive}{\tbd{miouTMburnCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\miouTMburnCoarseLOne}{\tbd{miouTMburnCoarseLOne}}
\providecommand{\miouTMburnCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{miouTMburnCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouTMburnCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{miouTMburnCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouTMburnCoarseLOneVarDecoderSamLite}{\tbd{miouTMburnCoarseLOneVarDecoderSamLite}}
\providecommand{\miouTMburnCoarseLOneVarDecoderSamPretrained}{\tbd{miouTMburnCoarseLOneVarDecoderSamPretrained}}
\providecommand{\miouTMburnCoarseLOneVarDecoderSegformerMlp}{\tbd{miouTMburnCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\miouTMburnCoarseLR}{\tbd{miouTMburnCoarseLR}}
\providecommand{\miouTMburnCoarseLTwo}{\tbd{miouTMburnCoarseLTwo}}
\providecommand{\miouTMburnCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{miouTMburnCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouTMburnCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouTMburnCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouTMburnCoarseLTwoVarDecoderSamLite}{\tbd{miouTMburnCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouTMburnCoarseLTwoVarDecoderSamPretrained}{\tbd{miouTMburnCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\miouTMburnCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouTMburnCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouTMburnCoarseLTwoVarFrozenEncoderTrue}{\tbd{miouTMburnCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\miouTMburnCoarseLTwoVarLossBootstrap}{\tbd{miouTMburnCoarseLTwoVarLossBootstrap}}
\providecommand{\miouTMburnCoarseLTwoVarLossGce}{\tbd{miouTMburnCoarseLTwoVarLossGce}}
\providecommand{\miouTMburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouTMburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouTMburnCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouTMburnCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouTMburnOmissionLOne}{\tbd{miouTMburnOmissionLOne}}
\providecommand{\miouTMburnOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{miouTMburnOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouTMburnOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{miouTMburnOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouTMburnOmissionLOneVarDecoderSamLite}{\tbd{miouTMburnOmissionLOneVarDecoderSamLite}}
\providecommand{\miouTMburnOmissionLOneVarDecoderSamPretrained}{\tbd{miouTMburnOmissionLOneVarDecoderSamPretrained}}
\providecommand{\miouTMburnOmissionLOneVarDecoderSegformerMlp}{\tbd{miouTMburnOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\miouTMburnOmissionLR}{\tbd{miouTMburnOmissionLR}}
\providecommand{\miouTMburnOmissionLTwo}{\tbd{miouTMburnOmissionLTwo}}
\providecommand{\miouTMburnOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{miouTMburnOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouTMburnOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouTMburnOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouTMburnOmissionLTwoVarDecoderSamLite}{\tbd{miouTMburnOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouTMburnOmissionLTwoVarDecoderSamPretrained}{\tbd{miouTMburnOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\miouTMburnOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouTMburnOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouTMburnOmissionLTwoVarFrozenEncoderTrue}{\tbd{miouTMburnOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\miouTMburnOmissionLTwoVarLossBootstrap}{\tbd{miouTMburnOmissionLTwoVarLossBootstrap}}
\providecommand{\miouTMburnOmissionLTwoVarLossGce}{\tbd{miouTMburnOmissionLTwoVarLossGce}}
\providecommand{\miouTMburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouTMburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouTMburnOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouTMburnOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouTMburnShiftLOne}{\tbd{miouTMburnShiftLOne}}
\providecommand{\miouTMburnShiftLOneVarDecoderMaskTwoformerFull}{\tbd{miouTMburnShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouTMburnShiftLOneVarDecoderMaskTwoformerLite}{\tbd{miouTMburnShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouTMburnShiftLOneVarDecoderSamLite}{\tbd{miouTMburnShiftLOneVarDecoderSamLite}}
\providecommand{\miouTMburnShiftLOneVarDecoderSamPretrained}{\tbd{miouTMburnShiftLOneVarDecoderSamPretrained}}
\providecommand{\miouTMburnShiftLOneVarDecoderSegformerMlp}{\tbd{miouTMburnShiftLOneVarDecoderSegformerMlp}}
\providecommand{\miouTMburnShiftLR}{\tbd{miouTMburnShiftLR}}
\providecommand{\miouTMburnShiftLTwo}{\tbd{miouTMburnShiftLTwo}}
\providecommand{\miouTMburnShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{miouTMburnShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouTMburnShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouTMburnShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouTMburnShiftLTwoVarDecoderSamLite}{\tbd{miouTMburnShiftLTwoVarDecoderSamLite}}
\providecommand{\miouTMburnShiftLTwoVarDecoderSamPretrained}{\tbd{miouTMburnShiftLTwoVarDecoderSamPretrained}}
\providecommand{\miouTMburnShiftLTwoVarDecoderSegformerMlp}{\tbd{miouTMburnShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouTMburnShiftLTwoVarFrozenEncoderTrue}{\tbd{miouTMburnShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\miouTMburnShiftLTwoVarLossBootstrap}{\tbd{miouTMburnShiftLTwoVarLossBootstrap}}
\providecommand{\miouTMburnShiftLTwoVarLossGce}{\tbd{miouTMburnShiftLTwoVarLossGce}}
\providecommand{\miouTMburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouTMburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouTMburnShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouTMburnShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouTMflairBoundaryLOne}{\tbd{miouTMflairBoundaryLOne}}
\providecommand{\miouTMflairBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{miouTMflairBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouTMflairBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{miouTMflairBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouTMflairBoundaryLOneVarDecoderSamLite}{\tbd{miouTMflairBoundaryLOneVarDecoderSamLite}}
\providecommand{\miouTMflairBoundaryLOneVarDecoderSamPretrained}{\tbd{miouTMflairBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\miouTMflairBoundaryLOneVarDecoderSegformerMlp}{\tbd{miouTMflairBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\miouTMflairBoundaryLR}{\tbd{miouTMflairBoundaryLR}}
\providecommand{\miouTMflairBoundaryLTwo}{\tbd{miouTMflairBoundaryLTwo}}
\providecommand{\miouTMflairBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{miouTMflairBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouTMflairBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{miouTMflairBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouTMflairBoundaryLTwoVarDecoderSamLite}{\tbd{miouTMflairBoundaryLTwoVarDecoderSamLite}}
\providecommand{\miouTMflairBoundaryLTwoVarDecoderSamPretrained}{\tbd{miouTMflairBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\miouTMflairBoundaryLTwoVarDecoderSegformerMlp}{\tbd{miouTMflairBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\miouTMflairBoundaryLTwoVarFrozenEncoderTrue}{\tbd{miouTMflairBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\miouTMflairBoundaryLTwoVarLossBootstrap}{\tbd{miouTMflairBoundaryLTwoVarLossBootstrap}}
\providecommand{\miouTMflairBoundaryLTwoVarLossGce}{\tbd{miouTMflairBoundaryLTwoVarLossGce}}
\providecommand{\miouTMflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouTMflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouTMflairBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouTMflairBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouTMflairClean}{\tbd{miouTMflairClean}}
\providecommand{\miouTMflairCleanVarDecoderMaskTwoformerFull}{\tbd{miouTMflairCleanVarDecoderMaskTwoformerFull}}
\providecommand{\miouTMflairCleanVarDecoderMaskTwoformerLite}{\tbd{miouTMflairCleanVarDecoderMaskTwoformerLite}}
\providecommand{\miouTMflairCleanVarDecoderSamLite}{\tbd{miouTMflairCleanVarDecoderSamLite}}
\providecommand{\miouTMflairCleanVarDecoderSamPretrained}{\tbd{miouTMflairCleanVarDecoderSamPretrained}}
\providecommand{\miouTMflairCleanVarDecoderSegformerMlp}{\tbd{miouTMflairCleanVarDecoderSegformerMlp}}
\providecommand{\miouTMflairCleanVarFrozenEncoderTrue}{\tbd{miouTMflairCleanVarFrozenEncoderTrue}}
\providecommand{\miouTMflairCleanVarLossBootstrap}{\tbd{miouTMflairCleanVarLossBootstrap}}
\providecommand{\miouTMflairCleanVarLossGce}{\tbd{miouTMflairCleanVarLossGce}}
\providecommand{\miouTMflairCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{miouTMflairCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouTMflairCleanVarTrainSubsetCleanTwoFive}{\tbd{miouTMflairCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\miouTMflairCoarseLOne}{\tbd{miouTMflairCoarseLOne}}
\providecommand{\miouTMflairCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{miouTMflairCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouTMflairCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{miouTMflairCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouTMflairCoarseLOneVarDecoderSamLite}{\tbd{miouTMflairCoarseLOneVarDecoderSamLite}}
\providecommand{\miouTMflairCoarseLOneVarDecoderSamPretrained}{\tbd{miouTMflairCoarseLOneVarDecoderSamPretrained}}
\providecommand{\miouTMflairCoarseLOneVarDecoderSegformerMlp}{\tbd{miouTMflairCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\miouTMflairCoarseLR}{\tbd{miouTMflairCoarseLR}}
\providecommand{\miouTMflairCoarseLTwo}{\tbd{miouTMflairCoarseLTwo}}
\providecommand{\miouTMflairCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{miouTMflairCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouTMflairCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{miouTMflairCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouTMflairCoarseLTwoVarDecoderSamLite}{\tbd{miouTMflairCoarseLTwoVarDecoderSamLite}}
\providecommand{\miouTMflairCoarseLTwoVarDecoderSamPretrained}{\tbd{miouTMflairCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\miouTMflairCoarseLTwoVarDecoderSegformerMlp}{\tbd{miouTMflairCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\miouTMflairCoarseLTwoVarFrozenEncoderTrue}{\tbd{miouTMflairCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\miouTMflairCoarseLTwoVarLossBootstrap}{\tbd{miouTMflairCoarseLTwoVarLossBootstrap}}
\providecommand{\miouTMflairCoarseLTwoVarLossGce}{\tbd{miouTMflairCoarseLTwoVarLossGce}}
\providecommand{\miouTMflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouTMflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouTMflairCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouTMflairCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouTMflairOmissionLOne}{\tbd{miouTMflairOmissionLOne}}
\providecommand{\miouTMflairOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{miouTMflairOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouTMflairOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{miouTMflairOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouTMflairOmissionLOneVarDecoderSamLite}{\tbd{miouTMflairOmissionLOneVarDecoderSamLite}}
\providecommand{\miouTMflairOmissionLOneVarDecoderSamPretrained}{\tbd{miouTMflairOmissionLOneVarDecoderSamPretrained}}
\providecommand{\miouTMflairOmissionLOneVarDecoderSegformerMlp}{\tbd{miouTMflairOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\miouTMflairOmissionLR}{\tbd{miouTMflairOmissionLR}}
\providecommand{\miouTMflairOmissionLTwo}{\tbd{miouTMflairOmissionLTwo}}
\providecommand{\miouTMflairOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{miouTMflairOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouTMflairOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{miouTMflairOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouTMflairOmissionLTwoVarDecoderSamLite}{\tbd{miouTMflairOmissionLTwoVarDecoderSamLite}}
\providecommand{\miouTMflairOmissionLTwoVarDecoderSamPretrained}{\tbd{miouTMflairOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\miouTMflairOmissionLTwoVarDecoderSegformerMlp}{\tbd{miouTMflairOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\miouTMflairOmissionLTwoVarFrozenEncoderTrue}{\tbd{miouTMflairOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\miouTMflairOmissionLTwoVarLossBootstrap}{\tbd{miouTMflairOmissionLTwoVarLossBootstrap}}
\providecommand{\miouTMflairOmissionLTwoVarLossGce}{\tbd{miouTMflairOmissionLTwoVarLossGce}}
\providecommand{\miouTMflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouTMflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouTMflairOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouTMflairOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouTMflairShiftLOne}{\tbd{miouTMflairShiftLOne}}
\providecommand{\miouTMflairShiftLOneVarDecoderMaskTwoformerFull}{\tbd{miouTMflairShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\miouTMflairShiftLOneVarDecoderMaskTwoformerLite}{\tbd{miouTMflairShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\miouTMflairShiftLOneVarDecoderSamLite}{\tbd{miouTMflairShiftLOneVarDecoderSamLite}}
\providecommand{\miouTMflairShiftLOneVarDecoderSamPretrained}{\tbd{miouTMflairShiftLOneVarDecoderSamPretrained}}
\providecommand{\miouTMflairShiftLOneVarDecoderSegformerMlp}{\tbd{miouTMflairShiftLOneVarDecoderSegformerMlp}}
\providecommand{\miouTMflairShiftLR}{\tbd{miouTMflairShiftLR}}
\providecommand{\miouTMflairShiftLTwo}{\tbd{miouTMflairShiftLTwo}}
\providecommand{\miouTMflairShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{miouTMflairShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\miouTMflairShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{miouTMflairShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\miouTMflairShiftLTwoVarDecoderSamLite}{\tbd{miouTMflairShiftLTwoVarDecoderSamLite}}
\providecommand{\miouTMflairShiftLTwoVarDecoderSamPretrained}{\tbd{miouTMflairShiftLTwoVarDecoderSamPretrained}}
\providecommand{\miouTMflairShiftLTwoVarDecoderSegformerMlp}{\tbd{miouTMflairShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\miouTMflairShiftLTwoVarFrozenEncoderTrue}{\tbd{miouTMflairShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\miouTMflairShiftLTwoVarLossBootstrap}{\tbd{miouTMflairShiftLTwoVarLossBootstrap}}
\providecommand{\miouTMflairShiftLTwoVarLossGce}{\tbd{miouTMflairShiftLTwoVarLossGce}}
\providecommand{\miouTMflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{miouTMflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\miouTMflairShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{miouTMflairShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\miouTMsenClean}{\tbd{miouTMsenClean}}
\providecommand{\miouTMsenOtsuLTwo}{\tbd{miouTMsenOtsuLTwo}}
\providecommand{\miouVITRburnClean}{\tbd{miouVITRburnClean}}
\providecommand{\miouVITRflairClean}{\tbd{miouVITRflairClean}}
\providecommand{\miouVitlRandomburnBoundaryLOneVarInitRandom}{\tbd{miouVitlRandomburnBoundaryLOneVarInitRandom}}
\providecommand{\miouVitlRandomburnBoundaryLTwoVarInitRandom}{\tbd{miouVitlRandomburnBoundaryLTwoVarInitRandom}}
\providecommand{\miouVitlRandomburnCleanVarInitRandom}{\tbd{miouVitlRandomburnCleanVarInitRandom}}
\providecommand{\miouVitlRandomburnCleanVarInitRandomLrMultOneZero}{\tbd{miouVitlRandomburnCleanVarInitRandomLrMultOneZero}}
\providecommand{\miouVitlRandomburnCleanVarInitRandomLrMultThree}{\tbd{miouVitlRandomburnCleanVarInitRandomLrMultThree}}
\providecommand{\miouVitlRandomburnCleanVarInitRandomTrainSubsetCleanTwoFive}{\tbd{miouVitlRandomburnCleanVarInitRandomTrainSubsetCleanTwoFive}}
\providecommand{\miouVitlRandomburnCoarseLOneVarInitRandom}{\tbd{miouVitlRandomburnCoarseLOneVarInitRandom}}
\providecommand{\miouVitlRandomburnCoarseLTwoVarInitRandom}{\tbd{miouVitlRandomburnCoarseLTwoVarInitRandom}}
\providecommand{\miouVitlRandomburnOmissionLOneVarInitRandom}{\tbd{miouVitlRandomburnOmissionLOneVarInitRandom}}
\providecommand{\miouVitlRandomburnOmissionLTwoVarInitRandom}{\tbd{miouVitlRandomburnOmissionLTwoVarInitRandom}}
\providecommand{\miouVitlRandomburnShiftLOneVarInitRandom}{\tbd{miouVitlRandomburnShiftLOneVarInitRandom}}
\providecommand{\miouVitlRandomburnShiftLTwoVarInitRandom}{\tbd{miouVitlRandomburnShiftLTwoVarInitRandom}}
\providecommand{\miouVitlRandomflairBoundaryLOneVarInitRandom}{\tbd{miouVitlRandomflairBoundaryLOneVarInitRandom}}
\providecommand{\miouVitlRandomflairBoundaryLTwoVarInitRandom}{\tbd{miouVitlRandomflairBoundaryLTwoVarInitRandom}}
\providecommand{\miouVitlRandomflairCleanVarInitRandom}{\tbd{miouVitlRandomflairCleanVarInitRandom}}
\providecommand{\miouVitlRandomflairCleanVarInitRandomLrMultOne}{\tbd{miouVitlRandomflairCleanVarInitRandomLrMultOne}}
\providecommand{\miouVitlRandomflairCleanVarInitRandomLrMultOneZero}{\tbd{miouVitlRandomflairCleanVarInitRandomLrMultOneZero}}
\providecommand{\miouVitlRandomflairCleanVarInitRandomTrainSubsetCleanTwoFive}{\tbd{miouVitlRandomflairCleanVarInitRandomTrainSubsetCleanTwoFive}}
\providecommand{\miouVitlRandomflairCoarseLOneVarInitRandom}{\tbd{miouVitlRandomflairCoarseLOneVarInitRandom}}
\providecommand{\miouVitlRandomflairCoarseLTwoVarInitRandom}{\tbd{miouVitlRandomflairCoarseLTwoVarInitRandom}}
\providecommand{\miouVitlRandomflairOmissionLOneVarInitRandom}{\tbd{miouVitlRandomflairOmissionLOneVarInitRandom}}
\providecommand{\miouVitlRandomflairOmissionLTwoVarInitRandom}{\tbd{miouVitlRandomflairOmissionLTwoVarInitRandom}}
\providecommand{\miouVitlRandomflairShiftLOneVarInitRandom}{\tbd{miouVitlRandomflairShiftLOneVarInitRandom}}
\providecommand{\miouVitlRandomflairShiftLTwoVarInitRandom}{\tbd{miouVitlRandomflairShiftLTwoVarInitRandom}}
\providecommand{\nDOFAChesBoundaryLOne}{\tbd{nDOFAChesBoundaryLOne}}
\providecommand{\nDOFAChesBoundaryLTwo}{\tbd{nDOFAChesBoundaryLTwo}}
\providecommand{\nDOFAChesClean}{\tbd{nDOFAChesClean}}
\providecommand{\nDOFAChesCoarseLOne}{\tbd{nDOFAChesCoarseLOne}}
\providecommand{\nDOFAChesCoarseLTwo}{\tbd{nDOFAChesCoarseLTwo}}
\providecommand{\nDOFAChesNlcdREAL}{\tbd{nDOFAChesNlcdREAL}}
\providecommand{\nDOFAChesOmissionLOne}{\tbd{nDOFAChesOmissionLOne}}
\providecommand{\nDOFAChesOmissionLTwo}{\tbd{nDOFAChesOmissionLTwo}}
\providecommand{\nDOFAChesShiftLOne}{\tbd{nDOFAChesShiftLOne}}
\providecommand{\nDOFAChesShiftLTwo}{\tbd{nDOFAChesShiftLTwo}}
\providecommand{\nDOFACsTwelveBoundaryLOne}{\tbd{nDOFACsTwelveBoundaryLOne}}
\providecommand{\nDOFACsTwelveBoundaryLTwo}{\tbd{nDOFACsTwelveBoundaryLTwo}}
\providecommand{\nDOFACsTwelveClean}{\tbd{nDOFACsTwelveClean}}
\providecommand{\nDOFACsTwelveCoarseLOne}{\tbd{nDOFACsTwelveCoarseLOne}}
\providecommand{\nDOFACsTwelveCoarseLTwo}{\tbd{nDOFACsTwelveCoarseLTwo}}
\providecommand{\nDOFACsTwelveOmissionLOne}{\tbd{nDOFACsTwelveOmissionLOne}}
\providecommand{\nDOFACsTwelveOmissionLTwo}{\tbd{nDOFACsTwelveOmissionLTwo}}
\providecommand{\nDOFACsTwelveSTwocloudlessREAL}{\tbd{nDOFACsTwelveSTwocloudlessREAL}}
\providecommand{\nDOFACsTwelveShiftLOne}{\tbd{nDOFACsTwelveShiftLOne}}
\providecommand{\nDOFACsTwelveShiftLTwo}{\tbd{nDOFACsTwelveShiftLTwo}}
\providecommand{\nDOFADfcBoundaryLOne}{\tbd{nDOFADfcBoundaryLOne}}
\providecommand{\nDOFADfcBoundaryLTwo}{\tbd{nDOFADfcBoundaryLTwo}}
\providecommand{\nDOFADfcClean}{\tbd{nDOFADfcClean}}
\providecommand{\nDOFADfcCleanVarTrainSubsetRealcov}{\tbd{nDOFADfcCleanVarTrainSubsetRealcov}}
\providecommand{\nDOFADfcCoarseLOne}{\tbd{nDOFADfcCoarseLOne}}
\providecommand{\nDOFADfcCoarseLTwo}{\tbd{nDOFADfcCoarseLTwo}}
\providecommand{\nDOFADfcModisREALVarTrainSubsetRealcov}{\tbd{nDOFADfcModisREALVarTrainSubsetRealcov}}
\providecommand{\nDOFADfcOmissionLOne}{\tbd{nDOFADfcOmissionLOne}}
\providecommand{\nDOFADfcOmissionLTwo}{\tbd{nDOFADfcOmissionLTwo}}
\providecommand{\nDOFADfcShiftLOne}{\tbd{nDOFADfcShiftLOne}}
\providecommand{\nDOFADfcShiftLTwo}{\tbd{nDOFADfcShiftLTwo}}
\providecommand{\nDOFAEnvaBoundaryLOne}{\tbd{nDOFAEnvaBoundaryLOne}}
\providecommand{\nDOFAEnvaBoundaryLTwo}{\tbd{nDOFAEnvaBoundaryLTwo}}
\providecommand{\nDOFAEnvaClean}{\tbd{nDOFAEnvaClean}}
\providecommand{\nDOFAEnvaCoarseLOne}{\tbd{nDOFAEnvaCoarseLOne}}
\providecommand{\nDOFAEnvaCoarseLTwo}{\tbd{nDOFAEnvaCoarseLTwo}}
\providecommand{\nDOFAEnvaNlcdREAL}{\tbd{nDOFAEnvaNlcdREAL}}
\providecommand{\nDOFAEnvaOmissionLOne}{\tbd{nDOFAEnvaOmissionLOne}}
\providecommand{\nDOFAEnvaOmissionLTwo}{\tbd{nDOFAEnvaOmissionLTwo}}
\providecommand{\nDOFAEnvaShiftLOne}{\tbd{nDOFAEnvaShiftLOne}}
\providecommand{\nDOFAEnvaShiftLTwo}{\tbd{nDOFAEnvaShiftLTwo}}
\providecommand{\nDOFAKuroBoundaryLOne}{\tbd{nDOFAKuroBoundaryLOne}}
\providecommand{\nDOFAKuroBoundaryLTwo}{\tbd{nDOFAKuroBoundaryLTwo}}
\providecommand{\nDOFAKuroCemsREALVarTrainSubsetRealcov}{\tbd{nDOFAKuroCemsREALVarTrainSubsetRealcov}}
\providecommand{\nDOFAKuroClean}{\tbd{nDOFAKuroClean}}
\providecommand{\nDOFAKuroCleanVarTrainSubsetRealcov}{\tbd{nDOFAKuroCleanVarTrainSubsetRealcov}}
\providecommand{\nDOFAKuroCoarseLOne}{\tbd{nDOFAKuroCoarseLOne}}
\providecommand{\nDOFAKuroCoarseLTwo}{\tbd{nDOFAKuroCoarseLTwo}}
\providecommand{\nDOFAKuroOmissionLOne}{\tbd{nDOFAKuroOmissionLOne}}
\providecommand{\nDOFAKuroOmissionLTwo}{\tbd{nDOFAKuroOmissionLTwo}}
\providecommand{\nDOFAKuroShiftLOne}{\tbd{nDOFAKuroShiftLOne}}
\providecommand{\nDOFAKuroShiftLTwo}{\tbd{nDOFAKuroShiftLTwo}}
\providecommand{\nDOFAOemBoundaryLOne}{\tbd{nDOFAOemBoundaryLOne}}
\providecommand{\nDOFAOemBoundaryLTwo}{\tbd{nDOFAOemBoundaryLTwo}}
\providecommand{\nDOFAOemClean}{\tbd{nDOFAOemClean}}
\providecommand{\nDOFAOemCoarseLOne}{\tbd{nDOFAOemCoarseLOne}}
\providecommand{\nDOFAOemCoarseLTwo}{\tbd{nDOFAOemCoarseLTwo}}
\providecommand{\nDOFAOemOmissionLOne}{\tbd{nDOFAOemOmissionLOne}}
\providecommand{\nDOFAOemOmissionLTwo}{\tbd{nDOFAOemOmissionLTwo}}
\providecommand{\nDOFAOemShiftLOne}{\tbd{nDOFAOemShiftLOne}}
\providecommand{\nDOFAOemShiftLTwo}{\tbd{nDOFAOemShiftLTwo}}
\providecommand{\nDOFASnTwoBoundaryLOne}{\tbd{nDOFASnTwoBoundaryLOne}}
\providecommand{\nDOFASnTwoBoundaryLTwo}{\tbd{nDOFASnTwoBoundaryLTwo}}
\providecommand{\nDOFASnTwoClean}{\tbd{nDOFASnTwoClean}}
\providecommand{\nDOFASnTwoCoarseLOne}{\tbd{nDOFASnTwoCoarseLOne}}
\providecommand{\nDOFASnTwoCoarseLTwo}{\tbd{nDOFASnTwoCoarseLTwo}}
\providecommand{\nDOFASnTwoOmissionLOne}{\tbd{nDOFASnTwoOmissionLOne}}
\providecommand{\nDOFASnTwoOmissionLTwo}{\tbd{nDOFASnTwoOmissionLTwo}}
\providecommand{\nDOFASnTwoShiftLOne}{\tbd{nDOFASnTwoShiftLOne}}
\providecommand{\nDOFASnTwoShiftLTwo}{\tbd{nDOFASnTwoShiftLTwo}}
\providecommand{\nDOFAburnBoundaryLOne}{\tbd{nDOFAburnBoundaryLOne}}
\providecommand{\nDOFAburnBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{nDOFAburnBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nDOFAburnBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{nDOFAburnBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nDOFAburnBoundaryLOneVarDecoderSamLite}{\tbd{nDOFAburnBoundaryLOneVarDecoderSamLite}}
\providecommand{\nDOFAburnBoundaryLOneVarDecoderSamPretrained}{\tbd{nDOFAburnBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\nDOFAburnBoundaryLOneVarDecoderSegformerMlp}{\tbd{nDOFAburnBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\nDOFAburnBoundaryLR}{\tbd{nDOFAburnBoundaryLR}}
\providecommand{\nDOFAburnBoundaryLTwo}{\tbd{nDOFAburnBoundaryLTwo}}
\providecommand{\nDOFAburnBoundaryLTwoVarBandsRgb}{\tbd{nDOFAburnBoundaryLTwoVarBandsRgb}}
\providecommand{\nDOFAburnBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{nDOFAburnBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nDOFAburnBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{nDOFAburnBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nDOFAburnBoundaryLTwoVarDecoderSamLite}{\tbd{nDOFAburnBoundaryLTwoVarDecoderSamLite}}
\providecommand{\nDOFAburnBoundaryLTwoVarDecoderSamPretrained}{\tbd{nDOFAburnBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\nDOFAburnBoundaryLTwoVarDecoderSegformerMlp}{\tbd{nDOFAburnBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\nDOFAburnBoundaryLTwoVarFrozenEncoderTrue}{\tbd{nDOFAburnBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\nDOFAburnBoundaryLTwoVarLossBootstrap}{\tbd{nDOFAburnBoundaryLTwoVarLossBootstrap}}
\providecommand{\nDOFAburnBoundaryLTwoVarLossGce}{\tbd{nDOFAburnBoundaryLTwoVarLossGce}}
\providecommand{\nDOFAburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nDOFAburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nDOFAburnBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{nDOFAburnBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nDOFAburnClean}{\tbd{nDOFAburnClean}}
\providecommand{\nDOFAburnCleanVarBandsRgb}{\tbd{nDOFAburnCleanVarBandsRgb}}
\providecommand{\nDOFAburnCleanVarDecoderMaskTwoformerFull}{\tbd{nDOFAburnCleanVarDecoderMaskTwoformerFull}}
\providecommand{\nDOFAburnCleanVarDecoderMaskTwoformerLite}{\tbd{nDOFAburnCleanVarDecoderMaskTwoformerLite}}
\providecommand{\nDOFAburnCleanVarDecoderSamLite}{\tbd{nDOFAburnCleanVarDecoderSamLite}}
\providecommand{\nDOFAburnCleanVarDecoderSamPretrained}{\tbd{nDOFAburnCleanVarDecoderSamPretrained}}
\providecommand{\nDOFAburnCleanVarDecoderSegformerMlp}{\tbd{nDOFAburnCleanVarDecoderSegformerMlp}}
\providecommand{\nDOFAburnCleanVarFrozenEncoderTrue}{\tbd{nDOFAburnCleanVarFrozenEncoderTrue}}
\providecommand{\nDOFAburnCleanVarLossBootstrap}{\tbd{nDOFAburnCleanVarLossBootstrap}}
\providecommand{\nDOFAburnCleanVarLossGce}{\tbd{nDOFAburnCleanVarLossGce}}
\providecommand{\nDOFAburnCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{nDOFAburnCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nDOFAburnCleanVarTrainSubsetCleanTwoFive}{\tbd{nDOFAburnCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\nDOFAburnCoarseLOne}{\tbd{nDOFAburnCoarseLOne}}
\providecommand{\nDOFAburnCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{nDOFAburnCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nDOFAburnCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{nDOFAburnCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nDOFAburnCoarseLOneVarDecoderSamLite}{\tbd{nDOFAburnCoarseLOneVarDecoderSamLite}}
\providecommand{\nDOFAburnCoarseLOneVarDecoderSamPretrained}{\tbd{nDOFAburnCoarseLOneVarDecoderSamPretrained}}
\providecommand{\nDOFAburnCoarseLOneVarDecoderSegformerMlp}{\tbd{nDOFAburnCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\nDOFAburnCoarseLR}{\tbd{nDOFAburnCoarseLR}}
\providecommand{\nDOFAburnCoarseLTwo}{\tbd{nDOFAburnCoarseLTwo}}
\providecommand{\nDOFAburnCoarseLTwoVarBandsRgb}{\tbd{nDOFAburnCoarseLTwoVarBandsRgb}}
\providecommand{\nDOFAburnCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{nDOFAburnCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nDOFAburnCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{nDOFAburnCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nDOFAburnCoarseLTwoVarDecoderSamLite}{\tbd{nDOFAburnCoarseLTwoVarDecoderSamLite}}
\providecommand{\nDOFAburnCoarseLTwoVarDecoderSamPretrained}{\tbd{nDOFAburnCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\nDOFAburnCoarseLTwoVarDecoderSegformerMlp}{\tbd{nDOFAburnCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\nDOFAburnCoarseLTwoVarFrozenEncoderTrue}{\tbd{nDOFAburnCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\nDOFAburnCoarseLTwoVarLossBootstrap}{\tbd{nDOFAburnCoarseLTwoVarLossBootstrap}}
\providecommand{\nDOFAburnCoarseLTwoVarLossGce}{\tbd{nDOFAburnCoarseLTwoVarLossGce}}
\providecommand{\nDOFAburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nDOFAburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nDOFAburnCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{nDOFAburnCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nDOFAburnOmissionLOne}{\tbd{nDOFAburnOmissionLOne}}
\providecommand{\nDOFAburnOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{nDOFAburnOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nDOFAburnOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{nDOFAburnOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nDOFAburnOmissionLOneVarDecoderSamLite}{\tbd{nDOFAburnOmissionLOneVarDecoderSamLite}}
\providecommand{\nDOFAburnOmissionLOneVarDecoderSamPretrained}{\tbd{nDOFAburnOmissionLOneVarDecoderSamPretrained}}
\providecommand{\nDOFAburnOmissionLOneVarDecoderSegformerMlp}{\tbd{nDOFAburnOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\nDOFAburnOmissionLR}{\tbd{nDOFAburnOmissionLR}}
\providecommand{\nDOFAburnOmissionLTwo}{\tbd{nDOFAburnOmissionLTwo}}
\providecommand{\nDOFAburnOmissionLTwoVarBandsRgb}{\tbd{nDOFAburnOmissionLTwoVarBandsRgb}}
\providecommand{\nDOFAburnOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{nDOFAburnOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nDOFAburnOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{nDOFAburnOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nDOFAburnOmissionLTwoVarDecoderSamLite}{\tbd{nDOFAburnOmissionLTwoVarDecoderSamLite}}
\providecommand{\nDOFAburnOmissionLTwoVarDecoderSamPretrained}{\tbd{nDOFAburnOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\nDOFAburnOmissionLTwoVarDecoderSegformerMlp}{\tbd{nDOFAburnOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\nDOFAburnOmissionLTwoVarFrozenEncoderTrue}{\tbd{nDOFAburnOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\nDOFAburnOmissionLTwoVarLossBootstrap}{\tbd{nDOFAburnOmissionLTwoVarLossBootstrap}}
\providecommand{\nDOFAburnOmissionLTwoVarLossGce}{\tbd{nDOFAburnOmissionLTwoVarLossGce}}
\providecommand{\nDOFAburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nDOFAburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nDOFAburnOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{nDOFAburnOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nDOFAburnShiftLOne}{\tbd{nDOFAburnShiftLOne}}
\providecommand{\nDOFAburnShiftLOneVarDecoderMaskTwoformerFull}{\tbd{nDOFAburnShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nDOFAburnShiftLOneVarDecoderMaskTwoformerLite}{\tbd{nDOFAburnShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nDOFAburnShiftLOneVarDecoderSamLite}{\tbd{nDOFAburnShiftLOneVarDecoderSamLite}}
\providecommand{\nDOFAburnShiftLOneVarDecoderSamPretrained}{\tbd{nDOFAburnShiftLOneVarDecoderSamPretrained}}
\providecommand{\nDOFAburnShiftLOneVarDecoderSegformerMlp}{\tbd{nDOFAburnShiftLOneVarDecoderSegformerMlp}}
\providecommand{\nDOFAburnShiftLR}{\tbd{nDOFAburnShiftLR}}
\providecommand{\nDOFAburnShiftLTwo}{\tbd{nDOFAburnShiftLTwo}}
\providecommand{\nDOFAburnShiftLTwoVarBandsRgb}{\tbd{nDOFAburnShiftLTwoVarBandsRgb}}
\providecommand{\nDOFAburnShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{nDOFAburnShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nDOFAburnShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{nDOFAburnShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nDOFAburnShiftLTwoVarDecoderSamLite}{\tbd{nDOFAburnShiftLTwoVarDecoderSamLite}}
\providecommand{\nDOFAburnShiftLTwoVarDecoderSamPretrained}{\tbd{nDOFAburnShiftLTwoVarDecoderSamPretrained}}
\providecommand{\nDOFAburnShiftLTwoVarDecoderSegformerMlp}{\tbd{nDOFAburnShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\nDOFAburnShiftLTwoVarFrozenEncoderTrue}{\tbd{nDOFAburnShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\nDOFAburnShiftLTwoVarLossBootstrap}{\tbd{nDOFAburnShiftLTwoVarLossBootstrap}}
\providecommand{\nDOFAburnShiftLTwoVarLossGce}{\tbd{nDOFAburnShiftLTwoVarLossGce}}
\providecommand{\nDOFAburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nDOFAburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nDOFAburnShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{nDOFAburnShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nDOFAflairBoundaryLOne}{\tbd{nDOFAflairBoundaryLOne}}
\providecommand{\nDOFAflairBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{nDOFAflairBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nDOFAflairBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{nDOFAflairBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nDOFAflairBoundaryLOneVarDecoderSamLite}{\tbd{nDOFAflairBoundaryLOneVarDecoderSamLite}}
\providecommand{\nDOFAflairBoundaryLOneVarDecoderSamPretrained}{\tbd{nDOFAflairBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\nDOFAflairBoundaryLOneVarDecoderSegformerMlp}{\tbd{nDOFAflairBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\nDOFAflairBoundaryLR}{\tbd{nDOFAflairBoundaryLR}}
\providecommand{\nDOFAflairBoundaryLTwo}{\tbd{nDOFAflairBoundaryLTwo}}
\providecommand{\nDOFAflairBoundaryLTwoVarBandsRgb}{\tbd{nDOFAflairBoundaryLTwoVarBandsRgb}}
\providecommand{\nDOFAflairBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{nDOFAflairBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nDOFAflairBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{nDOFAflairBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nDOFAflairBoundaryLTwoVarDecoderSamLite}{\tbd{nDOFAflairBoundaryLTwoVarDecoderSamLite}}
\providecommand{\nDOFAflairBoundaryLTwoVarDecoderSamPretrained}{\tbd{nDOFAflairBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\nDOFAflairBoundaryLTwoVarDecoderSegformerMlp}{\tbd{nDOFAflairBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\nDOFAflairBoundaryLTwoVarFrozenEncoderTrue}{\tbd{nDOFAflairBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\nDOFAflairBoundaryLTwoVarLossBootstrap}{\tbd{nDOFAflairBoundaryLTwoVarLossBootstrap}}
\providecommand{\nDOFAflairBoundaryLTwoVarLossGce}{\tbd{nDOFAflairBoundaryLTwoVarLossGce}}
\providecommand{\nDOFAflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nDOFAflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nDOFAflairBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{nDOFAflairBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nDOFAflairClean}{\tbd{nDOFAflairClean}}
\providecommand{\nDOFAflairCleanVarBandsRgb}{\tbd{nDOFAflairCleanVarBandsRgb}}
\providecommand{\nDOFAflairCleanVarDecoderMaskTwoformerFull}{\tbd{nDOFAflairCleanVarDecoderMaskTwoformerFull}}
\providecommand{\nDOFAflairCleanVarDecoderMaskTwoformerLite}{\tbd{nDOFAflairCleanVarDecoderMaskTwoformerLite}}
\providecommand{\nDOFAflairCleanVarDecoderSamLite}{\tbd{nDOFAflairCleanVarDecoderSamLite}}
\providecommand{\nDOFAflairCleanVarDecoderSamPretrained}{\tbd{nDOFAflairCleanVarDecoderSamPretrained}}
\providecommand{\nDOFAflairCleanVarDecoderSegformerMlp}{\tbd{nDOFAflairCleanVarDecoderSegformerMlp}}
\providecommand{\nDOFAflairCleanVarFrozenEncoderTrue}{\tbd{nDOFAflairCleanVarFrozenEncoderTrue}}
\providecommand{\nDOFAflairCleanVarLossBootstrap}{\tbd{nDOFAflairCleanVarLossBootstrap}}
\providecommand{\nDOFAflairCleanVarLossGce}{\tbd{nDOFAflairCleanVarLossGce}}
\providecommand{\nDOFAflairCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{nDOFAflairCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nDOFAflairCleanVarTrainSubsetCleanTwoFive}{\tbd{nDOFAflairCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\nDOFAflairCoarseLOne}{\tbd{nDOFAflairCoarseLOne}}
\providecommand{\nDOFAflairCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{nDOFAflairCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nDOFAflairCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{nDOFAflairCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nDOFAflairCoarseLOneVarDecoderSamLite}{\tbd{nDOFAflairCoarseLOneVarDecoderSamLite}}
\providecommand{\nDOFAflairCoarseLOneVarDecoderSamPretrained}{\tbd{nDOFAflairCoarseLOneVarDecoderSamPretrained}}
\providecommand{\nDOFAflairCoarseLOneVarDecoderSegformerMlp}{\tbd{nDOFAflairCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\nDOFAflairCoarseLR}{\tbd{nDOFAflairCoarseLR}}
\providecommand{\nDOFAflairCoarseLTwo}{\tbd{nDOFAflairCoarseLTwo}}
\providecommand{\nDOFAflairCoarseLTwoVarBandsRgb}{\tbd{nDOFAflairCoarseLTwoVarBandsRgb}}
\providecommand{\nDOFAflairCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{nDOFAflairCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nDOFAflairCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{nDOFAflairCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nDOFAflairCoarseLTwoVarDecoderSamLite}{\tbd{nDOFAflairCoarseLTwoVarDecoderSamLite}}
\providecommand{\nDOFAflairCoarseLTwoVarDecoderSamPretrained}{\tbd{nDOFAflairCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\nDOFAflairCoarseLTwoVarDecoderSegformerMlp}{\tbd{nDOFAflairCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\nDOFAflairCoarseLTwoVarFrozenEncoderTrue}{\tbd{nDOFAflairCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\nDOFAflairCoarseLTwoVarLossBootstrap}{\tbd{nDOFAflairCoarseLTwoVarLossBootstrap}}
\providecommand{\nDOFAflairCoarseLTwoVarLossGce}{\tbd{nDOFAflairCoarseLTwoVarLossGce}}
\providecommand{\nDOFAflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nDOFAflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nDOFAflairCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{nDOFAflairCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nDOFAflairOmissionLOne}{\tbd{nDOFAflairOmissionLOne}}
\providecommand{\nDOFAflairOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{nDOFAflairOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nDOFAflairOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{nDOFAflairOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nDOFAflairOmissionLOneVarDecoderSamLite}{\tbd{nDOFAflairOmissionLOneVarDecoderSamLite}}
\providecommand{\nDOFAflairOmissionLOneVarDecoderSamPretrained}{\tbd{nDOFAflairOmissionLOneVarDecoderSamPretrained}}
\providecommand{\nDOFAflairOmissionLOneVarDecoderSegformerMlp}{\tbd{nDOFAflairOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\nDOFAflairOmissionLR}{\tbd{nDOFAflairOmissionLR}}
\providecommand{\nDOFAflairOmissionLTwo}{\tbd{nDOFAflairOmissionLTwo}}
\providecommand{\nDOFAflairOmissionLTwoVarBandsRgb}{\tbd{nDOFAflairOmissionLTwoVarBandsRgb}}
\providecommand{\nDOFAflairOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{nDOFAflairOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nDOFAflairOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{nDOFAflairOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nDOFAflairOmissionLTwoVarDecoderSamLite}{\tbd{nDOFAflairOmissionLTwoVarDecoderSamLite}}
\providecommand{\nDOFAflairOmissionLTwoVarDecoderSamPretrained}{\tbd{nDOFAflairOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\nDOFAflairOmissionLTwoVarDecoderSegformerMlp}{\tbd{nDOFAflairOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\nDOFAflairOmissionLTwoVarFrozenEncoderTrue}{\tbd{nDOFAflairOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\nDOFAflairOmissionLTwoVarLossBootstrap}{\tbd{nDOFAflairOmissionLTwoVarLossBootstrap}}
\providecommand{\nDOFAflairOmissionLTwoVarLossGce}{\tbd{nDOFAflairOmissionLTwoVarLossGce}}
\providecommand{\nDOFAflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nDOFAflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nDOFAflairOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{nDOFAflairOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nDOFAflairShiftLOne}{\tbd{nDOFAflairShiftLOne}}
\providecommand{\nDOFAflairShiftLOneVarDecoderMaskTwoformerFull}{\tbd{nDOFAflairShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nDOFAflairShiftLOneVarDecoderMaskTwoformerLite}{\tbd{nDOFAflairShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nDOFAflairShiftLOneVarDecoderSamLite}{\tbd{nDOFAflairShiftLOneVarDecoderSamLite}}
\providecommand{\nDOFAflairShiftLOneVarDecoderSamPretrained}{\tbd{nDOFAflairShiftLOneVarDecoderSamPretrained}}
\providecommand{\nDOFAflairShiftLOneVarDecoderSegformerMlp}{\tbd{nDOFAflairShiftLOneVarDecoderSegformerMlp}}
\providecommand{\nDOFAflairShiftLR}{\tbd{nDOFAflairShiftLR}}
\providecommand{\nDOFAflairShiftLTwo}{\tbd{nDOFAflairShiftLTwo}}
\providecommand{\nDOFAflairShiftLTwoVarBandsRgb}{\tbd{nDOFAflairShiftLTwoVarBandsRgb}}
\providecommand{\nDOFAflairShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{nDOFAflairShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nDOFAflairShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{nDOFAflairShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nDOFAflairShiftLTwoVarDecoderSamLite}{\tbd{nDOFAflairShiftLTwoVarDecoderSamLite}}
\providecommand{\nDOFAflairShiftLTwoVarDecoderSamPretrained}{\tbd{nDOFAflairShiftLTwoVarDecoderSamPretrained}}
\providecommand{\nDOFAflairShiftLTwoVarDecoderSegformerMlp}{\tbd{nDOFAflairShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\nDOFAflairShiftLTwoVarFrozenEncoderTrue}{\tbd{nDOFAflairShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\nDOFAflairShiftLTwoVarLossBootstrap}{\tbd{nDOFAflairShiftLTwoVarLossBootstrap}}
\providecommand{\nDOFAflairShiftLTwoVarLossGce}{\tbd{nDOFAflairShiftLTwoVarLossGce}}
\providecommand{\nDOFAflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nDOFAflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nDOFAflairShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{nDOFAflairShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nDOFAsenClean}{\tbd{nDOFAsenClean}}
\providecommand{\nDOFAsenOtsuLTwo}{\tbd{nDOFAsenOtsuLTwo}}
\providecommand{\nDinovThreeConvnextLburnBoundaryLOne}{\tbd{nDinovThreeConvnextLburnBoundaryLOne}}
\providecommand{\nDinovThreeConvnextLburnBoundaryLTwo}{\tbd{nDinovThreeConvnextLburnBoundaryLTwo}}
\providecommand{\nDinovThreeConvnextLburnClean}{\tbd{nDinovThreeConvnextLburnClean}}
\providecommand{\nDinovThreeConvnextLburnCleanVarTrainSubsetCleanTwoFive}{\tbd{nDinovThreeConvnextLburnCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\nDinovThreeConvnextLburnCoarseLOne}{\tbd{nDinovThreeConvnextLburnCoarseLOne}}
\providecommand{\nDinovThreeConvnextLburnCoarseLTwo}{\tbd{nDinovThreeConvnextLburnCoarseLTwo}}
\providecommand{\nDinovThreeConvnextLburnOmissionLOne}{\tbd{nDinovThreeConvnextLburnOmissionLOne}}
\providecommand{\nDinovThreeConvnextLburnOmissionLTwo}{\tbd{nDinovThreeConvnextLburnOmissionLTwo}}
\providecommand{\nDinovThreeConvnextLburnShiftLOne}{\tbd{nDinovThreeConvnextLburnShiftLOne}}
\providecommand{\nDinovThreeConvnextLburnShiftLTwo}{\tbd{nDinovThreeConvnextLburnShiftLTwo}}
\providecommand{\nDinovThreeConvnextLflairBoundaryLOne}{\tbd{nDinovThreeConvnextLflairBoundaryLOne}}
\providecommand{\nDinovThreeConvnextLflairBoundaryLTwo}{\tbd{nDinovThreeConvnextLflairBoundaryLTwo}}
\providecommand{\nDinovThreeConvnextLflairClean}{\tbd{nDinovThreeConvnextLflairClean}}
\providecommand{\nDinovThreeConvnextLflairCleanVarTrainSubsetCleanTwoFive}{\tbd{nDinovThreeConvnextLflairCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\nDinovThreeConvnextLflairCoarseLOne}{\tbd{nDinovThreeConvnextLflairCoarseLOne}}
\providecommand{\nDinovThreeConvnextLflairCoarseLTwo}{\tbd{nDinovThreeConvnextLflairCoarseLTwo}}
\providecommand{\nDinovThreeConvnextLflairOmissionLOne}{\tbd{nDinovThreeConvnextLflairOmissionLOne}}
\providecommand{\nDinovThreeConvnextLflairOmissionLTwo}{\tbd{nDinovThreeConvnextLflairOmissionLTwo}}
\providecommand{\nDinovThreeConvnextLflairShiftLOne}{\tbd{nDinovThreeConvnextLflairShiftLOne}}
\providecommand{\nDinovThreeConvnextLflairShiftLTwo}{\tbd{nDinovThreeConvnextLflairShiftLTwo}}
\providecommand{\nLVDChesBoundaryLOne}{\tbd{nLVDChesBoundaryLOne}}
\providecommand{\nLVDChesBoundaryLTwo}{\tbd{nLVDChesBoundaryLTwo}}
\providecommand{\nLVDChesBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{nLVDChesBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDChesBoundaryLTwoVarDecoderSamLite}{\tbd{nLVDChesBoundaryLTwoVarDecoderSamLite}}
\providecommand{\nLVDChesBoundaryLTwoVarDecoderSegformerMlp}{\tbd{nLVDChesBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\nLVDChesBoundaryLTwoVarLrMultOne}{\tbd{nLVDChesBoundaryLTwoVarLrMultOne}}
\providecommand{\nLVDChesClean}{\tbd{nLVDChesClean}}
\providecommand{\nLVDChesCleanVarDecoderMaskTwoformerLite}{\tbd{nLVDChesCleanVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDChesCleanVarDecoderSamLite}{\tbd{nLVDChesCleanVarDecoderSamLite}}
\providecommand{\nLVDChesCleanVarDecoderSegformerMlp}{\tbd{nLVDChesCleanVarDecoderSegformerMlp}}
\providecommand{\nLVDChesCleanVarLrMultOne}{\tbd{nLVDChesCleanVarLrMultOne}}
\providecommand{\nLVDChesCoarseLOne}{\tbd{nLVDChesCoarseLOne}}
\providecommand{\nLVDChesCoarseLTwo}{\tbd{nLVDChesCoarseLTwo}}
\providecommand{\nLVDChesCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{nLVDChesCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDChesCoarseLTwoVarDecoderSamLite}{\tbd{nLVDChesCoarseLTwoVarDecoderSamLite}}
\providecommand{\nLVDChesCoarseLTwoVarDecoderSegformerMlp}{\tbd{nLVDChesCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\nLVDChesCoarseLTwoVarLrMultOne}{\tbd{nLVDChesCoarseLTwoVarLrMultOne}}
\providecommand{\nLVDChesNlcdREAL}{\tbd{nLVDChesNlcdREAL}}
\providecommand{\nLVDChesOmissionLOne}{\tbd{nLVDChesOmissionLOne}}
\providecommand{\nLVDChesOmissionLTwo}{\tbd{nLVDChesOmissionLTwo}}
\providecommand{\nLVDChesOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{nLVDChesOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDChesOmissionLTwoVarDecoderSamLite}{\tbd{nLVDChesOmissionLTwoVarDecoderSamLite}}
\providecommand{\nLVDChesOmissionLTwoVarDecoderSegformerMlp}{\tbd{nLVDChesOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\nLVDChesOmissionLTwoVarLrMultOne}{\tbd{nLVDChesOmissionLTwoVarLrMultOne}}
\providecommand{\nLVDChesShiftLOne}{\tbd{nLVDChesShiftLOne}}
\providecommand{\nLVDChesShiftLTwo}{\tbd{nLVDChesShiftLTwo}}
\providecommand{\nLVDChesShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{nLVDChesShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDChesShiftLTwoVarDecoderSamLite}{\tbd{nLVDChesShiftLTwoVarDecoderSamLite}}
\providecommand{\nLVDChesShiftLTwoVarDecoderSegformerMlp}{\tbd{nLVDChesShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\nLVDChesShiftLTwoVarLrMultOne}{\tbd{nLVDChesShiftLTwoVarLrMultOne}}
\providecommand{\nLVDCsTwelveBoundaryLOne}{\tbd{nLVDCsTwelveBoundaryLOne}}
\providecommand{\nLVDCsTwelveBoundaryLTwo}{\tbd{nLVDCsTwelveBoundaryLTwo}}
\providecommand{\nLVDCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{nLVDCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDCsTwelveBoundaryLTwoVarDecoderSamLite}{\tbd{nLVDCsTwelveBoundaryLTwoVarDecoderSamLite}}
\providecommand{\nLVDCsTwelveBoundaryLTwoVarDecoderSegformerMlp}{\tbd{nLVDCsTwelveBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\nLVDCsTwelveBoundaryLTwoVarLrMultOne}{\tbd{nLVDCsTwelveBoundaryLTwoVarLrMultOne}}
\providecommand{\nLVDCsTwelveClean}{\tbd{nLVDCsTwelveClean}}
\providecommand{\nLVDCsTwelveCleanVarDecoderMaskTwoformerLite}{\tbd{nLVDCsTwelveCleanVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDCsTwelveCleanVarDecoderSamLite}{\tbd{nLVDCsTwelveCleanVarDecoderSamLite}}
\providecommand{\nLVDCsTwelveCleanVarDecoderSegformerMlp}{\tbd{nLVDCsTwelveCleanVarDecoderSegformerMlp}}
\providecommand{\nLVDCsTwelveCleanVarLrMultOne}{\tbd{nLVDCsTwelveCleanVarLrMultOne}}
\providecommand{\nLVDCsTwelveCoarseLOne}{\tbd{nLVDCsTwelveCoarseLOne}}
\providecommand{\nLVDCsTwelveCoarseLTwo}{\tbd{nLVDCsTwelveCoarseLTwo}}
\providecommand{\nLVDCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{nLVDCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDCsTwelveCoarseLTwoVarDecoderSamLite}{\tbd{nLVDCsTwelveCoarseLTwoVarDecoderSamLite}}
\providecommand{\nLVDCsTwelveCoarseLTwoVarDecoderSegformerMlp}{\tbd{nLVDCsTwelveCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\nLVDCsTwelveCoarseLTwoVarLrMultOne}{\tbd{nLVDCsTwelveCoarseLTwoVarLrMultOne}}
\providecommand{\nLVDCsTwelveOmissionLOne}{\tbd{nLVDCsTwelveOmissionLOne}}
\providecommand{\nLVDCsTwelveOmissionLTwo}{\tbd{nLVDCsTwelveOmissionLTwo}}
\providecommand{\nLVDCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{nLVDCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDCsTwelveOmissionLTwoVarDecoderSamLite}{\tbd{nLVDCsTwelveOmissionLTwoVarDecoderSamLite}}
\providecommand{\nLVDCsTwelveOmissionLTwoVarDecoderSegformerMlp}{\tbd{nLVDCsTwelveOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\nLVDCsTwelveOmissionLTwoVarLrMultOne}{\tbd{nLVDCsTwelveOmissionLTwoVarLrMultOne}}
\providecommand{\nLVDCsTwelveSTwocloudlessREAL}{\tbd{nLVDCsTwelveSTwocloudlessREAL}}
\providecommand{\nLVDCsTwelveShiftLOne}{\tbd{nLVDCsTwelveShiftLOne}}
\providecommand{\nLVDCsTwelveShiftLTwo}{\tbd{nLVDCsTwelveShiftLTwo}}
\providecommand{\nLVDCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{nLVDCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDCsTwelveShiftLTwoVarDecoderSamLite}{\tbd{nLVDCsTwelveShiftLTwoVarDecoderSamLite}}
\providecommand{\nLVDCsTwelveShiftLTwoVarDecoderSegformerMlp}{\tbd{nLVDCsTwelveShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\nLVDCsTwelveShiftLTwoVarLrMultOne}{\tbd{nLVDCsTwelveShiftLTwoVarLrMultOne}}
\providecommand{\nLVDDfcBoundaryLOne}{\tbd{nLVDDfcBoundaryLOne}}
\providecommand{\nLVDDfcBoundaryLTwo}{\tbd{nLVDDfcBoundaryLTwo}}
\providecommand{\nLVDDfcBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{nLVDDfcBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDDfcBoundaryLTwoVarDecoderSamLite}{\tbd{nLVDDfcBoundaryLTwoVarDecoderSamLite}}
\providecommand{\nLVDDfcBoundaryLTwoVarDecoderSegformerMlp}{\tbd{nLVDDfcBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\nLVDDfcBoundaryLTwoVarLrMultOne}{\tbd{nLVDDfcBoundaryLTwoVarLrMultOne}}
\providecommand{\nLVDDfcClean}{\tbd{nLVDDfcClean}}
\providecommand{\nLVDDfcCleanVarDecoderMaskTwoformerLite}{\tbd{nLVDDfcCleanVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDDfcCleanVarDecoderSamLite}{\tbd{nLVDDfcCleanVarDecoderSamLite}}
\providecommand{\nLVDDfcCleanVarDecoderSegformerMlp}{\tbd{nLVDDfcCleanVarDecoderSegformerMlp}}
\providecommand{\nLVDDfcCleanVarLrMultOne}{\tbd{nLVDDfcCleanVarLrMultOne}}
\providecommand{\nLVDDfcCleanVarTrainSubsetRealcov}{\tbd{nLVDDfcCleanVarTrainSubsetRealcov}}
\providecommand{\nLVDDfcCoarseLOne}{\tbd{nLVDDfcCoarseLOne}}
\providecommand{\nLVDDfcCoarseLTwo}{\tbd{nLVDDfcCoarseLTwo}}
\providecommand{\nLVDDfcCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{nLVDDfcCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDDfcCoarseLTwoVarDecoderSamLite}{\tbd{nLVDDfcCoarseLTwoVarDecoderSamLite}}
\providecommand{\nLVDDfcCoarseLTwoVarDecoderSegformerMlp}{\tbd{nLVDDfcCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\nLVDDfcCoarseLTwoVarLrMultOne}{\tbd{nLVDDfcCoarseLTwoVarLrMultOne}}
\providecommand{\nLVDDfcModisREALVarTrainSubsetRealcov}{\tbd{nLVDDfcModisREALVarTrainSubsetRealcov}}
\providecommand{\nLVDDfcOmissionLOne}{\tbd{nLVDDfcOmissionLOne}}
\providecommand{\nLVDDfcOmissionLTwo}{\tbd{nLVDDfcOmissionLTwo}}
\providecommand{\nLVDDfcOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{nLVDDfcOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDDfcOmissionLTwoVarDecoderSamLite}{\tbd{nLVDDfcOmissionLTwoVarDecoderSamLite}}
\providecommand{\nLVDDfcOmissionLTwoVarDecoderSegformerMlp}{\tbd{nLVDDfcOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\nLVDDfcOmissionLTwoVarLrMultOne}{\tbd{nLVDDfcOmissionLTwoVarLrMultOne}}
\providecommand{\nLVDDfcShiftLOne}{\tbd{nLVDDfcShiftLOne}}
\providecommand{\nLVDDfcShiftLTwo}{\tbd{nLVDDfcShiftLTwo}}
\providecommand{\nLVDDfcShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{nLVDDfcShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDDfcShiftLTwoVarDecoderSamLite}{\tbd{nLVDDfcShiftLTwoVarDecoderSamLite}}
\providecommand{\nLVDDfcShiftLTwoVarDecoderSegformerMlp}{\tbd{nLVDDfcShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\nLVDDfcShiftLTwoVarLrMultOne}{\tbd{nLVDDfcShiftLTwoVarLrMultOne}}
\providecommand{\nLVDEnvaBoundaryLOne}{\tbd{nLVDEnvaBoundaryLOne}}
\providecommand{\nLVDEnvaBoundaryLTwo}{\tbd{nLVDEnvaBoundaryLTwo}}
\providecommand{\nLVDEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{nLVDEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDEnvaBoundaryLTwoVarDecoderSamLite}{\tbd{nLVDEnvaBoundaryLTwoVarDecoderSamLite}}
\providecommand{\nLVDEnvaBoundaryLTwoVarDecoderSegformerMlp}{\tbd{nLVDEnvaBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\nLVDEnvaBoundaryLTwoVarLrMultOne}{\tbd{nLVDEnvaBoundaryLTwoVarLrMultOne}}
\providecommand{\nLVDEnvaClean}{\tbd{nLVDEnvaClean}}
\providecommand{\nLVDEnvaCleanVarDecoderMaskTwoformerLite}{\tbd{nLVDEnvaCleanVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDEnvaCleanVarDecoderSamLite}{\tbd{nLVDEnvaCleanVarDecoderSamLite}}
\providecommand{\nLVDEnvaCleanVarDecoderSegformerMlp}{\tbd{nLVDEnvaCleanVarDecoderSegformerMlp}}
\providecommand{\nLVDEnvaCleanVarLrMultOne}{\tbd{nLVDEnvaCleanVarLrMultOne}}
\providecommand{\nLVDEnvaCoarseLOne}{\tbd{nLVDEnvaCoarseLOne}}
\providecommand{\nLVDEnvaCoarseLTwo}{\tbd{nLVDEnvaCoarseLTwo}}
\providecommand{\nLVDEnvaCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{nLVDEnvaCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDEnvaCoarseLTwoVarDecoderSamLite}{\tbd{nLVDEnvaCoarseLTwoVarDecoderSamLite}}
\providecommand{\nLVDEnvaCoarseLTwoVarDecoderSegformerMlp}{\tbd{nLVDEnvaCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\nLVDEnvaCoarseLTwoVarLrMultOne}{\tbd{nLVDEnvaCoarseLTwoVarLrMultOne}}
\providecommand{\nLVDEnvaNlcdREAL}{\tbd{nLVDEnvaNlcdREAL}}
\providecommand{\nLVDEnvaOmissionLOne}{\tbd{nLVDEnvaOmissionLOne}}
\providecommand{\nLVDEnvaOmissionLTwo}{\tbd{nLVDEnvaOmissionLTwo}}
\providecommand{\nLVDEnvaOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{nLVDEnvaOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDEnvaOmissionLTwoVarDecoderSamLite}{\tbd{nLVDEnvaOmissionLTwoVarDecoderSamLite}}
\providecommand{\nLVDEnvaOmissionLTwoVarDecoderSegformerMlp}{\tbd{nLVDEnvaOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\nLVDEnvaOmissionLTwoVarLrMultOne}{\tbd{nLVDEnvaOmissionLTwoVarLrMultOne}}
\providecommand{\nLVDEnvaShiftLOne}{\tbd{nLVDEnvaShiftLOne}}
\providecommand{\nLVDEnvaShiftLTwo}{\tbd{nLVDEnvaShiftLTwo}}
\providecommand{\nLVDEnvaShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{nLVDEnvaShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDEnvaShiftLTwoVarDecoderSamLite}{\tbd{nLVDEnvaShiftLTwoVarDecoderSamLite}}
\providecommand{\nLVDEnvaShiftLTwoVarDecoderSegformerMlp}{\tbd{nLVDEnvaShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\nLVDEnvaShiftLTwoVarLrMultOne}{\tbd{nLVDEnvaShiftLTwoVarLrMultOne}}
\providecommand{\nLVDKuroBoundaryLOne}{\tbd{nLVDKuroBoundaryLOne}}
\providecommand{\nLVDKuroBoundaryLTwo}{\tbd{nLVDKuroBoundaryLTwo}}
\providecommand{\nLVDKuroBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{nLVDKuroBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDKuroBoundaryLTwoVarDecoderSamLite}{\tbd{nLVDKuroBoundaryLTwoVarDecoderSamLite}}
\providecommand{\nLVDKuroBoundaryLTwoVarDecoderSegformerMlp}{\tbd{nLVDKuroBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\nLVDKuroBoundaryLTwoVarLrMultOne}{\tbd{nLVDKuroBoundaryLTwoVarLrMultOne}}
\providecommand{\nLVDKuroCemsREALVarTrainSubsetRealcov}{\tbd{nLVDKuroCemsREALVarTrainSubsetRealcov}}
\providecommand{\nLVDKuroClean}{\tbd{nLVDKuroClean}}
\providecommand{\nLVDKuroCleanVarDecoderMaskTwoformerLite}{\tbd{nLVDKuroCleanVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDKuroCleanVarDecoderSamLite}{\tbd{nLVDKuroCleanVarDecoderSamLite}}
\providecommand{\nLVDKuroCleanVarDecoderSegformerMlp}{\tbd{nLVDKuroCleanVarDecoderSegformerMlp}}
\providecommand{\nLVDKuroCleanVarLrMultOne}{\tbd{nLVDKuroCleanVarLrMultOne}}
\providecommand{\nLVDKuroCleanVarTrainSubsetRealcov}{\tbd{nLVDKuroCleanVarTrainSubsetRealcov}}
\providecommand{\nLVDKuroCoarseLOne}{\tbd{nLVDKuroCoarseLOne}}
\providecommand{\nLVDKuroCoarseLTwo}{\tbd{nLVDKuroCoarseLTwo}}
\providecommand{\nLVDKuroCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{nLVDKuroCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDKuroCoarseLTwoVarDecoderSamLite}{\tbd{nLVDKuroCoarseLTwoVarDecoderSamLite}}
\providecommand{\nLVDKuroCoarseLTwoVarDecoderSegformerMlp}{\tbd{nLVDKuroCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\nLVDKuroCoarseLTwoVarLrMultOne}{\tbd{nLVDKuroCoarseLTwoVarLrMultOne}}
\providecommand{\nLVDKuroOmissionLOne}{\tbd{nLVDKuroOmissionLOne}}
\providecommand{\nLVDKuroOmissionLTwo}{\tbd{nLVDKuroOmissionLTwo}}
\providecommand{\nLVDKuroOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{nLVDKuroOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDKuroOmissionLTwoVarDecoderSamLite}{\tbd{nLVDKuroOmissionLTwoVarDecoderSamLite}}
\providecommand{\nLVDKuroOmissionLTwoVarDecoderSegformerMlp}{\tbd{nLVDKuroOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\nLVDKuroOmissionLTwoVarLrMultOne}{\tbd{nLVDKuroOmissionLTwoVarLrMultOne}}
\providecommand{\nLVDKuroShiftLOne}{\tbd{nLVDKuroShiftLOne}}
\providecommand{\nLVDKuroShiftLTwo}{\tbd{nLVDKuroShiftLTwo}}
\providecommand{\nLVDKuroShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{nLVDKuroShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDKuroShiftLTwoVarDecoderSamLite}{\tbd{nLVDKuroShiftLTwoVarDecoderSamLite}}
\providecommand{\nLVDKuroShiftLTwoVarDecoderSegformerMlp}{\tbd{nLVDKuroShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\nLVDKuroShiftLTwoVarLrMultOne}{\tbd{nLVDKuroShiftLTwoVarLrMultOne}}
\providecommand{\nLVDOemBoundaryLOne}{\tbd{nLVDOemBoundaryLOne}}
\providecommand{\nLVDOemBoundaryLTwo}{\tbd{nLVDOemBoundaryLTwo}}
\providecommand{\nLVDOemBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{nLVDOemBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDOemBoundaryLTwoVarDecoderSamLite}{\tbd{nLVDOemBoundaryLTwoVarDecoderSamLite}}
\providecommand{\nLVDOemBoundaryLTwoVarDecoderSegformerMlp}{\tbd{nLVDOemBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\nLVDOemBoundaryLTwoVarLrMultOne}{\tbd{nLVDOemBoundaryLTwoVarLrMultOne}}
\providecommand{\nLVDOemClean}{\tbd{nLVDOemClean}}
\providecommand{\nLVDOemCleanVarDecoderMaskTwoformerLite}{\tbd{nLVDOemCleanVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDOemCleanVarDecoderSamLite}{\tbd{nLVDOemCleanVarDecoderSamLite}}
\providecommand{\nLVDOemCleanVarDecoderSegformerMlp}{\tbd{nLVDOemCleanVarDecoderSegformerMlp}}
\providecommand{\nLVDOemCleanVarLrMultOne}{\tbd{nLVDOemCleanVarLrMultOne}}
\providecommand{\nLVDOemCoarseLOne}{\tbd{nLVDOemCoarseLOne}}
\providecommand{\nLVDOemCoarseLTwo}{\tbd{nLVDOemCoarseLTwo}}
\providecommand{\nLVDOemCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{nLVDOemCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDOemCoarseLTwoVarDecoderSamLite}{\tbd{nLVDOemCoarseLTwoVarDecoderSamLite}}
\providecommand{\nLVDOemCoarseLTwoVarDecoderSegformerMlp}{\tbd{nLVDOemCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\nLVDOemCoarseLTwoVarLrMultOne}{\tbd{nLVDOemCoarseLTwoVarLrMultOne}}
\providecommand{\nLVDOemOmissionLOne}{\tbd{nLVDOemOmissionLOne}}
\providecommand{\nLVDOemOmissionLTwo}{\tbd{nLVDOemOmissionLTwo}}
\providecommand{\nLVDOemOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{nLVDOemOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDOemOmissionLTwoVarDecoderSamLite}{\tbd{nLVDOemOmissionLTwoVarDecoderSamLite}}
\providecommand{\nLVDOemOmissionLTwoVarDecoderSegformerMlp}{\tbd{nLVDOemOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\nLVDOemOmissionLTwoVarLrMultOne}{\tbd{nLVDOemOmissionLTwoVarLrMultOne}}
\providecommand{\nLVDOemShiftLOne}{\tbd{nLVDOemShiftLOne}}
\providecommand{\nLVDOemShiftLTwo}{\tbd{nLVDOemShiftLTwo}}
\providecommand{\nLVDOemShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{nLVDOemShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDOemShiftLTwoVarDecoderSamLite}{\tbd{nLVDOemShiftLTwoVarDecoderSamLite}}
\providecommand{\nLVDOemShiftLTwoVarDecoderSegformerMlp}{\tbd{nLVDOemShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\nLVDOemShiftLTwoVarLrMultOne}{\tbd{nLVDOemShiftLTwoVarLrMultOne}}
\providecommand{\nLVDSnTwoBoundaryLOne}{\tbd{nLVDSnTwoBoundaryLOne}}
\providecommand{\nLVDSnTwoBoundaryLTwo}{\tbd{nLVDSnTwoBoundaryLTwo}}
\providecommand{\nLVDSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{nLVDSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDSnTwoBoundaryLTwoVarDecoderSamLite}{\tbd{nLVDSnTwoBoundaryLTwoVarDecoderSamLite}}
\providecommand{\nLVDSnTwoBoundaryLTwoVarDecoderSegformerMlp}{\tbd{nLVDSnTwoBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\nLVDSnTwoBoundaryLTwoVarLrMultOne}{\tbd{nLVDSnTwoBoundaryLTwoVarLrMultOne}}
\providecommand{\nLVDSnTwoClean}{\tbd{nLVDSnTwoClean}}
\providecommand{\nLVDSnTwoCleanVarDecoderMaskTwoformerLite}{\tbd{nLVDSnTwoCleanVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDSnTwoCleanVarDecoderSamLite}{\tbd{nLVDSnTwoCleanVarDecoderSamLite}}
\providecommand{\nLVDSnTwoCleanVarDecoderSegformerMlp}{\tbd{nLVDSnTwoCleanVarDecoderSegformerMlp}}
\providecommand{\nLVDSnTwoCleanVarLrMultOne}{\tbd{nLVDSnTwoCleanVarLrMultOne}}
\providecommand{\nLVDSnTwoCoarseLOne}{\tbd{nLVDSnTwoCoarseLOne}}
\providecommand{\nLVDSnTwoCoarseLTwo}{\tbd{nLVDSnTwoCoarseLTwo}}
\providecommand{\nLVDSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{nLVDSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDSnTwoCoarseLTwoVarDecoderSamLite}{\tbd{nLVDSnTwoCoarseLTwoVarDecoderSamLite}}
\providecommand{\nLVDSnTwoCoarseLTwoVarDecoderSegformerMlp}{\tbd{nLVDSnTwoCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\nLVDSnTwoCoarseLTwoVarLrMultOne}{\tbd{nLVDSnTwoCoarseLTwoVarLrMultOne}}
\providecommand{\nLVDSnTwoOmissionLOne}{\tbd{nLVDSnTwoOmissionLOne}}
\providecommand{\nLVDSnTwoOmissionLTwo}{\tbd{nLVDSnTwoOmissionLTwo}}
\providecommand{\nLVDSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{nLVDSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDSnTwoOmissionLTwoVarDecoderSamLite}{\tbd{nLVDSnTwoOmissionLTwoVarDecoderSamLite}}
\providecommand{\nLVDSnTwoOmissionLTwoVarDecoderSegformerMlp}{\tbd{nLVDSnTwoOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\nLVDSnTwoOmissionLTwoVarLrMultOne}{\tbd{nLVDSnTwoOmissionLTwoVarLrMultOne}}
\providecommand{\nLVDSnTwoShiftLOne}{\tbd{nLVDSnTwoShiftLOne}}
\providecommand{\nLVDSnTwoShiftLTwo}{\tbd{nLVDSnTwoShiftLTwo}}
\providecommand{\nLVDSnTwoShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{nLVDSnTwoShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDSnTwoShiftLTwoVarDecoderSamLite}{\tbd{nLVDSnTwoShiftLTwoVarDecoderSamLite}}
\providecommand{\nLVDSnTwoShiftLTwoVarDecoderSegformerMlp}{\tbd{nLVDSnTwoShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\nLVDSnTwoShiftLTwoVarLrMultOne}{\tbd{nLVDSnTwoShiftLTwoVarLrMultOne}}
\providecommand{\nLVDburnBoundaryLOne}{\tbd{nLVDburnBoundaryLOne}}
\providecommand{\nLVDburnBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{nLVDburnBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nLVDburnBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{nLVDburnBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDburnBoundaryLOneVarDecoderSamLite}{\tbd{nLVDburnBoundaryLOneVarDecoderSamLite}}
\providecommand{\nLVDburnBoundaryLOneVarDecoderSamPretrained}{\tbd{nLVDburnBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\nLVDburnBoundaryLOneVarDecoderSegformerMlp}{\tbd{nLVDburnBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\nLVDburnBoundaryLR}{\tbd{nLVDburnBoundaryLR}}
\providecommand{\nLVDburnBoundaryLRVarLrMultOne}{\tbd{nLVDburnBoundaryLRVarLrMultOne}}
\providecommand{\nLVDburnBoundaryLTwo}{\tbd{nLVDburnBoundaryLTwo}}
\providecommand{\nLVDburnBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{nLVDburnBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nLVDburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{nLVDburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\nLVDburnBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{nLVDburnBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{nLVDburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\nLVDburnBoundaryLTwoVarDecoderSamLite}{\tbd{nLVDburnBoundaryLTwoVarDecoderSamLite}}
\providecommand{\nLVDburnBoundaryLTwoVarDecoderSamLiteLrMultOne}{\tbd{nLVDburnBoundaryLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\nLVDburnBoundaryLTwoVarDecoderSamPretrained}{\tbd{nLVDburnBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\nLVDburnBoundaryLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{nLVDburnBoundaryLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\nLVDburnBoundaryLTwoVarDecoderSegformerMlp}{\tbd{nLVDburnBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\nLVDburnBoundaryLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{nLVDburnBoundaryLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\nLVDburnBoundaryLTwoVarLossBootstrap}{\tbd{nLVDburnBoundaryLTwoVarLossBootstrap}}
\providecommand{\nLVDburnBoundaryLTwoVarLossGce}{\tbd{nLVDburnBoundaryLTwoVarLossGce}}
\providecommand{\nLVDburnBoundaryLTwoVarLrMultOne}{\tbd{nLVDburnBoundaryLTwoVarLrMultOne}}
\providecommand{\nLVDburnBoundaryLTwoVarLrMultThree}{\tbd{nLVDburnBoundaryLTwoVarLrMultThree}}
\providecommand{\nLVDburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nLVDburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nLVDburnBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{nLVDburnBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nLVDburnClean}{\tbd{nLVDburnClean}}
\providecommand{\nLVDburnCleanVarDecoderMaskTwoformerFull}{\tbd{nLVDburnCleanVarDecoderMaskTwoformerFull}}
\providecommand{\nLVDburnCleanVarDecoderMaskTwoformerFullLrMultOne}{\tbd{nLVDburnCleanVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\nLVDburnCleanVarDecoderMaskTwoformerLite}{\tbd{nLVDburnCleanVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDburnCleanVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{nLVDburnCleanVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\nLVDburnCleanVarDecoderSamLite}{\tbd{nLVDburnCleanVarDecoderSamLite}}
\providecommand{\nLVDburnCleanVarDecoderSamLiteLrMultOne}{\tbd{nLVDburnCleanVarDecoderSamLiteLrMultOne}}
\providecommand{\nLVDburnCleanVarDecoderSamPretrained}{\tbd{nLVDburnCleanVarDecoderSamPretrained}}
\providecommand{\nLVDburnCleanVarDecoderSamPretrainedLrMultOne}{\tbd{nLVDburnCleanVarDecoderSamPretrainedLrMultOne}}
\providecommand{\nLVDburnCleanVarDecoderSegformerMlp}{\tbd{nLVDburnCleanVarDecoderSegformerMlp}}
\providecommand{\nLVDburnCleanVarDecoderSegformerMlpLrMultOne}{\tbd{nLVDburnCleanVarDecoderSegformerMlpLrMultOne}}
\providecommand{\nLVDburnCleanVarLossBootstrap}{\tbd{nLVDburnCleanVarLossBootstrap}}
\providecommand{\nLVDburnCleanVarLossGce}{\tbd{nLVDburnCleanVarLossGce}}
\providecommand{\nLVDburnCleanVarLrMultOne}{\tbd{nLVDburnCleanVarLrMultOne}}
\providecommand{\nLVDburnCleanVarLrMultThree}{\tbd{nLVDburnCleanVarLrMultThree}}
\providecommand{\nLVDburnCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{nLVDburnCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nLVDburnCleanVarTrainSubsetCleanTwoFive}{\tbd{nLVDburnCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\nLVDburnCoarseLOne}{\tbd{nLVDburnCoarseLOne}}
\providecommand{\nLVDburnCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{nLVDburnCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nLVDburnCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{nLVDburnCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDburnCoarseLOneVarDecoderSamLite}{\tbd{nLVDburnCoarseLOneVarDecoderSamLite}}
\providecommand{\nLVDburnCoarseLOneVarDecoderSamPretrained}{\tbd{nLVDburnCoarseLOneVarDecoderSamPretrained}}
\providecommand{\nLVDburnCoarseLOneVarDecoderSegformerMlp}{\tbd{nLVDburnCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\nLVDburnCoarseLR}{\tbd{nLVDburnCoarseLR}}
\providecommand{\nLVDburnCoarseLRVarLrMultOne}{\tbd{nLVDburnCoarseLRVarLrMultOne}}
\providecommand{\nLVDburnCoarseLTwo}{\tbd{nLVDburnCoarseLTwo}}
\providecommand{\nLVDburnCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{nLVDburnCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nLVDburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{nLVDburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\nLVDburnCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{nLVDburnCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{nLVDburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\nLVDburnCoarseLTwoVarDecoderSamLite}{\tbd{nLVDburnCoarseLTwoVarDecoderSamLite}}
\providecommand{\nLVDburnCoarseLTwoVarDecoderSamLiteLrMultOne}{\tbd{nLVDburnCoarseLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\nLVDburnCoarseLTwoVarDecoderSamPretrained}{\tbd{nLVDburnCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\nLVDburnCoarseLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{nLVDburnCoarseLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\nLVDburnCoarseLTwoVarDecoderSegformerMlp}{\tbd{nLVDburnCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\nLVDburnCoarseLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{nLVDburnCoarseLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\nLVDburnCoarseLTwoVarLossBootstrap}{\tbd{nLVDburnCoarseLTwoVarLossBootstrap}}
\providecommand{\nLVDburnCoarseLTwoVarLossGce}{\tbd{nLVDburnCoarseLTwoVarLossGce}}
\providecommand{\nLVDburnCoarseLTwoVarLrMultOne}{\tbd{nLVDburnCoarseLTwoVarLrMultOne}}
\providecommand{\nLVDburnCoarseLTwoVarLrMultThree}{\tbd{nLVDburnCoarseLTwoVarLrMultThree}}
\providecommand{\nLVDburnCoarseLTwoVarLrMultZeroOneOneOneOne}{\tbd{nLVDburnCoarseLTwoVarLrMultZeroOneOneOneOne}}
\providecommand{\nLVDburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nLVDburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nLVDburnCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{nLVDburnCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nLVDburnOmissionLOne}{\tbd{nLVDburnOmissionLOne}}
\providecommand{\nLVDburnOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{nLVDburnOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nLVDburnOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{nLVDburnOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDburnOmissionLOneVarDecoderSamLite}{\tbd{nLVDburnOmissionLOneVarDecoderSamLite}}
\providecommand{\nLVDburnOmissionLOneVarDecoderSamPretrained}{\tbd{nLVDburnOmissionLOneVarDecoderSamPretrained}}
\providecommand{\nLVDburnOmissionLOneVarDecoderSegformerMlp}{\tbd{nLVDburnOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\nLVDburnOmissionLR}{\tbd{nLVDburnOmissionLR}}
\providecommand{\nLVDburnOmissionLRVarLrMultOne}{\tbd{nLVDburnOmissionLRVarLrMultOne}}
\providecommand{\nLVDburnOmissionLTwo}{\tbd{nLVDburnOmissionLTwo}}
\providecommand{\nLVDburnOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{nLVDburnOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nLVDburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{nLVDburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\nLVDburnOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{nLVDburnOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{nLVDburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\nLVDburnOmissionLTwoVarDecoderSamLite}{\tbd{nLVDburnOmissionLTwoVarDecoderSamLite}}
\providecommand{\nLVDburnOmissionLTwoVarDecoderSamLiteLrMultOne}{\tbd{nLVDburnOmissionLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\nLVDburnOmissionLTwoVarDecoderSamPretrained}{\tbd{nLVDburnOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\nLVDburnOmissionLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{nLVDburnOmissionLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\nLVDburnOmissionLTwoVarDecoderSegformerMlp}{\tbd{nLVDburnOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\nLVDburnOmissionLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{nLVDburnOmissionLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\nLVDburnOmissionLTwoVarLossBootstrap}{\tbd{nLVDburnOmissionLTwoVarLossBootstrap}}
\providecommand{\nLVDburnOmissionLTwoVarLossGce}{\tbd{nLVDburnOmissionLTwoVarLossGce}}
\providecommand{\nLVDburnOmissionLTwoVarLrMultOne}{\tbd{nLVDburnOmissionLTwoVarLrMultOne}}
\providecommand{\nLVDburnOmissionLTwoVarLrMultThree}{\tbd{nLVDburnOmissionLTwoVarLrMultThree}}
\providecommand{\nLVDburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nLVDburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nLVDburnOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{nLVDburnOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nLVDburnShiftLOne}{\tbd{nLVDburnShiftLOne}}
\providecommand{\nLVDburnShiftLOneVarDecoderMaskTwoformerFull}{\tbd{nLVDburnShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nLVDburnShiftLOneVarDecoderMaskTwoformerLite}{\tbd{nLVDburnShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDburnShiftLOneVarDecoderSamLite}{\tbd{nLVDburnShiftLOneVarDecoderSamLite}}
\providecommand{\nLVDburnShiftLOneVarDecoderSamPretrained}{\tbd{nLVDburnShiftLOneVarDecoderSamPretrained}}
\providecommand{\nLVDburnShiftLOneVarDecoderSegformerMlp}{\tbd{nLVDburnShiftLOneVarDecoderSegformerMlp}}
\providecommand{\nLVDburnShiftLR}{\tbd{nLVDburnShiftLR}}
\providecommand{\nLVDburnShiftLRVarLrMultOne}{\tbd{nLVDburnShiftLRVarLrMultOne}}
\providecommand{\nLVDburnShiftLTwo}{\tbd{nLVDburnShiftLTwo}}
\providecommand{\nLVDburnShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{nLVDburnShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nLVDburnShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{nLVDburnShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\nLVDburnShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{nLVDburnShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{nLVDburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\nLVDburnShiftLTwoVarDecoderSamLite}{\tbd{nLVDburnShiftLTwoVarDecoderSamLite}}
\providecommand{\nLVDburnShiftLTwoVarDecoderSamLiteLrMultOne}{\tbd{nLVDburnShiftLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\nLVDburnShiftLTwoVarDecoderSamPretrained}{\tbd{nLVDburnShiftLTwoVarDecoderSamPretrained}}
\providecommand{\nLVDburnShiftLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{nLVDburnShiftLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\nLVDburnShiftLTwoVarDecoderSegformerMlp}{\tbd{nLVDburnShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\nLVDburnShiftLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{nLVDburnShiftLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\nLVDburnShiftLTwoVarLossBootstrap}{\tbd{nLVDburnShiftLTwoVarLossBootstrap}}
\providecommand{\nLVDburnShiftLTwoVarLossGce}{\tbd{nLVDburnShiftLTwoVarLossGce}}
\providecommand{\nLVDburnShiftLTwoVarLrMultOne}{\tbd{nLVDburnShiftLTwoVarLrMultOne}}
\providecommand{\nLVDburnShiftLTwoVarLrMultThree}{\tbd{nLVDburnShiftLTwoVarLrMultThree}}
\providecommand{\nLVDburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nLVDburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nLVDburnShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{nLVDburnShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nLVDflairBoundaryLOne}{\tbd{nLVDflairBoundaryLOne}}
\providecommand{\nLVDflairBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{nLVDflairBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nLVDflairBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{nLVDflairBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDflairBoundaryLOneVarDecoderSamLite}{\tbd{nLVDflairBoundaryLOneVarDecoderSamLite}}
\providecommand{\nLVDflairBoundaryLOneVarDecoderSamPretrained}{\tbd{nLVDflairBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\nLVDflairBoundaryLOneVarDecoderSegformerMlp}{\tbd{nLVDflairBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\nLVDflairBoundaryLR}{\tbd{nLVDflairBoundaryLR}}
\providecommand{\nLVDflairBoundaryLRVarLrMultOne}{\tbd{nLVDflairBoundaryLRVarLrMultOne}}
\providecommand{\nLVDflairBoundaryLTwo}{\tbd{nLVDflairBoundaryLTwo}}
\providecommand{\nLVDflairBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{nLVDflairBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nLVDflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{nLVDflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\nLVDflairBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{nLVDflairBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{nLVDflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\nLVDflairBoundaryLTwoVarDecoderSamLite}{\tbd{nLVDflairBoundaryLTwoVarDecoderSamLite}}
\providecommand{\nLVDflairBoundaryLTwoVarDecoderSamLiteLrMultOne}{\tbd{nLVDflairBoundaryLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\nLVDflairBoundaryLTwoVarDecoderSamPretrained}{\tbd{nLVDflairBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\nLVDflairBoundaryLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{nLVDflairBoundaryLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\nLVDflairBoundaryLTwoVarDecoderSegformerMlp}{\tbd{nLVDflairBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\nLVDflairBoundaryLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{nLVDflairBoundaryLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\nLVDflairBoundaryLTwoVarLossBootstrap}{\tbd{nLVDflairBoundaryLTwoVarLossBootstrap}}
\providecommand{\nLVDflairBoundaryLTwoVarLossGce}{\tbd{nLVDflairBoundaryLTwoVarLossGce}}
\providecommand{\nLVDflairBoundaryLTwoVarLrMultOne}{\tbd{nLVDflairBoundaryLTwoVarLrMultOne}}
\providecommand{\nLVDflairBoundaryLTwoVarLrMultThree}{\tbd{nLVDflairBoundaryLTwoVarLrMultThree}}
\providecommand{\nLVDflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nLVDflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nLVDflairBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{nLVDflairBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nLVDflairClean}{\tbd{nLVDflairClean}}
\providecommand{\nLVDflairCleanVarDecoderMaskTwoformerFull}{\tbd{nLVDflairCleanVarDecoderMaskTwoformerFull}}
\providecommand{\nLVDflairCleanVarDecoderMaskTwoformerFullLrMultOne}{\tbd{nLVDflairCleanVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\nLVDflairCleanVarDecoderMaskTwoformerLite}{\tbd{nLVDflairCleanVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDflairCleanVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{nLVDflairCleanVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\nLVDflairCleanVarDecoderSamLite}{\tbd{nLVDflairCleanVarDecoderSamLite}}
\providecommand{\nLVDflairCleanVarDecoderSamLiteLrMultOne}{\tbd{nLVDflairCleanVarDecoderSamLiteLrMultOne}}
\providecommand{\nLVDflairCleanVarDecoderSamPretrained}{\tbd{nLVDflairCleanVarDecoderSamPretrained}}
\providecommand{\nLVDflairCleanVarDecoderSamPretrainedLrMultOne}{\tbd{nLVDflairCleanVarDecoderSamPretrainedLrMultOne}}
\providecommand{\nLVDflairCleanVarDecoderSegformerMlp}{\tbd{nLVDflairCleanVarDecoderSegformerMlp}}
\providecommand{\nLVDflairCleanVarDecoderSegformerMlpLrMultOne}{\tbd{nLVDflairCleanVarDecoderSegformerMlpLrMultOne}}
\providecommand{\nLVDflairCleanVarLossBootstrap}{\tbd{nLVDflairCleanVarLossBootstrap}}
\providecommand{\nLVDflairCleanVarLossGce}{\tbd{nLVDflairCleanVarLossGce}}
\providecommand{\nLVDflairCleanVarLrMultOne}{\tbd{nLVDflairCleanVarLrMultOne}}
\providecommand{\nLVDflairCleanVarLrMultThree}{\tbd{nLVDflairCleanVarLrMultThree}}
\providecommand{\nLVDflairCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{nLVDflairCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nLVDflairCleanVarTrainSubsetCleanTwoFive}{\tbd{nLVDflairCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\nLVDflairCoarseLOne}{\tbd{nLVDflairCoarseLOne}}
\providecommand{\nLVDflairCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{nLVDflairCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nLVDflairCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{nLVDflairCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDflairCoarseLOneVarDecoderSamLite}{\tbd{nLVDflairCoarseLOneVarDecoderSamLite}}
\providecommand{\nLVDflairCoarseLOneVarDecoderSamPretrained}{\tbd{nLVDflairCoarseLOneVarDecoderSamPretrained}}
\providecommand{\nLVDflairCoarseLOneVarDecoderSegformerMlp}{\tbd{nLVDflairCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\nLVDflairCoarseLR}{\tbd{nLVDflairCoarseLR}}
\providecommand{\nLVDflairCoarseLRVarLrMultOne}{\tbd{nLVDflairCoarseLRVarLrMultOne}}
\providecommand{\nLVDflairCoarseLTwo}{\tbd{nLVDflairCoarseLTwo}}
\providecommand{\nLVDflairCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{nLVDflairCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nLVDflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{nLVDflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\nLVDflairCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{nLVDflairCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{nLVDflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\nLVDflairCoarseLTwoVarDecoderSamLite}{\tbd{nLVDflairCoarseLTwoVarDecoderSamLite}}
\providecommand{\nLVDflairCoarseLTwoVarDecoderSamLiteLrMultOne}{\tbd{nLVDflairCoarseLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\nLVDflairCoarseLTwoVarDecoderSamPretrained}{\tbd{nLVDflairCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\nLVDflairCoarseLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{nLVDflairCoarseLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\nLVDflairCoarseLTwoVarDecoderSegformerMlp}{\tbd{nLVDflairCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\nLVDflairCoarseLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{nLVDflairCoarseLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\nLVDflairCoarseLTwoVarLossBootstrap}{\tbd{nLVDflairCoarseLTwoVarLossBootstrap}}
\providecommand{\nLVDflairCoarseLTwoVarLossGce}{\tbd{nLVDflairCoarseLTwoVarLossGce}}
\providecommand{\nLVDflairCoarseLTwoVarLrMultOne}{\tbd{nLVDflairCoarseLTwoVarLrMultOne}}
\providecommand{\nLVDflairCoarseLTwoVarLrMultThree}{\tbd{nLVDflairCoarseLTwoVarLrMultThree}}
\providecommand{\nLVDflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nLVDflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nLVDflairCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{nLVDflairCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nLVDflairOmissionLOne}{\tbd{nLVDflairOmissionLOne}}
\providecommand{\nLVDflairOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{nLVDflairOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nLVDflairOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{nLVDflairOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDflairOmissionLOneVarDecoderSamLite}{\tbd{nLVDflairOmissionLOneVarDecoderSamLite}}
\providecommand{\nLVDflairOmissionLOneVarDecoderSamPretrained}{\tbd{nLVDflairOmissionLOneVarDecoderSamPretrained}}
\providecommand{\nLVDflairOmissionLOneVarDecoderSegformerMlp}{\tbd{nLVDflairOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\nLVDflairOmissionLR}{\tbd{nLVDflairOmissionLR}}
\providecommand{\nLVDflairOmissionLRVarLrMultOne}{\tbd{nLVDflairOmissionLRVarLrMultOne}}
\providecommand{\nLVDflairOmissionLTwo}{\tbd{nLVDflairOmissionLTwo}}
\providecommand{\nLVDflairOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{nLVDflairOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nLVDflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{nLVDflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\nLVDflairOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{nLVDflairOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{nLVDflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\nLVDflairOmissionLTwoVarDecoderSamLite}{\tbd{nLVDflairOmissionLTwoVarDecoderSamLite}}
\providecommand{\nLVDflairOmissionLTwoVarDecoderSamLiteLrMultOne}{\tbd{nLVDflairOmissionLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\nLVDflairOmissionLTwoVarDecoderSamPretrained}{\tbd{nLVDflairOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\nLVDflairOmissionLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{nLVDflairOmissionLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\nLVDflairOmissionLTwoVarDecoderSegformerMlp}{\tbd{nLVDflairOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\nLVDflairOmissionLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{nLVDflairOmissionLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\nLVDflairOmissionLTwoVarLossBootstrap}{\tbd{nLVDflairOmissionLTwoVarLossBootstrap}}
\providecommand{\nLVDflairOmissionLTwoVarLossGce}{\tbd{nLVDflairOmissionLTwoVarLossGce}}
\providecommand{\nLVDflairOmissionLTwoVarLrMultOne}{\tbd{nLVDflairOmissionLTwoVarLrMultOne}}
\providecommand{\nLVDflairOmissionLTwoVarLrMultThree}{\tbd{nLVDflairOmissionLTwoVarLrMultThree}}
\providecommand{\nLVDflairOmissionLTwoVarLrMultZeroOneOneOneOne}{\tbd{nLVDflairOmissionLTwoVarLrMultZeroOneOneOneOne}}
\providecommand{\nLVDflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nLVDflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nLVDflairOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{nLVDflairOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nLVDflairShiftLOne}{\tbd{nLVDflairShiftLOne}}
\providecommand{\nLVDflairShiftLOneVarDecoderMaskTwoformerFull}{\tbd{nLVDflairShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nLVDflairShiftLOneVarDecoderMaskTwoformerLite}{\tbd{nLVDflairShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDflairShiftLOneVarDecoderSamLite}{\tbd{nLVDflairShiftLOneVarDecoderSamLite}}
\providecommand{\nLVDflairShiftLOneVarDecoderSamPretrained}{\tbd{nLVDflairShiftLOneVarDecoderSamPretrained}}
\providecommand{\nLVDflairShiftLOneVarDecoderSegformerMlp}{\tbd{nLVDflairShiftLOneVarDecoderSegformerMlp}}
\providecommand{\nLVDflairShiftLR}{\tbd{nLVDflairShiftLR}}
\providecommand{\nLVDflairShiftLRVarLrMultOne}{\tbd{nLVDflairShiftLRVarLrMultOne}}
\providecommand{\nLVDflairShiftLTwo}{\tbd{nLVDflairShiftLTwo}}
\providecommand{\nLVDflairShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{nLVDflairShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nLVDflairShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{nLVDflairShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\nLVDflairShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{nLVDflairShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nLVDflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{nLVDflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\nLVDflairShiftLTwoVarDecoderSamLite}{\tbd{nLVDflairShiftLTwoVarDecoderSamLite}}
\providecommand{\nLVDflairShiftLTwoVarDecoderSamLiteLrMultOne}{\tbd{nLVDflairShiftLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\nLVDflairShiftLTwoVarDecoderSamPretrained}{\tbd{nLVDflairShiftLTwoVarDecoderSamPretrained}}
\providecommand{\nLVDflairShiftLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{nLVDflairShiftLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\nLVDflairShiftLTwoVarDecoderSegformerMlp}{\tbd{nLVDflairShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\nLVDflairShiftLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{nLVDflairShiftLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\nLVDflairShiftLTwoVarLossBootstrap}{\tbd{nLVDflairShiftLTwoVarLossBootstrap}}
\providecommand{\nLVDflairShiftLTwoVarLossGce}{\tbd{nLVDflairShiftLTwoVarLossGce}}
\providecommand{\nLVDflairShiftLTwoVarLrMultOne}{\tbd{nLVDflairShiftLTwoVarLrMultOne}}
\providecommand{\nLVDflairShiftLTwoVarLrMultThree}{\tbd{nLVDflairShiftLTwoVarLrMultThree}}
\providecommand{\nLVDflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nLVDflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nLVDflairShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{nLVDflairShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nLVDsenClean}{\tbd{nLVDsenClean}}
\providecommand{\nLVDsenOtsuLTwo}{\tbd{nLVDsenOtsuLTwo}}
\providecommand{\nPRIburnBoundaryLOne}{\tbd{nPRIburnBoundaryLOne}}
\providecommand{\nPRIburnBoundaryLTwo}{\tbd{nPRIburnBoundaryLTwo}}
\providecommand{\nPRIburnClean}{\tbd{nPRIburnClean}}
\providecommand{\nPRIburnCleanVarTrainSubsetCleanTwoFive}{\tbd{nPRIburnCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\nPRIburnCoarseLOne}{\tbd{nPRIburnCoarseLOne}}
\providecommand{\nPRIburnCoarseLTwo}{\tbd{nPRIburnCoarseLTwo}}
\providecommand{\nPRIburnOmissionLOne}{\tbd{nPRIburnOmissionLOne}}
\providecommand{\nPRIburnOmissionLTwo}{\tbd{nPRIburnOmissionLTwo}}
\providecommand{\nPRIburnShiftLOne}{\tbd{nPRIburnShiftLOne}}
\providecommand{\nPRIburnShiftLTwo}{\tbd{nPRIburnShiftLTwo}}
\providecommand{\nPRIflairBoundaryLOne}{\tbd{nPRIflairBoundaryLOne}}
\providecommand{\nPRIflairBoundaryLTwo}{\tbd{nPRIflairBoundaryLTwo}}
\providecommand{\nPRIflairClean}{\tbd{nPRIflairClean}}
\providecommand{\nPRIflairCleanVarTrainSubsetCleanTwoFive}{\tbd{nPRIflairCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\nPRIflairCoarseLOne}{\tbd{nPRIflairCoarseLOne}}
\providecommand{\nPRIflairCoarseLTwo}{\tbd{nPRIflairCoarseLTwo}}
\providecommand{\nPRIflairOmissionLOne}{\tbd{nPRIflairOmissionLOne}}
\providecommand{\nPRIflairOmissionLTwo}{\tbd{nPRIflairOmissionLTwo}}
\providecommand{\nPRIflairShiftLOne}{\tbd{nPRIflairShiftLOne}}
\providecommand{\nPRIflairShiftLTwo}{\tbd{nPRIflairShiftLTwo}}
\providecommand{\nRNChesBoundaryLOne}{\tbd{nRNChesBoundaryLOne}}
\providecommand{\nRNChesBoundaryLTwo}{\tbd{nRNChesBoundaryLTwo}}
\providecommand{\nRNChesClean}{\tbd{nRNChesClean}}
\providecommand{\nRNChesCoarseLOne}{\tbd{nRNChesCoarseLOne}}
\providecommand{\nRNChesCoarseLTwo}{\tbd{nRNChesCoarseLTwo}}
\providecommand{\nRNChesNlcdREAL}{\tbd{nRNChesNlcdREAL}}
\providecommand{\nRNChesOmissionLOne}{\tbd{nRNChesOmissionLOne}}
\providecommand{\nRNChesOmissionLTwo}{\tbd{nRNChesOmissionLTwo}}
\providecommand{\nRNChesShiftLOne}{\tbd{nRNChesShiftLOne}}
\providecommand{\nRNChesShiftLTwo}{\tbd{nRNChesShiftLTwo}}
\providecommand{\nRNCsTwelveBoundaryLOne}{\tbd{nRNCsTwelveBoundaryLOne}}
\providecommand{\nRNCsTwelveBoundaryLTwo}{\tbd{nRNCsTwelveBoundaryLTwo}}
\providecommand{\nRNCsTwelveClean}{\tbd{nRNCsTwelveClean}}
\providecommand{\nRNCsTwelveCoarseLOne}{\tbd{nRNCsTwelveCoarseLOne}}
\providecommand{\nRNCsTwelveCoarseLTwo}{\tbd{nRNCsTwelveCoarseLTwo}}
\providecommand{\nRNCsTwelveOmissionLOne}{\tbd{nRNCsTwelveOmissionLOne}}
\providecommand{\nRNCsTwelveOmissionLTwo}{\tbd{nRNCsTwelveOmissionLTwo}}
\providecommand{\nRNCsTwelveSTwocloudlessREAL}{\tbd{nRNCsTwelveSTwocloudlessREAL}}
\providecommand{\nRNCsTwelveShiftLOne}{\tbd{nRNCsTwelveShiftLOne}}
\providecommand{\nRNCsTwelveShiftLTwo}{\tbd{nRNCsTwelveShiftLTwo}}
\providecommand{\nRNDfcBoundaryLOne}{\tbd{nRNDfcBoundaryLOne}}
\providecommand{\nRNDfcBoundaryLTwo}{\tbd{nRNDfcBoundaryLTwo}}
\providecommand{\nRNDfcClean}{\tbd{nRNDfcClean}}
\providecommand{\nRNDfcCleanVarTrainSubsetRealcov}{\tbd{nRNDfcCleanVarTrainSubsetRealcov}}
\providecommand{\nRNDfcCoarseLOne}{\tbd{nRNDfcCoarseLOne}}
\providecommand{\nRNDfcCoarseLTwo}{\tbd{nRNDfcCoarseLTwo}}
\providecommand{\nRNDfcModisREALVarTrainSubsetRealcov}{\tbd{nRNDfcModisREALVarTrainSubsetRealcov}}
\providecommand{\nRNDfcOmissionLOne}{\tbd{nRNDfcOmissionLOne}}
\providecommand{\nRNDfcOmissionLTwo}{\tbd{nRNDfcOmissionLTwo}}
\providecommand{\nRNDfcShiftLOne}{\tbd{nRNDfcShiftLOne}}
\providecommand{\nRNDfcShiftLTwo}{\tbd{nRNDfcShiftLTwo}}
\providecommand{\nRNEnvaBoundaryLOne}{\tbd{nRNEnvaBoundaryLOne}}
\providecommand{\nRNEnvaBoundaryLTwo}{\tbd{nRNEnvaBoundaryLTwo}}
\providecommand{\nRNEnvaClean}{\tbd{nRNEnvaClean}}
\providecommand{\nRNEnvaCoarseLOne}{\tbd{nRNEnvaCoarseLOne}}
\providecommand{\nRNEnvaCoarseLTwo}{\tbd{nRNEnvaCoarseLTwo}}
\providecommand{\nRNEnvaNlcdREAL}{\tbd{nRNEnvaNlcdREAL}}
\providecommand{\nRNEnvaOmissionLOne}{\tbd{nRNEnvaOmissionLOne}}
\providecommand{\nRNEnvaOmissionLTwo}{\tbd{nRNEnvaOmissionLTwo}}
\providecommand{\nRNEnvaShiftLOne}{\tbd{nRNEnvaShiftLOne}}
\providecommand{\nRNEnvaShiftLTwo}{\tbd{nRNEnvaShiftLTwo}}
\providecommand{\nRNKuroBoundaryLOne}{\tbd{nRNKuroBoundaryLOne}}
\providecommand{\nRNKuroBoundaryLTwo}{\tbd{nRNKuroBoundaryLTwo}}
\providecommand{\nRNKuroCemsREALVarTrainSubsetRealcov}{\tbd{nRNKuroCemsREALVarTrainSubsetRealcov}}
\providecommand{\nRNKuroClean}{\tbd{nRNKuroClean}}
\providecommand{\nRNKuroCleanVarTrainSubsetRealcov}{\tbd{nRNKuroCleanVarTrainSubsetRealcov}}
\providecommand{\nRNKuroCoarseLOne}{\tbd{nRNKuroCoarseLOne}}
\providecommand{\nRNKuroCoarseLTwo}{\tbd{nRNKuroCoarseLTwo}}
\providecommand{\nRNKuroOmissionLOne}{\tbd{nRNKuroOmissionLOne}}
\providecommand{\nRNKuroOmissionLTwo}{\tbd{nRNKuroOmissionLTwo}}
\providecommand{\nRNKuroShiftLOne}{\tbd{nRNKuroShiftLOne}}
\providecommand{\nRNKuroShiftLTwo}{\tbd{nRNKuroShiftLTwo}}
\providecommand{\nRNOemBoundaryLOne}{\tbd{nRNOemBoundaryLOne}}
\providecommand{\nRNOemBoundaryLTwo}{\tbd{nRNOemBoundaryLTwo}}
\providecommand{\nRNOemClean}{\tbd{nRNOemClean}}
\providecommand{\nRNOemCoarseLOne}{\tbd{nRNOemCoarseLOne}}
\providecommand{\nRNOemCoarseLTwo}{\tbd{nRNOemCoarseLTwo}}
\providecommand{\nRNOemOmissionLOne}{\tbd{nRNOemOmissionLOne}}
\providecommand{\nRNOemOmissionLTwo}{\tbd{nRNOemOmissionLTwo}}
\providecommand{\nRNOemShiftLOne}{\tbd{nRNOemShiftLOne}}
\providecommand{\nRNOemShiftLTwo}{\tbd{nRNOemShiftLTwo}}
\providecommand{\nRNSnTwoBoundaryLOne}{\tbd{nRNSnTwoBoundaryLOne}}
\providecommand{\nRNSnTwoBoundaryLTwo}{\tbd{nRNSnTwoBoundaryLTwo}}
\providecommand{\nRNSnTwoClean}{\tbd{nRNSnTwoClean}}
\providecommand{\nRNSnTwoCoarseLOne}{\tbd{nRNSnTwoCoarseLOne}}
\providecommand{\nRNSnTwoCoarseLTwo}{\tbd{nRNSnTwoCoarseLTwo}}
\providecommand{\nRNSnTwoOmissionLOne}{\tbd{nRNSnTwoOmissionLOne}}
\providecommand{\nRNSnTwoOmissionLTwo}{\tbd{nRNSnTwoOmissionLTwo}}
\providecommand{\nRNSnTwoShiftLOne}{\tbd{nRNSnTwoShiftLOne}}
\providecommand{\nRNSnTwoShiftLTwo}{\tbd{nRNSnTwoShiftLTwo}}
\providecommand{\nRNburnBoundaryLOne}{\tbd{nRNburnBoundaryLOne}}
\providecommand{\nRNburnBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{nRNburnBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nRNburnBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{nRNburnBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nRNburnBoundaryLOneVarDecoderSamLite}{\tbd{nRNburnBoundaryLOneVarDecoderSamLite}}
\providecommand{\nRNburnBoundaryLOneVarDecoderSamPretrained}{\tbd{nRNburnBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\nRNburnBoundaryLOneVarDecoderSegformerMlp}{\tbd{nRNburnBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\nRNburnBoundaryLR}{\tbd{nRNburnBoundaryLR}}
\providecommand{\nRNburnBoundaryLTwo}{\tbd{nRNburnBoundaryLTwo}}
\providecommand{\nRNburnBoundaryLTwoVarBandsRgb}{\tbd{nRNburnBoundaryLTwoVarBandsRgb}}
\providecommand{\nRNburnBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{nRNburnBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nRNburnBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{nRNburnBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nRNburnBoundaryLTwoVarDecoderSamLite}{\tbd{nRNburnBoundaryLTwoVarDecoderSamLite}}
\providecommand{\nRNburnBoundaryLTwoVarDecoderSamPretrained}{\tbd{nRNburnBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\nRNburnBoundaryLTwoVarDecoderSegformerMlp}{\tbd{nRNburnBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\nRNburnBoundaryLTwoVarInitRandom}{\tbd{nRNburnBoundaryLTwoVarInitRandom}}
\providecommand{\nRNburnBoundaryLTwoVarLossBootstrap}{\tbd{nRNburnBoundaryLTwoVarLossBootstrap}}
\providecommand{\nRNburnBoundaryLTwoVarLossGce}{\tbd{nRNburnBoundaryLTwoVarLossGce}}
\providecommand{\nRNburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nRNburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nRNburnBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{nRNburnBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nRNburnClean}{\tbd{nRNburnClean}}
\providecommand{\nRNburnCleanVarBandsRgb}{\tbd{nRNburnCleanVarBandsRgb}}
\providecommand{\nRNburnCleanVarDecoderMaskTwoformerFull}{\tbd{nRNburnCleanVarDecoderMaskTwoformerFull}}
\providecommand{\nRNburnCleanVarDecoderMaskTwoformerLite}{\tbd{nRNburnCleanVarDecoderMaskTwoformerLite}}
\providecommand{\nRNburnCleanVarDecoderSamLite}{\tbd{nRNburnCleanVarDecoderSamLite}}
\providecommand{\nRNburnCleanVarDecoderSamPretrained}{\tbd{nRNburnCleanVarDecoderSamPretrained}}
\providecommand{\nRNburnCleanVarDecoderSegformerMlp}{\tbd{nRNburnCleanVarDecoderSegformerMlp}}
\providecommand{\nRNburnCleanVarInitRandom}{\tbd{nRNburnCleanVarInitRandom}}
\providecommand{\nRNburnCleanVarInitRandomLrMultThree}{\tbd{nRNburnCleanVarInitRandomLrMultThree}}
\providecommand{\nRNburnCleanVarLossBootstrap}{\tbd{nRNburnCleanVarLossBootstrap}}
\providecommand{\nRNburnCleanVarLossGce}{\tbd{nRNburnCleanVarLossGce}}
\providecommand{\nRNburnCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{nRNburnCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nRNburnCleanVarTrainSubsetCleanTwoFive}{\tbd{nRNburnCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\nRNburnCoarseLOne}{\tbd{nRNburnCoarseLOne}}
\providecommand{\nRNburnCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{nRNburnCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nRNburnCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{nRNburnCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nRNburnCoarseLOneVarDecoderSamLite}{\tbd{nRNburnCoarseLOneVarDecoderSamLite}}
\providecommand{\nRNburnCoarseLOneVarDecoderSamPretrained}{\tbd{nRNburnCoarseLOneVarDecoderSamPretrained}}
\providecommand{\nRNburnCoarseLOneVarDecoderSegformerMlp}{\tbd{nRNburnCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\nRNburnCoarseLR}{\tbd{nRNburnCoarseLR}}
\providecommand{\nRNburnCoarseLTwo}{\tbd{nRNburnCoarseLTwo}}
\providecommand{\nRNburnCoarseLTwoVarBandsRgb}{\tbd{nRNburnCoarseLTwoVarBandsRgb}}
\providecommand{\nRNburnCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{nRNburnCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nRNburnCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{nRNburnCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nRNburnCoarseLTwoVarDecoderSamLite}{\tbd{nRNburnCoarseLTwoVarDecoderSamLite}}
\providecommand{\nRNburnCoarseLTwoVarDecoderSamPretrained}{\tbd{nRNburnCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\nRNburnCoarseLTwoVarDecoderSegformerMlp}{\tbd{nRNburnCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\nRNburnCoarseLTwoVarInitRandom}{\tbd{nRNburnCoarseLTwoVarInitRandom}}
\providecommand{\nRNburnCoarseLTwoVarLossBootstrap}{\tbd{nRNburnCoarseLTwoVarLossBootstrap}}
\providecommand{\nRNburnCoarseLTwoVarLossGce}{\tbd{nRNburnCoarseLTwoVarLossGce}}
\providecommand{\nRNburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nRNburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nRNburnCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{nRNburnCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nRNburnOmissionLOne}{\tbd{nRNburnOmissionLOne}}
\providecommand{\nRNburnOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{nRNburnOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nRNburnOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{nRNburnOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nRNburnOmissionLOneVarDecoderSamLite}{\tbd{nRNburnOmissionLOneVarDecoderSamLite}}
\providecommand{\nRNburnOmissionLOneVarDecoderSamPretrained}{\tbd{nRNburnOmissionLOneVarDecoderSamPretrained}}
\providecommand{\nRNburnOmissionLOneVarDecoderSegformerMlp}{\tbd{nRNburnOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\nRNburnOmissionLR}{\tbd{nRNburnOmissionLR}}
\providecommand{\nRNburnOmissionLTwo}{\tbd{nRNburnOmissionLTwo}}
\providecommand{\nRNburnOmissionLTwoVarBandsRgb}{\tbd{nRNburnOmissionLTwoVarBandsRgb}}
\providecommand{\nRNburnOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{nRNburnOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nRNburnOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{nRNburnOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nRNburnOmissionLTwoVarDecoderSamLite}{\tbd{nRNburnOmissionLTwoVarDecoderSamLite}}
\providecommand{\nRNburnOmissionLTwoVarDecoderSamPretrained}{\tbd{nRNburnOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\nRNburnOmissionLTwoVarDecoderSegformerMlp}{\tbd{nRNburnOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\nRNburnOmissionLTwoVarInitRandom}{\tbd{nRNburnOmissionLTwoVarInitRandom}}
\providecommand{\nRNburnOmissionLTwoVarLossBootstrap}{\tbd{nRNburnOmissionLTwoVarLossBootstrap}}
\providecommand{\nRNburnOmissionLTwoVarLossGce}{\tbd{nRNburnOmissionLTwoVarLossGce}}
\providecommand{\nRNburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nRNburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nRNburnOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{nRNburnOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nRNburnShiftLOne}{\tbd{nRNburnShiftLOne}}
\providecommand{\nRNburnShiftLOneVarDecoderMaskTwoformerFull}{\tbd{nRNburnShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nRNburnShiftLOneVarDecoderMaskTwoformerLite}{\tbd{nRNburnShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nRNburnShiftLOneVarDecoderSamLite}{\tbd{nRNburnShiftLOneVarDecoderSamLite}}
\providecommand{\nRNburnShiftLOneVarDecoderSamPretrained}{\tbd{nRNburnShiftLOneVarDecoderSamPretrained}}
\providecommand{\nRNburnShiftLOneVarDecoderSegformerMlp}{\tbd{nRNburnShiftLOneVarDecoderSegformerMlp}}
\providecommand{\nRNburnShiftLR}{\tbd{nRNburnShiftLR}}
\providecommand{\nRNburnShiftLTwo}{\tbd{nRNburnShiftLTwo}}
\providecommand{\nRNburnShiftLTwoVarBandsRgb}{\tbd{nRNburnShiftLTwoVarBandsRgb}}
\providecommand{\nRNburnShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{nRNburnShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nRNburnShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{nRNburnShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nRNburnShiftLTwoVarDecoderSamLite}{\tbd{nRNburnShiftLTwoVarDecoderSamLite}}
\providecommand{\nRNburnShiftLTwoVarDecoderSamPretrained}{\tbd{nRNburnShiftLTwoVarDecoderSamPretrained}}
\providecommand{\nRNburnShiftLTwoVarDecoderSegformerMlp}{\tbd{nRNburnShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\nRNburnShiftLTwoVarInitRandom}{\tbd{nRNburnShiftLTwoVarInitRandom}}
\providecommand{\nRNburnShiftLTwoVarLossBootstrap}{\tbd{nRNburnShiftLTwoVarLossBootstrap}}
\providecommand{\nRNburnShiftLTwoVarLossGce}{\tbd{nRNburnShiftLTwoVarLossGce}}
\providecommand{\nRNburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nRNburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nRNburnShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{nRNburnShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nRNflairBoundaryLOne}{\tbd{nRNflairBoundaryLOne}}
\providecommand{\nRNflairBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{nRNflairBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nRNflairBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{nRNflairBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nRNflairBoundaryLOneVarDecoderSamLite}{\tbd{nRNflairBoundaryLOneVarDecoderSamLite}}
\providecommand{\nRNflairBoundaryLOneVarDecoderSamPretrained}{\tbd{nRNflairBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\nRNflairBoundaryLOneVarDecoderSegformerMlp}{\tbd{nRNflairBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\nRNflairBoundaryLR}{\tbd{nRNflairBoundaryLR}}
\providecommand{\nRNflairBoundaryLTwo}{\tbd{nRNflairBoundaryLTwo}}
\providecommand{\nRNflairBoundaryLTwoVarBandsRgb}{\tbd{nRNflairBoundaryLTwoVarBandsRgb}}
\providecommand{\nRNflairBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{nRNflairBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nRNflairBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{nRNflairBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nRNflairBoundaryLTwoVarDecoderSamLite}{\tbd{nRNflairBoundaryLTwoVarDecoderSamLite}}
\providecommand{\nRNflairBoundaryLTwoVarDecoderSamPretrained}{\tbd{nRNflairBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\nRNflairBoundaryLTwoVarDecoderSegformerMlp}{\tbd{nRNflairBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\nRNflairBoundaryLTwoVarInitRandom}{\tbd{nRNflairBoundaryLTwoVarInitRandom}}
\providecommand{\nRNflairBoundaryLTwoVarLossBootstrap}{\tbd{nRNflairBoundaryLTwoVarLossBootstrap}}
\providecommand{\nRNflairBoundaryLTwoVarLossGce}{\tbd{nRNflairBoundaryLTwoVarLossGce}}
\providecommand{\nRNflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nRNflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nRNflairBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{nRNflairBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nRNflairClean}{\tbd{nRNflairClean}}
\providecommand{\nRNflairCleanVarBandsRgb}{\tbd{nRNflairCleanVarBandsRgb}}
\providecommand{\nRNflairCleanVarClassWeightedTrue}{\tbd{nRNflairCleanVarClassWeightedTrue}}
\providecommand{\nRNflairCleanVarDecoderMaskTwoformerFull}{\tbd{nRNflairCleanVarDecoderMaskTwoformerFull}}
\providecommand{\nRNflairCleanVarDecoderMaskTwoformerLite}{\tbd{nRNflairCleanVarDecoderMaskTwoformerLite}}
\providecommand{\nRNflairCleanVarDecoderSamLite}{\tbd{nRNflairCleanVarDecoderSamLite}}
\providecommand{\nRNflairCleanVarDecoderSamPretrained}{\tbd{nRNflairCleanVarDecoderSamPretrained}}
\providecommand{\nRNflairCleanVarDecoderSegformerMlp}{\tbd{nRNflairCleanVarDecoderSegformerMlp}}
\providecommand{\nRNflairCleanVarInitRandom}{\tbd{nRNflairCleanVarInitRandom}}
\providecommand{\nRNflairCleanVarInitRandomLrMultThree}{\tbd{nRNflairCleanVarInitRandomLrMultThree}}
\providecommand{\nRNflairCleanVarLossBootstrap}{\tbd{nRNflairCleanVarLossBootstrap}}
\providecommand{\nRNflairCleanVarLossGce}{\tbd{nRNflairCleanVarLossGce}}
\providecommand{\nRNflairCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{nRNflairCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nRNflairCleanVarTrainSubsetCleanTwoFive}{\tbd{nRNflairCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\nRNflairCoarseLOne}{\tbd{nRNflairCoarseLOne}}
\providecommand{\nRNflairCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{nRNflairCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nRNflairCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{nRNflairCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nRNflairCoarseLOneVarDecoderSamLite}{\tbd{nRNflairCoarseLOneVarDecoderSamLite}}
\providecommand{\nRNflairCoarseLOneVarDecoderSamPretrained}{\tbd{nRNflairCoarseLOneVarDecoderSamPretrained}}
\providecommand{\nRNflairCoarseLOneVarDecoderSegformerMlp}{\tbd{nRNflairCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\nRNflairCoarseLR}{\tbd{nRNflairCoarseLR}}
\providecommand{\nRNflairCoarseLTwo}{\tbd{nRNflairCoarseLTwo}}
\providecommand{\nRNflairCoarseLTwoVarBandsRgb}{\tbd{nRNflairCoarseLTwoVarBandsRgb}}
\providecommand{\nRNflairCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{nRNflairCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nRNflairCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{nRNflairCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nRNflairCoarseLTwoVarDecoderSamLite}{\tbd{nRNflairCoarseLTwoVarDecoderSamLite}}
\providecommand{\nRNflairCoarseLTwoVarDecoderSamPretrained}{\tbd{nRNflairCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\nRNflairCoarseLTwoVarDecoderSegformerMlp}{\tbd{nRNflairCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\nRNflairCoarseLTwoVarInitRandom}{\tbd{nRNflairCoarseLTwoVarInitRandom}}
\providecommand{\nRNflairCoarseLTwoVarLossBootstrap}{\tbd{nRNflairCoarseLTwoVarLossBootstrap}}
\providecommand{\nRNflairCoarseLTwoVarLossGce}{\tbd{nRNflairCoarseLTwoVarLossGce}}
\providecommand{\nRNflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nRNflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nRNflairCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{nRNflairCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nRNflairOmissionLOne}{\tbd{nRNflairOmissionLOne}}
\providecommand{\nRNflairOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{nRNflairOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nRNflairOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{nRNflairOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nRNflairOmissionLOneVarDecoderSamLite}{\tbd{nRNflairOmissionLOneVarDecoderSamLite}}
\providecommand{\nRNflairOmissionLOneVarDecoderSamPretrained}{\tbd{nRNflairOmissionLOneVarDecoderSamPretrained}}
\providecommand{\nRNflairOmissionLOneVarDecoderSegformerMlp}{\tbd{nRNflairOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\nRNflairOmissionLR}{\tbd{nRNflairOmissionLR}}
\providecommand{\nRNflairOmissionLTwo}{\tbd{nRNflairOmissionLTwo}}
\providecommand{\nRNflairOmissionLTwoVarBandsRgb}{\tbd{nRNflairOmissionLTwoVarBandsRgb}}
\providecommand{\nRNflairOmissionLTwoVarClassWeightedTrue}{\tbd{nRNflairOmissionLTwoVarClassWeightedTrue}}
\providecommand{\nRNflairOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{nRNflairOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nRNflairOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{nRNflairOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nRNflairOmissionLTwoVarDecoderSamLite}{\tbd{nRNflairOmissionLTwoVarDecoderSamLite}}
\providecommand{\nRNflairOmissionLTwoVarDecoderSamPretrained}{\tbd{nRNflairOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\nRNflairOmissionLTwoVarDecoderSegformerMlp}{\tbd{nRNflairOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\nRNflairOmissionLTwoVarInitRandom}{\tbd{nRNflairOmissionLTwoVarInitRandom}}
\providecommand{\nRNflairOmissionLTwoVarLossBootstrap}{\tbd{nRNflairOmissionLTwoVarLossBootstrap}}
\providecommand{\nRNflairOmissionLTwoVarLossGce}{\tbd{nRNflairOmissionLTwoVarLossGce}}
\providecommand{\nRNflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nRNflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nRNflairOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{nRNflairOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nRNflairShiftLOne}{\tbd{nRNflairShiftLOne}}
\providecommand{\nRNflairShiftLOneVarDecoderMaskTwoformerFull}{\tbd{nRNflairShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nRNflairShiftLOneVarDecoderMaskTwoformerLite}{\tbd{nRNflairShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nRNflairShiftLOneVarDecoderSamLite}{\tbd{nRNflairShiftLOneVarDecoderSamLite}}
\providecommand{\nRNflairShiftLOneVarDecoderSamPretrained}{\tbd{nRNflairShiftLOneVarDecoderSamPretrained}}
\providecommand{\nRNflairShiftLOneVarDecoderSegformerMlp}{\tbd{nRNflairShiftLOneVarDecoderSegformerMlp}}
\providecommand{\nRNflairShiftLR}{\tbd{nRNflairShiftLR}}
\providecommand{\nRNflairShiftLTwo}{\tbd{nRNflairShiftLTwo}}
\providecommand{\nRNflairShiftLTwoVarBandsRgb}{\tbd{nRNflairShiftLTwoVarBandsRgb}}
\providecommand{\nRNflairShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{nRNflairShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nRNflairShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{nRNflairShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nRNflairShiftLTwoVarDecoderSamLite}{\tbd{nRNflairShiftLTwoVarDecoderSamLite}}
\providecommand{\nRNflairShiftLTwoVarDecoderSamPretrained}{\tbd{nRNflairShiftLTwoVarDecoderSamPretrained}}
\providecommand{\nRNflairShiftLTwoVarDecoderSegformerMlp}{\tbd{nRNflairShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\nRNflairShiftLTwoVarInitRandom}{\tbd{nRNflairShiftLTwoVarInitRandom}}
\providecommand{\nRNflairShiftLTwoVarLossBootstrap}{\tbd{nRNflairShiftLTwoVarLossBootstrap}}
\providecommand{\nRNflairShiftLTwoVarLossGce}{\tbd{nRNflairShiftLTwoVarLossGce}}
\providecommand{\nRNflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nRNflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nRNflairShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{nRNflairShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nRNsenClean}{\tbd{nRNsenClean}}
\providecommand{\nRNsenOtsuLTwo}{\tbd{nRNsenOtsuLTwo}}
\providecommand{\nResnetFiveZeroSslFoureoburnBoundaryLOne}{\tbd{nResnetFiveZeroSslFoureoburnBoundaryLOne}}
\providecommand{\nResnetFiveZeroSslFoureoburnBoundaryLTwo}{\tbd{nResnetFiveZeroSslFoureoburnBoundaryLTwo}}
\providecommand{\nResnetFiveZeroSslFoureoburnClean}{\tbd{nResnetFiveZeroSslFoureoburnClean}}
\providecommand{\nResnetFiveZeroSslFoureoburnCleanVarTrainSubsetCleanTwoFive}{\tbd{nResnetFiveZeroSslFoureoburnCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\nResnetFiveZeroSslFoureoburnCoarseLOne}{\tbd{nResnetFiveZeroSslFoureoburnCoarseLOne}}
\providecommand{\nResnetFiveZeroSslFoureoburnCoarseLTwo}{\tbd{nResnetFiveZeroSslFoureoburnCoarseLTwo}}
\providecommand{\nResnetFiveZeroSslFoureoburnOmissionLOne}{\tbd{nResnetFiveZeroSslFoureoburnOmissionLOne}}
\providecommand{\nResnetFiveZeroSslFoureoburnOmissionLTwo}{\tbd{nResnetFiveZeroSslFoureoburnOmissionLTwo}}
\providecommand{\nResnetFiveZeroSslFoureoburnShiftLOne}{\tbd{nResnetFiveZeroSslFoureoburnShiftLOne}}
\providecommand{\nResnetFiveZeroSslFoureoburnShiftLTwo}{\tbd{nResnetFiveZeroSslFoureoburnShiftLTwo}}
\providecommand{\nResnetFiveZeroSslFoureoflairBoundaryLOne}{\tbd{nResnetFiveZeroSslFoureoflairBoundaryLOne}}
\providecommand{\nResnetFiveZeroSslFoureoflairBoundaryLTwo}{\tbd{nResnetFiveZeroSslFoureoflairBoundaryLTwo}}
\providecommand{\nResnetFiveZeroSslFoureoflairClean}{\tbd{nResnetFiveZeroSslFoureoflairClean}}
\providecommand{\nResnetFiveZeroSslFoureoflairCleanVarTrainSubsetCleanTwoFive}{\tbd{nResnetFiveZeroSslFoureoflairCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\nResnetFiveZeroSslFoureoflairCoarseLOne}{\tbd{nResnetFiveZeroSslFoureoflairCoarseLOne}}
\providecommand{\nResnetFiveZeroSslFoureoflairCoarseLTwo}{\tbd{nResnetFiveZeroSslFoureoflairCoarseLTwo}}
\providecommand{\nResnetFiveZeroSslFoureoflairOmissionLOne}{\tbd{nResnetFiveZeroSslFoureoflairOmissionLOne}}
\providecommand{\nResnetFiveZeroSslFoureoflairOmissionLTwo}{\tbd{nResnetFiveZeroSslFoureoflairOmissionLTwo}}
\providecommand{\nResnetFiveZeroSslFoureoflairShiftLOne}{\tbd{nResnetFiveZeroSslFoureoflairShiftLOne}}
\providecommand{\nResnetFiveZeroSslFoureoflairShiftLTwo}{\tbd{nResnetFiveZeroSslFoureoflairShiftLTwo}}
\providecommand{\nSATChesBoundaryLOne}{\tbd{nSATChesBoundaryLOne}}
\providecommand{\nSATChesBoundaryLTwo}{\tbd{nSATChesBoundaryLTwo}}
\providecommand{\nSATChesBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{nSATChesBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nSATChesBoundaryLTwoVarDecoderSamLite}{\tbd{nSATChesBoundaryLTwoVarDecoderSamLite}}
\providecommand{\nSATChesBoundaryLTwoVarDecoderSegformerMlp}{\tbd{nSATChesBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\nSATChesBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATChesBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATChesClean}{\tbd{nSATChesClean}}
\providecommand{\nSATChesCleanVarDecoderMaskTwoformerLite}{\tbd{nSATChesCleanVarDecoderMaskTwoformerLite}}
\providecommand{\nSATChesCleanVarDecoderSamLite}{\tbd{nSATChesCleanVarDecoderSamLite}}
\providecommand{\nSATChesCleanVarDecoderSegformerMlp}{\tbd{nSATChesCleanVarDecoderSegformerMlp}}
\providecommand{\nSATChesCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATChesCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATChesCoarseLOne}{\tbd{nSATChesCoarseLOne}}
\providecommand{\nSATChesCoarseLTwo}{\tbd{nSATChesCoarseLTwo}}
\providecommand{\nSATChesCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{nSATChesCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nSATChesCoarseLTwoVarDecoderSamLite}{\tbd{nSATChesCoarseLTwoVarDecoderSamLite}}
\providecommand{\nSATChesCoarseLTwoVarDecoderSegformerMlp}{\tbd{nSATChesCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\nSATChesCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATChesCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATChesNlcdREAL}{\tbd{nSATChesNlcdREAL}}
\providecommand{\nSATChesOmissionLOne}{\tbd{nSATChesOmissionLOne}}
\providecommand{\nSATChesOmissionLTwo}{\tbd{nSATChesOmissionLTwo}}
\providecommand{\nSATChesOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{nSATChesOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nSATChesOmissionLTwoVarDecoderSamLite}{\tbd{nSATChesOmissionLTwoVarDecoderSamLite}}
\providecommand{\nSATChesOmissionLTwoVarDecoderSegformerMlp}{\tbd{nSATChesOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\nSATChesOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATChesOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATChesShiftLOne}{\tbd{nSATChesShiftLOne}}
\providecommand{\nSATChesShiftLTwo}{\tbd{nSATChesShiftLTwo}}
\providecommand{\nSATChesShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{nSATChesShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nSATChesShiftLTwoVarDecoderSamLite}{\tbd{nSATChesShiftLTwoVarDecoderSamLite}}
\providecommand{\nSATChesShiftLTwoVarDecoderSegformerMlp}{\tbd{nSATChesShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\nSATChesShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATChesShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATCsTwelveBoundaryLOne}{\tbd{nSATCsTwelveBoundaryLOne}}
\providecommand{\nSATCsTwelveBoundaryLTwo}{\tbd{nSATCsTwelveBoundaryLTwo}}
\providecommand{\nSATCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{nSATCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nSATCsTwelveBoundaryLTwoVarDecoderSamLite}{\tbd{nSATCsTwelveBoundaryLTwoVarDecoderSamLite}}
\providecommand{\nSATCsTwelveBoundaryLTwoVarDecoderSegformerMlp}{\tbd{nSATCsTwelveBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\nSATCsTwelveBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATCsTwelveBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATCsTwelveClean}{\tbd{nSATCsTwelveClean}}
\providecommand{\nSATCsTwelveCleanVarDecoderMaskTwoformerLite}{\tbd{nSATCsTwelveCleanVarDecoderMaskTwoformerLite}}
\providecommand{\nSATCsTwelveCleanVarDecoderSamLite}{\tbd{nSATCsTwelveCleanVarDecoderSamLite}}
\providecommand{\nSATCsTwelveCleanVarDecoderSegformerMlp}{\tbd{nSATCsTwelveCleanVarDecoderSegformerMlp}}
\providecommand{\nSATCsTwelveCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATCsTwelveCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATCsTwelveCoarseLOne}{\tbd{nSATCsTwelveCoarseLOne}}
\providecommand{\nSATCsTwelveCoarseLTwo}{\tbd{nSATCsTwelveCoarseLTwo}}
\providecommand{\nSATCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{nSATCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nSATCsTwelveCoarseLTwoVarDecoderSamLite}{\tbd{nSATCsTwelveCoarseLTwoVarDecoderSamLite}}
\providecommand{\nSATCsTwelveCoarseLTwoVarDecoderSegformerMlp}{\tbd{nSATCsTwelveCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\nSATCsTwelveCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATCsTwelveCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATCsTwelveOmissionLOne}{\tbd{nSATCsTwelveOmissionLOne}}
\providecommand{\nSATCsTwelveOmissionLTwo}{\tbd{nSATCsTwelveOmissionLTwo}}
\providecommand{\nSATCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{nSATCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nSATCsTwelveOmissionLTwoVarDecoderSamLite}{\tbd{nSATCsTwelveOmissionLTwoVarDecoderSamLite}}
\providecommand{\nSATCsTwelveOmissionLTwoVarDecoderSegformerMlp}{\tbd{nSATCsTwelveOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\nSATCsTwelveOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATCsTwelveOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATCsTwelveSTwocloudlessREAL}{\tbd{nSATCsTwelveSTwocloudlessREAL}}
\providecommand{\nSATCsTwelveShiftLOne}{\tbd{nSATCsTwelveShiftLOne}}
\providecommand{\nSATCsTwelveShiftLTwo}{\tbd{nSATCsTwelveShiftLTwo}}
\providecommand{\nSATCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{nSATCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nSATCsTwelveShiftLTwoVarDecoderSamLite}{\tbd{nSATCsTwelveShiftLTwoVarDecoderSamLite}}
\providecommand{\nSATCsTwelveShiftLTwoVarDecoderSegformerMlp}{\tbd{nSATCsTwelveShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\nSATCsTwelveShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATCsTwelveShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATDfcBoundaryLOne}{\tbd{nSATDfcBoundaryLOne}}
\providecommand{\nSATDfcBoundaryLTwo}{\tbd{nSATDfcBoundaryLTwo}}
\providecommand{\nSATDfcBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{nSATDfcBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nSATDfcBoundaryLTwoVarDecoderSamLite}{\tbd{nSATDfcBoundaryLTwoVarDecoderSamLite}}
\providecommand{\nSATDfcBoundaryLTwoVarDecoderSegformerMlp}{\tbd{nSATDfcBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\nSATDfcBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATDfcBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATDfcClean}{\tbd{nSATDfcClean}}
\providecommand{\nSATDfcCleanVarDecoderMaskTwoformerLite}{\tbd{nSATDfcCleanVarDecoderMaskTwoformerLite}}
\providecommand{\nSATDfcCleanVarDecoderSamLite}{\tbd{nSATDfcCleanVarDecoderSamLite}}
\providecommand{\nSATDfcCleanVarDecoderSegformerMlp}{\tbd{nSATDfcCleanVarDecoderSegformerMlp}}
\providecommand{\nSATDfcCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATDfcCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATDfcCleanVarTrainSubsetRealcov}{\tbd{nSATDfcCleanVarTrainSubsetRealcov}}
\providecommand{\nSATDfcCoarseLOne}{\tbd{nSATDfcCoarseLOne}}
\providecommand{\nSATDfcCoarseLTwo}{\tbd{nSATDfcCoarseLTwo}}
\providecommand{\nSATDfcCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{nSATDfcCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nSATDfcCoarseLTwoVarDecoderSamLite}{\tbd{nSATDfcCoarseLTwoVarDecoderSamLite}}
\providecommand{\nSATDfcCoarseLTwoVarDecoderSegformerMlp}{\tbd{nSATDfcCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\nSATDfcCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATDfcCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATDfcModisREALVarTrainSubsetRealcov}{\tbd{nSATDfcModisREALVarTrainSubsetRealcov}}
\providecommand{\nSATDfcOmissionLOne}{\tbd{nSATDfcOmissionLOne}}
\providecommand{\nSATDfcOmissionLTwo}{\tbd{nSATDfcOmissionLTwo}}
\providecommand{\nSATDfcOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{nSATDfcOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nSATDfcOmissionLTwoVarDecoderSamLite}{\tbd{nSATDfcOmissionLTwoVarDecoderSamLite}}
\providecommand{\nSATDfcOmissionLTwoVarDecoderSegformerMlp}{\tbd{nSATDfcOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\nSATDfcOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATDfcOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATDfcShiftLOne}{\tbd{nSATDfcShiftLOne}}
\providecommand{\nSATDfcShiftLTwo}{\tbd{nSATDfcShiftLTwo}}
\providecommand{\nSATDfcShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{nSATDfcShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nSATDfcShiftLTwoVarDecoderSamLite}{\tbd{nSATDfcShiftLTwoVarDecoderSamLite}}
\providecommand{\nSATDfcShiftLTwoVarDecoderSegformerMlp}{\tbd{nSATDfcShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\nSATDfcShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATDfcShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATEnvaBoundaryLOne}{\tbd{nSATEnvaBoundaryLOne}}
\providecommand{\nSATEnvaBoundaryLTwo}{\tbd{nSATEnvaBoundaryLTwo}}
\providecommand{\nSATEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{nSATEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nSATEnvaBoundaryLTwoVarDecoderSamLite}{\tbd{nSATEnvaBoundaryLTwoVarDecoderSamLite}}
\providecommand{\nSATEnvaBoundaryLTwoVarDecoderSegformerMlp}{\tbd{nSATEnvaBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\nSATEnvaBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATEnvaBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATEnvaClean}{\tbd{nSATEnvaClean}}
\providecommand{\nSATEnvaCleanVarDecoderMaskTwoformerLite}{\tbd{nSATEnvaCleanVarDecoderMaskTwoformerLite}}
\providecommand{\nSATEnvaCleanVarDecoderSamLite}{\tbd{nSATEnvaCleanVarDecoderSamLite}}
\providecommand{\nSATEnvaCleanVarDecoderSegformerMlp}{\tbd{nSATEnvaCleanVarDecoderSegformerMlp}}
\providecommand{\nSATEnvaCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATEnvaCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATEnvaCoarseLOne}{\tbd{nSATEnvaCoarseLOne}}
\providecommand{\nSATEnvaCoarseLTwo}{\tbd{nSATEnvaCoarseLTwo}}
\providecommand{\nSATEnvaCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{nSATEnvaCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nSATEnvaCoarseLTwoVarDecoderSamLite}{\tbd{nSATEnvaCoarseLTwoVarDecoderSamLite}}
\providecommand{\nSATEnvaCoarseLTwoVarDecoderSegformerMlp}{\tbd{nSATEnvaCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\nSATEnvaCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATEnvaCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATEnvaNlcdREAL}{\tbd{nSATEnvaNlcdREAL}}
\providecommand{\nSATEnvaOmissionLOne}{\tbd{nSATEnvaOmissionLOne}}
\providecommand{\nSATEnvaOmissionLTwo}{\tbd{nSATEnvaOmissionLTwo}}
\providecommand{\nSATEnvaOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{nSATEnvaOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nSATEnvaOmissionLTwoVarDecoderSamLite}{\tbd{nSATEnvaOmissionLTwoVarDecoderSamLite}}
\providecommand{\nSATEnvaOmissionLTwoVarDecoderSegformerMlp}{\tbd{nSATEnvaOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\nSATEnvaOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATEnvaOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATEnvaShiftLOne}{\tbd{nSATEnvaShiftLOne}}
\providecommand{\nSATEnvaShiftLTwo}{\tbd{nSATEnvaShiftLTwo}}
\providecommand{\nSATEnvaShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{nSATEnvaShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nSATEnvaShiftLTwoVarDecoderSamLite}{\tbd{nSATEnvaShiftLTwoVarDecoderSamLite}}
\providecommand{\nSATEnvaShiftLTwoVarDecoderSegformerMlp}{\tbd{nSATEnvaShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\nSATEnvaShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATEnvaShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATKuroBoundaryLOne}{\tbd{nSATKuroBoundaryLOne}}
\providecommand{\nSATKuroBoundaryLTwo}{\tbd{nSATKuroBoundaryLTwo}}
\providecommand{\nSATKuroBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{nSATKuroBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nSATKuroBoundaryLTwoVarDecoderSamLite}{\tbd{nSATKuroBoundaryLTwoVarDecoderSamLite}}
\providecommand{\nSATKuroBoundaryLTwoVarDecoderSegformerMlp}{\tbd{nSATKuroBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\nSATKuroBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATKuroBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATKuroCemsREALVarTrainSubsetRealcov}{\tbd{nSATKuroCemsREALVarTrainSubsetRealcov}}
\providecommand{\nSATKuroClean}{\tbd{nSATKuroClean}}
\providecommand{\nSATKuroCleanVarDecoderMaskTwoformerLite}{\tbd{nSATKuroCleanVarDecoderMaskTwoformerLite}}
\providecommand{\nSATKuroCleanVarDecoderSamLite}{\tbd{nSATKuroCleanVarDecoderSamLite}}
\providecommand{\nSATKuroCleanVarDecoderSegformerMlp}{\tbd{nSATKuroCleanVarDecoderSegformerMlp}}
\providecommand{\nSATKuroCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATKuroCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATKuroCleanVarTrainSubsetRealcov}{\tbd{nSATKuroCleanVarTrainSubsetRealcov}}
\providecommand{\nSATKuroCoarseLOne}{\tbd{nSATKuroCoarseLOne}}
\providecommand{\nSATKuroCoarseLTwo}{\tbd{nSATKuroCoarseLTwo}}
\providecommand{\nSATKuroCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{nSATKuroCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nSATKuroCoarseLTwoVarDecoderSamLite}{\tbd{nSATKuroCoarseLTwoVarDecoderSamLite}}
\providecommand{\nSATKuroCoarseLTwoVarDecoderSegformerMlp}{\tbd{nSATKuroCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\nSATKuroCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATKuroCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATKuroOmissionLOne}{\tbd{nSATKuroOmissionLOne}}
\providecommand{\nSATKuroOmissionLTwo}{\tbd{nSATKuroOmissionLTwo}}
\providecommand{\nSATKuroOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{nSATKuroOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nSATKuroOmissionLTwoVarDecoderSamLite}{\tbd{nSATKuroOmissionLTwoVarDecoderSamLite}}
\providecommand{\nSATKuroOmissionLTwoVarDecoderSegformerMlp}{\tbd{nSATKuroOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\nSATKuroOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATKuroOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATKuroShiftLOne}{\tbd{nSATKuroShiftLOne}}
\providecommand{\nSATKuroShiftLTwo}{\tbd{nSATKuroShiftLTwo}}
\providecommand{\nSATKuroShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{nSATKuroShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nSATKuroShiftLTwoVarDecoderSamLite}{\tbd{nSATKuroShiftLTwoVarDecoderSamLite}}
\providecommand{\nSATKuroShiftLTwoVarDecoderSegformerMlp}{\tbd{nSATKuroShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\nSATKuroShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATKuroShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATOemBoundaryLOne}{\tbd{nSATOemBoundaryLOne}}
\providecommand{\nSATOemBoundaryLTwo}{\tbd{nSATOemBoundaryLTwo}}
\providecommand{\nSATOemBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{nSATOemBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nSATOemBoundaryLTwoVarDecoderSamLite}{\tbd{nSATOemBoundaryLTwoVarDecoderSamLite}}
\providecommand{\nSATOemBoundaryLTwoVarDecoderSegformerMlp}{\tbd{nSATOemBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\nSATOemBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATOemBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATOemClean}{\tbd{nSATOemClean}}
\providecommand{\nSATOemCleanVarDecoderMaskTwoformerLite}{\tbd{nSATOemCleanVarDecoderMaskTwoformerLite}}
\providecommand{\nSATOemCleanVarDecoderSamLite}{\tbd{nSATOemCleanVarDecoderSamLite}}
\providecommand{\nSATOemCleanVarDecoderSegformerMlp}{\tbd{nSATOemCleanVarDecoderSegformerMlp}}
\providecommand{\nSATOemCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATOemCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATOemCoarseLOne}{\tbd{nSATOemCoarseLOne}}
\providecommand{\nSATOemCoarseLTwo}{\tbd{nSATOemCoarseLTwo}}
\providecommand{\nSATOemCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{nSATOemCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nSATOemCoarseLTwoVarDecoderSamLite}{\tbd{nSATOemCoarseLTwoVarDecoderSamLite}}
\providecommand{\nSATOemCoarseLTwoVarDecoderSegformerMlp}{\tbd{nSATOemCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\nSATOemCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATOemCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATOemOmissionLOne}{\tbd{nSATOemOmissionLOne}}
\providecommand{\nSATOemOmissionLTwo}{\tbd{nSATOemOmissionLTwo}}
\providecommand{\nSATOemOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{nSATOemOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nSATOemOmissionLTwoVarDecoderSamLite}{\tbd{nSATOemOmissionLTwoVarDecoderSamLite}}
\providecommand{\nSATOemOmissionLTwoVarDecoderSegformerMlp}{\tbd{nSATOemOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\nSATOemOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATOemOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATOemShiftLOne}{\tbd{nSATOemShiftLOne}}
\providecommand{\nSATOemShiftLTwo}{\tbd{nSATOemShiftLTwo}}
\providecommand{\nSATOemShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{nSATOemShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nSATOemShiftLTwoVarDecoderSamLite}{\tbd{nSATOemShiftLTwoVarDecoderSamLite}}
\providecommand{\nSATOemShiftLTwoVarDecoderSegformerMlp}{\tbd{nSATOemShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\nSATOemShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATOemShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATSnTwoBoundaryLOne}{\tbd{nSATSnTwoBoundaryLOne}}
\providecommand{\nSATSnTwoBoundaryLTwo}{\tbd{nSATSnTwoBoundaryLTwo}}
\providecommand{\nSATSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{nSATSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nSATSnTwoBoundaryLTwoVarDecoderSamLite}{\tbd{nSATSnTwoBoundaryLTwoVarDecoderSamLite}}
\providecommand{\nSATSnTwoBoundaryLTwoVarDecoderSegformerMlp}{\tbd{nSATSnTwoBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\nSATSnTwoBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATSnTwoBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATSnTwoClean}{\tbd{nSATSnTwoClean}}
\providecommand{\nSATSnTwoCleanVarDecoderMaskTwoformerLite}{\tbd{nSATSnTwoCleanVarDecoderMaskTwoformerLite}}
\providecommand{\nSATSnTwoCleanVarDecoderSamLite}{\tbd{nSATSnTwoCleanVarDecoderSamLite}}
\providecommand{\nSATSnTwoCleanVarDecoderSegformerMlp}{\tbd{nSATSnTwoCleanVarDecoderSegformerMlp}}
\providecommand{\nSATSnTwoCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATSnTwoCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATSnTwoCoarseLOne}{\tbd{nSATSnTwoCoarseLOne}}
\providecommand{\nSATSnTwoCoarseLTwo}{\tbd{nSATSnTwoCoarseLTwo}}
\providecommand{\nSATSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{nSATSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nSATSnTwoCoarseLTwoVarDecoderSamLite}{\tbd{nSATSnTwoCoarseLTwoVarDecoderSamLite}}
\providecommand{\nSATSnTwoCoarseLTwoVarDecoderSegformerMlp}{\tbd{nSATSnTwoCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\nSATSnTwoCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATSnTwoCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATSnTwoOmissionLOne}{\tbd{nSATSnTwoOmissionLOne}}
\providecommand{\nSATSnTwoOmissionLTwo}{\tbd{nSATSnTwoOmissionLTwo}}
\providecommand{\nSATSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{nSATSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nSATSnTwoOmissionLTwoVarDecoderSamLite}{\tbd{nSATSnTwoOmissionLTwoVarDecoderSamLite}}
\providecommand{\nSATSnTwoOmissionLTwoVarDecoderSegformerMlp}{\tbd{nSATSnTwoOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\nSATSnTwoOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATSnTwoOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATSnTwoShiftLOne}{\tbd{nSATSnTwoShiftLOne}}
\providecommand{\nSATSnTwoShiftLTwo}{\tbd{nSATSnTwoShiftLTwo}}
\providecommand{\nSATSnTwoShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{nSATSnTwoShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nSATSnTwoShiftLTwoVarDecoderSamLite}{\tbd{nSATSnTwoShiftLTwoVarDecoderSamLite}}
\providecommand{\nSATSnTwoShiftLTwoVarDecoderSegformerMlp}{\tbd{nSATSnTwoShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\nSATSnTwoShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATSnTwoShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATburnBoundaryLOne}{\tbd{nSATburnBoundaryLOne}}
\providecommand{\nSATburnBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{nSATburnBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nSATburnBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{nSATburnBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nSATburnBoundaryLOneVarDecoderSamLite}{\tbd{nSATburnBoundaryLOneVarDecoderSamLite}}
\providecommand{\nSATburnBoundaryLOneVarDecoderSamPretrained}{\tbd{nSATburnBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\nSATburnBoundaryLOneVarDecoderSegformerMlp}{\tbd{nSATburnBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\nSATburnBoundaryLR}{\tbd{nSATburnBoundaryLR}}
\providecommand{\nSATburnBoundaryLRVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATburnBoundaryLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATburnBoundaryLTwo}{\tbd{nSATburnBoundaryLTwo}}
\providecommand{\nSATburnBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{nSATburnBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nSATburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{nSATburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATburnBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{nSATburnBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nSATburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{nSATburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATburnBoundaryLTwoVarDecoderSamLite}{\tbd{nSATburnBoundaryLTwoVarDecoderSamLite}}
\providecommand{\nSATburnBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{nSATburnBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATburnBoundaryLTwoVarDecoderSamPretrained}{\tbd{nSATburnBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\nSATburnBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{nSATburnBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATburnBoundaryLTwoVarDecoderSegformerMlp}{\tbd{nSATburnBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\nSATburnBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{nSATburnBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATburnBoundaryLTwoVarFrozenEncoderTrue}{\tbd{nSATburnBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\nSATburnBoundaryLTwoVarLossBootstrap}{\tbd{nSATburnBoundaryLTwoVarLossBootstrap}}
\providecommand{\nSATburnBoundaryLTwoVarLossGce}{\tbd{nSATburnBoundaryLTwoVarLossGce}}
\providecommand{\nSATburnBoundaryLTwoVarLrMultThree}{\tbd{nSATburnBoundaryLTwoVarLrMultThree}}
\providecommand{\nSATburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATburnBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{nSATburnBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nSATburnBoundaryLTwoVarValLabelsClean}{\tbd{nSATburnBoundaryLTwoVarValLabelsClean}}
\providecommand{\nSATburnClean}{\tbd{nSATburnClean}}
\providecommand{\nSATburnCleanVarDecoderMaskTwoformerFull}{\tbd{nSATburnCleanVarDecoderMaskTwoformerFull}}
\providecommand{\nSATburnCleanVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{nSATburnCleanVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATburnCleanVarDecoderMaskTwoformerLite}{\tbd{nSATburnCleanVarDecoderMaskTwoformerLite}}
\providecommand{\nSATburnCleanVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{nSATburnCleanVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATburnCleanVarDecoderSamLite}{\tbd{nSATburnCleanVarDecoderSamLite}}
\providecommand{\nSATburnCleanVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{nSATburnCleanVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATburnCleanVarDecoderSamPretrained}{\tbd{nSATburnCleanVarDecoderSamPretrained}}
\providecommand{\nSATburnCleanVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{nSATburnCleanVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATburnCleanVarDecoderSegformerMlp}{\tbd{nSATburnCleanVarDecoderSegformerMlp}}
\providecommand{\nSATburnCleanVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{nSATburnCleanVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATburnCleanVarFrozenEncoderTrue}{\tbd{nSATburnCleanVarFrozenEncoderTrue}}
\providecommand{\nSATburnCleanVarLossBootstrap}{\tbd{nSATburnCleanVarLossBootstrap}}
\providecommand{\nSATburnCleanVarLossGce}{\tbd{nSATburnCleanVarLossGce}}
\providecommand{\nSATburnCleanVarLrMultThree}{\tbd{nSATburnCleanVarLrMultThree}}
\providecommand{\nSATburnCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATburnCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATburnCleanVarTrainSubsetCleanTwoFive}{\tbd{nSATburnCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\nSATburnCleanVarValLabelsClean}{\tbd{nSATburnCleanVarValLabelsClean}}
\providecommand{\nSATburnCoarseLOne}{\tbd{nSATburnCoarseLOne}}
\providecommand{\nSATburnCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{nSATburnCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nSATburnCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{nSATburnCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nSATburnCoarseLOneVarDecoderSamLite}{\tbd{nSATburnCoarseLOneVarDecoderSamLite}}
\providecommand{\nSATburnCoarseLOneVarDecoderSamPretrained}{\tbd{nSATburnCoarseLOneVarDecoderSamPretrained}}
\providecommand{\nSATburnCoarseLOneVarDecoderSegformerMlp}{\tbd{nSATburnCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\nSATburnCoarseLR}{\tbd{nSATburnCoarseLR}}
\providecommand{\nSATburnCoarseLRVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATburnCoarseLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATburnCoarseLTwo}{\tbd{nSATburnCoarseLTwo}}
\providecommand{\nSATburnCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{nSATburnCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nSATburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{nSATburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATburnCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{nSATburnCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nSATburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{nSATburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATburnCoarseLTwoVarDecoderSamLite}{\tbd{nSATburnCoarseLTwoVarDecoderSamLite}}
\providecommand{\nSATburnCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{nSATburnCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATburnCoarseLTwoVarDecoderSamPretrained}{\tbd{nSATburnCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\nSATburnCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{nSATburnCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATburnCoarseLTwoVarDecoderSegformerMlp}{\tbd{nSATburnCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\nSATburnCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{nSATburnCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATburnCoarseLTwoVarEarlyStoppingFalse}{\tbd{nSATburnCoarseLTwoVarEarlyStoppingFalse}}
\providecommand{\nSATburnCoarseLTwoVarEarlyStoppingFalseFrozenEncoderTrue}{\tbd{nSATburnCoarseLTwoVarEarlyStoppingFalseFrozenEncoderTrue}}
\providecommand{\nSATburnCoarseLTwoVarFrozenEncoderTrue}{\tbd{nSATburnCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\nSATburnCoarseLTwoVarLossBootstrap}{\tbd{nSATburnCoarseLTwoVarLossBootstrap}}
\providecommand{\nSATburnCoarseLTwoVarLossGce}{\tbd{nSATburnCoarseLTwoVarLossGce}}
\providecommand{\nSATburnCoarseLTwoVarLrMultThree}{\tbd{nSATburnCoarseLTwoVarLrMultThree}}
\providecommand{\nSATburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATburnCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{nSATburnCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nSATburnCoarseLTwoVarValLabelsClean}{\tbd{nSATburnCoarseLTwoVarValLabelsClean}}
\providecommand{\nSATburnOmissionLOne}{\tbd{nSATburnOmissionLOne}}
\providecommand{\nSATburnOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{nSATburnOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nSATburnOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{nSATburnOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nSATburnOmissionLOneVarDecoderSamLite}{\tbd{nSATburnOmissionLOneVarDecoderSamLite}}
\providecommand{\nSATburnOmissionLOneVarDecoderSamPretrained}{\tbd{nSATburnOmissionLOneVarDecoderSamPretrained}}
\providecommand{\nSATburnOmissionLOneVarDecoderSegformerMlp}{\tbd{nSATburnOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\nSATburnOmissionLR}{\tbd{nSATburnOmissionLR}}
\providecommand{\nSATburnOmissionLRVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATburnOmissionLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATburnOmissionLTwo}{\tbd{nSATburnOmissionLTwo}}
\providecommand{\nSATburnOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{nSATburnOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nSATburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{nSATburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATburnOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{nSATburnOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nSATburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{nSATburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATburnOmissionLTwoVarDecoderSamLite}{\tbd{nSATburnOmissionLTwoVarDecoderSamLite}}
\providecommand{\nSATburnOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{nSATburnOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATburnOmissionLTwoVarDecoderSamPretrained}{\tbd{nSATburnOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\nSATburnOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{nSATburnOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATburnOmissionLTwoVarDecoderSegformerMlp}{\tbd{nSATburnOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\nSATburnOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{nSATburnOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATburnOmissionLTwoVarFrozenEncoderTrue}{\tbd{nSATburnOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\nSATburnOmissionLTwoVarLossBootstrap}{\tbd{nSATburnOmissionLTwoVarLossBootstrap}}
\providecommand{\nSATburnOmissionLTwoVarLossGce}{\tbd{nSATburnOmissionLTwoVarLossGce}}
\providecommand{\nSATburnOmissionLTwoVarLrMultThree}{\tbd{nSATburnOmissionLTwoVarLrMultThree}}
\providecommand{\nSATburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATburnOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{nSATburnOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nSATburnOmissionLTwoVarValLabelsClean}{\tbd{nSATburnOmissionLTwoVarValLabelsClean}}
\providecommand{\nSATburnShiftLOne}{\tbd{nSATburnShiftLOne}}
\providecommand{\nSATburnShiftLOneVarDecoderMaskTwoformerFull}{\tbd{nSATburnShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nSATburnShiftLOneVarDecoderMaskTwoformerLite}{\tbd{nSATburnShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nSATburnShiftLOneVarDecoderSamLite}{\tbd{nSATburnShiftLOneVarDecoderSamLite}}
\providecommand{\nSATburnShiftLOneVarDecoderSamPretrained}{\tbd{nSATburnShiftLOneVarDecoderSamPretrained}}
\providecommand{\nSATburnShiftLOneVarDecoderSegformerMlp}{\tbd{nSATburnShiftLOneVarDecoderSegformerMlp}}
\providecommand{\nSATburnShiftLR}{\tbd{nSATburnShiftLR}}
\providecommand{\nSATburnShiftLRVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATburnShiftLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATburnShiftLTwo}{\tbd{nSATburnShiftLTwo}}
\providecommand{\nSATburnShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{nSATburnShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nSATburnShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{nSATburnShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATburnShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{nSATburnShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nSATburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{nSATburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATburnShiftLTwoVarDecoderSamLite}{\tbd{nSATburnShiftLTwoVarDecoderSamLite}}
\providecommand{\nSATburnShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{nSATburnShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATburnShiftLTwoVarDecoderSamPretrained}{\tbd{nSATburnShiftLTwoVarDecoderSamPretrained}}
\providecommand{\nSATburnShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{nSATburnShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATburnShiftLTwoVarDecoderSegformerMlp}{\tbd{nSATburnShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\nSATburnShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{nSATburnShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATburnShiftLTwoVarFrozenEncoderTrue}{\tbd{nSATburnShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\nSATburnShiftLTwoVarLossBootstrap}{\tbd{nSATburnShiftLTwoVarLossBootstrap}}
\providecommand{\nSATburnShiftLTwoVarLossGce}{\tbd{nSATburnShiftLTwoVarLossGce}}
\providecommand{\nSATburnShiftLTwoVarLrMultThree}{\tbd{nSATburnShiftLTwoVarLrMultThree}}
\providecommand{\nSATburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATburnShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{nSATburnShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nSATburnShiftLTwoVarValLabelsClean}{\tbd{nSATburnShiftLTwoVarValLabelsClean}}
\providecommand{\nSATflairBoundaryLOne}{\tbd{nSATflairBoundaryLOne}}
\providecommand{\nSATflairBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{nSATflairBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nSATflairBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{nSATflairBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nSATflairBoundaryLOneVarDecoderSamLite}{\tbd{nSATflairBoundaryLOneVarDecoderSamLite}}
\providecommand{\nSATflairBoundaryLOneVarDecoderSamPretrained}{\tbd{nSATflairBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\nSATflairBoundaryLOneVarDecoderSegformerMlp}{\tbd{nSATflairBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\nSATflairBoundaryLR}{\tbd{nSATflairBoundaryLR}}
\providecommand{\nSATflairBoundaryLRVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATflairBoundaryLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATflairBoundaryLTwo}{\tbd{nSATflairBoundaryLTwo}}
\providecommand{\nSATflairBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{nSATflairBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nSATflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{nSATflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATflairBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{nSATflairBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nSATflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{nSATflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATflairBoundaryLTwoVarDecoderSamLite}{\tbd{nSATflairBoundaryLTwoVarDecoderSamLite}}
\providecommand{\nSATflairBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{nSATflairBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATflairBoundaryLTwoVarDecoderSamPretrained}{\tbd{nSATflairBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\nSATflairBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{nSATflairBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATflairBoundaryLTwoVarDecoderSegformerMlp}{\tbd{nSATflairBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\nSATflairBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{nSATflairBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATflairBoundaryLTwoVarFrozenEncoderTrue}{\tbd{nSATflairBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\nSATflairBoundaryLTwoVarLossBootstrap}{\tbd{nSATflairBoundaryLTwoVarLossBootstrap}}
\providecommand{\nSATflairBoundaryLTwoVarLossGce}{\tbd{nSATflairBoundaryLTwoVarLossGce}}
\providecommand{\nSATflairBoundaryLTwoVarLrMultThree}{\tbd{nSATflairBoundaryLTwoVarLrMultThree}}
\providecommand{\nSATflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATflairBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{nSATflairBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nSATflairBoundaryLTwoVarValLabelsClean}{\tbd{nSATflairBoundaryLTwoVarValLabelsClean}}
\providecommand{\nSATflairClean}{\tbd{nSATflairClean}}
\providecommand{\nSATflairCleanVarClassWeightedTrue}{\tbd{nSATflairCleanVarClassWeightedTrue}}
\providecommand{\nSATflairCleanVarDecoderMaskTwoformerFull}{\tbd{nSATflairCleanVarDecoderMaskTwoformerFull}}
\providecommand{\nSATflairCleanVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{nSATflairCleanVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATflairCleanVarDecoderMaskTwoformerLite}{\tbd{nSATflairCleanVarDecoderMaskTwoformerLite}}
\providecommand{\nSATflairCleanVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{nSATflairCleanVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATflairCleanVarDecoderSamLite}{\tbd{nSATflairCleanVarDecoderSamLite}}
\providecommand{\nSATflairCleanVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{nSATflairCleanVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATflairCleanVarDecoderSamPretrained}{\tbd{nSATflairCleanVarDecoderSamPretrained}}
\providecommand{\nSATflairCleanVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{nSATflairCleanVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATflairCleanVarDecoderSegformerMlp}{\tbd{nSATflairCleanVarDecoderSegformerMlp}}
\providecommand{\nSATflairCleanVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{nSATflairCleanVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATflairCleanVarFrozenEncoderTrue}{\tbd{nSATflairCleanVarFrozenEncoderTrue}}
\providecommand{\nSATflairCleanVarLossBootstrap}{\tbd{nSATflairCleanVarLossBootstrap}}
\providecommand{\nSATflairCleanVarLossGce}{\tbd{nSATflairCleanVarLossGce}}
\providecommand{\nSATflairCleanVarLrMultThree}{\tbd{nSATflairCleanVarLrMultThree}}
\providecommand{\nSATflairCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATflairCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATflairCleanVarTrainSubsetCleanTwoFive}{\tbd{nSATflairCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\nSATflairCleanVarValLabelsClean}{\tbd{nSATflairCleanVarValLabelsClean}}
\providecommand{\nSATflairCoarseLOne}{\tbd{nSATflairCoarseLOne}}
\providecommand{\nSATflairCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{nSATflairCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nSATflairCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{nSATflairCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nSATflairCoarseLOneVarDecoderSamLite}{\tbd{nSATflairCoarseLOneVarDecoderSamLite}}
\providecommand{\nSATflairCoarseLOneVarDecoderSamPretrained}{\tbd{nSATflairCoarseLOneVarDecoderSamPretrained}}
\providecommand{\nSATflairCoarseLOneVarDecoderSegformerMlp}{\tbd{nSATflairCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\nSATflairCoarseLR}{\tbd{nSATflairCoarseLR}}
\providecommand{\nSATflairCoarseLRVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATflairCoarseLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATflairCoarseLTwo}{\tbd{nSATflairCoarseLTwo}}
\providecommand{\nSATflairCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{nSATflairCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nSATflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{nSATflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATflairCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{nSATflairCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nSATflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{nSATflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATflairCoarseLTwoVarDecoderSamLite}{\tbd{nSATflairCoarseLTwoVarDecoderSamLite}}
\providecommand{\nSATflairCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{nSATflairCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATflairCoarseLTwoVarDecoderSamPretrained}{\tbd{nSATflairCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\nSATflairCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{nSATflairCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATflairCoarseLTwoVarDecoderSegformerMlp}{\tbd{nSATflairCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\nSATflairCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{nSATflairCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATflairCoarseLTwoVarFrozenEncoderTrue}{\tbd{nSATflairCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\nSATflairCoarseLTwoVarLossBootstrap}{\tbd{nSATflairCoarseLTwoVarLossBootstrap}}
\providecommand{\nSATflairCoarseLTwoVarLossGce}{\tbd{nSATflairCoarseLTwoVarLossGce}}
\providecommand{\nSATflairCoarseLTwoVarLrMultThree}{\tbd{nSATflairCoarseLTwoVarLrMultThree}}
\providecommand{\nSATflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATflairCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{nSATflairCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nSATflairCoarseLTwoVarValLabelsClean}{\tbd{nSATflairCoarseLTwoVarValLabelsClean}}
\providecommand{\nSATflairOmissionLOne}{\tbd{nSATflairOmissionLOne}}
\providecommand{\nSATflairOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{nSATflairOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nSATflairOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{nSATflairOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nSATflairOmissionLOneVarDecoderSamLite}{\tbd{nSATflairOmissionLOneVarDecoderSamLite}}
\providecommand{\nSATflairOmissionLOneVarDecoderSamPretrained}{\tbd{nSATflairOmissionLOneVarDecoderSamPretrained}}
\providecommand{\nSATflairOmissionLOneVarDecoderSegformerMlp}{\tbd{nSATflairOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\nSATflairOmissionLR}{\tbd{nSATflairOmissionLR}}
\providecommand{\nSATflairOmissionLRVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATflairOmissionLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATflairOmissionLTwo}{\tbd{nSATflairOmissionLTwo}}
\providecommand{\nSATflairOmissionLTwoVarClassWeightedTrue}{\tbd{nSATflairOmissionLTwoVarClassWeightedTrue}}
\providecommand{\nSATflairOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{nSATflairOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nSATflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{nSATflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATflairOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{nSATflairOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nSATflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{nSATflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATflairOmissionLTwoVarDecoderSamLite}{\tbd{nSATflairOmissionLTwoVarDecoderSamLite}}
\providecommand{\nSATflairOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{nSATflairOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATflairOmissionLTwoVarDecoderSamPretrained}{\tbd{nSATflairOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\nSATflairOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{nSATflairOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATflairOmissionLTwoVarDecoderSegformerMlp}{\tbd{nSATflairOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\nSATflairOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{nSATflairOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATflairOmissionLTwoVarEarlyStoppingFalse}{\tbd{nSATflairOmissionLTwoVarEarlyStoppingFalse}}
\providecommand{\nSATflairOmissionLTwoVarEarlyStoppingFalseFrozenEncoderTrue}{\tbd{nSATflairOmissionLTwoVarEarlyStoppingFalseFrozenEncoderTrue}}
\providecommand{\nSATflairOmissionLTwoVarFrozenEncoderTrue}{\tbd{nSATflairOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\nSATflairOmissionLTwoVarLossBootstrap}{\tbd{nSATflairOmissionLTwoVarLossBootstrap}}
\providecommand{\nSATflairOmissionLTwoVarLossGce}{\tbd{nSATflairOmissionLTwoVarLossGce}}
\providecommand{\nSATflairOmissionLTwoVarLrMultThree}{\tbd{nSATflairOmissionLTwoVarLrMultThree}}
\providecommand{\nSATflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATflairOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{nSATflairOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nSATflairOmissionLTwoVarValLabelsClean}{\tbd{nSATflairOmissionLTwoVarValLabelsClean}}
\providecommand{\nSATflairShiftLOne}{\tbd{nSATflairShiftLOne}}
\providecommand{\nSATflairShiftLOneVarDecoderMaskTwoformerFull}{\tbd{nSATflairShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nSATflairShiftLOneVarDecoderMaskTwoformerLite}{\tbd{nSATflairShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nSATflairShiftLOneVarDecoderSamLite}{\tbd{nSATflairShiftLOneVarDecoderSamLite}}
\providecommand{\nSATflairShiftLOneVarDecoderSamPretrained}{\tbd{nSATflairShiftLOneVarDecoderSamPretrained}}
\providecommand{\nSATflairShiftLOneVarDecoderSegformerMlp}{\tbd{nSATflairShiftLOneVarDecoderSegformerMlp}}
\providecommand{\nSATflairShiftLR}{\tbd{nSATflairShiftLR}}
\providecommand{\nSATflairShiftLRVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATflairShiftLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATflairShiftLTwo}{\tbd{nSATflairShiftLTwo}}
\providecommand{\nSATflairShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{nSATflairShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nSATflairShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{nSATflairShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATflairShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{nSATflairShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nSATflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{nSATflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATflairShiftLTwoVarDecoderSamLite}{\tbd{nSATflairShiftLTwoVarDecoderSamLite}}
\providecommand{\nSATflairShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{nSATflairShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATflairShiftLTwoVarDecoderSamPretrained}{\tbd{nSATflairShiftLTwoVarDecoderSamPretrained}}
\providecommand{\nSATflairShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{nSATflairShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATflairShiftLTwoVarDecoderSegformerMlp}{\tbd{nSATflairShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\nSATflairShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{nSATflairShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATflairShiftLTwoVarFrozenEncoderTrue}{\tbd{nSATflairShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\nSATflairShiftLTwoVarLossBootstrap}{\tbd{nSATflairShiftLTwoVarLossBootstrap}}
\providecommand{\nSATflairShiftLTwoVarLossGce}{\tbd{nSATflairShiftLTwoVarLossGce}}
\providecommand{\nSATflairShiftLTwoVarLrMultThree}{\tbd{nSATflairShiftLTwoVarLrMultThree}}
\providecommand{\nSATflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nSATflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nSATflairShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{nSATflairShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nSATflairShiftLTwoVarValLabelsClean}{\tbd{nSATflairShiftLTwoVarValLabelsClean}}
\providecommand{\nSATsenClean}{\tbd{nSATsenClean}}
\providecommand{\nSATsenOtsuLTwo}{\tbd{nSATsenOtsuLTwo}}
\providecommand{\nTMChesBoundaryLOne}{\tbd{nTMChesBoundaryLOne}}
\providecommand{\nTMChesBoundaryLTwo}{\tbd{nTMChesBoundaryLTwo}}
\providecommand{\nTMChesClean}{\tbd{nTMChesClean}}
\providecommand{\nTMChesCoarseLOne}{\tbd{nTMChesCoarseLOne}}
\providecommand{\nTMChesCoarseLTwo}{\tbd{nTMChesCoarseLTwo}}
\providecommand{\nTMChesNlcdREAL}{\tbd{nTMChesNlcdREAL}}
\providecommand{\nTMChesOmissionLOne}{\tbd{nTMChesOmissionLOne}}
\providecommand{\nTMChesOmissionLTwo}{\tbd{nTMChesOmissionLTwo}}
\providecommand{\nTMChesShiftLOne}{\tbd{nTMChesShiftLOne}}
\providecommand{\nTMChesShiftLTwo}{\tbd{nTMChesShiftLTwo}}
\providecommand{\nTMCsTwelveBoundaryLOne}{\tbd{nTMCsTwelveBoundaryLOne}}
\providecommand{\nTMCsTwelveBoundaryLTwo}{\tbd{nTMCsTwelveBoundaryLTwo}}
\providecommand{\nTMCsTwelveClean}{\tbd{nTMCsTwelveClean}}
\providecommand{\nTMCsTwelveCoarseLOne}{\tbd{nTMCsTwelveCoarseLOne}}
\providecommand{\nTMCsTwelveCoarseLTwo}{\tbd{nTMCsTwelveCoarseLTwo}}
\providecommand{\nTMCsTwelveOmissionLOne}{\tbd{nTMCsTwelveOmissionLOne}}
\providecommand{\nTMCsTwelveOmissionLTwo}{\tbd{nTMCsTwelveOmissionLTwo}}
\providecommand{\nTMCsTwelveSTwocloudlessREAL}{\tbd{nTMCsTwelveSTwocloudlessREAL}}
\providecommand{\nTMCsTwelveShiftLOne}{\tbd{nTMCsTwelveShiftLOne}}
\providecommand{\nTMCsTwelveShiftLTwo}{\tbd{nTMCsTwelveShiftLTwo}}
\providecommand{\nTMDfcBoundaryLOne}{\tbd{nTMDfcBoundaryLOne}}
\providecommand{\nTMDfcBoundaryLTwo}{\tbd{nTMDfcBoundaryLTwo}}
\providecommand{\nTMDfcClean}{\tbd{nTMDfcClean}}
\providecommand{\nTMDfcCleanVarTrainSubsetRealcov}{\tbd{nTMDfcCleanVarTrainSubsetRealcov}}
\providecommand{\nTMDfcCoarseLOne}{\tbd{nTMDfcCoarseLOne}}
\providecommand{\nTMDfcCoarseLTwo}{\tbd{nTMDfcCoarseLTwo}}
\providecommand{\nTMDfcModisREALVarTrainSubsetRealcov}{\tbd{nTMDfcModisREALVarTrainSubsetRealcov}}
\providecommand{\nTMDfcOmissionLOne}{\tbd{nTMDfcOmissionLOne}}
\providecommand{\nTMDfcOmissionLTwo}{\tbd{nTMDfcOmissionLTwo}}
\providecommand{\nTMDfcShiftLOne}{\tbd{nTMDfcShiftLOne}}
\providecommand{\nTMDfcShiftLTwo}{\tbd{nTMDfcShiftLTwo}}
\providecommand{\nTMEnvaBoundaryLOne}{\tbd{nTMEnvaBoundaryLOne}}
\providecommand{\nTMEnvaBoundaryLTwo}{\tbd{nTMEnvaBoundaryLTwo}}
\providecommand{\nTMEnvaClean}{\tbd{nTMEnvaClean}}
\providecommand{\nTMEnvaCoarseLOne}{\tbd{nTMEnvaCoarseLOne}}
\providecommand{\nTMEnvaCoarseLTwo}{\tbd{nTMEnvaCoarseLTwo}}
\providecommand{\nTMEnvaNlcdREAL}{\tbd{nTMEnvaNlcdREAL}}
\providecommand{\nTMEnvaOmissionLOne}{\tbd{nTMEnvaOmissionLOne}}
\providecommand{\nTMEnvaOmissionLTwo}{\tbd{nTMEnvaOmissionLTwo}}
\providecommand{\nTMEnvaShiftLOne}{\tbd{nTMEnvaShiftLOne}}
\providecommand{\nTMEnvaShiftLTwo}{\tbd{nTMEnvaShiftLTwo}}
\providecommand{\nTMKuroBoundaryLOne}{\tbd{nTMKuroBoundaryLOne}}
\providecommand{\nTMKuroBoundaryLTwo}{\tbd{nTMKuroBoundaryLTwo}}
\providecommand{\nTMKuroCemsREALVarTrainSubsetRealcov}{\tbd{nTMKuroCemsREALVarTrainSubsetRealcov}}
\providecommand{\nTMKuroClean}{\tbd{nTMKuroClean}}
\providecommand{\nTMKuroCleanVarTrainSubsetRealcov}{\tbd{nTMKuroCleanVarTrainSubsetRealcov}}
\providecommand{\nTMKuroCoarseLOne}{\tbd{nTMKuroCoarseLOne}}
\providecommand{\nTMKuroCoarseLTwo}{\tbd{nTMKuroCoarseLTwo}}
\providecommand{\nTMKuroOmissionLOne}{\tbd{nTMKuroOmissionLOne}}
\providecommand{\nTMKuroOmissionLTwo}{\tbd{nTMKuroOmissionLTwo}}
\providecommand{\nTMKuroShiftLOne}{\tbd{nTMKuroShiftLOne}}
\providecommand{\nTMKuroShiftLTwo}{\tbd{nTMKuroShiftLTwo}}
\providecommand{\nTMOemBoundaryLOne}{\tbd{nTMOemBoundaryLOne}}
\providecommand{\nTMOemBoundaryLTwo}{\tbd{nTMOemBoundaryLTwo}}
\providecommand{\nTMOemClean}{\tbd{nTMOemClean}}
\providecommand{\nTMOemCoarseLOne}{\tbd{nTMOemCoarseLOne}}
\providecommand{\nTMOemCoarseLTwo}{\tbd{nTMOemCoarseLTwo}}
\providecommand{\nTMOemOmissionLOne}{\tbd{nTMOemOmissionLOne}}
\providecommand{\nTMOemOmissionLTwo}{\tbd{nTMOemOmissionLTwo}}
\providecommand{\nTMOemShiftLOne}{\tbd{nTMOemShiftLOne}}
\providecommand{\nTMOemShiftLTwo}{\tbd{nTMOemShiftLTwo}}
\providecommand{\nTMSnTwoBoundaryLOne}{\tbd{nTMSnTwoBoundaryLOne}}
\providecommand{\nTMSnTwoBoundaryLTwo}{\tbd{nTMSnTwoBoundaryLTwo}}
\providecommand{\nTMSnTwoClean}{\tbd{nTMSnTwoClean}}
\providecommand{\nTMSnTwoCoarseLOne}{\tbd{nTMSnTwoCoarseLOne}}
\providecommand{\nTMSnTwoCoarseLTwo}{\tbd{nTMSnTwoCoarseLTwo}}
\providecommand{\nTMSnTwoOmissionLOne}{\tbd{nTMSnTwoOmissionLOne}}
\providecommand{\nTMSnTwoOmissionLTwo}{\tbd{nTMSnTwoOmissionLTwo}}
\providecommand{\nTMSnTwoShiftLOne}{\tbd{nTMSnTwoShiftLOne}}
\providecommand{\nTMSnTwoShiftLTwo}{\tbd{nTMSnTwoShiftLTwo}}
\providecommand{\nTMburnBoundaryLOne}{\tbd{nTMburnBoundaryLOne}}
\providecommand{\nTMburnBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{nTMburnBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nTMburnBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{nTMburnBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nTMburnBoundaryLOneVarDecoderSamLite}{\tbd{nTMburnBoundaryLOneVarDecoderSamLite}}
\providecommand{\nTMburnBoundaryLOneVarDecoderSamPretrained}{\tbd{nTMburnBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\nTMburnBoundaryLOneVarDecoderSegformerMlp}{\tbd{nTMburnBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\nTMburnBoundaryLR}{\tbd{nTMburnBoundaryLR}}
\providecommand{\nTMburnBoundaryLTwo}{\tbd{nTMburnBoundaryLTwo}}
\providecommand{\nTMburnBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{nTMburnBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nTMburnBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{nTMburnBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nTMburnBoundaryLTwoVarDecoderSamLite}{\tbd{nTMburnBoundaryLTwoVarDecoderSamLite}}
\providecommand{\nTMburnBoundaryLTwoVarDecoderSamPretrained}{\tbd{nTMburnBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\nTMburnBoundaryLTwoVarDecoderSegformerMlp}{\tbd{nTMburnBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\nTMburnBoundaryLTwoVarFrozenEncoderTrue}{\tbd{nTMburnBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\nTMburnBoundaryLTwoVarLossBootstrap}{\tbd{nTMburnBoundaryLTwoVarLossBootstrap}}
\providecommand{\nTMburnBoundaryLTwoVarLossGce}{\tbd{nTMburnBoundaryLTwoVarLossGce}}
\providecommand{\nTMburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nTMburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nTMburnBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{nTMburnBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nTMburnClean}{\tbd{nTMburnClean}}
\providecommand{\nTMburnCleanVarDecoderMaskTwoformerFull}{\tbd{nTMburnCleanVarDecoderMaskTwoformerFull}}
\providecommand{\nTMburnCleanVarDecoderMaskTwoformerLite}{\tbd{nTMburnCleanVarDecoderMaskTwoformerLite}}
\providecommand{\nTMburnCleanVarDecoderSamLite}{\tbd{nTMburnCleanVarDecoderSamLite}}
\providecommand{\nTMburnCleanVarDecoderSamPretrained}{\tbd{nTMburnCleanVarDecoderSamPretrained}}
\providecommand{\nTMburnCleanVarDecoderSegformerMlp}{\tbd{nTMburnCleanVarDecoderSegformerMlp}}
\providecommand{\nTMburnCleanVarFrozenEncoderTrue}{\tbd{nTMburnCleanVarFrozenEncoderTrue}}
\providecommand{\nTMburnCleanVarLossBootstrap}{\tbd{nTMburnCleanVarLossBootstrap}}
\providecommand{\nTMburnCleanVarLossGce}{\tbd{nTMburnCleanVarLossGce}}
\providecommand{\nTMburnCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{nTMburnCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nTMburnCleanVarTrainSubsetCleanTwoFive}{\tbd{nTMburnCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\nTMburnCoarseLOne}{\tbd{nTMburnCoarseLOne}}
\providecommand{\nTMburnCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{nTMburnCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nTMburnCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{nTMburnCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nTMburnCoarseLOneVarDecoderSamLite}{\tbd{nTMburnCoarseLOneVarDecoderSamLite}}
\providecommand{\nTMburnCoarseLOneVarDecoderSamPretrained}{\tbd{nTMburnCoarseLOneVarDecoderSamPretrained}}
\providecommand{\nTMburnCoarseLOneVarDecoderSegformerMlp}{\tbd{nTMburnCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\nTMburnCoarseLR}{\tbd{nTMburnCoarseLR}}
\providecommand{\nTMburnCoarseLTwo}{\tbd{nTMburnCoarseLTwo}}
\providecommand{\nTMburnCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{nTMburnCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nTMburnCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{nTMburnCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nTMburnCoarseLTwoVarDecoderSamLite}{\tbd{nTMburnCoarseLTwoVarDecoderSamLite}}
\providecommand{\nTMburnCoarseLTwoVarDecoderSamPretrained}{\tbd{nTMburnCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\nTMburnCoarseLTwoVarDecoderSegformerMlp}{\tbd{nTMburnCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\nTMburnCoarseLTwoVarFrozenEncoderTrue}{\tbd{nTMburnCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\nTMburnCoarseLTwoVarLossBootstrap}{\tbd{nTMburnCoarseLTwoVarLossBootstrap}}
\providecommand{\nTMburnCoarseLTwoVarLossGce}{\tbd{nTMburnCoarseLTwoVarLossGce}}
\providecommand{\nTMburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nTMburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nTMburnCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{nTMburnCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nTMburnOmissionLOne}{\tbd{nTMburnOmissionLOne}}
\providecommand{\nTMburnOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{nTMburnOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nTMburnOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{nTMburnOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nTMburnOmissionLOneVarDecoderSamLite}{\tbd{nTMburnOmissionLOneVarDecoderSamLite}}
\providecommand{\nTMburnOmissionLOneVarDecoderSamPretrained}{\tbd{nTMburnOmissionLOneVarDecoderSamPretrained}}
\providecommand{\nTMburnOmissionLOneVarDecoderSegformerMlp}{\tbd{nTMburnOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\nTMburnOmissionLR}{\tbd{nTMburnOmissionLR}}
\providecommand{\nTMburnOmissionLTwo}{\tbd{nTMburnOmissionLTwo}}
\providecommand{\nTMburnOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{nTMburnOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nTMburnOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{nTMburnOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nTMburnOmissionLTwoVarDecoderSamLite}{\tbd{nTMburnOmissionLTwoVarDecoderSamLite}}
\providecommand{\nTMburnOmissionLTwoVarDecoderSamPretrained}{\tbd{nTMburnOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\nTMburnOmissionLTwoVarDecoderSegformerMlp}{\tbd{nTMburnOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\nTMburnOmissionLTwoVarFrozenEncoderTrue}{\tbd{nTMburnOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\nTMburnOmissionLTwoVarLossBootstrap}{\tbd{nTMburnOmissionLTwoVarLossBootstrap}}
\providecommand{\nTMburnOmissionLTwoVarLossGce}{\tbd{nTMburnOmissionLTwoVarLossGce}}
\providecommand{\nTMburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nTMburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nTMburnOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{nTMburnOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nTMburnShiftLOne}{\tbd{nTMburnShiftLOne}}
\providecommand{\nTMburnShiftLOneVarDecoderMaskTwoformerFull}{\tbd{nTMburnShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nTMburnShiftLOneVarDecoderMaskTwoformerLite}{\tbd{nTMburnShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nTMburnShiftLOneVarDecoderSamLite}{\tbd{nTMburnShiftLOneVarDecoderSamLite}}
\providecommand{\nTMburnShiftLOneVarDecoderSamPretrained}{\tbd{nTMburnShiftLOneVarDecoderSamPretrained}}
\providecommand{\nTMburnShiftLOneVarDecoderSegformerMlp}{\tbd{nTMburnShiftLOneVarDecoderSegformerMlp}}
\providecommand{\nTMburnShiftLR}{\tbd{nTMburnShiftLR}}
\providecommand{\nTMburnShiftLTwo}{\tbd{nTMburnShiftLTwo}}
\providecommand{\nTMburnShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{nTMburnShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nTMburnShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{nTMburnShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nTMburnShiftLTwoVarDecoderSamLite}{\tbd{nTMburnShiftLTwoVarDecoderSamLite}}
\providecommand{\nTMburnShiftLTwoVarDecoderSamPretrained}{\tbd{nTMburnShiftLTwoVarDecoderSamPretrained}}
\providecommand{\nTMburnShiftLTwoVarDecoderSegformerMlp}{\tbd{nTMburnShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\nTMburnShiftLTwoVarFrozenEncoderTrue}{\tbd{nTMburnShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\nTMburnShiftLTwoVarLossBootstrap}{\tbd{nTMburnShiftLTwoVarLossBootstrap}}
\providecommand{\nTMburnShiftLTwoVarLossGce}{\tbd{nTMburnShiftLTwoVarLossGce}}
\providecommand{\nTMburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nTMburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nTMburnShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{nTMburnShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nTMflairBoundaryLOne}{\tbd{nTMflairBoundaryLOne}}
\providecommand{\nTMflairBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{nTMflairBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nTMflairBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{nTMflairBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nTMflairBoundaryLOneVarDecoderSamLite}{\tbd{nTMflairBoundaryLOneVarDecoderSamLite}}
\providecommand{\nTMflairBoundaryLOneVarDecoderSamPretrained}{\tbd{nTMflairBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\nTMflairBoundaryLOneVarDecoderSegformerMlp}{\tbd{nTMflairBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\nTMflairBoundaryLR}{\tbd{nTMflairBoundaryLR}}
\providecommand{\nTMflairBoundaryLTwo}{\tbd{nTMflairBoundaryLTwo}}
\providecommand{\nTMflairBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{nTMflairBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nTMflairBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{nTMflairBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nTMflairBoundaryLTwoVarDecoderSamLite}{\tbd{nTMflairBoundaryLTwoVarDecoderSamLite}}
\providecommand{\nTMflairBoundaryLTwoVarDecoderSamPretrained}{\tbd{nTMflairBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\nTMflairBoundaryLTwoVarDecoderSegformerMlp}{\tbd{nTMflairBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\nTMflairBoundaryLTwoVarFrozenEncoderTrue}{\tbd{nTMflairBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\nTMflairBoundaryLTwoVarLossBootstrap}{\tbd{nTMflairBoundaryLTwoVarLossBootstrap}}
\providecommand{\nTMflairBoundaryLTwoVarLossGce}{\tbd{nTMflairBoundaryLTwoVarLossGce}}
\providecommand{\nTMflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nTMflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nTMflairBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{nTMflairBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nTMflairClean}{\tbd{nTMflairClean}}
\providecommand{\nTMflairCleanVarDecoderMaskTwoformerFull}{\tbd{nTMflairCleanVarDecoderMaskTwoformerFull}}
\providecommand{\nTMflairCleanVarDecoderMaskTwoformerLite}{\tbd{nTMflairCleanVarDecoderMaskTwoformerLite}}
\providecommand{\nTMflairCleanVarDecoderSamLite}{\tbd{nTMflairCleanVarDecoderSamLite}}
\providecommand{\nTMflairCleanVarDecoderSamPretrained}{\tbd{nTMflairCleanVarDecoderSamPretrained}}
\providecommand{\nTMflairCleanVarDecoderSegformerMlp}{\tbd{nTMflairCleanVarDecoderSegformerMlp}}
\providecommand{\nTMflairCleanVarFrozenEncoderTrue}{\tbd{nTMflairCleanVarFrozenEncoderTrue}}
\providecommand{\nTMflairCleanVarLossBootstrap}{\tbd{nTMflairCleanVarLossBootstrap}}
\providecommand{\nTMflairCleanVarLossGce}{\tbd{nTMflairCleanVarLossGce}}
\providecommand{\nTMflairCleanVarLrMultZeroThreeThreeThreeThree}{\tbd{nTMflairCleanVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nTMflairCleanVarTrainSubsetCleanTwoFive}{\tbd{nTMflairCleanVarTrainSubsetCleanTwoFive}}
\providecommand{\nTMflairCoarseLOne}{\tbd{nTMflairCoarseLOne}}
\providecommand{\nTMflairCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{nTMflairCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nTMflairCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{nTMflairCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nTMflairCoarseLOneVarDecoderSamLite}{\tbd{nTMflairCoarseLOneVarDecoderSamLite}}
\providecommand{\nTMflairCoarseLOneVarDecoderSamPretrained}{\tbd{nTMflairCoarseLOneVarDecoderSamPretrained}}
\providecommand{\nTMflairCoarseLOneVarDecoderSegformerMlp}{\tbd{nTMflairCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\nTMflairCoarseLR}{\tbd{nTMflairCoarseLR}}
\providecommand{\nTMflairCoarseLTwo}{\tbd{nTMflairCoarseLTwo}}
\providecommand{\nTMflairCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{nTMflairCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nTMflairCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{nTMflairCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nTMflairCoarseLTwoVarDecoderSamLite}{\tbd{nTMflairCoarseLTwoVarDecoderSamLite}}
\providecommand{\nTMflairCoarseLTwoVarDecoderSamPretrained}{\tbd{nTMflairCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\nTMflairCoarseLTwoVarDecoderSegformerMlp}{\tbd{nTMflairCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\nTMflairCoarseLTwoVarFrozenEncoderTrue}{\tbd{nTMflairCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\nTMflairCoarseLTwoVarLossBootstrap}{\tbd{nTMflairCoarseLTwoVarLossBootstrap}}
\providecommand{\nTMflairCoarseLTwoVarLossGce}{\tbd{nTMflairCoarseLTwoVarLossGce}}
\providecommand{\nTMflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nTMflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nTMflairCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{nTMflairCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nTMflairOmissionLOne}{\tbd{nTMflairOmissionLOne}}
\providecommand{\nTMflairOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{nTMflairOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nTMflairOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{nTMflairOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nTMflairOmissionLOneVarDecoderSamLite}{\tbd{nTMflairOmissionLOneVarDecoderSamLite}}
\providecommand{\nTMflairOmissionLOneVarDecoderSamPretrained}{\tbd{nTMflairOmissionLOneVarDecoderSamPretrained}}
\providecommand{\nTMflairOmissionLOneVarDecoderSegformerMlp}{\tbd{nTMflairOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\nTMflairOmissionLR}{\tbd{nTMflairOmissionLR}}
\providecommand{\nTMflairOmissionLTwo}{\tbd{nTMflairOmissionLTwo}}
\providecommand{\nTMflairOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{nTMflairOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nTMflairOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{nTMflairOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nTMflairOmissionLTwoVarDecoderSamLite}{\tbd{nTMflairOmissionLTwoVarDecoderSamLite}}
\providecommand{\nTMflairOmissionLTwoVarDecoderSamPretrained}{\tbd{nTMflairOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\nTMflairOmissionLTwoVarDecoderSegformerMlp}{\tbd{nTMflairOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\nTMflairOmissionLTwoVarFrozenEncoderTrue}{\tbd{nTMflairOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\nTMflairOmissionLTwoVarLossBootstrap}{\tbd{nTMflairOmissionLTwoVarLossBootstrap}}
\providecommand{\nTMflairOmissionLTwoVarLossGce}{\tbd{nTMflairOmissionLTwoVarLossGce}}
\providecommand{\nTMflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nTMflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nTMflairOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{nTMflairOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nTMflairShiftLOne}{\tbd{nTMflairShiftLOne}}
\providecommand{\nTMflairShiftLOneVarDecoderMaskTwoformerFull}{\tbd{nTMflairShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\nTMflairShiftLOneVarDecoderMaskTwoformerLite}{\tbd{nTMflairShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\nTMflairShiftLOneVarDecoderSamLite}{\tbd{nTMflairShiftLOneVarDecoderSamLite}}
\providecommand{\nTMflairShiftLOneVarDecoderSamPretrained}{\tbd{nTMflairShiftLOneVarDecoderSamPretrained}}
\providecommand{\nTMflairShiftLOneVarDecoderSegformerMlp}{\tbd{nTMflairShiftLOneVarDecoderSegformerMlp}}
\providecommand{\nTMflairShiftLR}{\tbd{nTMflairShiftLR}}
\providecommand{\nTMflairShiftLTwo}{\tbd{nTMflairShiftLTwo}}
\providecommand{\nTMflairShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{nTMflairShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\nTMflairShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{nTMflairShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\nTMflairShiftLTwoVarDecoderSamLite}{\tbd{nTMflairShiftLTwoVarDecoderSamLite}}
\providecommand{\nTMflairShiftLTwoVarDecoderSamPretrained}{\tbd{nTMflairShiftLTwoVarDecoderSamPretrained}}
\providecommand{\nTMflairShiftLTwoVarDecoderSegformerMlp}{\tbd{nTMflairShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\nTMflairShiftLTwoVarFrozenEncoderTrue}{\tbd{nTMflairShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\nTMflairShiftLTwoVarLossBootstrap}{\tbd{nTMflairShiftLTwoVarLossBootstrap}}
\providecommand{\nTMflairShiftLTwoVarLossGce}{\tbd{nTMflairShiftLTwoVarLossGce}}
\providecommand{\nTMflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{nTMflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\nTMflairShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{nTMflairShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\nTMsenClean}{\tbd{nTMsenClean}}
\providecommand{\nTMsenOtsuLTwo}{\tbd{nTMsenOtsuLTwo}}
\providecommand{\nVitlRandomburnBoundaryLOneVarInitRandom}{\tbd{nVitlRandomburnBoundaryLOneVarInitRandom}}
\providecommand{\nVitlRandomburnBoundaryLTwoVarInitRandom}{\tbd{nVitlRandomburnBoundaryLTwoVarInitRandom}}
\providecommand{\nVitlRandomburnCleanVarInitRandom}{\tbd{nVitlRandomburnCleanVarInitRandom}}
\providecommand{\nVitlRandomburnCleanVarInitRandomLrMultOneZero}{\tbd{nVitlRandomburnCleanVarInitRandomLrMultOneZero}}
\providecommand{\nVitlRandomburnCleanVarInitRandomLrMultThree}{\tbd{nVitlRandomburnCleanVarInitRandomLrMultThree}}
\providecommand{\nVitlRandomburnCleanVarInitRandomTrainSubsetCleanTwoFive}{\tbd{nVitlRandomburnCleanVarInitRandomTrainSubsetCleanTwoFive}}
\providecommand{\nVitlRandomburnCoarseLOneVarInitRandom}{\tbd{nVitlRandomburnCoarseLOneVarInitRandom}}
\providecommand{\nVitlRandomburnCoarseLTwoVarInitRandom}{\tbd{nVitlRandomburnCoarseLTwoVarInitRandom}}
\providecommand{\nVitlRandomburnOmissionLOneVarInitRandom}{\tbd{nVitlRandomburnOmissionLOneVarInitRandom}}
\providecommand{\nVitlRandomburnOmissionLTwoVarInitRandom}{\tbd{nVitlRandomburnOmissionLTwoVarInitRandom}}
\providecommand{\nVitlRandomburnShiftLOneVarInitRandom}{\tbd{nVitlRandomburnShiftLOneVarInitRandom}}
\providecommand{\nVitlRandomburnShiftLTwoVarInitRandom}{\tbd{nVitlRandomburnShiftLTwoVarInitRandom}}
\providecommand{\nVitlRandomflairBoundaryLOneVarInitRandom}{\tbd{nVitlRandomflairBoundaryLOneVarInitRandom}}
\providecommand{\nVitlRandomflairBoundaryLTwoVarInitRandom}{\tbd{nVitlRandomflairBoundaryLTwoVarInitRandom}}
\providecommand{\nVitlRandomflairCleanVarInitRandom}{\tbd{nVitlRandomflairCleanVarInitRandom}}
\providecommand{\nVitlRandomflairCleanVarInitRandomLrMultOne}{\tbd{nVitlRandomflairCleanVarInitRandomLrMultOne}}
\providecommand{\nVitlRandomflairCleanVarInitRandomLrMultOneZero}{\tbd{nVitlRandomflairCleanVarInitRandomLrMultOneZero}}
\providecommand{\nVitlRandomflairCleanVarInitRandomTrainSubsetCleanTwoFive}{\tbd{nVitlRandomflairCleanVarInitRandomTrainSubsetCleanTwoFive}}
\providecommand{\nVitlRandomflairCoarseLOneVarInitRandom}{\tbd{nVitlRandomflairCoarseLOneVarInitRandom}}
\providecommand{\nVitlRandomflairCoarseLTwoVarInitRandom}{\tbd{nVitlRandomflairCoarseLTwoVarInitRandom}}
\providecommand{\nVitlRandomflairOmissionLOneVarInitRandom}{\tbd{nVitlRandomflairOmissionLOneVarInitRandom}}
\providecommand{\nVitlRandomflairOmissionLTwoVarInitRandom}{\tbd{nVitlRandomflairOmissionLTwoVarInitRandom}}
\providecommand{\nVitlRandomflairShiftLOneVarInitRandom}{\tbd{nVitlRandomflairShiftLOneVarInitRandom}}
\providecommand{\nVitlRandomflairShiftLTwoVarInitRandom}{\tbd{nVitlRandomflairShiftLTwoVarInitRandom}}
\providecommand{\retCIDOFAChesBoundaryLOne}{\tbd{retCIDOFAChesBoundaryLOne}}
\providecommand{\retCIDOFAChesBoundaryLTwo}{\tbd{retCIDOFAChesBoundaryLTwo}}
\providecommand{\retCIDOFAChesCoarseLOne}{\tbd{retCIDOFAChesCoarseLOne}}
\providecommand{\retCIDOFAChesCoarseLTwo}{\tbd{retCIDOFAChesCoarseLTwo}}
\providecommand{\retCIDOFAChesNlcdREAL}{\tbd{retCIDOFAChesNlcdREAL}}
\providecommand{\retCIDOFAChesOmissionLOne}{\tbd{retCIDOFAChesOmissionLOne}}
\providecommand{\retCIDOFAChesOmissionLTwo}{\tbd{retCIDOFAChesOmissionLTwo}}
\providecommand{\retCIDOFAChesShiftLOne}{\tbd{retCIDOFAChesShiftLOne}}
\providecommand{\retCIDOFAChesShiftLTwo}{\tbd{retCIDOFAChesShiftLTwo}}
\providecommand{\retCIDOFACsTwelveBoundaryLOne}{\tbd{retCIDOFACsTwelveBoundaryLOne}}
\providecommand{\retCIDOFACsTwelveBoundaryLTwo}{\tbd{retCIDOFACsTwelveBoundaryLTwo}}
\providecommand{\retCIDOFACsTwelveCoarseLOne}{\tbd{retCIDOFACsTwelveCoarseLOne}}
\providecommand{\retCIDOFACsTwelveCoarseLTwo}{\tbd{retCIDOFACsTwelveCoarseLTwo}}
\providecommand{\retCIDOFACsTwelveOmissionLOne}{\tbd{retCIDOFACsTwelveOmissionLOne}}
\providecommand{\retCIDOFACsTwelveOmissionLTwo}{\tbd{retCIDOFACsTwelveOmissionLTwo}}
\providecommand{\retCIDOFACsTwelveSTwocloudlessREAL}{\tbd{retCIDOFACsTwelveSTwocloudlessREAL}}
\providecommand{\retCIDOFACsTwelveShiftLOne}{\tbd{retCIDOFACsTwelveShiftLOne}}
\providecommand{\retCIDOFACsTwelveShiftLTwo}{\tbd{retCIDOFACsTwelveShiftLTwo}}
\providecommand{\retCIDOFADfcBoundaryLOne}{\tbd{retCIDOFADfcBoundaryLOne}}
\providecommand{\retCIDOFADfcBoundaryLTwo}{\tbd{retCIDOFADfcBoundaryLTwo}}
\providecommand{\retCIDOFADfcCoarseLOne}{\tbd{retCIDOFADfcCoarseLOne}}
\providecommand{\retCIDOFADfcCoarseLTwo}{\tbd{retCIDOFADfcCoarseLTwo}}
\providecommand{\retCIDOFADfcModisREALVarTrainSubsetRealcov}{\tbd{retCIDOFADfcModisREALVarTrainSubsetRealcov}}
\providecommand{\retCIDOFADfcOmissionLOne}{\tbd{retCIDOFADfcOmissionLOne}}
\providecommand{\retCIDOFADfcOmissionLTwo}{\tbd{retCIDOFADfcOmissionLTwo}}
\providecommand{\retCIDOFADfcShiftLOne}{\tbd{retCIDOFADfcShiftLOne}}
\providecommand{\retCIDOFADfcShiftLTwo}{\tbd{retCIDOFADfcShiftLTwo}}
\providecommand{\retCIDOFAEnvaBoundaryLOne}{\tbd{retCIDOFAEnvaBoundaryLOne}}
\providecommand{\retCIDOFAEnvaBoundaryLTwo}{\tbd{retCIDOFAEnvaBoundaryLTwo}}
\providecommand{\retCIDOFAEnvaCoarseLOne}{\tbd{retCIDOFAEnvaCoarseLOne}}
\providecommand{\retCIDOFAEnvaCoarseLTwo}{\tbd{retCIDOFAEnvaCoarseLTwo}}
\providecommand{\retCIDOFAEnvaNlcdREAL}{\tbd{retCIDOFAEnvaNlcdREAL}}
\providecommand{\retCIDOFAEnvaOmissionLOne}{\tbd{retCIDOFAEnvaOmissionLOne}}
\providecommand{\retCIDOFAEnvaOmissionLTwo}{\tbd{retCIDOFAEnvaOmissionLTwo}}
\providecommand{\retCIDOFAEnvaShiftLOne}{\tbd{retCIDOFAEnvaShiftLOne}}
\providecommand{\retCIDOFAEnvaShiftLTwo}{\tbd{retCIDOFAEnvaShiftLTwo}}
\providecommand{\retCIDOFAKuroBoundaryLOne}{\tbd{retCIDOFAKuroBoundaryLOne}}
\providecommand{\retCIDOFAKuroBoundaryLTwo}{\tbd{retCIDOFAKuroBoundaryLTwo}}
\providecommand{\retCIDOFAKuroCemsREALVarTrainSubsetRealcov}{\tbd{retCIDOFAKuroCemsREALVarTrainSubsetRealcov}}
\providecommand{\retCIDOFAKuroCoarseLOne}{\tbd{retCIDOFAKuroCoarseLOne}}
\providecommand{\retCIDOFAKuroCoarseLTwo}{\tbd{retCIDOFAKuroCoarseLTwo}}
\providecommand{\retCIDOFAKuroOmissionLOne}{\tbd{retCIDOFAKuroOmissionLOne}}
\providecommand{\retCIDOFAKuroOmissionLTwo}{\tbd{retCIDOFAKuroOmissionLTwo}}
\providecommand{\retCIDOFAKuroShiftLOne}{\tbd{retCIDOFAKuroShiftLOne}}
\providecommand{\retCIDOFAKuroShiftLTwo}{\tbd{retCIDOFAKuroShiftLTwo}}
\providecommand{\retCIDOFAOemBoundaryLOne}{\tbd{retCIDOFAOemBoundaryLOne}}
\providecommand{\retCIDOFAOemBoundaryLTwo}{\tbd{retCIDOFAOemBoundaryLTwo}}
\providecommand{\retCIDOFAOemCoarseLOne}{\tbd{retCIDOFAOemCoarseLOne}}
\providecommand{\retCIDOFAOemCoarseLTwo}{\tbd{retCIDOFAOemCoarseLTwo}}
\providecommand{\retCIDOFAOemOmissionLOne}{\tbd{retCIDOFAOemOmissionLOne}}
\providecommand{\retCIDOFAOemOmissionLTwo}{\tbd{retCIDOFAOemOmissionLTwo}}
\providecommand{\retCIDOFAOemShiftLOne}{\tbd{retCIDOFAOemShiftLOne}}
\providecommand{\retCIDOFAOemShiftLTwo}{\tbd{retCIDOFAOemShiftLTwo}}
\providecommand{\retCIDOFASnTwoBoundaryLOne}{\tbd{retCIDOFASnTwoBoundaryLOne}}
\providecommand{\retCIDOFASnTwoBoundaryLTwo}{\tbd{retCIDOFASnTwoBoundaryLTwo}}
\providecommand{\retCIDOFASnTwoCoarseLOne}{\tbd{retCIDOFASnTwoCoarseLOne}}
\providecommand{\retCIDOFASnTwoCoarseLTwo}{\tbd{retCIDOFASnTwoCoarseLTwo}}
\providecommand{\retCIDOFASnTwoOmissionLOne}{\tbd{retCIDOFASnTwoOmissionLOne}}
\providecommand{\retCIDOFASnTwoOmissionLTwo}{\tbd{retCIDOFASnTwoOmissionLTwo}}
\providecommand{\retCIDOFASnTwoShiftLOne}{\tbd{retCIDOFASnTwoShiftLOne}}
\providecommand{\retCIDOFASnTwoShiftLTwo}{\tbd{retCIDOFASnTwoShiftLTwo}}
\providecommand{\retCIDOFAburnBoundaryLOne}{\tbd{retCIDOFAburnBoundaryLOne}}
\providecommand{\retCIDOFAburnBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{retCIDOFAburnBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCIDOFAburnBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{retCIDOFAburnBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCIDOFAburnBoundaryLOneVarDecoderSamLite}{\tbd{retCIDOFAburnBoundaryLOneVarDecoderSamLite}}
\providecommand{\retCIDOFAburnBoundaryLOneVarDecoderSamPretrained}{\tbd{retCIDOFAburnBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\retCIDOFAburnBoundaryLOneVarDecoderSegformerMlp}{\tbd{retCIDOFAburnBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\retCIDOFAburnBoundaryLR}{\tbd{retCIDOFAburnBoundaryLR}}
\providecommand{\retCIDOFAburnBoundaryLTwo}{\tbd{retCIDOFAburnBoundaryLTwo}}
\providecommand{\retCIDOFAburnBoundaryLTwoVarBandsRgb}{\tbd{retCIDOFAburnBoundaryLTwoVarBandsRgb}}
\providecommand{\retCIDOFAburnBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{retCIDOFAburnBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCIDOFAburnBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retCIDOFAburnBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCIDOFAburnBoundaryLTwoVarDecoderSamLite}{\tbd{retCIDOFAburnBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retCIDOFAburnBoundaryLTwoVarDecoderSamPretrained}{\tbd{retCIDOFAburnBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\retCIDOFAburnBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retCIDOFAburnBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retCIDOFAburnBoundaryLTwoVarFrozenEncoderTrue}{\tbd{retCIDOFAburnBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\retCIDOFAburnBoundaryLTwoVarLossBootstrap}{\tbd{retCIDOFAburnBoundaryLTwoVarLossBootstrap}}
\providecommand{\retCIDOFAburnBoundaryLTwoVarLossGce}{\tbd{retCIDOFAburnBoundaryLTwoVarLossGce}}
\providecommand{\retCIDOFAburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCIDOFAburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCIDOFAburnBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCIDOFAburnBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCIDOFAburnCoarseLOne}{\tbd{retCIDOFAburnCoarseLOne}}
\providecommand{\retCIDOFAburnCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{retCIDOFAburnCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCIDOFAburnCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{retCIDOFAburnCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCIDOFAburnCoarseLOneVarDecoderSamLite}{\tbd{retCIDOFAburnCoarseLOneVarDecoderSamLite}}
\providecommand{\retCIDOFAburnCoarseLOneVarDecoderSamPretrained}{\tbd{retCIDOFAburnCoarseLOneVarDecoderSamPretrained}}
\providecommand{\retCIDOFAburnCoarseLOneVarDecoderSegformerMlp}{\tbd{retCIDOFAburnCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\retCIDOFAburnCoarseLR}{\tbd{retCIDOFAburnCoarseLR}}
\providecommand{\retCIDOFAburnCoarseLTwo}{\tbd{retCIDOFAburnCoarseLTwo}}
\providecommand{\retCIDOFAburnCoarseLTwoVarBandsRgb}{\tbd{retCIDOFAburnCoarseLTwoVarBandsRgb}}
\providecommand{\retCIDOFAburnCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{retCIDOFAburnCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCIDOFAburnCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retCIDOFAburnCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCIDOFAburnCoarseLTwoVarDecoderSamLite}{\tbd{retCIDOFAburnCoarseLTwoVarDecoderSamLite}}
\providecommand{\retCIDOFAburnCoarseLTwoVarDecoderSamPretrained}{\tbd{retCIDOFAburnCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\retCIDOFAburnCoarseLTwoVarDecoderSegformerMlp}{\tbd{retCIDOFAburnCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retCIDOFAburnCoarseLTwoVarFrozenEncoderTrue}{\tbd{retCIDOFAburnCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\retCIDOFAburnCoarseLTwoVarLossBootstrap}{\tbd{retCIDOFAburnCoarseLTwoVarLossBootstrap}}
\providecommand{\retCIDOFAburnCoarseLTwoVarLossGce}{\tbd{retCIDOFAburnCoarseLTwoVarLossGce}}
\providecommand{\retCIDOFAburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCIDOFAburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCIDOFAburnCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCIDOFAburnCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCIDOFAburnOmissionLOne}{\tbd{retCIDOFAburnOmissionLOne}}
\providecommand{\retCIDOFAburnOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{retCIDOFAburnOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCIDOFAburnOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{retCIDOFAburnOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCIDOFAburnOmissionLOneVarDecoderSamLite}{\tbd{retCIDOFAburnOmissionLOneVarDecoderSamLite}}
\providecommand{\retCIDOFAburnOmissionLOneVarDecoderSamPretrained}{\tbd{retCIDOFAburnOmissionLOneVarDecoderSamPretrained}}
\providecommand{\retCIDOFAburnOmissionLOneVarDecoderSegformerMlp}{\tbd{retCIDOFAburnOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\retCIDOFAburnOmissionLR}{\tbd{retCIDOFAburnOmissionLR}}
\providecommand{\retCIDOFAburnOmissionLTwo}{\tbd{retCIDOFAburnOmissionLTwo}}
\providecommand{\retCIDOFAburnOmissionLTwoVarBandsRgb}{\tbd{retCIDOFAburnOmissionLTwoVarBandsRgb}}
\providecommand{\retCIDOFAburnOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{retCIDOFAburnOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCIDOFAburnOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retCIDOFAburnOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCIDOFAburnOmissionLTwoVarDecoderSamLite}{\tbd{retCIDOFAburnOmissionLTwoVarDecoderSamLite}}
\providecommand{\retCIDOFAburnOmissionLTwoVarDecoderSamPretrained}{\tbd{retCIDOFAburnOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\retCIDOFAburnOmissionLTwoVarDecoderSegformerMlp}{\tbd{retCIDOFAburnOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retCIDOFAburnOmissionLTwoVarFrozenEncoderTrue}{\tbd{retCIDOFAburnOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\retCIDOFAburnOmissionLTwoVarLossBootstrap}{\tbd{retCIDOFAburnOmissionLTwoVarLossBootstrap}}
\providecommand{\retCIDOFAburnOmissionLTwoVarLossGce}{\tbd{retCIDOFAburnOmissionLTwoVarLossGce}}
\providecommand{\retCIDOFAburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCIDOFAburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCIDOFAburnOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCIDOFAburnOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCIDOFAburnShiftLOne}{\tbd{retCIDOFAburnShiftLOne}}
\providecommand{\retCIDOFAburnShiftLOneVarDecoderMaskTwoformerFull}{\tbd{retCIDOFAburnShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCIDOFAburnShiftLOneVarDecoderMaskTwoformerLite}{\tbd{retCIDOFAburnShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCIDOFAburnShiftLOneVarDecoderSamLite}{\tbd{retCIDOFAburnShiftLOneVarDecoderSamLite}}
\providecommand{\retCIDOFAburnShiftLOneVarDecoderSamPretrained}{\tbd{retCIDOFAburnShiftLOneVarDecoderSamPretrained}}
\providecommand{\retCIDOFAburnShiftLOneVarDecoderSegformerMlp}{\tbd{retCIDOFAburnShiftLOneVarDecoderSegformerMlp}}
\providecommand{\retCIDOFAburnShiftLR}{\tbd{retCIDOFAburnShiftLR}}
\providecommand{\retCIDOFAburnShiftLTwo}{\tbd{retCIDOFAburnShiftLTwo}}
\providecommand{\retCIDOFAburnShiftLTwoVarBandsRgb}{\tbd{retCIDOFAburnShiftLTwoVarBandsRgb}}
\providecommand{\retCIDOFAburnShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{retCIDOFAburnShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCIDOFAburnShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retCIDOFAburnShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCIDOFAburnShiftLTwoVarDecoderSamLite}{\tbd{retCIDOFAburnShiftLTwoVarDecoderSamLite}}
\providecommand{\retCIDOFAburnShiftLTwoVarDecoderSamPretrained}{\tbd{retCIDOFAburnShiftLTwoVarDecoderSamPretrained}}
\providecommand{\retCIDOFAburnShiftLTwoVarDecoderSegformerMlp}{\tbd{retCIDOFAburnShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retCIDOFAburnShiftLTwoVarFrozenEncoderTrue}{\tbd{retCIDOFAburnShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\retCIDOFAburnShiftLTwoVarLossBootstrap}{\tbd{retCIDOFAburnShiftLTwoVarLossBootstrap}}
\providecommand{\retCIDOFAburnShiftLTwoVarLossGce}{\tbd{retCIDOFAburnShiftLTwoVarLossGce}}
\providecommand{\retCIDOFAburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCIDOFAburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCIDOFAburnShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCIDOFAburnShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCIDOFAflairBoundaryLOne}{\tbd{retCIDOFAflairBoundaryLOne}}
\providecommand{\retCIDOFAflairBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{retCIDOFAflairBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCIDOFAflairBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{retCIDOFAflairBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCIDOFAflairBoundaryLOneVarDecoderSamLite}{\tbd{retCIDOFAflairBoundaryLOneVarDecoderSamLite}}
\providecommand{\retCIDOFAflairBoundaryLOneVarDecoderSamPretrained}{\tbd{retCIDOFAflairBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\retCIDOFAflairBoundaryLOneVarDecoderSegformerMlp}{\tbd{retCIDOFAflairBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\retCIDOFAflairBoundaryLR}{\tbd{retCIDOFAflairBoundaryLR}}
\providecommand{\retCIDOFAflairBoundaryLTwo}{\tbd{retCIDOFAflairBoundaryLTwo}}
\providecommand{\retCIDOFAflairBoundaryLTwoVarBandsRgb}{\tbd{retCIDOFAflairBoundaryLTwoVarBandsRgb}}
\providecommand{\retCIDOFAflairBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{retCIDOFAflairBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCIDOFAflairBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retCIDOFAflairBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCIDOFAflairBoundaryLTwoVarDecoderSamLite}{\tbd{retCIDOFAflairBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retCIDOFAflairBoundaryLTwoVarDecoderSamPretrained}{\tbd{retCIDOFAflairBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\retCIDOFAflairBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retCIDOFAflairBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retCIDOFAflairBoundaryLTwoVarFrozenEncoderTrue}{\tbd{retCIDOFAflairBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\retCIDOFAflairBoundaryLTwoVarLossBootstrap}{\tbd{retCIDOFAflairBoundaryLTwoVarLossBootstrap}}
\providecommand{\retCIDOFAflairBoundaryLTwoVarLossGce}{\tbd{retCIDOFAflairBoundaryLTwoVarLossGce}}
\providecommand{\retCIDOFAflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCIDOFAflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCIDOFAflairBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCIDOFAflairBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCIDOFAflairCoarseLOne}{\tbd{retCIDOFAflairCoarseLOne}}
\providecommand{\retCIDOFAflairCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{retCIDOFAflairCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCIDOFAflairCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{retCIDOFAflairCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCIDOFAflairCoarseLOneVarDecoderSamLite}{\tbd{retCIDOFAflairCoarseLOneVarDecoderSamLite}}
\providecommand{\retCIDOFAflairCoarseLOneVarDecoderSamPretrained}{\tbd{retCIDOFAflairCoarseLOneVarDecoderSamPretrained}}
\providecommand{\retCIDOFAflairCoarseLOneVarDecoderSegformerMlp}{\tbd{retCIDOFAflairCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\retCIDOFAflairCoarseLR}{\tbd{retCIDOFAflairCoarseLR}}
\providecommand{\retCIDOFAflairCoarseLTwo}{\tbd{retCIDOFAflairCoarseLTwo}}
\providecommand{\retCIDOFAflairCoarseLTwoVarBandsRgb}{\tbd{retCIDOFAflairCoarseLTwoVarBandsRgb}}
\providecommand{\retCIDOFAflairCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{retCIDOFAflairCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCIDOFAflairCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retCIDOFAflairCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCIDOFAflairCoarseLTwoVarDecoderSamLite}{\tbd{retCIDOFAflairCoarseLTwoVarDecoderSamLite}}
\providecommand{\retCIDOFAflairCoarseLTwoVarDecoderSamPretrained}{\tbd{retCIDOFAflairCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\retCIDOFAflairCoarseLTwoVarDecoderSegformerMlp}{\tbd{retCIDOFAflairCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retCIDOFAflairCoarseLTwoVarFrozenEncoderTrue}{\tbd{retCIDOFAflairCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\retCIDOFAflairCoarseLTwoVarLossBootstrap}{\tbd{retCIDOFAflairCoarseLTwoVarLossBootstrap}}
\providecommand{\retCIDOFAflairCoarseLTwoVarLossGce}{\tbd{retCIDOFAflairCoarseLTwoVarLossGce}}
\providecommand{\retCIDOFAflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCIDOFAflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCIDOFAflairCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCIDOFAflairCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCIDOFAflairOmissionLOne}{\tbd{retCIDOFAflairOmissionLOne}}
\providecommand{\retCIDOFAflairOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{retCIDOFAflairOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCIDOFAflairOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{retCIDOFAflairOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCIDOFAflairOmissionLOneVarDecoderSamLite}{\tbd{retCIDOFAflairOmissionLOneVarDecoderSamLite}}
\providecommand{\retCIDOFAflairOmissionLOneVarDecoderSamPretrained}{\tbd{retCIDOFAflairOmissionLOneVarDecoderSamPretrained}}
\providecommand{\retCIDOFAflairOmissionLOneVarDecoderSegformerMlp}{\tbd{retCIDOFAflairOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\retCIDOFAflairOmissionLR}{\tbd{retCIDOFAflairOmissionLR}}
\providecommand{\retCIDOFAflairOmissionLTwo}{\tbd{retCIDOFAflairOmissionLTwo}}
\providecommand{\retCIDOFAflairOmissionLTwoVarBandsRgb}{\tbd{retCIDOFAflairOmissionLTwoVarBandsRgb}}
\providecommand{\retCIDOFAflairOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{retCIDOFAflairOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCIDOFAflairOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retCIDOFAflairOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCIDOFAflairOmissionLTwoVarDecoderSamLite}{\tbd{retCIDOFAflairOmissionLTwoVarDecoderSamLite}}
\providecommand{\retCIDOFAflairOmissionLTwoVarDecoderSamPretrained}{\tbd{retCIDOFAflairOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\retCIDOFAflairOmissionLTwoVarDecoderSegformerMlp}{\tbd{retCIDOFAflairOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retCIDOFAflairOmissionLTwoVarFrozenEncoderTrue}{\tbd{retCIDOFAflairOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\retCIDOFAflairOmissionLTwoVarLossBootstrap}{\tbd{retCIDOFAflairOmissionLTwoVarLossBootstrap}}
\providecommand{\retCIDOFAflairOmissionLTwoVarLossGce}{\tbd{retCIDOFAflairOmissionLTwoVarLossGce}}
\providecommand{\retCIDOFAflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCIDOFAflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCIDOFAflairOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCIDOFAflairOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCIDOFAflairShiftLOne}{\tbd{retCIDOFAflairShiftLOne}}
\providecommand{\retCIDOFAflairShiftLOneVarDecoderMaskTwoformerFull}{\tbd{retCIDOFAflairShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCIDOFAflairShiftLOneVarDecoderMaskTwoformerLite}{\tbd{retCIDOFAflairShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCIDOFAflairShiftLOneVarDecoderSamLite}{\tbd{retCIDOFAflairShiftLOneVarDecoderSamLite}}
\providecommand{\retCIDOFAflairShiftLOneVarDecoderSamPretrained}{\tbd{retCIDOFAflairShiftLOneVarDecoderSamPretrained}}
\providecommand{\retCIDOFAflairShiftLOneVarDecoderSegformerMlp}{\tbd{retCIDOFAflairShiftLOneVarDecoderSegformerMlp}}
\providecommand{\retCIDOFAflairShiftLR}{\tbd{retCIDOFAflairShiftLR}}
\providecommand{\retCIDOFAflairShiftLTwo}{\tbd{retCIDOFAflairShiftLTwo}}
\providecommand{\retCIDOFAflairShiftLTwoVarBandsRgb}{\tbd{retCIDOFAflairShiftLTwoVarBandsRgb}}
\providecommand{\retCIDOFAflairShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{retCIDOFAflairShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCIDOFAflairShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retCIDOFAflairShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCIDOFAflairShiftLTwoVarDecoderSamLite}{\tbd{retCIDOFAflairShiftLTwoVarDecoderSamLite}}
\providecommand{\retCIDOFAflairShiftLTwoVarDecoderSamPretrained}{\tbd{retCIDOFAflairShiftLTwoVarDecoderSamPretrained}}
\providecommand{\retCIDOFAflairShiftLTwoVarDecoderSegformerMlp}{\tbd{retCIDOFAflairShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retCIDOFAflairShiftLTwoVarFrozenEncoderTrue}{\tbd{retCIDOFAflairShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\retCIDOFAflairShiftLTwoVarLossBootstrap}{\tbd{retCIDOFAflairShiftLTwoVarLossBootstrap}}
\providecommand{\retCIDOFAflairShiftLTwoVarLossGce}{\tbd{retCIDOFAflairShiftLTwoVarLossGce}}
\providecommand{\retCIDOFAflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCIDOFAflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCIDOFAflairShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCIDOFAflairShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCIDOFAsenOtsuLTwo}{\tbd{retCIDOFAsenOtsuLTwo}}
\providecommand{\retCIDinovThreeConvnextLburnBoundaryLOne}{\tbd{retCIDinovThreeConvnextLburnBoundaryLOne}}
\providecommand{\retCIDinovThreeConvnextLburnBoundaryLTwo}{\tbd{retCIDinovThreeConvnextLburnBoundaryLTwo}}
\providecommand{\retCIDinovThreeConvnextLburnCoarseLOne}{\tbd{retCIDinovThreeConvnextLburnCoarseLOne}}
\providecommand{\retCIDinovThreeConvnextLburnCoarseLTwo}{\tbd{retCIDinovThreeConvnextLburnCoarseLTwo}}
\providecommand{\retCIDinovThreeConvnextLburnOmissionLOne}{\tbd{retCIDinovThreeConvnextLburnOmissionLOne}}
\providecommand{\retCIDinovThreeConvnextLburnOmissionLTwo}{\tbd{retCIDinovThreeConvnextLburnOmissionLTwo}}
\providecommand{\retCIDinovThreeConvnextLburnShiftLOne}{\tbd{retCIDinovThreeConvnextLburnShiftLOne}}
\providecommand{\retCIDinovThreeConvnextLburnShiftLTwo}{\tbd{retCIDinovThreeConvnextLburnShiftLTwo}}
\providecommand{\retCIDinovThreeConvnextLflairBoundaryLOne}{\tbd{retCIDinovThreeConvnextLflairBoundaryLOne}}
\providecommand{\retCIDinovThreeConvnextLflairBoundaryLTwo}{\tbd{retCIDinovThreeConvnextLflairBoundaryLTwo}}
\providecommand{\retCIDinovThreeConvnextLflairCoarseLOne}{\tbd{retCIDinovThreeConvnextLflairCoarseLOne}}
\providecommand{\retCIDinovThreeConvnextLflairCoarseLTwo}{\tbd{retCIDinovThreeConvnextLflairCoarseLTwo}}
\providecommand{\retCIDinovThreeConvnextLflairOmissionLOne}{\tbd{retCIDinovThreeConvnextLflairOmissionLOne}}
\providecommand{\retCIDinovThreeConvnextLflairOmissionLTwo}{\tbd{retCIDinovThreeConvnextLflairOmissionLTwo}}
\providecommand{\retCIDinovThreeConvnextLflairShiftLOne}{\tbd{retCIDinovThreeConvnextLflairShiftLOne}}
\providecommand{\retCIDinovThreeConvnextLflairShiftLTwo}{\tbd{retCIDinovThreeConvnextLflairShiftLTwo}}
\providecommand{\retCILVDChesBoundaryLOne}{\tbd{retCILVDChesBoundaryLOne}}
\providecommand{\retCILVDChesBoundaryLTwo}{\tbd{retCILVDChesBoundaryLTwo}}
\providecommand{\retCILVDChesBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retCILVDChesBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDChesBoundaryLTwoVarDecoderSamLite}{\tbd{retCILVDChesBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retCILVDChesBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retCILVDChesBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retCILVDChesBoundaryLTwoVarLrMultOne}{\tbd{retCILVDChesBoundaryLTwoVarLrMultOne}}
\providecommand{\retCILVDChesCoarseLOne}{\tbd{retCILVDChesCoarseLOne}}
\providecommand{\retCILVDChesCoarseLTwo}{\tbd{retCILVDChesCoarseLTwo}}
\providecommand{\retCILVDChesCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retCILVDChesCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDChesCoarseLTwoVarDecoderSamLite}{\tbd{retCILVDChesCoarseLTwoVarDecoderSamLite}}
\providecommand{\retCILVDChesCoarseLTwoVarDecoderSegformerMlp}{\tbd{retCILVDChesCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retCILVDChesCoarseLTwoVarLrMultOne}{\tbd{retCILVDChesCoarseLTwoVarLrMultOne}}
\providecommand{\retCILVDChesNlcdREAL}{\tbd{retCILVDChesNlcdREAL}}
\providecommand{\retCILVDChesOmissionLOne}{\tbd{retCILVDChesOmissionLOne}}
\providecommand{\retCILVDChesOmissionLTwo}{\tbd{retCILVDChesOmissionLTwo}}
\providecommand{\retCILVDChesOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retCILVDChesOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDChesOmissionLTwoVarDecoderSamLite}{\tbd{retCILVDChesOmissionLTwoVarDecoderSamLite}}
\providecommand{\retCILVDChesOmissionLTwoVarDecoderSegformerMlp}{\tbd{retCILVDChesOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retCILVDChesOmissionLTwoVarLrMultOne}{\tbd{retCILVDChesOmissionLTwoVarLrMultOne}}
\providecommand{\retCILVDChesShiftLOne}{\tbd{retCILVDChesShiftLOne}}
\providecommand{\retCILVDChesShiftLTwo}{\tbd{retCILVDChesShiftLTwo}}
\providecommand{\retCILVDChesShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retCILVDChesShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDChesShiftLTwoVarDecoderSamLite}{\tbd{retCILVDChesShiftLTwoVarDecoderSamLite}}
\providecommand{\retCILVDChesShiftLTwoVarDecoderSegformerMlp}{\tbd{retCILVDChesShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retCILVDChesShiftLTwoVarLrMultOne}{\tbd{retCILVDChesShiftLTwoVarLrMultOne}}
\providecommand{\retCILVDCsTwelveBoundaryLOne}{\tbd{retCILVDCsTwelveBoundaryLOne}}
\providecommand{\retCILVDCsTwelveBoundaryLTwo}{\tbd{retCILVDCsTwelveBoundaryLTwo}}
\providecommand{\retCILVDCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retCILVDCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDCsTwelveBoundaryLTwoVarDecoderSamLite}{\tbd{retCILVDCsTwelveBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retCILVDCsTwelveBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retCILVDCsTwelveBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retCILVDCsTwelveBoundaryLTwoVarLrMultOne}{\tbd{retCILVDCsTwelveBoundaryLTwoVarLrMultOne}}
\providecommand{\retCILVDCsTwelveCoarseLOne}{\tbd{retCILVDCsTwelveCoarseLOne}}
\providecommand{\retCILVDCsTwelveCoarseLTwo}{\tbd{retCILVDCsTwelveCoarseLTwo}}
\providecommand{\retCILVDCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retCILVDCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDCsTwelveCoarseLTwoVarDecoderSamLite}{\tbd{retCILVDCsTwelveCoarseLTwoVarDecoderSamLite}}
\providecommand{\retCILVDCsTwelveCoarseLTwoVarDecoderSegformerMlp}{\tbd{retCILVDCsTwelveCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retCILVDCsTwelveCoarseLTwoVarLrMultOne}{\tbd{retCILVDCsTwelveCoarseLTwoVarLrMultOne}}
\providecommand{\retCILVDCsTwelveOmissionLOne}{\tbd{retCILVDCsTwelveOmissionLOne}}
\providecommand{\retCILVDCsTwelveOmissionLTwo}{\tbd{retCILVDCsTwelveOmissionLTwo}}
\providecommand{\retCILVDCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retCILVDCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDCsTwelveOmissionLTwoVarDecoderSamLite}{\tbd{retCILVDCsTwelveOmissionLTwoVarDecoderSamLite}}
\providecommand{\retCILVDCsTwelveOmissionLTwoVarDecoderSegformerMlp}{\tbd{retCILVDCsTwelveOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retCILVDCsTwelveOmissionLTwoVarLrMultOne}{\tbd{retCILVDCsTwelveOmissionLTwoVarLrMultOne}}
\providecommand{\retCILVDCsTwelveSTwocloudlessREAL}{\tbd{retCILVDCsTwelveSTwocloudlessREAL}}
\providecommand{\retCILVDCsTwelveShiftLOne}{\tbd{retCILVDCsTwelveShiftLOne}}
\providecommand{\retCILVDCsTwelveShiftLTwo}{\tbd{retCILVDCsTwelveShiftLTwo}}
\providecommand{\retCILVDCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retCILVDCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDCsTwelveShiftLTwoVarDecoderSamLite}{\tbd{retCILVDCsTwelveShiftLTwoVarDecoderSamLite}}
\providecommand{\retCILVDCsTwelveShiftLTwoVarDecoderSegformerMlp}{\tbd{retCILVDCsTwelveShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retCILVDCsTwelveShiftLTwoVarLrMultOne}{\tbd{retCILVDCsTwelveShiftLTwoVarLrMultOne}}
\providecommand{\retCILVDDfcBoundaryLOne}{\tbd{retCILVDDfcBoundaryLOne}}
\providecommand{\retCILVDDfcBoundaryLTwo}{\tbd{retCILVDDfcBoundaryLTwo}}
\providecommand{\retCILVDDfcBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retCILVDDfcBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDDfcBoundaryLTwoVarDecoderSamLite}{\tbd{retCILVDDfcBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retCILVDDfcBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retCILVDDfcBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retCILVDDfcBoundaryLTwoVarLrMultOne}{\tbd{retCILVDDfcBoundaryLTwoVarLrMultOne}}
\providecommand{\retCILVDDfcCoarseLOne}{\tbd{retCILVDDfcCoarseLOne}}
\providecommand{\retCILVDDfcCoarseLTwo}{\tbd{retCILVDDfcCoarseLTwo}}
\providecommand{\retCILVDDfcCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retCILVDDfcCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDDfcCoarseLTwoVarDecoderSamLite}{\tbd{retCILVDDfcCoarseLTwoVarDecoderSamLite}}
\providecommand{\retCILVDDfcCoarseLTwoVarDecoderSegformerMlp}{\tbd{retCILVDDfcCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retCILVDDfcCoarseLTwoVarLrMultOne}{\tbd{retCILVDDfcCoarseLTwoVarLrMultOne}}
\providecommand{\retCILVDDfcModisREALVarTrainSubsetRealcov}{\tbd{retCILVDDfcModisREALVarTrainSubsetRealcov}}
\providecommand{\retCILVDDfcOmissionLOne}{\tbd{retCILVDDfcOmissionLOne}}
\providecommand{\retCILVDDfcOmissionLTwo}{\tbd{retCILVDDfcOmissionLTwo}}
\providecommand{\retCILVDDfcOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retCILVDDfcOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDDfcOmissionLTwoVarDecoderSamLite}{\tbd{retCILVDDfcOmissionLTwoVarDecoderSamLite}}
\providecommand{\retCILVDDfcOmissionLTwoVarDecoderSegformerMlp}{\tbd{retCILVDDfcOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retCILVDDfcOmissionLTwoVarLrMultOne}{\tbd{retCILVDDfcOmissionLTwoVarLrMultOne}}
\providecommand{\retCILVDDfcShiftLOne}{\tbd{retCILVDDfcShiftLOne}}
\providecommand{\retCILVDDfcShiftLTwo}{\tbd{retCILVDDfcShiftLTwo}}
\providecommand{\retCILVDDfcShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retCILVDDfcShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDDfcShiftLTwoVarDecoderSamLite}{\tbd{retCILVDDfcShiftLTwoVarDecoderSamLite}}
\providecommand{\retCILVDDfcShiftLTwoVarDecoderSegformerMlp}{\tbd{retCILVDDfcShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retCILVDDfcShiftLTwoVarLrMultOne}{\tbd{retCILVDDfcShiftLTwoVarLrMultOne}}
\providecommand{\retCILVDEnvaBoundaryLOne}{\tbd{retCILVDEnvaBoundaryLOne}}
\providecommand{\retCILVDEnvaBoundaryLTwo}{\tbd{retCILVDEnvaBoundaryLTwo}}
\providecommand{\retCILVDEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retCILVDEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDEnvaBoundaryLTwoVarDecoderSamLite}{\tbd{retCILVDEnvaBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retCILVDEnvaBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retCILVDEnvaBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retCILVDEnvaBoundaryLTwoVarLrMultOne}{\tbd{retCILVDEnvaBoundaryLTwoVarLrMultOne}}
\providecommand{\retCILVDEnvaCoarseLOne}{\tbd{retCILVDEnvaCoarseLOne}}
\providecommand{\retCILVDEnvaCoarseLTwo}{\tbd{retCILVDEnvaCoarseLTwo}}
\providecommand{\retCILVDEnvaCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retCILVDEnvaCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDEnvaCoarseLTwoVarDecoderSamLite}{\tbd{retCILVDEnvaCoarseLTwoVarDecoderSamLite}}
\providecommand{\retCILVDEnvaCoarseLTwoVarDecoderSegformerMlp}{\tbd{retCILVDEnvaCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retCILVDEnvaCoarseLTwoVarLrMultOne}{\tbd{retCILVDEnvaCoarseLTwoVarLrMultOne}}
\providecommand{\retCILVDEnvaNlcdREAL}{\tbd{retCILVDEnvaNlcdREAL}}
\providecommand{\retCILVDEnvaOmissionLOne}{\tbd{retCILVDEnvaOmissionLOne}}
\providecommand{\retCILVDEnvaOmissionLTwo}{\tbd{retCILVDEnvaOmissionLTwo}}
\providecommand{\retCILVDEnvaOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retCILVDEnvaOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDEnvaOmissionLTwoVarDecoderSamLite}{\tbd{retCILVDEnvaOmissionLTwoVarDecoderSamLite}}
\providecommand{\retCILVDEnvaOmissionLTwoVarDecoderSegformerMlp}{\tbd{retCILVDEnvaOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retCILVDEnvaOmissionLTwoVarLrMultOne}{\tbd{retCILVDEnvaOmissionLTwoVarLrMultOne}}
\providecommand{\retCILVDEnvaShiftLOne}{\tbd{retCILVDEnvaShiftLOne}}
\providecommand{\retCILVDEnvaShiftLTwo}{\tbd{retCILVDEnvaShiftLTwo}}
\providecommand{\retCILVDEnvaShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retCILVDEnvaShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDEnvaShiftLTwoVarDecoderSamLite}{\tbd{retCILVDEnvaShiftLTwoVarDecoderSamLite}}
\providecommand{\retCILVDEnvaShiftLTwoVarDecoderSegformerMlp}{\tbd{retCILVDEnvaShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retCILVDEnvaShiftLTwoVarLrMultOne}{\tbd{retCILVDEnvaShiftLTwoVarLrMultOne}}
\providecommand{\retCILVDKuroBoundaryLOne}{\tbd{retCILVDKuroBoundaryLOne}}
\providecommand{\retCILVDKuroBoundaryLTwo}{\tbd{retCILVDKuroBoundaryLTwo}}
\providecommand{\retCILVDKuroBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retCILVDKuroBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDKuroBoundaryLTwoVarDecoderSamLite}{\tbd{retCILVDKuroBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retCILVDKuroBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retCILVDKuroBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retCILVDKuroBoundaryLTwoVarLrMultOne}{\tbd{retCILVDKuroBoundaryLTwoVarLrMultOne}}
\providecommand{\retCILVDKuroCemsREALVarTrainSubsetRealcov}{\tbd{retCILVDKuroCemsREALVarTrainSubsetRealcov}}
\providecommand{\retCILVDKuroCoarseLOne}{\tbd{retCILVDKuroCoarseLOne}}
\providecommand{\retCILVDKuroCoarseLTwo}{\tbd{retCILVDKuroCoarseLTwo}}
\providecommand{\retCILVDKuroCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retCILVDKuroCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDKuroCoarseLTwoVarDecoderSamLite}{\tbd{retCILVDKuroCoarseLTwoVarDecoderSamLite}}
\providecommand{\retCILVDKuroCoarseLTwoVarDecoderSegformerMlp}{\tbd{retCILVDKuroCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retCILVDKuroCoarseLTwoVarLrMultOne}{\tbd{retCILVDKuroCoarseLTwoVarLrMultOne}}
\providecommand{\retCILVDKuroOmissionLOne}{\tbd{retCILVDKuroOmissionLOne}}
\providecommand{\retCILVDKuroOmissionLTwo}{\tbd{retCILVDKuroOmissionLTwo}}
\providecommand{\retCILVDKuroOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retCILVDKuroOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDKuroOmissionLTwoVarDecoderSamLite}{\tbd{retCILVDKuroOmissionLTwoVarDecoderSamLite}}
\providecommand{\retCILVDKuroOmissionLTwoVarDecoderSegformerMlp}{\tbd{retCILVDKuroOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retCILVDKuroOmissionLTwoVarLrMultOne}{\tbd{retCILVDKuroOmissionLTwoVarLrMultOne}}
\providecommand{\retCILVDKuroShiftLOne}{\tbd{retCILVDKuroShiftLOne}}
\providecommand{\retCILVDKuroShiftLTwo}{\tbd{retCILVDKuroShiftLTwo}}
\providecommand{\retCILVDKuroShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retCILVDKuroShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDKuroShiftLTwoVarDecoderSamLite}{\tbd{retCILVDKuroShiftLTwoVarDecoderSamLite}}
\providecommand{\retCILVDKuroShiftLTwoVarDecoderSegformerMlp}{\tbd{retCILVDKuroShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retCILVDKuroShiftLTwoVarLrMultOne}{\tbd{retCILVDKuroShiftLTwoVarLrMultOne}}
\providecommand{\retCILVDOemBoundaryLOne}{\tbd{retCILVDOemBoundaryLOne}}
\providecommand{\retCILVDOemBoundaryLTwo}{\tbd{retCILVDOemBoundaryLTwo}}
\providecommand{\retCILVDOemBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retCILVDOemBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDOemBoundaryLTwoVarDecoderSamLite}{\tbd{retCILVDOemBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retCILVDOemBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retCILVDOemBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retCILVDOemBoundaryLTwoVarLrMultOne}{\tbd{retCILVDOemBoundaryLTwoVarLrMultOne}}
\providecommand{\retCILVDOemCoarseLOne}{\tbd{retCILVDOemCoarseLOne}}
\providecommand{\retCILVDOemCoarseLTwo}{\tbd{retCILVDOemCoarseLTwo}}
\providecommand{\retCILVDOemCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retCILVDOemCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDOemCoarseLTwoVarDecoderSamLite}{\tbd{retCILVDOemCoarseLTwoVarDecoderSamLite}}
\providecommand{\retCILVDOemCoarseLTwoVarDecoderSegformerMlp}{\tbd{retCILVDOemCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retCILVDOemCoarseLTwoVarLrMultOne}{\tbd{retCILVDOemCoarseLTwoVarLrMultOne}}
\providecommand{\retCILVDOemOmissionLOne}{\tbd{retCILVDOemOmissionLOne}}
\providecommand{\retCILVDOemOmissionLTwo}{\tbd{retCILVDOemOmissionLTwo}}
\providecommand{\retCILVDOemOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retCILVDOemOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDOemOmissionLTwoVarDecoderSamLite}{\tbd{retCILVDOemOmissionLTwoVarDecoderSamLite}}
\providecommand{\retCILVDOemOmissionLTwoVarDecoderSegformerMlp}{\tbd{retCILVDOemOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retCILVDOemOmissionLTwoVarLrMultOne}{\tbd{retCILVDOemOmissionLTwoVarLrMultOne}}
\providecommand{\retCILVDOemShiftLOne}{\tbd{retCILVDOemShiftLOne}}
\providecommand{\retCILVDOemShiftLTwo}{\tbd{retCILVDOemShiftLTwo}}
\providecommand{\retCILVDOemShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retCILVDOemShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDOemShiftLTwoVarDecoderSamLite}{\tbd{retCILVDOemShiftLTwoVarDecoderSamLite}}
\providecommand{\retCILVDOemShiftLTwoVarDecoderSegformerMlp}{\tbd{retCILVDOemShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retCILVDOemShiftLTwoVarLrMultOne}{\tbd{retCILVDOemShiftLTwoVarLrMultOne}}
\providecommand{\retCILVDSnTwoBoundaryLOne}{\tbd{retCILVDSnTwoBoundaryLOne}}
\providecommand{\retCILVDSnTwoBoundaryLTwo}{\tbd{retCILVDSnTwoBoundaryLTwo}}
\providecommand{\retCILVDSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retCILVDSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDSnTwoBoundaryLTwoVarDecoderSamLite}{\tbd{retCILVDSnTwoBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retCILVDSnTwoBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retCILVDSnTwoBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retCILVDSnTwoBoundaryLTwoVarLrMultOne}{\tbd{retCILVDSnTwoBoundaryLTwoVarLrMultOne}}
\providecommand{\retCILVDSnTwoCoarseLOne}{\tbd{retCILVDSnTwoCoarseLOne}}
\providecommand{\retCILVDSnTwoCoarseLTwo}{\tbd{retCILVDSnTwoCoarseLTwo}}
\providecommand{\retCILVDSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retCILVDSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDSnTwoCoarseLTwoVarDecoderSamLite}{\tbd{retCILVDSnTwoCoarseLTwoVarDecoderSamLite}}
\providecommand{\retCILVDSnTwoCoarseLTwoVarDecoderSegformerMlp}{\tbd{retCILVDSnTwoCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retCILVDSnTwoCoarseLTwoVarLrMultOne}{\tbd{retCILVDSnTwoCoarseLTwoVarLrMultOne}}
\providecommand{\retCILVDSnTwoOmissionLOne}{\tbd{retCILVDSnTwoOmissionLOne}}
\providecommand{\retCILVDSnTwoOmissionLTwo}{\tbd{retCILVDSnTwoOmissionLTwo}}
\providecommand{\retCILVDSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retCILVDSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDSnTwoOmissionLTwoVarDecoderSamLite}{\tbd{retCILVDSnTwoOmissionLTwoVarDecoderSamLite}}
\providecommand{\retCILVDSnTwoOmissionLTwoVarDecoderSegformerMlp}{\tbd{retCILVDSnTwoOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retCILVDSnTwoOmissionLTwoVarLrMultOne}{\tbd{retCILVDSnTwoOmissionLTwoVarLrMultOne}}
\providecommand{\retCILVDSnTwoShiftLOne}{\tbd{retCILVDSnTwoShiftLOne}}
\providecommand{\retCILVDSnTwoShiftLTwo}{\tbd{retCILVDSnTwoShiftLTwo}}
\providecommand{\retCILVDSnTwoShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retCILVDSnTwoShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDSnTwoShiftLTwoVarDecoderSamLite}{\tbd{retCILVDSnTwoShiftLTwoVarDecoderSamLite}}
\providecommand{\retCILVDSnTwoShiftLTwoVarDecoderSegformerMlp}{\tbd{retCILVDSnTwoShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retCILVDSnTwoShiftLTwoVarLrMultOne}{\tbd{retCILVDSnTwoShiftLTwoVarLrMultOne}}
\providecommand{\retCILVDburnBoundaryLOne}{\tbd{retCILVDburnBoundaryLOne}}
\providecommand{\retCILVDburnBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{retCILVDburnBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCILVDburnBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{retCILVDburnBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDburnBoundaryLOneVarDecoderSamLite}{\tbd{retCILVDburnBoundaryLOneVarDecoderSamLite}}
\providecommand{\retCILVDburnBoundaryLOneVarDecoderSamPretrained}{\tbd{retCILVDburnBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\retCILVDburnBoundaryLOneVarDecoderSegformerMlp}{\tbd{retCILVDburnBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\retCILVDburnBoundaryLR}{\tbd{retCILVDburnBoundaryLR}}
\providecommand{\retCILVDburnBoundaryLRVarLrMultOne}{\tbd{retCILVDburnBoundaryLRVarLrMultOne}}
\providecommand{\retCILVDburnBoundaryLTwo}{\tbd{retCILVDburnBoundaryLTwo}}
\providecommand{\retCILVDburnBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{retCILVDburnBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCILVDburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{retCILVDburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\retCILVDburnBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retCILVDburnBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{retCILVDburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\retCILVDburnBoundaryLTwoVarDecoderSamLite}{\tbd{retCILVDburnBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retCILVDburnBoundaryLTwoVarDecoderSamLiteLrMultOne}{\tbd{retCILVDburnBoundaryLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\retCILVDburnBoundaryLTwoVarDecoderSamPretrained}{\tbd{retCILVDburnBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\retCILVDburnBoundaryLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{retCILVDburnBoundaryLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\retCILVDburnBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retCILVDburnBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retCILVDburnBoundaryLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{retCILVDburnBoundaryLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\retCILVDburnBoundaryLTwoVarLossBootstrap}{\tbd{retCILVDburnBoundaryLTwoVarLossBootstrap}}
\providecommand{\retCILVDburnBoundaryLTwoVarLossGce}{\tbd{retCILVDburnBoundaryLTwoVarLossGce}}
\providecommand{\retCILVDburnBoundaryLTwoVarLrMultOne}{\tbd{retCILVDburnBoundaryLTwoVarLrMultOne}}
\providecommand{\retCILVDburnBoundaryLTwoVarLrMultThree}{\tbd{retCILVDburnBoundaryLTwoVarLrMultThree}}
\providecommand{\retCILVDburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCILVDburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCILVDburnBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCILVDburnBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCILVDburnCoarseLOne}{\tbd{retCILVDburnCoarseLOne}}
\providecommand{\retCILVDburnCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{retCILVDburnCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCILVDburnCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{retCILVDburnCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDburnCoarseLOneVarDecoderSamLite}{\tbd{retCILVDburnCoarseLOneVarDecoderSamLite}}
\providecommand{\retCILVDburnCoarseLOneVarDecoderSamPretrained}{\tbd{retCILVDburnCoarseLOneVarDecoderSamPretrained}}
\providecommand{\retCILVDburnCoarseLOneVarDecoderSegformerMlp}{\tbd{retCILVDburnCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\retCILVDburnCoarseLR}{\tbd{retCILVDburnCoarseLR}}
\providecommand{\retCILVDburnCoarseLRVarLrMultOne}{\tbd{retCILVDburnCoarseLRVarLrMultOne}}
\providecommand{\retCILVDburnCoarseLTwo}{\tbd{retCILVDburnCoarseLTwo}}
\providecommand{\retCILVDburnCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{retCILVDburnCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCILVDburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{retCILVDburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\retCILVDburnCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retCILVDburnCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{retCILVDburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\retCILVDburnCoarseLTwoVarDecoderSamLite}{\tbd{retCILVDburnCoarseLTwoVarDecoderSamLite}}
\providecommand{\retCILVDburnCoarseLTwoVarDecoderSamLiteLrMultOne}{\tbd{retCILVDburnCoarseLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\retCILVDburnCoarseLTwoVarDecoderSamPretrained}{\tbd{retCILVDburnCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\retCILVDburnCoarseLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{retCILVDburnCoarseLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\retCILVDburnCoarseLTwoVarDecoderSegformerMlp}{\tbd{retCILVDburnCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retCILVDburnCoarseLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{retCILVDburnCoarseLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\retCILVDburnCoarseLTwoVarLossBootstrap}{\tbd{retCILVDburnCoarseLTwoVarLossBootstrap}}
\providecommand{\retCILVDburnCoarseLTwoVarLossGce}{\tbd{retCILVDburnCoarseLTwoVarLossGce}}
\providecommand{\retCILVDburnCoarseLTwoVarLrMultOne}{\tbd{retCILVDburnCoarseLTwoVarLrMultOne}}
\providecommand{\retCILVDburnCoarseLTwoVarLrMultThree}{\tbd{retCILVDburnCoarseLTwoVarLrMultThree}}
\providecommand{\retCILVDburnCoarseLTwoVarLrMultZeroOneOneOneOne}{\tbd{retCILVDburnCoarseLTwoVarLrMultZeroOneOneOneOne}}
\providecommand{\retCILVDburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCILVDburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCILVDburnCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCILVDburnCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCILVDburnOmissionLOne}{\tbd{retCILVDburnOmissionLOne}}
\providecommand{\retCILVDburnOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{retCILVDburnOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCILVDburnOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{retCILVDburnOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDburnOmissionLOneVarDecoderSamLite}{\tbd{retCILVDburnOmissionLOneVarDecoderSamLite}}
\providecommand{\retCILVDburnOmissionLOneVarDecoderSamPretrained}{\tbd{retCILVDburnOmissionLOneVarDecoderSamPretrained}}
\providecommand{\retCILVDburnOmissionLOneVarDecoderSegformerMlp}{\tbd{retCILVDburnOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\retCILVDburnOmissionLR}{\tbd{retCILVDburnOmissionLR}}
\providecommand{\retCILVDburnOmissionLRVarLrMultOne}{\tbd{retCILVDburnOmissionLRVarLrMultOne}}
\providecommand{\retCILVDburnOmissionLTwo}{\tbd{retCILVDburnOmissionLTwo}}
\providecommand{\retCILVDburnOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{retCILVDburnOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCILVDburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{retCILVDburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\retCILVDburnOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retCILVDburnOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{retCILVDburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\retCILVDburnOmissionLTwoVarDecoderSamLite}{\tbd{retCILVDburnOmissionLTwoVarDecoderSamLite}}
\providecommand{\retCILVDburnOmissionLTwoVarDecoderSamLiteLrMultOne}{\tbd{retCILVDburnOmissionLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\retCILVDburnOmissionLTwoVarDecoderSamPretrained}{\tbd{retCILVDburnOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\retCILVDburnOmissionLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{retCILVDburnOmissionLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\retCILVDburnOmissionLTwoVarDecoderSegformerMlp}{\tbd{retCILVDburnOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retCILVDburnOmissionLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{retCILVDburnOmissionLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\retCILVDburnOmissionLTwoVarLossBootstrap}{\tbd{retCILVDburnOmissionLTwoVarLossBootstrap}}
\providecommand{\retCILVDburnOmissionLTwoVarLossGce}{\tbd{retCILVDburnOmissionLTwoVarLossGce}}
\providecommand{\retCILVDburnOmissionLTwoVarLrMultOne}{\tbd{retCILVDburnOmissionLTwoVarLrMultOne}}
\providecommand{\retCILVDburnOmissionLTwoVarLrMultThree}{\tbd{retCILVDburnOmissionLTwoVarLrMultThree}}
\providecommand{\retCILVDburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCILVDburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCILVDburnOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCILVDburnOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCILVDburnShiftLOne}{\tbd{retCILVDburnShiftLOne}}
\providecommand{\retCILVDburnShiftLOneVarDecoderMaskTwoformerFull}{\tbd{retCILVDburnShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCILVDburnShiftLOneVarDecoderMaskTwoformerLite}{\tbd{retCILVDburnShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDburnShiftLOneVarDecoderSamLite}{\tbd{retCILVDburnShiftLOneVarDecoderSamLite}}
\providecommand{\retCILVDburnShiftLOneVarDecoderSamPretrained}{\tbd{retCILVDburnShiftLOneVarDecoderSamPretrained}}
\providecommand{\retCILVDburnShiftLOneVarDecoderSegformerMlp}{\tbd{retCILVDburnShiftLOneVarDecoderSegformerMlp}}
\providecommand{\retCILVDburnShiftLR}{\tbd{retCILVDburnShiftLR}}
\providecommand{\retCILVDburnShiftLRVarLrMultOne}{\tbd{retCILVDburnShiftLRVarLrMultOne}}
\providecommand{\retCILVDburnShiftLTwo}{\tbd{retCILVDburnShiftLTwo}}
\providecommand{\retCILVDburnShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{retCILVDburnShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCILVDburnShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{retCILVDburnShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\retCILVDburnShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retCILVDburnShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{retCILVDburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\retCILVDburnShiftLTwoVarDecoderSamLite}{\tbd{retCILVDburnShiftLTwoVarDecoderSamLite}}
\providecommand{\retCILVDburnShiftLTwoVarDecoderSamLiteLrMultOne}{\tbd{retCILVDburnShiftLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\retCILVDburnShiftLTwoVarDecoderSamPretrained}{\tbd{retCILVDburnShiftLTwoVarDecoderSamPretrained}}
\providecommand{\retCILVDburnShiftLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{retCILVDburnShiftLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\retCILVDburnShiftLTwoVarDecoderSegformerMlp}{\tbd{retCILVDburnShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retCILVDburnShiftLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{retCILVDburnShiftLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\retCILVDburnShiftLTwoVarLossBootstrap}{\tbd{retCILVDburnShiftLTwoVarLossBootstrap}}
\providecommand{\retCILVDburnShiftLTwoVarLossGce}{\tbd{retCILVDburnShiftLTwoVarLossGce}}
\providecommand{\retCILVDburnShiftLTwoVarLrMultOne}{\tbd{retCILVDburnShiftLTwoVarLrMultOne}}
\providecommand{\retCILVDburnShiftLTwoVarLrMultThree}{\tbd{retCILVDburnShiftLTwoVarLrMultThree}}
\providecommand{\retCILVDburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCILVDburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCILVDburnShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCILVDburnShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCILVDflairBoundaryLOne}{\tbd{retCILVDflairBoundaryLOne}}
\providecommand{\retCILVDflairBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{retCILVDflairBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCILVDflairBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{retCILVDflairBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDflairBoundaryLOneVarDecoderSamLite}{\tbd{retCILVDflairBoundaryLOneVarDecoderSamLite}}
\providecommand{\retCILVDflairBoundaryLOneVarDecoderSamPretrained}{\tbd{retCILVDflairBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\retCILVDflairBoundaryLOneVarDecoderSegformerMlp}{\tbd{retCILVDflairBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\retCILVDflairBoundaryLR}{\tbd{retCILVDflairBoundaryLR}}
\providecommand{\retCILVDflairBoundaryLRVarLrMultOne}{\tbd{retCILVDflairBoundaryLRVarLrMultOne}}
\providecommand{\retCILVDflairBoundaryLTwo}{\tbd{retCILVDflairBoundaryLTwo}}
\providecommand{\retCILVDflairBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{retCILVDflairBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCILVDflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{retCILVDflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\retCILVDflairBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retCILVDflairBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{retCILVDflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\retCILVDflairBoundaryLTwoVarDecoderSamLite}{\tbd{retCILVDflairBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retCILVDflairBoundaryLTwoVarDecoderSamLiteLrMultOne}{\tbd{retCILVDflairBoundaryLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\retCILVDflairBoundaryLTwoVarDecoderSamPretrained}{\tbd{retCILVDflairBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\retCILVDflairBoundaryLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{retCILVDflairBoundaryLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\retCILVDflairBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retCILVDflairBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retCILVDflairBoundaryLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{retCILVDflairBoundaryLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\retCILVDflairBoundaryLTwoVarLossBootstrap}{\tbd{retCILVDflairBoundaryLTwoVarLossBootstrap}}
\providecommand{\retCILVDflairBoundaryLTwoVarLossGce}{\tbd{retCILVDflairBoundaryLTwoVarLossGce}}
\providecommand{\retCILVDflairBoundaryLTwoVarLrMultOne}{\tbd{retCILVDflairBoundaryLTwoVarLrMultOne}}
\providecommand{\retCILVDflairBoundaryLTwoVarLrMultThree}{\tbd{retCILVDflairBoundaryLTwoVarLrMultThree}}
\providecommand{\retCILVDflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCILVDflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCILVDflairBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCILVDflairBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCILVDflairCoarseLOne}{\tbd{retCILVDflairCoarseLOne}}
\providecommand{\retCILVDflairCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{retCILVDflairCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCILVDflairCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{retCILVDflairCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDflairCoarseLOneVarDecoderSamLite}{\tbd{retCILVDflairCoarseLOneVarDecoderSamLite}}
\providecommand{\retCILVDflairCoarseLOneVarDecoderSamPretrained}{\tbd{retCILVDflairCoarseLOneVarDecoderSamPretrained}}
\providecommand{\retCILVDflairCoarseLOneVarDecoderSegformerMlp}{\tbd{retCILVDflairCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\retCILVDflairCoarseLR}{\tbd{retCILVDflairCoarseLR}}
\providecommand{\retCILVDflairCoarseLRVarLrMultOne}{\tbd{retCILVDflairCoarseLRVarLrMultOne}}
\providecommand{\retCILVDflairCoarseLTwo}{\tbd{retCILVDflairCoarseLTwo}}
\providecommand{\retCILVDflairCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{retCILVDflairCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCILVDflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{retCILVDflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\retCILVDflairCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retCILVDflairCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{retCILVDflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\retCILVDflairCoarseLTwoVarDecoderSamLite}{\tbd{retCILVDflairCoarseLTwoVarDecoderSamLite}}
\providecommand{\retCILVDflairCoarseLTwoVarDecoderSamLiteLrMultOne}{\tbd{retCILVDflairCoarseLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\retCILVDflairCoarseLTwoVarDecoderSamPretrained}{\tbd{retCILVDflairCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\retCILVDflairCoarseLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{retCILVDflairCoarseLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\retCILVDflairCoarseLTwoVarDecoderSegformerMlp}{\tbd{retCILVDflairCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retCILVDflairCoarseLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{retCILVDflairCoarseLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\retCILVDflairCoarseLTwoVarLossBootstrap}{\tbd{retCILVDflairCoarseLTwoVarLossBootstrap}}
\providecommand{\retCILVDflairCoarseLTwoVarLossGce}{\tbd{retCILVDflairCoarseLTwoVarLossGce}}
\providecommand{\retCILVDflairCoarseLTwoVarLrMultOne}{\tbd{retCILVDflairCoarseLTwoVarLrMultOne}}
\providecommand{\retCILVDflairCoarseLTwoVarLrMultThree}{\tbd{retCILVDflairCoarseLTwoVarLrMultThree}}
\providecommand{\retCILVDflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCILVDflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCILVDflairCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCILVDflairCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCILVDflairOmissionLOne}{\tbd{retCILVDflairOmissionLOne}}
\providecommand{\retCILVDflairOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{retCILVDflairOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCILVDflairOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{retCILVDflairOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDflairOmissionLOneVarDecoderSamLite}{\tbd{retCILVDflairOmissionLOneVarDecoderSamLite}}
\providecommand{\retCILVDflairOmissionLOneVarDecoderSamPretrained}{\tbd{retCILVDflairOmissionLOneVarDecoderSamPretrained}}
\providecommand{\retCILVDflairOmissionLOneVarDecoderSegformerMlp}{\tbd{retCILVDflairOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\retCILVDflairOmissionLR}{\tbd{retCILVDflairOmissionLR}}
\providecommand{\retCILVDflairOmissionLRVarLrMultOne}{\tbd{retCILVDflairOmissionLRVarLrMultOne}}
\providecommand{\retCILVDflairOmissionLTwo}{\tbd{retCILVDflairOmissionLTwo}}
\providecommand{\retCILVDflairOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{retCILVDflairOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCILVDflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{retCILVDflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\retCILVDflairOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retCILVDflairOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{retCILVDflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\retCILVDflairOmissionLTwoVarDecoderSamLite}{\tbd{retCILVDflairOmissionLTwoVarDecoderSamLite}}
\providecommand{\retCILVDflairOmissionLTwoVarDecoderSamLiteLrMultOne}{\tbd{retCILVDflairOmissionLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\retCILVDflairOmissionLTwoVarDecoderSamPretrained}{\tbd{retCILVDflairOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\retCILVDflairOmissionLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{retCILVDflairOmissionLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\retCILVDflairOmissionLTwoVarDecoderSegformerMlp}{\tbd{retCILVDflairOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retCILVDflairOmissionLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{retCILVDflairOmissionLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\retCILVDflairOmissionLTwoVarLossBootstrap}{\tbd{retCILVDflairOmissionLTwoVarLossBootstrap}}
\providecommand{\retCILVDflairOmissionLTwoVarLossGce}{\tbd{retCILVDflairOmissionLTwoVarLossGce}}
\providecommand{\retCILVDflairOmissionLTwoVarLrMultOne}{\tbd{retCILVDflairOmissionLTwoVarLrMultOne}}
\providecommand{\retCILVDflairOmissionLTwoVarLrMultThree}{\tbd{retCILVDflairOmissionLTwoVarLrMultThree}}
\providecommand{\retCILVDflairOmissionLTwoVarLrMultZeroOneOneOneOne}{\tbd{retCILVDflairOmissionLTwoVarLrMultZeroOneOneOneOne}}
\providecommand{\retCILVDflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCILVDflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCILVDflairOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCILVDflairOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCILVDflairShiftLOne}{\tbd{retCILVDflairShiftLOne}}
\providecommand{\retCILVDflairShiftLOneVarDecoderMaskTwoformerFull}{\tbd{retCILVDflairShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCILVDflairShiftLOneVarDecoderMaskTwoformerLite}{\tbd{retCILVDflairShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDflairShiftLOneVarDecoderSamLite}{\tbd{retCILVDflairShiftLOneVarDecoderSamLite}}
\providecommand{\retCILVDflairShiftLOneVarDecoderSamPretrained}{\tbd{retCILVDflairShiftLOneVarDecoderSamPretrained}}
\providecommand{\retCILVDflairShiftLOneVarDecoderSegformerMlp}{\tbd{retCILVDflairShiftLOneVarDecoderSegformerMlp}}
\providecommand{\retCILVDflairShiftLR}{\tbd{retCILVDflairShiftLR}}
\providecommand{\retCILVDflairShiftLRVarLrMultOne}{\tbd{retCILVDflairShiftLRVarLrMultOne}}
\providecommand{\retCILVDflairShiftLTwo}{\tbd{retCILVDflairShiftLTwo}}
\providecommand{\retCILVDflairShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{retCILVDflairShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCILVDflairShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{retCILVDflairShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\retCILVDflairShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retCILVDflairShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCILVDflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{retCILVDflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\retCILVDflairShiftLTwoVarDecoderSamLite}{\tbd{retCILVDflairShiftLTwoVarDecoderSamLite}}
\providecommand{\retCILVDflairShiftLTwoVarDecoderSamLiteLrMultOne}{\tbd{retCILVDflairShiftLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\retCILVDflairShiftLTwoVarDecoderSamPretrained}{\tbd{retCILVDflairShiftLTwoVarDecoderSamPretrained}}
\providecommand{\retCILVDflairShiftLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{retCILVDflairShiftLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\retCILVDflairShiftLTwoVarDecoderSegformerMlp}{\tbd{retCILVDflairShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retCILVDflairShiftLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{retCILVDflairShiftLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\retCILVDflairShiftLTwoVarLossBootstrap}{\tbd{retCILVDflairShiftLTwoVarLossBootstrap}}
\providecommand{\retCILVDflairShiftLTwoVarLossGce}{\tbd{retCILVDflairShiftLTwoVarLossGce}}
\providecommand{\retCILVDflairShiftLTwoVarLrMultOne}{\tbd{retCILVDflairShiftLTwoVarLrMultOne}}
\providecommand{\retCILVDflairShiftLTwoVarLrMultThree}{\tbd{retCILVDflairShiftLTwoVarLrMultThree}}
\providecommand{\retCILVDflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCILVDflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCILVDflairShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCILVDflairShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCILVDsenOtsuLTwo}{\tbd{retCILVDsenOtsuLTwo}}
\providecommand{\retCIPRIburnBoundaryLOne}{\tbd{retCIPRIburnBoundaryLOne}}
\providecommand{\retCIPRIburnBoundaryLTwo}{\tbd{retCIPRIburnBoundaryLTwo}}
\providecommand{\retCIPRIburnCoarseLOne}{\tbd{retCIPRIburnCoarseLOne}}
\providecommand{\retCIPRIburnCoarseLTwo}{\tbd{retCIPRIburnCoarseLTwo}}
\providecommand{\retCIPRIburnOmissionLOne}{\tbd{retCIPRIburnOmissionLOne}}
\providecommand{\retCIPRIburnOmissionLTwo}{\tbd{retCIPRIburnOmissionLTwo}}
\providecommand{\retCIPRIburnShiftLOne}{\tbd{retCIPRIburnShiftLOne}}
\providecommand{\retCIPRIburnShiftLTwo}{\tbd{retCIPRIburnShiftLTwo}}
\providecommand{\retCIPRIflairBoundaryLOne}{\tbd{retCIPRIflairBoundaryLOne}}
\providecommand{\retCIPRIflairBoundaryLTwo}{\tbd{retCIPRIflairBoundaryLTwo}}
\providecommand{\retCIPRIflairCoarseLOne}{\tbd{retCIPRIflairCoarseLOne}}
\providecommand{\retCIPRIflairCoarseLTwo}{\tbd{retCIPRIflairCoarseLTwo}}
\providecommand{\retCIPRIflairOmissionLOne}{\tbd{retCIPRIflairOmissionLOne}}
\providecommand{\retCIPRIflairOmissionLTwo}{\tbd{retCIPRIflairOmissionLTwo}}
\providecommand{\retCIPRIflairShiftLOne}{\tbd{retCIPRIflairShiftLOne}}
\providecommand{\retCIPRIflairShiftLTwo}{\tbd{retCIPRIflairShiftLTwo}}
\providecommand{\retCIRNChesBoundaryLOne}{\tbd{retCIRNChesBoundaryLOne}}
\providecommand{\retCIRNChesBoundaryLTwo}{\tbd{retCIRNChesBoundaryLTwo}}
\providecommand{\retCIRNChesCoarseLOne}{\tbd{retCIRNChesCoarseLOne}}
\providecommand{\retCIRNChesCoarseLTwo}{\tbd{retCIRNChesCoarseLTwo}}
\providecommand{\retCIRNChesNlcdREAL}{\tbd{retCIRNChesNlcdREAL}}
\providecommand{\retCIRNChesOmissionLOne}{\tbd{retCIRNChesOmissionLOne}}
\providecommand{\retCIRNChesOmissionLTwo}{\tbd{retCIRNChesOmissionLTwo}}
\providecommand{\retCIRNChesShiftLOne}{\tbd{retCIRNChesShiftLOne}}
\providecommand{\retCIRNChesShiftLTwo}{\tbd{retCIRNChesShiftLTwo}}
\providecommand{\retCIRNCsTwelveBoundaryLOne}{\tbd{retCIRNCsTwelveBoundaryLOne}}
\providecommand{\retCIRNCsTwelveBoundaryLTwo}{\tbd{retCIRNCsTwelveBoundaryLTwo}}
\providecommand{\retCIRNCsTwelveCoarseLOne}{\tbd{retCIRNCsTwelveCoarseLOne}}
\providecommand{\retCIRNCsTwelveCoarseLTwo}{\tbd{retCIRNCsTwelveCoarseLTwo}}
\providecommand{\retCIRNCsTwelveOmissionLOne}{\tbd{retCIRNCsTwelveOmissionLOne}}
\providecommand{\retCIRNCsTwelveOmissionLTwo}{\tbd{retCIRNCsTwelveOmissionLTwo}}
\providecommand{\retCIRNCsTwelveSTwocloudlessREAL}{\tbd{retCIRNCsTwelveSTwocloudlessREAL}}
\providecommand{\retCIRNCsTwelveShiftLOne}{\tbd{retCIRNCsTwelveShiftLOne}}
\providecommand{\retCIRNCsTwelveShiftLTwo}{\tbd{retCIRNCsTwelveShiftLTwo}}
\providecommand{\retCIRNDfcBoundaryLOne}{\tbd{retCIRNDfcBoundaryLOne}}
\providecommand{\retCIRNDfcBoundaryLTwo}{\tbd{retCIRNDfcBoundaryLTwo}}
\providecommand{\retCIRNDfcCoarseLOne}{\tbd{retCIRNDfcCoarseLOne}}
\providecommand{\retCIRNDfcCoarseLTwo}{\tbd{retCIRNDfcCoarseLTwo}}
\providecommand{\retCIRNDfcModisREALVarTrainSubsetRealcov}{\tbd{retCIRNDfcModisREALVarTrainSubsetRealcov}}
\providecommand{\retCIRNDfcOmissionLOne}{\tbd{retCIRNDfcOmissionLOne}}
\providecommand{\retCIRNDfcOmissionLTwo}{\tbd{retCIRNDfcOmissionLTwo}}
\providecommand{\retCIRNDfcShiftLOne}{\tbd{retCIRNDfcShiftLOne}}
\providecommand{\retCIRNDfcShiftLTwo}{\tbd{retCIRNDfcShiftLTwo}}
\providecommand{\retCIRNEnvaBoundaryLOne}{\tbd{retCIRNEnvaBoundaryLOne}}
\providecommand{\retCIRNEnvaBoundaryLTwo}{\tbd{retCIRNEnvaBoundaryLTwo}}
\providecommand{\retCIRNEnvaCoarseLOne}{\tbd{retCIRNEnvaCoarseLOne}}
\providecommand{\retCIRNEnvaCoarseLTwo}{\tbd{retCIRNEnvaCoarseLTwo}}
\providecommand{\retCIRNEnvaNlcdREAL}{\tbd{retCIRNEnvaNlcdREAL}}
\providecommand{\retCIRNEnvaOmissionLOne}{\tbd{retCIRNEnvaOmissionLOne}}
\providecommand{\retCIRNEnvaOmissionLTwo}{\tbd{retCIRNEnvaOmissionLTwo}}
\providecommand{\retCIRNEnvaShiftLOne}{\tbd{retCIRNEnvaShiftLOne}}
\providecommand{\retCIRNEnvaShiftLTwo}{\tbd{retCIRNEnvaShiftLTwo}}
\providecommand{\retCIRNKuroBoundaryLOne}{\tbd{retCIRNKuroBoundaryLOne}}
\providecommand{\retCIRNKuroBoundaryLTwo}{\tbd{retCIRNKuroBoundaryLTwo}}
\providecommand{\retCIRNKuroCemsREALVarTrainSubsetRealcov}{\tbd{retCIRNKuroCemsREALVarTrainSubsetRealcov}}
\providecommand{\retCIRNKuroCoarseLOne}{\tbd{retCIRNKuroCoarseLOne}}
\providecommand{\retCIRNKuroCoarseLTwo}{\tbd{retCIRNKuroCoarseLTwo}}
\providecommand{\retCIRNKuroOmissionLOne}{\tbd{retCIRNKuroOmissionLOne}}
\providecommand{\retCIRNKuroOmissionLTwo}{\tbd{retCIRNKuroOmissionLTwo}}
\providecommand{\retCIRNKuroShiftLOne}{\tbd{retCIRNKuroShiftLOne}}
\providecommand{\retCIRNKuroShiftLTwo}{\tbd{retCIRNKuroShiftLTwo}}
\providecommand{\retCIRNOemBoundaryLOne}{\tbd{retCIRNOemBoundaryLOne}}
\providecommand{\retCIRNOemBoundaryLTwo}{\tbd{retCIRNOemBoundaryLTwo}}
\providecommand{\retCIRNOemCoarseLOne}{\tbd{retCIRNOemCoarseLOne}}
\providecommand{\retCIRNOemCoarseLTwo}{\tbd{retCIRNOemCoarseLTwo}}
\providecommand{\retCIRNOemOmissionLOne}{\tbd{retCIRNOemOmissionLOne}}
\providecommand{\retCIRNOemOmissionLTwo}{\tbd{retCIRNOemOmissionLTwo}}
\providecommand{\retCIRNOemShiftLOne}{\tbd{retCIRNOemShiftLOne}}
\providecommand{\retCIRNOemShiftLTwo}{\tbd{retCIRNOemShiftLTwo}}
\providecommand{\retCIRNSnTwoBoundaryLOne}{\tbd{retCIRNSnTwoBoundaryLOne}}
\providecommand{\retCIRNSnTwoBoundaryLTwo}{\tbd{retCIRNSnTwoBoundaryLTwo}}
\providecommand{\retCIRNSnTwoCoarseLOne}{\tbd{retCIRNSnTwoCoarseLOne}}
\providecommand{\retCIRNSnTwoCoarseLTwo}{\tbd{retCIRNSnTwoCoarseLTwo}}
\providecommand{\retCIRNSnTwoOmissionLOne}{\tbd{retCIRNSnTwoOmissionLOne}}
\providecommand{\retCIRNSnTwoOmissionLTwo}{\tbd{retCIRNSnTwoOmissionLTwo}}
\providecommand{\retCIRNSnTwoShiftLOne}{\tbd{retCIRNSnTwoShiftLOne}}
\providecommand{\retCIRNSnTwoShiftLTwo}{\tbd{retCIRNSnTwoShiftLTwo}}
\providecommand{\retCIRNburnBoundaryLOne}{\tbd{retCIRNburnBoundaryLOne}}
\providecommand{\retCIRNburnBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{retCIRNburnBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCIRNburnBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{retCIRNburnBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCIRNburnBoundaryLOneVarDecoderSamLite}{\tbd{retCIRNburnBoundaryLOneVarDecoderSamLite}}
\providecommand{\retCIRNburnBoundaryLOneVarDecoderSamPretrained}{\tbd{retCIRNburnBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\retCIRNburnBoundaryLOneVarDecoderSegformerMlp}{\tbd{retCIRNburnBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\retCIRNburnBoundaryLR}{\tbd{retCIRNburnBoundaryLR}}
\providecommand{\retCIRNburnBoundaryLTwo}{\tbd{retCIRNburnBoundaryLTwo}}
\providecommand{\retCIRNburnBoundaryLTwoVarBandsRgb}{\tbd{retCIRNburnBoundaryLTwoVarBandsRgb}}
\providecommand{\retCIRNburnBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{retCIRNburnBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCIRNburnBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retCIRNburnBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCIRNburnBoundaryLTwoVarDecoderSamLite}{\tbd{retCIRNburnBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retCIRNburnBoundaryLTwoVarDecoderSamPretrained}{\tbd{retCIRNburnBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\retCIRNburnBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retCIRNburnBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retCIRNburnBoundaryLTwoVarInitRandom}{\tbd{retCIRNburnBoundaryLTwoVarInitRandom}}
\providecommand{\retCIRNburnBoundaryLTwoVarLossBootstrap}{\tbd{retCIRNburnBoundaryLTwoVarLossBootstrap}}
\providecommand{\retCIRNburnBoundaryLTwoVarLossGce}{\tbd{retCIRNburnBoundaryLTwoVarLossGce}}
\providecommand{\retCIRNburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCIRNburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCIRNburnBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCIRNburnBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCIRNburnCoarseLOne}{\tbd{retCIRNburnCoarseLOne}}
\providecommand{\retCIRNburnCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{retCIRNburnCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCIRNburnCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{retCIRNburnCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCIRNburnCoarseLOneVarDecoderSamLite}{\tbd{retCIRNburnCoarseLOneVarDecoderSamLite}}
\providecommand{\retCIRNburnCoarseLOneVarDecoderSamPretrained}{\tbd{retCIRNburnCoarseLOneVarDecoderSamPretrained}}
\providecommand{\retCIRNburnCoarseLOneVarDecoderSegformerMlp}{\tbd{retCIRNburnCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\retCIRNburnCoarseLR}{\tbd{retCIRNburnCoarseLR}}
\providecommand{\retCIRNburnCoarseLTwo}{\tbd{retCIRNburnCoarseLTwo}}
\providecommand{\retCIRNburnCoarseLTwoVarBandsRgb}{\tbd{retCIRNburnCoarseLTwoVarBandsRgb}}
\providecommand{\retCIRNburnCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{retCIRNburnCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCIRNburnCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retCIRNburnCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCIRNburnCoarseLTwoVarDecoderSamLite}{\tbd{retCIRNburnCoarseLTwoVarDecoderSamLite}}
\providecommand{\retCIRNburnCoarseLTwoVarDecoderSamPretrained}{\tbd{retCIRNburnCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\retCIRNburnCoarseLTwoVarDecoderSegformerMlp}{\tbd{retCIRNburnCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retCIRNburnCoarseLTwoVarInitRandom}{\tbd{retCIRNburnCoarseLTwoVarInitRandom}}
\providecommand{\retCIRNburnCoarseLTwoVarLossBootstrap}{\tbd{retCIRNburnCoarseLTwoVarLossBootstrap}}
\providecommand{\retCIRNburnCoarseLTwoVarLossGce}{\tbd{retCIRNburnCoarseLTwoVarLossGce}}
\providecommand{\retCIRNburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCIRNburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCIRNburnCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCIRNburnCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCIRNburnOmissionLOne}{\tbd{retCIRNburnOmissionLOne}}
\providecommand{\retCIRNburnOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{retCIRNburnOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCIRNburnOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{retCIRNburnOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCIRNburnOmissionLOneVarDecoderSamLite}{\tbd{retCIRNburnOmissionLOneVarDecoderSamLite}}
\providecommand{\retCIRNburnOmissionLOneVarDecoderSamPretrained}{\tbd{retCIRNburnOmissionLOneVarDecoderSamPretrained}}
\providecommand{\retCIRNburnOmissionLOneVarDecoderSegformerMlp}{\tbd{retCIRNburnOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\retCIRNburnOmissionLR}{\tbd{retCIRNburnOmissionLR}}
\providecommand{\retCIRNburnOmissionLTwo}{\tbd{retCIRNburnOmissionLTwo}}
\providecommand{\retCIRNburnOmissionLTwoVarBandsRgb}{\tbd{retCIRNburnOmissionLTwoVarBandsRgb}}
\providecommand{\retCIRNburnOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{retCIRNburnOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCIRNburnOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retCIRNburnOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCIRNburnOmissionLTwoVarDecoderSamLite}{\tbd{retCIRNburnOmissionLTwoVarDecoderSamLite}}
\providecommand{\retCIRNburnOmissionLTwoVarDecoderSamPretrained}{\tbd{retCIRNburnOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\retCIRNburnOmissionLTwoVarDecoderSegformerMlp}{\tbd{retCIRNburnOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retCIRNburnOmissionLTwoVarInitRandom}{\tbd{retCIRNburnOmissionLTwoVarInitRandom}}
\providecommand{\retCIRNburnOmissionLTwoVarLossBootstrap}{\tbd{retCIRNburnOmissionLTwoVarLossBootstrap}}
\providecommand{\retCIRNburnOmissionLTwoVarLossGce}{\tbd{retCIRNburnOmissionLTwoVarLossGce}}
\providecommand{\retCIRNburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCIRNburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCIRNburnOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCIRNburnOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCIRNburnShiftLOne}{\tbd{retCIRNburnShiftLOne}}
\providecommand{\retCIRNburnShiftLOneVarDecoderMaskTwoformerFull}{\tbd{retCIRNburnShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCIRNburnShiftLOneVarDecoderMaskTwoformerLite}{\tbd{retCIRNburnShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCIRNburnShiftLOneVarDecoderSamLite}{\tbd{retCIRNburnShiftLOneVarDecoderSamLite}}
\providecommand{\retCIRNburnShiftLOneVarDecoderSamPretrained}{\tbd{retCIRNburnShiftLOneVarDecoderSamPretrained}}
\providecommand{\retCIRNburnShiftLOneVarDecoderSegformerMlp}{\tbd{retCIRNburnShiftLOneVarDecoderSegformerMlp}}
\providecommand{\retCIRNburnShiftLR}{\tbd{retCIRNburnShiftLR}}
\providecommand{\retCIRNburnShiftLTwo}{\tbd{retCIRNburnShiftLTwo}}
\providecommand{\retCIRNburnShiftLTwoVarBandsRgb}{\tbd{retCIRNburnShiftLTwoVarBandsRgb}}
\providecommand{\retCIRNburnShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{retCIRNburnShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCIRNburnShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retCIRNburnShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCIRNburnShiftLTwoVarDecoderSamLite}{\tbd{retCIRNburnShiftLTwoVarDecoderSamLite}}
\providecommand{\retCIRNburnShiftLTwoVarDecoderSamPretrained}{\tbd{retCIRNburnShiftLTwoVarDecoderSamPretrained}}
\providecommand{\retCIRNburnShiftLTwoVarDecoderSegformerMlp}{\tbd{retCIRNburnShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retCIRNburnShiftLTwoVarInitRandom}{\tbd{retCIRNburnShiftLTwoVarInitRandom}}
\providecommand{\retCIRNburnShiftLTwoVarLossBootstrap}{\tbd{retCIRNburnShiftLTwoVarLossBootstrap}}
\providecommand{\retCIRNburnShiftLTwoVarLossGce}{\tbd{retCIRNburnShiftLTwoVarLossGce}}
\providecommand{\retCIRNburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCIRNburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCIRNburnShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCIRNburnShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCIRNflairBoundaryLOne}{\tbd{retCIRNflairBoundaryLOne}}
\providecommand{\retCIRNflairBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{retCIRNflairBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCIRNflairBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{retCIRNflairBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCIRNflairBoundaryLOneVarDecoderSamLite}{\tbd{retCIRNflairBoundaryLOneVarDecoderSamLite}}
\providecommand{\retCIRNflairBoundaryLOneVarDecoderSamPretrained}{\tbd{retCIRNflairBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\retCIRNflairBoundaryLOneVarDecoderSegformerMlp}{\tbd{retCIRNflairBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\retCIRNflairBoundaryLR}{\tbd{retCIRNflairBoundaryLR}}
\providecommand{\retCIRNflairBoundaryLTwo}{\tbd{retCIRNflairBoundaryLTwo}}
\providecommand{\retCIRNflairBoundaryLTwoVarBandsRgb}{\tbd{retCIRNflairBoundaryLTwoVarBandsRgb}}
\providecommand{\retCIRNflairBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{retCIRNflairBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCIRNflairBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retCIRNflairBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCIRNflairBoundaryLTwoVarDecoderSamLite}{\tbd{retCIRNflairBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retCIRNflairBoundaryLTwoVarDecoderSamPretrained}{\tbd{retCIRNflairBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\retCIRNflairBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retCIRNflairBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retCIRNflairBoundaryLTwoVarInitRandom}{\tbd{retCIRNflairBoundaryLTwoVarInitRandom}}
\providecommand{\retCIRNflairBoundaryLTwoVarLossBootstrap}{\tbd{retCIRNflairBoundaryLTwoVarLossBootstrap}}
\providecommand{\retCIRNflairBoundaryLTwoVarLossGce}{\tbd{retCIRNflairBoundaryLTwoVarLossGce}}
\providecommand{\retCIRNflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCIRNflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCIRNflairBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCIRNflairBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCIRNflairCoarseLOne}{\tbd{retCIRNflairCoarseLOne}}
\providecommand{\retCIRNflairCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{retCIRNflairCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCIRNflairCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{retCIRNflairCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCIRNflairCoarseLOneVarDecoderSamLite}{\tbd{retCIRNflairCoarseLOneVarDecoderSamLite}}
\providecommand{\retCIRNflairCoarseLOneVarDecoderSamPretrained}{\tbd{retCIRNflairCoarseLOneVarDecoderSamPretrained}}
\providecommand{\retCIRNflairCoarseLOneVarDecoderSegformerMlp}{\tbd{retCIRNflairCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\retCIRNflairCoarseLR}{\tbd{retCIRNflairCoarseLR}}
\providecommand{\retCIRNflairCoarseLTwo}{\tbd{retCIRNflairCoarseLTwo}}
\providecommand{\retCIRNflairCoarseLTwoVarBandsRgb}{\tbd{retCIRNflairCoarseLTwoVarBandsRgb}}
\providecommand{\retCIRNflairCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{retCIRNflairCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCIRNflairCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retCIRNflairCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCIRNflairCoarseLTwoVarDecoderSamLite}{\tbd{retCIRNflairCoarseLTwoVarDecoderSamLite}}
\providecommand{\retCIRNflairCoarseLTwoVarDecoderSamPretrained}{\tbd{retCIRNflairCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\retCIRNflairCoarseLTwoVarDecoderSegformerMlp}{\tbd{retCIRNflairCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retCIRNflairCoarseLTwoVarInitRandom}{\tbd{retCIRNflairCoarseLTwoVarInitRandom}}
\providecommand{\retCIRNflairCoarseLTwoVarLossBootstrap}{\tbd{retCIRNflairCoarseLTwoVarLossBootstrap}}
\providecommand{\retCIRNflairCoarseLTwoVarLossGce}{\tbd{retCIRNflairCoarseLTwoVarLossGce}}
\providecommand{\retCIRNflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCIRNflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCIRNflairCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCIRNflairCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCIRNflairOmissionLOne}{\tbd{retCIRNflairOmissionLOne}}
\providecommand{\retCIRNflairOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{retCIRNflairOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCIRNflairOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{retCIRNflairOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCIRNflairOmissionLOneVarDecoderSamLite}{\tbd{retCIRNflairOmissionLOneVarDecoderSamLite}}
\providecommand{\retCIRNflairOmissionLOneVarDecoderSamPretrained}{\tbd{retCIRNflairOmissionLOneVarDecoderSamPretrained}}
\providecommand{\retCIRNflairOmissionLOneVarDecoderSegformerMlp}{\tbd{retCIRNflairOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\retCIRNflairOmissionLR}{\tbd{retCIRNflairOmissionLR}}
\providecommand{\retCIRNflairOmissionLTwo}{\tbd{retCIRNflairOmissionLTwo}}
\providecommand{\retCIRNflairOmissionLTwoVarBandsRgb}{\tbd{retCIRNflairOmissionLTwoVarBandsRgb}}
\providecommand{\retCIRNflairOmissionLTwoVarClassWeightedTrue}{\tbd{retCIRNflairOmissionLTwoVarClassWeightedTrue}}
\providecommand{\retCIRNflairOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{retCIRNflairOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCIRNflairOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retCIRNflairOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCIRNflairOmissionLTwoVarDecoderSamLite}{\tbd{retCIRNflairOmissionLTwoVarDecoderSamLite}}
\providecommand{\retCIRNflairOmissionLTwoVarDecoderSamPretrained}{\tbd{retCIRNflairOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\retCIRNflairOmissionLTwoVarDecoderSegformerMlp}{\tbd{retCIRNflairOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retCIRNflairOmissionLTwoVarInitRandom}{\tbd{retCIRNflairOmissionLTwoVarInitRandom}}
\providecommand{\retCIRNflairOmissionLTwoVarLossBootstrap}{\tbd{retCIRNflairOmissionLTwoVarLossBootstrap}}
\providecommand{\retCIRNflairOmissionLTwoVarLossGce}{\tbd{retCIRNflairOmissionLTwoVarLossGce}}
\providecommand{\retCIRNflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCIRNflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCIRNflairOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCIRNflairOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCIRNflairShiftLOne}{\tbd{retCIRNflairShiftLOne}}
\providecommand{\retCIRNflairShiftLOneVarDecoderMaskTwoformerFull}{\tbd{retCIRNflairShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCIRNflairShiftLOneVarDecoderMaskTwoformerLite}{\tbd{retCIRNflairShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCIRNflairShiftLOneVarDecoderSamLite}{\tbd{retCIRNflairShiftLOneVarDecoderSamLite}}
\providecommand{\retCIRNflairShiftLOneVarDecoderSamPretrained}{\tbd{retCIRNflairShiftLOneVarDecoderSamPretrained}}
\providecommand{\retCIRNflairShiftLOneVarDecoderSegformerMlp}{\tbd{retCIRNflairShiftLOneVarDecoderSegformerMlp}}
\providecommand{\retCIRNflairShiftLR}{\tbd{retCIRNflairShiftLR}}
\providecommand{\retCIRNflairShiftLTwo}{\tbd{retCIRNflairShiftLTwo}}
\providecommand{\retCIRNflairShiftLTwoVarBandsRgb}{\tbd{retCIRNflairShiftLTwoVarBandsRgb}}
\providecommand{\retCIRNflairShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{retCIRNflairShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCIRNflairShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retCIRNflairShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCIRNflairShiftLTwoVarDecoderSamLite}{\tbd{retCIRNflairShiftLTwoVarDecoderSamLite}}
\providecommand{\retCIRNflairShiftLTwoVarDecoderSamPretrained}{\tbd{retCIRNflairShiftLTwoVarDecoderSamPretrained}}
\providecommand{\retCIRNflairShiftLTwoVarDecoderSegformerMlp}{\tbd{retCIRNflairShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retCIRNflairShiftLTwoVarInitRandom}{\tbd{retCIRNflairShiftLTwoVarInitRandom}}
\providecommand{\retCIRNflairShiftLTwoVarLossBootstrap}{\tbd{retCIRNflairShiftLTwoVarLossBootstrap}}
\providecommand{\retCIRNflairShiftLTwoVarLossGce}{\tbd{retCIRNflairShiftLTwoVarLossGce}}
\providecommand{\retCIRNflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCIRNflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCIRNflairShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCIRNflairShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCIRNsenOtsuLTwo}{\tbd{retCIRNsenOtsuLTwo}}
\providecommand{\retCIResnetFiveZeroSslFoureoburnBoundaryLOne}{\tbd{retCIResnetFiveZeroSslFoureoburnBoundaryLOne}}
\providecommand{\retCIResnetFiveZeroSslFoureoburnBoundaryLTwo}{\tbd{retCIResnetFiveZeroSslFoureoburnBoundaryLTwo}}
\providecommand{\retCIResnetFiveZeroSslFoureoburnCoarseLOne}{\tbd{retCIResnetFiveZeroSslFoureoburnCoarseLOne}}
\providecommand{\retCIResnetFiveZeroSslFoureoburnCoarseLTwo}{\tbd{retCIResnetFiveZeroSslFoureoburnCoarseLTwo}}
\providecommand{\retCIResnetFiveZeroSslFoureoburnOmissionLOne}{\tbd{retCIResnetFiveZeroSslFoureoburnOmissionLOne}}
\providecommand{\retCIResnetFiveZeroSslFoureoburnOmissionLTwo}{\tbd{retCIResnetFiveZeroSslFoureoburnOmissionLTwo}}
\providecommand{\retCIResnetFiveZeroSslFoureoburnShiftLOne}{\tbd{retCIResnetFiveZeroSslFoureoburnShiftLOne}}
\providecommand{\retCIResnetFiveZeroSslFoureoburnShiftLTwo}{\tbd{retCIResnetFiveZeroSslFoureoburnShiftLTwo}}
\providecommand{\retCIResnetFiveZeroSslFoureoflairBoundaryLOne}{\tbd{retCIResnetFiveZeroSslFoureoflairBoundaryLOne}}
\providecommand{\retCIResnetFiveZeroSslFoureoflairBoundaryLTwo}{\tbd{retCIResnetFiveZeroSslFoureoflairBoundaryLTwo}}
\providecommand{\retCIResnetFiveZeroSslFoureoflairCoarseLOne}{\tbd{retCIResnetFiveZeroSslFoureoflairCoarseLOne}}
\providecommand{\retCIResnetFiveZeroSslFoureoflairCoarseLTwo}{\tbd{retCIResnetFiveZeroSslFoureoflairCoarseLTwo}}
\providecommand{\retCIResnetFiveZeroSslFoureoflairOmissionLOne}{\tbd{retCIResnetFiveZeroSslFoureoflairOmissionLOne}}
\providecommand{\retCIResnetFiveZeroSslFoureoflairOmissionLTwo}{\tbd{retCIResnetFiveZeroSslFoureoflairOmissionLTwo}}
\providecommand{\retCIResnetFiveZeroSslFoureoflairShiftLOne}{\tbd{retCIResnetFiveZeroSslFoureoflairShiftLOne}}
\providecommand{\retCIResnetFiveZeroSslFoureoflairShiftLTwo}{\tbd{retCIResnetFiveZeroSslFoureoflairShiftLTwo}}
\providecommand{\retCISATChesBoundaryLOne}{\tbd{retCISATChesBoundaryLOne}}
\providecommand{\retCISATChesBoundaryLTwo}{\tbd{retCISATChesBoundaryLTwo}}
\providecommand{\retCISATChesBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retCISATChesBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATChesBoundaryLTwoVarDecoderSamLite}{\tbd{retCISATChesBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retCISATChesBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retCISATChesBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retCISATChesBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATChesBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATChesCoarseLOne}{\tbd{retCISATChesCoarseLOne}}
\providecommand{\retCISATChesCoarseLTwo}{\tbd{retCISATChesCoarseLTwo}}
\providecommand{\retCISATChesCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retCISATChesCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATChesCoarseLTwoVarDecoderSamLite}{\tbd{retCISATChesCoarseLTwoVarDecoderSamLite}}
\providecommand{\retCISATChesCoarseLTwoVarDecoderSegformerMlp}{\tbd{retCISATChesCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retCISATChesCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATChesCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATChesNlcdREAL}{\tbd{retCISATChesNlcdREAL}}
\providecommand{\retCISATChesOmissionLOne}{\tbd{retCISATChesOmissionLOne}}
\providecommand{\retCISATChesOmissionLTwo}{\tbd{retCISATChesOmissionLTwo}}
\providecommand{\retCISATChesOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retCISATChesOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATChesOmissionLTwoVarDecoderSamLite}{\tbd{retCISATChesOmissionLTwoVarDecoderSamLite}}
\providecommand{\retCISATChesOmissionLTwoVarDecoderSegformerMlp}{\tbd{retCISATChesOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retCISATChesOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATChesOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATChesShiftLOne}{\tbd{retCISATChesShiftLOne}}
\providecommand{\retCISATChesShiftLTwo}{\tbd{retCISATChesShiftLTwo}}
\providecommand{\retCISATChesShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retCISATChesShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATChesShiftLTwoVarDecoderSamLite}{\tbd{retCISATChesShiftLTwoVarDecoderSamLite}}
\providecommand{\retCISATChesShiftLTwoVarDecoderSegformerMlp}{\tbd{retCISATChesShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retCISATChesShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATChesShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATCsTwelveBoundaryLOne}{\tbd{retCISATCsTwelveBoundaryLOne}}
\providecommand{\retCISATCsTwelveBoundaryLTwo}{\tbd{retCISATCsTwelveBoundaryLTwo}}
\providecommand{\retCISATCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retCISATCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATCsTwelveBoundaryLTwoVarDecoderSamLite}{\tbd{retCISATCsTwelveBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retCISATCsTwelveBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retCISATCsTwelveBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retCISATCsTwelveBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATCsTwelveBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATCsTwelveCoarseLOne}{\tbd{retCISATCsTwelveCoarseLOne}}
\providecommand{\retCISATCsTwelveCoarseLTwo}{\tbd{retCISATCsTwelveCoarseLTwo}}
\providecommand{\retCISATCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retCISATCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATCsTwelveCoarseLTwoVarDecoderSamLite}{\tbd{retCISATCsTwelveCoarseLTwoVarDecoderSamLite}}
\providecommand{\retCISATCsTwelveCoarseLTwoVarDecoderSegformerMlp}{\tbd{retCISATCsTwelveCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retCISATCsTwelveCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATCsTwelveCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATCsTwelveOmissionLOne}{\tbd{retCISATCsTwelveOmissionLOne}}
\providecommand{\retCISATCsTwelveOmissionLTwo}{\tbd{retCISATCsTwelveOmissionLTwo}}
\providecommand{\retCISATCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retCISATCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATCsTwelveOmissionLTwoVarDecoderSamLite}{\tbd{retCISATCsTwelveOmissionLTwoVarDecoderSamLite}}
\providecommand{\retCISATCsTwelveOmissionLTwoVarDecoderSegformerMlp}{\tbd{retCISATCsTwelveOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retCISATCsTwelveOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATCsTwelveOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATCsTwelveSTwocloudlessREAL}{\tbd{retCISATCsTwelveSTwocloudlessREAL}}
\providecommand{\retCISATCsTwelveShiftLOne}{\tbd{retCISATCsTwelveShiftLOne}}
\providecommand{\retCISATCsTwelveShiftLTwo}{\tbd{retCISATCsTwelveShiftLTwo}}
\providecommand{\retCISATCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retCISATCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATCsTwelveShiftLTwoVarDecoderSamLite}{\tbd{retCISATCsTwelveShiftLTwoVarDecoderSamLite}}
\providecommand{\retCISATCsTwelveShiftLTwoVarDecoderSegformerMlp}{\tbd{retCISATCsTwelveShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retCISATCsTwelveShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATCsTwelveShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATDfcBoundaryLOne}{\tbd{retCISATDfcBoundaryLOne}}
\providecommand{\retCISATDfcBoundaryLTwo}{\tbd{retCISATDfcBoundaryLTwo}}
\providecommand{\retCISATDfcBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retCISATDfcBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATDfcBoundaryLTwoVarDecoderSamLite}{\tbd{retCISATDfcBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retCISATDfcBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retCISATDfcBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retCISATDfcBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATDfcBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATDfcCoarseLOne}{\tbd{retCISATDfcCoarseLOne}}
\providecommand{\retCISATDfcCoarseLTwo}{\tbd{retCISATDfcCoarseLTwo}}
\providecommand{\retCISATDfcCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retCISATDfcCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATDfcCoarseLTwoVarDecoderSamLite}{\tbd{retCISATDfcCoarseLTwoVarDecoderSamLite}}
\providecommand{\retCISATDfcCoarseLTwoVarDecoderSegformerMlp}{\tbd{retCISATDfcCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retCISATDfcCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATDfcCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATDfcModisREALVarTrainSubsetRealcov}{\tbd{retCISATDfcModisREALVarTrainSubsetRealcov}}
\providecommand{\retCISATDfcOmissionLOne}{\tbd{retCISATDfcOmissionLOne}}
\providecommand{\retCISATDfcOmissionLTwo}{\tbd{retCISATDfcOmissionLTwo}}
\providecommand{\retCISATDfcOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retCISATDfcOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATDfcOmissionLTwoVarDecoderSamLite}{\tbd{retCISATDfcOmissionLTwoVarDecoderSamLite}}
\providecommand{\retCISATDfcOmissionLTwoVarDecoderSegformerMlp}{\tbd{retCISATDfcOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retCISATDfcOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATDfcOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATDfcShiftLOne}{\tbd{retCISATDfcShiftLOne}}
\providecommand{\retCISATDfcShiftLTwo}{\tbd{retCISATDfcShiftLTwo}}
\providecommand{\retCISATDfcShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retCISATDfcShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATDfcShiftLTwoVarDecoderSamLite}{\tbd{retCISATDfcShiftLTwoVarDecoderSamLite}}
\providecommand{\retCISATDfcShiftLTwoVarDecoderSegformerMlp}{\tbd{retCISATDfcShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retCISATDfcShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATDfcShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATEnvaBoundaryLOne}{\tbd{retCISATEnvaBoundaryLOne}}
\providecommand{\retCISATEnvaBoundaryLTwo}{\tbd{retCISATEnvaBoundaryLTwo}}
\providecommand{\retCISATEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retCISATEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATEnvaBoundaryLTwoVarDecoderSamLite}{\tbd{retCISATEnvaBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retCISATEnvaBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retCISATEnvaBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retCISATEnvaBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATEnvaBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATEnvaCoarseLOne}{\tbd{retCISATEnvaCoarseLOne}}
\providecommand{\retCISATEnvaCoarseLTwo}{\tbd{retCISATEnvaCoarseLTwo}}
\providecommand{\retCISATEnvaCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retCISATEnvaCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATEnvaCoarseLTwoVarDecoderSamLite}{\tbd{retCISATEnvaCoarseLTwoVarDecoderSamLite}}
\providecommand{\retCISATEnvaCoarseLTwoVarDecoderSegformerMlp}{\tbd{retCISATEnvaCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retCISATEnvaCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATEnvaCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATEnvaNlcdREAL}{\tbd{retCISATEnvaNlcdREAL}}
\providecommand{\retCISATEnvaOmissionLOne}{\tbd{retCISATEnvaOmissionLOne}}
\providecommand{\retCISATEnvaOmissionLTwo}{\tbd{retCISATEnvaOmissionLTwo}}
\providecommand{\retCISATEnvaOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retCISATEnvaOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATEnvaOmissionLTwoVarDecoderSamLite}{\tbd{retCISATEnvaOmissionLTwoVarDecoderSamLite}}
\providecommand{\retCISATEnvaOmissionLTwoVarDecoderSegformerMlp}{\tbd{retCISATEnvaOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retCISATEnvaOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATEnvaOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATEnvaShiftLOne}{\tbd{retCISATEnvaShiftLOne}}
\providecommand{\retCISATEnvaShiftLTwo}{\tbd{retCISATEnvaShiftLTwo}}
\providecommand{\retCISATEnvaShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retCISATEnvaShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATEnvaShiftLTwoVarDecoderSamLite}{\tbd{retCISATEnvaShiftLTwoVarDecoderSamLite}}
\providecommand{\retCISATEnvaShiftLTwoVarDecoderSegformerMlp}{\tbd{retCISATEnvaShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retCISATEnvaShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATEnvaShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATKuroBoundaryLOne}{\tbd{retCISATKuroBoundaryLOne}}
\providecommand{\retCISATKuroBoundaryLTwo}{\tbd{retCISATKuroBoundaryLTwo}}
\providecommand{\retCISATKuroBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retCISATKuroBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATKuroBoundaryLTwoVarDecoderSamLite}{\tbd{retCISATKuroBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retCISATKuroBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retCISATKuroBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retCISATKuroBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATKuroBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATKuroCemsREALVarTrainSubsetRealcov}{\tbd{retCISATKuroCemsREALVarTrainSubsetRealcov}}
\providecommand{\retCISATKuroCoarseLOne}{\tbd{retCISATKuroCoarseLOne}}
\providecommand{\retCISATKuroCoarseLTwo}{\tbd{retCISATKuroCoarseLTwo}}
\providecommand{\retCISATKuroCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retCISATKuroCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATKuroCoarseLTwoVarDecoderSamLite}{\tbd{retCISATKuroCoarseLTwoVarDecoderSamLite}}
\providecommand{\retCISATKuroCoarseLTwoVarDecoderSegformerMlp}{\tbd{retCISATKuroCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retCISATKuroCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATKuroCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATKuroOmissionLOne}{\tbd{retCISATKuroOmissionLOne}}
\providecommand{\retCISATKuroOmissionLTwo}{\tbd{retCISATKuroOmissionLTwo}}
\providecommand{\retCISATKuroOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retCISATKuroOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATKuroOmissionLTwoVarDecoderSamLite}{\tbd{retCISATKuroOmissionLTwoVarDecoderSamLite}}
\providecommand{\retCISATKuroOmissionLTwoVarDecoderSegformerMlp}{\tbd{retCISATKuroOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retCISATKuroOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATKuroOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATKuroShiftLOne}{\tbd{retCISATKuroShiftLOne}}
\providecommand{\retCISATKuroShiftLTwo}{\tbd{retCISATKuroShiftLTwo}}
\providecommand{\retCISATKuroShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retCISATKuroShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATKuroShiftLTwoVarDecoderSamLite}{\tbd{retCISATKuroShiftLTwoVarDecoderSamLite}}
\providecommand{\retCISATKuroShiftLTwoVarDecoderSegformerMlp}{\tbd{retCISATKuroShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retCISATKuroShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATKuroShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATOemBoundaryLOne}{\tbd{retCISATOemBoundaryLOne}}
\providecommand{\retCISATOemBoundaryLTwo}{\tbd{retCISATOemBoundaryLTwo}}
\providecommand{\retCISATOemBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retCISATOemBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATOemBoundaryLTwoVarDecoderSamLite}{\tbd{retCISATOemBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retCISATOemBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retCISATOemBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retCISATOemBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATOemBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATOemCoarseLOne}{\tbd{retCISATOemCoarseLOne}}
\providecommand{\retCISATOemCoarseLTwo}{\tbd{retCISATOemCoarseLTwo}}
\providecommand{\retCISATOemCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retCISATOemCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATOemCoarseLTwoVarDecoderSamLite}{\tbd{retCISATOemCoarseLTwoVarDecoderSamLite}}
\providecommand{\retCISATOemCoarseLTwoVarDecoderSegformerMlp}{\tbd{retCISATOemCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retCISATOemCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATOemCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATOemOmissionLOne}{\tbd{retCISATOemOmissionLOne}}
\providecommand{\retCISATOemOmissionLTwo}{\tbd{retCISATOemOmissionLTwo}}
\providecommand{\retCISATOemOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retCISATOemOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATOemOmissionLTwoVarDecoderSamLite}{\tbd{retCISATOemOmissionLTwoVarDecoderSamLite}}
\providecommand{\retCISATOemOmissionLTwoVarDecoderSegformerMlp}{\tbd{retCISATOemOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retCISATOemOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATOemOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATOemShiftLOne}{\tbd{retCISATOemShiftLOne}}
\providecommand{\retCISATOemShiftLTwo}{\tbd{retCISATOemShiftLTwo}}
\providecommand{\retCISATOemShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retCISATOemShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATOemShiftLTwoVarDecoderSamLite}{\tbd{retCISATOemShiftLTwoVarDecoderSamLite}}
\providecommand{\retCISATOemShiftLTwoVarDecoderSegformerMlp}{\tbd{retCISATOemShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retCISATOemShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATOemShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATSnTwoBoundaryLOne}{\tbd{retCISATSnTwoBoundaryLOne}}
\providecommand{\retCISATSnTwoBoundaryLTwo}{\tbd{retCISATSnTwoBoundaryLTwo}}
\providecommand{\retCISATSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retCISATSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATSnTwoBoundaryLTwoVarDecoderSamLite}{\tbd{retCISATSnTwoBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retCISATSnTwoBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retCISATSnTwoBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retCISATSnTwoBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATSnTwoBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATSnTwoCoarseLOne}{\tbd{retCISATSnTwoCoarseLOne}}
\providecommand{\retCISATSnTwoCoarseLTwo}{\tbd{retCISATSnTwoCoarseLTwo}}
\providecommand{\retCISATSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retCISATSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATSnTwoCoarseLTwoVarDecoderSamLite}{\tbd{retCISATSnTwoCoarseLTwoVarDecoderSamLite}}
\providecommand{\retCISATSnTwoCoarseLTwoVarDecoderSegformerMlp}{\tbd{retCISATSnTwoCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retCISATSnTwoCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATSnTwoCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATSnTwoOmissionLOne}{\tbd{retCISATSnTwoOmissionLOne}}
\providecommand{\retCISATSnTwoOmissionLTwo}{\tbd{retCISATSnTwoOmissionLTwo}}
\providecommand{\retCISATSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retCISATSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATSnTwoOmissionLTwoVarDecoderSamLite}{\tbd{retCISATSnTwoOmissionLTwoVarDecoderSamLite}}
\providecommand{\retCISATSnTwoOmissionLTwoVarDecoderSegformerMlp}{\tbd{retCISATSnTwoOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retCISATSnTwoOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATSnTwoOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATSnTwoShiftLOne}{\tbd{retCISATSnTwoShiftLOne}}
\providecommand{\retCISATSnTwoShiftLTwo}{\tbd{retCISATSnTwoShiftLTwo}}
\providecommand{\retCISATSnTwoShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retCISATSnTwoShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATSnTwoShiftLTwoVarDecoderSamLite}{\tbd{retCISATSnTwoShiftLTwoVarDecoderSamLite}}
\providecommand{\retCISATSnTwoShiftLTwoVarDecoderSegformerMlp}{\tbd{retCISATSnTwoShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retCISATSnTwoShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATSnTwoShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATburnBoundaryLOne}{\tbd{retCISATburnBoundaryLOne}}
\providecommand{\retCISATburnBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{retCISATburnBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCISATburnBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{retCISATburnBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATburnBoundaryLOneVarDecoderSamLite}{\tbd{retCISATburnBoundaryLOneVarDecoderSamLite}}
\providecommand{\retCISATburnBoundaryLOneVarDecoderSamPretrained}{\tbd{retCISATburnBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\retCISATburnBoundaryLOneVarDecoderSegformerMlp}{\tbd{retCISATburnBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\retCISATburnBoundaryLR}{\tbd{retCISATburnBoundaryLR}}
\providecommand{\retCISATburnBoundaryLRVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATburnBoundaryLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATburnBoundaryLTwo}{\tbd{retCISATburnBoundaryLTwo}}
\providecommand{\retCISATburnBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{retCISATburnBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCISATburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{retCISATburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATburnBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retCISATburnBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{retCISATburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATburnBoundaryLTwoVarDecoderSamLite}{\tbd{retCISATburnBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retCISATburnBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{retCISATburnBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATburnBoundaryLTwoVarDecoderSamPretrained}{\tbd{retCISATburnBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\retCISATburnBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{retCISATburnBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATburnBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retCISATburnBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retCISATburnBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{retCISATburnBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATburnBoundaryLTwoVarFrozenEncoderTrue}{\tbd{retCISATburnBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\retCISATburnBoundaryLTwoVarLossBootstrap}{\tbd{retCISATburnBoundaryLTwoVarLossBootstrap}}
\providecommand{\retCISATburnBoundaryLTwoVarLossGce}{\tbd{retCISATburnBoundaryLTwoVarLossGce}}
\providecommand{\retCISATburnBoundaryLTwoVarLrMultThree}{\tbd{retCISATburnBoundaryLTwoVarLrMultThree}}
\providecommand{\retCISATburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATburnBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCISATburnBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCISATburnBoundaryLTwoVarValLabelsClean}{\tbd{retCISATburnBoundaryLTwoVarValLabelsClean}}
\providecommand{\retCISATburnCoarseLOne}{\tbd{retCISATburnCoarseLOne}}
\providecommand{\retCISATburnCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{retCISATburnCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCISATburnCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{retCISATburnCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATburnCoarseLOneVarDecoderSamLite}{\tbd{retCISATburnCoarseLOneVarDecoderSamLite}}
\providecommand{\retCISATburnCoarseLOneVarDecoderSamPretrained}{\tbd{retCISATburnCoarseLOneVarDecoderSamPretrained}}
\providecommand{\retCISATburnCoarseLOneVarDecoderSegformerMlp}{\tbd{retCISATburnCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\retCISATburnCoarseLR}{\tbd{retCISATburnCoarseLR}}
\providecommand{\retCISATburnCoarseLRVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATburnCoarseLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATburnCoarseLTwo}{\tbd{retCISATburnCoarseLTwo}}
\providecommand{\retCISATburnCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{retCISATburnCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCISATburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{retCISATburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATburnCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retCISATburnCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{retCISATburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATburnCoarseLTwoVarDecoderSamLite}{\tbd{retCISATburnCoarseLTwoVarDecoderSamLite}}
\providecommand{\retCISATburnCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{retCISATburnCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATburnCoarseLTwoVarDecoderSamPretrained}{\tbd{retCISATburnCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\retCISATburnCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{retCISATburnCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATburnCoarseLTwoVarDecoderSegformerMlp}{\tbd{retCISATburnCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retCISATburnCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{retCISATburnCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATburnCoarseLTwoVarEarlyStoppingFalse}{\tbd{retCISATburnCoarseLTwoVarEarlyStoppingFalse}}
\providecommand{\retCISATburnCoarseLTwoVarEarlyStoppingFalseFrozenEncoderTrue}{\tbd{retCISATburnCoarseLTwoVarEarlyStoppingFalseFrozenEncoderTrue}}
\providecommand{\retCISATburnCoarseLTwoVarFrozenEncoderTrue}{\tbd{retCISATburnCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\retCISATburnCoarseLTwoVarLossBootstrap}{\tbd{retCISATburnCoarseLTwoVarLossBootstrap}}
\providecommand{\retCISATburnCoarseLTwoVarLossGce}{\tbd{retCISATburnCoarseLTwoVarLossGce}}
\providecommand{\retCISATburnCoarseLTwoVarLrMultThree}{\tbd{retCISATburnCoarseLTwoVarLrMultThree}}
\providecommand{\retCISATburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATburnCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCISATburnCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCISATburnCoarseLTwoVarValLabelsClean}{\tbd{retCISATburnCoarseLTwoVarValLabelsClean}}
\providecommand{\retCISATburnOmissionLOne}{\tbd{retCISATburnOmissionLOne}}
\providecommand{\retCISATburnOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{retCISATburnOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCISATburnOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{retCISATburnOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATburnOmissionLOneVarDecoderSamLite}{\tbd{retCISATburnOmissionLOneVarDecoderSamLite}}
\providecommand{\retCISATburnOmissionLOneVarDecoderSamPretrained}{\tbd{retCISATburnOmissionLOneVarDecoderSamPretrained}}
\providecommand{\retCISATburnOmissionLOneVarDecoderSegformerMlp}{\tbd{retCISATburnOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\retCISATburnOmissionLR}{\tbd{retCISATburnOmissionLR}}
\providecommand{\retCISATburnOmissionLRVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATburnOmissionLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATburnOmissionLTwo}{\tbd{retCISATburnOmissionLTwo}}
\providecommand{\retCISATburnOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{retCISATburnOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCISATburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{retCISATburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATburnOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retCISATburnOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{retCISATburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATburnOmissionLTwoVarDecoderSamLite}{\tbd{retCISATburnOmissionLTwoVarDecoderSamLite}}
\providecommand{\retCISATburnOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{retCISATburnOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATburnOmissionLTwoVarDecoderSamPretrained}{\tbd{retCISATburnOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\retCISATburnOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{retCISATburnOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATburnOmissionLTwoVarDecoderSegformerMlp}{\tbd{retCISATburnOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retCISATburnOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{retCISATburnOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATburnOmissionLTwoVarFrozenEncoderTrue}{\tbd{retCISATburnOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\retCISATburnOmissionLTwoVarLossBootstrap}{\tbd{retCISATburnOmissionLTwoVarLossBootstrap}}
\providecommand{\retCISATburnOmissionLTwoVarLossGce}{\tbd{retCISATburnOmissionLTwoVarLossGce}}
\providecommand{\retCISATburnOmissionLTwoVarLrMultThree}{\tbd{retCISATburnOmissionLTwoVarLrMultThree}}
\providecommand{\retCISATburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATburnOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCISATburnOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCISATburnOmissionLTwoVarValLabelsClean}{\tbd{retCISATburnOmissionLTwoVarValLabelsClean}}
\providecommand{\retCISATburnShiftLOne}{\tbd{retCISATburnShiftLOne}}
\providecommand{\retCISATburnShiftLOneVarDecoderMaskTwoformerFull}{\tbd{retCISATburnShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCISATburnShiftLOneVarDecoderMaskTwoformerLite}{\tbd{retCISATburnShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATburnShiftLOneVarDecoderSamLite}{\tbd{retCISATburnShiftLOneVarDecoderSamLite}}
\providecommand{\retCISATburnShiftLOneVarDecoderSamPretrained}{\tbd{retCISATburnShiftLOneVarDecoderSamPretrained}}
\providecommand{\retCISATburnShiftLOneVarDecoderSegformerMlp}{\tbd{retCISATburnShiftLOneVarDecoderSegformerMlp}}
\providecommand{\retCISATburnShiftLR}{\tbd{retCISATburnShiftLR}}
\providecommand{\retCISATburnShiftLRVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATburnShiftLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATburnShiftLTwo}{\tbd{retCISATburnShiftLTwo}}
\providecommand{\retCISATburnShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{retCISATburnShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCISATburnShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{retCISATburnShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATburnShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retCISATburnShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{retCISATburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATburnShiftLTwoVarDecoderSamLite}{\tbd{retCISATburnShiftLTwoVarDecoderSamLite}}
\providecommand{\retCISATburnShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{retCISATburnShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATburnShiftLTwoVarDecoderSamPretrained}{\tbd{retCISATburnShiftLTwoVarDecoderSamPretrained}}
\providecommand{\retCISATburnShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{retCISATburnShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATburnShiftLTwoVarDecoderSegformerMlp}{\tbd{retCISATburnShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retCISATburnShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{retCISATburnShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATburnShiftLTwoVarFrozenEncoderTrue}{\tbd{retCISATburnShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\retCISATburnShiftLTwoVarLossBootstrap}{\tbd{retCISATburnShiftLTwoVarLossBootstrap}}
\providecommand{\retCISATburnShiftLTwoVarLossGce}{\tbd{retCISATburnShiftLTwoVarLossGce}}
\providecommand{\retCISATburnShiftLTwoVarLrMultThree}{\tbd{retCISATburnShiftLTwoVarLrMultThree}}
\providecommand{\retCISATburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATburnShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCISATburnShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCISATburnShiftLTwoVarValLabelsClean}{\tbd{retCISATburnShiftLTwoVarValLabelsClean}}
\providecommand{\retCISATflairBoundaryLOne}{\tbd{retCISATflairBoundaryLOne}}
\providecommand{\retCISATflairBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{retCISATflairBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCISATflairBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{retCISATflairBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATflairBoundaryLOneVarDecoderSamLite}{\tbd{retCISATflairBoundaryLOneVarDecoderSamLite}}
\providecommand{\retCISATflairBoundaryLOneVarDecoderSamPretrained}{\tbd{retCISATflairBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\retCISATflairBoundaryLOneVarDecoderSegformerMlp}{\tbd{retCISATflairBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\retCISATflairBoundaryLR}{\tbd{retCISATflairBoundaryLR}}
\providecommand{\retCISATflairBoundaryLRVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATflairBoundaryLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATflairBoundaryLTwo}{\tbd{retCISATflairBoundaryLTwo}}
\providecommand{\retCISATflairBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{retCISATflairBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCISATflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{retCISATflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATflairBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retCISATflairBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{retCISATflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATflairBoundaryLTwoVarDecoderSamLite}{\tbd{retCISATflairBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retCISATflairBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{retCISATflairBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATflairBoundaryLTwoVarDecoderSamPretrained}{\tbd{retCISATflairBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\retCISATflairBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{retCISATflairBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATflairBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retCISATflairBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retCISATflairBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{retCISATflairBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATflairBoundaryLTwoVarFrozenEncoderTrue}{\tbd{retCISATflairBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\retCISATflairBoundaryLTwoVarLossBootstrap}{\tbd{retCISATflairBoundaryLTwoVarLossBootstrap}}
\providecommand{\retCISATflairBoundaryLTwoVarLossGce}{\tbd{retCISATflairBoundaryLTwoVarLossGce}}
\providecommand{\retCISATflairBoundaryLTwoVarLrMultThree}{\tbd{retCISATflairBoundaryLTwoVarLrMultThree}}
\providecommand{\retCISATflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATflairBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCISATflairBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCISATflairBoundaryLTwoVarValLabelsClean}{\tbd{retCISATflairBoundaryLTwoVarValLabelsClean}}
\providecommand{\retCISATflairCoarseLOne}{\tbd{retCISATflairCoarseLOne}}
\providecommand{\retCISATflairCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{retCISATflairCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCISATflairCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{retCISATflairCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATflairCoarseLOneVarDecoderSamLite}{\tbd{retCISATflairCoarseLOneVarDecoderSamLite}}
\providecommand{\retCISATflairCoarseLOneVarDecoderSamPretrained}{\tbd{retCISATflairCoarseLOneVarDecoderSamPretrained}}
\providecommand{\retCISATflairCoarseLOneVarDecoderSegformerMlp}{\tbd{retCISATflairCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\retCISATflairCoarseLR}{\tbd{retCISATflairCoarseLR}}
\providecommand{\retCISATflairCoarseLRVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATflairCoarseLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATflairCoarseLTwo}{\tbd{retCISATflairCoarseLTwo}}
\providecommand{\retCISATflairCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{retCISATflairCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCISATflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{retCISATflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATflairCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retCISATflairCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{retCISATflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATflairCoarseLTwoVarDecoderSamLite}{\tbd{retCISATflairCoarseLTwoVarDecoderSamLite}}
\providecommand{\retCISATflairCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{retCISATflairCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATflairCoarseLTwoVarDecoderSamPretrained}{\tbd{retCISATflairCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\retCISATflairCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{retCISATflairCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATflairCoarseLTwoVarDecoderSegformerMlp}{\tbd{retCISATflairCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retCISATflairCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{retCISATflairCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATflairCoarseLTwoVarFrozenEncoderTrue}{\tbd{retCISATflairCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\retCISATflairCoarseLTwoVarLossBootstrap}{\tbd{retCISATflairCoarseLTwoVarLossBootstrap}}
\providecommand{\retCISATflairCoarseLTwoVarLossGce}{\tbd{retCISATflairCoarseLTwoVarLossGce}}
\providecommand{\retCISATflairCoarseLTwoVarLrMultThree}{\tbd{retCISATflairCoarseLTwoVarLrMultThree}}
\providecommand{\retCISATflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATflairCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCISATflairCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCISATflairCoarseLTwoVarValLabelsClean}{\tbd{retCISATflairCoarseLTwoVarValLabelsClean}}
\providecommand{\retCISATflairOmissionLOne}{\tbd{retCISATflairOmissionLOne}}
\providecommand{\retCISATflairOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{retCISATflairOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCISATflairOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{retCISATflairOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATflairOmissionLOneVarDecoderSamLite}{\tbd{retCISATflairOmissionLOneVarDecoderSamLite}}
\providecommand{\retCISATflairOmissionLOneVarDecoderSamPretrained}{\tbd{retCISATflairOmissionLOneVarDecoderSamPretrained}}
\providecommand{\retCISATflairOmissionLOneVarDecoderSegformerMlp}{\tbd{retCISATflairOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\retCISATflairOmissionLR}{\tbd{retCISATflairOmissionLR}}
\providecommand{\retCISATflairOmissionLRVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATflairOmissionLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATflairOmissionLTwo}{\tbd{retCISATflairOmissionLTwo}}
\providecommand{\retCISATflairOmissionLTwoVarClassWeightedTrue}{\tbd{retCISATflairOmissionLTwoVarClassWeightedTrue}}
\providecommand{\retCISATflairOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{retCISATflairOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCISATflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{retCISATflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATflairOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retCISATflairOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{retCISATflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATflairOmissionLTwoVarDecoderSamLite}{\tbd{retCISATflairOmissionLTwoVarDecoderSamLite}}
\providecommand{\retCISATflairOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{retCISATflairOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATflairOmissionLTwoVarDecoderSamPretrained}{\tbd{retCISATflairOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\retCISATflairOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{retCISATflairOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATflairOmissionLTwoVarDecoderSegformerMlp}{\tbd{retCISATflairOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retCISATflairOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{retCISATflairOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATflairOmissionLTwoVarEarlyStoppingFalse}{\tbd{retCISATflairOmissionLTwoVarEarlyStoppingFalse}}
\providecommand{\retCISATflairOmissionLTwoVarEarlyStoppingFalseFrozenEncoderTrue}{\tbd{retCISATflairOmissionLTwoVarEarlyStoppingFalseFrozenEncoderTrue}}
\providecommand{\retCISATflairOmissionLTwoVarFrozenEncoderTrue}{\tbd{retCISATflairOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\retCISATflairOmissionLTwoVarLossBootstrap}{\tbd{retCISATflairOmissionLTwoVarLossBootstrap}}
\providecommand{\retCISATflairOmissionLTwoVarLossGce}{\tbd{retCISATflairOmissionLTwoVarLossGce}}
\providecommand{\retCISATflairOmissionLTwoVarLrMultThree}{\tbd{retCISATflairOmissionLTwoVarLrMultThree}}
\providecommand{\retCISATflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATflairOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCISATflairOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCISATflairOmissionLTwoVarValLabelsClean}{\tbd{retCISATflairOmissionLTwoVarValLabelsClean}}
\providecommand{\retCISATflairShiftLOne}{\tbd{retCISATflairShiftLOne}}
\providecommand{\retCISATflairShiftLOneVarDecoderMaskTwoformerFull}{\tbd{retCISATflairShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCISATflairShiftLOneVarDecoderMaskTwoformerLite}{\tbd{retCISATflairShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATflairShiftLOneVarDecoderSamLite}{\tbd{retCISATflairShiftLOneVarDecoderSamLite}}
\providecommand{\retCISATflairShiftLOneVarDecoderSamPretrained}{\tbd{retCISATflairShiftLOneVarDecoderSamPretrained}}
\providecommand{\retCISATflairShiftLOneVarDecoderSegformerMlp}{\tbd{retCISATflairShiftLOneVarDecoderSegformerMlp}}
\providecommand{\retCISATflairShiftLR}{\tbd{retCISATflairShiftLR}}
\providecommand{\retCISATflairShiftLRVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATflairShiftLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATflairShiftLTwo}{\tbd{retCISATflairShiftLTwo}}
\providecommand{\retCISATflairShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{retCISATflairShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCISATflairShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{retCISATflairShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATflairShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retCISATflairShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCISATflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{retCISATflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATflairShiftLTwoVarDecoderSamLite}{\tbd{retCISATflairShiftLTwoVarDecoderSamLite}}
\providecommand{\retCISATflairShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{retCISATflairShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATflairShiftLTwoVarDecoderSamPretrained}{\tbd{retCISATflairShiftLTwoVarDecoderSamPretrained}}
\providecommand{\retCISATflairShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{retCISATflairShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATflairShiftLTwoVarDecoderSegformerMlp}{\tbd{retCISATflairShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retCISATflairShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{retCISATflairShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATflairShiftLTwoVarFrozenEncoderTrue}{\tbd{retCISATflairShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\retCISATflairShiftLTwoVarLossBootstrap}{\tbd{retCISATflairShiftLTwoVarLossBootstrap}}
\providecommand{\retCISATflairShiftLTwoVarLossGce}{\tbd{retCISATflairShiftLTwoVarLossGce}}
\providecommand{\retCISATflairShiftLTwoVarLrMultThree}{\tbd{retCISATflairShiftLTwoVarLrMultThree}}
\providecommand{\retCISATflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCISATflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCISATflairShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCISATflairShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCISATflairShiftLTwoVarValLabelsClean}{\tbd{retCISATflairShiftLTwoVarValLabelsClean}}
\providecommand{\retCISATsenOtsuLTwo}{\tbd{retCISATsenOtsuLTwo}}
\providecommand{\retCITMChesBoundaryLOne}{\tbd{retCITMChesBoundaryLOne}}
\providecommand{\retCITMChesBoundaryLTwo}{\tbd{retCITMChesBoundaryLTwo}}
\providecommand{\retCITMChesCoarseLOne}{\tbd{retCITMChesCoarseLOne}}
\providecommand{\retCITMChesCoarseLTwo}{\tbd{retCITMChesCoarseLTwo}}
\providecommand{\retCITMChesNlcdREAL}{\tbd{retCITMChesNlcdREAL}}
\providecommand{\retCITMChesOmissionLOne}{\tbd{retCITMChesOmissionLOne}}
\providecommand{\retCITMChesOmissionLTwo}{\tbd{retCITMChesOmissionLTwo}}
\providecommand{\retCITMChesShiftLOne}{\tbd{retCITMChesShiftLOne}}
\providecommand{\retCITMChesShiftLTwo}{\tbd{retCITMChesShiftLTwo}}
\providecommand{\retCITMCsTwelveBoundaryLOne}{\tbd{retCITMCsTwelveBoundaryLOne}}
\providecommand{\retCITMCsTwelveBoundaryLTwo}{\tbd{retCITMCsTwelveBoundaryLTwo}}
\providecommand{\retCITMCsTwelveCoarseLOne}{\tbd{retCITMCsTwelveCoarseLOne}}
\providecommand{\retCITMCsTwelveCoarseLTwo}{\tbd{retCITMCsTwelveCoarseLTwo}}
\providecommand{\retCITMCsTwelveOmissionLOne}{\tbd{retCITMCsTwelveOmissionLOne}}
\providecommand{\retCITMCsTwelveOmissionLTwo}{\tbd{retCITMCsTwelveOmissionLTwo}}
\providecommand{\retCITMCsTwelveSTwocloudlessREAL}{\tbd{retCITMCsTwelveSTwocloudlessREAL}}
\providecommand{\retCITMCsTwelveShiftLOne}{\tbd{retCITMCsTwelveShiftLOne}}
\providecommand{\retCITMCsTwelveShiftLTwo}{\tbd{retCITMCsTwelveShiftLTwo}}
\providecommand{\retCITMDfcBoundaryLOne}{\tbd{retCITMDfcBoundaryLOne}}
\providecommand{\retCITMDfcBoundaryLTwo}{\tbd{retCITMDfcBoundaryLTwo}}
\providecommand{\retCITMDfcCoarseLOne}{\tbd{retCITMDfcCoarseLOne}}
\providecommand{\retCITMDfcCoarseLTwo}{\tbd{retCITMDfcCoarseLTwo}}
\providecommand{\retCITMDfcModisREALVarTrainSubsetRealcov}{\tbd{retCITMDfcModisREALVarTrainSubsetRealcov}}
\providecommand{\retCITMDfcOmissionLOne}{\tbd{retCITMDfcOmissionLOne}}
\providecommand{\retCITMDfcOmissionLTwo}{\tbd{retCITMDfcOmissionLTwo}}
\providecommand{\retCITMDfcShiftLOne}{\tbd{retCITMDfcShiftLOne}}
\providecommand{\retCITMDfcShiftLTwo}{\tbd{retCITMDfcShiftLTwo}}
\providecommand{\retCITMEnvaBoundaryLOne}{\tbd{retCITMEnvaBoundaryLOne}}
\providecommand{\retCITMEnvaBoundaryLTwo}{\tbd{retCITMEnvaBoundaryLTwo}}
\providecommand{\retCITMEnvaCoarseLOne}{\tbd{retCITMEnvaCoarseLOne}}
\providecommand{\retCITMEnvaCoarseLTwo}{\tbd{retCITMEnvaCoarseLTwo}}
\providecommand{\retCITMEnvaNlcdREAL}{\tbd{retCITMEnvaNlcdREAL}}
\providecommand{\retCITMEnvaOmissionLOne}{\tbd{retCITMEnvaOmissionLOne}}
\providecommand{\retCITMEnvaOmissionLTwo}{\tbd{retCITMEnvaOmissionLTwo}}
\providecommand{\retCITMEnvaShiftLOne}{\tbd{retCITMEnvaShiftLOne}}
\providecommand{\retCITMEnvaShiftLTwo}{\tbd{retCITMEnvaShiftLTwo}}
\providecommand{\retCITMKuroBoundaryLOne}{\tbd{retCITMKuroBoundaryLOne}}
\providecommand{\retCITMKuroBoundaryLTwo}{\tbd{retCITMKuroBoundaryLTwo}}
\providecommand{\retCITMKuroCemsREALVarTrainSubsetRealcov}{\tbd{retCITMKuroCemsREALVarTrainSubsetRealcov}}
\providecommand{\retCITMKuroCoarseLOne}{\tbd{retCITMKuroCoarseLOne}}
\providecommand{\retCITMKuroCoarseLTwo}{\tbd{retCITMKuroCoarseLTwo}}
\providecommand{\retCITMKuroOmissionLOne}{\tbd{retCITMKuroOmissionLOne}}
\providecommand{\retCITMKuroOmissionLTwo}{\tbd{retCITMKuroOmissionLTwo}}
\providecommand{\retCITMKuroShiftLOne}{\tbd{retCITMKuroShiftLOne}}
\providecommand{\retCITMKuroShiftLTwo}{\tbd{retCITMKuroShiftLTwo}}
\providecommand{\retCITMOemBoundaryLOne}{\tbd{retCITMOemBoundaryLOne}}
\providecommand{\retCITMOemBoundaryLTwo}{\tbd{retCITMOemBoundaryLTwo}}
\providecommand{\retCITMOemCoarseLOne}{\tbd{retCITMOemCoarseLOne}}
\providecommand{\retCITMOemCoarseLTwo}{\tbd{retCITMOemCoarseLTwo}}
\providecommand{\retCITMOemOmissionLOne}{\tbd{retCITMOemOmissionLOne}}
\providecommand{\retCITMOemOmissionLTwo}{\tbd{retCITMOemOmissionLTwo}}
\providecommand{\retCITMOemShiftLOne}{\tbd{retCITMOemShiftLOne}}
\providecommand{\retCITMOemShiftLTwo}{\tbd{retCITMOemShiftLTwo}}
\providecommand{\retCITMSnTwoBoundaryLOne}{\tbd{retCITMSnTwoBoundaryLOne}}
\providecommand{\retCITMSnTwoBoundaryLTwo}{\tbd{retCITMSnTwoBoundaryLTwo}}
\providecommand{\retCITMSnTwoCoarseLOne}{\tbd{retCITMSnTwoCoarseLOne}}
\providecommand{\retCITMSnTwoCoarseLTwo}{\tbd{retCITMSnTwoCoarseLTwo}}
\providecommand{\retCITMSnTwoOmissionLOne}{\tbd{retCITMSnTwoOmissionLOne}}
\providecommand{\retCITMSnTwoOmissionLTwo}{\tbd{retCITMSnTwoOmissionLTwo}}
\providecommand{\retCITMSnTwoShiftLOne}{\tbd{retCITMSnTwoShiftLOne}}
\providecommand{\retCITMSnTwoShiftLTwo}{\tbd{retCITMSnTwoShiftLTwo}}
\providecommand{\retCITMburnBoundaryLOne}{\tbd{retCITMburnBoundaryLOne}}
\providecommand{\retCITMburnBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{retCITMburnBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCITMburnBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{retCITMburnBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCITMburnBoundaryLOneVarDecoderSamLite}{\tbd{retCITMburnBoundaryLOneVarDecoderSamLite}}
\providecommand{\retCITMburnBoundaryLOneVarDecoderSamPretrained}{\tbd{retCITMburnBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\retCITMburnBoundaryLOneVarDecoderSegformerMlp}{\tbd{retCITMburnBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\retCITMburnBoundaryLR}{\tbd{retCITMburnBoundaryLR}}
\providecommand{\retCITMburnBoundaryLTwo}{\tbd{retCITMburnBoundaryLTwo}}
\providecommand{\retCITMburnBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{retCITMburnBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCITMburnBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retCITMburnBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCITMburnBoundaryLTwoVarDecoderSamLite}{\tbd{retCITMburnBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retCITMburnBoundaryLTwoVarDecoderSamPretrained}{\tbd{retCITMburnBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\retCITMburnBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retCITMburnBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retCITMburnBoundaryLTwoVarFrozenEncoderTrue}{\tbd{retCITMburnBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\retCITMburnBoundaryLTwoVarLossBootstrap}{\tbd{retCITMburnBoundaryLTwoVarLossBootstrap}}
\providecommand{\retCITMburnBoundaryLTwoVarLossGce}{\tbd{retCITMburnBoundaryLTwoVarLossGce}}
\providecommand{\retCITMburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCITMburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCITMburnBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCITMburnBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCITMburnCoarseLOne}{\tbd{retCITMburnCoarseLOne}}
\providecommand{\retCITMburnCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{retCITMburnCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCITMburnCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{retCITMburnCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCITMburnCoarseLOneVarDecoderSamLite}{\tbd{retCITMburnCoarseLOneVarDecoderSamLite}}
\providecommand{\retCITMburnCoarseLOneVarDecoderSamPretrained}{\tbd{retCITMburnCoarseLOneVarDecoderSamPretrained}}
\providecommand{\retCITMburnCoarseLOneVarDecoderSegformerMlp}{\tbd{retCITMburnCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\retCITMburnCoarseLR}{\tbd{retCITMburnCoarseLR}}
\providecommand{\retCITMburnCoarseLTwo}{\tbd{retCITMburnCoarseLTwo}}
\providecommand{\retCITMburnCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{retCITMburnCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCITMburnCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retCITMburnCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCITMburnCoarseLTwoVarDecoderSamLite}{\tbd{retCITMburnCoarseLTwoVarDecoderSamLite}}
\providecommand{\retCITMburnCoarseLTwoVarDecoderSamPretrained}{\tbd{retCITMburnCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\retCITMburnCoarseLTwoVarDecoderSegformerMlp}{\tbd{retCITMburnCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retCITMburnCoarseLTwoVarFrozenEncoderTrue}{\tbd{retCITMburnCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\retCITMburnCoarseLTwoVarLossBootstrap}{\tbd{retCITMburnCoarseLTwoVarLossBootstrap}}
\providecommand{\retCITMburnCoarseLTwoVarLossGce}{\tbd{retCITMburnCoarseLTwoVarLossGce}}
\providecommand{\retCITMburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCITMburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCITMburnCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCITMburnCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCITMburnOmissionLOne}{\tbd{retCITMburnOmissionLOne}}
\providecommand{\retCITMburnOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{retCITMburnOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCITMburnOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{retCITMburnOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCITMburnOmissionLOneVarDecoderSamLite}{\tbd{retCITMburnOmissionLOneVarDecoderSamLite}}
\providecommand{\retCITMburnOmissionLOneVarDecoderSamPretrained}{\tbd{retCITMburnOmissionLOneVarDecoderSamPretrained}}
\providecommand{\retCITMburnOmissionLOneVarDecoderSegformerMlp}{\tbd{retCITMburnOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\retCITMburnOmissionLR}{\tbd{retCITMburnOmissionLR}}
\providecommand{\retCITMburnOmissionLTwo}{\tbd{retCITMburnOmissionLTwo}}
\providecommand{\retCITMburnOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{retCITMburnOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCITMburnOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retCITMburnOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCITMburnOmissionLTwoVarDecoderSamLite}{\tbd{retCITMburnOmissionLTwoVarDecoderSamLite}}
\providecommand{\retCITMburnOmissionLTwoVarDecoderSamPretrained}{\tbd{retCITMburnOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\retCITMburnOmissionLTwoVarDecoderSegformerMlp}{\tbd{retCITMburnOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retCITMburnOmissionLTwoVarFrozenEncoderTrue}{\tbd{retCITMburnOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\retCITMburnOmissionLTwoVarLossBootstrap}{\tbd{retCITMburnOmissionLTwoVarLossBootstrap}}
\providecommand{\retCITMburnOmissionLTwoVarLossGce}{\tbd{retCITMburnOmissionLTwoVarLossGce}}
\providecommand{\retCITMburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCITMburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCITMburnOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCITMburnOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCITMburnShiftLOne}{\tbd{retCITMburnShiftLOne}}
\providecommand{\retCITMburnShiftLOneVarDecoderMaskTwoformerFull}{\tbd{retCITMburnShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCITMburnShiftLOneVarDecoderMaskTwoformerLite}{\tbd{retCITMburnShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCITMburnShiftLOneVarDecoderSamLite}{\tbd{retCITMburnShiftLOneVarDecoderSamLite}}
\providecommand{\retCITMburnShiftLOneVarDecoderSamPretrained}{\tbd{retCITMburnShiftLOneVarDecoderSamPretrained}}
\providecommand{\retCITMburnShiftLOneVarDecoderSegformerMlp}{\tbd{retCITMburnShiftLOneVarDecoderSegformerMlp}}
\providecommand{\retCITMburnShiftLR}{\tbd{retCITMburnShiftLR}}
\providecommand{\retCITMburnShiftLTwo}{\tbd{retCITMburnShiftLTwo}}
\providecommand{\retCITMburnShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{retCITMburnShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCITMburnShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retCITMburnShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCITMburnShiftLTwoVarDecoderSamLite}{\tbd{retCITMburnShiftLTwoVarDecoderSamLite}}
\providecommand{\retCITMburnShiftLTwoVarDecoderSamPretrained}{\tbd{retCITMburnShiftLTwoVarDecoderSamPretrained}}
\providecommand{\retCITMburnShiftLTwoVarDecoderSegformerMlp}{\tbd{retCITMburnShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retCITMburnShiftLTwoVarFrozenEncoderTrue}{\tbd{retCITMburnShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\retCITMburnShiftLTwoVarLossBootstrap}{\tbd{retCITMburnShiftLTwoVarLossBootstrap}}
\providecommand{\retCITMburnShiftLTwoVarLossGce}{\tbd{retCITMburnShiftLTwoVarLossGce}}
\providecommand{\retCITMburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCITMburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCITMburnShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCITMburnShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCITMflairBoundaryLOne}{\tbd{retCITMflairBoundaryLOne}}
\providecommand{\retCITMflairBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{retCITMflairBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCITMflairBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{retCITMflairBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCITMflairBoundaryLOneVarDecoderSamLite}{\tbd{retCITMflairBoundaryLOneVarDecoderSamLite}}
\providecommand{\retCITMflairBoundaryLOneVarDecoderSamPretrained}{\tbd{retCITMflairBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\retCITMflairBoundaryLOneVarDecoderSegformerMlp}{\tbd{retCITMflairBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\retCITMflairBoundaryLR}{\tbd{retCITMflairBoundaryLR}}
\providecommand{\retCITMflairBoundaryLTwo}{\tbd{retCITMflairBoundaryLTwo}}
\providecommand{\retCITMflairBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{retCITMflairBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCITMflairBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retCITMflairBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCITMflairBoundaryLTwoVarDecoderSamLite}{\tbd{retCITMflairBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retCITMflairBoundaryLTwoVarDecoderSamPretrained}{\tbd{retCITMflairBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\retCITMflairBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retCITMflairBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retCITMflairBoundaryLTwoVarFrozenEncoderTrue}{\tbd{retCITMflairBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\retCITMflairBoundaryLTwoVarLossBootstrap}{\tbd{retCITMflairBoundaryLTwoVarLossBootstrap}}
\providecommand{\retCITMflairBoundaryLTwoVarLossGce}{\tbd{retCITMflairBoundaryLTwoVarLossGce}}
\providecommand{\retCITMflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCITMflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCITMflairBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCITMflairBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCITMflairCoarseLOne}{\tbd{retCITMflairCoarseLOne}}
\providecommand{\retCITMflairCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{retCITMflairCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCITMflairCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{retCITMflairCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCITMflairCoarseLOneVarDecoderSamLite}{\tbd{retCITMflairCoarseLOneVarDecoderSamLite}}
\providecommand{\retCITMflairCoarseLOneVarDecoderSamPretrained}{\tbd{retCITMflairCoarseLOneVarDecoderSamPretrained}}
\providecommand{\retCITMflairCoarseLOneVarDecoderSegformerMlp}{\tbd{retCITMflairCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\retCITMflairCoarseLR}{\tbd{retCITMflairCoarseLR}}
\providecommand{\retCITMflairCoarseLTwo}{\tbd{retCITMflairCoarseLTwo}}
\providecommand{\retCITMflairCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{retCITMflairCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCITMflairCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retCITMflairCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCITMflairCoarseLTwoVarDecoderSamLite}{\tbd{retCITMflairCoarseLTwoVarDecoderSamLite}}
\providecommand{\retCITMflairCoarseLTwoVarDecoderSamPretrained}{\tbd{retCITMflairCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\retCITMflairCoarseLTwoVarDecoderSegformerMlp}{\tbd{retCITMflairCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retCITMflairCoarseLTwoVarFrozenEncoderTrue}{\tbd{retCITMflairCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\retCITMflairCoarseLTwoVarLossBootstrap}{\tbd{retCITMflairCoarseLTwoVarLossBootstrap}}
\providecommand{\retCITMflairCoarseLTwoVarLossGce}{\tbd{retCITMflairCoarseLTwoVarLossGce}}
\providecommand{\retCITMflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCITMflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCITMflairCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCITMflairCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCITMflairOmissionLOne}{\tbd{retCITMflairOmissionLOne}}
\providecommand{\retCITMflairOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{retCITMflairOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCITMflairOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{retCITMflairOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCITMflairOmissionLOneVarDecoderSamLite}{\tbd{retCITMflairOmissionLOneVarDecoderSamLite}}
\providecommand{\retCITMflairOmissionLOneVarDecoderSamPretrained}{\tbd{retCITMflairOmissionLOneVarDecoderSamPretrained}}
\providecommand{\retCITMflairOmissionLOneVarDecoderSegformerMlp}{\tbd{retCITMflairOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\retCITMflairOmissionLR}{\tbd{retCITMflairOmissionLR}}
\providecommand{\retCITMflairOmissionLTwo}{\tbd{retCITMflairOmissionLTwo}}
\providecommand{\retCITMflairOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{retCITMflairOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCITMflairOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retCITMflairOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCITMflairOmissionLTwoVarDecoderSamLite}{\tbd{retCITMflairOmissionLTwoVarDecoderSamLite}}
\providecommand{\retCITMflairOmissionLTwoVarDecoderSamPretrained}{\tbd{retCITMflairOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\retCITMflairOmissionLTwoVarDecoderSegformerMlp}{\tbd{retCITMflairOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retCITMflairOmissionLTwoVarFrozenEncoderTrue}{\tbd{retCITMflairOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\retCITMflairOmissionLTwoVarLossBootstrap}{\tbd{retCITMflairOmissionLTwoVarLossBootstrap}}
\providecommand{\retCITMflairOmissionLTwoVarLossGce}{\tbd{retCITMflairOmissionLTwoVarLossGce}}
\providecommand{\retCITMflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCITMflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCITMflairOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCITMflairOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCITMflairShiftLOne}{\tbd{retCITMflairShiftLOne}}
\providecommand{\retCITMflairShiftLOneVarDecoderMaskTwoformerFull}{\tbd{retCITMflairShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retCITMflairShiftLOneVarDecoderMaskTwoformerLite}{\tbd{retCITMflairShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retCITMflairShiftLOneVarDecoderSamLite}{\tbd{retCITMflairShiftLOneVarDecoderSamLite}}
\providecommand{\retCITMflairShiftLOneVarDecoderSamPretrained}{\tbd{retCITMflairShiftLOneVarDecoderSamPretrained}}
\providecommand{\retCITMflairShiftLOneVarDecoderSegformerMlp}{\tbd{retCITMflairShiftLOneVarDecoderSegformerMlp}}
\providecommand{\retCITMflairShiftLR}{\tbd{retCITMflairShiftLR}}
\providecommand{\retCITMflairShiftLTwo}{\tbd{retCITMflairShiftLTwo}}
\providecommand{\retCITMflairShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{retCITMflairShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retCITMflairShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retCITMflairShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retCITMflairShiftLTwoVarDecoderSamLite}{\tbd{retCITMflairShiftLTwoVarDecoderSamLite}}
\providecommand{\retCITMflairShiftLTwoVarDecoderSamPretrained}{\tbd{retCITMflairShiftLTwoVarDecoderSamPretrained}}
\providecommand{\retCITMflairShiftLTwoVarDecoderSegformerMlp}{\tbd{retCITMflairShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retCITMflairShiftLTwoVarFrozenEncoderTrue}{\tbd{retCITMflairShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\retCITMflairShiftLTwoVarLossBootstrap}{\tbd{retCITMflairShiftLTwoVarLossBootstrap}}
\providecommand{\retCITMflairShiftLTwoVarLossGce}{\tbd{retCITMflairShiftLTwoVarLossGce}}
\providecommand{\retCITMflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retCITMflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retCITMflairShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{retCITMflairShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retCITMsenOtsuLTwo}{\tbd{retCITMsenOtsuLTwo}}
\providecommand{\retCIVitlRandomburnBoundaryLOneVarInitRandom}{\tbd{retCIVitlRandomburnBoundaryLOneVarInitRandom}}
\providecommand{\retCIVitlRandomburnBoundaryLTwoVarInitRandom}{\tbd{retCIVitlRandomburnBoundaryLTwoVarInitRandom}}
\providecommand{\retCIVitlRandomburnCoarseLOneVarInitRandom}{\tbd{retCIVitlRandomburnCoarseLOneVarInitRandom}}
\providecommand{\retCIVitlRandomburnCoarseLTwoVarInitRandom}{\tbd{retCIVitlRandomburnCoarseLTwoVarInitRandom}}
\providecommand{\retCIVitlRandomburnOmissionLOneVarInitRandom}{\tbd{retCIVitlRandomburnOmissionLOneVarInitRandom}}
\providecommand{\retCIVitlRandomburnOmissionLTwoVarInitRandom}{\tbd{retCIVitlRandomburnOmissionLTwoVarInitRandom}}
\providecommand{\retCIVitlRandomburnShiftLOneVarInitRandom}{\tbd{retCIVitlRandomburnShiftLOneVarInitRandom}}
\providecommand{\retCIVitlRandomburnShiftLTwoVarInitRandom}{\tbd{retCIVitlRandomburnShiftLTwoVarInitRandom}}
\providecommand{\retCIVitlRandomflairBoundaryLOneVarInitRandom}{\tbd{retCIVitlRandomflairBoundaryLOneVarInitRandom}}
\providecommand{\retCIVitlRandomflairBoundaryLTwoVarInitRandom}{\tbd{retCIVitlRandomflairBoundaryLTwoVarInitRandom}}
\providecommand{\retCIVitlRandomflairCoarseLOneVarInitRandom}{\tbd{retCIVitlRandomflairCoarseLOneVarInitRandom}}
\providecommand{\retCIVitlRandomflairCoarseLTwoVarInitRandom}{\tbd{retCIVitlRandomflairCoarseLTwoVarInitRandom}}
\providecommand{\retCIVitlRandomflairOmissionLOneVarInitRandom}{\tbd{retCIVitlRandomflairOmissionLOneVarInitRandom}}
\providecommand{\retCIVitlRandomflairOmissionLTwoVarInitRandom}{\tbd{retCIVitlRandomflairOmissionLTwoVarInitRandom}}
\providecommand{\retCIVitlRandomflairShiftLOneVarInitRandom}{\tbd{retCIVitlRandomflairShiftLOneVarInitRandom}}
\providecommand{\retCIVitlRandomflairShiftLTwoVarInitRandom}{\tbd{retCIVitlRandomflairShiftLTwoVarInitRandom}}
\providecommand{\retDOFAChesBoundaryLOne}{\tbd{retDOFAChesBoundaryLOne}}
\providecommand{\retDOFAChesBoundaryLTwo}{\tbd{retDOFAChesBoundaryLTwo}}
\providecommand{\retDOFAChesCoarseLOne}{\tbd{retDOFAChesCoarseLOne}}
\providecommand{\retDOFAChesCoarseLTwo}{\tbd{retDOFAChesCoarseLTwo}}
\providecommand{\retDOFAChesNlcdREAL}{\tbd{retDOFAChesNlcdREAL}}
\providecommand{\retDOFAChesOmissionLOne}{\tbd{retDOFAChesOmissionLOne}}
\providecommand{\retDOFAChesOmissionLTwo}{\tbd{retDOFAChesOmissionLTwo}}
\providecommand{\retDOFAChesShiftLOne}{\tbd{retDOFAChesShiftLOne}}
\providecommand{\retDOFAChesShiftLTwo}{\tbd{retDOFAChesShiftLTwo}}
\providecommand{\retDOFACsTwelveBoundaryLOne}{\tbd{retDOFACsTwelveBoundaryLOne}}
\providecommand{\retDOFACsTwelveBoundaryLTwo}{\tbd{retDOFACsTwelveBoundaryLTwo}}
\providecommand{\retDOFACsTwelveCoarseLOne}{\tbd{retDOFACsTwelveCoarseLOne}}
\providecommand{\retDOFACsTwelveCoarseLTwo}{\tbd{retDOFACsTwelveCoarseLTwo}}
\providecommand{\retDOFACsTwelveOmissionLOne}{\tbd{retDOFACsTwelveOmissionLOne}}
\providecommand{\retDOFACsTwelveOmissionLTwo}{\tbd{retDOFACsTwelveOmissionLTwo}}
\providecommand{\retDOFACsTwelveSTwocloudlessREAL}{\tbd{retDOFACsTwelveSTwocloudlessREAL}}
\providecommand{\retDOFACsTwelveShiftLOne}{\tbd{retDOFACsTwelveShiftLOne}}
\providecommand{\retDOFACsTwelveShiftLTwo}{\tbd{retDOFACsTwelveShiftLTwo}}
\providecommand{\retDOFADfcBoundaryLOne}{\tbd{retDOFADfcBoundaryLOne}}
\providecommand{\retDOFADfcBoundaryLTwo}{\tbd{retDOFADfcBoundaryLTwo}}
\providecommand{\retDOFADfcCoarseLOne}{\tbd{retDOFADfcCoarseLOne}}
\providecommand{\retDOFADfcCoarseLTwo}{\tbd{retDOFADfcCoarseLTwo}}
\providecommand{\retDOFADfcModisREALVarTrainSubsetRealcov}{\tbd{retDOFADfcModisREALVarTrainSubsetRealcov}}
\providecommand{\retDOFADfcOmissionLOne}{\tbd{retDOFADfcOmissionLOne}}
\providecommand{\retDOFADfcOmissionLTwo}{\tbd{retDOFADfcOmissionLTwo}}
\providecommand{\retDOFADfcShiftLOne}{\tbd{retDOFADfcShiftLOne}}
\providecommand{\retDOFADfcShiftLTwo}{\tbd{retDOFADfcShiftLTwo}}
\providecommand{\retDOFAEnvaBoundaryLOne}{\tbd{retDOFAEnvaBoundaryLOne}}
\providecommand{\retDOFAEnvaBoundaryLTwo}{\tbd{retDOFAEnvaBoundaryLTwo}}
\providecommand{\retDOFAEnvaCoarseLOne}{\tbd{retDOFAEnvaCoarseLOne}}
\providecommand{\retDOFAEnvaCoarseLTwo}{\tbd{retDOFAEnvaCoarseLTwo}}
\providecommand{\retDOFAEnvaNlcdREAL}{\tbd{retDOFAEnvaNlcdREAL}}
\providecommand{\retDOFAEnvaOmissionLOne}{\tbd{retDOFAEnvaOmissionLOne}}
\providecommand{\retDOFAEnvaOmissionLTwo}{\tbd{retDOFAEnvaOmissionLTwo}}
\providecommand{\retDOFAEnvaShiftLOne}{\tbd{retDOFAEnvaShiftLOne}}
\providecommand{\retDOFAEnvaShiftLTwo}{\tbd{retDOFAEnvaShiftLTwo}}
\providecommand{\retDOFAKuroBoundaryLOne}{\tbd{retDOFAKuroBoundaryLOne}}
\providecommand{\retDOFAKuroBoundaryLTwo}{\tbd{retDOFAKuroBoundaryLTwo}}
\providecommand{\retDOFAKuroCemsREALVarTrainSubsetRealcov}{\tbd{retDOFAKuroCemsREALVarTrainSubsetRealcov}}
\providecommand{\retDOFAKuroCoarseLOne}{\tbd{retDOFAKuroCoarseLOne}}
\providecommand{\retDOFAKuroCoarseLTwo}{\tbd{retDOFAKuroCoarseLTwo}}
\providecommand{\retDOFAKuroOmissionLOne}{\tbd{retDOFAKuroOmissionLOne}}
\providecommand{\retDOFAKuroOmissionLTwo}{\tbd{retDOFAKuroOmissionLTwo}}
\providecommand{\retDOFAKuroShiftLOne}{\tbd{retDOFAKuroShiftLOne}}
\providecommand{\retDOFAKuroShiftLTwo}{\tbd{retDOFAKuroShiftLTwo}}
\providecommand{\retDOFAOemBoundaryLOne}{\tbd{retDOFAOemBoundaryLOne}}
\providecommand{\retDOFAOemBoundaryLTwo}{\tbd{retDOFAOemBoundaryLTwo}}
\providecommand{\retDOFAOemCoarseLOne}{\tbd{retDOFAOemCoarseLOne}}
\providecommand{\retDOFAOemCoarseLTwo}{\tbd{retDOFAOemCoarseLTwo}}
\providecommand{\retDOFAOemOmissionLOne}{\tbd{retDOFAOemOmissionLOne}}
\providecommand{\retDOFAOemOmissionLTwo}{\tbd{retDOFAOemOmissionLTwo}}
\providecommand{\retDOFAOemShiftLOne}{\tbd{retDOFAOemShiftLOne}}
\providecommand{\retDOFAOemShiftLTwo}{\tbd{retDOFAOemShiftLTwo}}
\providecommand{\retDOFASnTwoBoundaryLOne}{\tbd{retDOFASnTwoBoundaryLOne}}
\providecommand{\retDOFASnTwoBoundaryLTwo}{\tbd{retDOFASnTwoBoundaryLTwo}}
\providecommand{\retDOFASnTwoCoarseLOne}{\tbd{retDOFASnTwoCoarseLOne}}
\providecommand{\retDOFASnTwoCoarseLTwo}{\tbd{retDOFASnTwoCoarseLTwo}}
\providecommand{\retDOFASnTwoOmissionLOne}{\tbd{retDOFASnTwoOmissionLOne}}
\providecommand{\retDOFASnTwoOmissionLTwo}{\tbd{retDOFASnTwoOmissionLTwo}}
\providecommand{\retDOFASnTwoShiftLOne}{\tbd{retDOFASnTwoShiftLOne}}
\providecommand{\retDOFASnTwoShiftLTwo}{\tbd{retDOFASnTwoShiftLTwo}}
\providecommand{\retDOFAburnBoundaryLOne}{\tbd{retDOFAburnBoundaryLOne}}
\providecommand{\retDOFAburnBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{retDOFAburnBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retDOFAburnBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{retDOFAburnBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retDOFAburnBoundaryLOneVarDecoderSamLite}{\tbd{retDOFAburnBoundaryLOneVarDecoderSamLite}}
\providecommand{\retDOFAburnBoundaryLOneVarDecoderSamPretrained}{\tbd{retDOFAburnBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\retDOFAburnBoundaryLOneVarDecoderSegformerMlp}{\tbd{retDOFAburnBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\retDOFAburnBoundaryLR}{\tbd{retDOFAburnBoundaryLR}}
\providecommand{\retDOFAburnBoundaryLTwo}{\tbd{retDOFAburnBoundaryLTwo}}
\providecommand{\retDOFAburnBoundaryLTwoVarBandsRgb}{\tbd{retDOFAburnBoundaryLTwoVarBandsRgb}}
\providecommand{\retDOFAburnBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{retDOFAburnBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retDOFAburnBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retDOFAburnBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retDOFAburnBoundaryLTwoVarDecoderSamLite}{\tbd{retDOFAburnBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retDOFAburnBoundaryLTwoVarDecoderSamPretrained}{\tbd{retDOFAburnBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\retDOFAburnBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retDOFAburnBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retDOFAburnBoundaryLTwoVarFrozenEncoderTrue}{\tbd{retDOFAburnBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\retDOFAburnBoundaryLTwoVarLossBootstrap}{\tbd{retDOFAburnBoundaryLTwoVarLossBootstrap}}
\providecommand{\retDOFAburnBoundaryLTwoVarLossGce}{\tbd{retDOFAburnBoundaryLTwoVarLossGce}}
\providecommand{\retDOFAburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retDOFAburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retDOFAburnBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{retDOFAburnBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retDOFAburnCoarseLOne}{\tbd{retDOFAburnCoarseLOne}}
\providecommand{\retDOFAburnCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{retDOFAburnCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retDOFAburnCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{retDOFAburnCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retDOFAburnCoarseLOneVarDecoderSamLite}{\tbd{retDOFAburnCoarseLOneVarDecoderSamLite}}
\providecommand{\retDOFAburnCoarseLOneVarDecoderSamPretrained}{\tbd{retDOFAburnCoarseLOneVarDecoderSamPretrained}}
\providecommand{\retDOFAburnCoarseLOneVarDecoderSegformerMlp}{\tbd{retDOFAburnCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\retDOFAburnCoarseLR}{\tbd{retDOFAburnCoarseLR}}
\providecommand{\retDOFAburnCoarseLTwo}{\tbd{retDOFAburnCoarseLTwo}}
\providecommand{\retDOFAburnCoarseLTwoVarBandsRgb}{\tbd{retDOFAburnCoarseLTwoVarBandsRgb}}
\providecommand{\retDOFAburnCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{retDOFAburnCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retDOFAburnCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retDOFAburnCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retDOFAburnCoarseLTwoVarDecoderSamLite}{\tbd{retDOFAburnCoarseLTwoVarDecoderSamLite}}
\providecommand{\retDOFAburnCoarseLTwoVarDecoderSamPretrained}{\tbd{retDOFAburnCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\retDOFAburnCoarseLTwoVarDecoderSegformerMlp}{\tbd{retDOFAburnCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retDOFAburnCoarseLTwoVarFrozenEncoderTrue}{\tbd{retDOFAburnCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\retDOFAburnCoarseLTwoVarLossBootstrap}{\tbd{retDOFAburnCoarseLTwoVarLossBootstrap}}
\providecommand{\retDOFAburnCoarseLTwoVarLossGce}{\tbd{retDOFAburnCoarseLTwoVarLossGce}}
\providecommand{\retDOFAburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retDOFAburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retDOFAburnCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{retDOFAburnCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retDOFAburnOmissionLOne}{\tbd{retDOFAburnOmissionLOne}}
\providecommand{\retDOFAburnOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{retDOFAburnOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retDOFAburnOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{retDOFAburnOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retDOFAburnOmissionLOneVarDecoderSamLite}{\tbd{retDOFAburnOmissionLOneVarDecoderSamLite}}
\providecommand{\retDOFAburnOmissionLOneVarDecoderSamPretrained}{\tbd{retDOFAburnOmissionLOneVarDecoderSamPretrained}}
\providecommand{\retDOFAburnOmissionLOneVarDecoderSegformerMlp}{\tbd{retDOFAburnOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\retDOFAburnOmissionLR}{\tbd{retDOFAburnOmissionLR}}
\providecommand{\retDOFAburnOmissionLTwo}{\tbd{retDOFAburnOmissionLTwo}}
\providecommand{\retDOFAburnOmissionLTwoVarBandsRgb}{\tbd{retDOFAburnOmissionLTwoVarBandsRgb}}
\providecommand{\retDOFAburnOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{retDOFAburnOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retDOFAburnOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retDOFAburnOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retDOFAburnOmissionLTwoVarDecoderSamLite}{\tbd{retDOFAburnOmissionLTwoVarDecoderSamLite}}
\providecommand{\retDOFAburnOmissionLTwoVarDecoderSamPretrained}{\tbd{retDOFAburnOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\retDOFAburnOmissionLTwoVarDecoderSegformerMlp}{\tbd{retDOFAburnOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retDOFAburnOmissionLTwoVarFrozenEncoderTrue}{\tbd{retDOFAburnOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\retDOFAburnOmissionLTwoVarLossBootstrap}{\tbd{retDOFAburnOmissionLTwoVarLossBootstrap}}
\providecommand{\retDOFAburnOmissionLTwoVarLossGce}{\tbd{retDOFAburnOmissionLTwoVarLossGce}}
\providecommand{\retDOFAburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retDOFAburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retDOFAburnOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{retDOFAburnOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retDOFAburnShiftLOne}{\tbd{retDOFAburnShiftLOne}}
\providecommand{\retDOFAburnShiftLOneVarDecoderMaskTwoformerFull}{\tbd{retDOFAburnShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retDOFAburnShiftLOneVarDecoderMaskTwoformerLite}{\tbd{retDOFAburnShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retDOFAburnShiftLOneVarDecoderSamLite}{\tbd{retDOFAburnShiftLOneVarDecoderSamLite}}
\providecommand{\retDOFAburnShiftLOneVarDecoderSamPretrained}{\tbd{retDOFAburnShiftLOneVarDecoderSamPretrained}}
\providecommand{\retDOFAburnShiftLOneVarDecoderSegformerMlp}{\tbd{retDOFAburnShiftLOneVarDecoderSegformerMlp}}
\providecommand{\retDOFAburnShiftLR}{\tbd{retDOFAburnShiftLR}}
\providecommand{\retDOFAburnShiftLTwo}{\tbd{retDOFAburnShiftLTwo}}
\providecommand{\retDOFAburnShiftLTwoVarBandsRgb}{\tbd{retDOFAburnShiftLTwoVarBandsRgb}}
\providecommand{\retDOFAburnShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{retDOFAburnShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retDOFAburnShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retDOFAburnShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retDOFAburnShiftLTwoVarDecoderSamLite}{\tbd{retDOFAburnShiftLTwoVarDecoderSamLite}}
\providecommand{\retDOFAburnShiftLTwoVarDecoderSamPretrained}{\tbd{retDOFAburnShiftLTwoVarDecoderSamPretrained}}
\providecommand{\retDOFAburnShiftLTwoVarDecoderSegformerMlp}{\tbd{retDOFAburnShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retDOFAburnShiftLTwoVarFrozenEncoderTrue}{\tbd{retDOFAburnShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\retDOFAburnShiftLTwoVarLossBootstrap}{\tbd{retDOFAburnShiftLTwoVarLossBootstrap}}
\providecommand{\retDOFAburnShiftLTwoVarLossGce}{\tbd{retDOFAburnShiftLTwoVarLossGce}}
\providecommand{\retDOFAburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retDOFAburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retDOFAburnShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{retDOFAburnShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retDOFAflairBoundaryLOne}{\tbd{retDOFAflairBoundaryLOne}}
\providecommand{\retDOFAflairBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{retDOFAflairBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retDOFAflairBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{retDOFAflairBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retDOFAflairBoundaryLOneVarDecoderSamLite}{\tbd{retDOFAflairBoundaryLOneVarDecoderSamLite}}
\providecommand{\retDOFAflairBoundaryLOneVarDecoderSamPretrained}{\tbd{retDOFAflairBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\retDOFAflairBoundaryLOneVarDecoderSegformerMlp}{\tbd{retDOFAflairBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\retDOFAflairBoundaryLR}{\tbd{retDOFAflairBoundaryLR}}
\providecommand{\retDOFAflairBoundaryLTwo}{\tbd{retDOFAflairBoundaryLTwo}}
\providecommand{\retDOFAflairBoundaryLTwoVarBandsRgb}{\tbd{retDOFAflairBoundaryLTwoVarBandsRgb}}
\providecommand{\retDOFAflairBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{retDOFAflairBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retDOFAflairBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retDOFAflairBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retDOFAflairBoundaryLTwoVarDecoderSamLite}{\tbd{retDOFAflairBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retDOFAflairBoundaryLTwoVarDecoderSamPretrained}{\tbd{retDOFAflairBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\retDOFAflairBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retDOFAflairBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retDOFAflairBoundaryLTwoVarFrozenEncoderTrue}{\tbd{retDOFAflairBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\retDOFAflairBoundaryLTwoVarLossBootstrap}{\tbd{retDOFAflairBoundaryLTwoVarLossBootstrap}}
\providecommand{\retDOFAflairBoundaryLTwoVarLossGce}{\tbd{retDOFAflairBoundaryLTwoVarLossGce}}
\providecommand{\retDOFAflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retDOFAflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retDOFAflairBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{retDOFAflairBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retDOFAflairCoarseLOne}{\tbd{retDOFAflairCoarseLOne}}
\providecommand{\retDOFAflairCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{retDOFAflairCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retDOFAflairCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{retDOFAflairCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retDOFAflairCoarseLOneVarDecoderSamLite}{\tbd{retDOFAflairCoarseLOneVarDecoderSamLite}}
\providecommand{\retDOFAflairCoarseLOneVarDecoderSamPretrained}{\tbd{retDOFAflairCoarseLOneVarDecoderSamPretrained}}
\providecommand{\retDOFAflairCoarseLOneVarDecoderSegformerMlp}{\tbd{retDOFAflairCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\retDOFAflairCoarseLR}{\tbd{retDOFAflairCoarseLR}}
\providecommand{\retDOFAflairCoarseLTwo}{\tbd{retDOFAflairCoarseLTwo}}
\providecommand{\retDOFAflairCoarseLTwoVarBandsRgb}{\tbd{retDOFAflairCoarseLTwoVarBandsRgb}}
\providecommand{\retDOFAflairCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{retDOFAflairCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retDOFAflairCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retDOFAflairCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retDOFAflairCoarseLTwoVarDecoderSamLite}{\tbd{retDOFAflairCoarseLTwoVarDecoderSamLite}}
\providecommand{\retDOFAflairCoarseLTwoVarDecoderSamPretrained}{\tbd{retDOFAflairCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\retDOFAflairCoarseLTwoVarDecoderSegformerMlp}{\tbd{retDOFAflairCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retDOFAflairCoarseLTwoVarFrozenEncoderTrue}{\tbd{retDOFAflairCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\retDOFAflairCoarseLTwoVarLossBootstrap}{\tbd{retDOFAflairCoarseLTwoVarLossBootstrap}}
\providecommand{\retDOFAflairCoarseLTwoVarLossGce}{\tbd{retDOFAflairCoarseLTwoVarLossGce}}
\providecommand{\retDOFAflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retDOFAflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retDOFAflairCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{retDOFAflairCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retDOFAflairOmissionLOne}{\tbd{retDOFAflairOmissionLOne}}
\providecommand{\retDOFAflairOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{retDOFAflairOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retDOFAflairOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{retDOFAflairOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retDOFAflairOmissionLOneVarDecoderSamLite}{\tbd{retDOFAflairOmissionLOneVarDecoderSamLite}}
\providecommand{\retDOFAflairOmissionLOneVarDecoderSamPretrained}{\tbd{retDOFAflairOmissionLOneVarDecoderSamPretrained}}
\providecommand{\retDOFAflairOmissionLOneVarDecoderSegformerMlp}{\tbd{retDOFAflairOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\retDOFAflairOmissionLR}{\tbd{retDOFAflairOmissionLR}}
\providecommand{\retDOFAflairOmissionLTwo}{\tbd{retDOFAflairOmissionLTwo}}
\providecommand{\retDOFAflairOmissionLTwoVarBandsRgb}{\tbd{retDOFAflairOmissionLTwoVarBandsRgb}}
\providecommand{\retDOFAflairOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{retDOFAflairOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retDOFAflairOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retDOFAflairOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retDOFAflairOmissionLTwoVarDecoderSamLite}{\tbd{retDOFAflairOmissionLTwoVarDecoderSamLite}}
\providecommand{\retDOFAflairOmissionLTwoVarDecoderSamPretrained}{\tbd{retDOFAflairOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\retDOFAflairOmissionLTwoVarDecoderSegformerMlp}{\tbd{retDOFAflairOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retDOFAflairOmissionLTwoVarFrozenEncoderTrue}{\tbd{retDOFAflairOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\retDOFAflairOmissionLTwoVarLossBootstrap}{\tbd{retDOFAflairOmissionLTwoVarLossBootstrap}}
\providecommand{\retDOFAflairOmissionLTwoVarLossGce}{\tbd{retDOFAflairOmissionLTwoVarLossGce}}
\providecommand{\retDOFAflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retDOFAflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retDOFAflairOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{retDOFAflairOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retDOFAflairShiftLOne}{\tbd{retDOFAflairShiftLOne}}
\providecommand{\retDOFAflairShiftLOneVarDecoderMaskTwoformerFull}{\tbd{retDOFAflairShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retDOFAflairShiftLOneVarDecoderMaskTwoformerLite}{\tbd{retDOFAflairShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retDOFAflairShiftLOneVarDecoderSamLite}{\tbd{retDOFAflairShiftLOneVarDecoderSamLite}}
\providecommand{\retDOFAflairShiftLOneVarDecoderSamPretrained}{\tbd{retDOFAflairShiftLOneVarDecoderSamPretrained}}
\providecommand{\retDOFAflairShiftLOneVarDecoderSegformerMlp}{\tbd{retDOFAflairShiftLOneVarDecoderSegformerMlp}}
\providecommand{\retDOFAflairShiftLR}{\tbd{retDOFAflairShiftLR}}
\providecommand{\retDOFAflairShiftLTwo}{\tbd{retDOFAflairShiftLTwo}}
\providecommand{\retDOFAflairShiftLTwoVarBandsRgb}{\tbd{retDOFAflairShiftLTwoVarBandsRgb}}
\providecommand{\retDOFAflairShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{retDOFAflairShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retDOFAflairShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retDOFAflairShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retDOFAflairShiftLTwoVarDecoderSamLite}{\tbd{retDOFAflairShiftLTwoVarDecoderSamLite}}
\providecommand{\retDOFAflairShiftLTwoVarDecoderSamPretrained}{\tbd{retDOFAflairShiftLTwoVarDecoderSamPretrained}}
\providecommand{\retDOFAflairShiftLTwoVarDecoderSegformerMlp}{\tbd{retDOFAflairShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retDOFAflairShiftLTwoVarFrozenEncoderTrue}{\tbd{retDOFAflairShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\retDOFAflairShiftLTwoVarLossBootstrap}{\tbd{retDOFAflairShiftLTwoVarLossBootstrap}}
\providecommand{\retDOFAflairShiftLTwoVarLossGce}{\tbd{retDOFAflairShiftLTwoVarLossGce}}
\providecommand{\retDOFAflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retDOFAflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retDOFAflairShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{retDOFAflairShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retDOFAsenOtsuLTwo}{\tbd{retDOFAsenOtsuLTwo}}
\providecommand{\retDinovThreeConvnextLburnBoundaryLOne}{\tbd{retDinovThreeConvnextLburnBoundaryLOne}}
\providecommand{\retDinovThreeConvnextLburnBoundaryLTwo}{\tbd{retDinovThreeConvnextLburnBoundaryLTwo}}
\providecommand{\retDinovThreeConvnextLburnCoarseLOne}{\tbd{retDinovThreeConvnextLburnCoarseLOne}}
\providecommand{\retDinovThreeConvnextLburnCoarseLTwo}{\tbd{retDinovThreeConvnextLburnCoarseLTwo}}
\providecommand{\retDinovThreeConvnextLburnOmissionLOne}{\tbd{retDinovThreeConvnextLburnOmissionLOne}}
\providecommand{\retDinovThreeConvnextLburnOmissionLTwo}{\tbd{retDinovThreeConvnextLburnOmissionLTwo}}
\providecommand{\retDinovThreeConvnextLburnShiftLOne}{\tbd{retDinovThreeConvnextLburnShiftLOne}}
\providecommand{\retDinovThreeConvnextLburnShiftLTwo}{\tbd{retDinovThreeConvnextLburnShiftLTwo}}
\providecommand{\retDinovThreeConvnextLflairBoundaryLOne}{\tbd{retDinovThreeConvnextLflairBoundaryLOne}}
\providecommand{\retDinovThreeConvnextLflairBoundaryLTwo}{\tbd{retDinovThreeConvnextLflairBoundaryLTwo}}
\providecommand{\retDinovThreeConvnextLflairCoarseLOne}{\tbd{retDinovThreeConvnextLflairCoarseLOne}}
\providecommand{\retDinovThreeConvnextLflairCoarseLTwo}{\tbd{retDinovThreeConvnextLflairCoarseLTwo}}
\providecommand{\retDinovThreeConvnextLflairOmissionLOne}{\tbd{retDinovThreeConvnextLflairOmissionLOne}}
\providecommand{\retDinovThreeConvnextLflairOmissionLTwo}{\tbd{retDinovThreeConvnextLflairOmissionLTwo}}
\providecommand{\retDinovThreeConvnextLflairShiftLOne}{\tbd{retDinovThreeConvnextLflairShiftLOne}}
\providecommand{\retDinovThreeConvnextLflairShiftLTwo}{\tbd{retDinovThreeConvnextLflairShiftLTwo}}
\providecommand{\retLVDChesBoundaryLOne}{\tbd{retLVDChesBoundaryLOne}}
\providecommand{\retLVDChesBoundaryLTwo}{\tbd{retLVDChesBoundaryLTwo}}
\providecommand{\retLVDChesBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retLVDChesBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDChesBoundaryLTwoVarDecoderSamLite}{\tbd{retLVDChesBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retLVDChesBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retLVDChesBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retLVDChesBoundaryLTwoVarLrMultOne}{\tbd{retLVDChesBoundaryLTwoVarLrMultOne}}
\providecommand{\retLVDChesCoarseLOne}{\tbd{retLVDChesCoarseLOne}}
\providecommand{\retLVDChesCoarseLTwo}{\tbd{retLVDChesCoarseLTwo}}
\providecommand{\retLVDChesCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retLVDChesCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDChesCoarseLTwoVarDecoderSamLite}{\tbd{retLVDChesCoarseLTwoVarDecoderSamLite}}
\providecommand{\retLVDChesCoarseLTwoVarDecoderSegformerMlp}{\tbd{retLVDChesCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retLVDChesCoarseLTwoVarLrMultOne}{\tbd{retLVDChesCoarseLTwoVarLrMultOne}}
\providecommand{\retLVDChesNlcdREAL}{\tbd{retLVDChesNlcdREAL}}
\providecommand{\retLVDChesOmissionLOne}{\tbd{retLVDChesOmissionLOne}}
\providecommand{\retLVDChesOmissionLTwo}{\tbd{retLVDChesOmissionLTwo}}
\providecommand{\retLVDChesOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retLVDChesOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDChesOmissionLTwoVarDecoderSamLite}{\tbd{retLVDChesOmissionLTwoVarDecoderSamLite}}
\providecommand{\retLVDChesOmissionLTwoVarDecoderSegformerMlp}{\tbd{retLVDChesOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retLVDChesOmissionLTwoVarLrMultOne}{\tbd{retLVDChesOmissionLTwoVarLrMultOne}}
\providecommand{\retLVDChesShiftLOne}{\tbd{retLVDChesShiftLOne}}
\providecommand{\retLVDChesShiftLTwo}{\tbd{retLVDChesShiftLTwo}}
\providecommand{\retLVDChesShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retLVDChesShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDChesShiftLTwoVarDecoderSamLite}{\tbd{retLVDChesShiftLTwoVarDecoderSamLite}}
\providecommand{\retLVDChesShiftLTwoVarDecoderSegformerMlp}{\tbd{retLVDChesShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retLVDChesShiftLTwoVarLrMultOne}{\tbd{retLVDChesShiftLTwoVarLrMultOne}}
\providecommand{\retLVDCsTwelveBoundaryLOne}{\tbd{retLVDCsTwelveBoundaryLOne}}
\providecommand{\retLVDCsTwelveBoundaryLTwo}{\tbd{retLVDCsTwelveBoundaryLTwo}}
\providecommand{\retLVDCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retLVDCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDCsTwelveBoundaryLTwoVarDecoderSamLite}{\tbd{retLVDCsTwelveBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retLVDCsTwelveBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retLVDCsTwelveBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retLVDCsTwelveBoundaryLTwoVarLrMultOne}{\tbd{retLVDCsTwelveBoundaryLTwoVarLrMultOne}}
\providecommand{\retLVDCsTwelveCoarseLOne}{\tbd{retLVDCsTwelveCoarseLOne}}
\providecommand{\retLVDCsTwelveCoarseLTwo}{\tbd{retLVDCsTwelveCoarseLTwo}}
\providecommand{\retLVDCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retLVDCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDCsTwelveCoarseLTwoVarDecoderSamLite}{\tbd{retLVDCsTwelveCoarseLTwoVarDecoderSamLite}}
\providecommand{\retLVDCsTwelveCoarseLTwoVarDecoderSegformerMlp}{\tbd{retLVDCsTwelveCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retLVDCsTwelveCoarseLTwoVarLrMultOne}{\tbd{retLVDCsTwelveCoarseLTwoVarLrMultOne}}
\providecommand{\retLVDCsTwelveOmissionLOne}{\tbd{retLVDCsTwelveOmissionLOne}}
\providecommand{\retLVDCsTwelveOmissionLTwo}{\tbd{retLVDCsTwelveOmissionLTwo}}
\providecommand{\retLVDCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retLVDCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDCsTwelveOmissionLTwoVarDecoderSamLite}{\tbd{retLVDCsTwelveOmissionLTwoVarDecoderSamLite}}
\providecommand{\retLVDCsTwelveOmissionLTwoVarDecoderSegformerMlp}{\tbd{retLVDCsTwelveOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retLVDCsTwelveOmissionLTwoVarLrMultOne}{\tbd{retLVDCsTwelveOmissionLTwoVarLrMultOne}}
\providecommand{\retLVDCsTwelveSTwocloudlessREAL}{\tbd{retLVDCsTwelveSTwocloudlessREAL}}
\providecommand{\retLVDCsTwelveShiftLOne}{\tbd{retLVDCsTwelveShiftLOne}}
\providecommand{\retLVDCsTwelveShiftLTwo}{\tbd{retLVDCsTwelveShiftLTwo}}
\providecommand{\retLVDCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retLVDCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDCsTwelveShiftLTwoVarDecoderSamLite}{\tbd{retLVDCsTwelveShiftLTwoVarDecoderSamLite}}
\providecommand{\retLVDCsTwelveShiftLTwoVarDecoderSegformerMlp}{\tbd{retLVDCsTwelveShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retLVDCsTwelveShiftLTwoVarLrMultOne}{\tbd{retLVDCsTwelveShiftLTwoVarLrMultOne}}
\providecommand{\retLVDDfcBoundaryLOne}{\tbd{retLVDDfcBoundaryLOne}}
\providecommand{\retLVDDfcBoundaryLTwo}{\tbd{retLVDDfcBoundaryLTwo}}
\providecommand{\retLVDDfcBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retLVDDfcBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDDfcBoundaryLTwoVarDecoderSamLite}{\tbd{retLVDDfcBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retLVDDfcBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retLVDDfcBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retLVDDfcBoundaryLTwoVarLrMultOne}{\tbd{retLVDDfcBoundaryLTwoVarLrMultOne}}
\providecommand{\retLVDDfcCoarseLOne}{\tbd{retLVDDfcCoarseLOne}}
\providecommand{\retLVDDfcCoarseLTwo}{\tbd{retLVDDfcCoarseLTwo}}
\providecommand{\retLVDDfcCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retLVDDfcCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDDfcCoarseLTwoVarDecoderSamLite}{\tbd{retLVDDfcCoarseLTwoVarDecoderSamLite}}
\providecommand{\retLVDDfcCoarseLTwoVarDecoderSegformerMlp}{\tbd{retLVDDfcCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retLVDDfcCoarseLTwoVarLrMultOne}{\tbd{retLVDDfcCoarseLTwoVarLrMultOne}}
\providecommand{\retLVDDfcModisREALVarTrainSubsetRealcov}{\tbd{retLVDDfcModisREALVarTrainSubsetRealcov}}
\providecommand{\retLVDDfcOmissionLOne}{\tbd{retLVDDfcOmissionLOne}}
\providecommand{\retLVDDfcOmissionLTwo}{\tbd{retLVDDfcOmissionLTwo}}
\providecommand{\retLVDDfcOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retLVDDfcOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDDfcOmissionLTwoVarDecoderSamLite}{\tbd{retLVDDfcOmissionLTwoVarDecoderSamLite}}
\providecommand{\retLVDDfcOmissionLTwoVarDecoderSegformerMlp}{\tbd{retLVDDfcOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retLVDDfcOmissionLTwoVarLrMultOne}{\tbd{retLVDDfcOmissionLTwoVarLrMultOne}}
\providecommand{\retLVDDfcShiftLOne}{\tbd{retLVDDfcShiftLOne}}
\providecommand{\retLVDDfcShiftLTwo}{\tbd{retLVDDfcShiftLTwo}}
\providecommand{\retLVDDfcShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retLVDDfcShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDDfcShiftLTwoVarDecoderSamLite}{\tbd{retLVDDfcShiftLTwoVarDecoderSamLite}}
\providecommand{\retLVDDfcShiftLTwoVarDecoderSegformerMlp}{\tbd{retLVDDfcShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retLVDDfcShiftLTwoVarLrMultOne}{\tbd{retLVDDfcShiftLTwoVarLrMultOne}}
\providecommand{\retLVDEnvaBoundaryLOne}{\tbd{retLVDEnvaBoundaryLOne}}
\providecommand{\retLVDEnvaBoundaryLTwo}{\tbd{retLVDEnvaBoundaryLTwo}}
\providecommand{\retLVDEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retLVDEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDEnvaBoundaryLTwoVarDecoderSamLite}{\tbd{retLVDEnvaBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retLVDEnvaBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retLVDEnvaBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retLVDEnvaBoundaryLTwoVarLrMultOne}{\tbd{retLVDEnvaBoundaryLTwoVarLrMultOne}}
\providecommand{\retLVDEnvaCoarseLOne}{\tbd{retLVDEnvaCoarseLOne}}
\providecommand{\retLVDEnvaCoarseLTwo}{\tbd{retLVDEnvaCoarseLTwo}}
\providecommand{\retLVDEnvaCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retLVDEnvaCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDEnvaCoarseLTwoVarDecoderSamLite}{\tbd{retLVDEnvaCoarseLTwoVarDecoderSamLite}}
\providecommand{\retLVDEnvaCoarseLTwoVarDecoderSegformerMlp}{\tbd{retLVDEnvaCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retLVDEnvaCoarseLTwoVarLrMultOne}{\tbd{retLVDEnvaCoarseLTwoVarLrMultOne}}
\providecommand{\retLVDEnvaNlcdREAL}{\tbd{retLVDEnvaNlcdREAL}}
\providecommand{\retLVDEnvaOmissionLOne}{\tbd{retLVDEnvaOmissionLOne}}
\providecommand{\retLVDEnvaOmissionLTwo}{\tbd{retLVDEnvaOmissionLTwo}}
\providecommand{\retLVDEnvaOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retLVDEnvaOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDEnvaOmissionLTwoVarDecoderSamLite}{\tbd{retLVDEnvaOmissionLTwoVarDecoderSamLite}}
\providecommand{\retLVDEnvaOmissionLTwoVarDecoderSegformerMlp}{\tbd{retLVDEnvaOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retLVDEnvaOmissionLTwoVarLrMultOne}{\tbd{retLVDEnvaOmissionLTwoVarLrMultOne}}
\providecommand{\retLVDEnvaShiftLOne}{\tbd{retLVDEnvaShiftLOne}}
\providecommand{\retLVDEnvaShiftLTwo}{\tbd{retLVDEnvaShiftLTwo}}
\providecommand{\retLVDEnvaShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retLVDEnvaShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDEnvaShiftLTwoVarDecoderSamLite}{\tbd{retLVDEnvaShiftLTwoVarDecoderSamLite}}
\providecommand{\retLVDEnvaShiftLTwoVarDecoderSegformerMlp}{\tbd{retLVDEnvaShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retLVDEnvaShiftLTwoVarLrMultOne}{\tbd{retLVDEnvaShiftLTwoVarLrMultOne}}
\providecommand{\retLVDKuroBoundaryLOne}{\tbd{retLVDKuroBoundaryLOne}}
\providecommand{\retLVDKuroBoundaryLTwo}{\tbd{retLVDKuroBoundaryLTwo}}
\providecommand{\retLVDKuroBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retLVDKuroBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDKuroBoundaryLTwoVarDecoderSamLite}{\tbd{retLVDKuroBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retLVDKuroBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retLVDKuroBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retLVDKuroBoundaryLTwoVarLrMultOne}{\tbd{retLVDKuroBoundaryLTwoVarLrMultOne}}
\providecommand{\retLVDKuroCemsREALVarTrainSubsetRealcov}{\tbd{retLVDKuroCemsREALVarTrainSubsetRealcov}}
\providecommand{\retLVDKuroCoarseLOne}{\tbd{retLVDKuroCoarseLOne}}
\providecommand{\retLVDKuroCoarseLTwo}{\tbd{retLVDKuroCoarseLTwo}}
\providecommand{\retLVDKuroCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retLVDKuroCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDKuroCoarseLTwoVarDecoderSamLite}{\tbd{retLVDKuroCoarseLTwoVarDecoderSamLite}}
\providecommand{\retLVDKuroCoarseLTwoVarDecoderSegformerMlp}{\tbd{retLVDKuroCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retLVDKuroCoarseLTwoVarLrMultOne}{\tbd{retLVDKuroCoarseLTwoVarLrMultOne}}
\providecommand{\retLVDKuroOmissionLOne}{\tbd{retLVDKuroOmissionLOne}}
\providecommand{\retLVDKuroOmissionLTwo}{\tbd{retLVDKuroOmissionLTwo}}
\providecommand{\retLVDKuroOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retLVDKuroOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDKuroOmissionLTwoVarDecoderSamLite}{\tbd{retLVDKuroOmissionLTwoVarDecoderSamLite}}
\providecommand{\retLVDKuroOmissionLTwoVarDecoderSegformerMlp}{\tbd{retLVDKuroOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retLVDKuroOmissionLTwoVarLrMultOne}{\tbd{retLVDKuroOmissionLTwoVarLrMultOne}}
\providecommand{\retLVDKuroShiftLOne}{\tbd{retLVDKuroShiftLOne}}
\providecommand{\retLVDKuroShiftLTwo}{\tbd{retLVDKuroShiftLTwo}}
\providecommand{\retLVDKuroShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retLVDKuroShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDKuroShiftLTwoVarDecoderSamLite}{\tbd{retLVDKuroShiftLTwoVarDecoderSamLite}}
\providecommand{\retLVDKuroShiftLTwoVarDecoderSegformerMlp}{\tbd{retLVDKuroShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retLVDKuroShiftLTwoVarLrMultOne}{\tbd{retLVDKuroShiftLTwoVarLrMultOne}}
\providecommand{\retLVDOemBoundaryLOne}{\tbd{retLVDOemBoundaryLOne}}
\providecommand{\retLVDOemBoundaryLTwo}{\tbd{retLVDOemBoundaryLTwo}}
\providecommand{\retLVDOemBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retLVDOemBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDOemBoundaryLTwoVarDecoderSamLite}{\tbd{retLVDOemBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retLVDOemBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retLVDOemBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retLVDOemBoundaryLTwoVarLrMultOne}{\tbd{retLVDOemBoundaryLTwoVarLrMultOne}}
\providecommand{\retLVDOemCoarseLOne}{\tbd{retLVDOemCoarseLOne}}
\providecommand{\retLVDOemCoarseLTwo}{\tbd{retLVDOemCoarseLTwo}}
\providecommand{\retLVDOemCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retLVDOemCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDOemCoarseLTwoVarDecoderSamLite}{\tbd{retLVDOemCoarseLTwoVarDecoderSamLite}}
\providecommand{\retLVDOemCoarseLTwoVarDecoderSegformerMlp}{\tbd{retLVDOemCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retLVDOemCoarseLTwoVarLrMultOne}{\tbd{retLVDOemCoarseLTwoVarLrMultOne}}
\providecommand{\retLVDOemOmissionLOne}{\tbd{retLVDOemOmissionLOne}}
\providecommand{\retLVDOemOmissionLTwo}{\tbd{retLVDOemOmissionLTwo}}
\providecommand{\retLVDOemOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retLVDOemOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDOemOmissionLTwoVarDecoderSamLite}{\tbd{retLVDOemOmissionLTwoVarDecoderSamLite}}
\providecommand{\retLVDOemOmissionLTwoVarDecoderSegformerMlp}{\tbd{retLVDOemOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retLVDOemOmissionLTwoVarLrMultOne}{\tbd{retLVDOemOmissionLTwoVarLrMultOne}}
\providecommand{\retLVDOemShiftLOne}{\tbd{retLVDOemShiftLOne}}
\providecommand{\retLVDOemShiftLTwo}{\tbd{retLVDOemShiftLTwo}}
\providecommand{\retLVDOemShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retLVDOemShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDOemShiftLTwoVarDecoderSamLite}{\tbd{retLVDOemShiftLTwoVarDecoderSamLite}}
\providecommand{\retLVDOemShiftLTwoVarDecoderSegformerMlp}{\tbd{retLVDOemShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retLVDOemShiftLTwoVarLrMultOne}{\tbd{retLVDOemShiftLTwoVarLrMultOne}}
\providecommand{\retLVDSnTwoBoundaryLOne}{\tbd{retLVDSnTwoBoundaryLOne}}
\providecommand{\retLVDSnTwoBoundaryLTwo}{\tbd{retLVDSnTwoBoundaryLTwo}}
\providecommand{\retLVDSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retLVDSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDSnTwoBoundaryLTwoVarDecoderSamLite}{\tbd{retLVDSnTwoBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retLVDSnTwoBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retLVDSnTwoBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retLVDSnTwoBoundaryLTwoVarLrMultOne}{\tbd{retLVDSnTwoBoundaryLTwoVarLrMultOne}}
\providecommand{\retLVDSnTwoCoarseLOne}{\tbd{retLVDSnTwoCoarseLOne}}
\providecommand{\retLVDSnTwoCoarseLTwo}{\tbd{retLVDSnTwoCoarseLTwo}}
\providecommand{\retLVDSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retLVDSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDSnTwoCoarseLTwoVarDecoderSamLite}{\tbd{retLVDSnTwoCoarseLTwoVarDecoderSamLite}}
\providecommand{\retLVDSnTwoCoarseLTwoVarDecoderSegformerMlp}{\tbd{retLVDSnTwoCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retLVDSnTwoCoarseLTwoVarLrMultOne}{\tbd{retLVDSnTwoCoarseLTwoVarLrMultOne}}
\providecommand{\retLVDSnTwoOmissionLOne}{\tbd{retLVDSnTwoOmissionLOne}}
\providecommand{\retLVDSnTwoOmissionLTwo}{\tbd{retLVDSnTwoOmissionLTwo}}
\providecommand{\retLVDSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retLVDSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDSnTwoOmissionLTwoVarDecoderSamLite}{\tbd{retLVDSnTwoOmissionLTwoVarDecoderSamLite}}
\providecommand{\retLVDSnTwoOmissionLTwoVarDecoderSegformerMlp}{\tbd{retLVDSnTwoOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retLVDSnTwoOmissionLTwoVarLrMultOne}{\tbd{retLVDSnTwoOmissionLTwoVarLrMultOne}}
\providecommand{\retLVDSnTwoShiftLOne}{\tbd{retLVDSnTwoShiftLOne}}
\providecommand{\retLVDSnTwoShiftLTwo}{\tbd{retLVDSnTwoShiftLTwo}}
\providecommand{\retLVDSnTwoShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retLVDSnTwoShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDSnTwoShiftLTwoVarDecoderSamLite}{\tbd{retLVDSnTwoShiftLTwoVarDecoderSamLite}}
\providecommand{\retLVDSnTwoShiftLTwoVarDecoderSegformerMlp}{\tbd{retLVDSnTwoShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retLVDSnTwoShiftLTwoVarLrMultOne}{\tbd{retLVDSnTwoShiftLTwoVarLrMultOne}}
\providecommand{\retLVDburnBoundaryLOne}{\tbd{retLVDburnBoundaryLOne}}
\providecommand{\retLVDburnBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{retLVDburnBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retLVDburnBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{retLVDburnBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDburnBoundaryLOneVarDecoderSamLite}{\tbd{retLVDburnBoundaryLOneVarDecoderSamLite}}
\providecommand{\retLVDburnBoundaryLOneVarDecoderSamPretrained}{\tbd{retLVDburnBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\retLVDburnBoundaryLOneVarDecoderSegformerMlp}{\tbd{retLVDburnBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\retLVDburnBoundaryLR}{\tbd{retLVDburnBoundaryLR}}
\providecommand{\retLVDburnBoundaryLRVarLrMultOne}{\tbd{retLVDburnBoundaryLRVarLrMultOne}}
\providecommand{\retLVDburnBoundaryLTwo}{\tbd{retLVDburnBoundaryLTwo}}
\providecommand{\retLVDburnBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{retLVDburnBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retLVDburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{retLVDburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\retLVDburnBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retLVDburnBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{retLVDburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\retLVDburnBoundaryLTwoVarDecoderSamLite}{\tbd{retLVDburnBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retLVDburnBoundaryLTwoVarDecoderSamLiteLrMultOne}{\tbd{retLVDburnBoundaryLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\retLVDburnBoundaryLTwoVarDecoderSamPretrained}{\tbd{retLVDburnBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\retLVDburnBoundaryLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{retLVDburnBoundaryLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\retLVDburnBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retLVDburnBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retLVDburnBoundaryLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{retLVDburnBoundaryLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\retLVDburnBoundaryLTwoVarLossBootstrap}{\tbd{retLVDburnBoundaryLTwoVarLossBootstrap}}
\providecommand{\retLVDburnBoundaryLTwoVarLossGce}{\tbd{retLVDburnBoundaryLTwoVarLossGce}}
\providecommand{\retLVDburnBoundaryLTwoVarLrMultOne}{\tbd{retLVDburnBoundaryLTwoVarLrMultOne}}
\providecommand{\retLVDburnBoundaryLTwoVarLrMultThree}{\tbd{retLVDburnBoundaryLTwoVarLrMultThree}}
\providecommand{\retLVDburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retLVDburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retLVDburnBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{retLVDburnBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retLVDburnCoarseLOne}{\tbd{retLVDburnCoarseLOne}}
\providecommand{\retLVDburnCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{retLVDburnCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retLVDburnCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{retLVDburnCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDburnCoarseLOneVarDecoderSamLite}{\tbd{retLVDburnCoarseLOneVarDecoderSamLite}}
\providecommand{\retLVDburnCoarseLOneVarDecoderSamPretrained}{\tbd{retLVDburnCoarseLOneVarDecoderSamPretrained}}
\providecommand{\retLVDburnCoarseLOneVarDecoderSegformerMlp}{\tbd{retLVDburnCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\retLVDburnCoarseLR}{\tbd{retLVDburnCoarseLR}}
\providecommand{\retLVDburnCoarseLRVarLrMultOne}{\tbd{retLVDburnCoarseLRVarLrMultOne}}
\providecommand{\retLVDburnCoarseLTwo}{\tbd{retLVDburnCoarseLTwo}}
\providecommand{\retLVDburnCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{retLVDburnCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retLVDburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{retLVDburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\retLVDburnCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retLVDburnCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{retLVDburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\retLVDburnCoarseLTwoVarDecoderSamLite}{\tbd{retLVDburnCoarseLTwoVarDecoderSamLite}}
\providecommand{\retLVDburnCoarseLTwoVarDecoderSamLiteLrMultOne}{\tbd{retLVDburnCoarseLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\retLVDburnCoarseLTwoVarDecoderSamPretrained}{\tbd{retLVDburnCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\retLVDburnCoarseLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{retLVDburnCoarseLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\retLVDburnCoarseLTwoVarDecoderSegformerMlp}{\tbd{retLVDburnCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retLVDburnCoarseLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{retLVDburnCoarseLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\retLVDburnCoarseLTwoVarLossBootstrap}{\tbd{retLVDburnCoarseLTwoVarLossBootstrap}}
\providecommand{\retLVDburnCoarseLTwoVarLossGce}{\tbd{retLVDburnCoarseLTwoVarLossGce}}
\providecommand{\retLVDburnCoarseLTwoVarLrMultOne}{\tbd{retLVDburnCoarseLTwoVarLrMultOne}}
\providecommand{\retLVDburnCoarseLTwoVarLrMultThree}{\tbd{retLVDburnCoarseLTwoVarLrMultThree}}
\providecommand{\retLVDburnCoarseLTwoVarLrMultZeroOneOneOneOne}{\tbd{retLVDburnCoarseLTwoVarLrMultZeroOneOneOneOne}}
\providecommand{\retLVDburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retLVDburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retLVDburnCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{retLVDburnCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retLVDburnOmissionLOne}{\tbd{retLVDburnOmissionLOne}}
\providecommand{\retLVDburnOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{retLVDburnOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retLVDburnOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{retLVDburnOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDburnOmissionLOneVarDecoderSamLite}{\tbd{retLVDburnOmissionLOneVarDecoderSamLite}}
\providecommand{\retLVDburnOmissionLOneVarDecoderSamPretrained}{\tbd{retLVDburnOmissionLOneVarDecoderSamPretrained}}
\providecommand{\retLVDburnOmissionLOneVarDecoderSegformerMlp}{\tbd{retLVDburnOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\retLVDburnOmissionLR}{\tbd{retLVDburnOmissionLR}}
\providecommand{\retLVDburnOmissionLRVarLrMultOne}{\tbd{retLVDburnOmissionLRVarLrMultOne}}
\providecommand{\retLVDburnOmissionLTwo}{\tbd{retLVDburnOmissionLTwo}}
\providecommand{\retLVDburnOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{retLVDburnOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retLVDburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{retLVDburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\retLVDburnOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retLVDburnOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{retLVDburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\retLVDburnOmissionLTwoVarDecoderSamLite}{\tbd{retLVDburnOmissionLTwoVarDecoderSamLite}}
\providecommand{\retLVDburnOmissionLTwoVarDecoderSamLiteLrMultOne}{\tbd{retLVDburnOmissionLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\retLVDburnOmissionLTwoVarDecoderSamPretrained}{\tbd{retLVDburnOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\retLVDburnOmissionLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{retLVDburnOmissionLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\retLVDburnOmissionLTwoVarDecoderSegformerMlp}{\tbd{retLVDburnOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retLVDburnOmissionLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{retLVDburnOmissionLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\retLVDburnOmissionLTwoVarLossBootstrap}{\tbd{retLVDburnOmissionLTwoVarLossBootstrap}}
\providecommand{\retLVDburnOmissionLTwoVarLossGce}{\tbd{retLVDburnOmissionLTwoVarLossGce}}
\providecommand{\retLVDburnOmissionLTwoVarLrMultOne}{\tbd{retLVDburnOmissionLTwoVarLrMultOne}}
\providecommand{\retLVDburnOmissionLTwoVarLrMultThree}{\tbd{retLVDburnOmissionLTwoVarLrMultThree}}
\providecommand{\retLVDburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retLVDburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retLVDburnOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{retLVDburnOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retLVDburnShiftLOne}{\tbd{retLVDburnShiftLOne}}
\providecommand{\retLVDburnShiftLOneVarDecoderMaskTwoformerFull}{\tbd{retLVDburnShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retLVDburnShiftLOneVarDecoderMaskTwoformerLite}{\tbd{retLVDburnShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDburnShiftLOneVarDecoderSamLite}{\tbd{retLVDburnShiftLOneVarDecoderSamLite}}
\providecommand{\retLVDburnShiftLOneVarDecoderSamPretrained}{\tbd{retLVDburnShiftLOneVarDecoderSamPretrained}}
\providecommand{\retLVDburnShiftLOneVarDecoderSegformerMlp}{\tbd{retLVDburnShiftLOneVarDecoderSegformerMlp}}
\providecommand{\retLVDburnShiftLR}{\tbd{retLVDburnShiftLR}}
\providecommand{\retLVDburnShiftLRVarLrMultOne}{\tbd{retLVDburnShiftLRVarLrMultOne}}
\providecommand{\retLVDburnShiftLTwo}{\tbd{retLVDburnShiftLTwo}}
\providecommand{\retLVDburnShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{retLVDburnShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retLVDburnShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{retLVDburnShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\retLVDburnShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retLVDburnShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{retLVDburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\retLVDburnShiftLTwoVarDecoderSamLite}{\tbd{retLVDburnShiftLTwoVarDecoderSamLite}}
\providecommand{\retLVDburnShiftLTwoVarDecoderSamLiteLrMultOne}{\tbd{retLVDburnShiftLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\retLVDburnShiftLTwoVarDecoderSamPretrained}{\tbd{retLVDburnShiftLTwoVarDecoderSamPretrained}}
\providecommand{\retLVDburnShiftLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{retLVDburnShiftLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\retLVDburnShiftLTwoVarDecoderSegformerMlp}{\tbd{retLVDburnShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retLVDburnShiftLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{retLVDburnShiftLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\retLVDburnShiftLTwoVarLossBootstrap}{\tbd{retLVDburnShiftLTwoVarLossBootstrap}}
\providecommand{\retLVDburnShiftLTwoVarLossGce}{\tbd{retLVDburnShiftLTwoVarLossGce}}
\providecommand{\retLVDburnShiftLTwoVarLrMultOne}{\tbd{retLVDburnShiftLTwoVarLrMultOne}}
\providecommand{\retLVDburnShiftLTwoVarLrMultThree}{\tbd{retLVDburnShiftLTwoVarLrMultThree}}
\providecommand{\retLVDburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retLVDburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retLVDburnShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{retLVDburnShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retLVDflairBoundaryLOne}{\tbd{retLVDflairBoundaryLOne}}
\providecommand{\retLVDflairBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{retLVDflairBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retLVDflairBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{retLVDflairBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDflairBoundaryLOneVarDecoderSamLite}{\tbd{retLVDflairBoundaryLOneVarDecoderSamLite}}
\providecommand{\retLVDflairBoundaryLOneVarDecoderSamPretrained}{\tbd{retLVDflairBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\retLVDflairBoundaryLOneVarDecoderSegformerMlp}{\tbd{retLVDflairBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\retLVDflairBoundaryLR}{\tbd{retLVDflairBoundaryLR}}
\providecommand{\retLVDflairBoundaryLRVarLrMultOne}{\tbd{retLVDflairBoundaryLRVarLrMultOne}}
\providecommand{\retLVDflairBoundaryLTwo}{\tbd{retLVDflairBoundaryLTwo}}
\providecommand{\retLVDflairBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{retLVDflairBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retLVDflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{retLVDflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\retLVDflairBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retLVDflairBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{retLVDflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\retLVDflairBoundaryLTwoVarDecoderSamLite}{\tbd{retLVDflairBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retLVDflairBoundaryLTwoVarDecoderSamLiteLrMultOne}{\tbd{retLVDflairBoundaryLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\retLVDflairBoundaryLTwoVarDecoderSamPretrained}{\tbd{retLVDflairBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\retLVDflairBoundaryLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{retLVDflairBoundaryLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\retLVDflairBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retLVDflairBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retLVDflairBoundaryLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{retLVDflairBoundaryLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\retLVDflairBoundaryLTwoVarLossBootstrap}{\tbd{retLVDflairBoundaryLTwoVarLossBootstrap}}
\providecommand{\retLVDflairBoundaryLTwoVarLossGce}{\tbd{retLVDflairBoundaryLTwoVarLossGce}}
\providecommand{\retLVDflairBoundaryLTwoVarLrMultOne}{\tbd{retLVDflairBoundaryLTwoVarLrMultOne}}
\providecommand{\retLVDflairBoundaryLTwoVarLrMultThree}{\tbd{retLVDflairBoundaryLTwoVarLrMultThree}}
\providecommand{\retLVDflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retLVDflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retLVDflairBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{retLVDflairBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retLVDflairCoarseLOne}{\tbd{retLVDflairCoarseLOne}}
\providecommand{\retLVDflairCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{retLVDflairCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retLVDflairCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{retLVDflairCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDflairCoarseLOneVarDecoderSamLite}{\tbd{retLVDflairCoarseLOneVarDecoderSamLite}}
\providecommand{\retLVDflairCoarseLOneVarDecoderSamPretrained}{\tbd{retLVDflairCoarseLOneVarDecoderSamPretrained}}
\providecommand{\retLVDflairCoarseLOneVarDecoderSegformerMlp}{\tbd{retLVDflairCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\retLVDflairCoarseLR}{\tbd{retLVDflairCoarseLR}}
\providecommand{\retLVDflairCoarseLRVarLrMultOne}{\tbd{retLVDflairCoarseLRVarLrMultOne}}
\providecommand{\retLVDflairCoarseLTwo}{\tbd{retLVDflairCoarseLTwo}}
\providecommand{\retLVDflairCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{retLVDflairCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retLVDflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{retLVDflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\retLVDflairCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retLVDflairCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{retLVDflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\retLVDflairCoarseLTwoVarDecoderSamLite}{\tbd{retLVDflairCoarseLTwoVarDecoderSamLite}}
\providecommand{\retLVDflairCoarseLTwoVarDecoderSamLiteLrMultOne}{\tbd{retLVDflairCoarseLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\retLVDflairCoarseLTwoVarDecoderSamPretrained}{\tbd{retLVDflairCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\retLVDflairCoarseLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{retLVDflairCoarseLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\retLVDflairCoarseLTwoVarDecoderSegformerMlp}{\tbd{retLVDflairCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retLVDflairCoarseLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{retLVDflairCoarseLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\retLVDflairCoarseLTwoVarLossBootstrap}{\tbd{retLVDflairCoarseLTwoVarLossBootstrap}}
\providecommand{\retLVDflairCoarseLTwoVarLossGce}{\tbd{retLVDflairCoarseLTwoVarLossGce}}
\providecommand{\retLVDflairCoarseLTwoVarLrMultOne}{\tbd{retLVDflairCoarseLTwoVarLrMultOne}}
\providecommand{\retLVDflairCoarseLTwoVarLrMultThree}{\tbd{retLVDflairCoarseLTwoVarLrMultThree}}
\providecommand{\retLVDflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retLVDflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retLVDflairCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{retLVDflairCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retLVDflairOmissionLOne}{\tbd{retLVDflairOmissionLOne}}
\providecommand{\retLVDflairOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{retLVDflairOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retLVDflairOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{retLVDflairOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDflairOmissionLOneVarDecoderSamLite}{\tbd{retLVDflairOmissionLOneVarDecoderSamLite}}
\providecommand{\retLVDflairOmissionLOneVarDecoderSamPretrained}{\tbd{retLVDflairOmissionLOneVarDecoderSamPretrained}}
\providecommand{\retLVDflairOmissionLOneVarDecoderSegformerMlp}{\tbd{retLVDflairOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\retLVDflairOmissionLR}{\tbd{retLVDflairOmissionLR}}
\providecommand{\retLVDflairOmissionLRVarLrMultOne}{\tbd{retLVDflairOmissionLRVarLrMultOne}}
\providecommand{\retLVDflairOmissionLTwo}{\tbd{retLVDflairOmissionLTwo}}
\providecommand{\retLVDflairOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{retLVDflairOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retLVDflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{retLVDflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\retLVDflairOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retLVDflairOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{retLVDflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\retLVDflairOmissionLTwoVarDecoderSamLite}{\tbd{retLVDflairOmissionLTwoVarDecoderSamLite}}
\providecommand{\retLVDflairOmissionLTwoVarDecoderSamLiteLrMultOne}{\tbd{retLVDflairOmissionLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\retLVDflairOmissionLTwoVarDecoderSamPretrained}{\tbd{retLVDflairOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\retLVDflairOmissionLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{retLVDflairOmissionLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\retLVDflairOmissionLTwoVarDecoderSegformerMlp}{\tbd{retLVDflairOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retLVDflairOmissionLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{retLVDflairOmissionLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\retLVDflairOmissionLTwoVarLossBootstrap}{\tbd{retLVDflairOmissionLTwoVarLossBootstrap}}
\providecommand{\retLVDflairOmissionLTwoVarLossGce}{\tbd{retLVDflairOmissionLTwoVarLossGce}}
\providecommand{\retLVDflairOmissionLTwoVarLrMultOne}{\tbd{retLVDflairOmissionLTwoVarLrMultOne}}
\providecommand{\retLVDflairOmissionLTwoVarLrMultThree}{\tbd{retLVDflairOmissionLTwoVarLrMultThree}}
\providecommand{\retLVDflairOmissionLTwoVarLrMultZeroOneOneOneOne}{\tbd{retLVDflairOmissionLTwoVarLrMultZeroOneOneOneOne}}
\providecommand{\retLVDflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retLVDflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retLVDflairOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{retLVDflairOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retLVDflairShiftLOne}{\tbd{retLVDflairShiftLOne}}
\providecommand{\retLVDflairShiftLOneVarDecoderMaskTwoformerFull}{\tbd{retLVDflairShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retLVDflairShiftLOneVarDecoderMaskTwoformerLite}{\tbd{retLVDflairShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDflairShiftLOneVarDecoderSamLite}{\tbd{retLVDflairShiftLOneVarDecoderSamLite}}
\providecommand{\retLVDflairShiftLOneVarDecoderSamPretrained}{\tbd{retLVDflairShiftLOneVarDecoderSamPretrained}}
\providecommand{\retLVDflairShiftLOneVarDecoderSegformerMlp}{\tbd{retLVDflairShiftLOneVarDecoderSegformerMlp}}
\providecommand{\retLVDflairShiftLR}{\tbd{retLVDflairShiftLR}}
\providecommand{\retLVDflairShiftLRVarLrMultOne}{\tbd{retLVDflairShiftLRVarLrMultOne}}
\providecommand{\retLVDflairShiftLTwo}{\tbd{retLVDflairShiftLTwo}}
\providecommand{\retLVDflairShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{retLVDflairShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retLVDflairShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}{\tbd{retLVDflairShiftLTwoVarDecoderMaskTwoformerFullLrMultOne}}
\providecommand{\retLVDflairShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retLVDflairShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retLVDflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}{\tbd{retLVDflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultOne}}
\providecommand{\retLVDflairShiftLTwoVarDecoderSamLite}{\tbd{retLVDflairShiftLTwoVarDecoderSamLite}}
\providecommand{\retLVDflairShiftLTwoVarDecoderSamLiteLrMultOne}{\tbd{retLVDflairShiftLTwoVarDecoderSamLiteLrMultOne}}
\providecommand{\retLVDflairShiftLTwoVarDecoderSamPretrained}{\tbd{retLVDflairShiftLTwoVarDecoderSamPretrained}}
\providecommand{\retLVDflairShiftLTwoVarDecoderSamPretrainedLrMultOne}{\tbd{retLVDflairShiftLTwoVarDecoderSamPretrainedLrMultOne}}
\providecommand{\retLVDflairShiftLTwoVarDecoderSegformerMlp}{\tbd{retLVDflairShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retLVDflairShiftLTwoVarDecoderSegformerMlpLrMultOne}{\tbd{retLVDflairShiftLTwoVarDecoderSegformerMlpLrMultOne}}
\providecommand{\retLVDflairShiftLTwoVarLossBootstrap}{\tbd{retLVDflairShiftLTwoVarLossBootstrap}}
\providecommand{\retLVDflairShiftLTwoVarLossGce}{\tbd{retLVDflairShiftLTwoVarLossGce}}
\providecommand{\retLVDflairShiftLTwoVarLrMultOne}{\tbd{retLVDflairShiftLTwoVarLrMultOne}}
\providecommand{\retLVDflairShiftLTwoVarLrMultThree}{\tbd{retLVDflairShiftLTwoVarLrMultThree}}
\providecommand{\retLVDflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retLVDflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retLVDflairShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{retLVDflairShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retLVDsenOtsuLTwo}{\tbd{retLVDsenOtsuLTwo}}
\providecommand{\retPRIburnBoundaryLOne}{\tbd{retPRIburnBoundaryLOne}}
\providecommand{\retPRIburnBoundaryLTwo}{\tbd{retPRIburnBoundaryLTwo}}
\providecommand{\retPRIburnCoarseLOne}{\tbd{retPRIburnCoarseLOne}}
\providecommand{\retPRIburnCoarseLTwo}{\tbd{retPRIburnCoarseLTwo}}
\providecommand{\retPRIburnOmissionLOne}{\tbd{retPRIburnOmissionLOne}}
\providecommand{\retPRIburnOmissionLTwo}{\tbd{retPRIburnOmissionLTwo}}
\providecommand{\retPRIburnShiftLOne}{\tbd{retPRIburnShiftLOne}}
\providecommand{\retPRIburnShiftLTwo}{\tbd{retPRIburnShiftLTwo}}
\providecommand{\retPRIflairBoundaryLOne}{\tbd{retPRIflairBoundaryLOne}}
\providecommand{\retPRIflairBoundaryLTwo}{\tbd{retPRIflairBoundaryLTwo}}
\providecommand{\retPRIflairCoarseLOne}{\tbd{retPRIflairCoarseLOne}}
\providecommand{\retPRIflairCoarseLTwo}{\tbd{retPRIflairCoarseLTwo}}
\providecommand{\retPRIflairOmissionLOne}{\tbd{retPRIflairOmissionLOne}}
\providecommand{\retPRIflairOmissionLTwo}{\tbd{retPRIflairOmissionLTwo}}
\providecommand{\retPRIflairShiftLOne}{\tbd{retPRIflairShiftLOne}}
\providecommand{\retPRIflairShiftLTwo}{\tbd{retPRIflairShiftLTwo}}
\providecommand{\retRNChesBoundaryLOne}{\tbd{retRNChesBoundaryLOne}}
\providecommand{\retRNChesBoundaryLTwo}{\tbd{retRNChesBoundaryLTwo}}
\providecommand{\retRNChesCoarseLOne}{\tbd{retRNChesCoarseLOne}}
\providecommand{\retRNChesCoarseLTwo}{\tbd{retRNChesCoarseLTwo}}
\providecommand{\retRNChesNlcdREAL}{\tbd{retRNChesNlcdREAL}}
\providecommand{\retRNChesOmissionLOne}{\tbd{retRNChesOmissionLOne}}
\providecommand{\retRNChesOmissionLTwo}{\tbd{retRNChesOmissionLTwo}}
\providecommand{\retRNChesShiftLOne}{\tbd{retRNChesShiftLOne}}
\providecommand{\retRNChesShiftLTwo}{\tbd{retRNChesShiftLTwo}}
\providecommand{\retRNCsTwelveBoundaryLOne}{\tbd{retRNCsTwelveBoundaryLOne}}
\providecommand{\retRNCsTwelveBoundaryLTwo}{\tbd{retRNCsTwelveBoundaryLTwo}}
\providecommand{\retRNCsTwelveCoarseLOne}{\tbd{retRNCsTwelveCoarseLOne}}
\providecommand{\retRNCsTwelveCoarseLTwo}{\tbd{retRNCsTwelveCoarseLTwo}}
\providecommand{\retRNCsTwelveOmissionLOne}{\tbd{retRNCsTwelveOmissionLOne}}
\providecommand{\retRNCsTwelveOmissionLTwo}{\tbd{retRNCsTwelveOmissionLTwo}}
\providecommand{\retRNCsTwelveSTwocloudlessREAL}{\tbd{retRNCsTwelveSTwocloudlessREAL}}
\providecommand{\retRNCsTwelveShiftLOne}{\tbd{retRNCsTwelveShiftLOne}}
\providecommand{\retRNCsTwelveShiftLTwo}{\tbd{retRNCsTwelveShiftLTwo}}
\providecommand{\retRNDfcBoundaryLOne}{\tbd{retRNDfcBoundaryLOne}}
\providecommand{\retRNDfcBoundaryLTwo}{\tbd{retRNDfcBoundaryLTwo}}
\providecommand{\retRNDfcCoarseLOne}{\tbd{retRNDfcCoarseLOne}}
\providecommand{\retRNDfcCoarseLTwo}{\tbd{retRNDfcCoarseLTwo}}
\providecommand{\retRNDfcModisREALVarTrainSubsetRealcov}{\tbd{retRNDfcModisREALVarTrainSubsetRealcov}}
\providecommand{\retRNDfcOmissionLOne}{\tbd{retRNDfcOmissionLOne}}
\providecommand{\retRNDfcOmissionLTwo}{\tbd{retRNDfcOmissionLTwo}}
\providecommand{\retRNDfcShiftLOne}{\tbd{retRNDfcShiftLOne}}
\providecommand{\retRNDfcShiftLTwo}{\tbd{retRNDfcShiftLTwo}}
\providecommand{\retRNEnvaBoundaryLOne}{\tbd{retRNEnvaBoundaryLOne}}
\providecommand{\retRNEnvaBoundaryLTwo}{\tbd{retRNEnvaBoundaryLTwo}}
\providecommand{\retRNEnvaCoarseLOne}{\tbd{retRNEnvaCoarseLOne}}
\providecommand{\retRNEnvaCoarseLTwo}{\tbd{retRNEnvaCoarseLTwo}}
\providecommand{\retRNEnvaNlcdREAL}{\tbd{retRNEnvaNlcdREAL}}
\providecommand{\retRNEnvaOmissionLOne}{\tbd{retRNEnvaOmissionLOne}}
\providecommand{\retRNEnvaOmissionLTwo}{\tbd{retRNEnvaOmissionLTwo}}
\providecommand{\retRNEnvaShiftLOne}{\tbd{retRNEnvaShiftLOne}}
\providecommand{\retRNEnvaShiftLTwo}{\tbd{retRNEnvaShiftLTwo}}
\providecommand{\retRNKuroBoundaryLOne}{\tbd{retRNKuroBoundaryLOne}}
\providecommand{\retRNKuroBoundaryLTwo}{\tbd{retRNKuroBoundaryLTwo}}
\providecommand{\retRNKuroCemsREALVarTrainSubsetRealcov}{\tbd{retRNKuroCemsREALVarTrainSubsetRealcov}}
\providecommand{\retRNKuroCoarseLOne}{\tbd{retRNKuroCoarseLOne}}
\providecommand{\retRNKuroCoarseLTwo}{\tbd{retRNKuroCoarseLTwo}}
\providecommand{\retRNKuroOmissionLOne}{\tbd{retRNKuroOmissionLOne}}
\providecommand{\retRNKuroOmissionLTwo}{\tbd{retRNKuroOmissionLTwo}}
\providecommand{\retRNKuroShiftLOne}{\tbd{retRNKuroShiftLOne}}
\providecommand{\retRNKuroShiftLTwo}{\tbd{retRNKuroShiftLTwo}}
\providecommand{\retRNOemBoundaryLOne}{\tbd{retRNOemBoundaryLOne}}
\providecommand{\retRNOemBoundaryLTwo}{\tbd{retRNOemBoundaryLTwo}}
\providecommand{\retRNOemCoarseLOne}{\tbd{retRNOemCoarseLOne}}
\providecommand{\retRNOemCoarseLTwo}{\tbd{retRNOemCoarseLTwo}}
\providecommand{\retRNOemOmissionLOne}{\tbd{retRNOemOmissionLOne}}
\providecommand{\retRNOemOmissionLTwo}{\tbd{retRNOemOmissionLTwo}}
\providecommand{\retRNOemShiftLOne}{\tbd{retRNOemShiftLOne}}
\providecommand{\retRNOemShiftLTwo}{\tbd{retRNOemShiftLTwo}}
\providecommand{\retRNSnTwoBoundaryLOne}{\tbd{retRNSnTwoBoundaryLOne}}
\providecommand{\retRNSnTwoBoundaryLTwo}{\tbd{retRNSnTwoBoundaryLTwo}}
\providecommand{\retRNSnTwoCoarseLOne}{\tbd{retRNSnTwoCoarseLOne}}
\providecommand{\retRNSnTwoCoarseLTwo}{\tbd{retRNSnTwoCoarseLTwo}}
\providecommand{\retRNSnTwoOmissionLOne}{\tbd{retRNSnTwoOmissionLOne}}
\providecommand{\retRNSnTwoOmissionLTwo}{\tbd{retRNSnTwoOmissionLTwo}}
\providecommand{\retRNSnTwoShiftLOne}{\tbd{retRNSnTwoShiftLOne}}
\providecommand{\retRNSnTwoShiftLTwo}{\tbd{retRNSnTwoShiftLTwo}}
\providecommand{\retRNburnBoundaryLOne}{\tbd{retRNburnBoundaryLOne}}
\providecommand{\retRNburnBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{retRNburnBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retRNburnBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{retRNburnBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retRNburnBoundaryLOneVarDecoderSamLite}{\tbd{retRNburnBoundaryLOneVarDecoderSamLite}}
\providecommand{\retRNburnBoundaryLOneVarDecoderSamPretrained}{\tbd{retRNburnBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\retRNburnBoundaryLOneVarDecoderSegformerMlp}{\tbd{retRNburnBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\retRNburnBoundaryLR}{\tbd{retRNburnBoundaryLR}}
\providecommand{\retRNburnBoundaryLTwo}{\tbd{retRNburnBoundaryLTwo}}
\providecommand{\retRNburnBoundaryLTwoVarBandsRgb}{\tbd{retRNburnBoundaryLTwoVarBandsRgb}}
\providecommand{\retRNburnBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{retRNburnBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retRNburnBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retRNburnBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retRNburnBoundaryLTwoVarDecoderSamLite}{\tbd{retRNburnBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retRNburnBoundaryLTwoVarDecoderSamPretrained}{\tbd{retRNburnBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\retRNburnBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retRNburnBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retRNburnBoundaryLTwoVarInitRandom}{\tbd{retRNburnBoundaryLTwoVarInitRandom}}
\providecommand{\retRNburnBoundaryLTwoVarLossBootstrap}{\tbd{retRNburnBoundaryLTwoVarLossBootstrap}}
\providecommand{\retRNburnBoundaryLTwoVarLossGce}{\tbd{retRNburnBoundaryLTwoVarLossGce}}
\providecommand{\retRNburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retRNburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retRNburnBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{retRNburnBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retRNburnCoarseLOne}{\tbd{retRNburnCoarseLOne}}
\providecommand{\retRNburnCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{retRNburnCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retRNburnCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{retRNburnCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retRNburnCoarseLOneVarDecoderSamLite}{\tbd{retRNburnCoarseLOneVarDecoderSamLite}}
\providecommand{\retRNburnCoarseLOneVarDecoderSamPretrained}{\tbd{retRNburnCoarseLOneVarDecoderSamPretrained}}
\providecommand{\retRNburnCoarseLOneVarDecoderSegformerMlp}{\tbd{retRNburnCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\retRNburnCoarseLR}{\tbd{retRNburnCoarseLR}}
\providecommand{\retRNburnCoarseLTwo}{\tbd{retRNburnCoarseLTwo}}
\providecommand{\retRNburnCoarseLTwoVarBandsRgb}{\tbd{retRNburnCoarseLTwoVarBandsRgb}}
\providecommand{\retRNburnCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{retRNburnCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retRNburnCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retRNburnCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retRNburnCoarseLTwoVarDecoderSamLite}{\tbd{retRNburnCoarseLTwoVarDecoderSamLite}}
\providecommand{\retRNburnCoarseLTwoVarDecoderSamPretrained}{\tbd{retRNburnCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\retRNburnCoarseLTwoVarDecoderSegformerMlp}{\tbd{retRNburnCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retRNburnCoarseLTwoVarInitRandom}{\tbd{retRNburnCoarseLTwoVarInitRandom}}
\providecommand{\retRNburnCoarseLTwoVarLossBootstrap}{\tbd{retRNburnCoarseLTwoVarLossBootstrap}}
\providecommand{\retRNburnCoarseLTwoVarLossGce}{\tbd{retRNburnCoarseLTwoVarLossGce}}
\providecommand{\retRNburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retRNburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retRNburnCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{retRNburnCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retRNburnOmissionLOne}{\tbd{retRNburnOmissionLOne}}
\providecommand{\retRNburnOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{retRNburnOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retRNburnOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{retRNburnOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retRNburnOmissionLOneVarDecoderSamLite}{\tbd{retRNburnOmissionLOneVarDecoderSamLite}}
\providecommand{\retRNburnOmissionLOneVarDecoderSamPretrained}{\tbd{retRNburnOmissionLOneVarDecoderSamPretrained}}
\providecommand{\retRNburnOmissionLOneVarDecoderSegformerMlp}{\tbd{retRNburnOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\retRNburnOmissionLR}{\tbd{retRNburnOmissionLR}}
\providecommand{\retRNburnOmissionLTwo}{\tbd{retRNburnOmissionLTwo}}
\providecommand{\retRNburnOmissionLTwoVarBandsRgb}{\tbd{retRNburnOmissionLTwoVarBandsRgb}}
\providecommand{\retRNburnOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{retRNburnOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retRNburnOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retRNburnOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retRNburnOmissionLTwoVarDecoderSamLite}{\tbd{retRNburnOmissionLTwoVarDecoderSamLite}}
\providecommand{\retRNburnOmissionLTwoVarDecoderSamPretrained}{\tbd{retRNburnOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\retRNburnOmissionLTwoVarDecoderSegformerMlp}{\tbd{retRNburnOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retRNburnOmissionLTwoVarInitRandom}{\tbd{retRNburnOmissionLTwoVarInitRandom}}
\providecommand{\retRNburnOmissionLTwoVarLossBootstrap}{\tbd{retRNburnOmissionLTwoVarLossBootstrap}}
\providecommand{\retRNburnOmissionLTwoVarLossGce}{\tbd{retRNburnOmissionLTwoVarLossGce}}
\providecommand{\retRNburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retRNburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retRNburnOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{retRNburnOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retRNburnShiftLOne}{\tbd{retRNburnShiftLOne}}
\providecommand{\retRNburnShiftLOneVarDecoderMaskTwoformerFull}{\tbd{retRNburnShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retRNburnShiftLOneVarDecoderMaskTwoformerLite}{\tbd{retRNburnShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retRNburnShiftLOneVarDecoderSamLite}{\tbd{retRNburnShiftLOneVarDecoderSamLite}}
\providecommand{\retRNburnShiftLOneVarDecoderSamPretrained}{\tbd{retRNburnShiftLOneVarDecoderSamPretrained}}
\providecommand{\retRNburnShiftLOneVarDecoderSegformerMlp}{\tbd{retRNburnShiftLOneVarDecoderSegformerMlp}}
\providecommand{\retRNburnShiftLR}{\tbd{retRNburnShiftLR}}
\providecommand{\retRNburnShiftLTwo}{\tbd{retRNburnShiftLTwo}}
\providecommand{\retRNburnShiftLTwoVarBandsRgb}{\tbd{retRNburnShiftLTwoVarBandsRgb}}
\providecommand{\retRNburnShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{retRNburnShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retRNburnShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retRNburnShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retRNburnShiftLTwoVarDecoderSamLite}{\tbd{retRNburnShiftLTwoVarDecoderSamLite}}
\providecommand{\retRNburnShiftLTwoVarDecoderSamPretrained}{\tbd{retRNburnShiftLTwoVarDecoderSamPretrained}}
\providecommand{\retRNburnShiftLTwoVarDecoderSegformerMlp}{\tbd{retRNburnShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retRNburnShiftLTwoVarInitRandom}{\tbd{retRNburnShiftLTwoVarInitRandom}}
\providecommand{\retRNburnShiftLTwoVarLossBootstrap}{\tbd{retRNburnShiftLTwoVarLossBootstrap}}
\providecommand{\retRNburnShiftLTwoVarLossGce}{\tbd{retRNburnShiftLTwoVarLossGce}}
\providecommand{\retRNburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retRNburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retRNburnShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{retRNburnShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retRNflairBoundaryLOne}{\tbd{retRNflairBoundaryLOne}}
\providecommand{\retRNflairBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{retRNflairBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retRNflairBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{retRNflairBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retRNflairBoundaryLOneVarDecoderSamLite}{\tbd{retRNflairBoundaryLOneVarDecoderSamLite}}
\providecommand{\retRNflairBoundaryLOneVarDecoderSamPretrained}{\tbd{retRNflairBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\retRNflairBoundaryLOneVarDecoderSegformerMlp}{\tbd{retRNflairBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\retRNflairBoundaryLR}{\tbd{retRNflairBoundaryLR}}
\providecommand{\retRNflairBoundaryLTwo}{\tbd{retRNflairBoundaryLTwo}}
\providecommand{\retRNflairBoundaryLTwoVarBandsRgb}{\tbd{retRNflairBoundaryLTwoVarBandsRgb}}
\providecommand{\retRNflairBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{retRNflairBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retRNflairBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retRNflairBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retRNflairBoundaryLTwoVarDecoderSamLite}{\tbd{retRNflairBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retRNflairBoundaryLTwoVarDecoderSamPretrained}{\tbd{retRNflairBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\retRNflairBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retRNflairBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retRNflairBoundaryLTwoVarInitRandom}{\tbd{retRNflairBoundaryLTwoVarInitRandom}}
\providecommand{\retRNflairBoundaryLTwoVarLossBootstrap}{\tbd{retRNflairBoundaryLTwoVarLossBootstrap}}
\providecommand{\retRNflairBoundaryLTwoVarLossGce}{\tbd{retRNflairBoundaryLTwoVarLossGce}}
\providecommand{\retRNflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retRNflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retRNflairBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{retRNflairBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retRNflairCoarseLOne}{\tbd{retRNflairCoarseLOne}}
\providecommand{\retRNflairCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{retRNflairCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retRNflairCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{retRNflairCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retRNflairCoarseLOneVarDecoderSamLite}{\tbd{retRNflairCoarseLOneVarDecoderSamLite}}
\providecommand{\retRNflairCoarseLOneVarDecoderSamPretrained}{\tbd{retRNflairCoarseLOneVarDecoderSamPretrained}}
\providecommand{\retRNflairCoarseLOneVarDecoderSegformerMlp}{\tbd{retRNflairCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\retRNflairCoarseLR}{\tbd{retRNflairCoarseLR}}
\providecommand{\retRNflairCoarseLTwo}{\tbd{retRNflairCoarseLTwo}}
\providecommand{\retRNflairCoarseLTwoVarBandsRgb}{\tbd{retRNflairCoarseLTwoVarBandsRgb}}
\providecommand{\retRNflairCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{retRNflairCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retRNflairCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retRNflairCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retRNflairCoarseLTwoVarDecoderSamLite}{\tbd{retRNflairCoarseLTwoVarDecoderSamLite}}
\providecommand{\retRNflairCoarseLTwoVarDecoderSamPretrained}{\tbd{retRNflairCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\retRNflairCoarseLTwoVarDecoderSegformerMlp}{\tbd{retRNflairCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retRNflairCoarseLTwoVarInitRandom}{\tbd{retRNflairCoarseLTwoVarInitRandom}}
\providecommand{\retRNflairCoarseLTwoVarLossBootstrap}{\tbd{retRNflairCoarseLTwoVarLossBootstrap}}
\providecommand{\retRNflairCoarseLTwoVarLossGce}{\tbd{retRNflairCoarseLTwoVarLossGce}}
\providecommand{\retRNflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retRNflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retRNflairCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{retRNflairCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retRNflairOmissionLOne}{\tbd{retRNflairOmissionLOne}}
\providecommand{\retRNflairOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{retRNflairOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retRNflairOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{retRNflairOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retRNflairOmissionLOneVarDecoderSamLite}{\tbd{retRNflairOmissionLOneVarDecoderSamLite}}
\providecommand{\retRNflairOmissionLOneVarDecoderSamPretrained}{\tbd{retRNflairOmissionLOneVarDecoderSamPretrained}}
\providecommand{\retRNflairOmissionLOneVarDecoderSegformerMlp}{\tbd{retRNflairOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\retRNflairOmissionLR}{\tbd{retRNflairOmissionLR}}
\providecommand{\retRNflairOmissionLTwo}{\tbd{retRNflairOmissionLTwo}}
\providecommand{\retRNflairOmissionLTwoVarBandsRgb}{\tbd{retRNflairOmissionLTwoVarBandsRgb}}
\providecommand{\retRNflairOmissionLTwoVarClassWeightedTrue}{\tbd{retRNflairOmissionLTwoVarClassWeightedTrue}}
\providecommand{\retRNflairOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{retRNflairOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retRNflairOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retRNflairOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retRNflairOmissionLTwoVarDecoderSamLite}{\tbd{retRNflairOmissionLTwoVarDecoderSamLite}}
\providecommand{\retRNflairOmissionLTwoVarDecoderSamPretrained}{\tbd{retRNflairOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\retRNflairOmissionLTwoVarDecoderSegformerMlp}{\tbd{retRNflairOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retRNflairOmissionLTwoVarInitRandom}{\tbd{retRNflairOmissionLTwoVarInitRandom}}
\providecommand{\retRNflairOmissionLTwoVarLossBootstrap}{\tbd{retRNflairOmissionLTwoVarLossBootstrap}}
\providecommand{\retRNflairOmissionLTwoVarLossGce}{\tbd{retRNflairOmissionLTwoVarLossGce}}
\providecommand{\retRNflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retRNflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retRNflairOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{retRNflairOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retRNflairShiftLOne}{\tbd{retRNflairShiftLOne}}
\providecommand{\retRNflairShiftLOneVarDecoderMaskTwoformerFull}{\tbd{retRNflairShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retRNflairShiftLOneVarDecoderMaskTwoformerLite}{\tbd{retRNflairShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retRNflairShiftLOneVarDecoderSamLite}{\tbd{retRNflairShiftLOneVarDecoderSamLite}}
\providecommand{\retRNflairShiftLOneVarDecoderSamPretrained}{\tbd{retRNflairShiftLOneVarDecoderSamPretrained}}
\providecommand{\retRNflairShiftLOneVarDecoderSegformerMlp}{\tbd{retRNflairShiftLOneVarDecoderSegformerMlp}}
\providecommand{\retRNflairShiftLR}{\tbd{retRNflairShiftLR}}
\providecommand{\retRNflairShiftLTwo}{\tbd{retRNflairShiftLTwo}}
\providecommand{\retRNflairShiftLTwoVarBandsRgb}{\tbd{retRNflairShiftLTwoVarBandsRgb}}
\providecommand{\retRNflairShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{retRNflairShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retRNflairShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retRNflairShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retRNflairShiftLTwoVarDecoderSamLite}{\tbd{retRNflairShiftLTwoVarDecoderSamLite}}
\providecommand{\retRNflairShiftLTwoVarDecoderSamPretrained}{\tbd{retRNflairShiftLTwoVarDecoderSamPretrained}}
\providecommand{\retRNflairShiftLTwoVarDecoderSegformerMlp}{\tbd{retRNflairShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retRNflairShiftLTwoVarInitRandom}{\tbd{retRNflairShiftLTwoVarInitRandom}}
\providecommand{\retRNflairShiftLTwoVarLossBootstrap}{\tbd{retRNflairShiftLTwoVarLossBootstrap}}
\providecommand{\retRNflairShiftLTwoVarLossGce}{\tbd{retRNflairShiftLTwoVarLossGce}}
\providecommand{\retRNflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retRNflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retRNflairShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{retRNflairShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retRNsenOtsuLTwo}{\tbd{retRNsenOtsuLTwo}}
\providecommand{\retResnetFiveZeroSslFoureoburnBoundaryLOne}{\tbd{retResnetFiveZeroSslFoureoburnBoundaryLOne}}
\providecommand{\retResnetFiveZeroSslFoureoburnBoundaryLTwo}{\tbd{retResnetFiveZeroSslFoureoburnBoundaryLTwo}}
\providecommand{\retResnetFiveZeroSslFoureoburnCoarseLOne}{\tbd{retResnetFiveZeroSslFoureoburnCoarseLOne}}
\providecommand{\retResnetFiveZeroSslFoureoburnCoarseLTwo}{\tbd{retResnetFiveZeroSslFoureoburnCoarseLTwo}}
\providecommand{\retResnetFiveZeroSslFoureoburnOmissionLOne}{\tbd{retResnetFiveZeroSslFoureoburnOmissionLOne}}
\providecommand{\retResnetFiveZeroSslFoureoburnOmissionLTwo}{\tbd{retResnetFiveZeroSslFoureoburnOmissionLTwo}}
\providecommand{\retResnetFiveZeroSslFoureoburnShiftLOne}{\tbd{retResnetFiveZeroSslFoureoburnShiftLOne}}
\providecommand{\retResnetFiveZeroSslFoureoburnShiftLTwo}{\tbd{retResnetFiveZeroSslFoureoburnShiftLTwo}}
\providecommand{\retResnetFiveZeroSslFoureoflairBoundaryLOne}{\tbd{retResnetFiveZeroSslFoureoflairBoundaryLOne}}
\providecommand{\retResnetFiveZeroSslFoureoflairBoundaryLTwo}{\tbd{retResnetFiveZeroSslFoureoflairBoundaryLTwo}}
\providecommand{\retResnetFiveZeroSslFoureoflairCoarseLOne}{\tbd{retResnetFiveZeroSslFoureoflairCoarseLOne}}
\providecommand{\retResnetFiveZeroSslFoureoflairCoarseLTwo}{\tbd{retResnetFiveZeroSslFoureoflairCoarseLTwo}}
\providecommand{\retResnetFiveZeroSslFoureoflairOmissionLOne}{\tbd{retResnetFiveZeroSslFoureoflairOmissionLOne}}
\providecommand{\retResnetFiveZeroSslFoureoflairOmissionLTwo}{\tbd{retResnetFiveZeroSslFoureoflairOmissionLTwo}}
\providecommand{\retResnetFiveZeroSslFoureoflairShiftLOne}{\tbd{retResnetFiveZeroSslFoureoflairShiftLOne}}
\providecommand{\retResnetFiveZeroSslFoureoflairShiftLTwo}{\tbd{retResnetFiveZeroSslFoureoflairShiftLTwo}}
\providecommand{\retSATChesBoundaryLOne}{\tbd{retSATChesBoundaryLOne}}
\providecommand{\retSATChesBoundaryLTwo}{\tbd{retSATChesBoundaryLTwo}}
\providecommand{\retSATChesBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retSATChesBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retSATChesBoundaryLTwoVarDecoderSamLite}{\tbd{retSATChesBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retSATChesBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retSATChesBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retSATChesBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATChesBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATChesCoarseLOne}{\tbd{retSATChesCoarseLOne}}
\providecommand{\retSATChesCoarseLTwo}{\tbd{retSATChesCoarseLTwo}}
\providecommand{\retSATChesCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retSATChesCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retSATChesCoarseLTwoVarDecoderSamLite}{\tbd{retSATChesCoarseLTwoVarDecoderSamLite}}
\providecommand{\retSATChesCoarseLTwoVarDecoderSegformerMlp}{\tbd{retSATChesCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retSATChesCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATChesCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATChesNlcdREAL}{\tbd{retSATChesNlcdREAL}}
\providecommand{\retSATChesOmissionLOne}{\tbd{retSATChesOmissionLOne}}
\providecommand{\retSATChesOmissionLTwo}{\tbd{retSATChesOmissionLTwo}}
\providecommand{\retSATChesOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retSATChesOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retSATChesOmissionLTwoVarDecoderSamLite}{\tbd{retSATChesOmissionLTwoVarDecoderSamLite}}
\providecommand{\retSATChesOmissionLTwoVarDecoderSegformerMlp}{\tbd{retSATChesOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retSATChesOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATChesOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATChesShiftLOne}{\tbd{retSATChesShiftLOne}}
\providecommand{\retSATChesShiftLTwo}{\tbd{retSATChesShiftLTwo}}
\providecommand{\retSATChesShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retSATChesShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retSATChesShiftLTwoVarDecoderSamLite}{\tbd{retSATChesShiftLTwoVarDecoderSamLite}}
\providecommand{\retSATChesShiftLTwoVarDecoderSegformerMlp}{\tbd{retSATChesShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retSATChesShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATChesShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATCsTwelveBoundaryLOne}{\tbd{retSATCsTwelveBoundaryLOne}}
\providecommand{\retSATCsTwelveBoundaryLTwo}{\tbd{retSATCsTwelveBoundaryLTwo}}
\providecommand{\retSATCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retSATCsTwelveBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retSATCsTwelveBoundaryLTwoVarDecoderSamLite}{\tbd{retSATCsTwelveBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retSATCsTwelveBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retSATCsTwelveBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retSATCsTwelveBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATCsTwelveBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATCsTwelveCoarseLOne}{\tbd{retSATCsTwelveCoarseLOne}}
\providecommand{\retSATCsTwelveCoarseLTwo}{\tbd{retSATCsTwelveCoarseLTwo}}
\providecommand{\retSATCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retSATCsTwelveCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retSATCsTwelveCoarseLTwoVarDecoderSamLite}{\tbd{retSATCsTwelveCoarseLTwoVarDecoderSamLite}}
\providecommand{\retSATCsTwelveCoarseLTwoVarDecoderSegformerMlp}{\tbd{retSATCsTwelveCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retSATCsTwelveCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATCsTwelveCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATCsTwelveOmissionLOne}{\tbd{retSATCsTwelveOmissionLOne}}
\providecommand{\retSATCsTwelveOmissionLTwo}{\tbd{retSATCsTwelveOmissionLTwo}}
\providecommand{\retSATCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retSATCsTwelveOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retSATCsTwelveOmissionLTwoVarDecoderSamLite}{\tbd{retSATCsTwelveOmissionLTwoVarDecoderSamLite}}
\providecommand{\retSATCsTwelveOmissionLTwoVarDecoderSegformerMlp}{\tbd{retSATCsTwelveOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retSATCsTwelveOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATCsTwelveOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATCsTwelveSTwocloudlessREAL}{\tbd{retSATCsTwelveSTwocloudlessREAL}}
\providecommand{\retSATCsTwelveShiftLOne}{\tbd{retSATCsTwelveShiftLOne}}
\providecommand{\retSATCsTwelveShiftLTwo}{\tbd{retSATCsTwelveShiftLTwo}}
\providecommand{\retSATCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retSATCsTwelveShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retSATCsTwelveShiftLTwoVarDecoderSamLite}{\tbd{retSATCsTwelveShiftLTwoVarDecoderSamLite}}
\providecommand{\retSATCsTwelveShiftLTwoVarDecoderSegformerMlp}{\tbd{retSATCsTwelveShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retSATCsTwelveShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATCsTwelveShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATDfcBoundaryLOne}{\tbd{retSATDfcBoundaryLOne}}
\providecommand{\retSATDfcBoundaryLTwo}{\tbd{retSATDfcBoundaryLTwo}}
\providecommand{\retSATDfcBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retSATDfcBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retSATDfcBoundaryLTwoVarDecoderSamLite}{\tbd{retSATDfcBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retSATDfcBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retSATDfcBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retSATDfcBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATDfcBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATDfcCoarseLOne}{\tbd{retSATDfcCoarseLOne}}
\providecommand{\retSATDfcCoarseLTwo}{\tbd{retSATDfcCoarseLTwo}}
\providecommand{\retSATDfcCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retSATDfcCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retSATDfcCoarseLTwoVarDecoderSamLite}{\tbd{retSATDfcCoarseLTwoVarDecoderSamLite}}
\providecommand{\retSATDfcCoarseLTwoVarDecoderSegformerMlp}{\tbd{retSATDfcCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retSATDfcCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATDfcCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATDfcModisREALVarTrainSubsetRealcov}{\tbd{retSATDfcModisREALVarTrainSubsetRealcov}}
\providecommand{\retSATDfcOmissionLOne}{\tbd{retSATDfcOmissionLOne}}
\providecommand{\retSATDfcOmissionLTwo}{\tbd{retSATDfcOmissionLTwo}}
\providecommand{\retSATDfcOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retSATDfcOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retSATDfcOmissionLTwoVarDecoderSamLite}{\tbd{retSATDfcOmissionLTwoVarDecoderSamLite}}
\providecommand{\retSATDfcOmissionLTwoVarDecoderSegformerMlp}{\tbd{retSATDfcOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retSATDfcOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATDfcOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATDfcShiftLOne}{\tbd{retSATDfcShiftLOne}}
\providecommand{\retSATDfcShiftLTwo}{\tbd{retSATDfcShiftLTwo}}
\providecommand{\retSATDfcShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retSATDfcShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retSATDfcShiftLTwoVarDecoderSamLite}{\tbd{retSATDfcShiftLTwoVarDecoderSamLite}}
\providecommand{\retSATDfcShiftLTwoVarDecoderSegformerMlp}{\tbd{retSATDfcShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retSATDfcShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATDfcShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATEnvaBoundaryLOne}{\tbd{retSATEnvaBoundaryLOne}}
\providecommand{\retSATEnvaBoundaryLTwo}{\tbd{retSATEnvaBoundaryLTwo}}
\providecommand{\retSATEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retSATEnvaBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retSATEnvaBoundaryLTwoVarDecoderSamLite}{\tbd{retSATEnvaBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retSATEnvaBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retSATEnvaBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retSATEnvaBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATEnvaBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATEnvaCoarseLOne}{\tbd{retSATEnvaCoarseLOne}}
\providecommand{\retSATEnvaCoarseLTwo}{\tbd{retSATEnvaCoarseLTwo}}
\providecommand{\retSATEnvaCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retSATEnvaCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retSATEnvaCoarseLTwoVarDecoderSamLite}{\tbd{retSATEnvaCoarseLTwoVarDecoderSamLite}}
\providecommand{\retSATEnvaCoarseLTwoVarDecoderSegformerMlp}{\tbd{retSATEnvaCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retSATEnvaCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATEnvaCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATEnvaNlcdREAL}{\tbd{retSATEnvaNlcdREAL}}
\providecommand{\retSATEnvaOmissionLOne}{\tbd{retSATEnvaOmissionLOne}}
\providecommand{\retSATEnvaOmissionLTwo}{\tbd{retSATEnvaOmissionLTwo}}
\providecommand{\retSATEnvaOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retSATEnvaOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retSATEnvaOmissionLTwoVarDecoderSamLite}{\tbd{retSATEnvaOmissionLTwoVarDecoderSamLite}}
\providecommand{\retSATEnvaOmissionLTwoVarDecoderSegformerMlp}{\tbd{retSATEnvaOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retSATEnvaOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATEnvaOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATEnvaShiftLOne}{\tbd{retSATEnvaShiftLOne}}
\providecommand{\retSATEnvaShiftLTwo}{\tbd{retSATEnvaShiftLTwo}}
\providecommand{\retSATEnvaShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retSATEnvaShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retSATEnvaShiftLTwoVarDecoderSamLite}{\tbd{retSATEnvaShiftLTwoVarDecoderSamLite}}
\providecommand{\retSATEnvaShiftLTwoVarDecoderSegformerMlp}{\tbd{retSATEnvaShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retSATEnvaShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATEnvaShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATKuroBoundaryLOne}{\tbd{retSATKuroBoundaryLOne}}
\providecommand{\retSATKuroBoundaryLTwo}{\tbd{retSATKuroBoundaryLTwo}}
\providecommand{\retSATKuroBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retSATKuroBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retSATKuroBoundaryLTwoVarDecoderSamLite}{\tbd{retSATKuroBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retSATKuroBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retSATKuroBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retSATKuroBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATKuroBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATKuroCemsREALVarTrainSubsetRealcov}{\tbd{retSATKuroCemsREALVarTrainSubsetRealcov}}
\providecommand{\retSATKuroCoarseLOne}{\tbd{retSATKuroCoarseLOne}}
\providecommand{\retSATKuroCoarseLTwo}{\tbd{retSATKuroCoarseLTwo}}
\providecommand{\retSATKuroCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retSATKuroCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retSATKuroCoarseLTwoVarDecoderSamLite}{\tbd{retSATKuroCoarseLTwoVarDecoderSamLite}}
\providecommand{\retSATKuroCoarseLTwoVarDecoderSegformerMlp}{\tbd{retSATKuroCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retSATKuroCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATKuroCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATKuroOmissionLOne}{\tbd{retSATKuroOmissionLOne}}
\providecommand{\retSATKuroOmissionLTwo}{\tbd{retSATKuroOmissionLTwo}}
\providecommand{\retSATKuroOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retSATKuroOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retSATKuroOmissionLTwoVarDecoderSamLite}{\tbd{retSATKuroOmissionLTwoVarDecoderSamLite}}
\providecommand{\retSATKuroOmissionLTwoVarDecoderSegformerMlp}{\tbd{retSATKuroOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retSATKuroOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATKuroOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATKuroShiftLOne}{\tbd{retSATKuroShiftLOne}}
\providecommand{\retSATKuroShiftLTwo}{\tbd{retSATKuroShiftLTwo}}
\providecommand{\retSATKuroShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retSATKuroShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retSATKuroShiftLTwoVarDecoderSamLite}{\tbd{retSATKuroShiftLTwoVarDecoderSamLite}}
\providecommand{\retSATKuroShiftLTwoVarDecoderSegformerMlp}{\tbd{retSATKuroShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retSATKuroShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATKuroShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATOemBoundaryLOne}{\tbd{retSATOemBoundaryLOne}}
\providecommand{\retSATOemBoundaryLTwo}{\tbd{retSATOemBoundaryLTwo}}
\providecommand{\retSATOemBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retSATOemBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retSATOemBoundaryLTwoVarDecoderSamLite}{\tbd{retSATOemBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retSATOemBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retSATOemBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retSATOemBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATOemBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATOemCoarseLOne}{\tbd{retSATOemCoarseLOne}}
\providecommand{\retSATOemCoarseLTwo}{\tbd{retSATOemCoarseLTwo}}
\providecommand{\retSATOemCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retSATOemCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retSATOemCoarseLTwoVarDecoderSamLite}{\tbd{retSATOemCoarseLTwoVarDecoderSamLite}}
\providecommand{\retSATOemCoarseLTwoVarDecoderSegformerMlp}{\tbd{retSATOemCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retSATOemCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATOemCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATOemOmissionLOne}{\tbd{retSATOemOmissionLOne}}
\providecommand{\retSATOemOmissionLTwo}{\tbd{retSATOemOmissionLTwo}}
\providecommand{\retSATOemOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retSATOemOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retSATOemOmissionLTwoVarDecoderSamLite}{\tbd{retSATOemOmissionLTwoVarDecoderSamLite}}
\providecommand{\retSATOemOmissionLTwoVarDecoderSegformerMlp}{\tbd{retSATOemOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retSATOemOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATOemOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATOemShiftLOne}{\tbd{retSATOemShiftLOne}}
\providecommand{\retSATOemShiftLTwo}{\tbd{retSATOemShiftLTwo}}
\providecommand{\retSATOemShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retSATOemShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retSATOemShiftLTwoVarDecoderSamLite}{\tbd{retSATOemShiftLTwoVarDecoderSamLite}}
\providecommand{\retSATOemShiftLTwoVarDecoderSegformerMlp}{\tbd{retSATOemShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retSATOemShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATOemShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATSnTwoBoundaryLOne}{\tbd{retSATSnTwoBoundaryLOne}}
\providecommand{\retSATSnTwoBoundaryLTwo}{\tbd{retSATSnTwoBoundaryLTwo}}
\providecommand{\retSATSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retSATSnTwoBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retSATSnTwoBoundaryLTwoVarDecoderSamLite}{\tbd{retSATSnTwoBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retSATSnTwoBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retSATSnTwoBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retSATSnTwoBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATSnTwoBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATSnTwoCoarseLOne}{\tbd{retSATSnTwoCoarseLOne}}
\providecommand{\retSATSnTwoCoarseLTwo}{\tbd{retSATSnTwoCoarseLTwo}}
\providecommand{\retSATSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retSATSnTwoCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retSATSnTwoCoarseLTwoVarDecoderSamLite}{\tbd{retSATSnTwoCoarseLTwoVarDecoderSamLite}}
\providecommand{\retSATSnTwoCoarseLTwoVarDecoderSegformerMlp}{\tbd{retSATSnTwoCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retSATSnTwoCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATSnTwoCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATSnTwoOmissionLOne}{\tbd{retSATSnTwoOmissionLOne}}
\providecommand{\retSATSnTwoOmissionLTwo}{\tbd{retSATSnTwoOmissionLTwo}}
\providecommand{\retSATSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retSATSnTwoOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retSATSnTwoOmissionLTwoVarDecoderSamLite}{\tbd{retSATSnTwoOmissionLTwoVarDecoderSamLite}}
\providecommand{\retSATSnTwoOmissionLTwoVarDecoderSegformerMlp}{\tbd{retSATSnTwoOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retSATSnTwoOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATSnTwoOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATSnTwoShiftLOne}{\tbd{retSATSnTwoShiftLOne}}
\providecommand{\retSATSnTwoShiftLTwo}{\tbd{retSATSnTwoShiftLTwo}}
\providecommand{\retSATSnTwoShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retSATSnTwoShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retSATSnTwoShiftLTwoVarDecoderSamLite}{\tbd{retSATSnTwoShiftLTwoVarDecoderSamLite}}
\providecommand{\retSATSnTwoShiftLTwoVarDecoderSegformerMlp}{\tbd{retSATSnTwoShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retSATSnTwoShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATSnTwoShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATburnBoundaryLOne}{\tbd{retSATburnBoundaryLOne}}
\providecommand{\retSATburnBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{retSATburnBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retSATburnBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{retSATburnBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retSATburnBoundaryLOneVarDecoderSamLite}{\tbd{retSATburnBoundaryLOneVarDecoderSamLite}}
\providecommand{\retSATburnBoundaryLOneVarDecoderSamPretrained}{\tbd{retSATburnBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\retSATburnBoundaryLOneVarDecoderSegformerMlp}{\tbd{retSATburnBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\retSATburnBoundaryLR}{\tbd{retSATburnBoundaryLR}}
\providecommand{\retSATburnBoundaryLRVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATburnBoundaryLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATburnBoundaryLTwo}{\tbd{retSATburnBoundaryLTwo}}
\providecommand{\retSATburnBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{retSATburnBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retSATburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{retSATburnBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATburnBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retSATburnBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retSATburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{retSATburnBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATburnBoundaryLTwoVarDecoderSamLite}{\tbd{retSATburnBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retSATburnBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{retSATburnBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATburnBoundaryLTwoVarDecoderSamPretrained}{\tbd{retSATburnBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\retSATburnBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{retSATburnBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATburnBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retSATburnBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retSATburnBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{retSATburnBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATburnBoundaryLTwoVarFrozenEncoderTrue}{\tbd{retSATburnBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\retSATburnBoundaryLTwoVarLossBootstrap}{\tbd{retSATburnBoundaryLTwoVarLossBootstrap}}
\providecommand{\retSATburnBoundaryLTwoVarLossGce}{\tbd{retSATburnBoundaryLTwoVarLossGce}}
\providecommand{\retSATburnBoundaryLTwoVarLrMultThree}{\tbd{retSATburnBoundaryLTwoVarLrMultThree}}
\providecommand{\retSATburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATburnBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{retSATburnBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retSATburnBoundaryLTwoVarValLabelsClean}{\tbd{retSATburnBoundaryLTwoVarValLabelsClean}}
\providecommand{\retSATburnCoarseLOne}{\tbd{retSATburnCoarseLOne}}
\providecommand{\retSATburnCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{retSATburnCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retSATburnCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{retSATburnCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retSATburnCoarseLOneVarDecoderSamLite}{\tbd{retSATburnCoarseLOneVarDecoderSamLite}}
\providecommand{\retSATburnCoarseLOneVarDecoderSamPretrained}{\tbd{retSATburnCoarseLOneVarDecoderSamPretrained}}
\providecommand{\retSATburnCoarseLOneVarDecoderSegformerMlp}{\tbd{retSATburnCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\retSATburnCoarseLR}{\tbd{retSATburnCoarseLR}}
\providecommand{\retSATburnCoarseLRVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATburnCoarseLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATburnCoarseLTwo}{\tbd{retSATburnCoarseLTwo}}
\providecommand{\retSATburnCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{retSATburnCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retSATburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{retSATburnCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATburnCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retSATburnCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retSATburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{retSATburnCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATburnCoarseLTwoVarDecoderSamLite}{\tbd{retSATburnCoarseLTwoVarDecoderSamLite}}
\providecommand{\retSATburnCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{retSATburnCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATburnCoarseLTwoVarDecoderSamPretrained}{\tbd{retSATburnCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\retSATburnCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{retSATburnCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATburnCoarseLTwoVarDecoderSegformerMlp}{\tbd{retSATburnCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retSATburnCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{retSATburnCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATburnCoarseLTwoVarEarlyStoppingFalse}{\tbd{retSATburnCoarseLTwoVarEarlyStoppingFalse}}
\providecommand{\retSATburnCoarseLTwoVarEarlyStoppingFalseFrozenEncoderTrue}{\tbd{retSATburnCoarseLTwoVarEarlyStoppingFalseFrozenEncoderTrue}}
\providecommand{\retSATburnCoarseLTwoVarFrozenEncoderTrue}{\tbd{retSATburnCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\retSATburnCoarseLTwoVarLossBootstrap}{\tbd{retSATburnCoarseLTwoVarLossBootstrap}}
\providecommand{\retSATburnCoarseLTwoVarLossGce}{\tbd{retSATburnCoarseLTwoVarLossGce}}
\providecommand{\retSATburnCoarseLTwoVarLrMultThree}{\tbd{retSATburnCoarseLTwoVarLrMultThree}}
\providecommand{\retSATburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATburnCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{retSATburnCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retSATburnCoarseLTwoVarValLabelsClean}{\tbd{retSATburnCoarseLTwoVarValLabelsClean}}
\providecommand{\retSATburnOmissionLOne}{\tbd{retSATburnOmissionLOne}}
\providecommand{\retSATburnOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{retSATburnOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retSATburnOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{retSATburnOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retSATburnOmissionLOneVarDecoderSamLite}{\tbd{retSATburnOmissionLOneVarDecoderSamLite}}
\providecommand{\retSATburnOmissionLOneVarDecoderSamPretrained}{\tbd{retSATburnOmissionLOneVarDecoderSamPretrained}}
\providecommand{\retSATburnOmissionLOneVarDecoderSegformerMlp}{\tbd{retSATburnOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\retSATburnOmissionLR}{\tbd{retSATburnOmissionLR}}
\providecommand{\retSATburnOmissionLRVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATburnOmissionLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATburnOmissionLTwo}{\tbd{retSATburnOmissionLTwo}}
\providecommand{\retSATburnOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{retSATburnOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retSATburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{retSATburnOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATburnOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retSATburnOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retSATburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{retSATburnOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATburnOmissionLTwoVarDecoderSamLite}{\tbd{retSATburnOmissionLTwoVarDecoderSamLite}}
\providecommand{\retSATburnOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{retSATburnOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATburnOmissionLTwoVarDecoderSamPretrained}{\tbd{retSATburnOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\retSATburnOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{retSATburnOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATburnOmissionLTwoVarDecoderSegformerMlp}{\tbd{retSATburnOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retSATburnOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{retSATburnOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATburnOmissionLTwoVarFrozenEncoderTrue}{\tbd{retSATburnOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\retSATburnOmissionLTwoVarLossBootstrap}{\tbd{retSATburnOmissionLTwoVarLossBootstrap}}
\providecommand{\retSATburnOmissionLTwoVarLossGce}{\tbd{retSATburnOmissionLTwoVarLossGce}}
\providecommand{\retSATburnOmissionLTwoVarLrMultThree}{\tbd{retSATburnOmissionLTwoVarLrMultThree}}
\providecommand{\retSATburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATburnOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{retSATburnOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retSATburnOmissionLTwoVarValLabelsClean}{\tbd{retSATburnOmissionLTwoVarValLabelsClean}}
\providecommand{\retSATburnShiftLOne}{\tbd{retSATburnShiftLOne}}
\providecommand{\retSATburnShiftLOneVarDecoderMaskTwoformerFull}{\tbd{retSATburnShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retSATburnShiftLOneVarDecoderMaskTwoformerLite}{\tbd{retSATburnShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retSATburnShiftLOneVarDecoderSamLite}{\tbd{retSATburnShiftLOneVarDecoderSamLite}}
\providecommand{\retSATburnShiftLOneVarDecoderSamPretrained}{\tbd{retSATburnShiftLOneVarDecoderSamPretrained}}
\providecommand{\retSATburnShiftLOneVarDecoderSegformerMlp}{\tbd{retSATburnShiftLOneVarDecoderSegformerMlp}}
\providecommand{\retSATburnShiftLR}{\tbd{retSATburnShiftLR}}
\providecommand{\retSATburnShiftLRVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATburnShiftLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATburnShiftLTwo}{\tbd{retSATburnShiftLTwo}}
\providecommand{\retSATburnShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{retSATburnShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retSATburnShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{retSATburnShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATburnShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retSATburnShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retSATburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{retSATburnShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATburnShiftLTwoVarDecoderSamLite}{\tbd{retSATburnShiftLTwoVarDecoderSamLite}}
\providecommand{\retSATburnShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{retSATburnShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATburnShiftLTwoVarDecoderSamPretrained}{\tbd{retSATburnShiftLTwoVarDecoderSamPretrained}}
\providecommand{\retSATburnShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{retSATburnShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATburnShiftLTwoVarDecoderSegformerMlp}{\tbd{retSATburnShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retSATburnShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{retSATburnShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATburnShiftLTwoVarFrozenEncoderTrue}{\tbd{retSATburnShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\retSATburnShiftLTwoVarLossBootstrap}{\tbd{retSATburnShiftLTwoVarLossBootstrap}}
\providecommand{\retSATburnShiftLTwoVarLossGce}{\tbd{retSATburnShiftLTwoVarLossGce}}
\providecommand{\retSATburnShiftLTwoVarLrMultThree}{\tbd{retSATburnShiftLTwoVarLrMultThree}}
\providecommand{\retSATburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATburnShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{retSATburnShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retSATburnShiftLTwoVarValLabelsClean}{\tbd{retSATburnShiftLTwoVarValLabelsClean}}
\providecommand{\retSATflairBoundaryLOne}{\tbd{retSATflairBoundaryLOne}}
\providecommand{\retSATflairBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{retSATflairBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retSATflairBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{retSATflairBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retSATflairBoundaryLOneVarDecoderSamLite}{\tbd{retSATflairBoundaryLOneVarDecoderSamLite}}
\providecommand{\retSATflairBoundaryLOneVarDecoderSamPretrained}{\tbd{retSATflairBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\retSATflairBoundaryLOneVarDecoderSegformerMlp}{\tbd{retSATflairBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\retSATflairBoundaryLR}{\tbd{retSATflairBoundaryLR}}
\providecommand{\retSATflairBoundaryLRVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATflairBoundaryLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATflairBoundaryLTwo}{\tbd{retSATflairBoundaryLTwo}}
\providecommand{\retSATflairBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{retSATflairBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retSATflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{retSATflairBoundaryLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATflairBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retSATflairBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retSATflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{retSATflairBoundaryLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATflairBoundaryLTwoVarDecoderSamLite}{\tbd{retSATflairBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retSATflairBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{retSATflairBoundaryLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATflairBoundaryLTwoVarDecoderSamPretrained}{\tbd{retSATflairBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\retSATflairBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{retSATflairBoundaryLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATflairBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retSATflairBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retSATflairBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{retSATflairBoundaryLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATflairBoundaryLTwoVarFrozenEncoderTrue}{\tbd{retSATflairBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\retSATflairBoundaryLTwoVarLossBootstrap}{\tbd{retSATflairBoundaryLTwoVarLossBootstrap}}
\providecommand{\retSATflairBoundaryLTwoVarLossGce}{\tbd{retSATflairBoundaryLTwoVarLossGce}}
\providecommand{\retSATflairBoundaryLTwoVarLrMultThree}{\tbd{retSATflairBoundaryLTwoVarLrMultThree}}
\providecommand{\retSATflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATflairBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{retSATflairBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retSATflairBoundaryLTwoVarValLabelsClean}{\tbd{retSATflairBoundaryLTwoVarValLabelsClean}}
\providecommand{\retSATflairCoarseLOne}{\tbd{retSATflairCoarseLOne}}
\providecommand{\retSATflairCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{retSATflairCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retSATflairCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{retSATflairCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retSATflairCoarseLOneVarDecoderSamLite}{\tbd{retSATflairCoarseLOneVarDecoderSamLite}}
\providecommand{\retSATflairCoarseLOneVarDecoderSamPretrained}{\tbd{retSATflairCoarseLOneVarDecoderSamPretrained}}
\providecommand{\retSATflairCoarseLOneVarDecoderSegformerMlp}{\tbd{retSATflairCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\retSATflairCoarseLR}{\tbd{retSATflairCoarseLR}}
\providecommand{\retSATflairCoarseLRVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATflairCoarseLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATflairCoarseLTwo}{\tbd{retSATflairCoarseLTwo}}
\providecommand{\retSATflairCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{retSATflairCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retSATflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{retSATflairCoarseLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATflairCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retSATflairCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retSATflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{retSATflairCoarseLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATflairCoarseLTwoVarDecoderSamLite}{\tbd{retSATflairCoarseLTwoVarDecoderSamLite}}
\providecommand{\retSATflairCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{retSATflairCoarseLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATflairCoarseLTwoVarDecoderSamPretrained}{\tbd{retSATflairCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\retSATflairCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{retSATflairCoarseLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATflairCoarseLTwoVarDecoderSegformerMlp}{\tbd{retSATflairCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retSATflairCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{retSATflairCoarseLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATflairCoarseLTwoVarFrozenEncoderTrue}{\tbd{retSATflairCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\retSATflairCoarseLTwoVarLossBootstrap}{\tbd{retSATflairCoarseLTwoVarLossBootstrap}}
\providecommand{\retSATflairCoarseLTwoVarLossGce}{\tbd{retSATflairCoarseLTwoVarLossGce}}
\providecommand{\retSATflairCoarseLTwoVarLrMultThree}{\tbd{retSATflairCoarseLTwoVarLrMultThree}}
\providecommand{\retSATflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATflairCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{retSATflairCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retSATflairCoarseLTwoVarValLabelsClean}{\tbd{retSATflairCoarseLTwoVarValLabelsClean}}
\providecommand{\retSATflairOmissionLOne}{\tbd{retSATflairOmissionLOne}}
\providecommand{\retSATflairOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{retSATflairOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retSATflairOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{retSATflairOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retSATflairOmissionLOneVarDecoderSamLite}{\tbd{retSATflairOmissionLOneVarDecoderSamLite}}
\providecommand{\retSATflairOmissionLOneVarDecoderSamPretrained}{\tbd{retSATflairOmissionLOneVarDecoderSamPretrained}}
\providecommand{\retSATflairOmissionLOneVarDecoderSegformerMlp}{\tbd{retSATflairOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\retSATflairOmissionLR}{\tbd{retSATflairOmissionLR}}
\providecommand{\retSATflairOmissionLRVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATflairOmissionLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATflairOmissionLTwo}{\tbd{retSATflairOmissionLTwo}}
\providecommand{\retSATflairOmissionLTwoVarClassWeightedTrue}{\tbd{retSATflairOmissionLTwoVarClassWeightedTrue}}
\providecommand{\retSATflairOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{retSATflairOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retSATflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{retSATflairOmissionLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATflairOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retSATflairOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retSATflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{retSATflairOmissionLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATflairOmissionLTwoVarDecoderSamLite}{\tbd{retSATflairOmissionLTwoVarDecoderSamLite}}
\providecommand{\retSATflairOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{retSATflairOmissionLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATflairOmissionLTwoVarDecoderSamPretrained}{\tbd{retSATflairOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\retSATflairOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{retSATflairOmissionLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATflairOmissionLTwoVarDecoderSegformerMlp}{\tbd{retSATflairOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retSATflairOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{retSATflairOmissionLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATflairOmissionLTwoVarEarlyStoppingFalse}{\tbd{retSATflairOmissionLTwoVarEarlyStoppingFalse}}
\providecommand{\retSATflairOmissionLTwoVarEarlyStoppingFalseFrozenEncoderTrue}{\tbd{retSATflairOmissionLTwoVarEarlyStoppingFalseFrozenEncoderTrue}}
\providecommand{\retSATflairOmissionLTwoVarFrozenEncoderTrue}{\tbd{retSATflairOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\retSATflairOmissionLTwoVarLossBootstrap}{\tbd{retSATflairOmissionLTwoVarLossBootstrap}}
\providecommand{\retSATflairOmissionLTwoVarLossGce}{\tbd{retSATflairOmissionLTwoVarLossGce}}
\providecommand{\retSATflairOmissionLTwoVarLrMultThree}{\tbd{retSATflairOmissionLTwoVarLrMultThree}}
\providecommand{\retSATflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATflairOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{retSATflairOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retSATflairOmissionLTwoVarValLabelsClean}{\tbd{retSATflairOmissionLTwoVarValLabelsClean}}
\providecommand{\retSATflairShiftLOne}{\tbd{retSATflairShiftLOne}}
\providecommand{\retSATflairShiftLOneVarDecoderMaskTwoformerFull}{\tbd{retSATflairShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retSATflairShiftLOneVarDecoderMaskTwoformerLite}{\tbd{retSATflairShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retSATflairShiftLOneVarDecoderSamLite}{\tbd{retSATflairShiftLOneVarDecoderSamLite}}
\providecommand{\retSATflairShiftLOneVarDecoderSamPretrained}{\tbd{retSATflairShiftLOneVarDecoderSamPretrained}}
\providecommand{\retSATflairShiftLOneVarDecoderSegformerMlp}{\tbd{retSATflairShiftLOneVarDecoderSegformerMlp}}
\providecommand{\retSATflairShiftLR}{\tbd{retSATflairShiftLR}}
\providecommand{\retSATflairShiftLRVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATflairShiftLRVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATflairShiftLTwo}{\tbd{retSATflairShiftLTwo}}
\providecommand{\retSATflairShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{retSATflairShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retSATflairShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}{\tbd{retSATflairShiftLTwoVarDecoderMaskTwoformerFullLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATflairShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retSATflairShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retSATflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}{\tbd{retSATflairShiftLTwoVarDecoderMaskTwoformerLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATflairShiftLTwoVarDecoderSamLite}{\tbd{retSATflairShiftLTwoVarDecoderSamLite}}
\providecommand{\retSATflairShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}{\tbd{retSATflairShiftLTwoVarDecoderSamLiteLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATflairShiftLTwoVarDecoderSamPretrained}{\tbd{retSATflairShiftLTwoVarDecoderSamPretrained}}
\providecommand{\retSATflairShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}{\tbd{retSATflairShiftLTwoVarDecoderSamPretrainedLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATflairShiftLTwoVarDecoderSegformerMlp}{\tbd{retSATflairShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retSATflairShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}{\tbd{retSATflairShiftLTwoVarDecoderSegformerMlpLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATflairShiftLTwoVarFrozenEncoderTrue}{\tbd{retSATflairShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\retSATflairShiftLTwoVarLossBootstrap}{\tbd{retSATflairShiftLTwoVarLossBootstrap}}
\providecommand{\retSATflairShiftLTwoVarLossGce}{\tbd{retSATflairShiftLTwoVarLossGce}}
\providecommand{\retSATflairShiftLTwoVarLrMultThree}{\tbd{retSATflairShiftLTwoVarLrMultThree}}
\providecommand{\retSATflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retSATflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retSATflairShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{retSATflairShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retSATflairShiftLTwoVarValLabelsClean}{\tbd{retSATflairShiftLTwoVarValLabelsClean}}
\providecommand{\retSATsenOtsuLTwo}{\tbd{retSATsenOtsuLTwo}}
\providecommand{\retTMChesBoundaryLOne}{\tbd{retTMChesBoundaryLOne}}
\providecommand{\retTMChesBoundaryLTwo}{\tbd{retTMChesBoundaryLTwo}}
\providecommand{\retTMChesCoarseLOne}{\tbd{retTMChesCoarseLOne}}
\providecommand{\retTMChesCoarseLTwo}{\tbd{retTMChesCoarseLTwo}}
\providecommand{\retTMChesNlcdREAL}{\tbd{retTMChesNlcdREAL}}
\providecommand{\retTMChesOmissionLOne}{\tbd{retTMChesOmissionLOne}}
\providecommand{\retTMChesOmissionLTwo}{\tbd{retTMChesOmissionLTwo}}
\providecommand{\retTMChesShiftLOne}{\tbd{retTMChesShiftLOne}}
\providecommand{\retTMChesShiftLTwo}{\tbd{retTMChesShiftLTwo}}
\providecommand{\retTMCsTwelveBoundaryLOne}{\tbd{retTMCsTwelveBoundaryLOne}}
\providecommand{\retTMCsTwelveBoundaryLTwo}{\tbd{retTMCsTwelveBoundaryLTwo}}
\providecommand{\retTMCsTwelveCoarseLOne}{\tbd{retTMCsTwelveCoarseLOne}}
\providecommand{\retTMCsTwelveCoarseLTwo}{\tbd{retTMCsTwelveCoarseLTwo}}
\providecommand{\retTMCsTwelveOmissionLOne}{\tbd{retTMCsTwelveOmissionLOne}}
\providecommand{\retTMCsTwelveOmissionLTwo}{\tbd{retTMCsTwelveOmissionLTwo}}
\providecommand{\retTMCsTwelveSTwocloudlessREAL}{\tbd{retTMCsTwelveSTwocloudlessREAL}}
\providecommand{\retTMCsTwelveShiftLOne}{\tbd{retTMCsTwelveShiftLOne}}
\providecommand{\retTMCsTwelveShiftLTwo}{\tbd{retTMCsTwelveShiftLTwo}}
\providecommand{\retTMDfcBoundaryLOne}{\tbd{retTMDfcBoundaryLOne}}
\providecommand{\retTMDfcBoundaryLTwo}{\tbd{retTMDfcBoundaryLTwo}}
\providecommand{\retTMDfcCoarseLOne}{\tbd{retTMDfcCoarseLOne}}
\providecommand{\retTMDfcCoarseLTwo}{\tbd{retTMDfcCoarseLTwo}}
\providecommand{\retTMDfcModisREALVarTrainSubsetRealcov}{\tbd{retTMDfcModisREALVarTrainSubsetRealcov}}
\providecommand{\retTMDfcOmissionLOne}{\tbd{retTMDfcOmissionLOne}}
\providecommand{\retTMDfcOmissionLTwo}{\tbd{retTMDfcOmissionLTwo}}
\providecommand{\retTMDfcShiftLOne}{\tbd{retTMDfcShiftLOne}}
\providecommand{\retTMDfcShiftLTwo}{\tbd{retTMDfcShiftLTwo}}
\providecommand{\retTMEnvaBoundaryLOne}{\tbd{retTMEnvaBoundaryLOne}}
\providecommand{\retTMEnvaBoundaryLTwo}{\tbd{retTMEnvaBoundaryLTwo}}
\providecommand{\retTMEnvaCoarseLOne}{\tbd{retTMEnvaCoarseLOne}}
\providecommand{\retTMEnvaCoarseLTwo}{\tbd{retTMEnvaCoarseLTwo}}
\providecommand{\retTMEnvaNlcdREAL}{\tbd{retTMEnvaNlcdREAL}}
\providecommand{\retTMEnvaOmissionLOne}{\tbd{retTMEnvaOmissionLOne}}
\providecommand{\retTMEnvaOmissionLTwo}{\tbd{retTMEnvaOmissionLTwo}}
\providecommand{\retTMEnvaShiftLOne}{\tbd{retTMEnvaShiftLOne}}
\providecommand{\retTMEnvaShiftLTwo}{\tbd{retTMEnvaShiftLTwo}}
\providecommand{\retTMKuroBoundaryLOne}{\tbd{retTMKuroBoundaryLOne}}
\providecommand{\retTMKuroBoundaryLTwo}{\tbd{retTMKuroBoundaryLTwo}}
\providecommand{\retTMKuroCemsREALVarTrainSubsetRealcov}{\tbd{retTMKuroCemsREALVarTrainSubsetRealcov}}
\providecommand{\retTMKuroCoarseLOne}{\tbd{retTMKuroCoarseLOne}}
\providecommand{\retTMKuroCoarseLTwo}{\tbd{retTMKuroCoarseLTwo}}
\providecommand{\retTMKuroOmissionLOne}{\tbd{retTMKuroOmissionLOne}}
\providecommand{\retTMKuroOmissionLTwo}{\tbd{retTMKuroOmissionLTwo}}
\providecommand{\retTMKuroShiftLOne}{\tbd{retTMKuroShiftLOne}}
\providecommand{\retTMKuroShiftLTwo}{\tbd{retTMKuroShiftLTwo}}
\providecommand{\retTMOemBoundaryLOne}{\tbd{retTMOemBoundaryLOne}}
\providecommand{\retTMOemBoundaryLTwo}{\tbd{retTMOemBoundaryLTwo}}
\providecommand{\retTMOemCoarseLOne}{\tbd{retTMOemCoarseLOne}}
\providecommand{\retTMOemCoarseLTwo}{\tbd{retTMOemCoarseLTwo}}
\providecommand{\retTMOemOmissionLOne}{\tbd{retTMOemOmissionLOne}}
\providecommand{\retTMOemOmissionLTwo}{\tbd{retTMOemOmissionLTwo}}
\providecommand{\retTMOemShiftLOne}{\tbd{retTMOemShiftLOne}}
\providecommand{\retTMOemShiftLTwo}{\tbd{retTMOemShiftLTwo}}
\providecommand{\retTMSnTwoBoundaryLOne}{\tbd{retTMSnTwoBoundaryLOne}}
\providecommand{\retTMSnTwoBoundaryLTwo}{\tbd{retTMSnTwoBoundaryLTwo}}
\providecommand{\retTMSnTwoCoarseLOne}{\tbd{retTMSnTwoCoarseLOne}}
\providecommand{\retTMSnTwoCoarseLTwo}{\tbd{retTMSnTwoCoarseLTwo}}
\providecommand{\retTMSnTwoOmissionLOne}{\tbd{retTMSnTwoOmissionLOne}}
\providecommand{\retTMSnTwoOmissionLTwo}{\tbd{retTMSnTwoOmissionLTwo}}
\providecommand{\retTMSnTwoShiftLOne}{\tbd{retTMSnTwoShiftLOne}}
\providecommand{\retTMSnTwoShiftLTwo}{\tbd{retTMSnTwoShiftLTwo}}
\providecommand{\retTMburnBoundaryLOne}{\tbd{retTMburnBoundaryLOne}}
\providecommand{\retTMburnBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{retTMburnBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retTMburnBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{retTMburnBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retTMburnBoundaryLOneVarDecoderSamLite}{\tbd{retTMburnBoundaryLOneVarDecoderSamLite}}
\providecommand{\retTMburnBoundaryLOneVarDecoderSamPretrained}{\tbd{retTMburnBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\retTMburnBoundaryLOneVarDecoderSegformerMlp}{\tbd{retTMburnBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\retTMburnBoundaryLR}{\tbd{retTMburnBoundaryLR}}
\providecommand{\retTMburnBoundaryLTwo}{\tbd{retTMburnBoundaryLTwo}}
\providecommand{\retTMburnBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{retTMburnBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retTMburnBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retTMburnBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retTMburnBoundaryLTwoVarDecoderSamLite}{\tbd{retTMburnBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retTMburnBoundaryLTwoVarDecoderSamPretrained}{\tbd{retTMburnBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\retTMburnBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retTMburnBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retTMburnBoundaryLTwoVarFrozenEncoderTrue}{\tbd{retTMburnBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\retTMburnBoundaryLTwoVarLossBootstrap}{\tbd{retTMburnBoundaryLTwoVarLossBootstrap}}
\providecommand{\retTMburnBoundaryLTwoVarLossGce}{\tbd{retTMburnBoundaryLTwoVarLossGce}}
\providecommand{\retTMburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retTMburnBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retTMburnBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{retTMburnBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retTMburnCoarseLOne}{\tbd{retTMburnCoarseLOne}}
\providecommand{\retTMburnCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{retTMburnCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retTMburnCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{retTMburnCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retTMburnCoarseLOneVarDecoderSamLite}{\tbd{retTMburnCoarseLOneVarDecoderSamLite}}
\providecommand{\retTMburnCoarseLOneVarDecoderSamPretrained}{\tbd{retTMburnCoarseLOneVarDecoderSamPretrained}}
\providecommand{\retTMburnCoarseLOneVarDecoderSegformerMlp}{\tbd{retTMburnCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\retTMburnCoarseLR}{\tbd{retTMburnCoarseLR}}
\providecommand{\retTMburnCoarseLTwo}{\tbd{retTMburnCoarseLTwo}}
\providecommand{\retTMburnCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{retTMburnCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retTMburnCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retTMburnCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retTMburnCoarseLTwoVarDecoderSamLite}{\tbd{retTMburnCoarseLTwoVarDecoderSamLite}}
\providecommand{\retTMburnCoarseLTwoVarDecoderSamPretrained}{\tbd{retTMburnCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\retTMburnCoarseLTwoVarDecoderSegformerMlp}{\tbd{retTMburnCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retTMburnCoarseLTwoVarFrozenEncoderTrue}{\tbd{retTMburnCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\retTMburnCoarseLTwoVarLossBootstrap}{\tbd{retTMburnCoarseLTwoVarLossBootstrap}}
\providecommand{\retTMburnCoarseLTwoVarLossGce}{\tbd{retTMburnCoarseLTwoVarLossGce}}
\providecommand{\retTMburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retTMburnCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retTMburnCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{retTMburnCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retTMburnOmissionLOne}{\tbd{retTMburnOmissionLOne}}
\providecommand{\retTMburnOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{retTMburnOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retTMburnOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{retTMburnOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retTMburnOmissionLOneVarDecoderSamLite}{\tbd{retTMburnOmissionLOneVarDecoderSamLite}}
\providecommand{\retTMburnOmissionLOneVarDecoderSamPretrained}{\tbd{retTMburnOmissionLOneVarDecoderSamPretrained}}
\providecommand{\retTMburnOmissionLOneVarDecoderSegformerMlp}{\tbd{retTMburnOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\retTMburnOmissionLR}{\tbd{retTMburnOmissionLR}}
\providecommand{\retTMburnOmissionLTwo}{\tbd{retTMburnOmissionLTwo}}
\providecommand{\retTMburnOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{retTMburnOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retTMburnOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retTMburnOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retTMburnOmissionLTwoVarDecoderSamLite}{\tbd{retTMburnOmissionLTwoVarDecoderSamLite}}
\providecommand{\retTMburnOmissionLTwoVarDecoderSamPretrained}{\tbd{retTMburnOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\retTMburnOmissionLTwoVarDecoderSegformerMlp}{\tbd{retTMburnOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retTMburnOmissionLTwoVarFrozenEncoderTrue}{\tbd{retTMburnOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\retTMburnOmissionLTwoVarLossBootstrap}{\tbd{retTMburnOmissionLTwoVarLossBootstrap}}
\providecommand{\retTMburnOmissionLTwoVarLossGce}{\tbd{retTMburnOmissionLTwoVarLossGce}}
\providecommand{\retTMburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retTMburnOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retTMburnOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{retTMburnOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retTMburnShiftLOne}{\tbd{retTMburnShiftLOne}}
\providecommand{\retTMburnShiftLOneVarDecoderMaskTwoformerFull}{\tbd{retTMburnShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retTMburnShiftLOneVarDecoderMaskTwoformerLite}{\tbd{retTMburnShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retTMburnShiftLOneVarDecoderSamLite}{\tbd{retTMburnShiftLOneVarDecoderSamLite}}
\providecommand{\retTMburnShiftLOneVarDecoderSamPretrained}{\tbd{retTMburnShiftLOneVarDecoderSamPretrained}}
\providecommand{\retTMburnShiftLOneVarDecoderSegformerMlp}{\tbd{retTMburnShiftLOneVarDecoderSegformerMlp}}
\providecommand{\retTMburnShiftLR}{\tbd{retTMburnShiftLR}}
\providecommand{\retTMburnShiftLTwo}{\tbd{retTMburnShiftLTwo}}
\providecommand{\retTMburnShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{retTMburnShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retTMburnShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retTMburnShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retTMburnShiftLTwoVarDecoderSamLite}{\tbd{retTMburnShiftLTwoVarDecoderSamLite}}
\providecommand{\retTMburnShiftLTwoVarDecoderSamPretrained}{\tbd{retTMburnShiftLTwoVarDecoderSamPretrained}}
\providecommand{\retTMburnShiftLTwoVarDecoderSegformerMlp}{\tbd{retTMburnShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retTMburnShiftLTwoVarFrozenEncoderTrue}{\tbd{retTMburnShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\retTMburnShiftLTwoVarLossBootstrap}{\tbd{retTMburnShiftLTwoVarLossBootstrap}}
\providecommand{\retTMburnShiftLTwoVarLossGce}{\tbd{retTMburnShiftLTwoVarLossGce}}
\providecommand{\retTMburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retTMburnShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retTMburnShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{retTMburnShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retTMflairBoundaryLOne}{\tbd{retTMflairBoundaryLOne}}
\providecommand{\retTMflairBoundaryLOneVarDecoderMaskTwoformerFull}{\tbd{retTMflairBoundaryLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retTMflairBoundaryLOneVarDecoderMaskTwoformerLite}{\tbd{retTMflairBoundaryLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retTMflairBoundaryLOneVarDecoderSamLite}{\tbd{retTMflairBoundaryLOneVarDecoderSamLite}}
\providecommand{\retTMflairBoundaryLOneVarDecoderSamPretrained}{\tbd{retTMflairBoundaryLOneVarDecoderSamPretrained}}
\providecommand{\retTMflairBoundaryLOneVarDecoderSegformerMlp}{\tbd{retTMflairBoundaryLOneVarDecoderSegformerMlp}}
\providecommand{\retTMflairBoundaryLR}{\tbd{retTMflairBoundaryLR}}
\providecommand{\retTMflairBoundaryLTwo}{\tbd{retTMflairBoundaryLTwo}}
\providecommand{\retTMflairBoundaryLTwoVarDecoderMaskTwoformerFull}{\tbd{retTMflairBoundaryLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retTMflairBoundaryLTwoVarDecoderMaskTwoformerLite}{\tbd{retTMflairBoundaryLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retTMflairBoundaryLTwoVarDecoderSamLite}{\tbd{retTMflairBoundaryLTwoVarDecoderSamLite}}
\providecommand{\retTMflairBoundaryLTwoVarDecoderSamPretrained}{\tbd{retTMflairBoundaryLTwoVarDecoderSamPretrained}}
\providecommand{\retTMflairBoundaryLTwoVarDecoderSegformerMlp}{\tbd{retTMflairBoundaryLTwoVarDecoderSegformerMlp}}
\providecommand{\retTMflairBoundaryLTwoVarFrozenEncoderTrue}{\tbd{retTMflairBoundaryLTwoVarFrozenEncoderTrue}}
\providecommand{\retTMflairBoundaryLTwoVarLossBootstrap}{\tbd{retTMflairBoundaryLTwoVarLossBootstrap}}
\providecommand{\retTMflairBoundaryLTwoVarLossGce}{\tbd{retTMflairBoundaryLTwoVarLossGce}}
\providecommand{\retTMflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retTMflairBoundaryLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retTMflairBoundaryLTwoVarTrainSubsetCleanTwoFive}{\tbd{retTMflairBoundaryLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retTMflairCoarseLOne}{\tbd{retTMflairCoarseLOne}}
\providecommand{\retTMflairCoarseLOneVarDecoderMaskTwoformerFull}{\tbd{retTMflairCoarseLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retTMflairCoarseLOneVarDecoderMaskTwoformerLite}{\tbd{retTMflairCoarseLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retTMflairCoarseLOneVarDecoderSamLite}{\tbd{retTMflairCoarseLOneVarDecoderSamLite}}
\providecommand{\retTMflairCoarseLOneVarDecoderSamPretrained}{\tbd{retTMflairCoarseLOneVarDecoderSamPretrained}}
\providecommand{\retTMflairCoarseLOneVarDecoderSegformerMlp}{\tbd{retTMflairCoarseLOneVarDecoderSegformerMlp}}
\providecommand{\retTMflairCoarseLR}{\tbd{retTMflairCoarseLR}}
\providecommand{\retTMflairCoarseLTwo}{\tbd{retTMflairCoarseLTwo}}
\providecommand{\retTMflairCoarseLTwoVarDecoderMaskTwoformerFull}{\tbd{retTMflairCoarseLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retTMflairCoarseLTwoVarDecoderMaskTwoformerLite}{\tbd{retTMflairCoarseLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retTMflairCoarseLTwoVarDecoderSamLite}{\tbd{retTMflairCoarseLTwoVarDecoderSamLite}}
\providecommand{\retTMflairCoarseLTwoVarDecoderSamPretrained}{\tbd{retTMflairCoarseLTwoVarDecoderSamPretrained}}
\providecommand{\retTMflairCoarseLTwoVarDecoderSegformerMlp}{\tbd{retTMflairCoarseLTwoVarDecoderSegformerMlp}}
\providecommand{\retTMflairCoarseLTwoVarFrozenEncoderTrue}{\tbd{retTMflairCoarseLTwoVarFrozenEncoderTrue}}
\providecommand{\retTMflairCoarseLTwoVarLossBootstrap}{\tbd{retTMflairCoarseLTwoVarLossBootstrap}}
\providecommand{\retTMflairCoarseLTwoVarLossGce}{\tbd{retTMflairCoarseLTwoVarLossGce}}
\providecommand{\retTMflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retTMflairCoarseLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retTMflairCoarseLTwoVarTrainSubsetCleanTwoFive}{\tbd{retTMflairCoarseLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retTMflairOmissionLOne}{\tbd{retTMflairOmissionLOne}}
\providecommand{\retTMflairOmissionLOneVarDecoderMaskTwoformerFull}{\tbd{retTMflairOmissionLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retTMflairOmissionLOneVarDecoderMaskTwoformerLite}{\tbd{retTMflairOmissionLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retTMflairOmissionLOneVarDecoderSamLite}{\tbd{retTMflairOmissionLOneVarDecoderSamLite}}
\providecommand{\retTMflairOmissionLOneVarDecoderSamPretrained}{\tbd{retTMflairOmissionLOneVarDecoderSamPretrained}}
\providecommand{\retTMflairOmissionLOneVarDecoderSegformerMlp}{\tbd{retTMflairOmissionLOneVarDecoderSegformerMlp}}
\providecommand{\retTMflairOmissionLR}{\tbd{retTMflairOmissionLR}}
\providecommand{\retTMflairOmissionLTwo}{\tbd{retTMflairOmissionLTwo}}
\providecommand{\retTMflairOmissionLTwoVarDecoderMaskTwoformerFull}{\tbd{retTMflairOmissionLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retTMflairOmissionLTwoVarDecoderMaskTwoformerLite}{\tbd{retTMflairOmissionLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retTMflairOmissionLTwoVarDecoderSamLite}{\tbd{retTMflairOmissionLTwoVarDecoderSamLite}}
\providecommand{\retTMflairOmissionLTwoVarDecoderSamPretrained}{\tbd{retTMflairOmissionLTwoVarDecoderSamPretrained}}
\providecommand{\retTMflairOmissionLTwoVarDecoderSegformerMlp}{\tbd{retTMflairOmissionLTwoVarDecoderSegformerMlp}}
\providecommand{\retTMflairOmissionLTwoVarFrozenEncoderTrue}{\tbd{retTMflairOmissionLTwoVarFrozenEncoderTrue}}
\providecommand{\retTMflairOmissionLTwoVarLossBootstrap}{\tbd{retTMflairOmissionLTwoVarLossBootstrap}}
\providecommand{\retTMflairOmissionLTwoVarLossGce}{\tbd{retTMflairOmissionLTwoVarLossGce}}
\providecommand{\retTMflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retTMflairOmissionLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retTMflairOmissionLTwoVarTrainSubsetCleanTwoFive}{\tbd{retTMflairOmissionLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retTMflairShiftLOne}{\tbd{retTMflairShiftLOne}}
\providecommand{\retTMflairShiftLOneVarDecoderMaskTwoformerFull}{\tbd{retTMflairShiftLOneVarDecoderMaskTwoformerFull}}
\providecommand{\retTMflairShiftLOneVarDecoderMaskTwoformerLite}{\tbd{retTMflairShiftLOneVarDecoderMaskTwoformerLite}}
\providecommand{\retTMflairShiftLOneVarDecoderSamLite}{\tbd{retTMflairShiftLOneVarDecoderSamLite}}
\providecommand{\retTMflairShiftLOneVarDecoderSamPretrained}{\tbd{retTMflairShiftLOneVarDecoderSamPretrained}}
\providecommand{\retTMflairShiftLOneVarDecoderSegformerMlp}{\tbd{retTMflairShiftLOneVarDecoderSegformerMlp}}
\providecommand{\retTMflairShiftLR}{\tbd{retTMflairShiftLR}}
\providecommand{\retTMflairShiftLTwo}{\tbd{retTMflairShiftLTwo}}
\providecommand{\retTMflairShiftLTwoVarDecoderMaskTwoformerFull}{\tbd{retTMflairShiftLTwoVarDecoderMaskTwoformerFull}}
\providecommand{\retTMflairShiftLTwoVarDecoderMaskTwoformerLite}{\tbd{retTMflairShiftLTwoVarDecoderMaskTwoformerLite}}
\providecommand{\retTMflairShiftLTwoVarDecoderSamLite}{\tbd{retTMflairShiftLTwoVarDecoderSamLite}}
\providecommand{\retTMflairShiftLTwoVarDecoderSamPretrained}{\tbd{retTMflairShiftLTwoVarDecoderSamPretrained}}
\providecommand{\retTMflairShiftLTwoVarDecoderSegformerMlp}{\tbd{retTMflairShiftLTwoVarDecoderSegformerMlp}}
\providecommand{\retTMflairShiftLTwoVarFrozenEncoderTrue}{\tbd{retTMflairShiftLTwoVarFrozenEncoderTrue}}
\providecommand{\retTMflairShiftLTwoVarLossBootstrap}{\tbd{retTMflairShiftLTwoVarLossBootstrap}}
\providecommand{\retTMflairShiftLTwoVarLossGce}{\tbd{retTMflairShiftLTwoVarLossGce}}
\providecommand{\retTMflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}{\tbd{retTMflairShiftLTwoVarLrMultZeroThreeThreeThreeThree}}
\providecommand{\retTMflairShiftLTwoVarTrainSubsetCleanTwoFive}{\tbd{retTMflairShiftLTwoVarTrainSubsetCleanTwoFive}}
\providecommand{\retTMsenOtsuLTwo}{\tbd{retTMsenOtsuLTwo}}
\providecommand{\retVitlRandomburnBoundaryLOneVarInitRandom}{\tbd{retVitlRandomburnBoundaryLOneVarInitRandom}}
\providecommand{\retVitlRandomburnBoundaryLTwoVarInitRandom}{\tbd{retVitlRandomburnBoundaryLTwoVarInitRandom}}
\providecommand{\retVitlRandomburnCoarseLOneVarInitRandom}{\tbd{retVitlRandomburnCoarseLOneVarInitRandom}}
\providecommand{\retVitlRandomburnCoarseLTwoVarInitRandom}{\tbd{retVitlRandomburnCoarseLTwoVarInitRandom}}
\providecommand{\retVitlRandomburnOmissionLOneVarInitRandom}{\tbd{retVitlRandomburnOmissionLOneVarInitRandom}}
\providecommand{\retVitlRandomburnOmissionLTwoVarInitRandom}{\tbd{retVitlRandomburnOmissionLTwoVarInitRandom}}
\providecommand{\retVitlRandomburnShiftLOneVarInitRandom}{\tbd{retVitlRandomburnShiftLOneVarInitRandom}}
\providecommand{\retVitlRandomburnShiftLTwoVarInitRandom}{\tbd{retVitlRandomburnShiftLTwoVarInitRandom}}
\providecommand{\retVitlRandomflairBoundaryLOneVarInitRandom}{\tbd{retVitlRandomflairBoundaryLOneVarInitRandom}}
\providecommand{\retVitlRandomflairBoundaryLTwoVarInitRandom}{\tbd{retVitlRandomflairBoundaryLTwoVarInitRandom}}
\providecommand{\retVitlRandomflairCoarseLOneVarInitRandom}{\tbd{retVitlRandomflairCoarseLOneVarInitRandom}}
\providecommand{\retVitlRandomflairCoarseLTwoVarInitRandom}{\tbd{retVitlRandomflairCoarseLTwoVarInitRandom}}
\providecommand{\retVitlRandomflairOmissionLOneVarInitRandom}{\tbd{retVitlRandomflairOmissionLOneVarInitRandom}}
\providecommand{\retVitlRandomflairOmissionLTwoVarInitRandom}{\tbd{retVitlRandomflairOmissionLTwoVarInitRandom}}
\providecommand{\retVitlRandomflairShiftLOneVarInitRandom}{\tbd{retVitlRandomflairShiftLOneVarInitRandom}}
\providecommand{\retVitlRandomflairShiftLTwoVarInitRandom}{\tbd{retVitlRandomflairShiftLTwoVarInitRandom}}
\providecommand{\statFFourburnCIHi}{\tbd{statFFourburnCIHi}}
\providecommand{\statFFourburnCILo}{\tbd{statFFourburnCILo}}
\providecommand{\statFFourburnEst}{\tbd{statFFourburnEst}}
\providecommand{\statFFourburnMde}{\tbd{statFFourburnMde}}
\providecommand{\statFFourburnN}{\tbd{statFFourburnN}}
\providecommand{\statFFourburnP}{\tbd{statFFourburnP}}
\providecommand{\statFFourburnPHolm}{\tbd{statFFourburnPHolm}}
\providecommand{\statFFourburnTostCIHi}{\tbd{statFFourburnTostCIHi}}
\providecommand{\statFFourburnTostCILo}{\tbd{statFFourburnTostCILo}}
\providecommand{\statFFourburnTostEquivalent}{\tbd{statFFourburnTostEquivalent}}
\providecommand{\statFFourburnTostEst}{\tbd{statFFourburnTostEst}}
\providecommand{\statFFourburnTostN}{\tbd{statFFourburnTostN}}
\providecommand{\statFFourburnTostP}{\tbd{statFFourburnTostP}}
\providecommand{\statFFourburnWelchP}{\tbd{statFFourburnWelchP}}
\providecommand{\statFFourflairCIHi}{\tbd{statFFourflairCIHi}}
\providecommand{\statFFourflairCILo}{\tbd{statFFourflairCILo}}
\providecommand{\statFFourflairEst}{\tbd{statFFourflairEst}}
\providecommand{\statFFourflairMde}{\tbd{statFFourflairMde}}
\providecommand{\statFFourflairN}{\tbd{statFFourflairN}}
\providecommand{\statFFourflairP}{\tbd{statFFourflairP}}
\providecommand{\statFFourflairPHolm}{\tbd{statFFourflairPHolm}}
\providecommand{\statFFourflairTostCIHi}{\tbd{statFFourflairTostCIHi}}
\providecommand{\statFFourflairTostCILo}{\tbd{statFFourflairTostCILo}}
\providecommand{\statFFourflairTostEquivalent}{\tbd{statFFourflairTostEquivalent}}
\providecommand{\statFFourflairTostEst}{\tbd{statFFourflairTostEst}}
\providecommand{\statFFourflairTostN}{\tbd{statFFourflairTostN}}
\providecommand{\statFFourflairTostP}{\tbd{statFFourflairTostP}}
\providecommand{\statFFourflairWelchP}{\tbd{statFFourflairWelchP}}
\providecommand{\statFOneburnCIHi}{\tbd{statFOneburnCIHi}}
\providecommand{\statFOneburnCILo}{\tbd{statFOneburnCILo}}
\providecommand{\statFOneburnEst}{\tbd{statFOneburnEst}}
\providecommand{\statFOneburnMde}{\tbd{statFOneburnMde}}
\providecommand{\statFOneburnN}{\tbd{statFOneburnN}}
\providecommand{\statFOneburnP}{\tbd{statFOneburnP}}
\providecommand{\statFOneburnPHolm}{\tbd{statFOneburnPHolm}}
\providecommand{\statFOneburnTostCIHi}{\tbd{statFOneburnTostCIHi}}
\providecommand{\statFOneburnTostCILo}{\tbd{statFOneburnTostCILo}}
\providecommand{\statFOneburnTostEquivalent}{\tbd{statFOneburnTostEquivalent}}
\providecommand{\statFOneburnTostEst}{\tbd{statFOneburnTostEst}}
\providecommand{\statFOneburnTostN}{\tbd{statFOneburnTostN}}
\providecommand{\statFOneburnTostP}{\tbd{statFOneburnTostP}}
\providecommand{\statFOneburnWelchP}{\tbd{statFOneburnWelchP}}
\providecommand{\statFOneflairCIHi}{\tbd{statFOneflairCIHi}}
\providecommand{\statFOneflairCILo}{\tbd{statFOneflairCILo}}
\providecommand{\statFOneflairEst}{\tbd{statFOneflairEst}}
\providecommand{\statFOneflairMde}{\tbd{statFOneflairMde}}
\providecommand{\statFOneflairN}{\tbd{statFOneflairN}}
\providecommand{\statFOneflairP}{\tbd{statFOneflairP}}
\providecommand{\statFOneflairPHolm}{\tbd{statFOneflairPHolm}}
\providecommand{\statFOneflairTostCIHi}{\tbd{statFOneflairTostCIHi}}
\providecommand{\statFOneflairTostCILo}{\tbd{statFOneflairTostCILo}}
\providecommand{\statFOneflairTostEquivalent}{\tbd{statFOneflairTostEquivalent}}
\providecommand{\statFOneflairTostEst}{\tbd{statFOneflairTostEst}}
\providecommand{\statFOneflairTostN}{\tbd{statFOneflairTostN}}
\providecommand{\statFOneflairTostP}{\tbd{statFOneflairTostP}}
\providecommand{\statFOneflairWelchP}{\tbd{statFOneflairWelchP}}
\providecommand{\statFThreeburnCIHi}{\tbd{statFThreeburnCIHi}}
\providecommand{\statFThreeburnCILo}{\tbd{statFThreeburnCILo}}
\providecommand{\statFThreeburnEst}{\tbd{statFThreeburnEst}}
\providecommand{\statFThreeburnMde}{\tbd{statFThreeburnMde}}
\providecommand{\statFThreeburnN}{\tbd{statFThreeburnN}}
\providecommand{\statFThreeburnP}{\tbd{statFThreeburnP}}
\providecommand{\statFThreeburnPHolm}{\tbd{statFThreeburnPHolm}}
\providecommand{\statFThreeburnTostCIHi}{\tbd{statFThreeburnTostCIHi}}
\providecommand{\statFThreeburnTostCILo}{\tbd{statFThreeburnTostCILo}}
\providecommand{\statFThreeburnTostEquivalent}{\tbd{statFThreeburnTostEquivalent}}
\providecommand{\statFThreeburnTostEst}{\tbd{statFThreeburnTostEst}}
\providecommand{\statFThreeburnTostN}{\tbd{statFThreeburnTostN}}
\providecommand{\statFThreeburnTostP}{\tbd{statFThreeburnTostP}}
\providecommand{\statFThreeburnWelchP}{\tbd{statFThreeburnWelchP}}
\providecommand{\statFThreeflairCIHi}{\tbd{statFThreeflairCIHi}}
\providecommand{\statFThreeflairCILo}{\tbd{statFThreeflairCILo}}
\providecommand{\statFThreeflairEst}{\tbd{statFThreeflairEst}}
\providecommand{\statFThreeflairMde}{\tbd{statFThreeflairMde}}
\providecommand{\statFThreeflairN}{\tbd{statFThreeflairN}}
\providecommand{\statFThreeflairP}{\tbd{statFThreeflairP}}
\providecommand{\statFThreeflairPHolm}{\tbd{statFThreeflairPHolm}}
\providecommand{\statFThreeflairTostCIHi}{\tbd{statFThreeflairTostCIHi}}
\providecommand{\statFThreeflairTostCILo}{\tbd{statFThreeflairTostCILo}}
\providecommand{\statFThreeflairTostEquivalent}{\tbd{statFThreeflairTostEquivalent}}
\providecommand{\statFThreeflairTostEst}{\tbd{statFThreeflairTostEst}}
\providecommand{\statFThreeflairTostN}{\tbd{statFThreeflairTostN}}
\providecommand{\statFThreeflairTostP}{\tbd{statFThreeflairTostP}}
\providecommand{\statFThreeflairWelchP}{\tbd{statFThreeflairWelchP}}
\providecommand{\statFTwoburnCIHi}{\tbd{statFTwoburnCIHi}}
\providecommand{\statFTwoburnCILo}{\tbd{statFTwoburnCILo}}
\providecommand{\statFTwoburnEst}{\tbd{statFTwoburnEst}}
\providecommand{\statFTwoburnMde}{\tbd{statFTwoburnMde}}
\providecommand{\statFTwoburnN}{\tbd{statFTwoburnN}}
\providecommand{\statFTwoburnP}{\tbd{statFTwoburnP}}
\providecommand{\statFTwoburnPHolm}{\tbd{statFTwoburnPHolm}}
\providecommand{\statFTwoburnTostCIHi}{\tbd{statFTwoburnTostCIHi}}
\providecommand{\statFTwoburnTostCILo}{\tbd{statFTwoburnTostCILo}}
\providecommand{\statFTwoburnTostEquivalent}{\tbd{statFTwoburnTostEquivalent}}
\providecommand{\statFTwoburnTostEst}{\tbd{statFTwoburnTostEst}}
\providecommand{\statFTwoburnTostN}{\tbd{statFTwoburnTostN}}
\providecommand{\statFTwoburnTostP}{\tbd{statFTwoburnTostP}}
\providecommand{\statFTwoburnWelchP}{\tbd{statFTwoburnWelchP}}
\providecommand{\statFTwoflairCIHi}{\tbd{statFTwoflairCIHi}}
\providecommand{\statFTwoflairCILo}{\tbd{statFTwoflairCILo}}
\providecommand{\statFTwoflairEst}{\tbd{statFTwoflairEst}}
\providecommand{\statFTwoflairMde}{\tbd{statFTwoflairMde}}
\providecommand{\statFTwoflairN}{\tbd{statFTwoflairN}}
\providecommand{\statFTwoflairP}{\tbd{statFTwoflairP}}
\providecommand{\statFTwoflairPHolm}{\tbd{statFTwoflairPHolm}}
\providecommand{\statFTwoflairTostCIHi}{\tbd{statFTwoflairTostCIHi}}
\providecommand{\statFTwoflairTostCILo}{\tbd{statFTwoflairTostCILo}}
\providecommand{\statFTwoflairTostEquivalent}{\tbd{statFTwoflairTostEquivalent}}
\providecommand{\statFTwoflairTostEst}{\tbd{statFTwoflairTostEst}}
\providecommand{\statFTwoflairTostN}{\tbd{statFTwoflairTostN}}
\providecommand{\statFTwoflairTostP}{\tbd{statFTwoflairTostP}}
\providecommand{\statFTwoflairWelchP}{\tbd{statFTwoflairWelchP}}


==> planned/generated/macros_planned.tex <==
%
%
%
%
\providecommand{\gcvdry}[1]{\textcolor{red}{#1}}
\newcommand{\RunsNEleven}{550}  %
\newcommand{\NElevenJobsPro}{370}
\newcommand{\NElevenLaneHoursPro}{37.7}
\newcommand{\NElevenJobsRtx}{0}
\newcommand{\NElevenLaneHoursRtx}{0.0}
\newcommand{\NElevenJobsGb}{0}
\newcommand{\NElevenLaneHoursGb}{0.0}
\newcommand{\NElevenJobsRtxFiveZeroSixZeroTi}{0}
\newcommand{\NElevenLaneHoursRtxFiveZeroSixZeroTi}{0.0}
\newcommand{\NElevenJobsRtxThreeZeroEightZeroTi}{90}
\newcommand{\NElevenLaneHoursRtxThreeZeroEightZeroTi}{27.7}
\newcommand{\NElevenJobsRtxThreeZeroEightZero}{90}
\newcommand{\NElevenLaneHoursRtxThreeZeroEightZero}{15.7}
\newcommand{\NElevenLaneHoursTotal}{81.2}
\newcommand{\NElevenMakespanH}{38}  %
\newcommand{\NElevenLanes}{GB10 (0), RTX PRO 6000 (370), RTX 3080 (90), RTX 3080 Ti (90), RTX 4090 (0), RTX 5060 Ti (0)}
\newcommand{\RunsNTwelve}{280}  %
\newcommand{\NTwelveJobsPro}{200}
\newcommand{\NTwelveLaneHoursPro}{15.3}
\newcommand{\NTwelveJobsRtx}{0}
\newcommand{\NTwelveLaneHoursRtx}{0.0}
\newcommand{\NTwelveJobsGb}{0}
\newcommand{\NTwelveLaneHoursGb}{0.0}
\newcommand{\NTwelveJobsRtxFiveZeroSixZeroTi}{0}
\newcommand{\NTwelveLaneHoursRtxFiveZeroSixZeroTi}{0.0}
\newcommand{\NTwelveJobsRtxThreeZeroEightZeroTi}{40}
\newcommand{\NTwelveLaneHoursRtxThreeZeroEightZeroTi}{9.3}
\newcommand{\NTwelveJobsRtxThreeZeroEightZero}{40}
\newcommand{\NTwelveLaneHoursRtxThreeZeroEightZero}{5.3}
\newcommand{\NTwelveLaneHoursTotal}{30.0}
\newcommand{\NTwelveMakespanH}{15}  %
\newcommand{\NTwelveLanes}{GB10 (0), RTX PRO 6000 (200), RTX 3080 (40), RTX 3080 Ti (40), RTX 4090 (0), RTX 5060 Ti (0)}
\newcommand{\RunsNThirteen}{45}  %
\newcommand{\NThirteenJobsPro}{15}
\newcommand{\NThirteenLaneHoursPro}{1.0}
\newcommand{\NThirteenJobsRtx}{0}
\newcommand{\NThirteenLaneHoursRtx}{0.0}
\newcommand{\NThirteenJobsGb}{0}
\newcommand{\NThirteenLaneHoursGb}{0.0}
\newcommand{\NThirteenJobsRtxFiveZeroSixZeroTi}{0}
\newcommand{\NThirteenLaneHoursRtxFiveZeroSixZeroTi}{0.0}
\newcommand{\NThirteenJobsRtxThreeZeroEightZeroTi}{15}
\newcommand{\NThirteenLaneHoursRtxThreeZeroEightZeroTi}{2.2}
\newcommand{\NThirteenJobsRtxThreeZeroEightZero}{15}
\newcommand{\NThirteenLaneHoursRtxThreeZeroEightZero}{0.5}
\newcommand{\NThirteenLaneHoursTotal}{3.7}
\newcommand{\NThirteenMakespanH}{2}  %
\newcommand{\NThirteenLanes}{GB10 (0), RTX PRO 6000 (15), RTX 3080 (15), RTX 3080 Ti (15), RTX 4090 (0), RTX 5060 Ti (0)}
\newcommand{\RunsNFourteen}{500}  %
\newcommand{\NFourteenJobsPro}{300}
\newcommand{\NFourteenLaneHoursPro}{27.5}
\newcommand{\NFourteenJobsRtx}{0}
\newcommand{\NFourteenLaneHoursRtx}{0.0}
\newcommand{\NFourteenJobsGb}{0}
\newcommand{\NFourteenLaneHoursGb}{0.0}
\newcommand{\NFourteenJobsRtxFiveZeroSixZeroTi}{0}
\newcommand{\NFourteenLaneHoursRtxFiveZeroSixZeroTi}{0.0}
\newcommand{\NFourteenJobsRtxThreeZeroEightZeroTi}{100}
\newcommand{\NFourteenLaneHoursRtxThreeZeroEightZeroTi}{22.5}
\newcommand{\NFourteenJobsRtxThreeZeroEightZero}{100}
\newcommand{\NFourteenLaneHoursRtxThreeZeroEightZero}{3.3}
\newcommand{\NFourteenLaneHoursTotal}{53.3}
\newcommand{\NFourteenMakespanH}{28}  %
\newcommand{\NFourteenLanes}{GB10 (0), RTX PRO 6000 (300), RTX 3080 (100), RTX 3080 Ti (100), RTX 4090 (0), RTX 5060 Ti (0)}
\newcommand{\RunsNFifteen}{550}  %
\newcommand{\NFifteenJobsPro}{370}
\newcommand{\NFifteenLaneHoursPro}{37.0}
\newcommand{\NFifteenJobsRtx}{0}
\newcommand{\NFifteenLaneHoursRtx}{0.0}
\newcommand{\NFifteenJobsGb}{0}
\newcommand{\NFifteenLaneHoursGb}{0.0}
\newcommand{\NFifteenJobsRtxFiveZeroSixZeroTi}{0}
\newcommand{\NFifteenLaneHoursRtxFiveZeroSixZeroTi}{0.0}
\newcommand{\NFifteenJobsRtxThreeZeroEightZeroTi}{90}
\newcommand{\NFifteenLaneHoursRtxThreeZeroEightZeroTi}{22.5}
\newcommand{\NFifteenJobsRtxThreeZeroEightZero}{90}
\newcommand{\NFifteenLaneHoursRtxThreeZeroEightZero}{3.0}
\newcommand{\NFifteenLaneHoursTotal}{62.5}
\newcommand{\NFifteenMakespanH}{37}  %
\newcommand{\NFifteenLanes}{GB10 (0), RTX PRO 6000 (370), RTX 3080 (90), RTX 3080 Ti (90), RTX 4090 (0), RTX 5060 Ti (0)}
\newcommand{\RunsDOne}{450}  %
\newcommand{\DOneJobsPro}{350}
\newcommand{\DOneLaneHoursPro}{29.2}
\newcommand{\DOneJobsRtx}{0}
\newcommand{\DOneLaneHoursRtx}{0.0}
\newcommand{\DOneJobsGb}{0}
\newcommand{\DOneLaneHoursGb}{0.0}
\newcommand{\DOneJobsRtxFiveZeroSixZeroTi}{0}
\newcommand{\DOneLaneHoursRtxFiveZeroSixZeroTi}{0.0}
\newcommand{\DOneJobsRtxThreeZeroEightZeroTi}{50}
\newcommand{\DOneLaneHoursRtxThreeZeroEightZeroTi}{14.2}
\newcommand{\DOneJobsRtxThreeZeroEightZero}{50}
\newcommand{\DOneLaneHoursRtxThreeZeroEightZero}{8.3}
\newcommand{\DOneLaneHoursTotal}{51.7}
\newcommand{\DOneMakespanH}{29}  %
\newcommand{\DOneLanes}{GB10 (0), RTX PRO 6000 (350), RTX 3080 (50), RTX 3080 Ti (50), RTX 4090 (0), RTX 5060 Ti (0)}
\newcommand{\RunsDTwo}{450}  %
\newcommand{\DTwoJobsPro}{350}
\newcommand{\DTwoLaneHoursPro}{35.8}
\newcommand{\DTwoJobsRtx}{0}
\newcommand{\DTwoLaneHoursRtx}{0.0}
\newcommand{\DTwoJobsGb}{0}
\newcommand{\DTwoLaneHoursGb}{0.0}
\newcommand{\DTwoJobsRtxFiveZeroSixZeroTi}{0}
\newcommand{\DTwoLaneHoursRtxFiveZeroSixZeroTi}{0.0}
\newcommand{\DTwoJobsRtxThreeZeroEightZeroTi}{50}
\newcommand{\DTwoLaneHoursRtxThreeZeroEightZeroTi}{15.0}
\newcommand{\DTwoJobsRtxThreeZeroEightZero}{50}
\newcommand{\DTwoLaneHoursRtxThreeZeroEightZero}{8.3}
\newcommand{\DTwoLaneHoursTotal}{59.2}
\newcommand{\DTwoMakespanH}{36}  %
\newcommand{\DTwoLanes}{GB10 (0), RTX PRO 6000 (350), RTX 3080 (50), RTX 3080 Ti (50), RTX 4090 (0), RTX 5060 Ti (0)}
\newcommand{\RunsDThree}{475}  %
\newcommand{\DThreeJobsPro}{365}
\newcommand{\DThreeLaneHoursPro}{47.6}
\newcommand{\DThreeJobsRtx}{0}
\newcommand{\DThreeLaneHoursRtx}{0.0}
\newcommand{\DThreeJobsGb}{0}
\newcommand{\DThreeLaneHoursGb}{0.0}
\newcommand{\DThreeJobsRtxFiveZeroSixZeroTi}{0}
\newcommand{\DThreeLaneHoursRtxFiveZeroSixZeroTi}{0.0}
\newcommand{\DThreeJobsRtxThreeZeroEightZeroTi}{55}
\newcommand{\DThreeLaneHoursRtxThreeZeroEightZeroTi}{14.1}
\newcommand{\DThreeJobsRtxThreeZeroEightZero}{55}
\newcommand{\DThreeLaneHoursRtxThreeZeroEightZero}{8.3}
\newcommand{\DThreeLaneHoursTotal}{70.0}
\newcommand{\DThreeMakespanH}{48}  %
\newcommand{\DThreeLanes}{GB10 (0), RTX PRO 6000 (365), RTX 3080 (55), RTX 3080 Ti (55), RTX 4090 (0), RTX 5060 Ti (0)}
\newcommand{\RunsDFour}{450}  %
\newcommand{\DFourJobsPro}{350}
\newcommand{\DFourLaneHoursPro}{29.2}
\newcommand{\DFourJobsRtx}{0}
\newcommand{\DFourLaneHoursRtx}{0.0}
\newcommand{\DFourJobsGb}{0}
\newcommand{\DFourLaneHoursGb}{0.0}
\newcommand{\DFourJobsRtxFiveZeroSixZeroTi}{0}
\newcommand{\DFourLaneHoursRtxFiveZeroSixZeroTi}{0.0}
\newcommand{\DFourJobsRtxThreeZeroEightZeroTi}{50}
\newcommand{\DFourLaneHoursRtxThreeZeroEightZeroTi}{14.2}
\newcommand{\DFourJobsRtxThreeZeroEightZero}{50}
\newcommand{\DFourLaneHoursRtxThreeZeroEightZero}{8.3}
\newcommand{\DFourLaneHoursTotal}{51.7}
\newcommand{\DFourMakespanH}{29}  %
\newcommand{\DFourLanes}{GB10 (0), RTX PRO 6000 (350), RTX 3080 (50), RTX 3080 Ti (50), RTX 4090 (0), RTX 5060 Ti (0)}
\newcommand{\RunsDFive}{425}  %
\newcommand{\DFiveJobsPro}{335}
\newcommand{\DFiveLaneHoursPro}{56.6}
\newcommand{\DFiveJobsRtx}{0}
\newcommand{\DFiveLaneHoursRtx}{0.0}
\newcommand{\DFiveJobsGb}{0}
\newcommand{\DFiveLaneHoursGb}{0.0}
\newcommand{\DFiveJobsRtxFiveZeroSixZeroTi}{0}
\newcommand{\DFiveLaneHoursRtxFiveZeroSixZeroTi}{0.0}
\newcommand{\DFiveJobsRtxThreeZeroEightZeroTi}{45}
\newcommand{\DFiveLaneHoursRtxThreeZeroEightZeroTi}{14.2}
\newcommand{\DFiveJobsRtxThreeZeroEightZero}{45}
\newcommand{\DFiveLaneHoursRtxThreeZeroEightZero}{8.3}
\newcommand{\DFiveLaneHoursTotal}{79.1}
\newcommand{\DFiveMakespanH}{57}  %
\newcommand{\DFiveLanes}{GB10 (0), RTX PRO 6000 (335), RTX 3080 (45), RTX 3080 Ti (45), RTX 4090 (0), RTX 5060 Ti (0)}
\newcommand{\RunsDSix}{475}  %
\newcommand{\DSixJobsPro}{365}
\newcommand{\DSixLaneHoursPro}{24.1}
\newcommand{\DSixJobsRtx}{0}
\newcommand{\DSixLaneHoursRtx}{0.0}
\newcommand{\DSixJobsGb}{0}
\newcommand{\DSixLaneHoursGb}{0.0}
\newcommand{\DSixJobsRtxFiveZeroSixZeroTi}{0}
\newcommand{\DSixLaneHoursRtxFiveZeroSixZeroTi}{0.0}
\newcommand{\DSixJobsRtxThreeZeroEightZeroTi}{55}
\newcommand{\DSixLaneHoursRtxThreeZeroEightZeroTi}{14.2}
\newcommand{\DSixJobsRtxThreeZeroEightZero}{55}
\newcommand{\DSixLaneHoursRtxThreeZeroEightZero}{8.3}
\newcommand{\DSixLaneHoursTotal}{46.7}
\newcommand{\DSixMakespanH}{24}  %
\newcommand{\DSixLanes}{GB10 (0), RTX PRO 6000 (365), RTX 3080 (55), RTX 3080 Ti (55), RTX 4090 (0), RTX 5060 Ti (0)}
\newcommand{\RunsDSeven}{425}  %
\newcommand{\DSevenJobsPro}{335}
\newcommand{\DSevenLaneHoursPro}{45.4}
\newcommand{\DSevenJobsRtx}{0}
\newcommand{\DSevenLaneHoursRtx}{0.0}
\newcommand{\DSevenJobsGb}{0}
\newcommand{\DSevenLaneHoursGb}{0.0}
\newcommand{\DSevenJobsRtxFiveZeroSixZeroTi}{0}
\newcommand{\DSevenLaneHoursRtxFiveZeroSixZeroTi}{0.0}
\newcommand{\DSevenJobsRtxThreeZeroEightZeroTi}{45}
\newcommand{\DSevenLaneHoursRtxThreeZeroEightZeroTi}{13.5}
\newcommand{\DSevenJobsRtxThreeZeroEightZero}{45}
\newcommand{\DSevenLaneHoursRtxThreeZeroEightZero}{8.3}
\newcommand{\DSevenLaneHoursTotal}{67.2}
\newcommand{\DSevenMakespanH}{45}  %
\newcommand{\DSevenLanes}{GB10 (0), RTX PRO 6000 (335), RTX 3080 (45), RTX 3080 Ti (45), RTX 4090 (0), RTX 5060 Ti (0)}
\newcommand{\RunsExtensionTotal}{3,150}  %
\newcommand{\ExtensionLaneHoursTotal}{425}
\newcommand{\RunsRealDOne}{25}
\newcommand{\RunsRealDTwo}{25}
\newcommand{\RunsRealDThree}{25}
\newcommand{\RunsRealDFour}{25}
\newcommand{\RunsRealDFive}{0}
\newcommand{\RunsRealDSix}{25}
\newcommand{\RunsRealDSeven}{0}
%


==> preamble.tex <==
%
%
%
%
%
%
\usepackage[T1]{fontenc}
\usepackage{multirow}
\usepackage{microtype}
\usepackage{array}
\usepackage{adjustbox}
\graphicspath{{figs/}{generated/}}
%
%
%
%
%
%
%
\makeatletter
%
%
\providetoggle{wacvfinal}\providetoggle{cvprfinal}
\ifboolexpr{togl{wacvfinal} or togl{cvprfinal}}{}{%
  \ifdefined\pdfsavepos
    \newcommand\LN@rec[4]{%
      \@ifundefined{LN@page@#4}{\expandafter\gdef\csname LN@page@#4\endcsname{}}{}%
      \expandafter\g@addto@macro\csname LN@page@#4\endcsname{\LN@draw{#1}{#2}{#3}}}
    \def\LN@mid{20054016}%
    \newcommand\LN@draw[3]{%
      \ifnum#2<\LN@mid\relax
        \put(\LenToUnit{#2sp},\LenToUnit{#3sp}){\makebox[0pt][r]{\linenumberfont#1\hspace{\linenumbersep}}}%
      \else
        \put(\LenToUnit{#2sp},\LenToUnit{#3sp}){\makebox[0pt][l]{\hspace{\columnwidth}\hspace{\linenumbersep}\linenumberfont#1}}%
      \fi}
    \def\LN@record{%
      \pdfsavepos
      \edef\@tempa{\write\@auxout{\string\LN@rec{\the\c@linenumber}{\noexpand\the\noexpand\pdflastxpos}%
        {\noexpand\the\noexpand\pdflastypos}{\noexpand\the\noexpand\c@page}}}\@tempa}
    \let\makeLineNumberRunning\LN@record
    \let\makeLineNumberOdd\LN@record
    \let\makeLineNumberEven\LN@record
    \AddToShipoutPicture{\AtPageLowerLeft{\csname LN@page@\the\c@page\endcsname}}
  \fi
}
\makeatother

%
\setlength{\textfloatsep}{9pt plus 2pt minus 3pt}
\setlength{\dbltextfloatsep}{9pt plus 2pt minus 3pt}
\setlength{\floatsep}{7pt plus 2pt minus 2pt}
\setlength{\dblfloatsep}{7pt plus 2pt minus 2pt}
\setlength{\intextsep}{7pt plus 2pt minus 2pt}

%
%
%
\newcommand{\tbd}[1]{\textcolor{red}{\textbf{[TBD:} #1\textbf{]}}}
\newcommand{\figtbd}[1]{\begin{center}\textcolor{red}{\textbf{[FIGURE TBD:} #1\textbf{]}}\end{center}}
\newcommand{\citetbd}[1]{\tbd{cite #1, add via A-2b}}
%
%
\newcommand{\tabletbd}[2][2em]{\begin{tabular}{@{}c@{}}\toprule \parbox[c][#1][c]{0.95\linewidth}{\centering\tbd{#2}} \\ \bottomrule\end{tabular}}
%
\newcommand{\phfig}[2]{\fbox{\parbox[c][#1][c]{\dimexpr\linewidth-2\fboxsep-2\fboxrule\relax}{\centering\tbd{FIGURE #2}}}}
%
\IfFileExists{generated/config_macros.tex}{\input{generated/config_macros.tex}}{}
%
\IfFileExists{generated/macros.tex}{\input{generated/macros.tex}}{}
\providecommand{\ResultsProvenance}{\tbd{pending, no official analysis run yet}}
\providecommand{\ManifestConstants}{\tbd{run scripts/reflow\_tables.py}}
%
\IfFileExists{macro_fallbacks.tex}{\input{macro_fallbacks.tex}}{}
%
%
%
%
\ifdefined\cvprbuild\providecommand{\plannedbuild}{1}\fi
\ifdefined\plannedbuild
  \IfFileExists{planned/generated/macros_planned.tex}{\input{planned/generated/macros_planned.tex}}{}
\fi
%
%
\ifdefined\cvprbuild   %
  \IfFileExists{cvpr/generated/supp_refs_cvpr.tex}{\input{cvpr/generated/supp_refs_cvpr.tex}}{}
\else
  \IfFileExists{generated/supp_refs.tex}{\input{generated/supp_refs.tex}}{}
\fi
%
%
\ifdefined\arxivbuild
  \newcommand{\sref}[1]{\ref{#1}}
  \newcommand{\stab}[1]{Table~\ref{#1}}
  \newcommand{\sfig}[1]{Fig.~\ref{#1}}
  \newcommand{\ssec}[1]{Appendix~\ref{#1}}
  \newcommand{\Supp}{Appendix}
\else
  \newcommand{\sref}[1]{\ifcsname sref@#1\endcsname\csname sref@#1\endcsname\else\tbd{supp ref #1}\fi}
  \newcommand{\stab}[1]{Supp.~Table~\sref{#1}}
  \newcommand{\sfig}[1]{Supp.~Fig.~\sref{#1}}
  \newcommand{\ssec}[1]{Supp.~\sref{#1}}
  \newcommand{\Supp}{Supp.}
\fi
%
%
\ifdefined\arxivbuild
  \newcommand{\mtab}[1]{Table~\ref{#1}}
  \newcommand{\mfig}[1]{Fig.~\ref{#1}}
  \newcommand{\msec}[1]{Section~\ref{#1}}
\else
  \ifdefined\cvprbuild\IfFileExists{cvpr/generated/main_refs_cvpr.tex}{\input{cvpr/generated/main_refs_cvpr.tex}}{}\fi
  \newcommand{\mref}[1]{\ifcsname mref@#1\endcsname\csname mref@#1\endcsname\else\tbd{main ref #1}\fi}
  \newcommand{\mtab}[1]{Table~\mref{#1} of the main paper}
  \newcommand{\mfig}[1]{Fig.~\mref{#1} of the main paper}
  \newcommand{\msec}[1]{Section~\mref{#1} of the main paper}
\fi
%
%
%
%
\newcommand{\ProvSlot}[1]{}
%
%
\ifdefined\cvprmainpaper\newcommand{\suppnote}[1]{}\else\newcommand{\suppnote}[1]{#1}\fi
%
\providecommand{\NSeeds}{\tbd{seeds}}
\providecommand{\WorstBurn}{\tbd{worst type}}
\providecommand{\WorstFlair}{\tbd{worst type}}
\providecommand{\RunsCore}{\tbd{runs}}
\providecommand{\RunsStretch}{\tbd{runs}}

%
\newcommand{\gfm}{GFM\xspace}
\newcommand{\gfms}{GFMs\xspace}
\newcommand{\sat}{DINOv3-SAT\xspace}
\newcommand{\lvd}{DINOv3-LVD\xspace}
\newcommand{\dofa}{DOFA-L\xspace}
\newcommand{\tm}{TerraMind-L\xspace}
\newcommand{\rn}{ResNet-50\xspace}
\newcommand{\prithvi}{Prithvi-EO-2.0-300M-TL\xspace}
\newcommand{\rnssl}{ResNet-50 SSL4EO\xspace}
\newcommand{\vitr}{ViT-L/16 random init\xspace}
\newcommand{\cnxl}{DINOv3 ConvNeXt-L\xspace}
\newcommand{\burn}{HLS Burn Scars\xspace}
\newcommand{\flair}{FLAIR-2\xspace}
\newcommand{\sfloods}{Sen1Floods11\xspace}
\newcommand{\gbtwo}{GEO-Bench-2\xspace}
\newcommand{\miou}{mIoU\xspace}
\newcommand{\Lone}{L1\xspace}
\newcommand{\Ltwo}{L2\xspace}
\newcommand{\vd}[1]{\textit{#1}}   %
\newcommand{\Lpair}{LP\xspace}   %
\newcommand{\drop}{\ensuremath{\Delta}}
\newcommand{\ret}{\ensuremath{\bar{R}}}
\newcommand{\memrate}{\ensuremath{M}}
\newcommand{\etype}[1]{\textit{#1}}          %
\renewcommand{\arraystretch}{0.9}
%
\captionsetup{labelsep=colon}
\captionsetup[sub]{labelsep=colon}
%
%
\ifdefined\arxivbuild
\renewcommand{\arraystretch}{1.05}
\captionsetup{skip=13pt}
%
%
\captionsetup[table]{position=below,skip=13pt}
\captionsetup[figure]{position=below,skip=13pt}
\setlength{\textfloatsep}{18pt plus 4pt minus 2pt}
\setlength{\dbltextfloatsep}{18pt plus 4pt minus 2pt}
\setlength{\floatsep}{16pt plus 4pt minus 2pt}
\setlength{\dblfloatsep}{16pt plus 4pt minus 2pt}
\setlength{\intextsep}{14pt plus 3pt minus 2pt}
\fi

